Adaptive and anisotropic finite element approximation : Theory and algorithms

Mesh adaption procedures for finite element approximation allows one to adapt the resolution, by local refinement in the regions of strong variation of the function of interest. This procedure plays a key role in numerous applications of scientific computing. The use of anisotropic triangles allows to improve the efficiency of the procedure by introducing long and thin triangles that fit in particular the directions of the possible curves of discontinuity. Given a norm X of interest and a function f to be approximated, we formulate the problem of optimal mesh adaptation, as minimizing the approximation error over all (possibly anisotropic) triangulations of prescribed cardinality. We address the four following questions related to this problem: I. How does the approximation error behave in the asymptotic regime when the number of triangles N tends to infinity, when f is a smooth function ? II. Which classes of functions govern the rate of decay of the approximation error as N grows, and are in that sense naturally tied to the problem of optimal mesh adaptation? III. Could this optimization problem, which is posed on triangulations of a given cardinality N, be replaced by an equivalent more tractable problem posed on a continuous object? IV. Is it possible to produce a near-optimal sequence of triangulations using a hierarchical refinement procedure?

==> ApproxTheory/ApproxTheoryTheseOld.tex <==

\section{Introduction} %, and metrics on a periodic bounded domain}
\label{secPer}


The main purpose of adaptive mesh generation, compared uniform mesh generation, is to reduce the number of simplices required to achieve a given task. Here are two relevant examples which 
are further discussed in this chapter:
\begin{enumerate}
\item
Given two domains of interest, generate the mesh with smallest possible cardinality that separates these
domains with a layer of simplices.
\item
Given a function $f$, generate the mesh of a prescribed cardinality $N$ that yields the best 
finite element approximation to $f$ of a given order $m-1$ in some prescribed norm $L^p$ or $W^{1,p}$.
\end{enumerate}
Both examples can be viewed as optimization problems posed on the set of meshes.
The second problem was dealt with in Chapter 2 and 3 in the case where $f$ is smooth, 
and an optimal mesh was constructed in the asymptotic regime $N\to +\infty$. The results
of the previous chapter have revealed that certain relevant classes of meshes can be equivalently
described in terms of riemannian metrics, and a natural objective is therefore
to translate the above problems as {\it optimization problems posed on the set of metrics}.
Optimization problems posed on metrics may indeed be easier to solve practically  
due to the continuous nature of these objects.
The goal of this chapter is to explain how this objective can be met for the
above two examples.

In the previous chapter, we have introduced the classes of meshes
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
and characterized the respectively equivalent classes of metrics
$$
\bH_i\subset \bH_a\subset \bH_g.
$$
These classes of meshes are defined on the entire unbounded domain $\R^d$, and are therefore
not well suited for the purpose of this chapter.

\subsection{Periodic meshes and metrics}

We consider instead meshes of the infinite domain $\R^d$ which are $\Z^d$-periodic. Such a mesh only has a finite  number of elements up to translation by an element of $\Z^d$. These meshes, and the corresponding metrics, are introduced in the next definition.
\begin{definition}
We define as follows the sets $\bT_\per\subset \bT$ and $\bH_\per\subset \bH$ of periodic meshes and metrics.\begin{itemize}
\item (Periodic meshes) A mesh $\cT \in \bT$ belongs to $\bT_\per$ if and only if it satisfies the two following properties.

\begin{enumerate}[i)]
\item (Invariance by translation) For any $T\in \cT$ and any $u \in \Z^d$, one has $u+T \in \Z^d$.
\item (Constrained diameters) For any $T\in \cT$ one has $\cH_T\geq \Id$.
\end{enumerate}

\item (Periodic metrics) A metric $H \in \bH$ belongs to $\bH_\per$ if and only if it satisfies the two following properties.

\begin{enumerate}[i)]
\item (Invariance by translation) For any $z\in \R^d$ and any $u \in \Z^d$, one has $H(z) = H(z+u)$.
\item (Constrained positivity) For any $z\in \R^d$ one has $H(z)\geq \Id$.
\end{enumerate}

\end{itemize}
\end{definition}
A mesh $T\in \bT_\per$ can be regarded, thanks to the invariance by translation {\it i)}, as a mesh of the compact periodic space 
$$
\Pi^d := (\R/ \ZZ)^d,
$$
also called the $d$-dimensional torus. Note that $\Pi^d$ has no boundary.
The diameter constraint {\it ii)} ensures that the simplices $T$ of a periodic mesh $\cT \in \bT_\per$ do not have a significantly larger size than the fundamental cell $[0,1]^d$ of the standard $\Z^d$ periodic tiling of $\R^d$. 

Strictly speaking, a periodic mesh $\cT\in \bT_\per$ has an infinite cardinality. However it only contains a finite number of simplices up to translation by an element of $\Z^d$.  
For any $\cT\in \bT_\per$, we therefore denote by $\#(\cT)$ the number of equivalence classes in $\cT$ for the relation
$$
T \sim T' \text{ if and only if there exists } u \in \Z^d \text{ such that } \ T' = T+u.
$$
The number $\#(\cT)$ is finite, and is the the cardinality of $\cT$ seen as a mesh of the compact periodic space $\Pi^d$.
We define the mass $m(H)$ of a periodic metric $H \in \bH_\per$ by
$$
m(H) :=  \int_{[0,1]^d} \sqrt{\det H}.
$$
These two quantities are linked by the following proposition. We denote by $\TEq$ a fixed equilateral simplex centered at the origin of $\R^d$ and having its vertices on the unit ball. We established in Proposition \ref{propHT} of the previous chapter that for any simplex $T$
$$
|T| \sqrt{\det \cH_T} = |\TEq|. 
$$
\begin{prop}
\label{propCardMass}
The cardinality of a mesh $\cT\in \bT_\per$ and the mass of a metric $H\in \bH_\per$ satisfy the following properties:
\begin{itemize}
\item If $\cH_T \leq C^2 H(z)$ for all $T\in \cT$ and all $z\in T$, then 
$
|\TEq|\#(\cT) \leq C^d  m(H).
$
\item 
If $H(z) \leq C^2 \cH_T$ for all $T\in \cT$ and all $z\in T$, then 
$
 m(H) \leq C^d |\TEq|\#(\cT).
$
\end{itemize}
In particular, if $\cT$ is $C$-adapted to $H$ in the sense of Definition \ref{defEqHT}, then 
\be
\label{eqCardMass}
C^{-d} m(H) \leq |\TEq| \,\#(\cT) \leq C^d m(H) .
\ee
\end{prop}

\proof
For any $z\in \R^d$ we denote by $T(z)$ the simplex $T\in \cT$ containing $z$.
We thus have 
\be
\label{eqCardT}
\#(\cT) = \int_{[0,1]^d} \frac {dz}{|T(z)|} = |\TEq|^{-1} \int_{[0,1]^d} \sqrt{\det \cH_{T(z)}} \, dz.
\ee
Furthermore we have $\det S \leq C^d \det S'$ for any $S,S'\in S_d^+$ satisfying $S \leq C S'$.
Applying this remark to the matrices $H(z)$ and $\cH_{T(z)}$ we obtain the announced inequalities, which concludes the proof of the proposition.
\sq

Theorem \ref{thEquiv} has an immediate generalization to periodic meshes and metrics, which is stated below. 
\begin{theorem}
\label{thPer}
There exists a constant $C_0=C_0(d)$ such that for all $C \geq C_0$, 
\begin{enumerate}
\item The collection of meshes $\bT_{i,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_i \cap \bH_\per$.
\item If $d=2$, the collection of meshes $\bT_{a,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_a \cap \bH_\per$.
\item If $d=2$, the collection of meshes $\bT_{g,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_g \cap \bH_\per$.
\end{enumerate}
\end{theorem}

\proof
The proof of Theorem \ref{thEquiv} presented in the previous chapter can be adapted to periodic metrics and triangulations with only slight changes, which are left to the reader.
\sq



\subsection{Optimization on periodic meshes}

We equip the set $\bH_\per$ of continuous and $\Z^d$ periodic metrics with a distance $d_\per$ which is defined as follows: for all $H,H'\in \bH_\per$
$$
d_\per(H,H') := \sup_{z\in [0,1]^d} d_\times (H(z), H(z)) = \sup_{z\in \R^d} d_\times (H(z) , H'(z)).
$$
Consider $H, H'\in \bH_\per$ and define $\delta = d_\per(H,H')$. We thus have for all $z\in \R^d$,
$$
e^{-2 \delta} H(z)\leq H'(z) \leq e^{2 \delta} H(z). 
$$
Hence the mass $H \mapsto m(H)$ is a continuous function of $H \in \bH_\per$ 
\be
\label{massCont}
e^{-d\delta} m(H) \leq m(H') \leq e^{d\delta} m(H),
\ee
as well as the distance $H \mapsto d_H(x,y)$ for any fixed $x,y\in \R^d$ : 
\be
\label{distCont}
e^{-\delta} d_{H}(x,y) \leq d_{H'}(x,y) \leq e^\delta d_{H}(x,y).
\ee

We establish in \S \ref{secCompact} (Theorem \ref{thCompact}) the following compactness property : for any $M\geq 1$ and any symbol $\star \in \{i,a,g\}$ the following collection of metrics is a compact subset of $\bH_\perp$
$$
\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq M\}.
$$

This compactness result immediately implies the existence of an ``optimal metric'' for a number of relevant optimization problems posed 
It follows that most 



%
%One easily shows (see details in Lemma \ref{lemmaClosed}) that the collections of metrics
%$$
%\bH_\per \cap \bH_i \subset \bH_\per 
%$$
%
%These properties are used in Lemma \ref{lemmaClosed} to establish that the collections $\bH_\per \cap \bH_\star$, $\star \in \{i,a,g\}$, of isotropic, quasi-acute or graded metrics are closed in $\bH_\per$, as well as the collection of metrics of a given mass. 
%
%A more striking result is the following compactness property, which is established in \S\ref{secCompact}.
%\begin{theorem}
%\label{thCompact}
%For any symbol $\star \in \{i,a,g\}$ and any $M \geq 1$ the following set of metrics is non-empty and compact
%$$
%\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq M\}.
%$$
%%(Where $\bH = C^0(\R^d, S_d^+)$ is equipped with the standard compact open topology.)
%\end{theorem}
%
%This result immediately implies the existence of minimizers to the optimization probems \iref{optiHe} and \iref{optiHP}, under minimal assumptions.
%Namely if the optimized quantity $e$ is continuous and non-negative, $e\in C^0(\bH_\per, \R_+)$ and if $M\geq 1$ then there exists a minimizer to \iref{optiHe}. Similarly if $P$ is a closed condition, in other words if the set $\{H \in \bH_\per\cap \bH_\star \sep P(H) \text{ holds}\}$ is closed and non-empty, then there exists a minimizer to \iref{optiHP}.
%


\subsection{Separation of two domains}

\subsection{Approximation in a given norm}


%contain meshes of the entire unbounded domain $\R^d$, which therefore contain an infinite number of simplices. The number of simplices of two such meshes thus cannot be compared directly.
%In order to illustrate advantages of anisotropic mesh adaptation, in the sense that a smaller number of simplices are resuired to achieve the same task compared to a uniform or isotropic mesh, we therefore need to consider meshes of a compact domain.
%%the advantage of anisotropic mesh generation develop the theory as well as the applications, it is therefore necessary to extend the previous results to bounded domains.
%Unfortunately the generalization of Theorem \ref{thEquiv} to bounded domains $\Omega\subset \R^d$ comes with its share of difficulties, since the curvature and the singularities of the boundary $\partial \Omega$ need to be analyzed from the point of view of computational mesh generation. The author therefore has therefore chosen to postpone this analysis for future work.

%\subsection{Main results}
\paragraph{Optimization problems posed on triangulations\\}

Mesh adaptation is is generally used to solve, approximately at least, some problems of the type
%The general purpose of mesh adaptation is to solve some problems of the type
\be
\label{optiTe}
\min \{e(\cT) \sep \cT \text{ is a mesh of } \Omega \text{ satisfying } \#(\cT)\leq N\},
\ee
where $\Omega\subset \R^d$, $N \geq 1$ is an integer and $e(\cT)$ is a quantity that needs to be optimized. Typically $e(\cT)$ is the approximation error of a given function $f$, measured in some norm $X$, on a finite element space associated to $\cT$.

Another closely related type of optimization problem is the following.
\be
\label{optiTP}
\min \{\#(\cT) \sep \cT \text{ is a mesh of } \Omega \text{ and satisfies } P(\cT)\},
\ee
where $P(\cT)$ is some property. Some choices possible choices for $P(\cT)$ are related to approximation theory, for instance $P(\cT)$ could hold if the quantity $e(\cT)$ appearing in the previous problem \iref{optiTe} is smaller than a given threshold $\ve$. In addition to that possibility we explore in this chapter a geometrical property $P(\cT)$ which holds when the mesh $\cT$ ``separates'' two closed regions of $\Omega$, in a sense which is defined below. This condition heuristically means that $\cT$ creates a layer of simplices in between the boundaries of these regions.

The optimization problems \iref{optiTe} and \iref{optiTP} are not well posed and should be regarded as heuristics. For instance the problem \iref{optiTe} generally does not have a solution: consider a minimizing sequence $(\cT_k)_{k\geq 0}$, $\#(\cT_k)\leq N$, for the quantity $e(\cT)$. If a sequence of simplices $(T_k)_{k \geq 0}$, $T_k\in \cT_k$, degenerates, then it could be impossible to extract a conforming limit mesh.

In order to avoid this difficulty, one usually imposes some regularity on the meshes among which the optimization is done. The problem \iref{optiTe} can be replaced for instance by 
\be
\label{optiTStar}
\min \{e(\cT) \sep \cT\in \bT_\per \cap \bT_{\star,C} \text{ and } \#(\cT)\leq N\},
\ee
where $\star \in \{i,a,g\}$ is a symbol and $C\geq 1$ is a constant. 
If the quantity $e(\cT)$ depends continuously on the mesh $\cT$, then the minimization problem \iref{optiTStar} generally has a solution $\cT_C$.
The formulation \iref{optiTStar} unfortunately raises the problem of choosing the parameter $C$. Furthermore the optimization \iref{optiTStar} among a collection meshes if of combinatorial type and is therefore difficult to address from a theoretical or numerical point of view.

%presented in \iref{optiTe}, \iref{optiTP} or more precisely
We advocate in this chapter to trade the optimization among meshes \iref{optiTStar} for an optimization among Riemannian metrics.
\be
\label{optiHe}
\min \{e(H) \sep H \in \bH_\per \cap \bH_\star \text{ satisfies } m(H) \leq M\},
\ee
or 
\be
\label{optiHP}
\min \{m(H) \sep H \in \bH_\per \cap \bH_\star \text{ satisfies } P(H)\},
\ee
where $\star\in \{i,a,g\}$ is a symbol and where $e(H)$ and $P(H)$ are counterparts for metrics of the quantities $e(\cT)$ and $P(\cT)$. 

We first prove a compactness result which shows that the problems \iref{optiHe} and \iref{optiHP} generally have a solution. 
We then turn to two specific optimization problems. In each case we reformulate an optimization among triangulations into an optimization among matrices. We then take advantage of the fact that riemannian metrics in $\bH_i$, $\bH_a$ or $\bH_g$ are continuous objects governed by simple equations, rather than meshes which are discrete combinatorial structures, to gain a new insight on these problems and in certain cases to solve them.

\paragraph{Compactness of metrics of a given mass\\}


\paragraph{Separation of geometric sub-domains by a mesh or a metric\\}

Isotropic and anisotropic mesh adaptation is often used to separate some geometric sets, in the sense given by the following definition. For any closed subset $E \subset \R^d$ and any mesh $\cT\in \bT$ we define the neighborhood $V_\cT(E)$ of $E$ in $\cT$ as follows :
$$
V_\cT(E) := \bigcup_{\substack{T \in \cT,\\ T \cap E\neq\emptyset}} T
$$
\begin{definition}
We say that a mesh $\cT\in \bT$ separates two closed sets $X,Y\subset \R^d$ if and only if 
$$
V_\cT(X) \cap V_\cT(Y) = \emptyset,
$$
in other words if $X$ and $Y$ have disjoint neighborhoods in the mesh $\cT$. We say that a metric $H$ separates $X$ and $Y$ if 
$$
d_H(x,y) \geq 1 \text{ for all } (x,y) \in X\times Y.
$$
\end{definition}
The separation of domains by a mesh is a common need in applications.
In a finite element simulation involving several distinct physical phenomena, a separate treatment of different regions $X,Y, \ldots$ of the computational domain $\Omega$ can be necessary. This raises the need for a mesh $\cT$ which separates these regions.
In other simulations, the mesh $\cT$ needs to include a thin layer simplices of width $\ve>0$ close to a set $\Gamma$ where a singular phenomenon appears. 
In that case we define 
$$
X = \Gamma \stext{ and } Y := \{y\in \R^d \sep d(y,\Gamma) \geq \ve\}. %Y_\ve
$$
Such a mesh can be required if the exact solution is discontinuous through a surface $\Gamma$ included in the computational domain. For instance bi-dimensional anisotropic mesh adaptation is used [Frey] to simulate the evolution of two different and non mixing fluids separated by an interface $\Gamma$. 
%The pressure (??) variable is discontinuous at the interface.

A natural objective is therefore to build a mesh of minimal cardinality which separates two given regions. The next definition formulates this problem in the context of periodic meshes.
\begin{definition}
Let $\star \in \{i,a,g\}$ be a symbol and let $C_0\geq 1$.
Let $X,Y \subset \R^d$ be two closed, disjoint and periodic sets, in the sense that 
$$
x+u \in X \stext{  and }y+u \in Y, \ \text{ for any } x\in X, \, y\in Y \text{ and }u \in \Z^d.
$$
We define the optimization problem
\be
\label{optiTXY}
m_{\star,C_0}(X,Y) := \min\{ \#(\cT) \sep \cT\in \bT_\per \cap \bT_{\star,C_0} \text{ and }  \cT \text{ separates } X \text{ and } Y\}. %V_\cT(X) \cap V_\cT(Y)=\emptyset\}.
\ee
\end{definition}

The next proposition, which is proved in \S \ref{secOptGeom}, establishes that the optimisation problem \iref{optiTXY} is equivalent to a problem formulated in terms of metrics

\begin{proposition}
\label{propEquivSep}
We assume that the collection of meshes $\bT_\per \cap \bT_{\star,C_0}$ and the collection of metrics $\bH_\per \cap \bH_\star$ are equivalent in dimension $d$, where $\star \in \{a,b,c\}$ is a symbol and $C_0\geq 1$ is a constant.

Then there exists a constant $C\geq 1$ such that for any two closed, disjoint and periodic sets $X,Y\subset \R^d$, defining
\be
\label{optiHXY}
m_\star(X,Y) := \min\{ m(H) \sep H \in \bH_\per\cap \bH_\star \text{ and } H \text{ separates } X \text{ and } Y\}, %d_H(x,y) \geq 1 \text{ for all } (x,y) \in X \times Y\}, %
\ee
we have 
\be
%\label{eqMetricMeshSep}
C^{-1} m_\star(X,Y)\leq m_{\star,C_0}(X,Y) \leq C m_\star(X,Y).
\ee
%Furthermore a near minimizer of a problem can be built from a near minimizer of the other problem.
\end{proposition}

%This proposition thus translates the separation of the sets $X$ and $Y$ by a mesh $\cT$ into a separation formulated in terms of a metric $H$
%\be
%\label{eqSepTH}
%V_\cT(X) \cap V_\cT(Y) = \emptyset \stext{ becomes } d_H(x,y) \geq 1 \text{ for all } (x,y) \in X \times Y.
%\ee
Since $H \mapsto d_H(x,y)$ depends continuously on the metric $H \in \bH_\per$ for any fixed $x,y\in \R^d$, see \iref{distCont}, the separation of the sets $X$ and $Y$ by a metric $H$ is satisfied by a closed set of metrics. Therefore there exists a minimizer to \iref{optiHXY}.
Furthermore we can produce a near optimal mesh for \iref{optiTXY} from a near optimal metric for \iref{optiHXY}, and vice versa.

The collections of metrics satisfy the inclusion property $\bH_i \subset \bH_a \subset \bH_g$, which implies that  
$$
m_g(X,Y) \leq m_a(X,Y) \leq m_i(X,Y).
$$
This inequality reflects the fact that more regularity conditions on the metric typically raise the mass of the metric required to achieve a given task. Similarly more geometrical constraints on the meshes typically raise the cardinality of the mesh required to achieve a given task.

In order to emphasize on these differences we now turn to a specific example. We fix the parameter $r_0 = \frac 1 4$ and we define the periodic set 
$$
X := \{x\in \R^d \sep d(x,\Z^d) \leq r_0\},
$$
where $d(x,E) := \min \{|x-e|\sep e\in E\}$ for any close set $E\subset \R^d$. The set $X$ is therefore the reunion of the balls of radius $r_0$ centered at the points $u\in \Z^d$. %, as illustrated on Figure \ref{figXYDelta}.
For each $0<\delta\leq r_0$ we define 
$$
Y_\delta := \{y\in \R^d \sep d(y,\Z^d)\geq r_0 + \delta\}.
$$
The sets $X$ and $Y_\delta$ are illustrated on Figure \ref{figXYDelta}.
\begin{figure}
\centering
\includegraphics[width=4cm,height=4cm]{\pathPic/Meshing/XYDelta.pdf}
\caption{The sets $X$ (light gray) and $Y_\delta$ (dark gray), with $d=2$ and $\delta = 0.1$. \label{figXYDelta}}
\end{figure}
%The next Theorem \ref{thOptGeom} which gives an equivalent of the three quantities
%$$
%m_i(X,Y_\delta) \geq m_a(X,Y_\delta) \geq m_g(X,Y_\delta)
%$$
%as $\delta \to 0$, as well as an explicit expression of a near minimizer for each of the three optimization problems.
The next theorem, which is proved in \S \ref{secOptGeom}, gives a sharp estimate of the cost of separating the sets $X$ and $Y_\delta$ with the different classes of metrics, and therefore with the equivalent classes of meshes.
A closely related construction is illustrated on Figure \ref{figDiskApprox}.

In the following we write $F(\delta) \simeq G(\delta)$ if there exists a constant $C\geq 1$ such that for all $0 <\delta \leq r_0$,
$$
C^{-1}F(\delta) \leq G(\delta) \leq C F(\delta).
$$

\begin{theorem}
\label{thOptGeom}
We have the equivalences
\begin{eqnarray*}
m_i(X,Y_\delta) &\simeq& \delta^{-(d-1)},\\
m_a(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2 } |\ln \delta|,\\
m_g(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2}.
\end{eqnarray*}
Furthermore for any $\star \in \{i,a,g\}$  and any $0< \delta \leq r_0$ the explicit metric $H_\delta^\star\in \bH_\star \cap \bH_\per$ defined below is a near minimizer of the problem $m_\star(X,Y_\delta)$. In other words $H_\delta^\star$ separates $X$ and $Y_\delta$ and satisfies $m(H_\delta^\star) \simeq m_\star(X,Y_\delta)$.
\end{theorem}

\begin{figure}
	\centering
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskIso.pdf}
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskAigu.pdf}
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskGen.pdf}
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskNoReg.pdf}
	\caption{\label{figDiskApprox} Generation of a layer of simplices of width $\delta$ along the unit circle using $\delta^{-1}$ isotropic triangles (top left), $\delta^{-\frac 1 2} |\ln \delta|$ ``quasi-acute'' triangles (top right), $\delta^{-\frac 1 2}$ triangles satisfying the grading condition
	or not (bottom left and bottom right).}
\end{figure}


%\paragraph{Approximation of a function with respect to a mesh or a metric\\} %on a finite element space\\}

\paragraph{Approximation theory in the $L^p$ norm\\}

One of the key purposes of anisotropic mesh generation, aside from the geometrical application studied in the previous paragraph, is the adaptive approximation of functions. 
%We thus follow in this context the main objective of this chapter : the translation of the main properties of meshes into properties satisfied by the equivalent metrics. %, and we take advantage of this process to develop new tools. 
We study this application from the point of view of metrics, and for that purpose we introduce in particular two concepts : the approximation error $e_H(f)_p$ of a function $f$ with respect to a metric $H$, and the twisted mollification $f_H$ of $f$ by $H$. 

For any metric $H \in \bH$, any point $z\in \R^d$ and any $r>0$, we denote by $B_H(z,r)$ the closed ball of radius $r$ around $z$ for the norm $\|\cdot \|_{H(z)}$:
$$
B_H(z,r) := \{z+u \sep \|u\|_{H(z)}\leq r\}.
$$
When unspecified, the radius is assumed to be $1$ and the metric to be identically $\Id$
$$
B_H(z) := B_H(z,1) \stext{ and } B(z,r) := B_{\Id}(z,r) = \{z+u \sep |u|\leq r\}.
$$
For any exponent $p$, $1\leq p \leq \infty$, and any $f\in L^p_\loc(\R^d)$ we denote by $e_H(f\sep z)_p$ the error of best approximation of $f$ on $B_H(z)$:
\be
\label{defEH}
e_H(f\sep z)_p := \inf_{\mu\in \sP_{m-1} } \|f-\mu\|_{L^p(B_H(z))}.
\ee
We denote by $L^p_\per$ the collection of functions $f\in L^p_\loc(\R^d)$ which are $\Z^d$-periodic.
For all $f\in L^p_\per$ and all $H\in \bH_\per$ we define the approximation error $e_H(f)_p$ of $f$ associated to the metric $H$ as follows
$$
e_H(f)_p := \left\|\sqrt[2p]{\det H(z)} \, e_H(f\sep z)_p\right\|_{L^p([0,1]^d)}.
$$


We now turn to a second concept, the twisted mollification of a function. For that purpose we consider a fixed function $\vp\in L^\infty(\R_+, \R)$ supported in $[0,1)$ and satisfying the following moments property: for all $\mu\in \P_{m-1}$ one has 
\be
\label{eqPhiMoments}
\int_{\sR^d} \mu(z) \vp(|z|) dz = \mu(0).
\ee
For any $f\in L^1_\loc(\R^d)$ and any $H\in \bH$ we define the twisted mollification $f_H\in C^0(\R^d)$ of $f$ by the metric $H$ as follows
$$
f_H(z) := \sqrt{\det H(z)}\int_{\sR^d} f(z+u) \vp(\|u\|_{H(z)}) du.
$$

Our first result, proved in \S\ref{subsecErrMeshMetLP} compares the $L^p$ approximation error of a function with respect to a metric, and with respect to the finite element space associated to a mesh.
\begin{prop}
\label{propErrMeshMetIntro}
There exists $C=C(m,d, \vp)$ such that the following holds. Let $H\in \bH_\per \cap \bH_g$ and let $H':=4^2 H$. Let $\cT\in \bT_\per$ be such that for all $T\in \cT$ and all $z\in T$
$$
H'(z) \leq \cH_T.
$$
Let $1\leq p \leq \infty$ and let $f\in L^p_\per$, then
$$
\|f-\interp_\cT^{m-1} f_H\|_{L^p([0,1]^d)} \leq C e_H(f)_p.
$$
\end{prop}

Our next result, proved in \S\ref{subsecExistsMetLP} estimates the approximation error of a function with respect to a metric, when the function is sufficiently smooth an the mass of the metric is sufficiently large. The lower error estimate \iref{eqLowerLPD}, in Chapter \ref{chapOptAniso}, suggests that this bound is asymptotically sharp.
This result involves the shape function $K : \H_m \to \R_+$, already presented under the name $K_{m,d}^\cE$ in Chapter \ref{chapOptAniso}, which is defined as follows : for all $\pi \in \H_m$
\be
\label{defKIntro}
K(\pi) =\inf_{A\in \SL_d} \| \pi \circ A\|, %:= \inf\{(\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2}\|\leq 1\},
\ee
where $\SL_d := \{A\in \GL_d \sep \det A = 1\}$ is the special linear group. %where the infimum is taken among all symmetric positive definite matrices $M\in S_d^+$ satisfying the constraint $\|\pi\circ M^{-\frac 1 2}\|$.
We denote by $C^m_\per$ the collection of functions $f\in C^m(\R^d)$ which are $\Z^d$ periodic, and for each $z\in \R^d$ we identify $d^m f(z)$ to the corresponding homogeneous polynomial of degree $m$ in the Taylor development of $f$ near $z$.
%\be
%\label{defPizIntro}
$$
\frac{d^m f(z)}{m!} \sim \pi_z \sum_{|\alpha| = m} \frac{\partial^m f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!},
$$
%\ee
where $\alpha = (\alpha_1, \cdots, \alpha_d)$ stands for a $d$-plet of non-negative integers, and we denote $|\alpha| := \alpha_1+\cdots+\alpha_d$, $\alpha! := \alpha_1!\cdots\alpha_d!$ and $Z^\alpha := Z_1^{\alpha_1} \cdots Z_d^{\alpha_d}$. See \S\ref{subsecExistsMetLP} for more detail on these notations.
\begin{theorem}
\label{thExistsMetLPIntro}
There exists a constant $C=C(m,d)$ such that the following holds.\\
For each $f\in C^m_\per$ such that $z\mapsto K(d^m f(z))$ is not identically $0$, there exists a metric $H \in \bH_\per\cap \bH_g$, which is also $C^\infty$, and such that for all $\lambda \geq 1$
$$
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|K(d^m f)\right\|_\tau,
$$
where $\frac 1 \tau := \frac m d+ \frac 1 p$.
\end{theorem}


The heuristic guideline of this proof is the following. We first rephrase the optimization among the special linear group $\SL_d$ defining $K$ into an optimization among the collection $S_d^+$ symmetric positive definite matrices.
%We recall that $\SL_d := \{A\in \GL_d \sep \det A = 1\}$.
\begin{lemma}
\label{lemmaAM}
Let $\psi \in C^0( \GL_d, \R_+^*)$ be homogeneous of degree $r>0$ and satisfy $\psi(A) = \psi(AO)$ for any $A\in \GL_d$ and any $O\in \cO_d$. Then 
$$
\inf \{(\det M)^\frac r {2d} \sep M\in S_d^+ \text{ and } \psi(M^{-\frac 1 2}) \leq 1\} = \inf \{\psi(A) \sep A\in \SL_d\}.
$$
\end{lemma}

\proof
To each $M\in S_d^+$ we associate $A := (\det M)^\frac 1 {2d} M^{-\frac 1 2}\in \GL_d$, in such way that $\det(A) = 1$ and $\psi(A) = (\det M)^{\frac r {2d}} \psi(M^{-\frac 1 2})$. Conversely to  each $A\in \GL_d$ we associate $M := \psi(A)^\frac 2 r (A A^\trans)^{-1}\in S_d^+$, in such way that $(\det M)^\frac r{2d} = \psi(A)$ and $\psi(M^{-\frac 1 2}) = \psi(\psi(A)^{-\frac 1 r} (A A^\trans)^\frac 1 2) = \psi(A)^{-1}\psi(AO) = 1$ where $O := A^{-1} (A A^\trans)^\frac 1 2$ is orthogonal. 
\sq

We thus have 
\be
\label{defKMSD}
K(\pi) = \inf\{(\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2}\|\leq 1\},
\ee
Assume that for all $z\in \R^d$ there exists a unique minimizer $M_z\in S_d^+$ to the minimization problem on $S_d^+$ defining $K(d^m f(z))$, and assume that $M_z$ depends smoothly on $z$.
Define 
$$
H(z) := \Lambda \, (\det M_z)^{\frac {-1}{mp+d}} M_z,
$$
where $\Lambda>0$ is a sufficiently large constant. A simple analysis, using Taylor developments, shows that $H$ satisfies \iref{eqHSmooth}.

Unfortunately the minimization problem appearing in \ref{defKMSD} is not well posed : depending on the polynomial $\pi\in \H_m$ there may exist no minimizer or an infinity of minimizers. The key ingredient of the proof of Theorem \ref{thExistsMetLPIntro} is a variant $K^{(\alpha)}(\pi)$ of the shape function $K(\pi)$ which is defined by a well posed ``geometrically convex'' minimization problem among symmetric positive definite matrices. 

\paragraph{Approximation theory in the Sobolev $W^{1,p}$ norm\\}

The extension to the $W^{1,p}$ semi-norm of the previous results is not straightforward due to the following phenomenon. The gradient of the interpolation $\interp_\cT^{m-1} g$ of a function, or of the twisted mollification $f_H$ may have strong undesirable oscillations which are not present in the original function. The next key lemma
%, which is proved in \S\ref{subsubsecErrMeshMetW1PA}, 
guarantees the absence of these properties in the case of quasi-acute triangulations and metrics.

\begin{lemma}
\label{lemmaBoundedQA}
There exists $C=C(m,d, \vp)$ such that the following holds.
\begin{itemize}
\item (Gradient of an interpolation) Let $T$ be a simplex, and let $g\in W^{1,\infty}(T)$, then 
$$
\|\nabla \interp_T^{m-1} g\|_{L^\infty(T)} \leq C S(T) \|\nabla g\|_{L^\infty(T)}.
$$
\item (Gradient of a twisted mollification) Let $H\in \bH_a$ be a quasi-acute metric, and let $f\in W^{1,1}_\loc$. Then $f_H\in W^{1,\infty}_\loc$ and for all $z\in \R^d$
$$
\dil_z (f_H)  \leq C \|\nabla f\|_{L^1(B_H(z))}
$$
where $\dil_z(f_H) := \lim_{\ve \to 0} \|\nabla f_H\|_{L^\infty(B(z,\ve))}$ is the local dilatation of $f$ at $z$.
\end{itemize}
\end{lemma}
\proof
The first property, on the gradient of an interpolation, is established in Chapter \ref{chapW1P}. The second property, on the twisted mollification, is obtained as follows.
Denoting $S(z) := H(z)^{-\frac 1 2}$ we obtain  
\be
\label{eqfHS}
f_H(z) = \int_{|u|\leq 1} f(z +S(z) u) \vp(|u|) du,
\ee
and for any $u\in\R^d$, $|u|\leq 1$, the map
$$
z\mapsto z+S(z)u
$$
is $2$-Lipschitz, since $z\mapsto S(z)$ is Lipschitz.
Derivating \iref{eqfHS} we obtain the announced result.
\sq

We introduce two types of approximation error of a vector field $v$ with respect to a metric $H$.
For any $v\in L^p_\loc(\R^d, \R^d)$, any $H \in \bH$ and any $z\in \R^d$ we define 
\be
\label{defEHA}
e_H^a(v\sep z)_p := \min_{\nu\in \sP_{m-2}^d} \|v-\nu\|_{L^p(B_H(z))}
\ee
and 
%\stext{ and } 
\be
\label{defEHG}
e_H^g(v\sep z)_p := \|H(z)\|^{\frac 1 2} \min_{\nu\in \sP_{m-2}^d} \|H(z)^{-\frac 1 2} (v-\nu)\|_{L^p(B_H(z))},
\ee
where $\P_{m-2}^d$ denotes the collection of $d$-plet of polynomials of degree $m-2$. 
If $v$ is $\Z^d$ periodic, if $H\in \bH_\per$ and $\star\in \{a,g\}$, then we define 
$$
e_H^\star(v)_p := \left\|\sqrt[2p]{\det H(z)} \, e_H^\star(v\sep z)_p\right\|_{L^p([0,1]^d)}.
$$

Observe that $e_H^a(\nabla f)_p$ is the straightforward generalisation of $e_H(f)_p$ to the Sobolev $W^{1,p}$ semi-norm. In contrast the definition \iref{defEHG} implies that $e_H^g(\nabla f)_p \geq e_H^a(\nabla f)_p$. This inequality, which deteriorates as the anisotropy of the metric $H$ increases, represents the price to pay for the use of graded triangulations and metrics instead of quasi-acute ones (an point worth studying since current mesh generation software only produce graded meshes). 


The next propositions, which are established in \ref{subsecErrMeshMetW1P}, compare the $W^{1,p}$ finite element approximation error of a function on a mesh with these two types of errors with respect to a metric.

\begin{prop}
\label{propErrMeshMetAIntro}
There exists $C=C(m,d)$ such that the following holds. Let $H\in \bH_\per \cap \bH_a$ and let $H':=4^2 H$. Let $\cT\in \bT_\per$ be such that for all $T\in \cT$ and all $z\in T$
$$
H'(z) \leq \cH_T.
$$
Let $1\leq p \leq \infty$ and let $f\in W^{1,p}_\per$, then
$$
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p([0,1]^d)} \leq C \, e_H^a(f)_p \, \max_{T\in \cT} S(T).
$$
\end{prop}

\begin{prop}
\label{propErrMeshMetGIntro}
For all $C_0$ there there exists $C=C(C_0m,d)$ such that the following holds. Let $H\in \bH_\per \cap \bH_g$ and let $H':=4^2 H$. Let $\cT\in \bT_\per$ be such that for all $T\in \cT$ and all $z\in T$
$$
H'(z) \leq \cH_T\leq C_0^2 H'(z).
$$
Let $1\leq p \leq \infty$ and let $f\in W^{1,p}_\per$, then
$$
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p([0,1]^d)} \leq C e_H^g(f)_p.
$$
\end{prop}

Our next result, which generalizes Theorem \ref{thExistsMetLPIntro}, estimates the $W^{1,p}$ approximation error of a sufficiently smooth function with respect to a metric of sufficiently large mass. The lower error estimate established in Theorem \ref{optiTheoremD}, in Chapter \ref{chapW1P}, suggests that this bound is asymptotically sharp in the case of quasi-acute metrics.
We introduce 
two shape functions $L_a,L_g:\H_m \to \R_+$ which are defined as follows: for each $\pi\in \bH_m$
$$
L_a(\pi) := \inf_{A\in \SL_d} \|(\nabla \pi)\circ A\| 
\stext{ and }
L_g(\pi) := \inf_{A\in \SL_d} \|A^{-1}\| \|\nabla (\pi\circ A)\| %\inf \{ (\det M)^{\frac {m-1} {2d}} \sep \sqrt{\|M\|} \|\nabla 
$$
%\begin{eqnarray*}
%L_a(\pi) &:=& \inf_{A\in \SL_d} \|(\nabla \pi)\circ A\| \\%\inf \{ (\det M)^{\frac {m-1} {2d}} \sep \|(\nabla \pi)\circ M^{-\frac 1 2}\| \leq 1\}\\
%L_g(\pi) &:=& \inf_{A\in \SL_d} \|A^{-1}\| \|\nabla (\pi\circ A)\| %\inf \{ (\det M)^{\frac {m-1} {2d}} \sep \sqrt{\|M\|} \|\nabla (\pi\circ M^{-\frac 1 2})\| \leq 1\},
%\end{eqnarray*}
where for all $\nu\in \H_{m-1}^d$ we denote % the norm on $\H_{m-1}^d$ defined as follows 
$$
\|\nu\| := \sup_{|z|\leq 1} |\nu(z)|.
$$
The next theorem is proved in \S\ref{subsecExistsMetW1P}.
\begin{theorem}
\label{thExistsMetW1PIntro}
There exists a constant $C=C(m,d)$ such that the following holds.\\
Consider $f\in C^m_\per$, $\star\in \{a,g\}$, and $1\leq p\leq \infty$. %, and assuming that the right hand side in \ref{eqMetricA} and \ref{eqMetricG} is nonzero.
If $z\mapsto L_\star(d^m f(z))$ is not identically $0$, then
there exists a metric $H \in \bH_\per\cap \bH_\star$, which is also $C^\infty$, and such that for all $\lambda \geq 1$
\be
\label{eqMetricA}
m(\lambda H)^{\frac {m-1} d} e_{\lambda H}^\star(\nabla f)_p \leq C \left\|L_\star(d^m f)\right\|_\tau,
\ee
where $\frac 1 \tau := \frac {m-1} d+ \frac 1 p$.
\end{theorem}

The guideline of this proof is the same as for Theorem \ref{thExistsMetLPIntro} in the case of the $L^p$ norm.
We first remark using Lemma \ref{lemmaAM} that 
\be
\label{eqLALGM}
\begin{array}{rcl}
L_a(\pi) &:=& \inf \{ (\det M)^{\frac {m-1} {2d}} \sep \|(\nabla \pi)\circ M^{-\frac 1 2}\| \leq 1\}\vspace{2mm}\\
L_g(\pi) &:=& \inf \{ (\det M)^{\frac {m-1} {2d}} \sep \sqrt{\|M\|} \|\nabla (\pi\circ M^{-\frac 1 2})\| \leq 1\}.
\end{array}
\ee
Assume that for each $z\in \R^d$ the minimum on $S_d^+$ defining $L_\star(d^m f(z))$ is attained for a matrix $M_z\in S_d^+$ depending smoothly on $z$. We obtain \iref{eqMetricA} using the metric
$$
H(z) := \Lambda (\det M_z)^{\frac{-1}{(m-1)p+d} } M_z,
$$
where $\Lambda$ is denotes a sufficiently large constant. The key ingredient of the proof is thus to define a well posed variant of the minimization problems among symmetric matrices appearing in \iref{eqLALGM}.\\

For practical applications the existence result stated by Theorem \ref{thExistsMetW1PIntro} is not sufficient, and an efficient way to compute the metric $H$ from the (estimated) $m$-th order derivatives of $f$ is required.
For that purpose we give in Proposition \ref{propLmIntro} an explicit expression of minimizers or near minimizers of the shape functions $L_a$ and $L_g$ in the case of linear $m=2$ or quadratic $m=3$ approximation in dimension $2$. 

%problem with $S_d^+$ and $S_d^{++}$
Let $\phi : S_d^+\to \R_+$ be function, %a homogeneous function, 
let  $X$ be a set  and let $\psi_x : S_d^+ \to \R_+$ be a family of functions indexed by $x\in X$. % homogeneous functions of degree independent of $x$. 
A near minimizer of the optimization problem posed on $S_d^+$
$$
L(x) := \inf\{\phi(M) \sep \psi_x(M)\leq 1\}
$$
is a map $\cM : X \to S_d^+$ satisfying the following property : there exists two positive constants $C,C'$ such that for all $x\in X$ one has 
$$
\phi(C \cM(x)) \leq C' L(x) \stext{ and } \psi_x(C \cM(x)) \leq 1.
$$


\begin{prop}
\label{propLmIntro}
\begin{itemize}
\item (Piecewise linear approximation, in any dimension)
If $m=2$ and $d\geq 2$, then for any $\pi\in \H_2$, one has 
$$
L_a(\pi) = |\det \pi| \stext{ and } L_g(\pi) = \sqrt{\|\pi\|} \sqrt[4]{|\det \pi|}.
$$
The minimizing matrices $M$ in the minimization problems defining $L_a(\pi)$ and $L_g(\pi)$ are  respectively
$$
\cM_a(\pi) = [\pi]^2 \stext{ and } \cM_g = \|\pi\| \, |[\pi]|
$$
\item (Piecewise quadratic approximation, in two dimensions)
If $m=3$ and $d=2$, let $\pi =  a x^3+ 3 b x^2 y+ 3 c x y^2+ d y^3\in \H_3$,
let 
\be
\label{eqMaPi}
\cM_a(\pi) =  %\sqrt{ [\partial_x \pi]^2+ [\partial_y \pi]^2} = 
3 \sqrt{
\left(\begin{array}{cc}
a & b\\
b & c
\end{array}\right)^2
+
\left(\begin{array}{cc}
b & c\\
c & d
\end{array}\right)^2
}
\ee
and let 
\be
\label{eqMgPi}
\cM_g(\pi) := \cM_a(\pi) + \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}\Id
\ee
where $\disc \pi$ is the discriminant of the cubic polynomial $\pi$ :  
$$
\frac{1} {27} \disc \pi= 4(ac-b^2)(bd-c^2) - (ad-bc)^2.
$$
Then $\cM_a(\pi)$ and $\cM_g(\pi)$ are near minimizers of optimization problems defining $L_a(\pi)$ and $L_g(\pi)$ respectively.
\end{itemize}
\end{prop}

Let us mention that \iref{eqMgPi} is the only new result since \iref{eqMaPi} is established in Chapter \ref{chapW1P}, and since the case $m=2$ of linear approximation is already known.


\section{Compactness of metrics of a given mass} %A compactness property}
\label{secCompact}

We recall that the collection $\bH_\per$ of $\Z^d$ periodic metrics is equipped with the distance 
$$
d_\per(H,H') := \sup_{z\in \sR^d} d_\times (H(z), H'(z)).
$$
The purpose of this section is to establish Theorem \ref{thCompact} which states that for any $\star \in \{i,a,g\}$ and any $m_0 \geq 1$ the collection of metrics 
\be
\label{defHStarM}
\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq m_0\}
\ee
is compact.
Our first lemma establishes that this set is closed in $\bH_\per$.

\begin{lemma}
\label{lemmaClosed}
The sets $\bH_\per \cap \bH_\star$, where $\star\in \{i,a,g\}$, are closed in of  $\bH_\per$, as well as the collection of metrics $\{H \in \bH_\per \sep m(H) \leq m_0\}$. 
\end{lemma}

\proof
We remarked in \iref{distCont} that for any two fixed $x,y\in \R^d$ the map $\bH_\per \to \R_+$, $H \mapsto d_H(x,y)$ is continuous. Consequently for any $x,y\in \R^d$ the collection of metrics satisfying 
\be
\label{eqHdH}
d_\times (H(x), H(y)) \leq d_H(x,y)
\ee
is closed in $\bH_\per$. Since the intersection of closed sets is also a closed set the collection $\bH_\per \cap \bH_g$ of metrics which satisfying \iref{eqHdH} for all $x,y\in \R^d$ is closed in $\bH_\per$.

The pointwise evaluation $\bH_\per \to \R_+$, $H\mapsto H(z)$ at a fixed point $z$ is continuous. For any given $x,y\in \R^d$ the collection of metrics $H \in \bH_\per$ satisfying
$$
d_+(H(x),H(y)) \leq |x-y|
$$ 
is closed, which implies that $\bH_\per\cap \bH_a$ is a closed subset of $\bH_\per$. 
Recalling that the collection of isotropic metrics $\{\lambda \Id \sep \lambda\in \R_+^*\}$ is a closed subset of $S_d^+$, we obtain that $\bH_\per \cap \bH_i$ is closed in $\bH_\per$.

The collection of metrics satisfying  $m(H)\leq m_0$ is closed since $m(H)$ depends continuously on $H \in \bH_\per$, see \iref{massCont}, which concludes the proof.
\sq

In order to establish that \iref{defHStarM} is compact, we thus only have to prove that the set 
\be
\label{defHGM}
\{H \in \bH_\per \cap \bH_g \sep m(H) \leq m_0\}
\ee
corresponding to the case $\star = g$ is compact. Our next result, Lemma \ref{lemmaCompact}, shows that it is sufficient to prove that \iref{defHGM} is bounded.

The key ingredient of this lemma is the following classical theorem of Ascoli, which states that the collection of Lipschitz functions between two compact metric spaces is itself a compact metric space. 
\begin{theorem}[Ascoli]
\label{thAscoli}
If two metric spaces $(X,d_X)$ and $(Y,d_Y)$ are compact, then the collection $\Lip(X,Y)$  of Lipschitz functions from $X$ to $Y$ is also compact when
equipped with the distance 
$$
d(f,g) := \max_{x\in X} d_Y(f(x),g(x)).
$$
\end{theorem}

We use this theorem to establish that, similarly to finite dimensional spaces, closed and bounded subsets of $\bH_\per \cap \bH_g$ are compact.

\begin{lemma}
\label{lemmaCompact}
Any closed and bounded subset $\bH_*$ of $\bH_\per \cap \bH_g$ is compact.
\end{lemma}

\proof
Since the collection $\bH_*$ of metrics is bounded, the quantity $C$ defined below is finite
$$
C^2 := \sup_{H \in \bH_*} \sup_{z\in [0,1]^d} \|H(z)\|.
$$
For any $x,y\in \R^d$ and any $H \in \bH_*$ we thus have $d_H(x,y) \leq M|x-y|$.

We consider the compact metric space $X :=[0,1]^d$, equipped with the distance $d_X(x,y) := M|x-y|$, and the compact metric space $Y := \{M \in S_d^+ \sep \Id \leq M \leq C^2 \Id\}$ equipped with the distance $d_\times$.
According to Theorem \ref{thAscoli} the metric space $\Lip(X,Y)$ is thus compact.

Consider a sequence $(H_n)_{n\geq 0}$ of elements of $H_*$. For all $n \geq 0$, the restriction $H_{n|[0,1]^d}$ is an element of $\Lip(X,Y)$. Since this space is compact there exists a sub-sequence $H_{\vp(n)}$ which converges uniformly on $[0,1]^d$. Recalling that $H_n$ is periodic for all $n\geq 0$ we find that $H_{\vp(n)}$ converges uniformly to a periodic metric $H \in \bH_\per$. 

Since that $\bH_*$ is closed in $\bH_\per \cap \bH_g$, and since $\bH_\per \cap \bH_g$ is closed in $\bH_\per$, we obtain that $\bH_*$ is closed in $\bH_\per$ and therefore $H \in \bH_*$ which concludes the proof.
\sq

The second point of the next lemma establishes Theorem \ref{thCompact} as announced.
\begin{lemma}
\label{propCompact}
Let $m_0 \geq 1$ be a constant.
\begin{enumerate}
\item
There exists $C=C(m_0,d)$ such that for any $H \in \bH_g$ satisfying $H(z) \geq \Id \text{ for all } |z|\leq 1$ and 
$$
\int_{|z|\leq 1} \sqrt{\det H(z)} dz \leq m_0
$$
we have $\|H(0)\|\leq C^2$.
\item
The set 
$
\{H \in \bH_\per \cap \bH_g \sep m(H) \leq m_0\}
$
is bounded, and thus compact.
\end{enumerate}
\end{lemma}

\proof
We first show how 2. can be obtained assuming 1., and for that purpose we consider $H \in \bH_\per \cap \bH_g$ and $z_* = (z_1, \cdots ,z_d)\in \R^d$. The ball $\{z\in \R^d \sep |z-z_*|\leq 1\}$ is covered by the $2^d$ cubes 
$z_*+u+[0,1]^d$ where $u \in \{-1,0\}^d$. Consequently 
$$
\int_{|z-z_*|\leq 1} \sqrt{\det H(z)} dz \leq \sum_{u\in \{-1,0\}^d } \int_{z_*+u+[0,1]^d} \sqrt{\det H} = 2^d m_0
$$
and we already know that $H(z) \geq \Id$ for all $z\in \R^d$. It follows that $\|H(z_*)\|\leq C'^2$ where $C'$ is the constant associated to $2^d m_0$ in point 1. of this lemma, which concludes the proof of 2.\\


We now turn to the proof of 1., and for that purpose we consider a metric $H\in K_M$.
For each point $z\in \R^d$ we denote the eigenvalues of $H(z)$ by 
$$
\lambda_1^2(z) \geq \cdots \geq \lambda_d^2(z).
$$
For each $k \in \{1, \cdots ,d\}$ the function $\lambda_k$ is continuous and $\lambda(z)\geq 1$ for all $|z|\leq 2$.

Our purpose is to obtain an upper bound for $\lambda_1(0) = \sqrt{\|H(0)\|}$ in terms of $m_0$.
We shall proceed as follows : We first give an upper bound for $\lambda_d(0)$ that depends only on $m_0$, and then for each $1\leq k \leq d-1$ we give an upper bound for $\lambda_k(0)$ in terms of $m_0$ and $\lambda_{k+1}(0)$.


\paragraph{The upper bound on $\lambda_d(0)$.}
Denote by $\cE$ the ellipse $\cE := \{z\in \R^d \sep \|z\|_{H(0)} \leq \lambda_d(0)\}$, and observe that $|z|\leq 1$ for all $z\in \cE$.
We thus obtain using Corollary \ref{corolVol} 
$$
c_d \ln \lambda_d(0) \leq \int_\cE \sqrt{\det H(z)} dz \leq  \int_{|z|\leq 1} \sqrt{\det H(z)} dz \leq m_0,
$$
where the constant $c_d$ depends only on $d$. This gives as announced an upper bound on $\lambda_d(0)$ in terms of $m_0$.

\paragraph{The upper bound on $\lambda_k(0)$.}
The vector space $\R^d$ is the orthogonal sum $\R^d = U\oplus V$ where $U$ is the sum of the eigenspaces  associated to the eigenvalues $\lambda_1^2(0), \cdots, \lambda_k^2(0)$ of $H(0)$ and $V$ is associated to the other eigenvalues $\lambda_{k+1}^2(0), \cdots, \lambda_d^2(0)$ of $H(0)$.
In particular for all $u\in U$ and for all $v\in V$, 
$$
\|u\|_{H(0)} \geq \lambda_k(0) |u| \stext{ and } \|v\|_{H(0)} \leq \lambda_{k+1}(0) |v|.
$$

We consider an isometry $P\in \cO_{d,k}$ satisfying $P(\R^k) = U$. 
%We consider a $k\times d$ matrix $P\in M_{d,k}(\R^d)$, satisfying $P(\R^k) = U$. We assume that $P$ is an isometry, in other words the columns of $P$ form an orthonormal basis of $U$.
For each $v\in V$ we define a $k$-dimensional metric $H_v\in \bH(\R^k)$ as follows: for all $u \in \R^k$,
$$
H_v(u) := P^\trans H_v(v+ Pu) P.
$$
We define 
$$
B_U := \{u \in \R^k \sep |u|\leq 1/2\} \stext{ and } B_V := \{v\in V \sep \lambda_{k+1}(0) |v| \leq 1/2\},
$$
in such way that 
\be
\label{eqFubiniSet}
|P u+v| \leq 1 \text{ for all }  (u,v)\in B_U \times  B_V
\ee
%Consider $u\in \R^k$ and $v\in V$ satisfying $|u|\leq 1$ and $|v|\leq 1$, in such way that $|Pu+v|\leq 2$. 
Recalling that $\lambda_i(z)\geq 1$ for all $1\leq i \leq d$ and $|z| \leq 1$ we obtain for all $(u,v) \in B_U \times B_V$
\be
\label{eqDetHHV}
\begin{array}{rcl}
\det H_v(u) &\leq& \lambda_1^2(Pu +v) \cdots \lambda_k^2(Pu +v)\\
&\leq &  \lambda_1^2(Pu +v) \cdots \lambda_d^2(Pu +v)\\
& =& \det H(Pu+v)
\end{array}
\ee
For any $u\in \R^k$ and any $v\in V$ we have according to \iref{eqLocalNorm}
\be
\label{eqLowerHV}
\|u\|_{H_v(0)} = \|Pu\|_{H(v)} \geq (1-\|v\|_{H(0)}) \|Pu\|_{H(z_*)} \geq \lambda_k(0) |u|/2. %(1-\lambda_{k+1}(0) |v|) \lambda_k(0) |u|.
\ee

According to Proposition \ref{propHG}, the metric $H_v$ belongs to the set $\bH_g(\R^k)$ of graded metrics on $\R^k$. Denoting by $c_k$ the constant from Corollary \ref{corolVol} applied in dimension $k$, and recalling \iref{eqLowerHV}, we therefore obtain for any $v\in B_V$
\be
\label{eqHVBU}
\int_{B_U} \sqrt{\det H_v(u)} du \geq c_k \ln ( \lambda_k(0)/4)
\ee
We thus obtain successively %According to Proposition (restrictMet) we have $H_v\in \bH_g^k$, therefore 
\begin{eqnarray*}
\int_{|z|\leq 1} \sqrt{\det H(z)} dz &\geq& \int_{v\in B_V} \int_{u\in B_U} \sqrt{\det H(P u +v)} du dv\\
&\geq & \int_{v\in B_V} \int_{u \in B_U} \sqrt{\det H_v(u)} du dv\\
& \geq & \int_{v\in B_V} c_k \ln(\lambda_k(0)/4) dv\\
& = & |B_V| c_k \ln( \lambda_k(0)/4)\\
& = & \frac{\omega_{d-k}}{(2\lambda_{k+1}(0))^{d-k}} c_k \ln( \lambda_k(0)/4).
\end{eqnarray*}
Where we use\iref{eqFubiniSet} and Fubini integration formula in the first line, \iref{eqDetHHV} in the second line, and \iref{eqHVBU} in the third line. In the last line we denote by  $\omega_{d-k}$ the volume of the unit ball in $\R^{d-k}$.
%, and by $c_k$ the constant from Proposition (volBall) attached to the dimension $k$.
% and which is an isometry $P^\trans P = \Id_i$.
%We define for each $v\in V$ a metric $H_v$ on $\R^i$ as follows. For all $u\in \R^i$

This inequality yields an upper bound on $\lambda_k(0)$ in terms of $M$ and $\lambda_{k+1}(0)$
$$
\lambda_k(0) \leq 4 \exp\left(\frac {m_0 (2\lambda_{k+1}(0))^{d-k}}{\omega_{d-k}}\right),
$$
which concludes the proof of this Theorem.
\sq

%
%\subsection{Extension to non-periodic metrics (*useful?*)}
%
%The compactness property established above is not restricted to periodic metrics: 
%appropriately generalized it also holds for metrics defined on the unbounded domain $\R^d$.
%
%For that purpose we introduce some notations.
%For each $n \geq 1$ we introduce a semi-distance $d_n$ on the collection $\bH$ of metrics: for all $H,H' \in \bH$
%$$
%d_n(H,H') := \sup_{|z|\leq 1} d_\times (H(z), H'(z)).
%$$
%The standard compact-open topology on $\bH$ is defined by the family of semi-distances $(d_n)_{n \geq 1}$, or equivalently by the single distance 
%$$
%d_\infty(H,H') := \sum_{n \geq 1} \min \{2^{-n}, \, d_n(H,H')\}.
%$$
%
%\begin{lemma}
%For any $x,y\in \R^d$ the map $\bH_g \to \R_+$, $H \mapsto d_H(x,y)$ is continuous.
%\end{lemma}
%\proof
%To do.
%\sq
%
%
%We say that a subset $\bH_*\subset \bH_g$ is bounded if $\bH_*$ is bounded for any $n \geq 1$
%$$
%\sup_{H,H'\in \bH_*} d_n(H,H') <\infty.
%$$
%
%\begin{lemma}
%Any closed and bounded set $\bH_*\subset \bH_g$ is compact.
%\end{lemma}
%\proof
%To do.
%\sq
%
%\begin{theorem}
%Let $(\ve_n)_{n \geq 1}$ be a sequence of strictly positive reals. The collection of metrics $H \in \bH_g$ satisfying for all $n \geq 1$
%$$
%\int_{|z|\leq n} \sqrt{\det H(z)}dz \leq \ve_n^{-1} \stext{ and } H(z) \geq \ve_n \Id \text{ for all } |z|\leq n
%$$
%is compact.
%\end{theorem}
%
%\proof
%
%\sq


\section{An optimization problem : the separation of geometric subdomains}
\label{secOptGeom}

We study in this section a geometrical problem: the separation of two sets using a triangulation, of minimal cardinality. Our first result, Proposition \ref{propEquivSep2}, establishes that this problem has an equivalent formulation in terms of metrics. We then study a particular case in Theorem \ref{thOptGeom}.

Proposition \ref{propEquivSep2} was announced in the introduction under the number \ref{propEquivSep}.
\begin{proposition}
\label{propEquivSep2}
We assume that the collection of meshes $\bT_\per \cap \bT_{\star,C_0}$ and the collection of metrics $\bH_\per \cap \bH_\star$ are equivalent in dimension $d$, where $\star \in \{a,b,c\}$ is a symbol and $C_0\geq 1$ is a constant.\\

There exists a constant $C \geq 1$ such that the following holds:\\
Let $X,Y \subset \R^d$ be two closed, disjoint and periodic sets, in the sense that 
$$
x+u \in X \stext{  and }y+u \in Y, \ \text{ for any } x\in X, \, y\in Y \text{ and }u \in \Z^d.
$$
Consider the two optimization problems 
\begin{eqnarray*}
m_{\star,C_0}(X,Y) &:=& \min\{ \#(\cT) \sep \cT\in \bT_\per \cap \bT_{*,C_0} \text{ and } \cT \text{ separates } X \text{ and } Y\},\\
m_\star(X,Y) &:=& \min\{ m(H) \sep H \in \bH_\per\cap \bH_* \text{ and } H \text{ separates } Y \text{ and } Y\}.
\end{eqnarray*}
Then 
\be
\label{eqMetricMeshSep}
C^{-1} m_\star(X,Y)\leq m_{\star,C_0}(X,Y) \leq C m_\star(X,Y).
\ee
%Furthermore a near minimizer of a problem can be built from a near minimizer of the other problem.
\end{proposition}

\proof %(* name of constants?*)
The proof of this proposition is a simple translation between the vocabulary of meshes and the vocabulary of metrics.
We first establish that $m_\star(X,Y) \leq C m_{\star,C_0}(X,Y)$, and then that $m_{\star,C_0}(X,Y) \leq C m_\star(X,Y)$.

As announced in the proposition, we assume that there exists a constant $C_1\geq 1$ such that for and $\cT\in \bT_\per \cap \bT_{\star, C_0}$ there exists $H\in \bH_\per\cap \bH_\star$ which is $C_1$ equivalent to $\cT$, and vice versa.


\begin{itemize}
\item
Let $\cT\in \bT_\per \cap \bT_{\star,C_0}$ be a mesh which separates the sets $X$ and $Y$, and let $H \in \bH_\per \cap \bH_\star$ be a metric which is $C_1$ equivalent to $\cT$. We thus have for any $T\in \cT$ and any $z\in T$
$$
C_1^{-2}H(z)\leq \cH_T \leq C_1^2 H(z).
$$
Let $x\in X$ and let $y\in Y$. Let $T_0\in \cT$ be the simplex containing $x$ and let $V_{T_0}(\cT)$ be the neighborhood of $T_0$ in $\cT$, in other words union of all simplices in $\cT$ which intersect $T_0$.
Since $x\in T_0$ and $y\notin V_\cT(T_0)$ there exists according to Proposition \ref{propNeighborT} a constant $c=c(C_0,d)$ such that $\|x-y\|_{\cH_{T_0}}\geq c$. It follows that 
$$
d_H(x,y) \geq \ln (1+\|x-y\|_{H(x)}) \geq \ln(1+ \|x-y\|_{\cH_{T_0}}/C_1) \geq r:=\ln (1+c C_1^{-1}).
$$
Up to replacing $r$ with $\min\{1,r\}$ we may assume that $0<r\leq 1$.
The metric $\ti H := r^{-2} H$ thus belongs to $\bH_\per \cap \bH_\star$, separates the sets $X$ and $Y$, and satisfies according to Proposition \ref{propCardMass}
$$
m(\ti H)  \leq (C_1/r)^d |\TEq|\#(\cT). %=r^{-d} m(H)
$$ 

Taking the infimum over all meshes $\cT\in \bT_{*,C_0}$ which separate $X$ and $Y$ we obtain the announced inequality $m_*(X,Y) \leq |\TEq| (C_1/r)^d \, m_{*,C_0}(X,Y)$.

\item
We now consider a Riemannian metric $H\in \bH_*\cap \bH_\per$ which separates the sets $X$ and $Y$. We consider a parameter $\lambda \geq 1$, which value will be specified later, and we observe that $\ti H := \lambda^2 H \in \bH_*\cap \bH_\per$.  Therefore there exists a mesh $T\in \bT_{*, T_0}\cap\bT_\per$ such that for all $T\in \cT$ and all $z\in \cT$ one has
$$
C_1^{-2} \ti H(z)\leq \cH_T \leq C_1^2 \ti H(z).
$$

Let us assume for contradiction that $\cT$ does not separate the sets $X$ and $Y$, hence that $V_\cT(X) \cap V_\cT(Y) \neq \emptyset$. In that case there exists two simplices $T,T'\in \cT$ sharing a vertex $v$, and two points $x\in T \cap X$ and $y\in T'\cap Y$.
We recall that for any simplex $T$ and any $z,z'\in T$ we have $\|z-z'\|_{\cH_T}\leq 2$.
Therefore 
$$
\lambda \leq d_{\ti H}(x,y) \leq d_{\ti H}(x,v) + d_{\ti H} (v,y) \leq C_1 (\|x-v\|_{\cH_T}+ \|v-y\|_{\cH_{T'}}) \leq 4 C_1.
$$
We now choose the particular the value $\lambda := 4C_1+1$, which contradicts the the previous equation and shows that $\cT$ does separate $X$ and $Y$.
Furthermore
$$
|\TEq| \#(\cT) \leq  \, C_1^d \, m(\ti H) = (\lambda C_1)^d m(H).
$$
Taking the infimum among all metrics $H \in \bH_*$ which separate $X$ and $Y$ we obtain $|\TEq| m_{*,C_0}(X,Y) \leq  (\lambda C_1)^d m_*(X,Y)$, which concludes the proof of this proposition.
\sq
\end{itemize}

The rest of this section is devoted to the proof of Theorem \ref{thOptGeom}, in which we consider the particular sets 
\be
\label{defXYDelta}
X := \{x\in \R^d \sep d(x,\Z^d)\leq r_0\} \stext{ and } Y_\delta := \{y\in \R^d \sep d(y, \Z^d \geq r_0+ \delta\}
\ee
where $r_0 := 1/4$ and $0<\delta\leq r_0$. For any $\star\in \{i,a,g\}$ we obtain explicit equivalents of the quantities $m_\star(X,Y_\delta)$ as $\delta \to 0$, as well as an explicit expressions of a near minimizer $H_\delta^\star\in \bH_\per \cap \bH_\star$ to this optimization problem.

The proof is divided in two parts: we first give the explicit expression of the metrics $H_\delta^\star$ and use it to obtain an upper bound on $m_\star(X,Y_\delta)$. We then prove a lower bound for $m_\star(X,Y_\delta)$.

\subsection{Explicit metrics and upper bound}

%The proof of this Theorem is split into three lemmas. 
We define in this section the metrics $H_\delta^\star$, where $\star \in \{i,a,g\}$ and $0 < \delta \leq r_0 := 1/4$. We then establish in Lemma \ref{lemmaHInH} that $H_\delta^*\in \bH_*$ and $H_\delta^*$ separates $X$ and $Y_\delta$. We then prove in Lemma \ref{lemmaMHDelta} an upper estimate on the masses $m(H_\delta^*)$ of these metrics. 

%Eventually we establish in Lemma \ref{lemmaMLower} a lower estimate on $m_*(X,Y_\delta)$ which concludes the proof of this theorem.

%We begin the proof of this theorem by the definition of the metrics 
In order to define $H_\delta^*$ we need to introduce some notations. For any $z\in \R^d \sm\{0\}$ we define
\be
\label{defsz}
s(z) := \min\{r_0, \left| |z|-r_0\right|\} \stext{ and } \n_z := \frac z {|z|}.
\ee
For any $0 < \delta \leq r_0$ and any $z\in \R^d\sm\{0\}$ we define three matrices $S_\delta^\star(z) \in S_d^+$, where $\star\in \{i,a,g\}$, as follows 
\be
\label{defSDeltaStar}
\begin{array}{rcl}
S_\delta^i(z) &:=& \max\{s(z), \delta\} \, \Id\vspace{0.2ex}\\
S_\delta^a(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \max\left\{s(z), \sqrt \delta\right\} \, (\Id - \n_z \n_z^\trans)\vspace{0.2ex}\\
S_\delta^g(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \sqrt{r_0\max\{s(z), \delta\}} \, (\Id - \n_z \n_z^\trans).
\end{array}
\ee
%
%\begin{eqnarray*}
%S_\delta^i(z) &:=& \max\{s(z), \delta\} \, \Id\\
%S_\delta^a(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \max\left\{s(z), \sqrt \delta\right\} \, (\Id - \n_z \n_z^\trans)\\
%S_\delta^g(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \sqrt{r_0\max\{s(z), \delta\}} \, (\Id - \n_z \n_z^\trans).
%\end{eqnarray*}
We also define $S_\delta^\star(0) = r_0\Id$ for any $\star\in \{i,a,g\}$. Eventually we define the metrics $H_\delta^*$ by the equality 
\be
\label{eqHS2}
2  H_\delta^\star(z+u)^{-\frac 1 2} := S_\delta^*(z)
\ee
for all $z\in \left[-\frac 1 2, \frac 1 2\right]^d$ and all $u \in \Z^d$.
Observe that 
\be
\label{eqS2R0}
H_\delta^\star = \Id \stext{ for all } |z| \geq 2  r_0 =  1 / 2.
\ee
since $S_\delta^\star(z) = r_0 \Id$ on this set.

\begin{lemma}
For all $0<\delta\leq r_0$ and all $\star\in \{i,a,g\}$ one has $H_\delta^\star \in \bH_\per \cap \bH_\star$.
%\be
%\label{eqHInH}
%H_\delta^*\in \bH_* \cap \bH_\per.
%\ee
\end{lemma}
\proof
The function $s$ defined by \iref{defsz} Lipschitz, and thus also $\max\{s,\delta\}$ and $\max\{s, \sqrt \delta\}$ for any $\delta>0$.
It follows that $H_\delta^i = \Id/s_\delta(z)^2$ where 
$
s_\delta=  \min\{s,\delta\}/2
$
is Lipschitz, and therefore $H_\delta^i\in \bH_i$.

We now turn our attention to graded and quasi-acute metrics, and for that purpose we consider a fixed value of $\star\in\{a,g\}$ and $\delta>0$.
Since $2H^\star_\delta(z)^{-\frac 1 2} := S_\delta^\star(z)$ for all $z\in [-1/2,1/2]^d$, we easily obtain from 
Proposition \ref{propRadialMet} that $\dil_z (H^\star_\delta)_\times \leq 1$, and $\dil_z(H^a_\delta)_+\leq 1$, for all $z\in (-1/2,1/2)^d \sm\{0\}$.
Furthermore $H^\star_\delta(z) = \Id$ for all $z$ in an open neighborhood of the boundary $\partial ([-1/2,1/2]^d)$, hence $\dil_z(H_\delta^\star)_\times = \dil_z(H_\delta^a)_+ =0$ on this neighborhood.
Using the $\Z^d$ periodicity of $H_\delta^\star$ we obtain for all $z\in \R^d\sm \Z^d$
$$
\dil_z(H_\delta^\star)_\times \leq 1 \stext{ and } \dil_z(H_\delta^a)_+\leq 1.
$$
Consider a path $\gamma\in C^1([0,1], \R^d)$ joining two points $z=\gamma(0)$ and $z'= \gamma(1)$. There exists a sequence $(\ve_n)_{n \geq 0}$, $\ve_n\in \R^d$, $\ve_n \to 0$, such that for all $n\geq 0$ the translated path $\gamma+ \ve_n$ does not intersect $\Z^d$.
Reasonning as in Proposition \ref{propDilLoc} we obtain 
$$
d_\times(H_\delta^\star(z+\ve_n), \, H_\delta^\star(z'+\ve_n)) \leq l_{H_\delta^\star}(\gamma+\ve_n).
$$
Taking the limit of the previous inequality as $n \to \infty$ we obtain $d_\times(H_\delta^\star(z), \, H_\delta^\star(z')) \leq l_{H_\delta^\star}(\gamma)$ since $H_\delta^\star$ is continuous. Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_\times(H_\delta^\star(z), \, H_\delta^\star(z')) \leq d_{H_\delta^\star}(z,z')$. A similar argument yields $d_+(H_\delta^a(z), \, H_\delta^a(z')) \leq |z-z'|$ which concludes the proof of this lemma.
\sq

The next lemma establishes the ``constructive part'' of Theorem \ref{thOptGeom}.

\begin{lemma}
\label{lemmaHInH}
For all $0<\delta\leq r_0$ and all $\star\in \{i,a,g\}$ the metric $H_\delta^\star$ separates the sets $X$ and $Y_\delta$.\end{lemma}

\proof
%We now check the separation of $X$ and $Y_\delta$ by the metrics $H_\delta^*$, where $*\in \{i, a ,g\}$.
Let $\gamma\in C^1([0,1],\R^d)$ be such that $\gamma(0)\in X$ and $\gamma(1)\in Y_\delta$. Since the sets $X$, $Y_\delta$ and the metrics $H_\delta^*$ are $\Z^d$-periodic we may assume that $\gamma(0)\in \left[-\frac 1 2, \frac 1 2\right]^d$.
Recalling the definition \iref{defXYDelta} of $X$ and $Y_\delta$ we obtain
$$
|\gamma(0)|\leq r_0 \stext{ and } |\gamma(1)| \geq r_0+ \delta.
$$
We define 
$$
t_0 := \max \{t\in [0,1] \sep \gamma(t)\in X\} \stext{ and } t_1 := \min \{t\in [t_0, 1] \sep \gamma(t)\in Y_\delta\}.
$$
For any $t\in [t_0, t_1]$ we have 
$$
\gamma(t_0) = r_0  \leq |\gamma(t)| \leq r_0+\delta = \gamma(t_1),
$$
and therefore 
$$
\|\gamma'(t)\|_{H_\delta^\star(\gamma(t))} \geq \frac {2|\<\gamma'(t), \n_{\gamma(t)}\>|}\delta = \frac{2|\gamma|'(t)} \delta.
$$
Hence 
$$
l_{H_\delta^\star}(\gamma) \geq \int_0^1 \|\gamma'(t)\|_{H_\delta^\star(\gamma(t))} dt \geq \int_{t_0}^{t_1} \frac{2|\gamma|'(t)dt} \delta = 2\frac{|\gamma(t_1)|-|\gamma(t_0)|} \delta = 2.
$$
It follows that $d_{H_\delta^\star}(X,Y_\delta) \geq 2$ which concludes the proof.
\sq

\begin{lemma}
\label{lemmaMHDelta}
There exists a constant $C>0$ such that for all $0<\delta \leq r_0$
\begin{eqnarray}
\label{eqHDeltaI}
m(H_\delta^i) &\leq& C\delta^{-(d-1)},\\
\label{eqHDeltaA}
m(H_\delta^a) &\leq& C\delta^{-\frac{d-1} 2 } |\ln \delta|,\\
\label{eqHDeltaG}
m(H_\delta^g) &\leq& C\delta^{-\frac{d-1} 2}.
\end{eqnarray}
\end{lemma}

\proof
Recalling the definition \iref{eqHS2} of $H_\delta^\star$ in terms of $S_\delta^\star$ we obtain 
$$
m(H_\delta^\star) = c_0 + 2^d \int_{|z|\leq 2r_0}  \frac {dz}{\det S_\delta^\star(z)},
$$
where $c_0$ stands for the volume of the following set on which $H_\delta^\star = \Id$, see \iref{eqS2R0},
$$
\left\{z\in \left[-\frac 1 2,\frac 1 2\right]^d \sep |z| \geq 2 r_0\right\}.
$$
%and where we used the 
%%We first establish the three inequalities \iref{eqHDeltaI}, \iref{eqHDeltaA} and \iref{eqHDeltaG}, and we then turn to \iref{eqHInH}.
%Recalling the definition \iref{eqHS2} of $H_\delta^\star$ in terms of $S_\delta^\star$ we obtain 
%$$
%m(H_\delta^\star) = \int_{\left[-\frac 1 2,\frac 1 2\right]^d} \sqrt{\det H_\delta^\star(z)} dz = 2^d \int_{\left[-\frac 1 2,\frac 1 2\right]^d} \frac {dz}{\det S_\delta^\star(z)} 
%$$
Furthermore 
$$
\int_{|z|\leq 2r_0} \frac {dz}{\det S_\delta^\star(z)} = c_1 \int_{r=0}^{2r_0} \frac {r^{d-1}dr}{s_\delta^\star(r)},
$$
%where the constants $c_0,c_1>0$ are defined as follows.
%The constant $c_0$ and  stands for the contribution of the integral on the set 
%$$
%\left\{z\in \left[-\frac 1 2,\frac 1 2\right]^d \sep |z| \geq 2 r_0\right\},
%$$
%which is independent of $\delta$ according to \iref{eqS2R0}. The constant 
where $c_1$ stands for the $d-1$-dimensional volume of the sphere $\{z\in \R^d \sep |z|=1\}$, and where
$$
s_\delta^\star(r) := \det S_\delta^\star(z)
$$
for any $z$ such that $|z| = r$.
Therefore there exists a constant $c_2>0$, independent of $\delta$ and of $\star\in \{i,a,g\}$, and such that 
$$
m(H_\delta^\star) \leq c_2 \int_{r=0}^{2r_0} \frac {dr}{s_\delta^\star(r)}.
$$
Recalling the definition \iref{defSDeltaStar} of $S_\delta^i(z)$ we obtain $s_\delta^i(r) = \max\{\delta,|r_0-r|\}^d$ for all $0 \leq r\leq r_0$, hence 
\begin{eqnarray*}
 \int_{r=0}^{2r_0} \frac {dr}{s_\delta^i(r)} &=& \int_0^{r_0 - \delta} \frac {dr}{(r_0-r)^d} + \int_{r_0 - \delta}^{r_0+\delta} \frac {dr}{\delta^d} + \int_{r_0+\delta}^{2r_0} \frac {dr}{(r-r_0)^d} \\
&=& \frac{\delta^{-(d-1)}}{d-1} + 2 \delta^{-(d-1)} + \left(\frac{\delta^{-(d-1)}}{d-1} -\frac {r_0^{-(d-1)}} {d-1}\right)\\
&\leq & 4 \delta^{-(d-1)}
\end{eqnarray*}
which establishes \iref{eqHDeltaI}.
Similarly, we find 
%We have 
$s_\delta^g(r) = r_0^{\frac {d-1} 2} \max\{\delta,|r_0-r|\}^{\frac {d+1} 2}$, hence 
\begin{eqnarray*}
r_0^{\frac {d-1} 2} \int_{r=0}^{2r_0} \frac {dr}{s_\delta^g(r)} &=& \int_0^{r_0 - \delta} \frac {dr}{(r_0-r)^{\frac{d+1} 2}} + \int_{r_0 - \delta}^{r_0+\delta} \frac {dr}{\delta^{\frac{d+1} 2}} + \int_{r_0+\delta}^{2r_0} \frac {dr}{(r-r_0)^{\frac{d+1} 2}} \\
&=& \frac{2\delta^{-\frac{d-1} 2} }{d-1} + 2 \delta^{-\frac{d-1} 2} + \left( \frac{2\delta^{-\frac{d-1} 2} }{d-1} -\frac 2 {r_0^{\frac{d-1} 2}(d-1)}\right)\\
&\leq & 6 \delta^{-\frac{d-1} 2}
\end{eqnarray*}
which establishes \iref{eqHDeltaG}.
Eventually, we have $s_\delta^a(r) = \max\{\delta,|r-r_0|\} \max\left\{\sqrt\delta, |r-r_0|\right\}$, and therefore 
\be
\label{eqThreeInt}
\int_{r=0}^{2r_0} \frac {dr}{s_\delta^a(r)} = \int_{I_\delta} \frac {dr} {|r_0-r|^d} + \int_{J_\delta} \frac {dr}{|r_0-r| \delta ^{\frac {d-1} 2}} + \int_{r_0-\delta}^{r_0+\delta} \frac {dr}{\delta^{\frac{d+1} 2}},
\ee
where 
$$
I_\delta = \left[0,r_0-\sqrt \delta\right] \cup \left[r_0+ \sqrt \delta, 2 r_0\right] \stext{ and }J_\delta = \left[r_0-\sqrt \delta, r_0-\delta\right] \cup \left[r_0+ \delta, r_0+ \sqrt \delta\right].
$$
The contributions of the three integrals in \iref{eqThreeInt} are given in the next three lines %Computing the contributions of the three integrals we obtain 
\begin{eqnarray*}
\int_{r=0}^{2r_0} \frac {dr}{s_\delta^a(r)} &=& \frac 1 {d-1} \left(2\left(\sqrt{\delta}\right)^{-(d-1)}+r_0^{-(d-1)} \right)\\
& & +  2 \delta^{-\frac {d-1} 2} \left(\ln \left(\sqrt \delta\right) - \ln \delta\right) \\
& & + 2 \delta^{-\frac {d-1} 2}\\
&=& \delta^{-\frac {d-1} 2} |\ln \delta| + \frac {2d} {d-1} \delta^{-\frac {d-1} 2} + r_0^{-(d-1)}
\end{eqnarray*}
which establishes \iref{eqHDeltaA}.
\sq

\subsection{Lower bound}

We prove in this subsection the lower bound announced in Theorem \ref{thOptGeom}. 
\begin{lemma}
\label{lemmaMLower}
There exists a constant $c>0$ such that for all $0<\delta\leq r_0$, 
\begin{eqnarray}
\label{eqHILower}
m_i(X,Y_\delta) &\geq& c\delta^{-(d-1)},\\
\label{eqHALower}
m_a(X,Y_\delta) &\geq& c\delta^{-\frac{d-1} 2 } |\ln \delta|,\\
\label{eqHGLower}
m_g(X,Y_\delta) &\geq& c\delta^{-\frac{d-1} 2}.
\end{eqnarray}
\end{lemma}
\proof 
We consider a metric $H\in \bH_\star$, where $\star\in \{i,a,g\}$ which separates the sets $X$ and $Y_\delta$. In particular $H \in \bH_g$.
We denote by $\cS := \{v\in \R^d\sep |v| = 1\}$ the euclidean unit sphere of $\R^d$, and by $\omega$ the $d-1$-dimensional volume of $\cS$. We define for all $v\in \cS$
$$
n(v) := \|v\|_{H(r_0v)} \stext{ and } m(v) := \inf_{|w|=1} \|w\|_{H(r_0v)} =\|H(r_0v)^{-\frac 1 2}\|^{-1} .
$$
We recall, see \iref{eqEulidRiemann}, that for any $z,u\in \R^d$ we have 
\be
\label{eqER}
d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention if $\|u\|_{H(z)} \geq 1$. 

%Furthermore, see \iref{eqLocalNorm}, for all $v\in \R^d$
%$$
%\|v\|_{H(z+u)} \geq (1-\|u\|_{H(z)}) \|v\|.
%$$

We now consider $v\in \cS$ in such way that $r_0 v\in X$ and $(r_0+\delta)v\in Y_\delta$. Therefore 
$$
1 \leq d_H(r_0v, \, (r_0+ \delta) v) \leq -\ln\left(1-\delta \|v\|_{H(r_0 v)}\right)
$$
hence $\lambda \delta n(v) \geq 1$
%\be
%\label{eqHvv}
%\delta \|v\|_{H(r_0 v)} \geq 1-e^{-1} = \lambda^{-1},
%\ee
where we $\lambda := (1-e^{-1})^{-1}$ until the end of this proof.

Let $v,w\in \cS$, and let $\sigma\in \{-1,1\}$ be such that $\sigma \<v,w\>\geq 0$.  Remarking that $2r_0+ \delta \leq 3/4 \leq 1$ we obtain 
$$
\left|r_0 v+\sigma \sqrt {\delta} w\right|^2 = r_0^2 +\delta + 2 \sigma r_0 \sqrt \delta \<v,w\> \geq r_0^2 +\delta \geq r_0^2 + (2r_0 +\delta) \delta = (r_0+\delta)^2.
$$
Hence $r_0 v \in X$ and $r_0 v+\sigma \sqrt {\delta} w\in Y_\delta$. Therefore 
$$
1 \leq d_H(r_0 v, \, r_0 v+ \sigma \sqrt \delta w) \leq -\ln\left(1-\sqrt \delta \|w\|_{H(r_0 v)}\right),
$$
which implies $\lambda \sqrt \delta m(v) \geq 1$.

We we now distinguish the three possibilities $\star = i$, $a$ or $g$.
\begin{itemize}
\item If $\star = i$, then $H(z) = \Id/s(z)^2$ where $s$ is a Lipschitz function. Furthermore $s(r_0 v) = n(v)^{-1} \geq \lambda\delta$.
It follows that 
\begin{eqnarray*}
m(H) &\geq& \int_\cS \int_0^{2r_0} \frac {r^{d-1} dr dv}{s(rv)^d} \\
&\geq& \int_\cS\int_{r_0}^{r_0+\delta} \frac{r_0^{d-1} dr dv}{(n(v)+\delta)^d}\\
&\geq& \frac{r_0^{d-1}\delta\omega }{(\lambda\delta+ \delta)^d}\\
&=& \frac{r_0^{d-1} \omega}{(\lambda+1)^d} \delta^{-(d-1)}
\end{eqnarray*}
Taking the infimum among all metrics $H \in \bH_i$ which separate $X$ and $Y_\delta$ we obtain as announced
$$
m_i(X,Y_\delta) \geq c \delta^{-(d-1)} \stext{ where } c= \frac{r_0^{d-1} \omega}{(\lambda+1)^d}.
$$
\item If $\star =a$, then $z\mapsto \|H(z)\|^{-\frac 1 2}$ as well as $z\mapsto \|H(z)^{-\frac 1 2}\|$ are Lipschitz functions. Hence for any $v\in \cS$ and $\mu\in \R$ we have 
$$
\|H((r_0+\mu) v)\|^{-\frac 1 2} \leq n(v)^{-1}+ |\mu| \leq \lambda \delta + |\mu|
$$
and 
$$
\|H((r_0+\mu) v)^{-\frac 1 2}\| \leq m(v)^{-1} + |\mu| \leq \lambda \sqrt \delta + |\mu|,
$$
in particular recalling that $\det M \geq \|M\| \|M^{-1}\|^{-(d-1)}$ for any $M\in S_d^+$ we obtain 
$$
(\lambda\delta+|\mu|)(\lambda\sqrt\delta+|\mu|)^{d-1}\sqrt{\det H((r_0+\mu) v)} \geq 1,
$$
eventually 
\begin{eqnarray*}
m(H) &\geq& \omega \int_{-r_0}^{r_0} \frac {(r_0+\mu)^{d-1}d\mu}{(\lambda\delta+|\mu|)(\lambda\sqrt\delta+|\mu|)^{d-1}}\\
&\geq& \omega \int_0^{\sqrt \delta} \frac {r_0^{d-1}d\mu}{(\lambda \delta +\mu)(\lambda\sqrt{\delta} + \sqrt \delta)^{d-1}}\\ 
&\geq& \frac{\omega r_0^{d-1} }{((\lambda+1)\sqrt \delta)^{d-1}} (\ln \sqrt \delta -\ln (\lambda\delta)).
\end{eqnarray*}
Hence 
$$
m_a(X,Y_\delta) \geq c\delta^{-\frac{d-1} 2} (-\ln\delta-2\ln \lambda) \stext{ where } c=\frac{\omega}{2(\lambda+1)^{d-1}}
$$
which concludes the proof of \iref{eqHALower}.
\item We now consider the case $\star = g$. We first remark that for any $M,M'\in S_d^+$
$$
|\ln \det M -\ln \det M'| \leq 2d\,d_\times (M,M').
$$
Recalling that 
$$
n(v) (\lambda \sqrt d)^{d-1} \sqrt{\det H(r_0 v)}\geq n(v)m(v)^{d-1}\sqrt{\det H(r_0 v)} \geq 1
$$
we obtain 
$$
\sqrt{\det H((r_0+\mu) v)} \geq (1-|\mu| n(v))^d\sqrt{\det H(r_0v)} \geq \frac{(1-|\mu| n(v))^d } {n(v)(\lambda\sqrt d)^{d-1} }
$$
hence 
\begin{eqnarray*}
m(H) &\geq &\int_\cS \int_{-r_0}^{r_0} \frac{(r_0+\mu)^{d-1} (1-|\mu| n(v))^d d\mu dv}{n(v)(\lambda\sqrt d)^{d-1}}\\
&\geq &\int_\cS \int_0^{\frac 1{2n(v)}} \frac{r_0^{d-1} (1/2)^d d\mu dv}{n(v)(\lambda\sqrt d)^{d-1}}\\
&=& \frac{\omega r_0^{d-1}}{2^d (\lambda\sqrt d)^{d-1}}.
\end{eqnarray*}
We thus obtain the announced result \iref{eqHGLower}
$$
m_g(X,Y_\delta) \geq c \delta^{-\frac {d-1} 2} \stext{ where } c=\frac{\omega r_0^{d-1}}{2^d \lambda^{d-1}},
$$
which concludes the proof of this lemma. \sq
\end{itemize}

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Meshing/ConstrainedMesh.pdf}
\caption{Weak separation of two sets by a triangulation. \label{figWeakSeparation}}
\end{figure}

\begin{remark}[Constrained triangulations] 
A variation of the problem considered in this section is often considered in the litterature. 
We say that a mesh $\cT\in \bT$ weakly separates two regions $X, Y \subset \R^d$ if 
$$
\interior(V_\cT(X)) \cap \interior(V_\cT(Y)) = \emptyset,
%\mathring {V_\cT(X)} \cap \mathring{V_\cT(Y) } = \emptyset
$$
where $\interior(E)$ refers to the collection of interior points of $E$. 

%The optimization problems related to the weak separation of two sets generally cannot rephrased in terms of metrics (??? probably false???).
A common approach for weakly separating two closed and disjoint sets $X,Y\subset \R^d$, is to use ``constrained meshes'', proceeding as follows.
The first step is to build a polygonal hypersurface $\Gamma$ such that for any path $\gamma \in C^0([0,1], \R^d)$ satisfying $\gamma(0) \in X$ and $\gamma(1)\in Y$, there exists $s\in [0,1]$ such that $\gamma(s) \in \Gamma$.
The second step is to build a triangulation $\cT$ of the domain $\Omega$ which is constrained to contain the polygonal surface $\Gamma$ in its skeleton.

The main advantage of weak separation is that it can be achieved efficiently without anisotropic simplices, see Figure \ref{figWeakSeparation}. Heuristically the same number of simplices is required to separate the sets $X$ and $Y_\delta$ ``weakly'' with an isotropic triangulation, of ``strongly'' with a graded triangulation.

This method is out of the scope of this thesis, and is generally based on combinatorial techniques rather than Riemmannian metrics. We refer the interested reader to \cite{Shew3}.
\end{remark}

\section{Approximation in the $L^p$ norm}

We study in this section the theory of anisotropic finite element approximation in the $L^p$ norm, from the point of view of metrics. We first obtain in subsection \S\ref{subsecErrMeshMetLP} an estimation of the finite element approximation error of a function on a mesh in terms of the error with respect to a metric. We then establish in subsection \S\ref{subsecExistsMetLP} the existence of a metric which satisfies an estimate, believed to be asymptotically sharp, when the function is sufficiently smooth. We eventually discuss in subsection \S \ref{subsecApproxSpaceLP} a, probably naive, definition of anisotropic smoothness spaces which leads to the recovery of some classical results of (isotropic) approximation theory. 

\subsection{Comparison of the error associated to a mesh and to a metric}
\label{subsecErrMeshMetLP}

This subsection is devoted to the proof of Proposition \ref{propErrMeshMet}, announced in the introduction under the name Proposition \ref{propErrMeshMetIntro}, which compares the finite element approximation error of a function $f$ on a mesh $\cT$ and the error $e_H(f)_p$ with respect to a metric $H$.

Our first lemma establishes that the twisted mollification $f_H$ of a function $f\in L^1_\loc$ with a metric $H\in \bH_\per$, which is defined by
$$
f_H(z) := \sqrt{\det H(z)}\int_{\sR^d} f(z+u) \, \vp(\|u\|_{H(z)}) du,
$$
is locally bounded and reproduces polynomials. Note that the change of variables $v:= H(z)^\frac 1 2 u$ yields 
\be
\label{eqTwistChg}
f_H(z) := \int_{\sR^d} f(z+H(z)^{-\frac 1 2}v) \, \vp(|v|) du.
\ee
We recall that 
$$
B_H(z,r) := \{z+u \sep \|u\|_{H(z)} \leq 1\},
$$
and that the radius is one by default $B_H(z) := B_H(z,1)$, and $B(z,r) := B_{\Id}(z,r)$ is the standard euclidean ball.
Throughout this section we denote by $\omega$ the volume of the $d$-dimensional euclidean unit ball 
$
\omega := |B(0,1)|,
$
and we observe that 
\be
\label{eqVolBall}
|B_H(z,r)| = \frac {\omega \, r^d}{\sqrt {\det H(z)}}.
\ee
\begin{lemma}
Let $H\in \bH$.
\begin{itemize}
\item (Boundedness) For any $f\in L^1_\loc$ we have $f_H\in C^0(\R^d)$, and for any $z\in \R^d$ one has 
\be
\label{eqFHBounded}
|f_H(z)|\leq \sqrt{\det H(z)} \, \|\vp\|_{L^\infty} \|f\|_{L^1(B_H(z))} = \omega \|\vp\|_{L^\infty} \frac{\|f\|_{L^1(B_H(z))}}{|B_H(z)|}
\ee
\item (Reproduction of polynomials) For any $\mu\in \P_{m-1}$, one has $\mu_H = \mu$.
\end{itemize}
\end{lemma}

\proof
\begin{itemize}
\item (Boundedness) The continuity of the of $f$ is a consequence of general results on parameter dependent integrals. Inequality \iref{eqFHBounded} follows from the fact that $\vp$ is supported on $[0,1)$.
\item (Reproduction of polynomials) We define $\nu\in \P_{m-1}$ as follows
$$
\nu(u) := \mu(z +H(z)^{-\frac 1 2} u) -\mu(z),
$$
and we observe that $\nu(0) = 0$. Recalling the moments property \iref{eqPhiMoments} we obtain using \iref{eqTwistChg} 
$$
\mu_H(z) = \mu(z) + \int_{\R^d} \nu(|u|) \vp(u) du = \mu(z) + \nu(0) = \mu(z),
$$
which concludes the proof of this proposition.
\sq
\end{itemize}

Our next lemma studies the variations, in terms of volume and inclusion, of the balls $B_H(z,r)$ as $z\in \R^d$ and $r>0$ vary and when $H\in \bH_g$ is a graded metric. This is a first step for the comparison in Proposition \ref{propErrMeshMet} of the finite element approximation error on a mesh or with respect to a metric.

\begin{lemma}
\label{lemmaEllIncl}
Let $H\in \bH_g$, let $H' := 4^2 H$ and let $z\in \R^d$.
\begin{enumerate}
\item  For any $z'\in B_{H'}(z,2)$ one has $B_{H'}(z')\subset B_H(z)$ and $|B_{H'}(z')|\geq 8^{-d} |B_H(z)|$.
\item For any $z'\in B_{H'}(z, 2/3)$ one has $B_{H'}(z',2)\supset B_{H'}(z)$. % and ...%$B_{H'}(z')\geq 4^{-2d} B_H(z)$.
\end{enumerate}
\end{lemma}

\proof
We recall some regularity properties of the metrics in $\bH_g$, see \iref{eqLocalNorm}. For any $H \in \bH_g$, and for any $z,u,v\in \R^d$ satisfying $\|u\|_{H(z)}<1$ one has 
\be
\label{eqLocalNorm2}
\|v\|_{H(z+u)} (1-\|u\|_{H(z)} ) \leq \|v\|_{H(z)}\leq \|v\|_{H(z+u)} (1-\|u\|_{H(z)})^{-1},
\ee
and 
$$
\sqrt{\det H(z+u)} (1-\|u\|_{H(z)} )^d \leq \sqrt{\det H(z)} \leq \sqrt{\det H(z+u)} (1-\|u\|_{H(z)} )^{-d}.
$$
Observing that $|B_H(z)| = 4^d |B_{H'}(z)| = \omega \sqrt {\det H(z)}$, where $\omega$ denotes the volume of the $d$-dimensional unit ball $B(0,1)$, we easily obtain the announce volume estimate.  We thus turn to the properties of inclusion.
\begin{enumerate}
\item 
We have $2 \geq \|z-z'\|_{H'(z)} = 4  \|z-z'\|_{H(z)}$. 
Hence  we obtain for any $q\in \R^d$, using \iref{eqLocalNorm2} in the second line,
\begin{eqnarray*}
\frac 1 4 \|q-z'\|_{H'(z')} &=&  \|q-z'\|_{H(z')}\\
&\geq & (1-\|z'-z\|_{H(z)}) \|q-z'\|_{H(z)}\\
& \geq & (1-\|z'-z\|_{H(z)}) (\|q-z\|_{H(z)}-\|z'-z\|_{H(z)})\\
& \geq & (1-1/2) (\|q-z\|_{H(z)}-1/2)
\end{eqnarray*}
If $\|q-z\|_{H(z)}> 1$ then the previous equation implies $\|q-z'\|_{H'(z')}> 1$.
We have thus established that $\R^d \sm B_H(z) \supset \R^d \sm B_{H'}(z')$ which is equivalent to the announced inclusion $B_{H'}(z')\subset B_H(z)$.

\item We obtain for any $q\in \R^d$ %Recalling that $4 \|z-z'\|_{H(z)} = \|z-z'\|_{H(z')} \leq 2/3$ we obtain for any $q\in \R^d$
\begin{eqnarray*}
\|q-z'\|_{H'(z')} &\geq & (1-\|z'-z\|_{H(z)}) \|q-z'\|_{H'(z)}\\
& \geq & (1-\|z-z'\|_{H'(z)}/4) (\|q-z\|_{H'(z)}-\|z'-z\|_{H'(z)})\\
& \geq & (1-1/6) (\|q-z\|_{H'(z)}-2/3). %= 10/9 >1. %(2/3)/4
\end{eqnarray*}
If $\|q-z\|_{H'(z)} \geq 2$ then $\|q-z'\|_{H'(z')} \geq 10/9 >1$. Hence $B_{H'}(z',2)\supset B_{H'}(z)$ as announced which concludes the proof of this lemma.\sq
\end{enumerate}

The next proposition, announced under the reference Proposition \ref{propErrMeshMetIntro} in the introduction, compares the approximation error of a function associated to a mesh or to a metric.

\begin{prop}
\label{propErrMeshMet}
There exists $C=C(m,d)$ such that the following holds. Let $H\in \bH_g$, and let $H' := 4^2 H$. Let also $f\in L^p_\loc$.
\begin{itemize}
\item (Local error estimate) 
Let $\cT\in \bT$, let $z\in \R^d$ and let 
$$
\cT_z := \{T\in \cT \sep T \subset B_{H'}(z,2)\}
$$
and let $\Omega_z$ be the union of all triangles in $\cT_z$.
Then 
\be
\label{eqLocalMeshMet}
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p(\Omega_z)} \leq C \, e_H(f\sep z)_p.
\ee
%Let $T$ be a simplex let $z\in T$, and assume that $\cH_T \geq H'(z)$.
%
%For any $f\in L^p_\loc$ one has 
%$$
%\|f-\interp_T^{m-1} f_{H'}\|_{L^p} \leq C e_H(f\sep z)_p,
%$$
%where $C=C(m,d)$. ($C$ is independent of $H$, $T$ and $f$.)
\item (Global error estimate) Let $\cT\in \bT$ and assume that for all $T\in \cT$ and all $z\in \cT$ one has 
\be
\label{eqHTHp}
\cH_T \geq H'(z).
\ee
The quasi-interpolation error of $f$ is controlled by the error associated to the metric $H$
$$
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p([0,1]^d)} \leq C \, e_H(f)_p. 
$$
\end{itemize}
\end{prop}

\proof
\begin{itemize}
\item (Local error estimate)
We denote by $C_{\interp}$ the norm of the interpolation operator $\interp_\TEq^{m-1} : C^0(\TEq) \to C^0(\TEq)$, and we observe using a change of variables that for any triangle $T$ and any $g\in C^0(T)$ one has 
$$
\|\interp_T^{m-1} g\|_{L^\infty(T)}\leq C_{\interp} \|g\|_{L^\infty(T)}.
$$


Let $\mu\in \P_{m-1}$ be a polynomial satisfying $\|f-\mu\|_{L^p(B_H(z))} = e_H(f\sep z)_p$.
Let $g := f-\mu$ and let $T\in \cT_z$. 
We have 
\begin{eqnarray*}
\|\interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq & |T|^\frac 1 p \|\interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
&\leq & C_{\interp} |T|^\frac 1 p \|g_{H'}\|_{L^\infty(T)}\\
&\leq & C_{\interp} |T|^\frac 1 p \|g_{H'}\|_{L^\infty(B_{H'}(z,2))}\\
&\leq & C_{\interp} \|\vp\|_{L^\infty} |T|^\frac 1 p \max_{z'\in B_{H'}(z,2)}  \frac{\|g\|_{L^1(B_{H'}(z'))}}{|B_{H'}(z')|}\\
&\leq & \omega 8^d C_{\interp}  \|\vp\|_{L^\infty}  |T|^\frac 1 p \frac{\|g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|},
\end{eqnarray*}
where we used \iref{eqFHBounded} in the fourth line and Lemma \ref{lemmaEllIncl}, point 1., in the last line.

Defining $C_* := \omega 8^d C_{\interp}  \|\vp\|_{L^\infty}$ we thus obtain
\begin{eqnarray*}
\|\interp_\cT^{m-1} g_{H'}\|_{L^p(\Omega_z)} &=& \left(\sum_{T\in \cT_z} \|\interp_T^{m-1} g_{H'}\|_{L^p(T)}^p \right)^{\frac 1 p} \\
&\leq & C_* \frac{\|g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|} \left(\sum_{T\in \cT_z} |T|\right)^\frac 1 p\\
& \leq & C_* \|g\|_{L^1(B_{H}(z))}|B_{H}(z)|^{\frac 1 p-1}\\
& \leq & C_* \|g\|_{L^p(B_{H}(z))}
\end{eqnarray*}
Since the twisted convolution reproduces polynomials in $\P_{m-1}$ , as well as the interpolation operator $\interp_\cT^{m-1}$, we have
$$
g-\interp_\cT^{m-1} g_H = (f-\mu)-\interp_\cT^{m-1} (f-\mu)_H = f-\interp_\cT^{m-1} f_H.
$$ 
Therefore  
\begin{eqnarray*}
\|f-\interp_\cT^{m-1} f_H\|_{L^p(\Omega_z)} &=& \|g-\interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)} \\
&\leq &\|g\|_{L^p(\Omega_z)}+ \|\interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)}\\
& \leq & (1+C_*) \, \|g\|_{L^p(B_{H}(z))}\\
&=& (1+C_*) \, e_H(f\sep z)_p
\end{eqnarray*}
which concludes the proof of the local error estimate.

\item (Global error estimate)
For each triangle $T\in \cT$ we define 
$$
\Omega_T := \{z\in \R^d \sep T \subset B_{H'}(z,2)\} \stext{ and } n(T) := \int_{\Omega_T} \sqrt{\det H(z)} dz.
$$
Denoting by $z_T$ the barycenter of $T$, we have $T\subset B_{H'}(z_T)$ according to \iref{eqHTHp}.
Point 2. of \ref{lemmaEllIncl} thus implies that $B_{H'}(z_T,2/3) \subset \Omega_T$.
Eventually $n(T)$ is bounded below a constant independent of $H$ and $\cT$
$$
n(T) \geq |B_{H'}(z_T,2/3)| \min_{z\in B_{H'}(z_T,2/3)}  \sqrt{\det H(z)} \geq \omega 6^{-d} (1-1/2)^d (1-1/2-1/6)^d
$$
%(could be improved...??)
We denote by $\cT_*$ a system of representatives of $\cT$ for the equivalence relation 
$$
T \sim T' \stext{ if } T =T'+u \text{ for some } u \in \Z^d.
$$
Using the local estimate \iref{eqLocalMeshMet} we therefore obtain 
\begin{eqnarray*}
C^p e_H(f)_p^p &=& C^p\int_{z\in [0,1]^d} \sqrt{\det H(z)} \, e_H(f\sep z)_p^p dz\\
&\geq&  \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \|f-\interp_\cT^{m-1} f_H\|_{L^p(\Omega_z)}^p dz \\
&=&  \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \sum_{T\in \cT_z} \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p dz \\
&=& \sum_{T\in \cT_*} n_T \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p \\
& \geq &  \|f-\interp_\cT^{m-1} f_H\|_{L^p([0,1]^d)}^p \min_{T \in \cT} n_T,
\end{eqnarray*}
which concludes the proof of this proposition. \sq
\end{itemize}

\subsection{Existence of an optimal metric for smooth functions}

\label{subsecExistsMetLP}

This section is devoted to the proof of the following theorem, which is announced in the introduction under the reference Theorem \ref{thExistsMetLPIntro}.
\begin{theorem}
\label{thSmooth}
There exists a constant $C=C(m,d)$ such that the following holds.\\
For each $f\in C^m_\per$ such that $z\mapsto K(d^m f(z))$ is not identically $0$, there exists a metric $H \in \bH_\per\cap \bH_g$, which is also $C^\infty$, and such that for all $\lambda \geq 1$
\be
\label{eqHSmooth}
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|K(d^m f)\right\|_\tau,
\ee
where $\frac 1 \tau := \frac m d+ \frac 1 p$.
\end{theorem}

In order to prove this theorem we need to introduce some notation.
The greek letter $\alpha$ always refers %in this section 
to a $d$-plet of non-negative integers
$$
\alpha = (\alpha_1, \cdots, \alpha_d) \in \Z_+^d.
$$
For each $\alpha$ we define the following quantities
$$
|\alpha|:= \sum_{1\leq i\leq d} \alpha_i \stext{ and } \alpha! := \prod_{1\leq i\leq d} \alpha_i!. %, \quad \max(\alpha) := \max_{1\leq i\leq d} \alpha_i.
$$
We also define the monomial
$$
Z^\alpha := \prod_{1\leq i\leq d} Z_i^{\alpha_i},
$$
where the variable is $Z=(Z_1,...,Z_d)\in \R^d$.
For each $z\in \R^d$ we define the homogeneous polynomial $\pi_z\in \H_m$ as follows
$$
\pi_z(Z) := \sum_{|\alpha| = m} \frac{\partial^\alpha f(z)}{(\partial z)^\alpha} \frac{Z^\alpha}{\alpha!} .
$$
We recall that the quantity $K$ involved in this theorem is defined for all $\pi\in \H_m$ as follows
\be
\label{defKAT}
K(\pi) := \inf\{(\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2}\|\leq 1\},
\ee
where
$$
\|\pi\| := \sup_{|z|\leq 1} |\pi(z)|.
$$

The heuristic guideline of this proof is the following. Assume that for all $z\in \R^d$ there exists a unique minimizer $M_z\in S_d^+$ to the minimization procedure \iref{defKAT} defining $K(\pi_z)$, and that $M_z$ depends smoothly on $z$.
Define 
$$
H(z) := \Lambda \, (\det M_z)^{\frac {-1}{mp+d}} M_z,
$$
where $\Lambda>0$ is a sufficiently large constant. A simple analysis, using Taylor developments, shows that $H$ satisfies the conditions of Theorem \ref{thSmooth}. %\iref{eqHSmooth}.

The main difficulty of this proof is that the optimization problem \iref{defKAT} is not well posed. For some choices of $\pi$ there exists no minimizer, for others there exists an infinity of minimizers. 
These undesirable properties come from the fact that \iref{defKAT} is not a convex minimization problem. The key ingredient of our approach is to define a close variant of this optimization problem which is ``geometrically convex'', a  notion close to convexity which is sufficient for our purpose.

\subsubsection{Geometric convexity, and geometric average of two matrices}
\label{subsubsecGeomCvx}
%We also introduce the notion of geometric average of two matrices.
Let $M, M'\in S_d^+$, and let $S:=M^{-\frac 1 2}$. We define the geometric average $\Avg(M,M')\in S_d^+$ of $M$ and $M'$ as follows
\be
\label{defAvg}
S \Avg(M,M') S := \sqrt{S M' S}
\ee
For instance $\Avg(M,M^{-1}) = \Id$, and for any $k,k'>0$
$$
\Avg(k M , k'M') = \sqrt{k k'} \Avg(M,M').
$$

The following proposition gives a handy characterization \iref{eqAvgAD} of $\Avg(M,M')$. This proposition also shows that $\Avg(M,M')$ is a natural midpoint between $M$ and $M'$ for the distance $d_\times$, and establishes two basic properties of the geometric average of matrices.
% number of useful properties.

\begin{prop}
For any $M,M'\in S_d^+$ the following holds.
\begin{enumerate}
\item A matrix $\ti M$ satisfies $\tilde M = \Avg(M,M')$ if and only if there exists $A \in \GL_d$ and a diagonal matrix $D$ such that 
\be
\label{eqAvgAD}
\tilde M = A^\trans A, \quad M = A^\trans e^{2D} A, \quad M' = A^\trans e^{-2D} A.
\ee
\item The geometric average $\Avg(M,M')$ is a midpoint between $M$ and $M'$ for the distance $d_\times$ on $S_d^+$.
$$
d_\times (M, \Avg(M,M')) = d_\times (\Avg(M,M'), M') = \frac 1 2 d_\times (M,M').
$$
\item The geometric average is commutative and compatible with the inversion of matrices.
\begin{eqnarray}
\label{eqAvgCommut}
\Avg(M,M') &=& \Avg(M',M)\\
\label{eqAvgInv}
\Avg(M,M')^{-1} &=& \Avg(M^{-1}, M'^{-1})
\end{eqnarray}
\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item We first assume that $M,M'$ and $\tilde M$ have the form \iref{eqAvgAD}. We easily obtain 
$$
\tilde M M^{-1} \tilde M = M'
$$
Defining $S := M^{-\frac 1 2}$ we thus have 
$$
(S\tilde M S)^2 = S M' S.
$$
Taking the square root of the previous equation we obtain \iref{defAvg} which shows that $\tilde M = \Avg(M,M')$.

Conversely, for any $M,M'\in S_d^+$ %(??) 
the simultaneous reduction theorem shows that there exists $A\in \GL_d$ and $D$ diagonal satisfying $M = A^\trans e^{2D} A$ and $M' = A^\trans e^{-2D} A$, and the result follows.

\item Let $A\in \GL_d$ and let $D,D'$ be diagonal matrices, of diagonal coefficients $D_1, \cdots ,D_k$ and  $D'_1, \cdots , D'_d$ respectively. We define
$$
\delta := \max_{1\leq i \leq d} |D_i - D'_i|.
$$ 
We claim that the matrices $N := A^\trans e^{2D} A$ and $N':=A^\trans e^{2D'} A$ satisfy $d_\times(N,N') = \delta$.
Indeed
\begin{eqnarray*}
d_\times (N,\, N') &:= &\sup_{u\neq 0} \left|\ln \|u\|_N -\ln \|u\|_{N'}\right| \\
&=& \sup_{u\neq 0} \left|\ln |e^D Au| - \ln |e^{D'} Au|\right|\\
&=& \sup_{v\neq 0}  \left|\ln |e^D v| - \ln |e^{D'} v|\right|.
\end{eqnarray*}
For any $v=(v_1, \cdots ,v_d)\in \R^d$ we have 
$$
|e^D v|^2 = \sum_{1\leq i \leq d} e^{2D_i} v_i^2 \leq e^{2\delta}  \sum_{1\leq i \leq d} e^{2D'_i} v_i^2 = \left(e^\delta |e^{D'}v|\right)^2,
$$
and similarly $|e^{D'} v|\leq e^\delta |e^D v|$. Therefore $\left|\ln |e^D v| - \ln |e^{D'} v|\right|$ and taking the supremum among all $v\neq 0$ we obtain $d_\times(N,N') \leq \delta$. Furthermore denote by $i_0$, $1\leq i_0\leq d$, the position $|D_{i_0} - D'_{i_0}| = \delta$. Choosing $v = (0,\cdots ,1, \cdots ,0)$, with the nonzero coordinate at the position $i_0$, we obtain $\delta = \left|\ln |e^D v| - \ln |e^{D'} v|\right| \leq d_\times(N,N')$. We thus conclude that 
$$
d_\times (N,N') =  d_\times (A^\trans e^{2D} A, \, A^\trans e^{2D'} A) = \|D-D'\|.
$$

Recalling that $M,M'$ and $\ti M := \Avg(M,M')$ have the form \iref{eqAvgAD} we thus obtain 
$$
d_\times (M, \Avg(M,M')) = d_\times (\Avg(M,M'), M')= \|D\| \stext{ and } d_\times (M,M') = 2 \|D\|.
$$
which concludes the proof of this point.

\item 
Using the first point we obtain that $M,M'$ and $\tilde M := \Avg(M,M')$ have the form
$$
\tilde M = A^\trans A, \quad M = A^\trans e^{2D} A, \quad M' = A^\trans e^{-2D} A
$$
It follows that 
$$
\tilde M = A^\trans A, \quad M' = A^\trans e^{-2D} A, \quad M = A^\trans e^{2D} A,
$$
and 
$$
\tilde M^{-1} = (A^{-1})^\trans A^{-1}, \quad M^{-1} = (A^{-1})^\trans e^{-2D} A^{-1}, \quad M'^{-1} = (A^{-1})^\trans e^{2D} A^{-1}.
$$
Using again the first point we obtain the announced properties \iref{eqAvgCommut} and \iref{eqAvgInv}.\sq
\end{enumerate}

We recall that that a function $\psi\in C^0(S_d, \R)$ is convex if and only if for all $M,M'\in S_d$ one has 
\be
\label{defConv}
\psi\left(\frac{M+M'} 2\right) \leq \frac{\psi(M)+ \psi(M')} 2.
\ee
The next proposition introduces the family of geometrically convex functions, which are defined by a property similar to \iref{defConv} but in which the arithmetic averages are replaced with geometric averages.
\begin{definition}
We say that a function $\vp \in C^0(S_d^+ , \R_+^*)$ is GCH, Geometrically Convex and Homogenous, if it satisfies the following properties.
\begin{enumerate}[i)]
\item (Sub multiplicativity) For any $M,M'\in S_d^+$ one has
\be
\label{eqSubMult}
\vp(\Avg(M,M')) \leq \sqrt{\vp(M) \vp(M')}.
\ee
\item (Homogenous) There exists $\alpha \in \R$ , called the degree of $\vp$,
such that for all $M\in S_d^+$ and all $\lambda\in \R$ one has 
$$
\vp(\lambda M) = \lambda^\alpha \vp(M).
$$
\end{enumerate}
We say that the function $\vp$ is SGCH, Strictly Geometrically Convex and Homogeneous, if $\vp$ is GCH and if the equality in \iref{eqSubMult} only holds if $M$ and $M'$ are proportional.
\end{definition}

For instance the function $\det$ is GCH of degree $d$, since 
$$
\det \Avg(M,M') = \sqrt{\det M \det M'} \stext{ and } \det (\lambda M) = \lambda^d M.
$$
We insist on point that GCH functions are by assumption strictly positive on $S_d^+$, and continuous.
The next lemma enumerates some simple properties of geometrically convex functions.
\begin{lemma}
\label{lemmaAlgGCH}
\begin{enumerate}
\item The product of two GCH functions is GCH, and the product of a GCH function with a SGCH function is SGCH. Furthermore the degrees add.
\item The elevation to a positive power of a GCH (resp. SGCH) function is also GCH (resp. SGCH). Furthermore the degree is multiplied by $\alpha$.
\item If a function $\vp$ is GCH (resp. SGCH) then $M \mapsto \vp(M^{-1})$ is also GCH (resp. SGCH), and has the opposite degree.
\end{enumerate}
\end{lemma}
\proof
The first two points are easy, and the last point is a direct consequence of the compatibility \iref{eqAvgInv} of the geometric average with the inversion : if $\vp$ is GCH and $M,M'\in S_d^+$ then 
$$
\vp(\Avg(M,M')^{-1}) = \vp(\Avg(M^{-1}, M'^{-1})) \leq \sqrt{\vp(M^{-1}) \vp (M'^{-1})},
$$
which concludes the proof.
\sq

Aside from the determinant, a number of functions on $S_d^+$ are geometrically convex. The next proposition, which is based on an argument of complex analysis, enumerates some of them.
For all $\pi\in \H_m$ we define 
$$
\|\pi\|_\sC := \sup\{ |\pi(z)| \sep z\in \C^d, \, |z|\leq 1\}.
$$

\begin{prop}
\label{propExGCH}
\begin{enumerate}
\item The trace map $M \mapsto \Tr M$ is SGCH.
\item For any fixed polynomial $\pi\in \H_m\sm\{0\}$ the map $M \mapsto \|\pi \circ M^{\frac 1 2}\|_\sC$ is GCH, of degree $m/2$.
\item The norm map $M \mapsto \|M\|$ is GCH. 
\end{enumerate}

%For any $M,M'\in S_d^+$ the following holds.
%\begin{enumerate}
%\item 
%\be
%\label{eqTr}
%\Tr (\Avg(M,M'))\leq \sqrt{\Tr M \Tr M'} \stext{ and } \Tr (\Avg(M,M')^{-1})\leq \sqrt{\Tr (M^{-1}) \Tr (M'^{-1})}
%\ee
% with equality if and only if the matrices $M$ and $M'$ are proportionnal. %and inverse.
%\item For any polynomial $\mu \in \H_m$ one has %$\C$ %define S, S', \tilde S
%$$
%\|\mu \circ \Avg(M,M')^{-\frac 1 2}\|_\sC \leq \sqrt{\|\pi\circ M^{-\frac 1 2}\|_\sC \|\pi\circ M'^{-\frac 1 2}\|_\sC }
%$$
%\item We have 
%$$
%\|\Avg(M, M')\| \leq \sqrt{\|M\| \|M'\|}
%$$
%\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item 
Let $M,M'\in S_d^+$ and let $\ti M := \Avg(M)$. Let $A\in \GL_d$ and let the diagonal matrix $D$ be such that  $M = A^\trans e^{-2D}$, $M' = A^\trans e^{2D} A$ and $\ti M = A^\trans A$.
We denote by $A_{i,j}$ the coefficients of $A$, and we define for all $1\leq i \leq d$
$$
\cA_i^2 := \sum_{1\leq j \leq d} A_{ji}^2.
$$
Observe that $\cA_i>0$, since otherwise a full line of $A$ would be zero and $A$ would be degenerate.
Denoting by $D_i , \cdots , D_d$ the diagonal coefficients of $D$ we obtain  
$$
\Tr(M) = \sum_{1\leq i \leq d} \cA_i^2 e^{-2D_i}, \quad \Tr(M') = \sum_{1\leq i \leq d} \cA_i^2 e^{2D_i}, \quad \Tr(\ti M) = \sum_{1\leq i \leq d} \cA_i^2.
$$
It thus follows from Cauchy Schwartz inequality that $\Tr(\ti M)^2 \leq \Tr(M) \Tr(M')$. Furthermore equality occurs if and only if the vectors 
$$
(\cA_i e^{-D_i})_{1\leq i \leq d} \stext{ and }(\cA_i e^{D_i})_{1\leq i \leq d}
$$
are proportional, which implies that $D_i =D_j$ for all $1\leq i,j\leq d$ and therefore that $M$ and $M'$ are proportional. 

\item

We first a classical result of complex analysis, called Hadamard's the three lines theorem. %see [Rudin??], often
Let $\Omega:=\{\alpha\in \C \sep |\Re(\alpha)|<1\}$, where $\Re$ denotes the real part, and let $g$ be a continuous and bounded function on $\overline \Omega$ which is holomorphic on $\Omega$. Then 
\be
\label{eqComplex}
|g(0)|^2 \leq \left(\sup_{\Re \alpha = -1} |g(\alpha)|\right) \left(\sup_{\Re z = \alpha} |g(\alpha)|\right).
\ee

We say that a matrix $U$ is unitary if $|Uz| = |z|$ for all $z\in \C$, or equivalently if $U^* U = \Id$ where $U^*$ denotes the conjugate transpose of $U$. We recall that any orthogonal matrix $O\in \cO_d$ is also unitary, and that for any diagonal matrix $D$ with real diagonal coefficients and any $\beta\in \R$ the matrix $e^{\b i \beta D}$ is unitary, where $\b i^2 = -1$.


We consider a fixed $z\in \C^d$ satisfying $|z|\leq 1$, and we define for all $\alpha\in \overline \Omega$ 
%We consider a fixed $z\in \C^d$ and we define 
$$
g(\alpha) := \pi(A^\trans e^{\alpha D} z).
$$
The function $g$ is continuous, uniformly bounded on $\overline \Omega$ by $\|\pi\|_\sC (\|A\| e^{\|D\|})^d$, and holomorphic in $\Omega$, hence the three lines theorem applies.
For any $\sigma \in \{-1,1\}$ one has 
$$
\sup_{\Re(\alpha) = \sigma} |\pi(A^\trans e^{\alpha D} z)| \leq \|\pi\circ(A^\trans e^{\sigma D})\|_\sC,
$$
since $|e^{\b i\Im(\alpha) D}z| = |z|=1$. %$|e^{i\Im(\alpha) D} z| = |z|$ where $\Im$ denotes the imaginary part.
Applying \iref{eqComplex} to the function $g$ we thus obtain 
$$
|\pi(A^\trans z)|^2 \leq \|\pi\circ(A^\trans e^D)\|_\sC \|\pi\circ(A^\trans e^{-D})\|_\sC.%\left(\sup_{\Re \alpha = -1} f(A^\trans e^\alpha z)\right) \sup
$$
Taking the supremum among all $z\in \C^d$ such that $|z|\leq 1$ we conclude that 
$$
\|\pi\circ A^\trans\|_\sC \leq \|\pi\circ(A^\trans e^D)\|_\sC \|\pi\circ(A^\trans e^{-D})\|_\sC.
$$
%Last we recall (ref??) that
There exists three orthogonal matrices $O, O', \tilde O\in \cO_d$ such that 
$$
OM^\frac 1 2 =  e^D A, \quad O'M'{^\frac 1 2} = e^{-D} A \stext{ and } \tilde O \tilde M^\frac 1 2 = A.
$$
Since orthogonal matrices are also unitary matrices we have 
\begin{eqnarray*}
\|\pi \circ A^Te^{-D}\|_\sC &=& \|\pi \circ M^{\frac 1 2}\|_\sC,\\
\|\pi \circ A^T e^{-D}\|_\sC &=& \|\pi \circ  M'^{\frac 1 2}\|_\sC\\
\|\pi \circ A^T\|_\sC &=& \|\pi \circ \ti M^{\frac 1 2}\|_\sC,
\end{eqnarray*}
thus $\|\pi\circ M^\frac 1 2\|_\sC$ satisfies the sub-multiplicativity property \iref{eqSubMult}. Furthermore $M \mapsto \|\pi\circ M^\frac 1 2\|_\sC$ is clearly continuous and strictly positive on $S_d^+$, and homogeneous of degree $m/2$ which concludes the proof of this point.

\item
We denote by $\pi\in \H_2$ the canonical quadratic form 
$$
\pi(z) := \sum_{1\leq j \leq d} z_j^2.
$$
Our purpose is to establish that for any $M\in S_d^+$
\be
\label{eqPiMM}
\|\pi\circ M^{\frac 1 2}\|_\sC = \|M\|,
\ee
which implies that $\|M\|$ is GCH in view of the previous point.
For any $z\in \C$ such that $|z|\leq 1$ one has 
$$
|\pi(M^\frac 1 2 z)| = |z^\trans M^\frac 1 2 M^\frac 1 2 z| \leq |M^\frac 1 2 z|^2 \leq \|M^\frac 1 2\|^2  = \|M\|.
$$
Furthermore choosing a normalized eigenvector $z\in \R^d$ associated to the maximal eigenvalue of $M$ we obtain $|\pi(M^\frac 1 2 z)|=\|M\|$, which establishes \iref{eqPiMM} and concludes the proof.
\sq
\end{enumerate}

\subsubsection{A well posed variant of the shape function}

We define a function $\kappa\in C^0(S_d^+, \R_+^*)$ as follows : for all $M\in S_d^+$ 
$$
\kappa(M) :=  \frac 1 d\sqrt{\Tr(M) \Tr(M^{-1})}.
$$
The function $\kappa$ is SGCH, as the product of two SGCH functions see Lemma \ref{lemmaAlgGCH} and Proposition \ref{propExGCH}.
In terms of the eigenvalues $\lambda_1, \cdots, \lambda_d$ of $M$ we have 
$$
d^2 \kappa(M)^2 = \left(\sum_{1 \leq i \leq d} \lambda_i\right)\left(\sum_{1 \leq i \leq d} \lambda_i^{-1}\right).
$$  
We regard the function $\kappa$ as a close variation on the condition number $\sqrt{\|M\|\|M^{-1}\|}$ of the matrix $M^\frac 1 2$. Note that $\kappa(M) = 1$ if and only if $M = m\Id$ for some $m>0$, and that 
$$
\kappa(M)\leq \sqrt{\|M\|\|M^{-1}\|} \leq d \, \kappa(M).
$$
The following proposition illustrates the use of $\kappa$ as a regularization term.
\begin{prop}
\label{propContLift}
Let $\vp$ be a GSH function of degree $r>0$. 
Let $(X,d_X)$ be a metric space, and let $\psi\in C^0(S_d^+ \times X, \R_+^*)$ be such that $\psi(\cdot,x)$ is GCH of degree $-1$ for any fixed $x\in X$.
We define for all $x\in X$ and all $\alpha \in (0, \infty)$
$$
L^{(\alpha)}(x) := \inf\left\{\kappa(M)^{\frac 1 \alpha} \vp(M) \sep \psi(M,x) \leq 1 \text{ and } \kappa(M) \leq e^\alpha\right\}.
$$
For any $x\in X$ there exists a unique minimizer $\cM^{(\alpha)}(x)$ to the optimization problem defining $L^{(\alpha)}(x)$. Furthermore the map $\cM^{(\alpha)} : X \to S_d^+$ is continuous. 
\end{prop}

\proof
The parameter $\alpha\in (0, \infty)$ is fixed.
\begin{itemize}
\item
(Existence of a minimizer) We consider a fixed $x\in X$ and we establish that there exists a minimizer to the optimization problem $L^{(\alpha)}(x)$.
For any $\beta \geq 0$ the following collection of matrices is compact %(*det more natural?*)
\be
\label{defKBeta}
K_\beta := \{M\in S_d^+ \sep |\ln(\det M)|\leq \beta \text{ and } \kappa(M) \leq e^\alpha\}.
\ee
We define
$$
\Lambda := \sup_{M\in K_0} \vp(M) \stext{ and } \lambda := \inf_{M\in K_0} \psi(M,x)
$$
in such way that for any $M\in S_d^+$ satisfying $\kappa(M) \leq e^\alpha$
\be
\label{eqPhiPsi}
\vp(M) \leq \Lambda (\det M)^{\frac r d} \stext{ and } \psi(M,x) \geq \lambda (\det M)^{\frac 1 d}.
\ee
We consider a minimizing sequence $(M_n)_{n \in \sN}$, $M_n\in S_d^+$, for the optimization problem $L^{(\alpha)}(x)$. It follows from \iref{eqPhiPsi} that $\det (M_n)$ uniformly bounded above and below: there exists $\beta \geq 0$ such that $|\ln \det M_n|\leq \beta$ for all $n \geq 0$. Furthermore $\kappa(M_n) \leq e^\alpha$, hence $M_n \in K_\beta$. Since the set $K_\beta$ is compact there exists a converging subsequence $M_{\sigma(n)} \to M_\infty\in K_\beta$. By continuity of the functions $\vp$, $\psi(\cdot ,x)$ and $\kappa$ on $S_d^+$ the matrix $M_\infty$ is a minimizer of the optimization problem $L^{(\alpha)}(x)$.

\item (Uniqueness)  
We consider two minimizers $M,M'$ of the minimization problem $L^{(\alpha)}(x)$, and we denote $\ti M := \Avg(M,M')$. 
Since the functions $\psi(\cdot, x)$ and $\kappa$ are GCH, the matrix $\ti M$ satisfies the inequalities 
$$
\psi(\ti M,x) \leq 1 \stext{ and } \kappa(\ti M) \leq e^\alpha.
$$ 
We define a function $\Phi \in C^0(S_d^+, \R_+^*)$, which is SGCH of degree $r>0$ in view of Lemma \ref{lemmaAlgGCH}, as follows
\be
\label{defPhiSGCH}
\Phi(M) := \kappa(M)^\frac 1 \alpha \vp(M).
\ee
If $M$ is not proportionnal to $M'$ we thus have
$$
\Phi(\ti M) < \sqrt{\Phi( M) \Phi( M')} = L^{(\alpha)}(x),
$$
 which is a contradiction. Thus $M = m M'$ for some $m>0$, but this implies 
 $$
L^{(\alpha)}(x) = \Phi( M) = \Phi( M') = m^r  \Phi( M),
 $$
 therefore $m=1$ and $M=M'$. The minimizer is unique as announced.

\item (Continuity)  
For all $x,x'\in X$, we define
$$
\omega(x,x') := \sup_{M \in K_0} |\ln \psi(M,x) - \ln\psi(M,x')|,
$$
where the set $K_0$ is defined by \iref{defKBeta}, and we observe that $\omega(x,x') \to 0$ as $x'\to x$.
(Note that $\omega(x,x')$ is the modulus of continuity of the continuous function $X \to C^0(K_0, \R)$, defined by $x\mapsto \ln \psi (\cdot,x)$.)

Consider $x,x'\in X$ and define $M := e^{\omega(x,x')} \cM^{(\alpha)}(x)$ and $M' := e^{\omega(x,x')} \cM^{(\alpha)}(x')$. We thus have 
$$
\kappa(M) = \kappa(\cM^{(\alpha)}(x)) \leq e^\alpha,
$$
and likewise $\kappa(M') \leq e^\alpha$.
Since $\psi(\cdot ,x')$ is homogeneous of degree $-1$ we obtain
$$
\psi(M, x')\leq e^{\omega(x,x_n)} \psi(M, x') = e^{\omega(x,x_n)} \psi(e^{\omega(x,x_n)} \cM^{(\alpha)}(x_n)) \leq 1,
$$
and likewise $\psi(M',x)\leq 1$.
Furthermore since $\Phi$ defined by \iref{defPhiSGCH} is homogeneous of degree $r$ we obtain
$$
L^{(\alpha)}(x') \leq \Phi(M) = e^{r\omega(x,x')} L^{(\alpha)}(x),
$$
and likewise $L^{(\alpha)}(x) \leq \Phi(M') = e^{r\omega(x,x')} L^{(\alpha)}(x')$, in particular
$$
\Phi(M') = \Phi(e^{\omega(x,x')} \cM^{(\alpha)}(x'))  = e^{r\omega(x,x')} L^{(\alpha)}(x') \leq e^{2r\omega(x,x')} L^{(\alpha)}(x).
$$

Consider a converging sequence in $X$, $x_n \to x$, and define
$$
M_n := e^{\omega(x,x_n)} \cM^{(\alpha)} (x_n).
$$
The arguments above show that $M_n$ is a minimizing sequence for the optimization problem $L^{(\alpha)}(x)$. The arguments developed for the existence of a minimizer show that $\{M_n\sep n \geq 0\}$ is contained in the compact set $K_\beta$ for a sufficiently large value $\beta\geq 0$, and that any converging subsequence of $(M_n)_{n \geq 0}$ tends to a minimizer of the optimization problem $L^{(\alpha)}(x)$, thus to $\cM^{(\alpha)}(x)$ by uniqueness.

Since the sequence $M_n$ takes its values in the compact set $K_\beta$ and has the single adherence value $\cM^{(\alpha)}(x)$, we have the convergence $M_n \to \cM^{(\alpha)}(x)$ as $n \to \infty$. Since $\omega(x,x_n) \to 0$ we obtain as announced 
$$
\cM^{(\alpha)}(x_n)\to \cM^{(\alpha)}(x),
$$
which concludes the proof of this proposition.
\sq
\end{itemize}

For any $\alpha \in (0, \infty)$ we define a function $K^{(\alpha)} : \H_m \to \R_+$ as follows
$$
K^{(\alpha)}(\pi) := \inf\{ \kappa(M)^{\frac 1 \alpha} (\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2} \|_\sC \leq 1 \text{ and } \kappa(M) \leq e^\alpha\},
$$
where the infimum is taken among symmetric positive definite matrices $M\in S_d^+$.
According to the previous proposition the minimizer $\cM^{(\alpha)}(\pi)$ of $K^{(\alpha)}(\pi)$ defines a continuous map $\cM^{(\alpha)} : \H_m\sm\{0\} \to S_d^+$. %such that $K^{(\alpha)}(\pi) = 
As $\alpha\to \infty$ the functions $K^{(\alpha)}$ on $\H_m$ converge pointwise and decreasingly to the function $K_\sC : \H_m \to \R_+$ defined by 
$$
K_\sC(\pi) := \inf\{ (\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2} \|_\sC \leq 1\}.
$$

We obtain using Lemma \ref{lemmaAM}
$$
K(\pi) = \inf_{A\in \SL_d} \|\pi\circ A\| \stext{ and } K_\sC(\pi) = \inf_{A\in \SL_d} \|\pi\circ A\|_\sC.
$$ 
Since $\|\cdot\|\leq \|\cdot \|_\sC$, and since these two functions are norms on the finite dimensional space $\H_m$, there exists a constant $n_\sC = n_\sC(m,d)$ such that for all $\pi\in \H_m$
$$
\|\pi\|\leq \|\pi\|_\sC \leq n_\sC \|\pi\|.
$$ 
It follows that
\be
\label{eqKKC}
K(\pi) \leq K_\sC(\pi) \leq n_\sC K(\pi).
\ee

The next proposition is not necessary for our analysis but gives a worthwhile insight of the properties of the shape function $K$. We show in particular that the function $K$, which is only upper semi continuous in general, is equivalent to a continuous function. We deduce a from this point a property of convergence the the functions$K^{(\alpha)}$.

% which converge only pointwise to $K$, satisfy a good substitute 
%
%The convergence of $K^{(\alpha)}$ towards $K_\sC$ is not uniform.
%The next lemma gives a substitute for this uniform convergence.

\begin{prop}
\label{lemmaKAK}
\begin{enumerate}
\item (Vanishing property)
Let $(\pi_n)_{n \geq 0}$, $\pi_n \in \H_m$,  $\pi_n \to \pi$ as $n \to \infty$, be a converging sequence of homogeneous polynomials. 
Let  $(A_n)_{n \geq 0}$, $A_n \in \SL_d$ be a sequence of matrices of unit determinant.

If $\pi_n \circ A_n \to 0$ then there exists $A\in \SL_d$, such that $\pi\circ (A^n) \to 0$.

\item (Equivalence to a lower semi continuous function) We denote by $\underline K_\sC$ the lower semi-continuous envelope of $K_\sC$ : for all $\pi\in \H_m$ 
$$
\underline K_\sC(\pi) := \lim_{\ve \to 0} \inf_{\|\pi-\pi'\|\leq \ve} K_\sC(\pi).
$$
There exists a constant $C_\lsc= C_\lsc(m,d)$ such that $\underline K_\sC \leq K_\sC\leq  C_\lsc \underline K_\sC$ on $\H_m$.

Furthermore there exist a continuous function $K_c$ on $\H_m$ such that $(C_\lsc+1)^{-1}K_c\leq K_\sC\leq (C_\lsc+1) K_c$.

\item (Substitute for uniform convergence)
For all $\ve >0$ there exists $\alpha = \alpha(m,d,\ve)$ such that for all $\pi \in \H_m$
\be
\label{eqKAKU}
K^{(\alpha)}(\pi) \leq C_\lsc \underline K_\sC(\pi)+ \ve \|\pi\|_\sC,
\ee
where $C$ is the constant appearing in 2. In particular 
\be
\label{eqKAK}
K^{(\alpha)}(\pi) \leq n_\sC (C_\lsc  K(\pi)+ \ve \|\pi\|).
\ee
\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item
For each $n\geq 0$ we consider the singular value decomposition $A_n = U_n D_n V_n$, where $U_n, V_n \in \cO_d$ and the diagonal matrix $D_n$ has positive coefficients and satisfies $\det D_n = 1$.
Since $V_n$ is orthogonal we have 
$$
\|\pi_n \circ A_n \| = \|\pi_n \circ (U_n D_n V_n)\| = \|\pi_n \circ (U_n D_n)\|.
$$
Since $\cO_d$ is compact the sequence of orthogonal matrices $U_n$ admits a converging sub-sequence $U_{\sigma(n)} \to U$. 
We define $\pi' := \pi\circ U$, $\pi'_n := \pi_{\sigma(n)} \circ U_{\sigma(n)}$ and $D'_n := D_{\sigma(n)}$, in such way that 
$$
\pi'_n \to \pi' \stext{ and } \pi'_n \circ D'_n \to 0.
$$
We recognise the hypotheses of the lemma, except that the matrices $D'_n$ replacing $A_n$ are now diagonal. We show below that there exists a diagonal matrix $D$, $\det D=1$, such that $\pi'\circ (D^n) \to 0$. Defining $A := UDU^\trans$ leads to the announced result $\pi \circ (A^n) \to 0$.

In order to avoid notational clutter we do not keep track of the extraction procedure and we simply write $\pi$, $\pi_n$ and $D_n$ in place for $\pi'$, $\pi'_n$ and $D'_n$.
We define the finite set 
$$
\Lambda := \{\alpha \in \Z_+^d\sep |\alpha| \leq k\},
$$
and to any $t\in (\R_+^*)^d$ we associate a subset $\Lambda(t)\subset \Lambda$
$$
\Lambda(t) := \{\alpha \in \Lambda \sep t^\alpha \geq 1\}.
$$
For each $n$ we denote by $\Lambda_n$ the set $\Lambda(t_n)$ associated to the list $t_n$ of diagonal entries of $D_n$.

There are only a finite number of subsets of $\Lambda$, namely $2^{\#(\Lambda)}$, thus there exists an extraction $\tau$ such that $\Lambda_* := \Lambda_{\tau(n)}$ us independent of $n$.

For any $\alpha\in \Lambda$ we denote by $\pi_{n,\alpha}$ the coefficient of $Z^\alpha$ in $\pi_n$, and by $\pi_\alpha$ the coefficient of $Z^\alpha$ in $\pi$, where $Z=(Z_1, \cdots ,Z_d)$ is the $d$-dimensional variable. 
$$
\pi_n = \sum_{\alpha \in \Lambda} \pi_{n , \alpha} Z^\alpha \stext{ and } \pi = \sum_{\alpha \in \Lambda} \pi_\alpha Z^\alpha.
$$
We recall that $t_n$ denotes the list of coefficients of the diagonal matrix $D_n$, we denote by $t$ the list of coefficients of a diagonal matrix $D$. We thus have 
$$
\pi_n \circ D_n = \sum_{\alpha \in \Lambda} \pi_{n , \alpha} t_n^\alpha Z^\alpha \stext{ and } \pi \circ D^n= \sum_{\alpha \in \Lambda} \pi_\alpha t^{n \alpha} Z^\alpha.
$$
Since $\pi_n \circ D_n \to 0$ we have 
$
\pi_{n ,\alpha} t_n ^\alpha \to 0
$
for any $\alpha \in \Lambda$.
For any $\alpha$ in the subset $\Lambda_*\subset \Lambda$ we obtain recalling that $t_{\tau(n)}^\alpha \geq 1$
$$
\pi_\alpha = \lim_{n \to \infty} \pi_{\tau(n) ,\alpha} = 0.
$$
We now define $D = D_{\tau(0)}$, we denote by $t$ the list of coefficients of $D$,
and we observe that 
$$
\pi \circ D^n \to 0.
$$
Indeed $\pi_\alpha t^{n \alpha} = 0$ for all $\alpha\in \Lambda_*$, and $\pi_\alpha t^{n \alpha} \to 0$ for all $\alpha \notin \Lambda_*$ since $t^\alpha <1$, which concludes the proof of this point.


\item
As a consequence of 1. we obtain the following vanishing property : for any $\pi \in \H_m$, if $\underline K_\sC(\pi) = 0$ then $K_\sC(\pi) = 0$. Indeed if $\underline K_\sC(\pi) = 0$ then there exists a sequence of homogeneous polynomials $\pi_n\to \pi$ such that $K_\sC(\pi_n) \to 0$, and therefore a sequence of matrices $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, such that $\pi_n \circ A_n$. Therefore there exists $A\in \SL_d$ such that $\pi\circ (A^n)\to 0$, which implies that $K_\sC(\pi) = 0$.

%We define $\cS := \{\pi \in \H_m \sep \|\pi\|_\sC = 1\}$ and we consider the closed set 
We consider the compact set 
$$
\cA := \{\pi \in \H_m \sep \|\pi\|_\sC = 1 \text{ and } \|\pi \circ A\|_\sC \geq 1 \text{ for all } A\in \SL_d\}.
$$
For any $\pi \in \cA$ we thus have $K_\sC(\pi) = \|\pi\|_\sC=1$, and therefore $\underline K_\sC(\pi) >0$. 
Since $\cA$ is compact and since $\underline K_\sC$ is lower semi-continuous, the function $\underline K_\sC$ attains its lower bound on $\cA$ and we define
$$
C^{-1}_\lsc := \inf_{\pi \in \cA} \underline K_\sC(\pi).
$$
Let $\pi\in \H_m$, and let $(A_n)_{n \geq 0}$, $A_n\in \SL_d$, be a sequence of matrices satisfying $\|\pi\circ A_n\|_\sC \to K_\sC(\pi)$ as $n \to \infty$. If $K_\sC(\pi) = 0$ then $\underline K_\sC(\pi) = 0$ also according to the first point of this lemma, and there is nothing to prove.
If $K_\sC(\pi) = 0$ then consider an extraction $\vp$ such that we have the convergence 
$$
\frac{\pi \circ A_n}{\|\pi\circ A_n\|_\sC} \to \pi_*.
$$
We now prove that $\pi_*\in \cA$. Indeed $\|\pi_*\|_\sC = 1$ by construction. If, by contradiction, there exists $A\in SL_d$ such that $\|\pi_*\circ A\| = \delta<1$, then we obtain 
$$
K_\sC(\pi) \leq \lim_{n \to \infty} \|\pi \circ (A_n A)\|_\sC = \lim_{n \to \infty} \frac{\|\pi \circ (A_n A)\|_\sC}{\|\pi\circ A_n\|_\sC} \|\pi\circ A_n\|_\sC = \delta K_\sC(\pi)
$$
which is a contradiction, hence $\pi_*\in \cA$ as announced.
We now observe that 
$$
\underline K_\sC \left(\frac{\pi\circ A_n}{\|\pi\circ A_n\|_\sC} \right) = \frac {\underline K_\sC(\pi)}{\|\pi\circ A_n\|_\sC} \underset {n \to \infty} \longrightarrow \frac {\underline K_\sC(\pi)}{K_\sC(\pi)}.
$$
On the other hand, since $\underline K_\sC$ is lower semi continuous and $\pi_*\in \cA$,
$$
\lim_{n \to \infty} \underline K_\sC \left(\frac{\pi\circ A_n}{\|\pi\circ A_n\|_\sC} \right) \geq \underline K_\sC(\pi_*) \geq C_\lsc^{-1}.
$$
Combining the last two equations we obtain as announced $K_\sC(\pi) \leq C_\lsc \underline K_\sC(\pi)$. 

We now construct a continuous function $K_c$ on $\H_m$ which is equivalent to $K_\sC$.
For each $n\in \Z$ we define
$$
E_n := \{\pi\in \H_m \sep K_\sC(\pi) \geq (C_\lsc+1)^n\}.
$$
Note that the closed sets $E_{n+1}$ and $\overline {\H_m \sm E_n}$ are disjoint, since $K_\sC \leq C_\lsc \underline K_\sC \leq C_\lsc (C_\lsc+1)^n$ on the latter. The following functions is thus continuous
$$
r_n(\pi) := \frac{d(\pi, \H_m \sm E_n)}{d(\pi, \H_m \sm E_n)+ d(x,E_{n+1})} \stext{ where } d(\pi,X) := \inf_{\pi'\in X} \|\pi-\pi'\|_\sC.
$$
We define a continuous function $r : \H_m \to [-\infty, \infty)$ (observe that $-\infty$ is included) but the sum
$$
r(\pi) := \sum_{n <0} (r_n(\pi)-1) + \sum_{n \geq 0} r_n(\pi),
$$
which is finite for any $\pi$ such that $K_\sC(\pi)>0$.
Eventually we set 
$$
K_c(\pi) := (C_\lsc+1)^{r(\pi)},
$$
which concludes the proof.

\item
We consider a fixed $\ve>0$ and we recall that $K^{(\alpha)}$ converges pointwise decreasingly to $K_\sC$ as $\alpha\to \infty$. To each $\pi \in \cS := \{\pi \in \H_m \sep \|\pi\|_\sC = 1\}$ we associate $\alpha_\pi\in (0, \infty)$ satisfying 
$$
K^{(\alpha_\pi)}(\pi) < K_\sC(\pi)+ \ve.
$$
In particular $K^{(\alpha_\pi)}(\pi) < C_\lsc \underline K_\sC(\pi)+ \ve$, and since $\underline K_\sC$ is lower continuous the collection $V_\pi$ of all $\pi'\in \cS$ satisfying 
$$
K^{(\alpha_\pi)}(\pi') < C_\lsc \underline K_\sC(\pi')+ \ve
$$
is an open neighborhood of $\pi$ in $\cS$. 

Since $\cS$ is compact there exists a finite subset $\cS_0$ of $\cS$ such that 
$$
\bigcup_{\pi \in \cS_0} V_\pi = \cS. 
$$
Defining $\alpha := \max \{\alpha_\pi \sep \pi \in \cS_0\}$, and recalling that $K^{(\alpha)} \leq K^{(\alpha')}$ if $\alpha \geq \alpha'$, we obtain for all $\pi\in \H_m \sm \{0\}$
$$
K^{(\alpha)}\left(\frac \pi {\|\pi\|_\sC}\right) \leq C_\lsc \underline K_\sC\left(\frac \pi {\|\pi\|_\sC}\right)+ \ve,
$$
which implies \iref{eqKAKU} since $K^{(\alpha)}$ and $\underline K_\sC$ are $1$-homogeneous on $\H_m$.
The inequality \iref{eqKAK} is a direct consequence of \iref{eqKKC}.
\end{enumerate}
\sq

\subsubsection{The metric}
\label{subsubsecExplicitMetricLP}
We consider a function $f\in C^m_\per(\R^d)$ and we define for all $z\in \R^d$ a homogeneous polynomial $\pi_z\in \H_m$ as follows 
\be
\label{defPizLpMet}
\pi_z := \sum_{|\alpha| = m} \frac{\partial^m f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!},
\ee
and a non homogeneous polynomial $\mu_z\in \P_{m-1}$
\be
\label{defMuzLpMet}
\mu_z := \sum_{|\alpha| < m} \frac{\partial^{|\alpha|} f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!}.
\ee
We recall the classical Taylor formula : for any $z, h\in \R^d$
\be
\label{defTaylor}
f(z+h) - \mu_z(h) = m\int_0^1 \pi_{z+th}(h) (1-t)^{m-1} dt,
\ee
and we denote by $\omega$ the modulus of continuity of the $\Z^d$ periodic function $z\mapsto \pi_z$
$$
\omega(r) := \sup_{|z-z'|\leq r} \|\pi_z - \pi_{z'}\|.
$$
We recall that $\volBall$ denotes the volume of the euclidean unit ball $B(0,1)$.
\begin{lemma}
\label{lemmaEstimSmooth}
\begin{itemize}
\item (Difference of two values of $f$)
We have for any $z,h\in \R^d$
$$
|f(z+h)- \mu_z(h)| \leq |\pi_z(h)| + |h|^m \omega(|h|).
$$
\item (Error estimate on an ellipse)
Defining $S(z) := H(z)^{-\frac 1 2}$ we have 
\be
\label{eqLocSmooth}
e_H(f\sep z)_p \leq (\volBall \det S(z))^\frac 1 p (\|\pi_z\circ S(z)\|+ \|S(z)\|^m \omega(\|S(z)\|)).
\ee
\item (Error with respect to a metric)
Assume that $H\in \bH_\per$ has the form
$$
H(z) = (\det M(z))^{\frac{-1}{mp+d}} M(z)
$$
where $\|\pi_z \circ M(z)^{-\frac 1 2}\|\leq 1$ for all $z\in \R^d$.
Then for all $\lambda>0$
$$
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq \volBall^{\frac 1 p} (1+ \omega_H(\lambda^{-\frac 1 2}))\|(\det M)^{\frac m {2d}}\|_{L^\tau([0,1]^d)},
$$
where $\omega_H$ is a function expressed in terms of $\omega$ and $H$, which satisfies $\omega_H(\mu) \to 0$ as $\mu\to 0$.
\end{itemize}
\end{lemma}

\proof
\begin{itemize}
\item 
This point is a direct consequence of the Taylor formula \iref{defTaylor}. Indeed 
$$
f(z+h) - \mu_z(h) = \pi_z(h)+ m\int_0^1 (\pi_{z+th}(h)-\pi_z(h)) (1-t)^{m-1} dt,
$$
thus 
$$
|f(z+h) - \mu_z(h)-\pi_z(h)|\leq m\int_0^1  |h|^m\omega(|h|) (1-t)^{m-1} dt = \omega(|h|) |h|^m.
$$

\item Observing that $B_H(z) = \{z+S(z) u \sep |u|\leq 1\}$ we obtain 
\begin{eqnarray*}
e_H(f\sep z)_p &\leq& |B_H(z)|^{\frac 1 p} \sup_{|h|_{H(z)} \leq 1} |f(z+h) - \mu_z(h)| \\
&\leq&  |B_H(z)|^{\frac 1 p}\sup_{|h|_{H(z)} \leq 1} |\pi_z(h)|+|h|^m \omega(|h|)\\
&=& (\volBall \det S(z))^\frac 1 p (\|\pi_z\circ S(z)\|+ \|S(z)\|^m \omega(\|S(z)\|)).\\
%& = & \left(\frac \cPi {\sqrt{\det H(z)}}\right)^\frac 1 p \left(\left\|\pi_z \circ H(z)^{-\frac 1 2}\right\| + \left\|H(z)^{-\frac 1 2}\right\|^m \omega\left(\left\|H(z)^{-\frac 1 2}\right\|\right)\right)
\end{eqnarray*}
\item Defining 
$$
S(z) := H(z)^{-\frac 1 2} = (\det M(z))^{\frac 1 {2(mp+d)}} M(z)^{-\frac 1 2}
$$
and recalling that $\pi_z$ is homogeneous of degree $m$ we obtain 
$$
\det S(z) = (\det M(z))^{\frac {-mp} {2(mp+d)}} \stext{ and } \|\pi_z \circ S(z)\|\leq (\det M(z))^{\frac m {2(mp+d)}}.
%, \quad \|S(z)\| = ??
$$
Applying \iref{eqLocSmooth} to $\mu S$ for some $\mu>0$ we obtain 
\begin{eqnarray*}
e_{\mu^{-2} H}(f\sep z)_p &\leq& (\volBall \det (\mu S(z)))^\frac 1 p (\|\pi_z\circ (\mu S(z))\|+ \|\mu S(z)\|^m \omega(\|\mu S(z)\|)),\\
&=& \mu^{\frac d p+m} (\volBall \det S(z))^\frac 1 p (\|\pi_z\circ S(z)\|+ \|S(z)\|^m \omega(\mu \|S(z)\|)),\\
&=& \mu^{\frac d p+m} \volBall^\frac 1 p \left(1+\|M(z)^{-\frac 1 2}\|^m \omega(\mu \|S(z)\|)\right)
\end{eqnarray*}
Hence
$$
e_{\mu^{-2} H}(f\sep z)_p \leq \mu^{\frac d p+m} \volBall^\frac 1 p (1+ \omega_H(\mu))
$$
where 
$$
\omega_H(\mu) := \sup_{z\in \sR^d} \|M(z)^{-\frac 1 2}\|^m \omega(\mu \|S(z)\|).
$$
Note that $\omega_H(\mu)$ is finite and tends to zero as $\mu\to 0$, since the functions $M$ and $S$, which are defined in terms of  $H \in \H_\per$, are continuous and $\Z^d$ periodic.
Therefore 
\begin{eqnarray*}
e_{\mu^{-2} H}(f)_p &:=& \left\|\sqrt[2p]{\det (\mu^{-2} H(z))}\, e_{\mu^{-2} H}(f\sep z)_p\right\|_{L^p([0,1]^d)}\\
&\leq & \mu^m \volBall^\frac 1 p (1+ \omega_H(\mu)) \left\|\sqrt[2p]{\det H(z)}\right\|_{L^p([0,1]^d)}\\
&=& \mu^m \volBall^\frac 1 p (1+ \omega_H(\mu)) m(H)^\frac 1 p
\end{eqnarray*}

On the other hand 
$$
m(H) =\int_{[0,1]^d} \sqrt{\det H(z)} dz =\int_{[0,1]^d} (\det M(z))^{\frac {mp} {2(mp+d)}}.
$$
Since $\frac 1 \tau = \frac m d+ \frac 1 p$ we thus have 
$$
\frac {mp} {2(mp+d)} = \frac {m\tau}{2d}.
$$
Recalling that $m(\mu^{-2} H) = \mu^{-d} m(H)$, we obtain as announced
\begin{eqnarray*}
m(\mu^{-2} H)^\frac m d e_{\mu^{-2} H}(f)_p &\leq& \volBall^\frac 1 p (1+ \omega_H(\mu)) m(H)^{\frac m d+ \frac 1p}\\
&=& \volBall^\frac 1 p (1+ \omega_H(\mu)) \|(\det M)^{\frac m {2d}}\|_{L^\tau([0,1]^d)}
\end{eqnarray*}
which concludes the proof of this lemma. \sq
\end{itemize}

The next result is announced in the introduction under the reference Theorem \ref{thSmooth}.

\begin{theorem}
There exists a constant $C=C(m,d)$ such that the following holds.\\
For each $f\in C^m_\per$ such that $z\mapsto K(d^m f(z))$ is not identically $0$, there exists a metric $H \in \bH_\per\cap \bH_g$, which is also $C^\infty$, and such that for all $\lambda \geq 1$
$$
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|K(d^m f)\right\|_\tau,
$$
where $\frac 1 \tau := \frac m d+ \frac 1 p$.
\end{theorem}
\proof
We recall that $K^{(\alpha)}(\pi) \leq \|\pi\|_\sC$ for any $\alpha\in(0, \infty)$, and that $K^{(\alpha)}$ converges pointwise to $K_\sC$ as $\alpha\to \infty$.
It follows, using the theorem of dominated convergence for integrals, that 
$$
\lim_{\alpha\to \infty} \|K^{(\alpha)}(\pi_z)\|_{L^\tau([0,1]^d)} = C_0 := \|K_\sC(\pi_z)\|_{L^\tau([0,1]^d)}.
$$
Observe that $\|K_\sC(\pi_z)\|_{L^\tau([0,1]^d)}$ since $z\mapsto K(d^m f(z))$ is not identically $0$ and is equivalent to a continuous function according to Lemma \ref{lemmaKAK}. From this point we consider a fixed $\alpha\in (0, \infty)$ such that $\|K^{(\alpha)}(\pi_z)\|_{L^\tau([0,1]^d)} < 2C_0$.
Since $\cM^{(\alpha)} : \H_m \sm\{0\}\to S_d^+$ is continuous, and since $\cM^{(\alpha)}(\pi) \to 0$ as $\pi \to 0$, the extended map $\cM^{(\alpha)} : \H_m\to S_d$ where $\cM^{(\alpha)}(0) = 0$ is also continuous.

The function $M_0 : \R^d \to S_d$ defined by 
$$
M_0(z) := \cM^{(\alpha)} (\pi_z)
$$
is therefore continuous and satisfies 
$
\|(\det M_0)^\frac m {2d}\|_{L^\tau([0,1]^d)} <2C_0
$
and for all $z\in \R^d$ we have either $\pi_z=0$ or $\|\pi_z \circ M_0(z)^{-\frac 1 2}\| \leq 1$.
We consider $\ve_1>0$ sufficiently small in such way that $M_1 := M_0+ \ve_1\Id$ still satisfies $\|(\det M_1)^\frac m {2d}\|_{L^\tau([0,1]^d)} <2C_0$, and we observe that $\|\pi_z \circ M_1(z)^{-\frac 1 2}\| < 1$ for all $z\in \R^d$.

We consider a $C^\infty$ non-negative radially symmetric compactly supported function $\psi$ of integral one, a mollifier, and we set $\psi_\ve(z) := \ve^{-d}\psi(z/\ve)$. We choose $\ve_2>0$ sufficiently small in such way that the $C^\infty$ mollification $M_2 := \psi_{\ve_2} * M_1$ of $M_1$ still satisfies $\|(\det M_2)^\frac m {2d}\|_{L^\tau([0,1]^d)} <2C_0$ and $\|\pi_z \circ M_2(z)^{-\frac 1 2}\| < 1$ for all $z$ in the compact set $[0,1]^d$, hence for all $z\in \R^d$ by periodicity.

Defining $H\in \bH_\per$ by
$$
H_0(z) := (\det M_2(z))^{\frac {-1}{mp+d}} M_2(z).
$$
Hence 
$$
m(\lambda H_0) e_{\lambda H_0}(f)_p \leq \volBall^\frac 1 p (1+\omega_{H_0}(\lambda^{-\frac 1 2})) \|(\det M_2)^\frac m {2d}\|_{L^\tau([0,1]^d)}
$$
Since $\omega_{H_0}(\lambda^{-\frac 1 2}) \to 0$ as $\lambda \to \infty$, we obtain for $\lambda$ sufficiently large
$$
m(\lambda H_0) e_{\lambda H_0}(f)_p \leq 2 \volBall^\frac 1 p \|K_\sC(\pi_z)\|_{L^\tau([0,1]^d)}\leq C \|K(d^m f)\|_{L^\tau([0,1]^d)} 
$$
where $C := \frac{2 \volBall^\frac 1 pn_\sC}{m!}.$
Since $H_0$ is $C^\infty$ and periodic, we obtain from Remark \ref{remHomog} in the previous chapter that $\lambda H_0\in \bH_a$ when $\lambda$ is sufficiently large.
Defining $H := \Lambda H_0$, where $\Lambda$ is a sufficiently large constant we conclude the proof of this theorem.
\sq


\subsection{Approximation spaces}
\label{subsecApproxSpaceLP}

We present in this subsection a (naive) definition of anisotropic approximation spaces, which are based on the approximation of a function with respect to a metric, measured in the $L^p$ norm and approximating locally with $\P_{m-1}$ polynomials. This approach is strongly tied with the study [Petrushev] of anisotropic Besov spaces associated to ellipsoid covers of $\R^n$.

For any $\star\in \{i,g\}$ and any $f\in L^p_\per$ we define a (nonlinear) quantity $|f|_{\star,p} \in [0, \infty]$ as follows \be
\label{defFStarP}
|f|_{\star,p} := \sup_{\mu \geq 1} \left(\mu^\frac m d\inf_{\substack{H \in \bH_\star\cap \bH_\per\\ m(H) \leq \mu}}e_H(f)_p\right).
\ee
This quantity is more or less understood in the isotropic case $\star = i$, using an approach based on the Hardy-Littlewood maximal function  $\mathfrak M(g)$ associated to a function $g\in L^1_\per$, 
$$
\mathfrak M(g \sep z) := \sup_{r>0} \frac 1 {r^d} \int_{B(z,r)} |g|.
$$
The next lemma gives some key properties of a variant $\gM_\delta$ of the maximal function $\gM$.
\begin{lemma}
For all $\delta > 0$ let,
$$
T_\delta(s) := 
\left\{
\begin{array}{cc}
s & \text{ if } s\geq \delta,\\
0 & \text{ otherwise}.
\end{array}
\right.
$$
Let $g\in L^1_\per(\R^d)$, which is not identically zero, and let
$$
\gM_\delta(g\sep z) := \sup_{r>0} \frac 1 {r^d} T_\delta\left(\int_{B(z,r)} |g|\right).
$$
Then $s_\delta(z) := (\delta/\gM_\delta(g\sep z))^\frac 1 d$ is a positive Lipschitz function and satisfies for all $z\in \R^d$
\be
\label{intSDelta}
\int_{B(z,s_\delta(z))} |g|\leq \delta.
\ee
\end{lemma}

\proof
We consider a fixed value of the parameter $\delta>0$.
Since $g\in L^1_\per$ we have for any $z\in \R^d$ 
$$
\lim_{r\to \infty} \frac 1 {r^d} \int_{B(z,r)}|g| = \volBall \int_{[0,1]^d} |g|>0. %\lim_{r\to \infty} \frac{|B(z,r)|}{r^d}
$$ 
Furthermore there exists $r_0>0$ such that for any $z\in \R^d$ one has 
$$
\int_{B(z,r_0)} |g| < \delta.
$$
Combining the two last equations we obtain that $\gM_\delta(g\sep z)\in (0, \infty)$ for any $z\in \R^d$.
We define $I_\delta(z,r)$ by 
$$
I_\delta(z,r)^d := \frac 1 \delta T_\delta\left(\int_{B(z,r)} |g|\right).
$$
Note that $I_\delta(z,r)\in \{0\} \cup [1, \infty)$ and that for any $z,u\in \R^d$ and and $r>0$
$$
I_\delta(z+u, r)\leq I_\delta(z,r+|u|),
$$
since $B(z+u,r) \subset B(z,r+|u|)$.
Note also that %Furthermore 
\be
\label{defSDelta}
s_\delta(z) = \inf_{r>0} \frac r {I_\delta(z,r)}.
\ee
Let $z,z'\in \R^d$ be such that $|z-z'|\leq r_0$. We therefore have 
\begin{eqnarray*}
s_\delta(z') &=& \inf_{r>0} \frac r {I_\delta(z',r)} \\
& \geq & \inf_{r>0} \frac r {I_\delta(z,r+|z-z'|)} \\
& = & \inf_{r>|z-z'|} \frac{r- |z-z'|}{I_\delta(z,r)}\\ 
& \geq &  \inf_{r>|z-z'|} \frac r {I_\delta(z,r)} - |z-z'| \\
&=&  s_\delta(z)- |z-z'| 
\end{eqnarray*}
In the fourth line we used the fact that one always have $I_\delta(z,r)\geq 1$ or $I_\delta(z,r)=0$, and that the later case does not correspond to the infimum. In the last line we used the fact that $I_\delta(z,r)=0$ for all $r\leq |z-z'| \leq r_0$ %, which implies that $r/I_\delta(z,r) = \infty$, 
and therefore the infimum can be restricted to $r>|z-z'|$.

Exchanging $z$ and $z'$ we obtain that $|s_\delta(z) - s_\delta(z')| \leq |z-z'|$ for all $z,z'\in \R^d$ satisfying $|z-z'| \leq r_0$. 
If $z,z'$ are arbitrary then we consider an integer $n>0$ such that  $|z-z'| \leq n r_0$ and we obtain 
\begin{eqnarray*}
|s_\delta(z) - s_\delta(z')| &\leq& \sum_{1\leq i \leq n} \left|s_\delta\left(\frac {iz} n +\frac{(n-i)z'} n\right)-s_\delta\left(\frac {(i-1)z} n +\frac{(n-i+1)z'} n\right) \right| \\
&\leq& n \frac{|z-z'|} n = |z-z'|, 
\end{eqnarray*}
hence $s_\delta$ is Lipschitz on $\R^d$ as announced.


The proof of the second point  \iref{intSDelta} is simpler. Indeed injecting $r = s_\delta(z)$ in \iref{defSDelta} we obtain 
$$
s_\delta(z) \leq  s_\delta(z) \left(\frac \delta {T_\delta\left(\int_{B(z,s_\delta(z))} g\right)}\right)^{\frac 1 d}.
$$
which implies \iref{intSDelta} and concludes the proof.
\sq

\begin{theorem}
Let $\frac 1 \tau := \frac m d +\frac 1 p$. If $\tau \geq 1$ and if the Sobolev injection $W^{m, \tau} \to L^p$ holds (which excludes the case $m=1$ and $p=\infty$) then one has
$$
|f|_{i,p} \leq C\left(\int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz\right)^\frac 1 \tau,
$$
where $C=C(m,d,p)$.
\end{theorem}

\proof
We assume that $d^m f$ is not identically zero, otherwise $f$ is a periodic polynomial of degree $m-1$, thus a constant, and $|f|_{i,p} = 0$.
For each $\delta>0$ we define
$$
H_\delta(z) := \max\{1, \ \gM_\delta(|d^m f|^\tau \sep z)^{\frac 2 d}/\delta^\frac 2 d\} \Id = \frac \Id {\min \{1 , s_\delta(z)\}^2},
$$
where $s_\delta(z) := (\delta/ \gM_\delta(|d^m f|^\tau \sep z))^\frac 1 d$ is a Lipschitz function according to the previous proposition. We observe that $H_\delta\in \bH_i$ and that 
\be
\label{eqMHDelta}
m(H_\delta) \leq \int_{[0,1]^d} \max\{1, \gM_\delta(|d^m f|^\tau \sep z)/\delta\} dz \leq 1+M/\delta.
\ee
where 
$$
M := \int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz.
$$
%Define $B := \{z\in \R^d \sep |z|\leq 1\}$ 
We recall the following classical Sobolev estimate : there exists $C_{\rm sob}$ such that for any $g\in W^{m, \tau}(B(0,1))$
$$
\inf_{\mu\in \sP_{m-1}} \|g-\mu\|_{L^p(B(0,1))} \leq C_{\rm sob} \|d^m g\|_{L^\tau(B(0,1))}.
$$
Using an isotropic change of variables we obtain for any $z\in \R^d$, any $r>0$ and any $g\in W^{m, \tau}(B(z,r))$
$$
\inf_{\mu\in \sP_{m-1}} \|g-\mu\|_{L^p(B(z,r))} \leq C_{\rm sob} \|d^m g\|_{L^\tau(B(z,r))}.
$$
Therefore, using \iref{intSDelta},
\begin{eqnarray*}
e_{H_\delta}(f\sep z)_p &\leq & \inf_{\mu\in \sP_{m-1}} \|f-\mu\|_{L^p(B(z,s_\delta(z)))} \\
& \leq & C_\sob \|d^m f\|_{L^\tau(B(z,s_\delta(z)))}\\
& \leq & C_\sob \delta^\frac 1 \tau.
\end{eqnarray*}
It follows that 
$$
e_{H_\delta}(f)_p^p := \int_{[0,1]^d} \sqrt{\det H_\delta(z)} \, e_{H_\delta}(f\sep z)_p^p \, dz \leq m(H_\delta) (C_\sob \delta^\frac 1 \tau)^p
$$
Recalling that $m(H_\delta)\leq 1+M/\delta$, see \iref{eqMHDelta}, we obtain  
$$
(1+M/\delta)^\frac m d e_{H_\delta}(f)_p \leq  (1+M/\delta)^\frac 1 \tau C_\sob \delta^\frac 1 \tau = C_\sob (\delta+M)^\frac 1 \tau
$$
We apply the previous estimate to the range of parameters $0<\delta \leq M$, which corresponds to the range $2\leq 1+M/\delta< \infty$ of our upper bound for the mass of $H_\delta$, and we obtain 
$$
\sup_{\mu\geq 2} \left(\mu^\frac m d\inf_{\substack{H \in \bH_\star\cap \bH_\per\\ m(H) \leq \mu}}e_H(f)_p\right)\leq C_\sob (2M)^\frac 1 \tau.
$$
In order to estimate $|f|_{i,p}$, see \iref{defFStarP}, we need in addition to address the range of parameters $1\leq \mu \leq 2$. For that purpose we consider the constant metric $H_\infty := \Id$, which satisfies $m(H_\infty)=1$. For any $z\in \R^d$, observing that $B(z,1)$ is covered by $2^d$ translates of the cube $[0,1]^d$, we obtain  
\begin{eqnarray*}
e_{H_\infty}(f\sep z)_p &=& \inf_{\mu\in \sP_{m-1}} \|f-\mu\|_{L^p(B(z,1))} \\
&\leq &C_\sob \|d^m f\|_{L^\tau(B(z,1))} \\
&\leq & 2^d C_\sob \|d^m f\|_{L^\tau([0,1]^d)}\\
& \leq & 2^d C_\sob M^\frac 1 \tau.
%C_\sob \gM(|d^mf|^\tau \sep z)^\frac 1 \tau
\end{eqnarray*}
Where we used the fact that $|d^m f(z)|^\tau \leq \gM(|d^mf|^\tau \sep z)$ for almost every $z\in \R^d$. Therefore $e_{H_\infty}(f)_p \leq 2^d C_\sob M^\frac 1 \tau$ which concludes the proof of this theorem.
\sq

%\begin{theorem}
%There exists a constant $C=C(m,d)$ such that the following holds.\\
%\begin{itemize}
%\item (Quasi triangle inequality) ?? Needs to be checked.
%For all $f,g\in L^p$ one has 
%$$
%|f+g|_{i,p} \leq C (|f|_{i,p}+ |g|_{i,p}).
%$$
%\item (Link to Sobolev norms) If $\tau \geq 1$ and if the Sobolev injection $W^{m, \tau} \to L^p$ holds (which excludes the case $m=1$ and $p=\infty$) then one has
%$$
%|f|_{i,p} \leq C\left(\int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz\right)^\frac 1 \tau.
%$$
%\end{itemize}
%\end{theorem}
%
%\proof
%\begin{itemize}
%\item Consider $\mu\geq 1$ and $H, H'\in \bH_i$, satisfying $m(H) = m(H')=\mu$. There exists two Lipschitz functions $s,s' : \R^d \to R_+^*$ such that $H = Id/s^2$ and $H' =  \Id/s'^2$,
%%$$
%%H = \frac \Id {s^2}, H' =  \frac \Id {s'^2}
%%$$
%and we define
%$$
%\ti H(z) := \frac \Id {\min\{s(z), s'(z)\}^2}.
%$$
%We have $\ti H \in \bH_i$ since the function $z\mapsto \min\{s(z), s'(z)\}$ is Lipschitz. Furthermore 
%$$
%m(\ti H) = \int_{[0,1]^d} \max \left\{\frac 1 {s(z)^d}, \ \frac 1 {s'(z)^d}\right\} dz \leq m(H)+m(H')=2\mu.
%$$
%The approximation error satisfies 
%$$
%e_{\ti H} (f+g)_p \leq e_{\ti H}(f)_p + e_{\ti H}(g)_p \leq ? e_H(f)_p + e_{H'}(g)_p
%$$
%
%
%\item
%\end{itemize}
%\sq

In contrast to $|f|_{i,p}$, %does not satisfy the quasi triangle inequality and 
there is no known relevant %``close to sharp'' 
bound for $|f|_{g,p}$ explicit in terms of the $m$-th derivatives of $f$.
We intend to study this quantity in more detail in the future, but for now we can only make some conjectures. 
In the case $p=m=d=2$, Chapter \ref{chapCartoon} suggests that $|f|_{g,2}$ is finite for any cartoon function $f$, probably with the lower bound 
\be
\label{eqLowerCartoon}
J(f) := \left( \int_{[0,1]^2 \sm \Gamma } |\det d^2 f(z)|^\frac 1 3 dz+ \int_\Gamma |[f](s)|^\frac 2 3 |\kappa(s)|^\frac 1 3\right)^\frac 3 2 \stackrel ? \leq C |f|_{g,2}
\ee
where $[f](s)$ denotes the jump of $f$ at a point $s\in \Gamma$, and $\kappa(s)$ the curvature of $\Gamma$ at $s$.

We study in Chapter \ref{chapCartoon} the convolution of a cartoon function with a mollifier $\psi$ (compactly supported, for simplicity), and we have shown that the left hand side of \iref{eqLowerCartoon} is stable under mollification, see Theorem [??] :  for any cartoon function $f$
\be
\label{eqStableJ}
\lim_{\delta \to 0} J(f*\psi_\delta) \leq C(\psi) J(f) \stext{ where } \psi_\delta := \frac 1 \delta \psi \left( \frac \cdot {\sqrt{\delta}}\right).
\ee
This point is not trivial since the discontinuities of $f$ are traded for an (anisotropic) explosion of the derivatives of $f_\delta$, as $\delta \to 0$.

We consider $f\in L^p_\per$ and denote by $f_t$ the transportation of $f$ by the heat semi-group
$$
\partial f_t + \triangle f_t = 0,
$$
equivalently
$$
f_t = f* \vp_t \stext{ where } \vp_t := \frac 1 t \vp\left(\frac{\cdot}{\sqrt t} \right) \stext{ and }  \vp (z) := \frac 1 {\sqrt{2 \pi} } \exp\left(\frac{-|z|^2}{t}\right).
$$
This result suggests that anisotropic smoothness classes are not unrelated with classical PDE's. In some circumstances at least, we may have 
$$
|f_t|_{g,2} \stackrel ? \leq  C(t) |f|_{g,2}.
$$

\section{Approximation in the $W^{1,p}$ norm}

We extend in this section to the $W^{1,p}$ norm the results presented in the previous section for the $L^p$ norm. This extension is not straightforward due to the following phenomenon : the gradient of the interpolation $\interp_\cT^{m-1} g$ of a function, or of the twisted mollification $f_H$ may have strong undesirable oscillations which are not present in the original function. 
These effects are avoided in the case of quasi-acute meshes and metrics, but these objects have less flexibility than the larger class of graded meshes and metrics. Furthermore current anisotropic mesh generation software seem to be based on graded classes rather than quasi acute ones.
We therefore split the theory into two parts, one devoted to quasi-acute classes, and the other to graded ones.



\subsection{Comparison of the error associated to a mesh and to a metric}
\label{subsecErrMeshMetW1P}

We compare in this section the $W^{1,p}$ finite element approximation error of a function on a mesh with the errors $e_H^a(\nabla f)_p$ or $e_H^g(\nabla f)_p$ associated to a metric. 
Let us recall that for any $f\in W^{1,p}_\per$, $H\in \bH_\per$ and $\star\in \{a,g\}$ one has 
$$
e_H^\star(\nabla f)_p := \left\|\sqrt[2p]{\det H(z)} \, e_H^\star(\nabla f\sep z)_p\right\|_{L^p([0,1]^d)}
$$
where 
\begin{eqnarray*}
e_H^a(\nabla f\sep z) &:=& \inf_{\nu \in \sP_{m-2}^d} \|\nabla f-\nu\|_{L^p(B_H(z))}\\
% \stext{ and } 
e_H^g(\nabla f\sep z) &:=& \sqrt{\|H(z)\|}\inf_{\nu \in \sP_{m-2}^d} \|H(z)^{-\frac 1 2} (\nabla f-\nu)\|_{L^p(B_H(z))}.
\end{eqnarray*}
Observe that $e_H^a(\nabla f)_p\leq e_H^g(\nabla f)_p$. This inequality, which deteriorates as the metrics $H$ becomes more anisotropic, is the price to pay for the use of graded meshes and metrics instead of quasi-acute ones.

Before turning to the details of these proofs, we establish a common lemma which states that the optimization among all $\nu \in \P_{m-2}^d$ involved in the definition of $e_H^a(f\sep z)_p$ and $e_H^g(f\sep z)_p$ can be replaced with an optimization among gradients of polynomials $\nabla \mu$, where $\mu\in \P_{m-1}$.

\begin{lemma}
\label{lemmaProj}
\begin{itemize}
\item (Orthogonal projection is compatible with gradients)
We equip the space $L^2(B(0,1), \R^d)$ with the scalar product 
$$
\<v,w\> := \int_{B(0,1)} v(z)\cdot w(z) dz.
$$
For any $f\in H^1(B(0,1))$ there exists $\mu\in \P_{m-1}$ such that the orthogonal projection of $\nabla f$ onto $\P_{m-2}^d$ is $\nabla \mu$.
\item (Optimization among gradients)
There exists $C_\proj=C_\proj(m,d)$ such that for any ellipsoid $\cE\subset \R^d$, any $1\leq p \leq \infty$ and any $f\in W^{1,p}(\cE)$ one has  %and any $A\in \GL_d$ 
one has 
\be
\label{eqGradApp}
\inf_{\mu \in \sP_{m-1}} \|\nabla f-\nabla \mu\|_{L^p(\cE)}
\leq 
C_\proj \inf_{\nu \in \sP_{m-2}^d} \|\nabla f-\nu\|_{L^p(\cE)}
\ee
%$$
%\inf_{\mu \in \sP_{m-1}} \|A(\nabla f-\nabla \mu)\|_{L^p(\cE)}
%\leq 
%C_\proj \inf_{\nu \in \sP_{m-2}^d} \|A(\nabla f-\nu)\|_{L^p(\cE)}
%$$
\end{itemize}
\end{lemma}

\proof
\begin{itemize}
\item (Orthogonal projection is compatible with gradients) In order to simplify the notations we define $k := m-1$.
We define $\cS := \{z\in \R^d \sep |z| = 1\}$ and we denote by $D_k$ the collection of polynomial vector fields $\nu\in  \P_{k-1}^d$ satisfying %\subset \P_{k-1}^d
$$
\left\{
\begin{array}{cl}
\diver \nu (z)=0 & \text{ for all } z\in B(0,1)\\
\nu(z) \cdot z = 0 &\text{ for all } z\in \cS
\end{array}
\right.
$$
For any $g\in H^1(B(0,1))$ and any $\nu \in D_k$ we thus have   
\be
\label{eqGradDiv}
\int_{B(0,1)} \nabla g \cdot \nu = -\int_{B(0,1)} g(z) \diver \nu(z)dz + \int_{\cS} g(z)  \, \nu(z) \cdot z \, dz =0.
\ee
%therefore the same holds for the orthogonal projection of $\nabla f$ onto $\P_{k-1}^d$.
Our purpose is now to establish the orthogonal decomposition
$$
\P_{k-1}^d = D_k \oplus \nabla \P_k.
$$
Equation \iref{eqGradDiv} shows that $\nabla \P_k$ and $D_k$ are orthogonal, and we know that $\dim \nabla \P_k = \dim \P_k -1$. Therefore we only have to show that 
$\dim D_k \geq \dim (\P_k^{d-1})  - \dim \P_k +1$.

The vector space $D_k$ is the kernel of the map $d_k$ defined as follows
$$
\begin{array}{ccc}
d_k :\P_{k-1}^d &\to& \P_{k-2} \oplus \P_k(\cS)\\
\nu  &\mapsto & (\diver \nu, \ (\nu (z) \cdot z)_{|\cS}),
\end{array}
$$
where  
$
\P_k(\cS)
$
denotes the collection of restrictions to $\cS$ of elements of $\P_k$. 
The kernel of the map
$$
\begin{array}{ccc}
\gamma_k : \P_k &\to & \P_k(\cS)\\
\mu &\mapsto &\mu_{|\cS}
\end{array}
$$
is 
$
\Ker(\gamma_k) = (1-|z|^2) \P_{k-2}.
$
Hence 
$
\dim(\P_k(\cS)) = \dim \P_k - \dim \P_{k-2}.
$

The map $d_k$ is not surjective, indeed we have the linear relation 
$$
\int_{B(0,1)} \diver \nu(z)\, dz = \int_\cS \nu(z)\cdot z \, dz,
$$
%if $\diver(V) = 0$, then $\int_{\partial E} \<V,\n\> = 0$, 
hence in particular $(0,1) \notin \Image(d_k)$.
Therefore 
\begin{eqnarray*}
\dim D_k &=& \dim \Ker d_k \\
&=& \dim (\P_k^{d-1}) - \dim \Image d_k \\
&\geq &  \dim (\P_k^{d-1}) - (\dim \P_{k-2} + \dim \P_k(\Gamma) -1) \\
&=& \dim (\P_k^{d-1})  - \dim \P_k +1,
\end{eqnarray*}
which implies the orthogonal decomposition $\P_{k-1}^d = D_k \oplus \nabla \P_k$ as announced.

Eventually for any $f\in H^1(B(0,1))$ the equation \iref{eqGradDiv} shows that $\nabla f$ is orthogonal to $D_k$. Therefore the orthogonal projection of $\nabla f$ onto $\P_{k-1}^d$ is also orthogonal to $D_k$, and therefore is an element of $\nabla \P_k$ as announced, which concludes the proof.

\item
We denote by $Q : L^2(B(0,1),\R^d) \to \P_{k-1}^d$ the $L^2(B(0,1))$ orthogonal projection.
We recall that for any $v\in L^2(B(0,1),\R^d)$ the projection $Q(v)\in \P_{k-1}^d$ is defined by the collection of linear conditions
$$
\int_{B(0,1)} (v-Q(v))\cdot \nu  = 0 \text{ for all } \nu \in \P_{k-1}^d.
$$
Hence $Q(v)$ depends linearly on a finite number of moments of $v$, and therefore continuously extends to all $v\in L^1(B(0,1), \R^d)$. Therefore there exists a constant $C_0$ such that for all $1\leq p \leq \infty$ and all $v\in L^p(B(0,1),\R^d)$
$$
\|Q(v)\|_{L^p(B(0,1))} \leq C_0 \|v\|_{L^p(B(0,1))}.
$$
For any $A\in \GL_d$ and any $v\in L^2(B(0,1),\R^d)$ we claim that $Q(A(v)) = A(Q(v))$. Indeed for any $\nu\in \P_{k-1}^d$ one has 
$$
\int_{B(0,1)} (A(v(z))-A(Q(v(z))))\cdot \nu(z) dz= \int_{B(0,1)} (v(z)-Q(v(z))\cdot (A^\trans(\nu(z))) dz = 0.
$$
Consider  $1\leq p \leq \infty$, $f\in W^{1,p}(B)$ and $A\in \GL_d$. Let $\mu\in \P_{m-1}$ be such that $Q(\nabla f) = \nabla \mu$, and let $\nu \in \P_{m-1}^d$, we obtain 
\begin{eqnarray*}
\|A(\nabla f-\nabla \mu)\|_{L^p(B(0,1))} &=& \|A(\nabla f)-A(Q(\nabla f))\|_{L^p(B(0,1))}\\
&=& \|A(\nabla f)-Q(A(\nabla f))\|_{L^p(B(0,1))}\\
& = & \|A(\nabla f-\nu)-Q(A(\nabla f)-\nu)\|_{L^p(B(0,1))}\\
&\leq& (1+C_0)  \|A(\nabla f-\nu)\|_{L^p(B(0,1))}.
\end{eqnarray*}
Therefore 
$$
\inf_{\mu\in \sP_{m-1}} \|A(\nabla f-\nabla \mu)\|_{L^p(B(0,1))} \leq (1+C_0) \inf_{\nu\in \sP_{m-2}^d} \|A(\nabla f-\nu)\|_{L^p(B(0,1))}
$$
We obtain the announced result \iref{eqGradApp} using a change of variables from the ellipse $\cE$ to the ball $B(0,1)$, with the constant $C_\proj := C_0+1$. This concludes the proof of this proposition.\sq
\end{itemize}


\subsubsection{Graded triangulations and metrics} 
\label{subsubsecErrMeshMetW1PG}

The next lemma estimates the $W^{1,p}$ approximation error of a function $f$ on a graded mesh, in terms of the approximation error $e_H^g(\nabla f)_p$ with respect to a metric. This approach does not allow to recover the optimal anisotropic error estimates for $W^{1,p}$ norms developed in Chapter \ref{chapW1P}. However it is perhaps more taylored to current anisotropic mesh generation software, which generally do not guarantee a bound on the angles. 
%Some classical approximation theory results also seem easier to generalise to the anisotropic context using this approach, as illustrated the Sobolev inequality presented in Proposition \ref{propSob}.

\begin{prop}
For all $C_0\geq 1$ there exists $C=C(C_0,m,d)$ such that the following holds. Let $H\in \bH_g$, and let $H' := 4^2 H$, let $\cT\in \bT$ and assume that for all $T\in \cT$ and all $z\in T$
$$
H'(z) \leq \cH_T \leq C_0^2 H'(z).
$$
\begin{itemize}
\item (Local error estimate) 
Let $T\in \cT$ and let $z\in T$, then 
\be
\label{eqLocGW1P}
\|\nabla (f- \interp_\cT^{m-1} f_{H'})\|_{L^p(T)} \leq C e_H^g(\nabla f\sep z)_p.
\ee
\item (Global error estimate)
One has
$$
\|\nabla (f- \interp_\cT^{m-1} f_{H'})\|_{L^p([0,1]^d)} \leq C e_H^g(\nabla f \sep z)_p.
$$
\end{itemize}
\end{prop}

\proof %The proof is extremely similar to the proof of Lemma ??, for the approximation in the $L^p$ norm.

\begin{itemize}
\item
We assume in a first time that $z=0$ and that $H(z) = \Id$, in such way that $B_H(z) = B(0,1)$ is the euclidean unit ball, denoted below by $B := B(0,1)$.
We consider a polynomial $\mu\in \P_{m-1}$ such that 
$
\|\nabla (f-\mu)\|_{L^p(B)}
$
is minimal, and such that $\int_B (f-\mu) = 0$. The latter point can be ensured by adding an appropriate constant to $\mu$. Defining $g:=f-\mu$, we obtain using Lemma \ref{lemmaProj}
$$
\|\nabla g\|_{L^p(B)} \leq C_\proj \,e_H(f\sep z)_p.
$$
%Sobolev Injection's Theorem states that the embedding 
According to Sobolev's injection theorem, recalling $g\in W^{1,1}(B)$ and that $\int_B g=0$, there exists a constant $C_\sob=C_\sob(m,d)$ such that 
$$
\|g\|_{L^1(B)} \leq C_\sob \|\nabla g\|_{L^1(B)}
$$
The function $g_{H'}$, which is continuous on $T$, satisfies 
$$
\|g_{H'}\|_{L^\infty(T)} \leq \|\vp\|_{\infty} \frac{\max_{z'\in T} \|g\|_{L^1(B_{H'}(z'))}}{\min_{z'\in T} |B_{H'}(z')|} \leq C_1 \|g\|_{L^1(B)},
$$
where $C_1 := \|\vp\|_\infty\volBall^{-1} 8^d$. %details? 
We denote by $C_{\interp}$ the norm of the operator defined on the reference equilateral triangle $\nabla \interp_\TEq^{m-1} : C^0(\TEq)\to \P_{m-2}^d$. Thus for any $h\in C^0(\TEq)$
$$
\|\nabla \interp_\TEq^{m-1} h\|_{L^\infty(\TEq)} \leq C_{\interp} \|h\|_{L^\infty(\TEq)}. 
$$
Recalling that $\cH_T^{\frac 1 2}(T)$ is the image $\TEq$ by a translation and a rotation, and using this change of variables, we obtain for the function $g_{H'}\in C^0(T)$
$$
\|\cH_T^{-\frac 1 2}(\nabla \interp_T^{m-1} g_{H'})\|_{L^\infty(T)} \leq C_{\interp} \|g_{H'}\|_{L^\infty(T)}.
$$
Thus 
$$
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)} \leq C_{\interp}\|\cH_T^\frac 1 2\|  \|g_{H'}\|_{L^\infty(T)},
$$
and eventually, since $\cH_T\leq C_0^2 H'(z) = 4^2 C_0^2 \Id$ and since $|T|\leq |B|$,
\begin{eqnarray*}
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq& |B|^\frac 1 p \|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
& \leq & 4C_0 C_{\interp} |B|^\frac 1 p   \|g_{H'}\|_{L^\infty(T)}\\
& \leq & 4C_0 C_1 C_{\interp} |B|^\frac 1 p   \|g\|_{L^1(B)}\\
& \leq & 4C_0 C_1 C_{\interp} C_\sob |B|^\frac 1 p   \|\nabla g\|_{L^1(B)}\\
&\leq &  4C_0 C_1 C_{\interp} C_\sob |B|  \|\nabla g\|_{L^p(B)}\\
\end{eqnarray*}
Defining $C_* := 4C_0 C_1 C_{\interp} C_\sob |B|$ we thus obtain 
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)} &=& \|\nabla (g-\interp_T^{m-1} g)\|_{L^p(T)}\\
&\leq& (1+C_*) \|\nabla g\|_{L^p(B)}\\
&\leq& (1+C_*) C_\proj e_H(\nabla f\sep z)_p
\end{eqnarray*}

We now turn to the general case, and we do not any more assume that $z=0$ and $H(z) =\Id$.
We define the affine change of coordinates $\Phi(z') := H(z)^{-\frac 1 2} z'+z$, and we apply our previous reasonning to the metric $H_\Phi$, the triangle $T_\Phi := \Phi^{-1}(T)$ which is equilateral and centered at the origin, and the function $f_\Phi := f\circ \Phi$.
We thus obtain 
$$
\|\nabla (f_\Phi-\interp_{T_\Phi}^{m-1} f_\Phi)\|_{L^p(T_\Phi)} \leq C e_{H_\Phi}(\nabla f_\Phi \sep 0)_p
$$
where $C := (1+C_*) C_\proj$. It follows that 
$$
\|H(z)^{-\frac 1 2} (\nabla (f-\interp_T^{m-1} f))\|_{L^p(T)} \leq C e_{H}(H(z)^{-\frac 1 2}(\nabla f) \sep z)_p.
$$
which concludes the proof since $\|H(z)\|^\frac 1 2 e_H(H(z)^{-\frac 1 2}(\nabla f) \sep z)_p = e_H^g(f\sep z)_p$.

\item
For any $T\in \cT$ and any $z\in T$,  recalling that $\cH_T\leq C_0^2 H(z) = (4C_0)^2 H(z)$ we obtain 
$$
|\TEq|/|T| =  \sqrt{\det \cH_T} \leq (4C_0)^d  \sqrt{\det H(z)}.
$$
Averaging  \iref{eqLocGW1P} over $T$, it follows that 
$$
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)}^p \leq \frac C {|T|} \int_T e_H^g(f\sep z)_p^p dz \leq C'  \int_T \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz
$$
where $C' := (4C_0)^d C/|\TEq|$.We denote by $\cT_0$ a collection of representatives in $\cT$ for the equivalence relation : $T\sim T'$ if and only if there exists $u\in \Z^d$ such that $T' = u+T$. We thus obtain
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p([0,1]^d)}^p &=& \sum_{T\in \cT_0} \|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)}^p \\
&\leq& C'  \sum_{T\in \cT_0} \int_T \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz\\
&=& C'  \int_{[0,1]^d} \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz
\end{eqnarray*}
which concludes the proof of this proposition.
\sq
\end{itemize}

%The Sobolev approximation error $e_H^g(\nabla f)_q$ dominates the $e_H(f)_p$ when the Sobolev embedding $W^{1,q} \to L^p$ holds. In contrast this property does not hold for $e_H^a(\nabla f)_q$.
%\begin{prop}[Sobolev inequality]
%\label{propSob}
%Consider $1\leq p\leq \infty$, and let $q$ be such that $\frac 1 q := \frac 1 d + \frac 1 p$. Assume that $q\geq 1$ and that the Sobolev injection $W^{1,q} \to L^p$ holds (which excludes the case $p = \infty$). 
%There exists $C = C(m,d,p)$ such that for all $f$,
%$$
%e_H(f)_p \leq C e_H^g(\nabla f)_q
%$$
%\end{prop}
%
%\proof (*review*)
%We denote by $B$ the unit ball of $\R^n$.
%The Sobolev injection theorem yields for all $g\in W^{1,p}(B)$, 
%$$
%\|g-m\|_{L^p(B)} \leq C_0 \|\nabla g\|_{W^{1,q}(B)}
%$$
%where $m$ denotes the average of $g$.
%
%Consider a function $f\in W^{1,q}(B)$. According to (??), $Q^{m-1}_B \nabla f = \nabla \mu$ for some $\mu\in \P_m$. 
%Therefore, denoting by $m$ the average of $f-\mu$ on $B$,
%\begin{eqnarray*}
%\|f-P^m_B f\|_{L^p(B)} &\leq& C_1 \inf_{\nu\in \sP_m} \|f-\nu\|_{L^p(B)} \\
%&\leq& C_1 \|f-\mu-m\|_{L^p(B)} \\
%&\leq& C_0 C_1 \|\nabla (f-\mu)\|_{L^p(B)}\\
%&=& C \| \nabla f-Q^{m-1}_B \nabla f\|_{L^p(B)}.
%\end{eqnarray*}
%where $C = C_0C_1$. 
%Using a linear change of coordinates by $H(z)^{-\frac 1 2}$ we thus obtain %change of variables, thus obtain 
%\begin{eqnarray*}
%\|f-P^m_{B_H(z)} f\|_{L^p(B_H(z))} &\leq& (\det H(z))^{\frac 1 {2d}}  \| H(z)^{-\frac 1 2}(\nabla f-Q^{m-1}_{B_H(z)} \nabla f)\|_{L^p(B_H(z))}\\
%&\leq & \sqrt {\|H\|} \|H(z)^{-\frac 1 2} (\nabla f-Q^{m-1}_{B_H(z)} \nabla f)\|_{L^p(B_H(z))}
%\end{eqnarray*}
%From this point \iref{eqSobInject} immediately follows.
%Note that we used the upper bound $\det H(z) \leq \|H(z)\|^d$, which becomes less and less sharp for anisotropic $H(z)$.
%\sq


\subsubsection{Quasi-acute triangulations and metrics}
\label{subsubsecErrMeshMetW1PA}

It is established in Chapter \ref{chapW1P} that the gradient of the interpolation of a function on a quasi-acute mesh is well behaved. More precisely, there exists a constant $C=C(m,d)$ such that for any simplex $T$ and any $g\in W^{1,\infty}(T)$ one has 
\be
\label{eqGradS}
\|\nabla \interp_T^{m-1} g\|_{L^\infty(T)} \leq C S(T) \|\nabla g\|_{L^\infty(T)}.
\ee
The next lemma establishes a counterpart of this property in the context of metrics : the gradient of the twisted mollification of a function by a quasi-acute metric is also well behaved.
\be
\label{eqGradQA}
\dil_z (f_H)  \leq C \sqrt{\det H(z)} \, \|\nabla f\|_{L^1(B_H(z))}
\ee

%\begin{lemma}[does  not seem to work $\to$ simpler option $H^{-\frac 1 2}$ Lipschitz.]
%%\label{lemmaBoundedQA}
%There exists $C=C(m,d, \vp)$ such that the following holds.
% Let $H\in \bH_a$ be a quasi-acute metric, and let $f\in W^{1,1}_\loc$. Then $f_H\in W^{1,\infty}_\loc$ and for all $z\in \R^d$
%\be
%\label{eqGradQA}
%\dil_z (f_H)  \leq C \sqrt{\det H(z)} \, \|\nabla f\|_{L^1(B_H(z))}
%\ee
%where $\dil_z(f_H) := \lim_{\ve \to 0} \|\nabla f_H\|_{L^\infty(B(z,\ve))}$ is the local dilatation of $f$ at $z$.
%\end{lemma}
%\proof
%We denote by $B_d:= \{z\in \R^d \sep |z|\leq 1\}$ the euclidean unit ball in $\R^d$.
%%$$
%%B_d := \{z\in \R^d \sep |z|\leq 1\}.
%%$$
%%We denote by $B_d
%%For any matrix $A \in \M_{d,d}$ such that $A^\trans A = H^{-1}$ we thus have
%Defining $S(z) := H(z)^{-\frac 1 2}$ we thus have 
%\be
%\label{eqFHS}
%f_H(z) = \int_{B_d} f\left(z- S(z) u\right) \vp(|u|) du.
%\ee
%For any isometry $p\in \cO_{2d,d}$, the transposed map $p^\trans : B_{2d}\to B_d$ transports the Lebesgue measure on $B_{2d}$ onto a measure on $B_d$, proportional to the Lebesgue density by a radial factor $\mu(|\cdot|)$ which is independent of $p$. Indeed $p^\trans : B_{2d}\to B_d$ is simply the projection onto the $d$ first coordinates, in an appropriate orthogonal basis of $\R^{2d}$.
%We thus have for any $g\in L^1(B_d)$ and any $p\in \cO_{2d,d}$
%\be
%\label{eqChg2dd}
%\int_{B_d} g(u) \mu(|u|) du= \int_{B_{2d}} g(p^\trans v) dv.
%\ee
%For any matrix $A \in \M_{2d,d}$ such that $A^\trans A = H(z)^{-1}$, there exists an isometry $p\in \cO_{2d,d}$ such that 
%$
%A = pS(z).
%$
%Applying \iref{eqChg2dd} to the function 
%$$
%g(u) := f(z-S(z) u) \frac{\vp(|u|)}{\mu(|u|)}
%$$
%and recalling \iref{eqFHS} we obtain
%\begin{eqnarray*}
%f_H(z) = \int_{B_d} g(u) \mu(|u|) du = \int_{B_{2d}} g(p^\trans v) dv = \int_{B_{2d}} g(z-S(z)p^\trans v) \, \frac{\vp(|p^\trans v|)}{ \mu(|p^\trans v|)} dv
%\end{eqnarray*}
%%$$
%%g^H(z) = \int_{B_{2d}} g(z-S(z)p^\trans v) \, \vp(|p^\trans v|) \, \mu(|v|) dv
%%$$
%Therefore, for any $z'\in \R^d$ and any $A,B\in M_{2d,d}$ such that $A^\trans A = H(z)^{-1}$ and $B^\trans B = H(z')^{-1}$ we obtain 
%$$
%f_H(z) - f_H(z') = \int_{B_{2d}} (f(z-A^\trans v)-f(z-B^\trans v)) \frac{ \vp(|p^\trans v|)}{ \mu(|p^\trans v|)} dv.
%$$
%Hence 
%$$
%|f_H(z)-f_H(z')| \leq C \int_{B_{2d}} |f(z-A^\trans v)-f(z-B^\trans v)|  dv.
%$$
%where
%$$
%C := \sup_{r\geq 0} \frac{|\vp(r)|}{\mu(r)}.
%$$
%Note that $C$ is finite since $\supp(\vp) \subset [0,1)$, hence since the support of a function is always a closed set  $\supp(\vp) \subset [0,r_0]$ for some $0\leq r_0<1$, and since $\mu$ is positive on $[0,1)$. Since $H\in \bH_a$ there the matrices $A,B\in M_{2d,d}$ satisfying $A^\trans A = H(z)^{-1}$ and $B^\trans B = H(z')^{-1}$ can be chosen in such way that $|A-B| \leq |z-z'|$.
%%We denote $\delta := |z-z'|$, and we choose the matrices $A,B$ in such way that $\|B-A\|\leq \delta$.
%We thus have for any $v\in B_{2d}$
%$$
%|(z-A^\trans v) - (z'-B^\trans v)|\leq |z-z'|+|(A-B)^\trans v| \leq 2 |z-z'|
%$$
%and therefore
%\begin{eqnarray*}
%|f_H(z)-f_H(z')| &\leq& C \int_{B_{2d}} 2 |z-z'| \dil(f_{|B(z+A^\trans v, 2|z-z'|)}) dv \\ %\dil_{z+A^\trans v}(g\sep 2 |z-z'|) dv\\
%&=& 2C |z-z'| \sqrt{\det H(z)} \int_{B(z,H)} \dil(f_{B(z+u , 2 |z-z'|)}) \mu(|u|) du%\dil_{z+u}(g\sep 2 ) dv
%\end{eqnarray*}
%We assume in the next equations that $g\in C^1_\per$, in such way that $\dil_z(g,\ve)$ tends uniformly to $\dil_z(g)$ as $\ve \to 0$. Therefore
%\begin{eqnarray*}
%\dil_{z_0}(g^H) &:=& \lim_{\ve\to 0} \sup_{z,z'\in B(z_0, \ve)} \frac{|g^H(z)-g^H(z')|}{|z-z'|}\\
%&\leq & \lim_{\ve \to 0} \sup_{z\in B(z_0, \ve)} 2C  \sqrt{\det H(z)} \int_{B(z,H)} \dil_{z+u}(g\sep 2 \times 2 \ve) dv\\
%&=& 2 C \sqrt{\det H(z_0)} \int_{B(z_0,H)} |\nabla g(z_0+u)| dv.
%\end{eqnarray*}
%
%By density of $C^1_\per$ in $W^{1,1}_\per$ we obtain that $L_H$ defines a bounded operator $W^{1,1}\to W^{1,\infty}$ with norm
%$$
%\|L_H\|_{W^{1,1}\to W^{1, \infty}} \leq 2C \max_{z_0} \sqrt{\det H(z_0)}
%$$
%The left and right hand side of \iref{eqDilInt} are thus continuous functions of $g\in W^{1,1}_\per$. Since the inequality holds for all $g\in C^1_\per$ it holds by continuity for all $g\in W^{1,1}_\per$.
%
%\sq

\begin{lemma}
There exists $C=C(m,d)$ such that the following holds. Let $H\in \bH_a$, and let $H' := 4^2 H$.
\begin{itemize}
\item (Local error estimate) 
Let $\cT\in \bT$, let $z\in \R^d$, let 
$
\cT_z := \{T\in \cT \sep T \subset B_{H'}(z,2)\}
$
and let $\Omega_z$ be the union of all triangles in $\cT_z$.
Then for any $f\in W^{1,p}_\loc$
\be
\label{eqLocFA}
\|\nabla( f-\interp_\cT^{m-1} f_{H'})\|_{L^p(\Omega_z)} \leq C e_H^a(f\sep z)_p \max_{T\in \cT_z} S(T).
\ee

%and $S(T)\leq S_0$ for all $T\in \cT_z$ then 
%Let $T$ be a simplex let $z\in T$, and assume that $\cH_T \geq H'(z)$.
%
%For any $f\in L^p_\loc$ one has 
%$$
%\|f-\interp_T^{m-1} f_{H'}\|_{L^p} \leq C e_H(f\sep z)_p,
%$$
%where $C=C(m,d)$. ($C$ is independent of $H$, $T$ and $f$.)
\item (Global error estimate)
Let $\cT\in \bT_\per$ and assume that for all $T\in \cT$ and all $z\in \cT$ one has 
$
\cH_T \geq H'(z).
$
Then for any $f\in W^{1,p}_\per$
\be
\label{eqGloFA}
\|\nabla (f-\interp_\cT^{m-1} f_{H'})\|_{L^p([0,1]^d)} \leq C e_H^a(f \sep z) \max_{T\in \cT} S(T).
\ee
\end{itemize}
\end{lemma}

\proof The proof is extremely similar to the proof of Proposition \ref{propErrMeshMet}, for the approximation in the $L^p$ norm.

\begin{itemize}
\item
%We define $S_z:= \max \{S(T) \sep T \in \cT_z\}$, in such way that  and we obtain for all $T\in \cT_z$
%We recall that there exists a constant $C_a = C_a(m,d)$ such that for any simplex $T$ and any $g\in W^{1,\infty}(T)$ one has
%$$
%\|\nabla \interp_T^{m-1} g\|_{L^\infty(T)} \leq C_a\, S(T) \,  \|\nabla g\|_{L^\infty(T)}. 
%$$
%We define $S_z:= \max \{S(T) \sep T \in \cT_z\}$.
%The proof is nearly identical to the proof of Lemma ??, where $C_{\interp}$ is replaced with $C_a S_z$ and $\|\vp\|_{L^\infty}$ with $C_\vp$.

%We denote by $C_{\interp,g}$ the norm of the interpolation operator $\nabla \interp_\TEq^{m-1} : C^0(\TEq) \to C^0(\TEq)$. We recall that for any simplex $T$, the simplex $\cH_T^{-\frac 1 2}(T)$ is the image of the reference equilateral simplex $\TEq$ by a rotation and a translation. It follows that 
%%, and we observe using the change of variables that for any triangle $T$ and any $g\in C^0(T)$ one has 
%$$
%\|\cH_T^{-\frac 1 2} (\nabla \interp_T^{m-1} g)\|_{L^\infty(T)}\leq C_{\interp} \|\cH_T^{-\frac 1 2}(\nabla g)\|_{L^\infty(T)}.
%$$
%We define $C_{\interp a} := C_a \max\{S(T) \sep T \in \cT_z\}$.
We denote by $C_a$ the constant appearing in \iref{eqGradS}, and by $C_\vp$ the constant appearing in \iref{eqGradQA}.

Let $\mu\in \P_{m-1}$ be a polynomial satisfying $\|\nabla (f-\mu)\|_{L^p(B_H(z))} \leq C_\proj e_H^a(\nabla f\sep z)_p$.
Let $g := f-\mu$ and let $T\in \cT_z$.
We have 
\begin{eqnarray*}
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq & |T|^\frac 1 p \|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
&\leq & C_a S(T) |T|^\frac 1 p \|\nabla g_{H'}\|_{L^\infty(T)}\\
&\leq & C_a S(T) |T|^\frac 1 p \|\nabla g_{H'}\|_{L^\infty(B_{H'}(z,2))}\\
&\leq & C_a S(T) C_\vp |T|^\frac 1 p \max_{z'\in B_{H'}(z,2)}  \frac{\|\nabla g\|_{L^1(B_{H'}(z'))}}{|B_{H'}(z')|}\\
&\leq & 8^dC_a S(T) C_\vp  |T|^\frac 1 p \frac{\|\nabla g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|}.
\end{eqnarray*}
Denoting $C_* := 8^dC_a C_\vp$ and $S_z := \max\{S(T) \sep T\in \cT_z\}$ we obtain as in \iref{propErrMeshMet}
%Therefore as previously 
\begin{eqnarray*}
\|\nabla \interp_\cT^{m-1} g_{H'}\|_{L^p(\Omega_z)} %&=& \left(\sum_{T\in \cT_z} \|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)}^p \right)^{\frac 1 p} \\
%&\leq & C_* S_z \frac{\|\nabla g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|} \left(\sum_{T\in \cT_z} |T|\right)^\frac 1 p\\
%& \leq & C_* S_z  \|\nabla g\|_{L^1(B_{H}(z))}|B_{H}(z)|^{1-\frac 1 p}\\
& \leq & C_* S_z  \|\nabla g\|_{L^p(B_{H}(z))}
\end{eqnarray*}

Eventually we obtain 
\begin{eqnarray*}
\|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p(\Omega_z)} &=& \|\nabla (g-\interp_\cT^{m-1} g_H)\|_{L^p(\Omega_z)} \\
&\leq &\|\nabla g\|_{L^p(\Omega_z)}+ \|\nabla \interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)}\\
& \leq & (1+C_*S_z) \|\nabla g\|_{L^p(B_{H}(z))}\\
&\leq & (1+C_* S_z) C_\proj e_H(\nabla f\sep z)_p
\end{eqnarray*}
which concludes the proof of \iref{eqLocFA}.

\item
This proof \iref{eqGloFA} is nearly identical to the proof of the second point of Proposition \ref{propErrMeshMet}, and details are left to the reader.
%We define $S_\cT$ and we proceed identically to identical to Lemma ??.
%
%For each triangle $T\in \cT$ we define 
%$$
%\Omega_T := \{z\in \R^d \sep T \subset B_{H'}(z,2)\} \stext{ and } n(T) := \int_{\Omega_T} \sqrt{\det H(z)} dz.
%$$
%It follows from Lemma ?? that $n_T \geq ??$.
%
%We denote by $\cT_*$ a system of representatives of $\cT$ for the equivalence relation 
%$$
%T \sim T' \stext{ if } T =T'+u \text{ for some } u \in \Z^d.
%$$
%We therefore obtain 
%\begin{eqnarray*}
%e_H(\nabla f)_p^p &=& \int_{z\in [0,1]^d} \sqrt{\det H(z)} \, e_H(\nabla f\sep z)_p^p dz\\
%&\geq& (CS_\cT)^{-p} \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p(\Omega_z)}^p dz \\
%&=& (CS_\cT)^{-p} \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \sum_{T\in \cT_z} \|\nabla(f-\interp_\cT^{m-1} f_H)\|_{L^p(T)}^p dz \\
%&=& (CS_\cT)^{-p}\sum_{T\in \cT_*} n_T \|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p(T)}^p \\
%& \geq & (CS_\cT)^{-p} \|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p([0,1]^d)}^p \min_{T \in \cT} n_T.
%\end{eqnarray*}
\sq
\end{itemize}


\subsection{Existence of an optimal metric for smooth functions}
\label{subsecExistsMetW1P}

We construct in this subsection a metric adapted to the approximation of a sufficiently smooth function, when a sufficiently large mass of the metric is authorized. Our method is similar to the proof of the analogous results in the case of the $L^p$ norm, and requires in particular to solve an optimization problem at each point.
We then focus on the more specific case of piecewise linear an piecewise quadratic approximation in two dimensions, and we give an explicit expression of the metric in terms of the the derivatives of the approximated function.

\subsubsection{A well posed variant of the shape function} 
\paragraph{Quasi-acute metrics.\\}

The shape function $L_a$, associated to quasi-acute metrics and triangulations for finite element approximation in the $W^{1,p}$ norm, is defined as follows
$$
L_a(\pi) := \inf_{A\in \SL_d} \|(\nabla \pi) \circ A\| = \inf\{(\det M)^{\frac{m-1}{2d }} \sep \|(\nabla \pi) \circ M^{-\frac 1 2}\| \leq 1 \}.
$$
For each $\pi\in \H_m$ we denote by $G(\pi)\in \H_{2m-2}$ the squared norm of the gradient of $\pi$
$$
G(\pi) := |\nabla \pi|^2 = \sum_{1\leq i \leq d} \left(\frac{\partial\pi}{\partial x_i}\right)^2.
$$
We thus obtain  
\be
\label{eqLK}
L_a(\pi) = \inf_{A\in \SL_d} \sqrt{\|G(\pi) \circ A\|} =\sqrt{K'( G(\pi))}, 
\ee
where $K' : \H_{2m-2} \to \R_+$ refers to the shape function previously studied in the context of the $L^p$ norm, but applied to polynomials of degree $2m-2$ instead of $m$: 
for all $\Pi \in \H_{2m-2}$, 
$$
K'(\Pi) := \inf \{\|\Pi\circ A\| \sep A\in \SL_d\} = \inf\{(\det M)^{\frac{2m-2}{2d}} \sep \|\Pi \circ M^{-\frac 1 2}\|\leq 1\}.
$$

Our results developed for the shape function $K$ in \S \ref{subsecExistsMetLP} therefore extend in a straightforward manner to the shape function $L_a$. %, and we obtain the following
\begin{prop}
\label{propLALA}
For each $\alpha\in (0, \infty)$ define $L_a^{(\alpha)} : \H_m \to \R_+$ as follows
$$
L_a^{(\alpha)}(\pi) :=  \inf\{\kappa(M)^\frac 1 \alpha (\det M)^{\frac{m-1}{2d }} \sep \|G(\pi) \circ M^{-\frac 1 2} \|_{\sC} \leq 1 \text{ and } \kappa(M) \leq e^\alpha \}.
$$
%\begin{itemize}
%\item (Existence of a minimizer)
For each $\pi\in \H_m\sm \{0\}$ the minimum defining $L_a^{(\alpha)}(\pi)$ is attained for an unique matrix $\cM_a^{(\alpha)}(\pi)$, and depends continuously on $\pi$.
%\end{itemize}
\end{prop}
\proof
This proposition is a direct consequence of Proposition \ref{propContLift}.
\sq
The functions $L^{(\alpha)}_a$ converge pointwise decreasingly to the function 
$$
L_{a, \sC} := \inf_{A\in \SL_d} \sqrt{\|G(\pi) \circ A\|_\sC}
$$
which is equivalent to $L_a$. This property is sufficient for our analysis, but we find it worthwhile nevertheless to mention a few additional properties of $L_a$.
\begin{prop}
There exists $C = C(m,d)$ such that the following holds.
\begin{itemize}
\item (Equivalence to a continuous function)
There exists a continuous function $L_{a,c} : \H_m \to \R_+$ such that for all $\pi\in \H_m$
$$
C^{-1}L_{a,c} \leq L_a \leq C L_{a,c}.
$$
\item (Convergence to the unconstrained problem)
For all $\ve>0$ there exists $\alpha$ such that for all $\pi \in \H_m$
$$
L_a^{(\alpha)}(\pi) \leq C L_a(\pi) + \ve \|\pi\|.
$$
\end{itemize}
\end{prop}
\proof
These results are a direct consequence of \iref{eqLK} and Proposition \ref{lemmaKAK}.
\sq

\paragraph{Graded metrics}
The shape function $L_g$ associated to graded metrics and triangulations for finite element approximation in the $W^{1,p}$ norm, is defined as follows
$$
L_g(\pi) := \inf_{A\in \SL_d} \|A^{-1}\| \|\nabla (\pi\circ A)\| = \inf \{(\det M)^{\frac{m-1} {2d}} \sep \|M\|^{\frac 1 2} \| \nabla (\pi \circ M^{-\frac 1 2})\|\leq 1\}.
$$
The next proposition introduces a variant of the shape function $L_g$, which is defined by a well posed optimization problem.
%Similarly to the other shape functions $K$ and $L_a$, the next proposition 
%Our results developed for the shape function $K$ in \S \ref{subsecExistsMetLP} therefore extend in a straightforward manner to the shape function $L_a$. %, and we obtain the following
\begin{prop}
\label{propLALG}
For each $\alpha\in (0, \infty)$ define $L_g^{(\alpha)} : \H_m \to \R_+$ as follows
$$
L_g^{(\alpha)}(\pi) := \inf\{\kappa(M)^\frac 1 \alpha (\det M)^\frac{m-1}{2d} \sep \sqrt{\|M\|} \|\pi\circ M^{-\frac 1 2}\|_\sC \leq 1 \text{ and } \kappa(M) \leq e^\alpha\}.
$$
For each $\pi\in \H_m\sm \{0\}$ the minimum defining $L_g^{(\alpha)}(\pi)$ is attained for an unique matrix $\cM_a^{(\alpha)}(\pi)$, and depends continuously on $\pi$.
\end{prop}
\proof
This proposition is a direct consequence of Proposition \ref{propContLift}.
\sq
The functions $L^{(\alpha)}_g$ converge pointwise decreasingly to the function 
$$
L_{g, \sC} := \inf_{A\in \SL_d} \sqrt{\|A^{-1}\|} \|\pi\circ A\|_\sC
$$
which is equivalent to $L_g$. Indeed there exists a constant $C$ such that $
C^{-1} \|\pi\|_\sC\leq \|\nabla \pi\|\leq C\|\pi \|_\sC
$ for all $\pi\in \H_m$, since these two quantities are norms on $\H_m$.
This property is sufficient for our analysis, but we find it worthwhile nevertheless to mention a few additional properties of $L_g$.
\begin{prop}
\label{propLGCont}
There exists $C = C(m,d)$ such that the following holds.
\begin{itemize}
\item (Equivalence to a continuous function)
There exists a continuous function $L_{g,c} : \H_m \to \R_+$ such that for all $\pi\in \H_m$
$$
C^{-1}L_{g,c} \leq L_a \leq C L_{g,c}.
$$
\item (Convergence to the unconstrained problem)
For all $\ve>0$ there exists $\alpha$ such that for all $\pi \in \H_m$
$$
L_g^{(\alpha)}(\pi) \leq C L_g(\pi) + \ve \|\pi\|.
$$
\end{itemize}
\end{prop}
\proof
The key property is to establish that the upper semi continuous function $L_g$ is equivalent to its lower semi continuous envelope $\underline L_g$, as established in Lemma \ref{lemmaLGSemi} belov. From this point to equivalence to a continuous function and the convergence to the unconstrained problem are obtained proceeding exactly as in Proposition \ref{lemmaKAK}.
\sq

The next lemma is the key technical ingredient to the proof of Proposition  \ref{propLGCont} above.
\begin{lemma}
\label{lemmaLGSemi}
Denote by $\underline L_g$ the lower semi continuous envelope of $L_g$, which is defined as follows 
$$
\underline L_g(\pi) := \liminf_{\pi'\to \pi} L_g(\pi') = \lim_{\ve \to 0} \inf_{\|\pi'-\pi\|\leq \ve} L_g(\pi'). 
$$
There exists a constant $C_\lsc = C_\lsc(m,d)$ such that $L_g \leq C_\lsc \underline L_g$ on $\H_m$.
%for all $\pi\in \H_m$
%$$
%L_g(\pi) \leq C \underline L_g(\pi).
%$$
\end{lemma}

\proof
This proof is extremely similar to the proof the analog property for the shape function $K$ in point 2. of Lemma \ref{lemmaKAK}, but nevertheless we need to introduce an intermediate : a variant  variant $\gL$ of the shape function $L_g$.
%We apply the same method to a variant $\gL$ of the shape function $L_g$.
%Nevertheless the same method cannot be directly applied we need to introduce an intermediate : the shape Yet the same method cannot be directly applied

\paragraph{A variant $\gL$ of the shape function $L_g$\\}
We define an auxiliary function $\gL$ on $M_d \times \H_m$ as follows 
\be
\label{defgL}
\gL(B,\pi) := \inf_{A\in \SL_d} \|A^{-1}B\| \|\pi\circ A\|.
\ee
We denote by $C_0$ a constant such that
$
C_0^{-1} \|\pi\|\leq \|\nabla \pi\| \leq C_0 \|\pi\|
$
for all $\pi \in \H_m$,
%Observing that 
%$$
%L_g(\pi) = \inf \{\|A\| \|\nabla(\pi\circ A^{-1})\| \sep |\det A| = 1\}
%$$
we obtain  
\be
\label{eqGLL}
C_0^{-1} L_g(\pi) \leq \gL(\Id, \pi) \leq C_0 L_g(\pi).
\ee
Taking the lower limit of the previous inequality as $(B', \pi') \to (\Id, \pi)$ we obtain 
\be
\label{eqGLLInf}
C_0^{-1} \underline L_g(\pi) \leq \underline \gL(\Id, \pi) \leq C_0 \underline L_g(\pi).
\ee
We establish below that there exists $C$ such that $\gL \leq C \underline \gL$ on $M_d \times \H_m$. Combining this point with \iref{eqGLL} and \iref{eqGLLInf} yields the announced result.

\paragraph{Vanishing of $\gL$\\}

Consider a converging sequence $(B_n, \pi_n) \to (B,\pi)$ in $M_d \times \H_m$. We establish in this paragraph that following property : 
$$
\text{ if } \lim_{n \to \infty} \gL(B_n, \pi_n)=0 \stext{ then } \gL(B, \pi) = 0.
$$
If $\gL(B_n, \pi_n) \to 0$ then there exists a sequence $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, such that 
\be
\label{eqAnBnPin}
\lim_{n \to \infty} \|A_n^{-1} B_n\| \|\pi_n\circ A_n\| =0.
\ee
For each $n$ consider the principal value decomposition $A_n = U_n D_n V_n$, where $U_n, V_n \in \cO_d$ and $D_n$ is a diagonal matrix satisfying $\det D_n = 1$, with positive %and decreasing 
diagonal coefficients $t_n = (t_{n,1}, \cdots, t_{n,d})$.
% where 
%\be
%\label{eqtni}
%t_{n,1} \geq \cdots \geq t_{n,d}>0.
%\ee
We have for any $n \geq 0$, since $U_n$ is orthogonal,
$$
\|A_n^{-1} B_n \| \|\pi\circ A_n\| = \| V_n^\trans D_n^{-1} U_n^\trans B_n \| \|\pi\circ (U_n D_n V_n)\| = \|D_n^{-1} U_n^\trans B_n \| \|\pi\circ (U_n D_n)\|.
$$
Since the collection $\cO_d$ of orthogonal matrices is compact, the sequence of orthogonal matrices $V_n$ admits a converging sub-sequence $V_{\vp(n)} \to V$. We define $B' := U^\trans B$, $\pi' := \pi \circ U$, and we observe that
\be
\label{eqgLBPip}
\cL(B, \pi) = \cL(B', \pi').
\ee
We also define
$$
B'_n := U_{\vp(n)}^\trans B_{\vp(n)}, \quad  \pi'_n := \pi_{\vp(n)} \circ U_{\vp(n)}, \stext{ and } D'_n := D_{\vp(n)}
$$
in such way that 
\be
\label{eqBpPip}
\lim_{n \to \infty} (B'_n,\pi'_n) = (B',\pi') \stext{ and } \lim_{n \to \infty} \|D'^{-1}_n B'_n\| \|\pi'_n\circ D'_n\| = 0.
\ee
We thus recognise \iref{eqAnBnPin} except that the matrices $A_n$ are replaced with diagonal matrices $D'_n$ with their diagonal coefficients 
$$
t'_n := (t'_{n,1}, \cdots , t'_{n,d}) =  (t_{\vp(n),1}, \cdots , t_{\vp(n),d}) 
$$
ordered decreasingly. In order to avoid notational clutter we do not keep track of the sub-sequence extraction, and we simply write $\pi$, $\pi_n$, $B$, $B_n$, $D_n$, $t_n$ and $t_{n,i}$ instead of $\pi'$, $\pi_n'$, $B'$, $B_n'$, $D'_n$, $t_n'$ and $t_{n,i}'$.

We denote by $I\subset \{1, \cdots, d\}$ the collection of indices $i$ such that the associated line of $B$ is nonzero. There exists a constant $c>0$ such that for %all $n \geq 0$
%$$
%\|D_n B\| \leq C t_{n,i_0}
%$$
%and for 
all $n$ sufficiently large
\be
\label{eqDnB}
\|D_n^{-1} B_n\| \geq c \max_{i\in I} t_{n,i}^{-1}.
\ee
We denote by $\Lambda$ the collection of exponents
$$
\Lambda := \{\alpha\in \Z_+^d \sep |\alpha| \leq m\}
$$
and by $\pi_\alpha$, $\pi_{n,\alpha}$ the coefficients of $\pi$ and $\pi_n$ respectively, in such way that 
$$
\pi = \sum_{\alpha \in \Lambda} \pi_\alpha Z^\alpha \stext{ and } \pi_n = \sum_{\alpha\in \Lambda} \pi_{n, \alpha} Z^\alpha.
$$
It follows from \iref{eqBpPip} and \iref{eqDnB} that for any $\alpha\in \Lambda$ we have 
\be
\label{eqTnPin}
\lim_{n \to \infty} \left(\max_{i\in I} t_{n,i}^{-1}\right) \pi_{n, \alpha} t_n^\alpha = 0.
\ee
For each $t = (t_1, \cdots , t_d)\in \R_+^d$ we define 
$$
\Lambda(t) := \left\{\alpha\in \Lambda \sep\left(\max_{i\in I} t_{n,i}^{-1}\right) t_n^{\alpha} \geq 1\right\}.
$$
The set $\Lambda$, which is finite, has only a finite number of subsets. Hence there exists an extraction $\psi$ such that $\Lambda_* := \Lambda(t_\psi(n))$ does not depend on $n$. In view of \iref{eqTnPin} we thus have for all $\alpha\in \Lambda_*$
$$
\pi_\alpha = \lim_{n \to \infty} \pi_{n, \alpha} = 0. %\text{ for all } \alpha\in \Lambda_*. 
$$
Defining $D := D_{\psi(0)}$, and denoting by $t=(t_1, \cdots ,t_d)$, its diagonal coefficients we thus obtain 
$$
\lim_{n \to \infty} \|D^{-n} B\| \|\pi\circ D^n\| = 0. 
$$
Indeed $\|D^{-n} B\|\leq C \max_{i\in I}t_i^{-n}$ and 
$$
\left( \max_{i\in I}t_i^{-n}\right) \pi_\alpha t^{n\alpha} =  \pi_\alpha \left(t^{\alpha} \max_{i\in I}t_i^{-1}\right)^n
$$
equals $0$ if $\alpha\in \Lambda_*$, and tends to zero if $\alpha\in \Lambda\sm\Lambda_*$. It follows that $\gL(B,\pi) = 0$ as announced.

\paragraph{Lower semi-continuity\\}
We denote by $\cA$ the following compact subset of $M_d\times \H_m$
$$
\cA := \{(B,\pi) \in M_d \times \H_m \sep \|B\|=\|\pi\| = 1 \text{ and for all } A\in \GL_d \text{ one has } \|A^{-1}B\| \|\pi\circ A\|\geq 1\}.
$$

Clearly $\gL(B,\pi) = 1$ for all $(B, \pi)\in \cA$, therefore $\underline \gL$ does not vanish on $\cA$. Since $\underline \gL$ is lower semi continuous, it attains its minimum on $\cA$, we thus define 
$$
C^{-1} := \inf_\cA \underline \gL.
$$
Consider $(B, \pi) \in M_d \times \H_m$, and denote by $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, a minimizing sequence for the problem defining $\gL(B, \pi)$
\be
\label{eqAngLMin}
\lim_{n \to \infty} \|A_n^{-1} B \| \|\pi \circ A_n\| = \gL(B, \pi) = \inf_{A\in \SL_d} \|A^{-1} B \| \|\pi \circ A\|.
\ee
If $\gL(B, \pi) = 0$, then $\underline \gL(B, \pi)=0$ and there is nothing to prove. If $\gL(B, \pi)>0$, then consider an extraction $\vp$ such that the following quantities converge
$$
\lim_{n \to \infty} \frac{A_{\vp(n)}^{-1} B}{\|A_{\vp(n)}^{-1} B\|} = B_* \stext{ and } \lim_{n \to \infty} \frac{\pi\circ A_{\vp(n)}}{\|\pi\circ A_{\vp(n)}\|} = \pi_*.
$$

We now prove that $(B_*, \pi_*)\in \cA$.
Indeed $\|B_*\| = \|\pi_*\|=1$ by construction. Assume for contradiction that there exists $A\in \GL_d$ such that $\|A^{-1} B_*\|\|\pi_*\circ A\| = \delta <1$. We obtain 
\begin{eqnarray*}
& &\lim_{n \to \infty}  \|(A_{\vp(n)} A)^{-1} B \| \|\pi \circ (A_{\vp(n)} A)\| \\
&=& \lim_{n \to \infty} \|A_{\vp(n)}^{-1} B \| \|\pi\circ A_{\vp(n)}\| \frac {\|A^{-1}(A_{\vp(n)}^{-1} B) \|}{\|A_{\vp(n)}^{-1} B \|} \frac { \|(\pi\circ A_{\vp(n)})\circ A\|}{\|\pi\circ A_{\vp(n)}\|} \\
&=& \delta \gL(B, \pi)
\end{eqnarray*}
%$$
%\lim_{n \to \infty}  \|(A_{\vp(n)} A)^{-1} B \| \|\pi \circ (A_{\vp(n)} A)\| = \lim_{n \to \infty} \|A_{\vp(n)}^{-1} B \| \|\pi\circ A_{\vp(n)}\| \frac {\|A^{-1}(A_{\vp(n)}^{-1} B) \|}{\|A_{\vp(n)}^{-1} B \|} \frac { \|(\pi\circ A_{\vp(n)})\circ A\|}{\|\pi\circ A_{\vp(n)}\|} = \delta \gL(B, \pi)
%$$
which is a contradiction with the definition \iref{defgL} of $\gL$, hence $(B_*, \pi_*)\in \cA$ as announced.

Observe that  
\be
\label{eqLuLRatio}
\underline \gL\left(\frac{A_n^{-1} B}{\|A_n^{-1} B\|} \frac{\pi\circ A_n}{\|\pi\circ A_n\|}\right) = \frac{\underline \gL(B,\pi) }{\|A_n^{-1} B\|\|\pi\circ A_n\|} \ \underset {n \to \infty}  \longrightarrow \ \frac{\underline \gL(B,\pi)}{\gL(B,\pi)}
\ee
Since $\underline \gL$ is lower semi continuous and $(B_*, \pi_*)\in \cA$ we obtain
$$
\lim_{n \to \infty} \underline \gL\left(\frac{A_n^{-1} B}{\|A_n^{-1} B\|} \frac{\pi\circ A_n}{\|\pi\circ A_n\|}\right) \geq  \underline \gL(B_*, \pi_*) \geq C^{-1}.
$$
Combining this with \iref{eqLuLRatio} yields $\underline \gL(B,\pi) \geq \gL(B, \pi)$, which concludes the proof of this lemma.
\sq

\subsubsection{The metric}

We consider a function $f\in C^m_\per(\R^d)$ and we define for all $z\in \R^d$ the polynomials $\pi_z\in \H_m$ and $\mu_z\in \P_{m-1}$ as before, see \iref{defPizLpMet} and \iref{defMuzLpMet}.
%$$
%\frac{\pi_z}{m!} := \sum_{|\alpha| = m} \frac{\partial^m f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!},
%$$
%and $\mu_z\in \P_{m-1}$
%$$
%\mu_z := \sum_{|\alpha| < m} \frac{\partial^{|\alpha|} f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!}.
%$$
The Taylor development of $\nabla f$ close to a point $z\in \R^d$ is obtained by taking the gradient of the Taylor development of $f$ : 
$$
\nabla f(z+h) = \nabla \mu_z(h) + \nabla \pi_z(h) + o_z(|h|^{m-1}).
$$
The Taylor formula for the function $\nabla f : \R^d \to \R^d$ reads as follows 
\be
\label{defTaylorGrad}
\nabla f(z+h) - \nabla \mu_z(h) = (m-1)\int_0^1 \nabla \pi_{z+th}(h) (1-t)^{m-2} dt.
\ee
The previous analysis for the $L^p$ error $e_H(f)_p$ of a function $f$ with respect to a metric $H$, is easily extended to the $W^{1,p}$ errors $e_H^a(\nabla f)_p$ and $e_H^g(\nabla f)_p$.
Indeed this analysis is simply based on Taylor developments and on the properties of the shape function $K
$ exposed in Proposition \ref{lemmaKAK}. These properties are extended to the shape functions $L_a$ and $L_g$ in  Propositions \ref{propLALA} and \ref{propLALG} respectively.

Similarly to the $L^p$ norm, the key idea produce a metric of the form 
$$
H_\star := \Lambda (\det M_\star)^\frac{-1}{(m-1)p+d} M_\star %or \frac{-\tau}{dp}
$$
where $\star\in \{g,a\}$, and $M_\star$ as the form 
$$
M_\star(z) := \psi_{\ve_2}*(\cM^{(\alpha)}(\pi_z)+\ve_1\Id),
$$
where $\alpha$ is sufficiently large, $\ve_1$ is sufficiently small, $\psi$ is a mollifier and $\ve_2$ is sufficiently small, and eventually $\Lambda$ is sufficiently large. Except for the technical point presented in Lemma \ref{lemmaLGAdd}, we refer the reader to the case of the $L^p$ norm \S\ref{subsubsecExplicitMetricLP} for more details.


\begin{lemma}
\label{lemmaLGAdd}
Let $\pi\in \H_m$, let $M\in S_d^+$ and let $\alpha>0$. Then
\be
\label{eqMMALG}
\sqrt{\|M+\alpha\Id\|}\|\nabla (\pi\circ (M+\alpha\Id)^{-\frac 1 2})\| \leq \sqrt{\|M\|}\|\nabla (\pi\circ M^{-\frac 1 2})\|
%\text{If } \|M\|^\frac 1 2 \|\pi\circ M^{-\frac 1 2}\| \leq 1 \text{ then } \|M'\|^\frac 1 2 \|\pi\circ M'^{-\frac 1 2}\| \leq 1
\ee
\end{lemma}
\proof
We have for any $z\neq 0$
$$
\frac{\|M+ \alpha\Id\|}{\|M\|} = 1+ \frac\alpha{\|M\|} \leq 1+\frac{\alpha |z|^2}{\|z\|_M^2} = \frac{\|z\|_{M+\alpha\Id}^2}{\|z\|_M^2}.
$$
Furthermore $|(M+\alpha\Id)^{-\frac 1 2} u| \leq |M^{-\frac 1 2} u|$ for any $u \in \R^d$ since $M\leq M+\alpha \Id$.
Choosing $u = \nabla \pi(z)$, where $z\in \R^d$ is arbitrary; we thus obtain for any $m\geq 2$
$$
\sqrt{\|M+\alpha\Id\|} \frac{|(M+\alpha\Id)^{-\frac 1 2} (\nabla \pi (z))|}{\|z\|_{M+\alpha\Id}^{m-1}}\leq \sqrt{\|M\|} \frac{|M^{-\frac 1 2} (\nabla \pi (z))|}{\|z\|_M^{m-1}}
$$
Taking the infimum among all $z\neq 0$ we obtain the announced equation \iref{eqMMALG}, which concludes the proof of this lemma.
\sq

The construction of the metric adapted to the function $f$ presented above is unfortunately not very practical, because the map $\cM_\star^{(\alpha)} : \H_m\sm \{0\} \to S_d^+$, defined for each $\pi\in \H_m\sm\{0\}$ by a minimization problem, seems to be hard to compute.
The next proposition shows that this difficulty is avoided in the case of linear approximation or quadratic approximation in dimension $2$, since in that case there exists an explicit minimizer or near minimizer of the optimization problem defining $L_\star(\pi)$. The next proposition is announced in the introduction under the reference Proposition \ref{propLmIntro}.
\begin{prop}
\label{propLm}
\begin{itemize}
\item (Piecewise linear approximation, in any dimension)
If $m=2$ and $d\geq 2$, then for any $\pi\in \H_2$, one has 
$$
L_a(\pi) = 2|\det \pi|^\frac 1 d \stext{ and } L_g(\pi) =2 \sqrt{\|\pi\|} \sqrt[2d]{|\det \pi|}.
$$
The minimizing matrices $M$ in the minimization problems defining $L_a(\pi)$ and $L_g(\pi)$ are  respectively
$$
\cM_a(\pi) = 4[\pi]^2 \stext{ and } \cM_g(\pi) = \|\pi\| \, |[\pi]|
$$
\item (Piecewise quadratic approximation, in two dimensions)
If $m=3$ and $d=2$, let $\pi =  a x^3+ 3 b x^2 y+ 3 c x y^2+ d y^3\in \H_3$,
let 
$$
\cM_a(\pi) =  %\sqrt{ [\partial_x \pi]^2+ [\partial_y \pi]^2} = 
3 \sqrt{
\left(\begin{array}{cc}
a & b\\
b & c
\end{array}\right)^2
+
\left(\begin{array}{cc}
b & c\\
c & d
\end{array}\right)^2
}
$$
and let 
$$
\cM_g(\pi) := \cM_a(\pi) + \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}\Id
$$
where $\disc \pi$ is the discriminant of the cubic polynomial $\pi$ :  
\be
\label{eqDiscDet}
\frac{1} {27} \disc \pi= 4(ac-b^2)(bd-c^2) - (ad-bc)^2.
\ee

Then $\cM_a(\pi)$ and $\cM_g(\pi)$ are near minimizers of optimization problems defining $L_a(\pi)$ and $L_g(\pi)$ respectively. %(*details...*)
\end{itemize}
\end{prop}

\proof
For any homogeneous quadratic polynomial $\pi$ we denote by $[\pi]\in S_d$ the associated symmetric matrix, satisfying $z^\trans [\pi] z = \pi(z)$ for all $z\in \R^d$. Note that $\|\pi\| = \|[\pi]\|$.
\begin{itemize}
\item (The quadratic case)
%\paragraph{The quadratic case}
For any $\pi\in \H_2$ we have $\nabla \pi(z) = 2[\pi] z$. Hence $|\nabla \pi(z)|^2 = 4 z^\trans [\pi]^2 z$ and the announced result for $L_a$ easily follows.
For $L_g$, we are looking for $M$ of minimal determinant such that 
\be
\label{eqMPi}
2\|M^{\frac 1 2}\| \, \|M^{-\frac 1 2} [\pi] M^{-\frac 1 2}\|\leq 1.
\ee
Recalling that $\|AB\|\geq \|A\| \|B^{-1}\|^{-1}$ we obtain from \iref{eqMPi} that $2\|\pi \| \leq \|M^\frac 1 2\|$.
Hence 
\be
\label{eqMPiWeak}
4\|\pi\| \| M^{-\frac 1 2} [\pi] M^{-\frac 1 2}\|\leq 1.
\ee
The matrix of minimal determinant which achieves this equality is clearly $M = 4\|\pi\| \ |[\pi]|$. Since condition \iref{eqMPiWeak} is weaker than \iref{eqMPi}, and since $M$ also satisfies \iref{eqMPi} this concludes the proof.
%Furthermore, it also achieves the initial equality which concludes the proof.

\item (The cubic case)
The case of $L_a$ and $\cM_a$ is exposed in Chapter \ref{chapW1P}. We therefore turn to the case of $L_g$. 
Combining the homogeneity and the continuity of the functions involved, one easily shows that there exists a constant $C_0$ such that for all $\pi\in \H_3$
\be
\label{eqContHomog}
\begin{array}{ccccc}
C_0^{-1} \|\pi \| &\leq& \|\nabla \pi \| &\leq& C_0 \| \pi\|\\
C_0^{-1} \|\pi \| &\leq&  \lambda(\pi) :=\|\cM_a(\pi) \| &\leq& C_0 \| \pi\|,
\end{array}
\ee
and 
\be
\label{eqContHomog2}
\begin{array}{ccc}
\mu(\pi) := \|\cM_a(\pi)^{-1} \|^{-1} & \leq& C_0 \|\pi\|\\
\nu(\pi) := \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^\frac 1 3 &\leq&  C_0 \|\pi\|.
\end{array}
\ee
%\begin{eqnarray*}
%\label{eqNormGrad}
%C^{-1} \|\pi \| \leq& \|\nabla \pi \| &\leq C \| \pi\|\\
%\label{eqNormM}
%C^{-1} \|\pi \| \leq&  \lambda(\pi) :=\|\cM_a(\pi) \| &\leq C \| \pi\|\\
%&\mu(\pi) := \|\cM_a(\pi)^{-1} \|^{-1} & \leq C \|\pi\|\\
%\label{eqNormDisc}
%& \nu(\pi) := \left(\frac{|\disc\pi|}{\|\pi\|}\right)^\frac 1 3 &\leq  C \|\pi\|  
%\end{eqnarray*}
We consider below a fixed polynomial $\pi\in \H_3$, and we recall that 
$$
L_g(\pi) := \inf \{\sqrt{\det M} \sep \sqrt{\|M\|} \|\pi \circ M^{-\frac 1 2}\| \leq 1\}.
$$
\paragraph{Lower bound $L_g(\pi)\geq c \sqrt{\det \cM_g(\pi)}$.}
We consider $M\in S_d^+$ satisfying $1 \geq \|M^{\frac 1 2}\| \| \nabla (\pi \circ M^{-\frac 1 2}) \|$. Combining this with \iref{eqNormGrad} we obtain
$$
1 \geq C_0^{-1}  \|M^{\frac 1 2}\| \| \pi \circ M^{-\frac 1 2} \| \geq C_0^{-1} \|M^{\frac 1 2}\| \frac{\| \pi \|}{\| M^{\frac 1 2}\|^3} = \frac{\|\pi\|}{C_0 \|M\|},
$$
hence $\|\pi\| \leq C_0 \|M\|$. It follows that 
$$
1 \geq C_0^{-1} (C_0^{-1} \|\pi\|)^{\frac 1 2} \| \pi\circ M^{-\frac 1 2}\| = \|\ti \pi \circ M^{-\frac 1 2}\|,
$$
where $\ti \pi := C_0^{-\frac 3 2} \| \pi\|^{\frac 1 2} \pi$. %$\ti \pi := \mu \pi$ and $\mu := C^{-\frac 3 2} \| \pi\|^{\frac 1 2}$.
The solution $M_*$ of the minimization problem
$$
\inf\{ \det M \sep \|\ti \pi \circ M^{-\frac 1 2}\| \leq 1\}
$$
is known exactly in the case of cubic polynomials in two dimensions, see Chapter \ref{chapOptAniso}, and satisfies 
$$
(\det M_*)^3 = \kappa |\disc \ti \pi| = \kappa (C_0^{-\frac 3 2} \| \pi\|^{\frac 1 2})^4 |\disc \pi| = \kappa C_0^{-6} \| \pi\|^2 |\disc \pi|.
$$
where $\kappa$ is a positive constant which depends only on the sign of $\disc \ti \pi$.
Defining $c_0:=\kappa_*^\frac 1 6 C_0^{-1}$, where $\kappa_*$ stands for the minimial value of $\kappa$, we obtain 
\begin{eqnarray*}
L_g(\pi) &\geq& (\det M_*)^{\frac 1 2} \\
&= & \kappa^\frac 1 6 C_0^{-1} \|\pi\|^{\frac 1 3} |\disc \pi|^{\frac 1 6} \\
&\geq& c_0 \sqrt{\|\pi\| \nu(\pi)} %\left(\frac{|\disc\pi|}{\|\pi\|}\right)^\frac 1 6\\
%&\geq & \kappa^\frac 1 6 C^{-\frac 3 2} \|\cM_a(\pi)\|^\frac 1 2 
\end{eqnarray*}
On the other hand, there exists $c_1>0$ such that 
$$
L_g(\pi) \geq L_a(\pi) \geq c_1 \sqrt{\det \cM_a(\pi)} = c_1\sqrt{\lambda(\pi) \mu(\pi)}.
$$
Furthermore we have 
\begin{eqnarray*}
\det \cM_g(\pi) &=& (\lambda(\pi)+\nu(\pi))(\mu(\pi)+\nu(\pi)) \\
&\leq& (1+C_0^2)\min \{\lambda(\pi),\, \|\pi\|\} \left( 2\max\{\mu(\pi),\, \nu(\pi)\}\right)\\
&\leq & 2(1+C_0^2) \max \{\lambda(\pi) \mu(\pi), \, \|\pi\| \nu(\pi)\}.
\end{eqnarray*}
Thus leads us to the conclusion of our lower estimate for $L_g$
%Combining the last two equations, and recalling \iref{eqContHomog} and \iref{eqContHomog2} we obtain 
$$
\sqrt{\det \cM_g(\pi)}\leq C_* L_g(\pi) \stext{ where } C_*:= 2(1+C_0^2) \max \{c_0^{-1}, \, c_1^{-1}\}.
$$

\paragraph{The matrix $C\cM_g(\pi)$ satisfies the constraint for sufficiently large $C$.}
We establish in the paragraph that the matrix $M = C \cM_g(\pi)$ satisfies the inequality $\|M^{\frac 1 2}\| \| \nabla (\pi \circ M^{-\frac 1 2})\|\leq 1$ when $C$ is large enough (but independent of $\pi$), or equivalently that 
$$
\|\cM_g(\pi)\|^\frac 1 2 \|\cM_g(\pi)^{-\frac 1 2}( \nabla \pi(x,y))\| \leq C \stext{ when } \|(x,y)\|_{\cM_g(\pi)} \leq 1.
$$
It is established in Chapter \ref{chapW1P} that $\cM_a(\pi \circ U) = U^\trans \cM_a(\pi) U$ for any $U\in \cO_2$, and we have $\disc (\pi \circ U) = (\disc \pi) (\det U)^6 = \disc \pi$, see Chapter \ref{chapOptiAniso}. We may therefore assume, up to a rotation, that $\cM_a(\pi)$ is a diagonal diagonal matrix and that the first diagonal  coefficient is larger than the second one.
Therefore 
$$
\lambda(\pi)^2 = a^2+2b^2+c^2 \stext{ and } \mu(\pi)^2 = b^2+2c^2+d^2. (*\text{factor }3*)
$$
In order to avoid notational clutter, and since the polynomial $\pi\in \H_3$ is fixed, we denote below by $\lambda$, $\mu$ and $\nu$ the quantities $\lambda(\pi)$, $\mu(\pi)$ and $\nu(\pi)$.
%For that purpose we define 
%$$
%\mu^2 := a^2+2b^2+c^2 \stext{ and } \mu^2 := b^2+2c^2+d^2.
%$$
% The eigenvalues of $\cM_a(\pi)$ are therefore $\mu$ and $\mu$, and we may assume furthermore that $\mu \geq \mu$.
%We also define 
%$$
%\nu := \frac 1 3 \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}
%$$
Our purpose is to establish an upper bound on the quantity
\be
\label{eqMGGradPi}
\begin{array}{cl}
& \displaystyle\|\cM_g(\pi)\|^\frac 1 2 \|\cM_g(\pi)^{-\frac 1 2}( \nabla \pi(x,y))\| \\
=&  \displaystyle(a x^2+ 2 b xy + c y^2)^2 + \left(\frac {\lambda+\nu} {\mu+\nu}\right) (b x^2+ 2 c xy+ d y^2)^2.
\end{array}
\ee
%Our purpose is to bound
%$$
% (a x^2+ 2 b xy + c y^2)^2 + \left(\frac \mu {\max\{\mu, \nu\}}\right) (b x^2+ 2 c xy+ d y^2)^2 
%$$
under the hypothesis 
$$
\|(x,y)\|_{\cM_g(\pi)} = (\lambda+\nu) x^2+ (\mu+\nu) y^2 \leq 1,%\frac {x^2} {\lambda+\nu} + \frac {y^2} {\mu+\nu} \leq 1.
$$
which implies in particular $\lambda x\leq 1$ and $\max\{\mu,\nu\} y\leq 1$.
Injecting this in \iref{eqMGGradPi}, and recalling that $\nu\leq C_0^3 \lambda$, we see that we only need to bound the following quantities %We thus need to bound the quantities
\be
\label{eqabcLl}
\frac a {\lambda^2}, \, \frac b {\lambda \mu}, \, \frac c {\mu^2}
\stext{ and }
\frac \lambda \mu \frac b {\lambda^2}, \ \frac \lambda \mu \frac c {\mu \lambda}, \ \frac \lambda {\max\{\mu,\nu\}} \frac d {\max\{\mu, \nu\}^2}.
\ee
Observing that 
\be
\label{eqLlMax}
\mu \geq \max\{b,c,d\}
\stext{ and }
\lambda \geq \max\{a,b,c,\mu\} \geq \{a,b,c,d\}
\ee
we find that all the quantities appearing in \iref{eqabcLl} are smaller than one, except perhaps the last one : 
%
%Since $\lambda \leq \lambda+\nu \leq (1+C_0^2)\lambda$ and $\max\{\mu, \nu\} \leq \mu+\nu \leq 2\max\{\mu,\nu\}$ we only need to bound 
%The only difficulty comes from 
\be
\label{eqd}
\frac {\lambda d^2}{\max\{\mu, \nu\}^3}
\ee
Using the expression \iref{eqDiscDet} of the discriminant we find that 
$$
\frac{-\disc \pi}{27} = (a^2+b^2+c^2) d^2 + a Q(b,c,d)+R(b,c,d)
$$
where $Q$ and $R$ are homogenous polynomials of degree $3$ and $4$ respectively. Using \iref{eqLlMax} we therefore obtain, for a constant $C_1$ sufficiently large (but independent of $\pi$),
\begin{eqnarray*}
\lambda^2 d^2 &=& \frac{-\disc \pi}{27} - (a Q(b,c,d)+R(b,c,d)) \\
&\leq &\frac{\|\pi\| \nu^3} {27} +C_1 \lambda \mu^3 \\
&\leq &\left(\frac{C_0}{27} + C_1\right) \lambda \max \{\mu, \nu\}^3
\end{eqnarray*}
%It follows from the expression \iref{eqDiscDet} of the discriminant, and from \iref{eqLlMax}, that there exists a constant $C_1$ independent of $\pi$ and satisfying %norm of pi???
%$$
%%\sqrt 2 \nu ^3 \mu \geq \nu^3 \sqrt{\mu^2+ \mu^2} \geq 
%\frac{-\disc \pi} {27} \geq \lambda^2 d^2 - C_1 \lambda \mu^3.
%$$
%On the other hand we have $-\disc \pi \leq \nu^3 \|\pi\| \leq C_0 \nu^3 \lambda$.
%%On the other hand we have $\|\pi\|\leq \sqrt{\mu^2+\mu^2}\leq \sqrt 2 \mu$ and therefore 
%%$$
%%\frac{-\disc \pi} {27} \leq  \nu^3 \sqrt{\mu^2+ \mu^2}  \leq \sqrt 2 \nu ^3 \mu
%%$$
%Combining the last two equations we obtain
%$$
%\lambda^2 d^2 \leq \frac C {27} \nu^3 \lambda + C_1 \mu^3 \lambda \leq \left(\frac{C_0}{27} + C_1\right) \lambda \max \{\mu, \nu\}^3
%$$
The previous inequality yields a uniform bound on \iref{eqd}, which concludes the proof of this proposition.
%where $C_2 := \max\{C/27, C_1\}$.
%and therefore
%$$
%\frac{\lambda d^2}{\nu^3} \leq \sqrt 2 + C\left(\frac \lambda \nu\right)^3 \stext{ and } \frac{\lambda d^2}{\mu^3} \leq \sqrt 2\left(\frac \lambda \nu\right)^3 + C.
%$$
%Using the left part of the previous equation if $\mu\leq \nu$, and the right part otherwise, we obtain a bound on \iref{eqd} which concludes the proof.
\sq
\end{itemize}

\subsection{Approximation spaces}

For any $\star\in \{i,a,g\}$ and any $f\in W^{1,p}_\per$ we define a (nonlinear) quantity $|\nabla f|_{\star,p} \in [0, \infty]$ as follows 
$$
|\nabla f|_{\star,p} := \sup_{\mu \geq 1} \left(\mu^\frac m d\inf_{\substack{H \in \bH_\star\cap \bH_\per\\ m(H) \leq \mu}}e_H^\star(\nabla f)_p\right),
$$
where $e_H^i(\nabla f)_p$ refers to the quantity $e_H^a(\nabla f)_p$ or $e_H^g(\nabla f)_p$, since they coincide for isotropic metrics $H\in \bH_\per \cap \bH_i$.
\begin{theorem}
Define $\frac 1 \tau := \frac {m-1} d+ \frac 1 p$. If $\tau \geq 1$ and if the Sobolev injection $W^{m, \tau} \to W^{1,p}$ holds (which excludes the case $(m,p) = (2,\infty)$
%$m=2$ and $p=\infty$
) then one has
$$
|\nabla f|_{i,p} \leq C\left(\int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz\right)^\frac 1 \tau.
$$
\end{theorem}
\proof
The proof is nearly identical to the $L^p$ case presented in \S \ref{subsecApproxSpaceLP}, and the details are thus left to the reader. The key argument is again the use of the metric
$$
\max\{1, \gM_\delta (|d^m f|^\tau\sep z) \} \Id.
$$
%The remaining details are left to the reader.
\sq


The quantities $|\nabla f|_{a,p}$ and $|\nabla f|_{g,p}$ are both smaller than $|\nabla f|_{i,p}$ but are not easily compared in general.
The author needs to admit that the quantity $|f|_{a,p}$ is not totally satisfying. Indeed, depending on the approximated function, quasi-acute metrics and simplices are generally not needed everywhere.

For instance, in the case $d=2$, $m=3$ of piecewise quadratic approximation in dimension $2$, it follows from the explicit expressions of near minimizers of $L_a$ and $L_g$ given in Proposition \ref{propLm} that 
$$
L_g(a x^3+ d y^3) \simeq \sqrt[3]{|ad| \max\{|a|,\, |d|\}} \stext{ and } L_a(a x^3+ d y^3) \simeq \sqrt{|ad|}.
$$
In contrast we obtain %using \ref{propLm} that 
$$
L_g(ax^3+3cx y^2) \simeq L_a(a x^3+3c xy^2) \simeq \sqrt{\max\{|a|,\, |c|\} |c|}.
$$
If the approximated function only exhibits anisotropic features of the type $ax^3+3cx y^2$, then the production of quasi-acute metrics is useless.
A typical example is the approximation of the mollification $f=\vp_\ve *g$ of a cartoon function $g$. The analysis presented in Chapter \ref{chapCartoon} shows that, close to the curves where $g$ is discontinuous, the mollification $f$ does have anisotropic features of the type $ax^3+3cx y^2$, where $|c|\ll |a|$. Therefore quasi-acute triangulations are not required in the neighborhood of these curves. In fact graded triangulations should be preferred in this context since they require a smaller number of triangles to create a thin layer along a curve, as illustrated by Theorem \ref{thOptGeom}.


==> ApproxTheory/ApproxTheoryTheseOld2.tex <==
\input{../PreambleThese}
\section{Introduction} %, and metrics on a periodic bounded domain}
\label{secPer}


The main purpose of adaptive mesh generation, compared uniform mesh generation, is to reduce the number of simplices required to achieve a given task. Here are two relevant examples which 
are further discussed in this chapter:
\begin{enumerate}
\item
Given two domains of interest, generate the mesh with smallest possible cardinality that separates these
domains with a layer of simplices.
\item
Given a function $f$, generate the mesh of a prescribed cardinality $N$ that yields the best 
finite element approximation to $f$ of a given order $m-1$ in some prescribed norm $L^p$ or $W^{1,p}$.
\end{enumerate}
Both examples can be viewed as optimization problems posed on the set of meshes.
The second problem was dealt with in Chapter 2 and 3 in the case where $f$ is smooth, 
and an optimal mesh was constructed in the asymptotic regime $N\to +\infty$. The results
of the previous chapter have revealed that certain relevant classes of meshes can be equivalently
described in terms of riemannian metrics, and a natural objective is therefore
to translate the above problems as {\it optimization problems posed on the set of metrics}.
Optimization problems posed on metrics may indeed be easier to solve practically  
due to the continuous nature of these objects.
The goal of this chapter is to explain how this objective can be met for the
above two examples.

In the previous chapter, we have introduced the classes of meshes
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
and characterized the respectively equivalent classes of metrics
$$
\bH_i\subset \bH_a\subset \bH_g.
$$
These classes of meshes and metrics are defined on the entire unbounded domain $\R^d$.
The above optimization problems do not make sense in this setting since the 
number of element in such meshes is infinite. In order to circumvent this difficulty
while still avoiding the difficulties related to the boundary of a domain, we 
work in a periodized setting that we describe below.

\subsection{Periodic meshes and metrics}

We denote by $\bT_\per$ the collection of meshes $T\in \bT$ which satisfy the following properties:
\begin{enumerate}[i)]
\item (Translation invariance) For any $T\in \cT$ and any $u \in \Z^d$, one has $u+T \in \Z^d$.
\item (Constrained diameters) For any $T\in \cT$ one has $\cH_T\geq \Id$.
\end{enumerate}

Accordingly, we denote by $\bH_\per$ the collection of metrics $H \in \bH$ which satisfy the following properties:
\begin{enumerate}[i)]
\item (Translation invariance) For any $z\in \R^d$ and any $u \in \Z^d$, one has $H(z) = H(z+u)$.
\item (Constrained positivity) For any $z\in \R^d$ one has $H(z)\geq \Id$.
\end{enumerate}

A mesh $\cT\in \bT_\per$ can be regarded, thanks to the translation invariance property 
as a mesh of the compact periodic space 
\be
\label{perSpace}
\Pi^d := (\R/ \ZZ)^d,
\ee
also called the $d$-dimensional torus. %Note that $\Pi^d$ has no boundary.
The diameter constraint property ensures that the simplices $T$ of a periodic mesh $\cT \in \bT_\per$ do not have a significantly larger size than the fundamental cell $[0,1]^d$ of the standard $\Z^d$ periodic tiling of $\R^d$. 

Strictly speaking, a periodic mesh $\cT\in \bT_\per$ has an infinite cardinality. However it only contains a finite number of simplices up to translation by an element of $\Z^d$.  
For any $\cT\in \bT_\per$, we therefore denote by $\#(\cT)$ the number of equivalence classes in $\cT$ for the relation
$$
T \sim T' \text{ if and only if there exists } u \in \Z^d \text{ such that } \ T' = T+u.
$$
The number $\#(\cT)$ is finite, and is the the cardinality of $\cT$ seen as a mesh of the compact periodic space \iref{perSpace}.
We define the {\it mass} $m(H)$ of a periodic metric $H \in \bH_\per$ as follows
$$
m(H) :=  \int_{[0,1]^d} \sqrt{\det H}.
$$
Intuitively the mass of a metric $H$ and the cardinality of a mesh $\cT$ should be linked when
$H$ and $\cT$ are equivalent in the sense studied in the previous chapter.
We denote by $\TEq$ a fixed equilateral simplex centered at the origin of $\R^d$ and having its vertices on the unit sphere.
\begin{prop}
\label{propCardMass}
The cardinality of a mesh $\cT\in \bT_\per$ and the mass of a metric $H\in \bH_\per$ satisfy the following properties:
\begin{itemize}
\item If $\cH_T \leq C^2 H(z)$ for all $T\in \cT$ and all $z\in T$, then 
$
|\TEq|\#(\cT) \leq C^d  m(H).
$
\item 
If $H(z) \leq C^2 \cH_T$ for all $T\in \cT$ and all $z\in T$, then 
$
 m(H) \leq C^d |\TEq|\#(\cT).
$
\end{itemize}
In particular, if $\cT$ is $C$-adapted to $H$ in the sense of Definition \ref{defEqHT}, then 
\be
\label{eqCardMass}
C^{-d} m(H) \leq |\TEq| \,\#(\cT) \leq C^d m(H) .
\ee
\end{prop}

\proof
For any $z\in \R^d$ we denote by $T(z)$ the simplex $T\in \cT$ containing $z$.
Recalling (see Proposition \ref{propHT} in the previous chapter) that for any simplex $T$
$$
|T| \sqrt{\det \cH_T} = |\TEq|,
$$
we thus have 
\be
\label{eqCardT}
\#(\cT) = \int_{[0,1]^d} \frac {dz}{|T(z)|} = |\TEq|^{-1} \int_{[0,1]^d} \sqrt{\det \cH_{T(z)}} \, dz.
\ee
Furthermore we have $\det S \leq C^d \det S'$ for any $S,S'\in S_d^+$ satisfying $S \leq C S'$.
Applying this remark to the matrices $H(z)$ and $\cH_{T(z)}$ we obtain the announced inequalities, which concludes the proof of the proposition.
\sq

The equivalence between classes of meshes and metrics of $\R^d$ established in
Theorem \ref{thEquiv} of the previous chapter has an immediate generalization to periodic meshes and metrics.

\begin{theorem}
\label{thPer}
There exists a constant $C_0=C_0(d)$ such that for all $C \geq C_0$, 
\begin{enumerate}
\item The collection of meshes $\bT_{i,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_i \cap \bH_\per$.
\item If $d=2$, the collection of meshes $\bT_{a,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_a \cap \bH_\per$.
\item If $d=2$, the collection of meshes $\bT_{g,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_g \cap \bH_\per$.
\end{enumerate}
\end{theorem}

\proof
The proof of Theorem \ref{thEquiv} presented in the previous chapter can be adapted to periodic metrics and triangulations with only slight changes, which are left to the reader.
\sq



\subsection{Compactness of metrics}
\label{subsecIntroCompact}

In order to ensure the existence of an ``optimal metric'' for a number of optimization problems 
posed on periodic and isotropic, quasi-acute or graded metrics, we need a property of 
compactness for such metrics.

We equip the set $\bH_\per$ of continuous and $\Z^d$ periodic metrics with a distance $d_\per$ which is defined as follows: for all $H,H'\in \bH_\per$
$$
d_\per(H,H') := \sup_{z\in [0,1]^d} d_\times (H(z), H(z)) = \sup_{z\in \R^d} d_\times (H(z) , H'(z)).
$$
Consider $H, H'\in \bH_\per$ and define $\delta = d_\per(H,H')$. We thus have for all $z\in \R^d$,
\be
\label{pointwiseCont}
e^{-2 \delta} H(z)\leq H'(z) \leq e^{2 \delta} H(z). 
\ee
One easily checks that 
%Hence the mass $H \mapsto m(H)$ is a continuous function of $H \in \bH_\per$ 
\be
\label{massCont}
e^{-d\delta} m(H) \leq m(H') \leq e^{d\delta} m(H),
\ee
and 
%as well as the distance $H \mapsto d_H(x,y)$ for any fixed $x,y\in \R^d$ : 
\be
\label{distCont}
e^{-\delta} d_{H}(x,y) \leq d_{H'}(x,y) \leq e^\delta d_{H}(x,y).
\ee
which shows that the mass $m \mapsto m(H)$ and the distance between to fixed points $H \mapsto d_H(x,y)$ depend continuously on $H \in \bH_\per$.


We establish in \S \ref{secCompact} the following compactness property : for any $M\geq 1$ and any symbol $\star \in \{i,a,g\}$ the collection of metrics 
$$
\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq M\}
$$
is a compact subset of $\bH_\per$.



\subsection{Separation of two domains}

Isotropic and anisotropic mesh adaptation is often used to separate some geometric sets, in the sense given by the following definition. For any closed subset $E \subset \R^d$ and any mesh $\cT\in \bT$ we define the neighborhood $V_\cT(E)$ of $E$ in $\cT$ as follows :
$$
V_\cT(E) := \bigcup_{\substack{T \in \cT,\\ T \cap E\neq\emptyset}} T.
$$
We say that a mesh $\cT\in \bT$ separates two closed sets $X,Y\subset \R^d$ if and only if 
$$
V_\cT(X) \cap V_\cT(Y) = \emptyset,
$$
in other words if $X$ and $Y$ have disjoint neighborhoods in the mesh $\cT$. 

A natural objective is to build a mesh of minimal cardinality which separates two given regions. 
Consider two closed, disjoint and $\Z^d$-periodic sets $X,Y\subset \R^d$. We consider in \S \ref{secOptGeom} the optimization problem posed on triangulations 
$$
m_{\star,C_0}(X,Y) := \min\{ \#(\cT) \sep \cT\in \bT_\per \cap \bT_{\star,C_0} \text{ and }  \cT \text{ separates } X \text{ and } Y\}
$$
where $\star \in \{i,a,g\}$ is a symbol and $C_0\geq 1$ is a constant.
We establish then this problem is equivalent to the following
optimization problem posed on metrics, if the dimension is $d=2$:
$$
m_\star(X,Y) := \min\{ m(H) \sep H \in \bH_\per\cap \bH_\star \text{ and } H \text{ separates } X \text{ and } Y\}, 
$$
where say that a metric $H$ separates $X$ and $Y$ if 
$$
d_H(x,y) \geq 1 \text{ for all } (x,y) \in X\times Y.
$$
Precisely, we show that there exists a constant $C = C(C_0)\geq 1$, independent of the sets $X,Y$,
such that 
$$
C^{-1} m_\star(X,Y)\leq m_{\star,C_0}(X,Y) \leq C m_\star(X,Y).
$$

Imposing more constraints on the triangulation typically raises the number of triangles required to achieve a given task, and likewise assuming more regularity of the metric raises the mass required for a given task.
We illustrate this remark in the context of the separation of domains as follows.
We fix the parameter $r_0 := 1/4$ and we define the periodic set 
$$
X := \{x\in \R^d \sep d(x,\Z^d) \leq r_0\},
$$
where $d(x,E) := \min \{|x-e|\sep e\in E\}$,
and for any $0<\delta\leq r_0$ 
$$
Y_\delta := \{y\in \R^d \sep d(y,\Z^d)\geq r_0 + \delta\}.
$$
The sets $X$ and $Y_\delta$ are illustrated on Figure \ref{figXYDelta}.
The following equivalences are established as $\delta\to 0$
\begin{eqnarray*}
m_i(X,Y_\delta) &\simeq& \delta^{-(d-1)},\\
m_a(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2 } |\ln \delta|,\\
m_g(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2}.
\end{eqnarray*}

A construction closely related to the separation of the sets $X$ and $Y_\delta$ is presented on Figure \ref{figDisk} in the main introduction of this thesis.
\begin{figure}
\centering
\includegraphics[width=4cm,height=4cm]{\pathPic/Meshing/XYDelta.pdf}
\caption{The sets $X$ (light gray) and $Y_\delta$ (dark gray), with $d=2$ and $\delta = 0.1$. \label{figXYDelta}}
\end{figure}

\subsection{Approximation in a given norm}

One of the key purposes of anisotropic mesh generation is the adaptive approximation of functions,
as discussed extensively in Chapters 2 and 3. In order to study this problem from the point of view of metrics, we introduce an error $e_H(f)_p$ associated to a function and a metric, and we compare this quantity with the approximation error of $f$ on a mesh.

For that purpose we denote by $B_H(z)$ the open ball of radius $r$ around $z$ for the norm $\|\cdot \|_{H(z)}$
(therefore an ellipse):
$$
B_H(z) := \{z+u \sep \|u\|_{H(z)} < 1\}.
$$
For any exponent $p$, $1\leq p \leq \infty$, and any $f\in L^p_\loc(\R^d)$ we denote by $e_H(f\sep z)_p$ the error of best approximation of $f$ on $B_H(z)$:
\be
\label{defEH}
e_H(f\sep z)_p := \inf_{\mu\in \sP_{m-1} } \|f-\mu\|_{L^p(B_H(z))}.
\ee
We denote by $L^p_\per$ the collection of functions $f\in L^p_\loc(\R^d)$ which are $\Z^d$-periodic.
For all $f\in L^p_\per$ and all $H\in \bH_\per$ we define the approximation error $e_H(f)_p$ of $f$ associated to the metric $H$ as follows
\be
\label{defEHGlobal}
e_H(f)_p^p := \int_{[0,1]^d} \sqrt {\det H(z)} \, e_H(f\sep z)_p^p \, dz.
\ee

Consider a metric $H\in \bH_\per \cap \bH_g$ and a mesh $\cT\in \bH_\per$ such that 
\be
\label{eqTH4}
\cH_T \geq 4^2 H(z), \;\;  \,z\in T,\; T\in \cT,
\ee
%for any $T\in \cT$ and any $z\in T$.
which heuristically means that that the mesh $\cT$ is ``more refined'' than the metric $H$.
We establish in \S \ref{secApproxLP} that for any $f\in L^p_\per$  
\be
\label{eqBestLP}
\inf_{g\in V_{m-1}(\cT)} \|f-g\|_p \leq C e_H(f)_p
\ee
where $V_k(\cT)$ stands for the space of finite elements of degree $k$ on $\cT$, and $C$ is an absolute constant. Furthermore we give an explicit expression of a finite element approximation $g\in V_k(\cT)$ which satisfies \iref{eqBestLP}, namely
\be
\label{defGOpt}
g := \interp_\cT^{m-1} f_H,
\ee
where $f_H$ is the convolution \emph{distorted by the metric $H$} of $f$  with a compactly supported mollifier $\vp$ (which satisfies a moments condition) 
$$
f_H(z) := \int_{\R^d} f(z+H(z)^{-\frac 1 2} u) \vp(|u|)du.
$$

The extension of the approximation result \iref{eqBestLP} to the $W^{1,p}$ semi-norm is not trivial sue to the fact that interpolation on simplices of large measure of sliverness is not a stable procedure. 

For any vector field $v\in L^p_\loc(\R^d, \R^d)$ and any metric $H\in \bH$ we introduce the two quantities
\be
\label{defEHA}
e_H^a(v\sep z)_p := \min_{\nu\in \sP_{m-2}^d} \|v-\nu\|_{L^p(B_H(z))}
\ee
and 
\be
\label{defEHG}
e_H^g(v\sep z)_p := \|H(z)\|^{\frac 1 2} \min_{\nu\in \sP_{m-2}^d} \|H(z)^{-\frac 1 2} (v-\nu)\|_{L^p(B_H(z))}.
\ee
%where $\P_{m-2}^d$ denotes the collection of $d$-plets of polynomials of degree $m-2$. 
If $v$ is $\Z^d$ periodic and if $H\in \bH_\per$, then we define $e_H^a(v)_p$ and $e_H^g(v)_p$ similarly to \iref{defEHGlobal}.

Consider a metric $H\in \bH_\per \cap \bH_a$ and mesh $\cT\in \bH_\per$ which satisfy \iref{eqTH4}. We establish in \S \ref{secApproxW1P} that for any $f\in W^{1,p}_\per$  
\be
\label{eqBestW1PA}
\inf_{g\in V_{m-1}(\cT)} \|\nabla(f-g)\|_p \leq C \,e_H^a(\nabla f)_p \,\max_{T\in \cT} S(T)
\ee

This estimate should be compared with the following. Consider a metric $H\in \bH_\per \cap \bH_g$ and a mesh $\cT\in \bT$ which satisfy \iref{eqTH4} and in addition $C_0^2 H(z) \geq \cH_T$, for all $T\in \cT$,$z\in T$ (which means that the mesh $\cT$ is $C_0$-adapted to the metric $H$).
We establish in \S \ref{secApproxW1P} that 
\be
\label{eqBestW1PG}
\inf_{g\in V_{m-1}(\cT)} \|\nabla(f-g)\|_p \leq C \, e_H^g(\nabla f)_p,
\ee
where the constant $C$ depends on $C_0$.

The function $g$ given by \iref{defGOpt} satisfies both estimates \iref{eqBestW1PA} and \iref{eqBestW1PG}.
These results put in light the price to pay to obtain the best error estimate \iref{eqBestW1PA} in the $W^{1,p}$ norm: the measure of sliverness should be uniformly bounded on $\cT$, and the metric $H$ should belong to $\bH_a$. If these conditions are not satisfied then we can only prove the estimate \iref{eqBestW1PG} which is sub-optimal since it penalizes the anisotropy of the metric $H$, see \iref{defEHG}.

\subsection{Asymptotic approximation and explicit metrics}

We establish some counterparts for metrics of the asymptotic estimates presented in Chapters 2 and 3 for triangulations and more general meshes. 
Our estimates hold without restriction on the degree or the dimension, and apply to a sufficiently smooth function and to metrics an asymptotically large mass.

We denote by $\H_m$ the vector space of all homogeneous polynomials of degree $m$ in $d$ variables, and we define the \emph{shape function} $K$ as follows : for all $\pi \in \H_m$
\be
\label{defKIntro}
K(\pi) =\inf_{A\in \SL_d} \| \pi \circ A\|.
\ee
We establish in \S\ref{secApproxLP} that for any $\Z^d$ periodic and $C^m$ function
\be
\label{asymptLPMet}
\limsup_{\substack{H \in \bH_g\\  m(H)\leq M}} M^{\frac m d} e_H(f)_p \leq C \|K(d^m f)\|_\tau,
\ee
where the exponent $\tau$ is defined by $\frac 1 \tau := \frac m d+ \frac 1 p$.

The proof of this result would be greatly simplified if one could establish the existence of a smooth map $\pi\in \H_m \mapsto A(\pi)\in \SL_d$ such that $A(\pi)$ minimizes $\| \pi \circ A\|$. This is unfortunately not the case, and the key ingredient of the proof of \iref{asymptLPMet} is the definition and the analysis of a family $K^{(\alpha)}$ of functions which tend to $K$ as $\alpha\to \infty$ and which are defined by a well posed optimization problem (for which there exists a unique minimizer depending continuously on the parameter $\pi$).\\

In the case of $W^{1,p}$ norms we introduce two distinct \emph{shape functions}
\begin{eqnarray*}
L_a(\pi) &:=& \inf_{A\in \SL_d} \|(\nabla \pi)\circ A\| \\
L_g(\pi) &:=& \inf_{A\in \SL_d} \|A^{-1}\| \|\nabla (\pi\circ A)\| 
\end{eqnarray*}
We establish similar results to \iref{asymptLPMet}, for any $C^m$ and $\Z^d$ periodic function $f$
\begin{eqnarray*}
\limsup_{\substack{H \in \bH_a\\  m(H)\leq M}} M^\frac m d e_H^a(\nabla f)_p &\leq& C \|L_a(d^m f)\|_\tau\\
\limsup_{\substack{H \in \bH_g\\  m(H)\leq M}} M^\frac m d e_H^g(f)_p &\leq& C \|L_g(d^m f)\|_\tau,
\end{eqnarray*}
where $\tau$ is defined by $\frac 1 \tau := \frac {m-1} d + \frac 1 p$.\\

We give an explicit expression of near-minimizers of the optimization problems defining $L_a(\pi)$ and $L_g(\pi)$ in terms of the coefficients of a quadratic or cubic (in two dimensions) homogeneous polynomial $\pi$ (which needs to be quadratic or cubic in two dimensions). 
This expression can be used to compute efficiently in numerical applications a metric $H$ adapted to the approximated function $f$ using the available information on the derivatives of $f$.

We also use these minimizers to compute the ratio $L_a(\pi) / L_g(\pi)\leq 1$, and we discuss for which polynomials this ratio is significantly small. In other words for which types of anisotropic features of the approximated function $f$ the use of quasi-acute triangulations leads to a significantly smaller approximation error than the use of graded anisotropic triangulations (which is the case in all numerical software known to the author).



\section{Compactness of metrics of a given mass} %A compactness property}
\label{secCompact}

The purpose of this section is to establish the following compactness result.
We recall that the collection $\bH_\per$ of $\Z^d$ periodic metrics is equipped with the distance 
$$
d_\per(H,H') := \sup_{z\in \sR^d} d_\times (H(z), H'(z)).
$$
\begin{theorem}
\label{thCompact}
For any symbol $\star \in \{i,a,g\}$ and any $m_0\geq 1$ the collection of metrics 
\be
\label{defHStarM}
\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq m_0\}
\ee
is a compact subset of $\bH_\per$ 
\end{theorem}

The rest of this section is devoted to the proof of this theorem. Our first lemma establishes that the set \iref{defHStarM} is closed in $\bH_\per$.

\begin{lemma}
\label{lemmaClosed}
The set \iref{defHStarM} is closed in $\bH_\per$, as well as the sets $\bH_i, \bH_a, \bH_g$.
%The sets $\bH_\per \cap \bH_\star$, where $\star\in \{i,a,g\}$, are closed in of  $\bH_\per$, as well as the collection of metrics $\{H \in \bH_\per \sep m(H) \leq m_0\}$. 
\end{lemma}

\proof
As observed in \S \ref{subsecIntroCompact}, the pointwise evaluation, the distance between two fixed points $x,y\in \R^d$ and the mass define continuous maps on $\bH_\per$, see \iref{pointwiseCont},  \iref{massCont} and \iref{massCont}.
For any fixed $x,y\in \R^d$, the collection of all metrics $H \in \bH_\per$ which satisfy one of the following conditions
%\begin{enumerate}
%\item $m(H) \leq m_0$\\
%\item $d_\times (H(x),H(y)) \leq d_H(x,y)$\\
%\item $d_+ (H(x),H(y)) \leq |x-y|$\\
%\item $\|H(x)\| \|H(x)^{-1}\| =1$\\
%\end{enumerate}
\begin{eqnarray*}
 d_\times (H(x),H(y)) &\leq& d_H(x,y)\\
 d_+ (H(x),H(y)) &\leq& |x-y|\\
 \|H(x)\| \|H(x)^{-1}\| &=&1\\
m(H) &\leq& m_0
\end{eqnarray*}
is therefore a closed subset of $\bH_\per$.

A metric $H$ belongs to $\bH_g$ (resp. $\bH_a$, resp. $\bH_i$)
if and only if it satisfies the first of these inequalities for all $x,y\in \R^d$ (resp. the two first , resp. the three first).
The sets $\bH_i$, $\bH_a$ and $\bH_g$ are thus an intersection of closed subsets of $\bH_\per$, hence are closed.
% as well as the last inequality on the mass.
%
%the set \iref{defHStarM} if and only if, in the case $\star = g$ (resp. $\star = a$, resp. $\star = i$), it satisfies the first of these inequalities for all $x,y\in \R^d$ (resp. the two first , resp. the three first) as well as the last inequality on the mass.
%The set \iref{defHStarM} is therefore an intersection of closed sets, hence a closed set which concludes the proof.
The set \iref{defHStarM} is obtained by imposing the fourth inequality, and is therefore also closed.
\sq


%The key ingredient of this lemma is the 
%following classical
We recall a classical theorem of Ascoli, which states that the collection of Lipschitz functions between two compact metric spaces is itself a compact metric space. 
\begin{theorem}[Ascoli]
\label{thAscoli}
If two metric spaces $(X,d_X)$ and $(Y,d_Y)$ are compact, then the collection $\Lip(X,Y)$  of Lipschitz functions from $X$ to $Y$ is also compact when
equipped with the distance 
$$
d(f,g) := \max_{x\in X} d_Y(f(x),g(x)).
$$
\end{theorem}

We use this theorem to establish that %, similarly to finite dimensional spaces, 
closed and bounded subsets of $\bH_\per \cap \bH_g$ are compact.

\begin{lemma}
\label{lemmaCompact}
Any closed and bounded subset $\bH_*$ of $\bH_\per \cap \bH_g$ is compact.
\end{lemma}

\proof
Since the collection $\bH_*$ of metrics is bounded, the following quantity $M$ is finite %defined below is finite
$$
M^2 := \sup_{H \in \bH_*} \sup_{z\in [0,1]^d} \|H(z)\|.
$$
For any $x,y\in \R^d$ and any $H \in \bH_*$ we thus have $d_H(x,y) \leq M|x-y|$.

We consider the compact metric space $X :=[0,1]^d$, equipped with the distance $d_X(x,y) := M|x-y|$, and the compact metric space 
$$
Y := \{M \in S_d^+ \sep \Id \leq M \leq C^2 \Id\}
$$
equipped with the distance $d_\times$.
According to Theorem \ref{thAscoli} the metric space $\Lip(X,Y)$ is thus compact.

Consider a sequence $(H_n)_{n\geq 0}$ of elements of $H_*$. For all $n \geq 0$, the restriction $H_{n|[0,1]^d}$ is an element of $\Lip(X,Y)$. Since this space is compact there exists a sub-sequence $H_{\vp(n)}$ which converges uniformly on $[0,1]^d$. Recalling that $H_n$ is periodic for all $n\geq 0$ we find that $H_{\vp(n)}$ converges uniformly to a periodic metric $H \in \bH_\per$. 

Since that $\bH_*$ is closed in $\bH_\per \cap \bH_g$, and since $\bH_\per \cap \bH_g$ is closed in $\bH_\per$, we obtain that $\bH_*$ is closed in $\bH_\per$ and therefore $H \in \bH_*$ which concludes the proof.
\sq

The next lemma establishes that the set \iref{defHStarM} appearing in Theorem \ref{thCompact} is bounded. This set is closed according to Lemma \ref{lemmaClosed}, hence compact according to Lemma \ref{lemmaCompact}, which concludes the proof of Theorem \ref{thCompact}.

\begin{lemma}
\label{propCompact}
Let $m_0 \geq 1$ be a constant.
\begin{enumerate}
\item
There exists $C=C(m_0,d)$ such that for any $H \in \bH_g$ satisfying $H(z) \geq \Id \text{ for all } |z|\leq 1$ and 
$$
\int_{|z|\leq 1} \sqrt{\det H(z)} dz \leq m_0
$$
we have $\|H(0)\|\leq C^2$.
\item
The set 
$
\{H \in \bH_\per \cap \bH_g \sep m(H) \leq m_0\}
$
is bounded. %, and thus compact.
\end{enumerate}
\end{lemma}

\proof
We first show how 2. can be obtained assuming 1., and for that purpose we consider $H \in \bH_\per \cap \bH_g$ and $z_* %= (z_1, \cdots ,z_d)\in \R^d
$. The ball $\{z\in \R^d \sep |z-z_*|\leq 1\}$ is covered by the $2^d$ cubes 
$z_*+u+[0,1]^d$ where $u \in \{-1,0\}^d$. Consequently 
$$
\int_{|z-z_*|\leq 1} \sqrt{\det H(z)} dz \leq \sum_{u\in \{-1,0\}^d } \int_{z_*+u+[0,1]^d} \sqrt{\det H} = 2^d m_0
$$
and we already know that $H(z) \geq \Id$ for all $z\in \R^d$. It follows that $\|H(z_*)\|\leq C'^2$ where $C'$ is the constant associated to $2^d m_0$ in point 1., which concludes the proof of 2.\\


We now turn to the proof of 1. %, and for that purpose we consider a metric $H\in K_M$.
At each point $z\in \R^d$ we denote the eigenvalues of $H(z)$ by 
$$
\lambda_1^2(z) \geq \cdots \geq \lambda_d^2(z).
$$
For each $k \in \{1, \cdots ,d\}$ the function $\lambda_k$ is continuous and $\lambda(z)\geq 1$ for all $|z|\leq 1$.

Our purpose is to obtain an upper bound for $\lambda_1(0) = \sqrt{\|H(0)\|}$ in terms of $m_0$.
We shall proceed as follows : We first give an upper bound for $\lambda_d(0)$ that depends only on $m_0$, and then for each $1\leq k \leq d-1$ we give an upper bound for $\lambda_k(0)$ in terms of $m_0$ and $\lambda_{k+1}(0)$.


\paragraph{The upper bound on $\lambda_d(0)$.}
We define the ellipse 
%Denote by $\cE$ the ellipse 
$$
\cE := \{z\in \R^d \sep \|z\|_{H(0)} \leq \lambda_d(0)\}
$$
and observe that $|z|\leq 1$ for all $z\in \cE$.
We thus obtain using Corollary \ref{corolVol} 
$$
c_d \ln \lambda_d(0) \leq \int_\cE \sqrt{\det H(z)} dz \leq  \int_{|z|\leq 1} \sqrt{\det H(z)} dz \leq m_0,
$$
where $c_d>0$ is a constant. This gives as announced an upper bound on $\lambda_d(0)$ in terms of $m_0$.

\paragraph{The upper bound on $\lambda_k(0)$.}
The vector space $\R^d$ is the orthogonal sum 
$$
\R^d = U\oplus V
$$
 where $U$ is the sum of the eigenspaces  associated to the eigenvalues $\lambda_1^2(0), \cdots, \lambda_k^2(0)$ of $H(0)$ and $V$ is associated to the other eigenvalues $\lambda_{k+1}^2(0), \cdots, \lambda_d^2(0)$ of $H(0)$.
We have for all $u\in U$ and all $v\in V$, 
$$
\|u\|_{H(0)} \geq \lambda_k(0) |u| \stext{ and } \|v\|_{H(0)} \leq \lambda_{k+1}(0) |v|.
$$

We consider an isometry $P\in \cO_{d,k}$ (in the sense that $P^\trans P$ is the $k\times k$ identity matrix) satisfying $P(\R^k) = U$. 
For each $v\in V$ we define a metric $H_v$ on $\R^k$ as follows: for all $u \in \R^k$
$$
H_v(u) := P^\trans H_v(v+ Pu) P.
$$
It follows from Proposition \ref{propHG} (in the previous chapter) that $H_v$ belongs to the collection $\bH_g(\R^k)$.
We define 
$$
B_U := \{u \in \R^k \sep |u|\leq 1/2\} \stext{ and } B_V := \{v\in V \sep \lambda_{k+1}(0) |v| \leq 1/2\},
$$
as we observe that 
\be
\label{eqFubiniSet}
|P u+v| \leq 1 \text{ for all }  (u,v)\in B_U \times  B_V.
\ee
Recalling that $\lambda_i(z)\geq 1$ for all $1\leq i \leq d$ and $|z| \leq 1$ we obtain for all $(u,v) \in B_U \times B_V$
\be
\label{eqDetHHV}
\begin{array}{rcl}
\det H_v(u) &\leq& \lambda_1^2(Pu +v) \cdots \lambda_k^2(Pu +v)\\
&\leq &  \lambda_1^2(Pu +v) \cdots \lambda_d^2(Pu +v)\\
& =& \det H(Pu+v)
\end{array}
\ee
For any $u\in \R^k$ and any $v\in V$ we have according to \iref{eqLocalNorm}
\be
\label{eqLowerHV}
\|u\|_{H_v(0)} = \|Pu\|_{H(v)} \geq (1-\|v\|_{H(0)}) \|Pu\|_{H(z_*)} \geq \lambda_k(0) |u|/2, %(1-\lambda_{k+1}(0) |v|) \lambda_k(0) |u|.
\ee
and therefore 
$$
\{u\in \R^k \sep \|u\|_{H_v(0)} \leq \lambda_k(0)/4\} \subset B_U.
$$ 
Denoting by $c_k$ the constant from Corollary \ref{corolVol} applied in dimension $k$
%, and recalling \iref{eqLowerHV}, 
we therefore obtain for any $v\in B_V$
\be
\label{eqHVBU}
\int_{B_U} \sqrt{\det H_v(u)} du \geq c_k \ln ( \lambda_k(0)/4)
\ee
We thus obtain successively %According to Proposition (restrictMet) we have $H_v\in \bH_g^k$, therefore 
\begin{eqnarray*}
\int_{|z|\leq 1} \sqrt{\det H(z)} dz &\geq& \int_{v\in B_V} \int_{u\in B_U} \sqrt{\det H(P u +v)} du dv\\
&\geq & \int_{v\in B_V} \int_{u \in B_U} \sqrt{\det H_v(u)} du dv\\
& \geq & \int_{v\in B_V} c_k \ln(\lambda_k(0)/4) dv\\
& = & |B_V| c_k \ln( \lambda_k(0)/4)\\
& = & \frac{\omega_{d-k}}{(2\lambda_{k+1}(0))^{d-k}} c_k \ln( \lambda_k(0)/4).
\end{eqnarray*}
Where we use\iref{eqFubiniSet} and Fubini integration formula in the first line, \iref{eqDetHHV} in the second line, and \iref{eqHVBU} in the third line. In the last line we denote by  $\omega_{d-k}$ the volume of the unit ball in $\R^{d-k}$.

This inequality yields an upper bound on $\lambda_k(0)$ in terms of $M$ and $\lambda_{k+1}(0)$
$$
\lambda_k(0) \leq 4 \exp\left(\frac {m_0 (2\lambda_{k+1}(0))^{d-k}}{\omega_{d-k}}\right),
$$
which concludes the proof of this Theorem.
\sq


\section{Separation of two subdomains}
\label{secOptGeom}

We study in this section a geometrical problem: the separation of two sets using a triangulation, of minimal cardinality. Our first result, Proposition \ref{propEquivSep2}, establishes that this problem has an equivalent formulation in terms of metrics. 

\begin{proposition}
\label{propEquivSep2}
We assume that the collection of meshes $\bT_\per \cap \bT_{\star,C_0}$ and the collection of metrics $\bH_\per \cap \bH_\star$ are equivalent in dimension $d$, where $\star \in \{a,b,c\}$ is a symbol and $C_0\geq 1$ is a constant (this condition holds at least if $d=2$ according to Theorem \ref{thPer}).\\

There exists a constant $C \geq 1$ such that the following holds:\\
Let $X,Y \subset \R^d$ be two closed, disjoint and periodic sets, in the sense that 
$$
x+u \in X \stext{  and }y+u \in Y, \ \text{ for any } x\in X, \, y\in Y \text{ and }u \in \Z^d.
$$
Consider the two optimization problems 
\begin{eqnarray*}
m_{\star,C_0}(X,Y) &:=& \min\{ \#(\cT) \sep \cT\in \bT_\per \cap \bT_{*,C_0} \text{ and } \cT \text{ separates } X \text{ and } Y\},\\
m_\star(X,Y) &:=& \min\{ m(H) \sep H \in \bH_\per\cap \bH_* \text{ and } H \text{ separates } Y \text{ and } Y\}.
\end{eqnarray*}
Then 
\be
\label{eqMetricMeshSep}
C^{-1} m_\star(X,Y)\leq m_{\star,C_0}(X,Y) \leq C m_\star(X,Y).
\ee
%Furthermore a near minimizer of a problem can be built from a near minimizer of the other problem.
\end{proposition}

\proof %(* name of constants?*)
We denote by $C_1\geq 1$ a constant such that for any $\cT\in \bT_\per \cap \bT_{\star, C_0}$ there exists $H\in \bH_\per\cap \bH_\star$ which is $C_1$-equivalent to $\cT$, and vice versa.

The proof of this proposition is a simple translation between the vocabulary of meshes and the vocabulary of metrics.
We first establish that $m_\star(X,Y) \leq C m_{\star,C_0}(X,Y)$, and then that $m_{\star,C_0}(X,Y) \leq C m_\star(X,Y)$.\\

%\begin{itemize}
%\item
Let $\cT\in \bT_\per \cap \bT_{\star,C_0}$ be a mesh which separates the sets $X$ and $Y$, and let $H \in \bH_\per \cap \bH_\star$ be a metric which is $C_1$ equivalent to $\cT$. We thus have for any $T\in \cT$ and any $z\in T$
$$
C_1^{-2}H(z)\leq \cH_T \leq C_1^2 H(z).
$$
Let $x\in X$ and let $y\in Y$. Let $T_0\in \cT$ be the simplex containing $x$ and let $V_\cT(T_0)$ be the neighborhood of $T_0$ in $\cT$. %, in other words union of all simplices in $\cT$ which intersect $T_0$.
Since $x\in T_0$ and $y\notin V_\cT(T_0)$ we have $\|x-y\|_{\cH_{T_0}}\geq c := (C_0\sqrt d)^{-1}$ according to Proposition \ref{propNeighborT} (in the previous chapter). It follows that 
$$
d_H(x,y) \geq \ln (1+\|x-y\|_{H(x)}) \geq \ln(1+ \|x-y\|_{\cH_{T_0}}/C_1) \geq r:=\ln (1+c C_1^{-1}).
$$
%Up to replacing $r$ with $\min\{1,r\}$ we may assume that $0<r\leq 1$.
 The metric $\ti H := r^{-2} H$ thus belongs to $\bH_\per \cap \bH_\star$ since $0<r\leq 1$, see Remark \ref{remHomog}. Furthermore this metric separates the sets $X$ and $Y$ and satisfies according to Proposition \ref{propCardMass}
$$
m(\ti H)  \leq (C_1/r)^d |\TEq|\#(\cT).
$$ 
Taking the infimum over all meshes $\cT\in \bT_{*,C_0}$ which separate $X$ and $Y$ we obtain the left part of \iref{eqMetricMeshSep} : $m_*(X,Y) \leq |\TEq| (C_1/r)^d \, m_{*,C_0}(X,Y)$.\\

%\item
We now turn to the proof of the right part of \iref{eqMetricMeshSep}, and for that purpose we consider a Riemannian metric $H\in \bH_*\cap \bH_\per$ which separates the sets $X$ and $Y$. We consider a parameter $\lambda \geq 1$, which value will be specified later, and we observe that $\ti H := \lambda^2 H \in \bH_*\cap \bH_\per$.  Therefore there exists a mesh $T\in \bT_{*, T_0}\cap\bT_\per$ such that for all $T\in \cT$ and all $z\in \cT$ one has
$$
C_1^{-2} \ti H(z)\leq \cH_T \leq C_1^2 \ti H(z).
$$

Let us assume %for contradiction 
that $\cT$ does not separate the sets $X$ and $Y$, hence that $V_\cT(X) \cap V_\cT(Y) \neq \emptyset$. In that case there exists two simplices $T,T'\in \cT$ sharing a vertex $v$, and two points $x\in T \cap X$ and $y\in T'\cap Y$.
For any simplex $T$ and any $z,z'\in T$ we have $\|z-z'\|_{\cH_T} \leq 2$, see \iref{eqDiamTHT}.
%$$
%\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2
%$$
Therefore 
$$
\lambda \leq d_{\ti H}(x,y) \leq d_{\ti H}(x,v) + d_{\ti H} (v,y) \leq C_1 (\|x-v\|_{\cH_T}+ \|v-y\|_{\cH_{T'}}) \leq 4 C_1.
$$
We now choose the particular the value $\lambda := 4C_1+1$, which contradicts the the previous equation and shows that $\cT$ does separate $X$ and $Y$.
Furthermore
$$
|\TEq| \#(\cT) \leq  \, C_1^d \, m(\ti H) = (\lambda C_1)^d m(H).
$$
Taking the infimum among all metrics $H \in \bH_*$ which separate $X$ and $Y$ we obtain $|\TEq| m_{*,C_0}(X,Y) \leq  (\lambda C_1)^d m_*(X,Y)$, which %establishes the right part of \iref{eqMetricSep} and 
concludes the proof of this proposition.
\sq
%\end{itemize}

We define $r_0 := 1/4$ and for any $0<\delta\leq r_0$ we consider in the following the sets 
%The rest of this section is devoted to the proof of Theorem \ref{thOptGeom}, in which we consider the particular sets 
\be
\label{defXYDelta}
X := \{x\in \R^d \sep d(x,\Z^d)\leq r_0\} \stext{ and } Y_\delta := \{y\in \R^d \sep d(y, \Z^d) \geq r_0+ \delta\},
\ee
which are illustrated on Figure \ref{figXYDelta}.
%where $r_0 := 1/4$ and $0<\delta\leq r_0$. 
%For any $\star\in \{i,a,g\}$ we obtain explicit equivalents of the quantities $m_\star(X,Y_\delta)$ as $\delta \to 0$, as well as an explicit expressions of a near minimizer $H_\delta^\star\in \bH_\per \cap \bH_\star$ to this optimization problem.
The next theorem gives a sharp estimate of the minimal mass of a metric which separates the sets $X$ and $Y_\delta$, as $\delta\to 0$.
The notation $\alpha_\delta \simeq \beta_\delta$ stands for the following : there exists a constant 
%For any two functions $F,G : (0,r_0]\to \R_+$ we write $F \simeq G$ if there exists a constant
 $C\geq 1$ such that for all $0 <\delta \leq r_0$
$$
C^{-1}\alpha_\delta \leq \beta_\delta \leq C \alpha_\delta.
$$

\begin{theorem}
\label{thOptGeom}
We have the equivalences
\begin{eqnarray*}
m_i(X,Y_\delta) &\simeq& \delta^{-(d-1)}\\
m_a(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2 } |\ln \delta|\\
m_g(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2}.
\end{eqnarray*}
Furthermore for any $\star \in \{i,a,g\}$  and any $0< \delta \leq r_0$ the explicit metric $H_\delta^\star\in \bH_\star \cap \bH_\per$ defined below is a near minimizer of the problem $m_\star(X,Y_\delta)$. In other words $H_\delta^\star$ separates $X$ and $Y_\delta$ and satisfies $m(H_\delta^\star) \simeq m_\star(X,Y_\delta)$.
\end{theorem}

The proof is divided in two parts: we first give the explicit expression of the metrics $H_\delta^\star$ and use it to obtain an upper bound on $m_\star(X,Y_\delta)$. We then prove a lower bound for $m_\star(X,Y_\delta)$.

\subsection{Explicit metrics and upper bound}

%The proof of this Theorem is split into three lemmas. 
We define in this section the metrics $H_\delta^\star$, where $\star \in \{i,a,g\}$ and $0 < \delta \leq r_0 := 1/4$. We then establish in Lemma \ref{lemmaHInH} that $H_\delta^*\in \bH_*$ and $H_\delta^*$ separates $X$ and $Y_\delta$, and we prove in Lemma \ref{lemmaMHDelta} an upper estimate on the masses $m(H_\delta^*)$ of these metrics. 

In order to define $H_\delta^*$ we need to introduce some notations. For any $z\in \R^d \sm\{0\}$ we define
\be
\label{defsz}
s(z) := \min\{r_0, \left| |z|-r_0\right|\} \stext{ and } \theta(z) := \frac z {|z|}.
\ee
For any $0 < \delta \leq r_0$ and any $z\in \R^d\sm\{0\}$ we define three matrices $S_\delta^\star(z) \in S_d^+$, where $\star\in \{i,a,g\}$, as follows 
\be
\label{defSDeltaStar}
\begin{array}{rcl}
S_\delta^i(z) &:=& \max\{s(z), \delta\} \, \Id\vspace{0.2ex}\\
S_\delta^a(z) &:=& \max\{s(z), \delta\} \, \theta(z) \theta(z)^\trans + \max\left\{s(z), \sqrt \delta\right\} \, (\Id - \theta(z) \theta(z)^\trans)\vspace{0.2ex}\\
S_\delta^g(z) &:=& \max\{s(z), \delta\} \, \theta(z) \theta(z)^\trans + \sqrt{r_0\max\{s(z), \delta\}} \, (\Id - \theta(z) \theta(z)^\trans).
\end{array}
\ee
%
%\begin{eqnarray*}
%S_\delta^i(z) &:=& \max\{s(z), \delta\} \, \Id\\
%S_\delta^a(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \max\left\{s(z), \sqrt \delta\right\} \, (\Id - \n_z \n_z^\trans)\\
%S_\delta^g(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \sqrt{r_0\max\{s(z), \delta\}} \, (\Id - \n_z \n_z^\trans).
%\end{eqnarray*}
We also define $S_\delta^\star(0) = r_0\Id$ for any $\star\in \{i,a,g\}$. Eventually we define the metrics $H_\delta^*$ by the equality 
\be
\label{eqHS2}
2  H_\delta^\star(z+u)^{-\frac 1 2} := S_\delta^*(z)
\ee
for all $z\in \left[-\frac 1 2, \frac 1 2\right]^d$ and all $u \in \Z^d$.
Observe that 
\be
\label{eqS2R0}
H_\delta^\star = \Id \stext{ for all } |z| \geq 2  r_0 =  1 / 2.
\ee
since $S_\delta^\star(z) = r_0 \Id$ on this set.

\begin{lemma}
For all $0<\delta \leq  r_0$ and all $\star\in \{i,a,g\}$ one has $H_\delta^\star \in \bH_\per \cap \bH_\star$.
%\be
%\label{eqHInH}
%H_\delta^*\in \bH_* \cap \bH_\per.
%\ee
\end{lemma}
\proof
We first remark that $s = r_0$ on the boundary $\partial ([-\frac 1 2, \frac 1 2]^d)$, and therefore $H_\delta^\star = \Id$ on this set for any $\star \in \{i,a,g\}$. Using \iref{eqHS2} we thus obtain that $H_\delta^\star$ is continuous and $\Z^d$ periodic.

We denote  
$$
s_\per(z) := \min\{r_0, |d(z, \Z^d) -r_0|\}
$$
and we observe that $s_\per$ is a Lipschitz function.
Observing that 
$
H_\delta^i = 4\Id /\max\{s_\per , \delta\}^2,
$
we obtain that $H_\delta^i\in \bH_i$ since the function $z\mapsto \min \{s(z), \delta\}/2$ is Lipschitz, which concludes the case $\star = i$.\\

We now consider the case $\star =g$, and for that purpose we use the notations of \S \ref{secEigen} (in the previous chapter). Our first step is to establish that the local dilatation $\dil_z(H)_\times$ defined in \iref{defDilH} is smaller than $1$ for all $z$ on the set 
$$
\Omega := \{z\in \R^d \sep 0 < |z| < r_0 - \delta\}. % \text{ or } (-1/2, 1/2)^d \sm \{0\}
$$
We define the functions
$$
\lambda := s/2 \stext{ and } \mu := \sqrt s /4 
$$
and we observe that 
$
H_\delta^g = \lambda^{-2} \theta \theta^\trans + \mu^{-2} \theta \theta^\trans
$
on $\Omega$.
The functions $\lambda$ and $\mu$ are $C^\infty$ on $\Omega$ and we have
$$
\nabla \lambda = \frac{-\theta} 2 \stext{ and } \nabla \mu = \frac {-\theta}{8 \sqrt s},
$$
Therefore for any $z\in \Omega$ 
$$
\dil_z(\ln \lambda\sep d_H) = \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)} =  \frac{\|\nabla \lambda(z)\|_{H(z)^{-1}}}{ \lambda(z)}
= \frac{\|-\theta(z)/2\|_{H(z)^{-1}}}{ \lambda(z)} = 1/2.
$$
and 
$$
\dil_z(\ln \mu\sep d_H) = \frac{\dil_z(\mu \sep d_H)}{\mu(z)}
=  \frac{\|\nabla \mu(z)\|_{H(z)^{-1}} }{\mu(z)} %\\
%&=& \frac{\|-\theta(z)/(8\sqrt {s(z)})\|_{H(z)^{-1}}}{\mu(z)}
= \frac{\lambda(z)}{8 \sqrt{s(z)} \mu(z)} = 1/4.
$$
On the other hand the derivative of $\theta$ at a point $z\in \R^d\sm \{0\}$ in the direction $u\in \R^d$ is the component of $u$ orthogonal to $\theta$ and divided by $|z|$ : 
$$
\frac{\partial \theta}{\partial u}(z) = \frac{u-\<u, \theta(z)\>\theta(z)}{|z|},
$$
therefore 
$$
\dil_z(\theta \sep d_H) = \frac {\mu(z)} {|z|}.
$$
On the other hand for $z\in \Omega$
$$
\left|\frac{\lambda(z)}{\mu(z)} - \frac {\mu(z)}{\lambda(z)}\right| = \sqrt{\frac {r_0}{s(z)}} -  \sqrt{\frac {s(z)}{r_0}} \leq r_0-s(z) = |z|,
$$
where we used the fact that $\sqrt t- 1/\sqrt t\leq t$ for all $t\geq 1$ (easily checked by derivation).
Therefore 
$$
\frac 1 2 \left|\frac{\lambda(z)}{\mu(z)} - \frac {\mu(z)}{\lambda(z)}\right|\dil_z(\theta \sep d_H) \leq \frac {\mu(z)} 2 \leq 1/8.
$$
It follows that the quantity $D_z(a)_\times$ defined in \iref{eqDZA} is smaller than $1/2$, and therefore that $\dil_z(H_\delta^g)_\times \leq 1$ on $\Omega$ according to Theorem \ref{th2Spaces}.
Proceeding likewise we also obtain that $\dil_z(H_\delta^g) \leq 1$ on the annulus $\{z\in \R^d \sep r_0+\delta<|z|<2r_0\}$. Furthermore $H_\delta^g$ is constant on the annulus $\{z\in \R^d \sep r_0-\delta <|z|<r_0+\delta \}$ and on the domain $\{z\in (-1/2,1/2)^d  \sep |z|> 2r_0\}$. Defining 
$$
\Gamma_0 := \{z\in \R^d \sep |z| \in \{0,r_0-\delta, r_0+\delta, 2r_0\}\} \cup \partial ([-1/2,1/2]^d),
$$
and $\Gamma := \{z+u \sep z\in \Gamma_0, \, u\in \Z^d\}$ we have thus established that $\dil_z(H_\delta^g) \leq 1$ on $\R^d\sm \Gamma$. Corollary \ref{corolLipNoGamma} thus implies that $H_\delta^g\in \bH_g$.

The proof that $H_\delta^a\in \bH_a$ is extremely similar to the proof that $H_\delta^g\in \bH_g$: 
the quantities $D_z(a)_\times$ and $D_z(a)_+$ defined in \iref{eqDZA} and \iref{eqDZAP} can be explicitely computed on $\R^d\sm\Gamma$ and are smaller that $1/2$. Theorem \ref{th2Spaces} thus implies that 
the local dilatations $\dil_z(H_\delta^a)_\times$ and $\dil_z(H_\delta^a)_+$ are bounded by $1$ on this set, and it follows from Corollary \ref{corolLipNoGamma} that $H_\delta^a\in \bH_a$. The details of the proof are left to the reader.
\sq

The next lemma establishes the that the metrics $H_\delta^\star$ do separate the sets of interest.

\begin{lemma}
\label{lemmaHInH}
For all $0<\delta\leq r_0$ and all $\star\in \{i,a,g\}$ the metric $H_\delta^\star$ separates the sets $X$ and $Y_\delta$.\end{lemma}

\proof
%We now check the separation of $X$ and $Y_\delta$ by the metrics $H_\delta^*$, where $*\in \{i, a ,g\}$.
Let $\gamma\in C^1([0,1],\R^d)$ be such that $\gamma(0)\in X$ and $\gamma(1)\in Y_\delta$. Since the sets $X$, $Y_\delta$ are $\Z^d$-periodic, as well as the metrics $H_\delta^*$, we may assume that $\gamma(0)\in \left[-\frac 1 2, \frac 1 2\right]^d$.
Recalling the definition \iref{defXYDelta} of $X$ and $Y_\delta$ we obtain
$$
|\gamma(0)|\leq r_0 \stext{ and } |\gamma(1)| \geq r_0+ \delta.
$$
We define 
$$
t_0 := \max \{t\in [0,1] \sep \gamma(t)\in X\} \stext{ and } t_1 := \min \{t\in [t_0, 1] \sep \gamma(t)\in Y_\delta\}.
$$
For any $t\in [t_0, t_1]$ we have 
$$
\gamma(t_0) = r_0  \leq |\gamma(t)| \leq r_0+\delta = \gamma(t_1).
$$
and therefore 
$$
\|\gamma'(t)\|_{H_\delta^\star(\gamma(t))} \geq \frac {2|\<\gamma'(t), \theta(\gamma(t))\>|}\delta = \frac{2 ||\gamma|'(t)|} \delta,
$$
where $|\gamma|$ stands for the function $z\mapsto |\gamma(z)|$.
Hence 
$$
l_{H_\delta^\star}(\gamma) \geq \int_0^1 \|\gamma'(t)\|_{H_\delta^\star(\gamma(t))} dt \geq \int_{t_0}^{t_1} \frac{2|\gamma|'(t)dt} \delta = 2\frac{|\gamma(t_1)|-|\gamma(t_0)|} \delta = 2.
$$
It follows that $d_{H_\delta^\star}(X,Y_\delta) \geq 2$ which concludes the proof.
\sq

The next lemma estimates the mass of the metrics $m(H_\delta^\star)$, which yields an upper estimate on the minimal mass $m_\star(X,Y_\delta)$ required to separate the sets $X$ and $Y_\delta$ using a metric in $\bH_\per \cap \bH_\star$.

\begin{lemma}
\label{lemmaMHDelta}
There exists a constant $C>0$ such that for all $0<\delta \leq r_0$
\begin{eqnarray}
\label{eqHDeltaI}
m(H_\delta^i) &\leq& C\delta^{-(d-1)},\\
\label{eqHDeltaA}
m(H_\delta^a) &\leq& C\delta^{-\frac{d-1} 2 } |\ln \delta|,\\
\label{eqHDeltaG}
m(H_\delta^g) &\leq& C\delta^{-\frac{d-1} 2}.
\end{eqnarray}
\end{lemma}

\proof
Recalling the definition \iref{eqHS2} of $H_\delta^\star$ in terms of $S_\delta^\star$ we obtain 
$$
m(H_\delta^\star) = c_0 + 2^d \int_{|z|\leq 2r_0}  \frac {dz}{\det S_\delta^\star(z)},
$$
where $c_0$ stands for the volume of the following set, on which $H_\delta^\star = \Id$ according to \iref{eqS2R0},
$$
\left\{z\in \left[-\frac 1 2,\frac 1 2\right]^d \sep |z| \geq 2 r_0\right\}.
$$
%and where we used the 
%%We first establish the three inequalities \iref{eqHDeltaI}, \iref{eqHDeltaA} and \iref{eqHDeltaG}, and we then turn to \iref{eqHInH}.
%Recalling the definition \iref{eqHS2} of $H_\delta^\star$ in terms of $S_\delta^\star$ we obtain 
%$$
%m(H_\delta^\star) = \int_{\left[-\frac 1 2,\frac 1 2\right]^d} \sqrt{\det H_\delta^\star(z)} dz = 2^d \int_{\left[-\frac 1 2,\frac 1 2\right]^d} \frac {dz}{\det S_\delta^\star(z)} 
%$$
Furthermore 
$$
\int_{|z|\leq 2r_0} \frac {dz}{\det S_\delta^\star(z)} = c_1 \int_{r=0}^{2r_0} \frac {r^{d-1}dr}{s_\delta^\star(r)},
$$
%where the constants $c_0,c_1>0$ are defined as follows.
%The constant $c_0$ and  stands for the contribution of the integral on the set 
%$$
%\left\{z\in \left[-\frac 1 2,\frac 1 2\right]^d \sep |z| \geq 2 r_0\right\},
%$$
%which is independent of $\delta$ according to \iref{eqS2R0}. The constant 
where $c_1$ stands for the $d-1$-dimensional volume of the sphere $\{z\in \R^d \sep |z|=1\}$, and where
$$
s_\delta^\star(r) := \det S_\delta^\star(z)
$$
for any $z$ such that $|z| = r$.
Therefore there exists a constant $c_2>0$, independent of $\delta$ and of $\star\in \{i,a,g\}$, and such that 
$$
m(H_\delta^\star) \leq c_2 \int_{r=0}^{2r_0} \frac {dr}{s_\delta^\star(r)}.
$$
Recalling the definition \iref{defSDeltaStar} of $S_\delta^i(z)$ we obtain $s_\delta^i(r) = \max\{\delta,|r_0-r|\}^d$ for all $0 \leq r\leq r_0$, hence 
\begin{eqnarray*}
 \int_{r=0}^{2r_0} \frac {dr}{s_\delta^i(r)} &=& \int_0^{r_0 - \delta} \frac {dr}{(r_0-r)^d} + \int_{r_0 - \delta}^{r_0+\delta} \frac {dr}{\delta^d} + \int_{r_0+\delta}^{2r_0} \frac {dr}{(r-r_0)^d} \\
&=& \frac{\delta^{-(d-1)}}{d-1} + 2 \delta^{-(d-1)} + \left(\frac{\delta^{-(d-1)}}{d-1} -\frac {r_0^{-(d-1)}} {d-1}\right)\\
&\leq & 4 \delta^{-(d-1)}
\end{eqnarray*}
which establishes \iref{eqHDeltaI}.
Similarly, we find 
%We have 
$s_\delta^g(r) = r_0^{\frac {d-1} 2} \max\{\delta,|r_0-r|\}^{\frac {d+1} 2}$, hence 
\begin{eqnarray*}
r_0^{\frac {d-1} 2} \int_{r=0}^{2r_0} \frac {dr}{s_\delta^g(r)} &=& \int_0^{r_0 - \delta} \frac {dr}{(r_0-r)^{\frac{d+1} 2}} + \int_{r_0 - \delta}^{r_0+\delta} \frac {dr}{\delta^{\frac{d+1} 2}} + \int_{r_0+\delta}^{2r_0} \frac {dr}{(r-r_0)^{\frac{d+1} 2}} \\
&=& \frac{2\delta^{-\frac{d-1} 2} }{d-1} + 2 \delta^{-\frac{d-1} 2} + \left( \frac{2\delta^{-\frac{d-1} 2} }{d-1} -\frac {2r_0^{-\frac{d-1} 2}} {(d-1)}\right)\\
&\leq & 6 \delta^{-\frac{d-1} 2}
\end{eqnarray*}
which establishes \iref{eqHDeltaG}.
Eventually, we have $s_\delta^a(r) = \max\{\delta,|r-r_0|\} \max\left\{\sqrt\delta, |r-r_0|\right\}$, and therefore 
\be
\label{eqThreeInt}
\int_{r=0}^{2r_0} \frac {dr}{s_\delta^a(r)} = \int_{I_\delta} \frac {dr} {|r_0-r|^d} + \int_{J_\delta} \frac {dr}{|r_0-r| \delta ^{\frac {d-1} 2}} + \int_{r_0-\delta}^{r_0+\delta} \frac {dr}{\delta^{\frac{d+1} 2}},
\ee
where 
$$
I_\delta = \left[0,r_0-\sqrt \delta\right] \cup \left[r_0+ \sqrt \delta, 2 r_0\right] \stext{ and }J_\delta = \left[r_0-\sqrt \delta, r_0-\delta\right] \cup \left[r_0+ \delta, r_0+ \sqrt \delta\right].
$$
Therefore %The contributions of the three integrals in \iref{eqThreeInt} are given in the next three lines %Computing the contributions of the three integrals we obtain 
\begin{eqnarray*}
\int_{r=0}^{2r_0} \frac {dr}{s_\delta^a(r)} &=& \frac 1 {d-1} \left(2\left(\sqrt{\delta}\right)^{-(d-1)}+r_0^{-(d-1)} \right)\\
& & +  2 \delta^{-\frac {d-1} 2} \left(\ln \left(\sqrt \delta\right) - \ln \delta\right) \\
& & + 2 \delta^{-\frac {d-1} 2}\\
&=& \delta^{-\frac {d-1} 2} |\ln \delta| + \frac {2d} {d-1} \delta^{-\frac {d-1} 2} + r_0^{-(d-1)}
\end{eqnarray*}
which establishes \iref{eqHDeltaA}.
\sq

\subsection{Lower bound}

We prove in this subsection the lower bound announced in Theorem \ref{thOptGeom}. 
\begin{lemma}
\label{lemmaMLower}
There exists a constant $c>0$ such that for all $0<\delta\leq r_0$, 
\begin{eqnarray}
\label{eqHILower}
m_i(X,Y_\delta) &\geq& c\delta^{-(d-1)},\\
\label{eqHALower}
m_a(X,Y_\delta) &\geq& c\delta^{-\frac{d-1} 2 } |\ln \delta|,\\
\label{eqHGLower}
m_g(X,Y_\delta) &\geq& c\delta^{-\frac{d-1} 2}.
\end{eqnarray}
\end{lemma}
\proof 
We consider a metric $H\in \bH_\star$, where $\star\in \{i,a,g\}$ which separates the sets $X$ and $Y_\delta$. In particular $H \in \bH_g$.
We denote by $\bbS := \{v\in \R^d\sep |v| = 1\}$ the euclidean unit sphere of $\R^d$, and by $\omega$ the $d-1$-dimensional volume of $\bbS$. We define for all $v\in \bbS$
$$
n(v) := \|v\|_{H(r_0v)} \stext{ and } m(v) := \inf_{|w|=1} \|w\|_{H(r_0v)} =\|H(r_0v)^{-\frac 1 2}\|^{-1} .
$$
Proposition \iref{propEulidRiemann} (in the previous chapter), states that for any $z,u\in \R^d$ we have 
\be
\label{eqER}
d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention if $\|u\|_{H(z)} \geq 1$. 

%Furthermore, see \iref{eqLocalNorm}, for all $v\in \R^d$
%$$
%\|v\|_{H(z+u)} \geq (1-\|u\|_{H(z)}) \|v\|.
%$$

We now consider a point $v\in \bbS$ and we observe that $r_0 v\in X$ and $(r_0+\delta)v\in Y_\delta$. Therefore 
$$
1 \leq d_H(r_0v, \, (r_0+ \delta) v) \leq -\ln\left(1-\delta \|v\|_{H(r_0 v)}\right)
$$
hence $\lambda \delta n(v) \geq 1$
%\be
%\label{eqHvv}
%\delta \|v\|_{H(r_0 v)} \geq 1-e^{-1} = \lambda^{-1},
%\ee
where
$
\lambda := (1-e^{-1})^{-1}.
$
Let $v,w\in \bbS$, and let $\sigma\in \{-1,1\}$ be such that $\sigma \<v,w\>\geq 0$.  Remarking that $2r_0+ \delta \leq 3/4 \leq 1$ we obtain 
$$
\left|r_0 v+\sigma \sqrt {\delta} w\right|^2 = r_0^2 +\delta + 2  r_0 \sqrt \delta \sigma\<v,w\> \geq r_0^2 +\delta \geq r_0^2 + (2r_0 +\delta) \delta = (r_0+\delta)^2.
$$
Hence $r_0 v \in X$ and $r_0 v+\sigma \sqrt {\delta} w\in Y_\delta$. Therefore 
$$
1 \leq d_H(r_0 v, \, r_0 v+ \sigma \sqrt \delta w) \leq -\ln\left(1-\sqrt \delta \|w\|_{H(r_0 v)}\right),
$$
which implies $\lambda \sqrt \delta m(v) \geq 1$.
We we now distinguish between the three cases $\star = i$, $a$ or $g$.
\begin{itemize}
\item If $\star = i$, then $H(z) = \Id/s(z)^2$ where $s$ is a Lipschitz function. Furthermore $s(r_0 v) = n(v)^{-1} \geq \lambda\delta$.
It follows that 
\begin{eqnarray*}
m(H) &\geq& \int_\bbS \int_0^{2r_0} \frac {r^{d-1} dr dv}{s(rv)^d} \\
&\geq& \int_\bbS\int_{r_0}^{r_0+\delta} \frac{r_0^{d-1} dr dv}{(n(v)^{-1}+\delta)^d}\\
&\geq& \frac{r_0^{d-1}\delta\omega }{(\lambda\delta+ \delta)^d}\\
&=& \frac{r_0^{d-1} \omega}{(\lambda+1)^d} \delta^{-(d-1)}
\end{eqnarray*}
Taking the infimum among all metrics $H \in \bH_i$ which separate the sets $X$ and $Y_\delta$ we obtain as announced
$$
m_i(X,Y_\delta) \geq c \delta^{-(d-1)} \stext{ where } c= \frac{r_0^{d-1} \omega}{(\lambda+1)^d}.
$$
\item If $\star =a$, then the functions $z\mapsto \|H(z)\|^{-\frac 1 2}$ as well as $z\mapsto \|H(z)^{-\frac 1 2}\|$ are Lipschitz. Hence for any $v\in \bbS$ and any $\mu\in \R$ we have 
$$
\|H((r_0+\mu) v)\|^{-\frac 1 2} \leq n(v)^{-1}+ |\mu| \leq \lambda \delta + |\mu|
$$
and 
$$
\|H((r_0+\mu) v)^{-\frac 1 2}\| \leq m(v)^{-1} + |\mu| \leq \lambda \sqrt \delta + |\mu|,
$$
in particular recalling that $\det M \geq \|M\| \|M^{-1}\|^{-(d-1)}$ for any $M\in S_d^+$ we obtain 
$$
(\lambda\delta+|\mu|)(\lambda\sqrt\delta+|\mu|)^{d-1}\sqrt{\det H((r_0+\mu) v)} \geq 1.
$$
It follows that  
\begin{eqnarray*}
m(H) &\geq& \omega \int_{-r_0}^{r_0} \frac {(r_0+\mu)^{d-1}d\mu}{(\lambda\delta+|\mu|)(\lambda\sqrt\delta+|\mu|)^{d-1}}\\
&\geq& \omega \int_0^{\sqrt \delta} \frac {r_0^{d-1}d\mu}{(\lambda \delta +\mu)(\lambda\sqrt{\delta} + \sqrt \delta)^{d-1}}\\ 
&\geq& \frac{\omega r_0^{d-1} }{((\lambda+1)\sqrt \delta)^{d-1}} (\ln \sqrt \delta -\ln (\lambda\delta)).
\end{eqnarray*}
Hence 
$$
m_a(X,Y_\delta) \geq c\delta^{-\frac{d-1} 2} (-\ln\delta-2\ln \lambda) \stext{ where } c=\frac{\omega}{2(\lambda+1)^{d-1}}
$$
which concludes the proof of \iref{eqHALower}.
\item We now consider the case $\star = g$. 
%We first remark that for any $M,M'\in S_d^+$
%$$
%|\ln \det M -\ln \det M'| \leq 2d\,d_\times (M,M').
%$$
We have for any $v\in \bbS$%Recalling that 
$$
\sqrt{\det H(r_0 v)} \geq \frac 1 {n(v)m(v)^{d-1}} \geq \frac  1 {n(v) (\lambda \sqrt \delta)^{d-1}}.
$$
%$$
%n(v) (\lambda \sqrt d)^{d-1} \sqrt{\det H(r_0 v)}\geq n(v)m(v)^{d-1}\sqrt{\det H(r_0 v)} \geq 1
%$$
Using \iref{eqLocalDet} (in the previous chapter) we therefore obtain for any $\mu\in \R$
$$
\sqrt{\det H((r_0+\mu) v)} \geq (1-|\mu| n(v))^d\sqrt{\det H(r_0v)} \geq \frac{(1-|\mu| n(v))^d } {n(v)(\lambda\sqrt \delta)^{d-1} }
$$
hence 
\begin{eqnarray*}
m(H) &\geq &\int_\bbS \int_{-r_0}^{r_0} \frac{(r_0+\mu)^{d-1} (1-|\mu| n(v))^d d\mu dv}{n(v)(\lambda\sqrt \delta)^{d-1}}\\
&\geq &\int_\bbS \int_0^{\frac 1{2n(v)}} \frac{r_0^{d-1} (1/2)^d d\mu dv}{n(v)(\lambda\sqrt \delta)^{d-1}}\\
&=& \frac{\omega r_0^{d-1}}{2^d (\lambda\sqrt \delta)^{d-1}} %= \frac{\omega r_0^{d-1}}{2^d (\lambda)^{d-1}}\delta^{-\frac{d-1} 2},
\end{eqnarray*}
We thus obtain the announced result \iref{eqHGLower}
$$
m_g(X,Y_\delta) \geq c \delta^{-\frac {d-1} 2} \stext{ where } c=\frac{\omega r_0^{d-1}}{2^d \lambda^{d-1}},
$$
which concludes the proof of this lemma. \sq
\end{itemize}

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Meshing/ConstrainedMesh.pdf}
\caption{Weak separation of two sets by a triangulation. \label{figWeakSeparation}}
\end{figure}

\begin{remark}[Constrained triangulations] 
A variation of the problem considered in this section is often considered in the litterature. 
We say that a mesh $\cT\in \bT$ weakly separates two regions $X, Y \subset \R^d$ if 
$$
\interior(V_\cT(X)) \cap \interior(V_\cT(Y)) = \emptyset,
%\mathring {V_\cT(X)} \cap \mathring{V_\cT(Y) } = \emptyset
$$
where $\interior(E)$ refers to the collection of interior points of $E$. 

%The optimization problems related to the weak separation of two sets generally cannot rephrased in terms of metrics (??? probably false???).
A common approach for weakly separating two closed and disjoint sets $X,Y\subset \R^d$, is to use the following approach which is based on \emph{constrained mesh} generation.
The first step is to build a polygonal hypersurface $\Gamma$ such that for any path $\gamma \in C^0([0,1], \R^d)$ satisfying $\gamma(0) \in X$ and $\gamma(1)\in Y$, there exists $s\in [0,1]$ such that $\gamma(s) \in \Gamma$.
The second step is to build a mesh $\cT$ of the domain $\Omega$ which is \emph{constrained} to contain the polygonal surface $\Gamma$ in its skeleton.

The main advantage of weak separation is that it can be achieved efficiently without anisotropic simplices, see Figure \ref{figWeakSeparation}. Heuristically the same number of simplices is required to separate the sets $X$ and $Y_\delta$ ``weakly'' with an isotropic triangulation, or ``strongly'' with a graded triangulation.
%The techniques of constrained mesh generation are out of the scope of this thesis, (and are not based on riemannian metrics). 
We refer the interested reader to \cite{Shew3} for a survey on constrained mesh generation.
\end{remark}

\section{Approximation in a given norm}

We compare in this section the approximation error, measured in the $L^p$ norm or the $W^{1,p}$ semi norm, of a function $f$ on a mesh $\cT$ by finite elements with the error associated to $f$ and a metric $H$ adapted to $\cT$.
The integer $m\geq 2$ is fixed in this chapter and the next, and we consider finite elements of degree $m-1$.

For that purpose we introduce some notation.
The greek letter $\alpha$ always refers %in this section 
to a $d$-plet of non-negative integers
$$
\alpha = (\alpha_1, \cdots, \alpha_d) \in \Z_+^d.
$$
%For each $\alpha$ we define the following quantities
%$$
%|\alpha|:= \sum_{1\leq i\leq d} \alpha_i \stext{ and } \alpha! := \prod_{1\leq i\leq d} \alpha_i!. %, \quad \max(\alpha) := \max_{1\leq i\leq d} \alpha_i.
%$$
We define the monomial
$$
Z^\alpha := \prod_{1\leq i\leq d} Z_i^{\alpha_i},
$$
where the variable is $Z=(Z_1,...,Z_d)$, and 
we denote by $\P_k$ the collection of all polynomials of degree at most $k$.
$$
\P_k := \Vect\{Z^\alpha \sep |\alpha|\leq k\}.
$$


We now introduce the main tool of our analysis : the distorted mollification $f_H$ of a function by a metric $H$.
For that purpose we introduce a fixed function $\vp\in L^\infty(\R_+, \R)$ supported in $[0,1)$ and satisfying the following moments property: for all $\mu\in \P_{m-1}$ one has 
\be
\label{eqPhiMoments}
\int_{\sR^d} \mu(z) \vp(|z|) dz = \mu(0).
\ee
For any $f\in L^1_\loc(\R^d)$ and any $H\in \bH$ we denote by $f_H$ the convolution of $f$ with $\vp(|\cdot|)$ distorted by the metric $H$, referred to as the distorted mollification of $f$ by $H$, which is defined as follows
\begin{eqnarray}
\label{defConvH}
f_H(z) &:=& \int_{\sR^d} f(z+H(z)^{-\frac 1 2} u) \vp(|u|) du\\
\label{convHDet}
&=& \sqrt{\det H(z)}\int_{\sR^d} f(z+u) \vp(\|u\|_{H(z)}) du
\end{eqnarray}
Note that $\mu_H = \mu$ for any polynomial $\mu\in \P_{m-1}$. Indeed we obtain using the moments property \iref{eqPhiMoments} that for all $z\in \R^d$ 
$$
\mu_H(z) = \mu(z+H(z)^{-\frac 1 2} 0) = \mu(z).
$$



The next proposition establishes that the distorted mollification $f\mapsto f_H$ is bounded in some functional spaces. 
\begin{lemma}
%Consider a metric $H\in \bH$.
\begin{enumerate}
\item (Boundedness from $L^1_\loc$ to $C^0$) For any $H\in \bH$ and any $f\in L^1_\loc$ we have $f_H\in C^0(\R^d)$. Furthermore one has for any $z\in \R^d$ 
\be
\label{eqFHBounded}
|f_H(z)|\leq \sqrt{\det H(z)} \, \|\vp\|_{L^\infty} \|f\|_{L^1(B_H(z))},
\ee
where $B_H(z) := \{u\in \R^d \sep \|u\|_{H(z)} <1\}$.
\item (Boundedness from $W^{1,1}_\loc$ to $W^{1,\infty}_\loc$) If $H\in \bH_a$ and $f\in W^{1,1}_\loc$, then $f_H\in W^{1,\infty}_\loc$. Furthermore for any $z\in \R^d$ one has 
$$
\dil_z (f_H)  \leq 2 \sqrt{\det H(z)} \|\vp\|_{L^\infty} \|\nabla f\|_{L^1(B_H(z))}
$$
where $\dil_z(f_H) := \lim_{\ve \to 0} \|\nabla f_H\|_{L^\infty(B(z,\ve))}$ is the local dilatation of $f$ at $z$.
\end{enumerate}
\end{lemma}

\proof
We first establish 1. The continuity of $f_H$ follows from the expression \iref{defConvH} of the distorted mollification, and from general results on parameter dependent integrals. Inequality \iref{eqFHBounded} follows from the fact that $\vp$ is supported on $[0,1)$ and from \iref{convHDet}.

We now turn to 2. Metrics $H\in \bH_a$ satisfy $\|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\|\leq |z-z'|$ for any $z,z'\in \R^d$, see their definition \iref{eqLipAdd} (in the previous chapter). Hence for any fixed $u\in B(0,1)$ the map 
$$
z\mapsto z+H(z)^{-\frac 1 2} u
$$
is $2$-Lipschitz.
Derivating \iref{defConvH} under the integral sign we therefore obtain 
\begin{eqnarray*}
\dil_z (f_H) &\leq& \int_{\sR^d} 2|\nabla f(z+H(z)^{-\frac 1 2} u)| \, |\vp(|u|)| du\\
&\leq& 2 \|\vp\L_{L^\infty} \int_{\sR^d} |\nabla f(z+H(z)^{-\frac 1 2} u)|  du\\
&=& 2 \sqrt{\det H(z)} \|\vp\|_{L^\infty} \|\nabla f\|_{L^1(B_H(z))}
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

Before turning to the detail of our results, we fix some notations. For any metric $H\in \bH$, any point $z\in \R^d$ and any radius $r>0$ we define
$$
B_H(z,r) := \{z+u \sep \|u\|_{H(z)} \leq 1\},
$$
as well as 
$$
B_H(z) := B_H(z,1) \stext{ and } B(z,r) := B_{\Id}(z,r)
$$
(the latter being the standard open euclidean ball).
Note that 
\be
\label{eqVolBall}
|B_H(z,r)|\sqrt {\det H(z)} = \omega \, r^d \stext{ where } \omega := |B(0,1)|.
\ee

\subsection{Comparison of the error associated to a mesh and to a metric}
\label{subsecErrMeshMetLP}

This subsection is devoted to the proof of the following proposition, 
which that the finite element approximation error measured in the $L^p$ norm of a function $f$ on a mesh $\cT$, is controlled by the error $e_H(f)_p$ associated to a metric $H$. The mesh $\cT$ needs to be ``more refined'' than the metric $H$, in the following sense :
\be
\label{eqHT4}
4^2H(z) \leq \cH_T,\;\; T\in\cT, \; z\in T.
\ee
\begin{prop}
\label{propErrMeshMetIntro}
There exists a constant $C=C(m,d, \vp)$ such that the following holds. Let $H\in \bH_\per \cap \bH_g$ and  
$\cT\in \bT_\per$ be such that \iref{eqHT4} holds.
Then for all $1\leq p \leq \infty$ and all $f\in L^p_\per$ we have 
$$
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p([0,1]^d)} \leq C e_H(f)_p,
$$
where we denoted $H' := 4^2 H$.
\end{prop}


Our next lemma studies the variations, in terms of volume and inclusion, of the balls $B_H(z,r)$ as $z\in \R^d$ and $r>0$ vary and when $H\in \bH_g$ is a graded metric. 

\begin{lemma}
\label{lemmaEllIncl}
Let $H\in \bH_g$ and let $z\in \R^d$. %let $H' := 4^2 H$
\begin{enumerate}
\item  For any $z'\in B_{H'}(z,2)$ one has $B_{H'}(z')\subset B_H(z)$ and $|B_{H'}(z')|\geq 8^{-d} |B_H(z)|$.
\item For any $z'\in B_{H'}(z, 2/3)$ one has $B_{H'}(z',2)\supset B_{H'}(z)$. % and ...%$B_{H'}(z')\geq 4^{-2d} B_H(z)$.
\end{enumerate}
\end{lemma}

\proof
%We recall some regularity properties of the metrics in $\bH_g$, see \iref{eqLocalNorm}. 
We recall, see \iref{eqLocalNorm}, that for any $H \in \bH_g$, and for any $z,u,v\in \R^d$ satisfying $\|u\|_{H(z)}<1$ one has 
\be
\label{eqLocalNorm2}
\|v\|_{H(z+u)} (1-\|u\|_{H(z)} ) \leq \|v\|_{H(z)}\leq \|v\|_{H(z+u)} (1-\|u\|_{H(z)})^{-1},
\ee
and 
$$
\sqrt{\det H(z+u)} (1-\|u\|_{H(z)} )^d \leq \sqrt{\det H(z)} \leq \sqrt{\det H(z+u)} (1-\|u\|_{H(z)} )^{-d}.
$$
Observing that $|B_H(z)| = 4^d |B_{H'}(z)| = \omega \sqrt {\det H(z)}$, where $\omega$ denotes the volume of the $d$-dimensional unit ball $B(0,1)$, we easily obtain the announce volume estimate.  We thus turn to the properties of inclusion.
\begin{enumerate}
\item 
We have $2 \geq \|z-z'\|_{H'(z)} = 4  \|z-z'\|_{H(z)}$. 
Hence  we obtain for any $q\in \R^d$, using \iref{eqLocalNorm2} in the second line,
\begin{eqnarray*}
\frac 1 4 \|q-z'\|_{H'(z')} &=&  \|q-z'\|_{H(z')}\\
&\geq & (1-\|z'-z\|_{H(z)}) \|q-z'\|_{H(z)}\\
& \geq & (1-\|z'-z\|_{H(z)}) (\|q-z\|_{H(z)}-\|z'-z\|_{H(z)})\\
& \geq & (1-1/2) (\|q-z\|_{H(z)}-1/2)
\end{eqnarray*}
If $\|q-z\|_{H(z)}> 1$ then the previous equation implies $\|q-z'\|_{H'(z')}> 1$.
We have thus established that $\R^d \sm B_H(z) \supset \R^d \sm B_{H'}(z')$ which is equivalent to the announced inclusion $B_{H'}(z')\subset B_H(z)$.

\item We obtain for any $q\in \R^d$ %Recalling that $4 \|z-z'\|_{H(z)} = \|z-z'\|_{H(z')} \leq 2/3$ we obtain for any $q\in \R^d$
\begin{eqnarray*}
\|q-z'\|_{H'(z')} &\geq & (1-\|z'-z\|_{H(z)}) \|q-z'\|_{H'(z)}\\
& \geq & (1-\|z-z'\|_{H'(z)}/4) (\|q-z\|_{H'(z)}-\|z'-z\|_{H'(z)})\\
& \geq & (1-1/6) (\|q-z\|_{H'(z)}-2/3). %= 10/9 >1. %(2/3)/4
\end{eqnarray*}
If $\|q-z\|_{H'(z)} \geq 2$ then $\|q-z'\|_{H'(z')} \geq 10/9 >1$. Hence $B_{H'}(z',2)\supset B_{H'}(z)$ as announced which concludes the proof of this lemma.\sq
\end{enumerate}

The next lemma estimates the \emph{local} finite element approximation error, close to a point $z$.

\begin{lemma}
There exists $C=C(m,d, \vp)$ such that the following holds. Let $H\in \bH_g$, $\cT\in \bT$, $z\in \R^d$ and let 
$$
\cT_z := \{T\in \cT \sep T \subset B_{H}(z,1/2)\}.
$$
Then 
\be
\label{eqLocalMeshMet}
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p(\Omega_z)} \leq C \, e_H(f\sep z)_p.
\ee
where $H':=4^2 H$ and $\Omega_z$ denotes the union of all triangles in $\cT_z$.
\end{lemma}

\proof
We denote by $C_{\interp}$ the norm of the interpolation operator $\interp_\TEq^{m-1} : C^0(\TEq) \to C^0(\TEq)$, and we observe using a change of variables that for any triangle $T$ and any $g\in C^0(T)$ one has 
$$
\|\interp_T^{m-1} g\|_{L^\infty(T)}\leq C_{\interp} \|g\|_{L^\infty(T)}.
$$


Let $\mu\in \P_{m-1}$ be a polynomial satisfying $\|f-\mu\|_{L^p(B_H(z))} = e_H(f\sep z)_p$.
Let $g := f-\mu$ and let $T\in \cT_z$. 
We have 
\begin{eqnarray*}
\|\interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq & |T|^\frac 1 p \|\interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
&\leq & C_{\interp} |T|^\frac 1 p \|g_{H'}\|_{L^\infty(T)}\\
&\leq & C_{\interp} |T|^\frac 1 p \|g_{H'}\|_{L^\infty(B_{H'}(z,2))}\\
&\leq & C_{\interp} \|\vp\|_{L^\infty} |T|^\frac 1 p \max_{z'\in B_{H'}(z,2)}  \frac{\|g\|_{L^1(B_{H'}(z'))}}{|B_{H'}(z')|}\\
&\leq & \omega 8^d C_{\interp}  \|\vp\|_{L^\infty}  |T|^\frac 1 p \frac{\|g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|},
\end{eqnarray*}
where we used \iref{eqFHBounded} in the fourth line and Lemma \ref{lemmaEllIncl}, point 1., in the last line.

Defining $C_* := \omega 8^d C_{\interp}  \|\vp\|_{L^\infty}$ we thus obtain
\begin{eqnarray*}
\|\interp_\cT^{m-1} g_{H'}\|_{L^p(\Omega_z)} &=& \left(\sum_{T\in \cT_z} \|\interp_T^{m-1} g_{H'}\|_{L^p(T)}^p \right)^{\frac 1 p} \\
&\leq & C_* \frac{\|g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|} \left(\sum_{T\in \cT_z} |T|\right)^\frac 1 p\\
& \leq & C_* \|g\|_{L^1(B_{H}(z))}|B_{H}(z)|^{\frac 1 p-1}\\
& \leq & C_* \|g\|_{L^p(B_{H}(z))}
\end{eqnarray*}
Since the twisted convolution reproduces polynomials in $\P_{m-1}$ , as well as the interpolation operator $\interp_\cT^{m-1}$, we have
$$
g-\interp_\cT^{m-1} g_H = (f-\mu)-\interp_\cT^{m-1} (f-\mu)_H = f-\interp_\cT^{m-1} f_H.
$$ 
Therefore  
\begin{eqnarray*}
\|f-\interp_\cT^{m-1} f_H\|_{L^p(\Omega_z)} &=& \|g-\interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)} \\
&\leq &\|g\|_{L^p(\Omega_z)}+ \|\interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)}\\
& \leq & (1+C_*) \, \|g\|_{L^p(B_{H}(z))}\\
&=& (1+C_*) \, e_H(f\sep z)_p
\end{eqnarray*}
which concludes the proof.
\sq

\begin{prop}
\label{propErrMeshMet}
There exists $C=C(m,d)$ such that the following holds. Let $H\in \bH_g$, and let $H' := 4^2 H$. Let also $f\in L^p_\loc$.
\begin{itemize}
\item (Local error estimate) 
Let $\cT\in \bT$, let $z\in \R^d$ and let 
$$
\cT_z := \{T\in \cT \sep T \subset B_{H'}(z,2)\}
$$
and let $\Omega_z$ be the union of all triangles in $\cT_z$.
Then 
\be
\label{eqLocalMeshMet}
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p(\Omega_z)} \leq C \, e_H(f\sep z)_p.
\ee
%Let $T$ be a simplex let $z\in T$, and assume that $\cH_T \geq H'(z)$.
%
%For any $f\in L^p_\loc$ one has 
%$$
%\|f-\interp_T^{m-1} f_{H'}\|_{L^p} \leq C e_H(f\sep z)_p,
%$$
%where $C=C(m,d)$. ($C$ is independent of $H$, $T$ and $f$.)
\item (Global error estimate) Let $\cT\in \bT$ and assume that for all $T\in \cT$ and all $z\in \cT$ one has 
\be
\label{eqHTHp}
\cH_T \geq H'(z).
\ee
The quasi-interpolation error of $f$ is controlled by the error associated to the metric $H$
$$
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p([0,1]^d)} \leq C \, e_H(f)_p. 
$$
\end{itemize}
\end{prop}

\proof
\begin{itemize}
\item (Local error estimate)
\item (Global error estimate)
For each triangle $T\in \cT$ we define 
$$
\Omega_T := \{z\in \R^d \sep T \subset B_{H'}(z,2)\} \stext{ and } n(T) := \int_{\Omega_T} \sqrt{\det H(z)} dz.
$$
Denoting by $z_T$ the barycenter of $T$, we have $T\subset B_{H'}(z_T)$ according to \iref{eqHTHp}.
Point 2. of \ref{lemmaEllIncl} thus implies that $B_{H'}(z_T,2/3) \subset \Omega_T$.
Eventually $n(T)$ is bounded below a constant independent of $H$ and $\cT$
$$
n(T) \geq |B_{H'}(z_T,2/3)| \min_{z\in B_{H'}(z_T,2/3)}  \sqrt{\det H(z)} \geq \omega 6^{-d} (1-1/2)^d (1-1/2-1/6)^d
$$
%(could be improved...??)
We denote by $\cT_*$ a system of representatives of $\cT$ for the equivalence relation 
$$
T \sim T' \stext{ if } T =T'+u \text{ for some } u \in \Z^d.
$$
Using the local estimate \iref{eqLocalMeshMet} we therefore obtain 
\begin{eqnarray*}
C^p e_H(f)_p^p &=& C^p\int_{z\in [0,1]^d} \sqrt{\det H(z)} \, e_H(f\sep z)_p^p dz\\
&\geq&  \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \|f-\interp_\cT^{m-1} f_H\|_{L^p(\Omega_z)}^p dz \\
&=&  \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \sum_{T\in \cT_z} \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p dz \\
&=& \sum_{T\in \cT_*} n_T \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p \\
& \geq &  \|f-\interp_\cT^{m-1} f_H\|_{L^p([0,1]^d)}^p \min_{T \in \cT} n_T,
\end{eqnarray*}
which concludes the proof of this proposition. \sq
\end{itemize}


\subsection{Comparison of the error associated to a mesh and to a metric}
\label{subsecErrMeshMetW1P}

We compare in this section the $W^{1,p}$ finite element approximation error of a function on a mesh with the errors $e_H^a(\nabla f)_p$ or $e_H^g(\nabla f)_p$ associated to a metric. 
Let us recall that for any $f\in W^{1,p}_\per$, $H\in \bH_\per$ and $\star\in \{a,g\}$ one has 
$$
e_H^\star(\nabla f)_p := \left\|\sqrt[2p]{\det H(z)} \, e_H^\star(\nabla f\sep z)_p\right\|_{L^p([0,1]^d)}
$$
where 
\begin{eqnarray*}
e_H^a(\nabla f\sep z) &:=& \inf_{\nu \in \sP_{m-2}^d} \|\nabla f-\nu\|_{L^p(B_H(z))}\\
% \stext{ and } 
e_H^g(\nabla f\sep z) &:=& \sqrt{\|H(z)\|}\inf_{\nu \in \sP_{m-2}^d} \|H(z)^{-\frac 1 2} (\nabla f-\nu)\|_{L^p(B_H(z))}.
\end{eqnarray*}
Observe that $e_H^a(\nabla f)_p\leq e_H^g(\nabla f)_p$. This inequality, which deteriorates as the metrics $H$ becomes more anisotropic, is the price to pay for the use of graded meshes and metrics instead of quasi-acute ones.

Before turning to the details of these proofs, we establish a common lemma which states that the optimization among all $\nu \in \P_{m-2}^d$ involved in the definition of $e_H^a(f\sep z)_p$ and $e_H^g(f\sep z)_p$ can be replaced with an optimization among gradients of polynomials $\nabla \mu$, where $\mu\in \P_{m-1}$.

\begin{lemma}
\label{lemmaProj}
\begin{itemize}
\item (Orthogonal projection is compatible with gradients)
We equip the space $L^2(B(0,1), \R^d)$ with the scalar product 
$$
\<v,w\> := \int_{B(0,1)} v(z)\cdot w(z) dz.
$$
For any $f\in H^1(B(0,1))$ there exists $\mu\in \P_{m-1}$ such that the orthogonal projection of $\nabla f$ onto $\P_{m-2}^d$ is $\nabla \mu$.
\item (Optimization among gradients)
There exists $C_\proj=C_\proj(m,d)$ such that for any ellipsoid $\cE\subset \R^d$, any $1\leq p \leq \infty$ and any $f\in W^{1,p}(\cE)$ one has  %and any $A\in \GL_d$ 
one has 
\be
\label{eqGradApp}
\inf_{\mu \in \sP_{m-1}} \|\nabla f-\nabla \mu\|_{L^p(\cE)}
\leq 
C_\proj \inf_{\nu \in \sP_{m-2}^d} \|\nabla f-\nu\|_{L^p(\cE)}
\ee
%$$
%\inf_{\mu \in \sP_{m-1}} \|A(\nabla f-\nabla \mu)\|_{L^p(\cE)}
%\leq 
%C_\proj \inf_{\nu \in \sP_{m-2}^d} \|A(\nabla f-\nu)\|_{L^p(\cE)}
%$$
\end{itemize}
\end{lemma}

\proof
\begin{itemize}
\item (Orthogonal projection is compatible with gradients) In order to simplify the notations we define $k := m-1$.
We define $\cS := \{z\in \R^d \sep |z| = 1\}$ and we denote by $D_k$ the collection of polynomial vector fields $\nu\in  \P_{k-1}^d$ satisfying %\subset \P_{k-1}^d
$$
\left\{
\begin{array}{cl}
\diver \nu (z)=0 & \text{ for all } z\in B(0,1)\\
\nu(z) \cdot z = 0 &\text{ for all } z\in \cS
\end{array}
\right.
$$
For any $g\in H^1(B(0,1))$ and any $\nu \in D_k$ we thus have   
\be
\label{eqGradDiv}
\int_{B(0,1)} \nabla g \cdot \nu = -\int_{B(0,1)} g(z) \diver \nu(z)dz + \int_{\cS} g(z)  \, \nu(z) \cdot z \, dz =0.
\ee
%therefore the same holds for the orthogonal projection of $\nabla f$ onto $\P_{k-1}^d$.
Our purpose is now to establish the orthogonal decomposition
$$
\P_{k-1}^d = D_k \oplus \nabla \P_k.
$$
Equation \iref{eqGradDiv} shows that $\nabla \P_k$ and $D_k$ are orthogonal, and we know that $\dim \nabla \P_k = \dim \P_k -1$. Therefore we only have to show that 
$\dim D_k \geq \dim (\P_k^{d-1})  - \dim \P_k +1$.

The vector space $D_k$ is the kernel of the map $d_k$ defined as follows
$$
\begin{array}{ccc}
d_k :\P_{k-1}^d &\to& \P_{k-2} \oplus \P_k(\cS)\\
\nu  &\mapsto & (\diver \nu, \ (\nu (z) \cdot z)_{|\cS}),
\end{array}
$$
where  
$
\P_k(\cS)
$
denotes the collection of restrictions to $\cS$ of elements of $\P_k$. 
The kernel of the map
$$
\begin{array}{ccc}
\gamma_k : \P_k &\to & \P_k(\cS)\\
\mu &\mapsto &\mu_{|\cS}
\end{array}
$$
is 
$
\Ker(\gamma_k) = (1-|z|^2) \P_{k-2}.
$
Hence 
$
\dim(\P_k(\cS)) = \dim \P_k - \dim \P_{k-2}.
$

The map $d_k$ is not surjective, indeed we have the linear relation 
$$
\int_{B(0,1)} \diver \nu(z)\, dz = \int_\cS \nu(z)\cdot z \, dz,
$$
%if $\diver(V) = 0$, then $\int_{\partial E} \<V,\n\> = 0$, 
hence in particular $(0,1) \notin \Image(d_k)$.
Therefore 
\begin{eqnarray*}
\dim D_k &=& \dim \Ker d_k \\
&=& \dim (\P_k^{d-1}) - \dim \Image d_k \\
&\geq &  \dim (\P_k^{d-1}) - (\dim \P_{k-2} + \dim \P_k(\Gamma) -1) \\
&=& \dim (\P_k^{d-1})  - \dim \P_k +1,
\end{eqnarray*}
which implies the orthogonal decomposition $\P_{k-1}^d = D_k \oplus \nabla \P_k$ as announced.

Eventually for any $f\in H^1(B(0,1))$ the equation \iref{eqGradDiv} shows that $\nabla f$ is orthogonal to $D_k$. Therefore the orthogonal projection of $\nabla f$ onto $\P_{k-1}^d$ is also orthogonal to $D_k$, and therefore is an element of $\nabla \P_k$ as announced, which concludes the proof.

\item
We denote by $Q : L^2(B(0,1),\R^d) \to \P_{k-1}^d$ the $L^2(B(0,1))$ orthogonal projection.
We recall that for any $v\in L^2(B(0,1),\R^d)$ the projection $Q(v)\in \P_{k-1}^d$ is defined by the collection of linear conditions
$$
\int_{B(0,1)} (v-Q(v))\cdot \nu  = 0 \text{ for all } \nu \in \P_{k-1}^d.
$$
Hence $Q(v)$ depends linearly on a finite number of moments of $v$, and therefore continuously extends to all $v\in L^1(B(0,1), \R^d)$. Therefore there exists a constant $C_0$ such that for all $1\leq p \leq \infty$ and all $v\in L^p(B(0,1),\R^d)$
$$
\|Q(v)\|_{L^p(B(0,1))} \leq C_0 \|v\|_{L^p(B(0,1))}.
$$
For any $A\in \GL_d$ and any $v\in L^2(B(0,1),\R^d)$ we claim that $Q(A(v)) = A(Q(v))$. Indeed for any $\nu\in \P_{k-1}^d$ one has 
$$
\int_{B(0,1)} (A(v(z))-A(Q(v(z))))\cdot \nu(z) dz= \int_{B(0,1)} (v(z)-Q(v(z))\cdot (A^\trans(\nu(z))) dz = 0.
$$
Consider  $1\leq p \leq \infty$, $f\in W^{1,p}(B)$ and $A\in \GL_d$. Let $\mu\in \P_{m-1}$ be such that $Q(\nabla f) = \nabla \mu$, and let $\nu \in \P_{m-1}^d$, we obtain 
\begin{eqnarray*}
\|A(\nabla f-\nabla \mu)\|_{L^p(B(0,1))} &=& \|A(\nabla f)-A(Q(\nabla f))\|_{L^p(B(0,1))}\\
&=& \|A(\nabla f)-Q(A(\nabla f))\|_{L^p(B(0,1))}\\
& = & \|A(\nabla f-\nu)-Q(A(\nabla f)-\nu)\|_{L^p(B(0,1))}\\
&\leq& (1+C_0)  \|A(\nabla f-\nu)\|_{L^p(B(0,1))}.
\end{eqnarray*}
Therefore 
$$
\inf_{\mu\in \sP_{m-1}} \|A(\nabla f-\nabla \mu)\|_{L^p(B(0,1))} \leq (1+C_0) \inf_{\nu\in \sP_{m-2}^d} \|A(\nabla f-\nu)\|_{L^p(B(0,1))}
$$
We obtain the announced result \iref{eqGradApp} using a change of variables from the ellipse $\cE$ to the ball $B(0,1)$, with the constant $C_\proj := C_0+1$. This concludes the proof of this proposition.\sq
\end{itemize}


\subsubsection{Graded triangulations and metrics} 
\label{subsubsecErrMeshMetW1PG}

The next lemma estimates the $W^{1,p}$ approximation error of a function $f$ on a graded mesh, in terms of the approximation error $e_H^g(\nabla f)_p$ with respect to a metric. This approach does not allow to recover the optimal anisotropic error estimates for $W^{1,p}$ norms developed in Chapter \ref{chapW1P}. However it is perhaps more taylored to current anisotropic mesh generation software, which generally do not guarantee a bound on the angles. 
%Some classical approximation theory results also seem easier to generalise to the anisotropic context using this approach, as illustrated the Sobolev inequality presented in Proposition \ref{propSob}.

\begin{prop}
For all $C_0\geq 1$ there exists $C=C(C_0,m,d)$ such that the following holds. Let $H\in \bH_g$, and let $H' := 4^2 H$, let $\cT\in \bT$ and assume that for all $T\in \cT$ and all $z\in T$
$$
H'(z) \leq \cH_T \leq C_0^2 H'(z).
$$
\begin{itemize}
\item (Local error estimate) 
Let $T\in \cT$ and let $z\in T$, then 
\be
\label{eqLocGW1P}
\|\nabla (f- \interp_\cT^{m-1} f_{H'})\|_{L^p(T)} \leq C e_H^g(\nabla f\sep z)_p.
\ee
\item (Global error estimate)
One has
$$
\|\nabla (f- \interp_\cT^{m-1} f_{H'})\|_{L^p([0,1]^d)} \leq C e_H^g(\nabla f \sep z)_p.
$$
\end{itemize}
\end{prop}

\proof %The proof is extremely similar to the proof of Lemma ??, for the approximation in the $L^p$ norm.

\begin{itemize}
\item
We assume in a first time that $z=0$ and that $H(z) = \Id$, in such way that $B_H(z) = B(0,1)$ is the euclidean unit ball, denoted below by $B := B(0,1)$.
We consider a polynomial $\mu\in \P_{m-1}$ such that 
$
\|\nabla (f-\mu)\|_{L^p(B)}
$
is minimal, and such that $\int_B (f-\mu) = 0$. The latter point can be ensured by adding an appropriate constant to $\mu$. Defining $g:=f-\mu$, we obtain using Lemma \ref{lemmaProj}
$$
\|\nabla g\|_{L^p(B)} \leq C_\proj \,e_H(f\sep z)_p.
$$
%Sobolev Injection's Theorem states that the embedding 
According to Sobolev's injection theorem, recalling $g\in W^{1,1}(B)$ and that $\int_B g=0$, there exists a constant $C_\sob=C_\sob(m,d)$ such that 
$$
\|g\|_{L^1(B)} \leq C_\sob \|\nabla g\|_{L^1(B)}
$$
The function $g_{H'}$, which is continuous on $T$, satisfies 
$$
\|g_{H'}\|_{L^\infty(T)} \leq \|\vp\|_{\infty} \frac{\max_{z'\in T} \|g\|_{L^1(B_{H'}(z'))}}{\min_{z'\in T} |B_{H'}(z')|} \leq C_1 \|g\|_{L^1(B)},
$$
where $C_1 := \|\vp\|_\infty\volBall^{-1} 8^d$. %details? 
We denote by $C_{\interp}$ the norm of the operator defined on the reference equilateral triangle $\nabla \interp_\TEq^{m-1} : C^0(\TEq)\to \P_{m-2}^d$. Thus for any $h\in C^0(\TEq)$
$$
\|\nabla \interp_\TEq^{m-1} h\|_{L^\infty(\TEq)} \leq C_{\interp} \|h\|_{L^\infty(\TEq)}. 
$$
Recalling that $\cH_T^{\frac 1 2}(T)$ is the image $\TEq$ by a translation and a rotation, and using this change of variables, we obtain for the function $g_{H'}\in C^0(T)$
$$
\|\cH_T^{-\frac 1 2}(\nabla \interp_T^{m-1} g_{H'})\|_{L^\infty(T)} \leq C_{\interp} \|g_{H'}\|_{L^\infty(T)}.
$$
Thus 
$$
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)} \leq C_{\interp}\|\cH_T^\frac 1 2\|  \|g_{H'}\|_{L^\infty(T)},
$$
and eventually, since $\cH_T\leq C_0^2 H'(z) = 4^2 C_0^2 \Id$ and since $|T|\leq |B|$,
\begin{eqnarray*}
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq& |B|^\frac 1 p \|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
& \leq & 4C_0 C_{\interp} |B|^\frac 1 p   \|g_{H'}\|_{L^\infty(T)}\\
& \leq & 4C_0 C_1 C_{\interp} |B|^\frac 1 p   \|g\|_{L^1(B)}\\
& \leq & 4C_0 C_1 C_{\interp} C_\sob |B|^\frac 1 p   \|\nabla g\|_{L^1(B)}\\
&\leq &  4C_0 C_1 C_{\interp} C_\sob |B|  \|\nabla g\|_{L^p(B)}\\
\end{eqnarray*}
Defining $C_* := 4C_0 C_1 C_{\interp} C_\sob |B|$ we thus obtain 
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)} &=& \|\nabla (g-\interp_T^{m-1} g)\|_{L^p(T)}\\
&\leq& (1+C_*) \|\nabla g\|_{L^p(B)}\\
&\leq& (1+C_*) C_\proj e_H(\nabla f\sep z)_p
\end{eqnarray*}

We now turn to the general case, and we do not any more assume that $z=0$ and $H(z) =\Id$.
We define the affine change of coordinates $\Phi(z') := H(z)^{-\frac 1 2} z'+z$, and we apply our previous reasonning to the metric $H_\Phi$, the triangle $T_\Phi := \Phi^{-1}(T)$ which is equilateral and centered at the origin, and the function $f_\Phi := f\circ \Phi$.
We thus obtain 
$$
\|\nabla (f_\Phi-\interp_{T_\Phi}^{m-1} f_\Phi)\|_{L^p(T_\Phi)} \leq C e_{H_\Phi}(\nabla f_\Phi \sep 0)_p
$$
where $C := (1+C_*) C_\proj$. It follows that 
$$
\|H(z)^{-\frac 1 2} (\nabla (f-\interp_T^{m-1} f))\|_{L^p(T)} \leq C e_{H}(H(z)^{-\frac 1 2}(\nabla f) \sep z)_p.
$$
which concludes the proof since $\|H(z)\|^\frac 1 2 e_H(H(z)^{-\frac 1 2}(\nabla f) \sep z)_p = e_H^g(f\sep z)_p$.

\item
For any $T\in \cT$ and any $z\in T$,  recalling that $\cH_T\leq C_0^2 H(z) = (4C_0)^2 H(z)$ we obtain 
$$
|\TEq|/|T| =  \sqrt{\det \cH_T} \leq (4C_0)^d  \sqrt{\det H(z)}.
$$
Averaging  \iref{eqLocGW1P} over $T$, it follows that 
$$
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)}^p \leq \frac C {|T|} \int_T e_H^g(f\sep z)_p^p dz \leq C'  \int_T \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz
$$
where $C' := (4C_0)^d C/|\TEq|$.We denote by $\cT_0$ a collection of representatives in $\cT$ for the equivalence relation : $T\sim T'$ if and only if there exists $u\in \Z^d$ such that $T' = u+T$. We thus obtain
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p([0,1]^d)}^p &=& \sum_{T\in \cT_0} \|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)}^p \\
&\leq& C'  \sum_{T\in \cT_0} \int_T \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz\\
&=& C'  \int_{[0,1]^d} \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz
\end{eqnarray*}
which concludes the proof of this proposition.
\sq
\end{itemize}

\subsection{Isotropic approximation}
%\subsection{Approximation spaces}
%\label{subsecApproxSpaceLP}




We present in this subsection a (naive) definition of anisotropic approximation spaces, which are based on the approximation of a function with respect to a metric, measured in the $L^p$ norm and approximating locally with $\P_{m-1}$ polynomials. This approach is strongly tied with the study [Petrushev] of anisotropic Besov spaces associated to ellipsoid covers of $\R^n$.

For any $\star\in \{i,g\}$ and any $f\in L^p_\per$ we define a (nonlinear) quantity $|f|_{\star,p} \in [0, \infty]$ as follows \be
\label{defFStarP}
|f|_{\star,p} := \sup_{\mu \geq 1} \left(\mu^\frac m d\inf_{\substack{H \in \bH_\star\cap \bH_\per\\ m(H) \leq \mu}}e_H(f)_p\right).
\ee
This quantity is more or less understood in the isotropic case $\star = i$, using an approach based on the Hardy-Littlewood maximal function  $\mathfrak M(g)$ associated to a function $g\in L^1_\per$, 
$$
\mathfrak M(g \sep z) := \sup_{r>0} \frac 1 {r^d} \int_{B(z,r)} |g|.
$$
The next lemma gives some key properties of a variant $\gM_\delta$ of the maximal function $\gM$.
\begin{lemma}
For all $\delta > 0$ let,
$$
T_\delta(s) := 
\left\{
\begin{array}{cc}
s & \text{ if } s\geq \delta,\\
0 & \text{ otherwise}.
\end{array}
\right.
$$
Let $g\in L^1_\per(\R^d)$, which is not identically zero, and let
$$
\gM_\delta(g\sep z) := \sup_{r>0} \frac 1 {r^d} T_\delta\left(\int_{B(z,r)} |g|\right).
$$
Then $s_\delta(z) := (\delta/\gM_\delta(g\sep z))^\frac 1 d$ is a positive Lipschitz function and satisfies for all $z\in \R^d$
\be
\label{intSDelta}
\int_{B(z,s_\delta(z))} |g|\leq \delta.
\ee
\end{lemma}

\proof
We consider a fixed value of the parameter $\delta>0$.
Since $g\in L^1_\per$ we have for any $z\in \R^d$ 
$$
\lim_{r\to \infty} \frac 1 {r^d} \int_{B(z,r)}|g| = \volBall \int_{[0,1]^d} |g|>0. %\lim_{r\to \infty} \frac{|B(z,r)|}{r^d}
$$ 
Furthermore there exists $r_0>0$ such that for any $z\in \R^d$ one has 
$$
\int_{B(z,r_0)} |g| < \delta.
$$
Combining the two last equations we obtain that $\gM_\delta(g\sep z)\in (0, \infty)$ for any $z\in \R^d$.
We define $I_\delta(z,r)$ by 
$$
I_\delta(z,r)^d := \frac 1 \delta T_\delta\left(\int_{B(z,r)} |g|\right).
$$
Note that $I_\delta(z,r)\in \{0\} \cup [1, \infty)$ and that for any $z,u\in \R^d$ and and $r>0$
$$
I_\delta(z+u, r)\leq I_\delta(z,r+|u|),
$$
since $B(z+u,r) \subset B(z,r+|u|)$.
Note also that %Furthermore 
\be
\label{defSDelta}
s_\delta(z) = \inf_{r>0} \frac r {I_\delta(z,r)}.
\ee
Let $z,z'\in \R^d$ be such that $|z-z'|\leq r_0$. We therefore have 
\begin{eqnarray*}
s_\delta(z') &=& \inf_{r>0} \frac r {I_\delta(z',r)} \\
& \geq & \inf_{r>0} \frac r {I_\delta(z,r+|z-z'|)} \\
& = & \inf_{r>|z-z'|} \frac{r- |z-z'|}{I_\delta(z,r)}\\ 
& \geq &  \inf_{r>|z-z'|} \frac r {I_\delta(z,r)} - |z-z'| \\
&=&  s_\delta(z)- |z-z'| 
\end{eqnarray*}
In the fourth line we used the fact that one always have $I_\delta(z,r)\geq 1$ or $I_\delta(z,r)=0$, and that the later case does not correspond to the infimum. In the last line we used the fact that $I_\delta(z,r)=0$ for all $r\leq |z-z'| \leq r_0$ %, which implies that $r/I_\delta(z,r) = \infty$, 
and therefore the infimum can be restricted to $r>|z-z'|$.

Exchanging $z$ and $z'$ we obtain that $|s_\delta(z) - s_\delta(z')| \leq |z-z'|$ for all $z,z'\in \R^d$ satisfying $|z-z'| \leq r_0$. 
If $z,z'$ are arbitrary then we consider an integer $n>0$ such that  $|z-z'| \leq n r_0$ and we obtain 
\begin{eqnarray*}
|s_\delta(z) - s_\delta(z')| &\leq& \sum_{1\leq i \leq n} \left|s_\delta\left(\frac {iz} n +\frac{(n-i)z'} n\right)-s_\delta\left(\frac {(i-1)z} n +\frac{(n-i+1)z'} n\right) \right| \\
&\leq& n \frac{|z-z'|} n = |z-z'|, 
\end{eqnarray*}
hence $s_\delta$ is Lipschitz on $\R^d$ as announced.


The proof of the second point  \iref{intSDelta} is simpler. Indeed injecting $r = s_\delta(z)$ in \iref{defSDelta} we obtain 
$$
s_\delta(z) \leq  s_\delta(z) \left(\frac \delta {T_\delta\left(\int_{B(z,s_\delta(z))} g\right)}\right)^{\frac 1 d}.
$$
which implies \iref{intSDelta} and concludes the proof.
\sq

\begin{theorem}
Let $\frac 1 \tau := \frac m d +\frac 1 p$. If $\tau \geq 1$ and if the Sobolev injection $W^{m, \tau} \to L^p$ holds (which excludes the case $m=1$ and $p=\infty$) then one has
$$
|f|_{i,p} \leq C\left(\int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz\right)^\frac 1 \tau,
$$
where $C=C(m,d,p)$.
\end{theorem}

\proof
We assume that $d^m f$ is not identically zero, otherwise $f$ is a periodic polynomial of degree $m-1$, thus a constant, and $|f|_{i,p} = 0$.
For each $\delta>0$ we define
$$
H_\delta(z) := \max\{1, \ \gM_\delta(|d^m f|^\tau \sep z)^{\frac 2 d}/\delta^\frac 2 d\} \Id = \frac \Id {\min \{1 , s_\delta(z)\}^2},
$$
where $s_\delta(z) := (\delta/ \gM_\delta(|d^m f|^\tau \sep z))^\frac 1 d$ is a Lipschitz function according to the previous proposition. We observe that $H_\delta\in \bH_i$ and that 
\be
\label{eqMHDelta}
m(H_\delta) \leq \int_{[0,1]^d} \max\{1, \gM_\delta(|d^m f|^\tau \sep z)/\delta\} dz \leq 1+M/\delta.
\ee
where 
$$
M := \int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz.
$$
%Define $B := \{z\in \R^d \sep |z|\leq 1\}$ 
We recall the following classical Sobolev estimate : there exists $C_{\rm sob}$ such that for any $g\in W^{m, \tau}(B(0,1))$
$$
\inf_{\mu\in \sP_{m-1}} \|g-\mu\|_{L^p(B(0,1))} \leq C_{\rm sob} \|d^m g\|_{L^\tau(B(0,1))}.
$$
Using an isotropic change of variables we obtain for any $z\in \R^d$, any $r>0$ and any $g\in W^{m, \tau}(B(z,r))$
$$
\inf_{\mu\in \sP_{m-1}} \|g-\mu\|_{L^p(B(z,r))} \leq C_{\rm sob} \|d^m g\|_{L^\tau(B(z,r))}.
$$
Therefore, using \iref{intSDelta},
\begin{eqnarray*}
e_{H_\delta}(f\sep z)_p &\leq & \inf_{\mu\in \sP_{m-1}} \|f-\mu\|_{L^p(B(z,s_\delta(z)))} \\
& \leq & C_\sob \|d^m f\|_{L^\tau(B(z,s_\delta(z)))}\\
& \leq & C_\sob \delta^\frac 1 \tau.
\end{eqnarray*}
It follows that 
$$
e_{H_\delta}(f)_p^p := \int_{[0,1]^d} \sqrt{\det H_\delta(z)} \, e_{H_\delta}(f\sep z)_p^p \, dz \leq m(H_\delta) (C_\sob \delta^\frac 1 \tau)^p
$$
Recalling that $m(H_\delta)\leq 1+M/\delta$, see \iref{eqMHDelta}, we obtain  
$$
(1+M/\delta)^\frac m d e_{H_\delta}(f)_p \leq  (1+M/\delta)^\frac 1 \tau C_\sob \delta^\frac 1 \tau = C_\sob (\delta+M)^\frac 1 \tau
$$
We apply the previous estimate to the range of parameters $0<\delta \leq M$, which corresponds to the range $2\leq 1+M/\delta< \infty$ of our upper bound for the mass of $H_\delta$, and we obtain 
$$
\sup_{\mu\geq 2} \left(\mu^\frac m d\inf_{\substack{H \in \bH_\star\cap \bH_\per\\ m(H) \leq \mu}}e_H(f)_p\right)\leq C_\sob (2M)^\frac 1 \tau.
$$
In order to estimate $|f|_{i,p}$, see \iref{defFStarP}, we need in addition to address the range of parameters $1\leq \mu \leq 2$. For that purpose we consider the constant metric $H_\infty := \Id$, which satisfies $m(H_\infty)=1$. For any $z\in \R^d$, observing that $B(z,1)$ is covered by $2^d$ translates of the cube $[0,1]^d$, we obtain  
\begin{eqnarray*}
e_{H_\infty}(f\sep z)_p &=& \inf_{\mu\in \sP_{m-1}} \|f-\mu\|_{L^p(B(z,1))} \\
&\leq &C_\sob \|d^m f\|_{L^\tau(B(z,1))} \\
&\leq & 2^d C_\sob \|d^m f\|_{L^\tau([0,1]^d)}\\
& \leq & 2^d C_\sob M^\frac 1 \tau.
%C_\sob \gM(|d^mf|^\tau \sep z)^\frac 1 \tau
\end{eqnarray*}
Where we used the fact that $|d^m f(z)|^\tau \leq \gM(|d^mf|^\tau \sep z)$ for almost every $z\in \R^d$. Therefore $e_{H_\infty}(f)_p \leq 2^d C_\sob M^\frac 1 \tau$ which concludes the proof of this theorem.
\sq

%\begin{theorem}
%There exists a constant $C=C(m,d)$ such that the following holds.\\
%\begin{itemize}
%\item (Quasi triangle inequality) ?? Needs to be checked.
%For all $f,g\in L^p$ one has 
%$$
%|f+g|_{i,p} \leq C (|f|_{i,p}+ |g|_{i,p}).
%$$
%\item (Link to Sobolev norms) If $\tau \geq 1$ and if the Sobolev injection $W^{m, \tau} \to L^p$ holds (which excludes the case $m=1$ and $p=\infty$) then one has
%$$
%|f|_{i,p} \leq C\left(\int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz\right)^\frac 1 \tau.
%$$
%\end{itemize}
%\end{theorem}
%
%\proof
%\begin{itemize}
%\item Consider $\mu\geq 1$ and $H, H'\in \bH_i$, satisfying $m(H) = m(H')=\mu$. There exists two Lipschitz functions $s,s' : \R^d \to R_+^*$ such that $H = Id/s^2$ and $H' =  \Id/s'^2$,
%%$$
%%H = \frac \Id {s^2}, H' =  \frac \Id {s'^2}
%%$$
%and we define
%$$
%\ti H(z) := \frac \Id {\min\{s(z), s'(z)\}^2}.
%$$
%We have $\ti H \in \bH_i$ since the function $z\mapsto \min\{s(z), s'(z)\}$ is Lipschitz. Furthermore 
%$$
%m(\ti H) = \int_{[0,1]^d} \max \left\{\frac 1 {s(z)^d}, \ \frac 1 {s'(z)^d}\right\} dz \leq m(H)+m(H')=2\mu.
%$$
%The approximation error satisfies 
%$$
%e_{\ti H} (f+g)_p \leq e_{\ti H}(f)_p + e_{\ti H}(g)_p \leq ? e_H(f)_p + e_{H'}(g)_p
%$$
%
%
%\item
%\end{itemize}
%\sq

In contrast to $|f|_{i,p}$, %does not satisfy the quasi triangle inequality and 
there is no known relevant %``close to sharp'' 
bound for $|f|_{g,p}$ explicit in terms of the $m$-th derivatives of $f$.
We intend to study this quantity in more detail in the future, but for now we can only make some conjectures. 
In the case $p=m=d=2$, Chapter \ref{chapCartoon} suggests that $|f|_{g,2}$ is finite for any cartoon function $f$, probably with the lower bound 
\be
\label{eqLowerCartoon}
J(f) := \left( \int_{[0,1]^2 \sm \Gamma } |\det d^2 f(z)|^\frac 1 3 dz+ \int_\Gamma |[f](s)|^\frac 2 3 |\kappa(s)|^\frac 1 3\right)^\frac 3 2 \stackrel ? \leq C |f|_{g,2}
\ee
where $[f](s)$ denotes the jump of $f$ at a point $s\in \Gamma$, and $\kappa(s)$ the curvature of $\Gamma$ at $s$.

We study in Chapter \ref{chapCartoon} the convolution of a cartoon function with a mollifier $\psi$ (compactly supported, for simplicity), and we have shown that the left hand side of \iref{eqLowerCartoon} is stable under mollification, see Theorem [??] :  for any cartoon function $f$
\be
\label{eqStableJ}
\lim_{\delta \to 0} J(f*\psi_\delta) \leq C(\psi) J(f) \stext{ where } \psi_\delta := \frac 1 \delta \psi \left( \frac \cdot {\sqrt{\delta}}\right).
\ee
This point is not trivial since the discontinuities of $f$ are traded for an (anisotropic) explosion of the derivatives of $f_\delta$, as $\delta \to 0$.

We consider $f\in L^p_\per$ and denote by $f_t$ the transportation of $f$ by the heat semi-group
$$
\partial f_t + \triangle f_t = 0,
$$
equivalently
$$
f_t = f* \vp_t \stext{ where } \vp_t := \frac 1 t \vp\left(\frac{\cdot}{\sqrt t} \right) \stext{ and }  \vp (z) := \frac 1 {\sqrt{2 \pi} } \exp\left(\frac{-|z|^2}{t}\right).
$$
This result suggests that anisotropic smoothness classes are not unrelated with classical PDE's. In some circumstances at least, we may have 
$$
|f_t|_{g,2} \stackrel ? \leq  C(t) |f|_{g,2}.
$$

\section{Asymptotic approximation and explicit metrics}

\section{Approximation in the $L^p$ norm}
\label{secApproxLP}
We study in this section the theory of anisotropic finite element approximation in the $L^p$ norm, from the point of view of metrics. We first obtain in subsection \S\ref{subsecErrMeshMetLP} an estimation of the finite element approximation error of a function on a mesh in terms of the error with respect to a metric. We then establish in subsection \S\ref{subsecExistsMetLP} the existence of a metric which satisfies an estimate, believed to be asymptotically sharp, when the function is sufficiently smooth. We eventually discuss in subsection \S \ref{subsecApproxSpaceLP} a, probably naive, definition of anisotropic smoothness spaces which leads to the recovery of some classical results of (isotropic) approximation theory. 

\subsection{Existence of an optimal metric for smooth functions}

\label{subsecExistsMetLP}

This section is devoted to the proof of the following theorem, which is announced in the introduction under the reference Theorem \ref{thExistsMetLPIntro}.
\begin{theorem}
\label{thSmooth}
There exists a constant $C=C(m,d)$ such that the following holds.\\
For each $f\in C^m_\per$ such that $z\mapsto K(d^m f(z))$ is not identically $0$, there exists a metric $H \in \bH_\per\cap \bH_g$, which is also $C^\infty$, and such that for all $\lambda \geq 1$
\be
\label{eqHSmooth}
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|K(d^m f)\right\|_\tau,
\ee
where $\frac 1 \tau := \frac m d+ \frac 1 p$.
\end{theorem}

In order to prove this theorem we need to introduce some notation.
The greek letter $\alpha$ always refers %in this section 
to a $d$-plet of non-negative integers
$$
\alpha = (\alpha_1, \cdots, \alpha_d) \in \Z_+^d.
$$
For each $\alpha$ we define the following quantities
$$
|\alpha|:= \sum_{1\leq i\leq d} \alpha_i \stext{ and } \alpha! := \prod_{1\leq i\leq d} \alpha_i!. %, \quad \max(\alpha) := \max_{1\leq i\leq d} \alpha_i.
$$
We also define the monomial
$$
Z^\alpha := \prod_{1\leq i\leq d} Z_i^{\alpha_i},
$$
where the variable is $Z=(Z_1,...,Z_d)\in \R^d$.
For each $z\in \R^d$ we define the homogeneous polynomial $\pi_z\in \H_m$ as follows
$$
\pi_z(Z) := \sum_{|\alpha| = m} \frac{\partial^\alpha f(z)}{(\partial z)^\alpha} \frac{Z^\alpha}{\alpha!} .
$$
We recall that the quantity $K$ involved in this theorem is defined for all $\pi\in \H_m$ as follows
\be
\label{defKAT}
K(\pi) := \inf\{(\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2}\|\leq 1\},
\ee
where
$$
\|\pi\| := \sup_{|z|\leq 1} |\pi(z)|.
$$

The heuristic guideline of this proof is the following. Assume that for all $z\in \R^d$ there exists a unique minimizer $M_z\in S_d^+$ to the minimization procedure \iref{defKAT} defining $K(\pi_z)$, and that $M_z$ depends smoothly on $z$.
Define 
$$
H(z) := \Lambda \, (\det M_z)^{\frac {-1}{mp+d}} M_z,
$$
where $\Lambda>0$ is a sufficiently large constant. A simple analysis, using Taylor developments, shows that $H$ satisfies the conditions of Theorem \ref{thSmooth}. %\iref{eqHSmooth}.

The main difficulty of this proof is that the optimization problem \iref{defKAT} is not well posed. For some choices of $\pi$ there exists no minimizer, for others there exists an infinity of minimizers. 
These undesirable properties come from the fact that \iref{defKAT} is not a convex minimization problem. The key ingredient of our approach is to define a close variant of this optimization problem which is ``geometrically convex'', a  notion close to convexity which is sufficient for our purpose.

\subsubsection{Geometric convexity, and geometric average of two matrices}
\label{subsubsecGeomCvx}
%We also introduce the notion of geometric average of two matrices.
Let $M, M'\in S_d^+$, and let $S:=M^{-\frac 1 2}$. We define the geometric average $\Avg(M,M')\in S_d^+$ of $M$ and $M'$ as follows
\be
\label{defAvg}
S \Avg(M,M') S := \sqrt{S M' S}
\ee
For instance $\Avg(M,M^{-1}) = \Id$, and for any $k,k'>0$
$$
\Avg(k M , k'M') = \sqrt{k k'} \Avg(M,M').
$$

The following proposition gives a handy characterization \iref{eqAvgAD} of $\Avg(M,M')$. This proposition also shows that $\Avg(M,M')$ is a natural midpoint between $M$ and $M'$ for the distance $d_\times$, and establishes two basic properties of the geometric average of matrices.
% number of useful properties.

\begin{prop}
For any $M,M'\in S_d^+$ the following holds.
\begin{enumerate}
\item A matrix $\ti M$ satisfies $\tilde M = \Avg(M,M')$ if and only if there exists $A \in \GL_d$ and a diagonal matrix $D$ such that 
\be
\label{eqAvgAD}
\tilde M = A^\trans A, \quad M = A^\trans e^{2D} A, \quad M' = A^\trans e^{-2D} A.
\ee
\item The geometric average $\Avg(M,M')$ is a midpoint between $M$ and $M'$ for the distance $d_\times$ on $S_d^+$.
$$
d_\times (M, \Avg(M,M')) = d_\times (\Avg(M,M'), M') = \frac 1 2 d_\times (M,M').
$$
\item The geometric average is commutative and compatible with the inversion of matrices.
\begin{eqnarray}
\label{eqAvgCommut}
\Avg(M,M') &=& \Avg(M',M)\\
\label{eqAvgInv}
\Avg(M,M')^{-1} &=& \Avg(M^{-1}, M'^{-1})
\end{eqnarray}
\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item We first assume that $M,M'$ and $\tilde M$ have the form \iref{eqAvgAD}. We easily obtain 
$$
\tilde M M^{-1} \tilde M = M'
$$
Defining $S := M^{-\frac 1 2}$ we thus have 
$$
(S\tilde M S)^2 = S M' S.
$$
Taking the square root of the previous equation we obtain \iref{defAvg} which shows that $\tilde M = \Avg(M,M')$.

Conversely, for any $M,M'\in S_d^+$ %(??) 
the simultaneous reduction theorem shows that there exists $A\in \GL_d$ and $D$ diagonal satisfying $M = A^\trans e^{2D} A$ and $M' = A^\trans e^{-2D} A$, and the result follows.

\item Let $A\in \GL_d$ and let $D,D'$ be diagonal matrices, of diagonal coefficients $D_1, \cdots ,D_k$ and  $D'_1, \cdots , D'_d$ respectively. We define
$$
\delta := \max_{1\leq i \leq d} |D_i - D'_i|.
$$ 
We claim that the matrices $N := A^\trans e^{2D} A$ and $N':=A^\trans e^{2D'} A$ satisfy $d_\times(N,N') = \delta$.
Indeed
\begin{eqnarray*}
d_\times (N,\, N') &:= &\sup_{u\neq 0} \left|\ln \|u\|_N -\ln \|u\|_{N'}\right| \\
&=& \sup_{u\neq 0} \left|\ln |e^D Au| - \ln |e^{D'} Au|\right|\\
&=& \sup_{v\neq 0}  \left|\ln |e^D v| - \ln |e^{D'} v|\right|.
\end{eqnarray*}
For any $v=(v_1, \cdots ,v_d)\in \R^d$ we have 
$$
|e^D v|^2 = \sum_{1\leq i \leq d} e^{2D_i} v_i^2 \leq e^{2\delta}  \sum_{1\leq i \leq d} e^{2D'_i} v_i^2 = \left(e^\delta |e^{D'}v|\right)^2,
$$
and similarly $|e^{D'} v|\leq e^\delta |e^D v|$. Therefore $\left|\ln |e^D v| - \ln |e^{D'} v|\right|$ and taking the supremum among all $v\neq 0$ we obtain $d_\times(N,N') \leq \delta$. Furthermore denote by $i_0$, $1\leq i_0\leq d$, the position $|D_{i_0} - D'_{i_0}| = \delta$. Choosing $v = (0,\cdots ,1, \cdots ,0)$, with the nonzero coordinate at the position $i_0$, we obtain $\delta = \left|\ln |e^D v| - \ln |e^{D'} v|\right| \leq d_\times(N,N')$. We thus conclude that 
$$
d_\times (N,N') =  d_\times (A^\trans e^{2D} A, \, A^\trans e^{2D'} A) = \|D-D'\|.
$$

Recalling that $M,M'$ and $\ti M := \Avg(M,M')$ have the form \iref{eqAvgAD} we thus obtain 
$$
d_\times (M, \Avg(M,M')) = d_\times (\Avg(M,M'), M')= \|D\| \stext{ and } d_\times (M,M') = 2 \|D\|.
$$
which concludes the proof of this point.

\item 
Using the first point we obtain that $M,M'$ and $\tilde M := \Avg(M,M')$ have the form
$$
\tilde M = A^\trans A, \quad M = A^\trans e^{2D} A, \quad M' = A^\trans e^{-2D} A
$$
It follows that 
$$
\tilde M = A^\trans A, \quad M' = A^\trans e^{-2D} A, \quad M = A^\trans e^{2D} A,
$$
and 
$$
\tilde M^{-1} = (A^{-1})^\trans A^{-1}, \quad M^{-1} = (A^{-1})^\trans e^{-2D} A^{-1}, \quad M'^{-1} = (A^{-1})^\trans e^{2D} A^{-1}.
$$
Using again the first point we obtain the announced properties \iref{eqAvgCommut} and \iref{eqAvgInv}.\sq
\end{enumerate}

We recall that that a function $\psi\in C^0(S_d, \R)$ is convex if and only if for all $M,M'\in S_d$ one has 
\be
\label{defConv}
\psi\left(\frac{M+M'} 2\right) \leq \frac{\psi(M)+ \psi(M')} 2.
\ee
The next proposition introduces the family of geometrically convex functions, which are defined by a property similar to \iref{defConv} but in which the arithmetic averages are replaced with geometric averages.
\begin{definition}
We say that a function $\vp \in C^0(S_d^+ , \R_+^*)$ is GCH, Geometrically Convex and Homogenous, if it satisfies the following properties.
\begin{enumerate}[i)]
\item (Sub multiplicativity) For any $M,M'\in S_d^+$ one has
\be
\label{eqSubMult}
\vp(\Avg(M,M')) \leq \sqrt{\vp(M) \vp(M')}.
\ee
\item (Homogenous) There exists $\alpha \in \R$ , called the degree of $\vp$,
such that for all $M\in S_d^+$ and all $\lambda\in \R$ one has 
$$
\vp(\lambda M) = \lambda^\alpha \vp(M).
$$
\end{enumerate}
We say that the function $\vp$ is SGCH, Strictly Geometrically Convex and Homogeneous, if $\vp$ is GCH and if the equality in \iref{eqSubMult} only holds if $M$ and $M'$ are proportional.
\end{definition}

For instance the function $\det$ is GCH of degree $d$, since 
$$
\det \Avg(M,M') = \sqrt{\det M \det M'} \stext{ and } \det (\lambda M) = \lambda^d M.
$$
We insist on point that GCH functions are by assumption strictly positive on $S_d^+$, and continuous.
The next lemma enumerates some simple properties of geometrically convex functions.
\begin{lemma}
\label{lemmaAlgGCH}
\begin{enumerate}
\item The product of two GCH functions is GCH, and the product of a GCH function with a SGCH function is SGCH. Furthermore the degrees add.
\item The elevation to a positive power of a GCH (resp. SGCH) function is also GCH (resp. SGCH). Furthermore the degree is multiplied by $\alpha$.
\item If a function $\vp$ is GCH (resp. SGCH) then $M \mapsto \vp(M^{-1})$ is also GCH (resp. SGCH), and has the opposite degree.
\end{enumerate}
\end{lemma}
\proof
The first two points are easy, and the last point is a direct consequence of the compatibility \iref{eqAvgInv} of the geometric average with the inversion : if $\vp$ is GCH and $M,M'\in S_d^+$ then 
$$
\vp(\Avg(M,M')^{-1}) = \vp(\Avg(M^{-1}, M'^{-1})) \leq \sqrt{\vp(M^{-1}) \vp (M'^{-1})},
$$
which concludes the proof.
\sq

Aside from the determinant, a number of functions on $S_d^+$ are geometrically convex. The next proposition, which is based on an argument of complex analysis, enumerates some of them.
For all $\pi\in \H_m$ we define 
$$
\|\pi\|_\sC := \sup\{ |\pi(z)| \sep z\in \C^d, \, |z|\leq 1\}.
$$

\begin{prop}
\label{propExGCH}
\begin{enumerate}
\item The trace map $M \mapsto \Tr M$ is SGCH.
\item For any fixed polynomial $\pi\in \H_m\sm\{0\}$ the map $M \mapsto \|\pi \circ M^{\frac 1 2}\|_\sC$ is GCH, of degree $m/2$.
\item The norm map $M \mapsto \|M\|$ is GCH. 
\end{enumerate}

%For any $M,M'\in S_d^+$ the following holds.
%\begin{enumerate}
%\item 
%\be
%\label{eqTr}
%\Tr (\Avg(M,M'))\leq \sqrt{\Tr M \Tr M'} \stext{ and } \Tr (\Avg(M,M')^{-1})\leq \sqrt{\Tr (M^{-1}) \Tr (M'^{-1})}
%\ee
% with equality if and only if the matrices $M$ and $M'$ are proportionnal. %and inverse.
%\item For any polynomial $\mu \in \H_m$ one has %$\C$ %define S, S', \tilde S
%$$
%\|\mu \circ \Avg(M,M')^{-\frac 1 2}\|_\sC \leq \sqrt{\|\pi\circ M^{-\frac 1 2}\|_\sC \|\pi\circ M'^{-\frac 1 2}\|_\sC }
%$$
%\item We have 
%$$
%\|\Avg(M, M')\| \leq \sqrt{\|M\| \|M'\|}
%$$
%\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item 
Let $M,M'\in S_d^+$ and let $\ti M := \Avg(M)$. Let $A\in \GL_d$ and let the diagonal matrix $D$ be such that  $M = A^\trans e^{-2D}$, $M' = A^\trans e^{2D} A$ and $\ti M = A^\trans A$.
We denote by $A_{i,j}$ the coefficients of $A$, and we define for all $1\leq i \leq d$
$$
\cA_i^2 := \sum_{1\leq j \leq d} A_{ji}^2.
$$
Observe that $\cA_i>0$, since otherwise a full line of $A$ would be zero and $A$ would be degenerate.
Denoting by $D_i , \cdots , D_d$ the diagonal coefficients of $D$ we obtain  
$$
\Tr(M) = \sum_{1\leq i \leq d} \cA_i^2 e^{-2D_i}, \quad \Tr(M') = \sum_{1\leq i \leq d} \cA_i^2 e^{2D_i}, \quad \Tr(\ti M) = \sum_{1\leq i \leq d} \cA_i^2.
$$
It thus follows from Cauchy Schwartz inequality that $\Tr(\ti M)^2 \leq \Tr(M) \Tr(M')$. Furthermore equality occurs if and only if the vectors 
$$
(\cA_i e^{-D_i})_{1\leq i \leq d} \stext{ and }(\cA_i e^{D_i})_{1\leq i \leq d}
$$
are proportional, which implies that $D_i =D_j$ for all $1\leq i,j\leq d$ and therefore that $M$ and $M'$ are proportional. 

\item

We first a classical result of complex analysis, called Hadamard's the three lines theorem. %see [Rudin??], often
Let $\Omega:=\{\alpha\in \C \sep |\Re(\alpha)|<1\}$, where $\Re$ denotes the real part, and let $g$ be a continuous and bounded function on $\overline \Omega$ which is holomorphic on $\Omega$. Then 
\be
\label{eqComplex}
|g(0)|^2 \leq \left(\sup_{\Re \alpha = -1} |g(\alpha)|\right) \left(\sup_{\Re z = \alpha} |g(\alpha)|\right).
\ee

We say that a matrix $U$ is unitary if $|Uz| = |z|$ for all $z\in \C$, or equivalently if $U^* U = \Id$ where $U^*$ denotes the conjugate transpose of $U$. We recall that any orthogonal matrix $O\in \cO_d$ is also unitary, and that for any diagonal matrix $D$ with real diagonal coefficients and any $\beta\in \R$ the matrix $e^{\b i \beta D}$ is unitary, where $\b i^2 = -1$.


We consider a fixed $z\in \C^d$ satisfying $|z|\leq 1$, and we define for all $\alpha\in \overline \Omega$ 
%We consider a fixed $z\in \C^d$ and we define 
$$
g(\alpha) := \pi(A^\trans e^{\alpha D} z).
$$
The function $g$ is continuous, uniformly bounded on $\overline \Omega$ by $\|\pi\|_\sC (\|A\| e^{\|D\|})^d$, and holomorphic in $\Omega$, hence the three lines theorem applies.
For any $\sigma \in \{-1,1\}$ one has 
$$
\sup_{\Re(\alpha) = \sigma} |\pi(A^\trans e^{\alpha D} z)| \leq \|\pi\circ(A^\trans e^{\sigma D})\|_\sC,
$$
since $|e^{\b i\Im(\alpha) D}z| = |z|=1$. %$|e^{i\Im(\alpha) D} z| = |z|$ where $\Im$ denotes the imaginary part.
Applying \iref{eqComplex} to the function $g$ we thus obtain 
$$
|\pi(A^\trans z)|^2 \leq \|\pi\circ(A^\trans e^D)\|_\sC \|\pi\circ(A^\trans e^{-D})\|_\sC.%\left(\sup_{\Re \alpha = -1} f(A^\trans e^\alpha z)\right) \sup
$$
Taking the supremum among all $z\in \C^d$ such that $|z|\leq 1$ we conclude that 
$$
\|\pi\circ A^\trans\|_\sC \leq \|\pi\circ(A^\trans e^D)\|_\sC \|\pi\circ(A^\trans e^{-D})\|_\sC.
$$
%Last we recall (ref??) that
There exists three orthogonal matrices $O, O', \tilde O\in \cO_d$ such that 
$$
OM^\frac 1 2 =  e^D A, \quad O'M'{^\frac 1 2} = e^{-D} A \stext{ and } \tilde O \tilde M^\frac 1 2 = A.
$$
Since orthogonal matrices are also unitary matrices we have 
\begin{eqnarray*}
\|\pi \circ A^Te^{-D}\|_\sC &=& \|\pi \circ M^{\frac 1 2}\|_\sC,\\
\|\pi \circ A^T e^{-D}\|_\sC &=& \|\pi \circ  M'^{\frac 1 2}\|_\sC\\
\|\pi \circ A^T\|_\sC &=& \|\pi \circ \ti M^{\frac 1 2}\|_\sC,
\end{eqnarray*}
thus $\|\pi\circ M^\frac 1 2\|_\sC$ satisfies the sub-multiplicativity property \iref{eqSubMult}. Furthermore $M \mapsto \|\pi\circ M^\frac 1 2\|_\sC$ is clearly continuous and strictly positive on $S_d^+$, and homogeneous of degree $m/2$ which concludes the proof of this point.

\item
We denote by $\pi\in \H_2$ the canonical quadratic form 
$$
\pi(z) := \sum_{1\leq j \leq d} z_j^2.
$$
Our purpose is to establish that for any $M\in S_d^+$
\be
\label{eqPiMM}
\|\pi\circ M^{\frac 1 2}\|_\sC = \|M\|,
\ee
which implies that $\|M\|$ is GCH in view of the previous point.
For any $z\in \C$ such that $|z|\leq 1$ one has 
$$
|\pi(M^\frac 1 2 z)| = |z^\trans M^\frac 1 2 M^\frac 1 2 z| \leq |M^\frac 1 2 z|^2 \leq \|M^\frac 1 2\|^2  = \|M\|.
$$
Furthermore choosing a normalized eigenvector $z\in \R^d$ associated to the maximal eigenvalue of $M$ we obtain $|\pi(M^\frac 1 2 z)|=\|M\|$, which establishes \iref{eqPiMM} and concludes the proof.
\sq
\end{enumerate}

\subsubsection{A well posed variant of the shape function}

We define a function $\kappa\in C^0(S_d^+, \R_+^*)$ as follows : for all $M\in S_d^+$ 
$$
\kappa(M) :=  \frac 1 d\sqrt{\Tr(M) \Tr(M^{-1})}.
$$
The function $\kappa$ is SGCH, as the product of two SGCH functions see Lemma \ref{lemmaAlgGCH} and Proposition \ref{propExGCH}.
In terms of the eigenvalues $\lambda_1, \cdots, \lambda_d$ of $M$ we have 
$$
d^2 \kappa(M)^2 = \left(\sum_{1 \leq i \leq d} \lambda_i\right)\left(\sum_{1 \leq i \leq d} \lambda_i^{-1}\right).
$$  
We regard the function $\kappa$ as a close variation on the condition number $\sqrt{\|M\|\|M^{-1}\|}$ of the matrix $M^\frac 1 2$. Note that $\kappa(M) = 1$ if and only if $M = m\Id$ for some $m>0$, and that 
$$
\kappa(M)\leq \sqrt{\|M\|\|M^{-1}\|} \leq d \, \kappa(M).
$$
The following proposition illustrates the use of $\kappa$ as a regularization term.
\begin{prop}
\label{propContLift}
Let $\vp$ be a GSH function of degree $r>0$. 
Let $(X,d_X)$ be a metric space, and let $\psi\in C^0(S_d^+ \times X, \R_+^*)$ be such that $\psi(\cdot,x)$ is GCH of degree $-1$ for any fixed $x\in X$.
We define for all $x\in X$ and all $\alpha \in (0, \infty)$
$$
L^{(\alpha)}(x) := \inf\left\{\kappa(M)^{\frac 1 \alpha} \vp(M) \sep \psi(M,x) \leq 1 \text{ and } \kappa(M) \leq e^\alpha\right\}.
$$
For any $x\in X$ there exists a unique minimizer $\cM^{(\alpha)}(x)$ to the optimization problem defining $L^{(\alpha)}(x)$. Furthermore the map $\cM^{(\alpha)} : X \to S_d^+$ is continuous. 
\end{prop}

\proof
The parameter $\alpha\in (0, \infty)$ is fixed.
\begin{itemize}
\item
(Existence of a minimizer) We consider a fixed $x\in X$ and we establish that there exists a minimizer to the optimization problem $L^{(\alpha)}(x)$.
For any $\beta \geq 0$ the following collection of matrices is compact %(*det more natural?*)
\be
\label{defKBeta}
K_\beta := \{M\in S_d^+ \sep |\ln(\det M)|\leq \beta \text{ and } \kappa(M) \leq e^\alpha\}.
\ee
We define
$$
\Lambda := \sup_{M\in K_0} \vp(M) \stext{ and } \lambda := \inf_{M\in K_0} \psi(M,x)
$$
in such way that for any $M\in S_d^+$ satisfying $\kappa(M) \leq e^\alpha$
\be
\label{eqPhiPsi}
\vp(M) \leq \Lambda (\det M)^{\frac r d} \stext{ and } \psi(M,x) \geq \lambda (\det M)^{\frac 1 d}.
\ee
We consider a minimizing sequence $(M_n)_{n \in \sN}$, $M_n\in S_d^+$, for the optimization problem $L^{(\alpha)}(x)$. It follows from \iref{eqPhiPsi} that $\det (M_n)$ uniformly bounded above and below: there exists $\beta \geq 0$ such that $|\ln \det M_n|\leq \beta$ for all $n \geq 0$. Furthermore $\kappa(M_n) \leq e^\alpha$, hence $M_n \in K_\beta$. Since the set $K_\beta$ is compact there exists a converging subsequence $M_{\sigma(n)} \to M_\infty\in K_\beta$. By continuity of the functions $\vp$, $\psi(\cdot ,x)$ and $\kappa$ on $S_d^+$ the matrix $M_\infty$ is a minimizer of the optimization problem $L^{(\alpha)}(x)$.

\item (Uniqueness)  
We consider two minimizers $M,M'$ of the minimization problem $L^{(\alpha)}(x)$, and we denote $\ti M := \Avg(M,M')$. 
Since the functions $\psi(\cdot, x)$ and $\kappa$ are GCH, the matrix $\ti M$ satisfies the inequalities 
$$
\psi(\ti M,x) \leq 1 \stext{ and } \kappa(\ti M) \leq e^\alpha.
$$ 
We define a function $\Phi \in C^0(S_d^+, \R_+^*)$, which is SGCH of degree $r>0$ in view of Lemma \ref{lemmaAlgGCH}, as follows
\be
\label{defPhiSGCH}
\Phi(M) := \kappa(M)^\frac 1 \alpha \vp(M).
\ee
If $M$ is not proportionnal to $M'$ we thus have
$$
\Phi(\ti M) < \sqrt{\Phi( M) \Phi( M')} = L^{(\alpha)}(x),
$$
 which is a contradiction. Thus $M = m M'$ for some $m>0$, but this implies 
 $$
L^{(\alpha)}(x) = \Phi( M) = \Phi( M') = m^r  \Phi( M),
 $$
 therefore $m=1$ and $M=M'$. The minimizer is unique as announced.

\item (Continuity)  
For all $x,x'\in X$, we define
$$
\omega(x,x') := \sup_{M \in K_0} |\ln \psi(M,x) - \ln\psi(M,x')|,
$$
where the set $K_0$ is defined by \iref{defKBeta}, and we observe that $\omega(x,x') \to 0$ as $x'\to x$.
(Note that $\omega(x,x')$ is the modulus of continuity of the continuous function $X \to C^0(K_0, \R)$, defined by $x\mapsto \ln \psi (\cdot,x)$.)

Consider $x,x'\in X$ and define $M := e^{\omega(x,x')} \cM^{(\alpha)}(x)$ and $M' := e^{\omega(x,x')} \cM^{(\alpha)}(x')$. We thus have 
$$
\kappa(M) = \kappa(\cM^{(\alpha)}(x)) \leq e^\alpha,
$$
and likewise $\kappa(M') \leq e^\alpha$.
Since $\psi(\cdot ,x')$ is homogeneous of degree $-1$ we obtain
$$
\psi(M, x')\leq e^{\omega(x,x_n)} \psi(M, x') = e^{\omega(x,x_n)} \psi(e^{\omega(x,x_n)} \cM^{(\alpha)}(x_n)) \leq 1,
$$
and likewise $\psi(M',x)\leq 1$.
Furthermore since $\Phi$ defined by \iref{defPhiSGCH} is homogeneous of degree $r$ we obtain
$$
L^{(\alpha)}(x') \leq \Phi(M) = e^{r\omega(x,x')} L^{(\alpha)}(x),
$$
and likewise $L^{(\alpha)}(x) \leq \Phi(M') = e^{r\omega(x,x')} L^{(\alpha)}(x')$, in particular
$$
\Phi(M') = \Phi(e^{\omega(x,x')} \cM^{(\alpha)}(x'))  = e^{r\omega(x,x')} L^{(\alpha)}(x') \leq e^{2r\omega(x,x')} L^{(\alpha)}(x).
$$

Consider a converging sequence in $X$, $x_n \to x$, and define
$$
M_n := e^{\omega(x,x_n)} \cM^{(\alpha)} (x_n).
$$
The arguments above show that $M_n$ is a minimizing sequence for the optimization problem $L^{(\alpha)}(x)$. The arguments developed for the existence of a minimizer show that $\{M_n\sep n \geq 0\}$ is contained in the compact set $K_\beta$ for a sufficiently large value $\beta\geq 0$, and that any converging subsequence of $(M_n)_{n \geq 0}$ tends to a minimizer of the optimization problem $L^{(\alpha)}(x)$, thus to $\cM^{(\alpha)}(x)$ by uniqueness.

Since the sequence $M_n$ takes its values in the compact set $K_\beta$ and has the single adherence value $\cM^{(\alpha)}(x)$, we have the convergence $M_n \to \cM^{(\alpha)}(x)$ as $n \to \infty$. Since $\omega(x,x_n) \to 0$ we obtain as announced 
$$
\cM^{(\alpha)}(x_n)\to \cM^{(\alpha)}(x),
$$
which concludes the proof of this proposition.
\sq
\end{itemize}

For any $\alpha \in (0, \infty)$ we define a function $K^{(\alpha)} : \H_m \to \R_+$ as follows
$$
K^{(\alpha)}(\pi) := \inf\{ \kappa(M)^{\frac 1 \alpha} (\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2} \|_\sC \leq 1 \text{ and } \kappa(M) \leq e^\alpha\},
$$
where the infimum is taken among symmetric positive definite matrices $M\in S_d^+$.
According to the previous proposition the minimizer $\cM^{(\alpha)}(\pi)$ of $K^{(\alpha)}(\pi)$ defines a continuous map $\cM^{(\alpha)} : \H_m\sm\{0\} \to S_d^+$. %such that $K^{(\alpha)}(\pi) = 
As $\alpha\to \infty$ the functions $K^{(\alpha)}$ on $\H_m$ converge pointwise and decreasingly to the function $K_\sC : \H_m \to \R_+$ defined by 
$$
K_\sC(\pi) := \inf\{ (\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2} \|_\sC \leq 1\}.
$$

We obtain using Lemma \ref{lemmaAM}
$$
K(\pi) = \inf_{A\in \SL_d} \|\pi\circ A\| \stext{ and } K_\sC(\pi) = \inf_{A\in \SL_d} \|\pi\circ A\|_\sC.
$$ 
Since $\|\cdot\|\leq \|\cdot \|_\sC$, and since these two functions are norms on the finite dimensional space $\H_m$, there exists a constant $n_\sC = n_\sC(m,d)$ such that for all $\pi\in \H_m$
$$
\|\pi\|\leq \|\pi\|_\sC \leq n_\sC \|\pi\|.
$$ 
It follows that
\be
\label{eqKKC}
K(\pi) \leq K_\sC(\pi) \leq n_\sC K(\pi).
\ee

The next proposition is not necessary for our analysis but gives a worthwhile insight of the properties of the shape function $K$. We show in particular that the function $K$, which is only upper semi continuous in general, is equivalent to a continuous function. We deduce a from this point a property of convergence the the functions$K^{(\alpha)}$.

% which converge only pointwise to $K$, satisfy a good substitute 
%
%The convergence of $K^{(\alpha)}$ towards $K_\sC$ is not uniform.
%The next lemma gives a substitute for this uniform convergence.

\begin{prop}
\label{lemmaKAK}
\begin{enumerate}
\item (Vanishing property)
Let $(\pi_n)_{n \geq 0}$, $\pi_n \in \H_m$,  $\pi_n \to \pi$ as $n \to \infty$, be a converging sequence of homogeneous polynomials. 
Let  $(A_n)_{n \geq 0}$, $A_n \in \SL_d$ be a sequence of matrices of unit determinant.

If $\pi_n \circ A_n \to 0$ then there exists $A\in \SL_d$, such that $\pi\circ (A^n) \to 0$.

\item (Equivalence to a lower semi continuous function) We denote by $\underline K_\sC$ the lower semi-continuous envelope of $K_\sC$ : for all $\pi\in \H_m$ 
$$
\underline K_\sC(\pi) := \lim_{\ve \to 0} \inf_{\|\pi-\pi'\|\leq \ve} K_\sC(\pi).
$$
There exists a constant $C_\lsc= C_\lsc(m,d)$ such that $\underline K_\sC \leq K_\sC\leq  C_\lsc \underline K_\sC$ on $\H_m$.

Furthermore there exist a continuous function $K_c$ on $\H_m$ such that $(C_\lsc+1)^{-1}K_c\leq K_\sC\leq (C_\lsc+1) K_c$.

\item (Substitute for uniform convergence)
For all $\ve >0$ there exists $\alpha = \alpha(m,d,\ve)$ such that for all $\pi \in \H_m$
\be
\label{eqKAKU}
K^{(\alpha)}(\pi) \leq C_\lsc \underline K_\sC(\pi)+ \ve \|\pi\|_\sC,
\ee
where $C$ is the constant appearing in 2. In particular 
\be
\label{eqKAK}
K^{(\alpha)}(\pi) \leq n_\sC (C_\lsc  K(\pi)+ \ve \|\pi\|).
\ee
\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item
For each $n\geq 0$ we consider the singular value decomposition $A_n = U_n D_n V_n$, where $U_n, V_n \in \cO_d$ and the diagonal matrix $D_n$ has positive coefficients and satisfies $\det D_n = 1$.
Since $V_n$ is orthogonal we have 
$$
\|\pi_n \circ A_n \| = \|\pi_n \circ (U_n D_n V_n)\| = \|\pi_n \circ (U_n D_n)\|.
$$
Since $\cO_d$ is compact the sequence of orthogonal matrices $U_n$ admits a converging sub-sequence $U_{\sigma(n)} \to U$. 
We define $\pi' := \pi\circ U$, $\pi'_n := \pi_{\sigma(n)} \circ U_{\sigma(n)}$ and $D'_n := D_{\sigma(n)}$, in such way that 
$$
\pi'_n \to \pi' \stext{ and } \pi'_n \circ D'_n \to 0.
$$
We recognise the hypotheses of the lemma, except that the matrices $D'_n$ replacing $A_n$ are now diagonal. We show below that there exists a diagonal matrix $D$, $\det D=1$, such that $\pi'\circ (D^n) \to 0$. Defining $A := UDU^\trans$ leads to the announced result $\pi \circ (A^n) \to 0$.

In order to avoid notational clutter we do not keep track of the extraction procedure and we simply write $\pi$, $\pi_n$ and $D_n$ in place for $\pi'$, $\pi'_n$ and $D'_n$.
We define the finite set 
$$
\Lambda := \{\alpha \in \Z_+^d\sep |\alpha| \leq k\},
$$
and to any $t\in (\R_+^*)^d$ we associate a subset $\Lambda(t)\subset \Lambda$
$$
\Lambda(t) := \{\alpha \in \Lambda \sep t^\alpha \geq 1\}.
$$
For each $n$ we denote by $\Lambda_n$ the set $\Lambda(t_n)$ associated to the list $t_n$ of diagonal entries of $D_n$.

There are only a finite number of subsets of $\Lambda$, namely $2^{\#(\Lambda)}$, thus there exists an extraction $\tau$ such that $\Lambda_* := \Lambda_{\tau(n)}$ us independent of $n$.

For any $\alpha\in \Lambda$ we denote by $\pi_{n,\alpha}$ the coefficient of $Z^\alpha$ in $\pi_n$, and by $\pi_\alpha$ the coefficient of $Z^\alpha$ in $\pi$, where $Z=(Z_1, \cdots ,Z_d)$ is the $d$-dimensional variable. 
$$
\pi_n = \sum_{\alpha \in \Lambda} \pi_{n , \alpha} Z^\alpha \stext{ and } \pi = \sum_{\alpha \in \Lambda} \pi_\alpha Z^\alpha.
$$
We recall that $t_n$ denotes the list of coefficients of the diagonal matrix $D_n$, we denote by $t$ the list of coefficients of a diagonal matrix $D$. We thus have 
$$
\pi_n \circ D_n = \sum_{\alpha \in \Lambda} \pi_{n , \alpha} t_n^\alpha Z^\alpha \stext{ and } \pi \circ D^n= \sum_{\alpha \in \Lambda} \pi_\alpha t^{n \alpha} Z^\alpha.
$$
Since $\pi_n \circ D_n \to 0$ we have 
$
\pi_{n ,\alpha} t_n ^\alpha \to 0
$
for any $\alpha \in \Lambda$.
For any $\alpha$ in the subset $\Lambda_*\subset \Lambda$ we obtain recalling that $t_{\tau(n)}^\alpha \geq 1$
$$
\pi_\alpha = \lim_{n \to \infty} \pi_{\tau(n) ,\alpha} = 0.
$$
We now define $D = D_{\tau(0)}$, we denote by $t$ the list of coefficients of $D$,
and we observe that 
$$
\pi \circ D^n \to 0.
$$
Indeed $\pi_\alpha t^{n \alpha} = 0$ for all $\alpha\in \Lambda_*$, and $\pi_\alpha t^{n \alpha} \to 0$ for all $\alpha \notin \Lambda_*$ since $t^\alpha <1$, which concludes the proof of this point.


\item
As a consequence of 1. we obtain the following vanishing property : for any $\pi \in \H_m$, if $\underline K_\sC(\pi) = 0$ then $K_\sC(\pi) = 0$. Indeed if $\underline K_\sC(\pi) = 0$ then there exists a sequence of homogeneous polynomials $\pi_n\to \pi$ such that $K_\sC(\pi_n) \to 0$, and therefore a sequence of matrices $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, such that $\pi_n \circ A_n$. Therefore there exists $A\in \SL_d$ such that $\pi\circ (A^n)\to 0$, which implies that $K_\sC(\pi) = 0$.

%We define $\cS := \{\pi \in \H_m \sep \|\pi\|_\sC = 1\}$ and we consider the closed set 
We consider the compact set 
$$
\cA := \{\pi \in \H_m \sep \|\pi\|_\sC = 1 \text{ and } \|\pi \circ A\|_\sC \geq 1 \text{ for all } A\in \SL_d\}.
$$
For any $\pi \in \cA$ we thus have $K_\sC(\pi) = \|\pi\|_\sC=1$, and therefore $\underline K_\sC(\pi) >0$. 
Since $\cA$ is compact and since $\underline K_\sC$ is lower semi-continuous, the function $\underline K_\sC$ attains its lower bound on $\cA$ and we define
$$
C^{-1}_\lsc := \inf_{\pi \in \cA} \underline K_\sC(\pi).
$$
Let $\pi\in \H_m$, and let $(A_n)_{n \geq 0}$, $A_n\in \SL_d$, be a sequence of matrices satisfying $\|\pi\circ A_n\|_\sC \to K_\sC(\pi)$ as $n \to \infty$. If $K_\sC(\pi) = 0$ then $\underline K_\sC(\pi) = 0$ also according to the first point of this lemma, and there is nothing to prove.
If $K_\sC(\pi) = 0$ then consider an extraction $\vp$ such that we have the convergence 
$$
\frac{\pi \circ A_n}{\|\pi\circ A_n\|_\sC} \to \pi_*.
$$
We now prove that $\pi_*\in \cA$. Indeed $\|\pi_*\|_\sC = 1$ by construction. If, by contradiction, there exists $A\in SL_d$ such that $\|\pi_*\circ A\| = \delta<1$, then we obtain 
$$
K_\sC(\pi) \leq \lim_{n \to \infty} \|\pi \circ (A_n A)\|_\sC = \lim_{n \to \infty} \frac{\|\pi \circ (A_n A)\|_\sC}{\|\pi\circ A_n\|_\sC} \|\pi\circ A_n\|_\sC = \delta K_\sC(\pi)
$$
which is a contradiction, hence $\pi_*\in \cA$ as announced.
We now observe that 
$$
\underline K_\sC \left(\frac{\pi\circ A_n}{\|\pi\circ A_n\|_\sC} \right) = \frac {\underline K_\sC(\pi)}{\|\pi\circ A_n\|_\sC} \underset {n \to \infty} \longrightarrow \frac {\underline K_\sC(\pi)}{K_\sC(\pi)}.
$$
On the other hand, since $\underline K_\sC$ is lower semi continuous and $\pi_*\in \cA$,
$$
\lim_{n \to \infty} \underline K_\sC \left(\frac{\pi\circ A_n}{\|\pi\circ A_n\|_\sC} \right) \geq \underline K_\sC(\pi_*) \geq C_\lsc^{-1}.
$$
Combining the last two equations we obtain as announced $K_\sC(\pi) \leq C_\lsc \underline K_\sC(\pi)$. 

We now construct a continuous function $K_c$ on $\H_m$ which is equivalent to $K_\sC$.
For each $n\in \Z$ we define
$$
E_n := \{\pi\in \H_m \sep K_\sC(\pi) \geq (C_\lsc+1)^n\}.
$$
Note that the closed sets $E_{n+1}$ and $\overline {\H_m \sm E_n}$ are disjoint, since $K_\sC \leq C_\lsc \underline K_\sC \leq C_\lsc (C_\lsc+1)^n$ on the latter. The following functions is thus continuous
$$
r_n(\pi) := \frac{d(\pi, \H_m \sm E_n)}{d(\pi, \H_m \sm E_n)+ d(x,E_{n+1})} \stext{ where } d(\pi,X) := \inf_{\pi'\in X} \|\pi-\pi'\|_\sC.
$$
We define a continuous function $r : \H_m \to [-\infty, \infty)$ (observe that $-\infty$ is included) but the sum
$$
r(\pi) := \sum_{n <0} (r_n(\pi)-1) + \sum_{n \geq 0} r_n(\pi),
$$
which is finite for any $\pi$ such that $K_\sC(\pi)>0$.
Eventually we set 
$$
K_c(\pi) := (C_\lsc+1)^{r(\pi)},
$$
which concludes the proof.

\item
We consider a fixed $\ve>0$ and we recall that $K^{(\alpha)}$ converges pointwise decreasingly to $K_\sC$ as $\alpha\to \infty$. To each $\pi \in \cS := \{\pi \in \H_m \sep \|\pi\|_\sC = 1\}$ we associate $\alpha_\pi\in (0, \infty)$ satisfying 
$$
K^{(\alpha_\pi)}(\pi) < K_\sC(\pi)+ \ve.
$$
In particular $K^{(\alpha_\pi)}(\pi) < C_\lsc \underline K_\sC(\pi)+ \ve$, and since $\underline K_\sC$ is lower continuous the collection $V_\pi$ of all $\pi'\in \cS$ satisfying 
$$
K^{(\alpha_\pi)}(\pi') < C_\lsc \underline K_\sC(\pi')+ \ve
$$
is an open neighborhood of $\pi$ in $\cS$. 

Since $\cS$ is compact there exists a finite subset $\cS_0$ of $\cS$ such that 
$$
\bigcup_{\pi \in \cS_0} V_\pi = \cS. 
$$
Defining $\alpha := \max \{\alpha_\pi \sep \pi \in \cS_0\}$, and recalling that $K^{(\alpha)} \leq K^{(\alpha')}$ if $\alpha \geq \alpha'$, we obtain for all $\pi\in \H_m \sm \{0\}$
$$
K^{(\alpha)}\left(\frac \pi {\|\pi\|_\sC}\right) \leq C_\lsc \underline K_\sC\left(\frac \pi {\|\pi\|_\sC}\right)+ \ve,
$$
which implies \iref{eqKAKU} since $K^{(\alpha)}$ and $\underline K_\sC$ are $1$-homogeneous on $\H_m$.
The inequality \iref{eqKAK} is a direct consequence of \iref{eqKKC}.
\end{enumerate}
\sq

\subsubsection{The metric}
\label{subsubsecExplicitMetricLP}
We consider a function $f\in C^m_\per(\R^d)$ and we define for all $z\in \R^d$ a homogeneous polynomial $\pi_z\in \H_m$ as follows 
\be
\label{defPizLpMet}
\pi_z := \sum_{|\alpha| = m} \frac{\partial^m f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!},
\ee
and a non homogeneous polynomial $\mu_z\in \P_{m-1}$
\be
\label{defMuzLpMet}
\mu_z := \sum_{|\alpha| < m} \frac{\partial^{|\alpha|} f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!}.
\ee
We recall the classical Taylor formula : for any $z, h\in \R^d$
\be
\label{defTaylor}
f(z+h) - \mu_z(h) = m\int_0^1 \pi_{z+th}(h) (1-t)^{m-1} dt,
\ee
and we denote by $\omega$ the modulus of continuity of the $\Z^d$ periodic function $z\mapsto \pi_z$
$$
\omega(r) := \sup_{|z-z'|\leq r} \|\pi_z - \pi_{z'}\|.
$$
We recall that $\volBall$ denotes the volume of the euclidean unit ball $B(0,1)$.
\begin{lemma}
\label{lemmaEstimSmooth}
\begin{itemize}
\item (Difference of two values of $f$)
We have for any $z,h\in \R^d$
$$
|f(z+h)- \mu_z(h)| \leq |\pi_z(h)| + |h|^m \omega(|h|).
$$
\item (Error estimate on an ellipse)
Defining $S(z) := H(z)^{-\frac 1 2}$ we have 
\be
\label{eqLocSmooth}
e_H(f\sep z)_p \leq (\volBall \det S(z))^\frac 1 p (\|\pi_z\circ S(z)\|+ \|S(z)\|^m \omega(\|S(z)\|)).
\ee
\item (Error with respect to a metric)
Assume that $H\in \bH_\per$ has the form
$$
H(z) = (\det M(z))^{\frac{-1}{mp+d}} M(z)
$$
where $\|\pi_z \circ M(z)^{-\frac 1 2}\|\leq 1$ for all $z\in \R^d$.
Then for all $\lambda>0$
$$
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq \volBall^{\frac 1 p} (1+ \omega_H(\lambda^{-\frac 1 2}))\|(\det M)^{\frac m {2d}}\|_{L^\tau([0,1]^d)},
$$
where $\omega_H$ is a function expressed in terms of $\omega$ and $H$, which satisfies $\omega_H(\mu) \to 0$ as $\mu\to 0$.
\end{itemize}
\end{lemma}

\proof
\begin{itemize}
\item 
This point is a direct consequence of the Taylor formula \iref{defTaylor}. Indeed 
$$
f(z+h) - \mu_z(h) = \pi_z(h)+ m\int_0^1 (\pi_{z+th}(h)-\pi_z(h)) (1-t)^{m-1} dt,
$$
thus 
$$
|f(z+h) - \mu_z(h)-\pi_z(h)|\leq m\int_0^1  |h|^m\omega(|h|) (1-t)^{m-1} dt = \omega(|h|) |h|^m.
$$

\item Observing that $B_H(z) = \{z+S(z) u \sep |u|\leq 1\}$ we obtain 
\begin{eqnarray*}
e_H(f\sep z)_p &\leq& |B_H(z)|^{\frac 1 p} \sup_{|h|_{H(z)} \leq 1} |f(z+h) - \mu_z(h)| \\
&\leq&  |B_H(z)|^{\frac 1 p}\sup_{|h|_{H(z)} \leq 1} |\pi_z(h)|+|h|^m \omega(|h|)\\
&=& (\volBall \det S(z))^\frac 1 p (\|\pi_z\circ S(z)\|+ \|S(z)\|^m \omega(\|S(z)\|)).\\
%& = & \left(\frac \cPi {\sqrt{\det H(z)}}\right)^\frac 1 p \left(\left\|\pi_z \circ H(z)^{-\frac 1 2}\right\| + \left\|H(z)^{-\frac 1 2}\right\|^m \omega\left(\left\|H(z)^{-\frac 1 2}\right\|\right)\right)
\end{eqnarray*}
\item Defining 
$$
S(z) := H(z)^{-\frac 1 2} = (\det M(z))^{\frac 1 {2(mp+d)}} M(z)^{-\frac 1 2}
$$
and recalling that $\pi_z$ is homogeneous of degree $m$ we obtain 
$$
\det S(z) = (\det M(z))^{\frac {-mp} {2(mp+d)}} \stext{ and } \|\pi_z \circ S(z)\|\leq (\det M(z))^{\frac m {2(mp+d)}}.
%, \quad \|S(z)\| = ??
$$
Applying \iref{eqLocSmooth} to $\mu S$ for some $\mu>0$ we obtain 
\begin{eqnarray*}
e_{\mu^{-2} H}(f\sep z)_p &\leq& (\volBall \det (\mu S(z)))^\frac 1 p (\|\pi_z\circ (\mu S(z))\|+ \|\mu S(z)\|^m \omega(\|\mu S(z)\|)),\\
&=& \mu^{\frac d p+m} (\volBall \det S(z))^\frac 1 p (\|\pi_z\circ S(z)\|+ \|S(z)\|^m \omega(\mu \|S(z)\|)),\\
&=& \mu^{\frac d p+m} \volBall^\frac 1 p \left(1+\|M(z)^{-\frac 1 2}\|^m \omega(\mu \|S(z)\|)\right)
\end{eqnarray*}
Hence
$$
e_{\mu^{-2} H}(f\sep z)_p \leq \mu^{\frac d p+m} \volBall^\frac 1 p (1+ \omega_H(\mu))
$$
where 
$$
\omega_H(\mu) := \sup_{z\in \sR^d} \|M(z)^{-\frac 1 2}\|^m \omega(\mu \|S(z)\|).
$$
Note that $\omega_H(\mu)$ is finite and tends to zero as $\mu\to 0$, since the functions $M$ and $S$, which are defined in terms of  $H \in \H_\per$, are continuous and $\Z^d$ periodic.
Therefore 
\begin{eqnarray*}
e_{\mu^{-2} H}(f)_p &:=& \left\|\sqrt[2p]{\det (\mu^{-2} H(z))}\, e_{\mu^{-2} H}(f\sep z)_p\right\|_{L^p([0,1]^d)}\\
&\leq & \mu^m \volBall^\frac 1 p (1+ \omega_H(\mu)) \left\|\sqrt[2p]{\det H(z)}\right\|_{L^p([0,1]^d)}\\
&=& \mu^m \volBall^\frac 1 p (1+ \omega_H(\mu)) m(H)^\frac 1 p
\end{eqnarray*}

On the other hand 
$$
m(H) =\int_{[0,1]^d} \sqrt{\det H(z)} dz =\int_{[0,1]^d} (\det M(z))^{\frac {mp} {2(mp+d)}}.
$$
Since $\frac 1 \tau = \frac m d+ \frac 1 p$ we thus have 
$$
\frac {mp} {2(mp+d)} = \frac {m\tau}{2d}.
$$
Recalling that $m(\mu^{-2} H) = \mu^{-d} m(H)$, we obtain as announced
\begin{eqnarray*}
m(\mu^{-2} H)^\frac m d e_{\mu^{-2} H}(f)_p &\leq& \volBall^\frac 1 p (1+ \omega_H(\mu)) m(H)^{\frac m d+ \frac 1p}\\
&=& \volBall^\frac 1 p (1+ \omega_H(\mu)) \|(\det M)^{\frac m {2d}}\|_{L^\tau([0,1]^d)}
\end{eqnarray*}
which concludes the proof of this lemma. \sq
\end{itemize}

The next result is announced in the introduction under the reference Theorem \ref{thSmooth}.

\begin{theorem}
There exists a constant $C=C(m,d)$ such that the following holds.\\
For each $f\in C^m_\per$ such that $z\mapsto K(d^m f(z))$ is not identically $0$, there exists a metric $H \in \bH_\per\cap \bH_g$, which is also $C^\infty$, and such that for all $\lambda \geq 1$
$$
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|K(d^m f)\right\|_\tau,
$$
where $\frac 1 \tau := \frac m d+ \frac 1 p$.
\end{theorem}
\proof
We recall that $K^{(\alpha)}(\pi) \leq \|\pi\|_\sC$ for any $\alpha\in(0, \infty)$, and that $K^{(\alpha)}$ converges pointwise to $K_\sC$ as $\alpha\to \infty$.
It follows, using the theorem of dominated convergence for integrals, that 
$$
\lim_{\alpha\to \infty} \|K^{(\alpha)}(\pi_z)\|_{L^\tau([0,1]^d)} = C_0 := \|K_\sC(\pi_z)\|_{L^\tau([0,1]^d)}.
$$
Observe that $\|K_\sC(\pi_z)\|_{L^\tau([0,1]^d)}$ since $z\mapsto K(d^m f(z))$ is not identically $0$ and is equivalent to a continuous function according to Lemma \ref{lemmaKAK}. From this point we consider a fixed $\alpha\in (0, \infty)$ such that $\|K^{(\alpha)}(\pi_z)\|_{L^\tau([0,1]^d)} < 2C_0$.
Since $\cM^{(\alpha)} : \H_m \sm\{0\}\to S_d^+$ is continuous, and since $\cM^{(\alpha)}(\pi) \to 0$ as $\pi \to 0$, the extended map $\cM^{(\alpha)} : \H_m\to S_d$ where $\cM^{(\alpha)}(0) = 0$ is also continuous.

The function $M_0 : \R^d \to S_d$ defined by 
$$
M_0(z) := \cM^{(\alpha)} (\pi_z)
$$
is therefore continuous and satisfies 
$
\|(\det M_0)^\frac m {2d}\|_{L^\tau([0,1]^d)} <2C_0
$
and for all $z\in \R^d$ we have either $\pi_z=0$ or $\|\pi_z \circ M_0(z)^{-\frac 1 2}\| \leq 1$.
We consider $\ve_1>0$ sufficiently small in such way that $M_1 := M_0+ \ve_1\Id$ still satisfies $\|(\det M_1)^\frac m {2d}\|_{L^\tau([0,1]^d)} <2C_0$, and we observe that $\|\pi_z \circ M_1(z)^{-\frac 1 2}\| < 1$ for all $z\in \R^d$.

We consider a $C^\infty$ non-negative radially symmetric compactly supported function $\psi$ of integral one, a mollifier, and we set $\psi_\ve(z) := \ve^{-d}\psi(z/\ve)$. We choose $\ve_2>0$ sufficiently small in such way that the $C^\infty$ mollification $M_2 := \psi_{\ve_2} * M_1$ of $M_1$ still satisfies $\|(\det M_2)^\frac m {2d}\|_{L^\tau([0,1]^d)} <2C_0$ and $\|\pi_z \circ M_2(z)^{-\frac 1 2}\| < 1$ for all $z$ in the compact set $[0,1]^d$, hence for all $z\in \R^d$ by periodicity.

Defining $H\in \bH_\per$ by
$$
H_0(z) := (\det M_2(z))^{\frac {-1}{mp+d}} M_2(z).
$$
Hence 
$$
m(\lambda H_0) e_{\lambda H_0}(f)_p \leq \volBall^\frac 1 p (1+\omega_{H_0}(\lambda^{-\frac 1 2})) \|(\det M_2)^\frac m {2d}\|_{L^\tau([0,1]^d)}
$$
Since $\omega_{H_0}(\lambda^{-\frac 1 2}) \to 0$ as $\lambda \to \infty$, we obtain for $\lambda$ sufficiently large
$$
m(\lambda H_0) e_{\lambda H_0}(f)_p \leq 2 \volBall^\frac 1 p \|K_\sC(\pi_z)\|_{L^\tau([0,1]^d)}\leq C \|K(d^m f)\|_{L^\tau([0,1]^d)} 
$$
where $C := \frac{2 \volBall^\frac 1 pn_\sC}{m!}.$
Since $H_0$ is $C^\infty$ and periodic, we obtain from Remark \ref{remHomog} in the previous chapter that $\lambda H_0\in \bH_a$ when $\lambda$ is sufficiently large.
Defining $H := \Lambda H_0$, where $\Lambda$ is a sufficiently large constant we conclude the proof of this theorem.
\sq

\section{Approximation in the $W^{1,p}$ norm}
\label{secApproxW1P}
We extend in this section to the $W^{1,p}$ norm the results presented in the previous section for the $L^p$ norm. This extension is not straightforward due to the following phenomenon : the gradient of the interpolation $\interp_\cT^{m-1} g$ of a function, or of the twisted mollification $f_H$ may have strong undesirable oscillations which are not present in the original function. 
These effects are avoided in the case of quasi-acute meshes and metrics, but these objects have less flexibility than the larger class of graded meshes and metrics. Furthermore current anisotropic mesh generation software seem to be based on graded classes rather than quasi acute ones.
We therefore split the theory into two parts, one devoted to quasi-acute classes, and the other to graded ones.

\subsubsection{Quasi-acute triangulations and metrics}
\label{subsubsecErrMeshMetW1PA}

It is established in Chapter \ref{chapW1P} that the gradient of the interpolation of a function on a quasi-acute mesh is well behaved. More precisely, there exists a constant $C=C(m,d)$ such that for any simplex $T$ and any $g\in W^{1,\infty}(T)$ one has 
\be
\label{eqGradS}
\|\nabla \interp_T^{m-1} g\|_{L^\infty(T)} \leq C S(T) \|\nabla g\|_{L^\infty(T)}.
\ee
The next lemma establishes a counterpart of this property in the context of metrics : the gradient of the twisted mollification of a function by a quasi-acute metric is also well behaved.
\be
\label{eqGradQA}
\dil_z (f_H)  \leq C \sqrt{\det H(z)} \, \|\nabla f\|_{L^1(B_H(z))}
\ee

%\begin{lemma}[does  not seem to work $\to$ simpler option $H^{-\frac 1 2}$ Lipschitz.]
%%\label{lemmaBoundedQA}
%There exists $C=C(m,d, \vp)$ such that the following holds.
% Let $H\in \bH_a$ be a quasi-acute metric, and let $f\in W^{1,1}_\loc$. Then $f_H\in W^{1,\infty}_\loc$ and for all $z\in \R^d$
%\be
%\label{eqGradQA}
%\dil_z (f_H)  \leq C \sqrt{\det H(z)} \, \|\nabla f\|_{L^1(B_H(z))}
%\ee
%where $\dil_z(f_H) := \lim_{\ve \to 0} \|\nabla f_H\|_{L^\infty(B(z,\ve))}$ is the local dilatation of $f$ at $z$.
%\end{lemma}
%\proof
%We denote by $B_d:= \{z\in \R^d \sep |z|\leq 1\}$ the euclidean unit ball in $\R^d$.
%%$$
%%B_d := \{z\in \R^d \sep |z|\leq 1\}.
%%$$
%%We denote by $B_d
%%For any matrix $A \in \M_{d,d}$ such that $A^\trans A = H^{-1}$ we thus have
%Defining $S(z) := H(z)^{-\frac 1 2}$ we thus have 
%\be
%\label{eqFHS}
%f_H(z) = \int_{B_d} f\left(z- S(z) u\right) \vp(|u|) du.
%\ee
%For any isometry $p\in \cO_{2d,d}$, the transposed map $p^\trans : B_{2d}\to B_d$ transports the Lebesgue measure on $B_{2d}$ onto a measure on $B_d$, proportional to the Lebesgue density by a radial factor $\mu(|\cdot|)$ which is independent of $p$. Indeed $p^\trans : B_{2d}\to B_d$ is simply the projection onto the $d$ first coordinates, in an appropriate orthogonal basis of $\R^{2d}$.
%We thus have for any $g\in L^1(B_d)$ and any $p\in \cO_{2d,d}$
%\be
%\label{eqChg2dd}
%\int_{B_d} g(u) \mu(|u|) du= \int_{B_{2d}} g(p^\trans v) dv.
%\ee
%For any matrix $A \in \M_{2d,d}$ such that $A^\trans A = H(z)^{-1}$, there exists an isometry $p\in \cO_{2d,d}$ such that 
%$
%A = pS(z).
%$
%Applying \iref{eqChg2dd} to the function 
%$$
%g(u) := f(z-S(z) u) \frac{\vp(|u|)}{\mu(|u|)}
%$$
%and recalling \iref{eqFHS} we obtain
%\begin{eqnarray*}
%f_H(z) = \int_{B_d} g(u) \mu(|u|) du = \int_{B_{2d}} g(p^\trans v) dv = \int_{B_{2d}} g(z-S(z)p^\trans v) \, \frac{\vp(|p^\trans v|)}{ \mu(|p^\trans v|)} dv
%\end{eqnarray*}
%%$$
%%g^H(z) = \int_{B_{2d}} g(z-S(z)p^\trans v) \, \vp(|p^\trans v|) \, \mu(|v|) dv
%%$$
%Therefore, for any $z'\in \R^d$ and any $A,B\in M_{2d,d}$ such that $A^\trans A = H(z)^{-1}$ and $B^\trans B = H(z')^{-1}$ we obtain 
%$$
%f_H(z) - f_H(z') = \int_{B_{2d}} (f(z-A^\trans v)-f(z-B^\trans v)) \frac{ \vp(|p^\trans v|)}{ \mu(|p^\trans v|)} dv.
%$$
%Hence 
%$$
%|f_H(z)-f_H(z')| \leq C \int_{B_{2d}} |f(z-A^\trans v)-f(z-B^\trans v)|  dv.
%$$
%where
%$$
%C := \sup_{r\geq 0} \frac{|\vp(r)|}{\mu(r)}.
%$$
%Note that $C$ is finite since $\supp(\vp) \subset [0,1)$, hence since the support of a function is always a closed set  $\supp(\vp) \subset [0,r_0]$ for some $0\leq r_0<1$, and since $\mu$ is positive on $[0,1)$. Since $H\in \bH_a$ there the matrices $A,B\in M_{2d,d}$ satisfying $A^\trans A = H(z)^{-1}$ and $B^\trans B = H(z')^{-1}$ can be chosen in such way that $|A-B| \leq |z-z'|$.
%%We denote $\delta := |z-z'|$, and we choose the matrices $A,B$ in such way that $\|B-A\|\leq \delta$.
%We thus have for any $v\in B_{2d}$
%$$
%|(z-A^\trans v) - (z'-B^\trans v)|\leq |z-z'|+|(A-B)^\trans v| \leq 2 |z-z'|
%$$
%and therefore
%\begin{eqnarray*}
%|f_H(z)-f_H(z')| &\leq& C \int_{B_{2d}} 2 |z-z'| \dil(f_{|B(z+A^\trans v, 2|z-z'|)}) dv \\ %\dil_{z+A^\trans v}(g\sep 2 |z-z'|) dv\\
%&=& 2C |z-z'| \sqrt{\det H(z)} \int_{B(z,H)} \dil(f_{B(z+u , 2 |z-z'|)}) \mu(|u|) du%\dil_{z+u}(g\sep 2 ) dv
%\end{eqnarray*}
%We assume in the next equations that $g\in C^1_\per$, in such way that $\dil_z(g,\ve)$ tends uniformly to $\dil_z(g)$ as $\ve \to 0$. Therefore
%\begin{eqnarray*}
%\dil_{z_0}(g^H) &:=& \lim_{\ve\to 0} \sup_{z,z'\in B(z_0, \ve)} \frac{|g^H(z)-g^H(z')|}{|z-z'|}\\
%&\leq & \lim_{\ve \to 0} \sup_{z\in B(z_0, \ve)} 2C  \sqrt{\det H(z)} \int_{B(z,H)} \dil_{z+u}(g\sep 2 \times 2 \ve) dv\\
%&=& 2 C \sqrt{\det H(z_0)} \int_{B(z_0,H)} |\nabla g(z_0+u)| dv.
%\end{eqnarray*}
%
%By density of $C^1_\per$ in $W^{1,1}_\per$ we obtain that $L_H$ defines a bounded operator $W^{1,1}\to W^{1,\infty}$ with norm
%$$
%\|L_H\|_{W^{1,1}\to W^{1, \infty}} \leq 2C \max_{z_0} \sqrt{\det H(z_0)}
%$$
%The left and right hand side of \iref{eqDilInt} are thus continuous functions of $g\in W^{1,1}_\per$. Since the inequality holds for all $g\in C^1_\per$ it holds by continuity for all $g\in W^{1,1}_\per$.
%
%\sq

\begin{lemma}
There exists $C=C(m,d)$ such that the following holds. Let $H\in \bH_a$, and let $H' := 4^2 H$.
\begin{itemize}
\item (Local error estimate) 
Let $\cT\in \bT$, let $z\in \R^d$, let 
$
\cT_z := \{T\in \cT \sep T \subset B_{H'}(z,2)\}
$
and let $\Omega_z$ be the union of all triangles in $\cT_z$.
Then for any $f\in W^{1,p}_\loc$
\be
\label{eqLocFA}
\|\nabla( f-\interp_\cT^{m-1} f_{H'})\|_{L^p(\Omega_z)} \leq C e_H^a(f\sep z)_p \max_{T\in \cT_z} S(T).
\ee

%and $S(T)\leq S_0$ for all $T\in \cT_z$ then 
%Let $T$ be a simplex let $z\in T$, and assume that $\cH_T \geq H'(z)$.
%
%For any $f\in L^p_\loc$ one has 
%$$
%\|f-\interp_T^{m-1} f_{H'}\|_{L^p} \leq C e_H(f\sep z)_p,
%$$
%where $C=C(m,d)$. ($C$ is independent of $H$, $T$ and $f$.)
\item (Global error estimate)
Let $\cT\in \bT_\per$ and assume that for all $T\in \cT$ and all $z\in \cT$ one has 
$
\cH_T \geq H'(z).
$
Then for any $f\in W^{1,p}_\per$
\be
\label{eqGloFA}
\|\nabla (f-\interp_\cT^{m-1} f_{H'})\|_{L^p([0,1]^d)} \leq C e_H^a(f \sep z) \max_{T\in \cT} S(T).
\ee
\end{itemize}
\end{lemma}

\proof The proof is extremely similar to the proof of Proposition \ref{propErrMeshMet}, for the approximation in the $L^p$ norm.

\begin{itemize}
\item
%We define $S_z:= \max \{S(T) \sep T \in \cT_z\}$, in such way that  and we obtain for all $T\in \cT_z$
%We recall that there exists a constant $C_a = C_a(m,d)$ such that for any simplex $T$ and any $g\in W^{1,\infty}(T)$ one has
%$$
%\|\nabla \interp_T^{m-1} g\|_{L^\infty(T)} \leq C_a\, S(T) \,  \|\nabla g\|_{L^\infty(T)}. 
%$$
%We define $S_z:= \max \{S(T) \sep T \in \cT_z\}$.
%The proof is nearly identical to the proof of Lemma ??, where $C_{\interp}$ is replaced with $C_a S_z$ and $\|\vp\|_{L^\infty}$ with $C_\vp$.

%We denote by $C_{\interp,g}$ the norm of the interpolation operator $\nabla \interp_\TEq^{m-1} : C^0(\TEq) \to C^0(\TEq)$. We recall that for any simplex $T$, the simplex $\cH_T^{-\frac 1 2}(T)$ is the image of the reference equilateral simplex $\TEq$ by a rotation and a translation. It follows that 
%%, and we observe using the change of variables that for any triangle $T$ and any $g\in C^0(T)$ one has 
%$$
%\|\cH_T^{-\frac 1 2} (\nabla \interp_T^{m-1} g)\|_{L^\infty(T)}\leq C_{\interp} \|\cH_T^{-\frac 1 2}(\nabla g)\|_{L^\infty(T)}.
%$$
%We define $C_{\interp a} := C_a \max\{S(T) \sep T \in \cT_z\}$.
We denote by $C_a$ the constant appearing in \iref{eqGradS}, and by $C_\vp$ the constant appearing in \iref{eqGradQA}.

Let $\mu\in \P_{m-1}$ be a polynomial satisfying $\|\nabla (f-\mu)\|_{L^p(B_H(z))} \leq C_\proj e_H^a(\nabla f\sep z)_p$.
Let $g := f-\mu$ and let $T\in \cT_z$.
We have 
\begin{eqnarray*}
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq & |T|^\frac 1 p \|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
&\leq & C_a S(T) |T|^\frac 1 p \|\nabla g_{H'}\|_{L^\infty(T)}\\
&\leq & C_a S(T) |T|^\frac 1 p \|\nabla g_{H'}\|_{L^\infty(B_{H'}(z,2))}\\
&\leq & C_a S(T) C_\vp |T|^\frac 1 p \max_{z'\in B_{H'}(z,2)}  \frac{\|\nabla g\|_{L^1(B_{H'}(z'))}}{|B_{H'}(z')|}\\
&\leq & 8^dC_a S(T) C_\vp  |T|^\frac 1 p \frac{\|\nabla g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|}.
\end{eqnarray*}
Denoting $C_* := 8^dC_a C_\vp$ and $S_z := \max\{S(T) \sep T\in \cT_z\}$ we obtain as in \iref{propErrMeshMet}
%Therefore as previously 
\begin{eqnarray*}
\|\nabla \interp_\cT^{m-1} g_{H'}\|_{L^p(\Omega_z)} %&=& \left(\sum_{T\in \cT_z} \|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)}^p \right)^{\frac 1 p} \\
%&\leq & C_* S_z \frac{\|\nabla g\|_{L^1(B_{H}(z))}}{|B_{H}(z)|} \left(\sum_{T\in \cT_z} |T|\right)^\frac 1 p\\
%& \leq & C_* S_z  \|\nabla g\|_{L^1(B_{H}(z))}|B_{H}(z)|^{1-\frac 1 p}\\
& \leq & C_* S_z  \|\nabla g\|_{L^p(B_{H}(z))}
\end{eqnarray*}

Eventually we obtain 
\begin{eqnarray*}
\|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p(\Omega_z)} &=& \|\nabla (g-\interp_\cT^{m-1} g_H)\|_{L^p(\Omega_z)} \\
&\leq &\|\nabla g\|_{L^p(\Omega_z)}+ \|\nabla \interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)}\\
& \leq & (1+C_*S_z) \|\nabla g\|_{L^p(B_{H}(z))}\\
&\leq & (1+C_* S_z) C_\proj e_H(\nabla f\sep z)_p
\end{eqnarray*}
which concludes the proof of \iref{eqLocFA}.

\item
This proof \iref{eqGloFA} is nearly identical to the proof of the second point of Proposition \ref{propErrMeshMet}, and details are left to the reader.
%We define $S_\cT$ and we proceed identically to identical to Lemma ??.
%
%For each triangle $T\in \cT$ we define 
%$$
%\Omega_T := \{z\in \R^d \sep T \subset B_{H'}(z,2)\} \stext{ and } n(T) := \int_{\Omega_T} \sqrt{\det H(z)} dz.
%$$
%It follows from Lemma ?? that $n_T \geq ??$.
%
%We denote by $\cT_*$ a system of representatives of $\cT$ for the equivalence relation 
%$$
%T \sim T' \stext{ if } T =T'+u \text{ for some } u \in \Z^d.
%$$
%We therefore obtain 
%\begin{eqnarray*}
%e_H(\nabla f)_p^p &=& \int_{z\in [0,1]^d} \sqrt{\det H(z)} \, e_H(\nabla f\sep z)_p^p dz\\
%&\geq& (CS_\cT)^{-p} \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p(\Omega_z)}^p dz \\
%&=& (CS_\cT)^{-p} \int_{z\in [0,1]^d} \sqrt{\det H(z)}\, \sum_{T\in \cT_z} \|\nabla(f-\interp_\cT^{m-1} f_H)\|_{L^p(T)}^p dz \\
%&=& (CS_\cT)^{-p}\sum_{T\in \cT_*} n_T \|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p(T)}^p \\
%& \geq & (CS_\cT)^{-p} \|\nabla (f-\interp_\cT^{m-1} f_H)\|_{L^p([0,1]^d)}^p \min_{T \in \cT} n_T.
%\end{eqnarray*}
\sq
\end{itemize}


\subsection{Existence of an optimal metric for smooth functions}
\label{subsecExistsMetW1P}

We construct in this subsection a metric adapted to the approximation of a sufficiently smooth function, when a sufficiently large mass of the metric is authorized. Our method is similar to the proof of the analogous results in the case of the $L^p$ norm, and requires in particular to solve an optimization problem at each point.
We then focus on the more specific case of piecewise linear an piecewise quadratic approximation in two dimensions, and we give an explicit expression of the metric in terms of the the derivatives of the approximated function.

\subsubsection{A well posed variant of the shape function} 
\paragraph{Quasi-acute metrics.\\}

The shape function $L_a$, associated to quasi-acute metrics and triangulations for finite element approximation in the $W^{1,p}$ norm, is defined as follows
$$
L_a(\pi) := \inf_{A\in \SL_d} \|(\nabla \pi) \circ A\| = \inf\{(\det M)^{\frac{m-1}{2d }} \sep \|(\nabla \pi) \circ M^{-\frac 1 2}\| \leq 1 \}.
$$
For each $\pi\in \H_m$ we denote by $G(\pi)\in \H_{2m-2}$ the squared norm of the gradient of $\pi$
$$
G(\pi) := |\nabla \pi|^2 = \sum_{1\leq i \leq d} \left(\frac{\partial\pi}{\partial x_i}\right)^2.
$$
We thus obtain  
\be
\label{eqLK}
L_a(\pi) = \inf_{A\in \SL_d} \sqrt{\|G(\pi) \circ A\|} =\sqrt{K'( G(\pi))}, 
\ee
where $K' : \H_{2m-2} \to \R_+$ refers to the shape function previously studied in the context of the $L^p$ norm, but applied to polynomials of degree $2m-2$ instead of $m$: 
for all $\Pi \in \H_{2m-2}$, 
$$
K'(\Pi) := \inf \{\|\Pi\circ A\| \sep A\in \SL_d\} = \inf\{(\det M)^{\frac{2m-2}{2d}} \sep \|\Pi \circ M^{-\frac 1 2}\|\leq 1\}.
$$

Our results developed for the shape function $K$ in \S \ref{subsecExistsMetLP} therefore extend in a straightforward manner to the shape function $L_a$. %, and we obtain the following
\begin{prop}
\label{propLALA}
For each $\alpha\in (0, \infty)$ define $L_a^{(\alpha)} : \H_m \to \R_+$ as follows
$$
L_a^{(\alpha)}(\pi) :=  \inf\{\kappa(M)^\frac 1 \alpha (\det M)^{\frac{m-1}{2d }} \sep \|G(\pi) \circ M^{-\frac 1 2} \|_{\sC} \leq 1 \text{ and } \kappa(M) \leq e^\alpha \}.
$$
%\begin{itemize}
%\item (Existence of a minimizer)
For each $\pi\in \H_m\sm \{0\}$ the minimum defining $L_a^{(\alpha)}(\pi)$ is attained for an unique matrix $\cM_a^{(\alpha)}(\pi)$, and depends continuously on $\pi$.
%\end{itemize}
\end{prop}
\proof
This proposition is a direct consequence of Proposition \ref{propContLift}.
\sq
The functions $L^{(\alpha)}_a$ converge pointwise decreasingly to the function 
$$
L_{a, \sC} := \inf_{A\in \SL_d} \sqrt{\|G(\pi) \circ A\|_\sC}
$$
which is equivalent to $L_a$. This property is sufficient for our analysis, but we find it worthwhile nevertheless to mention a few additional properties of $L_a$.
\begin{prop}
There exists $C = C(m,d)$ such that the following holds.
\begin{itemize}
\item (Equivalence to a continuous function)
There exists a continuous function $L_{a,c} : \H_m \to \R_+$ such that for all $\pi\in \H_m$
$$
C^{-1}L_{a,c} \leq L_a \leq C L_{a,c}.
$$
\item (Convergence to the unconstrained problem)
For all $\ve>0$ there exists $\alpha$ such that for all $\pi \in \H_m$
$$
L_a^{(\alpha)}(\pi) \leq C L_a(\pi) + \ve \|\pi\|.
$$
\end{itemize}
\end{prop}
\proof
These results are a direct consequence of \iref{eqLK} and Proposition \ref{lemmaKAK}.
\sq

\paragraph{Graded metrics}
The shape function $L_g$ associated to graded metrics and triangulations for finite element approximation in the $W^{1,p}$ norm, is defined as follows
$$
L_g(\pi) := \inf_{A\in \SL_d} \|A^{-1}\| \|\nabla (\pi\circ A)\| = \inf \{(\det M)^{\frac{m-1} {2d}} \sep \|M\|^{\frac 1 2} \| \nabla (\pi \circ M^{-\frac 1 2})\|\leq 1\}.
$$
The next proposition introduces a variant of the shape function $L_g$, which is defined by a well posed optimization problem.
%Similarly to the other shape functions $K$ and $L_a$, the next proposition 
%Our results developed for the shape function $K$ in \S \ref{subsecExistsMetLP} therefore extend in a straightforward manner to the shape function $L_a$. %, and we obtain the following
\begin{prop}
\label{propLALG}
For each $\alpha\in (0, \infty)$ define $L_g^{(\alpha)} : \H_m \to \R_+$ as follows
$$
L_g^{(\alpha)}(\pi) := \inf\{\kappa(M)^\frac 1 \alpha (\det M)^\frac{m-1}{2d} \sep \sqrt{\|M\|} \|\pi\circ M^{-\frac 1 2}\|_\sC \leq 1 \text{ and } \kappa(M) \leq e^\alpha\}.
$$
For each $\pi\in \H_m\sm \{0\}$ the minimum defining $L_g^{(\alpha)}(\pi)$ is attained for an unique matrix $\cM_a^{(\alpha)}(\pi)$, and depends continuously on $\pi$.
\end{prop}
\proof
This proposition is a direct consequence of Proposition \ref{propContLift}.
\sq
The functions $L^{(\alpha)}_g$ converge pointwise decreasingly to the function 
$$
L_{g, \sC} := \inf_{A\in \SL_d} \sqrt{\|A^{-1}\|} \|\pi\circ A\|_\sC
$$
which is equivalent to $L_g$. Indeed there exists a constant $C$ such that $
C^{-1} \|\pi\|_\sC\leq \|\nabla \pi\|\leq C\|\pi \|_\sC
$ for all $\pi\in \H_m$, since these two quantities are norms on $\H_m$.
This property is sufficient for our analysis, but we find it worthwhile nevertheless to mention a few additional properties of $L_g$.
\begin{prop}
\label{propLGCont}
There exists $C = C(m,d)$ such that the following holds.
\begin{itemize}
\item (Equivalence to a continuous function)
There exists a continuous function $L_{g,c} : \H_m \to \R_+$ such that for all $\pi\in \H_m$
$$
C^{-1}L_{g,c} \leq L_a \leq C L_{g,c}.
$$
\item (Convergence to the unconstrained problem)
For all $\ve>0$ there exists $\alpha$ such that for all $\pi \in \H_m$
$$
L_g^{(\alpha)}(\pi) \leq C L_g(\pi) + \ve \|\pi\|.
$$
\end{itemize}
\end{prop}
\proof
The key property is to establish that the upper semi continuous function $L_g$ is equivalent to its lower semi continuous envelope $\underline L_g$, as established in Lemma \ref{lemmaLGSemi} belov. From this point to equivalence to a continuous function and the convergence to the unconstrained problem are obtained proceeding exactly as in Proposition \ref{lemmaKAK}.
\sq

The next lemma is the key technical ingredient to the proof of Proposition  \ref{propLGCont} above.
\begin{lemma}
\label{lemmaLGSemi}
Denote by $\underline L_g$ the lower semi continuous envelope of $L_g$, which is defined as follows 
$$
\underline L_g(\pi) := \liminf_{\pi'\to \pi} L_g(\pi') = \lim_{\ve \to 0} \inf_{\|\pi'-\pi\|\leq \ve} L_g(\pi'). 
$$
There exists a constant $C_\lsc = C_\lsc(m,d)$ such that $L_g \leq C_\lsc \underline L_g$ on $\H_m$.
%for all $\pi\in \H_m$
%$$
%L_g(\pi) \leq C \underline L_g(\pi).
%$$
\end{lemma}

\proof
This proof is extremely similar to the proof the analog property for the shape function $K$ in point 2. of Lemma \ref{lemmaKAK}, but nevertheless we need to introduce an intermediate : a variant  variant $\gL$ of the shape function $L_g$.
%We apply the same method to a variant $\gL$ of the shape function $L_g$.
%Nevertheless the same method cannot be directly applied we need to introduce an intermediate : the shape Yet the same method cannot be directly applied

\paragraph{A variant $\gL$ of the shape function $L_g$\\}
We define an auxiliary function $\gL$ on $M_d \times \H_m$ as follows 
\be
\label{defgL}
\gL(B,\pi) := \inf_{A\in \SL_d} \|A^{-1}B\| \|\pi\circ A\|.
\ee
We denote by $C_0$ a constant such that
$
C_0^{-1} \|\pi\|\leq \|\nabla \pi\| \leq C_0 \|\pi\|
$
for all $\pi \in \H_m$,
%Observing that 
%$$
%L_g(\pi) = \inf \{\|A\| \|\nabla(\pi\circ A^{-1})\| \sep |\det A| = 1\}
%$$
we obtain  
\be
\label{eqGLL}
C_0^{-1} L_g(\pi) \leq \gL(\Id, \pi) \leq C_0 L_g(\pi).
\ee
Taking the lower limit of the previous inequality as $(B', \pi') \to (\Id, \pi)$ we obtain 
\be
\label{eqGLLInf}
C_0^{-1} \underline L_g(\pi) \leq \underline \gL(\Id, \pi) \leq C_0 \underline L_g(\pi).
\ee
We establish below that there exists $C$ such that $\gL \leq C \underline \gL$ on $M_d \times \H_m$. Combining this point with \iref{eqGLL} and \iref{eqGLLInf} yields the announced result.

\paragraph{Vanishing of $\gL$\\}

Consider a converging sequence $(B_n, \pi_n) \to (B,\pi)$ in $M_d \times \H_m$. We establish in this paragraph that following property : 
$$
\text{ if } \lim_{n \to \infty} \gL(B_n, \pi_n)=0 \stext{ then } \gL(B, \pi) = 0.
$$
If $\gL(B_n, \pi_n) \to 0$ then there exists a sequence $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, such that 
\be
\label{eqAnBnPin}
\lim_{n \to \infty} \|A_n^{-1} B_n\| \|\pi_n\circ A_n\| =0.
\ee
For each $n$ consider the principal value decomposition $A_n = U_n D_n V_n$, where $U_n, V_n \in \cO_d$ and $D_n$ is a diagonal matrix satisfying $\det D_n = 1$, with positive %and decreasing 
diagonal coefficients $t_n = (t_{n,1}, \cdots, t_{n,d})$.
% where 
%\be
%\label{eqtni}
%t_{n,1} \geq \cdots \geq t_{n,d}>0.
%\ee
We have for any $n \geq 0$, since $U_n$ is orthogonal,
$$
\|A_n^{-1} B_n \| \|\pi\circ A_n\| = \| V_n^\trans D_n^{-1} U_n^\trans B_n \| \|\pi\circ (U_n D_n V_n)\| = \|D_n^{-1} U_n^\trans B_n \| \|\pi\circ (U_n D_n)\|.
$$
Since the collection $\cO_d$ of orthogonal matrices is compact, the sequence of orthogonal matrices $V_n$ admits a converging sub-sequence $V_{\vp(n)} \to V$. We define $B' := U^\trans B$, $\pi' := \pi \circ U$, and we observe that
\be
\label{eqgLBPip}
\cL(B, \pi) = \cL(B', \pi').
\ee
We also define
$$
B'_n := U_{\vp(n)}^\trans B_{\vp(n)}, \quad  \pi'_n := \pi_{\vp(n)} \circ U_{\vp(n)}, \stext{ and } D'_n := D_{\vp(n)}
$$
in such way that 
\be
\label{eqBpPip}
\lim_{n \to \infty} (B'_n,\pi'_n) = (B',\pi') \stext{ and } \lim_{n \to \infty} \|D'^{-1}_n B'_n\| \|\pi'_n\circ D'_n\| = 0.
\ee
We thus recognise \iref{eqAnBnPin} except that the matrices $A_n$ are replaced with diagonal matrices $D'_n$ with their diagonal coefficients 
$$
t'_n := (t'_{n,1}, \cdots , t'_{n,d}) =  (t_{\vp(n),1}, \cdots , t_{\vp(n),d}) 
$$
ordered decreasingly. In order to avoid notational clutter we do not keep track of the sub-sequence extraction, and we simply write $\pi$, $\pi_n$, $B$, $B_n$, $D_n$, $t_n$ and $t_{n,i}$ instead of $\pi'$, $\pi_n'$, $B'$, $B_n'$, $D'_n$, $t_n'$ and $t_{n,i}'$.

We denote by $I\subset \{1, \cdots, d\}$ the collection of indices $i$ such that the associated line of $B$ is nonzero. There exists a constant $c>0$ such that for %all $n \geq 0$
%$$
%\|D_n B\| \leq C t_{n,i_0}
%$$
%and for 
all $n$ sufficiently large
\be
\label{eqDnB}
\|D_n^{-1} B_n\| \geq c \max_{i\in I} t_{n,i}^{-1}.
\ee
We denote by $\Lambda$ the collection of exponents
$$
\Lambda := \{\alpha\in \Z_+^d \sep |\alpha| \leq m\}
$$
and by $\pi_\alpha$, $\pi_{n,\alpha}$ the coefficients of $\pi$ and $\pi_n$ respectively, in such way that 
$$
\pi = \sum_{\alpha \in \Lambda} \pi_\alpha Z^\alpha \stext{ and } \pi_n = \sum_{\alpha\in \Lambda} \pi_{n, \alpha} Z^\alpha.
$$
It follows from \iref{eqBpPip} and \iref{eqDnB} that for any $\alpha\in \Lambda$ we have 
\be
\label{eqTnPin}
\lim_{n \to \infty} \left(\max_{i\in I} t_{n,i}^{-1}\right) \pi_{n, \alpha} t_n^\alpha = 0.
\ee
For each $t = (t_1, \cdots , t_d)\in \R_+^d$ we define 
$$
\Lambda(t) := \left\{\alpha\in \Lambda \sep\left(\max_{i\in I} t_{n,i}^{-1}\right) t_n^{\alpha} \geq 1\right\}.
$$
The set $\Lambda$, which is finite, has only a finite number of subsets. Hence there exists an extraction $\psi$ such that $\Lambda_* := \Lambda(t_\psi(n))$ does not depend on $n$. In view of \iref{eqTnPin} we thus have for all $\alpha\in \Lambda_*$
$$
\pi_\alpha = \lim_{n \to \infty} \pi_{n, \alpha} = 0. %\text{ for all } \alpha\in \Lambda_*. 
$$
Defining $D := D_{\psi(0)}$, and denoting by $t=(t_1, \cdots ,t_d)$, its diagonal coefficients we thus obtain 
$$
\lim_{n \to \infty} \|D^{-n} B\| \|\pi\circ D^n\| = 0. 
$$
Indeed $\|D^{-n} B\|\leq C \max_{i\in I}t_i^{-n}$ and 
$$
\left( \max_{i\in I}t_i^{-n}\right) \pi_\alpha t^{n\alpha} =  \pi_\alpha \left(t^{\alpha} \max_{i\in I}t_i^{-1}\right)^n
$$
equals $0$ if $\alpha\in \Lambda_*$, and tends to zero if $\alpha\in \Lambda\sm\Lambda_*$. It follows that $\gL(B,\pi) = 0$ as announced.

\paragraph{Lower semi-continuity\\}
We denote by $\cA$ the following compact subset of $M_d\times \H_m$
$$
\cA := \{(B,\pi) \in M_d \times \H_m \sep \|B\|=\|\pi\| = 1 \text{ and for all } A\in \GL_d \text{ one has } \|A^{-1}B\| \|\pi\circ A\|\geq 1\}.
$$

Clearly $\gL(B,\pi) = 1$ for all $(B, \pi)\in \cA$, therefore $\underline \gL$ does not vanish on $\cA$. Since $\underline \gL$ is lower semi continuous, it attains its minimum on $\cA$, we thus define 
$$
C^{-1} := \inf_\cA \underline \gL.
$$
Consider $(B, \pi) \in M_d \times \H_m$, and denote by $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, a minimizing sequence for the problem defining $\gL(B, \pi)$
\be
\label{eqAngLMin}
\lim_{n \to \infty} \|A_n^{-1} B \| \|\pi \circ A_n\| = \gL(B, \pi) = \inf_{A\in \SL_d} \|A^{-1} B \| \|\pi \circ A\|.
\ee
If $\gL(B, \pi) = 0$, then $\underline \gL(B, \pi)=0$ and there is nothing to prove. If $\gL(B, \pi)>0$, then consider an extraction $\vp$ such that the following quantities converge
$$
\lim_{n \to \infty} \frac{A_{\vp(n)}^{-1} B}{\|A_{\vp(n)}^{-1} B\|} = B_* \stext{ and } \lim_{n \to \infty} \frac{\pi\circ A_{\vp(n)}}{\|\pi\circ A_{\vp(n)}\|} = \pi_*.
$$

We now prove that $(B_*, \pi_*)\in \cA$.
Indeed $\|B_*\| = \|\pi_*\|=1$ by construction. Assume for contradiction that there exists $A\in \GL_d$ such that $\|A^{-1} B_*\|\|\pi_*\circ A\| = \delta <1$. We obtain 
\begin{eqnarray*}
& &\lim_{n \to \infty}  \|(A_{\vp(n)} A)^{-1} B \| \|\pi \circ (A_{\vp(n)} A)\| \\
&=& \lim_{n \to \infty} \|A_{\vp(n)}^{-1} B \| \|\pi\circ A_{\vp(n)}\| \frac {\|A^{-1}(A_{\vp(n)}^{-1} B) \|}{\|A_{\vp(n)}^{-1} B \|} \frac { \|(\pi\circ A_{\vp(n)})\circ A\|}{\|\pi\circ A_{\vp(n)}\|} \\
&=& \delta \gL(B, \pi)
\end{eqnarray*}
%$$
%\lim_{n \to \infty}  \|(A_{\vp(n)} A)^{-1} B \| \|\pi \circ (A_{\vp(n)} A)\| = \lim_{n \to \infty} \|A_{\vp(n)}^{-1} B \| \|\pi\circ A_{\vp(n)}\| \frac {\|A^{-1}(A_{\vp(n)}^{-1} B) \|}{\|A_{\vp(n)}^{-1} B \|} \frac { \|(\pi\circ A_{\vp(n)})\circ A\|}{\|\pi\circ A_{\vp(n)}\|} = \delta \gL(B, \pi)
%$$
which is a contradiction with the definition \iref{defgL} of $\gL$, hence $(B_*, \pi_*)\in \cA$ as announced.

Observe that  
\be
\label{eqLuLRatio}
\underline \gL\left(\frac{A_n^{-1} B}{\|A_n^{-1} B\|} \frac{\pi\circ A_n}{\|\pi\circ A_n\|}\right) = \frac{\underline \gL(B,\pi) }{\|A_n^{-1} B\|\|\pi\circ A_n\|} \ \underset {n \to \infty}  \longrightarrow \ \frac{\underline \gL(B,\pi)}{\gL(B,\pi)}
\ee
Since $\underline \gL$ is lower semi continuous and $(B_*, \pi_*)\in \cA$ we obtain
$$
\lim_{n \to \infty} \underline \gL\left(\frac{A_n^{-1} B}{\|A_n^{-1} B\|} \frac{\pi\circ A_n}{\|\pi\circ A_n\|}\right) \geq  \underline \gL(B_*, \pi_*) \geq C^{-1}.
$$
Combining this with \iref{eqLuLRatio} yields $\underline \gL(B,\pi) \geq \gL(B, \pi)$, which concludes the proof of this lemma.
\sq

\subsubsection{The metric}

We consider a function $f\in C^m_\per(\R^d)$ and we define for all $z\in \R^d$ the polynomials $\pi_z\in \H_m$ and $\mu_z\in \P_{m-1}$ as before, see \iref{defPizLpMet} and \iref{defMuzLpMet}.
%$$
%\frac{\pi_z}{m!} := \sum_{|\alpha| = m} \frac{\partial^m f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!},
%$$
%and $\mu_z\in \P_{m-1}$
%$$
%\mu_z := \sum_{|\alpha| < m} \frac{\partial^{|\alpha|} f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!}.
%$$
The Taylor development of $\nabla f$ close to a point $z\in \R^d$ is obtained by taking the gradient of the Taylor development of $f$ : 
$$
\nabla f(z+h) = \nabla \mu_z(h) + \nabla \pi_z(h) + o_z(|h|^{m-1}).
$$
The Taylor formula for the function $\nabla f : \R^d \to \R^d$ reads as follows 
\be
\label{defTaylorGrad}
\nabla f(z+h) - \nabla \mu_z(h) = (m-1)\int_0^1 \nabla \pi_{z+th}(h) (1-t)^{m-2} dt.
\ee
The previous analysis for the $L^p$ error $e_H(f)_p$ of a function $f$ with respect to a metric $H$, is easily extended to the $W^{1,p}$ errors $e_H^a(\nabla f)_p$ and $e_H^g(\nabla f)_p$.
Indeed this analysis is simply based on Taylor developments and on the properties of the shape function $K
$ exposed in Proposition \ref{lemmaKAK}. These properties are extended to the shape functions $L_a$ and $L_g$ in  Propositions \ref{propLALA} and \ref{propLALG} respectively.

Similarly to the $L^p$ norm, the key idea produce a metric of the form 
$$
H_\star := \Lambda (\det M_\star)^\frac{-1}{(m-1)p+d} M_\star %or \frac{-\tau}{dp}
$$
where $\star\in \{g,a\}$, and $M_\star$ as the form 
$$
M_\star(z) := \psi_{\ve_2}*(\cM^{(\alpha)}(\pi_z)+\ve_1\Id),
$$
where $\alpha$ is sufficiently large, $\ve_1$ is sufficiently small, $\psi$ is a mollifier and $\ve_2$ is sufficiently small, and eventually $\Lambda$ is sufficiently large. Except for the technical point presented in Lemma \ref{lemmaLGAdd}, we refer the reader to the case of the $L^p$ norm \S\ref{subsubsecExplicitMetricLP} for more details.


\begin{lemma}
\label{lemmaLGAdd}
Let $\pi\in \H_m$, let $M\in S_d^+$ and let $\alpha>0$. Then
\be
\label{eqMMALG}
\sqrt{\|M+\alpha\Id\|}\|\nabla (\pi\circ (M+\alpha\Id)^{-\frac 1 2})\| \leq \sqrt{\|M\|}\|\nabla (\pi\circ M^{-\frac 1 2})\|
%\text{If } \|M\|^\frac 1 2 \|\pi\circ M^{-\frac 1 2}\| \leq 1 \text{ then } \|M'\|^\frac 1 2 \|\pi\circ M'^{-\frac 1 2}\| \leq 1
\ee
\end{lemma}
\proof
We have for any $z\neq 0$
$$
\frac{\|M+ \alpha\Id\|}{\|M\|} = 1+ \frac\alpha{\|M\|} \leq 1+\frac{\alpha |z|^2}{\|z\|_M^2} = \frac{\|z\|_{M+\alpha\Id}^2}{\|z\|_M^2}.
$$
Furthermore $|(M+\alpha\Id)^{-\frac 1 2} u| \leq |M^{-\frac 1 2} u|$ for any $u \in \R^d$ since $M\leq M+\alpha \Id$.
Choosing $u = \nabla \pi(z)$, where $z\in \R^d$ is arbitrary; we thus obtain for any $m\geq 2$
$$
\sqrt{\|M+\alpha\Id\|} \frac{|(M+\alpha\Id)^{-\frac 1 2} (\nabla \pi (z))|}{\|z\|_{M+\alpha\Id}^{m-1}}\leq \sqrt{\|M\|} \frac{|M^{-\frac 1 2} (\nabla \pi (z))|}{\|z\|_M^{m-1}}
$$
Taking the infimum among all $z\neq 0$ we obtain the announced equation \iref{eqMMALG}, which concludes the proof of this lemma.
\sq

The construction of the metric adapted to the function $f$ presented above is unfortunately not very practical, because the map $\cM_\star^{(\alpha)} : \H_m\sm \{0\} \to S_d^+$, defined for each $\pi\in \H_m\sm\{0\}$ by a minimization problem, seems to be hard to compute.
The next proposition shows that this difficulty is avoided in the case of linear approximation or quadratic approximation in dimension $2$, since in that case there exists an explicit minimizer or near minimizer of the optimization problem defining $L_\star(\pi)$. The next proposition is announced in the introduction under the reference Proposition \ref{propLmIntro}.
\begin{prop}
\label{propLm}
\begin{itemize}
\item (Piecewise linear approximation, in any dimension)
If $m=2$ and $d\geq 2$, then for any $\pi\in \H_2$, one has 
$$
L_a(\pi) = 2|\det \pi|^\frac 1 d \stext{ and } L_g(\pi) =2 \sqrt{\|\pi\|} \sqrt[2d]{|\det \pi|}.
$$
The minimizing matrices $M$ in the minimization problems defining $L_a(\pi)$ and $L_g(\pi)$ are  respectively
$$
\cM_a(\pi) = 4[\pi]^2 \stext{ and } \cM_g(\pi) = \|\pi\| \, |[\pi]|
$$
\item (Piecewise quadratic approximation, in two dimensions)
If $m=3$ and $d=2$, let $\pi =  a x^3+ 3 b x^2 y+ 3 c x y^2+ d y^3\in \H_3$,
let 
$$
\cM_a(\pi) =  %\sqrt{ [\partial_x \pi]^2+ [\partial_y \pi]^2} = 
3 \sqrt{
\left(\begin{array}{cc}
a & b\\
b & c
\end{array}\right)^2
+
\left(\begin{array}{cc}
b & c\\
c & d
\end{array}\right)^2
}
$$
and let 
$$
\cM_g(\pi) := \cM_a(\pi) + \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}\Id
$$
where $\disc \pi$ is the discriminant of the cubic polynomial $\pi$ :  
\be
\label{eqDiscDet}
\frac{1} {27} \disc \pi= 4(ac-b^2)(bd-c^2) - (ad-bc)^2.
\ee

Then $\cM_a(\pi)$ and $\cM_g(\pi)$ are near minimizers of optimization problems defining $L_a(\pi)$ and $L_g(\pi)$ respectively. %(*details...*)
\end{itemize}
\end{prop}

\proof
For any homogeneous quadratic polynomial $\pi$ we denote by $[\pi]\in S_d$ the associated symmetric matrix, satisfying $z^\trans [\pi] z = \pi(z)$ for all $z\in \R^d$. Note that $\|\pi\| = \|[\pi]\|$.
\begin{itemize}
\item (The quadratic case)
%\paragraph{The quadratic case}
For any $\pi\in \H_2$ we have $\nabla \pi(z) = 2[\pi] z$. Hence $|\nabla \pi(z)|^2 = 4 z^\trans [\pi]^2 z$ and the announced result for $L_a$ easily follows.
For $L_g$, we are looking for $M$ of minimal determinant such that 
\be
\label{eqMPi}
2\|M^{\frac 1 2}\| \, \|M^{-\frac 1 2} [\pi] M^{-\frac 1 2}\|\leq 1.
\ee
Recalling that $\|AB\|\geq \|A\| \|B^{-1}\|^{-1}$ we obtain from \iref{eqMPi} that $2\|\pi \| \leq \|M^\frac 1 2\|$.
Hence 
\be
\label{eqMPiWeak}
4\|\pi\| \| M^{-\frac 1 2} [\pi] M^{-\frac 1 2}\|\leq 1.
\ee
The matrix of minimal determinant which achieves this equality is clearly $M = 4\|\pi\| \ |[\pi]|$. Since condition \iref{eqMPiWeak} is weaker than \iref{eqMPi}, and since $M$ also satisfies \iref{eqMPi} this concludes the proof.
%Furthermore, it also achieves the initial equality which concludes the proof.

\item (The cubic case)
The case of $L_a$ and $\cM_a$ is exposed in Chapter \ref{chapW1P}. We therefore turn to the case of $L_g$. 
Combining the homogeneity and the continuity of the functions involved, one easily shows that there exists a constant $C_0$ such that for all $\pi\in \H_3$
\be
\label{eqContHomog}
\begin{array}{ccccc}
C_0^{-1} \|\pi \| &\leq& \|\nabla \pi \| &\leq& C_0 \| \pi\|\\
C_0^{-1} \|\pi \| &\leq&  \lambda(\pi) :=\|\cM_a(\pi) \| &\leq& C_0 \| \pi\|,
\end{array}
\ee
and 
\be
\label{eqContHomog2}
\begin{array}{ccc}
\mu(\pi) := \|\cM_a(\pi)^{-1} \|^{-1} & \leq& C_0 \|\pi\|\\
\nu(\pi) := \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^\frac 1 3 &\leq&  C_0 \|\pi\|.
\end{array}
\ee
%\begin{eqnarray*}
%\label{eqNormGrad}
%C^{-1} \|\pi \| \leq& \|\nabla \pi \| &\leq C \| \pi\|\\
%\label{eqNormM}
%C^{-1} \|\pi \| \leq&  \lambda(\pi) :=\|\cM_a(\pi) \| &\leq C \| \pi\|\\
%&\mu(\pi) := \|\cM_a(\pi)^{-1} \|^{-1} & \leq C \|\pi\|\\
%\label{eqNormDisc}
%& \nu(\pi) := \left(\frac{|\disc\pi|}{\|\pi\|}\right)^\frac 1 3 &\leq  C \|\pi\|  
%\end{eqnarray*}
We consider below a fixed polynomial $\pi\in \H_3$, and we recall that 
$$
L_g(\pi) := \inf \{\sqrt{\det M} \sep \sqrt{\|M\|} \|\pi \circ M^{-\frac 1 2}\| \leq 1\}.
$$
\paragraph{Lower bound $L_g(\pi)\geq c \sqrt{\det \cM_g(\pi)}$.}
We consider $M\in S_d^+$ satisfying $1 \geq \|M^{\frac 1 2}\| \| \nabla (\pi \circ M^{-\frac 1 2}) \|$. Combining this with \iref{eqNormGrad} we obtain
$$
1 \geq C_0^{-1}  \|M^{\frac 1 2}\| \| \pi \circ M^{-\frac 1 2} \| \geq C_0^{-1} \|M^{\frac 1 2}\| \frac{\| \pi \|}{\| M^{\frac 1 2}\|^3} = \frac{\|\pi\|}{C_0 \|M\|},
$$
hence $\|\pi\| \leq C_0 \|M\|$. It follows that 
$$
1 \geq C_0^{-1} (C_0^{-1} \|\pi\|)^{\frac 1 2} \| \pi\circ M^{-\frac 1 2}\| = \|\ti \pi \circ M^{-\frac 1 2}\|,
$$
where $\ti \pi := C_0^{-\frac 3 2} \| \pi\|^{\frac 1 2} \pi$. %$\ti \pi := \mu \pi$ and $\mu := C^{-\frac 3 2} \| \pi\|^{\frac 1 2}$.
The solution $M_*$ of the minimization problem
$$
\inf\{ \det M \sep \|\ti \pi \circ M^{-\frac 1 2}\| \leq 1\}
$$
is known exactly in the case of cubic polynomials in two dimensions, see Chapter \ref{chapOptAniso}, and satisfies 
$$
(\det M_*)^3 = \kappa |\disc \ti \pi| = \kappa (C_0^{-\frac 3 2} \| \pi\|^{\frac 1 2})^4 |\disc \pi| = \kappa C_0^{-6} \| \pi\|^2 |\disc \pi|.
$$
where $\kappa$ is a positive constant which depends only on the sign of $\disc \ti \pi$.
Defining $c_0:=\kappa_*^\frac 1 6 C_0^{-1}$, where $\kappa_*$ stands for the minimial value of $\kappa$, we obtain 
\begin{eqnarray*}
L_g(\pi) &\geq& (\det M_*)^{\frac 1 2} \\
&= & \kappa^\frac 1 6 C_0^{-1} \|\pi\|^{\frac 1 3} |\disc \pi|^{\frac 1 6} \\
&\geq& c_0 \sqrt{\|\pi\| \nu(\pi)} %\left(\frac{|\disc\pi|}{\|\pi\|}\right)^\frac 1 6\\
%&\geq & \kappa^\frac 1 6 C^{-\frac 3 2} \|\cM_a(\pi)\|^\frac 1 2 
\end{eqnarray*}
On the other hand, there exists $c_1>0$ such that 
$$
L_g(\pi) \geq L_a(\pi) \geq c_1 \sqrt{\det \cM_a(\pi)} = c_1\sqrt{\lambda(\pi) \mu(\pi)}.
$$
Furthermore we have 
\begin{eqnarray*}
\det \cM_g(\pi) &=& (\lambda(\pi)+\nu(\pi))(\mu(\pi)+\nu(\pi)) \\
&\leq& (1+C_0^2)\min \{\lambda(\pi),\, \|\pi\|\} \left( 2\max\{\mu(\pi),\, \nu(\pi)\}\right)\\
&\leq & 2(1+C_0^2) \max \{\lambda(\pi) \mu(\pi), \, \|\pi\| \nu(\pi)\}.
\end{eqnarray*}
Thus leads us to the conclusion of our lower estimate for $L_g$
%Combining the last two equations, and recalling \iref{eqContHomog} and \iref{eqContHomog2} we obtain 
$$
\sqrt{\det \cM_g(\pi)}\leq C_* L_g(\pi) \stext{ where } C_*:= 2(1+C_0^2) \max \{c_0^{-1}, \, c_1^{-1}\}.
$$

\paragraph{The matrix $C\cM_g(\pi)$ satisfies the constraint for sufficiently large $C$.}
We establish in the paragraph that the matrix $M = C \cM_g(\pi)$ satisfies the inequality $\|M^{\frac 1 2}\| \| \nabla (\pi \circ M^{-\frac 1 2})\|\leq 1$ when $C$ is large enough (but independent of $\pi$), or equivalently that 
$$
\|\cM_g(\pi)\|^\frac 1 2 \|\cM_g(\pi)^{-\frac 1 2}( \nabla \pi(x,y))\| \leq C \stext{ when } \|(x,y)\|_{\cM_g(\pi)} \leq 1.
$$
It is established in Chapter \ref{chapW1P} that $\cM_a(\pi \circ U) = U^\trans \cM_a(\pi) U$ for any $U\in \cO_2$, and we have $\disc (\pi \circ U) = (\disc \pi) (\det U)^6 = \disc \pi$, see Chapter \ref{chapOptiAniso}. We may therefore assume, up to a rotation, that $\cM_a(\pi)$ is a diagonal diagonal matrix and that the first diagonal  coefficient is larger than the second one.
Therefore 
$$
\lambda(\pi)^2 = a^2+2b^2+c^2 \stext{ and } \mu(\pi)^2 = b^2+2c^2+d^2. (*\text{factor }3*)
$$
In order to avoid notational clutter, and since the polynomial $\pi\in \H_3$ is fixed, we denote below by $\lambda$, $\mu$ and $\nu$ the quantities $\lambda(\pi)$, $\mu(\pi)$ and $\nu(\pi)$.
%For that purpose we define 
%$$
%\mu^2 := a^2+2b^2+c^2 \stext{ and } \mu^2 := b^2+2c^2+d^2.
%$$
% The eigenvalues of $\cM_a(\pi)$ are therefore $\mu$ and $\mu$, and we may assume furthermore that $\mu \geq \mu$.
%We also define 
%$$
%\nu := \frac 1 3 \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}
%$$
Our purpose is to establish an upper bound on the quantity
\be
\label{eqMGGradPi}
\begin{array}{cl}
& \displaystyle\|\cM_g(\pi)\|^\frac 1 2 \|\cM_g(\pi)^{-\frac 1 2}( \nabla \pi(x,y))\| \\
=&  \displaystyle(a x^2+ 2 b xy + c y^2)^2 + \left(\frac {\lambda+\nu} {\mu+\nu}\right) (b x^2+ 2 c xy+ d y^2)^2.
\end{array}
\ee
%Our purpose is to bound
%$$
% (a x^2+ 2 b xy + c y^2)^2 + \left(\frac \mu {\max\{\mu, \nu\}}\right) (b x^2+ 2 c xy+ d y^2)^2 
%$$
under the hypothesis 
$$
\|(x,y)\|_{\cM_g(\pi)} = (\lambda+\nu) x^2+ (\mu+\nu) y^2 \leq 1,%\frac {x^2} {\lambda+\nu} + \frac {y^2} {\mu+\nu} \leq 1.
$$
which implies in particular $\lambda x\leq 1$ and $\max\{\mu,\nu\} y\leq 1$.
Injecting this in \iref{eqMGGradPi}, and recalling that $\nu\leq C_0^3 \lambda$, we see that we only need to bound the following quantities %We thus need to bound the quantities
\be
\label{eqabcLl}
\frac a {\lambda^2}, \, \frac b {\lambda \mu}, \, \frac c {\mu^2}
\stext{ and }
\frac \lambda \mu \frac b {\lambda^2}, \ \frac \lambda \mu \frac c {\mu \lambda}, \ \frac \lambda {\max\{\mu,\nu\}} \frac d {\max\{\mu, \nu\}^2}.
\ee
Observing that 
\be
\label{eqLlMax}
\mu \geq \max\{b,c,d\}
\stext{ and }
\lambda \geq \max\{a,b,c,\mu\} \geq \{a,b,c,d\}
\ee
we find that all the quantities appearing in \iref{eqabcLl} are smaller than one, except perhaps the last one : 
%
%Since $\lambda \leq \lambda+\nu \leq (1+C_0^2)\lambda$ and $\max\{\mu, \nu\} \leq \mu+\nu \leq 2\max\{\mu,\nu\}$ we only need to bound 
%The only difficulty comes from 
\be
\label{eqd}
\frac {\lambda d^2}{\max\{\mu, \nu\}^3}
\ee
Using the expression \iref{eqDiscDet} of the discriminant we find that 
$$
\frac{-\disc \pi}{27} = (a^2+b^2+c^2) d^2 + a Q(b,c,d)+R(b,c,d)
$$
where $Q$ and $R$ are homogenous polynomials of degree $3$ and $4$ respectively. Using \iref{eqLlMax} we therefore obtain, for a constant $C_1$ sufficiently large (but independent of $\pi$),
\begin{eqnarray*}
\lambda^2 d^2 &=& \frac{-\disc \pi}{27} - (a Q(b,c,d)+R(b,c,d)) \\
&\leq &\frac{\|\pi\| \nu^3} {27} +C_1 \lambda \mu^3 \\
&\leq &\left(\frac{C_0}{27} + C_1\right) \lambda \max \{\mu, \nu\}^3
\end{eqnarray*}
%It follows from the expression \iref{eqDiscDet} of the discriminant, and from \iref{eqLlMax}, that there exists a constant $C_1$ independent of $\pi$ and satisfying %norm of pi???
%$$
%%\sqrt 2 \nu ^3 \mu \geq \nu^3 \sqrt{\mu^2+ \mu^2} \geq 
%\frac{-\disc \pi} {27} \geq \lambda^2 d^2 - C_1 \lambda \mu^3.
%$$
%On the other hand we have $-\disc \pi \leq \nu^3 \|\pi\| \leq C_0 \nu^3 \lambda$.
%%On the other hand we have $\|\pi\|\leq \sqrt{\mu^2+\mu^2}\leq \sqrt 2 \mu$ and therefore 
%%$$
%%\frac{-\disc \pi} {27} \leq  \nu^3 \sqrt{\mu^2+ \mu^2}  \leq \sqrt 2 \nu ^3 \mu
%%$$
%Combining the last two equations we obtain
%$$
%\lambda^2 d^2 \leq \frac C {27} \nu^3 \lambda + C_1 \mu^3 \lambda \leq \left(\frac{C_0}{27} + C_1\right) \lambda \max \{\mu, \nu\}^3
%$$
The previous inequality yields a uniform bound on \iref{eqd}, which concludes the proof of this proposition.
%where $C_2 := \max\{C/27, C_1\}$.
%and therefore
%$$
%\frac{\lambda d^2}{\nu^3} \leq \sqrt 2 + C\left(\frac \lambda \nu\right)^3 \stext{ and } \frac{\lambda d^2}{\mu^3} \leq \sqrt 2\left(\frac \lambda \nu\right)^3 + C.
%$$
%Using the left part of the previous equation if $\mu\leq \nu$, and the right part otherwise, we obtain a bound on \iref{eqd} which concludes the proof.
\sq
\end{itemize}

\subsection{Approximation spaces}

For any $\star\in \{i,a,g\}$ and any $f\in W^{1,p}_\per$ we define a (nonlinear) quantity $|\nabla f|_{\star,p} \in [0, \infty]$ as follows 
$$
|\nabla f|_{\star,p} := \sup_{\mu \geq 1} \left(\mu^\frac m d\inf_{\substack{H \in \bH_\star\cap \bH_\per\\ m(H) \leq \mu}}e_H^\star(\nabla f)_p\right),
$$
where $e_H^i(\nabla f)_p$ refers to the quantity $e_H^a(\nabla f)_p$ or $e_H^g(\nabla f)_p$, since they coincide for isotropic metrics $H\in \bH_\per \cap \bH_i$.
\begin{theorem}
Define $\frac 1 \tau := \frac {m-1} d+ \frac 1 p$. If $\tau \geq 1$ and if the Sobolev injection $W^{m, \tau} \to W^{1,p}$ holds (which excludes the case $(m,p) = (2,\infty)$
%$m=2$ and $p=\infty$
) then one has
$$
|\nabla f|_{i,p} \leq C\left(\int_{[0,1]^2} \mathfrak M\left(|d^m f|^\tau\sep z\right) dz\right)^\frac 1 \tau.
$$
\end{theorem}
\proof
The proof is nearly identical to the $L^p$ case presented in \S \ref{subsecApproxSpaceLP}, and the details are thus left to the reader. The key argument is again the use of the metric
$$
\max\{1, \gM_\delta (|d^m f|^\tau\sep z) \} \Id.
$$
%The remaining details are left to the reader.
\sq


The quantities $|\nabla f|_{a,p}$ and $|\nabla f|_{g,p}$ are both smaller than $|\nabla f|_{i,p}$ but are not easily compared in general.
The author needs to admit that the quantity $|f|_{a,p}$ is not totally satisfying. Indeed, depending on the approximated function, quasi-acute metrics and simplices are generally not needed everywhere.

For instance, in the case $d=2$, $m=3$ of piecewise quadratic approximation in dimension $2$, it follows from the explicit expressions of near minimizers of $L_a$ and $L_g$ given in Proposition \ref{propLm} that 
$$
L_g(a x^3+ d y^3) \simeq \sqrt[3]{|ad| \max\{|a|,\, |d|\}} \stext{ and } L_a(a x^3+ d y^3) \simeq \sqrt{|ad|}.
$$
In contrast we obtain %using \ref{propLm} that 
$$
L_g(ax^3+3cx y^2) \simeq L_a(a x^3+3c xy^2) \simeq \sqrt{\max\{|a|,\, |c|\} |c|}.
$$
If the approximated function only exhibits anisotropic features of the type $ax^3+3cx y^2$, then the production of quasi-acute metrics is useless.
A typical example is the approximation of the mollification $f=\vp_\ve *g$ of a cartoon function $g$. The analysis presented in Chapter \ref{chapCartoon} shows that, close to the curves where $g$ is discontinuous, the mollification $f$ does have anisotropic features of the type $ax^3+3cx y^2$, where $|c|\ll |a|$. Therefore quasi-acute triangulations are not required in the neighborhood of these curves. In fact graded triangulations should be preferred in this context since they require a smaller number of triangles to create a thin layer along a curve, as illustrated by Theorem \ref{thOptGeom}.


\input{../Bibliography/Bibliography.tex}
\end{document}


==> ApproxTheory/ApproxTheoryTheseOld3.tex <==
%\input{../PreambleThese}
\section{Introduction} %, and metrics on a periodic bounded domain}
\label{secPer}


The main purpose of adaptive mesh generation, compared uniform mesh generation, is to reduce the number of simplices required to achieve a given task. Here are two relevant examples which 
are further discussed in this chapter:
\begin{enumerate}
\item
Given two domains of interest, generate the mesh with smallest possible cardinality that separates these
domains with a layer of simplices.
\item
Given a function $f$, generate the mesh of a prescribed cardinality $N$ that yields the best 
finite element approximation to $f$ of a given order $m-1$ in some prescribed norm $L^p$ or $W^{1,p}$.
\end{enumerate}
Both examples can be viewed as optimization problems posed on the set of meshes.
The second problem was dealt with in Chapter 2 and 3 in the case where $f$ is smooth, 
and an optimal mesh was constructed in the asymptotic regime $N\to +\infty$. The results
of the previous chapter have revealed that certain relevant classes of meshes can be equivalently
described in terms of riemannian metrics, and a natural objective is therefore
to translate the above problems as {\it optimization problems posed on the set of metrics}.
Optimization problems posed on metrics may indeed be easier to solve practically  
due to the continuous nature of these objects.
The goal of this chapter is to explain how this objective can be met for the
above two examples.

In the previous chapter, we have introduced the classes of meshes
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
and characterized the respectively equivalent classes of metrics
$$
\bH_i\subset \bH_a\subset \bH_g.
$$
These classes of meshes and metrics are defined on the entire unbounded domain $\R^d$.
The above optimization problems do not make sense in this setting since the 
number of element in such meshes is infinite. In order to circumvent this difficulty
while still avoiding the difficulties related to the boundary of a domain, we 
work in a periodized setting that we describe below.

\subsection{Periodic meshes and metrics}

We denote by $\bT_\per$ the collection of meshes $T\in \bT$ which satisfy the following properties:
\begin{enumerate}[i)]
\item (Translation invariance) For any $T\in \cT$ and any $u \in \Z^d$, one has $u+T \in \Z^d$.
\item (Constrained diameters) For any $T\in \cT$ one has $\cH_T\geq \Id$.
\end{enumerate}

Accordingly, we denote by $\bH_\per$ the collection of metrics $H \in \bH$ which satisfy the following properties:
\begin{enumerate}[i)]
\item (Translation invariance) For any $z\in \R^d$ and any $u \in \Z^d$, one has $H(z) = H(z+u)$.
\item (Constrained positivity) For any $z\in \R^d$ one has $H(z)\geq \Id$.
\end{enumerate}

A mesh $\cT\in \bT_\per$ can be regarded, thanks to the translation invariance property 
as a mesh of the compact periodic space 
\be
\label{perSpace}
\Pi^d := (\R/ \ZZ)^d,
\ee
also called the $d$-dimensional torus. %Note that $\Pi^d$ has no boundary.
The diameter constraint property ensures that the simplices $T$ of a periodic mesh $\cT \in \bT_\per$ do not have a significantly larger size than the fundamental cell $[0,1]^d$ of the standard $\Z^d$ periodic tiling of $\R^d$. 

Strictly speaking, a periodic mesh $\cT\in \bT_\per$ has an infinite cardinality. However it only contains a finite number of simplices up to translation by an element of $\Z^d$.  
For any $\cT\in \bT_\per$, we therefore denote by $\#(\cT)$ the number of equivalence classes in $\cT$ for the relation
$$
T \sim T' \text{ if and only if there exists } u \in \Z^d \text{ such that } \ T' = T+u.
$$
The number $\#(\cT)$ is finite, and is the the cardinality of $\cT$ seen as a mesh of the compact periodic space \iref{perSpace}.
We define the {\it mass} $m(H)$ of a periodic metric $H \in \bH_\per$ as follows
$$
m(H) :=  \int_{[0,1]^d} \sqrt{\det H}.
$$
Intuitively the mass of a metric $H$ and the cardinality of a mesh $\cT$ should be linked when
$H$ and $\cT$ are equivalent in the sense studied in the previous chapter.
We denote by $\TEq$ a fixed equilateral simplex centered at the origin of $\R^d$ and having its vertices on the unit sphere.
\begin{prop}
\label{propCardMass}
The cardinality of a mesh $\cT\in \bT_\per$ and the mass of a metric $H\in \bH_\per$ satisfy the following properties:
\begin{itemize}
\item If $\cH_T \leq C^2 H(z)$ for all $T\in \cT$ and all $z\in T$, then 
$
|\TEq|\#(\cT) \leq C^d  m(H).
$
\item 
If $H(z) \leq C^2 \cH_T$ for all $T\in \cT$ and all $z\in T$, then 
$
 m(H) \leq C^d |\TEq|\#(\cT).
$
\end{itemize}
In particular, if $\cT$ is $C$-adapted to $H$ in the sense of Definition \ref{defEqHT}, then 
\be
\label{eqCardMass}
C^{-d} m(H) \leq |\TEq| \,\#(\cT) \leq C^d m(H) .
\ee
\end{prop}

\proof
For any $z\in \R^d$ we denote by $T(z)$ the simplex $T\in \cT$ containing $z$.
Recalling (see Proposition \ref{propHT} in the previous chapter) that for any simplex $T$
$$
|T| \sqrt{\det \cH_T} = |\TEq|,
$$
we thus have 
\be
\label{eqCardT}
\#(\cT) = \int_{[0,1]^d} \frac {dz}{|T(z)|} = |\TEq|^{-1} \int_{[0,1]^d} \sqrt{\det \cH_{T(z)}} \, dz.
\ee
Furthermore we have $\det S \leq C^d \det S'$ for any $S,S'\in S_d^+$ satisfying $S \leq C S'$.
Applying this remark to the matrices $H(z)$ and $\cH_{T(z)}$ we obtain the announced inequalities, which concludes the proof of the proposition.
\sq

The equivalence between classes of meshes and metrics of $\R^d$ established in
Theorem \ref{thEquiv} of the previous chapter has an immediate generalization to periodic meshes and metrics.

\begin{theorem}
\label{thPer}
There exists a constant $C_0=C_0(d)$ such that for all $C \geq C_0$, 
\begin{enumerate}
\item The collection of meshes $\bT_{i,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_i \cap \bH_\per$.
\item If $d=2$, the collection of meshes $\bT_{a,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_a \cap \bH_\per$.
\item If $d=2$, the collection of meshes $\bT_{g,C} \cap \bT_\per$ is equivalent to the collection of metrics $\bH_g \cap \bH_\per$.
\end{enumerate}
\end{theorem}

\proof
The proof of Theorem \ref{thEquiv} presented in the previous chapter can be adapted to periodic metrics and triangulations with only slight changes, which are left to the reader.
\sq



\subsection{Compactness of metrics}
\label{subsecIntroCompact}

In order to ensure the existence of an ``optimal metric'' for a number of optimization problems 
posed on periodic and isotropic, quasi-acute or graded metrics, we need a property of 
compactness for such metrics.

We equip the set $\bH_\per$ of continuous and $\Z^d$ periodic metrics with a distance $d_\per$ which is defined as follows: for all $H,H'\in \bH_\per$
$$
d_\per(H,H') := \sup_{z\in [0,1]^d} d_\times (H(z), H(z)) = \sup_{z\in \R^d} d_\times (H(z) , H'(z)).
$$
Consider $H, H'\in \bH_\per$ and define $\delta = d_\per(H,H')$. We thus have for all $z\in \R^d$,
\be
\label{pointwiseCont}
e^{-2 \delta} H(z)\leq H'(z) \leq e^{2 \delta} H(z). 
\ee
One easily checks that 
%Hence the mass $H \mapsto m(H)$ is a continuous function of $H \in \bH_\per$ 
\be
\label{massCont}
e^{-d\delta} m(H) \leq m(H') \leq e^{d\delta} m(H),
\ee
and 
%as well as the distance $H \mapsto d_H(x,y)$ for any fixed $x,y\in \R^d$ : 
\be
\label{distCont}
e^{-\delta} d_{H}(x,y) \leq d_{H'}(x,y) \leq e^\delta d_{H}(x,y).
\ee
which shows that the mass $m \mapsto m(H)$ and the distance between to fixed points $H \mapsto d_H(x,y)$ depend continuously on $H \in \bH_\per$.


We establish in \S \ref{secCompact} the following compactness property : for any $M\geq 1$ and any symbol $\star \in \{i,a,g\}$ the collection of metrics 
$$
\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq M\}
$$
is a compact subset of $\bH_\per$.



\subsection{Separation of two domains}

Isotropic and anisotropic mesh adaptation is often used to separate some geometric sets, in the sense given by the following definition. For any closed subset $E \subset \R^d$ and any mesh $\cT\in \bT$ we define the neighborhood $V_\cT(E)$ of $E$ in $\cT$ as follows :
$$
V_\cT(E) := \bigcup_{\substack{T \in \cT,\\ T \cap E\neq\emptyset}} T.
$$
We say that a mesh $\cT\in \bT$ separates two closed sets $X,Y\subset \R^d$ if and only if 
$$
V_\cT(X) \cap V_\cT(Y) = \emptyset,
$$
in other words if $X$ and $Y$ have disjoint neighborhoods in the mesh $\cT$. 

A natural objective is to build a mesh of minimal cardinality which separates two given regions. 
Consider two closed, disjoint and $\Z^d$-periodic sets $X,Y\subset \R^d$. We consider in \S \ref{secOptGeom} the optimization problem posed on triangulations 
$$
m_{\star,C_0}(X,Y) := \min\{ \#(\cT) \sep \cT\in \bT_\per \cap \bT_{\star,C_0} \text{ and }  \cT \text{ separates } X \text{ and } Y\}
$$
where $\star \in \{i,a,g\}$ is a symbol and $C_0\geq 1$ is a constant.
We establish then this problem is equivalent to the following
optimization problem posed on metrics, if the dimension is $d=2$:
$$
m_\star(X,Y) := \min\{ m(H) \sep H \in \bH_\per\cap \bH_\star \text{ and } H \text{ separates } X \text{ and } Y\}, 
$$
where say that a metric $H$ separates $X$ and $Y$ if 
$$
d_H(x,y) \geq 1 \text{ for all } (x,y) \in X\times Y.
$$
Precisely, we show that there exists a constant $C = C(C_0)\geq 1$, independent of the sets $X,Y$,
such that 
$$
C^{-1} m_\star(X,Y)\leq m_{\star,C_0}(X,Y) \leq C m_\star(X,Y).
$$

Imposing more constraints on the triangulation typically raises the number of triangles required to achieve a given task, and likewise assuming more regularity of the metric raises the mass required for a given task.
We illustrate this remark in the context of the separation of domains as follows.
We fix the parameter $r_0 := 1/4$ and we define the periodic set 
$$
X := \{x\in \R^d \sep d(x,\Z^d) \leq r_0\},
$$
where $d(x,E) := \min \{|x-e|\sep e\in E\}$,
and for any $0<\delta\leq r_0$ 
$$
Y_\delta := \{y\in \R^d \sep d(y,\Z^d)\geq r_0 + \delta\}.
$$
The sets $X$ and $Y_\delta$ are illustrated on Figure \ref{figXYDelta}.
The following equivalences are established as $\delta\to 0$
\begin{eqnarray*}
m_i(X,Y_\delta) &\simeq& \delta^{-(d-1)},\\
m_a(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2 } |\ln \delta|,\\
m_g(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2}.
\end{eqnarray*}

A construction closely related to the separation of the sets $X$ and $Y_\delta$ is presented on Figure \ref{figDisk} in the main introduction of this thesis.
\begin{figure}
\centering
\includegraphics[width=4cm,height=4cm]{\pathPic/Meshing/XYDelta.pdf}
\caption{The sets $X$ (light gray) and $Y_\delta$ (dark gray), with $d=2$ and $\delta = 0.1$. \label{figXYDelta}}
\end{figure}

\subsection{Approximation in a given norm}

One of the key purposes of anisotropic mesh generation is the adaptive approximation of functions,
as discussed extensively in Chapters 2 and 3. In order to study this problem from the point of view of metrics, we introduce an error $e_H(f)_p$ associated to a function and a metric, and we compare this quantity with the approximation error of $f$ on a mesh.

For that purpose we denote by $B_H(z)$ the open ball of radius $r$ around $z$ for the norm $\|\cdot \|_{H(z)}$
(therefore an ellipse):
$$
B_H(z) := \{z+u \sep \|u\|_{H(z)} < 1\}.
$$
For any exponent $p$, $1\leq p \leq \infty$, and any $f\in L^p_\loc(\R^d)$ we denote by $e_H(f\sep z)_p$ the error of best approximation of $f$ on $B_H(z)$:
\be
\label{defEH}
e_H(f\sep z)_p := \inf_{\mu\in \sP_{m-1} } \|f-\mu\|_{L^p(B_H(z))}.
\ee
We denote by $L^p_\per$ the collection of functions $f\in L^p_\loc(\R^d)$ which are $\Z^d$-periodic.
For all $f\in L^p_\per$ and all $H\in \bH_\per$ we define the approximation error $e_H(f)_p$ of $f$ associated to the metric $H$ as follows
\be
\label{defEHGlobal}
e_H(f)_p^p := \int_{[0,1]^d} \sqrt {\det H(z)} \, e_H(f\sep z)_p^p \, dz.
\ee

Consider a metric $H\in \bH_\per \cap \bH_g$ and a mesh $\cT\in \bH_\per$ such that 
\be
\label{eqTH4}
\cH_T \geq 4^2 H(z), \;\;  \,z\in T,\; T\in \cT,
\ee
%for any $T\in \cT$ and any $z\in T$.
which heuristically means that that the mesh $\cT$ is ``more refined'' than the metric $H$.
We establish in \S \ref{secApproxLP} that for any $f\in L^p_\per$  
\be
\label{eqBestLP}
\inf_{g\in V_{m-1}(\cT)} \|f-g\|_p \leq C e_H(f)_p
\ee
where $V_k(\cT)$ stands for the space of finite elements of degree $k$ on $\cT$, and $C$ is an absolute constant. Furthermore we give an explicit expression of a finite element approximation $g\in V_k(\cT)$ which satisfies \iref{eqBestLP}, namely
\be
\label{defGOpt}
g := \interp_\cT^{m-1} f_{H'}, %in fact 4^2 H
\ee
where $H' := 4^2 H$. We denote by $f_H$ the convolution \emph{distorted by the metric $H$} of a function $f$  with a fixed compactly supported mollifier $\vp$ (which satisfies a moments condition) 
$$
f_H(z) := \int_{\R^d} f(z+H(z)^{-\frac 1 2} u) \vp(|u|)du.
$$

The extension of the approximation result \iref{eqBestLP} to the $W^{1,p}$ semi-norm is not trivial sue to the fact that interpolation on simplices of large measure of sliverness is not a stable procedure. 

For any vector field $v\in L^p_\loc(\R^d, \R^d)$ and any metric $H\in \bH$ we introduce the two quantities
\be
\label{defEHA}
e_H^a(v\sep z)_p := \min_{\nu\in \sP_{m-2}^d} \|v-\nu\|_{L^p(B_H(z))}
\ee
and 
\be
\label{defEHG}
e_H^g(v\sep z)_p := \|H(z)\|^{\frac 1 2} \min_{\nu\in \sP_{m-2}^d} \|H(z)^{-\frac 1 2} (v-\nu)\|_{L^p(B_H(z))}.
\ee
%where $\P_{m-2}^d$ denotes the collection of $d$-plets of polynomials of degree $m-2$. 
If $v$ is $\Z^d$ periodic and if $H\in \bH_\per$, then we define $e_H^a(v)_p$ and $e_H^g(v)_p$ similarly to \iref{defEHGlobal}.

Consider a metric $H\in \bH_\per \cap \bH_a$ and mesh $\cT\in \bH_\per$ which satisfy \iref{eqTH4}. We establish that for any $f\in W^{1,p}_\per$  
\be
\label{eqBestW1PA}
\inf_{g\in V_{m-1}(\cT)} \|\nabla(f-g)\|_p \leq C \,e_H^a(\nabla f)_p \,\max_{T\in \cT} S(T)
\ee

This estimate should be compared with the following. Consider a metric $H\in \bH_\per \cap \bH_g$ and a mesh $\cT\in \bT$ which satisfy \iref{eqTH4} and in addition $C_0^2 H(z) \geq \cH_T$ for all $T\in \cT$ and $z\in T$. % (which means that the mesh $\cT$ is $C_0$-adapted to the metric $H$).
We establish that 
\be
\label{eqBestW1PG}
\inf_{g\in V_{m-1}(\cT)} \|\nabla(f-g)\|_p \leq C \, e_H^g(\nabla f)_p,
\ee
where the constant $C$ depends on $C_0$.

The function $g$ given by \iref{defGOpt} satisfies both estimates \iref{eqBestW1PA} and \iref{eqBestW1PG}.
These results put in light the price to pay to obtain the best error estimate \iref{eqBestW1PA} in the $W^{1,p}$ norm: the measure of sliverness should be uniformly bounded on $\cT$, and the metric $H$ should belong to $\bH_a$. If these conditions are not satisfied then we can only prove the estimate \iref{eqBestW1PG} which is sub-optimal since it penalizes the anisotropy of the metric $H$, see \iref{defEHG}.

\subsection{Asymptotic approximation and explicit metrics}
\label{subsecIntroAsympt}
We establish some counterparts for metrics of the asymptotic estimates presented in Chapters 2 and 3 for triangulations and more general meshes. 
Our estimates hold without restriction on the degree or the dimension, and apply to a sufficiently smooth function and to metrics an asymptotically large mass.

We denote by $\H_m$ the vector space of all homogeneous polynomials of degree $m$ in $d$ variables, and we define the \emph{shape function} $K$ as follows : for all $\pi \in \H_m$
\be
\label{defKIntro}
K(\pi) =\inf_{A\in \SL_d} \| \pi \circ A\|.
\ee
We establish that for any $\Z^d$ periodic and $C^m$ function
\be
\label{asymptLPMet}
\limsup_{\substack{H \in \bH_g\\  m(H)\leq M}} M^{\frac m d} e_H(f)_p \leq C \|K(d^m f)\|_\tau,
\ee
where the exponent $\tau$ is defined by $\frac 1 \tau := \frac m d+ \frac 1 p$.

The proof of this result would be greatly simplified if one could establish the existence of a smooth map $\pi\in \H_m \mapsto A(\pi)\in \SL_d$ such that $A(\pi)$ minimizes $\| \pi \circ A\|$. This is unfortunately not the case, and the key ingredient of the proof of \iref{asymptLPMet} is the definition and the analysis of a family $K^{(\alpha)}$ of functions which tend to $K$ as $\alpha\to \infty$ and which are defined by a well posed optimization problem (for which there exists a unique minimizer depending continuously on the parameter $\pi$).\\

In the case of $W^{1,p}$ norms we introduce two distinct \emph{shape functions}
\begin{eqnarray*}
L_a(\pi) &:=& \inf_{A\in \SL_d} \|(\nabla \pi)\circ A\| \\
L_g(\pi) &:=& \inf_{A\in \SL_d} \|A^{-1}\| \|\nabla (\pi\circ A)\| 
\end{eqnarray*}
We establish similar results to \iref{asymptLPMet}, for any $C^m$ and $\Z^d$ periodic function $f$
\be
\label{asymptA}
\limsup_{\substack{H \in \bH_a\\  m(H)\leq M}} M^\frac {m-1} d e_H^a(\nabla f)_p \leq C \|L_a(d^m f)\|_\tau\\
\ee
and 
\be
\label{asymptG}
\limsup_{\substack{H \in \bH_g\\  m(H)\leq M}} M^\frac {m-1} d e_H^g(f)_p \leq C \|L_g(d^m f)\|_\tau,
\ee
where $\tau$ is defined by $\frac 1 \tau := \frac {m-1} d + \frac 1 p$.\\

For a quadratic or cubic (in two dimensions) homogeneous polynomial $\pi$, we give an explicit expression of near-minimizers of the optimization problems defining $L_a(\pi)$ and $L_g(\pi)$ in terms of the coefficients of $\pi$.
This expression can be used to compute efficiently in numerical applications a metric $H$ adapted to the approximated function $f$ using the available information on the derivatives of $f$.

We also use these minimizers to compute the ratio $L_a(\pi) / L_g(\pi)\leq 1$, and we discuss for which polynomials this ratio is significantly small. In other words for which types of anisotropic features of the approximated function $f$ the use of quasi-acute triangulations leads to a significantly smaller approximation error than the use of graded anisotropic triangulations (which is the case in all numerical software known to the author).



\section{Compactness of metrics of a given mass} %A compactness property}
\label{secCompact}

The purpose of this section is to establish the following compactness result.
We recall that the collection $\bH_\per$ of $\Z^d$ periodic metrics is equipped with the distance 
$$
d_\per(H,H') := \sup_{z\in \sR^d} d_\times (H(z), H'(z)).
$$
\begin{theorem}
\label{thCompact}
For any symbol $\star \in \{i,a,g\}$ and any $m_0\geq 1$ the collection of metrics 
\be
\label{defHStarM}
\{H \in \bH_\per \cap \bH_\star \sep m(H) \leq m_0\}
\ee
is a compact subset of $\bH_\per$ 
\end{theorem}

The rest of this section is devoted to the proof of this theorem. Our first lemma establishes that the set \iref{defHStarM} is closed in $\bH_\per$.

\begin{lemma}
\label{lemmaClosed}
The set \iref{defHStarM} is closed in $\bH_\per$, as well as the sets $\bH_i, \bH_a, \bH_g$.
%The sets $\bH_\per \cap \bH_\star$, where $\star\in \{i,a,g\}$, are closed in of  $\bH_\per$, as well as the collection of metrics $\{H \in \bH_\per \sep m(H) \leq m_0\}$. 
\end{lemma}

\proof
As observed in \S \ref{subsecIntroCompact}, the pointwise evaluation, the distance between two fixed points $x,y\in \R^d$ and the mass define continuous maps on $\bH_\per$, see \iref{pointwiseCont},  \iref{massCont} and \iref{massCont}.
For any fixed $x,y\in \R^d$, the collection of all metrics $H \in \bH_\per$ which satisfy one of the following conditions
%\begin{enumerate}
%\item $m(H) \leq m_0$\\
%\item $d_\times (H(x),H(y)) \leq d_H(x,y)$\\
%\item $d_+ (H(x),H(y)) \leq |x-y|$\\
%\item $\|H(x)\| \|H(x)^{-1}\| =1$\\
%\end{enumerate}
\begin{eqnarray*}
 d_\times (H(x),H(y)) &\leq& d_H(x,y)\\
 d_+ (H(x),H(y)) &\leq& |x-y|\\
 \|H(x)\| \|H(x)^{-1}\| &=&1\\
m(H) &\leq& m_0
\end{eqnarray*}
is therefore a closed subset of $\bH_\per$.

A metric $H$ belongs to $\bH_g$ (resp. $\bH_a$, resp. $\bH_i$)
if and only if it satisfies the first of these inequalities for all $x,y\in \R^d$ (resp. the two first , resp. the three first).
The sets $\bH_i$, $\bH_a$ and $\bH_g$ are thus an intersection of closed subsets of $\bH_\per$, hence are closed.
% as well as the last inequality on the mass.
%
%the set \iref{defHStarM} if and only if, in the case $\star = g$ (resp. $\star = a$, resp. $\star = i$), it satisfies the first of these inequalities for all $x,y\in \R^d$ (resp. the two first , resp. the three first) as well as the last inequality on the mass.
%The set \iref{defHStarM} is therefore an intersection of closed sets, hence a closed set which concludes the proof.
The set \iref{defHStarM} is obtained by imposing the fourth inequality, and is therefore also closed.
\sq


%The key ingredient of this lemma is the 
%following classical
We recall a classical result which states that the collection of Lipschitz functions between two compact metric spaces is itself a compact metric space. It is an immediate consequence of Ascoli theorem.
\begin{theorem}
\label{thAscoli}
If two metric spaces $(X,d_X)$ and $(Y,d_Y)$ are compact, then the collection $\Lip(X,Y)$  of Lipschitz functions from $X$ to $Y$ is also compact when
equipped with the distance 
$$
d(f,g) := \max_{x\in X} d_Y(f(x),g(x)).
$$
\end{theorem}

We use this theorem to establish that %, similarly to finite dimensional spaces, 
closed and bounded subsets of $\bH_\per \cap \bH_g$ are compact.

\begin{lemma}
\label{lemmaCompact}
Any closed and bounded subset $\bH_*$ of $\bH_\per \cap \bH_g$ is compact.
\end{lemma}

\proof
Since the collection $\bH_*$ of metrics is bounded, the following quantity $M$ is finite %defined below is finite
$$
M^2 := \sup_{H \in \bH_*} \sup_{z\in [0,1]^d} \|H(z)\|.
$$
For any $x,y\in \R^d$ and any $H \in \bH_*$ we thus have $d_H(x,y) \leq M|x-y|$.

We consider the compact metric space $X :=[0,1]^d$, equipped with the distance $d_X(x,y) := M|x-y|$, and the compact metric space 
$$
Y := \{M \in S_d^+ \sep \Id \leq M \leq C^2 \Id\}
$$
equipped with the distance $d_\times$.
According to Theorem \ref{thAscoli} the metric space $\Lip(X,Y)$ is thus compact.

Consider a sequence $(H_n)_{n\geq 0}$ of elements of $H_*$. For all $n \geq 0$, the restriction $H_{n|[0,1]^d}$ is an element of $\Lip(X,Y)$. Since this space is compact there exists a sub-sequence $H_{\vp(n)}$ which converges uniformly on $[0,1]^d$. Recalling that $H_n$ is periodic for all $n\geq 0$ we find that $H_{\vp(n)}$ converges uniformly to a periodic metric $H \in \bH_\per$. 

Since that $\bH_*$ is closed in $\bH_\per \cap \bH_g$, and since $\bH_\per \cap \bH_g$ is closed in $\bH_\per$, we obtain that $\bH_*$ is closed in $\bH_\per$ and therefore $H \in \bH_*$ which concludes the proof.
\sq

The next lemma establishes that the set \iref{defHStarM} appearing in Theorem \ref{thCompact} is bounded. This set is closed according to Lemma \ref{lemmaClosed}, hence compact according to Lemma \ref{lemmaCompact}, which concludes the proof of Theorem \ref{thCompact}.

\begin{lemma}
\label{propCompact}
Let $m_0 \geq 1$ be a constant.
\begin{enumerate}
\item
There exists $C=C(m_0,d)$ such that for any $H \in \bH_g$ satisfying $H(z) \geq \Id \text{ for all } |z|\leq 1$ and 
$$
\int_{|z|\leq 1} \sqrt{\det H(z)} dz \leq m_0
$$
we have $\|H(0)\|\leq C^2$.
\item
The set 
$
\{H \in \bH_\per \cap \bH_g \sep m(H) \leq m_0\}
$
is bounded. %, and thus compact.
\end{enumerate}
\end{lemma}

\proof
We first show how 2. can be obtained assuming 1., and for that purpose we consider $H \in \bH_\per \cap \bH_g$ and $z_* %= (z_1, \cdots ,z_d)\in \R^d
$. The ball $\{z\in \R^d \sep |z-z_*|\leq 1\}$ is covered by the $2^d$ cubes 
$z_*+u+[0,1]^d$ where $u \in \{-1,0\}^d$. Consequently 
$$
\int_{|z-z_*|\leq 1} \sqrt{\det H(z)} dz \leq \sum_{u\in \{-1,0\}^d } \int_{z_*+u+[0,1]^d} \sqrt{\det H} = 2^d m_0
$$
and we already know that $H(z) \geq \Id$ for all $z\in \R^d$. It follows that $\|H(z_*)\|\leq C'^2$ where $C'$ is the constant associated to $2^d m_0$ in point 1., which concludes the proof of 2.\\


We now turn to the proof of 1. %, and for that purpose we consider a metric $H\in K_M$.
At each point $z\in \R^d$ we denote the eigenvalues of $H(z)$ by 
$$
\lambda_1^2(z) \geq \cdots \geq \lambda_d^2(z).
$$
For each $k \in \{1, \cdots ,d\}$ the function $\lambda_k$ is continuous and $\lambda(z)\geq 1$ for all $|z|\leq 1$.

Our purpose is to obtain an upper bound for $\lambda_1(0) = \sqrt{\|H(0)\|}$ in terms of $m_0$.
We shall proceed as follows : We first give an upper bound for $\lambda_d(0)$ that depends only on $m_0$, and then for each $1\leq k \leq d-1$ we give an upper bound for $\lambda_k(0)$ in terms of $m_0$ and $\lambda_{k+1}(0)$.


\paragraph{The upper bound on $\lambda_d(0)$.}
We define the ellipse 
%Denote by $\cE$ the ellipse 
$$
\cE := \{z\in \R^d \sep \|z\|_{H(0)} \leq \lambda_d(0)\}
$$
and observe that $|z|\leq 1$ for all $z\in \cE$.
We thus obtain using Corollary \ref{corolVol} 
$$
c_d \ln \lambda_d(0) \leq \int_\cE \sqrt{\det H(z)} dz \leq  \int_{|z|\leq 1} \sqrt{\det H(z)} dz \leq m_0,
$$
where $c_d>0$ is a constant. This gives as announced an upper bound on $\lambda_d(0)$ in terms of $m_0$.

\paragraph{The upper bound on $\lambda_k(0)$.}
The vector space $\R^d$ is the orthogonal sum 
$$
\R^d = U\oplus V
$$
 where $U$ is the sum of the eigenspaces  associated to the eigenvalues $\lambda_1^2(0), \cdots, \lambda_k^2(0)$ of $H(0)$ and $V$ is associated to the other eigenvalues $\lambda_{k+1}^2(0), \cdots, \lambda_d^2(0)$ of $H(0)$.
We have for all $u\in U$ and all $v\in V$, 
$$
\|u\|_{H(0)} \geq \lambda_k(0) |u| \stext{ and } \|v\|_{H(0)} \leq \lambda_{k+1}(0) |v|.
$$

We consider an isometry $P\in \cO_{d,k}$ (in the sense that $P^\trans P$ is the $k\times k$ identity matrix) satisfying $P(\R^k) = U$. 
For each $v\in V$ we define a metric $H_v$ on $\R^k$ as follows: for all $u \in \R^k$
$$
H_v(u) := P^\trans H_v(v+ Pu) P.
$$
It follows from Proposition \ref{propHG} (in the previous chapter) that $H_v$ belongs to the collection $\bH_g(\R^k)$.
We define 
$$
B_U := \{u \in \R^k \sep |u|\leq 1/2\} \stext{ and } B_V := \{v\in V \sep \lambda_{k+1}(0) |v| \leq 1/2\},
$$
as we observe that 
\be
\label{eqFubiniSet}
|P u+v| \leq 1 \text{ for all }  (u,v)\in B_U \times  B_V.
\ee
Recalling that $\lambda_i(z)\geq 1$ for all $1\leq i \leq d$ and $|z| \leq 1$ we obtain for all $(u,v) \in B_U \times B_V$
\be
\label{eqDetHHV}
\begin{array}{rcl}
\det H_v(u) &\leq& \lambda_1^2(Pu +v) \cdots \lambda_k^2(Pu +v)\\
&\leq &  \lambda_1^2(Pu +v) \cdots \lambda_d^2(Pu +v)\\
& =& \det H(Pu+v)
\end{array}
\ee
For any $u\in \R^k$ and any $v\in V$ we have according to \iref{eqLocalNorm}
\be
\label{eqLowerHV}
\|u\|_{H_v(0)} = \|Pu\|_{H(v)} \geq (1-\|v\|_{H(0)}) \|Pu\|_{H(z_*)} \geq \lambda_k(0) |u|/2, %(1-\lambda_{k+1}(0) |v|) \lambda_k(0) |u|.
\ee
and therefore 
$$
\{u\in \R^k \sep \|u\|_{H_v(0)} \leq \lambda_k(0)/4\} \subset B_U.
$$ 
Denoting by $c_k$ the constant from Corollary \ref{corolVol} applied in dimension $k$
%, and recalling \iref{eqLowerHV}, 
we therefore obtain for any $v\in B_V$
\be
\label{eqHVBU}
\int_{B_U} \sqrt{\det H_v(u)} du \geq c_k \ln ( \lambda_k(0)/4)
\ee
We thus obtain successively %According to Proposition (restrictMet) we have $H_v\in \bH_g^k$, therefore 
\begin{eqnarray*}
\int_{|z|\leq 1} \sqrt{\det H(z)} dz &\geq& \int_{v\in B_V} \int_{u\in B_U} \sqrt{\det H(P u +v)} du dv\\
&\geq & \int_{v\in B_V} \int_{u \in B_U} \sqrt{\det H_v(u)} du dv\\
& \geq & \int_{v\in B_V} c_k \ln(\lambda_k(0)/4) dv\\
& = & |B_V| c_k \ln( \lambda_k(0)/4)\\
& = & \frac{\omega_{d-k}}{(2\lambda_{k+1}(0))^{d-k}} c_k \ln( \lambda_k(0)/4).
\end{eqnarray*}
Where we use\iref{eqFubiniSet} and Fubini integration formula in the first line, \iref{eqDetHHV} in the second line, and \iref{eqHVBU} in the third line. In the last line we denote by  $\omega_{d-k}$ the volume of the unit ball in $\R^{d-k}$.

This inequality yields an upper bound on $\lambda_k(0)$ in terms of $M$ and $\lambda_{k+1}(0)$
$$
\lambda_k(0) \leq 4 \exp\left(\frac {m_0 (2\lambda_{k+1}(0))^{d-k}}{\omega_{d-k}}\right),
$$
which concludes the proof of this Theorem.
\sq


\section{Separation of two domains}
\label{secOptGeom}

We study in this section a geometrical problem: the separation of two sets using a triangulation, of minimal cardinality. Our first result, Proposition \ref{propEquivSep2}, establishes that this problem has an equivalent formulation in terms of metrics. 

\begin{proposition}
\label{propEquivSep2}
We assume that the collection of meshes $\bT_\per \cap \bT_{\star,C_0}$ and the collection of metrics $\bH_\per \cap \bH_\star$ are equivalent in dimension $d$, where $\star \in \{a,b,c\}$ is a symbol and $C_0\geq 1$ is a constant (this condition holds at least if $d=2$ according to Theorem \ref{thPer}).\\

There exists a constant $C \geq 1$ such that the following holds:\\
Let $X,Y \subset \R^d$ be two closed, disjoint and periodic sets, in the sense that 
$$
x+u \in X \stext{  and }y+u \in Y, \ \text{ for any } x\in X, \, y\in Y \text{ and }u \in \Z^d.
$$
Consider the two optimization problems 
\begin{eqnarray*}
m_{\star,C_0}(X,Y) &:=& \min\{ \#(\cT) \sep \cT\in \bT_\per \cap \bT_{*,C_0} \text{ and } \cT \text{ separates } X \text{ and } Y\},\\
m_\star(X,Y) &:=& \min\{ m(H) \sep H \in \bH_\per\cap \bH_* \text{ and } H \text{ separates } Y \text{ and } Y\}.
\end{eqnarray*}
Then 
\be
\label{eqMetricMeshSep}
C^{-1} m_\star(X,Y)\leq m_{\star,C_0}(X,Y) \leq C m_\star(X,Y).
\ee
%Furthermore a near minimizer of a problem can be built from a near minimizer of the other problem.
\end{proposition}

\proof %(* name of constants?*)
We denote by $C_1\geq 1$ a constant such that for any $\cT\in \bT_\per \cap \bT_{\star, C_0}$ there exists $H\in \bH_\per\cap \bH_\star$ which is $C_1$-equivalent to $\cT$, and vice versa.

The proof of this proposition is a simple translation between the vocabulary of meshes and the vocabulary of metrics.
We first establish that $m_\star(X,Y) \leq C m_{\star,C_0}(X,Y)$, and then that $m_{\star,C_0}(X,Y) \leq C m_\star(X,Y)$.\\

%\begin{itemize}
%\item
Let $\cT\in \bT_\per \cap \bT_{\star,C_0}$ be a mesh which separates the sets $X$ and $Y$, and let $H \in \bH_\per \cap \bH_\star$ be a metric which is $C_1$ equivalent to $\cT$. We thus have for any $T\in \cT$ and any $z\in T$
$$
C_1^{-2}H(z)\leq \cH_T \leq C_1^2 H(z).
$$
Let $x\in X$ and let $y\in Y$. Let $T_0\in \cT$ be the simplex containing $x$ and let $V_\cT(T_0)$ be the neighborhood of $T_0$ in $\cT$. %, in other words union of all simplices in $\cT$ which intersect $T_0$.
Since $x\in T_0$ and $y\notin V_\cT(T_0)$ we have $\|x-y\|_{\cH_{T_0}}\geq c := (C_0\sqrt d)^{-1}$ according to Proposition \ref{propNeighborT} (in the previous chapter). It follows that 
$$
d_H(x,y) \geq \ln (1+\|x-y\|_{H(x)}) \geq \ln(1+ \|x-y\|_{\cH_{T_0}}/C_1) \geq r:=\ln (1+c C_1^{-1}).
$$
%Up to replacing $r$ with $\min\{1,r\}$ we may assume that $0<r\leq 1$.
 The metric $\ti H := r^{-2} H$ thus belongs to $\bH_\per \cap \bH_\star$ since $0<r\leq 1$, see Remark \ref{remHomog}. Furthermore this metric separates the sets $X$ and $Y$ and satisfies according to Proposition \ref{propCardMass}
$$
m(\ti H)  \leq (C_1/r)^d |\TEq|\#(\cT).
$$ 
Taking the infimum over all meshes $\cT\in \bT_{*,C_0}$ which separate $X$ and $Y$ we obtain the left part of \iref{eqMetricMeshSep} : $m_*(X,Y) \leq |\TEq| (C_1/r)^d \, m_{*,C_0}(X,Y)$.\\

%\item
We now turn to the proof of the right part of \iref{eqMetricMeshSep}, and for that purpose we consider a Riemannian metric $H\in \bH_*\cap \bH_\per$ which separates the sets $X$ and $Y$. We consider a parameter $\lambda \geq 1$, which value will be specified later, and we observe that $\ti H := \lambda^2 H \in \bH_*\cap \bH_\per$.  Therefore there exists a mesh $T\in \bT_{*, T_0}\cap\bT_\per$ such that for all $T\in \cT$ and all $z\in \cT$ one has
$$
C_1^{-2} \ti H(z)\leq \cH_T \leq C_1^2 \ti H(z).
$$

Let us assume %for contradiction 
that $\cT$ does not separate the sets $X$ and $Y$, hence that $V_\cT(X) \cap V_\cT(Y) \neq \emptyset$. In that case there exists two simplices $T,T'\in \cT$ sharing a vertex $v$, and two points $x\in T \cap X$ and $y\in T'\cap Y$.
For any simplex $T$ and any $z,z'\in T$ we have $\|z-z'\|_{\cH_T} \leq 2$, see \iref{eqDiamTHT}.
%$$
%\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2
%$$
Therefore 
$$
\lambda \leq d_{\ti H}(x,y) \leq d_{\ti H}(x,v) + d_{\ti H} (v,y) \leq C_1 (\|x-v\|_{\cH_T}+ \|v-y\|_{\cH_{T'}}) \leq 4 C_1.
$$
We now choose the particular the value $\lambda := 4C_1+1$, which contradicts the the previous equation and shows that $\cT$ does separate $X$ and $Y$.
Furthermore
$$
|\TEq| \#(\cT) \leq  \, C_1^d \, m(\ti H) = (\lambda C_1)^d m(H).
$$
Taking the infimum among all metrics $H \in \bH_*$ which separate $X$ and $Y$ we obtain $|\TEq| m_{*,C_0}(X,Y) \leq  (\lambda C_1)^d m_*(X,Y)$, which %establishes the right part of \iref{eqMetricSep} and 
concludes the proof of this proposition.
\sq
%\end{itemize}

As a concrete example, we define $r_0 := 1/4$ and for any $0<\delta\leq r_0$ we consider in the following the sets 
%The rest of this section is devoted to the proof of Theorem \ref{thOptGeom}, in which we consider the particular sets 
\be
\label{defXYDelta}
X := \{x\in \R^d \sep d(x,\Z^d)\leq r_0\} \stext{ and } Y_\delta := \{y\in \R^d \sep d(y, \Z^d) \geq r_0+ \delta\},
\ee
which are illustrated on Figure \ref{figXYDelta}.
%where $r_0 := 1/4$ and $0<\delta\leq r_0$. 
%For any $\star\in \{i,a,g\}$ we obtain explicit equivalents of the quantities $m_\star(X,Y_\delta)$ as $\delta \to 0$, as well as an explicit expressions of a near minimizer $H_\delta^\star\in \bH_\per \cap \bH_\star$ to this optimization problem.
The next theorem gives a sharp estimate of the minimal mass of a metric which separates the sets $X$ and $Y_\delta$, as $\delta\to 0$.
The notation $\alpha_\delta \simeq \beta_\delta$ stands for the following : there exists a constant 
%For any two functions $F,G : (0,r_0]\to \R_+$ we write $F \simeq G$ if there exists a constant
 $C\geq 1$ such that for all $0 <\delta \leq r_0$
$$
C^{-1}\alpha_\delta \leq \beta_\delta \leq C \alpha_\delta.
$$

\begin{theorem}
\label{thOptGeom}
We have the equivalences
\begin{eqnarray*}
m_i(X,Y_\delta) &\simeq& \delta^{-(d-1)}\\
m_a(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2 } |\ln \delta|\\
m_g(X,Y_\delta) &\simeq& \delta^{-\frac{d-1} 2}.
\end{eqnarray*}
Furthermore for any $\star \in \{i,a,g\}$  and any $0< \delta \leq r_0$ the explicit metric $H_\delta^\star\in \bH_\star \cap \bH_\per$ defined below is a near minimizer of the problem $m_\star(X,Y_\delta)$. In other words $H_\delta^\star$ separates $X$ and $Y_\delta$ and satisfies $m(H_\delta^\star) \simeq m_\star(X,Y_\delta)$.
\end{theorem}

The proof is divided in two parts: we first give the explicit expression of the metrics $H_\delta^\star$ and we use it to obtain an upper bound on $m_\star(X,Y_\delta)$. We then prove a lower bound for $m_\star(X,Y_\delta)$.

\subsection{Explicit metrics and upper bound}

%The proof of this Theorem is split into three lemmas. 
We define in this section the metrics $H_\delta^\star$, where $\star \in \{i,a,g\}$ and $0 < \delta \leq r_0 := 1/4$. We then establish in Lemma \ref{lemmaHInH} that $H_\delta^*\in \bH_*$ and $H_\delta^*$ separates $X$ and $Y_\delta$, and we prove in Lemma \ref{lemmaMHDelta} an upper estimate on the masses $m(H_\delta^*)$ of these metrics. 

In order to define $H_\delta^*$ we need to introduce some notations. For any $z\in \R^d \sm\{0\}$ we define
\be
\label{defsz}
s(z) := \min\{r_0, \left| |z|-r_0\right|\} \stext{ and } \theta(z) := \frac z {|z|}.
\ee
For any $0 < \delta \leq r_0$ and any $z\in \R^d\sm\{0\}$ we define three matrices $S_\delta^\star(z) \in S_d^+$, where $\star\in \{i,a,g\}$, as follows 
\be
\label{defSDeltaStar}
\begin{array}{rcl}
S_\delta^i(z) &:=& \max\{s(z), \delta\} \, \Id\vspace{0.2ex}\\
S_\delta^a(z) &:=& \max\{s(z), \delta\} \, \theta(z) \theta(z)^\trans + \max\left\{s(z), \sqrt \delta\right\} \, (\Id - \theta(z) \theta(z)^\trans)\vspace{0.2ex}\\
S_\delta^g(z) &:=& \max\{s(z), \delta\} \, \theta(z) \theta(z)^\trans + \sqrt{r_0\max\{s(z), \delta\}} \, (\Id - \theta(z) \theta(z)^\trans).
\end{array}
\ee
%
%\begin{eqnarray*}
%S_\delta^i(z) &:=& \max\{s(z), \delta\} \, \Id\\
%S_\delta^a(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \max\left\{s(z), \sqrt \delta\right\} \, (\Id - \n_z \n_z^\trans)\\
%S_\delta^g(z) &:=& \max\{s(z), \delta\} \, \n_z \n_z^\trans + \sqrt{r_0\max\{s(z), \delta\}} \, (\Id - \n_z \n_z^\trans).
%\end{eqnarray*}
We also define $S_\delta^\star(0) = r_0\Id$ for any $\star\in \{i,a,g\}$. Eventually we define the metrics $H_\delta^*$ by the equality 
\be
\label{eqHS2}
2  H_\delta^\star(z+u)^{-\frac 1 2} := S_\delta^*(z)
\ee
for all $z\in \left[-\frac 1 2, \frac 1 2\right]^d$ and all $u \in \Z^d$.
Observe that 
\be
\label{eqS2R0}
H_\delta^\star = \Id \stext{ for all } |z| \geq 2  r_0 =  1 / 2.
\ee
since $S_\delta^\star(z) = r_0 \Id$ on this set.

\begin{lemma}
For all $0<\delta \leq  r_0$ and all $\star\in \{i,a,g\}$ one has $H_\delta^\star \in \bH_\per \cap \bH_\star$.
%\be
%\label{eqHInH}
%H_\delta^*\in \bH_* \cap \bH_\per.
%\ee
\end{lemma}
\proof
We first remark that $s = r_0$ on the boundary $\partial ([-\frac 1 2, \frac 1 2]^d)$, and therefore $H_\delta^\star = \Id$ on this set for any $\star \in \{i,a,g\}$. Using \iref{eqHS2} we thus obtain that $H_\delta^\star$ is continuous and $\Z^d$ periodic.

We denote  
$$
s_\per(z) := \min\{r_0, |d(z, \Z^d) -r_0|\}
$$
and we observe that $s_\per$ is a Lipschitz function.
Since 
$
H_\delta^i = 4\Id /\max\{s_\per , \delta\}^2,
$
we obtain that $H_\delta^i\in \bH_i$ (because $z\mapsto \min \{s(z), \delta\}/2$ is Lipschitz), which concludes the case $\star = i$.\\

We now consider the case $\star =g$, and for that purpose we use the notations of \S \ref{secEigen} (in the previous chapter). Our first step is to establish that the local dilatation $\dil_z(H)_\times$ defined in \iref{defDilH} is smaller than $1$ for all $z$ on the set 
$$
\Omega := \{z\in \R^d \sep 0 < |z| < r_0 - \delta\}. % \text{ or } (-1/2, 1/2)^d \sm \{0\}
$$
We define the functions
$$
\lambda := s/2 \stext{ and } \mu := \sqrt s /4 
$$
and we observe that 
$
H_\delta^g = \lambda^{-2} \theta \theta^\trans + \mu^{-2} \theta \theta^\trans
$
on $\Omega$.
The functions $\lambda$ and $\mu$ are $C^\infty$ on $\Omega$ and we have
$$
\nabla \lambda = \frac{-\theta} 2 \stext{ and } \nabla \mu = \frac {-\theta}{8 \sqrt s},
$$
Therefore for any $z\in \Omega$ 
$$
\dil_z(\ln \lambda\sep d_H) = \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)} =  \frac{\|\nabla \lambda(z)\|_{H(z)^{-1}}}{ \lambda(z)}
= \frac{\|-\theta(z)/2\|_{H(z)^{-1}}}{ \lambda(z)} = 1/2.
$$
and 
$$
\dil_z(\ln \mu\sep d_H) = \frac{\dil_z(\mu \sep d_H)}{\mu(z)}
=  \frac{\|\nabla \mu(z)\|_{H(z)^{-1}} }{\mu(z)} %\\
%&=& \frac{\|-\theta(z)/(8\sqrt {s(z)})\|_{H(z)^{-1}}}{\mu(z)}
= \frac{\lambda(z)}{8 \sqrt{s(z)} \mu(z)} = 1/4.
$$
On the other hand the derivative of $\theta$ at a point $z\in \R^d\sm \{0\}$ in the direction $u\in \R^d$ is the component of $u$ orthogonal to $\theta$ and divided by $|z|$ : 
$$
\frac{\partial \theta}{\partial u}(z) = \frac{u-\<u, \theta(z)\>\theta(z)}{|z|},
$$
therefore 
$$
\dil_z(\theta \sep d_H) = \frac {\mu(z)} {|z|}.
$$
On the other hand for $z\in \Omega$
$$
\left|\frac{\lambda(z)}{\mu(z)} - \frac {\mu(z)}{\lambda(z)}\right| = \sqrt{\frac {r_0}{s(z)}} -  \sqrt{\frac {s(z)}{r_0}} \leq r_0-s(z) = |z|,
$$
where we used the fact that $\sqrt t- 1/\sqrt t\leq t$ for all $t\geq 1$ (which is easily checked by derivation).
Therefore 
$$
\frac 1 2 \left|\frac{\lambda(z)}{\mu(z)} - \frac {\mu(z)}{\lambda(z)}\right|\dil_z(\theta \sep d_H) \leq \frac {\mu(z)} 2 \leq 1/8.
$$
It follows that the quantity $D_z(a)_\times$ defined in \iref{eqDZA} is smaller than $1/2$, and therefore that $\dil_z(H_\delta^g)_\times \leq 1$ on $\Omega$ according to Theorem \ref{th2Spaces}.
Proceeding likewise we also obtain that $\dil_z(H_\delta^g) \leq 1$ on the annulus $\{z\in \R^d \sep r_0+\delta<|z|<2r_0\}$. Furthermore $H_\delta^g$ is constant on the annulus $\{z\in \R^d \sep r_0-\delta <|z|<r_0+\delta \}$ and on the domain $\{z\in (-1/2,1/2)^d  \sep |z|> 2r_0\}$. Defining 
$$
\Gamma_0 := \{z\in \R^d \sep |z| \in \{0,r_0-\delta, r_0+\delta, 2r_0\}\} \cup \partial ([-1/2,1/2]^d),
$$
and $\Gamma := \{z+u \sep z\in \Gamma_0, \, u\in \Z^d\}$ we have thus established that $\dil_z(H_\delta^g)_\times \leq 1$ on $\R^d\sm \Gamma$. Corollary \ref{corolLipNoGamma} thus implies that $H_\delta^g\in \bH_g$.

The proof that $H_\delta^a\in \bH_a$ is extremely similar to the proof that $H_\delta^g\in \bH_g$: 
the quantities $D_z(a)_\times$ and $D_z(a)_+$ defined in \iref{eqDZA} and \iref{eqDZAP} can be explicitely computed on $\R^d\sm\Gamma$ and are smaller that $1/2$. Theorem \ref{th2Spaces} thus implies that 
the local dilatations $\dil_z(H_\delta^a)_\times$ and $\dil_z(H_\delta^a)_+$ are bounded by $1$ on $\R^d\sm \Gamma$, and it follows from Corollary \ref{corolLipNoGamma} that $H_\delta^a\in \bH_a$. The details of the proof are left to the reader.
\sq

The next lemma establishes the that the metrics $H_\delta^\star$ do separate the sets of interest.

\begin{lemma}
\label{lemmaHInH}
For all $0<\delta\leq r_0$ and all $\star\in \{i,a,g\}$ the metric $H_\delta^\star$ separates the sets $X$ and $Y_\delta$.\end{lemma}

\proof
%We now check the separation of $X$ and $Y_\delta$ by the metrics $H_\delta^*$, where $*\in \{i, a ,g\}$.
Let $\gamma\in C^1([0,1],\R^d)$ be such that $\gamma(0)\in X$ and $\gamma(1)\in Y_\delta$. Since the sets $X$, $Y_\delta$ are $\Z^d$-periodic, as well as the metrics $H_\delta^*$, we may assume that $\gamma(0)\in \left[-\frac 1 2, \frac 1 2\right]^d$.
Recalling the definition \iref{defXYDelta} of $X$ and $Y_\delta$ we obtain
$$
|\gamma(0)|\leq r_0 \stext{ and } |\gamma(1)| \geq r_0+ \delta.
$$
We define 
$$
t_0 := \max \{t\in [0,1] \sep \gamma(t)\in X\} \stext{ and } t_1 := \min \{t\in [t_0, 1] \sep \gamma(t)\in Y_\delta\}.
$$
For any $t\in [t_0, t_1]$ we have 
$$
\gamma(t_0) = r_0  \leq |\gamma(t)| \leq r_0+\delta = \gamma(t_1).
$$
and therefore 
$$
\|\gamma'(t)\|_{H_\delta^\star(\gamma(t))} \geq \frac {2|\<\gamma'(t), \theta(\gamma(t))\>|}\delta = \frac{2 ||\gamma|'(t)|} \delta,
$$
where $|\gamma|$ stands for the function $z\mapsto |\gamma(z)|$.
Hence 
$$
l_{H_\delta^\star}(\gamma) \geq \int_0^1 \|\gamma'(t)\|_{H_\delta^\star(\gamma(t))} dt \geq \int_{t_0}^{t_1} \frac{2|\gamma|'(t)dt} \delta = 2\frac{|\gamma(t_1)|-|\gamma(t_0)|} \delta = 2.
$$
It follows that $d_{H_\delta^\star}(X,Y_\delta) \geq 2$ which concludes the proof.
\sq

The next lemma estimates the mass of the metrics $m(H_\delta^\star)$, which yields an upper estimate on the minimal mass $m_\star(X,Y_\delta)$ required to separate the sets $X$ and $Y_\delta$ using a metric in $\bH_\per \cap \bH_\star$.

\begin{lemma}
\label{lemmaMHDelta}
There exists a constant $C>0$ such that for all $0<\delta \leq r_0$
\begin{eqnarray}
\label{eqHDeltaI}
m(H_\delta^i) &\leq& C\delta^{-(d-1)},\\
\label{eqHDeltaA}
m(H_\delta^a) &\leq& C\delta^{-\frac{d-1} 2 } |\ln \delta|,\\
\label{eqHDeltaG}
m(H_\delta^g) &\leq& C\delta^{-\frac{d-1} 2}.
\end{eqnarray}
\end{lemma}

\proof
Recalling the definition \iref{eqHS2} of $H_\delta^\star$ in terms of $S_\delta^\star$ we obtain 
$$
m(H_\delta^\star) = c_0 + 2^d \int_{|z|\leq 2r_0}  \frac {dz}{\det S_\delta^\star(z)},
$$
where $c_0$ stands for the volume of the following set, on which $H_\delta^\star = \Id$ according to \iref{eqS2R0},
$$
\left\{z\in \left[-\frac 1 2,\frac 1 2\right]^d \sep |z| \geq 2 r_0\right\}.
$$
%and where we used the 
%%We first establish the three inequalities \iref{eqHDeltaI}, \iref{eqHDeltaA} and \iref{eqHDeltaG}, and we then turn to \iref{eqHInH}.
%Recalling the definition \iref{eqHS2} of $H_\delta^\star$ in terms of $S_\delta^\star$ we obtain 
%$$
%m(H_\delta^\star) = \int_{\left[-\frac 1 2,\frac 1 2\right]^d} \sqrt{\det H_\delta^\star(z)} dz = 2^d \int_{\left[-\frac 1 2,\frac 1 2\right]^d} \frac {dz}{\det S_\delta^\star(z)} 
%$$
Furthermore 
$$
\int_{|z|\leq 2r_0} \frac {dz}{\det S_\delta^\star(z)} = c_1 \int_{r=0}^{2r_0} \frac {r^{d-1}dr}{s_\delta^\star(r)},
$$
%where the constants $c_0,c_1>0$ are defined as follows.
%The constant $c_0$ and  stands for the contribution of the integral on the set 
%$$
%\left\{z\in \left[-\frac 1 2,\frac 1 2\right]^d \sep |z| \geq 2 r_0\right\},
%$$
%which is independent of $\delta$ according to \iref{eqS2R0}. The constant 
where $c_1$ stands for the $d-1$-dimensional volume of the sphere $\{z\in \R^d \sep |z|=1\}$, and where
$$
s_\delta^\star(r) := \det S_\delta^\star(z)
$$
for any $z$ such that $|z| = r$.
Therefore there exists a constant $c_2>0$, independent of $\delta$ and of $\star\in \{i,a,g\}$, and such that 
$$
m(H_\delta^\star) \leq c_2 \int_{r=0}^{2r_0} \frac {dr}{s_\delta^\star(r)}.
$$
Recalling the definition \iref{defSDeltaStar} of $S_\delta^i(z)$ we obtain $s_\delta^i(r) = \max\{\delta,|r_0-r|\}^d$ for all $0 \leq r\leq r_0$, hence 
\begin{eqnarray*}
 \int_{r=0}^{2r_0} \frac {dr}{s_\delta^i(r)} &=& \int_0^{r_0 - \delta} \frac {dr}{(r_0-r)^d} + \int_{r_0 - \delta}^{r_0+\delta} \frac {dr}{\delta^d} + \int_{r_0+\delta}^{2r_0} \frac {dr}{(r-r_0)^d} \\
&=& \frac{\delta^{-(d-1)}}{d-1} + 2 \delta^{-(d-1)} + \left(\frac{\delta^{-(d-1)}}{d-1} -\frac {r_0^{-(d-1)}} {d-1}\right)\\
&\leq & 4 \delta^{-(d-1)}
\end{eqnarray*}
which establishes \iref{eqHDeltaI}.
Similarly, we find 
%We have 
$s_\delta^g(r) = r_0^{\frac {d-1} 2} \max\{\delta,|r_0-r|\}^{\frac {d+1} 2}$, hence 
\begin{eqnarray*}
r_0^{\frac {d-1} 2} \int_{r=0}^{2r_0} \frac {dr}{s_\delta^g(r)} &=& \int_0^{r_0 - \delta} \frac {dr}{(r_0-r)^{\frac{d+1} 2}} + \int_{r_0 - \delta}^{r_0+\delta} \frac {dr}{\delta^{\frac{d+1} 2}} + \int_{r_0+\delta}^{2r_0} \frac {dr}{(r-r_0)^{\frac{d+1} 2}} \\
&=& \frac{2\delta^{-\frac{d-1} 2} }{d-1} + 2 \delta^{-\frac{d-1} 2} + \left( \frac{2\delta^{-\frac{d-1} 2} }{d-1} -\frac {2r_0^{-\frac{d-1} 2}} {(d-1)}\right)\\
&\leq & 6 \delta^{-\frac{d-1} 2}
\end{eqnarray*}
which establishes \iref{eqHDeltaG}.
Eventually, we have $s_\delta^a(r) = \max\{\delta,|r-r_0|\} \max\left\{\sqrt\delta, |r-r_0|\right\}$, and therefore 
\be
\label{eqThreeInt}
\int_{r=0}^{2r_0} \frac {dr}{s_\delta^a(r)} = \int_{I_\delta} \frac {dr} {|r_0-r|^d} + \int_{J_\delta} \frac {dr}{|r_0-r| \delta ^{\frac {d-1} 2}} + \int_{r_0-\delta}^{r_0+\delta} \frac {dr}{\delta^{\frac{d+1} 2}},
\ee
where 
$$
I_\delta = \left[0,r_0-\sqrt \delta\right] \cup \left[r_0+ \sqrt \delta, 2 r_0\right] \stext{ and }J_\delta = \left[r_0-\sqrt \delta, r_0-\delta\right] \cup \left[r_0+ \delta, r_0+ \sqrt \delta\right].
$$
Therefore %The contributions of the three integrals in \iref{eqThreeInt} are given in the next three lines %Computing the contributions of the three integrals we obtain 
\begin{eqnarray*}
\int_{r=0}^{2r_0} \frac {dr}{s_\delta^a(r)} &=& \frac 1 {d-1} \left(2\left(\sqrt{\delta}\right)^{-(d-1)}+r_0^{-(d-1)} \right)\\
& & +  2 \delta^{-\frac {d-1} 2} \left(\ln \left(\sqrt \delta\right) - \ln \delta\right) \\
& & + 2 \delta^{-\frac {d-1} 2}\\
&=& \delta^{-\frac {d-1} 2} |\ln \delta| + \frac {2d} {d-1} \delta^{-\frac {d-1} 2} + r_0^{-(d-1)}
\end{eqnarray*}
which establishes \iref{eqHDeltaA}.
\sq

\subsection{Lower bound}

We prove in this subsection the lower bound announced in Theorem \ref{thOptGeom}. 
\begin{lemma}
\label{lemmaMLower}
There exists a constant $c>0$ such that for all $0<\delta\leq r_0$, 
\begin{eqnarray}
\label{eqHILower}
m_i(X,Y_\delta) &\geq& c\delta^{-(d-1)},\\
\label{eqHALower}
m_a(X,Y_\delta) &\geq& c\delta^{-\frac{d-1} 2 } |\ln \delta|,\\
\label{eqHGLower}
m_g(X,Y_\delta) &\geq& c\delta^{-\frac{d-1} 2}.
\end{eqnarray}
\end{lemma}
\proof 
We consider a metric $H\in \bH_\star$, where $\star\in \{i,a,g\}$ which separates the sets $X$ and $Y_\delta$. In particular $H \in \bH_g$.
We denote by $\bbS := \{v\in \R^d\sep |v| = 1\}$ the euclidean unit sphere of $\R^d$, and by $\omega$ the $d-1$-dimensional volume of $\bbS$. We define for all $v\in \bbS$
$$
n(v) := \|v\|_{H(r_0v)} \stext{ and } m(v) := \inf_{|w|=1} \|w\|_{H(r_0v)} =\|H(r_0v)^{-\frac 1 2}\|^{-1} .
$$
Proposition \ref{propEuclidRiemann} (in the previous chapter), states that for any $z,u\in \R^d$ we have 
\be
\label{eqER}
d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention if $\|u\|_{H(z)} \geq 1$. 

%Furthermore, see \iref{eqLocalNorm}, for all $v\in \R^d$
%$$
%\|v\|_{H(z+u)} \geq (1-\|u\|_{H(z)}) \|v\|.
%$$

We now consider a point $v\in \bbS$ and we observe that $r_0 v\in X$ and $(r_0+\delta)v\in Y_\delta$. Therefore 
$$
1 \leq d_H(r_0v, \, (r_0+ \delta) v) \leq -\ln\left(1-\delta \|v\|_{H(r_0 v)}\right)
$$
hence $\lambda \delta n(v) \geq 1$
%\be
%\label{eqHvv}
%\delta \|v\|_{H(r_0 v)} \geq 1-e^{-1} = \lambda^{-1},
%\ee
where
$
\lambda := (1-e^{-1})^{-1}.
$
Let $v,w\in \bbS$, and let $\sigma\in \{-1,1\}$ be such that $\sigma \<v,w\>\geq 0$.  Remarking that $2r_0+ \delta \leq 3/4 \leq 1$ we obtain 
$$
\left|r_0 v+\sigma \sqrt {\delta} w\right|^2 = r_0^2 +\delta + 2  r_0 \sqrt \delta \sigma\<v,w\> \geq r_0^2 +\delta \geq r_0^2 + (2r_0 +\delta) \delta = (r_0+\delta)^2.
$$
Hence $r_0 v \in X$ and $r_0 v+\sigma \sqrt {\delta} w\in Y_\delta$. Therefore 
$$
1 \leq d_H(r_0 v, \, r_0 v+ \sigma \sqrt \delta w) \leq -\ln\left(1-\sqrt \delta \|w\|_{H(r_0 v)}\right),
$$
which implies $\lambda \sqrt \delta m(v) \geq 1$.
We we now distinguish between the three cases $\star = i$, $a$ or $g$.
\begin{itemize}
\item If $\star = i$, then $H(z) = \Id/s(z)^2$ where $s$ is a Lipschitz function. Furthermore $s(r_0 v) = n(v)^{-1} \geq \lambda\delta$.
It follows that 
\begin{eqnarray*}
m(H) &\geq& \int_\bbS \int_0^{2r_0} \frac {r^{d-1} dr dv}{s(rv)^d} \\
&\geq& \int_\bbS\int_{r_0}^{r_0+\delta} \frac{r_0^{d-1} dr dv}{(n(v)^{-1}+\delta)^d}\\
&\geq& \frac{r_0^{d-1}\delta\omega }{(\lambda\delta+ \delta)^d}\\
&=& \frac{r_0^{d-1} \omega}{(\lambda+1)^d} \delta^{-(d-1)}
\end{eqnarray*}
Taking the infimum among all metrics $H \in \bH_i$ which separate the sets $X$ and $Y_\delta$ we obtain as announced
$$
m_i(X,Y_\delta) \geq c \delta^{-(d-1)} \stext{ where } c= \frac{r_0^{d-1} \omega}{(\lambda+1)^d}.
$$
\item If $\star =a$, then the functions $z\mapsto \|H(z)\|^{-\frac 1 2}$ as well as $z\mapsto \|H(z)^{-\frac 1 2}\|$ are Lipschitz. Hence for any $v\in \bbS$ and any $\mu\in \R$ we have 
$$
\|H((r_0+\mu) v)\|^{-\frac 1 2} \leq n(v)^{-1}+ |\mu| \leq \lambda \delta + |\mu|
$$
and 
$$
\|H((r_0+\mu) v)^{-\frac 1 2}\| \leq m(v)^{-1} + |\mu| \leq \lambda \sqrt \delta + |\mu|,
$$
in particular recalling that $\det M \geq \|M\| \|M^{-1}\|^{-(d-1)}$ for any $M\in S_d^+$ we obtain 
$$
(\lambda\delta+|\mu|)(\lambda\sqrt\delta+|\mu|)^{d-1}\sqrt{\det H((r_0+\mu) v)} \geq 1.
$$
It follows that  
\begin{eqnarray*}
m(H) &\geq& \omega \int_{-r_0}^{r_0} \frac {(r_0+\mu)^{d-1}d\mu}{(\lambda\delta+|\mu|)(\lambda\sqrt\delta+|\mu|)^{d-1}}\\
&\geq& \omega \int_0^{\sqrt \delta} \frac {r_0^{d-1}d\mu}{(\lambda \delta +\mu)(\lambda\sqrt{\delta} + \sqrt \delta)^{d-1}}\\ 
&\geq& \frac{\omega r_0^{d-1} }{((\lambda+1)\sqrt \delta)^{d-1}} (\ln \sqrt \delta -\ln (\lambda\delta)).
\end{eqnarray*}
Hence 
$$
m_a(X,Y_\delta) \geq c\delta^{-\frac{d-1} 2} (-\ln\delta-2\ln \lambda) \stext{ where } c=\frac{\omega}{2(\lambda+1)^{d-1}}
$$
which concludes the proof of \iref{eqHALower}.
\item We now consider the case $\star = g$. 
%We first remark that for any $M,M'\in S_d^+$
%$$
%|\ln \det M -\ln \det M'| \leq 2d\,d_\times (M,M').
%$$
We have for any $v\in \bbS$%Recalling that 
$$
\sqrt{\det H(r_0 v)} \geq \frac 1 {n(v)m(v)^{d-1}} \geq \frac  1 {n(v) (\lambda \sqrt \delta)^{d-1}}.
$$
%$$
%n(v) (\lambda \sqrt d)^{d-1} \sqrt{\det H(r_0 v)}\geq n(v)m(v)^{d-1}\sqrt{\det H(r_0 v)} \geq 1
%$$
Using \iref{eqLocalDet} (in the previous chapter) we therefore obtain for any $\mu\in \R$
$$
\sqrt{\det H((r_0+\mu) v)} \geq (1-|\mu| n(v))^d\sqrt{\det H(r_0v)} \geq \frac{(1-|\mu| n(v))^d } {n(v)(\lambda\sqrt \delta)^{d-1} }
$$
hence 
\begin{eqnarray*}
m(H) &\geq &\int_\bbS \int_{-r_0}^{r_0} \frac{(r_0+\mu)^{d-1} (1-|\mu| n(v))^d d\mu dv}{n(v)(\lambda\sqrt \delta)^{d-1}}\\
&\geq &\int_\bbS \int_0^{\frac 1{2n(v)}} \frac{r_0^{d-1} (1/2)^d d\mu dv}{n(v)(\lambda\sqrt \delta)^{d-1}}\\
&=& \frac{\omega r_0^{d-1}}{2^d (\lambda\sqrt \delta)^{d-1}} %= \frac{\omega r_0^{d-1}}{2^d (\lambda)^{d-1}}\delta^{-\frac{d-1} 2},
\end{eqnarray*}
We thus obtain the announced result \iref{eqHGLower}
$$
m_g(X,Y_\delta) \geq c \delta^{-\frac {d-1} 2} \stext{ where } c=\frac{\omega r_0^{d-1}}{2^d \lambda^{d-1}},
$$
which concludes the proof of this lemma. \sq
\end{itemize}

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Meshing/ConstrainedMesh.pdf}
\caption{Weak separation of two sets by a triangulation. \label{figWeakSeparation}}
\end{figure}

\begin{remark}[Constrained triangulations] 
A variation of the problem considered in this section is often considered in the litterature. 
We say that a mesh $\cT\in \bT$ weakly separates two regions $X, Y \subset \R^d$ if 
$$
\interior(V_\cT(X)) \cap \interior(V_\cT(Y)) = \emptyset,
$$
where $\interior(E)$ refers to the collection of interior points of $E$. 

A common approach for weakly separating two closed and disjoint sets $X,Y\subset \R^d$, is to use the following approach which is based on \emph{constrained mesh} generation.
The first step is to build a polygonal hypersurface $\Gamma$ such that for any path $\gamma \in C^0([0,1], \R^d)$ satisfying $\gamma(0) \in X$ and $\gamma(1)\in Y$, there exists $s\in [0,1]$ such that $\gamma(s) \in \Gamma$.
The second step is to build a mesh $\cT$ of the domain $\Omega$ which is \emph{constrained} to contain the polygonal surface $\Gamma$ in its skeleton $\cup_{T\in\cT} \partial T$.

The main advantage of weak separation is that it can be achieved efficiently without requiring anisotropic simplices, see Figure \ref{figWeakSeparation}. Heuristically the same number of simplices is required to separate the sets $X$ and $Y_\delta$ ``weakly'' with an isotropic triangulation, or ``strongly'' with a graded triangulation.
We refer the interested reader to \cite{Shew3} for a survey on constrained mesh generation.
\end{remark}

\section{Approximation in a given norm}

We compare in this section the approximation error, measured in the $L^p$ norm or the $W^{1,p}$ semi norm, of a function $f$ on a mesh $\cT$ by finite elements with the error associated to $f$ and a metric $H$ adapted to $\cT$
as defined e.g. in \iref{defEHGlobal} for the $L^p$ norm.
In this section, as well as in the next one, we fix an integer $m\geq 2$ 
and we consider finite elements of degree $m-1$.

For that purpose we introduce some notation.
The greek letter $\alpha$ always refers %in this section 
to a $d$-plet of non-negative integers
$$
\alpha = (\alpha_1, \cdots, \alpha_d) \in \Z_+^d,
$$
and we denote $|\alpha| = \alpha_1+\cdots+\alpha_d$.
%For each $\alpha$ we define the following quantities
%$$
%|\alpha|:= \sum_{1\leq i\leq d} \alpha_i \stext{ and } \alpha! := \prod_{1\leq i\leq d} \alpha_i!. %, \quad \max(\alpha) := \max_{1\leq i\leq d} \alpha_i.
%$$
We define the monomial
$$
Z^\alpha := \prod_{1\leq i\leq d} Z_i^{\alpha_i},
$$
where the variable is $Z=(Z_1,...,Z_d)$, and 
we denote by $\P_k$ the collection of all polynomials of degree at most $k$.
$$
\P_k := \Vect\{Z^\alpha \sep |\alpha|\leq k\}.
$$

We introduce a fixed function $\vp\in L^\infty(\R_+, \R)$ supported in $[0,1)$ and satisfying the following moments property: for all $\mu\in \P_{m-1}$ one has 
\be
\label{eqPhiMoments}
\int_{\sR^d} \mu(z) \vp(|z|) dz = \mu(0).
\ee
For any $f\in L^1_\loc(\R^d)$ and any $H\in \bH$ we denote by $f_H$ the convolution of $f$ with $\vp(|\cdot|)$ distorted by the metric $H$, referred to as the distorted mollification of $f$ by $H$, which is defined as follows
\begin{eqnarray}
\label{defConvH}
f_H(z) &:=& \int_{\sR^d} f(z+H(z)^{-\frac 1 2} u) \vp(|u|) du\\
\label{convHDet}
&=& \sqrt{\det H(z)}\int_{\sR^d} f(z+u) \vp(\|u\|_{H(z)}) du
\end{eqnarray}
Note that $\mu_H = \mu$ for any polynomial $\mu\in \P_{m-1}$. Indeed we obtain using the moments property \iref{eqPhiMoments} that for all $z\in \R^d$ 
$$
\mu_H(z) = \mu(z+H(z)^{-\frac 1 2} 0) = \mu(z).
$$



The next proposition establishes that the distorted mollification $f\mapsto f_H$ is bounded in some functional spaces. 
\begin{lemma}
%Consider a metric $H\in \bH$.
\begin{enumerate}
\label{lemmaBoundedConv}
\item (Boundedness from $L^1_\loc$ to $C^0$) For any $H\in \bH$ and any $f\in L^1_\loc$ we have $f_H\in C^0(\R^d)$. Furthermore one has for any $z\in \R^d$ 
\be
\label{eqFHBounded}
|f_H(z)|\leq \sqrt{\det H(z)} \, \|\vp\|_{L^\infty} \|f\|_{L^1(B_H(z))},
\ee
where $B_H(z) := \{u\in \R^d \sep \|u\|_{H(z)} <1\}$.
\item (Boundedness from $W^{1,1}_\loc$ to $W^{1,\infty}_\loc$) If $H\in \bH_a$ and $f\in W^{1,1}_\loc$, then $f_H\in W^{1,\infty}_\loc$. Furthermore for any $z\in \R^d$ one has 
$$
\dil_z (f_H)  \leq 2 \sqrt{\det H(z)} \|\vp\|_{L^\infty} \|\nabla f\|_{L^1(B_H(z))}
$$
where $\dil_z(f_H) := \lim_{\ve \to 0} \|\nabla f_H\|_{L^\infty(B(z,\ve))}$ is the local dilatation of $f$ at $z$.
\end{enumerate}
\end{lemma}

\proof
We first establish 1. The continuity of $f_H$ follows from the expression \iref{defConvH} of the distorted mollification, and from general results on parameter dependent integrals. Inequality \iref{eqFHBounded} follows from the fact that $\vp$ is supported on $[0,1)$ and from \iref{convHDet}.

We now turn to the proof of 2. Metrics $H\in \bH_a$ satisfy $\|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\|\leq |z-z'|$ for any $z,z'\in \R^d$, see their definition \iref{eqLipAdd} (in the previous chapter). Hence for any fixed $u\in B(0,1)$ the map 
$$
z\mapsto z+H(z)^{-\frac 1 2} u
$$
is $2$-Lipschitz.
Derivating \iref{defConvH} under the integral sign we therefore obtain 
\begin{eqnarray*}
\dil_z (f_H) &\leq& \int_{\sR^d} 2|\nabla f(z+H(z)^{-\frac 1 2} u)| \, |\vp(|u|)| du\\
&\leq& 2 \|\vp\|_{L^\infty} \int_{\sR^d} |\nabla f(z+H(z)^{-\frac 1 2} u)|  du\\
&=& 2 \sqrt{\det H(z)} \|\vp\|_{L^\infty} \|\nabla f\|_{L^1(B_H(z))}
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

Before turning to the detail of our results, we fix some notations. For any metric $H\in \bH$, any point $z\in \R^d$ and any radius $r>0$ we define
$$
B_H(z,r) := \{z+u \sep \|u\|_{H(z)} < r\},
$$
as well as 
$$
B_H(z) := B_H(z,1) \stext{ and } B(z,r) := B_{\Id}(z,r)
$$
(the latter being the standard open euclidean ball).
Note that 
\be
\label{eqVolBall}
|B_H(z,r)|\sqrt {\det H(z)} = \omega \, r^d \stext{ where } \omega := |B(0,1)|.
\ee

\subsection{The $L^p$ error}
\label{subsecErrMeshMetLP}

This subsection is devoted to the proof of the following proposition, 
which states that the finite element approximation error measured in the $L^p$ norm of a function $f$ on a mesh $\cT$, is controlled by the error $e_H(f)_p$ associated to a metric $H$ when the mesh satisfies the size condition \iref{eqHT4}. 

\begin{prop}
\label{propErrMeshMet}
There exists a constant $C=C(m,d, \vp)$ such that the following holds. Let $H\in \bH_\per \cap \bH_g$ and  
$\cT\in \bT_\per$ be such that 
\be
\label{eqHT4}
4^2H(z) \leq \cH_T,\;\; T\in\cT, \; z\in T.
\ee %\iref{eqHT4} holds.
Then for all $1\leq p \leq \infty$ and all $f\in L^p_\per$ we have 
$$
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p([0,1]^d)} \leq C e_H(f)_p,
$$
where we denoted $H' := 4^2 H$.
\end{prop}


A first intermediate lemma studies the variations, in terms of volume and inclusion, of the balls $B_H(z,r)$ as $z\in \R^d$ and $r>0$ vary and when $H\in \bH_g$ is a graded metric. 
We recall, see \iref{eqLocalNorm} and \iref{eqLocalDet} (in the previous chapter), that for any $H \in \bH_g$, and for any $z,u,v\in \R^d$ satisfying $\|u\|_{H(z)}<1$ one has
\be
\label{eqLocalNormDet}
\begin{array}{ccccc}
\|v\|_{H(z+u)} (1-\|u\|_{H(z)} ) &\leq& \|v\|_{H(z)} &\leq& \|v\|_{H(z+u)} (1-\|u\|_{H(z)})^{-1},\vspace{1mm}\\
\sqrt{\det H(z+u)} (1-\|u\|_{H(z)} )^d &\leq& \sqrt{\det H(z)} &\leq& \sqrt{\det H(z+u)} (1-\|u\|_{H(z)} )^{-d}.
\end{array}
\ee

\begin{lemma}
\label{lemmaEllIncl}
Let $H\in \bH_g$ and let $z\in \R^d$. %let $H' := 4^2 H$
\begin{enumerate}
\item  For any $z'\in B_H(z,1/2)$ one has $B_H(z',1/4)\subset B_H(z)$. % and $|B_{H'}(z')|\geq 8^{-d} |B_H(z)|$.
\item For any $z'\in B_H(z, 1/6)$ one has $B_H(z',1/2)\supset B_H(z,1/4)$. % and ...%$B_{H'}(z')\geq 4^{-2d} B_H(z)$.
\end{enumerate}
\end{lemma}

\proof
We first prove 1., and for that purpose we observe that for any $q\in \R^d$
\begin{eqnarray*}
\|q-z'\|_{H(z')}
&\geq & (1-\|z'-z\|_{H(z)}) \|q-z'\|_{H(z)}\\
& \geq & (1-\|z'-z\|_{H(z)}) (\|q-z\|_{H(z)}-\|z'-z\|_{H(z)})\\
& \geq & (1-1/2) (\|q-z\|_{H(z)}-1/2)
\end{eqnarray*}
If $\|q-z\|_{H(z)}\geq 1$ then the previous equation implies $\|q-z'\|_{H(z')}\geq  1/4$, which establishes the first inclusion.

We now turn to the proof of 2.
We obtain for any $q\in \R^d$ %Recalling that $4 \|z-z'\|_{H(z)} = \|z-z'\|_{H(z')} \leq 2/3$ we obtain for any $q\in \R^d$
\begin{eqnarray*}
\|q-z'\|_{H(z')} &\geq & (1-\|z'-z\|_{H(z)}) \|q-z'\|_{H(z)}\\
& \geq & (1-\|z-z'\|_{H(z)}) (\|q-z\|_{H(z)}-\|z'-z\|_{H(z)})\\
& \geq & (1-1/6) (\|q-z\|_{H(z)}-1/6). %= 10/9 >1. %(2/3)/4
\end{eqnarray*}
If $\|q-z\|_{H(z)} \geq 1/2$ then $\|q-z'\|_{H(z')} \geq 5/18 >1/4$. Hence $B_H(z',1/2)\supset B_H(z, 1/4)$ as announced which concludes the proof of this lemma.\sq

The next lemma estimates the finite element approximation error \emph{locally}. %, close to a point $z$.

\begin{lemma}
There exists $C=C(m,d, \vp)$ such that the following holds. Let $H\in \bH_g$, $\cT\in \bT$, $z\in \R^d$ and let 
\be
\label{defTz}
\cT_z := \{T\in \cT \sep T \subset B_{H}(z,1/2)\}.
\ee
Then 
\be
\label{eqLocalMeshMet}
\|f-\interp_\cT^{m-1} f_{H'}\|_{L^p(\Omega_z)} \leq C \, e_H(f\sep z)_p.
\ee
where $H':=4^2 H$ and $\Omega_z$ denotes the union of all triangles in $\cT_z$.
\end{lemma}

\proof
We denote by $C_{\interp}$ the norm of the interpolation operator 
$$
\interp_\TEq^{m-1} : C^0(\TEq) \to C^0(\TEq),
$$
where $\TEq$ denotes the reference equilateral simplex.
We obtain using a change of variables that for any triangle $T$ and any $g\in C^0(T)$ one has 
$$
\|\interp_T^{m-1} g\|_{L^\infty(T)}\leq C_{\interp} \|g\|_{L^\infty(T)}.
$$


Let $\mu\in \P_{m-1}$ be a polynomial satisfying $\|f-\mu\|_{L^p(B_H(z))} = e_H(f\sep z)_p$.
Let $g := f-\mu$ and let $T\in \cT_z$. 
We have
\begin{eqnarray*}
\|\interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq & |T|^\frac 1 p \|\interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
&\leq & C_{\interp} |T|^\frac 1 p \|g_{H'}\|_{L^\infty(T)}\\
&\leq & C_{\interp} |T|^\frac 1 p \|g_{H'}\|_{L^\infty(B_H(z,1/2))}.
\end{eqnarray*}
Using \iref{eqFHBounded} and the inclusion stated in point 1. of  Lemma \ref{lemmaEllIncl} we obtain furthermore
\begin{eqnarray*}
\|g_{H'}\|_{L^\infty(B_H(z,1/2))} &\leq & \|\vp\|_{L^\infty} \max \{ \|g\|_{L^1(B_{H'}(z'))} \sqrt{\det H'(z')}\sep z'\in B_H(z,1/2)\}\\
&\leq & \|\vp\|_{L^\infty}   \|g\|_{L^1(B_{H}(z))} 4^d (1-1/2)^{-d} \sqrt {\det H(z)},
\end{eqnarray*}
where we used \iref{eqLocalNormDet} in the second line.
Defining $C_* := 8^d C_{\interp}  \|\vp\|_{L^\infty}$ we thus obtain
\begin{eqnarray*}
\|\interp_\cT^{m-1} g_{H'}\|_{L^p(\Omega_z)} &=& \left(\sum_{T\in \cT_z} \|\interp_T^{m-1} g_{H'}\|_{L^p(T)}^p \right)^{\frac 1 p} \\
&\leq & C_* \|g\|_{L^1(B_{H}(z))} \sqrt{\det H(z)} \left(\sum_{T\in \cT_z} |T|\right)^\frac 1 p\\
& \leq & C_* \|g\|_{L^1(B_{H}(z))}\frac{\omega}{|B_H(z)|} |B_{H}(z)|^\frac 1 p\\
& \leq & C_*\omega \|g\|_{L^p(B_{H}(z))},
\end{eqnarray*}
where we used in the third line the expression \iref{eqVolBall} of the volume $|B_H(z)|$, and the inclusion \iref{defTz}.
Since the distorted convolution reproduces polynomials in $\P_{m-1}$ , as well as the interpolation operator $\interp_\cT^{m-1}$, we have
$$
g-\interp_\cT^{m-1} g_H = (f-\mu)-\interp_\cT^{m-1} (f-\mu)_H = f-\interp_\cT^{m-1} f_H.
$$ 
Therefore  
\begin{eqnarray*}
\|f-\interp_\cT^{m-1} f_H\|_{L^p(\Omega_z)} &=& \|g-\interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)} \\
&\leq &\|g\|_{L^p(\Omega_z)}+ \|\interp_\cT^{m-1} g_H\|_{L^p(\Omega_z)}\\
& \leq & (1+C_*\omega) \, \|g\|_{L^p(B_{H}(z))}\\
&=& (1+C_*\omega) \, e_H(f\sep z)_p
\end{eqnarray*}
which concludes the proof.
\sq

We now prove Proposition \ref{propErrMeshMet}.
For each triangle $T\in \cT$ we define 
$$
\Omega_T := \{z\in \R^d \sep T \subset B_H(z,1/2)\} \stext{ and } n(T) := \int_{\Omega_T} \sqrt{\det H(z)} dz,
$$
and we observe that 
$$
z\in \Omega_T \stext{ if and only if } T \in \cT_z,
$$
where $\cT_z$ is defined in \iref{defTz}.
%(could be improved...??)
Note also that $\Omega_T\subset B(z_T, 1/2)$ since $H(z) \geq \Id$ for all $z\in \R^d$, hence the sets $u+ \Omega_T$, $u\in \Z^d$, are pairwise disjoint.
We denote by $\cT_*$ a system of representatives of the set $\cT$ for the relation of equivalence  
$$
T \sim T' \stext{ if } T =T'+u \text{ for some } u \in \Z^d.
$$
It follows from the local error estimate \iref{eqLocalMeshMet} that 
\begin{eqnarray*}
C^p e_H(f)_p^p &=& C^p\int_{[0,1]^d} \sqrt{\det H(z)} \, e_H(f\sep z)_p^p \, dz\\
&\geq&  \int_{[0,1]^d} \sqrt{\det H(z)}\, \|f-\interp_\cT^{m-1} f_H\|_{L^p(\Omega_z)}^p \, dz \\
&=&  \int_{[0,1]^d} \sqrt{\det H(z)}\, \sum_{T\in \cT_z} \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p \, dz \\
&=& \sum_{T\in \cT_*} \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p \int_{[0,1]^d} \sqrt{\det H(z)} \sum_{u\in \Z^d} \chi_{\Omega_T} (z-u) dz\\
&=&\sum_{T\in \cT_*} \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p \int_{\R^d} \sqrt{\det H(z)} \chi_{\Omega_T} (z) dz\\
&=& \sum_{T\in \cT_*}  \|f-\interp_\cT^{m-1} f_H\|_{L^p(T)}^p n_T \\
& \geq &  \|f-\interp_\cT^{m-1} f_H\|_{L^p([0,1]^d)}^p \min_{T \in \cT} n_T.
\end{eqnarray*}
We now establish that $n_T$ is uniformly bounded below, which concludes the proof of Proposition \ref{propErrMeshMet}.
It follows from  \iref{eqHT4} that $T\subset B_H(z_T,1/4)$, where $z_T$ denotes the barycenter of $T$.
The inclusion property established in Point 2. of Lemma \ref{lemmaEllIncl} thus implies that $B_H(z_T,1/6) \subset \Omega_T$. We thus obtain the lower bound %, independent of $\cT$ and $H$, 
\begin{eqnarray*}
n(T) &\geq& |B_H(z_T,1/6)| \min_{z\in B_H(z_T,1/6)}  \sqrt{\det H(z)}\\
&\geq& \frac{\omega 6^{-d}}{\sqrt{\det H(z_T)}}  \sqrt{\det H(z_T)} (1-1/6)^d\\
&=& \omega (5/36)^d,
\end{eqnarray*}
where we used the explicit expression \iref{eqVolBall} of the volume of $|B_H(z,r)|$ and the estimate \iref{eqLocalNormDet} on the variations of $\sqrt{\det H(z)}$.



\subsection{The $W^{1,p}$ error, when the measure of sliverness is uniformly bounded}
We establish in this subsection the following proposition, 
which shows that the finite element approximation error measured in the $W^{1,p}$ on a mesh with bounded measure of sliverness, is controlled by error $e_H^a(\nabla f)_p$.
%The mesh $\cT$ needs to be ``more refined'' than the metric $H$, in the following sense :

\begin{prop}
\label{propErrMeshMetA}
There exists a constant $C=C(m,d, \vp)$ such that the following holds. Let $H\in \bH_\per \cap \bH_a$ and  
$\cT\in \bT_\per$ be such that 
\be
\label{eqHT4A}
4^2H(z) \leq \cH_T,\;\; T\in\cT, \; z\in T.
\ee %\iref{eqHT4} holds.
Then for all $1\leq p \leq \infty$ and all $f\in W^{1,p}_\per$ we have 
$$
\|\nabla (f-\interp_\cT^{m-1} f_{H'})\|_{L^p([0,1]^d)} \leq C e_H^a(f)_p \max_{T\in \cT} S(T),
$$
where we denoted $H' := 4^2 H$.
\end{prop}

The main difficulty of this proof is contained in the following lemma, which states that a near-best approximation of the gradient of a function, on an ellipse, has the form of the gradient of a polynomial.

\begin{lemma}
\label{lemmaProj}
\begin{enumerate}
\item (Orthogonal projection is compatible with gradients)
We equip the space $L^2(\bbB, \R^d)$, where $\bbB := B(0,1)$, with the scalar product 
$$
\<v,w\> := \int_\bbB v(z)\cdot w(z) dz.
$$
For any $f\in H^1(\bbB)$ there exists $\mu\in \P_{m-1}$ such that the orthogonal projection of $\nabla f$ onto $\P_{m-2}^d$ is $\nabla \mu$.
\item (Optimization among gradients)
There exists $C_\proj=C_\proj(m,d)$ such that for any ellipsoid $\cE\subset \R^d$, any $1\leq p \leq \infty$ and any $f\in W^{1,p}(\cE)$ one has 
\be
\label{eqGradApp}
\inf_{\mu \in \sP_{m-1}} \|\nabla f-\nabla \mu\|_{L^p(\cE)}
\leq 
C_\proj \inf_{\nu \in \sP_{m-2}^d} \|\nabla f-\nu\|_{L^p(\cE)}
\ee
\end{enumerate}
\end{lemma}

\proof
We denote $k:=m-1$.
We first establish Point 1. We define $\bbS := \partial \bbB$ and we denote by $D_k$ the collection of polynomial vector fields $\nu\in  \P_{k-1}^d$ satisfying %\subset \P_{k-1}^d
$$
\left\{
\begin{array}{cl}
\diver \nu (z)=0 & \text{ for all } z\in \bbB\\
\nu(z) \cdot z = 0 &\text{ for all } z\in \bbS
\end{array}
\right.
$$
For any $g\in H^1(\bbB)$ and any $\nu \in D_k$ we thus have   
\be
\label{eqGradDiv}
\int_{B(0,1)} \nabla g \cdot \nu = -\int_{B(0,1)} g(z) \diver \nu(z)dz + \int_{\cS} g(z)  \, \nu(z) \cdot z \, dz =0.
\ee
%therefore the same holds for the orthogonal projection of $\nabla f$ onto $\P_{k-1}^d$.
Our first objective is to establish the orthogonal decomposition
$$
\P_{k-1}^d = D_k \oplus \nabla \P_k.
$$
The spaces $\nabla \P_k$ and $D_k$ are orthogonal according to \iref{eqGradDiv}, and we know that $\dim \nabla \P_k = \dim \P_k -1$. Therefore we only have to show that 
$\dim D_k \geq \dim (\P_k^{d-1})  - \dim \P_k +1$.

The vector space $D_k$ is the kernel of the map $d_k$ defined as follows
$$
\begin{array}{ccc}
d_k :\P_{k-1}^d &\to& \P_{k-2} \oplus \P_k(\bbS)\\
\nu  &\mapsto & (\diver \nu, \ (\nu (z) \cdot z)_{|\bbS}),
\end{array}
$$
where  
$
\P_k(\bbS)
$
denotes the collection of restrictions to $\bbS$ of elements of $\P_k$. 
The kernel of the map
$$
\begin{array}{ccc}
\gamma_k : \P_k &\to & \P_k(\bbS)\\
\mu &\mapsto &\mu_{|\bbS}
\end{array}
$$
is 
$
\Ker(\gamma_k) = (1-|z|^2) \P_{k-2}.
$
Hence 
$
\dim(\P_k(\bbS)) = \dim \P_k - \dim \P_{k-2}.
$

The map $d_k$ is not surjective, since we have the linear relation 
$$
\int_{\bbB} \diver \nu(z)\, dz = \int_\bbS \nu(z)\cdot z \, dz.
$$
Therefore 
\begin{eqnarray*}
\dim D_k &=& \dim \Ker d_k \\
&=& \dim (\P_k^{d-1}) - \dim \Image d_k \\
&\geq &  \dim (\P_k^{d-1}) - (\dim \P_{k-2} + \dim \P_k(\bbS) -1) \\
&=& \dim (\P_k^{d-1})  - \dim \P_k +1,
\end{eqnarray*}
which implies the orthogonal decomposition $\P_{k-1}^d = D_k \oplus \nabla \P_k$ as announced.

Finally for any $f\in H^1(\bbB)$ the vector field $\nabla f$ is orthogonal to $D_k$ according to \iref{eqGradDiv}. The orthogonal projection of $\nabla f$ onto $\P_{k-1}^d$ is therefore also orthogonal to $D_k$, hence is an element of $\nabla \P_k$ which concludes the proof Point 1.\\

We now turn to the proof of Point 2.
We denote by $Q : L^2(\bbB,\R^d) \to \P_{k-1}^d$ the $L^2(\bbB)$ orthogonal projection.
We recall that for any $v\in L^2(\bbB,\R^d)$ the projection $Q(v)\in \P_{k-1}^d$ is defined by the collection of linear conditions
$$
\int_{\bbB} (v-Q(v))\cdot \nu  = 0 \text{ for all } \nu \in \P_{k-1}^d.
$$
Hence $Q(v)$ depends linearly on a finite number of moments of $v$, and therefore continuously extends to all $v\in L^1(\bbB, \R^d)$. %We denote by $C_0$ a constant such that 
Therefore there exists a constant $C_0$ such that for all $1\leq p \leq \infty$ and all $v\in L^p(\bbB,\R^d)$
$$
\|Q(v)\|_{L^p(\bbB)} \leq C_0 \|v\|_{L^p(\bbB)}.
$$
For any $A\in \GL_d$ and any $v\in L^2(\bbB,\R^d)$ we claim that $Q(A(v)) = A(Q(v))$. Indeed for any $\nu\in \P_{k-1}^d$ one has 
$$
\int_{\bbB} (A(v(z))-A(Q(v(z))))\cdot \nu(z) dz= \int_{\bbB} (v(z)-Q(v(z))\cdot (A^\trans(\nu(z))) dz = 0.
$$
Consider  $1\leq p \leq \infty$, $f\in W^{1,p}(\bbB)$ and $A\in \GL_d$. Let $\mu\in \P_{m-1}$ be such that $Q(\nabla f) = \nabla \mu$, and let $\nu \in \P_{m-1}^d$, we obtain 
\begin{eqnarray*}
\|A(\nabla f-\nabla \mu)\|_{L^p(\bbB)} &=& \|A(\nabla f)-A(Q(\nabla f))\|_{L^p(\bbB)}\\
&=& \|A(\nabla f)-Q(A(\nabla f))\|_{L^p(\bbB)}\\
& = & \|A(\nabla f-\nu)-Q(A(\nabla f)-\nu)\|_{L^p(\bbB)}\\
&\leq& (1+C_0)  \|A(\nabla f-\nu)\|_{L^p(\bbB)}.
\end{eqnarray*}
Therefore 
$$
\inf_{\mu\in \sP_{m-1}} \|A(\nabla f-\nabla \mu)\|_{L^p(\bbB)} \leq (1+C_0) \inf_{\nu\in \sP_{m-2}^d} \|A(\nabla f-\nu)\|_{L^p(\bbB)}
$$
Using a linear change of variables $\cE \to \bbB$ we obtain the announced result \iref{eqGradApp}, with the constant $C_\proj := C_0+1$. This concludes the proof of this lemma.
\sq

The rest of the proof of Proposition \ref{propErrMeshMetA} is extremely similar to the proof of Proposition \ref{propErrMeshMet}.
The estimates 
\begin{eqnarray*}
|f_H(z)| &\leq& \sqrt{\det H(z)} \, \|\vp\|_{L^\infty} \|f\|_{L^1(B_H(z))}\\
\| \interp_T^{m-1} g\|_{L^\infty(T)} &\leq& C_I \|\nabla g\|_{L^\infty(T)},
\end{eqnarray*}
used in the proof of Proposition \ref{propErrMeshMet} have the counterparts
\begin{eqnarray*}
\dil_z (f_H)  &\leq& 2 \sqrt{\det H(z)} \|\vp\|_{L^\infty} \|\nabla f\|_{L^1(B_H(z))}\\
\| \nabla \interp_T^{m-1} g\|_{L^\infty(T)} &\leq& C_I' \|\nabla g\|_{L^\infty(T)} S(T),
\end{eqnarray*}
which are proved respectively in Lemma \ref{lemmaBoundedConv} and Lemma \ref{lemmaSD} (in Chapter \ref{chapW1P}).
From this point the adaptation of the proof is straightforward and is therefore left to the reader.

\subsection{The $W^{1,p}$ error, on a general mesh} 
\label{subsubsecErrMeshMetW1PG}

This subsection is devoted to the proof of Proposition \ref{propErrMeshMetG}, which estimates the $W^{1,p}$ approximation error of a function $f$ on a mesh with arbitrary measure of sliverness, in terms of the approximation error $e_H^g(\nabla f)_p$ with respect to a metric. This approach does not allow to recover the optimal anisotropic error estimates for $W^{1,p}$ norms developed in Chapter \ref{chapW1P}. However it is perhaps more taylored to current anisotropic mesh generation software, which generally do not guarantee any bound on the measure of sliverness (or the maximal angle in dimension $2$). 

\begin{prop}
\label{propErrMeshMetG}
For all $C_0 \geq 1$ there exists a constant $C=C(C_0, m,d, \vp)$ such that the following holds. Let $H\in \bH_\per \cap \bH_g$ and  let
$\cT\in \bT_\per$ be such that 
\be
\label{eqHT4G}
4^2H(z) \leq \cH_T\leq (4C_0)^2 H(z),\;\; T\in\cT, \; z\in T.
\ee %\iref{eqHT4} holds.
Then for all $1\leq p \leq \infty$ and all $f\in W^{1,p}_\per$ we have 
$$
\|\nabla (f-\interp_\cT^{m-1} f_{H'})\|_{L^p([0,1]^d)} \leq C e_H^g(f)_p,
$$
where we denoted $H' := 4^2 H$.
\end{prop}

Our first step in the proof of this proposition is the next lemma which estimates the \emph{local} approximation error.

\begin{lemma}
For all $C_0\geq 1$ there exists $C=C(C_0,m,d)$ such that the following holds. 
Let $H\in \bH_\per$ and $\cT \in \bT_\per$ be such that \iref{eqHT4G} holds. Let $T\in \cT$ and $z\in T$. Then for all $1\leq p \leq \infty$ and all $f\in W^{1,p}_\per$ we have 
\be
\label{eqLocGW1P}
\|\nabla (f- \interp_\cT^{m-1} f_{H'})\|_{L^p(T)} \leq C e_H^g(\nabla f\sep z)_p,
\ee
where we denoted $H' := 4^2 H$.
\end{lemma}

\proof %The proof is extremely similar to the proof of Lemma ??, for the approximation in the $L^p$ norm.
We assume in a first time that $z=0$ and that $H(z) = \Id$, in such way that $B_H(z) = \bbB := B(0,1)$ is the euclidean unit ball.
We consider a polynomial $\mu\in \P_{m-1}$ such that 
$
\|\nabla (f-\mu)\|_{L^p(B)}
$
is minimal, and such that $\int_B (f-\mu) = 0$. The latter point can be ensured by adding an appropriate constant to $\mu$. Defining $g:=f-\mu$, we obtain using Lemma \ref{lemmaProj}
$$
\|\nabla g\|_{L^p(\bbB)} \leq C_\proj \,e_H^a(f\sep z)_p.
$$
%Sobolev Injection's Theorem states that the embedding 
Since  $g\in W^{1,1}(B)$ and $\int_B g=0$ there exists according to Sobolev's injection theorem a constant $C_\sob=C_\sob(m,d)$ such that 
$$
\|g\|_{L^1(\bbB)} \leq C_\sob \|\nabla g\|_{L^1(\bbB)}
$$
The function $g_{H'}$ is continuous on $T$ and satisfies according to Lemma \ref{lemmaBoundedConv}
\begin{eqnarray*}
\|g_{H'}\|_{L^\infty(T)} &\leq& \|\vp\|_{\infty} \max \{ \|g\|_{L^1(B_{H'}(z'))} \sqrt{\det H'(z)} \sep z'\in T\}\\
 &\leq& \|\vp\|_\infty \|g\|_{L^1(\bbB)} 4^d (1-1/2)^d\\ 
 &=& C_1\|g\|_{L^1(\bbB)},
\end{eqnarray*}
where we used \iref{eqLocalNormDet} and the fact that $\|z-z'\|_{H(z)} \leq 2$ for all $z'\in T$.

We denote by $C_{\interp}$ the norm of the operator $\nabla \interp_\TEq^{m-1} : C^0(\TEq)\to \P_{m-2}^d$, where $\TEq$ denotes the reference equilateral simplex : for any $h\in C^0(\TEq)$
$$
\|\nabla \interp_\TEq^{m-1} h\|_{L^\infty(\TEq)} \leq C_{\interp} \|h\|_{L^\infty(\TEq)}. 
$$
We recall that $\cH_T^{\frac 1 2}(T)$ is the image $\TEq$ by a translation and a rotation, see Proposition \ref{propHT} in the previous chapter. Using this change of variables, and choosing the function $h=g_{H'}\in C^0(T)$, we obtain
$$
\|\cH_T^{-\frac 1 2}(\nabla \interp_T^{m-1} g_{H'})\|_{L^\infty(T)} \leq C_{\interp} \|g_{H'}\|_{L^\infty(T)}.
$$
which implies 
$$
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)} \leq C_{\interp}\|\cH_T^\frac 1 2\|  \|g_{H'}\|_{L^\infty(T)}.
$$
We thus obtain, since $\|\cH_T^\frac 1 2\|\leq C_0 \|H'(z)^\frac 1 2\| = 4 C_0$ and since $|T|\leq |\bbB|$,
\begin{eqnarray*}
\|\nabla \interp_T^{m-1} g_{H'}\|_{L^p(T)} &\leq& |\bbB|^\frac 1 p \|\nabla \interp_T^{m-1} g_{H'}\|_{L^\infty(T)}\\
& \leq & 4C_0 C_{\interp} |\bbB|^\frac 1 p   \|g_{H'}\|_{L^\infty(T)}\\
& \leq & 4C_0 C_1 C_{\interp} |\bbB|^\frac 1 p   \|g\|_{L^1(\bbB)}\\
& \leq & 4C_0 C_1 C_{\interp} C_\sob |\bbB|^\frac 1 p   \|\nabla g\|_{L^1(\bbB)}\\
&\leq &  4C_0 C_1 C_{\interp} C_\sob |\bbB|  \|\nabla g\|_{L^p(\bbB)}\\
\end{eqnarray*}
Defining $C_* := 4C_0 C_1 C_{\interp} C_\sob |\bbB|$ we obtain 
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f_{H'})\|_{L^p(T)} &=& \|\nabla (g-\interp_T^{m-1} g_{H'})\|_{L^p(T)}\\
&\leq& (1+C_*) \|\nabla g\|_{L^p(B)}\\
&\leq& C\, e_H^a(\nabla f\sep z)_p,
\end{eqnarray*}
where $C=(1+C_*) C_\proj$.

We now turn to the general case, and we do not any more assume that $z=0$ and $H(z) =\Id$.
We define the affine change of coordinates $\Phi(z') := H(z)^{-\frac 1 2} z'+z$, and we apply our previous reasonning to the metric $H_\Phi$ defined by \iref{defHPhi} (in the previous chapter), 
$$
H_\Phi(z') := H(z)^{-\frac 1 2} H(\Phi(z')) H(z)^{-\frac 1 2},
$$
which satisfies $H_\Phi(0) = \Id$ and $H_\Phi\in \bH_g$ according to Proposition \ref{propHG} (in the previous chapter).
We also define the triangle $T_\Phi := \Phi^{-1}(T)$ and the function $f^\Phi := f\circ \Phi$ and the metric $H'_\Phi = 4^2 H_\Phi$.
The first part of this proof implies that 
$$
\|\nabla (f^\Phi-\interp_{T_\Phi}^{m-1} f^\Phi_{H_\Phi'})\|_{L^p(T_\Phi)} \leq C e_{H_\Phi}^a(\nabla f^\Phi \sep 0)_p.
$$ 
We thus obtain
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f_{H'})\|_{L^p(T)} &\leq & \|H(z)\|^{\frac 1 2} \|H(z)^{-\frac 1 2}(\nabla (f-\interp_T^{m-1} f_{H'}))\|_{L^p(T)}\\
&= &  \|H(z)\|^{\frac 1 2} (\det H(z))^{-\frac 1 {2p}}  \|\nabla (f^\Phi-\interp_{T_\Phi}^{m-1} f^\Phi_{H_\Phi'})\|_{L^p(T_\Phi)}\\
& \leq & C\|H(z)\|^{\frac 1 2} (\det H(z))^{-\frac 1 {2p}} e_{H_\Phi}^a(\nabla f^\Phi \sep 0)_p\\
& = & C\|H(z)\|^{\frac 1 2} e_H(H(z)^{-\frac 1 2}(\nabla f) \sep z)_p\\
&=&e_H^g(f\sep z)_p,
\end{eqnarray*}
where we used the change of variables $\Phi : T \to T_\Phi$ in the second and fourth lines. This concludes the proof of this lemma.\sq

We now conclude the proof of Proposition \ref{propErrMeshMetG}.
For any $T\in \cT$ and any $z\in T$,  recalling that $\cH_T\leq (4C_0)^2 H(z)$ we obtain 
$$
|\TEq|/|T| =  \sqrt{\det \cH_T} \leq (4C_0)^d  \sqrt{\det H(z)}.
$$
Averaging  \iref{eqLocGW1P} over $T$, it follows that 
$$
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)}^p \leq \frac C {|T|} \int_T e_H^g(f\sep z)_p^p dz \leq C'  \int_T \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz
$$
where $C' := (4C_0)^d C/|\TEq|$. 

We denote by $\cT_*$ a system of representatives of the set $\cT$ for the relation of equivalence  
$$
T \sim T' \stext{ if } T =T'+u \text{ for some } u \in \Z^d.
$$
We thus obtain
\begin{eqnarray*}
\|\nabla (f-\interp_T^{m-1} f)\|_{L^p([0,1]^d)}^p &=& \sum_{T\in \cT_*} \|\nabla (f-\interp_T^{m-1} f)\|_{L^p(T)}^p \\
&\leq& C'  \sum_{T\in \cT_*} \int_T \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz\\
&=& C'  \int_{[0,1]^d} \sqrt{\det H(z)}\,  e_H^g(f\sep z)_p^p dz
\end{eqnarray*}
which concludes the proof of this proposition.


\section{Asymptotic approximation and explicit metrics}

This section is devoted to the explicit construction of a metric $H$ adapted to a given function $f$, in the setting where the function $f$ is sufficiently smooth and the mass of metric is asymptotically large. 
%We give both a theoretical construction of the metric $H$ which is valid in arbitrary dimension and degree $m-1$ of approximation, and an explicit construction which can be directly applied to finite element software .

Our main result is the following theorem, which is the counterpart for metrics of the results developed in Chapters 2 and 3. It involves the shape functions $K$, $L_a$ and $L_g$ which are defined in the introduction, \S \ref{subsecIntroAsympt}.
\begin{theorem}
\label{thSmooth}
There exists a constant $C=C(m,d)$ such that for each $f\in C^m_\per$
$$
\limsup_{M\to \infty} \left(M^{\frac m d} \inf_{\substack{H \in \bH_g\\  m(H)\leq M}} M^{\frac m d} e_H(f)_p\right) \leq C \|K(d^m f)\|_\tau, \\
$$
where $\frac 1 \tau := \frac m d+ \frac 1 p$.
Furthermore 
\begin{eqnarray*}
\limsup_{M\to \infty}\left(M^\frac {m-1} d \inf_{\substack{H \in \bH_a\\  m(H)\leq M}}  e_H^a(\nabla f)_p\right) &\leq& C \|L_a(d^m f)\|_\tau\\
\limsup_{M\to \infty}\left(M^\frac {m-1} d \inf_{\substack{H \in \bH_g\\  m(H)\leq M}}  e_H^g(\nabla f)_p\right) &\leq& C \|L_g(d^m f)\|_\tau\\
\end{eqnarray*}
where $\frac 1 \tau := \frac {m-1} d+ \frac 1 p$.

%\item
%If $z\mapsto K(d^m f(z))$ is not identically $0$, then there exists a $C^\infty$ metric $H \in \bH_\per\cap \bH_g$ such that for all $\lambda \geq 1$
%\be
%\label{eqHSmooth}
%m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|K(d^m f)\right\|_{L^\tau([0,1]^d)},
%\ee
%where $\frac 1 \tau := \frac m d+ \frac 1 p$.
%\item
%If $z\mapsto L_a(d^m f(z))$ is not identically $0$, then there exists a $C^\infty$ metric $H \in \bH_\per\cap \bH_a$ such that for all $\lambda \geq 1$
%\be
%\label{eqHSmooth}
%m(\lambda H)^{\frac m d} e_{\lambda H}^a(\nabla f)_p \leq C \left\|L_a(d^m f)\right\|_{L^\tau([0,1]^d)},
%\ee
%where $\frac 1 \tau := \frac {m-1} d+ \frac 1 p$.
%\item
%If $z\mapsto L_g(d^m f(z))$ is not identically $0$, then there exists a $C^\infty$ metric $H \in \bH_\per\cap \bH_g$ such that for all $\lambda \geq 1$
%\be
%\label{eqHSmooth}
%m(\lambda H)^{\frac m d} e_{\lambda H}^g(\nabla f)_p \leq C \left\|L_g(d^m f)\right\|_{L^\tau([0,1]^d)},
%\ee
%where $\frac 1 \tau := \frac {m-1} d+ \frac 1 p$.
%\end{enumerate}
\end{theorem}

In order to prove this theorem we need to introduce some notation.
For each $d$-plet
$
\alpha = (\alpha_1, \cdots, \alpha_d) \in \Z_+^d
$
of non-negative integers we define the following quantities
$$
|\alpha|:= \sum_{1\leq i\leq d} \alpha_i \stext{ and } \alpha! := \prod_{1\leq i\leq d} \alpha_i!. %, \quad \max(\alpha) := \max_{1\leq i\leq d} \alpha_i.
$$
We denote by $\H_m$ the space of all homogeneous polynomials of degree $m$
$$
\H_m := \Vect \{Z^\alpha \sep |\alpha| = m\},
$$
equipped with the norm
$
\|\pi\| := \sup \{ |\pi(z)| \sep |z|\leq 1\}.
$

Our first lemma shows that the optimization problems on $\SL_d$ defining the shape functions $K$, $L_a$ and $L_g$ can be reformulated as optimization problems on the collection $S_d^+$ of symmetric positive definite matrices.

\begin{lemma}
\label{lemmaAM}
Let $\psi \in C^0( \GL_d, \R_+^*)$ be homogeneous of degree $r>0$ and satisfy $\psi(A) = \psi(AO)$ for any $A\in \GL_d$ and any $O\in \cO_d$. Then 
$$
\inf \{(\det M)^\frac r {2d} \sep M\in S_d^+ \text{ and } \psi(M^{-\frac 1 2}) \leq 1\} = \inf \{\psi(A) \sep A\in \SL_d\}.
$$
\end{lemma}

\proof
To each $M\in S_d^+$ we associate $A := (\det M)^\frac 1 {2d} M^{-\frac 1 2}\in \GL_d$, in such way that $\det(A) = 1$ and $\psi(A) = (\det M)^{\frac r {2d}} \psi(M^{-\frac 1 2})$. Conversely to  each $A\in \GL_d$ we associate $M := \psi(A)^\frac 2 r (A A^\trans)^{-1}\in S_d^+$, in such way that $(\det M)^\frac r{2d} = \psi(A)$ and $\psi(M^{-\frac 1 2}) = \psi(\psi(A)^{-\frac 1 r} (A A^\trans)^\frac 1 2) = \psi(A)^{-1}\psi(AO) = 1$ where $O := A^{-1} (A A^\trans)^\frac 1 2$ is orthogonal. 
\sq

It follows from this lemma that for any $\pi \in \H_m$
\begin{eqnarray}
\label{defKM}
K(\pi) &=& \inf\{(\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2}\|\leq 1\}\\
\label{defLAM}
L_a(\pi) &=& \inf \{ (\det M)^{\frac {m-1} {2d}} \sep \|(\nabla \pi)\circ M^{-\frac 1 2}\| \leq 1\}\vspace{2mm}\\
\label{defLGM}
L_g(\pi) &=& \inf \{ (\det M)^{\frac {m-1} {2d}} \sep \sqrt{\|M\|} \|\nabla (\pi\circ M^{-\frac 1 2})\| \leq 1\}.
\end{eqnarray}

\begin{remark}
The optimizations among symmetric matrices appearing in these expressions have a geometrical interpretation: finding the ellipsoid of maximal volume included in a set of algebraic boundary.
Indeed one easily checks that the three following properties are equivalent for all $\pi \in \H_m$ and all $M\in S_d^+$
\begin{enumerate}[i)]
\item $\|\pi\circ M^{-\frac 1 2}\|\leq 1$ (resp. $\|(\nabla \pi)\circ M^{-\frac 1 2}\|\leq 1$, resp. $\sqrt{\|M\|} \|\nabla (\pi\circ M^{-\frac 1 2})\| \leq 1$)
\item $|\pi(z)|\leq |z|_M^m$ for all $z\in \R^d$ (resp. $|\nabla \pi(z)|\leq |z|_M^{m-1}$, resp. $\|M\|^\frac 1 2 |M^{-\frac 1 2}(\nabla \pi(z))| \leq |z|_M^{m-1}$)
\item The ellipsoid defined by the inequality $|z|_M\leq 1$, $z\n \R^d$ is included in the set of algebraic boundary defined by the inequality $|\pi(z)|\leq 1$ (resp. $|\nabla \pi(z)|\leq 1$, resp. $\|M\|^\frac 1 2 |M^{-\frac 1 2}(\nabla \pi(z))|\leq 1$)
\end{enumerate}
\end{remark}

We consider a fixed function $f\in \C^m$ and for each $z\in \R^d$ we define the homogeneous polynomial $\pi_z\in \H_m$ as follows
\be
\label{defPiZ}
\pi_z(Z) := \sum_{|\alpha| = m} \frac{\partial^\alpha f(z)}{(\partial z)^\alpha} \frac{Z^\alpha}{\alpha!} .
\ee



The heuristic guideline of the proof of Theorem \ref{thSmooth} is the following, here in the case 1. of approximation in the $L^p$ norm. 
Consider a $C^\infty$ periodic map $M : \R^d \to S_d^+$ such that $\|\pi_z \circ M(z)^{-\frac 1 2}\|\leq 1$ for all $z\in \R^d$, and define 
$$
H(z) := (\det M(z))^{\frac {-1}{mp+d}} M(z).
$$
Then is is not difficult to show that for all $\lambda$ \emph{sufficiently large} one has $\lambda H \in \bH_a$ and 
$$
m(\lambda H)^{\frac m d} e_{\lambda H}(f)_p \leq C \left\|(\det M)^\frac m {2d}\right\|_{L^\tau([0,1]^d)}.
$$
This leads to the announced estimate \iref{eqHSmooth} if $\left\|(\det M)^\frac m {2d}\right\|_{L^\tau([0,1]^d)}$ is comparable to $\left\|K(d^m f)\right\|_{L^\tau([0,1]^d)}$, in other words if $(\det M(z))^\frac m {2d}$ is comparable to $K(\pi_z)$ for all $z\in \R^d$. Let us mention that the same ideas apply to points $2.$ and $3.$ of Theorem \ref{thSmooth}.

The main ingredient of the proof of Theorem \ref{thSmooth} is the construction of a continuous map $\pi \mapsto \cM(\pi)$ such that  $\|\pi\circ \cM(\pi)^{-\frac 1 2}\|\leq 1$ and such that $(\det \cM(\pi))^\frac m r$ is sufficiently close to $K(\pi)$. Up to a few technicalities, which are adressed in \S\ref{subsecExplicitMtricLP}, defining $M(z) := \cM(\pi_z)$ then concludes the proof. We give in \S \ref{subsecExplicit} an explicit expression of such a map, in terms of the coefficients of $\pi$, in the case of piecewise linear and piecewise quadratic approximation in two dimensions. Such explicit expressions are valuable for numerical implementation in finite element software which use anisotropic meshes, and have been implemented by the author in \cite{FreeFem}.

The rest of the chapter is then devoted to the construction in arbitrary dimension $d$ and degree $m$ of such a map $\pi \mapsto \cM(\pi)$. 
The main difficulty of this constructionis that the optimization problem \iref{defKM} is not well posed. For some choices of $\pi$ there exists no minimizer, for others there exists an infinity of minimizers. 
These undesirable properties come from the fact that \iref{defKM} is not a convex minimization problem. The key ingredient of our approach is to define a close variant of this optimization problem which is ``geometrically convex'', a  notion close to convexity which is sufficient for our purpose.

%


\subsection{Explicit Metrics}
\label{subsecExplicit}

We give in this section some explicit minimizers, or near minimizers (in a sense defined below) of the optimization problems among symmetric matrices appearing in the expressions \iref{defKM}, \iref{defLAM} and \iref{defLGM} of the shape functions $K$, $L_a$ and $L_g$. Our results are so far limited to the case $m=2$, which corresponds to piecewise linear approximation, and to $m=3$ in dimension $d=2$

These minimizers or near-minimizers have already been presented in Chapter 2 for the shape function $K$, and Chapter $3$ for the shape function $L_a$. The latter are recalled in the next proposition, and completed with their counterparts for the shape function $L_g$.

For any homogeneous quadratic polynomial $\pi$ we denote by $[\pi]\in S_d$ the associated symmetric matrix, which satisfies $z^\trans [\pi] z = \pi(z)$ for all $z\in \R^d$. Note that $\|\pi\| = \|[\pi]\|$.


\begin{prop}
\label{propLm}
\begin{enumerate}[i)]
\item (Piecewise linear approximation, in any dimension)
If $m=2$ and $d\geq 2$, then for any $\pi\in \H_2$, one has 
$$
L_a(\pi) = 2|\det \pi|^\frac 1 d \stext{ and } L_g(\pi) =2 \sqrt{\|\pi\|} \sqrt[2d]{|\det \pi|}.
$$
The minimizing matrices $M$ in the expressions \iref{defLAM} and \iref{defLGM} of $L_a(\pi)$ and $L_g(\pi)$ are  respectively
$$
\cM_a(\pi) = 4[\pi]^2 \stext{ and } \cM_g(\pi) = \|\pi\| \, |[\pi]|
$$
\item (Piecewise quadratic approximation, in two dimensions)
If $m=3$ and $d=2$, let $\pi =  a x^3+ 3 b x^2 y+ 3 c x y^2+ d y^3\in \H_3$,
let 
$$
\cM_a(\pi) =  %\sqrt{ [\partial_x \pi]^2+ [\partial_y \pi]^2} = 
\sqrt{
\left(\begin{array}{cc}
a & b\\
b & c
\end{array}\right)^2
+
\left(\begin{array}{cc}
b & c\\
c & d
\end{array}\right)^2
}
$$
and let 
$$
\cM_g(\pi) := \cM_a(\pi) + \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}\Id
$$
where $\disc \pi$ is the discriminant of the cubic polynomial $\pi$ :  
\be
\label{eqDiscDet}
 \disc \pi= 4(ac-b^2)(bd-c^2) - (ad-bc)^2.
\ee

Then $\cM_a(\pi)$ and $\cM_g(\pi)$ are near minimizers of optimization problems defining $L_a(\pi)$ and $L_g(\pi)$ respectively, in the following sense: there exists a constant $C$ such that for all $\pi \in \H_3$
$$
\sqrt{\det \cM_a(\pi)}\leq C L_a (\pi) \stext{ and }  \sqrt{\det \cM_a(\pi)} \leq  L_a (\pi).
$$
Furthermore if $\pi$ is not univariate then $\cM_a(\pi)$ and $\cM_g(\pi)$ are non degenerate and we have
\be
\label{eqConstraint}
\|\nabla \pi\circ \cM_a^{-\frac 1 2}\|\leq C \stext{ and } \|\cM_g\|^\frac 1 2 \|\nabla \pi\circ \cM_g^{-\frac 1 2}\|\leq C.
\ee
\end{enumerate}
\end{prop}

\proof
We begin with the case i) of a quadratic polynomial $\pi\in \H_2$, and we observe that $\nabla \pi(z) = 2[\pi] z$. Hence $|\nabla \pi(z)|^2 = 4 z^\trans [\pi]^2 z$ and the announced result for $L_a$ easily follows.
For $L_g$, we are looking for a matrix $M\in S_d^+$ such that 
\be
\label{eqMPi}
2\|M^{\frac 1 2}\| \, \|M^{-\frac 1 2} [\pi] M^{-\frac 1 2}\|\leq 1,
\ee
and of minimal determinant.
Recalling that $\|AB\|\geq \|A\| \|B^{-1}\|^{-1}$ we obtain from \iref{eqMPi} that $2\|\pi \| \leq \|M^\frac 1 2\|$.
Hence 
\be
\label{eqMPiWeak}
4\|\pi\| \| M^{-\frac 1 2} [\pi] M^{-\frac 1 2}\|\leq 1.
\ee
The matrix of minimal determinant which achieves this equality is clearly $M = 4\|\pi\| \ |[\pi]|$. Observing that this matrix also satisfies the condition \iref{eqMPi} we conclude the proof of point i).\\
%Furthermore, it also achieves the initial equality which concludes the proof.

We now turn to the case ii) of cubic polynomials $\pi \in \H_3$.
The case of $L_a$ and $\cM_a$ is exposed in Chapter \ref{chapW1P}. We therefore turn to the case of $L_g$. 
%Since the functions $\pi \mapsto \|\pi\|$, $\pi \mapsto \|\nabla \pi\|$ and $\pi \mapsto \|\cH_a(\pi)$ are continuous, homogeneous of degree $1$ and do not vanish on $\H_3$
Combining the homogeneity and the continuity of the functions involved, one easily shows that there exists a constant $C_0$ such that for all $\pi\in \H_3$
\be
\label{eqContHomog}
\begin{array}{ccccc}
C_0^{-1} \|\pi \| &\leq& \|\nabla \pi \| &\leq& C_0 \| \pi\|\\
C_0^{-1} \|\pi \| &\leq&  \lambda(\pi) :=\|\cM_a(\pi) \| &\leq& C_0 \| \pi\|,
\end{array}
\ee
and 
\be
\label{eqContHomog2}
\begin{array}{ccc}
\mu(\pi) := \|\cM_a(\pi)^{-1} \|^{-1} & \leq& C_0 \|\pi\|\\
\nu(\pi) := \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^\frac 1 3 &\leq&  C_0 \|\pi\|.
\end{array}
\ee
We consider below a fixed polynomial $\pi\in \H_3$, and we recall that 
$$
L_g(\pi) := \inf \{\sqrt{\det M} \sep \sqrt{\|M\|} \|\pi \circ M^{-\frac 1 2}\| \leq 1\}.
$$

We first prove the lower bound $L_g(\pi)\geq c \sqrt{\det \cM_g(\pi)}$, where $c>0$ is an absolute constant.
For that purpose we consider a matrix $M\in S_d^+$ satisfying the constraint $\|M^{\frac 1 2}\| \| \nabla (\pi \circ M^{-\frac 1 2}) \|\leq 1$. Combining this with \iref{eqContHomog} we obtain
$$
1 \geq C_0^{-1}  \|M^{\frac 1 2}\| \| \pi \circ M^{-\frac 1 2} \| \geq C_0^{-1} \|M^{\frac 1 2}\| \frac{\| \pi \|}{\| M^{\frac 1 2}\|^3} = \frac{\|\pi\|}{C_0 \|M\|},
$$
hence $\|\pi\| \leq C_0 \|M\|$. It follows that 
$$
1 \geq C_0^{-1} (C_0^{-1} \|\pi\|)^{\frac 1 2} \| \pi\circ M^{-\frac 1 2}\| = \|\ti \pi \circ M^{-\frac 1 2}\|,
$$
where $\ti \pi := C_0^{-\frac 3 2} \| \pi\|^{\frac 1 2} \pi$. %$\ti \pi := \mu \pi$ and $\mu := C^{-\frac 3 2} \| \pi\|^{\frac 1 2}$.
The solution $M_*$ of the minimization problem
$$
\inf\{ \det M \sep \|\ti \pi \circ M^{-\frac 1 2}\| \leq 1\}
$$
is known exactly in the case of cubic polynomials in two dimensions, see Chapter \ref{chapOptAniso}, and satisfies 
$$
(\det M_*)^3 = \kappa |\disc \ti \pi| = \kappa (C_0^{-\frac 3 2} \| \pi\|^{\frac 1 2})^4 |\disc \pi| = \kappa C_0^{-6} \| \pi\|^2 |\disc \pi|.
$$
where $\kappa$ is a positive constant which depends only on the sign of $\disc \ti \pi$.
Defining $c_0:=\kappa_*^\frac 1 6 C_0^{-1}$, where $\kappa_*$ stands for the minimial value of $\kappa$ for the two possible signs, we obtain 
\begin{eqnarray*}
L_g(\pi) &\geq& (\det M_*)^{\frac 1 2} \\
&= & \kappa^\frac 1 6 C_0^{-1} \|\pi\|^{\frac 1 3} |\disc \pi|^{\frac 1 6} \\
&\geq& c_0 \sqrt{\|\pi\| \nu(\pi)} %\left(\frac{|\disc\pi|}{\|\pi\|}\right)^\frac 1 6\\
%&\geq & \kappa^\frac 1 6 C^{-\frac 3 2} \|\cM_a(\pi)\|^\frac 1 2 
\end{eqnarray*}
On the other hand, there exists $c_1>0$ such that 
$$
L_g(\pi) \geq L_a(\pi) \geq c_1 \sqrt{\det \cM_a(\pi)} = c_1\sqrt{\lambda(\pi) \mu(\pi)}.
$$
Furthermore we have 
\begin{eqnarray*}
\det \cM_g(\pi) &=& (\lambda(\pi)+\nu(\pi))(\mu(\pi)+\nu(\pi)) \\
&\leq& (1+C_0^2)\min \{\lambda(\pi),\, \|\pi\|\} \left( 2\max\{\mu(\pi),\, \nu(\pi)\}\right)\\
&\leq & 2(1+C_0^2) \max \{\lambda(\pi) \mu(\pi), \, \|\pi\| \nu(\pi)\}.
\end{eqnarray*}
We thus obtain
%Combining the last two equations, and recalling \iref{eqContHomog} and \iref{eqContHomog2} we obtain 
$$
\sqrt{\det \cM_g(\pi)}\leq C_* L_g(\pi) \stext{ where } C_*:= 2(1+C_0^2) \max \{c_0^{-1}, \, c_1^{-1}\}.
$$
which concludes the proof of our lower estimate for $L_g$.\\

We now turn to the proof of the property \iref{eqConstraint}, which is equivalent to the following 
%We establish in the paragraph that the matrix $M = C \cM_g(\pi)$ satisfies the inequality $\|M^{\frac 1 2}\| \| \nabla (\pi \circ M^{-\frac 1 2})\|\leq 1$ when $C$ is large enough (but independent of $\pi$), or equivalently that 
$$
\|\cM_g(\pi)\|^\frac 1 2 \|\cM_g(\pi)^{-\frac 1 2}( \nabla \pi(x,y))\| \leq C \stext{ when } \|(x,y)\|_{\cM_g(\pi)} \leq 1.
$$
For any rotation $U\in \cO_2$ we have $\cM_a(\pi \circ U) = U^\trans \cM_a(\pi) U$, see Chapter \ref{chapW1P}, and $\disc (\pi \circ U) = (\disc \pi) (\det U)^6 = \disc \pi$, see Chapter \ref{chapOptiAniso}. We may therefore assume, up to a rotation, that $\cM_a(\pi)$ is a diagonal matrix and that the first diagonal  coefficient is larger than the second one.
Therefore 
$$
\lambda(\pi)^2 = a^2+2b^2+c^2 \stext{ and } \mu(\pi)^2 = b^2+2c^2+d^2,
$$
and 
$\cM_a(\pi) = 
\left(
\begin{array}{cc}
\lambda(\pi) & 0 \\
0 & \mu(\pi)
\end{array}
\right)
$.
Note that this matrix is degenerate if and only if $\mu(\pi) = 0$, which means that $\pi$ is the univariate polynomial $a x^3$.
In order to avoid notational clutter, and since the polynomial $\pi\in \H_3$ is fixed, we denote below by $\lambda$, $\mu$ and $\nu$ the quantities $\lambda(\pi)$, $\mu(\pi)$ and $\nu(\pi)$.
%For that purpose we define 
%$$
%\mu^2 := a^2+2b^2+c^2 \stext{ and } \mu^2 := b^2+2c^2+d^2.
%$$
% The eigenvalues of $\cM_a(\pi)$ are therefore $\mu$ and $\mu$, and we may assume furthermore that $\mu \geq \mu$.
%We also define 
%$$
%\nu := \frac 1 3 \left(\frac{-\disc\pi}{\|\pi\|}\right)_+^{\frac 1 3}
%$$
Our purpose is to establish an upper bound on the quantity
\be
\label{eqMGGradPi}
\begin{array}{cl}
& \displaystyle\|\cM_g(\pi)\|^\frac 1 2 \|\cM_g(\pi)^{-\frac 1 2}( \nabla \pi(x,y))\| \\
=&  \displaystyle(a x^2+ 2 b xy + c y^2)^2 + \left(\frac {\lambda+\nu} {\mu+\nu}\right) (b x^2+ 2 c xy+ d y^2)^2.
\end{array}
\ee
%Our purpose is to bound
%$$
% (a x^2+ 2 b xy + c y^2)^2 + \left(\frac \mu {\max\{\mu, \nu\}}\right) (b x^2+ 2 c xy+ d y^2)^2 
%$$
under the hypothesis 
$$
\|(x,y)\|_{\cM_g(\pi)} = (\lambda+\nu) x^2+ (\mu+\nu) y^2 \leq 1,%\frac {x^2} {\lambda+\nu} + \frac {y^2} {\mu+\nu} \leq 1.
$$
which implies in particular $\lambda x\leq 1$ and $\max\{\mu,\nu\} y\leq 1$.
Injecting this in \iref{eqMGGradPi}, and observing using \iref{eqContHomog} and \iref{eqContHomog2} that $\nu\leq C_0^2 \lambda$, we see that it is sufficient to bound the following quantities %We thus need to bound the quantities
\be
\label{eqabcLl}
\frac a {\lambda^2}, \, \frac b {\lambda \mu}, \, \frac c {\mu^2}
\stext{ and }
\frac \lambda \mu \frac b {\lambda^2}, \ \frac \lambda \mu \frac c {\mu \lambda}, \ \frac \lambda {\max\{\mu,\nu\}} \frac d {\max\{\mu, \nu\}^2}.
\ee
Observing that 
\be
\label{eqLlMax}
\mu \geq \max\{b,c,d\}
\stext{ and }
\lambda \geq \max\{a,b,c,\mu\} \geq \{a,b,c,d\}
\ee
we find that all the quantities appearing in \iref{eqabcLl} are smaller than one, except perhaps the last one : 
%
%Since $\lambda \leq \lambda+\nu \leq (1+C_0^2)\lambda$ and $\max\{\mu, \nu\} \leq \mu+\nu \leq 2\max\{\mu,\nu\}$ we only need to bound 
%The only difficulty comes from 
\be
\label{eqd}
\frac {\lambda d^2}{\max\{\mu, \nu\}^3}
\ee
Using the expression \iref{eqDiscDet} of the discriminant we find that 
$$
-\disc \pi = (a^2+b^2+c^2) d^2 + a Q(b,c,d)+R(b,c,d)
$$
where $Q$ and $R$ are homogenous polynomials of degree $3$ and $4$ respectively. Hence there exists a constant $C_1$, independent of $\pi$, such that %Using \iref{eqLlMax} we therefore obtain, for a constant $C_1$ sufficiently large (but independent of $\pi$),
\begin{eqnarray*}
\lambda^2 d^2 &=& -\disc \pi - (a Q(b,c,d)+R(b,c,d)) \\
&\leq &\|\pi\| \nu^3 +C_1 \lambda \mu^3 \\
&\leq &\left(C_0 + C_1\right) \lambda \max \{\mu, \nu\}^3
\end{eqnarray*}
The previous inequality yields a uniform bound on \iref{eqd}, which concludes the proof of this proposition.
\sq

Proposition \iref{propLm} immediately gives an explicit expression, up to a fixed multiplicative constant, of the shape functions $L_a$ and $L_g$ in the case $m=3$ and $d=2$. For instance
$$
L_g(a x^3+ d y^3) \simeq \sqrt[3]{|ad| \max\{|a|,\, |d|\}} \stext{ and } L_a(a x^3+ d y^3) \simeq \sqrt{|ad|},
$$
and 
$$
L_g(ax^3+3cx y^2) \simeq L_a(a x^3+3c xy^2) \simeq \sqrt{\max\{|a|,\, |c|\} |c|}.
$$
For a function which has anisotropic features of the type $a x^3+ d y^3$, where $a$ and $d$ have different orders of magnitude, the use of quasi-acute meshes and metrics may therefore lead to a substantial improvement of the approximation error compared to graded meshes and metrics. This is not the case in contrast if all the anisotropic features of the approximated function are of the type $ax^3+3cx y^2$.

\subsection{Geometric convexity} %Geometric convexity, and 
\label{subsubsecGeomCvx}
We introduce in this section the geometric average of two symmetric positive definite matrices, and the property of geometric convexity for functions defined on $S_d^+$. This notion is a variant of the classical property of convexity, which is appropriate for the study of the minimization problems appearing in the expressions \ref{defKM}, \ref{defLAM} and \ref{defLGM} of the shape functions $K$, $L_a$ and $L_g$.

%We also introduce the notion of geometric average of two matrices.
Let $M, M'\in S_d^+$, and let $S:=M^{-\frac 1 2}$. We define the geometric average $\Avg(M,M')\in S_d^+$ of $M$ and $M'$ as follows
\be
\label{defAvg}
S \Avg(M,M') S := \sqrt{S M' S}
\ee
For instance $\Avg(M,M^{-1}) = \Id$, and for any $k,k'>0$
$$
\Avg(k M , k'M') = \sqrt{k k'} \Avg(M,M').
$$

The following proposition gives an alternative characterization \iref{eqAvgAD} of $\Avg(M,M')$. This proposition also shows that $\Avg(M,M')$ is a natural midpoint between $M$ and $M'$ for the distance $d_\times$, and establishes two basic properties of the geometric average of matrices.
% number of useful properties.

\begin{prop}
For any $M,M'\in S_d^+$ the following holds.
\begin{enumerate}
\item A matrix $\ti M$ satisfies $\tilde M = \Avg(M,M')$ if and only if there exists $A \in \GL_d$ and a diagonal matrix $D$ such that 
\be
\label{eqAvgAD}
\tilde M = A^\trans A, \quad M = A^\trans e^{2D} A, \quad M' = A^\trans e^{-2D} A.
\ee
\item The geometric average $\Avg(M,M')$ is a midpoint between $M$ and $M'$ for the distance $d_\times$ on $S_d^+$:
$$
d_\times (M, \Avg(M,M')) = d_\times (\Avg(M,M'), M') = \frac 1 2 d_\times (M,M').
$$
\item The geometric average is commutative and compatible with the inversion of matrices:
\begin{eqnarray}
\label{eqAvgCommut}
\Avg(M,M') &=& \Avg(M',M)\\
\label{eqAvgInv}
\Avg(M,M')^{-1} &=& \Avg(M^{-1}, M'^{-1})
\end{eqnarray}
\end{enumerate}
\end{prop}

\proof
We first establish point 1.
Let us assume in a first time that $M,M'$ and $\tilde M$ have the form \iref{eqAvgAD}. We easily obtain 
$$
\tilde M M^{-1} \tilde M = M'
$$
Defining $S := M^{-\frac 1 2}$ we thus have 
$$
(S\tilde M S)^2 = S M' S.
$$
Taking the square root of the previous equation we obtain \iref{defAvg} which shows that $\tilde M = \Avg(M,M')$.

In order to establish the converse of this property we only need to show that for any $M,M'\in S_d^+$ there exists $A\in \GL_d$ and a diagonal matrix $D$ such that $M = A^\trans e^{2D} A$ and $M' = A^\trans e^{-2D} A$. The expression of $\Avg(M,M')$ then automatically follows from the previous argument.
Since the matrix $M'^{-\frac 1 2} M M'^{-\frac 1 2}$ is symmetric positive definite, there exists $U\in \cO_d$ and a diagonal matrix $D$ such that this matrix equals $U^\trans \exp (4D) U$. Choosing $A := e^D U M'^{\frac 1 2}$ we obtain the announced result.\\

We now turn to the proof of Point 2. Let $A\in \GL_d$ and let $D,D'$ be diagonal matrices, of diagonal coefficients $D_1, \cdots ,D_k$ and  $D'_1, \cdots , D'_d$ respectively. We define
$$
\delta := \max_{1\leq i \leq d} |D_i - D'_i|.
$$ 
We claim that the matrices $N := A^\trans e^{2D} A$ and $N':=A^\trans e^{2D'} A$ satisfy $d_\times(N,N') = \delta$.
Indeed
\begin{eqnarray*}
d_\times (N,\, N') &:= &\sup_{u\neq 0} \left|\ln \|u\|_N -\ln \|u\|_{N'}\right| \\
&=& \sup_{u\neq 0} \left|\ln |e^D Au| - \ln |e^{D'} Au|\right|\\
&=& \sup_{v\neq 0}  \left|\ln |e^D v| - \ln |e^{D'} v|\right|.
\end{eqnarray*}
For any $v=(v_1, \cdots ,v_d)\in \R^d$ we have 
$$
|e^D v|^2 = \sum_{1\leq i \leq d} e^{2D_i} v_i^2 \leq e^{2\delta}  \sum_{1\leq i \leq d} e^{2D'_i} v_i^2 = \left(e^\delta |e^{D'}v|\right)^2,
$$
and similarly $|e^{D'} v|\leq e^\delta |e^D v|$. Therefore $\left|\ln |e^D v| - \ln |e^{D'} v|\right|\leq \delta$ and taking the supremum among all $v\neq 0$ we obtain $d_\times(N,N') \leq \delta$. Furthermore denote by $i_0$, $1\leq i_0\leq d$, the position such that $|D_{i_0} - D'_{i_0}| = \delta$. Choosing $v = (0,\cdots ,1, \cdots ,0)$, with the nonzero coordinate at the position $i_0$, we obtain $\delta = \left|\ln |e^D v| - \ln |e^{D'} v|\right| \leq d_\times(N,N')$. We thus conclude that 
$$
d_\times (N,N') =  d_\times (A^\trans e^{2D} A, \, A^\trans e^{2D'} A) = \|D-D'\|.
$$

Recalling that $M,M'$ and $\ti M := \Avg(M,M')$ have the form \iref{eqAvgAD} we thus obtain 
$$
d_\times (M, \Avg(M,M')) = d_\times (\Avg(M,M'), M')= \|D\| \stext{ and } d_\times (M,M') = 2 \|D\|.
$$
which concludes the proof of this point.\\

Finally we establish Point 3.
Using the first point we obtain that $M,M'$ and $\tilde M := \Avg(M,M')$ have the form
$$
\tilde M = A^\trans A, \quad M = A^\trans e^{2D} A, \quad M' = A^\trans e^{-2D} A
$$
It follows that 
\be
\label{charCommut}
\tilde M = A^\trans A, \quad M' = A^\trans e^{-2D} A, \quad M = A^\trans e^{2D} A,
\ee
and 
\be
\label{charInv}
\tilde M^{-1} = (A^{-1})^\trans A^{-1}, \quad M^{-1} = (A^{-1})^\trans e^{-2D} A^{-1}, \quad M'^{-1} = (A^{-1})^\trans e^{2D} A^{-1}.
\ee
Equation  \iref{eqAvgCommut} (resp. \iref{eqAvgInv}) is the consequence of \iref{charCommut} (resp. \iref{charInv}) and of the characterization of the geometric average given in the first point.\sq

We recall that that a function $\psi\in C^0(S_d, \R)$ is convex if and only if for all $M,M'\in S_d$ one has 
\be
\label{defConv}
\psi\left(\frac{M+M'} 2\right) \leq \frac{\psi(M)+ \psi(M')} 2.
\ee
The next proposition introduces the family of geometrically convex functions on $S_d^+$, which is defined by a property similar to \iref{defConv} but in which the arithmetic averages are replaced with geometric averages.
\begin{definition}
We say that a function $\vp \in C^0(S_d^+ , \R_+^*)$ is Geometrically Convex and Homogenous (GCH), if it satisfies the following properties.
\begin{enumerate}[i)]
\item (Sub multiplicativity) For any $M,M'\in S_d^+$ one has
\be
\label{eqSubMult}
\vp(\Avg(M,M')) \leq \sqrt{\vp(M) \vp(M')}.
\ee
\item (Homogenous) There exists $\alpha \in \R$ , called the degree of $\vp$,
such that for all $M\in S_d^+$ and all $\lambda\in \R$ one has 
$$
\vp(\lambda M) = \lambda^\alpha \vp(M).
$$
\end{enumerate}
We say that the function $\vp$ is Strictly Geometrically Convex and Homogeneous (SGCH), if $\vp$ is GCH and if the equality in \iref{eqSubMult} only holds if $M$ and $M'$ are proportional.
\end{definition}

For instance the function $\det$ is GCH of degree $d$, since 
$$
\det \Avg(M,M') = \sqrt{\det M \det M'} \stext{ and } \det (\lambda M) = \lambda^d M.
$$
We insist on point that GCH functions are by assumption strictly positive on $S_d^+$, and continuous.
The next lemma enumerates some simple properties of geometrically convex functions.
\begin{lemma}
\label{lemmaAlgGCH}
\begin{enumerate}
\item The product of two GCH functions is GCH, and the product of a GCH function with a SGCH function is SGCH. Furthermore the degrees add.
\item The elevation to a positive power $\alpha\in \R_+^*$ of a GCH (resp. SGCH) function is also GCH (resp. SGCH). Furthermore the degree is multiplied by $\alpha$.
\item If a function $\vp$ is GCH (resp. SGCH) then $M \mapsto \vp(M^{-1})$ is also GCH (resp. SGCH), and has the opposite degree.
\end{enumerate}
\end{lemma}
\proof
The first two points are immediate, and the last point is a direct consequence of the compatibility \iref{eqAvgInv} of the geometric average with the inversion : if $\vp$ is GCH and $M,M'\in S_d^+$ then 
$$
\vp(\Avg(M,M')^{-1}) = \vp(\Avg(M^{-1}, M'^{-1})) \leq \sqrt{\vp(M^{-1}) \vp (M'^{-1})},
$$
which concludes the proof.
\sq

Aside from the determinant, a number of functions on $S_d^+$ are geometrically convex. The next proposition, which is based on an argument of complex analysis, enumerates some of them.
For all $\pi\in \H_m$ we define 
$$
\|\pi\|_\sC := \sup\{ |\pi(z)| \sep z\in \C^d, \, |z|\leq 1\}.
$$

\begin{prop}
\label{propExGCH}
\begin{enumerate}
\item The trace map $M \mapsto \Tr M$ is SGCH.
\item For any fixed polynomial $\pi\in \H_m\sm\{0\}$ the map $M \mapsto \|\pi \circ M^{\frac 1 2}\|_\sC$ is GCH, of degree $m/2$.
\item The norm map $M \mapsto \|M\|$ is GCH. 
\end{enumerate}

%For any $M,M'\in S_d^+$ the following holds.
%\begin{enumerate}
%\item 
%\be
%\label{eqTr}
%\Tr (\Avg(M,M'))\leq \sqrt{\Tr M \Tr M'} \stext{ and } \Tr (\Avg(M,M')^{-1})\leq \sqrt{\Tr (M^{-1}) \Tr (M'^{-1})}
%\ee
% with equality if and only if the matrices $M$ and $M'$ are proportionnal. %and inverse.
%\item For any polynomial $\mu \in \H_m$ one has %$\C$ %define S, S', \tilde S
%$$
%\|\mu \circ \Avg(M,M')^{-\frac 1 2}\|_\sC \leq \sqrt{\|\pi\circ M^{-\frac 1 2}\|_\sC \|\pi\circ M'^{-\frac 1 2}\|_\sC }
%$$
%\item We have 
%$$
%\|\Avg(M, M')\| \leq \sqrt{\|M\| \|M'\|}
%$$
%\end{enumerate}
\end{prop}

\proof
We first establish Point 1.
Let $M,M'\in S_d^+$ and let $\ti M := \Avg(M)$. Let $A\in \GL_d$ and $D$ be a diagonal matrix be such that  $M = A^\trans e^{-2D}$, $M' = A^\trans e^{2D} A$ and $\ti M = A^\trans A$.
We denote by $A_{i,j}$ the coefficients of $A$, and we define for all $1\leq i \leq d$
$$
\cA_i^2 := \sum_{1\leq j \leq d} A_{ji}^2.
$$
Note that $\cA_i>0$ for all $1\leq i \leq d$, since otherwise a full line of $A$ would be zero and $A$ would be degenerate.
Denoting by $D_i , \cdots , D_d$ the diagonal coefficients of $D$ we obtain  
$$
\Tr(M) = \sum_{1\leq i \leq d} \cA_i^2 e^{-2D_i}, \quad \Tr(M') = \sum_{1\leq i \leq d} \cA_i^2 e^{2D_i}, \quad \Tr(\ti M) = \sum_{1\leq i \leq d} \cA_i^2.
$$
It thus follows from Cauchy Schwartz inequality that $\Tr(\ti M)^2 \leq \Tr(M) \Tr(M')$. Furthermore equality occurs if and only if the vectors 
$$
(\cA_i e^{-D_i})_{1\leq i \leq d} \stext{ and }(\cA_i e^{D_i})_{1\leq i \leq d}
$$
are proportional, which implies that $D_i =D_j$ for all $1\leq i,j\leq d$ and therefore that $M$ and $M'$ are proportional. \\

We now turn to the proof of Point 2. and for that purpose we recall a classical result of complex analysis, called Hadamard's three lines theorem. %see [Rudin??], often
Let $\Omega:=\{\alpha\in \C \sep |\Re(\alpha)|<1\}$, where $\Re$ denotes the real part, and let $g$ be a continuous and bounded function on $\overline \Omega$ which is holomorphic on $\Omega$. Then 
\be
\label{eqComplex}
|g(0)|^2 \leq \left(\sup_{\Re \alpha = -1} |g(\alpha)|\right) \left(\sup_{\Re z = \alpha} |g(\alpha)|\right).
\ee

%We say that a matrix $U$ with complex coefficients is unitary if $|Uz| = |z|$ for all $z\in \C$, or equivalently if $U^* U = \Id$ where $U^*$ denotes the conjugate transpose of $U$. We recall that any orthogonal matrix $O\in \cO_d$ is also unitary, and that for any diagonal matrix $D$ with real diagonal coefficients and any $\beta\in \R$ the matrix $e^{\b i \beta D}$ is unitary, where $\b i^2 = -1$.


We consider a fixed $z\in \C^d$ satisfying $|z|\leq 1$, and we define for all $\alpha\in \overline \Omega$ 
%We consider a fixed $z\in \C^d$ and we define 
$$
g(\alpha) := \pi(A^\trans e^{\alpha D} z).
$$
The function $g$ is continuous, uniformly bounded on $\overline \Omega$ by $\|\pi\|_\sC (\|A\| e^{\|D\|})^d$, and holomorphic in $\Omega$, hence the three lines theorem applies.
For any $\sigma \in \{-1,1\}$ one has 
$$
\sup_{\Re(\alpha) = \sigma} |\pi(A^\trans e^{\alpha D} z)| \leq \|\pi\circ(A^\trans e^{\sigma D})\|_\sC,
$$
since $|e^{\b i\Im(\alpha) D}z| = |z|=1$, where $\Im$ denotes the imaginary part. %$|e^{i\Im(\alpha) D} z| = |z|$ where $\Im$ denotes the imaginary part.
Applying \iref{eqComplex} to the function $g$ we thus obtain 
$$
|\pi(A^\trans z)|^2 \leq \|\pi\circ(A^\trans e^D)\|_\sC \|\pi\circ(A^\trans e^{-D})\|_\sC.%\left(\sup_{\Re \alpha = -1} f(A^\trans e^\alpha z)\right) \sup
$$
Taking the supremum among all $z\in \C^d$ such that $|z|\leq 1$ we conclude that 
$$
\|\pi\circ A^\trans\|_\sC \leq \|\pi\circ(A^\trans e^D)\|_\sC \|\pi\circ(A^\trans e^{-D})\|_\sC.
$$
%Last we recall (ref??) that
One easily checks that the matrices $O, O', \tilde O\in \GL_d$ defined by  
$$
OM^\frac 1 2 =  e^D A, \quad O'M'{^\frac 1 2} = e^{-D} A \stext{ and } \tilde O \tilde M^\frac 1 2 = A,
$$
are orthogonal.
Since orthogonal matrices are also unitary matrices, in the sense that $|Oz| = |z|$ for all $z\in \C$, we obtain
\begin{eqnarray*}
\|\pi \circ A^Te^{-D}\|_\sC &=& \|\pi \circ M^{\frac 1 2}\|_\sC,\\
\|\pi \circ A^T e^{-D}\|_\sC &=& \|\pi \circ  M'^{\frac 1 2}\|_\sC\\
\|\pi \circ A^T\|_\sC &=& \|\pi \circ \ti M^{\frac 1 2}\|_\sC,
\end{eqnarray*}
thus $\|\pi\circ M^\frac 1 2\|_\sC$ satisfies the sub-multiplicativity property \iref{eqSubMult}. Furthermore the function $M\in S_d^+ \mapsto \|\pi\circ M^\frac 1 2\|_\sC$ is clearly continuous, strictly positive, and homogeneous of degree $m/2$ which concludes the proof of this point.\\

We now establish Point 3, and for that purpose we denote by $\pi\in \H_2$ the canonical quadratic form 
$$
\pi(z) := \sum_{1\leq j \leq d} z_j^2.
$$
Our purpose is to establish that for any $M\in S_d^+$
\be
\label{eqPiMM}
\|\pi\circ M^{\frac 1 2}\|_\sC = \|M\|,
\ee
which implies that $\|M\|$ is GCH in view of the previous point.
For any $z\in \C$ such that $|z|\leq 1$ one has 
$$
|\pi(M^\frac 1 2 z)| = |z^\trans M^\frac 1 2 M^\frac 1 2 z| \leq |M^\frac 1 2 z|^2 \leq \|M^\frac 1 2\|^2  = \|M\|.
$$
Furthermore choosing a normalized eigenvector $z\in \R^d$ associated to the maximal eigenvalue of $M$ we obtain $|\pi(M^\frac 1 2 z)|=\|M\|$, which establishes \iref{eqPiMM} and concludes the proof.
\sq

\subsection{A well posed variant of the shape function}
\label{subsecWellPosed}
We define in this section three variants of the shape functions $K$, $L_a$ and $L_g$ : for all $\pi \in \H_m$
\begin{eqnarray*}
K^\sC(\pi) &:=& \inf_{A\in \SL_d} \|\pi\circ A\|_\sC\\
L_a^\sC(\pi) &:=& \inf_{A\in \SL_d} \sqrt{\|G(\pi)\circ A\|_\sC}\\
L_g^\sC(\pi) &:=& \inf_{A\in \SL_d} \|A^{-1}\| \|\pi\circ A\|_\sC,
\end{eqnarray*}
where $G(\pi) := |\nabla \pi|^2 \in \H_{2m-2}$,
We also define a function $\kappa\in C^0(S_d^+, [1,\infty))$ as follows : for all $M\in S_d^+$ 
$$
\kappa(M) :=  \frac 1 d\sqrt{\Tr(M) \Tr(M^{-1})}.
$$
For each $\alpha\in (0,\infty)$ we define three new variants of the shape functions
\begin{eqnarray*}
K^{(\alpha)}(\pi) &:=& \inf\{\kappa(M)^{\frac 1\alpha} (\det M)^{\frac m {2d}} \sep \|\pi\circ M^{-\frac 1 2}\|_\sC\leq 1\text{ and } \kappa(M)\leq e^\alpha\}\\
L_a^{(\alpha)}(\pi) &:=& \inf\{\kappa(M)^{\frac 1\alpha} (\det M)^{\frac {m-1} {2d}} \sep \|G(\pi)\circ M^{-\frac 1 2}\|_\sC\leq 1\text{ and } \kappa(M)\leq e^\alpha\}\\
L_g^{(\alpha)}(\pi) &:=& \inf\{\kappa(M)^{\frac 1\alpha} (\det M)^{\frac {m-1} {2d}} \sep \|M\|^\frac 1 2 \|\pi\circ M^{-\frac 1 2}\|_\sC\leq 1\text{ and } \kappa(M)\leq e^\alpha\}.
\end{eqnarray*}
This section is devoted to the proof of the following theorem. %, which shows that the above optimization problems are well posed.
\begin{theorem}
\label{thWellPosed}
\begin{enumerate}
\item
The shape function $K$ (resp. $L_a$, resp. $L_g$) is uniformly equivalent to $K^\sC$ on $\H_m$ (resp. $L_a^\sC$, resp. $L_g^\sC$).
\item
For each $\pi\in \H_m$ we have the decreasing convergence
$$
\lim_{\alpha \to \infty} K^{(\alpha)}(\pi) = K^\sC(\pi)
$$ 
(resp. $L_a^{(\alpha)}(\pi) \to L_a^\sC(\pi)$, resp. $L_g^{(\alpha)}(\pi) \to L_g^\sC(\pi)$ as $\alpha \to \infty$).
\item
For each $\alpha \in (0,\infty)$ and each $\pi \in \H_m\sm\{0\}$ there exists a unique minimizer $\cM^{(\alpha)}(\pi)\in S_d^+$ to the optimization problem defining $K^{(\alpha)}(\pi)$ 
and the map 
$$
\pi\in \H_m\sm\{0\} \to \cM^{(\alpha)}(\pi)\in S_d^+
$$
%%from $\H_m \to S_d$ defined by 
%$$
%\pi \mapsto 
%\left\{
%\begin{array}{cc}
%\cM^{(\alpha)}(\pi) &  \text{ if } \pi \neq 0\\
%0 & \text{ if } \pi = 0
%\end{array}
%\right.
%$$
is continuous.
(resp. likewise for $L^{(\alpha)}(\pi)$ and $\cM^{(\alpha)}_a(\pi)$, resp. likewise for $L_g^{(\alpha)}(\pi)$ and $\cM^{(\alpha)}_g(\pi)$).
\end{enumerate}
\end{theorem}

We first establish point 1. of this theorem.
%These variants are equivalent to the original shape functions on $\H_m$. Indeed 
Since the vector spaces $\H_m$ and $\H_{2m-2}$ have finite dimension, there exists three constants $C_K$, $C_a$ and $C_g$ such that 
\be
\label{defCKAG}
\begin{array}{rcccll}
\|\pi\| &\leq & \|\pi\|_\sC&\leq &C_K \|\pi\|, & \pi \in \H_m\\
\|\pi'\| &\leq & \|\pi'\|_\sC&\leq &C_a \|\pi'\|, & \pi \in \H_{2m-2}\\
C_g^{-1} \|\nabla \pi\| &\leq & \|\pi\|_\sC&\leq& C_g \|\nabla \pi\|, & \pi \in \H_m.
\end{array}
\ee
Hence it follows from the definition of the original shape functions, given in \S\ref{subsecIntroAsympt}, that $K\leq K^\sC\leq C_K K$, $L_a \leq L_a^\sC \leq C_a L_a$ and $C_g ^{-1}L_g  \leq L_g^\sC \leq C_g L_g$ on $\H_m$.\\

We now turn to the proof of Point 2. of this theorem.
In terms of the eigenvalues $\lambda_1, \cdots, \lambda_d$ of $M$ we have 
$$
d^2 \kappa(M)^2 = \left(\sum_{1 \leq i \leq d} \lambda_i\right)\left(\sum_{1 \leq i \leq d} \lambda_i^{-1}\right).
$$ 
Therefore $1\leq \kappa(M) < \infty$ for each $M\in S_d^+$, which immediately implies Point 2. of Theorem \ref{thWellPosed}.
Note that $\kappa(M) = 1$ if and only if $M = m\Id$ for some $m>0$, and that 
$$
\kappa(M)\leq \sqrt{\|M\|\|M^{-1}\|} \leq d \, \kappa(M).
$$
Since the function $M\mapsto \Tr(M)$ is SGCH, the function $\kappa\in C^0(S_d^+, [1, \infty)$ is also SGCH according to Lemma \ref{lemmaAlgGCH}. 
We regard the function $\kappa$ as a close variation on the condition number $\sqrt{\|M\|\|M^{-1}\|}$ of the matrix $M^\frac 1 2$. Note that $\kappa(M) = 1$ if and only if $M = m\Id$ for some $m>0$, and that 
$$
\kappa(M)\leq \sqrt{\|M\|\|M^{-1}\|} \leq d \, \kappa(M).
$$
The following proposition illustrates the use of $\kappa$ as a regularization term, and immediately implies Point 3. of Theorem \ref{thWellPosed}.
\begin{prop}
\label{propContLift}
Let $\vp$ be a GSH function of degree $r>0$. 
Let $(X,d_X)$ be a metric space, and let $\psi\in C^0(S_d^+ \times X, \R_+^*)$ be such that $\psi(\cdot,x)$ is GCH of degree $-1$ for any fixed $x\in X$.
We define for all $x\in X$ and all $\alpha \in (0, \infty)$
$$
L^{(\alpha)}(x) := \inf\left\{\kappa(M)^{\frac 1 \alpha} \vp(M) \sep \psi(M,x) \leq 1 \text{ and } \kappa(M) \leq e^\alpha\right\}.
$$
For any $x\in X$ there exists a unique minimizer $\cM^{(\alpha)}(x)$ to the optimization problem defining $L^{(\alpha)}(x)$. Furthermore the map $\cM^{(\alpha)} : X \to S_d^+$ is continuous. 
\end{prop}

\proof
We consider a fixed parameter $\alpha\in (0, \infty)$.
We first establish the existence of a minimizer to the optimization problem defining $L^{(\alpha)}(x)$, and we thus consider a fixed $x\in X$.
For any $\beta \geq 0$ the following collection of matrices is clearly a compact subset of $S_d^+$
\be
\label{defKBeta}
K_\beta := \{M\in S_d^+ \sep |\ln(\det M)|\leq \beta \text{ and } \kappa(M) \leq e^\alpha\}.
\ee
We define
$$
\Lambda := \sup_{M\in K_0} \vp(M) \stext{ and } \lambda := \inf_{M\in K_0} \psi(M,x)
$$
in such way that for any $M\in S_d^+$ satisfying $\kappa(M) \leq e^\alpha$
\be
\label{eqPhiPsi}
\vp(M) \leq \Lambda (\det M)^{\frac r d} \stext{ and } \psi(M,x) \geq \lambda (\det M)^{\frac 1 d}.
\ee
Let $(M_n)_{n \geq 0}$, $M_n\in S_d^+$, be a minimizing sequence for the optimization problem defining  $L^{(\alpha)}(x)$. It follows from \iref{eqPhiPsi} that $\det (M_n)$ uniformly bounded above and below: hence there exists $\beta \geq 0$ such that $|\ln \det M_n|\leq \beta$ for all $n \geq 0$. 
Furthermore $\kappa(M_n) \leq e^\alpha$ for each $n\geq 0$, hence $M_n \in K_\beta$. Since the set $K_\beta$ is compact there exists a converging subsequence $M_{\sigma(n)} \to M_\infty\in K_\beta$. By continuity of the functions $\vp$, $\psi(\cdot ,x)$ and $\kappa$ on $S_d^+$ the matrix $M_\infty$ is a minimizer of the optimization problem $L^{(\alpha)}(x)$.\\

We now consider tow minimizers $M,M'$ to the optimization problem defining $L^{(\alpha)}(x)$, and we intend to show that $M=M'$. We denote $\ti M := \Avg(M,M')$. 
Since the functions $\psi(\cdot, x)$ and $\kappa$ are GCH, the matrix $\ti M$ satisfies the inequalities 
$$
\psi(\ti M,x) \leq 1 \stext{ and } \kappa(\ti M) \leq e^\alpha.
$$ 
We define for each $M\in S_d^+$ the quantity
\be
\label{defPhiSGCH}
\Phi(M) := \kappa(M)^\frac 1 \alpha \vp(M),
\ee
and we observe that $\Phi : S_d^+ \to \R_+^*$ is a SGCH function of degree $r>0$ according to Lemma \ref{lemmaAlgGCH}.
If $M$ is not proportionnal to $M'$ we thus have
$$
\Phi(\ti M) < \sqrt{\Phi( M) \Phi( M')} = L^{(\alpha)}(x),
$$
 which is a contradicts the fact that $M$ and $M'$ are minimizers to the optimization problem defining $L^{(\alpha)}(x)$. Thus $M = m M'$ for some $m>0$, but this implies 
 $$
L^{(\alpha)}(x) = \Phi( M) = \Phi( M') = m^r  \Phi( M),
 $$
 therefore $m=1$ and $M=M'$, which establishes as announced that the minimizer is unique.\\

Finally we establish that the map $x \mapsto \cM^{(\alpha)}(x)$ is continuous.
For all $x,x'\in X$, we define
$$
\omega(x,x') := \sup_{M \in K_0} |\ln \psi(M,x) - \ln\psi(M,x')|,
$$
where the set $K_0$ is defined by \iref{defKBeta}, and we observe that $\omega(x,x') \to 0$ as $x'\to x$.
(Note that $\omega(x,x')$ is the modulus of continuity of the continuous function $X \to C^0(K_0, \R)$, defined by $x\mapsto \ln \psi (\cdot,x)$.)

Let $x,x'\in X$ and let $M := e^{\omega(x,x')} \cM^{(\alpha)}(x)$ and $M' := e^{\omega(x,x')} \cM^{(\alpha)}(x')$. We thus have 
$$
\kappa(M) = \kappa(\cM^{(\alpha)}(x)) \leq e^\alpha,
$$
and likewise $\kappa(M') \leq e^\alpha$.
Since $\psi(\cdot ,x')$ is homogeneous of degree $-1$ we obtain
$$
\psi(M, x')\leq e^{\omega(x,x_n)} \psi(M, x') = e^{\omega(x,x')} \psi(e^{\omega(x,x')} \cM^{(\alpha)}(x'),x') \leq 1,
$$
and likewise $\psi(M',x)\leq 1$.
Furthermore since the function $\Phi$ defined by \iref{defPhiSGCH} is homogeneous of degree $r$ we obtain
$$
L^{(\alpha)}(x') \leq \Phi(M) = e^{r\omega(x,x')} L^{(\alpha)}(x),
$$
%and likewise $L^{(\alpha)}(x) \leq \Phi(M') = e^{r\omega(x,x')} L^{(\alpha)}(x')$. It follows that 
which implies
$$
\Phi(M') = \Phi(e^{\omega(x,x')} \cM^{(\alpha)}(x'))  = e^{r\omega(x,x')} L^{(\alpha)}(x') \leq e^{2r\omega(x,x')} L^{(\alpha)}(x).
$$

Consider a converging sequence in $X$, $x_n \to x$, and define
$$
M_n := e^{\omega(x,x_n)} \cM^{(\alpha)} (x_n).
$$
The arguments above show that $M_n$ is a minimizing sequence for the optimization problem $L^{(\alpha)}(x)$. The arguments developed for the existence of a minimizer show that $\{M_n\sep n \geq 0\}$ is contained in the compact set $K_\beta$ if the constant $\beta\geq 0$ is sufficiently large, and that any converging subsequence of $(M_n)_{n \geq 0}$ tends to a minimizer of the optimization problem $L^{(\alpha)}(x)$, thus to $\cM^{(\alpha)}(x)$ by uniqueness.

Since the sequence $M_n$ takes its values in the compact set $K_\beta$ and has the single adherence value $\cM^{(\alpha)}(x)$, we have the convergence $M_n \to \cM^{(\alpha)}(x)$ as $n \to \infty$. Since $\omega(x,x_n) \to 0$ we obtain as announced 
$$
\cM^{(\alpha)}(x_n)\to \cM^{(\alpha)}(x),
$$
which concludes the proof of this proposition.
\sq

\begin{remark}
\label{remHomog2}
One easily checks that for each $\pi\in \H_m$, each $\alpha\in (0,\infty)$ and each $\lambda\in \R_+^*$ we have $K^{(\alpha)}(\lambda \pi) = \lambda L^{(\alpha)}(\pi)$ and 
$$
\cM^{(\alpha)}(\lambda \pi) = \lambda^\frac 2 m \cM^{(\alpha)}(\pi).
$$
It follows that $\cM^{(\alpha)}(\pi) \to 0$ as $\pi\to 0$, and therefore that the map 
from $\H_m \to S_d$ defined by 
$$
\pi \mapsto 
\left\{
\begin{array}{cc}
\cM^{(\alpha)}(\pi) &  \text{ if } \pi \neq 0\\
0 & \text{ if } \pi = 0
\end{array}
\right.
$$
is continuous.
Likewise $L^{(\alpha)}_a$ and $L^{(\alpha)}$ are $1$-homogeneous on $\H_m$, and $\cM^{(\alpha)}_a(\pi)$ and $\cM^{(\alpha)}_g(\lambda \pi)$ are $\frac 2 {m-1}$ homogeneous on $\H_m$ which implies that they tend to $0$ as $\pi \to 0$.
\end{remark}


\subsection{Construction of the metric}
\label{subsubsecExplicitMetricLP}


This subsection is devoted to the construction of a metric $H$ which is \emph{adapted} to a given smooth function $f$ in the sense that the error $e_H(f)_p$ (resp. $e_H^a(\nabla f)_p$, resp. $e_H^g(\nabla f)_p$) is \emph{optimally small} among all metrics of the \emph{same mass} $m(H)$. Our construction only applies to an asymptotically large mass of the metric $H$, and producing a such a metric of a given mass independent of $f$ is so far an open question.


%Our first lemma shows for any sufficiently smooth metric $H\in \bH_\per$ we have $\lambda^2 H\in \bH_a$ for all $\lambda$ sufficiently large. 
Our first lemma shows that the regularity constraints defining by the classes $\bH_a$ and $\bH_g$ of metrics ``disappear'' when one multiplies a metric with a large constant. %we consider metrics of arbitrarily large mass. %when we have from an asymptotical point of view
\begin{lemma}
For any $H\in\bH_\per$ which is $C^1$, there exists $\lambda_0 = \lambda_0(H)$ such that $\lambda^2 H\in \bH_a$ for all $\lambda\geq \lambda_0$.
\end{lemma}
\proof
The following maps are $C^1$ since they are the composition of $C^1$ maps
$$
\begin{array}{ccl}
z\in \R^d &\mapsto& H(z)^{-\frac 1 2} \in S_d\\
z\in \R^d &\mapsto& \vp_\times (H(z)) := (u \mapsto \ln \|u\|_{H(z)}) \in C^0(\bbS, \R)
\end{array}
$$
where $\bbS$ denotes the unit euclidean sphere (see \S\ref{secEigen} in the previous Chapter for a more in depth discussion on the map $\vp_\times$).
Since $H$ is $\Z^d$-periodic these maps are uniformly Lipschitz, hence there exists two constants $C_+, C_\times$ such that for all $z,z'\in \R^d$
$$
\begin{array}{ccccc}
d_+(H(z), H(z')) &:=& \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| &\leq& C_+ |z-z'| \\
d_\times(H(z), H(z')) &:=& \|\vp_\times(H(z))-\vp_\times(H(z'))\|_{L^\infty(\bbS)} &\leq& C_\times |z-z'| 
\end{array}
$$
Furthermore, again since $H$ is periodic, there exists $\ve>0$ such that $H(z) \geq \ve^2 \Id$ for all $z\in \R^d$. Hence
$$
d_H(z,z') \geq \ve |z-z'|,
$$
for all $z,z'\in \R^d$.
From this point, it follows from Remark \ref{remHomog} in the previous chapter that $\lambda^2 H\in \bH_a$ for all $\lambda \geq \lambda_0 := \max \{C_+, C_\times /\ve\}$.
\sq

Given a function $f\in C^m_\per$, an exponent $0\leq p\leq \infty$, and a triplet  $s=(\alpha, \rho, \delta)\in (\R_+^*)^3$ of parameters we construct a $C^\infty$ metric $H$ as follows.
For each $z\in \R^d$ we define 
$$
M(z) := \cM^{(\alpha)}(\pi_z) + \rho\Id,
$$
where the homogeneous polynomial $\pi_z\in \H_m$ is defined by \iref{defPiZ}. Note that $M$ is continuous according to Remark \ref{remHomog2}.
We consider a fixed mollifier $\psi$, namely a radial compactly supported $C^\infty$ function of integral one, and we denote $\psi_\delta := \psi(\cdot/\delta)/\delta^d$. We then define 
\be
\label{defHs}
H(z) := (\det M'(z))^\frac{-1}{mp+d} M'(z) \stext{ where } M' := \psi_\delta*M
\ee

Given a symbol $\star\in \{a,g\}$ we define similarly $M_\star := \cM^{(\alpha)}_\star(\pi_z) + \rho\Id$, $M' := \psi_\delta*M_\star$ and 
$$
H_\star (z) := (\det M'_\star(z))^\frac{-1}{(m-1)p+d} M'_\star(z).
$$

The rest of this subsection is devoted to the proof of the following theorem, which immediately implies the asymptotic estimates \iref{asymptLPMet}, \iref{asymptA} and \iref{asymptG} announced in the introduction. We do not prove that these estimates are optimal, but this is suggested by the lower bounds on the interpolation error on a mesh obtained in Chapters 2 and 3.
\begin{theorem}
There exists a constant $C=C(m,d)$ such that the following holds for any $f\in C^m_\per$, any $0\leq p\leq \infty$ and any $\ve>0$. If the triplet of parameters $s=(\alpha, \ve, \delta)$ is a well chosen then 
\begin{enumerate}
\item Defining $\tau$ by $\frac 1 \tau := \frac m d+ \frac 1p$ we have %\in (0, \infty)
\be
\label{asymptK}
\lim_{\lambda \to \infty} m(\lambda^2 H)^\frac m d e_{\lambda^2 H}(f)_p \leq C\|K(d^m f)\|_{L^\tau([0,1]^d)}+\ve.
\ee
\item Defining $\tau$ by $\frac 1 \tau := \frac {m-1} d+ \frac 1p$ we have
$$
\lim_{\lambda \to \infty} m(\lambda^2 H_a)^\frac {m-1} d e_{\lambda^2 H_a}^a(\nabla f)_p \leq C\|L_a(d^m f)\|_{L^\tau([0,1]^d)}+\ve
$$
and
$$
\lim_{\lambda \to \infty} m(\lambda^2 H_g)^\frac {m-1} d e_{\lambda^2 H_g}^g(f)_p \leq C\|L_g(d^m f)\|_{L^\tau([0,1]^d)}+\ve.
$$
\end{enumerate}
\end{theorem}

The proof of the three estimates are completely similar. We therefore focus on the proof of \iref{asymptK}, and the details of the two other estimates are left to the reader.
We identify the polynomial $\pi_z$ with the collection $d^m f(z)/m!$ of $m$-th order derivatives of $f$, and we observe that 
\begin{eqnarray*}
\|\det(\cM^{(\alpha)}(d^m f))^\frac m {2d}\|_{L^\tau([0,1]^d)} &=& \|K^{(\alpha)}(d^m f)\|_{L^\tau([0,1]^d)}\\ 
&\underset {\alpha\to \infty} \longrightarrow &\|K^\sC(d^m f)\|_{L^\tau([0,1])}\\
&\leq & C_K \|K(d^m f)\|_{L^\tau([0,1])}
\end{eqnarray*}
where the constant $C_K$ is defined in \iref{defCKAG}.
In the second line we used the fact that $K^{(\alpha)}(d^m f)$ converges pointwise \emph{decreasingly} to $K^\sC(d^m f)$, which implies the convergence of the integrals.
We may therefore choose $\alpha$ sufficiently large and $\ve$ sufficiently small such that 
$$
\|(\det M)^\frac m {2d}\|_{L^\tau([0,1]^d)} < C \|K(d^m f)\|_{L^\tau([0,1])} + \ve,
$$
where $C=C_K/m!$ (recall that $\cM^{(\alpha)}$ and $K^{(\alpha)}$ are homogeneous functions, as observed in Remark \ref{remHomog2}).

For each $z\in \R^d$ such that $\pi_z\neq 0$ we have 
\begin{eqnarray*}
\|\pi_z\circ M(z)^{-\frac 1 2}\| &=& \sup_{|u|=1} \frac{|\pi_z(u)|}{\|u\|_{M(z)}^m}\\
&=& \sup_{|u|=1} \frac {|\pi_z(u)|}{(\|u\|^2_{\cM(\pi_z)} +\ve)^\frac m 2}\\
&<& \sup_{|u|=1} \frac {|\pi_z(u)|}{\|u\|_{\cM(\pi_z)}^m}\\
&=& \|\pi_z\circ \cM(\pi_z)^{-\frac 1 2}\| \\
&\leq& 1.
\end{eqnarray*}
We may therefore choose $\delta>0$ sufficiently small in such way that 
$
\|\pi_z\circ M'(z)^{-\frac 1 2}\| <1
$
for all $z\in [0,1]^d$ %, hence for all $z\in \R^d$ since $f$ is periodic, 
and such that 
\be
\label{eqMK}
\|(\det M'(z))^\frac m {2d}\|_{L^\tau([0,1]^d)} < C \|K(d^m f)\|_{L^\tau([0,1])} + \ve.
\ee
Note that according to \iref{defHs}
$$
m(H)^\frac 1 \tau =\|(\det M'(z))^\frac m {2d}\|_{L^\tau([0,1]^d)}.
$$
We define for each $z\in \R^d$
\be
\label{defMuzLpMet}
\mu_z := \sum_{|\alpha| < m} \frac{\partial^{|\alpha|} f(z)}{(\partial z)^\alpha} \frac{Z^\alpha} {\alpha!}.
\ee
and for each $\lambda>0$
$$
f_{z,\lambda}(h) := \lambda^d(f(z+h/\lambda) - \mu_z(h/\lambda)).
$$
Defining the ellipse $\cE_z := \{u \sep \|u\|_{H(z)}\leq 1\}$, and using the isotropic change of variables $h \mapsto z+h/\lambda$, we obtain
$$
e_{\lambda^2 H} (f \sep z)_p = \inf_{\mu\in \sP_{m-1}} \|f - \mu\|_{L^p(B_H(z,1/\lambda))}=  \lambda^{-(m+\frac d p)}\inf_{\mu\in \sP_{m-1}} \|f_{z,\lambda} - \mu\|_{L^p(\cE_z)}.
$$
The function $f_{z,\lambda}$ converges uniformly to $\pi_z$ : 
\be
\label{eqConvfPi}
\lim_{\lambda\to \infty}\|f_{z,\lambda} -\pi_z\|_{L^\infty(B(0,1))} = 0,
\ee
since $\pi_z$ is the $m$-term in the Taylor development of $f$ at $z$. Since $\cE_z \subset B(0,1)$ we therefore obtain  
\begin{eqnarray*}
\lim_{\lambda \to \infty}  \lambda^{m+\frac d p}e_{\lambda^2 H} (f \sep z)_p &=& 
\lim_{\lambda\to \infty}  \lambda^{m+\frac d p} \inf_{\mu\in \sP_{m-1}} \|f_{z,\lambda} - \mu\|_{L^p(\cE_z)}\\
&=&\inf_{\mu\in \sP_{m-1}} \|\pi_z - \mu\|_{L^p(\cE_z)}\\
& \leq & \|\pi_z\|_{L^p(\cE_z)}\\
& \leq & |\cE_z|^\frac 1 p \|\pi_z\|_{L^\infty(\cE_z)}\\
&=& \omega \, (\det H(z))^{-\frac 1 {2p}} \|\pi_z \circ H(z)^{-\frac 1 2}\|\\
&=& \omega \|\pi_z \circ M(z)^{-\frac 1 2}\|\\
& \leq & \omega,
\end{eqnarray*}
where $\omega := |B(0,1)|$ denotes the volume of the unit euclidean ball. We used in the third line the proportionality relation $H(z)= (\det M(z))^{-\frac 1 {mp+d}}M(z)$ and the  fact that $\pi_z$ is homogeneous of degree $m$, which imply 
$$
\det H(z) = \det M(z)^{\frac {mp}{mp+d}} \stext{ and } \|\pi_z \circ H(z)^{-\frac 1 2}\| = (\det M(z))^{\frac m{2(mp+d)}}\|\pi_z \circ M(z)^{-\frac 1 2}\|.
$$

The convergence \iref{eqConvfPi} is uniform over all $z\in [0,1]^d$, and therefore 
\begin{eqnarray*}
\lim_{\lambda \to \infty} \lambda^{mp} e_{\lambda^2 H} (f)_p^p &=& \lim_{\lambda \to \infty} \lambda^{mp+d} \int_{[0,1]^d} \sqrt{\det (\lambda^2 H(z))}  e_{\lambda^2 H}(f\sep z)_p^p dz\\
&=& \int_{[0,1]^d} \sqrt{\det  H(z)}  \left( \lim_{\lambda \to \infty} \lambda^{mp+d} e_{\lambda^2 H}(f\sep z)_p^p\right) dz\\
& \leq &\omega^p \int_{[0,1]^d} \sqrt{\det H(z)}   dz.\\
&=&\omega^p m(H).
\end{eqnarray*}
Since $m(\lambda^2 H) = \lambda^d m(H)$ we therefore obtain injecting \iref{eqMK}
\begin{eqnarray*}
\lim_{\lambda \to \infty} m(\lambda^2 H)^\frac m d e_{\lambda^2 H}(f)_p & \leq & \omega \, m(H)^{\frac m d+ \frac 1 p}\\
& = & 
C\|K(d^m f)\|_{L^\tau([0,1]^d)}+\ve,
\end{eqnarray*}
which concludes the proof.




\subsection{The shape function is equivalent to a continuous function}

The shape functions $K$, $L_a$ and $L_g$ are defined in \S\ref{subsecIntroAsympt} by an infimum, which may or may not be attained, over the collection $\SL_d$ of all matrices of unit determinant. 
One can infer from this property that the shape functions are upper-semi continuous, but they are not continuous in general as illustrated in Remark \ref{overfitting} (in Chapter 2) for the shape function $K$ when $m=4$ and $d=2$.

The purpose of this subsection is to establish the following theorem, which states that the shape functions are nevertheless uniformly equivalent to a continuous function on $\H_m$.

\begin{theorem}
\label{thContShape}
There exists a constant $C=C(m,d)$ and three continuous functions $K^c$, $L^c_a$ and $L^c_g$ on $\H_m$ such that for all $\pi \in \H_m$
$$
\begin{array}{ccccc}
C^{-1} K^c(\pi) &\leq& K(\pi) &\leq& C K^c(\pi)\\
C^{-1} L^c_a(\pi) &\leq& L_a(\pi) &\leq& C L^c_a(\pi)\\
C^{-1} L^c_g(\pi) &\leq& L_g(\pi) &\leq& C L^c_g(\pi).
\end{array}
$$
\end{theorem}

Note that in the case of the shape functions $K$ and $L_a$, in dimension $d=2$, this theorem is a consequence of the explicit algebraic equivalents of these shape functions given in Chapters 2 and 3.

The analysis presented below applies to all three shape functions, without restriction on the dimension $d$.
As observed in \S \ref{subsecWellPosed} the shape functions $L_a$ and $L_g$ are uniformly equivalent on $\H_m$ to the following functions respectively, defined for all $\pi\in \H_m$ by
\begin{eqnarray}
L_a^*(\pi) &:=& \inf_{A\in \SL_d} \sqrt{\|G(\pi)\circ A\|}\\
\label{defLGS}
L_g^*(\pi) &:=& \inf_{A\in \SL_d} \|A^{-1}\| \|\pi\circ A\|,
\end{eqnarray}
where $G(\pi) := |\nabla \pi|^2 \in \H_{2m-2}$. Let us also recall that 
\be
\label{defKCont}
K(\pi) := \inf_{A\in \SL_d} \|\pi\circ A\|.\\
\ee
The fact that $L_a^*$ is uniformly equivalent to a continuous function therefore directly follows from the same property for the shape function $K$ (in degree $2m-2$ instead of $m$), by composition with the continuous functions $G : \H_m \to \H_{2m-2}$ and $\sqrt{\cdot} : \R_+ \to \R_+$.


The next lemma gives a criterion on the lower semi-continuous envelope of a function, which guarantees that this function is equivalent to a continuous function. %Note that the shape functions $K$ and $L_g^*$ are upper semi-continuous, since they are defined as the infimum of a family of continuous functions. 
\begin{lemma}
\label{lemmaToCont}
Let $(X,d_X)$ be an arbitrary metric space, and let $f : X \to \R_+$. We define the lower semi continuous envelope $\underline f$ of $f$ as follows : for all $x\in X$
$$
\underline f(x) := \lim_{\ve \to 0} \inf_{y\in B(x,\ve)} f(y).
$$
Assume that $f$ is upper semi-continuous and that there exists a constant $C$ such that 
\be
\label{eqffLow}
f(x) < C \underline f(x) \stext{ or } f(x) = 0
\ee
for all $x\in X$. Then there exists a continuous function $f^c \in C^0(X,\R_+)$ such that 
\be
\label{eqffc}
C^{-1} f^c \leq f \leq C f^c.
\ee
\end{lemma}

\proof
For each $n\in \Z$ we define the set 
\be
\label{defEn}
E_n := \{x\in X \sep f(x) \geq C^n\},
\ee
which is closed since $f$ is upper semi-continuous. 
For any $x\in \overline{X\sm E_n}$ there exists a sequence $(x_k)_{n\geq 0}$, $x_k\in X\sm E_n$ (hence $f(x_k) < C$), converging to $x$. Therefore
$$
\underline f(x)\leq \liminf_{k \to \infty} f(x_k)\leq C.
$$
Combining this with \iref{eqffLow} we obtain that $x\notin E_{n+1}$, hence the sets $E_{n+1}$ and $\overline{X\sm E_n}$ are disjoint.
We denote by $(r_n)_{n \in \Z}$,  $r_n\in C^0(X, [0,1])$, a family of continuous functions such that
$$
r_{n|E_{n+1}} = 1\stext{ and } r_{n|\overline{X\sm E_n}} = 0.
$$ 
The simplest construction of such functions is the following:
$$
r_n(x) := \frac{d_X(x, X \sm E_n)}{d_X(x, X\sm E_n)+ d_X(x,E_{n+1})},
$$
where 
$d_X(x,E) := \inf \{d_X(x,e)\sep e\in E\}$.
We define a function $r : X \to [-\infty, \infty)$ (observe that $-\infty$ is included) by the sum
$$
r(x) := \sum_{n <0} (r_n(x)-1) + \sum_{n \geq 0} r_n(x).
$$
For each $n\in \Z$ the function $r$ is equal to $n+r_n+r_{n+1}$ on the open set $\interior(E_n\sm E_{n+2})$. Therefore $r$ is continuous on the reunion
$$
\bigcup_{n \in \Z} \interior(E_n\sm E_{n+2}) \supset \bigcup_{n \in \Z} E_{n+1}\sm E_{n+2} = \{x\in X\sep f(x) >0\}.
$$
Consider $x\in X$ such that $f(x) = 0$, hence $r(x) = -\infty$. Since $f$ is upper semi-continuous there exists for each $n\in \Z$ a constant $\delta>0$ such that $f < C^n$ on $B(x,\delta)$. It follows that $r\leq n$ on $B(x,\delta)$, hence that $r$ is continuous at $x$. 

The function $r$ is therefore continuous on the whole space $X$, hence the function $f^c : X \to \R_+$ defined by 
$$
f^c(x) := C^{\,r(x)},
$$
is also continuous. We have $f^c(x) = 0$ if and only if $r(x)=-\infty$, which implies $f(x) = 0$.
Furthermore for each $n\in \Z$ and each $x\in E_n\sm E_{n+1}$ we have $C^n \leq f(x) < C^{n+1}$ and $C^n \leq f^c(x) \leq C^{n+1}$ by construction, which establishes \iref{eqffc} and concludes the proof of this lemma.
\sq



The proofs that the functions $K$ and $L_g^*$ are uniformly equivalent on $\H_m$ to a continuous function are extremely similar. The case of $L_g^*$ is nevertheless slightly more involved due to the term $\|A^{-1}\|$ appearing in \iref{defLGS} which is not present in \iref{defKCont}. We therefore focus our attention on this function, and we leave to the reader the details of the adaptation of the proof to the shape function $K$.


We define an auxiliary function $\gL$ on $M_d \times \H_m$ as follows : for all $(B, \pi)\in M_d\times \H_m$
\be
\label{defgL}
\gL(B,\pi) := \inf_{A\in \SL_d} \|A^{-1}B\| \|\pi\circ A\|,
\ee
hence $\gL(\Id, \pi) = L_g(\pi)$ for all $\pi \in \H_m$.

The function $\gL$ is upper semi continuous since it is defined as the infimum of a family of continuous functions. Hence for any converging sequence $(B_n, \pi_n) \to (B,\pi)$ in $M_d \times \H_m$ we have 
$$
\gL(B, \pi) \geq \limsup_{n \to \infty} \gL(B_n, \pi_n).
$$
The next lemma shows that this inequality becomes an equality if the limit is zero.
\begin{lemma}
\label{lemmaVanishGL}
For any converging sequence $(B_n, \pi_n) \to (B,\pi)$ in $M_d \times \H_m$ the following holds:
$$
\text{ if } \lim_{n \to \infty} \gL(B_n, \pi_n)=0 \stext{ then } \gL(B, \pi) = 0.
$$
\end{lemma}

\proof
If $\gL(B_n, \pi_n) \to 0$ then there exists a sequence $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, such that 
\be
\label{eqAnBnPin}
\lim_{n \to \infty} \|A_n^{-1} B_n\| \|\pi_n\circ A_n\| =0.
\ee
For each $n$ we consider the principal value decomposition $A_n = U_n D_n V_n$, where $U_n, V_n \in \cO_d$ and $D_n$ is a diagonal matrix satisfying $\det D_n = 1$, with positive %and decreasing 
diagonal coefficients $t_n = (t_{n,1}, \cdots, t_{n,d})$. 
% where 
%\be
%\label{eqtni}
%t_{n,1} \geq \cdots \geq t_{n,d}>0.
%\ee
We have for any $n \geq 0$, since $V_n$ is orthogonal,
\begin{eqnarray*}
\|A_n^{-1} B_n \| \|\pi\circ A_n\| &=& \| V_n^\trans D_n^{-1} U_n^\trans B_n \| \|\pi\circ (U_n D_n V_n)\|\\
&=& \|D_n^{-1} U_n^\trans B_n \| \|\pi\circ (U_n D_n)\|.
\end{eqnarray*}
Since the collection $\cO_d$ of orthogonal matrices is compact, the sequence of orthogonal matrices $U_n$ admits a converging sub-sequence $U_{\vp(n)} \to U$. We define $B' := U^\trans B$, $\pi' := \pi \circ U$, and we observe that since $|\det U| = 1$
\be
\label{eqgLBPip}
\cL(B, \pi) = \cL(B', \pi').
\ee
We also define for each $n$
$$
B'_n := U_{\vp(n)}^\trans B_{\vp(n)}, \quad  \pi'_n := \pi_{\vp(n)} \circ U_{\vp(n)}, \stext{ and } D'_n := D_{\vp(n)}
$$
in such way that 
\be
\label{eqBpPip}
\lim_{n \to \infty} (B'_n,\pi'_n) = (B',\pi') \stext{ and } \lim_{n \to \infty} \|D'^{-1}_n B'_n\| \|\pi'_n\circ D'_n\| = 0.
\ee
We thus recognize our starting point \iref{eqAnBnPin} except that the matrices $A_n$ are replaced with diagonal matrices $D'_n$, of coefficients 
$$
t'_n := (t'_{n,1}, \cdots , t'_{n,d}) =  (t_{\vp(n),1}, \cdots , t_{\vp(n),d}).
$$
In order to avoid notational clutter we do not keep track of the sub-sequence extraction, and until the end of this proof we write $\pi$, $\pi_n$, $B$, $B_n$, $D_n$, $t_n$ and $t_{n,i}$ for the variables $\pi'$, $\pi_n'$, $B'$, $B_n'$, $D'_n$, $t_n'$ and $t_{n,i}'$.

We denote by $I\subset \{1, \cdots, d\}$ the collection of indices $i$ such that the associated line of $B$ is nonzero. There exists a constant $c>0$ such that for %all $n \geq 0$
%$$
%\|D_n B\| \leq C t_{n,i_0}
%$$
%and for 
all $n$ sufficiently large
\be
\label{eqDnB}
\|D_n^{-1} B_n\| \geq c \max_{i\in I} t_{n,i}^{-1}.
\ee
We denote by $\Lambda$ the collection of exponents
$$
\Lambda := \{\alpha\in \Z_+^d \sep |\alpha| \leq m\}
$$
and by $\pi_\alpha$, $\pi_{n,\alpha}$ the coefficients of $\pi$ and $\pi_n$ respectively : 
$$
\pi = \sum_{\alpha \in \Lambda} \pi_\alpha Z^\alpha \stext{ and } \pi_n = \sum_{\alpha\in \Lambda} \pi_{n, \alpha} Z^\alpha.
$$
It follows from \iref{eqBpPip} and \iref{eqDnB} that for any $\alpha\in \Lambda$ we have 
\be
\label{eqTnPin}
\lim_{n \to \infty} \left(\max_{i\in I} t_{n,i}^{-1}\right) \pi_{n, \alpha} t_n^\alpha = 0.
\ee
For each $t = (t_1, \cdots , t_d)\in \R_+^d$ we define 
$$
\Lambda(t) := \left\{\alpha\in \Lambda \sep\left(\max_{i\in I} t_i^{-1}\right) t^{\alpha} \geq 1\right\}.
$$
The set $\Lambda$ has only a finite number of subsets, since it is finite. Hence there exists an extraction $\psi$ such that $\Lambda_* := \Lambda(t_{\psi(n)})$ does not depend on $n$. In view of \iref{eqTnPin} we thus have for all $\alpha\in \Lambda_*$
$$
\pi_\alpha = \lim_{n \to \infty} \pi_{\psi(n), \alpha} = 0. %\text{ for all } \alpha\in \Lambda_*. 
$$
Defining $D := D_{\psi(0)}$, and denoting by $t=(t_1, \cdots ,t_d)$, its diagonal coefficients we thus obtain 
$$
\lim_{n \to \infty} \|D^{-n} B\| \|\pi\circ D^n\| = 0. 
$$
Indeed $\|D^{-n} B\|\leq C \max_{i\in I}t_i^{-n}$ and 
$$
\left( \max_{i\in I}t_i^{-n}\right) \pi_\alpha t^{n\alpha} =  \pi_\alpha \left(t^{\alpha} \max_{i\in I}t_i^{-1}\right)^n,
$$
which equals $0$ if $\alpha\in \Lambda_*$, and tends to zero if $\alpha\in \Lambda\sm\Lambda_*$. It follows that $\gL(B,\pi) = 0$ as announced.
\sq

The next lemma compares the function $\gL$ with its lower semi-continuous envelope.
\begin{lemma}
\label{lemmagLLower}
There exists a constant $C$ such that $\gL \leq C \underline \gL$ on $M_d \times \H_m$.
\end{lemma}
\proof
We denote by $\cA$ the following compact subset of $M_d\times \H_m$
$$
\cA := \{(B,\pi) \in M_d \times \H_m \sep \|B\|=\|\pi\| = 1 \text{ and }  \|A^{-1}B\| \|\pi\circ A\|\geq 1 \text{ for all } A\in \SL_d \}.
$$
It follows from the definition \iref{defgL} of $\gL$ that $\gL(B,\pi) = 1$ for all $(B, \pi)\in \cA$. Therefore  $\underline \gL$ does not vanish on $\cA$ according to Lemma \ref{lemmaVanishGL}. Since $\underline \gL$ is lower semi continuous, it attains its minimum on $\cA$, we thus define 
$$
C^{-1} := \inf_\cA \underline \gL.
$$
Let $(B, \pi) \in M_d \times \H_m$, and let $(A_n)_{n \geq 0}$, $A_n \in \SL_d$ be a sequence such that %, a minimizing sequence for the problem defining $\gL(B, \pi)$
\be
\label{eqAngLMin}
\lim_{n \to \infty} \|A_n^{-1} B \| \|\pi \circ A_n\| = \gL(B, \pi) := \inf_{A\in \SL_d} \|A^{-1} B \| \|\pi \circ A\|.
\ee
If $\gL(B, \pi) = 0$, then $\underline \gL(B, \pi)=0$ and there is nothing to prove. If $\gL(B, \pi)>0$, then consider an extraction $\vp$ such that the following quantities converge
$$
\lim_{n \to \infty} \frac{A_{\vp(n)}^{-1} B}{\|A_{\vp(n)}^{-1} B\|} = B_* \stext{ and } \lim_{n \to \infty} \frac{\pi\circ A_{\vp(n)}}{\|\pi\circ A_{\vp(n)}\|} = \pi_*.
$$

We now prove that $(B_*, \pi_*)\in \cA$.
We first remark that $\|B_*\| = \|\pi_*\|=1$ by construction. Assume for contradiction that there exists $A\in \GL_d$ such that $\|A^{-1} B_*\|\|\pi_*\circ A\| = \delta <1$. We obtain 
\begin{eqnarray*}
& &\lim_{n \to \infty}  \|(A_{\vp(n)} A)^{-1} B \| \|\pi \circ (A_{\vp(n)} A)\| \\
&=& \lim_{n \to \infty} \frac {\|A^{-1}(A_{\vp(n)}^{-1} B) \|}{\|A_{\vp(n)}^{-1} B \|} \frac { \|(\pi\circ A_{\vp(n)})\circ A\|}{\|\pi\circ A_{\vp(n)}\|} \|A_{\vp(n)}^{-1} B \| \|\pi\circ A_{\vp(n)}\| \\
&=& \delta \gL(B, \pi)
\end{eqnarray*}
which contradicts the definition \iref{defgL} of $\gL$, hence $(B_*, \pi_*)\in \cA$ as announced.
We thus obtain, since $\underline \gL$ is lower semi continuous, 
$$
\lim_{n \to \infty} \underline \gL\left(\frac{A_n^{-1} B}{\|A_n^{-1} B\|} \frac{\pi\circ A_n}{\|\pi\circ A_n\|}\right) \geq  \underline \gL(B_*, \pi_*) \geq C^{-1}. % := \inf_\cA \underline \gL.
$$
On the other hand we have for each $n\geq 0$
$$
\underline \gL\left(\frac{A_n^{-1} B}{\|A_n^{-1} B\|} \frac{\pi\circ A_n}{\|\pi\circ A_n\|}\right) = \frac{\underline \gL(B,\pi) }{\|A_n^{-1} B\|\|\pi\circ A_n\|}, % \ \underset {n \to \infty}  \longrightarrow \ 
$$
which tends to $\underline \gL(B,\pi)/\gL(B,\pi)$ as $n \to \infty$.
If follows that $\underline \gL(B,\pi) \geq \gL(B, \pi)$, which concludes the proof of this lemma.
\sq

We now conclude the proof that $L_g^*$ is equivalent to a continuous function. % as follows.
Applying Lemma \ref{lemmaToCont} to the function $\gL$ and the constant $C+1$, where $C$ is the constant from Lemma \ref{lemmagLLower} we obtain that that $\gL$ is equivalent to a continuous function on $M_d \times \H_m$. Recalling that $L_g^*(\pi) = \gL(\Id,\pi)$ we obtain that $L_g^*$ is also equivalent to a continuous function, on $\H_m$, which concludes the proof of Theorem \ref{thContShape}.


%\input{../Bibliography/Bibliography.tex}
%\end{document}


==> ApproxTheory/ContK.tex <==

The next proposition is not necessary for our analysis but gives a worthwhile insight of the properties of the shape function $K$. We show in particular that the function $K$, which is only upper semi continuous in general, is equivalent to a continuous function. We deduce a from this point a property of convergence the the functions$K^{(\alpha)}$.

% which converge only pointwise to $K$, satisfy a good substitute 
%
%The convergence of $K^{(\alpha)}$ towards $K_\sC$ is not uniform.
%The next lemma gives a substitute for this uniform convergence.

\begin{prop}
\label{lemmaKAK}
\begin{enumerate}
\item (Vanishing property)
Let $(\pi_n)_{n \geq 0}$, $\pi_n \in \H_m$,  $\pi_n \to \pi$ as $n \to \infty$, be a converging sequence of homogeneous polynomials. 
Let  $(A_n)_{n \geq 0}$, $A_n \in \SL_d$ be a sequence of matrices of unit determinant.

If $\pi_n \circ A_n \to 0$ then there exists $A\in \SL_d$, such that $\pi\circ (A^n) \to 0$.

\item (Equivalence to a lower semi continuous function) We denote by $\underline K_\sC$ the lower semi-continuous envelope of $K_\sC$ : for all $\pi\in \H_m$ 
$$
\underline K_\sC(\pi) := \lim_{\ve \to 0} \inf_{\|\pi-\pi'\|\leq \ve} K_\sC(\pi).
$$
There exists a constant $C_\lsc= C_\lsc(m,d)$ such that $\underline K_\sC \leq K_\sC\leq  C_\lsc \underline K_\sC$ on $\H_m$.

Furthermore there exist a continuous function $K_c$ on $\H_m$ such that $(C_\lsc+1)^{-1}K_c\leq K_\sC\leq (C_\lsc+1) K_c$.

\item (Substitute for uniform convergence)
For all $\ve >0$ there exists $\alpha = \alpha(m,d,\ve)$ such that for all $\pi \in \H_m$
\be
\label{eqKAKU}
K^{(\alpha)}(\pi) \leq C_\lsc \underline K_\sC(\pi)+ \ve \|\pi\|_\sC,
\ee
where $C$ is the constant appearing in 2. In particular 
\be
\label{eqKAK}
K^{(\alpha)}(\pi) \leq n_\sC (C_\lsc  K(\pi)+ \ve \|\pi\|).
\ee
\end{enumerate}
\end{prop}

\proof
\begin{enumerate}
\item
For each $n\geq 0$ we consider the singular value decomposition $A_n = U_n D_n V_n$, where $U_n, V_n \in \cO_d$ and the diagonal matrix $D_n$ has positive coefficients and satisfies $\det D_n = 1$.
Since $V_n$ is orthogonal we have 
$$
\|\pi_n \circ A_n \| = \|\pi_n \circ (U_n D_n V_n)\| = \|\pi_n \circ (U_n D_n)\|.
$$
Since $\cO_d$ is compact the sequence of orthogonal matrices $U_n$ admits a converging sub-sequence $U_{\sigma(n)} \to U$. 
We define $\pi' := \pi\circ U$, $\pi'_n := \pi_{\sigma(n)} \circ U_{\sigma(n)}$ and $D'_n := D_{\sigma(n)}$, in such way that 
$$
\pi'_n \to \pi' \stext{ and } \pi'_n \circ D'_n \to 0.
$$
We recognise the hypotheses of the lemma, except that the matrices $D'_n$ replacing $A_n$ are now diagonal. We show below that there exists a diagonal matrix $D$, $\det D=1$, such that $\pi'\circ (D^n) \to 0$. Defining $A := UDU^\trans$ leads to the announced result $\pi \circ (A^n) \to 0$.

In order to avoid notational clutter we do not keep track of the extraction procedure and we simply write $\pi$, $\pi_n$ and $D_n$ in place for $\pi'$, $\pi'_n$ and $D'_n$.
We define the finite set 
$$
\Lambda := \{\alpha \in \Z_+^d\sep |\alpha| \leq k\},
$$
and to any $t\in (\R_+^*)^d$ we associate a subset $\Lambda(t)\subset \Lambda$
$$
\Lambda(t) := \{\alpha \in \Lambda \sep t^\alpha \geq 1\}.
$$
For each $n$ we denote by $\Lambda_n$ the set $\Lambda(t_n)$ associated to the list $t_n$ of diagonal entries of $D_n$.

There are only a finite number of subsets of $\Lambda$, namely $2^{\#(\Lambda)}$, thus there exists an extraction $\tau$ such that $\Lambda_* := \Lambda_{\tau(n)}$ us independent of $n$.

For any $\alpha\in \Lambda$ we denote by $\pi_{n,\alpha}$ the coefficient of $Z^\alpha$ in $\pi_n$, and by $\pi_\alpha$ the coefficient of $Z^\alpha$ in $\pi$, where $Z=(Z_1, \cdots ,Z_d)$ is the $d$-dimensional variable. 
$$
\pi_n = \sum_{\alpha \in \Lambda} \pi_{n , \alpha} Z^\alpha \stext{ and } \pi = \sum_{\alpha \in \Lambda} \pi_\alpha Z^\alpha.
$$
We recall that $t_n$ denotes the list of coefficients of the diagonal matrix $D_n$, we denote by $t$ the list of coefficients of a diagonal matrix $D$. We thus have 
$$
\pi_n \circ D_n = \sum_{\alpha \in \Lambda} \pi_{n , \alpha} t_n^\alpha Z^\alpha \stext{ and } \pi \circ D^n= \sum_{\alpha \in \Lambda} \pi_\alpha t^{n \alpha} Z^\alpha.
$$
Since $\pi_n \circ D_n \to 0$ we have 
$
\pi_{n ,\alpha} t_n ^\alpha \to 0
$
for any $\alpha \in \Lambda$.
For any $\alpha$ in the subset $\Lambda_*\subset \Lambda$ we obtain recalling that $t_{\tau(n)}^\alpha \geq 1$
$$
\pi_\alpha = \lim_{n \to \infty} \pi_{\tau(n) ,\alpha} = 0.
$$
We now define $D = D_{\tau(0)}$, we denote by $t$ the list of coefficients of $D$,
and we observe that 
$$
\pi \circ D^n \to 0.
$$
Indeed $\pi_\alpha t^{n \alpha} = 0$ for all $\alpha\in \Lambda_*$, and $\pi_\alpha t^{n \alpha} \to 0$ for all $\alpha \notin \Lambda_*$ since $t^\alpha <1$, which concludes the proof of this point.


\item
As a consequence of 1. we obtain the following vanishing property : for any $\pi \in \H_m$, if $\underline K_\sC(\pi) = 0$ then $K_\sC(\pi) = 0$. Indeed if $\underline K_\sC(\pi) = 0$ then there exists a sequence of homogeneous polynomials $\pi_n\to \pi$ such that $K_\sC(\pi_n) \to 0$, and therefore a sequence of matrices $(A_n)_{n \geq 0}$, $A_n \in \SL_d$, such that $\pi_n \circ A_n$. Therefore there exists $A\in \SL_d$ such that $\pi\circ (A^n)\to 0$, which implies that $K_\sC(\pi) = 0$.

%We define $\cS := \{\pi \in \H_m \sep \|\pi\|_\sC = 1\}$ and we consider the closed set 
We consider the compact set 
$$
\cA := \{\pi \in \H_m \sep \|\pi\|_\sC = 1 \text{ and } \|\pi \circ A\|_\sC \geq 1 \text{ for all } A\in \SL_d\}.
$$
For any $\pi \in \cA$ we thus have $K_\sC(\pi) = \|\pi\|_\sC=1$, and therefore $\underline K_\sC(\pi) >0$. 
Since $\cA$ is compact and since $\underline K_\sC$ is lower semi-continuous, the function $\underline K_\sC$ attains its lower bound on $\cA$ and we define
$$
C^{-1}_\lsc := \inf_{\pi \in \cA} \underline K_\sC(\pi).
$$
Let $\pi\in \H_m$, and let $(A_n)_{n \geq 0}$, $A_n\in \SL_d$, be a sequence of matrices satisfying $\|\pi\circ A_n\|_\sC \to K_\sC(\pi)$ as $n \to \infty$. If $K_\sC(\pi) = 0$ then $\underline K_\sC(\pi) = 0$ also according to the first point of this lemma, and there is nothing to prove.
If $K_\sC(\pi) = 0$ then consider an extraction $\vp$ such that we have the convergence 
$$
\frac{\pi \circ A_n}{\|\pi\circ A_n\|_\sC} \to \pi_*.
$$
We now prove that $\pi_*\in \cA$. Indeed $\|\pi_*\|_\sC = 1$ by construction. If, by contradiction, there exists $A\in SL_d$ such that $\|\pi_*\circ A\| = \delta<1$, then we obtain 
$$
K_\sC(\pi) \leq \lim_{n \to \infty} \|\pi \circ (A_n A)\|_\sC = \lim_{n \to \infty} \frac{\|\pi \circ (A_n A)\|_\sC}{\|\pi\circ A_n\|_\sC} \|\pi\circ A_n\|_\sC = \delta K_\sC(\pi)
$$
which is a contradiction, hence $\pi_*\in \cA$ as announced.
We now observe that 
$$
\underline K_\sC \left(\frac{\pi\circ A_n}{\|\pi\circ A_n\|_\sC} \right) = \frac {\underline K_\sC(\pi)}{\|\pi\circ A_n\|_\sC} \underset {n \to \infty} \longrightarrow \frac {\underline K_\sC(\pi)}{K_\sC(\pi)}.
$$
On the other hand, since $\underline K_\sC$ is lower semi continuous and $\pi_*\in \cA$,
$$
\lim_{n \to \infty} \underline K_\sC \left(\frac{\pi\circ A_n}{\|\pi\circ A_n\|_\sC} \right) \geq \underline K_\sC(\pi_*) \geq C_\lsc^{-1}.
$$
Combining the last two equations we obtain as announced $K_\sC(\pi) \leq C_\lsc \underline K_\sC(\pi)$. 

We now construct a continuous function $K_c$ on $\H_m$ which is equivalent to $K_\sC$.
For each $n\in \Z$ we define
$$
E_n := \{\pi\in \H_m \sep K_\sC(\pi) \geq (C_\lsc+1)^n\}.
$$
Note that the closed sets $E_{n+1}$ and $\overline {\H_m \sm E_n}$ are disjoint, since $K_\sC \leq C_\lsc \underline K_\sC \leq C_\lsc (C_\lsc+1)^n$ on the latter. The following functions is thus continuous
$$
r_n(\pi) := \frac{d(\pi, \H_m \sm E_n)}{d(\pi, \H_m \sm E_n)+ d(x,E_{n+1})} \stext{ where } d(\pi,X) := \inf_{\pi'\in X} \|\pi-\pi'\|_\sC.
$$
We define a continuous function $r : \H_m \to [-\infty, \infty)$ (observe that $-\infty$ is included) but the sum
$$
r(\pi) := \sum_{n <0} (r_n(\pi)-1) + \sum_{n \geq 0} r_n(\pi),
$$
which is finite for any $\pi$ such that $K_\sC(\pi)>0$.
Eventually we set 
$$
K_c(\pi) := (C_\lsc+1)^{r(\pi)},
$$
which concludes the proof.

\item
We consider a fixed $\ve>0$ and we recall that $K^{(\alpha)}$ converges pointwise decreasingly to $K_\sC$ as $\alpha\to \infty$. To each $\pi \in \cS := \{\pi \in \H_m \sep \|\pi\|_\sC = 1\}$ we associate $\alpha_\pi\in (0, \infty)$ satisfying 
$$
K^{(\alpha_\pi)}(\pi) < K_\sC(\pi)+ \ve.
$$
In particular $K^{(\alpha_\pi)}(\pi) < C_\lsc \underline K_\sC(\pi)+ \ve$, and since $\underline K_\sC$ is lower continuous the collection $V_\pi$ of all $\pi'\in \cS$ satisfying 
$$
K^{(\alpha_\pi)}(\pi') < C_\lsc \underline K_\sC(\pi')+ \ve
$$
is an open neighborhood of $\pi$ in $\cS$. 

Since $\cS$ is compact there exists a finite subset $\cS_0$ of $\cS$ such that 
$$
\bigcup_{\pi \in \cS_0} V_\pi = \cS. 
$$
Defining $\alpha := \max \{\alpha_\pi \sep \pi \in \cS_0\}$, and recalling that $K^{(\alpha)} \leq K^{(\alpha')}$ if $\alpha \geq \alpha'$, we obtain for all $\pi\in \H_m \sm \{0\}$
$$
K^{(\alpha)}\left(\frac \pi {\|\pi\|_\sC}\right) \leq C_\lsc \underline K_\sC\left(\frac \pi {\|\pi\|_\sC}\right)+ \ve,
$$
which implies \iref{eqKAKU} since $K^{(\alpha)}$ and $\underline K_\sC$ are $1$-homogeneous on $\H_m$.
The inequality \iref{eqKAK} is a direct consequence of \iref{eqKKC}.
\end{enumerate}
\sq


==> Bayesian/BayesianThese.tex <==

This chapter is dedicated to image restoration, adapting the bayesian approach developed in the thesis \cite{LMo}, see also the paper \cite{LMo2}. %[Moisan, Louchet]. 
Our purpose is to explore a variation of this method based on the results presented in the previous chapter \S \ref{chapCartoon}.
Unfortunately, our attempts did not lead to significant results, neither from the theoretical or the numerical point of view. Therefore, please be warned that the discussion throughout this chapter is purely heuristical, and the numerical results are only illustrative (and limited to one dimensional functions, instead of bi-dimensional images). 
Nevertheless, the author invites the interested reader to share the insight he had of the domain of image restoration, and to discover an original attempt to contribute.

In this chapter, an image is a map $a_0 : [0,1]\times [0,1] \to [0,1]$ which is ``sufficiently regular'' in a certain sense.
The author suggests to imagine $a_0$ as a cartoon function, see Definition \ref{defcartoon}.

At the heart of many image processing algorithms, there is a functional $\kappa$, usually non-negative and defined on ``images''. The quantity 
$
\kappa(a_0)
$ 
reflects the the complexity of the image $a_0$. In particular $\kappa(a_0) = 0$ only for very simple (e.g. constant) images, and $\kappa(a_0) = \infty$ generally if $a_0$ is a sample of white noise.

Very often, this functional is the total variation semi-norm $\kappa = \TV$. If $a_0$ is a $C^1$ smooth image, then this quantity is simply
\be
\label{defTVa}
\TV(a_0) := \int_{[0,1]^2} |\nabla a_0|.
\ee
We present in this chapter an image processing technique based instead on the functional $\kappa = D$, which is defined for $C^2$ functions by the formula 
\be
\label{defDa}
D(a_0) := \int_{[0,1]^2} |\det (d^2 a_0)|^{\frac 1 3}.
\ee
This quantity appears in the previous chapter under the form $D(a_0) =  A_2^{\frac 2 3} (a_0)$,
and is only defined when $a_0\in C^2([0,1]^2)$.
However if $a_0$ is a cartoon function, see Definition \ref{defcartoon}, then Theorem \ref{threg} suggests 
that $D(a_0)$ may still have a meaning, possibly of form
\be
\label{eqDCartoona}
D(a_0) \overset ? = \int_{[0,1]^2\sm E}  |\det (d^2 a_0)|^{\frac 1 3} + C \int_E \left|[a_0]\right|^{\frac 2 3} |\kappa|^{\frac 1 3}
\ee
where $E$ is the set of discontinuities of $a_0$, which is a reunion of smooth curves. At each point $s\in E$, the jump of $a_0$ is denoted by $[a_0](s)$ and the curvature of $E$ by $\kappa(s)$. The value of the constant $C$ is not clear, but Proposition \ref{propLowerCPhi} gives a lower bound. \\

Let us assume that our image $a_0$ has been corrupted by some additive white noise $\omega$, and that we only have access to $a$ defined by 
\be
\label{eqCartoonNoise}
a= a_0 + \omega.
\ee

The following method, originally proposed by Tikhonov, see for instance \cite{Ti}, 
uses the functional $\kappa$ to define an image regularization procedure $a\mapsto a^*_\kappa$, in an attempt to eliminate the noise component $\omega$ and recover the original image $a_0$.
The regularization method consists in solving the following optimization problem,
\be
\label{eqTychonov}
a^*_\kappa := \underset {a'} \argmin \(\alpha \|a'-a\|_2^2+ \kappa(a')\).
\ee
where $\alpha$ is a parameter chosen by the user depending on the amount of regularisation desired. The quantity $\alpha \|a'-a\|_2^2+ \kappa(a')$ is often called the ``Tikhonov energy'', and the functionnal $\kappa$ is regarded as a penalty term.

In the case $\kappa = \TV$, the minimisation problem \iref{eqTychonov} can be rigorously formulated, is convex, and efficient numerical algorithms allow to find some approximations of $a^*_{\TV}$. 
From a ``quantitative'' point of view, the method is rather satisfying since $\|a_0-a^*_{\TV}\|_{L^2([0,1]^2)}$ is generally smaller (for a well chosen parameter $\alpha$) than $\|a_0-a\|_{L^2([0,1]^2)}$.
In other words the regularization procedure $a\mapsto a^*_{\TV}$ has partially restored the original image $a_0$ since the quantity $\PSNR_{a_0}$ (Peak Signal to Noise Ratio to $a_0$) has increased, where 
$$
\PSNR_{a_0} (a') := -\frac {20}{\ln 10} \ln\left(\|a'-a_0\|_{L^2([0,1]^2)}\right).
$$
 
Unfortunately, the estimator $a^*_{\TV}$ is generally not very satisfying from a ``qualitative'' point of  view. Indeed, it is usually constant across large regions, delimited by sharp discontinuities, which do not correspond a feature of the original image $a_0$. The human eye is very sensitive to these spurious discontinuities, and this forbids to use directly the regularization method \iref{eqTychonov} in photography.

From our point of view, a good regularization procedure should in contrast posses the two following ``qualitative'' properties, which are apparently antinomic.
\begin{enumerate}[(i)]
\item (Sharp features are preserved.)
The original image $a_0$ may have discontinuities along a collection $E$ of smooth edges, for instance if $a_0$ is a cartoon function. These features play an important role in the analysis of the image by the human eye, and should therefore be preserved. Qualitatively, the regularized image should also have discontinuities close to $E$, or at least very sharp transitions. 

\item (Strong smoothness) %Second order 
The regularized image should look very smooth away from the collection $E$ of discontinuities of the original image $a_0$.
In particular %A basic requirement is that 
the regularized image and its gradient 
should be continuous in these regions.
\end{enumerate}

In order to achieve these requirements, a common approach is to use ``edge adapted techniques''. These procedures work under the assumption that $a_0$ is a cartoon image and attempt to identify the set $E$ of its discontinuities in the noisy image $a$. A separate treatment is then performed for the smooth regions and the edge set. The author does not follow this path in this chapter, and refers the interested reader to \cite{ACDDM}.

On the contrary, the thesis \cite{LMo} shows how to associate to each functional $\kappa$ a regularization procedure 
$$
a \mapsto a_\kappa,
$$
which treats the whole image in a unified way. When $\kappa = \TV$ the theoretical results and numerical illustrations presented in \cite{LMo} seem to confirm that the properties (i) and (ii) are satisfied. 

As shown in the rest of this chapter, this procedure can be adapted to the functional $\kappa = D$. 
Heuristic arguments, and in particular the fact that $D(a_0)$ is finite for any cartoon image $a_0$, suggest that this modified procedure may also posses the properties (i) and (ii). Furthermore a qualitative analysis given in \S\ref{secLike} shows that the functional $D$ corresponds to a prior of ``high smoothness'', compared to $\TV$, which might be appropriate for cartoon images. 

Let us mention that, contrary to the method %of \cite{LMo}
 presented below, the regularization method \iref{eqTychonov} cannot be adapted to the functionnal $\kappa = D$. 
Indeed if $\cT$ is a triangulation of the domain $[0,1]^2$, and if $a'$ is piecewise affine on $\cT$, then $D(a') = 0$ according to \iref{eqDCartoona}. Since piecewise affine functions on triangulations are dense in $L^2$, we obtain 
\be
\label{eqMinZero}
0 = \min_{a'} \(\alpha \|a'-a\|_2^2+ D(a')\).
\ee
and this minimum is not attained. Note also that, contrary to $\TV$, the functional $D$ is non-convex.\\




Using a similar approach, we also develop a regularization and restoration method for piecewise smooth one dimensional functions $f : [0,1]\to [0,1]$.
Classical procedures are based on the total variation 
\be
\label{defTVf}
\TV(f) := \int_{[0,1]} |f'|.
\ee
Instead we explore a procedure based on the quantity
\be
\label{defDf}
D(f) := \int_{[0,1]} \sqrt{|f''|}.
\ee
In the following, it will always be clear wether the functionals $\TV$ and $D$ are applied to an image $a$, or a function $f$.
The quantity $D(f)$ is only defined when $f\in C^2([0,1])$, but the following proposition suggests that, similarly to its bi-dimensional counterpart $D(a_0)$ in \iref{eqDCartoona},  it may be extended to piecewise $C^2$ functions, possibly with the formula
\be
\label{eqDCartoonf}
D(f) \overset ? = \int_{[0,1]\sm E} \sqrt{|f''|} + C \sum_{e\in E} \sqrt{|[f](e)|} 
\ee
where $E$ is the collection of discontinuities of $f$ in $]-1,1[$ and $[f](e)$ is the jump of $f$ at $e\in E$. 
The value of the constant $C$ is not clear. %, but should lie within the bounds \iref{eqBoundCf}.

\begin{prop}
%Let $\cM$ be the following class of mollifiers,
%$$
%\cM := \left\{\vp \in C^2(\R, \R_+) \sep \supp \vp \subset [-1,1] \text{ and } \int_\R \vp = 1\right\}.
%$$
Let $f : [0,1] \to \R$ be piecewise $C^2$.
Let $\vp$ be a $C^2$ mollifier supported in $[-1,1]$, satisfying $\int_\R \vp = 1$ and $\vp(x) = \vp(-x)$ for all $x\in \R$. For all $\delta>0$ let $\vp_\delta := \frac 1 \delta \vp(\frac \cdot \delta)$ 
 and let $f_\delta := f* \vp_\delta$.
Then $f_\delta \in C^2([\delta, 1-\delta])$ and satisfies
$$
\lim_{\delta\to 0} \int_{[\delta, 1-\delta]} \sqrt{|f_\delta ''|} = \int_{]0,1[\sm E} \sqrt{|f''|} + C(\vp) \sum_{e\in E} \sqrt{|[f](e)|}
$$
where $C(\vp) := \int_\R \sqrt{|\vp'|}$. 
%Furthermore
%\be
%\label{eqBoundCf}
%\inf_{\vp\in \cM} C(\vp) = 0 \stext{ and } \sup_{\vp \in \cM} C(\vp) = 2.
%\ee
\end{prop}

\proof
We denote by $0 = e_0<e_1< e_2 < \cdots< e_n = 1$ the points where the function $f$ is not $C^2$, and the extremal points $e_0 = 0$ and $e_n = 1$ of $[0,1]$. % the elements of $E$ in $]0,1[$ : the points where $f$ is not $C^2$. 
The function $f$ can written as the sum 
$$
f=J+A+S
$$
where $J$ (the Jump part) is piecewise constant, and $A$ is continuous and piecewise Affine, 
with respect to the partition $\left(\, ]e_i,e_{i+1}[\,\right)_{0\leq i\leq n-1}$ of the interval $[0,1]$. % (up to the finite set of points $(e_i)_{0\leq i\leq n})$.
The function $S$ is $C^1$ on $]0,1[$, and $S''$ is uniformly bounded. 
Then, on the interval $[\delta, 1-\delta]$, 
$$
f_\delta = f*\vp_\delta = (J+A+S)*\vp_\delta %J*\vp_\delta + A*\vp_\delta+ S*\vp_\delta 
= J_\delta+ A_\delta+ S_\delta.
$$
We now assume that the parameter $\delta$ satisfies
$$
0< \delta <  \min_{0 \leq i \leq n-1} \frac{e_{i+1}-e_i} 2.
$$
For any $0 \leq i \leq n-1$ one has 
%Let us assume that $i\in \{0, \cdots , n-1\}$ and $\delta>0$ are such that  $2\delta <e_{i+1}-e_i$. Then
$$
J_\delta = J, 
\quad 
A_\delta = A
\stext{ and }
S_\delta = f_\delta - A- J,
$$
on the interval $[e_i+\delta,e_{i+1}-\delta]$.
Hence $J_\delta'' = A_\delta'' = 0$, and $S_\delta'' = f_\delta''$ converges uniformly to $f''$ as $\delta \to 0$, on this interval. Therefore 
\be
\label{eqIntSmooth}
\lim_{\delta \to 0} \sum_{0 \leq i \leq n-1} \int_{e_i+\delta}^{e_{i+1}-\delta} \sqrt{|f_\delta''|} = \int_{]0,1[\sm E} \sqrt{|f''|}.
\ee
Furthermore for any $1\leq i\leq n-1$ and any $|x|\leq 1$ one easily checks that 
$$
J_\delta''(e_i+\delta x) = \frac 1 {\delta^2}[f](e_i) \, \vp'(x)
\stext{ and } 
A_\delta''(e_i+\delta x) = \frac 1 \delta [f'](e_i) \, \vp(x)
$$
where
$$
[f](e_i) = \lim_{\ve\to 0} f(e_i+\ve) - f(e_i - \ve) \stext{ and } [f'](e_i) = \lim_{\ve\to 0} f'(e_i+\ve) - f'(e_i-\ve).
$$
On the other hand $S''_\delta(e_i+ \delta x)$ is uniformly bounded. Hence the contribution of $J_\delta''$ is dominant on the intervals $[e_i-\delta, e_i+\delta]$, and we obtain 
\be
\label{eqIntDisc}
\lim_{\delta\to 0} \sum_{1\leq i\leq n-1} \int_{e_i-\delta}^{e_i+\delta} \sqrt{|f_\delta''|} = \sum_{1\leq i \leq n-1} |[f](e_i)| \int_{-1}^1 \sqrt{|\vp'|}.
\ee
Combining \iref{eqIntSmooth} and \iref{eqIntDisc} we conclude the proof of this proposition.
\sq

\section{Likeliness of images}
\label{secLike}

The functionals $\TV$ and $D$ are different ways to measure the complexity (or regularity) of an image $a$ or function $f$. They have different behaviors that we explore here on a few examples.
The results presented in equations \iref{eqComplexfCos}, \iref{eqComplexfStair}, \iref{eqComplexaCos}, \iref{eqComplexaStair} and \iref{eqComplexaFlower} are easily obtained using the explicit expressions of $D$ for cartoon images \iref{eqDCartoona}  and piecewise $C^2$ functions \iref{eqDCartoonf}, and the following expressions of the total variation %(with the same notations)
\begin{eqnarray*}
\TV(a) &=& \int_{[0,1]^2\sm E}  |\nabla a | +  \int_E \left|[a]\right|,\\
\TV(f) &=& \int_{[0,1]\sm E} |f'| + \sum_{e\in E} |[f](e)|.
\end{eqnarray*}
where as before $E$ is the set of discontinuities of $a$ or $f$, and the jump at a point $e\in E$ is denoted by $[a](e)$ or $[f](e)$.

Here and below, the notation $a(\omega) \simeq b(\omega)$ means that there exists a constant $C>0$ such that 
$$
C^{-1} a(\omega)\leq b(\omega)\leq C a(\omega)
$$ 
for all $\omega \in [2, \infty[$.

We review below some examples of one dimensional functions, illustrated on Figure \ref{figTVDf}, and bi-dimensional images, illustrated on Figure \ref{figTVDa}.
For the simple oscillating function $f(x) := \cos(\omega x)$, illustrated on Figure \ref{figTVDf} (left), the two functionals $\TV$ and $D$ behave similarly :
\be
\label{eqComplexfCos}
\TV( \cos(\omega x) ) \simeq \omega \stext{ and } D(\cos(\omega x)) \simeq \omega.
\ee
On the contrary for the function $f(x) := \frac {\lfloor \omega x\rfloor} \omega$, illustrated on Figure \ref{figTVDf} (right), where $\lfloor x \rfloor$ is the integer part of $x$, we have 
\be
\label{eqComplexfStair}
\TV\left(  \frac {\lfloor \omega x\rfloor} \omega \right) \simeq 1 \stext{ and } D\left( \frac {\lfloor \omega x\rfloor} \omega\right) \simeq \sqrt \omega.
\ee
Hence the functionals $\TV$ and $D$ treat discontinuities very differently, and the latter penalizes functions which have the appearance of a staircase, see Figure \ref{figTVDf} (right).

\begin{figure}
\centering
\includegraphics[height=3cm,width=4.5cm]{\pathPic/Bayesien/Sinf.pdf}
\hspace{1cm}
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Stairf.pdf}
\caption{\label{figTVDf} Behavior of the functionals $\TV$ and $D$ on different types of functions.}
\end{figure}

We now explore similar examples among images, which are functions of the bi-dimensional variable $z=(x,y)\in [0,1]^2$. Let us recall that for any $g\in C^2(R_+)$ one has 
$$
\det \left(d^2 g(|z|)\right) = \frac 1 {|z|} g'(z) g''(z).
$$
As a result we find that the two functionals $\TV$ and $D$ behave similarly on the image $a(z) = \cos(\omega |z|)$ illustrated on Figure \ref{figTVDa} (left),
\be
\label{eqComplexaCos}
\TV( \cos(\omega |z|) ) \simeq \omega \stext{ and } D(\cos(\omega |z|)) \simeq \omega.
\ee
For the image defined by $a(z) = \frac {\lfloor \omega |z|\rfloor} \omega$, illustrated on Figure \ref{figTVDa} (center), we obtain using \iref{eqDCartoona} that 
\be
\label{eqComplexaStair}
\TV\left(  \frac {\lfloor \omega |z|\rfloor} \omega \right) \simeq 1 \stext{ and } D\left( \frac {\lfloor \omega |z|\rfloor} \omega\right) \simeq \omega^{\frac 1 3}.
\ee
This shows that the functional $D$, contrary to $\TV$, penalizes images which have the appearance of a staircase.
Eventually we consider the characteristic function $a= \chi_{\Omega_\delta}$ of the set %is the characteristic function the set 
$$
\Omega_\delta := \left\{z=(r\cos \theta, r \sin \theta) \sep 0 \leq \theta \leq \frac \cPi 2, \text{ and } 0 \leq r \leq 1 + \frac 1 \omega \cos(\omega \theta)\right\},
$$
see Figure \ref{figTVDa} (right).
We obtain
\be
\label{eqComplexaFlower}
\TV(\chi_{\Omega_\delta}) \simeq 1 \stext{ and } D(\chi_{\Omega_\delta}) \simeq \omega^{\frac 1 3}.
\ee
This shows that the functional $D$, contrary to $\TV$ penalizes the fact that the curve of discontinuity $\partial\Omega_\delta$ of $a$ strongly oscillates, see Figure \ref{figTVDa} (right). Note that, despite these oscillations, the length of the curve $\partial \Omega_\delta$ remains bounded as $\delta \to \infty$.

The previous examples suggest that the functional $D$ is a measure of complexity, of cartoon images and piecewise constant functions, which gives an more relevant account of the complexity of their discontinuities than the total variation $\TV$. In particular staircasing effects and oscillating curves of discontinuity are penalized.\\

\begin{figure}
\centering
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Sina.pdf}
\hspace{1cm}
\includegraphics[height=4cm,width=4cm]{\pathPic/Bayesien/Staira.pdf}
\hspace{1cm}
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Flowera.pdf}
\caption{\label{figTVDa} Behavior of the functionals $\TV$ and $D$ on different types of images.}
\end{figure}

It would be useful to define, for any measure $\kappa$ of the complexity of images, such as $\TV$ or $D$, 
%one would like to define 
a probability measure $\mu_\kappa$ on the set of of all images such that ``the probability density near an image $a$'' is proportional to 
$$
e^{-\kappa(a)}.
$$
Unfortunately, for reasons which are out of the scope of this thesis, it is generally impossible to do so. 
In order to follow this idea nevertheless, we turn from this point to the discrete setting.


We consider a fixed positive integer $N>0$ which reflects the fineness of discretization, typically $N = 512$. A discretized image  $A$ is simply a $N \times N$ array of grayscale values $A_{i,j} \in [0,1]$, $1\leq i\leq N$, $1\leq j \leq N$ and 
the collection of images is therefore 
$$
\cA := [0,1]^{N \times N}.
$$
The set $\cA$ is canonically equipped with the Lebesgue measure $dA$ of $N\times N$ dimensional volume. 
We associate to any functional $\kappa\in C^0(\cA, \R)$ %which measures the complexity of discrete images, 
a probability measure $\mu_\kappa$ on $\cA$ as follows. For any Lebesgue measurable subset $\cB \subset \cA$, we define $\mu_\kappa(\cB)$ by the formula
\be
\label{defMuKappa}
\mu_\kappa(\cB) := \frac 1 {Z_\kappa} \int_\cB e^{-\kappa(A)} dA
\ee
where the constant $Z_\kappa$ is a normalizing factor chosen in such way that $\mu_\kappa(\cA) = 1$. 

If $\kappa \equiv 0$, then $\mu_\kappa$ is the standard Lebesgue measure and a typical element of 
$\cA$ with respect to $\mu_\kappa$ appears as ``noise'' to the human eye.

In contrast, we would like to equip $\cA$ with a probability measure $\nu$ that represents the ``likeliness'' of its elements. 
Ideally imagine a ``random photographer'' travelling the world with a camera taking pictures of $N \times N$ resolution. We would like to define a measure $\nu$ on $\cA$ such that $\nu(\cB)$ for $\cB\subset \cA$ represents the likeliness that the next picture will be in the set $\cB$. 

There is clearly no simple expression for the measure $\nu$. However if a functional $\kappa\in C^0(\cA, \R)$ reflects accurately the complexity of discrete images, then $\mu_\kappa$ can be a good enough replacement for $\nu$.\\

For any discrete image $A\in \cA$, we denote by $\TV(A)$ and $D(A)$ the discretization of the functionals $\TV$ and $D$ using finite differences. They are defined as follows 
\be
\label{eqTVA}
\TV(A) := \frac 1 N\left(\sum_{\substack{1\leq i\leq N-1\\1\leq j \leq N}} |A_{i,j} - A_{i+1,j}| +  \sum_{\substack{1\leq i\leq N\\1\leq j \leq N-1}} |A_{i,j} - A_{i,j+1}|\right).
\ee
and 
\be
\label{eqDA}
D(A) := \frac 1 {N^2} \sum_{\substack{2\leq i\leq N-1\\ 2\leq j \leq N-1}} |d_{i,j}|^{\frac 1 3},
\ee
where 
$$\frac 1 {N^4} d_{i,j} := (A_{i,j+1}-2A_{i,j}+A_{i,j-1}) (A_{i+1,j}-2A_{i,j}+A_{i-1,j}) - \frac {(A_{i+1,j+1}+A_{i-1,j-1}-A_{i+1,j-1}-A_{i-1,j+1})^2}{16}.
$$
An image randomly drawn from $\cA$ with respect to the measures $\mu_{\TV}$ or $\mu_D$ will not look ``too noisy'' to the human eye. Still, it may contain sharp features since the continuous versions of $\TV$ and $D$ take finite values on cartoon functions.
This point is important because most natural images contain such discontinuities, which correspond to the boundary of the bi-dimensional projection of the photographed objects. % on the photographic captor.
The examples shown in the beginning of this section suggest that a random draft from $\cA$ with respect to the probability $\mu_D$ will generally look ``smoother'' to the eye in general than a random draft with respect to $\mu_{\TV}$.\\

Similarly, we also consider discrete functions $F$, which are arrays of $N$ values $F_i\in [0,1]$, $1\leq i\leq N$. The collection of discrete functions is therefore
$$
\cF = [0,1]^N.
$$
For any discrete function $F\in F$, we denote by $\TV(F)$ and $D(F)$ the discretization of the functionals $\TV$ and $D$ using finite differences, which are defined as follows 
\be
\label{eqTVF}
\TV(F) := \sum_{1\leq i\leq N-1} |F_i - F_{i+1}|.
\ee
and 
\be
\label{eqDF}
D(F) := \frac 1 N \sum_{2\leq i\leq N-1} \sqrt{|d_i|},
\ee
where 
$$
\frac 1 {N^2} d_i := F_{i+1} - 2 F_i+ F_{i-1}.
$$

\section{A bayesian approach to image denoising} 

We consider a random variable $A\in \R^{N \times N}$ equal to the sum 
$$
A = A_0+ \Omega,
$$
where 
\begin{itemize}
\item $A_0\in \cA$ is a discrete image drawn randomly with respect to the probability measure $\mu_\kappa$ associated to a complexity measure $\kappa$.
\item $\Omega\in \R^{N\times N}$ is some gaussian noise, drawn randomly with respect to the probability measure 
\be
\label{eqDistGaussian}
\frac 1 {Z_\alpha} e^{- \alpha \|\Omega\|^2_2} d\Omega
\ee
on $\R^{N \times N}$, where $\alpha>0$ and $Z_\alpha$ is a normalizing factor.
\end{itemize}


We denote by $p(A)$ (resp. $p(A_0)$) the density of probability of the random variable $A$ (resp.  $A_0$) on $\R^{N\times N}$. We denote by $p(A | A_0)$ and $p(A_0 | A)$ the conditional density of probability of the random variable $A$ given a fixed $A_0$ (resp. $A_0$ given a fixed $A$).

It follows from \iref{defMuKappa} and \iref{eqDistGaussian} that 
$$
p(A_0) = \frac 1 {Z_\kappa} e^{-\kappa(A_0)} \stext{ and } p(A|A_0) = \frac 1 {Z_\alpha} e^{-\alpha \|A-A_0\|^2_2}.
$$
The bayesian rule of conditional probabilities reads
$$
p(A_0|A) \, p(A) = p(A|A_0) \, p(A_0)
$$
Replacing $p(A|A_0)$ and $p(A_0)$ with their explicit expressions, 
we obtain 
\begin{eqnarray*}
p(A_0|A) &=&  \frac 1 {p(A)} p(A|A_0) \, p(A_0)\\
&=& \frac 1 {p(A)} \left(\frac 1 {Z_\alpha} e^{-\alpha \|A-A_0\|^2_2}\right) \left(\frac 1 {Z_\kappa} e^{-\kappa(A_0)} \right)\\
&=& \frac 1 {p(A) Z_\alpha Z_\kappa} e^{-\alpha \|A-A_0\|^2_2 - \kappa(A_0)}.
\end{eqnarray*}
We define
$$
\sigma(A_0,A) = \exp( -\alpha \|A-A_0\|^2_2 - \kappa(A_0)).
$$ 
For any fixed $A$, 
the function $\sigma(A_0,A)$ %has an explicit expression and 
is proportional to $p(A_0|A)$ as $A_0$ varies in $\cA$.\\
%up to to the normalizing constant $Z = p(A) Z_\alpha Z_\kappa$.

From a practical point of view, let us assume that Bob receives the data $A\in \R^{N\times N}$ and knows that it is the sum $A=A_0+ \Omega$ of a picture $A_0\in \cA$ produced by Alice, which can be regarded as a random draft in $\cA$ with respect to the probability $\mu_\kappa$, and of some Gaussian noise $\Omega$ following the probability \iref{eqDistGaussian}. 
Then Bob can attempt to recover the original image $A_0$ using the explicit expression $\sigma(A_0,A)$ of the conditional probability $p(A_0|A)$. 
For instance, Bob can use one of the two following estimators $A_\kappa$ and $A_\kappa^*$ of the original image  $A_0$.

The first estimator $A_k^*$ of $A_0$ is the maximizer of $\sigma(\cdot , A)$,
\begin{eqnarray*}
A^*_\kappa &:=& \underset {A' \in \cA} \argmax \, \sigma (A',A), \\
&= &\underset {A_* \in \cA} \argmin \ \alpha \|A-A'\|^2_2 + \kappa(A').
\end{eqnarray*}
Knowing $A$, the estimator $A_\kappa^*$ is the most probable value of the original image $A_0$. This approach is called the ``Maximum a posteriori'', and abbreviated as ``MAP''. It is clearly equivalent to minimization of the Tikhonov energy, see \iref{eqTychonov}. As exposed in the introduction, the estimator $A_{\TV}^*$ can be efficiently computed but is not satisfying qualitatively. The estimator $A_D^*$ is hard to compute numerically since the functional $D$ is non-convex, and the heuristic analysis \iref{eqMinZero} suggests that it is not relevant.

These points lead us to define another estimator $A_\kappa$ of $A_0$, which is defined as follows.
\begin{eqnarray}
\label{eqMMSE} 
\vspace{5mm}
A_\kappa &:=& \underset {A''\in \cA} \argmin \int_\cA \|A''-A'\|^2 \, \sigma (A',A) \, dA',\\
\label{eqMoySigma}
&=& \frac 1 {Z} \int_\cA A' \, \sigma(A',A) \, dA'. \end{eqnarray}
where 
$
Z = \int_\cA \sigma(A', A) \, dA' 
$ 
 is a normalizing factor.
Knowing $A$, the estimator $A_\kappa$ minimizes the empirical quadratic risk, in other words the quadratic error to $\|A_\kappa-A_0\|^2$, averaged with respect to the probability density $A_0 \mapsto p(A_0|A)$. This approach is called the ``Minimum mean square error'', and abbreviated as ``MMSE''. 
The estimator $A_{\TV}$ is extensively studied in \cite{LMo}, 
in particular it is proved that almost surely the values $(A_{\TV})_{i,j}$ are pairwise distinct. This must be contrasted with the estimator $A_{\TV}^*$ which is often constant over large regions, delimited by undesirable sharp discontinuities.
The thesis \cite{LMo} also describes an algorithm for computing the average \iref{eqMoySigma} defining $A_{\TV}$. We present this algorithm in the next section and adapt it to the computation of $A_D$.

\section{The algorithm}

The computation of the estimator $A_\kappa$ is a numerical challenge, since it involves an integration \iref{eqMoySigma} on the space $\cA = [0,1]^{N \times N}$ which has dimension $N \times N \simeq 250000$ in the (conservative) case $N = 512$.
We have used an algorithm which was first proposed in the thesis \cite{LMo}. We shall only sum up its main ideas and we refer to the original thesis for more details. 

The central point is to define a Markov chain $(A_k)_{k\geq 0}$ on $\cA$ which is recurrent with respect to the probability measure $\sigma(A',A) dA'/Z$, where $A$ is the image to regularize  and $Z$ is a normalizing factor.
Then, almost surely,
\be
\label{eqConAvg}
\lim_{K\to \infty} \frac 1 K \sum_{0\leq k \leq K-1} A_k = \frac 1 Z \int_\cA A' \, \sigma(A',A) \, dA'.
\ee
Two successive images $A_k$ and $A_{k+1}$ generated by this algorithm only differ by the value of a single pixel. The cost of a step of the algorithm, generating a new image $A_k$, comes mainly from the computation of 
$$
\frac {\sigma(U)}{\sigma(V)} = \exp\( \|V-A\|^2 - \|U-A\|^2 +\kappa(V) - \kappa(U)\).%density function
$$
where $U$ and $V$ are two elements of $\cA$ which differ at a single position $(i,j)$. 
If the functional $\kappa$ is $\TV$ or $D$, then the difference $\kappa(V) - \kappa(U)$, as well as $\|V-A\|^2 - \|U-A\|^2$, can be computed from the values of $U$ and $V$ at the positions $(i+k, j+l)$ where $\max\{|k|, |l|\} \leq 2$. The fact that this computation is extremely cheap in terms of computer run time is a key point of the algorithm.

From a theoretical point of view, the averaging procedure \iref{eqConAvg} converges at the speed $\cO(K^{-\frac 1 2})$ or $C K^{-\frac 1 2}$. 
Unfortunately the constant $C$ plays a key role in practice, and we did not manage to ``reach the convergence'' for realistic $512 \times 512$ images with $\kappa = D$. We thus only present one-dimensional results.  

\section{Numerical results and interpretation (1d)}

We present and discuss in this section some one-dimensional numerical results. 
Given $F\in \R^N$, a ``discrete function'', three different regularizations of $F$ are computed.
\begin{eqnarray*}
F_{\TV}^* &:= & \underset {F'\in \R^N} \argmin \ \alpha_1 \|F-F'\|^2+ \TV(F')\\
F_{\TV} &:= & \frac 1 {Z_2} \int_{\R^N} F' e^{-\alpha_2 \|F-F'\|^2 - \beta_2 \TV(F') }dF'\\
F_{D} &:= & \frac 1 {Z_3} \int_{\R^N} F' e^{-\alpha_3 \|F-F'\|^2 - \beta_3 D(F') }dF',\\
\end{eqnarray*}
where $Z_2$ and $Z_3$ are normalizing coefficients. The parameters $\alpha_1, \alpha_2, \alpha_3$ and $\beta_2, \beta_3$ can be freely chosen.

We have not attempted to denoise some data and to compare the $\PSNR$ of the restoration by the different methods.  Indeed such a comparison should, in order to be fair, involve an in depth analysis of the role of the parameters $\alpha_1, \alpha_2, \alpha_3$ and $\beta_2, \beta_3$, that we did not have the time to do. Note also that $F_{\TV}^*$ involves a single parameter, while two parameters are needed for $F_{\TV}$ and $F_D$. We refer to the thesis \cite{LMo} for the comparison of $F_{\TV}^*$ and $F_{\TV}$ from the point of view of the $\PSNR$.

Instead we regard the three procedures as regularization methods, that we apply to different test functions.
We focus on the qualitative differences of the regularizations $F_{\TV}$, $F_{\TV}$ and $F_D$ of different functions $F$, and we discuss on how these differences traduce the different priors implicit in the three methods. \\

\begin{figure}
	\centering
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/Noise.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/NoiseTVMap.pdf}\vspace{0.5cm}\\
	
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/NoiseTV.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/NoiseD.pdf}
	\caption{\label{figRandomWalk}Regularization of a random walk. (Top, Left) Original $F$, (Top, Right) $F^*_{\TV}$, (Bottom,Left) $F_{\TV}$, (Bottom, Right) $F_D$.}
\end{figure}

Our first experiment, see Figure \ref{figRandomWalk}, is the regularization of a random walk. As remarked in \cite{LMo}, $F_{\TV}^*$ is constant over large intervals and also has several sharp discontinuities. These two types of features were not present in the original function $F$ and are undesirable. They are avoided in the two other regularizations $F_{\TV}$ and $F_D$. \\%Qualitatively, $F_{\TV}$ and $F_D$ are not significantly different.

\begin{figure}
	\centering
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/Step.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/StepTVMap.pdf}\vspace{0.5cm}\\
	
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/StepTV.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/StepD.pdf}
	\caption{\label{figHeaviside}Heaviside function. (Top, Left) Original $F$, (Top, Right) $F^*_{\TV}$, (Bottom,Left) $F_{\TV}$, (Bottom, Right) $F_D$.}
\end{figure}

Our second experiment, see Figure \ref{figHeaviside} is the regularization of a Heaviside function. Up to numerical artifacts, the functions $F$ and $F_{\TV}^*$ are identical, which is precisely what is wanted in this situation.
The discontinuity disappears in $F_{\TV}$ and $F_D$, and is replaced with a smooth but sharp and well localized transition. Numerical experiments on real (bidimensional) images in \cite{LMo} show that generally, and with appropriate parameters, the regularization $a_{\TV}$ of an image $a$ does not cause a perceptible blurring of the discontinuities along edges which appear in the original image. 

This example puts in light a strong flaw of the regularization method $F_D$ : it does not obey the maximum principle. Indeed, it is clear on Figure \ref{figHeaviside} that $F_{\TV}^*$ and $F_{\TV}$ take their values in the interval $[\min F, \max F]$, but $F_D$ does not.\\


\begin{figure}
	\centering
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/Churp.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/ChurpTVMap.pdf}\vspace{0.5cm}\\
	
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/ChurpTV.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/ChurpD.pdf}
	\caption{\label{figChurp}Churp : $\sin(x^3)$ where $x\in [0,4]$. (Top, Left) Original $F$, (Top, Right) $F^*_{\TV}$, (Bottom,Left) $F_{\TV}$, (Bottom, Right) $F_D$.}
\end{figure}

Our third and last experiment, see Figure \ref{figChurp} is the regularization of a ``Churp'' : an oscillating function of increasing frequency, here $\sin (x^3)$ where $x\in [0,4]$.
Qualitatively, most regularization algorithms regard slow oscillations as valuable data which should be preserved, and fast oscillations as noise which should be eliminated. The regularization of a churp allows to analyse the behavior of a regularization algorithm in the intermediate regimes.

From a qualitative point of view, the MAP regularization $F_{\TV}^*$ again introduces undesirable visual artefacts : $F_{\TV}^*$ is exactly constant on some regions, and $\nabla F_{\TV}^*$ has sharp discontinuities which do not correspond to a feature of the original function. In contrast the MMSE regularizations $F_{\TV}$ and $F_D$ do not exhibit these artefacts. As anticipated, the slow oscillations of the original function $F$ are preserved, while the fast oscillations are attenuated. It seems qualitatively that fast oscillations are more strongly attenuated in $F_D$ than in $F_{\TV}$. The author could not prove this last property, but a heuristical analysis suggests that sinuosidal oscillations of large frequency $\omega\gg 1$ are attenuated by a factor $\omega^2$ in $F_{\TV}$ and $\omega^4$ in $F_D$.



==> Bibliography/BibliographyOld.tex <==
%--------------------------------------------
% Bibliographie en ordre non alphabetique
%--------------------------------------------


\begin{thebibliography}{99}

%---------------------------------------------
% Bibliographie Issue de OptAniso
%---------------------------------------------

 
\bibitem{Ap} T. Apel, {\it Anisotropic finite elements: Local estimates and applications}, Advances
in Numerical Mathematics, Teubner, Stuttgart, 1999.

\bibitem{BBLS} V. Babenko, Y. Babenko, A. Ligun and A. Shumeiko,
{\it On Asymptotical
Behavior of the Optimal Linear Spline Interpolation Error of $C^2$
Functions}, East J. Approx. 12(1), 71--101, 2006.

%\bibitem{B} Yuliya Babenko,  {\it Asymptotically Optimal Triangulations and Exact Asymptotics for the Optimal $L^2$-Error for Linear Spline Interpolation of $C^2$ Functions}, submitted. 

\bibitem{B} Yuliya Babenko, V. Babenko, A. Ligun, A. Shumeiko, {\it On asymptotical behavior of the
optimal linear spline interpolation error of $C^2$ functions}, East Journal on Approx., 12, N.
1 (2006), pp. 71-101.

\bibitem{Bochner} M. Bocher, {\it Introduction to Higher Algebra}, Courier Dover Publications, 2004
ISBN 0486495701, 9780486495705

\bibitem{Bois} J-D. Boissonnat, C. Wormser and M. Yvinec.
{\it Locally uniform anisotropic meshing},
Proceedings of the twenty-fourth annual symposium on Computational geometry, 2008
%june 2008 (SOCG 2008) 

\bibitem{Peyre} Sebastien Bougleux and Gabriel Peyr\'e and Laurent D. Cohen. {\it Anisotropic Geodesics for Perceptual Grouping and Domain Meshing.} Proc. tenth European Conference on Computer Vision (ECCV'08), Marseille, France, October 12-18, 2008.

\bibitem{A} Y. Bourgault, M. Picasso, F. Alauzet and A. Loseille, {\it On the use of anisotropic a posteriori error estimators for the adaptative solution of 3-D inviscid compressible flows,}  Int. J. Numer. Meth. Fluids., 2009, vol. 59, no. 1, pp. 47-74

\bibitem{C3} W. Cao. {\it An interpolation error estimate on anisotropic meshes in $\R^n$ and optimal metrics for mesh refinement.} SIAM J. Numer. Anal. 45 no. 6, 2368--2391, 2007.

\bibitem{C1} W. Cao, {\it Anisotropic measure of third order derivatives and the quadratic interpolation error on triangular elements}, SIAM J.Sci.Comp. 29(2007), 756-781. 

\bibitem{C2} W. Cao. {\it An interpolation error estimate in $\R^2$ based on the anisotropic measures of higher order derivatives}. Math. Comp. 77, 265-286, 2008.

\bibitem{CSX} L. Chen, P. Sun and J. Xu, {\it Optimal anisotropic meshes for
minimizing interpolation error in $L^p$-norm}, Math. of Comp. 76, 179--204, 2007.

\bibitem{CDHM} A. Cohen, N. Dyn, F. Hecht and J.-M. Mirebeau,
{\it Adaptive multiresolution analysis based on anisotropic triangulations},
preprint, Laboratoire J.-L.Lions, submitted 2008.

\bibitem{dix} J. Dixmier, {\it Quelques aspects de la th\'eorie des invariants}, Gazette des Math\'ematiciens, vol. 43, pp. 39-64, January 1990.

\bibitem{FG} P.J. Frey and P.L. George, {\it Mesh generation. Application to finite elements}, 
Second edition. ISTE, London; John Wiley \& Sons, Inc., Hoboken, NJ, 2008.

\bibitem{Hartshorne} R. Hartshorne, {\it Algebraic Geometry}. New York: Springer-Verlag, 1999. 

\bibitem{Hilbert} D. Hilbert, {\it Theory of algebraic invariants}, Translated by R. C. Laubenbacher,
Cambridge University Press, 1993.

\bibitem{Shew}
F. Labelle and J. R. Shewchuk, {\it Anisotropic Voronoi Diagrams and Guaranteed-Quality Anisotropic Mesh Generation}, Proceedings of the Nineteenth AnnualSymposium on Computational Geometry, 191-200, 2003.

\bibitem{Lang} S. Lang, {\it Algebra}, 
Lang, Serge (2004), Algebra, Graduate Texts in Mathematics, 211 (Corrected fourth printing, revised third ed.), New York: Springer-Verlag, ISBN 978-0-387-95385-4

\bibitem{OST} P.J. Olver, G. Sapiro and A. Tannenbaum, {\it Affine invariant detection; edge maps, anisotropic diffusion
and active contours}, Acta Applicandae Mathematicae 59, 45-77, 1999.

\bibitem{Salmon} G. Salmon, {\it Higher plane curves}, third edition, 1879: http://www.archive.org/details/117724690

\bibitem{Shew2} J. R. ShewChuk, {\it What is a good linear finite element}: www.cs.berkeley.edu/\~{}jrs/papers/elemj.pdf

\bibitem{Bamg} The 2-d anisotropic mesh generator BAMG: 
http://www.freefem.org/ff++/  (included in the FreeFem++ software)

%---------------------------------------------
% Bibliographie Issue de W1P
%---------------------------------------------

\bibitem{Ba} I. Babu$\rm \check s$ka, A. K. Aziz {\it On the angle condition in the finite element method} 
%chapeau

\bibitem{CMi} A. Cohen, J.-M. Mirebeau, {\it Greedy bisection generates optimally adapted triangulations},
preprint, Laboratoire J.-L.Lions, submitted 2008.

\bibitem{CMi2} A. Cohen, J.-M. Mirebeau, {\it Adaptive and anisotropic piecewise polynomial approximation},
chapter 4 of the book {\it Multiscale, Nonlinear and Adaptive Approximation}, Springer, 2009

\bibitem{bookGeorge} P.L. George, H. Borouchaki, P.J. Frey, P. Laug and E. Saltel, {\it Mesh generation and mesh adaptivity: theory, techniques}, in Encyclopedia of computational mechanics, E. Stein, R. de Borst and T.J.R. Hughes ed., John Wiley \& Sons Ltd., 2004.

\bibitem{Ja} P. Jamet {\it Estimations d'erreur pour des \'el\'ements finis droits presque d\'eg\'en\'er\'es}, CRM-447, Centre d'Etudes de Limiel.

\bibitem{Kuate} R. Kuate, Thesis directed by F. Hecht, {\it Adaptation de maillage anisotrope : étude, construction d'estimateurs et raffinement hexaédrique}, LJLL, UPMC

\bibitem{sitejm} Personnal page with numerical examples and source codes :
www.ann.jussieu.fr/\~{}mirebeau/
%pour le code mathematica et FreeFem

\bibitem{FreeFem} FreeFem++ software, developped by Frederic Hecht, http://www.freefem.org/ff++/ 
%generation de maillage anisotrope

\bibitem{Inria} A 3-d anisotropic mesh generator: http://www.math.u-bordeaux1.fr/\~{}dobj/logiciels/ mmg3d.php
%Le mailleur de l'Inria Paris, Paul Louis Geoge, Alauzet,...

%---------------------------------------------
% Bibliographie Issue de Rectangles
%---------------------------------------------
\bibitem{Bab}
{V.F. Babenko}, {Interpolation of continuous functions by piecewise linear ones}, Math. Notes, 24, no.1,
(1978) 43--53.

\bibitem{us}
{ V. Babenko, Yu. Babenko, A. Ligun, A. Shumeiko,} {On asymptotical behavior of the optimal linear spline
interpolation error of $C^2$ functions}, East J. Approx., V. 12, N. 1 (2006), 71--101.

\bibitem{us2}
{Yu. Babenko, V. Babenko, D. Skorokhodov,} { {Exact asymptotics of the optimal $L_{p,\Omega}$-error of linear spline interpolation},
} East Journal on Approximations, V. 14, N. 3 (2008), pp. 285--317.

\bibitem{PhD}
{Yu. Babenko}, { On the asymptotic behavior of the optimal error of spline interpolation of multivariate functions}, PhD thesis, 2006.

\bibitem{JAT}
{Yu. Babenko}, Exact asymptotics of the uniform error of interpolation by multilinear splines, to appear in J.  Approx. Theory.

\bibitem{KL}
{K. B$\rm{\ddot{o}}$r$\rm{\ddot{o}}$czky, M. Ludwig,}  { Approximation of convex bodies and a momentum lemma
for power diagrams}, Monatshefte f$\it{\ddot{u}}$r Mathematik, V. 127, N. 2, (1999) 101--110.

\bibitem{Cohen}
{A. Cohen, J.-M. Mirebeau,}  {\it Adaptive and anisotropic piecewise polynomial approximation},
chapter 4 of the book {\it Multiscale, Nonlinear and Adaptive Approximation}, Springer, 2009


\bibitem{Daz1}
{ E. F. D'Azevedo} { Are bilinear quadrilaterals better than linear triangles?} SIAM J. Sci. Comput. 22
(2000), no. 1, 198--217.

\bibitem{DDI}
{L. Demaret, N. Dyn, A. Iske,} { Image compression by linear splines over adaptive triangulations},  IEEE
Transactions on Image Processing.

\bibitem{Toth}
{L. Fejes Toth,} Lagerungen in der Ebene, auf der Kugel und im Raum, 2nd edn. Berlin: Springer, 1972.

\bibitem {Gr3}
{P. Gruber}, { Error of asymptotic formulae for volume approximation of convex bodies in $E^d$,} Monatsh.
Math. 135 (2002) 279-304.

\bibitem{LSh}
{Ligun A.A., Shumeiko A.A.,} Asymptotic methods of curve recovery, {Kiev. Inst. of Math. NAS of Ukraine},
1997. (in Russian)

\bibitem{JM}
{J.-M. Mirebeau,}  Optimally adapted finite elements meshes, Constructive Approximation, 2010
 
\bibitem{Nadler}
{E. Nadler}, { Piecewise linear best $L_2$ approximation on triangles,}  in: Chui, C.K., Schumaker, L.L. and
Ward, J.D. (Eds.), Approximation Theory V, Academic Press, (1986) 499--502.

\bibitem{kodla1}
{H. Pottmann, R. Krasauskas, B. Hamann, K. Joy, W. Seibold}, { On piecewise linear approximation of quadratic
functions}, J. Geom. Graph. 4, no. 1, (2000) 31--53.

%--------------------------------------------
% Bibliographie issue de Cartoon
%--------------------------------------------

\bibitem{ACDDM} F. Arandiga, A. Cohen, R. Donat, N. Dyn and B. Matei, 
{\it Approximation of piecewise smooth images by edge-adapted
techniques}, Appl. Comp. Harm. Anal. 24, 225--250, 2008.

\bibitem{CD} E. Candes and D. L. Donoho, {\it Curvelets and curvilinear integrals},
J. Approx. Theory. 113, 59--90, 2000.

\bibitem{Ca} F. Cao, {\it Geometric curve evolution and image processing},
Lecture Notes in Mathematics, Springer, 2003.

\bibitem{Co} A. Cohen, {\it Numerical analysis of wavelet methods}, Elsevier, 2003.

\bibitem{CDDD1} A. Cohen, W. Dahmen, I. Daubechies, and R. DeVore, {\it Tree approximation and optimal encoding}, Appl. Comp. Harm. Anal. 11, pp. 192-226, 2001.

\bibitem{CDDD2} A. Cohen, W. Dahmen, I. Daubechies and R. DeVore, {\it Harmonic analysis of the space BV}, Rev. Mat. Iberoamericana 19, 235-262, 2003.

\bibitem{CDPX} A. Cohen, R. DeVore, P. Petrushev, and H. Xu, {\it Nonlinear approximation and the space ${\rm BV}(\R^2)$}, Amer. J. Math. 121, 587-628, 1999.

\bibitem{DPW} R. DeVore, G. Petrova and P. Wojtactzyck, {\it Anisotropic Smoothness via Level Sets}, 
Comm. Pure and Applied Math. 61, 1264-1297, 2008.

\bibitem{DLu} R. DeVore and B. Lucier, {\it High order regularity for conservation laws}, Indiana Math.,
413-430, 1990.

\bibitem{DL} R. DeVore and G. Lorentz, {\it Constructive approximation}, Springer Grundlehren, Vol. 303, 1993. 

\bibitem{Do} D. Donoho, {\it Unconditional bases are optimal bases for data compression and statistical estimation.}  Appl. Comp. Harm. Anal. 1, 100-115, 1993.

\bibitem{DJKP} D. Donoho, I. Johnstone, G. Kerkyacharian and D. Picard, {\it Wavelet shrinkage: Asymptotia.} 
J. Roy. Stat. Soc. B 57, 301-369, 1995.

\bibitem{EG} L.C. Evans and R.F. Gariepy,
{\it  Measure Theory and Fine Properties of Functions}, CRC Press, 1992.

\bibitem{FOR} E. Fatemi, S. Osher and L. Rudin, {\it Non linear total variation based noise removal algorithms}, Physica D 60, 259-268, 1992

\bibitem{GR} E. Godlewski and P.A. Raviart
{\it Numerical approximation of hyperbolic systems of conservation laws}, Applied Mathematical Sciences 118,  Springer-Verlag, New-York, 1996.

\bibitem {KP} B. Karaivanov
and P. Petrushev, {\it Nonlinear piecewise polynomial approximation beyond Besov spaces}, 
Appl. Comput. Harmon. Anal. 15, 177-223, 2003.

\bibitem{LM} E. Le Pennec and S. Mallat, {\it Bandelet image approximation
and compression},  
SIAM Journal of Multiscale Modeling. and Simulation 4, 992-1039, 2005.

\bibitem{Le} R. LeVeque, {\it Numerical methods for conservation laws}, Birkhauser, 1992.

\bibitem{LMo} C. Louchet and L. Moisan,
{\it Total Variation denoising using posterior expectation}, proceedings of the European Signal Processing Conference (Eusipco), 2008 

\bibitem{M} J.M. Mirebeau, {\it Optimal meshes for finite elements of higher order}, to appear in Constructive Approximation, 2010.

\bibitem{Ni} S.M. Nikol'skij, {\it Approximation of functions of several variables and imbedding theorems}, Springer, 1975.

\bibitem{Ol} P. J. Olver, G. Sapiro and A. Tannenbaum, {\it Invariant geometric evolutions of surfaces and volumetric smoothing}, SIAM J. Appl. Math. 57,176-194, 1997.

\bibitem{Whitney} H. Whitney, {\it Analytic extensions of differentiable functions defined in closed sets}, Transactions of the American Mathematical Society, 36, 63-89, 1934.

\bibitem{Te} V. Temlyakov, {\it Approximation of periodic functions},
Nova Science, New York, 1993.

%--------------------------------------------
% Bibliographie issue de CDHM
%--------------------------------------------

\bibitem{Alp} B. Alpert, {\it A class of bases in $L^2$ for the sparse representation
of integral operators}, SIAM J. Math. Anal. 24, 246-262, 1993.

\bibitem{Apel} T. Apel, 
{\it Anisotropic finite elements: Local estimates and applications}, 
Series ``Advances in Numerical Mathematics'', Teubner, Stuttgart, 1999.

\bibitem{BDD} P. Binev, W. Dahmen and R. DeVore,
{\it Adaptive Finite Element Methods with Convergence Rates}, 
Numerische Mathematik 97, 219--268, 2004.

\bibitem{BRW} R. Baraniuk, H. Choi, J. Romberg and M. Wakin, 
{\it Wavelet-domain approximation and compression 
of piecewise smooth images}, IEEE Transactions on Image Processing, 
15(5), 1071--1087, 2006.

\bibitem{BFOS} L. Breiman, J.H. Friedman,  R.A. Olshen and C.J. Stone,
{\it Classification and regression trees}, Wadsworth international, Belmont, CA, 1984. 

\bibitem{CDDD} A. Cohen, W. Dahmen, I. Daubechies and R. DeVore,
{\it Tree-structured approximation and optimal encoding},
App. Comp. Harm. Anal. 11, 192--226, 2001.

\bibitem{CM} A. Cohen and J.M. Mirebeau, {\it Greedy bisection generates optimally adapted
triangulations}, preprint, Laboratoire J.-L. Lions, 2008.

\bibitem{DLe} S. Dekel and D. Leviathan,
{\it Adaptive multivariate approximation using binary space partitions and geometric wavelets},
SIAM Journal on Numerical Analysis 43, 707--732, 2005.

\bibitem{DDFI} L. Demaret, N. Dyn, M. Floater and A. Iske,
{\it Adaptive thinning for terrain modelling and image compression},
in Advances in Multiresolution for Geometric Modelling,
N.A. Dodgson, M.S. Floater, and M.A. Sabin (eds.),
Springer-Verlag, Heidelberg, 321-340, 2005. 

\bibitem{D} D. Donoho, {\it Wedgelets: nearly minimax estimation of edges},
Ann. Statist. 27(3), 859--897, 1999.

\bibitem{Do2} D. Donoho, {\it CART and best basis: a connexion},
Ann. Statist. 25(5), 1870--1911, 1997.

\bibitem{Dor} W. D\"orfler, {\it A convergent adaptive algorithm for Poisson's equation},
SIAM J. Numer. Anal. 33, 1106--1124, 1996.

\bibitem{KS} B. S. Kashin and A. A. Saakian, {\it Orthogonal series}, 
Amer. Math. Soc., Providence, 1989.

\bibitem{MNS} P. Morin, R. Nochetto and K. Siebert,
{\it Convergence of adaptive finite element methods},
SIAM Review 44, 631--658, 2002.

\bibitem{St} R. Stevenson, {\it An optimal adaptive finite element method}, 
SIAM J. Numer. Anal., 42(5), 2188--2217, 2005. 

\bibitem{Ve} R. Verfurth, {\it A Review of A Posteriori Error Estimation and Adaptive Mesh-Refinement Techniques},
Wiley-Teubner, 1996.


%---------------------------------------------
% Bibliographie Issue de CM
%---------------------------------------------
\bibitem{BDDP} P. Binev, W. Dahmen, R. DeVore and P. Petrushev,
{\it Approximation Classes for Adaptive Methods}, 
Serdica Math. J. 28, 391--416, 2002.

\bibitem{BFGLS} H. Borouchaki, P.J. Frey,  P.L. George, P. Laug and E. Saltel,
{\it Mesh generation and mesh adaptivity: theory, techniques},  in Encyclopedia of computational mechanics, E. Stein, R. de Borst and T.J.R. Hughes ed., John Wiley \& Sons Ltd., 2004.

\bibitem{Cao} W. Cao, {\it On the error of linear interpolation and the orientation, aspect ratio, and
internal angles of a triangle}, SIAM J. Numer. Anal. 43(1), 19--40, 2005.

\bibitem{Chen1} L. Chen, {\it On minimizing the linear interpolation error
of convex quadratic functions}, East Journal of Approximation 14(3), 271--284, 2008.

\bibitem{Chen2} L. Chen, {\it Mesh smoothing schemes based on optimal Delaunay
triangulations}, in {\it 13th International Meshing Roundtable}, 109--120, Williamsburg VA, Sandia National
Laboratories, 2004.

\bibitem{De} R. DeVore, {\it Nonlinear approximation},
Acta Numerica 51-150, 1998

\bibitem{Mi} J.-M. Mirebeau, {\it  Optimal bidimensional finite element meshes},
preprint, Laboratoire J.-L. Lions.

\bibitem{Ri} M.C. Rivara, {\it New longest-edge algorithms for the refinement and/or improvement of unstructured triangulations}, 
Int. J. Num. Methods 40, 3313--3324, 1997.


\end{thebibliography}



==> Cartoon/cartoonThese.tex <==
%\input{../PreambleThese}
%------------------------------
% Remplacements
% \t -> \bt
% I_{m,T} -> \interp
%------------------------------

\section{Introduction}
There exists various ways of measuring the smoothness of functions
on a domain $\Omega\subset \RR^d$, 
generally through the definition of an appropriate {\it smoothness space}. 
Classical instances are Sobolev, H\"older and Besov spaces. Such spaces are of common use
when describing the regularity of solutions to partial differential equations.
From a numerical perspective, they are also useful in order to sharply characterize at which
rate a function $f$ may be approximated by simpler functions such as Fourier series,
finite elements, splines or wavelets (see \cite{Co,DL,De} for surveys on
such results).

Functions arising in concrete applications may have
inhomogeneous smoothness properties, in the sense that they exhibit
area of smoothness separated by localized discontinuities. Two typical
instances are (i) edge in functions representing real images and 
(ii) shock profiles in solutions to non-linear hyperbolic PDE's.
The smoothness space that is best taylored to take such features
into account is the space $BV(\Omega)$ of bounded variation functions. This space
consists of those $f$ in $L^1(\Omega)$ such that $\nabla f$ is a bounded measure,
i.e. such that their total variation
$$
\TV(f)=|f|_{BV}:=\max \left\{\int_\Omega f {\rm div}(\vp)\; ; \; \vp\in\cD(\Omega)^d,\; \|\vp\|_{L^\infty}\leq 1\right\}
$$
is finite. Functions of bounded variation are allowed to have jump discontinuities
along hypersurfaces of finite measure. In particular, the characteristic function of a smooth
subdomain $D\subset \Omega$ has finite total variation equal to the $d-1$-dimensional
Hausdorff measure of its boundary:
\be
|\Chi_D|_{BV}=\cH_{d-1}(\partial D).
\label{haus}
\ee
It is well known that $BV$ is a regularity space for certain 
hyperbolic conservation laws \cite{GR,Le}, in the sense that the total variation
of their solutions remains finite for all time $t>0$. This space also plays an
important role in image processing since the seminal paper \cite{FOR}.
Here, a small total variation is used as a prior to describe the mathematical 
properties of ``plausible images'', when trying to restore an unknown
image $f$ from an observation $h=Tf+e$ where $T$ is a known operator
and $e$ a measurement noise of norm $\|e\|_{L^2}\leq \e$. The restored image
is then defined as the solution to the minimization problem
\be
\min_{g\in BV} \{|g|_{BV}\; ; \; \|Tg-h\|_{L^2}\leq \e\}.
\label{minBV}
\ee
From the point of view of approximation theory, it was shown in \cite{CDPX,CDDD2} that
the space $BV$ is almost characterized by expansions in wavelet bases. For example,
in dimension $d=2$, if $f=\sum d_\lambda\psi_\lambda$ 
is an expansion in a tensor-product $L^2$-orthonormal wavelet basis, one has
$$
(d_\lambda)\in \ell^1 \Rightarrow f\in BV \Rightarrow (d_\lambda)\in w\ell^1,
$$
where $w\ell^1$ is the space of weakly summable sequences. The fact that 
the wavelet coefficients of a $BV$ function are weakly summable implies
the convergence estimate
\be
\|f-f_N\|_{L^2}\leq CN^{-1/2}|f|_{BV},
\label{wavN}
\ee
where $f_N$ is the {\it nonlinear} approximation of $f$ obtained by retaining the
$N$ largest coefficients in its wavelet expansion. Such approximation results 
have been further used in order to justify the performance of compression or
denoising algorithms based on wavelet thresholding \cite{CDDD1,DJKP,Do}.

In recent years, it has been observed that the space $BV$ (and more generally
classical smoothness spaces) do not provide a fully satisfactory description of
piecewise smooth functions arising in the above mentioned applications.
Indeed, formula \iref{haus} reveals that the total variation only takes into account
the {\it size} of the sets of discontinuities and not their geometric {\it smoothness}.
In image processing, this means that the set of bounded variation images does
not make the distinction between smooth and non-smooth edges as long as they have finite length.

The fact that edges have some geometric smoothness can be exploited in order to study
approximation procedures which outperform wavelet thresholding in terms of 
convergence rates. For instance, it is easy to prove that if $f=\Chi_D$ 
where $D$ is a bidimensional domain with smooth boundary, one can find a sequence
of triangulations $\cT_N$ with $N$ triangles such that the convergence estimate
\be
\|f-\interp_{\cT_N}f\|_{L^2} \leq CN^{-1},
\label{triN}
\ee
holds, where $\interp_\cT$ denotes the 
piecewise linear interpolation operator on a triangulation $\cT$.
Other methods are based on thresholding a decomposition of the 
function in bases or frames which differ from classical wavelets, see e.g. \cite{CD,LM,ACDDM}.
These methods also yield improvements over \iref{wavN} similar to \iref{triN}. The common feature in
all these approaches is that they achieve 
{\it anisotropic refinement} near the edges. For example,
in order to obtain the estimate \iref{triN}, 
the triangulation $\cT_N$ should include a thin layer of triangles
which approximates the boundary $\partial D$. These triangles typically have
size $N^{-2}$ in the normal direction to $\partial D$ and $N^{-1}$ in the tangential direction,
and are therefore highly anisotropic.  

Intuitively, these methods are well adapted to
functions which have anisotropic smoothness properties
in the sense that their local variation is significantly stronger
in one direction. Such properties are not well described by
classical smoothness spaces such as $BV$, and a natural
question to ask is therefore:
\nl
\nl
{\it What type of smoothness properties 
govern the convergence rate of anisotropic refinement
methods and how can one quantify these properties ?}
\nl
\nl
The goal of this chapter is to answer this question,
by proposing and studying measures of smoothness which are suggested
by recent results on anisotropic finite element approximation
\cite{BBLS, CSX} and Chapter 2. Before going further, 
let us mention several existing approaches which have been developed
for describing and quantifying anisotropic smoothness,
and explain their limitations.
\begin{enumerate}
\item
The so-called {\it mixed smoothness} classes have been introduced 
and studied in order to
describe functions which have a different order of
smoothness in each coordinate, see e.g. \cite{Ni,Te}. These spaces
are therefore not adapted to our present goal since
the anisotropic smoothness that we want to describe 
may have preferred directions that are not 
aligned with the coordinate axes and that may vary from
one point to another (for example an image with a curved edge).
\item
Anisotropic smoothness spaces
with more general and locally varying directions have
been investigated in \cite{KP}. Yet, in such spaces
the amount of smoothness in different directions
at each point is still fixed in advance and therefore
again not adapted to our goal, since this amount
may differ from one function to another (for example
two images with edges located at different positions).
\item
A  class of functions which is often used to 
study the convergence properties of anisotropic approximation
methods is the family of $C^m-C^n$ {\it cartoon images}, i.e.
functions which are $C^m$ smooth on a finite number
of subdomains $(\Omega_i)_{i=1,\cdots,k}$ separated by a union of
discontinuity curves 
$(\Gamma_{j})_{j=1,\cdots,l}$
that are $C^n$ smooth. The defects of this class are revealed
when searching for simple expression that quantifies the amount of
smoothness in this sense. A natural choice is
to take the supremum of all $C^m(\Omega_i)$ norms of $f$ and
$C^n$ norms of the normal parametrization of $\Gamma_{j}$.
We then observe that this quantity is unstable 
in the sense that it becomes extremely large
for blurry images obtained by convolving
a cartoon image by a mollifier $\vp_\delta=\frac 1{\delta^{2}}\vp(\frac \cdot h)$
as $\delta \to 0$.  In addition, this quantity does not
control the number of subdomains in the partition.
\item
A recent approach proposed in \cite{DPW} defines
anisotropic smoothness through the geometric 
smoothness properties of the {\it level sets} of the function $f$.
In this approach the measure of smoothness 
is not simple to compute directly from $f$ since it involves each of its level sets
and a smoothness measure of their local parametrization.
\end{enumerate}

The results of \cite{BBLS,CSX} and Chapter \ref{chapOptAniso} describe 
the $L^p$-error of piecewise linear interpolation by 
an optimally adapted triangulation of at most $N$ elements,
when $f$ is a $C^2$ function of two variables. This error is defined
as
$$
\sigma_N(f)_p:=\inf_{\#(\cT)\leq N}\|f-\interp_\cT f\|_{L^p}.
$$
It is shown in \cite{BBLS} for $p=\infty$
and in Chapter \ref{chapOptAniso} for all $1\leq p\leq \infty$ that
that 
\be
\limsup_{N\to +\infty} N\sigma_N(f)_p\leq CA_p(f),
\label{limsupest}
\ee
where $C$ is an absolute constant and
\be
A_p(f):=\|\sqrt {|{\rm det}(d^2f)|}\|_{L^\tau},\;\; \frac 1\tau:= 1+\frac 1 p.
\label{nonlinnorm}
\ee
Moreover, this estimate is known to be optimal in the sense that
$\liminf_{N\to +\infty} N\sigma_N(f)_p\geq cA_p(f)$ also holds, under some mild restriction
on the class of triangulations in which one selects the optimal one.
These results are extended in Chapter \ref{chapOptAniso} to the case of
higher order finite elements and space dimension $d>2$,
for which one can identify similar measures $f\mapsto A(f)$ governing the
convergence estimate. Such quantities thus constitute natural 
candidates to measure anisotropic smoothness properties. Note
that $A_p(f)$ is not a semi-norm due to the presence of the determinant
in \iref{nonlinnorm}, and in particular the
quasi-triangle inequality $A_p(f+g)\leq C(A_p(f)+A_p(g))$ 
does not hold even with $C>1$.

This chapter is organized as follows.
We begin in \S \ref{secCartoon2} by a brief account of the
available estimates on anisotropic finite element 
interpolation, and we recall in particular the argument that
leads to \iref{limsupest} with the quantity $A_p(f)$ defined by \iref{nonlinnorm}.

Since $A_p(f)$ is not a norm, we cannot associate
a linear smoothness space to it by a standard completion
process. We are thus facing a difficulty in extending
the definition of $A_p(f)$ to functions which are not
$C^2$-smooth and in particular to cartoon images
such as in item 3 above. Since we know from \iref{triN}
that for such cartoon images the $L^2$ error of adaptive
piecewise linear interpolation decays like $N^{-1}$, we would expect that the
quantity 
$$
A_2(f)=\|\sqrt {|{\rm det}(d^2f)|}\|_{L^{2/3}},
$$
corresponding to the case $p=2$ can be properly defined for
piecewise smooth functions. We address this difficulty in 
\S \ref{secCartoon3} by a regularization process:
if $f$ is a cartoon image we introduce its regularized version
\be
f_\delta:=f*\vp_{\delta},
\ee
where $\vp_\delta=\frac 1{\delta^{2}}\vp(\frac \cdot h)$ 
is a standard mollifier. Our
main result is the following: for any cartoon image $f$ of $C^2-C^2$ type, the quantity $A_2(f_\delta)$
remains uniformly bounded as $\delta\to 0$ and one has
\be
\lim_{\delta \to 0} A_2(f_\delta)^{2/3}= \sum_{i=1}^k \int_{\Omega_i}\left |\sqrt {|{\rm det}(d^2f)|}\right |^{2/3}
+C(\vp)\sum_{j=1}^l \int_{\Gamma_j} |[f](s)|^{2/3} |\kappa(s)|^{1/3} ds,
\label{lima2}
\ee
where $[f](s)$ and $\kappa(s)$ respectively denote
the jump of $f$ and the curvature of $\Gamma_j$ at the point $s$,
and where $C(\vp)$ is a constant that only depends on the choice of the mollifier.
This constant can be shown to be uniformly bounded by below for the class of
radially decreasing mollifiers. 
This result reveals that $A_2(f)$ is stable under regularization of cartoon images
(in contrast to the measure of smoothness described in item 3 above). 
We also discuss the behaviour of $A_p$ when $p\neq 2$.

These results lead us in \S \ref{secCartoon4} to a comparison
between the quantity $A_2(f)$ and the total variation $\TV(f)$. We also
make some remarks on the existing links between the limit expression
in \iref{lima2} and classical results on adaptive approximation
of curves, as well as
with operators of affine-invariant image processing which also
involve the power $1/3$ of the curvature. 

We devote \S \ref{secCartoon5} to numerical tests performed on cartoon images that illustrate the validity 
of our results. In addition, we compare the quantity $A_2(f)$
with the total variation $\TV(f)$ as a model for plausible images.

One could be tempted to use the quantity $A_2(f)$
in place of the total variation $\TV(f)$ as a prior 
in image processing, and in particular to replace $|g|_{BV}$
by $A_2(g)$ in a restoration procedure such as \iref{minBV}. 
In \S \ref{secCartoon5.5}, we show that this optimization program is
ill-posed in the sense that the restored image would be the noisy image itself.
An alternate strategy is to use $A_2(f)$ in the framework of a
bayesian least-square estimator, as proposed in \cite{LMo} in the
case of the total variation. At the present stage, the algorithm 
implementing this approach did not give satisfactory results due
to its very slow convergence. For this reason, we only present
some numerical illustration of this approach in a simplified one-dimensional setting.

Eventually we describe in \S \ref{secCartoon6} the extension of our results
to finite elements of higher degree and higher space dimensions.
Concluding remarks and perspectives of our work are given in \S \ref{secCartoon7}.

\section{Anisotropic finite element approximation}
\label{secCartoon2}
A standard estimate in finite element approximation states that 
if $f\in W^{2,p}(\Omega)$ then
$$
\|f-\interp_{\cT_h} f\|_{L^p} \leq C  h^{2}\|d^2f\|_{L^{p}},
$$
where $\cT_h$ is a triangulation of mesh size
$h:=\max_{T\in\cT_h} {\rm diam}(T)$. If we restrict our attention
to a family {\it quasi-uniform} triangulations, $h$ is linked with 
the complexity $N:=\#(\cT_h)$ according to
$$
C_1 h^{-2} \leq N \leq  C_2 h^{-2}
$$
Therefore, denoting by $\sigma^{\rm unif}_N(f)_{L^p}$ the $L^p$ approximation
by quasi-uniform triangulations of cardinality $N$, we can re-express the above
estimate as
\be
%\label{uniferror}
\sigma^{\rm unif}_N(f)_{L^p} \leq CN^{-1}\|d^2f\|_{L^p}.
\ee
In order to explain how this estimate can be improved
when using adaptive partitions, we first give some
heuristic arguments which are based on the assumption that on each triangle $T$
the relative variation of $d^2f$ is small so that it can be considered
as constant over $T$, which means that 
$f$ coincides with a quadratic function $q_T$ on each $T$.
Denoting by $\interp_T$ the local interpolation operator
on a triangle $T$ and by $e_{T}(f)_p:=\|f-\interp_T f\|_{L^p(T)}$
the local $L^p$ error, we thus have according to
this heuristics
$$
\|f-\interp_\cT f\|_{L^p} =\(\sum_{T\in \cT} e_T(f)_p^p\)^{\frac 1 p}=\(\sum_{T\in \cT} e_T(q_T)_p^p\)^{\frac 1 p}
$$
We are thus led to study the local interpolation error $e_T(q)_p$ when $q\in \P_2$
is a a quadratic polynomial. Denoting by $\bq$ the homogeneous part of $q$, we
remark that
$$
e_T(q)_p=e_T(\bq)_p.
$$
We optimize the shape of $T$ with respect to the quadratic form $\bq$
by introducing a function $K_p$ defined on the space of quadratic forms by
$$
K_p(\bq):=\inf_{|T|=1}e_T(\bq)_p,
$$
where the infimum is taken among all triangles of area $1$. 
It is easily seen that $e_T(\bq)_p$ is invariant
by translation of $T$ and so is therefore the minimizing triangle
if it exists. By homogeneity, it is also easily seen
that 
$$
\inf_{|T|=a} e_T(\bq)_p=a^{\frac 1 \tau}K_p(\bq),\;\; \frac 1 \tau=\frac 1 p+1,
$$
and that the minimizing triangle of area $a$ is obtained by rescaling the minimizing
triangle of area $1$ if it exists. Finally, it is easily seen that if $\vp$ is an invertible
linear transform 
$$
K_p(\bq \circ \vp)=|{\rm det} (\vp)|K_p(\bq),
$$
and that the minimizing triangle of area $|{\rm det} (\vp)|^{-1}$ for $\bq \circ \vp$
is obtained by application of $\vp^{-1}$ to the minimizing triangle of 
area $1$ for $\bq$ if it exists. If ${\rm det} (\bq)\neq 0$, there exists 
a $\vp$ such that $\bq \circ \vp$ is either $x^2+y^2$ or $x^2-y^2$ up to 
a sign change, and we have $|{\rm det} (\bq)|=|{\rm det} (\vp)|^{-2}$.
It follows that $K_p(\bq)$ has the simple form
\be
K_p(\bq)=\sigma  |{\rm det} (\bq)|^{1/2},
\label{Kpexp}
\ee
where $\sigma$ is a constant 
equal to $K_p(x^2+y^2)$ 
if ${\rm det} (\bq)>0$ and to  $K_p(x^2-y^2)$ if ${\rm det} (\bq)<0$. 
One easily checks that this equality
also holds when ${\rm det} (\bq)= 0$ in which case $K_p(\bq)=0$.

Assuming that the triangulation $\cT$ is
such that all its triangles $T$ have optimized shape in the above sense
with respect to the quadratic form $\bq_T$ associated with $q_T$, we thus have
for any triangle $T\in\cT$
$$
e_T(f)_p=e_T(\bq_T)_p=|T|^{\frac 1 \tau}K_p(\bq_T)=\left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(T)}.
$$
since we have assumed $\frac {d^2f} 2=\bq_T$ on $T$. In order to optimize the trade-off
between the global error and the complexity $N=\#(\cT)$,
we apply the principle of {\it error equidistribution}: the triangles $T$ have
area such that all errors $e_T(\bq_T)_p$ are equal
i.e. $e_T(\bq_T)_p= \eta$ for some $\eta>0$ independent of $T$.
It follows that
$$
N\eta^\tau\leq \left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}^\tau,
$$
and therefore
$$
\sigma_N(f)_p \leq \|f-\interp_\cT f\|_{L^p} \leq N^{1/p} \eta \leq\left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}N^{-1},
$$
which according to \iref{Kpexp} implies 
\be
\sigma_N(f)_p \leq CN^{-1}A_p(f),
\label{false}
\ee
with $A_p$ defined as in \iref{nonlinnorm}.

The estimate \iref{false} is too optimistic to be correct:
if $f$ is a univariate function then $A_p(f)=0$ while $\sigma_N(f)_p$
may not vanish. In a rigorous 
derivation such as in \cite{BBLS} and Chapter 2, one observes that
if $f\in C^2$, the replacement of $d^2f$ by a constant over $T$
induces an error which becomes negligible only when the
triangles are sufficiently small, and therefore a
correct statement is that for any $\e>0$ there exists 
$N_0=N_0(f,\e)$ such that 
\be
\sigma_N(f)_p \leq N^{-1}\left(\left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}+\e\right),
\label{true}
\ee
for all $N\geq N_0$, i.e.
\be
\limsup_{N\to +\infty} N\sigma_N(f)_p\leq \left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}
\label{limsupest1}
\ee
which according to \iref{Kpexp} implies \iref{limsupest}.

\section{Piecewise smooth functions and images}
\label{secCartoon3}
As already observed, the quantities $A_p(f)$ are well defined for
functions $f\in C^2$, but 
we expect that they should in some sense also be well defined for
functions representing $C^2-C^2$ ``cartoon images'' when $p\leq 2$. We first give 
a precise definition of such functions.

\begin{definition} 
\label{defcartoon}
A cartoon function on an open set $\Omega$ is a function almost everywhere of the form 
$$
f=\sum_{1\leq i\leq k} f_i \Chi_{\Omega_i},
$$
where the $\Omega_i$ are disjoint open sets with piecewise $C^2$ boundary, no cusps (i.e. satisfying an interior and exterior cone condition), and such that $\overline \Omega = \cup_{i=1}^k \overline \Omega_i$, and where the function $f_i$ is $C^2$ on $\overline \Omega_i$ for each $1\leq i\leq k$. %a neighbourhood of
\end{definition}

Let us consider a fixed cartoon function $f$ on an open polygonal domain $\Omega$ (i.e.
$\Omega$ is such that $\overline\Omega$ is a closed polygon)
associated with a decomposition $(\Omega_i)_{1\leq i\leq k}$. We define 
\be
\Gamma :=\bigcup_{1\leq i\leq k} \partial \Omega_i,
\ee
the union of the boundaries of the $\Omega_i$. The above definition
implies that $\Gamma$ is the disjoint union of a finite set of points $\cP$ and a finite number of open curves $(\Gamma_i)_{1\leq i\leq l}$.
$$
\Gamma = \(\bigcup_{1\leq i\leq l} \Gamma_i\) \cup \cP.
$$
Furthermore for all $1\leq i < j \leq l$, we may impose that $\overline \Gamma_i\cap \overline \Gamma_j \subset \cP$ (this may be ensured by a splitting of some of the $\Gamma_i$ if necessary).

We now consider the piecewise linear interpolation
$\interp_{\cT_N}f$ of $f$ on a triangulation $\cT_N$ of cardinality $N$. 
We distinguish two types of elements of $\cT_N$. A 
triangle $T\in \cT_N$ is called ``regular'' if $T\cap \Gamma=\emptyset$, 
and we denote the set of such triangles by $\cT_N^r$. 
Other triangles are called ``edgy'' and their set is denoted by $\cT_N^e$.
We can thus split $\Omega$ according to
$$
\Omega:=\left(\cup_{T\in \cT_N^r}T\right) \cup \left(\cup_{T\in \cT_N^e}T\right)=\Omega_N^r \cup \Omega_N^e.
$$
We split accordingly the $L^p$ interpolation error into
$$
\|f-\interp_{\cT_N}f\|_{L^p(\Omega)}^p = \int_{\Omega_N^r} |f-\interp_{\cT_N}f|^p +\int_{\Omega_N^e} |f-\interp_{\cT_N}f|^p.
$$
We may use $\cO(N)$ triangles in $\cT_N^e$ and $\cT_N^r$ (for example $N/2$
in each set). Since $f$ has discontinuities along $\Gamma$, the $L^\infty$ interpolation error on 
$\Omega_N^e$ does not tend to zero and $\cT_N^e$ should be chosen so 
that $\Omega_N^e$ has the aspect of a thin layer around $\Gamma$. 
Since $\Gamma$  is a finite union of $C^2$ curves, we can build this layer
of width $\cO(N^{-2})$ and therefore of global area $|\Omega_N^e|\leq C N^{-2}$,
by choosing long and thin triangles in $\cT_N^e$. 
On the other hand, since $f$ is uniformly $C^2$ on $\Omega_N^r$, we may
choose all triangles in $\cT_N^r$ of regular shape 
and diameter $h_T\leq C N^{-1/2}$.
Hence we obtain the following heuristic error estimate, 
for a well designed anisotropic triangulation:
\begin{eqnarray*}
\|f-\interp_{\cT_N}f\|_{L^p(\Omega)} &=& \(\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^r)}^p +\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^e)}^p\)^{1/p}\\
&\leq&\( \|f-\interp_{\cT_N}f\|_{L^\infty(\Omega_N^r)}^p |\Omega_N^r|+  
\|f-\interp_{\cT_N}f\|_{L^\infty(\Omega_N^e)}^p |\Omega_N^e|\)^{1/p}\\
& \leq & C(N^{-p}+ N^{-2})^{1/p},
\end{eqnarray*}
and therefore
\be
 \|f-\interp_{\cT_N}f\|_{L^p(\Omega)} \leq C N^{-\min\{1,2/p\}},
 \label{heurist}
 \ee
where the constant $C$ depends on $\|d^2f\|_{L^\infty(\Omega\sm \Gamma)}$, $\|f\|_{L^\infty(\Omega)}$
and on the number, length and maximal curvature of the $C^2$ curves which constitute $\Gamma$.

Observe in particular that the error
is dominated by the edge term $\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^e)}$
when $p>2$ and by the smooth term $\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^r)}$
when $p<2$. For the critical value $p=2$ the two terms have the same order. 

For $p\leq 2$, we obtain the approximation rate $N^{-1}$ 
which suggests that approximation results such as \iref{limsupest}
should also apply to cartoon functions and
that the quantity $A_p(f)$ should be
finite. We would therefore like to bridge the gap 
between anisotropic approximation of cartoon functions and smooth functions. 
For this purpose, we first need to give a proper meaning
to $A_p(f)$ when $f$ is a cartoon function. This is not 
straightforward, due to the fact that
the product of two distributions has no meaning in general.
Therefore, we cannot define $\det (d^2 f)$ in a distributional sense,
when the coefficients of $d^2 f$ are distributions without sufficient smoothness.
Our approach will rather be based on regularisation. This is additionally justified by the fact that sharp curves of discontinuity are a mathematical idealisation. In real world applications, such as photography, several physical limitations (depth of field, optical blurring) impose a certain level of blur on the edges.

In the following, we consider a fixed
radial nonnegative function $\vp$ of unit integral and supported in the unit ball,
and we define for all $\delta>0$ and $f$ defined on $\Omega$,
\be
\vp_\delta(z) := \frac 1 {\delta^2} \vp\left(\frac z \delta\right) \text{ and } f_\delta = f * \vp_\delta.
\label{defphih}
\ee
Our main result gives a meaning to $A_p(f)$ based on this regularization.
If $f$ is a cartoon function on a set $\Omega$, 
and if $x\in \Gamma\sm\cP$, we denote by $[f](x)$ the jump of $f$
at this point.
We also denote $\bt(x)$ and $\bn(x)$ the unit tangent and normal
vectors to $\Gamma$ at $x$ oriented in such way that $\det(\bt,\bn)=+1$,
and by $\kappa(x)$ the curvature
at $x$ which is defined by the relation
$$
\partial_{\bt(x)}\bt(x)=\kappa(x)\bn(x).
$$
For $p\in [1,\infty]$ and $\tau$ defined by $\frac 1 \tau := 1+\frac 1 p$,
we introduce the two quantities
\begin{eqnarray*}
S_p(f) &:= & \|\sqrt{|\det (d^2 f) |}\|_{L^\tau(\Omega\sm \Gamma)}=A_p(f_{|\Omega\sm \Gamma}),\\
E_p(f) &:= & \|\sqrt{|\kappa|} [f]\|_{L^\tau(\Gamma)},\\
\end{eqnarray*}
which respectively measure the ``smooth part'' and the ``edge part'' of $f$. We
also introduce the constant
\be
C_{p,\vp}:=\|\sqrt {|\Phi\Phi'|}\|_{L^\tau(\R)},\;\; \text{ where } \ \Phi(x) := \int_{y\in\R} \vp(x,y)dy.
\label{defchi}
\ee
Note that $f_\delta$ is only properly defined on the set
$$
\Omega^\delta:=\{z\in \Omega\; ; \; B(z,\delta)\subset \Omega\},
$$
and therefore, we define
$A_p(f_\delta)$ as the $L^\tau$ norm of $\sqrt{|\det(d^2f_\delta)|}$ on this set.

\begin{theorem}
\label{threg}
For all cartoon functions $f$, the quantity $A_p(f_\delta)$ behaves as follows:
\begin{itemize}
\item If $p<2$, then
$$
\lim_{\delta\to 0} A_p(f_\delta) = S_p(f).
$$
\item If $p=2$, then $\tau=\frac 2 3$ and 
\be
\lim_{\delta\to 0} A_2(f_\delta) = \(S_2(f)^\tau+ E_2(f)^\tau C_{2,\vp}^\tau\)^{\frac 1 \tau}.
\label{Acartoon}
\ee
\item If $p>2$, then $A_p(f_\delta) \to \infty$ according to
\be
\lim_{\delta\to 0}  \delta^{\frac 1 2 - \frac 1 p} A_p(f_\delta)= E_p(f) C_{p,\vp}.
\label{equivAphih}
\ee
\end{itemize}
\end{theorem}


\begin{remark}
This theorem reveals that as $\delta\to 0$, the 
contribution of the neighbourhood of $\Gamma$ to $A_p(f_\delta)$
is negligible when $p<2$ and 
dominant when $p>2$, which was already remarked in
the heuristic computation leading to {\rm \iref{heurist}}.
\end{remark}


\begin{remark}
It seems to be possible to eliminate the ``no cusps'' condition
in the definition of cartoon functions, while still retaining the validity of
this theorem. It also seems possible to take the more natural choice 
$\vp(z) = \frac 1 \pi e^{-\|z\|^2}$, which is not compactly supported.
However, both require higher technicality in the proof
which we avoid here.
\end{remark}


Before attacking the proof of Theorem \ref{threg},
we show below that the constant $C_{p,\vp}$ involved in 
the result for $p\geq 2$ is uniformly bounded by below
for a mild class of mollifiers.

\begin{proposition}
\label{propLowerCPhi}
Let $\vp$ be a radial and positive function supported on the unit ball
such that $\int \vp=1$ and that $\vp(x)$ decreases as $|x|$ increases. For any $p\geq 2$ we have 
$$
C_{p, \vp} \geq \frac 2 \pi \left(\frac 4 {\tau+2}\right)^{\frac 1 \tau}.
$$
and this lower bound is optimal. 
There is no such bound if $p<2$, but note that Theorem \ref{threg} does not involve $C_{p, \vp}$ for $p<2$.
\end{proposition}

\proof
Let $D$ be the unit disc of $\R^2$. We define a non smooth mollifier $\psi$ and a function $\Psi$ as follows
$$
\psi := \frac {\Chi_D} \pi \ \text{ and } \ \Psi(x) :=  \int_\R\psi(x,y) dy.
$$
One easily obtains that
$
\Psi(x) = \frac 2 \pi \sqrt{1-x^2} \Chi_{[-1,1]}(x)\text{ and } \Psi'(x) = \frac {-2x}{\pi \sqrt{1-x^2}} \Chi_{[-1,1]}(x), 
$
hence 
$$
\Psi(x) \Psi' (x)=  \frac {-4x} {\pi^2} \Chi_{[-1,1]}(x).
$$
For all $\delta>0$ we define $\psi_\delta := \delta^{-2} \psi(\delta^{-1} \cdot)$, and  $\Psi_\delta(x) :=  \int_\R\psi_\delta(x,y) dy$. Similarly we obtain 
$$
\Psi_\delta(x) \Psi'_\delta (x) = \frac {-4x} {\pi^2}  \Chi_{[-\delta,\delta]} \delta^{-4}.
$$
Hence 
\begin{eqnarray*}
C_{p,\psi_\delta} &=& \left\|\sqrt{\Psi_\delta(x) |\Psi'_\delta (x)|}\right\|_{L^\tau(\R)} \\
&=& \frac 2 {\pi \delta^2} \left(\int_{-\delta}^\delta |x|^{\frac\tau 2} dx\right)^{\frac 1 \tau} \\
&=& \frac 2 {\pi \delta^2} \left(\frac{2 \delta^{\frac \tau 2 +1}}{\frac \tau 2 +1}\right)^{\frac 1 \tau}\\
&=& \frac 2 \pi \left(\frac 4 {\tau+2}\right)^{\frac 1 \tau} \delta^{\frac 1 p -\frac 1 2}.
\end{eqnarray*}
Note that
\be
\label{ineqPsiDelta}
\text{ If } p\geq 2 \text{ and }\delta \in (0,1] \text{ then }  C_{p,\psi_\delta} \geq C_{p,\psi} =   \frac 2 \pi \left(\frac 4 {\tau+2}\right)^{\frac 1 \tau}.
\ee
The mollifier $\vp$ of interest is radially decreasing, has unit integral and is supported on the unit ball. It follows that there exists a Lebesgue measure $\mu$ on $(0,1]$, of mass $1$, such that 
$$
\vp = \int_0^1\psi_\delta \ d\mu(\delta).
$$
Hence
$
\Phi(x) := \int_\R \vp(x, y) dy = \int_0^1\Psi_\delta(x) \ d\mu(\delta)
$,
 for any $x\in \R$.
Since $s\mapsto s^\tau$ is concave on $\R_+$ when $0<\tau \leq 1$, we obtain
$$
\Phi(x)^\tau = \left(\int_0^1 \Psi_\delta(x) \ d\mu(\delta)\right)^\tau \geq \int_0^1 \Psi_\delta(x)^\tau \ d\mu(\delta)
$$
Similarly, since the sign of $\Psi'_\delta(x)$ is independent of $\delta$, 
$
|\Phi'(x)|^\tau = \left(\int_0^1 |\Psi_\delta'(x)| \ d\mu(\delta)\right)^\tau \geq \int_0^1 |\Psi_\delta'(x)|^\tau \ d\mu(\delta).
$
Applying the Cauchy-Schwartz inequality we obtain
\begin{eqnarray*}
\sqrt{\Phi(x) |\Phi'(x)|}^{\, \tau} &\geq& 
\sqrt{\left(\int_0^1 \Psi_\delta(x)^\tau \ d\mu(\delta)\right)\left(\int_0^1 |\Psi_\delta'(x)|^\tau \ d\mu(\delta)\right)} \\
&\geq& \int_0^1 \sqrt{\Psi_\delta(x) |\Psi_\delta'(x)|}^{\, \tau} \ d\mu(\delta)
\end{eqnarray*}
Eventually we obtain using the previous equation and \iref{ineqPsiDelta} that
$$
C_{p,\vp}^\tau = \int_\R \sqrt{\Phi |\Phi'|}^{\,\tau}
 \geq \int_0^1 \left(\int_\R \sqrt{\Psi_\delta |\Psi_\delta'|}^{\,\tau}\right) d\mu(\delta)\\
=  \int_0^1  C_{p,\psi_\delta}^\tau d\mu(\delta) \geq  C_{p,\psi}^\tau,
$$
which concludes the proof of this lemma.
\sq

The rest of this section is devoted to the proof of Theorem \ref{threg}. Since
it is rather involved, we split its presentation into several main steps.
\nl
\nl
{\bf Step 1: decomposition of $A_p(f_\delta)$.}
Using the notation $K(M):= \sqrt{|\det M|}$, we can write
\be
\label{tointegrate2d}
A_p(f_\delta)^\tau = \int_{\Omega^\delta} K(d^2 f_\delta)^\tau.
\ee
We decompose this quantity based on a partition of
$\Omega^\delta$ into three subsets 
$$
\Omega^\delta=\Omega_\delta \cup \Gamma_\delta \cup \cP_\delta.
$$
The first set $\Omega_\delta$ corresponds to the
{\it smooth part}:
$$
\Omega_\delta :=  \bigcup_{1\leq i\leq k} \Omega_{i,\ssdelta}, \;\;{\rm where}\;\; 
\Omega_{i,\ssdelta} := \{z\in \Omega_i\sep d(z,\Omega\sm\Omega_i)>\delta\}.
$$
Note that $\Omega_\delta$ is strictly contained in $\Omega^\delta$.
The second set corresponds to the {\it edge part}:  we first define
$$
 \Gamma_\delta^0 := \bigcup_{1\leq j\leq l} \Gamma_{j,\ssdelta}^0, \;\;{\rm where}\;\; 
\Gamma_{j,\ssdelta}^0 := \{z\in \Gamma_j\sep d(z,\Gamma\sm\Gamma_j)>2\delta\},
$$
and then set
$$
\Gamma_\delta := \bigcup_{1\leq j\leq l} \Gamma_{j,\ssdelta}\;\;{\rm where}\;\; 
\Gamma_{j,\ssdelta} :=  \{z\in \Omega \sep d(z,\Gamma)< \delta \text{ and } \pi_\Gamma(z)\in \Gamma_{j,\ssdelta}^0\} 
$$
where $\pi_\Gamma(z)$ denotes the point of $\Gamma$ which is the closest to $z$.
The third set corresponds the {\it corner part}:
$$
\cP_\delta :=  \Omega^\delta \sm (\Omega_\delta\cup\Gamma_\delta).
$$
The measures of the sets $\Gamma_\delta$ and $\cP_\delta$ tends to
$0$ as $\delta\to 0$, while $|\Omega_\delta|$ tends to $|\Omega|$. More
precisely, we have
$$
 |\Gamma_\delta|\leq C\delta\;\;{\rm and}\;\; |\cP_\delta|\leq C  \delta^2
$$
where the last estimate exploits the ``no cusps'' property of the cartoon function.
We analyze separately the contributions of these three sets to 
\iref{tointegrate2d}.
\nl
\nl
{\bf Step 2: Contribution of the smooth part $\Omega_\delta$.}
The contribution of $\Omega_\delta$ to the integral \iref{tointegrate2d} is easily measured. Indeed, let us define
$$
Q_\delta(z):= \left\{
\begin{array}{cc}
K(d^2 f_\delta (z))^\tau & \text{ if } z\in \Omega_\delta,\\
0 & \text{ otherwise.}
\end{array}
\right.
$$
Then we have pointwise convergence $Q_\delta(z)\to K(d^2 f(z))^\tau$ on $\Omega\sm \Gamma$.
Since the  $\delta$-neighbourhood of $\Omega_\delta$ is included in $\Omega\sm\Gamma$, we have 
$$
\|d^2 (f*\vp_\delta) \|_{L^\infty(\Omega_\delta)} = \|(d^2 f)*\vp_\delta \|_{L^\infty(\Omega_\delta)}\leq \|d^2 f\|_{L^\infty(\Omega\sm \Gamma)} \|\vp_\delta\|_{L^1} = \|d^2 f\|_{L^\infty(\Omega\sm \Gamma)} 
$$
Since 
$$
K(M) = \sqrt{|\det M|} \leq \|M\|
$$ 
we have
$
K(d^2 f_\delta)\leq \|d^2 f\|_{L^\infty(\Omega\sm \Gamma)} 
$ on $\Omega_\delta$,
and we conclude by dominated convergence that 
$$
\lim_{\delta \to 0}\int_{\Omega_\delta} K(d^2 f_\delta)^\tau = \lim_{\delta\to 0} \int_{\Omega \sm \Gamma} Q_\delta =  \int_{\Omega \sm \Gamma} K(d^2 f)^\tau.
$$
\nl
{\bf Step 3: Contribution of the corner part $\cP_\delta$.}
We only need a rough upper estimate of the contribution of $\cP_\delta$ 
to the integral \iref{tointegrate2d}.
We observe that 
$$
\|d^2 (f*\vp_\delta) \|_{L^\infty(\Omega)} = \|f*(d^2  \vp_\delta)\|_{L^\infty(\Omega)}\leq \|f\|_{L^\infty(\Omega)} \|d^2 \vp_\delta\|_{L^1(\R^2)} =   \frac M {\delta^2},
$$
where $M:=\|f\|_{L^\infty(\Omega)} \|d^2 \vp\|_{L^1(\R^2)}$.
It follows that 
$$
\int_{\cP_\delta} K(d^2 f_\delta)^\tau \leq |\cP_\delta| \left(\frac M {\delta^2}\right)^\tau \leq C  \delta^{2-2 \tau}.
$$
If $\tau<1$, this quantity tends to $0$ and is therefore negligible compared to the 
contribution of the smooth part. If $\tau=1$, which corresponds to $p=\infty$, our
further analysis shows that the contribution of the edge part tends
to $+\infty$, and therefore the contribution of the corner part is always negligible.
\nl
\nl
{\bf Step 4: Contribution of the edge part $\Gamma_\delta$.} {
This step is the main difficulty of the proof. We make a key use
of an asymptotic analysis of $f_\delta$ on $\Gamma_\delta$, which relates
its second derivatives to the jump $[f]$ and the curvature $\kappa$ as $\delta\to 0$. 
We first define for all $\delta>0$ the map
$$
\begin{array}{ccc}
U_\delta : \Gamma\sm\cP \times [-1,1] &\to& \Omega\\
(x,u) &\mapsto & x+\delta u \bn (x).
\end{array}
$$
We notice that according to our definitions,
for $\delta$ small enough, the map $U_\delta$ induces a diffeomorphism 
between $\Gamma_\delta^0\times [-1,1]$ and $\Gamma_\delta$, such
that $\pi_\Gamma(U_\delta(x,u))=x$ and $d(U_\delta(x,u),\Gamma)=|U_\delta(x,u)-x|=\delta |u|$.
We establish asymptotic estimates on the
second derivatives of $f_\delta$ which have the following form:
\begin{eqnarray}
\label{estimnn2d}
\left |\partial_{\bn,\bn} f_\delta(z) -  \frac 1 { \delta^2} [f](x) \Phi'(u)\right| &\leq & \frac C { \delta}\\ 
\label{estimnt2d}
|\partial_{\bn,\bt} f_\delta(z)| &\leq &  \frac C \delta\\%\cO\left(\frac 1 \delta\right)\\
\label{estimtt2d}
\left |\partial_{\bt,\bt} f_\delta(z) +  \frac 1 \delta [f](x) \kappa(x)\Phi(u)\right| &\leq &\frac {\omega(\delta)} \delta
\end{eqnarray}
where $\lim_{\delta\to 0} \omega(\delta) = 0$ and with the notation
$z=U_\delta(x,u)$. The constant $C$ and the function $\omega$ depend only on $f$.
The proof of these estimates is given in the appendix. As an immediate consequence,
we obtain an asymptotic estimate of $K(d^2 f_\delta)=\sqrt{|\det(d^2 f_\delta)|}$ of the form
\be
\label{estimK2d}
\left|  \delta^{\frac 3 2} K(d^2 f_\delta(z)) - \sqrt{|\kappa(x)|} \, |[f](x)| \sqrt{|\Phi(u) \Phi'(u)|} \right|\leq \ti \omega(\delta),
\ee
where $\lim_{\delta\to 0} \ti \omega(\delta) = 0$, and the function $\ti \omega$ depends only on $f$. 
Using the notations
$$
g_\delta(z):=\delta^{\frac 3 2} K(d^2 f_\delta(z)),\;\;  \lambda(x):=\sqrt{|\kappa(x)|}\, |[f](x)|,\;\; \mu(u):=\sqrt{|\Phi(u) \Phi'(u)|},
$$
we thus have
\be
|g_\delta(z) - \lambda(x) \mu(u)|\leq \ti \omega(\delta), 
\label{glambmu}
\ee
for all $x\in \Gamma^0_\delta$, $u\in [-1,1]$ and $\delta>0$
sufficiently small, with $z=U_\delta(x,u)$. We claim that
for any continuous functions $(g_\delta,\lambda,\mu)$ satisfying \iref{glambmu},
we have for any $\tau>0$, 
\be
\lim_{\delta\to 0}  \delta^{-1} \int_{\Gamma_\delta} g_\delta^\tau =\int_{\Gamma} \lambda(x)^\tau dx  \int_{-1}^1 \mu(u)^\tau du,
\label{claim}
\ee
which is in our case equivalent to the estimate
\be
\lim_{\delta\to 0}  \delta^{ \frac 3 2 \tau-1} \int_{\Gamma_\delta} K(d^2 f_\delta)^\tau = 
 \int_\Gamma |[f]|^\tau |\kappa|^{\tau/2} \int_\R |\Phi \Phi'|^{\tau/2}.
\label{estimgammadelta}
\ee
In order to prove \iref{claim}, we may assume without loss of generality that $\tau =1$
up to replacing $(g_\delta,\lambda,\mu)$  by $(g_\delta^\tau,\lambda^\tau,\mu^\tau)$.
We first express the jacobian matrix of $U_\delta$
using the bases $B_1 = ((\bt(x),0),(0,1))$ and $B_2 =(\bt(x),\bn(x))$ 
for the tangent spaces of $\Gamma\times [-1,1]$ and $\Omega$.
This gives the expression
$$
[d U_\delta(x,u)]_{B_1,B_2} = \left(
\begin{array}{c|c}
1- \delta u\kappa(x)& 0\\
\hline
0 & \delta
\end{array}
\right)
$$
and therefore $|\det([dU_\delta(x,u)]_{B_1,B_2})| = \delta -\delta^2 u\kappa(x)$. Since
$B_1$ and $B_2$ are orthonormal bases, this quantity is the jabobian of $U_\delta$ at $(x,u)$,
and therefore
$$
\int_{\Gamma_\delta} g_\delta =\delta\int_{\Gamma_\delta^0 \times [-1,1]} g_\delta(x+\delta u \bn (x)) 
(1 -\delta u\kappa(x)) dx\, du
$$
Combining with \iref{glambmu}, and using dominated
convergence we obtain \iref{claim}.
\nl
\nl
{\bf Step 5: summation of the different contributions.}
Summing up the contributions of $\Omega_\delta$, $\cP_\delta$ and $\Gamma_\delta$,
we reach the estimate
\begin{eqnarray*}
\int_\Omega K(d^2 f_\delta)^\tau &=&  \int_{\Omega_\delta} K(d^2 f_\delta)^\tau+ \int_{\cP_\delta} K(d^2 f_\delta)^\tau+ \int_{\Gamma_\delta} K(d^2 f_\delta)^\tau\\
&=& \left(\int_{\Omega\sm\Gamma} K(d^2 f)^\tau +\e_1(\delta) 
\right) + B(\delta) \delta^{2-2\tau} \\
& &+  \delta^{1-\frac 3 2 \tau} \left( \int_\Gamma |[f]|^\tau |\kappa|^{\tau/2}\int_\R |\Phi \Phi'|^{\tau/2} +\e_2(\delta)\right),\\
&=& (S_p(f)^\tau +\e_1(\delta)) + B(\delta) \delta^{2-2\tau}+  \delta^{1-\frac 3 2 \tau} (E_p(f)^\tau C_{p,\phi}^\tau+\e_2(\delta)),\\
\end{eqnarray*}
where $\lim_{\delta\to 0}\e_1(\delta)=\lim_{\delta\to 0}\e_2(\delta)=0$ and $B(\delta)$ is uniformly bounded.
This concludes the proof of Theorem \ref{threg}. 


\section{Relation with other works}
\label{secCartoon4}
Theorem \ref{threg} allows us to extend
the definition of $A_2(f)$ when $f$ is a cartoon
function, according to
\be
A_2(f):= \(S_2(f)^{2/3}+ E_2(f)^{2/3} C_{2,\vp}^{2/3} \)^{3/2}.
\label{addita2}
\ee
We first compare this additive form
with the total variation $\TV(f)$. If $f$ is a
cartoon function,
its total variation has the additive form
\be
\TV(f):=\|\nabla f\|_{L^1(\Omega\sm\Gamma)}+ \|[f]\|_{L^1(\Gamma)},
\label{additv}
\ee
Both \iref{addita2} and \iref{additv}
include a ``smooth term'' and an ``edge term''.
It is interesting to compare the edge term
of $A_2(f)$, which is given by
$$
E_2(f)=\|\sqrt {|\kappa|}[f]\|_{L^{2/3}(\Gamma)},
$$
up to the multiplicative constant $C_{2,\vp}$, with the
one of $\TV(f)$ which is simply the integral of the jump
$$
J(f):=\|[f]\|_{L^{1}(\Gamma)},
$$
Both terms are $1$-homogeneous with the value of the jump of the
function $f$. In particular, if the value of this jump is $1$
(for example when $f$ is the characteristic function of a set of boundary $\Gamma$), we have
\be
E_2(f)=\(\int_\Gamma |\kappa|^{1/3}\)^{3/2},
\label{powercurv}
\ee
while $J(f)$ coincides with the length of $\Gamma$. 
In summary, $A_2(f)$ takes into account the {\it smoothness} of
edges, through their curvature $\kappa$, while 
$\TV(f)$ only takes into account their {\it length}.

Let us now investigate more closely the measure of
smoothness of edges which is incorporated in $A_2(f)$. According to 
\iref{powercurv}, this smoothness is meant in the sense
that the arc length parametrizations of the curves that
constitute $\Gamma$ admit  
second order derivatives in $L^{\frac 1 3}$. In the following,
we show that this particular measure of smoothness is 
naturally related to some known results in two different areas:
adaptive approximation of curves and affine-invariant image
processing.

We first revisit the derivation of the heuristic estimate
\iref{heurist} for the error between a cartoon function
and its linear interpolation on an optimally adapted 
triangulation. In this computation, the contribution of the
``edgy triangles'' was estimated by the area of the layer $\Omega_N^e$ according to
$$
\|f-\interp_{\cT_N} f\|_{L^p(\Omega^{e}_N)} \leq \|f\|_{L^\infty} |\Omega_N^e|^{1/p}.
$$
Then we invoke the fact that $\Gamma$ is a finite union of $C^2$ curves $\Gamma_j$
in order to build a layer of global area $|\Omega_N^e| \leq CN^{-2}$, 
which results in the case $p=2$ into a contribution to the $L^p$ error
of the order $\cO(N^{-1})$. The area of the layer $\Omega_N^e$ 
is indeed of the same order as the area between the edge $\Gamma$
and its approximation by a polygonal line with $\cO(N)$ segments.

Each of the curves $\Gamma_j$
can be identified to the graph of a $C^2$ function
in a suitable orthogonal coordinate system.
If $\gamma$ is one of these functions, the area
between $\Gamma$
and its polygonal approximation can thus be 
locally measured by the $L^1$ error
between the one-dimensional function
$\gamma$ and a piecewise linear approximation
of this function.
Since $\gamma$ is $C^2$, it is obvious
that it can be approximated by a piecewise linear function on $\cO(N)$ intervals
with accuracy $\cO(N^{-2})$ in the $L^\infty$ norm and therefore
in the $L^1$ norm. However, we may ask whether such a rate
could be achieved under weaker conditions on the smoothness of $\gamma$.
The answer to this question is a chapter of {\it nonlinear} approximation theory
which identifies the exact conditions for a function $\gamma$ to be approximated
at a certain rate by piecewise polynomial functions on adaptive one-dimensional
partitions. We refer to \cite{De} for a detailed
treatment and only state the result which is of interest to us. We say that a function
$\gamma$ defined on a bounded interval $I$ belongs to the approximation
space ${\cal A}^s(L^p)$ if and only if there exists a sequence $(p_N)_{N>0}$ of functions where
each $p_N$ is piecewise affine on a partition of $I$ by $N$ intervals
such that 
$$
\|\gamma-p_N\|_{L^p} \leq CN^{-s}.
$$
For $0<s\leq 2$, it is known that 
$\gamma\in {\cal A}^s(L^p)$ provided that $\gamma\in B^{s}_{\tau,\tau}(I)$ with $\frac 1 \tau:=\frac 1 p+s$,
where $B^s_{\tau,\tau}(I)$ is the standard Besov space
that roughly describes those functions having $s$ derivatives in $L^{\tau}$.
In the case $s=2$ and $p=1$ which is of interest to us, we find $\tau=\frac 1 3$ and therefore $\gamma$ should
belong to the Besov space $B^2_{\frac 1 3,\frac 1 3}(I)$. Note that in our definition 
of cartoon functions, we assume much more than $B^2_{\frac 1 3,\frac 1 3}$ smoothness on $\gamma$,
and it is not clear to us if Theorem \iref{threg} can be derived under this minimal smoothness 
assumption. However it is striking to see that the quantity $E_2(f)$
that is revealed by Theorem \iref{threg} precisely measures the second derivative of the
arc-length parametrization of $\Gamma$ in the $L^{\frac 1 3}$ norm, up to
the multiplicative weight $|[f]|^{2/3}$. Let us also mention
that Besov spaces have been used in \cite{DPW} in order to describe
the smoothness of functions through the regularity of their level sets.
Note that edges and level sets are two distinct concepts, which
coincide in the case of piecewise constant cartoon functions.

The quantity $|\kappa|^{1/3}$ is also encountered in
mathematical image processing, for the design of
simple smoothing semi-groups that respect {\it affine invariance}
with respect to the image. Since these semi-groups should also
have the property of {\it contrast invariance}, they can be defined
through curve evolution operators acting on the level sets
of the image. The simplest curve evolution operator
that respects affine invariance is given by the equation
$$
\frac {d \Gamma}{d t}=-|\kappa|^{1/3}{\rm n},
$$
where ${\rm n}$ is the outer normal, see e.g. \cite{Ca}.
Here the value $1/3$ of the exponent plays a critical
role. The fact that we also find it in $E_2(f)$ suggests
that some affine invariance property also holds for this quantity
as well as for $A_2(f)$. 
We first notice that if $f$ is a compactly supported
$C^2$ function of two variables and $T$ is a 
bijective affine transformation, then with
$\ti f$ such that
$$
f=\ti f\circ T,
$$
we have
the property
$$
d^2 f(z)=L^\trans d^2 \ti f(Tz) L,
$$
where $L$ is the linear part of $T$ and $L^\trans$ its transpose, so that
$$
\sqrt {|\det (d^2f(z))|}=|\det L|\sqrt{|\det (d^2 \ti f(Tz))|}.
$$
By change of variable, we thus find that
\be
A_p(\ti f)=|\det L|^{1/\tau-1}A_p(f)=|\det L|^{1/p}A_p(f).
\label{invap}
\ee
A similar invariance property can be  derived on the interpolation error
$\sigma_N(f)_p=\|f-\interp_{\cT_N}f\|_{L^p}$ where $\cT_N$ is a triangulation which is optimally adapted
to $f$  in the
sense of minimizing the linear interpolation error in the $L^p$ norm
among all triangulations of cardinality $N$. We indeed remark that
an optimal triangulation for $\ti f$ is then given by applying $T$ to
all elements of $\cT_N$. For such a triangulation 
$\ti \cT_N:=T(\cT_N)$, one has the commutation formula
$$
\interp_{\cT_N}f=(\interp_{\ti \cT_N} \ti f)\circ T,
$$
and therefore we obtain by a change of variable that
\be
\sigma_N(\ti f)_p=\|\ti f-\interp_{\ti\cT_N}\ti f\|_{L^p}=|\det L|^{1/p}\|f-\interp_{\cT_N}f\|_{L^p}=|\det L|^{1/p}\sigma_N(f)_p.
\label{invsigmap}
\ee
Let us finally show that if $f$ is a cartoon function, then $E_2(f)$ satisfies a similar invariance property
corresponding to $p=2$, namely
\be
E_2(\ti f)=|\det L|^{1/2} E_2(f).
\label{inve2}
\ee
Note that this cannot be derived by arguing that $A_2(f)$ satisfies this
invariance property when $f$ and $\ti f$ are smooth, since we lose
the affine invariance property as we introduce the convolution by $\vp_\delta$: 
we do not have
$$
(f\circ T) * \vp_\delta = (f* \vp_\delta)\circ T.
$$
unless $T$ is a rotation or a translation. 

Let $\Gamma_j$ be one of the $C^2$ pieces of $\Gamma$
and  $\gamma_j: [0,B_i]\to \Omega$ a regular parametrisation of 
$\Gamma_j$. The curvature 
of $\Gamma$ on $\Gamma_j$ at the point $\gamma_j(t)$ is therefore given by
\be
\label{exprKappa}
\kappa(\gamma_j(t))= \frac{\det(\gamma_j'(t),\gamma_j'' (t))}{\|\gamma'_j(t)\|^{3}}
\ee
Since $f=\ti f\circ T$, the discontinuity curves of $\ti f$ are the images of those of $f$ by $T$:
$$
\ti \Gamma_j=T(\Gamma_j).
$$
The curvature of $\ti \Gamma_j$ at the point 
$T(\gamma_j(t))$ is therefore given by 
$$
\ti \kappa(T(\gamma_j(t))) = \frac{\det(L\gamma'_j(t), \ L\gamma''_j(t))}{\|L\gamma'_j(t)\|^3} = \det(L) \frac{\det (\gamma'_j(t),\gamma''_j(t))}{\|L\gamma'_j(t)\|^3} .
$$
This leads us to the relation : 
\be
\label{relKappa}
|\det(L)|^{1/3} |\kappa(\gamma_j(t))|^{1/3} \ \|\gamma'_j(t)\| =  |\ti\kappa(T(\gamma_j(t)))|^{1/3}
\|L\gamma'_j(t)\| ,
\ee
and therefore
\begin{eqnarray*}
\int_{\ti \Gamma_j} |[\ti f]|^{2/3} |\ti \kappa|^{1/3} &=& \int_0^{B_j}  |[\ti f](T(\gamma_j(t)))|^{2/3}
|\ti\kappa(T(\gamma_j(t)))|^{1/3} \ \|L\gamma'_j(t)\| dt,\\
&=& |\det L|^{1/3} \int_0^{B_j}  |[f](\gamma_j(t))|^{2/3} |\kappa(\gamma_j(t))|^{1/3} \  \|\gamma'_j(t)\|dt,\\
&=& |\det L|^{1/3} \int_{ \Gamma_i} |[ f]|^{2/3} |\kappa|^{1/3}.
\end{eqnarray*}
Summing over all $j=1,\cdots,l$ and elevating to the $3/2$ power
we obtain \iref{inve2}.

\section{Numerical tests}
\label{secCartoon5}

We first validate our previous results
by  numerical tests applied to a simple cartoon image:
the Logan-Shepp phantom. We use a $256\times 256$ pixel
version of this image, with a slight modification which is motivated
further. This image is iteratively smoothed
by the numerical scheme 
\be
\label{numSmoothing}
u_{i,j}^{n+1} = \frac {u_{i,j}^n} 2 + \frac {u_{i+1,j}^n+u_{i-1,j}^n+u_{i,j+1}^n+u_{i,j-1}^n} 8.
\ee
This scheme is an explicit discretization of the heat equation.
Formally, as $n$ grows,
$u^n$ is a discretization of 
\be
\label{Gaussian}
u * \vp_{\lambda \sqrt n} \text{ with } \vp_\delta (z) := \frac 1 { \pi\delta^2 } e^{-\frac {\|z\|^2}{\delta^2}},
\ee 
where $u$ stands for the continuous image. The determinant of the hessian 
is discretised by the following $9$-points formula
\be
\begin{array}{lll}
d_{i,j}^n &:=& (u_{i,j+1}^n-2u_{i,j}^n+u_{i,j-1}^n) (u_{i+1,j}^n-2u_{i,j}^n+u_{i-1,j}^n) \vspace{2mm}\\
& &\displaystyle- \frac {(u_{i+1,j+1}^n+u_{i-1,j-1}^n-u_{i+1,j-1}^n-u_{i-1,j+1}^n)^2}{16}
\end{array}
\label{ninepoint}
\ee
For each value of $n$, we then compute the $\ell^\tau$ norm of the array
$\left(\sqrt{|d^n_{i,j}|}\right)$ for $\tau \in [\frac 1 2,1]$, which corresponds to
$p\in [1,\infty]$ with $\frac 1 \tau := 1 + \frac 1 p$. This norm is thus a discretization of the quantity
$$
\left \|\sqrt{|\det(d^2(u*\vp_{\lambda \sqrt n}))|}\right \|_{L^\tau}.
$$
For each value of $n$ we obtain a function $\tau\in  [\frac 1 2,1]\to D_n(\tau) \in\R_+$.

As $n$ grows, three consecutive but potentially overlapping phases appear 
in the behaviour of the functions $D_n$, which are illustrated on Figure \ref{fig2Cartoon}.

\begin{enumerate}

\item For small $n$, the $9$-points discretisation is not a good approximation of the determinant of the hessian
due to the fact that the pixel discretization is too coarse compared to the 
smoothing width. During this phase, the functions $D_n$ decay rapidly for all values of $\tau$. 

\item For some range of $n$, the edges have been smoothed by the action of \iref{numSmoothing}, 
but the parameter $\lambda \sqrt n$ in \iref{Gaussian} remains rather small. Our previous analysis applies and we observe that $D_n(2/3)$ is (approximately) constant while $D_n(\tau)$ increases for 
$\tau < 2/3$ and decreases for $\tau > 2/3$. 

\item For large $n$, the details of the picture fade and begin to disappear. The picture begins to resemble a constant picture. Therefore the functions $D_n$ decay for all values of $\tau$, and eventually tend to $0$. 

\end{enumerate}


\begin{figure}
	\centering
		\includegraphics[width=5cm,height=5cm]{\pathPic/PaperCartoon/PicShepp.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=5cm]{\pathPic/PaperCartoon/PicSheppSimpler.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=5cm]{\pathPic/PaperCartoon/PicSmoothedShepp.pdf}
	\caption{\label{fig1Cartoon}The Logan-Shepp image (left), modified image (center), smoothed image (right).}
\end{figure}



\begin{figure}
	\centering
		\includegraphics[width=5cm,height=4cm]{\pathPic/PaperCartoon/PicBeginShepp.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=4cm]{\pathPic/PaperCartoon/PicMidShepp.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=4cm]{\pathPic/PaperCartoon/PicEndShepp.pdf}
	\caption{\label{fig2Cartoon}The curves $D_n(\tau)$ for $n\leq 50$ (left),
	$50\leq n\leq 100$ (center) and 
	$100\leq n\leq 200$ (right).}
\end{figure}


In our numerical experiments, we used the well known Shepp-Logan Phantom  with a slight modification
as shown on Figure \ref{fig1Cartoon}: we have removed the thin layer around the head, which represents the skull, 
because it disappears too quickly by the smoothing procedure
and causes phases 1 and 3 to overlap, masking phase 2.
For more complicated functions $f$, such as most photographic pictures, phases $1$ and $3$ 
also tend to overlap for similar reasons. 
Indeed, these pictures often have details at the pixel scale, including electronic noise due to the captor. 
Since these details disappear early phase 3 begins immediately, therefore phase 2 cannot be observed.\\

Our next discussion aims at comparing the quantities $A_2(f)$ with the
total variation $\TV(f)$ on numerical images. In particular, we want to compare how these quantities 
measure the geometric complexity of images. Here, we consider non-discretized images
$$
z=(x,y)\in [0,1]^2 \mapsto f(z),
$$
and we compare the numerical behaviour of  $A_2(f)$ and $\TV(f)$ for some relevant cases.
Let us recall that for any $g\in C^2(\R_+)$, if $f$ is the
radial function
$$
f(z)=g(|z|),
$$
one has 
$$
\det \left(d^2f (z)\right) = \frac 1 {|z|} g'(|z|) g''(|z|).
$$
As a result we find that the two functionals $\TV$ and $A_2^{2/3}$ behave similar 
on the oscillatory images $f_\omega(z):= \cos(\omega |z|)$ illustrated on Figure \ref{figTVDa} (left),
as $\omega \to +\infty$:
\be
\label{eqComplexaCos}
\TV( f_\omega ) \simeq \omega \stext{ and } A_2(f_\omega) \simeq \omega^{3/2}.
\ee
We next consider the cartoon images defined by 
$g_\omega(z) = \frac {\lfloor \omega |z|\rfloor} \omega$, which
have the form of a circular staircase with approximately $\omega$ steps of height $1/\omega$,
%more and more steps as $\omega$ grows,
as illustrated on Figure \ref{figTVDa} (center). 
In this case, we may give a meaning to $A_2(g_\omega)$ based on \iref{addita2}, 
which since $g_\omega$ is piecewise constant gives
$$
A_2(g_\omega)^{2/3}=C\int_\Gamma  |[g_\omega]|^{\frac 2 3} |\kappa|^{\frac 1 3},
$$
where $\Gamma$ are the circular curves of discontinuities. From this we find that
as $\omega\to +\infty$,
\be
\label{eqComplexaStair}
\TV(g_\omega) \simeq 1 \stext{ and } A_2(g_\omega) \simeq \sqrt \omega.
\ee
This shows that in contrast to $\TV$, the functional $A_2$ penalizes images which 
have the appearance of a staircase.

Finally we consider the cartoons functions $h_\omega(z)= \chi_{S_\omega}$ 
where the set $S_\omega$ is defined by
$$
S_\omega := \left\{z=(r\cos \theta, r \sin \theta) \sep 0 \leq \theta \leq \frac \cPi 2, \text{ and } 0 \leq r \leq 1 + \frac 1 \omega \cos(\omega \theta)\right\},
$$
see Figure \ref{figTVDa} (right). These functions have therefore only one step
but its geometry becomes more and more oscillatory as $\omega$ grows. More precisely 
its length remains finite, but its curvature behaves like $\omega$. In turn, we obtain
that as $\omega\to +\infty$,
\be
\label{eqComplexaFlower}
\TV(h_\omega) \simeq 1 \stext{ and } A_2(h_\omega) \simeq \sqrt \omega.
\ee
This shows that in contrast to $\TV$, the functional $A_2$ penalizes 
the fact that the curve of discontinuity $\partial S_\omega$ strongly oscillates.

These examples suggest that the functional $A_2$ 
gives a more relevant account of the complexity of cartoon images 
than the total variation $\TV$. In particular staircasing effects and 
oscillatory curves of discontinuity are penalized.\\

%\begin{figure}
%\centering
%\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Sina.pdf}
%\hspace{1cm}
%\includegraphics[height=4cm,width=4cm]{\pathPic/Bayesien/Staira.pdf}
%\hspace{1cm}
%\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Flowera.pdf}
%\caption{\label{figTVDa} Behavior of the functionals $\TV$ and $D=A_2^{2/3}$ on different types of images.}
%\end{figure}

\begin{figure}
\centering
\begin{tabular}[c]{ccc}
\includegraphics[height=3.5cm,width=5cm]{\pathPic/Bayesien/SinaNoText.pdf}
&\includegraphics[height=4cm,width=4cm]{\pathPic/Bayesien/StairaNoText.pdf}
&\includegraphics[height=3.5cm,width=5cm]{\pathPic/Bayesien/FloweraNoText.pdf}\\
 $\TV \simeq A_2^{2/3} \simeq \omega$
& $\TV \simeq 1$, $A_2 \simeq \sqrt \omega$
& $\TV \simeq 1$, $A_2 \simeq \sqrt \omega$
\end{tabular}
\caption{Some representatives of families $f_\omega$, $g_\omega$ and $h_\omega$ of images, and behavior of the functionals $\TV$ and $A_2$.\label{figTVDa}}
\end{figure}

%----------------------------------------------------------
%Image regularization based on a bayesian approach, specific to the thesis
%----------------------------------------------------------

\section{Applications to image restoration} %A Bayesian approach for
\label{secCartoon5.5}

The previous discussion suggests that we could use $A_2$ as an alternative
to $\TV$ as a prior in image restoration. In particular, we may try to replace $|g|_{BV}$
by $A_2(g)$ in \iref{minBV}, and therefore consider the minimization problem
$$
\min_{g} \{A_2(g)\; ; \; \|Tg-h\|_{L^2}\leq \e\},
$$
or its formulation using a Lagrange multiplier 
\be
\label{eqMinLagrange}
\min_g \|Tg-h\|_{L^2}^2 + t A_2(g)^{2/3}.
\ee
Our first observation is that, in contrast to \iref{minBV}, these problems are non-convex.

Moreover, it is easily seen that even in the very simple case of image denoising corresponding to 
$T=Id$, the above problems are ill-posed, in the following sense.

\begin{prop}
\label{propNotWellPosed}
For any $f\in L^2([0,1]^2)$, there exists a sequence $(f_n)_{n\geq 0}$ of $C^\infty$ functions
such that 
$$
\|f-f_n\|_{L^2}\to 0\;\;{\rm and}\;\; A_2(f_n) \to 0.
$$
Consequently the infimums of $A_2(g)$ over those $g\in C^\infty$ such that $\|g-h\|_{L^2}\leq \e$
and of $\|g-h\|_{L^2}^2 + t A_2(g)^{2/3}$ over all $g\in C^\infty$ are both equal to $0$, and are
not attained in general.
\end{prop}

\proof
If $\cT$ is a triangulation of the domain $[0,1]^2$, and if $g$ is piecewise affine on $\cT$,
we may consider its regularized version $g_\delta:=g*\vp_\delta$. From Theorem \ref{threg},
we find that $A_2(g_\delta)\to 0$ as $\delta \to 0$. The proof follows by observing that 
piecewise affine functions on triangulations are dense in $L^2$.
\sq

Note that the above result is formulated in the setting of non-discretized
images, and does not exactly hold for numerical images if we define $A_2$ 
using the $9$-points formula \iref{ninepoint} for the discretization of the 
determinant of the hessian. However, we expect that the ill-posedness
in the continuous setting is reflected by a bad behaviour of the solution
of the discrete optimization problem.

In summary, a straightforward generalization of the minimization
approach \iref{minBV} with $A_2$ in place of $\TV$ is doomed to fail.
In order to circumvent this difficulty, we propose a different strategy 
based on a restoration algorithm introduced in \cite{LMo}
and \cite{LMo2}. This algorithm is based on a bayesian framework that we briefely recall.

\subsection{A bayesian approach to image denoising} 

For simplicity, we focus from this point on the discrete setting, in which images are discretized on a $N \times N$ grid where $N\geq 1$.
%We consider the collection of discrete images $\cF$The collection of all discrete images is therefore the set 
We denote by 
$$
\cF := \R^{N \times N}.
$$
the collection of all discrete images. Bayesian restauration 
algorithms are based on a prior probability distribution on $\cF$ describing
how certain images are more ``plausible'' than others. One way to
build such priors is through a functional 
$$
J : \cF \to \R_+
$$
which reflects the plausibility of an image: typically
the value of $J$ is large for complex images and zero only for few very simple images. 
The functional $J$ is typically obtained as the discretization of a measure of smoothness, such as the total variation $\TV$ or the quantity $A_2^{2/3}$ (discretized with the nine points formula \iref{ninepoint}) which is shown in \S\ref{secCartoon5} to give a good account of the complexity of cartoon images. 

Assuming that the quantity %We assume in the following that the quantity 
$$
Z_J := \int_\cF \exp(-J(F)) dF
$$
is finite, our bayesian prior for \emph{plausible images} is the probability distribution
\be
\label{defProbaF}
\frac{e^{-J(F)}}{Z_J} dF
\ee
where $dF$ stands for the Lebesgue measure on $\cF$.

We use the simplistic, although popular, model of additive gaussian noise in which random drafts from $\cF$ with respect to the probability 
\be
\label{defProbaOmega}
\frac{e^{-\alpha\|\Omega\|^2}}{Z_\alpha} d\Omega,
\ee
where $\alpha>0$ is a parameter and $Z_\alpha$ is a normalizing factor, represent \emph{typical noise}.

We regard a \emph{corrupted image} $G$ as a random variable defined as the sum 
$$
G = F+\Omega
$$
of a random variable $F$ of distribution \iref{defProbaF}, the \emph{original image}, and a random variable $\Omega$ of distribution \iref{defProbaOmega}, the \emph{corruption} by additive gaussian noise.

By construction the conditional probability density $p(G|F)$ of the corrupted image $G$ with respect to the original image $F$ is 
$$
p(G|F) = \frac {e^{-\alpha\|\Omega\|^2}}{Z_\alpha} = \frac{e^{-\alpha\|G-F\|^2}}{Z_\alpha}.
$$
The conditional probability density $p(F|G)$ of the original image $F$ with respect to the corrupted one $G$ is obtained by the bayesian rule of conditional probabilities
$$
p(F|G)p(G) = p(G|F) p(F).
$$
Replacing $p(G|F)$ and $p(F)$ with their explicit expressions
we obtain 
\begin{eqnarray*}
p(F|G) &=&  \frac 1 {p(G)} p(G|F) \, p(F)\\
&=& \frac 1 {p(G)} \left(\frac 1 {Z_\alpha} e^{-\alpha \|G-F\|^2_2}\right) \left(\frac 1 {Z_J} e^{-J(F)} \right)\\
&=& \frac 1 {p(G) Z_\alpha Z_J} e^{-\alpha \|G-F\|^2_2 - J(F)}.
\end{eqnarray*}
We define
$$
\sigma(F,G) = \exp( -\alpha \|G-F\|^2_2 - J(F)).
$$ 
For any fixed $G$, 
the explicit function $F\in \cF \mapsto \sigma(F,G)\in \R_+^*$ 
is therefore proportional to the conditional probability density $F\mapsto p(F|G)$.

In order to recover the original image $F$ from the corrupted one $G$ a first approach, called the maximum a posteriori (MAP), consists in maximizing the conditional probability density %$F\mapsto p(F|G)$
\begin{eqnarray*}
F_J^* &:=& \underset {F\in \cF} \argmax \ p(F|G)\\
&=& \underset {F\in \cF}\argmax \ \sigma(F,G)\\
&=& \underset{F\in \cF}\argmin\ \alpha \|F-G\|^2 + J(F)
\end{eqnarray*}
We thus recover the optimization procedure \iref{eqMinLagrange} in the case $T=\Id$ of image denoising, and of the functionnal $J = A_2^{2/3}$. As observed in Proposition \ref{propNotWellPosed} this approach is doomed to fail for the functional $A_2^{2/3}$. For the total variation functional $J = \TV$, the MAP approach gives 
good results, but is also known to produce visual artifacts:  the restored image is exactly constant on large regions, delimited by sharp discontinuities which do not correspond to a feature of the original image.
The heuristical reason of this problem is that the maximum of a probability density is generally not a good representative of a random draft for this probability, as discussed in \cite{LMo}.

A second approach, called the minimum mean square error (MMSE), consists in finding $F$ which minimizes the empirical quadratic risk $\|F-F'\|^2$ with respect to a random image $F'$ distributed according to the conditional probability density $p(F'|G)$:
\begin{eqnarray*}
%\label{eqMMSE} 
%\vspace{5mm}
F_J &:=& \underset {F\in \cF} \argmin \int_\cF \|F-F'\|^2 \, p(F'|G) \, dF',\\
&=&\underset {F\in \cF} \argmin \int_\cF \|F-F'\|^2 \, \sigma (F',G) \, dF',\\
%\label{eqMoySigma}
&=& \frac 1 {Z} \int_\cF F\, \sigma(F,G) \, dF. 
\end{eqnarray*}
where 
$
Z = \int_\cF \sigma(F, G) \, dF
$ 
 is a normalizing factor. This method is studied in depth in \cite{LMo} in the case $J = \TV$ where it
 is shown that it has the advantage of suppressing the visual artifacts observed in the MAP approach, and we describe in the next section its adaptation to the case $J = A_2^{2/3}$.

\subsection{The restauration algorithm}
\label{secAlgoBayes}
%Expliquer l'algo.
%
%Interet : a-priori ne necessite pas la convexité, donc applicable a $J=A_2$
%
%Inconvenient: lenteur, actuellement ca marche pas bien.
%Pistes d'amélioration: parallellisme, traitement par groupes de pixel.

The computation of the estimator $F_J$ is a numerical challenge, since it involves an integration on the space $\cF = \R^{N \times N}$ which has dimension at least $512 \times 512 \simeq 250000$ in realistic cases.
We use an algorithm which was first proposed in the thesis \cite{LMo}, and which is a variation on the Metropolis Hastings algorithm. We shall only sketch its main principles and we refer to the original thesis for more details. 

The central point is to define a Markov chain $(F_k)_{k\geq 0}$ of images in $\cF$ which is recurrent with respect to the probability measure $\sigma(F,G) dF/Z$, where $G$ is the denoised image and $Z$ is a normalizing factor.
Then, almost surely,
\be
\label{eqConAvg}
\lim_{K\to \infty} \frac 1 K \sum_{0\leq k \leq K-1} F_k = \frac 1 Z \int_\cF F \, \sigma(F,G) \, dF.
\ee
Two successive images $F_k$ and $F_{k+1}$ generated by the algorithm proposed in \cite{LMo} only differ by the value of a single pixel. The cost of a step of the algorithm, generating a new image $F_k$, comes mainly from the computation of the ratio
\be
\label{eqRatioSigma}
\frac {\sigma(U,G)}{\sigma(V,G)} = \exp\( \|V-G\|^2 - \|U-G\|^2 +J(V) - J(U)\),%density function
\ee
where $U$ and $V$ are two elements of $\cF$ which differ at a single position $(i,j)$. 

This algorithm applies to any continuous functional $J \in C^0(\cF, \R_+)$, hence in particular to {\it non-convex functionals} such as $J=A_2^{2/3}$.
For numerical applications, in order to have a good speed of convergence, the ratio \iref{eqRatioSigma} needs to be extremely cheap to compute in terms of computer time. 
The discretisation of the total variation $\TV$ or of the functional $A_2^{2/3}$, are given for an image $F$ by respectively
$$
\frac 1 N \sum_{i,j} |F_{i,j}-F_{i+1,j}|+|F_{i,j} - F_{i,j+1}|\stext{ and } N^{-2/3} \sum_{i,j} |d_{i,j}|^\frac 1 3
$$
where $d_{i,j}$ is given by the formula \iref{ninepoint}.
The ratio \iref{eqRatioSigma} is cheap to compute numerically, as required by the algorithm, since it has an explicit algebraic expression which only involves the 
the values of the images $U,V\in \cF$ at the positions $(i+k, j+l)$ where $\max\{|k|, |l|\} \leq 2$, where $(i,j)$ denotes the single position at which these images differ.

From a theoretical point of view, the averaging procedure \iref{eqConAvg} converges at the speed $\cO(K^{-\frac 1 2})$. 
Unfortunately the \emph{constant} in front of the convergence rate plays a key role in practice, and we did not manage to ``reach the convergence'' for realistic $512 \times 512$ images with the functional $J = A_2^{2/3}$. This issue might be solved by a parallelization of the algorithm, or a modification of the algorithm in which a group of neighboring pixels is modified at each step instead of a single pixel. For the time being, we thus only present one-dimensional results.  


\subsection{Numerical illustration in the 1D case}

%We have developed our numerical Le modele 1D, $J(f)=..$.
%
%Justifier l'analogie (proposition 4.6.1 et figure 4.3)
%
%Tests numérique dans ce cas

We present numerical results in one dimension only, using some counterparts of the total variation $\TV$ and of the functional $A_2^{2/ 3}$ in that context.
We define for each function $f\in C^2([0,1])$ the quantity
\be
\label{defDf}
D(f) := \int_{[0,1]} \sqrt{|f''|}.
\ee
The next proposition shows that $D(f)$ can be given a meaning when $f$ has localized discontinuites, similarly to the functional $A_2^{2/3}$ for cartoon images.
\begin{prop}
Let $f : [0,1] \to \R$ be piecewise $C^2$, with a finite set $E$ of discontinuity points in $]0,1[$.
Let $\vp$ be a $C^2$ mollifier supported in $[-1,1]$, satisfying $\int_\R \vp = 1$ and $\vp(x) = \vp(-x)$ for all $x\in \R$. For all $\delta>0$ let $\vp_\delta := \frac 1 \delta \vp(\frac \cdot \delta)$ 
 and let $f_\delta := f* \vp_\delta$.
Then $f_\delta \in C^2([\delta, 1-\delta])$ and satisfies
\be
\label{defDDisc}
\lim_{\delta\to 0} \int_{[\delta, 1-\delta]} \sqrt{|f_\delta ''|} = \int_{]0,1[\sm E} \sqrt{|f''|} + C(\vp) \sum_{e\in E} \sqrt{|[f](e)|}
\ee
where $C(\vp) := \int_\R \sqrt{|\vp'|}$. 
\end{prop}

\proof
We denote by $0 <e_1< e_2 < \cdots< e_{n-1}< 1$ the points of $E$
and we define $e_0 = 0$ and $e_n = 1$.  
The function $f$ can written as the sum 
$$
f=J+A+S,
$$
where $J$ (the Jump part) is piecewise constant, and $A$ is continuous and piecewise Affine, 
with respect to the partition $\left(\, ]e_i,e_{i+1}[\,\right)_{0\leq i\leq n-1}$ of the interval $[0,1]$. % (up to the finite set of points $(e_i)_{0\leq i\leq n})$.
The function $S$ is $C^1$ on $]0,1[$, and $S''$ is uniformly bounded. 
Then, on the interval $[\delta, 1-\delta]$, 
$$
f_\delta = f*\vp_\delta = (J+A+S)*\vp_\delta %J*\vp_\delta + A*\vp_\delta+ S*\vp_\delta 
= J_\delta+ A_\delta+ S_\delta.
$$
We now assume that the parameter $\delta$ satisfies
$$
0< \delta <  \min_{0 \leq i \leq n-1} \frac{e_{i+1}-e_i} 2.
$$
For any $0 \leq i \leq n-1$ one has on the interval $[e_i+\delta,e_{i+1}-\delta]$
%Let us assume that $i\in \{0, \cdots , n-1\}$ and $\delta>0$ are such that  $2\delta <e_{i+1}-e_i$. Then
$$
J_\delta = J, 
\quad 
A_\delta = A
\stext{ and }
S_\delta = f_\delta - A- J.
$$
Hence $J_\delta'' = A_\delta'' = 0$, and $S_\delta'' = f_\delta''$ converges uniformly to $f''$ as $\delta \to 0$, on this interval. Therefore 
\be
\label{eqIntSmooth}
\lim_{\delta \to 0} \sum_{0 \leq i \leq n-1} \int_{e_i+\delta}^{e_{i+1}-\delta} \sqrt{|f_\delta''|} = \int_{]0,1[\sm E} \sqrt{|f''|}.
\ee
Furthermore for any $1\leq i\leq n-1$ and any $|x|\leq 1$ one easily checks that 
$$
J_\delta''(e_i+\delta x) = \frac 1 {\delta^2}[f](e_i) \, \vp'(x)
\stext{ and } 
A_\delta''(e_i+\delta x) = \frac 1 \delta [f'](e_i) \, \vp(x)
$$
where
$$
[f](e_i) := \lim_{\ve\to 0^+} f(e_i+\ve) - f(e_i - \ve) \stext{ and } [f'](e_i) := \lim_{\ve\to 0^+} f'(e_i+\ve) - f'(e_i-\ve).
$$
On the other hand $S''_\delta(e_i+ \delta x)$ is uniformly bounded independently of $x$ and $\delta$. Hence the contribution of $J_\delta''$ is dominant on the intervals $[e_i-\delta, e_i+\delta]$, and we obtain 
\be
\label{eqIntDisc}
\lim_{\delta\to 0} \sum_{1\leq i\leq n-1} \int_{e_i-\delta}^{e_i+\delta} \sqrt{|f_\delta''|} = \sum_{1\leq i \leq n-1} |[f](e_i)| \int_{-1}^1 \sqrt{|\vp'|}.
\ee
Combining \iref{eqIntSmooth} and \iref{eqIntDisc} we conclude the proof of this proposition.
\sq

For the simple oscillating function $f_\omega(x) := \cos(\omega x)$, illustrated on Figure \ref{figTVDf} (left), the two functionals $\TV$ and $D$ behave similarly as $\omega \to \infty$:
\be
\label{eqComplexfCos}
\TV( f_\omega) \simeq \omega \stext{ and } D(f_\omega) \simeq \omega.
\ee
On the contrary for the function $g_\omega(x) := \frac {\lfloor \omega x\rfloor} \omega$, illustrated on Figure \ref{figTVDf} (right) %, where $\lfloor x \rfloor$ is the integer part of $x$, 
we obtain as $\omega\to \infty$
\be
\label{eqComplexfStair}
\TV( g_\omega) \simeq 1 \stext{ and } D( g_\omega)\simeq \sqrt \omega,
\ee
where $D(g_\omega)$ is understood in the sense of \iref{defDDisc}.
Hence the functionals $\TV$ and $D$ treat discontinuities very differently, and the latter penalizes functions which have the appearance of a staircase. %, see Figure \ref{figTVDf} (right).

\begin{figure}
\centering
\includegraphics[height=3cm,width=4.5cm]{\pathPic/Bayesien/Sinf.pdf}
\hspace{1cm}
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Stairf.pdf}
\caption{ Behavior of the functionals $\TV$ and $D$ on different types of functions.\label{figTVDf}}
\end{figure}

We denote by 
$$
\cF := \R^N.
$$
the collection of discretized one-dimensional functions. For any $F\in \cF$, we denote by $\TV(F)$ and $D(F)$ the discretization of the functionals $\TV$ and $D$ using finite differences, as follows 
\be
\label{eqTVF}
\TV(F) := \sum_{1\leq i\leq N-1} |F_i - F_{i+1}|.
\ee
and 
\be
\label{eqDF}
D(F) := \sum_{2\leq i\leq N-1} \sqrt{|F_{i+1} - 2 F_i+ F_{i-1}|},
\ee

%We present and discuss in this section some one-dimensional numerical results. 
We now turn to numerical results. Given a one dimensional discretized function $F\in \cF := \R^N$ we compute using the algorithm described in \S \ref{secAlgoBayes} three different regularizations of $F$.
\begin{eqnarray*}
F_{\TV}^* &:= & \underset {F'\in \R^N} \argmin \ \alpha_1 \|F-F'\|^2+ \TV(F')\\
F_{\TV} &:= & \frac 1 {Z_2} \int_{\R^N} F' \exp(-\alpha_2 \|F-F'\|^2 - \beta_2 \TV(F') )dF'\\
F_{D} &:= & \frac 1 {Z_3} \int_{\R^N} F' \exp(-\alpha_3 \|F-F'\|^2 - \beta_3 D(F') )dF',\\
\end{eqnarray*}
where $Z_2$ and $Z_3$ are normalizing coefficients. The parameters $\alpha_1, \alpha_2, \alpha_3$ and $\beta_2, \beta_3$ can be freely chosen.

We have not attempted to denoise some data and to compare the $\PSNR$ of the restoration by the different methods.  Indeed such a comparison should, in order to be fair, involve an in depth analysis of the role of the parameters $\alpha_1, \alpha_2, \alpha_3$ and $\beta_2, \beta_3$, that we did not have the time to do. Note also that $F_{\TV}^*$ involves a single parameter, while two parameters are needed for $F_{\TV}$ and $F_D$. We refer to the thesis \cite{LMo} for the comparison of $F_{\TV}^*$ and $F_{\TV}$ from the point of view of the $\PSNR$.

Instead we regard the three procedures as regularization methods, that we apply to different test functions.
We focus on the qualitative differences of the regularizations $F_{\TV}^*$, $F_{\TV}$ and $F_D$ of different functions $F$, and we discuss on how these differences traduce the different bayesian priors implicit in the three methods. \\

\begin{figure}
	\centering
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/Noise.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/NoiseTVMap.pdf}\vspace{0.5cm}\\
	
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/NoiseTV.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/NoiseD.pdf}
	\caption{\label{figRandomWalk}Regularization of a random walk. (Top, Left) Original $F$, (Top, Right) $F^*_{\TV}$, (Bottom,Left) $F_{\TV}$, (Bottom, Right) $F_D$.}
\end{figure}

Our first experiment, see Figure \ref{figRandomWalk}, is the regularization of a random walk. As remarked in \cite{LMo}, $F_{\TV}^*$ is constant over large intervals and also has several sharp discontinuities. These two types of features were not present in the original function $F$ and are undesirable. They are avoided in the two other regularizations $F_{\TV}$ and $F_D$. \\%Qualitatively, $F_{\TV}$ and $F_D$ are not significantly different.

\begin{figure}
	\centering
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/Step.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/StepTVMap.pdf}\vspace{0.5cm}\\
	
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/StepTV.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/StepD.pdf}
	\caption{\label{figHeaviside}Heaviside function. (Top, Left) Original $F$, (Top, Right) $F^*_{\TV}$, (Bottom,Left) $F_{\TV}$, (Bottom, Right) $F_D$.}
\end{figure}

Our second experiment, see Figure \ref{figHeaviside} is the regularization of a Heaviside function. Up to numerical artifacts, the functions $F$ and $F_{\TV}^*$ are identical, which is precisely what is wanted in this situation.
The discontinuity disappears in $F_{\TV}$ and $F_D$, and is replaced with a smooth but sharp and well localized transition. Numerical experiments on real (bidimensional) images in \cite{LMo} show that generally, and with appropriate parameters, the regularization $F_{\TV}$ of an image $F$ does not cause a perceptible blurring of the edges which appear in the original image. 

This example puts in light a strong flaw of the regularization method $F_D$ : it does not obey the maximum principle. Indeed, it is clear on Figure \ref{figHeaviside} that $F_{\TV}^*$ and $F_{\TV}$ take their values in the interval $[\min F, \max F]$, but $F_D$ does not.\\


\begin{figure}
	\centering
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/Churp.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/ChurpTVMap.pdf}\vspace{0.5cm}\\
	
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/ChurpTV.pdf}\hspace{0.5cm}
	\includegraphics[height = 3.5cm, width = 5cm]{\pathPic/bayesien/ChurpD.pdf}
	\caption{\label{figChurp}Churp : $\sin(x^3)$ where $x\in [0,4]$. (Top, Left) Original $F$, (Top, Right) $F^*_{\TV}$, (Bottom,Left) $F_{\TV}$, (Bottom, Right) $F_D$.}
\end{figure}

Our third and last experiment, see Figure \ref{figChurp} is the regularization of a ``Churp'' : an oscillating function of increasing frequency, here $\sin (x^3)$ where $x\in [0,4]$.
Qualitatively, most regularization algorithms regard slow oscillations as valuable data which should be preserved, and fast oscillations as noise which should be eliminated. The regularization of a churp allows to analyse the behavior of a regularization algorithm in the intermediate regimes.

From a qualitative point of view, the MAP regularization $F_{\TV}^*$ again introduces undesirable visual artefacts : $F_{\TV}^*$ is exactly constant on some regions, and $\nabla F_{\TV}^*$ has sharp discontinuities which do not correspond to a feature of the original function. In contrast the MMSE regularizations $F_{\TV}$ and $F_D$ do not exhibit these artefacts. As anticipated, the slow oscillations of the original function $F$ are preserved, while the fast oscillations are attenuated. It seems qualitatively that fast oscillations are more strongly attenuated in $F_D$ than in $F_{\TV}$. The author could not prove this last property, but a heuristical analysis suggests that sinuosidal oscillations of large frequency $\omega\gg 1$ are attenuated by a factor $\omega^{-2}$ in 
$F_{\TV}$ and $\omega^{-4}$ in $F_D$.



%----------------------------------------------------------
%Back to original paper
%----------------------------------------------------------
\section{Extension to higher dimensions and higher order elements}
\label{secCartoon6}
The results on approximation by anisotropic bidimensional piecewise linear
finite elements that we have exposed in \S \ref{secCartoon2} have been generalized in Chapter \ref{chapOptAniso}
to the case of elements of arbitrary order $m-1$
defined on partitions of $\Omega\subset \RR^d$ by simplices.
Here, the local error is defined as
$$
e_{m,T}(f)_p:=\|f-\interp^{m-1}_T f\|_{L^p(T)},
$$
where $\interp^{m-1}_T$ denotes the local interpolation operator
on $\P_{m-1}$ for a $d$-dimensional simplex $T$. This operator
is defined by the condition
$$
\interp^{m-1}_T v(\gamma)=v(\gamma),
$$
for all points $\gamma\in T$ with barycentric coordinates in
the set $\{0, \frac 1 {m-1},\frac 2 {m-1},\cdots,1\}$. We denote by $\H_m\subset \P_m$ the collection of homogeneous polynomials of degree $m$, and we define for any $\bq\in \H_m$ the quantity
$$
K_{m,p}(\bq):=\inf_{|T|=1}e_{m,T}(\bq)_p.
$$
We refer to $K_{m,p}$ as the {\it shape function}. 
For piecewise linear elements in dimension two, i.e. $m=d=2$, 
we have observed that $K_p=K_{2,p}$ has the
special form given by \iref{Kpexp} which justifies the
introduction of the quantity $A_p(f)$. In a similar way, it can 
easily be proved that for piecewise linear elements in higher dimension,
i.e. $m=2$ and $d>2$, one has
$$
c_1 |{\rm det} (\bq)|^{1/d}\leq K_{2,p}(\bq) \leq  c_2 |{\rm det} (\bq)|^{1/d}.
$$
For piecewise quadratic elements in dimension two, i.e. $m=3$ and $d=2$, 
it is proved in Chapter \ref{chapOptAniso} that
$$
c_1 |{\rm disc} (\bq)|^{1/4}\leq K_{3,p}(\bq) \leq  c_2 |{\rm disc} (\bq)|^{1/4}.
$$
for any {\it homogeneous} polynomial $\bq\in \H_3$, where
$$
{\rm disc}(a x^3+ b x^2 y+ c x y^2+ d y^3):= b^2 c^2 - 4 a c^3 - 4 b^3 d + 18 a b c d - 27 a^2 d^2.
$$
For other values of $m$ and $d$, equivalent expressions
of $K_{m,p}(\bq)$ in terms of polynomials in the coefficients of $\bq$
are available but of less simple form, see Chapter 2.

Defining the finite element interpolation error by an optimally adapted partition
$$
\sigma_N(f)_p:=\inf_{\#(\cT)\leq N}\|f-\interp^{m-1}_\cT f\|_{L^p},
$$
where $\interp^{m-1}_\cT$ is the global interpolation operator for the 
simplicial partition (possibly non conforming) $\cT$, the following generalization of 
\iref{limsupest1} is proved in Chapter \ref{chapOptAniso}:
\be
\limsup_{N\to +\infty} N^{\frac m d}\sigma_N(f)_p\leq C_d\left\|K_{m,p}\(\frac {d^mf}{m!}\)\right\|_{L^\tau(\Omega)},
\;\; \frac 1 \tau=\frac 1 p+\frac m d.
\label{limsupest2}
\ee
The constant $C_d$ is equal to $1$ when $d=2$ but larger
than $1$ when $d>2$ due to the impossibility of exactly tiling the
space with locally optimized simplices.
If $f$ is a $C^m$ function of $d$ variables, it is therefore natural to 
consider the quantity 
\be
A_{m,p}(f):=\|K_{m,p}(d^m f)\|_{L^\tau(\Omega)},
\;\; \frac 1 \tau=\frac 1 p+\frac m d,
\ee
as a possible way to measuring anisotropic smoothness. For $d=2$ and piecewise
linear elements, we have seen in \S \ref{secCartoon2} that $A_{2,p}(f)$ is equivalent to the quantity $A_p(f)$.

Similarly to $A_p$ we are interested in the possible extension of $A_{m,p}$
to cartoon functions. We first introduce a generalisation 
of the notion of cartoon functions to higher piecewise smoothness $m$ and dimension $d$.
\begin{definition} 
\label{defcartoongen}
Let $m\geq 2$ and $d\geq 2$ be two integers. Let $\Omega\subset \R^d$ be an open set.
We say that a function $f$ defined
on $\Omega$ is a $C^m$ cartoon function if it is almost everywhere of the form 
$$
f=\sum_{1\leq i\leq k} f_i \Chi_{\Omega_i},
$$
where the $\Omega_i$ are disjoint open sets with piecewise $C^2$ boundary, no cusps (i.e. satisfying an interior and exterior cone condition), and such that $\overline \Omega = \cup_{i=1}^k \overline \Omega_i$.
Additionally, for each $1\leq i\leq k$, the function $f_i$ is assumed to be $C^m$ on $\overline \Omega_i$. %a neighbourhood of
\end{definition}

Let us consider a fixed cartoon function $f$ on a polyhedral domain $\Omega\subset\R^d$ (i.e. $\Omega$ is
such that $\overline \Omega$ is a closed polyhedron), and a decomposition 
$(\Omega_i)_{1\leq i\leq k}$ of $\Omega$ as in definition \ref{defcartoongen}. As before we define 
$ 
\Gamma := \bigcup_{1\leq i\leq k} \partial \Omega_i,
$
the union of the boundaries of the $\Omega_i$. Our assumptions on the sets $(\Omega_i)_{1\leq i\leq k}$ imply that $\Gamma$ 
is the union of a finite number of open hypersurfaces $(\Gamma_j)_{1\leq j\leq l}$, and of a set $\cP$ of dimension $d-2$.

As in \S \ref{secCartoon3}, we now consider a sequence $f_N$ of piecewise linear approximations of $f$ on 
simplicial partitions $\cT_N$ of cardinality $N$. We distinguish two types of elements of $\cT_N$. A simplex $T\in \cT_N$ is called ``regular'' if $T\cap \Gamma=\emptyset$, and we denote the set of these simplices by $\cT_N^r$. Other simplices are called ``edgy'' and their set is denoted by $\cT_N^e$.
We can again split $\Omega$ according to
$$
\Omega:=(\cup_{T\in \cT_N^r}T) \cup (\cup_{T\in \cT_N^e}T)=\Omega_N^r \cup \Omega_N^e.
$$
Heuristically, if the partitions $\cT_N$ are built with approximation error minimisation in mind, the number of elements should be balanced between $\cT_N^r$ and $\cT_N^e$. The partition $\cT_N^r$ tends to cover most of the surface of $\Omega$, with simplices of diameter $\leq C  N^{-\frac 1 d}$, and $L^\infty$ approximation error $|f-f_N|\leq C N^{-\frac m d}$ (since we use $\P_{m-1}$ elements).
On the other hand, since $f$ has discontinuities along $\Gamma$, the $L^\infty$ approximation error on $\cT_N^e$ does not tend to zero, and $\cT_N^e$ should thus be chosen so as to produce a thin layer around $\Gamma$. 
Let $h$ be the typical diameter of an element of $\cT_N^e$. Since the $\Gamma_j$ has
bounded curvature, this layer can be made of width $\cO(h^2)$
and therefore the layer around $\Gamma$ has volume bounded by
$h^2 \cH_{d-1}(\Gamma)$  up to a fixed multiplicative constant, 
where $\cH_{d-1}(\Gamma)$ is the $d-1$ dimensional
Hausdorff measure of $\Gamma$. On the other hand the minimal number of 
such elements of diameters $h$ needed to cover $\Gamma$ is 
bounded by $h^{1-d}\cH_{d-1}(\Gamma)$ up to a fixed multiplicative constant.
Eventually, we find that the layer around $\Gamma$ has volume bounded by $C N^{-\frac 2 {d-1}}$. 

Hence we have the following heuristic error estimate, for a well designed anisotropic partition:
\begin{eqnarray*}
\|f-f_N\|_{L^p(\Omega)} &\leq& \|f-f_N\|_{L^p(\Omega_N^r)} +\|f-f_N\|_{L^p(\Omega_N^e)}\\
&\leq& \|f-f_N\|_{L^\infty(\Omega_N^r)} |\Omega_N^r|^{\frac 1 p}+  \|f-f_N\|_{L^\infty(\Omega_N^e)} |\Omega_N^e|^{\frac 1 p}\\
& \leq & C (N^{-\frac m d}  + N^{\frac {-2} {p (d-1)}})
\end{eqnarray*}
This leads us to define a critical exponent
$$
p_c = p_c(m,d):=\frac{2d}{m (d-1)}.%, \text{ equivalently } 1 = \frac 1 d + \frac 2 {m p_c(m,d)}.
$$
If one measures the error in $L^p$ norm with $p>p_c(m,d)$, then the contribution of the edge neighbourhood
$\Omega_N^e$ dominates, while if $p<p_c(m,d)$ it is negligible compared to the contribution
of the smooth region $\Omega_N^r$. 
For the critical exponent $p=p_c(m,d)$ the two terms have the same order, which makes the situation more interesting. Note in particular that $p_c(2,2) =2$, which is consistent with our previous analysis.

For $p\leq p_c(m,d)$, we obtain the approximation rate $N^{-m/d}$ which suggests that approximation
results such as \iref{limsupest2} should also apply to cartoon functions and that the 
quantity $A_{m,p}(f)$ should be finite for such functions. We again need to
use a regularization approach, for the same reasons as in \S \ref{secCartoon3}.
For a given dimension $d$, we consider a radial nonnegative function $\vp$ 
of unit integral and supported in the unit ball of $\R^d$, and we define for $\delta >0$
\be
\vp_\delta(z) := \frac 1 { \delta^d} \vp\left(\frac z \delta\right) \stext{ and } f_\delta = f * \vp_\delta.
\ee

In order to define the quantities of involved in our conjecture, we need to introduce the second fundamental form of an hypersurface.
At any point $x\in \Gamma\sm \cP$ we denote by $\bn(x)$ the unit normal to $\Gamma$. Note that since 
$\Gamma$ is piecewise $C^2$, the map $x\mapsto \bn(x)$ is 
$C^1$ on $\Gamma\sm \cP$.
We define $T_x\Gamma := \bn(x)^\perp$, the tangent space to $\Gamma$ at $x$.
In a neighbourhood of $x\in \Gamma\sm \cP$, the hypersurface $\Gamma$ admits a parametrization of the form
$$
u\in T_x\Gamma \mapsto x + u+ \lambda(u) \bn(x) \in \Gamma \sm \cP,
$$
where $\lambda$ is a scalar valued $C^2$ function.
By definition, the second fundamental form of $\Gamma$ at the point $x$ is the quadratic form $\II_x$ associated
to $d^2\lambda(0)$ which is defined on $T_x \Gamma\times T_x \Gamma$.
Alternatively, for all $u,v\in T_x\Gamma$ we have $\II_x(u,v) := -\<\partial_u \bn, v\>$.
The Gauss curvature $\kappa(x)$ is the determinant of $\II_x$, in any orthonormal basis of $T_x \Gamma$,
$$
\kappa(x):= \det \II_x.
$$
For example, in two space dimensions the tangent space $T_x\Gamma$ is one dimensional, and we simply have 
$\II_x(u,v) = \kappa(x) \<u,v\>$.
We also denote by $\sigma(x)\in \{0, \cdots, d-1\}$ the signature of the quadratic form $\II_x$, which is defined as the number of its positive eigenvalues. 

With $\tau$ such that $\frac 1 \tau :=\frac m d+\frac 1 p$, we 
define
$$
S_p(f) :=  \|K(d^m f )\|_{L^\tau(\Omega\sm \Gamma)}=A_p(f_{|\Omega\sm \Gamma}).
$$
We conjecture the following generalization to Theorem \ref{threg}.

\begin{conjecture}
There exists $d$ positive constants $C(k)$, $k\in \{0,\cdots, d-1\}$, that depend on  $\vp,p,m,d$, such that,
with 
$$
E_p(f):= \| C(\sigma) |\kappa|^{\frac m {2d}} [f] \|_{L^\tau(\Gamma)}=
\(\int_\Gamma \left |C(\sigma(x)) |\kappa(x)|^{\frac m {2d}} [f(x)] \right |^\tau dx\)^{\frac 1 \tau},
$$
we have
\label{thAmdp}
\begin{itemize}
\item If $p<p_c$ then 
$$
\lim_{\delta\to 0} A_{m,p}(f_\delta) = S_p(f).
$$ 
\item If $p=p_c$ then 
$$
\lim_{\delta \to 0} \left(A_{m,p}(f_\delta)\right)  = \left(S_p(f)^\tau +  E_p(f)^\tau\right)^{1/\tau}.
$$ 
\item If $p>p_c$ then
$$
\lim_{\delta \to 0}  \delta^{\frac 1 {p_c} - \frac 1 p} A_{m,p}(f_\delta) =  E_p(f).
$$ 
\end{itemize}
\end{conjecture}

In the remainder of this section, we give some 
arguments that justify this conjecture. Given a cartoon function $f$, 
we define the sets $\Omega_\delta$, $\Gamma_\delta^0$, 
$\Gamma_\delta$ and $\cP_\delta$ similarly to \S \ref{secCartoon3}.
We need to perform an asymptotic analysis of the integral
\be
\label{tointegrate}
\int_\Omega K(d^m f_\delta)^\tau = \int_{\Omega_\delta} K(d^m f_\delta)^\tau+\int_{\cP_\delta} K(d^m f_\delta)^\tau
+\int_{\Gamma_\delta} K(d^m f_\delta)^\tau.
\ee
As in the proof of Theorem \ref{threg} the contribution of $\cP_\delta$ can be proved to be negligible 
compared with those of $\Omega_\delta$ and $\Gamma_\delta$ as $\delta \to 0$. The contribution of
$\Omega_\delta$ satisfies
$$
\lim_{\delta \to 0} \int_{\Omega_\delta} K(d^m f_\delta)^\tau =\int_{\Omega\sm \Gamma} K(d^m f)^\tau.
$$ 
The main difficulty lies again in the contribution of $\Gamma_\delta$. Let us define $\tau_c$ by 
$$
\frac 1 {\tau_c} := \frac m d+ \frac 1 {p_c}.
$$
The contribution of $\Gamma_\delta$ can be 
computed if one can establish an estimate generalizing \iref{estimK2d} according to 
\be
\label{estimK}
\left|  \delta^{\frac 1 {\tau_c}} K_{m,p}(d^m f_\delta(z)) - |[f](x)| |\kappa(x)|^{\frac m {2 d}} \Phi_{m,d,\sigma(x)}(u) \right|\leq \omega(\delta)
\ee
where $\omega(\delta)\to 0$ as $\delta\to 0$, $x\in \Gamma_\delta^0$, $u\in [-1,1]$, $z = x+\delta u \bn(x)$,
and where the function $\Phi_{m,d,k} : [-1,1]\to \R$ only depends on $m,d,k$ and $\vp$. If
\iref{estimK} holds, we then easily derive that
$$
\lim_{\delta \to 0} \delta^{\frac {\tau}{\tau_c}-1}\int_{\Gamma_\delta} K(d^m f_\delta)^\tau=\int_\Gamma C(\sigma) |\kappa|^{\frac {\tau m} {2d}} |[f]|^\tau,
$$
with $C(k):=\int_{-1}^1|\Phi_{m,d,k}(u)|^\tau du$, which leads to the proof of the conjecture.

We do not have a general proof of \iref{estimK} for any $m$, $p$ and $d$. 
In the following, we justify its validity in
two particular cases for which the explicit expression of $K_{m,p}$ is known to us:
piecewise quadratic in two space dimensions ($d=2$ and $m=3$)
and piecewise linear  in any dimension ($m=2$).

\paragraph{Piecewise quadratic elements in two dimensions.}
For all $\delta>0$, $x\in \Gamma_\delta^0$ and $u\in [-1,1]$, let $\pi_{x,\delta,u}\in \H_3$
 be the homogeneous cubic polynomial on $\R^2$ corresponding to $d^3 f_\delta (x+\delta u \bn(x))$.
Let also $\pi_{x,u}\in \H_3$ be the homogeneous cubic polynomial on $\R^2$ defined by 
\be
\label{eqThirdCartoon}
\pi_{x,u}(\lambda \bn(x)+\mu \bt(x)) = -\lambda(\Phi''(u) \lambda^2- 3\Phi'(u) \kappa(x) \mu^2)
\ee
for all $(\lambda,\mu)\in \R^2$, where $\Phi$ is defined
by \iref{defchi}. For all $x\in \Gamma$, we denote by $M_{x,\delta}$ the (symmetric) linear map defined by 
$$
M_{x,\delta}\bn(x) = \delta \bn(x) \text{ and } M_{x,\delta} \bt(x)= \sqrt \delta \bt(x).
$$
Then, using a reasoning similar to the one used in the appendix of this chapter, it can be proved that
\be
\label{limdiscD}
\|\pi_{x,\delta,u} \circ M_{x,\delta} -[f](x)\pi_{x,u}\|\leq \omega(\delta).
\ee
where $\lim_{\delta\to 0} \omega(\delta) = 0$ and the function $\omega$ depends only on $f$.
Furthermore, it is proved in Chapter \ref{chapOptAniso} that for all $\bq\in \H_3$
$$
K_{3,p}(\bq) = C \sqrt[4]{|\disc \bq|}
$$
where the positive constant $C$ depends on $p$ and the sign of $\disc \bq$. Combining this expression with \iref{limdiscD} proves \iref{estimK} and thus the conjecture in the case $m=3$ and $d=2$.


\paragraph{Piecewise linear elements in any dimension.} We use the second 
fundamental form of the discontinuity set $\Gamma$ in order to evaluate
$d^m f_\delta$ on $\Gamma_\delta$.
Characteristic functions are one of the simplest types of cartoon functions. In that case, it is possible
to establish a simple relation between the second fundamental form of
the edge set and the second derivatives of $f$ in a distributional sense:
if $\Omega\subset \R^d$ is a bounded domain with smooth boundary $\Gamma$ and inward normal $\bn$,
we then have for all $C^2$ test function $\psi$ and $u,v\in \R^d$ 
\be
-\int_\Omega \partial^2_{u,v}\psi = \int_\Gamma \<u,\bn\>\<v,\bn\> (\partial_\bn \psi - \Tr(\II) \psi) +\II'(u,v)\psi,
\label{d2charR2eqd}
\ee
where $\II'_x(u,v)$ is the second fundamental form $\II_x$ applied to the orthogonal projection of $u$ and $v$ on $T_x\Gamma$.
The proof of this formula (that generalizes the simpler bidimensional case \iref{d2charR2eq} which is proved in the appendix) is given further below. For all $x\in \Gamma$, 
we denote by $M_{x,\delta}$ the (symmetric) linear map defined by 
$$
M_{x,\delta}\bn(x) = \delta \bn(x) \text{ and } M_{x,\delta} \bt = \sqrt \delta \bt  
$$
for all $\bt\in T_x\Gamma$.
For all $\delta>0$, $x\in \Gamma_\delta^0$ and $u\in [-1,1]$, let $\pi_{x,\delta,u}\in \H_2$ be the homogeneous quadratic polynomial on $\R^d$ corresponding to $d^2 f_\delta (x+\delta u \bn(x))$.
Let also $\pi_{x,u}\in \H_2$ be the homogeneous quadratic polynomial on $\R^d$ defined by 
$$
\pi_{x,u}(\lambda \bn(x)+\bt) = \Phi'(u) \lambda^2- \Phi(u) \II_x(\bt,\bt)
$$
for all $\lambda\in \R$ and $\bt\in T_x \Gamma$, where $\Phi(x):=\int_{\R^{d-1}}\vp(x,y)dy$.
Then, using \iref{d2charR2eqd} and a reasoning analogous to the one presented in the appendix, 
it can be proved that 
\be
\label{limQuadD}
\|\pi_{x,\delta,u} \circ M_{x,\delta} -[f](x)\pi_{x,u}\|\leq \omega(\delta).
\ee
where $\lim_{\delta\to 0} \omega(\delta) = 0$ and the function $\omega$ depends only on $f$.
Furthermore, it is proved in Chapter \ref{chapOptAniso} that 
$$
K_{2,p}(\bq) = C \sqrt[d]{|\det \bq|}
$$
where the positive constant $C$ depends on $d,p$ and the signature of $\bq\in \H_2$. Combining this expression with \iref{limQuadD} proves the estimate \iref{estimK} and thus the conjecture in the case $m=2$ in any dimension $d>1$.
\nl
\nl
{\bf Proof of \iref{d2charR2eqd}:}
Let $\proj_\Gamma$ be the orthogonal projection onto $\Gamma$, and for all $x\in \Gamma$ let $\proj_x$ be the orthogonal projection onto $T_x\Gamma$. 
We consider a vector $u\in \R^d$ and we define $\move : \Gamma\to\Gamma$ by $\move (x) := \proj_\Gamma(x+u)$. If $\|u\| \|\II\|_{L^\infty(\Gamma)}<1$, then $\move$ is smooth and its differential $d_x \move : T_x\Gamma\to T_{x'}\Gamma$, where 
$$
x' = \move(x),
$$ 
is given by the following formula
$$
d_x \move = (\Id - \<u, \bn(x')\>\II_{x'})^{-1} \proj_{x'} 
$$
The determinant of $d_x U$ (more precisely the determinant of the matrix of $d_x U$ in direct orthogonal bases of $T_x\Gamma$ and $T_{x'} \Gamma$) is 
$$
\det (d_x \move) = \det(\Id - \<u, \bn(x')\>\II_{x'})^{-1}\<\bn(x),\bn(x')\> = 1+\<u, \bn(x')\> \Tr(\II_{x'})+ \|u\|\omega_1(u,x).
$$
where %$\|\omega_u(x)\|_{L^\infty(\Gamma)} \to 0$ as $u \to 0$.
$\omega_1(u,x)$ tends uniformly to $0$ as $u\to 0$.
Furthermore, it is easy to show that 
$$
|\psi(x+u) - \psi(x') -  \<u, \bn(x)\> \partial_{\bn(x')} \psi(x')|\leq C\|u\|^2,
$$
and $\|n(x') - n(x) - \II_{x'}(\proj_{x'}(u))\|\leq \|u\|\omega_2(u)$, where $C$ and $\omega_2$ are independent of $x\in \Gamma$ and $\omega_2(u) \to 0$ as $u \to 0$ (the quadratic form $\II_x(r,s) := -\<\partial_r \n(x),s\>$ for all $r,s\in T_x\Gamma$ is identified here to the differential of $\n$). Combining these results, we obtain
\begin{eqnarray*}
& &\int_\Gamma \psi(x+u)\<\bn(x),v\> dx\\
&=& \int_\Gamma \psi(x+u)\<\bn(x),v\> \det (d_{x'} \move_u)^{-1} dx'\\
&=&\int_\Gamma \<\bn(x'), v\> \psi(x')dx'\\
& &+ \int_\Gamma \<\bn(x'), v\> \<\bn(x'),u\>(\partial_{\bn(x')} \psi- \Tr(\II_x')\psi(x'))
 +\<v,\II_x'(\proj_{x'}(u))\>\psi(x') dx' \\
& &+ \|u\|\omega_3(u).
\end{eqnarray*}
where $\omega_3(u)\to 0$ as $u \to 0$.
We conclude the proof of \iref{d2charR2eqd} using the formula
$$
- \int_\Omega \partial^2_{u,v}\psi = \lim_{h\to 0} h^{-1}\int_\Gamma (\psi(x+hu)-\psi(x))\<\bn(x),v\> dx.
$$ %this concludes the proof.
\sq

\begin{remark}
Similarly to the results presented in \S \ref{secCartoon4}, there is an affine invariance property associated to $\kappa$: if $T$ is an affine transformation of $\R^d$ with linear part $L$, 
and if $f = \ti f\circ T$, $\ti \Gamma = T(\Gamma)$ and $\ti \kappa$ is the Gauss curvature of $\ti \Gamma$, then
one has for any $s \geq 0$, 
$$
(\det L)^{\frac{d-1}{d+1}}\int_\Gamma |C(\sigma) [f]|^s |\kappa|^{\frac 1 {d+1}} = \int_{\ti\Gamma} |C(\ti \sigma)[\ti f]|^s |\ti \kappa|^{\frac 1 {d+1}}.
$$
It follows from this observation that when $p=p_c$, the contribution of the edges is affine invariant in the sense
that 
$$
E_{p_c}(\ti f) = (\det L)^{\frac {d-1}{d+1}} E_{p_c}(f).
$$
Since one also has $A_{m,p}(\ti f) = (\det L)^{\frac {d-1}{d+1}} A_{m,p} (f)$ this comforts the conjecture.
Let us mention that the quantity $|\kappa|^{\frac 1 {d+1}}$ has been used in \cite{Ol} 
in order to define surface smoothing operators that are invariant under affine change of coordinates.
\end{remark}

\section{Conclusion}
\label{secCartoon7}
In this chapter we have investigated the quantity $A_p(f)$ which
governs the rate of approximation by anisotropic $\P_1$ finite elements as a way to
describe anisotropic smoothness of functions. This quantity is not a semi-norm
due to the presence of the non-linear quantity $\det(d^2f)$ 
and cannot be defined in a straightforward manner for general distributions.
We nevertheless have shown that this quantity can be defined
for cartoon images with geometrically smooth edges when $p\leq 2$.
A theoretical issue remains to give a satisfactory meaning to 
the full class of functions for which this quantity is finite.

From a more applied perspective, it could be interesting to
investigate the role of $A_p(f)$ in problems where anisotropic
features naturally arise: 

\begin{enumerate}
\item
Approximation of PDE's: in the case of one dimensional hyperbolic conservation laws, it was proved
in \cite{DLu} that despite the appearance of discontinuities
the solution has high order smoothness in Besov spaces
that govern the rate of adaptive approximation by piecewise polynomials.
A natural question is to ask wether similar results hold
in higher dimension, which corresponds to understanding
if $A_p(f)$ remains bounded despite the appearance of shocks.
\item
Image processing: as illustrated in \S \ref{secCartoon5}, the quantity $A_p(f)$ can easily be discretized
and defined for pixelized images. It is therefore tempting to use
$A_2(f)$ in a similar way
as the total variation in \iref{minBV}, by solving a problem of the form
\be
\min_{g\in BV} \{A_2(g)\; ; \; \|Tg-h\|_{L^2}\leq \e\},
\label{minA2}
\ee
with the objective of promoting images with piecewise smooth edges. The main
difficulty is that $A_2$ is not a convex functional. One way to solve this
difficulty could be to reformulate \iref{minA2} in a Bayesian framework as the search of a maximum
of an a-posteriori probability distribution (MAP) as an estimator of $f$. In this framework, we
may instead search for a minimal mean-square error estimator (MMSE),
and this search can be implemented by stochastic algorithms which
do not require the convexity of $A_2$, see \cite{LMo} and \S\ref{secCartoon5.5}.
\end{enumerate}


\section{Appendix: proof of the estimates \iref{estimnn2d}-\iref{estimnt2d}-\iref{estimtt2d}.}

It is known since
the work of Whitney on extension theorems 
(see in particular \cite{Whitney}) 
that for any open set $U\subset \R^d$, and any $g\in C^2(\overline U)$ there exists $\ti g \in C^2(\R^d)$ such that $\ti g_{|U} = g$.
It follows that for each $1\leq i \leq k$, there exists $\ti f_i\in C^2(\R^2)$, compactly supported, and such that $\ti f_{i|\Omega_i} = f_i$. 

Let $\Gamma_j$ be one of the pieces of $\Gamma$, between the domains $\Omega_k$ and $\Omega_l$, and let  $s=\ti f_k$ and $t = \ti f_l- \ti f_k$. Although the domains $\Omega_k$ and $\Omega_l$ are only piecewise smooth, there exists an open set $\Omega'$ with $C^2$ boundary such that for $\delta_0>0$ small enough
$$
f = s \Chi_{\Omega'} + t \ \text{ on } \ \bigcup_{0<\delta\leq \delta_0} (\Gamma_{j,\delta}+B_\delta),
$$
where $B_\delta$ is the ball of radius $\delta$ centered at $0$.
Note that $\Gamma_j\subset \Gamma' := \partial \Omega'$ and that $s = [f]$ on $\Gamma_j$.
In the following, the variables $x,z$ are always subject to the restriction
\be
\label{restrictXZ}
x\in \Gamma_{j,\delta}^0 \text{ and } z = U_\delta(x,u) = x+\delta u \bn(x) \text{ where } 0<\delta\leq \delta_0 \text{ and } |u|\leq 1,
\ee
note that $z\in \Gamma_{j,\delta}$ and $\|x-z\|\leq \delta$. We therefore have %for $z\in \Gamma_j^\delta$
$$
f_\delta(z) = \int_{\Omega'} s(\ti x) \vp_\delta(z-\ti x) d\ti x + t_\delta(z),
$$
where $t_\delta:=t * \vp_\delta$. The second derivatives of $t_\delta$ are uniformly bounded, and are therefore negligible in regard of all three estimates \iref{estimnn2d}, \iref{estimnt2d} and \iref{estimtt2d}, indeed
$$
\|d^2 t_\delta\|_{L^\infty} = \|(d^2 t)* \vp_\delta\|_{L^\infty} \leq \|d^2 t\|_{L^\infty} \|\vp_\delta\|_{L^1} = \|d^2 t\|_{L^\infty} \|\vp\|_{L^1} <\infty.
$$
We now define the $2\times 2$ symmetric matrices
$$
I(z,x) := \int_{\Omega'} (s(\ti x)-s(x)) \ d^2 \vp_\delta(z-\ti x) \ d\ti x \text{ and } J(z) := \int_{\Omega'} d^2 \vp_\delta(z-\ti x) d\ti x 
$$
so that 
\be
d^2 f_\delta(z) =  d^2 t_\delta + I(z,x) + [f](x)  J(z).
\label{d2fdelta}
\ee
We already know that the contribution of $d^2t_\delta$ is negligible. We now prove that
the same holds for the contribution of $I(z,x)$. Since $\vp_\delta(z-\ti x)$ is non-zero
only if $\|\ti x-z\| \leq \delta$ and therefore $\|\ti x-x\| \leq 2\delta$, we
can bound the norm of the matrix $I(z,x)$ by
\be
\label{d2f1}
\|I(z,x)\| \leq 2\delta \|ds\|_{L^\infty} \|d^2 \vp_\delta\|_{L^1} \leq 2\delta \|ds\|_{L^\infty} \|d^2\vp\|_{L^1} \delta^{-2} = C\delta^{-1}.
\ee
This proves that the contribution of $I(z,x)$ is negligible for the two estimates
\iref{estimnn2d} and \iref{estimnt2d}. In order to prove that it is
also negligible in the estimate \iref{estimtt2d},
we need a finer analysis of $\bt(x)^\trans I(z,x) \bt(x)$.
For this purpose we fix a unit vector $u$ and the pair $(x,z)$. We introduce
$$
\Lambda(\ti x) := (s(\ti x)-s(x)) \ \partial_u \vp_\delta(z-\ti x) + \partial_u s(\ti x) \ \vp_\delta(z-\ti x),
$$
so that by Leibniz rule
$$
(s(\ti x)-s(x)) \ \partial^2_{u,u} \vp_\delta(z-\ti x)= \partial^2_{u,u} s(\ti x) \ \vp_\delta(z-\ti x) - \partial_u \Lambda(\ti x).
$$
Therefore
\begin{eqnarray*}
u^\trans I(z,x)u &=& \int_{\Omega'} \left( \partial^2_{u,u} s(\ti x) \ \vp_\delta(z-\ti x) - \partial_u \Lambda(\ti x)\right) d\ti x, \\
&=&  \int_{\Omega'} \partial^2_{u,u} s(\ti x) \ \vp_\delta(z-\ti x) d\ti x - \int_{\Gamma'} \Lambda(\ti x) \<\bn(\ti x), u\> d \ti x.
\end{eqnarray*}
The first integral clearly satisfies 
$$
\left |\int_{\Omega'} \partial^2_{u,u} s(\ti x) \ \vp_\delta(z-\ti x) d\ti x \right |\leq \|d^2 s\|_{L^\infty} \|\vp_\delta\|_{L^1},
$$
and is therefore bounded independently of $\delta$. We estimate the second integral 
for the special case $u = \bt(x)$, remarking that  $|\<\bn(\ti x), \bt(x)\>|\leq C_1 \delta$ on the domain of integration.
Therefore
$$
\left| \int_{\Gamma'} \Lambda(\ti x) \<\bn(\ti x), \bt(x)\> d \ti x\right| \leq C_1 \delta |\Gamma'\cap B(z,\delta)| \|\Lambda\|_{L^\infty},
$$
where, slightly abusing notations, we denote by $|\Gamma'\cap B(z,\delta)|$ the length ($1$-dimensional Hausdorff measure) of the curve $\Gamma'\cap B(z,\delta)$.
Clearly $\Lambda(\ti x) = 0$ if $\|z-\ti x\|\geq \delta$. If $\|z-\ti x\|\leq \delta$ we have 
\be
\label{upperPsi}
|\Lambda(\ti x)|\leq (\|x-z\|+\|z-\ti x\|) \|ds\|_{L^\infty} \|d\vp\|_{L^\infty} \delta^{-3} + \|ds\|_{L^\infty} \|\vp\|_{L^\infty} \delta^{-2} \leq C_0\delta^{-2}.
\ee
Since in addition $|\Gamma'\cap B(z,\delta)|\leq C_2 \delta$, we finally find that
$$
\left| \int_{\Gamma'} \Lambda(\ti x) \<\bn(\ti x), \bt(x)\> d \ti x\right| \leq C_0C_1C_2.
$$
We have therefore proved that 
 $$
|\bt(x)^\trans I(z,x) \bt(x)|\leq C,
 $$
 where the constant $C$ is independent of $\delta$, which shows that 
 the contribution of $I(z,x)$ is negligible in \iref{estimtt2d}.

We now analyze the contribution the quantity $[f](x)J(z)$ in \iref{d2fdelta}.
For this purpose, we use an expression of the second derivative of 
the characteristic function $\Chi_{\Omega'}$ of a smooth set $\Omega'$
in the distribution sense. 
We assume without loss of generality that $\Gamma'$ is parametrized 
in the trigonometric sense, and therefore that $\bn$ is the inward normal to $\Omega$.
For all test function $\psi$, we have
$$
-\int_{\Omega'} \partial^2_{u,v} \psi = \int_{\Gamma'} \partial_u \psi \<v,\bn\> =  \int_{\Gamma'} (\partial_\bn \psi \<u,\bn\> + \partial_\bt\psi \<u,\bt\>) \<v,\bn\>
$$
and, by integration by parts, 
$$
\int_{\Gamma'} \partial_\bt \psi \<u,\bt\>\<v,\bn\> = - \int_{\Gamma'} \psi (\<u,\kappa\bn\>\<v,\bn\>- \<u,\bt\>\<v,\kappa\bt\>). 
$$
Therefore, we have
\be
\label{d2charR2eq}
-\int_{\Omega'} \partial^2_{u,v} \psi = \int_{\Gamma'} \<u,\bn\>\<v,\bn\> (\partial_\bn \psi-\kappa \psi) +\kappa \<u,\bt\>\<v,\bt\> \psi
\ee
Applying this formula to $\psi(\ti x):=\vp_{\delta}(z-\ti x)$ we obtain
\be
\begin{array}{rcl}
\displaystyle-u^\trans J(z) v &=&  \displaystyle\int_{\Gamma'} \<u,\bn(\ti x)\>\<v,\bn(\ti x)\> (\partial_\bn \vp_\delta(z-\ti x) - \kappa(\ti x)\vp_\delta(z-\ti x))d \ti x\\
& & \displaystyle+\int_{\Gamma'} \kappa(\ti x) \<u,\bt(\ti x)\>\<v,\bt(\ti x)\> \vp_\delta(z-\ti x) d\ti x.
\end{array}
\label{uJv}
\ee
Since $\Gamma_j$ is $C^2$, there exists a constant $C_0$ such that for all $x_1,x_2\in \Gamma_j$, we have 
$$
|\<\bt(x_1),\bn(x_2)\>|\leq C_0 \|x_1- x_2\|,
$$
and 
$$
|1-\<\bn(x_1),\bn( x_2)\>| = |1-\<\bt(x_1),\bt( x_2)\>|\leq C_0 \|x_1- x_2\|^2.
$$
We finally remark that $ |\Gamma'\cap B(z,\delta)|\leq C_1 \delta$, and that 
$\|\vp_\delta\|_{L^\infty}\leq \|\vp\|_{L^\infty}\delta^{-2}$ and  $\|\partial_\bn \vp_\delta\|_{L^\infty} \leq \|d\vp\|_{L^\infty} \delta^{-3}$. 

Taking the vectors $\bt(x)$ or $\bn(x)$ as possible values of $u$ and $v$ in \iref{uJv} and using the
above remarks, we obtain the estimates
\begin{eqnarray}
\label{threeineq1}
\left|\bn(x)^\trans J(z)\bn(x) + \int_{\Gamma'} \partial_\bn \vp_\delta(z-\ti x) d \ti x\right| &\leq& C \delta^{-1},\\
\label{threeineq2}
|\bt(x)^\trans J(z)\bn(x)| &\leq& C \delta^{-1},\\
\label{threeineq3}
\left|\bt(x)^\trans J(z)\bt(x) + \int_{\Gamma'} \kappa(\ti x) \vp_\delta(z-\ti x)d \ti x\right| &\leq& C,
\end{eqnarray}
where the constant $C$ depends only on $f$. In view of \iref{d2fdelta}
we can immediately derive estimate
\iref{estimnt2d} from \iref{threeineq2}.

In order to derive the estimate \iref{estimtt2d} from \iref{threeineq3}, we first
introduce the modulus of continuity  $\omega$ of $\kappa$ on $\Gamma_j$, 
$$
\omega(\delta) := \sup_{x_1, x_2\in \Gamma_j\sep \|x_1- x_2\|\leq \delta} |\kappa(x_1)-\kappa( x_2)|.
$$
Therefore
\begin{eqnarray*}
\left|\bt(x)^\trans J(z)\bt(x) + \int_{\Gamma'} \kappa(\ti x) \vp_\delta(z-\ti x)d \ti x\right| 
&\leq& \left|\bt(x)^\trans J(z)\bt(x) + \kappa(x)\int_{\Gamma'}  \vp_\delta(z-\ti x)d \ti x\right| \\
& &+ C\omega(\delta)\delta^{-1}.
\end{eqnarray*}
We now claim that 
\be
\left| \int_\Gamma \vp_\delta( z-\ti x) d\ti x - \delta^{-1} \Phi(u) \right| \leq C,
\label{phiPhi}
\ee
holds with $C$ independent of $\delta$ which implies the validity of  \iref{estimtt2d}. 
In order to prove \iref{phiPhi}, we use a local parametrization of $\Gamma'$: let 
$\lambda:\R\to \R$ be such that for $h$ small enough we have, $x+h\bt(x)+\lambda(h)\bn(x)\in \Gamma$. 
Note that we have $|\lambda(h)|\leq C_0 h^2$ and $|\lambda'(h)|\leq C_0h$ for $h$ small enough. 
Then for $\delta$ small enough,
\begin{eqnarray*}
\left| \int_{\Gamma'} \vp_\delta( z-\ti x) d\ti x - \delta^{-1} \Phi(u) \right|  &\leq&  \left|\int_{\R} \vp_\delta(h\bt(x)+ (\delta u-\lambda(h))\bn(x))\sqrt{1+\lambda'(h)^2} dh \right.\\
& &\left.- \int_\R  \vp_\delta(h\bt(x)+ \delta u\bn(x)) dh \right|\\
&\leq & C\delta(\|\vp_\delta\|_{L^\infty} (\sqrt{1+(C_0\delta)^2}-1)+  \|d\vp_\delta\|_{L^\infty} C_0 \delta^2 ) \leq C
\end{eqnarray*}
Finally, we can derive the estimate \iref{estimnn2d} from \iref{threeineq1} using
the inequality
\be
\left| \int_\Gamma \partial_\bn \vp_\delta(z - \ti x) d\ti x + \delta^{-2} \Phi'(u)\right|  \leq C \delta^{-1}
\label{phiPhin}
\ee
which proof is very similar to the one of \iref{phiPhi}. %, using that $\|\bn(x_1)-\bn(x_2)\|\leq C \|x_1-x_2\|$ for all $x_1, x_2\in \Gamma_j$.

%\input{../Bibliography/Bibliography.tex}
%\end{document}



==> Cartoon/cartoonTheseOld.tex <==
%------------------------------
% Remplacements
% \t -> \bt
% I_{m,T} -> \interp
%------------------------------


There exists various ways of measuring the smoothness of functions
on a domain $\Omega\subset \RR^d$, 
generally through the definition of an appropriate {\it smoothness space}. 
Classical instances are Sobolev, H\"older and Besov spaces. Such spaces are of common use
when describing the regularity of solutions to partial differential equations.
From a numerical perspective, they are also useful in order to sharply characterize at which
rate a function $f$ may be approximated by simpler functions such as Fourier series,
finite elements, splines or wavelets (see \cite{Co,DL,De} for surveys on
such results).

Functions arising in concrete applications may have
inhomogeneous smoothness properties, in the sense that they exhibit
area of smoothness separated by localized discontinuities. Two typical
instances are (i) edge in functions representing real images and 
(ii) shock profiles in solutions to non-linear hyperbolic PDE's.
The smoothness space that is best taylored to take such features
into account is the space $BV(\Omega)$ of bounded variation functions. This space
consists of those $f$ in $L^1(\Omega)$ such that $\nabla f$ is a bounded measure,
i.e. such that their total variation
$$
TV(f)=|f|_{BV}:=\max \left\{\int_\Omega f {\rm div}(\vp)\; ; \; \vp\in\cD(\Omega)^d,\; \|\vp\|_{L^\infty}\leq 1\right\}
$$
is finite. Functions of bounded variation are allowed to have jump discontinuities
along hypersurfaces of finite measure. In particular, the characteristic function of a smooth
subdomain $D\subset \Omega$ has finite total variation equal to the $d-1$-dimensional
Hausdorff measure of its boundary:
\be
|\Chi_D|_{BV}=\cH_{d-1}(\partial D).
\label{haus}
\ee
It is well known that $BV$ is a regularity space for certain 
hyperbolic conservation laws \cite{GR,Le}, in the sense that the total variation
of their solutions remains finite for all time $t>0$. This space also plays an
important role in image processing since the seminal paper \cite{FOR}.
Here, a small total variation is used as a prior to describe the mathematical 
properties of ``plausible images'', when trying to restore an unknown
image $f$ from an observation $h=Tf+e$ where $T$ is a known operator
and $e$ a measurement noise of norm $\|e\|_{L^2}\leq \e$. The restored image
is then defined as the solution to the minimization problem
\be
\min_{g\in BV} \{|g|_{BV}\; ; \; \|Tg-h\|_{L^2}\leq \e\}.
\label{minBV}
\ee
From the point of view of approximation theory, it was shown in \cite{CDPX,CDDD2} that
the space $BV$ is almost characterized by expansions in wavelet bases. For example,
in dimension $d=2$, if $f=\sum d_\lambda\psi_\lambda$ 
is an expansion in a tensor-product $L^2$-orthonormal wavelet basis, one has
$$
(d_\lambda)\in \ell^1 \Rightarrow f\in BV \Rightarrow (d_\lambda)\in w\ell^1,
$$
where $w\ell^1$ is the space of weakly summable sequences. The fact that 
the wavelet coefficients of a $BV$ function are weakly summable implies
the convergence estimate
\be
\|f-f_N\|_{L^2}\leq CN^{-1/2}|f|_{BV},
\label{wavN}
\ee
where $f_N$ is the {\it nonlinear} approximation of $f$ obtained by retaining the
$N$ largest coefficients in its wavelet expansion. Such approximation results 
have been further used in order to justify the performance of compression or
denoising algorithms based on wavelet thresholding \cite{CDDD1,DJKP,Do}.

In recent years, it has been observed that the space $BV$ (and more generally
classical smoothness spaces) do not provide a fully satisfactory description of
piecewise smooth functions arising in the above mentioned applications.
Indeed, formula \iref{haus} reveals that the total variation only takes into account
the {\it size} of the sets of discontinuities and not their geometric {\it smoothness}.
In image processing, this means that the set of bounded variation images does
not make the distinction between smooth and non-smooth edges as long as they have finite length.

The fact that edges have some geometric smoothness can be exploited in order to study
approximation procedures which outperform wavelet thresholding in terms of 
convergence rates. For instance, it is easy to prove that if $f=\Chi_D$ 
where $D$ is a bidimensional domain with smooth boundary, one can find a sequence
of triangulations $\cT_N$ with $N$ triangles such that the convergence estimate
\be
\|f-\interp_{\cT_N}f\|_{L^2} \leq CN^{-1},
\label{triN}
\ee
holds, where $\interp_\cT$ denotes the 
piecewise linear interpolation operator on a triangulation $\cT$.
Other methods are based on thresholding a decomposition of the 
function in bases or frames which differ from classical wavelets, see e.g. \cite{CD,LM,ACDDM}.
These methods also yield improvements over \iref{wavN} similar to \iref{triN}. The common feature in
all these approaches is that they achieve 
{\it anisotropic refinement} near the edges. For example,
in order to obtain the estimate \iref{triN}, 
the triangulation $\cT_N$ should include a thin layer of triangles
which approximates the boundary $\partial D$. These triangles typically have
size $N^{-2}$ in the normal direction to $\partial D$ and $N^{-1}$ in the tangential direction,
and are therefore highly anisotropic.  

Intuitively, these methods are well adapted to
functions which have anisotropic smoothness properties
in the sense that their local variation is significantly stronger
in one direction. Such properties are not well described by
classical smoothness spaces such as $BV$, and a natural
question to ask is therefore:
\nl
\nl
{\it What type of smoothness properties 
govern the convergence rate of anisotropic refinement
methods and how can one quantify these properties ?}
\nl
\nl
The goal of this paper is to answer this question,
by proposing and studying measures of smoothness which are suggested
by recent results on anisotropic finite element approximation
\cite{BBLS, CSX}. Before going further, 
let us mention several existing approaches which have been developed
for describing and quantifying anisotropic smoothness,
and explain their limitations.
\begin{enumerate}
\item
The so-called {\it mixed smoothness} classes have been introduced 
and studied in order to
describe functions which have a different order of
smoothness in each coordinate, see e.g. \cite{Ni,Te}. These spaces
are therefore not adapted to our present goal since
the anisotropic smoothness that we want to describe 
may have preferred directions that are not 
aligned with the coordinate axes and that may vary from
one point to another (for example an image with a curved edge).
\item
Anisotropic smoothness spaces
with more general and locally varying directions have
been investigated in \cite{KP}. Yet, in such spaces
the amount of smoothness in different directions
at each point is still fixed in advance and therefore
again not adapted to our goal, since this amount
may differ from one function to another (for example
two images with edges located at different positions).
\item
A  class of functions which is often used to 
study the convergence properties of anisotropic approximation
methods is the family of $C^m-C^n$ {\it cartoon images}, i.e.
functions which are $C^m$ smooth on a finite number
of subdomains $(\Omega_i)_{i=1,\cdots,k}$ separated by a union of
discontinuity curves 
$(\Gamma_{j})_{j=1,\cdots,l}$
that are $C^n$ smooth. The defects of this class are revealed
when searching for simple expression that quantifies the amount of
smoothness in this sense. A natural choice is
to take the supremum of all $C^m(\Omega_i)$ norms of $f$ and
$C^n$ norms of the normal parametrization of $\Gamma_{j}$.
We then observe that this quantity is unstable 
in the sense that it becomes extremely large
for blurry images obtained by convolving
a cartoon image by a mollifier $\vp_\delta=\frac 1{\delta^{2}}\vp(\frac \cdot h)$
as $\delta \to 0$.  In addition, this quantity does not
control the number of subdomains in the partition.
\item
A recent approach proposed in \cite{DPW} defines
anisotropic smoothness through the geometric 
smoothness properties of the {\it level sets} of the function $f$.
In this approach the measure of smoothness 
is not simple to compute directly from $f$ since it involves each of its level sets
and a smoothness measure of their local parametrization.
\end{enumerate}

The results of \cite{BBLS,CSX,M} describe 
the $L^p$-error of piecewise linear interpolation by 
an optimally adapted triangulation of at most $N$ elements,
when $f$ is a $C^2$ function of two variables. This error is defined
as
$$
\sigma_N(f)_p:=\inf_{\#(\cT)\leq N}\|f-\interp_\cT f\|_{L^p}.
$$
It is shown in \cite{BBLS} for $p=\infty$
and in \cite{M} for all $1\leq p\leq \infty$ that
that 
\be
\limsup_{N\to +\infty} N\sigma_N(f)_p\leq CA_p(f),
\label{limsupest}
\ee
where $C$ is an absolute constant and
\be
A_p(f):=\|\sqrt {|{\rm det}(d^2f)|}\|_{L^\tau},\;\; \frac 1\tau= 1+\frac 1 p.
\label{nonlinnorm}
\ee
Moreover, this estimate is known to be optimal in the sense that
$\liminf_{N\to +\infty} N\sigma_N(f)_p\geq cA_p(f)$ also holds, under some mild restriction
on the class of triangulations in which one selects the optimal one.
These results are extended in \cite{M} to the case of
higher order finite elements and space dimension $d>2$,
for which one can identify similar measures $f\mapsto A(f)$ governing the
convergence estimate. Such quantities thus constitute natural 
candidates to measure anisotropic smoothness properties. Note
that $A_p(f)$ is not a semi-norm due to the presence of the determinant
in \iref{nonlinnorm}, and in particular the
quasi-triangle inequality $A_p(f+g)\leq C(A_p(f)+A_p(g))$ 
does not hold even with $C>1$.

Our paper is organized as follows.
We begin in \S 2 by a brief account of the
available estimates on anisotropic finite element 
interpolation, and we recall in particular the argument that
leads to \iref{limsupest} with the quantity $A_p(f)$ defined by \iref{nonlinnorm}.

Since $A_p(f)$ is not a norm, we cannot associate
a linear smoothness space to it by a standard completion
process. We are thus facing a difficulty in extending
the definition of $A_p(f)$ to functions which are not
$C^2$-smooth and in particular to cartoon images
such as in item 3 above. Since we know from \iref{triN}
that for such cartoon images the $L^2$ error of adaptive
piecewise linear interpolation decays like $N^{-1}$, we would expect that the
quantity 
$$
A_2(f)=\|\sqrt {|{\rm det}(d^2f)|}\|_{L^{2/3}},
$$
corresponding to the case $p=2$ can be properly defined for
piecewise smooth functions. We address this difficulty in 
\S 3 by a regularization process:
if $f$ is a cartoon image we introduce its regularized version
\be
f_\delta:=f*\vp_{\delta},
\ee
where $\vp_\delta=\frac 1{\delta^{2}}\vp(\frac \cdot h)$ 
is a standard mollifier. Our
main result is the following: for any cartoon image $f$ of $C^2-C^2$ type, the quantity $A_2(f_\delta)$
remains uniformly bounded as $\delta\to 0$ and one has
\be
\lim_{\delta \to 0} A_2(f_\delta)^{2/3}= \sum_{i=1}^k \int_{\Omega_i}\left |\sqrt {|{\rm det}(d^2f)|}\right |^{2/3}
+C(\vp)\sum_{j=1}^l \int_{\Gamma_j} |[f](s)|^{2/3} |\kappa(s)|^{1/3} ds,
\label{lima2}
\ee
where $[f](s)$ and $\kappa(s)$ respectively denote
the jump of $f$ and the curvature of $\Gamma_j$ at the point $s$,
and where $C(\vp)$ is a constant that only depends on the choice of the mollifier.
This constant can be shown to be uniformly bounded by below for the class of
radially decreasing mollifiers. 
This result reveals that $A_2(f)$ is stable under regularization of cartoon images
(in contrast to the measure of smoothness described in item 3 above). 
We also discuss the behaviour of $A_p$ when $p\neq 2$.

These results lead us in \S 4 to a comparison
between the quantity $A_2(f)$ and the total variation $TV(f)$. We also
make some remarks on the existing links between the limit expression
in \iref{lima2} and classical results on adaptive approximation
of curves, as well as
with operators of affine-invariant image processing which also
involve the power $1/3$ of the curvature. 

We devote \S 5 to numerical tests performed on cartoon images that illustrate the validity 
of our results and we describe in \S 6 the extension of our results
to finite elements of higher degree and higher space dimensions.
Concluding remarks and perspectives of our work are given in \S 7.

\section{Anisotropic finite element approximation}

A standard estimate in finite element approximation states that 
if $f\in W^{2,p}(\Omega)$ then
$$
\|f-\interp_{\cT_h} f\|_{L^p} \leq C  h^{2}\|d^2f\|_{L^{p}},
$$
where $\cT_h$ is a triangulation of mesh size
$h:=\max_{T\in\cT_h} {\rm diam}(T)$. If we restrict our attention
to a family {\it quasi-uniform} triangulations, $h$ is linked with 
the complexity $N:=\#(\cT_h)$ according to
$$
C_1 h^{-2} \leq N \leq  C_2 h^{-2}
$$
Therefore, denoting by $\sigma^{\rm unif}_N(f)_{L^p}$ the $L^p$ approximation
by quasi-uniform triangulations of cardinality $N$, we can re-express the above
estimate as
\be
\label{uniferror}
\sigma^{\rm unif}_N(f)_{L^p} \leq CN^{-1}\|d^2f\|_{L^p}.
\ee
In order to explain how this estimate can be improved
when using adaptive partitions, we first give some
heuristic arguments which are based on the assumption that on each triangle $T$
the relative variation of $d^2f$ is small so that it can be considered
as constant over $T$, which means that 
$f$ coincides with a quadratic function $q_T$ on each $T$.
Denoting by $\interp_T$ the local interpolation operator
on a triangle $T$ and by $e_{T}(f)_p:=\|f-\interp_T f\|_{L^p(T)}$
the local $L^p$ error, we thus have according to
this heuristics
$$
\|f-\interp_\cT f\|_{L^p} =\(\sum_{T\in \cT} e_T(f)_p^p\)^{\frac 1 p}=\(\sum_{T\in \cT} e_T(q_T)_p^p\)^{\frac 1 p}
$$
We are thus led to study the local interpolation error $e_T(q)_p$ when $q\in \P_2$
is a a quadratic polynomial. Denoting by $\bq$ the homogeneous part of $q$, we
remark that
$$
e_T(q)_p=e_T(\bq)_p.
$$
We optimize the shape of $T$ with respect to the quadratic form $\bq$
by introducing a function $K_p$ defined on the space of quadratic forms by
$$
K_p(\bq):=\inf_{|T|=1}e_T(\bq)_p,
$$
where the infimum is taken among all triangles of area $1$. 
It is easily seen that $e_T(\bq)_p$ is invariant
by translation of $T$ and so is therefore the minimizing triangle
if it exists. By homogeneity, it is also easily seen
that 
$$
\inf_{|T|=a} e_T(\bq)_p=a^{\frac 1 \tau}K_p(\bq),\;\; \frac 1 \tau=\frac 1 p+1,
$$
and that the minimizing triangle of area $a$ is obtained by rescaling the minimizing
triangle of area $1$ if it exists. Finally, it is easily seen that if $\vp$ is an invertible
linear transform 
$$
K_p(\bq \circ \vp)=|{\rm det} (\vp)|K_p(\bq),
$$
and that the minimizing triangle of area $|{\rm det} (\vp)|^{-1}$ for $\bq \circ \vp$
is obtained by application of $\vp^{-1}$ to the minimizing triangle of 
area $1$ for $\bq$ if it exists. If ${\rm det} (\bq)\neq 0$, there exists 
a $\vp$ such that $\bq \circ \vp$ is either $x^2+y^2$ or $x^2-y^2$ up to 
a sign change, and we have $|{\rm det} (\bq)|=|{\rm det} (\vp)|^{-2}$.
It follows that $K_p(\bq)$ has the simple form
\be
K_p(\bq)=\sigma  |{\rm det} (\bq)|^{1/2},
\label{Kpexp}
\ee
where $\sigma$ is a constant 
equal to $K_p(x^2+y^2)$ 
if ${\rm det} (\bq)>0$ and to  $K_p(x^2-y^2)$ if ${\rm det} (\bq)<0$. 
One easily checks that this equality
also holds when ${\rm det} (\bq)= 0$ in which case $K_p(\bq)=0$.

Assuming that the triangulation $\cT$ is
such that all its triangles $T$ have optimized shape in the above sense
with respect to the quadratic form $\bq_T$ associated with $q_T$, we thus have
for any triangle $T\in\cT$
$$
e_T(f)_p=e_T(\bq_T)_p=|T|^{\frac 1 \tau}K_p(\bq_T)=\left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(T)}.
$$
since we have assumed $\frac {d^2f} 2=\bq_T$ on $T$. In order to optimize the trade-off
between the global error and the complexity $N=\#(\cT)$,
we apply the principle of {\it error equidistribution}: the triangles $T$ have
area such that all errors $e_T(\bq_T)_p$ are equal
i.e. $e_T(\bq_T)_p= \eta$ for some $\eta>0$ independent of $T$.
It follows that
$$
N\eta^\tau\leq \left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}^\tau,
$$
and therefore
$$
\sigma_N(f)_p \leq \|f-\interp_\cT f\|_{L^p} \leq N^{1/p} \eta \leq\left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}N^{-1},
$$
which according to \iref{Kpexp} implies 
\be
\sigma_N(f)_p \leq CN^{-1}A_p(f),
\label{false}
\ee
with $A_p$ defined as in \iref{nonlinnorm}.

The estimate \iref{false} is too optimistic to be correct:
if $f$ is a univariate function then $A_p(f)=0$ while $\sigma_N(f)_p$
may not vanish. In a rigorous 
derivation such as in \cite{BBLS}, one observes that
if $f\in C^2$, the replacement of $d^2f$ by a constant over $T$
induces an error which becomes negligible only when the
triangles are sufficiently small, and therefore a
correct statement is that for any $\e>0$ there exists 
$N_0=N_0(f,\e)$ such that 
\be
\sigma_N(f)_p \leq N^{-1}\left(\left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}+\e\right),
\label{true}
\ee
for all $N\geq N_0$, i.e.
\be
\limsup_{N\to +\infty} N\sigma_N(f)_p\leq \left\|K_p\(\frac {d^2f}2\)\right\|_{L^\tau(\Omega)}
\label{limsupest1}
\ee
which according to \iref{Kpexp} implies \iref{limsupest}.

\section{Piecewise smooth functions and images}

As already observed, the quantities $A_p(f)$ are well defined for
functions $f\in C^2$, but 
we expect that they should in some sense also be well defined for
functions representing $C^2-C^2$ ``cartoon images'' when $p\leq 2$. We first give 
a precise definition of such functions.

\begin{definition} 
\label{defcartoon}
A cartoon function on an open set $\Omega$ is a function almost everywhere of the form 
$$
f=\sum_{1\leq i\leq k} f_i \Chi_{\Omega_i},
$$
where the $\Omega_i$ are disjoint open sets with piecewise $C^2$ boundary, no cusps (i.e. satisfying an interior and exterior cone condition), and such that $\overline \Omega = \cup_{i=1}^k \overline \Omega_i$, and where for each $1\leq i\leq k$, the function $f_i$ is $C^2$ on $\overline \Omega_i$. %a neighbourhood of
\end{definition}

Let us consider a fixed cartoon function $f$ on an open polygonal domain $\Omega$ (i.e.
$\Omega$ is such that $\overline\Omega$ is a closed polygon)
associated with a decomposition $(\Omega_i)_{1\leq i\leq k}$. We define 
\be
\Gamma :=\bigcup_{1\leq i\leq k} \partial \Omega_i,
\ee
the union of the boundaries of the $\Omega_i$. The above definition
implies that $\Gamma$ is the disjoint union of a finite set of points $\cP$ and a finite number of open curves $(\Gamma_i)_{1\leq i\leq l}$.
$$
\Gamma = \(\bigcup_{1\leq i\leq l} \Gamma_i\) \cup \cP.
$$
Furthermore for all $1\leq i < j \leq l$, we may impose that $\overline \Gamma_i\cap \overline \Gamma_j \subset \cP$ (this may be ensured by a splitting of some of the $\Gamma_i$ if necessary).

We now consider the piecewise linear interpolation
$\interp_{\cT_N}f$ of $f$ on a triangulation $\cT_N$ of cardinality $N$. 
We distinguish two types of elements of $\cT_N$. A 
triangle $T\in \cT_N$ is called ``regular'' if $T\cap \Gamma=\emptyset$, 
and we denote the set of such triangles by $\cT_N^r$. 
Other triangles are called ``edgy'' and their set is denoted by $\cT_N^e$.
We can thus split $\Omega$ according to
$$
\Omega:=\left(\cup_{T\in \cT_N^r}T\right) \cup \left(\cup_{T\in \cT_N^e}T\right)=\Omega_N^r \cup \Omega_N^e.
$$
We split accordingly the $L^p$ interpolation error into
$$
\|f-\interp_{\cT_N}f\|_{L^p(\Omega)}^p = \int_{\Omega_N^r} |f-\interp_{\cT_N}f|^p +\int_{\Omega_N^e} |f-\interp_{\cT_N}f|^p.
$$
We may use $\cO(N)$ triangles in $\cT_N^e$ and $\cT_N^r$ (for example $N/2$
in each set). Since $f$ has discontinuities along $\Gamma$, the $L^\infty$ interpolation error on 
$\Omega_N^e$ does not tend to zero and $\cT_N^e$ should be chosen so 
that $\Omega_N^e$ has the aspect of a thin layer around $\Gamma$. 
Since $\Gamma$  is a finite union of $C^2$ curves, we can build this layer
of width $\cO(N^{-2})$ and therefore of global area $|\Omega_N^e|\leq C N^{-2}$,
by choosing long and thin triangles in $\cT_N^e$. 
On the other hand, since $f$ is uniformly $C^2$ on $\Omega_N^r$, we may
choose all triangles in $\cT_N^r$ of regular shape 
and diameter $h_T\leq C N^{-1/2}$.
Hence we obtain the following heuristic error estimate, 
for a well designed anisotropic triangulation:
\begin{eqnarray*}
\|f-\interp_{\cT_N}f\|_{L^p(\Omega)} &=& \(\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^r)}^p +\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^e)}^p\)^{1/p}\\
&\leq&\( \|f-\interp_{\cT_N}f\|_{L^\infty(\Omega_N^r)}^p |\Omega_N^r|+  
\|f-\interp_{\cT_N}f\|_{L^\infty(\Omega_N^e)}^p |\Omega_N^e|\)^{1/p}\\
& \leq & C(N^{-p}+ N^{-2})^{1/p},
\end{eqnarray*}
and therefore
\be
 \|f-\interp_{\cT_N}f\|_{L^p(\Omega)} \leq C N^{-\min\{1,2/p\}},
 \label{heurist}
 \ee
where the constant $C$ depends on $\|d^2f\|_{L^\infty(\Omega\sm \Gamma)}$, $\|f\|_{L^\infty(\Omega)}$
and on the number, length and maximal curvature of the $C^2$ curves which constitute $\Gamma$.

Observe in particular that the error
is dominated by the edge term $\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^e)}$
when $p>2$ and by the smooth term $\|f-\interp_{\cT_N}f\|_{L^p(\Omega_N^r)}$
when $p<2$. For the critical value $p=2$ the two terms have the same order. 

For $p\leq 2$, we obtain the approximation rate $N^{-1}$ 
which suggests that approximation results such as \iref{limsupest}
should also apply to cartoon functions and
that the quantity $A_p(f)$ should be
finite. We would therefore like to bridge the gap 
between anisotropic approximation of cartoon functions and smooth functions. 
For this purpose, we first need to give a proper meaning
to $A_p(f)$ when $f$ is a cartoon function. This is not 
straightforward, due to the fact that
the product of two distributions has no meaning in general.
Therefore, we cannot define $\det (d^2 f)$ in a distributional sense,
when the coefficients of $d^2 f$ are distributions without sufficient smoothness.
Our approach will rather be based on regularisation. This is additionally justified by the fact that sharp curves of discontinuity are a mathematical idealisation. In real world applications, such as photography, several physical limitations (depth of field, optical blurring) impose a certain level of blur on the edges.

In the following, we consider a fixed
radial nonnegative function $\vp$ of unit integral and supported in the unit ball,
and define for all $\delta>0$ and $f$ defined on $\Omega$,
\be
\vp_\delta(z) := \frac 1 {\delta^2} \vp\left(\frac z \delta\right) \text{ and } f_\delta = f * \vp_\delta.
\label{defphih}
\ee
Our main result gives a meaning to $A_p(f)$ based on this regularization.
If $f$ is a cartoon function on a set $\Omega$, 
and if $x\in \Gamma\sm\cP$, we denote by $[f](x)$ the jump of $f$
at this point.
We also denote $\bt(x)$ and $\bn(x)$ the unit tangent and normal
vectors to $\Gamma$ at $x$ oriented in such way that $\det(\bt,\bn)=+1$,
and by $\kappa(x)$ the curvature
at $x$ which is defined by the relation
$$
\partial_{\bt(x)}\bt(x)=\kappa(x)\bn(x).
$$
For $p\in [1,\infty]$ and $\tau$ defined by $\frac 1 \tau := 1+\frac 1 p$,
we introduce the two quantities
\begin{eqnarray*}
S_p(f) &:= & \|\sqrt{|\det (d^2 f) |}\|_{L^\tau(\Omega\sm \Gamma)}=A_p(f_{|\Omega\sm \Gamma}),\\
E_p(f) &:= & \|\sqrt{|\kappa|} [f]\|_{L^\tau(\Gamma)},\\
\end{eqnarray*}
which respectively measure the ``smooth part'' and the ``edge part'' of $f$. We
also introduce the constant
\be
C_{p,\vp}:=\|\sqrt {|\Phi\Phi'|}\|_{L^\tau(\R)},\;\; \text{ where } \ \Phi(x) := \int_{y\in\R} \vp(x,y)dy.
\label{defchi}
\ee
Note that $f_\delta$ is only properly defined on the set
$$
\Omega^\delta:=\{z\in \Omega\; ; \; B(z,\delta)\subset \Omega\},
$$
and therefore, we define
$A_p(f_\delta)$ as the $L^\tau$ norm of $\sqrt{|\det(d^2f_\delta)|}$ on this set.

\begin{theorem}
\label{threg}
For all cartoon functions $f$, the quantity $A_p(f_\delta)$ behaves as follows:
\begin{itemize}
\item If $p<2$, then
$$
\lim_{\delta\to 0} A_p(f_\delta) = S_p(f).
$$
\item If $p=2$, then $\tau=\frac 2 3$ and 
\be
\lim_{\delta\to 0} A_2(f_\delta) = \(S_2(f)^\tau+ E_2(f)^\tau C_{2,\vp}^\tau\)^{\frac 1 \tau}.
\label{Acartoon}
\ee
\item If $p>2$, then $A_p(f_\delta) \to \infty$ according to
\be
\lim_{\delta\to 0}  \delta^{\frac 1 2 - \frac 1 p} A_p(f_\delta)= E_p(f) C_{p,\vp}.
\label{equivAphih}
\ee
\end{itemize}
\end{theorem}


\begin{remark}
This theorem reveals that as $\delta\to 0$, the 
contribution of the neighbourhood of $\Gamma$ to $A_p(f_\delta)$
is negligible when $p<2$ and 
dominant when $p>2$, which was already remarked in
the heuristic computation leading to {\rm \iref{heurist}}.
\end{remark}


\begin{remark}
It seems to be possible to eliminate the ``no cusps'' condition
in the definition of cartoon functions, while still retaining the validity of
this theorem. It also seems possible to take the more natural choice 
$\vp(z) = \frac 1 \pi e^{-\|z\|^2}$, which is not compactly supported.
However, both require higher technicality in the proof
which we avoid here.
\end{remark}


Before attacking the proof of Theorem \ref{threg},
we show below that the constant $C_{p,\vp}$ involved in 
the result for $p\geq 2$ is uniformly bounded by below
for a mild class of mollifiers.

\begin{proposition}
Let $\vp$ a radial and positive function supported on the unit ball
such that $\int \vp=1$ and that $\vp(x)$ decreases as $|x|$ increases. For any $p\geq 2$ we have 
$$
C_{p, \vp} \geq \frac 2 \pi \left(\frac 4 {\tau+2}\right)^{\frac 1 \tau}.
$$
and this lower bound is optimal. 
There is no such bound if $p<2$, but note that Theorem \ref{threg} does not involve $C_{p, \vp}$ for $p<2$.
\end{proposition}

\proof
Let $D$ be the unit disc of $\R^2$. We define a non smooth mollifier $\psi$ and a function $\Psi$ as follows
$$
\psi := \frac {\Chi_D} \pi \ \text{ and } \ \Psi(x) :=  \int_\R\psi(x,y) dy.
$$
One easily obtains that
$
\Psi(x) = \frac 2 \pi \sqrt{1-x^2} \Chi_{[-1,1]}(x)\text{ and } \Psi'(x) = \frac {-2x}{\pi \sqrt{1-x^2}} \Chi_{[-1,1]}(x), 
$
hence 
$$
\Psi(x) \Psi' (x)=  \frac {-4x} {\pi^2} \Chi_{[-1,1]}(x).
$$
For all $\delta>0$ we define $\psi_\delta := \delta^{-2} \psi(\delta^{-1} \cdot)$, and  $\Psi_\delta(x) :=  \int_\R\psi_\delta(x,y) dy$. Similarly we obtain 
$$
\Psi_\delta(x) \Psi'_\delta (x) = \frac {-4x} {\pi^2}  \Chi_{[-\delta,\delta]} \delta^{-4}.
$$
Hence 
$$
C_{p,\psi_\delta} = \left\|\sqrt{\Psi_\delta(x) |\Psi'_\delta (x)|}\right\|_{L^\tau(\R)} = \frac 2 {\pi \delta^2} \left(\int_{-\delta}^\delta |x|^{\frac\tau 2} dx\right)^{\frac 1 \tau} 
= \frac 2 {\pi \delta^2} \left(\frac{2 \delta^{\frac \tau 2 +1}}{\frac \tau 2 +1}\right)^{\frac 1 \tau}
= \frac 2 \pi \left(\frac 4 {\tau+2}\right)^{\frac 1 \tau} \delta^{\frac 1 p -\frac 1 2}.
$$
Note that
\be
\label{ineqPsiDelta}
\text{ If } p\geq 2 \text{ and }\delta \in (0,1] \text{ then }  C_{p,\psi_\delta} \geq C_{p,\psi} =   \frac 2 \pi \left(\frac 4 {\tau+2}\right)^{\frac 1 \tau}.
\ee
The mollifier $\vp$ of interest is radially decreasing, has unit integral and is supported on the unit ball. It follows that there exists a Lebesgue measure $\mu$ on $(0,1]$, of mass $1$, such that 
$$
\vp = \int_0^1\psi_\delta \ d\mu(\delta).
$$
Hence
$
\Phi(x) := \int_\R \vp(x, y) dy = \int_0^1\Psi_\delta(x) \ d\mu(\delta)
$,
 for any $x\in \R$.
Since $s\mapsto s^\tau$ is concave on $\R_+$ when $0<\tau \leq 1$, we obtain
$$
\Phi(x)^\tau = \left(\int_0^1 \Psi_\delta(x) \ d\mu(\delta)\right)^\tau \geq \int_0^1 \Psi_\delta(x)^\tau \ d\mu(\delta)
$$
Similarly, since the sign of $\Psi'_\delta(x)$ is independent of $\delta$, 
$
|\Phi'(x)|^\tau = \left(\int_0^1 |\Psi_\delta'(x)| \ d\mu(\delta)\right)^\tau \geq \int_0^1 |\Psi_\delta'(x)|^\tau \ d\mu(\delta).
$
Applying the Cauchy-Schwartz inequality we obtain
$$
\sqrt{\Phi(x) |\Phi'(x)|}^{\, \tau} \geq 
\sqrt{\left(\int_0^1 \Psi_\delta(x)^\tau \ d\mu(\delta)\right)\left(\int_0^1 |\Psi_\delta'(x)|^\tau \ d\mu(\delta)\right)} 
\geq \int_0^1 \sqrt{\Psi_\delta(x) |\Psi_\delta'(x)|}^{\, \tau} \ d\mu(\delta)
$$
Eventually we conclude using the previous equation and \iref{ineqPsiDelta} as follows
$$
C_{p,\vp}^\tau = \int_\R \sqrt{\Phi |\Phi'|}^{\,\tau}\\
 \geq \int_0^1 \left(\int_\R \sqrt{\Psi_\delta |\Psi_\delta'|}^{\,\tau}\right) d\mu(\delta)\\
=  \int_0^1  C_{p,\psi_\delta}^\tau d\mu(\delta) \geq  C_{p,\psi}^\tau
$$
\sq

The rest of this section is devoted to the proof of Theorem \ref{threg}. Since
it is rather involved, we split its presentation into several main steps.
\nl
\nl
{\bf Step 1: decomposition of $A_p(f_\delta)$.}
Using the notation $K(M):= \sqrt{|\det M|}$, we can write
\be
\label{tointegrate2d}
A_p(f_\delta)^\tau = \int_{\Omega^\delta} K(d^2 f_\delta)^\tau.
\ee
We decompose this quantity based on a partition of
$\Omega^\delta$ into three subsets 
$$
\Omega^\delta=\Omega_\delta \cup \Gamma_\delta \cup \cP_\delta.
$$
The first set $\Omega_\delta$ corresponds to the
{\it smooth part}:
$$
\Omega_\delta :=  \bigcup_{1\leq i\leq k} \Omega_{i,\ssdelta}, \;\;{\rm where}\;\; 
\Omega_{i,\ssdelta} := \{z\in \Omega_i\sep d(z,\Omega\sm\Omega_i)>\delta\}.
$$
Note that $\Omega_\delta$ is strictly contained in $\Omega^\delta$.
The second set corresponds to the {\it edge part}:  we first define
$$
 \Gamma_\delta^0 := \bigcup_{1\leq j\leq l} \Gamma_{j,\ssdelta}^0, \;\;{\rm where}\;\; 
\Gamma_{j,\ssdelta}^0 := \{z\in \Gamma_j\sep d(z,\Gamma\sm\Gamma_j)>2\delta\},
$$
and then set
$$
\Gamma_\delta := \bigcup_{1\leq j\leq l} \Gamma_{j,\ssdelta}\;\;{\rm where}\;\; 
\Gamma_{j,\ssdelta} :=  \{z\in \Omega \sep d(z,\Gamma)< \delta \text{ and } \pi_\Gamma(z)\in \Gamma_{j,\ssdelta}^0\} 
$$
where $\pi_\Gamma(z)$ denotes the point of $\Gamma$ which is the closest to $z$.
The third set corresponds the {\it corner part}:
$$
\cP_\delta :=  \Omega^\delta \sm (\Omega_\delta\cup\Gamma_\delta).
$$
The measures of the sets $\Gamma_\delta$ and $\cP_\delta$ tends to
$0$ as $\delta\to 0$, while $|\Omega_\delta|$ tends to $|\Omega|$. More
precisely, we have
$$
 |\Gamma_\delta|\leq C\delta\;\;{\rm and}\;\; |\cP_\delta|\leq C  \delta^2
$$
where the last estimate exploits the ``no cusps'' property of the cartoon function.
We analyze separately the contributions of these three sets to 
\iref{tointegrate2d}.
\nl
\nl
{\bf Step 2: Contribution of the smooth part $\Omega_\delta$.}
The contribution of $\Omega_\delta$ to the integral \iref{tointegrate2d} is easily measured. Indeed, let us define
$$
Q_\delta(z):= \left\{
\begin{array}{cc}
K(d^2 f_\delta (z))^\tau & \text{ if } z\in \Omega_\delta,\\
0 & \text{ otherwise.}
\end{array}
\right.
$$
then we have pointwise convergence $Q_\delta(z)\to K(d^2 f(z))^\tau$ on $\Omega\sm \Gamma$.
Since the  $\delta$-neighbourhood of $\Omega_\delta$ is included in $\Omega\sm\Gamma$, we have 
$$
\|d^2 (f*\vp_\delta) \|_{L^\infty(\Omega_\delta)} = \|(d^2 f)*\vp_\delta \|_{L^\infty(\Omega_\delta)}\leq \|d^2 f\|_{L^\infty(\Omega\sm \Gamma)} \|\vp_\delta\|_{L^1} = \|d^2 f\|_{L^\infty(\Omega\sm \Gamma)} 
$$
Since $K$ is $1$-homogeneous and continuous, we have
$$
K(d^2 f_\delta)\leq C_K\|d^2 f\|_{L^\infty(\Omega\sm \Gamma)}, \;\; C_K:=\max_{\|M\|=1}K(M),
$$
and we conclude by dominated convergence that 
$$
\lim_{\delta \to 0}\int_{\Omega_\delta} K(d^2 f_\delta)^\tau = \lim_{\delta\to 0} \int_{\Omega \sm \Gamma} Q_\delta =  \int_{\Omega \sm \Gamma} K(d^2 f)^\tau.
$$
\nl
{\bf Step 3: Contribution of the corner part $\cP_\delta$.}
We only need a rough upper estimate of the contribution of $\cP_\delta$ 
to the integral \iref{tointegrate2d}.
We observe that 
$$
\|d^2 (f*\vp_\delta) \|_{L^\infty(\Omega)} = \|f*(d^2  \vp_\delta)\|_{L^\infty(\Omega)}\leq \|f\|_{L^\infty(\Omega)} \|d^2 \vp_\delta\|_{L^1(\R^2)} =   \frac M {\delta^2},
$$
where $M:=\|f\|_{L^\infty(\Omega)} \|d^2 \vp\|_{L^1(\R^2)}$.
It follows that 
$$
\int_{\cP_\delta} K(d^2 f_\delta)^\tau \leq |\cP_\delta| \left(C_K \left(\frac M {\delta^2}\right)\right)^\tau \leq C  \delta^{2-2 \tau}.
$$
If $\tau<1$, this quantity tends to $0$ and is therefore negligible compared to the 
contribution of the smooth part. If $\tau=1$, which corresponds to $p=\infty$, our
further analysis shows that the contribution of the edge part tends
to $+\infty$, and therefore the contribution of the corner part is always negligible.
\nl
\nl
{\bf Step 4: Contribution of the edge part $\Gamma_\delta$.} {
This step is the main difficulty of the proof. We make a key use
of an asymptotic analysis of $f_\delta$ on $\Gamma_\delta$, which relates
its second derivatives to the jump $[f]$ and the curvature $\kappa$ as $\delta\to 0$. 
We first define for all $\delta>0$ the map
$$
\begin{array}{ccc}
U_\delta : \Gamma\sm\cP \times [-1,1] &\to& \Omega\\
(x,u) &\mapsto & x+\delta u \bn (x).
\end{array}
$$
We notice that according to our definitions,
for $\delta$ small enough, the map $U_\delta$ induces a diffeomorphism 
between $\Gamma_\delta^0\times [-1,1]$ and $\Gamma_\delta$, such
that $\pi_\Gamma(U_\delta(x,u))=x$ and $d(U_\delta(x,u),\Gamma)=|U_\delta(x,u)-x|=\delta |u|$.
We establish asymptotic estimates on the
second derivatives of $f_\delta$ which have the following form:
\begin{eqnarray}
\label{estimnn2d}
\left |\partial_{\bn,\bn} f_\delta(z) -  \frac 1 { \delta^2} [f](x) \Phi'(u)\right| &\leq & \frac C { \delta}\\ 
\label{estimnt2d}
|\partial_{\bn,\bt} f_\delta(z)| &\leq &  \frac C \delta\\%\cO\left(\frac 1 \delta\right)\\
\label{estimtt2d}
\left |\partial_{\bt,\bt} f_\delta(z) +  \frac 1 \delta [f](x) \kappa(x)\Phi(u)\right| &\leq &\frac {\omega(\delta)} \delta
\end{eqnarray}
where $\lim_{\delta\to 0} \omega(\delta) = 0$ and with the notation
$z=U_\delta(x,u)$. The constant $C$ and the function $\omega$ depend only on $f$.
The proof of these estimates is given in the appendix. As an immediate consequence,
we obtain an asymptotic estimate of $K(d^2 f_\delta)=\sqrt{|\det(d^2 f_\delta)|}$ of the form
\be
\label{estimK2d}
\left|  \delta^{\frac 3 2} K(d^2 f_\delta(z)) - \sqrt{|\kappa(x)|} \, |[f](x)| \sqrt{|\Phi(u) \Phi'(u)|} \right|\leq \omega(\delta),
\ee
where $\lim_{\delta\to 0} \omega(\delta) = 0$, and the function $\omega$ depends only on $f$. 
Using the notations
$$
g_\delta(z):=\delta^{\frac 3 2} K(d^2 f_\delta(z)),\;\;  \lambda(x):=\sqrt{|\kappa(x)|}\, |[f](x)|,\;\; \mu(u):=\sqrt{|\Phi(u) \Phi'(u)|},
$$
we thus have
\be
|g_\delta(z) - \lambda(x) \mu(u)|\leq \omega(\delta), 
\label{glambmu}
\ee
for all $x\in \Gamma^0_\delta$, $u\in [-1,1]$ and $\delta>0$
sufficiently small, with $z=U_\delta(x,u)$. We claim that
for any functions $(g_\delta,\lambda,\mu)$ satisfying \iref{glambmu},
we have for any $\tau>0$, 
\be
\lim_{\delta\to 0}  \delta^{-1} \int_{\Gamma_\delta} g_\delta^\tau =\int_{\Gamma} \lambda(x)^\tau dx  \int_{-1}^1 \mu(u)^\tau du,
\label{claim}
\ee
which is in our case equivalent to the estimate
\be
\lim_{\delta\to 0}  \delta^{ \frac 3 2 \tau-1} \int_{\Gamma_\delta} K(d^2 f_\delta)^\tau = 
 \int_\Gamma |[f]|^\tau |\kappa|^{\tau/2} \int_\R |\Phi \Phi'|^{\tau/2}.
\label{estimgammadelta}
\ee
In order to prove \iref{claim}, we may assume without loss of generality that $\tau =1$
up to replacing $(g_\delta,\lambda,\mu)$  by $(g_\delta^\tau,\lambda^\tau,\mu^\tau)$.
We first express the jacobian matrix of $U_\delta$
using the bases $B_1 = ((\bt(x),0),(0,1))$ and $B_2 =(\bt(x),\bn(x))$ 
for the tangent spaces of $\Gamma\times [-1,1]$ and $\Omega$.
This gives the expression
$$
[d U_\delta(x,u)]_{B_1,B_2} = \left(
\begin{array}{c|c}
1- \delta u\kappa(x)& 0\\
\hline
0 & \delta
\end{array}
\right)
$$
and therefore $|\det(dU_\delta(x,u))| = \delta -\delta^2 u\kappa(x)$. Since
$(B_1,B_2)$ are orthonormal bases, this quantity is the jabobian of $U_\delta$ at $(x,u)$,
and therefore
$$
\int_{\Gamma_\delta} g_\delta =\delta\int_{\Gamma_\delta^0 \times [-1,1]} g_\delta(x+\delta u \bn (x)) 
(1 -\delta u\kappa(x)) dx\, du
$$
Combining with \iref{glambmu}, and using dominated
convergence we obtain \iref{claim}.
\nl
\nl
{\bf Step 5: summation of the different contributions.}
Summing up the contributions of $\Omega_\delta$, $\cP_\delta$ and $\Gamma_\delta$,
we reach the estimate
\begin{eqnarray*}
\int_\Omega K(d^2 f_\delta)^\tau &=&  \int_{\Omega_\delta} K(d^2 f_\delta)^\tau+ \int_{\cP_\delta} K(d^2 f_\delta)^\tau+ \int_{\Gamma_\delta} K(d^2 f_\delta)^\tau\\
&=& \left(\int_{\Omega\sm\Gamma} K(d^2 f)^\tau +\e_1(\delta) 
\right) + B(\delta) \delta^{2-2\tau}+  \delta^{1-\frac 3 2 \tau} \left( \int_\Gamma |[f]|^\tau |\kappa|^{\tau/2}\int_\R |\Phi \Phi'|^{\tau/2} +\e_2(\delta)\right),\\
&=& (S_p(f)^\tau +\e_1(\delta)) + B(\delta) \delta^{2-2\tau}+  \delta^{1-\frac 3 2 \tau} (E_p(f)^\tau C_{p,\phi}^\tau+\e_2(\delta)),\\
\end{eqnarray*}
where $\lim_{\delta\to 0}\e_1(\delta)=\lim_{\delta\to 0}\e_2(\delta)=0$ and $B(\delta)$ is uniformly bounded.
This concludes the proof of Theorem \ref{threg}. 


\section{Relation with other works}

Theorem \ref{threg} allows us to extend
the definition of $A_2(f)$ when $f$ is a cartoon
function, according to
\be
A_2(f):= \(S_2(f)^{2/3}+ E_2(f)^{2/3} C_{2,\vp}^{2/3} \)^{3/2}.
\label{addita2}
\ee
We first compare this additive form
with the total variation $TV(f)$. If $f$ is a
cartoon function,
its total variation has the additive form
\be
TV(f):=\|\nabla f\|_{L^1(\Omega\sm\Gamma)}+ \|[f]\|_{L^1(\Gamma)},
\label{additv}
\ee
Both \iref{addita2} and \iref{additv}
include a ``smooth term'' and an ``edge term''.
It is interesting to compare the edge term
of $A_2(f)$, which is given by
$$
E_2(f)=\|\sqrt {|\kappa|}[f]\|_{L^{2/3}(\Gamma)},
$$
up to the multiplicative constant $C_{2,\vp}$, with the
one of $TV(f)$ which is simply the integral of the jump
$$
J(f):=\|[f]\|_{L^{1}(\Gamma)},
$$
Both terms are $1$-homogeneous with the value of the jump of the
function $f$. In particular, if the value of this jump is $1$
(for example when $f$ is the characteristic function of a set of boundary $\Gamma$), we have
\be
E_2(f)=\(\int_\Gamma |\kappa|^{1/3}\)^{3/2},
\label{powercurv}
\ee
while $J(f)$ coincides with the length of $\Gamma$. 
In summary, $A_2(f)$ takes into account the {\it smoothness} of
edges, through their curvature $\kappa$, while 
$TV(f)$ only takes into account their {\it length}.

Let us now investigate more closely the measure of
smoothness of edges which is incorporated in $A_2(f)$. According to 
\iref{powercurv}, this smoothness is meant in the sense
that the arc length parametrizations of the curves that
constitute $\Gamma$ admit  
second order derivatives in $L^{\frac 1 3}$. In the following,
we show that this particular measure of smoothness is 
naturally related to some known results in two different areas:
adaptive approximation of curves and affine-invariant image
processing.

We first revisit the derivation of the heuristic estimate
\iref{heurist} for the error between a cartoon function
and its linear interpolation on an optimally adapted 
triangulation. In this computation, the contribution of the
``edgy triangles'' was estimated by the area of the layer $\Omega_N^e$ according to
$$
\|f-\interp_{\cT_N} f\|_{L^p(\Omega^{e}_N)} \leq \|f\|_{L^\infty} |\Omega_N^e|^{1/p}.
$$
Then we invoke the fact that $\Gamma$ is a finite union of $C^2$ curves $\Gamma_j$
in order to build a layer of global area $|\Omega_N^e| \leq CN^{-2}$, 
which results in the case $p=2$ into a contribution to the $L^p$ error
of the order $\cO(N^{-1})$. The area of the layer $\Omega_N^e$ 
is indeed of the same order as the area between the edge $\Gamma$
and its approximation by a polygonal line with $\cO(N)$ segments.

Each of the curves $\Gamma_j$
can be identified to the graph of a $C^2$ function
in a suitable orthogonal coordinate system.
If $\gamma$ is one of these functions, the area
between $\Gamma$
and its polygonal approximation can thus be 
locally measured by the $L^1$ error
between the one-dimensional function
$\gamma$ and a piecewise linear approximation
of this function.
Since $\gamma$ is $C^2$, it is obvious
that it can be approximated by a piecewise linear function on $\cO(N)$ intervals
with accuracy $\cO(N^{-2})$ in the $L^\infty$ norm and therefore
in the $L^1$ norm. However, we may ask whether such a rate
could be achieved under weaker conditions on the smoothness of $\gamma$.
The answer to this question is a chapter of {\it nonlinear} approximation theory
which identifies the exact conditions for a function $\gamma$ to be approximated
at a certain rate by piecewise polynomial functions on adaptive one-dimensional
partitions. We refer to \cite{De} for a detailed
treatment and only state the result which is of interest to us. We say that a function
$\gamma$ defined on a bounded interval $I$ belongs to the approximation
space ${\cal A}^s(L^p)$ if and only if there exists a sequence $(p_N)_{N>0}$ of functions where
each $p_N$ is piecewise affine on a partition of $I$ by $N$ intervals
such that 
$$
\|\gamma-p_N\|_{L^p} \leq CN^{-s}.
$$
For $0<s\leq 2$, it is known that 
$\gamma\in {\cal A}^s(L^p)$ provided that $\gamma\in B^{s}_{\tau,\tau}(I)$ with $\frac 1 \tau:=\frac 1 p+s$,
where $B^s_{\tau,\tau}(I)$ is the standard Besov space
that roughly describes those functions having $s$ derivatives in $L^{\tau}$.
In the case $s=2$ and $p=1$ which is of interest to us, we find $\tau=\frac 1 3$ and therefore $\gamma$ should
belong to the Besov space $B^2_{\frac 1 3,\frac 1 3}(I)$. Note that in our definition 
of cartoon functions, we assume much more than $B^2_{\frac 1 3,\frac 1 3}$ smoothness on $\gamma$,
and it is not clear to us if Theorem \iref{threg} can be derived under this minimal smoothness 
assumption. However it is striking to see that the quantity $E_2(f)$
that is revealed by Theorem \iref{threg} precisely measures the second derivative of the
arc-length parametrization of $\Gamma$ in the $L^{\frac 1 3}$ norm, up to
the multiplicative weight $|[f]|^{2/3}$. Let us also mention
that Besov spaces have been used in \cite{DPW} in order to describe
the smoothness of functions through the regularity of their level sets.
Note that edges and level sets are two distinct concepts, which
coincide in the case of piecewise constant cartoon functions.

The quantity $|\kappa|^{1/3}$ is also encountered in
mathematical image processing, for the design of
simple smoothing semi-groups that respect {\it affine invariance}
with respect to the image. Since these semi-groups should also
have the property of {\it contrast invariance}, they can be defined
through curve evolution operators acting on the level sets
of the image. The simplest curve evolution operator
that respects affine invariance is given by the equation
$$
\frac {d \Gamma}{d t}=-|\kappa|^{1/3}{\rm n},
$$
where ${\rm n}$ is the outer normal, see e.g. \cite{Ca}.
Here the value $1/3$ of the exponent plays a critical
role. The fact that we also find it in $E_2(f)$ suggests
that some affine invariance property also holds for this quantity
as well as for $A_2(f)$. 
We first notice that if $f$ is a compactly supported
$C^2$ function of two variables and $T$ is a 
bijective affine transformation, then with
$\ti f$ such that
$$
f=\ti f\circ T,
$$
we have
the property
$$
d^2 f(z)=L^\trans d^2 \ti f(Tz) L,
$$
where $L$ is the linear part of $T$ and $L^\trans$ its transpose, so that
$$
\sqrt {|\det (d^2f(z))|}=|\det L|\sqrt{|\det (d^2 \ti f(Tz))|}.
$$
By change of variable, we thus find that
\be
A_p(\ti f)=|\det L|^{1/\tau-1}A_p(f)=|\det L|^{1/p}A_p(f).
\label{invap}
\ee
A similar invariance property can be  derived on the interpolation error
$\sigma_N(f)_p=\|f-\interp_{\cT_N}f\|_{L^p}$ where $\cT_N$ is a triangulation which is optimally adapted
to $f$  in the
sense of minimizing the linear interpolation error in the $L^p$ norm
among all triangulations of cardinality $N$. We indeed remark that
an optimal triangulation for $\ti f$ is then given by applying $T$ to
all elements of $\cT_N$. For such a triangulation 
$\ti \cT_N:=T(\cT_N)$, one has the commutation formula
$$
\interp_{\cT_N}f=(\interp_{\ti \cT_N} \ti f)\circ T,
$$
and therefore we obtain by a change of variable that
\be
\sigma_N(\ti f)_p=\|\ti f-\interp_{\ti\cT_N}\ti f\|_{L^p}=|\det L|^{1/p}\|f-\interp_{\cT_N}f\|_{L^p}=|\det L|^{1/p}\sigma_N(f)_p.
\label{invsigmap}
\ee
Let us finally show that if $f$ is a cartoon function, then $E_2(f)$ satisfies a similar invariance property
corresponding to $p=2$, namely
\be
E_2(\ti f)=|\det L|^{1/2} E_2(f).
\label{inve2}
\ee
Note that this cannot be derived by arguing that $A_2(f)$ satisfies this
invariance property when $f$ and $\ti f$ are smooth, since we lose
the affine invariance property as we introduce the convolution by $\vp_\delta$: 
we do not have
$$
(f\circ T) * \vp_\delta = (f* \vp_\delta)\circ T.
$$
unless $T$ is a rotation or a translation. 

Let $\Gamma_j$ be one of the $C^2$ pieces of $\Gamma$
and  $\gamma_j: [0,B_i]\to \Omega$ a regular parametrisation of 
$\Gamma_j$. The curvature 
of $\Gamma$ on $\Gamma_j$ at the point $\gamma_j(t)$ is therefore given by
\be
\label{exprKappa}
\kappa(\gamma_j(t))= \frac{\det(\gamma_j'(t),\gamma_j'' (t))}{\|\gamma'_j(t)\|^{3}}
\ee
Since $f=\ti f\circ T$, the discontinuity curves of $\ti f$ are the images of those of $f$ by $T$:
$$
\ti \Gamma_j=T(\Gamma_j).
$$
The curvature of $\tiÊ\Gamma_j$ at the point 
$T(\gamma_j(t))$ is therefore given by 
$$
\ti \kappa(T(\gamma_j(t))) = \frac{\det(L\gamma'_j(t), \ L\gamma''_j(t))}{\|L\gamma'_j(t)\|^3} = \det(L) \frac{\det (\gamma'_j(t),\gamma''_j(t))}{\|L\gamma'_j(t)\|^3} .
$$
This leads us to the relation : 
\be
\label{relKappa}
|\det(L)|^{1/3} |\kappa(\gamma_j(t))|^{1/3} \ \|\gamma'_j(t)\| =  |\ti\kappa(T(\gamma_j(t)))|^{1/3}
\|L\gamma'_j(t)\| ,
\ee
and therefore
\begin{eqnarray*}
\int_{\ti \Gamma_j} |[\ti f]|^{2/3} |\ti \kappa|^{1/3} &=& \int_0^{B_j}  |[\ti f](T(\gamma_j(t)))|^{2/3}
|\ti\kappa(T(\gamma_j(t))|^{1/3} \ \|L\gamma'_j(t)\| dt,\\
&=& |\det L|^{1/3} \int_0^{B_j}  |[f](\gamma_j(t))|^{2/3} |\kappa(\gamma_j(t))|^{1/3} \  \|\gamma'_j(t)\|dt,\\
&=& |\det L|^{1/3} \int_{ \Gamma_i} |[ f]|^{2/3} |\kappa|^{1/3}.
\end{eqnarray*}
Summing over all $j=1,\cdots,l$ and elevating to the $3/2$ power
we obtain \iref{inve2}.

\section{Numerical tests}

In this section, we validate our previous results
by  numerical tests applied to a simple cartoon image:
the Logan-Shepp phantom. We use a $256\times 256$ pixel
version of this image, with a slight modification which is motivated
further. This image is iteratively smoothed
by the numerical scheme 
\be
\label{numSmoothing}
u_{i,j}^{n+1} = \frac {u_{i,j}^n} 2 + \frac {u_{i+1,j}^n+u_{i-1,j}^n+u_{i,j+1}^n+u_{i,j-1}^n} 8
\ee
This scheme is an explicit discretization of the heat equation.
Formally, as $n$ grows,
$u^n$ is a discretization of 
\be
\label{Gaussian}
u * \vp_{\lambda \sqrt n} \text{ with } \vp_\delta (z) := \frac 1 { \pi\delta^2 } e^{-\frac {\|z\|^2}{\delta^2}},
\ee 
where $u$ stands for the continuous image. The determinant of the hessian 
is discretised by the following $9$-points formula
$$
d_{i,j}^n := (u_{i,j+1}^n-2u_{i,j}^n+u_{i,j-1}^n) (u_{i+1,j}^n-2u_{i,j}^n+u_{i-1,j}^n) - \frac {(u_{i+1,j+1}^n+u_{i-1,j-1}^n-u_{i+1,j-1}^n-u_{i-1,j+1}^n)^2}{16}
$$
For each value of $n$, we then compute the $\ell^\tau$ norm of the array
$\left(\sqrt{|d^n_{i,j}|}\right)$ for $\tau \in [\frac 1 2,1]$, which corresponds to
$p\in [1,\infty]$ with $\frac 1 \tau := 1 + \frac 1 p$. This norm is thus a discretization of the quantity
$$
\left \|\sqrt{|\det(d^2(u*\vp_{\lambda \sqrt n}))|}\right \|_{L^\tau}.
$$
For each value of $n$ we obtain a function $\tau\in  [\frac 1 2,1]\to D_n(\tau) \in\R_+$.

As $n$ grows, three consecutive but potentially overlapping phases appear 
in the behaviour of the functions $D_n$, which are illustrated on Figure \ref{fig2Cartoon}.

\begin{enumerate}

\item For small $n$, the $9$-points discretisation is not a good approximation of the determinant of the hessian
due to the fact that the pixel discretization is too coarse compared to the 
smoothing width. During this phase, the functions $D_n$ decay rapidly for all values of $\tau$. 

\item For some range of $n$, the edges have been smoothed by the action of \iref{numSmoothing}, 
but the parameter $\lambda \sqrt n$ in \iref{Gaussian} remains rather small. Our previous analysis applies and we observe that $D_n(2/3)$ is (approximately) constant while $D_n(\tau)$ increases for 
$\tau < 2/3$ and decreases for $\tau > 2/3$. 

\item For large $n$, the details of the picture fade and begin to disappear. The picture begins to resemble a constant picture. Therefore the functions $D_n$ decay for all values of $\tau$, and eventually tend to $0$. 

\end{enumerate}


\begin{figure}
	\centering
		\includegraphics[width=5cm,height=5cm]{\pathPic/PaperCartoon/PicShepp.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=5cm]{\pathPic/PaperCartoon/PicSheppSimpler.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=5cm]{\pathPic/PaperCartoon/PicSmoothedShepp.pdf}
	\caption{\label{fig1Cartoon}The Logan-Shepp image (left), modified image (center), smoothed image (right).}
\end{figure}



\begin{figure}
	\centering
		\includegraphics[width=5cm,height=4cm]{\pathPic/PaperCartoon/PicBeginShepp.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=4cm]{\pathPic/PaperCartoon/PicMidShepp.pdf}
		\hspace{0.2cm}
		\includegraphics[width=5cm,height=4cm]{\pathPic/PaperCartoon/PicEndShepp.pdf}
	\caption{\label{fig2Cartoon}The curves $D_n(\tau)$ for $n\leq 50$ (left),
	$50\leq n\leq 100$ (center) and 
	$100\leq n\leq 200$ (right).}
\end{figure}


In our numerical experiments, we used the well known Shepp-Logan Phantom  with a slight modification
as shown on Figure \ref{fig1Cartoon}: we have removed the thin layer around the head, which represents the skull, 
because it disappears too quickly by the smoothing procedure
and causes phases 1 and 3 to overlap, masking phase 2.
For more complicated functions $f$, such as most photographic pictures, phases $1$ and $3$ 
also tend to overlap for similar reasons. 
Indeed, these pictures often have details at the pixel scale, including electronic noise due to the captor. 
Since these details disappear early phase 3 begins immediately, therefore phase 2 cannot be observed.

\section{Extension to higher dimensions and higher order elements}

The results on approximation by anisotropic bidimensional piecewise linear
finite element that we have exposed in \S 2 have been generalized in \cite{M}
to the case of elements of arbitrary order $m-1$
defined on partitions of $\Omega\subset \RR^d$ by simplices.
Here, the local error is defined as
$$
e_{m,T}(f):=\|f-\interp^{m-1}_T f\|_{L^P(T)},
$$
where $\interp^{m-1}_T$ denotes the local interpolation operator
on $\P_{m-1}$ for a $d$-dimensional simplex $T$. This operator
is defined by the condition
$$
\interp^{m-1}_T v(\gamma)=v(\gamma),
$$
for all points $\gamma\in T$ with barycentric coordinates in
the set $\{0, \frac 1 {m-1},\frac 2 {m-1},\cdots,1\}$. Then
one defines for any homogeneous polynomial $\bq\in \P_{m}$,
$$
K_{m,p}(\bq):=\inf_{|T|=1}e_{m,T}(\bq)_p.
$$
We refer to $K_{m,p}$ as the {\it shape function}. 
For piecewise linear elements in dimension two, i.e. $m=d=2$, 
we have observed that $K_p=K_{2,p}$ has the
special form given by \iref{Kpexp} which justifies the
introduction of the quantity $A_p(f)$. In a similar way, it can 
easily be proved that for piecewise linear elements in higher dimension,
i.e. $m=2$ and $d>2$, one has
$$
c_1 |{\rm det} (\bq)|^{1/d}\leq K_{2,p}(\bq) \leq  c_2 |{\rm det} (\bq)|^{1/d}.
$$
For piecewise quadratic elements in dimension two, i.e. $m=3$ and $d=2$, 
it was proved in \cite{M} that
$$
c_1 |{\rm disc} (\bq)|^{1/4}\leq K_{3,p}(\bq) \leq  c_2 |{\rm disc} (\bq)|^{1/4}.
$$
for any {\it homogeneous} polynomial $\bq\in \PP_{3}$, where
$$
{\rm disc}(a x^3+ b x^2 y+ c x y^2+ d y^3):= b^2 c^2 - 4 a c^3 - 4 b^3 d + 18 a b c d - 27 a^2 d^2.
$$
For other values of $m$ and $d$, equivalent expressions
of $K_{m,p}(\bq)$ in terms of polynomials in the coefficients of $\bq$
are available but of less simple form.

Defining the finite element interpolation error by an optimally adapted partition
$$
\sigma_N(f)_p:=\inf_{\#(\cT)\leq N}\|f-\interp^{m-1}_\cT f\|_{L^p},
$$
where $\interp^{m-1}_\cT$ is the global interpolation operator for the 
simplicial partition $\cT$, the following generalization of 
\iref{limsupest1} is proved in \cite{M}:
\be
\limsup_{N\to +\infty} N^{\frac m d}\sigma_N(f)_p\leq C_d\left\|K_{m,p}\(\frac {d^mf}{m!}\)\right\|_{L^\tau(\Omega)},
\;\; \frac 1 \tau=\frac 1 p+\frac m d.
\label{limsupest2}
\ee
The constant $C_d$ is equal to $1$ when $d=2$ but larger
than $1$ when $d>2$ due to the impossibility of exactly tiling the
space with locally optimized simplices.
If $f$ is a $C^m$ function of $d$ variables, it is therefore natural to 
consider the quantity 
\be
A_{m,p}(f):=\|K_{m,p}(d^m f)\|_{L^\tau(\Omega)},
\;\; \frac 1 \tau=\frac 1 p+\frac m d.
\ee
as a possible way to measuring anisotropic smoothness. For $d=2$ and piecewise
linear elements, we have seen in \S 2 that $A_{2,p}(f)$ is equivalent to the quantity $A_p(f)$.

Similarly to $A_p$ we are interested in the possible extension of $A_{m,p}$
to cartoon functions. We first introduce a generalisation 
of the notion of cartoon functions to higher piecewise smoothness $m$ and dimension $d$.
\begin{definition} 
\label{defcartoongen}
Let $m\geq 2$ and $d\geq 2$ be two integers. Let $\Omega\subset \R^d$ be an open set.
We say that a function $f$ defined
on $\Omega$ is a $C^m$ cartoon function if it is almost everywhere of the form 
$$
f=\sum_{1\leq i\leq k} f_i \Chi_{\Omega_i},
$$
where the $\Omega_i$ are disjoint open sets with piecewise $C^2$ boundary, no cusps (i.e. satisfying an interior and exterior cone condition), and such that $\overline \Omega = \cup_{i=1}^k \overline \Omega_i$.
Additionally, for each $1\leq i\leq k$, the function $f_i$ is assumed to be $C^m$ on $\overline \Omega_i$. %a neighbourhood of
\end{definition}

Let us consider a fixed cartoon function $f$ on a polyhedral domain $\Omega\subset\R^d$ (i.e. $\Omega$ is
such that $\overline \Omega$ is a closed polyhedron), and a decomposition 
$(\Omega_i)_{1\leq i\leq k}$ of $\Omega$ as in definition \ref{defcartoongen}. As before we define 
$ 
\Gamma := \bigcup_{1\leq i\leq k} \partial \Omega_i,
$
the union of the boundaries of the $\Omega_i$. Our assumptions on the sets $(\Omega_i)_{1\leq i\leq k}$ imply that $\Gamma$ 
is the union of a finite number of open hypersurfaces $(\Gamma_j)_{1\leq j\leq l}$, and of a set $\cP$ of dimension $d-2$.

As in \S 3, we now consider a sequence $f_N$ of piecewise linear approximations of $f$ on 
simplicial partitions $\cT_N$ of cardinality $N$. We distinguish two types of elements of $\cT_N$. A simplex $T\in \cT_N$ is called ``regular'' if $T\cap \Gamma=\emptyset$, and we denote the set of these simplices by $\cT_N^r$. Other simplices are called ``edgy'' and their set is denoted by $\cT_N^e$.
We can again split $\Omega$ according to
$$
\Omega:=(\cup_{T\in \cT_N^r}T) \cup (\cup_{T\in \cT_N^e}T)=\Omega_N^r \cup \Omega_N^e.
$$
Heuristically, if the partitions $\cT_N$ are built with approximation error minimisation in mind, the number of elements should be balanced between $\cT_N^r$ and $\cT_N^e$. The partition $\cT_N^r$ tends to cover most of the surface of $\Omega$, with simplices of diameter $\leq C  N^{-\frac 1 d}$, and $L^\infty$ approximation error $|f-f_N|\leq C N^{-\frac m d}$ (since we use $\cP_{m-1}$ elements).
On the other hand, since $f$ has discontinuities along $\Gamma$, the $L^\infty$ approximation error on $\cT_N^e$ does not tend to zero, and $\cT_N^e$ should thus be chosen so as to produce a thin layer around $\Gamma$. 
Let $h$ be the typical diameter of an element of $\cT_N^e$. Since the $\Gamma_j$ has
bounded curvature, this layer can be made of width $\cO(h^2)$. Furthermore, an element of diameter $h$ covers a $d-1$-dimensional volume of at most $h^{d-1}$ on the hypersurface $\Gamma$, and therefore 
$h\geq C N^{-\frac 1 {d-1}}$. Eventually, we find that the layer around $\Gamma$ has volume at least $C N^{-\frac 2 {d-1}}$. 

Hence we have the following heuristic error estimate, for a well designed anisotropic partition:
\begin{eqnarray*}
\|f-f_N\|_{L^p(\Omega)} &\leq& \|f-f_N\|_{L^p(\Omega_N^r)} +\|f-f_N\|_{L^p(\Omega_N^e)}\\
&\leq& \|f-f_N\|_{L^\infty(\Omega_N^r)} |\Omega_N^r|^{\frac 1 p}+  \|f-f_N\|_{L^\infty(\Omega_N^e)} |\Omega_N^e|^{\frac 1 p}\\
& \leq & C (N^{-\frac m d}  + N^{\frac {-2} {p (d-1)}})
\end{eqnarray*}
This leads us to define a critical exponent
$$
p_c = p_c(m,d):=\frac{2d}{m (d-1)}.%, \text{ equivalently } 1 = \frac 1 d + \frac 2 {m p_c(m,d)}.
$$
If one measures the error in $L^p$ norm with $p>p_c(m,d)$, then the contribution of the edge neighbourhood
$\Omega_N^e$ dominates, while if $p<p_c(m,d)$ it is negligible compared to the contribution
of the smooth region $\Omega_N^r$. 
For the critical exponent $p=p_c(m,d)$ the two terms have the same order, which makes the situation more interesting. Note in particular that $p_c(2,2) =2$, which is consistent with our previous analysis.

For $p\leq p_c(m,d)$, we obtain the approximation rate $N^{-m/d}$ which suggests that approximation
results such as \iref{limsupest2} should also apply to cartoon functions and that the 
quantity $A_{m,p}(f)$ should be finite for such functions. We again need to
use a regularization approach, for the same reasons as in \S 3.
For a given dimension $d$, we consider a radial nonnegative function $\vp$ 
of unit integral and supported in the unit ball of $\R^d$, and define for $\delta >0$
\be
\vp_\delta(z) := \frac 1 { \delta^d} \vp\left(\frac z \delta\right) \text{ and } f_\delta = f * \vp_\delta.
\ee
With $\tau$ such that $\frac 1 \tau :=\frac m d+\frac 1 p$, we 
define
\begin{eqnarray*}
S_p(f) &:= & \|K(d^m f )\|_{L^\tau(\Omega\sm \Gamma)}=A_p(f_{|\Omega\sm \Gamma}),\\
E_p(f) &:= & \| |\kappa|^{\frac m {2d}} [f] \|_{L^\tau(\Gamma)},\\
\end{eqnarray*}
where $\kappa$ is the Gauss curvature and $[f]$ the jump of $f$.
We conjecture the following generalization to Theorem \ref{threg}.

\begin{conjecture}
\label{thAmdp}
\begin{itemize}
\item If $p<p_c$ then 
$$
\lim_{\delta\to 0} A_{m,p}(f_\delta) = S_p(f).
$$ 
\item If $p=p_c$ then 
$$
\lim_{\delta \to 0} \left(A_{m,p}(f_\delta)\right)  = \left(S_p(f)^\tau + C E_p(f)^\tau\right)^{1/\tau}.
$$ 
\item If $p>p_c$ then
$$
\lim_{\delta \to 0}  \delta^{\frac 1 {p_c} - \frac 1 p} A_{m,p}(f_\delta) = C E_p(f).
$$ 
\end{itemize}
where $C$ is a positive constant that depends on $\vp,p,m,d$.
\end{conjecture}

In the remainder of this section, we give some 
arguments that justify this conjecture. Given a cartoon function $f$, 
we define the sets $\Omega_\delta$, $\Gamma_\delta^0$, 
$\Gamma_\delta$ and $\cP_\delta$ similarly to \S 3.
We need to perform an asymptotic analysis of the integral
\be
\label{tointegrate}
\int_\Omega K(d^m f_\delta)^\tau = \int_{\Omega_\delta} K(d^m f_\delta)^\tau+\int_{\cP_\delta} K(d^m f_\delta)^\tau
+\int_{\Gamma_\delta} K(d^m f_\delta)^\tau.
\ee
As in the proof of Theorem \ref{threg} the contribution of $\cP_\delta$ can be proved to be negligible 
compared with those of $\Omega_\delta$ and $\Gamma_\delta$ as $\delta \to 0$. The contribution of
$\Omega_\delta$ satisfies
$$
\lim_{\delta \to 0} \int_{\Omega_\delta} K(d^m f_\delta)^\tau =\int_{\Omega\sm \Gamma} K(d^m f)^\tau.
$$ 
The main difficulty lies again in the contribution of $\Gamma_\delta$. Let us define $\tau_c$ by 
$$
\frac 1 {\tau_c} := \frac m d+ \frac 1 {p_c}.
$$
The contribution of $\Gamma_\delta$ can be 
computed if one can establish an estimate generalizing \iref{estimK2d} according to 
\be
\label{estimK}
\left|  \delta^{\frac 1 {\tau_c}} K_{m,p}(d^m f_\delta(z)) - |[f](x)| |\kappa(x)|^{\frac m {2 d}} \Phi_{m,d}(u) \right|\leq \omega(\delta)
\ee
where $\omega(\delta)\to 0$ as $\delta\to 0$, $x\in \Gamma_\delta^0$, $u\in [-1,1]$, $z = x+\delta u \bn(x)$,
and where the function $\Phi_{m,d} : [-1,1]\to \R$ only depends on $m,d$ and $\vp$. If
\iref{estimK} holds, we then easily derive that
$$
\lim_{\delta \to 0} \delta^{\frac {\tau}{\tau_c}-1}\int_{\Gamma_\delta} K(d^m f_\delta)^\tau=C\int_\Gamma |\kappa|^{\frac {\tau m} {2d}} |[f]|^\tau,
$$
with $C:=\int_{-1}^1|\Phi_{m,d}(u)|^\tau du$, which leads to the proof of the conjecture.

We do not have a general proof of \iref{estimK} for any $m$, $p$ and $d$. 
In the following, we justify its validity in
two particular cases for which the explicit expression of $K_{m,p}$ is known to us:
piecewise quadratic in two space dimensions ($d=2$ and $m=3$)
and piecewise linear  in any dimension ($m=2$).

\paragraph{Piecewise quadratic elements in two dimensions}
For all $\delta>0$, $x\in \Gamma_\delta^0$ and $u\in [-1,1]$, let $\pi_{x,\delta,u}\in \P_3$
 be the homogeneous cubic polynomial on $\R^2$ corresponding to $d^3 f_\delta (x+\delta u \bn(x))$.
Let also $\pi_{x,u}\in \P_3$ be the homogeneous cubic polynomial on $\R^2$ defined by 
$$
\pi_{x,u}(\lambda \bn(x)+\mu \bt(x)) = -\lambda(\Phi''(u) \lambda^2- 3\Phi'(u) \kappa(x) \mu^2)
$$
for all $(\lambda,\mu)\in \R^2$, where $\Phi$ is defined
by \iref{defchi}. For all $x\in \Gamma$, we denote by $M_{x,\delta}$ the (symmetric) linear map defined by 
$$
M_{x,\delta}\bn(x) = \delta \bn(x) \text{ and } M_{x,\delta} \bt(x)= \sqrt \delta \bt(x).
$$
Then, using a reasoning similar to the one used in the appendix of this paper, it can be proved that
\be
\label{limdiscD}
\|\pi_{x,\delta,u} \circ M_{x,\delta} -[f](x)\pi_{x,u}\|\leq \omega(\delta).
\ee
where $\lim_{\delta\to 0} \omega(\delta) = 0$ and the function $\omega$ depends only on $f$.
Furthermore, it is proved in \cite{M} that 
$$
K_{3,p}(\bq) = C \sqrt[4]{|\disc \bq|}
$$
where the positive constant $C$ depends on $p$ and the sign of $\disc \bq$. Combining this expression with \iref{limdiscD} proves the Estimate \iref{estimK} and thus the conjecture in the case $m=3$ and $d=2$.


\paragraph{Piecewise linear elements in any dimension.} We use the second 
fundamental form of the discontinuity set $\Gamma$ in order to evaluate
$d^m f_\delta$ on $\Gamma_\delta$.
At any point $x\in \Gamma\sm \cP$ be denote by $\bn(x)$ the unit normal to $\Gamma$. Note that since 
$\Gamma$ is piecewise $C^2$, the map $x\mapsto \bn(x)$ is 
$C^1$ on $\Gamma\sm \cP$.
Furthermore, we define $T_x\Gamma := \bn(x)^\perp$, the tangent space to $\Gamma$ at $x$.
In a neighbourhood of $x\in \Gamma\sm \cP$, the hypersurface $\Gamma$ admits a parametrization of the form
$$
u\in T_x\Gamma \mapsto x + u+ \lambda(u) \bn(x) \in \Gamma \sm \cP,
$$
where $\lambda$ is a scalar valued $C^2$ function.
By definition, the second fundamental form of $\Gamma$ at the point $x$ is the quadratic form $\II_x$ associated
to $d^2\lambda(0)$ which is defined on $T_x \Gamma\times T_x \Gamma$.
Alternatively, for all $u,v\in T_x\Gamma$ we have $\II_x(u,v) := -\<\partial_u \bn, v\>$.
The Gauss curvature $\kappa(x)$ is the determinant of $\II_x$, in any orthonormal basis of $T_x \Gamma$,
$$
\kappa(z):= \det \II_z.
$$
For example, in two space dimensions the tangent space $T_x\Gamma$ is one dimensional, and we simply have 
$\II_x(u,v) = \kappa(x) \<u,v\>$. Characteristic functions are the simplest type of cartoon functions. In that case, it is possible
to establish a simple relation between the second fundamental form of
the edge set and the second derivatives of $f$ in a distributional sense:
if $\Omega'\subset \R^d$ is a domain with smooth boundary $\Gamma'$ and inward normal $\bn$,
we then have for all $C^2$ test function $\psi$ and $u,v\in \R^d$ 
\be
-\int_\Omega \partial^2_{u,v}\psi = \int_\Gamma \<u,\bn\>\<v,\bn\> (\partial_\bn \psi - \tr(\II) \psi) +\II'(u,v)\psi,
\label{d2charR2eqd}
\ee
where $\II'_x(u,v)$ is the second fundamental form $\II_x$ applied to the orthogonal projection of $u$ and $v$ on $T_x\Gamma$.
The proof of this formula (that generalizes \iref{d2charR2eq} which is proved in the appendix and
corresponds to the two-dimensional case $d=2$) is given further below. For all $x\in \Gamma$, 
we denote by $M_{x,\delta}$ the (symmetric) linear map defined by 
$$
M_{x,\delta}\bn(x) = \delta \bn(x) \text{ and } M_{x,\delta} \bt = \sqrt \delta \bt  
$$
for all $\bt\in T_x\Gamma$.
For all $\delta>0$, $x\in \Gamma_\delta^0$ and $u\in [-1,1]$, let $\pi_{x,\delta,u}\in \P_2$ be the homogeneous quadratic polynomial on $\R^d$ corresponding to $d^2 f_\delta (x+\delta u \bn(x))$.
Let also $\pi_{x,u}\in \P_2$ be the homogeneous quadratic polynomial on $\R^d$ defined by 
$$
\pi_{x,u}(\lambda \bn(x)+\bt) = \Phi'(u) \lambda^2- \Phi(u) \II_x(\bt,\bt)
$$
for all $\bt\in T_x \Gamma$, where $\Phi(x):=\int_{\R^{d-1}}\vp(x,y)dy$.
Then, using formula \iref{d2charR2eqd} and a reasoning analogous to the one presented in the appendix, 
it can be proved that 
\be
\label{limQuadD}
\|\pi_{x,\delta,u} \circ M_{x,\delta} -[f](x)\pi_{x,u}\|\leq \omega(\delta).
\ee
where $\lim_{\delta\to 0} \omega(\delta) = 0$ and the function $\omega$ depends only on $f$.
Furthermore, it is proved in \cite{M} that 
$$
K_{2,p}(\bq) = C \sqrt[d]{|\det \bq|}
$$
where the positive constant $C$ depends on $d,p$ and the signature of $\bq$. Combining this expression with \iref{limQuadD} proves the estimate \iref{estimK} and thus the conjecture in the case $m=2$ in any dimension $d>1$.
\nl
\nl
{\bf Proof of \iref{d2charR2eqd}:}
Let $\proj_\Gamma$ be the orthogonal projection onto $\Gamma$, and for all $x\in \Gamma$ let $\proj_x$ be the orthogonal projection onto $T_x\Gamma$. 
We define $\move : x\in \Gamma\to \proj_\Gamma(x+u)\in \Gamma$. If $\|u\| \|\II\|_{L^\infty(\Gamma)}<1$, then $\move$ is smooth and its differential is given by the following formula
$$
d_x \move = (\Id - \<u, \bn(x')\>\II_{x'})^{-1} \proj_{x'} \in T_{x'} \Gamma
$$
where $x' = \move(x)$, and $d_x \move : T_x\Gamma\to T_{x'}\Gamma$. If follows that 
$$
\det (d_x \move) = \det(\Id - \<u, \bn(x')\>\II_{x'})^{-1}\<\bn(x),\bn(x')\> = 1+\<u, \bn(x')\> \tr(\II_{x'})+ \|u\|\omega(u).
$$
where $\lim_{u\to 0} \omega(u) = 0$.
Furthermore, it is easy to show that 
$$
|\psi(x+u) - \psi(x') -  \<u, \bn(x')\> \partial_{\bn(x')} f(x')|\leq C\|u\|^2,
$$
and $\|n(x') - n(x) - \II_{x'}(\proj_{x'}(u))\|\leq \|u\|\omega(u)$. Combining these results, we obtain
$$
\int_\Gamma \psi(x+u)\<\bn(x),v\> dx = \int_\Gamma \psi(x+u)\<\bn(x),v\> \det (d_{x'} \move_u)^{-1} dx'\\
$$
$$
=\int_\Gamma \<\bn(x'), v\> \psi(x')dx'+ \int_\Gamma \<\bn(x'), v\> \<\bn(x'),u\>(\partial_{\bn(x')} \psi- \tr(\II_x')\psi(x'))
 +\<v,\II_x'(\proj_{x'}(u))\>\psi(x') dx' + \|u\|\omega(u).
$$
Since $- \int_\Omega \partial^2_{u,v}\psi = \lim_{h\to 0} h^{-1}\int_\Gamma (\psi(x+hu)-\psi(x))\<\bn(x),v\> dx$, this concludes the proof.
\sq

\begin{remark}
Similarly to the results presented in \S4, there is an affine invariance property associated to $\kappa$: if $T$ is an affine transformation of $\R^d$ with linear part $L$, 
and if $f = \ti f\circ T$, $\ti \Gamma = T(\Gamma)$ and $\ti \kappa$ is the Gauss curvature of $\ti \Gamma$, then
one has for any $s \geq 0$, 
$$
(\det L)^{\frac{d-1}{d+1}}\int_\Gamma |[f]|^s |\kappa|^{\frac 1 {d+1}} = \int_{\ti\Gamma} |[\ti f]|^s |\ti \kappa|^{\frac 1 {d+1}}.
$$
It follows from this observation that when $p=p_c$, the contribution of the edges is affine invariant in the sense
that 
$$
E_{p_c}(\ti f) = (\det L)^{\frac {d-1}{d+1}} E_{p_c}(f).
$$
Since one also has $A_{m,p}(\ti f) = (\det L)^{\frac {d-1}{d+1}} A_{m,p} (f)$ this comforts the conjecture.
Let us mention that the quantity $|\kappa|^{\frac 1 {d+1}}$ has been used in \cite{Ol} 
in order to define surface smoothing operators that are invariant under affine change of coordinates.
\end{remark}

\section{Conclusion}

In this paper we have investigated the quantity $A_p(f)$ which
governs the rate of approximation by anisotropic $\P_1$ finite elements as a way to
describe anisotropic smoothness of functions. This quantity is not a semi-norm
due to the presence of the non-linear quantity $\det(d^2f)$ 
and cannot be defined in a straightforward manner for general distributions.
We nevertheless have shown that this quantity can be defined
for cartoon images with geometrically smooth edges when $p\leq 2$.
A theoretical issue remains to give a satisfactory meaning to 
the full class of function for which this quantity is finite.

From a more applied perspective, it could be interesting to
investigate the role of $A_p(f)$ in problems where anisotropic
features naturally arise: 

\begin{enumerate}
\item
Approximation of PDE's: in the case of one dimensional hyperbolic conservation laws, it was proved
in \cite{DLu} that despite the appearance of discontinuities
the solution has high order smoothness in Besov spaces
that govern the rate of adaptive approximation by piecewise polynomial.
A natural question is to ask wether similar results hold
in higher dimension, which corresponds to understanding
if $A_p(f)$ remains bounded despite the appearance of shocks.
\item
Image processing: as illustrated in \S 5, the quantity $A_p(f)$ can easily be discretized
and defined for pixelized images. It is therefore tempting to use
$A_2(f)$ in a similar way
as the total variation in \iref{minBV}, by solving a problem of the form
\be
\min_{g\in BV} \{A_2(g)\; ; \; \|Tg-h\|_{L^2}\leq \e\},
\label{minA2}
\ee
with the objective of promoting images with piecewise smooth edges. The main
difficulty is that $A_2$ is not a convex functional. One way to solve this
difficulty could be to reformulate \iref{minA2} in a Bayesian framework as the search of a maximum
of an a-posteriori probability distribution (MAP) as an estimator of $f$. In this framework, we
may instead search for a minimal mean-square error estimator (MMSE)
and this search can be implemented by stochastic algorithms which
does not require the convexity of $A_2$, see \cite{LMo}.
\end{enumerate}


==> Introduction/IntroEngTheseOld.tex <==
%\title{Adaptive and anisotropic finite element approximation:\\Theory and Algorithms}
%%Approximation adaptative et anisotrope par éléments finis\\Théorie et Algorithmes}
%\maketitle
%\tableofcontents

Important : this introduction is only draft, and is not ready to be reviewed.

\section{Anisotropic finite element approximation : why and how?} %Finite element approximation : Motivations, State of the art and Open questions}

Given a triangulation $\cT$ of a bounded polygonal domain $\Omega\subset\R^2$, and a fixed integer $k\geq 1$, we denote by $V_k(\cT)$ the space of finite elements of degree $k$ on $\cT$. The space $V_k(\cT)$ consists of all continuous % almost everywhere bounded 
functions which coincide on each triangle $T\in \cT$ with a polynomial of degree $k$
$$
V_k( \cT) := \{g\in C^0(\Omega) \sep g_{|T}  \text{ is a polynomial of degree $k$ for each } T \in \cT\}.
$$
The dimension of $V_k(\cT)$ is approximately $k^2 \#(\cT)$, and the elements of $V_k(\cT)$ can be efficiently manipulated numerically.

Given a function $f : \Omega \to \R$ and a triangulation $\cT$ of $\Omega$, a natural objective is thus to approximate $f$ using a function $g$ in the space $V_k(\cT)$ of finite elements of degree $k$ on $\cT$, for instance for the purpose of manipulating $f$ numerically. 
This problem, finite element approximation on a given triangulation, is formulated as follows:
\be
\label{eqApproxG}
e_\cT(f)_X := \inf_{g\in V_k(\cT)} \|f-g\|_X.
\ee
The letter $X$ indicates the norm or semi-norm in which the approximation error $\|f-g\|_X$ is measured. In this thesis we restrict our attention to the $L^p$ norm and the $W^{1,p}$ semi-norm, where $1\leq p \leq \infty$. They are defined as follows: 
$$
\|h\|_{L^p(\Omega)} := \left(\int_\Omega |h|^p\right)^{\frac 1 p} \stext{ et } |h|_{W^{1,p}(\Omega)} := \left(\int_\Omega |\nabla h|^p\right)^{\frac 1 p}
$$
The best approximation $g\in V_k(\cT)$ of $f$ can be exactly computed in the case of the $L^2$ norm or the $W^{1,2}$ semi norm: $g$ is the orthogonal projection of $f$ onto $V_k(\cT)$ with respect to the scalar product associated to the norm of interest. In the case $p\neq 2$ of non hilbertian norms the best approximation of $f$ is generally hard to compute, but satisfactory approximations can be obtained using a quasi-interpolant of $f$, see Chapter \ref{chapApproxMet}.
The problem of approximating a given function $f$ on a given triangulation $\cT$, using finite elements of a given degree $k$, is thus solved in good part.

In the context of adaptive approximation, the triangulation $\cT$ of the domain $\Omega$ is not given, but can be freely chosen - in contrast we assume in this thesis that the integer $k$ is fixed although arbitrary. The triangles constituting the mesh $\cT$ may vary strongly in shape an size for a better adaptation to the local features of the approximated function $f$, which naturally raises the objective of characterizing and constructing an optimal mesh for a given function $f$. Given a norm $X$ of interest, an integer $N>0$ and a function $f$ to be approximated, we formulate this optimization problem, optimal mesh adaptation, as follows:
\be
\label{eqApproxT}
e_N(f)_X := \inf_{\#(\cT) \leq N} e_\cT(f)_X.
\ee
In contrast to the problem \iref{eqApproxG} of finite element approximation on a fixed mesh, the problem of adaptive and anisotropic approximation \iref{eqApproxT} is not yet well understood.
Heuristically, the simplicity of \iref{eqApproxG} comparatively to \iref{eqApproxT} is due to the fact that the optimization is posed on the linear space $V_k(\cT)$. %: for any $g,g'\in V_k(\cT)$ we have $g+g'\in V_m(\cT)$. 
The methods mentioned for solving \iref{eqApproxG}, such as the orthogonal projection or the quasi-interpolation, make indeed a key use of this property.
In contrast the optimization problem \iref{eqApproxT} is posed on the collection of triangulations $\cT$ satisfying $\#(\cT)\leq N$, which is certainly not a vector space.
%and the sum $\cT+\cT'$ of two triangulations has no meaning in general.

%In order to compensate for this problem one o
The optimization \iref{eqApproxT} is restricted in a number of applications to a family $\bT_*$ of triangulations possessing a property of hierarchy, see for instance \cite{Nochetto}. For each pair of triangulations $\cT, \cT'\in \bT_*$, the hierarchy property guarantees that there exists a common refinement $\wti \cT\in \bT_*$ of $\cT$ and $\cT'$ satisfying $\#(\wti \cT) \leq C (\#(\cT)+ \#(\cT'))$. The common refinement $\wti \cT$ plays in a certain sense the role of the sum $\cT+ \cT'$, and the techniques of linear analysis can be used to understand most aspects of the optimization problem \iref{eqApproxT} restricted to triangulations in $\bT_*$:
\be
\label{eqApproxIso}
\inf \{ e_\cT(f)_X \sep \#(\cT) \leq N \text{ and } \cT \in \bT_* \}.
\ee
This approach has led to successful developments which are out of the scope of this thesis, we refer the interested reader to \cite{Nochetto} for an application of this method to numerical solutions of partial differential equations.

%The problem \iref{eqApproxIso} imposes a strong restriction on the triangulations. Indeed T
The families $\bT_*$ of triangulations satisfying a property of hierarchy usually consist of uniformly isotropic triangulations. In other words the approximation problem \iref{eqApproxIso} allows to finely tune the areas of the triangles $T\in \cT$ with respect to the approximated function $f$, but not their elongation and orientation.
%In other words a triangulation $\cT\in \bT_*$ consists of elements $T\in \cT$ which may have areas of distinct orders of magnitude, but which shapes vary little and remain close to the equilateral triangle.
This restriction strongly penalizes the approximation of certain classes of function $f$, in particular  the class of cartoon functions which involve discontinuities along some smooth curves. As illustrated on Figure \ref{figPeyre} the use of anisotropic triangulations, which involve thin and long triangles aligned with the discontinuities of $f$, is particularly appropriate in that context and significantly reduces the approximation error $e_\cT(f)_X$ for a given cardinality $\#(\cT)=N$. 
%The minimum \iref{eqApproxT} is therefore significantly smaller than the minimum \iref{eqApproxIso} which is restricted to the family $\bT_*$ of triangulations, which are generally isotropic. %of, usually isotropic, triangulations.

The purpose of this thesis is to better understand the problem \iref{eqApproxT} posed on the full class of (potentially anisotropic) triangulations. We have addressed in particular the following questions:
%\begin{enumerate}[$\bullet$]
\begin{enumerate}[I]
\item 
What is the behavior of $e_N(f)_X$ in the asymptotic setting where the number $N$ of triangles is sufficiently large and the approximated function $f$ is sufficiently smooth? In that context the resolution is sufficient to produce a triangulation $\cT$ well adapted to the local features of $f$, and to obtain an explicit equivalent of (a slightly modified version of) $e_N(f)_X$. 
\item 
Which classes of functions are naturally tied to the approximation problem \iref{eqApproxT}? In particular what can be said of the model of cartoon functions? These functions are smooth except along a collection of smooth curves, where they exhibit discontinuities, and anisotropic methods are particularly appropriate for their approximation, see Figure \ref{figPeyre}. Cartoon functions are a popular image model in the image processing community.
\item 
%Is there a mathematical object which is rigorously equivalent to triangulations
%Could the optimization problem \iref{eqApproxT} posed on triangulations $\cT$ of a given cardinality $N$, be replaced with a more well posed mathematical object?
Triangulations are combinatorial objects, described in terms of points and edges, 
which is not handy when solving optimization problems of the form \iref{eqApproxT}. 
We study the correspondence between certain classes of triangulations and of riemanninan metrics. The latter are continuous objects governed by simple equations, which allows reformulate and to solve some optimization problems posed on triangulations. %of the family of \iref{eqApproxT}.
\item 
How to combine adaptive anisotropy with hierarchy?
%Is it possible to combine hierarchy with adaptive anisotropic triangulations?
This is indeed possible, but at the following price: the hierarchical family needs to be adapted to the approximated function $f$. This must be contrasted with the hierarchical family  $\bT_*$ of triangulations, involved in \iref{eqApproxIso}, which is defined independently $f$.
\end{enumerate}
%\end{itemize}
The four parts of this thesis are devoted to these four questions respectively, which are also discussed in more detail in the second half of this introduction.
We now give some motivations to the subject of this thesis, the in depth study of the approximation error $e_N(f)_X$. %, we give some motivations to the study of the problem \iref{eqApproxT}.
Note that, depending on the context, the approximated function $f$ may be fully known to us: through an explicit formula or a discrete sampling; or observed through noisy measurements; or implicitly defined as the solution to a partial differential equation.

\subsection{Motivations}
\paragraph{Partial differential equations.\\} %Equations aux dérivées partielles.\\} %La méthode des éléments finis}

Numerical methods for partial differential equations, PDEs, attempt, for a given cost in terms of computer time, to obtain the best possible approximation of a function $f$ implicitly  defined as the solution to a partial differential equation.
Some of these methods take as input a mesh $\cT$ of the computational domain $\Omega$, and return an approximate solution under the form of a finite element approximation $f_\cT\in V_k(\cT)$ of the exact solution $f$. 
As observed below for the heat equation \iref{eqOptiHeat}, if the norm $X$ is well chosen and the problem is well posed, then the approximate solution $f_\cT\in V_k(\cT)$ may not be far from the being the best approximation of $f$ on $\cT$. Furthermore the cost of the computation of the approximate solution $f_\cT\in V_k(\cT)$ is heavily tied to the cardinality $\#(\cT)=N$.

The solutions of partial differential equations often exhibit some strongly anisotropic features. We think in particular of boundary layers in fluid simulation,
metallic spikes and edges in electromagnetism,
or shock waves in transport equations.
This observation raises the need for adapting the mesh $\cT$ to the exact solution $f$ of the PDE. Ideally for a given budget of computer time, which corresponds to a simulation on an arbitrary triangulation of cardinality $N>0$, one should run the simulation on the triangulation $\cT$ which minimizes $e_\cT(f)_X$.
This optimal triangulation can  generally not be obtained because the exact solution $f$ to the PDE is not known, and because the optimization among triangulations of a given cardinality of the approximation error $e_\cT(f)_X$ is a difficult problem, even in the case where the approximated function is explicitly known. Before considering the difficulties of adaptive mesh generation, let us nevertheless contemplate its possible advantages.

%In order to illustrate this point w
We consider the simplest class of PDEs : elliptic equations. Let $\Omega$ be a bounded polygonal domain, let $a\in L^\infty(\Omega)$ and let $b\in L^2(\Omega)$. We assume that there exists two positive constants $\lambda, \Lambda$ such that $0 < \lambda \leq a \leq \Lambda$ on $\Omega$ and we look for the solution of the classical Poisson problem
\be
\label{eqEllSystem}
\left\{\begin{array}{rcl}
-\diver(a \nabla f) &= b & \text{ on } \Omega \\
f  &=  0 & \text{ on } \partial \Omega.
\end{array}
\right.
\ee
This system of equations can be reformulated as a convex minimization problem: find $f\in H^1_0(\Omega)$ which minimizes the following ``energy''
\be
\label{eqMinCvx}
\frac 1 2\int_\Omega a |\nabla f|^2 - \int_\Omega f b.
\ee
Given a mesh $\cT$ of $\Omega$, denote by $f_\cT$ the element of $V_k(\cT)$ which vanishes on $\Omega$ and minimizes \iref{eqMinCvx}. Cea's lemma guarantees an error estimate in the $H^1_0$ norm, which is also the  $X=W^{1,2}$ semi-norm:
\be
\label{eqOptiHeat}
|f-f_\cT|_X %{H^1_0(\Omega)} 
:= \|\nabla f-\nabla f_\cT\|_{L^2(\Omega)} \leq \sqrt{\Lambda/ \lambda} \ e_\cT(f)_X. %\frac {\Lambda}{\lambda}
\ee
As announced, the approximation $f_\cT$ is not far from being the best possible approximation of $f$ in $V_k(\cT)$. From a numerical point of view, the cost of computing $f_\cT$ mostly depends on $\#(\cT)$, at least for isotropic triangulations (In the case of anisotropic triangulations this cost may increase because of the deterioration of the conditioning of the linear system). 
%Furthermore the solution $f$ of the elliptic system \iref{eqEllSystem} does exhibit varying degrees of regularity, depending on the position in $\Omega$ and on the direction. 
The exact function $f$ has relatively low regularity at the corners of $\Omega$ and at the places where the diffusivity coefficient $a$ is discontinuous, which raises the need for adaptive triangulations. We are thus naturally led to the problem \iref{eqApproxT}. 

One of the difficulties of mesh adaptation for PDEs is that the approximated function $f$, which is by nature unknown, cannot be directly exploited to build the triangulation $\cT$. One therefore uses an iterative approach: starting from a coarse triangulation $\cT_0$ of $\Omega$ the following loop is executed for $n \geq 0$:
\begin{enumerate}
\item (Solve) The approximate solution $f_{\cT_n}$ of $f$ on the mesh $\cT_n$ is computed. 
\item (Estimate) Some properties of the exact solution $f$ are estimated from its approximation $f_{\cT_n}$. In particular some error indicators.
\item (Mark) The positions in the domain $\Omega$ where the triangulation should be refined, potentially anisotropically, are marked.
\item (Refine) A mesh generator produces the triangulation $\cT_{n+1}$, and the algorithm goes back to step 1. 
\end{enumerate}
The loop is interrupted when $\#(\cT_n)$ exceeds some value $N$ fixed in advance, or when $|f-f_{\cT_n}|_X$ passes beyond a threshold value $\ve$.

This procedure is analysed in depth in \cite{Nochetto} in the case of hierarchical isotropic mesh adaptation  mentioned in \iref{eqApproxIso}.  Some optimality results are established and the improvement due to mesh adaptation is illustrated by numerical examples. Unfortunately this approach seems difficult to extend to anisotropic triangulations, because it heavily relies on the hierarchy of a family of isotropic triangulations, defined independently of $f$. 
The paper \cite{St2} considers tensor product anisotropic wavelet spaces, instead of triangulations, and establishes that adaptive and anisotropic methods can be successfully used to solve elliptic PDEs, when they are posed on the domain $\Omega = [0,1]^2$ or $[0,1]^d$ in $d$-dimensions. The drawback of anisotropic tensor product wavelets, compared to anisotropic triangulations, is their strong coordinate bias: they are only useful for anisotropic features of the approximated function $f$ aligned with the coordinate axes - such features appear on the boundary of $[0,1]^d$ for the solutions of elliptic equations posed on this domain.

Various numerical methods for PDEs take advantage of anisotropic triangulations using similar ideas, in particular the algorithmic loop mentioned above, see for instance the software \cite{FreeFem, Inria}. However these methods are not yet well understood theoretically, and they only apply to linear finite elements.
One of the purposes of this thesis obtain a better understanding of the steps Mark and Refine of the mesh adaptation loop, and to extend them at least to quadratic finite elements.

\begin{figure}
	\centering		
	\includegraphics[width=4.5cm,height=3cm]{\pathPic/SimuExt/AlauzetPlane.pdf}
	\hspace{1cm}
	\includegraphics[width=3.5cm,height=3cm]{\pathPic/SimuExt/AlauzetShock.pdf}
	\caption{Airflow around a supersonic plane. (credit : Fr\'ed\'eric Alauzet \cite{A}.\label{figInria}})
\end{figure}

\paragraph{Image compression.\\}

In the context of image compression the domain $\Omega$ is generally the unit square $\Omega = [0,1]^2$. For simplicity we restrict our attention to monochromatic images, which are defined by the value at each point $x\in \Omega$ of a brightness $f(x) \in [0,1]$. Given a triangulation $\cT$ of $\Omega$, an approximation of the image can be stored under the form of an approximation $g\in V_k(\cT)$ of the brightness $f$.

The quality of the approximation $g$ of a monochromatic image of defined by a brightness $f$ is usually measured using the $\PSNR_f$ (Peak Signal Noise Ratio with respect to $f$)
$$
\PSNR_f (g) := - 10 \frac {\ln \|f-g\|_{L^2}}{\ln 10}. %r \ln \|f-g\|_{L^2(\Omega)} \text{ %10 \frac {\ln \|f-g\|_{L^2}}{\ln 10}.
$$
A natural objective is store an approximation $g$ of an image defined by the brightness $f$, for a given cost in terms of computer memory, with the smallest possible distortion $\PSNR_f(g)$.
Given a triangulation $\cT$ of $\Omega$, the minimal value of $\PSNR_f(g)$, or equivalently $\|f-g\|_{L^2}$, is attained by the orthogonal projection of $f$ on $\cT$ which is easy to compute numerically.
The cost in terms of computer memory of storing the orthogonal projection of $f$ on $V_k(\cT)$, or any other element of $V_k(\cT)$, is approximately equal to $\dim(V_k(\cT)) \simeq k^2\#(\cT)$. We are thus again led to the mesh optimization problem \iref{eqApproxT}, with the norm $X=L^2$.
Obtaining the optimal mesh is known to be a NP hard problem, and is therefore not a realistic objective. Nevertheless the method proposed for instance in \cite{DDI} provides good candidates which leads to a competitive approximation method.

Methods based on (potentially) anisotropic triangulations are particularly well adapted to images of geometrical nature, such as ``cartoon'' images, which are smooth except along some discontinuities, themselves occuring along smooth curves.
As illustrated on Figure \ref{figPeyre}, anisotropic triangulations featuring thin and long triangles aligned with these discontinuities allow to produce faithful approximations of cartoon functions with only few degrees of freedom.
In contrast, methods based on (anisotropic) triangulations generally do not show any gain compared for instance to wavelet based methods for images containing a lot of texture. Chapter \ref{chapCartoon} examines in detail the link between image models and adaptive anisotropic approximation.

The production of a good triangulation $\cT$ for the approximation of a function $f$ is a difficult problem for which several algorithms have been proposed. The iterative thinning algorithm presented in \cite{DDI} is particularly competitive in practice, but is not guaranteed from a theoretical point of view.
The algorithm presented in \cite{Peyre} first produces continuous object, a riemannian metric from the image, and then generates a mesh based from this metric. This type of mesh generation is analysed in Chapter \ref{chapMeshMet}. Last we study in Chapter \ref{chapCDHM} and algorithm producing anisotropic and hierarchical triangulations, which can be used in the context in image approximation.

\begin{figure}
\centering
\includegraphics[width=3.5cm,height=3.4cm]{\pathPic/Cartoon/Triangle.pdf}
\hspace{0.0cm}
{\raise -0.07cm \hbox{\includegraphics[width=3.7cm,height=3.55cm]{\pathPic/Cartoon/Haar.pdf}}}
\includegraphics[width=3.5cm,height=3.4cm]{\pathPic/Cartoon/TriangleMeshed.pdf}
\caption{A Cartoon function, isotropic refinement associated to the Haar wavelet, an adapted anisotropic triangulation. (credit : Gabriel Peyr\'e\label{figPeyre}\label{figPeyre}})
\end{figure}



\subsection{State of the art}

We give in this section a short overview of the state of the art in the following problem of anisotropic finite element approximation : the evaluation of the minimal approximation error $e_N(f)_X$ and the construction of a close to optimal triangulation. For that purpose we need to introduce some notations.
We assume in the following that $f\in C^0(\overline \Omega)$, where $\Omega \subset \R^2$ is a bounded polygonal domain. For each triangulation $\cT$ of $\Omega$ we denote by $\interp^k_\cT$ the standard interpolation operator on Lagrange finite elements of degree $k$ on $\cT$. If the triangulation $\cT$ is conforming, then $\interp_\cT^k f$ is continuous and therefore $\interp_\cT^k f\in V_k(\cT)$. In order to be consistent with the rest of this thesis we define $m := k+1\geq 2$, and we thus have 
$$
e_\cT(f)_{L^p} \leq \|f-\interp_\cT^{m-1} f\|_{L^p(\Omega)} \stext{ and } e_\cT(f)_{W^{1,p}} \leq  \|\nabla f-\nabla \interp_\cT^{m-1} f\|_{L^p(\Omega)}.
$$
Any estimate on the interpolation error thus automatically yields an upper estimate on the best approximation error $e_\cT(f)_X$. Furthermore if $f$ is sufficiently smooth and if $\cT$ is sufficiently fine, then these quantities are generally comparable.



One of the founding results of adaptive anisotropic finite element approximation is the following, see \cite{CSX} or \S \ref{secOptAniso}. For any bounded polygonal domain $\Omega\subset \R^2$, for any $1 \leq p < \infty$, and for any function $f\in C^2(\overline \Omega)$ there exists a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqCSX}
\limsup_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \leq C \left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)}.
\ee
In the previous equation the exponent $\tau \in (0, \infty)$ is defined by $\frac 1 \tau := 1 + \frac 1 p$, and $C$ is a universal constant ($C$ is independent of $p$, $\Omega$ and $f$).
This result can be extended to the exponent $p=\infty$, and to dimensional domains $\Omega$ of higher dimension, but the triangulations $\cT_N$ may not be conforming

The result \iref{eqCSX} reveals that the quality of the approximation of $f$ is governed by the quantity $\sqrt{|\det(d^2 f)|}$, which depends non-linearly on the hessian matrix $d^2 f$. This non-linear dependency is heavily tied to the fact that we authorize triangles of potentially highly anisotropic shape. The estimate \iref{eqCSX} is obtained by producing sufficiently fine triangulations which combine the two following properties:
\begin{enumerate}[a)]
\item (Error equidistribution) The triangulations $\cT_N$ follow a general rule of adaptive approximation theory: the contribution $\|f-\interp_T^{m-1}f\|_{L^p(T)}$ of each triangle $T \in \cT_N$ to the global interpolation error $\|f-\interp_{\cT_N}^{m-1}f\|_{L^p(\Omega)}$ is approximately the same. This condition can be translated into a local constraint on the area of the triangles, which is dictated by the local behavior of $f$ and in particular by $\det(d^2f(z))$.
\item (Optimal shape of the triangles) 
The elements of $\cT_N$ have a shape which is dictated locally by the hessian matrix $d^2 f(z)$. This shape is potentially highly anisotropic, elongated and oriented is a precise manner which depends on the eigenvalues and eigenvectors of the hessian matrix $d^2f(z)$.
\end{enumerate}
The simplest method for producing a sequence $(\cT_N)_{N \geq N_0}$ of triangulations satisfying \iref{eqCSX} is to use a ``local patching strategy'' as follows. In a first step the domain $\Omega$ is split in regions $\Omega_i$, $1\leq i \leq k$, sufficiently small so that the hessian matrix $d^2f(z)$, $z\in \Omega_i$, varies little around an average value $M_i$. Each region $\Omega_i$ is then tiled using a periodic triangulation $\cT_N^i$ based on $M_i$, in other words $f$ is identified to a quadratic polynomial on each $\Omega_i$. Eventually the triangulations $\cT_N^i$ of $\Omega_i$ are glued together into a triangulation $\cT_N$ of $\Omega$, at the price of a few additional triangles at the boundaries of the $\Omega_i$. 

This construction is sufficient for the proof of the asymptotical result \iref{eqCSX}, but not for practical applications since it only becomes efficient for a large number of triangles. The following approach, based on riemannian metrics, is often preferred in applications.
We assume for simiplicity that the hessian matrix $M(z) := d^2f(z)$ is positive definite for each $z\in \Omega$, and we define 
\be
\label{defHHessian}
H(z) := \lambda^2 (\det M(z))^{-\frac 1 {2p+2}} M(z)
\ee
where $\lambda>0$ is a constant which role is specified later. Such a map $H : \Omega\to S_2^+$ associates continuously to each point a positive definite matrix, and is called a riemannian metric. Note that for each $z\in \Omega$ the matrix $H(z)$ defines an ellipse
$$
\cE_z := \{z+u \sep u^\trans H(z) u\leq 1\}.
$$ 
As illustrated on the left part of Figure \ref{figEllTri}, a metric encodes at each point $z\in \Omega$ an information of area, elongation and orientation, under the form of a symmetric positive definite matrix $H(z)$, or equivalently of an ellipse $\cE_z$. 
Several algorithms, such as \cite{FreeFem,Inria} are able to produce a triangulation adapted in the following sense to a given metric  : for each $z\in \Omega$ the triangle $T\in \cT$ containing $z$ has a shape similar to $\cE_z$.
%We now assume that $\lambda$ is sufficiently large, and that a triangulation $\cT$ of $\Omega$ has been produced in such way that for each $z\in \Omega$ the triangle $T\in \cT$ containing $z$ has a shape similar to $\cE_z$.
If $\cT$ is such a triangulation and if $\lambda$ is sufficiently large, a heuristic argument developed in Chapter \ref{chapOptAniso} %\ref{secOptAniso4} 
shows that 
$$
\#(\cT) \|f-\interp_{\cT}^1 f\|_{L^p(\Omega)} \leq C \|\sqrt{|\det (d^2f)|}\|_{L^\tau(\Omega)}.
$$
Varying the parameter $\lambda$ we obtain different triangulations $\cT_\lambda$, of cardinality proportional to $\lambda$, which leads to the error estimate \iref{eqCSX}.
The production of the mesh $\cT$ from the metric $H$ is not straightforward, and some aspects of this question are addressed in Chapter \ref{chapMeshMet}.
\begin{figure}
\centering
\includegraphics[height = 4cm,width = 8cm]{\pathPic/Ellipses/EllShewChuk.pdf}
\caption{A metric and an adapted triangulation, (credit : J. Schoen\label{figEllTri}})
\end{figure}

The approximation result \iref{eqCSX} is optimal if we restrict our attention to admissible sequences of triangulations, a technical condition as follows. %provided the following technical condition is satisfied.
We say that a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of a polygonal domain $\Omega \subset \R^2$ is admissible if  $\#(\cT_N) \leq N$ and if 
\be
\label{defAdmiIntro}
\sup_{N \geq N_0} \left(\sqrt N \max_{T \in \cT_N} \diam(T)\right) <\infty.
\ee
For any admissible sequence $(\cT_N)_{N \geq N_0}$ of triangulations of a $\Omega$, one can establish the lower bound 
\be
\label{eqCSXOpt}
\liminf_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \geq c \left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)},
\ee
where the constant $c>0$ is universal, see also Theorem \ref{thLowerLPIntro} below. % Therefore \iref{eqCSX} is optimal if we restrict our attention to admissible 
Furthermore the admissibility condition is not too restrictive : for each $\ve>0$ there exists an admissible sequence of triangulations $(\cT_N)_{N \geq N_0}$ which satisfies the upper estimate \iref{eqCSX} up to the additive constant $\ve$.

Similar results to \iref{eqCSX} and \iref{eqCSXOpt} can be developed for isotropic meshes, in which the elements may vary in size but are constrained to be isotropic in the sense that the measure of degeneracy $\rho(T) := \diam(T)^2/|T|$ is uniformly bounded by a constant $\rho_0$, see for instance \cite{CMi2}.
In that case one needs to replace 
$$
\left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)} \stext{ with } \|d^2f\|_{L^\tau(\Omega)}
$$
in \iref{eqCSX} and \iref{eqCSXOpt}, and the constants $c$ and $C$ depend on the bound $\rho_0$ on the measure of degeneracy, see for instance \cite{CMi2}.
%The improvement due to anisotropy is thus the replacement at each point $z\in \Omega$ of the norm $\|d^2 f(z)\|$ with the non-linear quantity $\sqrt{|\det (d^2f(z))|}$. 
In terms of the eigenvalues $\lambda_1(z), \lambda_2(z)$ of the symmetric matrix $d^2 f(z)$ we thus replace
$$
\sqrt{|\lambda_1(z) \lambda_2(z)|}  \stext{ with } \max \{|\lambda_1(z)|, |\lambda_2(z)|\}.
$$
The use of anisotropic triangulations is therefore particularly advised when the eigenvalues of $d^2 f(z)$ have very different orders of magnitude. This is the case if the approximated function $f$ exhibit strongly anisotropic features in certain regions.

\subsection{Open Questions}
The result \iref{eqCSX} gives a sharp account of the improvement that anisotropic triangulations can provide compared to isotropic triangulation, under certain restrictive conditions. 
We have attempted to list these restrictions and to eliminate them when possible.
The four conditions mentioned below are the object of an in depth study in this thesis and could be eliminated, at least partly.
\begin{enumerate}[I]
\item (Other degrees, other norms)
We extend in Chapter \ref{chapOptAniso} the estimate \iref{eqCSX} to finite elements of arbitrary degree $m-1$, and to the Sobolev $W^{1,p}$ norms.
 Comparatively, the original result only applies to piecewise linear finite elements $m-1= 1$ and to $L^p$ norms. We obtain asymptotical error estimates and optimality results which are similar to \iref{eqCSX} and \iref{eqCSXOpt}. The determinant of the hessian matrix $\det (d^2 f)$ appearing in the original estimate is replaced with an ``invariant polynomial'' applied to the collection $d^m f$ of the $m$-th derivatives of $f$.

The combination of the following properties guarantees that a triangulation $\cT$ satisfies the optimal error estimate up to a fixed multiplicative constant, see Chapter \ref{secW1P2} for more quantitative analysis of these properties. First the interpolation error needs to be equidistributed among all triangles $T\in \cT$. Second the triangles need to have an optimal shape, which is now dictated by the $m$-th order derivatives of $f$, instead of the hessian matrix. Third the triangulation needs to be sufficiently fine in such way that $f$ is well approximated on each triangle by a polynomial of degree $m$. In the case of Sobolev $W^{1,p}$ norms a fourth property needs to be satisfied : any angle $\theta$ of any triangle $T\in \cT$ should be sufficiently far away from the flat angle, in other words $\theta< \theta_{\rm max} < \cPi$.

\item (Non smooth functions) 
We consider in Chapter \ref{chapCartoon} the model of cartoon functions, which is popular in image processing. These function are smooth except along a finite collection of smooth curves where they have jump discontinuities.

Cartoon functions are not differentiable, and the quantity $\|\sqrt{|\det d^2f|}\|_{L^\tau}$ which appears in \iref{eqCSX} has therefore no meaning a-priori. We show nevertheless that for some values of $\tau$ this quantity has a natural extension to cartoon functions $f$, which includes a one-dimensional integral along the collection $\Gamma$ of curves where $f$ is discontinuous. This contribution takes into account the jump of $f$ across $\Gamma$ as well as the curvature of $\Gamma$. However the extension of the approximation result \iref{eqCSX} in that context remains so far a conjecture.

\item (Mesh generation)
The most popular methods for anisotropic mesh generation in applications are based on Riemannian metrics, as exposed in \iref{defHHessian}. These metrics encode at each point the desired size, elongation and orientation of the triangles.

This raises the objective of defining and proving precise equivalence results between some classes of triangulations and of metrics. We answer this question in Chapter \ref{chapMeshMet}, and thus provide a translation of some geometrical properties of triangulations into regularity properties satisfied by the corresponding metrics. We pay a particular attention to the angle condition evoked in 1. for the approximation of function in the $W^{1,p}$ semi-norm, the fact that the angles appearing in the triangulation are uniformly bounded away from $\cPi$. These results are used in Chapter \ref{chapApproxMet} to reformulate, and solve in some cases, several optimization problems posed on triangulations.

\item (Combining hierarchy with anisotropy) 
A number of algorithms are based on hierarchical sequences of triangulations $(\cT_N)_{N \geq N_0}$, a property which guarantees % The fact that $\cT_{N+1}$ is a refinement of $\cT_N$ implies 
the inclusion of the associated finite element spaces $V_k(\cT_N)\subset V_k(\cT_{N+1})$. This property allows to separate details of different scales in the context of image processing, and is also a key to the in the analysis of some PDEs.

We define in Chapter \ref{chapCDHM} an algorithm producing sequences of (non conforming) anisotropic triangulations which satisfy this property of hierarchy, and in certain circumstances also satisfy the optimal error estimate \iref{eqCSX}. This algorithm strongly differs from the mesh generation methods presented previously, the local patching strategy and the approach based on riemannian metrics, since these are not adapted to hierarchical mesh refinement.
\end{enumerate}

Current results in anisotropic mesh adaptation for finite element approximation %, the study of $e_N(f)_X$, 
also suffer from two other important restrictions : they are only asymptotical, and they extend with difficulty to dimensions larger than two.
%The results presented in this section, which are more or less the state of the art in anisotropic mesh adaptation, also suffer from two other weaknesses. 
Removing these two restrictions raises difficult problems and remains mostly an open question at the time of writing.
\begin{itemize}
\item (Non asymptotical results) 
The optimal error estimate \iref{eqCSX} involves a limit as the number $N$ of triangles constituting the mesh $\cT_N$ tends to infinity, recall that % We recall that 
for any sequence $(u_N)_{N \geq N_0}$ %one has
$$
\limsup_{N \to \infty} u_N := \lim_{N \to \infty} \sup_{n \geq N} u_n.
$$
The asymptotic nature of this error estimate reveals that a sufficiently large number of triangles is needed to finely tune the triangulation $\cT_N$ to the local properties of the approximated function $f$. A smaller number of triangles raises the need for a compromise between the adaptation to the local features approximated function $f$ and the geometrical constraints involved in the production of a bi-dimensional triangulation.

We give in Chapter \ref{chapMeshMet} a translation of these geometrical constraints into the form of regularity properties satisfied by riemannian metrics, continuous objects which are equivalent to triangulations, see Theorem \ref{thMeshMetIntro}. In the case of isotropic triangulations we recover in Chapter \ref{chapApproxMet} some classical error estimates, expressed in terms of the Hardy-Littlewood maximal function of $|d^mf|$,  for the quantity 
$$
\sup_{N \geq 1} N^\frac m 2 e_{\cT_N} (f)_X \quad \left(\text{ instead of } \limsup_{N \to \infty} N^\frac m 2 e_{\cT_N} (f)_X\right).
$$
Obtaining a relevant estimate of this quantity in the case of anisotropic triangulations remains today an open question. \\

\item (Meshes in three or more dimensions) 
Throughout this introduction, we have yet only considered functions of two variables and bi-dimensional triangulations. 
Our discussion remains relevant in dimension three or higher, and three dimensional anisotropic mesh adaptation is already successfully used in applications, see for instance \cite{A}.

However a number of theoretical aspects of these methods remain unanswered. The key difficulty is the production of three dimensional anisotropic meshes, which is difficult from a practical point of view and not well understood from a theoretical point of view. We formulate in Chapter \ref{chapMeshMet} several conjectures which extend our bi-dimensional results on the equivalence of meshes and riemannian metrics.

We also consider dimensions larger than $2$ in parts I and II of this thesis, % (OptAniso??) and (Cartoon??),
which leads us to several types of difficulties. Some of these difficulties have an algebraic nature in Chapter \ref{chapOptAniso}, a geometric nature in Chapter \ref{chapCartoon}, or are related to mesh generation in Chapter\ref{chapW1P}. We formulate a precise conjecture each time that we cannot solve these difficulties.\\ 
\end{itemize}

Last, the two following questions could be raised about the results \iref{eqCSX} and \iref{eqCSXOpt} on optimal mesh adaptation presented in this introduction. We regard them as more minor and they are not the subject of in depth discussion in this thesis.
\begin{itemize}
\item (Interpolation instead of best approximation)
Some estimates presented in this introduction, such as \iref{eqCSX}, are based on the interpolation error instead of the best approximation error. In other words, for a given function $f$ and triangulation $\cT$ they provide an upper bound for 
\be
\label{eqInterp}
\|f-\interp_\cT^{m-1} f\|_{L^p} \stext{ or } \|\nabla (f - \interp_\cT^{m-1} f)\|_{L^p}
\ee
instead of 
\be
\label{eqBestApprox}
e_\cT(f)_{L^p} := \min_{g\in V_{m-1}(\cT)} \|f-g\|_{L^p} \stext{ or } e_\cT(f)_{W^{1,p}} := \min_{g\in V_{m-1}(\cT)} \|\nabla (f-g)\|_{L^p}.
\ee
The quantities \iref{eqInterp} correspond to the particular choice $g=\interp_\cT^{m-1} f$ and are therefore an upper bound for the corresponding quantities in \iref{eqBestApprox}. The difference is it so big that an estimate on \iref{eqInterp} is not relevant in the case \iref{eqBestApprox}?
The answer is generally no if the function $f$ is sufficiently smooth and if the triangulation $\cT$ is sufficiently fine, which is the case in the asymptotic setting considered in \iref{eqCSX}.
In contrast we consider in the Chapter \ref{chapApproxMet} some functions of weaker regularity, and triangulations of fixed cardinality, which forbids the use of the standard Lagrange interpolation operator. The interpolation of $f$ is thus replaced with an quasi-interpolation of the local averages of $f$.\\

\item (The admissibility condition) 
The optimality results presented in this thesis, such as \iref{eqCSXOpt}, require the admissibility of the sequence $(\cT_N)_{N\geq N_0}$ of triangulations. This technical hypothesis can be removed in certain cases, such as the interpolation of a convex function by finite elements of degree one, see \cite{BBLS}.
We have not been able to remove this hypothesis in the general case, but we believe that the admissibility condition is rather a technical inelegancy than a weakness of the theory.
\end{itemize}

\section{Outline of the thesis}
%\label{secIntro2}

This thesis is composed of four parts I to IV which correspond to four key questions in anisotropic finite element approximation : approximation using finite elements of arbitrary degree, or measured in Sobolev norms; the link between anisotropic smoothness classes and image models; the equivalence between certain classes of triangulations and of  riemannian metrics; and eventually the combination of hierarchy with anisotropy.

These four parts, as well as the nine chapters composing them, are mostly self consistent and can be read independently.

\subsection{Finite elements of arbitrary degree, and Sobolev norms} %Elements finis de plus haut degré, normes de Sobolev}%Premier objectif : que peut-on faire de mieux, asymptotiquement?}

We have extended the optimal asymptotic estimate \iref{eqCSX} to finite elements of arbitrary degree. In order to present our results we need to introduce some notations.

We denote by $\H_m$ the space of homogeneous polynomials of degree $m$:
$$
\H_m := \Span\{x^k y^l \sep k+l = m\}.
$$
A key ingredient of our approach is the shape function $K_{m,p} : \H_m \to \R_+$, where $1\leq p\leq \infty$ is an exponent. 
This function is defined as an optimization of the $L^p$ interpolation error among the collection of triangles of unit area of all possible shapes: for all $\pi\in \H_m$,
\be
\label{defKMPIntro}
K_{m,p}(\pi) := \inf_{|T| = 1} \|\pi-\interp_T^{m-1} \pi\|_{L^p(T)}.
\ee
Our main result is the following asymptotic error estimate.
\begin{theoremIntro}
\label{thOptiLPIntro}
Let $\Omega\subset \R^2$ be a bounded polygonal domain, let $f\in C^m(\overline \Omega)$ and let  $1\leq p < \infty$.
There exists a sequence $(\cT_N)_{N \geq N_0}$ of conforming triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqLPIntro}
\limsup_{N \to \infty} N^{\frac m 2}\|f-\interp_{\cT_N}^{m-1} f\|_{L^p(\Omega)} \leq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)}, \stext{ where } \frac 1 \tau := \frac m 2 + \frac 1 p.
\ee
\end{theoremIntro}

In the error estimate \iref{eqLPIntro}, we identify the collection $d^m f(z)$ of derivatives of order $m$ of $f$ at the point $z\in \Omega$ to the corresponding homogeneous polynomial in the Taylor development of $f$ at $z$. In other words
$$
\frac {d^m f(z)}{m!} \sim \sum_{k+l = m} \frac{\partial^m f(z)}{\partial^k x\, \partial^l y} \, \frac {x^k}{k!} \frac {y^l}{l!}.
$$

Theorem \ref{thOptiLPIntro} extends the known result \iref{eqCSX} to finite elements of arbitrary degree $m-1$. The quality of the approximation of $f$ is similarly determined by a non-linear quantity of its derivatives: the shape function $K_{m,p}(d^m f(z))$ replaces $\sqrt{|\det (d^2f(z))|}$ appearing in \iref{eqCSX}. 
In the case of isotropic triangulations, in which the measure of non degeneracy $\rho(T) := \diam(T)^2/|T|$ is uniformly bounded among all triangles $T\in \cT_N$, $N \geq N_0$, by a given constant $\rho_0$, the nonlinear quantity $K_{m,p}(\frac {d^m f(z)} {m!})$ needs to be replaced by the larger quantity $\|d^mf(z)\|$. The improvement due to anisotropy is thus expressed through the shape function $K_{m,p}$, at least for an asymptotically large number of triangles.

This remark raises the need for an in depth study of the shape function $K_{m,p}$. For $m=2$ we have established that $K_{2,p}(\pi)$ is proportional to the square root of the determinant of the quadratic polynomial $\pi = a x^2 + 2 b xy + cy^2\in \H^2$:
$$
K_{2,p}(\pi) = c_{2,p}(\det \pi) \sqrt{|\det \pi|} = c_{2,p}(ac-b^2)\sqrt {|ac-b^2|},
$$
where the constant $c_{2,p}(s)>0$ only depends on the sign of $s$. We thus recover the earlier result \iref{eqCSX}.
For $m=3$, the shape function $K_{3,p}$ is the fourth root of the discriminant of the homogenous cubic polynomial $\pi = a x^3+3bx^2y+3cxy^2+dy^3\in \H_3$:
$$
K_{3,p}(\pi) = c_{3,p}(\disc \pi) \sqrt{|\disc \pi|} = c_{3,p}(\disc \pi)\sqrt {|4(ac-b^2)(bd-c^2) - (ad-bc)^2|},
$$
where the constant $c_{3,p}(s)>0$ only depends on the sign of $s$. For larger values $m\geq 4$ we have obtained an explicit quantity uniformly equivalent to the shape function $K_{m,p}$, but not an explicit expression of $K_{m,p}$. This equivalent has the following form : there exists a polynomial $Q_m(a_0, \cdots, a_m)$ of the $m+1$ variables $a_0, \cdots, a_m$ and a constant $C_m>0$ such that for all $\pi = a_0 x^m+ a_1 x^{m-1}y+ \cdots a_m y^m\in \H_m$ one has with $r_m := \deg Q_m$,
\be
\label{equivKQ}
C_m^{-1} \sqrt[r_m]{Q_m(a_0, \cdots , a_m)} \leq K_{m,p}(\pi) \leq  C_m\sqrt[r_m]{Q_m(a_0, \cdots , a_m)}.
\ee
The polynomial $Q_m$ is obtained using the theory of invariant polynomials developed by Hilbert in \cite{Hilbert}. We also characterise %the polynomials $\pi\in \H_m$ on which the function $K_{m,p}$ vanishes, and thus 
the possible cases of ``super-convergence'' : $K_{m,p}(\pi)=0$ if and only if $\pi$ has a linear factor $ax+by$ of multiplicity $s>m/2$, in other words the homogeneous polynomial $\pi$ is sufficiently degenerated.\\

The proof of theorem \ref{thOptiLPIntro} is based on a ``local patching strategy'', a two scale mesh generation procedure which proceeds as follows: we consider a first triangulation $\cR$ of the polygonal domain $\Omega$ which is sufficiently fine in such way that the derivatives of order $m$ of $f$ vary little on each triangle $R\in \cR$ around an average value denoted by $\pi_R\in \H_m$. To each polynomial $\pi_R$, $R\in \cR$, we then associate a triangle $T_R$ which is a minimizer, or a near minimizer, of the optimization problem defining $K_{m,p}(\pi_R)$. We then on each $R\in \cR$ using the triangle $T_R$ a properly scaled and its symmetric with respect to the origin. Eventually, as illustrated on Figure \ref{figLocPatch} the triangulation $\cT_N$ is obtained by gluing together the periodic tilings on each $R\in \cR$, with a few additional triangles in order obtain a globally conforming mesh.

\begin{figure}
	\centering
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/NonConformTiling.pdf}
		\hspace{1cm}
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/ConformTiling.pdf}
		\hspace{1cm}
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/TriangleClasses.pdf}
	\caption{\label{figLocPatch} Illustration of the local patching strategy : the elements of a macro triangulation $\cR$ are covered by periodic tilings, which are then glued together.}
\end{figure}

The next theorem establishes that the asymptotic error estimate \iref{eqLPIntro} is sharp, at least if we restrict our attention to admissible sequences of triangulations, see \iref{defAdmiIntro} for the definition of this condition. Furthermore \iref{eqLPEpsIntro} shows that the admissibility condition is not too restrictive.

\begin{theoremIntro}
\label{thLowerLPIntro}
Let  $\Omega\subset \R^2$ be a bounded polygonal domain, let $f\in C^m(\overline \Omega)$, and let $1\leq p\leq \infty$.
Let $(\cT_N)_{N \geq N_0}$, $\#(\cT_N) \leq N$, be an admissible sequence of triangulations of $\Omega$. Then
\be
\label{eqLPLowerIntro}
\liminf_{N \to \infty} N^{\frac m 2} \|f-\interp_{\cT_N}^{m-1} f\|_{L^p(\Omega)} \geq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)},
\ee
where  $\frac 1 \tau := \frac m 2 + \frac 1 p$. Furthermore for any $\ve>0$ there exists an admissible sequence $(\cT_N^\ve)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N^\ve) \leq N$, and such that: 
\be
\label{eqLPEpsIntro}
\limsup_{N \to \infty} N^{\frac m 2} \|f-\interp_{\cT^\ve_N}^{m-1} f\|_{L^p(\Omega)} \geq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)}.
\ee
\end{theoremIntro}

We extend in Chapter \ref{chapW1P} Theorems \ref{thOptiLPIntro} and \ref{thLowerLPIntro} to Sobolev $W^{1,p}$ semi-norms. For that purpose the shape function $K_{m,p}$ is be replaced by the analogous quantity for $W^{1,p}$ semi-norms $L_{m,p} : \H_m \to \R_+$ which is defined as follows: for all $\pi \in \H_m$ 
$$
L_{m,p}(\pi) := \inf_{|T|=1} \|\nabla (\pi-\interp_T^{m-1} \pi)\|_{L^p(T)},
$$
and the exponent $\tau$ becomes $\frac 1 \tau := \frac {m-1} 2+ \frac 1 p$.
Similarly to \iref{equivKQ} we have also found some explicit equivalents of $L_{m,p}(\pi)$ defined by an algebraic expression in the coefficients of $\pi\in \H_m$.
Our results for the $W^{1,p}$ semi-norm are thus extremely similar to the results obtained for the $L^p$ norm.
The extension of the proofs however is not straightforward, because of the following new phenomenon: the presence of flat angles in a triangulation deteriorates the interpolation in the $W^{1,p}$ semi-norm, which is not the case in the $L^p$ norm. 

Eventually we also extend in Chapter \ref{chapBlocks} Theorems \ref{thOptiLPIntro} and \ref{thLowerLPIntro}  to partitions of a rectangular domain into anisotropic rectangles aligned with the coordinate axes, instead of triangles, with the approximation error measured in the $L^p$ norm. %, which are again potentially highly anisotropic.
 Such partitions are relevant when the coordinate axes play a privileged role, in such way that the anisotropic features of the approximated function $f$ are likely to be aligned with the coordinate axes.
The proof of the results for partitions into blocks or into triangles uses the same key ideas, but the technicalities are greatly reduced in the first case due to the presence of privileged axes.

Part \ref{partAsymptApprox} is organized as follows. We first consider in Chapter \ref{chapBlocks} partitions of a domain into rectangles or blocks aligned with the coordinate axes, with the error measured in the $L^p$ norm. 
We take advantage of this simple setting to introduce and examine in detail the shape function and the local patching strategy.
We then turn in Chapter \ref{chapOptAniso} to finite element interpolation error on anisotropic triangulations measured in the $L^p$ norm, and we eventually consider in Chapter \ref{chapW1P} the $W^{1,p}$ interpolation error.
The three chapters composing Part \ref{partAsymptApprox} are self consistent and can be read independently.

\subsection{Anisotropic smoothness classes and image models}

There exists various ways of measuring the smoothness of functions on a domain $\Omega\subset \R^2$, generally through the definition of an {\it appropriate smoothness} space and an associated norm. Classical instances are Sobolev and Besov spaces. Such spaces  are of common use when describing the regularity of solutions to partial differential equations. From a numerical perspective they are also useful in order to sharply characterize at which rate a function $f$ may be approximated by simpler functions such as Fourier series, finite elements (on isotropic triangulations), splines or wavelets.

Functions arising in concrete applications, for instance in image processing or in the solution of hyperbolic PDEs, often %may have inhomogeneous smoothness properties, in the sense that they 
exhibit areas of smoothness separated by local discontinuities.
The smoothness space that is best taylored to take these features into account is the space $BV$ of functions of bounded variation. 
This space consists of those $f\in L^1(\Omega)$ such that $\nabla f$ is a bounded measure, i.e. such that their total variation 
$$
\TV(f) = |f|_{BV} := \max\left\{\int_\Omega f \diver \vp \sep \vp\in \cD(\Omega), \|\vp\|_{L^\infty} \leq 1\right\}.
$$
is finite. Assume that $\Omega := ]0,1[^2$ is the unit square, and denote by $f_N$ the approximation of $f$ by the $N$ terms of its development on the Haar basis which correspond to the largest coefficients. It is established in \cite{CDPX, CDDD2} that 
\be
\label{eqApproxTV}
\sup_{N \geq 2} \sqrt N \|f-f_N\|_{L^2(\Omega)} \leq C \TV(f).
\ee

The result \iref{eqCSX} and its generalisation Theorem \iref{thOptiLPIntro} establish that the quality of the approximation of a function $f$ by finite elements on anisotropic triangulations is governed by some non-linear quantities of the derivatives of $f$, at least from an asymptotical point of view.
In the case of finite elements of degree $1$, and of the approximation in $L^2$ norm, the relevant quantity is the following
$$
A(f) := \left\|\sqrt {|\det(d^2f)|}\right\|_{L^{2/3}(\Omega)}.
$$
For any bounded polygonal domain $\Omega$ and any $f\in C^2(\overline \Omega)$ there exists, see \iref{eqCSX}, a sequence $\cT_N$ of triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqApproxA}
\limsup_{N \to \infty} N \|f-\interp_{\cT_N}^1 f\|_{L^2(\Omega)} \leq C A(f).
\ee

The functional $A$ strongly differs from the total variation $\TV$, and also from the Sobolev, Holder or Besov norms, because of its nonlinear behavior: $A$ does not satisfy the triangle inequality, or any quasi-triangle inequality. In other words for any constant $C$ there exists $f,g\in C^2(\overline \Omega)$ such that 
\be
\label{eqNoTri}
A(f+g) \not \leq C(A(f)+A(g)).
\ee
%Contrary to the total variation $\TV$, the functional $A$ is not a priori attached to an smoothness space. If such a space exists then the \iref{eqNoTri} 
The lack of a triangular inequality forbids to use the classical techniques of linear analysis to define a smoothness space attached to the functional $A$. Another problem comes from the limit appearing in \iref{eqApproxA}, which not present in classical approximation theory, see for instance \iref{eqApproxTV}. (A naive attempt to define an approximation space associated to the functional $A$ is nevertheless presented in Chapter \ref{chapApproxMet}.)

Concrete applications require nevertheless that results of the type of \iref{eqApproxA} be extended to non smooth functions and in particular to the class of cartoon functions.
A heuristical analysis presented in Chapter \ref{chapCartoon} suggests that for any cartoon function $f$ defined on a bounded polygonal domain $\Omega$, there exists a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N)\leq N$, and such that 
\be
\label{eqApproxCartoon}
\sup_{N\geq N_0} N \|f-\interp_{\cT_N}^1 f\|_{L^2(\Omega)} < \infty. % \text{ est borné, \quad où } r_p := \min\left\{1, \frac 2 p\right\}.
\ee
The compact form of this estimate hides the balance between to different phenomena in the approximation of $f$, each of them requiring approximately half of the cardinality of $\cT_N$. First the function $f$ is approximated by the linear interpolant $\interp_{\cT_N}^1 f$ on the regions where $f$ is smooth. Second the collection $\Gamma$ of curves along which $f$ is discontinuous is approximated by the boundaries $\partial T$, of the triangles $T\in \cT_N$. The difference $f-\interp_{\cT_N}^1 f$ does not tend to zero on the neighborhood of $\Gamma$, but the width of this neighborhood tends to $0$.

The approximation result \iref{eqApproxCartoon} raises the hope that a precise and quantitative asymptotic estimate, similar to \iref{eqApproxA}, can be obtained for cartoon functions.
So far we have only fulfilled one part of this program: the extension of the functional $A$ to cartoon functions. More precisely, consider a radial and compactly supported function $\vp\in C^\infty(\R^2)$ of unit integral. 
For any $\delta>0$ we define $\vp_\delta(z) := \frac 1 {\delta^2} \vp\left(\frac z \delta\right)$ and we denote by $f_\delta := f*\vp_\delta$ the convolution of $f$ with $\vp_\delta$. 
We establish in Chapter \ref{chapCartoon} that $A(f_\delta)$ converges as $\delta \to 0$, to an explicit expression
\begin{eqnarray*}
\lim_{\delta \to 0} A(f_\delta)^{2/3} &=& \left\|\sqrt{|\det(d^2 f)|}\right\|_{L^{2/3}(\Omega\sm\Gamma)}^{2/3} + C(\vp) \left\|\sqrt{|\kappa|} \gamma\right\|_{L^{2/3}(\Gamma)}^{2/3}\\ %\left(\|\right)
&=& \int_{\Omega\sm\Gamma} \sqrt[3]{|\det (d^2 f(z))|}dz+ C(\vp)\int_\Gamma |\kappa(s)|^{1/3} |\gamma(s)|^{2/3}ds.
\end{eqnarray*} %\frac 1 3 \frac 2 3
In the previous equation, we denote by $\Gamma$ the collection of curves where the cartoon function $f$ is discontinuous, by $\gamma(s)$ the jump of $f$ at the point $s\in \Gamma$, and by $\kappa(s)$ the curvature of $\Gamma$ at $s$. The constant $C(\vp)$ is positive and explicit in terms of $\vp$.

Part \ref{partCartoon} consists of the single chapter, Chapter \ref{chapCartoon}, containing in particular the above result. The rest of this chapter is organized as follows.
The extension of the nonlinear functional $A$ to cartoon functions puts in light a link, explored in section \S\ref{secCartoon4}, 
between anisotropic finite element approximation and several other mathematical fields. We think in particular of affine invariant image processing \cite{Ca} and of the definition in \cite{DPW} of smoothness spaces through the regularity of the level lines of a function.
The functional $A$ also can be thought of as a new quantitative image model : a monochromatic image, described by a brightness function $f: [0,1]^2 \to [0,1]$, is plausible if $A(f)$ is sufficiently small. Generalising the work \cite{LMo} we explore in section \S\ref{secCartoon5.5} an image recovery procedure using this model as a bayesian prior. 
Eventually we describe in section \S\ref{secCartoon6} the extension to cartoon functions of other non-linear quantities appearing in anisotropic finite element approximation such as the norm $\|K_{m,p}(d^m f)\|_{L^\tau}$ of the shape function for $m\geq 2$, or the counterpart of this quantitiy for functions $f$ of more than two variables.


\subsection{Mesh generation and riemannian metrics} %Génération de maillage et métriques riemanniennes} %Problèmes de génération de maillage}

Triangulations are discrete objects of combinatorial nature : they can be described by the collection of their vertices and of the edges between them. This description is fruitful for the demonstration of algebraic results such as the Euler formula, or for computer processing.

In the context of anisotropic mesh adaptation, several works \cite{Shew,Bois,A} choose in contrast to replace triangulations of a domain $\Omega$ with a continuous object during the optimisation procedure : a riemannian metric, in other words a continuous function $H$ from $\Omega$ to the set $S_2^+$ of symmetric positive definite matrices. Our purpose is to give a theoretical background to this replacement, through the formulation of precise equivalence results between some classes of triangulations and of riemannian metrics. In particular the geometrical properties of the triangulations need to be translated under the form regularity properties of the riemannian metrics.

In order to state our results we need to introduce some notations. We associate to each triangle $T$ its barycenter $z_T\in R^2$ and the symmetric positive definite matrix $\cH_T\in S_2^+$ such that the ellipse $\cE_T$ defined by 
$$
\cE_T := \{z\in \R^2 \sep (z-z_T)^\trans \cH_T (z-z_T)\},
$$
is the ellipse of minimal area containing $T$. The point $z_T$ thus encodes the position of $T$, while the matrix $\cH_T\in S_2^+$ encodes the area, the elongation and the orientation (but not the angles) of the triangle $T$ .

We denote by $\bT$ the collection of triangulations of the infinite domain $\R^2$ - the choice to consider infinite triangulations is guided by simplicity, and further work will be devoted to triangulations of bounded domains.
We denote by $\bH := C^0(\R^2, S_2^+)$ the collection of riemannian metrics on $\R^2$. A metric $H\in \bH$ continuously associates to each point $z\in \R^2$ a symmetric positive matrix $H(z)\in S_2^+$.
We say that a triangulation $\cT\in \bT$ is $C$-equivalent to a metric $H \in \bH$ if for all $T\in \cT$ and for all $z\in T$ we have 
$$
C^{-2} H(z) \leq \cH_T \leq C^2 H(z). 
$$
We say that a class of triangulations $\bT_*\subset \bT$ is equivalent to a class of metrics $\bH_*\subset \bH$ if there exists a uniform constant $C>0$ such that 
\begin{itemize}
\item For any triangulation $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C$-équivalent.
\item For any metric $H\in \bH_*$ there exists a triangulation $\cT\in \bT_*$ such that $\cT$ and $H$ are $C$-équivalent.
\end{itemize}

%The full class $\bT$ of all triangulations is not equivalent to the full class $\bH$ of all metrics. 
We define below three particularly relevant classes of triangulation
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}
$$
which have a minor dependency on a parameter $C\geq 1$.
When $C$ is sufficiently large, these classes of triangulations are equivalent to three classes of metrics respectively 
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
We now turn to the description of these classes of triangulations and of metrics.
The class $\bT_{g,C}$ of \emph{graded} triangulations, is defined by the following condition which imposes a minimum of consistency among the shapes of neighbouring triangles. A triangulation $\cT$ belongs to $\bT_{g,C}$ if for all $T, T'\in \cT$ one has
$$
T \cap T' \neq \emptyset \quad \Ra \quad C^{-2} \cH_T \leq \cH_{T'} \leq C \cH_T.
$$
A triangulation $\cT$ belongs to the class $\bT_{i,C}$ of \emph{isotropic} triangulations if $\cT$ is graded : $\cT\in \bT_{g,C}$,
%(cette condition peut être supprimée, voir ??) 
and if the elements of $\cT$ are sufficiently close to the equilateral triangle, as expressed by the following condition: for all $T\in \cT$
$$
\|\cH_T\| \|\cH_T^{-1}\|\leq C^2.
$$
Eventually the class $\bT_{a,C}$ of \emph{quasi-acute} triangulations is defined by a slightly more technical condition on the maximal angles of the triangles, see Chapter \ref{chapMeshMet}. This condition guarantees the stability of the gradient of the interpolation of a function, but raises difficulties in terms of mesh generation which diminish the flexibility of use of quasi-acute triangulations in practical applications. One of our key results is the reformulation of this diminished flexibility under the form of a regularity assumption on an equivalent riemannian metric.

When the constant $C$ is sufficiently large, the class $\bT_{i,C}$ of isotropic triangulations is equivalent to the class $\bH_i$ of metrics $H$ which are proportional to the identity
$
H(z) = \Id /s(z)^2 ,
$
and such that the proportionality factor $s$ satisfies one of the following \emph{equivalent} properties
\begin{itemize}
\item Euclidean Lipschitz Property: $|s(z) - s(z')| \leq |z-z'|$ for all $z,z'\in \R^2.$
\item Riemannian Lipschitz Property: $|\ln s(z) - \ln s(z')| \leq d_H(z,z')$ for all $z,z'\in \R^2.$
\end{itemize}
We recall that the riemannian distance $d_H(z,z')$ measures the length, distorted by the metric $H$, of the smallest path joining $z$ and $z'$, see Chapter \label{chapMeshMet}.

The two lipschitz properties presented above have (non equivalent) natural extensions to general anisotropic riemannian metrics. They involve two distances $d_+$ and $d_\times$ on the collection $S_2^+$ of symmetric positive definite  riemannian metrics %, see ??
\begin{eqnarray}
\label{eqDPlusIntro}
d_+(H(z), H(z') ) & \leq & |z-z'| \stext{ for all } z,z'\in \R^2,\\
\label{eqDTimesIntro}
d_\times(H(z), H(z') ) & \leq &d_H(z,z') \stext{ for all } z,z'\in \R^2.
\end{eqnarray}

Our main result reformulates under the form of the above Lipschitz properties the flexibility offered by the class of graded triangulations $\bT_{g,C}$ and of quasi-acute triangulations $\bT_{a,C}$ - note that the latter is more rigid due to the angle constraint.
\begin{theoremIntro}
\label{thMeshMetIntro}
If the constant $C$ is sufficiently large, then the class $\bT_{g,C}$ of graded triangulations is equivalent to the class $\bH_g$ of metrics satisfying \iref{eqDTimesIntro}. The class $\bT_{a,C}$ of quasi-acute triangulations is equivalent to the class $\bH_a$ of metrics satisfying simultaneously \iref{eqDTimesIntro} and \iref{eqDPlusIntro}.
\end{theoremIntro}

%(*Séparation de deux ensembles, un mot sur l'approx Theory*)

\subsection{Hierarchical refinement of triangulations}

In classical approximation theory, one often defines an increasing sequence $(V_N)_{N \geq 0}$ of vector spaces of finite dimension which are included and of dense union $\cup_{N \geq 0} V_N$ in some Hilbert space $V$
\be
\label{eqInclusionVN}
V_0 \subset \cdots \subset V_N \subset V_{N+1} \cdots 
\ee
For instance $V_N$ can be formed of all polynomials of degree $\leq N$, or of the Fourier modes $e^{ikx}$ where $|k| \leq N$, or of wavelets of generation smaller than $N$ on the unit square. In the case of interest to us $V_N = V_{m-1}(\cT_N)$ is the space of finite elements of degree $m-1$ on a triangulation $\cT_N$. In that context the inclusion \iref{eqInclusionVN} of the vector spaces $(V_N)_{N \geq 0}$ is equivalent to the hierarchy of the triangulations $(\cT_N)_{N\geq 0}$, indeed %for any two triangulations $\cT, \cT'$
$$
V_N \subset V_{N+1} \ \Longleftrightarrow \ \cT_{N+1} \text{ is a refinement of } \cT_N.
$$

The inclusion property \iref{eqInclusionVN} is particularly handful from a theoretical point of view, as illustrated by the two following examples. Consider the case of the minimization of a functional $J$ continuous on $V$, for instance $J$ can be the energy functional attached to the heat equation \iref{eqMinCvx}, or simply the approximation error with respect to a given function $f\in V$. The inclusions \iref{eqInclusionVN}, combined with the density of $\cup_{N \geq 0} V_N$ imply that 
\be
\label{eqJVN}
\min_{v\in V_N} J(v) \stext{ tends decreasingly to } \min_{v\in V} J(v).
\ee
We now turn to a second example. Denote by $W_N$ the orthogonal complement of $V_N$ in $V_{N+1}$. Consider $v\in V$, denote by $\underline v$ the orthogonal projection of $v$ onto $V_0$, and by $v_N$ the orthogonal projection of $v$ onto $W_N$. We thus have
$$
v=\underline v + \sum_{N \geq 0} v_N.
$$
This decomposition is at the heart of multiresolution analyses, based on wavelets or finite elements. The component $v_N$ is regarded as the collection of details of $v$ at the scale $N$.
The combination of these two examples is heuristically the key to obtain a precise estimate the minimum of a functional $J$ on $V_N$ for each $N$, in terms of the regularity of the exact minimizer $f$ of $J$ on $V$. See for instance \cite{Nochetto} for the heat equation using finite elements on isotropic triangulations. The paper \cite{St2} achieves the same result for elliptic and parabolic PDEs using anisotropic tensor product wavelet spaces. 
%Note that these wavelet spaces combine hierarchy with anisotropy, but only aligned with the directions of the coordinate axes.

A natural objective is to extend these methods to anisotropic finite element approximation.
The first step of this approach is the production of anisotropic triangulations adapted to given function $f$, which satisfy a property of hierarchy.
For that purpose Cohen, Dyn and Hecht have proposed an algorithm which is studied in the last part of this thesis.
%The last part \ref{partGreedy} of this thesis is devoted to the study an algorithm proposed by Cohen, Dyn and Hecht which produces hierarchical sequences $(\cT_N)_{N\geq N_0}$ of (non-conforming) anisotropic triangulations adapted to a given function $f$.
Given a triangulation $\cT$ of a domain $\Omega$ and a function $f\in L^p(\Omega)$, this algorithm creates in one step a triangulation $\cT'$ of $\Omega$, of cardinality $\#(\cT') = \#(\cT)+1$, proceeding as follows:
\begin{enumerate}
\item (Greedy triangle selection) A triangle $T\in \cT$ which has a maximal contribution to the error is selected 
$$
T := \argmax_{T'\in \cT} \|f-\cA_{T'} f\|_{L^p(T')},
$$
where $\cA_T : L^p(T) \to \P_1$ a projection operator, for instance the $L^2(T)$ orthogonal projection onto $\P_1$.
\item (Decision of a bisection)
The refinement procedure considers the three following bisection choices for the triangle $T$ : from the midpoint of an edge $e\in \{a,b,c\}$ of $T$ to the opposite vertex, creating the sub-triangles $T_e^1$ and $T_e^2$. The edge which minimizes a given decision function $d_T(e,f)$ is selected,  and we define 
$$
\cT' := \cT-\{T\} + \{T_e^1, T_e^2\}.
$$
\end{enumerate}
Starting from a triangulation $\cT_0$ of cardinality $N_0$ of the domain $\Omega$, the algorithm produces step after step a sequence $(\cT_N)_{N\geq N_0}$ of triangulations ``adapted'' to a given function $f\in L^p(\Omega)$. The properties of these triangulations strongly depend on the approximated function $f$ and on the choice of the decision function $d_T(e,f)$, which guides the creation of anisotropy - in contrast the projection operator $\cA_T$ plays a rather minor role.

We present this algorithm in more detail in Chapter \ref{chapCDHM}, and we prove the convergence of this algorithm
%a general convergence result for any bounded polygonal domain $\Omega$ and any $f\in L^p(\Omega)$, 
under some assumptions on the projection operator $\cA_T$ and the decision function $d_T(e,f)$.
Our main result, presented in Chapter \ref{chapBisecOpt}, states that when $f$ is a strictly convex $C^2$ function, for a particular choice \iref{eqDecisionL1} of the decision function, the sequence $(\cT_N)_{N\geq N_0}$ of triangulations generated by this algorithm satisfies the best possible asymptotic convergence estimate
$$
\limsup_{N \to \infty} N \| f-\cA_{\cT_N} f\|_{L^p(\Omega)} \leq C \|\sqrt{|\det (d^2f)|}\|_{L^\tau(\Omega)},
$$
where $\frac 1 \tau := 1+ \frac 1 p$ and where $\cA_\cT f$ denotes the piecewise linear function on $\Omega$ which coincides with $\cA_T f$ on each $T\in \cT$.

Eventually we study in Chapter \ref{chapVariations} some variants of the hierarchical refinement algorithm presented above. %, which is also referred to as the ``greedy algorithm''. 
More precisely we consider in section \S\ref{secAltDec} a decision function based on the $L^2$ approximation error, which is particularly well suited to the numerical implementation since an trick allows to evaluate it in a comparatively small computer time.

We then focus in section \S\ref{secAltBi} on the approximation of cartoon functions. The original algorithm is not well suited to this context, and we therefore introduce and study some modifications of the bisection choices offered to the decision function.

Eventually we consider in section \S\ref{secGreedyRect} another variant of the algorithm, which is based on rectangles aligned with with the coordinate axes instead of triangles of arbitrary direction. This simplification leads to Theorem \ref{thRect} which guarantees the best possible convergence estimate for all $C^1$ functions, in the case of piecewise constant approximations on rectangles aligned with the coordinate axes.


==> Introduction/IntroEngTheseOld2.tex <==
%\title{Adaptive and anisotropic finite element approximation:\\Theory and Algorithms}
%%Approximation adaptative et anisotrope par éléments finis\\Théorie et Algorithmes}
%\maketitle
%\tableofcontents

%Important : this introduction is only draft, and is not ready to be reviewed.

\section{Anisotropic finite element approximation : why and how?} %Finite element approximation : Motivations, State of the art and Open questions}

The thesis is devoted to the problem of approximating a function by piecewise polynomial ones on a triangulation. The triangulation is adaptively chosen depending on the approximated function, and may include triangles of arbitrary size, aspect ratio and orientation.\\

Approximation by piecewise polynomial functions
is a procedure that occurs in numerous applications. 
In some of them such as 
terrain data simplification or image compression,
the function $f$ to be approximated might be fully known,
while it might be only partially known or fully
unknown in other applications such as denoising, statistical learning or 
in the finite element discretization of PDE's.
In all these applications, one usually makes the 
distinction between {\it uniform} and {\it adaptive} approximation.
In the uniform case, the domain of interest is decomposed into
a partition where all elements have comparable shape and size,
while these attributes are allowed to vary strongly in the adaptive case.
The partition may therefore be adapted to the local properties
of $f$, with the objective of 
optimizing the trade-off between accuracy and complexity of
the approximation.\\

In approximation theory, the accuracy of the approximation of a function is tied to two parameters: the smoothness of the function, and resolution of the approximation procedure.
Functions arising in concrete applications may have in homogeneous smoothness properties, in the sense that they exhibit areas of smoothness separated by localized discontinuities, see Figure \ref{figEllTri}. Two typical instances are (i) edges in functions representing real images, and (ii) shock profiles in the solutions to non-linear hyperbolic PDE's. 
%These functions often need to be processed numerically, for instance for image denoising or compression, or for the simulation of the evolution of a PDE. 
Numerical procedures for image processing, such as image denoising or compression, or for the simulation of PDE's  greatly benefit from economical and faithful approximations of these functions.
A piecewise polynomial approximation on a uniform partition of the domain, see Figure \ref{figEllTri}, is generally not sufficient for these purposes which raises the need for raises the need for adaptive approximation procedures, in which the resolution of the decomposition of the domain is not uniform, but depends on the local smoothness properties of the approximated function. A first step is to adapt the size of cells forming the partition, see Figure \ref{figEllTri} (iii). A second step is to observe that a higher resolution is needed in the direction orthogonal to the curve of discontinuity than in the tangential direction, and to take advantage of this property by using an anisotropic partition of the domain, built of triangles of high aspect ratio aligned with the discontinuities, see Figure \ref{figEllTri} (iv).\\

\begin{figure}
\centering
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/Triangle.pdf}
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/TriangleUnif.pdf}\\
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/Haar.pdf}
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/TriangleMeshed.pdf}
\caption{A piecewise smooth function (i), Uniform partition of the domain (ii), Partition associated to the adaptive approximation using the Haar basis (iii), Partition associated to the adaptive anisotropic finite element approximation (iv). (credit : G. Peyr\'e)\label{figEllTri}}
\end{figure}

The use of adaptive approximation in numerical algorithms raises a number of difficulties. 
From a numerical point of view, adaptive methods requires more complex algorithms and more intricate data structures than their non-adaptive counterparts. From a theoretical point of view the analysis of these algorithms, when it is possible, is generally involved. As a matter, on fact the improvement brought by the adaptive procedure compared to a non-adaptive one is rigorously established only for few systems in the case of the numerical simulation of PDE's. 
We need to mention that these difficulties are exacerbated when anisotropic adaptivity is used, which means that the cells forming the partition of the domain may have large aspect ratios and arbitrary orientations taylored to the approximated function.
We refer to the paper \cite{Nochetto} for a theoretical analysis of the improvement brought by adaptive isotropic finite elements in the case of the heat equation. Several numerical software, such as \cite{FreeFem, Inria, A}, see also Figure \ref{figInria}, successfully use anisotropic adaptativity for the numerical simulation of PDE's. From a numerical point of view, the improvement brought by these methods seems obvious compared to non-adaptive or adaptive isotropic methods. However, many aspects of the theoretical analysis of these methods remain open question.\\

\begin{figure}
	\centering		
	\includegraphics[width=4.5cm,height=3cm]{\pathPic/SimuExt/AlauzetPlane.pdf}
	\hspace{1cm}
	\includegraphics[width=3.5cm,height=3cm]{\pathPic/SimuExt/AlauzetShock.pdf}
	\caption{Airflow around a supersonic plane, computed using a three dimensional highly anisotropic mesh. (credit : F. Alauzet \cite{A}.\label{figInria})}
\end{figure}

This thesis studies the problem of anisotropic mesh adaptation for the approximation of a function, which can be regarded as a preliminary question for the analysis of anisotropic mesh adaptation for the numerical simulation of PDE's.
Given a triangulation $\cT$ of a bounded polygonal domain $\Omega\subset\R^2$, and a fixed integer $k\geq 1$, we denote by $V_k(\cT)$ the space of finite elements of degree $k$ on $\cT$. The space $V_k(\cT)$ consists of all
%, potentially discontinuous, %continuous % almost everywhere bounded 
functions which coincide on the interior of each triangle $T\in \cT$ with a polynomial of degree $k$
$$
V_k( \cT) := \{g\in C^0(\Omega) \sep g_{|T}  \text{ is a polynomial of degree $k$ for each } T \in \cT\}.
$$
The dimension of $V_k(\cT)$ is approximately $k^2 \#(\cT)$. %, and the elements of $V_k(\cT)$ can be efficiently manipulated numerically.
Given a function $f : \Omega \to \R$ and a triangulation $\cT$ of $\Omega$, a natural objective is to approximate $f$ using a function $g$ in the space $V_k(\cT)$ of finite elements of degree $k$ on $\cT$, for instance for the purpose of manipulating $f$ numerically. 
This problem, finite element approximation on a given triangulation, is formulated as follows:
\be
\label{eqApproxG}
e_\cT(f)_X := \inf_{g\in V_k(\cT)} \|f-g\|_X.
\ee
The letter $X$ indicates the norm or semi-norm in which the approximation error $\|f-g\|_X$ is measured. In this thesis we restrict our attention to the $L^p$ norm and the $W^{1,p}$ semi-norm, where $1\leq p \leq \infty$. They are defined as follows: 
$$
\|h\|_{L^p(\Omega)} := \left(\int_\Omega |h|^p\right)^{\frac 1 p} \stext{ and } |h|_{W^{1,p}(\Omega)} := \left(\int_\Omega |\nabla h|^p\right)^{\frac 1 p}
$$
The best approximation $g\in V_k(\cT)$ of $f$ can be exactly computed in the case of the $L^2$ norm or the $W^{1,2}$ semi norm: $g$ is the orthogonal projection of $f$ onto $V_k(\cT)$ with respect to the scalar product associated to the norm of interest. In the case $p\neq 2$ of non hilbertian norms the best approximation of $f$ is generally hard to compute, but ``satisfactory'' approximations can be obtained by different methods. If the function is sufficiently smooth and the triangulation is sufficiently fine, then the standard Lagrange interpolation is sufficient. In other case a quasi interpolant of $f$ is preferred, see Chapter \ref{chapApproxMet}.
The problem of approximating a given function $f$ on a given triangulation $\cT$, using finite elements of a given degree $k$, is thus solved in good part.\\

In the context of adaptive approximation, the triangulation $\cT$ of the domain $\Omega$ is not given, but can be freely chosen - in contrast we assume in this thesis that the integer $k$ is fixed although arbitrary. 
The areas of the triangles constituting the mesh $\cT$ may vary strongly for a better adaptation to the local features of the approximated function $f$. In the case of anisotropic mesh adaptation the aspect ratio and the orientation of these triangles may also vary strongly. This naturally raises the objective of characterizing and constructing an optimal mesh for a given function $f$. Given a norm $X$ of interest, an integer $N>0$ and a function $f$ to be approximated, we formulate this optimization problem, optimal mesh adaptation, as follows:
\be
\label{eqApproxT}
e_N(f)_X := \inf_{\#(\cT) \leq N} e_\cT(f)_X.
\ee
In contrast to the problem \iref{eqApproxG} of finite element approximation on a fixed mesh, the problem of adaptive and anisotropic approximation \iref{eqApproxT} is not yet well understood.
Heuristically, the simplicity of \iref{eqApproxG} comparatively to \iref{eqApproxT} is due to the fact that the optimization is posed on the linear space $V_k(\cT)$. %: for any $g,g'\in V_k(\cT)$ we have $g+g'\in V_m(\cT)$. 
The methods mentioned for solving \iref{eqApproxG}, such as the orthogonal projection or the interpolation, make indeed a key use of this property.
In contrast the optimization problem \iref{eqApproxT} is posed on the collection of triangulations $\cT$ satisfying $\#(\cT)\leq N$, which is certainly not a vector space. This problem is nevertheless well understood is the isotropic setting where the optimization is restricted to triangulations in which the triangles satisfy a uniform shape constraint. In contrast it is an open research subject in the general setting of potentially anisotropic triangulations.\\


%and the sum $\cT+\cT'$ of two triangulations has no meaning in general.

%%In order to compensate for this problem one o
%The optimization \iref{eqApproxT} is restricted in a number of applications to a family $\bT_*$ of triangulations possessing a property of hierarchy, see for instance \cite{Nochetto}. For each pair of triangulations $\cT, \cT'\in \bT_*$, the hierarchy property guarantees that there exists a common refinement $\wti \cT\in \bT_*$ of $\cT$ and $\cT'$ satisfying $\#(\wti \cT) \leq C (\#(\cT)+ \#(\cT'))$. The common refinement $\wti \cT$ plays in a certain sense the role of the sum $\cT+ \cT'$, and the techniques of linear analysis can be used to understand most aspects of the optimization problem \iref{eqApproxT} restricted to triangulations in $\bT_*$:
%\be
%\label{eqApproxIso}
%\inf \{ e_\cT(f)_X \sep \#(\cT) \leq N \text{ and } \cT \in \bT_* \}.
%\ee
%This approach has led to successful developments which are out of the scope of this thesis, we refer the interested reader to \cite{Nochetto} for an application of this method to numerical solutions of partial differential equations.
%
%%The problem \iref{eqApproxIso} imposes a strong restriction on the triangulations. Indeed T
%The families $\bT_*$ of triangulations satisfying a property of hierarchy usually consist of uniformly isotropic triangulations. In other words the approximation problem \iref{eqApproxIso} allows to finely tune the areas of the triangles $T\in \cT$ with respect to the approximated function $f$, but not their aspect ratio and orientation.
%%In other words a triangulation $\cT\in \bT_*$ consists of elements $T\in \cT$ which may have areas of distinct orders of magnitude, but which shapes vary little and remain close to the equilateral triangle.
%This restriction strongly penalizes the approximation of certain classes of function $f$, in particular  the class of cartoon functions which involve discontinuities along some smooth curves. As illustrated on Figure \ref{figPeyre} the use of anisotropic triangulations, which involve thin and long triangles aligned with the discontinuities of $f$, is particularly appropriate in that context and significantly reduces the approximation error $e_\cT(f)_X$ for a given cardinality $\#(\cT)=N$. 
%The minimum \iref{eqApproxT} is therefore significantly smaller than the minimum \iref{eqApproxIso} which is restricted to the family $\bT_*$ of triangulations, which are generally isotropic. %of, usually isotropic, triangulations.

The purpose of this thesis is to better understand the approximation problem \iref{eqApproxT} posed on the full class of potentially anisotropic triangulations. 
We study this problem from four different points of view which are summarized by the questions I to IV below, to which the four parts of this thesis are devoted. 
%Each part 
%We discuss this problem through four different questions, which reflect four different point of views, a
%The four parts of this thesis are devoted the following questions, which are also discussed in more detail in the second half of this introduction. 
%We have addressed in particular the following questions:
%\begin{enumerate}[$\bullet$]
\begin{enumerate}[I]
\item 
What is the behavior of the approximation error $e_N(f)_X$ in the asymptotic setting where the number $N$ of triangles is sufficiently large and the approximated function $f$ is sufficiently smooth? In that context the resolution is sufficient to produce a triangulation $\cT$ well adapted to the local features of $f$, and to obtain an explicit equivalent of (a slightly modified version of) $e_N(f)_X$. 
\item 
Which classes of functions are naturally tied to the approximation problem \iref{eqApproxT}? In particular what can be said of the model of cartoon functions? These functions are smooth except along a collection of smooth curves, where they exhibit discontinuities, and anisotropic methods are particularly appropriate for their approximation, see Figure \ref{figEllTri}. Cartoon functions are a popular image model in the image processing community.
\item 
%Is there a mathematical object which is rigorously equivalent to triangulations
%Could the optimization problem \iref{eqApproxT} posed on triangulations $\cT$ of a given cardinality $N$, be replaced with a more well posed mathematical object?
Triangulations are combinatorial objects, described in terms of points and edges, 
which is not handy when solving optimization problems of the form \iref{eqApproxT}. 
We study the correspondence between certain classes of triangulations and of riemanninan metrics. The latter are continuous objects governed by simple equations, which allows reformulate and to solve some optimization problems posed on triangulations. %of the family of \iref{eqApproxT}.
\item 
Is it possible to produce a near-optimal sequence of triangulations $(\cT_N)_{N \geq _0}$, using a hierarchical refinement procedure? A number of algorithms indeed require this property, which guarantees the inclusion of the associated finite element spaces $V_k(\cT_N) \subset V_k(\cT_{N+1})$. We provide a simple and explicit algorithm which gives a positive answer to this question under some conditions. %in some circumstances.
%How to combine adaptive anisotropy with hierarchy?
%%Is it possible to combine hierarchy with adaptive anisotropic triangulations?
%This is indeed possible, but at the following price: the hierarchical family needs to be adapted to the approximated function $f$. This must be contrasted with the hierarchical family  $\bT_*$ of triangulations, involved in \iref{eqApproxIso}, which is defined independently $f$.
\end{enumerate}
%\end{itemize}
%We now give some motivations to the subject of this thesis, the in depth study of the approximation error $e_N(f)_X$. %, we give some motivations to the study of the problem \iref{eqApproxT}.
%Note that, depending on the context, the approximated function $f$ may be fully known to us: through an explicit formula or a discrete sampling; or observed through noisy measurements; or implicitly defined as the solution to a partial differential equation.

%\subsection{Motivations}
%\paragraph{Partial differential equations.\\} %Equations aux dérivées partielles.\\} %La méthode des éléments finis}
%
%Numerical methods for partial differential equations, PDEs, attempt, for a given cost in terms of computer time, to obtain the best possible approximation of a function $f$ implicitly  defined as the solution to a partial differential equation.
%Some of these methods take as input a mesh $\cT$ of the computational domain $\Omega$, and return an approximate solution under the form of a finite element approximation $f_\cT\in V_k(\cT)$ of the exact solution $f$. 
%As observed below for the heat equation \iref{eqOptiHeat}, if the norm $X$ is well chosen and the problem is well posed, then the approximate solution $f_\cT\in V_k(\cT)$ may not be far from the being the best approximation of $f$ on $\cT$. Furthermore the cost of the computation of the approximate solution $f_\cT\in V_k(\cT)$ is heavily tied to the cardinality $\#(\cT)=N$.
%
%The solutions of partial differential equations often exhibit some strongly anisotropic features. We think in particular of boundary layers in fluid simulation,
%metallic spikes and edges in electromagnetism,
%or shock waves in transport equations.
%This observation raises the need for adapting the mesh $\cT$ to the exact solution $f$ of the PDE. Ideally for a given budget of computer time, which corresponds to a simulation on an arbitrary triangulation of cardinality $N>0$, one should run the simulation on the triangulation $\cT$ which minimizes $e_\cT(f)_X$.
%This optimal triangulation can  generally not be obtained because the exact solution $f$ to the PDE is not known, and because the optimization among triangulations of a given cardinality of the approximation error $e_\cT(f)_X$ is a difficult problem, even in the case where the approximated function is explicitly known. Before considering the difficulties of adaptive mesh generation, let us nevertheless contemplate its possible advantages.
%
%%In order to illustrate this point w
%We consider the simplest class of PDEs : elliptic equations. Let $\Omega$ be a bounded polygonal domain, let $a\in L^\infty(\Omega)$ and let $b\in L^2(\Omega)$. We assume that there exists two positive constants $\lambda, \Lambda$ such that $0 < \lambda \leq a \leq \Lambda$ on $\Omega$ and we look for the solution of the classical Poisson problem
%\be
%\label{eqEllSystem}
%\left\{\begin{array}{rcl}
%-\diver(a \nabla f) &= b & \text{ on } \Omega \\
%f  &=  0 & \text{ on } \partial \Omega.
%\end{array}
%\right.
%\ee
%This system of equations can be reformulated as a convex minimization problem: find $f\in H^1_0(\Omega)$ which minimizes the following ``energy''
%\be
%\label{eqMinCvx}
%\frac 1 2\int_\Omega a |\nabla f|^2 - \int_\Omega f b.
%\ee
%Given a mesh $\cT$ of $\Omega$, denote by $f_\cT$ the element of $V_k(\cT)$ which vanishes on $\Omega$ and minimizes \iref{eqMinCvx}. Cea's lemma guarantees an error estimate in the $H^1_0$ norm, which is also the  $X=W^{1,2}$ semi-norm:
%\be
%\label{eqOptiHeat}
%|f-f_\cT|_X %{H^1_0(\Omega)} 
%:= \|\nabla f-\nabla f_\cT\|_{L^2(\Omega)} \leq \sqrt{\Lambda/ \lambda} \ e_\cT(f)_X. %\frac {\Lambda}{\lambda}
%\ee
%As announced, the approximation $f_\cT$ is not far from being the best possible approximation of $f$ in $V_k(\cT)$. From a numerical point of view, the cost of computing $f_\cT$ mostly depends on $\#(\cT)$, at least for isotropic triangulations (In the case of anisotropic triangulations this cost may increase because of the deterioration of the conditioning of the linear system). 
%%Furthermore the solution $f$ of the elliptic system \iref{eqEllSystem} does exhibit varying degrees of regularity, depending on the position in $\Omega$ and on the direction. 
%The exact function $f$ has relatively low regularity at the corners of $\Omega$ and at the places where the diffusivity coefficient $a$ is discontinuous, which raises the need for adaptive triangulations. We are thus naturally led to the problem \iref{eqApproxT}. 
%
%One of the difficulties of mesh adaptation for PDEs is that the approximated function $f$, which is by nature unknown, cannot be directly exploited to build the triangulation $\cT$. One therefore uses an iterative approach: starting from a coarse triangulation $\cT_0$ of $\Omega$ the following loop is executed for $n \geq 0$:
%\begin{enumerate}
%\item (Solve) The approximate solution $f_{\cT_n}$ of $f$ on the mesh $\cT_n$ is computed. 
%\item (Estimate) Some properties of the exact solution $f$ are estimated from its approximation $f_{\cT_n}$. In particular some error indicators.
%\item (Mark) The positions in the domain $\Omega$ where the triangulation should be refined, potentially anisotropically, are marked.
%\item (Refine) A mesh generator produces the triangulation $\cT_{n+1}$, and the algorithm goes back to step 1. 
%\end{enumerate}
%The loop is interrupted when $\#(\cT_n)$ exceeds some value $N$ fixed in advance, or when $|f-f_{\cT_n}|_X$ passes beyond a threshold value $\ve$.
%
%This procedure is analysed in depth in \cite{Nochetto} in the case of hierarchical isotropic mesh adaptation  mentioned in \iref{eqApproxIso}.  Some optimality results are established and the improvement due to mesh adaptation is illustrated by numerical examples. Unfortunately this approach seems difficult to extend to anisotropic triangulations, because it heavily relies on the hierarchy of a family of isotropic triangulations, defined independently of $f$. 
%The paper \cite{St2} considers tensor product anisotropic wavelet spaces, instead of triangulations, and establishes that adaptive and anisotropic methods can be successfully used to solve elliptic PDEs, when they are posed on the domain $\Omega = [0,1]^2$ or $[0,1]^d$ in $d$-dimensions. The drawback of anisotropic tensor product wavelets, compared to anisotropic triangulations, is their strong coordinate bias: they are only useful for anisotropic features of the approximated function $f$ aligned with the coordinate axes - such features appear on the boundary of $[0,1]^d$ for the solutions of elliptic equations posed on this domain.
%
%Various numerical methods for PDEs take advantage of anisotropic triangulations using similar ideas, in particular the algorithmic loop mentioned above, see for instance the software \cite{FreeFem, Inria}. However these methods are not yet well understood theoretically, and they only apply to linear finite elements.
%One of the purposes of this thesis obtain a better understanding of the steps Mark and Refine of the mesh adaptation loop, and to extend them at least to quadratic finite elements.
%
%\begin{figure}
%	\centering		
%	\includegraphics[width=4.5cm,height=3cm]{\pathPic/SimuExt/AlauzetPlane.pdf}
%	\hspace{1cm}
%	\includegraphics[width=3.5cm,height=3cm]{\pathPic/SimuExt/AlauzetShock.pdf}
%	\caption{Airflow around a supersonic plane. (credit : Fr\'ed\'eric Alauzet \cite{A}.\label{figInria}})
%\end{figure}
%
%\paragraph{Image compression.\\}
%
%In the context of image compression the domain $\Omega$ is generally the unit square $\Omega = [0,1]^2$. For simplicity we restrict our attention to monochromatic images, which are defined by the value at each point $x\in \Omega$ of a brightness $f(x) \in [0,1]$. Given a triangulation $\cT$ of $\Omega$, an approximation of the image can be stored under the form of an approximation $g\in V_k(\cT)$ of the brightness $f$.
%
%The quality of the approximation $g$ of a monochromatic image of defined by a brightness $f$ is usually measured using the $\PSNR_f$ (Peak Signal Noise Ratio with respect to $f$)
%$$
%\PSNR_f (g) := - 10 \frac {\ln \|f-g\|_{L^2}}{\ln 10}. %r \ln \|f-g\|_{L^2(\Omega)} \text{ %10 \frac {\ln \|f-g\|_{L^2}}{\ln 10}.
%$$
%A natural objective is store an approximation $g$ of an image defined by the brightness $f$, for a given cost in terms of computer memory, with the smallest possible distortion $\PSNR_f(g)$.
%Given a triangulation $\cT$ of $\Omega$, the minimal value of $\PSNR_f(g)$, or equivalently $\|f-g\|_{L^2}$, is attained by the orthogonal projection of $f$ on $\cT$ which is easy to compute numerically.
%The cost in terms of computer memory of storing the orthogonal projection of $f$ on $V_k(\cT)$, or any other element of $V_k(\cT)$, is approximately equal to $\dim(V_k(\cT)) \simeq k^2\#(\cT)$. We are thus again led to the mesh optimization problem \iref{eqApproxT}, with the norm $X=L^2$.
%Obtaining the optimal mesh is known to be a NP hard problem, and is therefore not a realistic objective. Nevertheless the method proposed for instance in \cite{DDI} provides good candidates which leads to a competitive approximation method.
%
%Methods based on (potentially) anisotropic triangulations are particularly well adapted to images of geometrical nature, such as ``cartoon'' images, which are smooth except along some discontinuities, themselves occuring along smooth curves.
%As illustrated on Figure \ref{figPeyre}, anisotropic triangulations featuring thin and long triangles aligned with these discontinuities allow to produce faithful approximations of cartoon functions with only few degrees of freedom.
%In contrast, methods based on (anisotropic) triangulations generally do not show any gain compared for instance to wavelet based methods for images containing a lot of texture. Chapter \ref{chapCartoon} examines in detail the link between image models and adaptive anisotropic approximation.
%
%The production of a good triangulation $\cT$ for the approximation of a function $f$ is a difficult problem for which several algorithms have been proposed. The iterative thinning algorithm presented in \cite{DDI} is particularly competitive in practice, but is not guaranteed from a theoretical point of view.
%The algorithm presented in \cite{Peyre} first produces continuous object, a riemannian metric from the image, and then generates a mesh based from this metric. This type of mesh generation is analysed in Chapter \ref{chapMeshMet}. Last we study in Chapter \ref{chapCDHM} and algorithm producing anisotropic and hierarchical triangulations, which can be used in the context in image approximation.
%
%\begin{figure}
%\centering
%\includegraphics[width=3.5cm,height=3.4cm]{\pathPic/Cartoon/Triangle.pdf}
%\hspace{0.0cm}
%{\raise -0.07cm \hbox{\includegraphics[width=3.7cm,height=3.55cm]{\pathPic/Cartoon/Haar.pdf}}}
%\includegraphics[width=3.5cm,height=3.4cm]{\pathPic/Cartoon/TriangleMeshed.pdf}
%\caption{A Cartoon function, isotropic refinement associated to the Haar wavelet, an adapted anisotropic triangulation. (credit : Gabriel Peyr\'e\label{figPeyre}\label{figPeyre}})
%\end{figure}



\subsection{State of the art}

We give in this section a short overview of the state of the art in the following problem of anisotropic finite element approximation : the evaluation of the minimal approximation error $e_N(f)_X$ and the construction of a close to optimal triangulation. For that purpose we need to introduce some notations.
We assume in the following that $f\in C^0(\overline \Omega)$, where $\Omega \subset \R^2$ is a bounded polygonal domain and $\overline \Omega$ denotes the closure of $\Omega$. For each triangulation $\cT$ of $\Omega$ we denote by $\interp^k_\cT$ the standard interpolation operator on Lagrange finite elements of degree $k$ on $\cT$. If the triangulation $\cT$ is conforming, then $\interp_\cT^k f$ is continuous and therefore $\interp_\cT^k f\in V_k(\cT)$. In order to be consistent with the rest of this thesis we define $m := k+1\geq 2$, and we thus have 
$$
e_\cT(f)_{L^p} \leq \|f-\interp_\cT^{m-1} f\|_{L^p(\Omega)} \stext{ and } e_\cT(f)_{W^{1,p}} \leq  \|\nabla f-\nabla \interp_\cT^{m-1} f\|_{L^p(\Omega)}.
$$
Any estimate on the interpolation error thus automatically yields an upper estimate on the best approximation error $e_\cT(f)_X$. Furthermore if $f$ is sufficiently smooth and if $\cT$ is sufficiently fine, then these quantities are generally comparable.\\



One of the founding results of adaptive anisotropic finite element approximation is the following, see \cite{CSX} or Chapter \ref{chapOptAniso}. For any bounded polygonal domain $\Omega\subset \R^2$, for any $1 \leq p < \infty$, and for any function $f\in C^2(\overline \Omega)$ there exists a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqCSX}
\limsup_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \leq C \left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)}.
\ee
In the previous equation the exponent $\tau \in (0, \infty)$ is defined by $\frac 1 \tau := 1 + \frac 1 p$, and $C$ is a universal constant ($C$ is independent of $p$, $\Omega$ and $f$).
We recall that the upper limit of a sequence $(u_N)_{N \geq N_0}$ is defined by %one has
\be
\label{defLimSup}
\limsup_{N \to \infty} u_N := \lim_{N \to \infty} \sup_{n \geq N} u_n,
\ee
and is in general strictly smaller than the supremum $\sup_{N\geq N_0} u_n$. It is still an open question to find an appropriate upper bound for $\sup_N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)}$ when optimally adapted anisotropic partitions are used.
The result \iref{eqCSX} can be extended to the exponent $p=\infty$, and to dimensional domains $\Omega$ of higher dimension, but the triangulations $\cT_N$ may not be conforming

The result \iref{eqCSX} reveals that the accuracy of the approximation of $f$ is governed by the quantity $\sqrt{|\det(d^2 f)|}$, which depends non-linearly on the hessian matrix $d^2 f$. This non-linear dependency is heavily tied to the fact that we authorize triangles of potentially highly anisotropic shape. The estimate \iref{eqCSX} is obtained by producing sufficiently fine triangulations which combine the two following properties:
\begin{enumerate}[a)]
\item (Error equidistribution) The triangulations $\cT_N$ follow a general rule of adaptive approximation theory: the contribution $\|f-\interp_T^{m-1}f\|_{L^p(T)}$ of each triangle $T \in \cT_N$ to the global interpolation error $\|f-\interp_{\cT_N}^{m-1}f\|_{L^p(\Omega)}$ is approximately the same. This condition can be translated into a local constraint on the area of the triangles, which is dictated by the local behavior of $f$ and in particular by $\det(d^2f(z))$.
\item (Optimal shape of the triangles) 
The elements of $\cT_N$ have a shape which is dictated locally by the hessian matrix $d^2 f(z)$. %This shape is potentially highly anisotropic, 
The aspect ratio and the orientation of these triangles are dictated by the eigenvalues and the eigenvectors of the hessian matrix $d^2f(z)$.
\end{enumerate}
The simplest method for producing a sequence $(\cT_N)_{N \geq N_0}$ of triangulations satisfying \iref{eqCSX} is to use a ``local patching strategy'' as follows. In a first step the domain $\Omega$ is split into regions $\Omega_i$, $1\leq i \leq k$, sufficiently small so that the hessian matrix $d^2f(z)$, $z\in \Omega_i$, varies little around an average value $M_i$. Each region $\Omega_i$ is then tiled using a periodic triangulation $\cT_N^i$ based on $M_i$, in other words $f$ is identified to a quadratic polynomial on each $\Omega_i$. Eventually the triangulations $\cT_N^i$ of $\Omega_i$ are glued together into a triangulation $\cT_N$ of $\Omega$, at the price of a few additional triangles at the boundaries of the $\Omega_i$. 

This construction is sufficient for the proof of the asymptotical result \iref{eqCSX}, but not for practical applications since it only becomes efficient for a large number of triangles. The following approach, based on riemannian metrics, is often preferred in applications.
We assume for simiplicity that the hessian matrix $M(z) := d^2f(z)$ is positive definite for each $z\in \Omega$, and we define 
\be
\label{defHHessian}
H(z) := \lambda^2 (\det M(z))^{-\frac 1 {2p+2}} M(z)
\ee
where $\lambda>0$ is a constant which role is specified later. Such a map $H$ is called a riemannian metric, and continuously associates to each point $z\in \Omega$ a symmetric positive definite matrix $H(z)$. Note that for each $z\in \Omega$ the matrix $H(z)$ defines an ellipse
$$
\cE_z := \{z+u \sep u^\trans H(z) u\leq 1\}.
$$ 
As illustrated on the left part of Figure \ref{figEllTri}, a metric encodes at each point $z\in \Omega$ an information of area, aspect ratio and orientation, under the form of a symmetric positive definite matrix $H(z)$, or equivalently of an ellipse $\cE_z$. 
Several algorithms, such as \cite{FreeFem,Inria} are able to produce a triangulation adapted in the following sense to a given metric  : for each $z\in \Omega$ the triangle $T\in \cT$ containing $z$ has a shape ``similar'' to the ellipse $\cE_z$.
%We now assume that $\lambda$ is sufficiently large, and that a triangulation $\cT$ of $\Omega$ has been produced in such way that for each $z\in \Omega$ the triangle $T\in \cT$ containing $z$ has a shape similar to $\cE_z$.
If $\cT$ is such a triangulation and if $\lambda$ is sufficiently large, a heuristic argument developed in Chapter \ref{chapOptAniso} %\ref{secOptAniso4} 
shows that 
$$
\#(\cT) \|f-\interp_{\cT}^1 f\|_{L^p(\Omega)} \leq C \|\sqrt{|\det (d^2f)|}\|_{L^\tau(\Omega)}.
$$
Varying the parameter $\lambda$ we obtain different triangulations $\cT_\lambda$, of cardinality proportional to $\lambda$, which leads to the error estimate \iref{eqCSX}.
The production of the mesh $\cT$ from the metric $H$ is not straightforward, and some aspects of this question are addressed in Chapter \ref{chapMeshMet}.\\
\begin{figure}
\centering
\includegraphics[height = 4cm,width = 8cm]{\pathPic/Ellipses/EllShewChuk.pdf}
\caption{A metric and an adapted triangulation, (credit : J. Schoen)\label{figEllTri}}
\end{figure}

The approximation result \iref{eqCSX} is optimal if we restrict our attention to admissible sequences of triangulations, a technical condition defined as follows. %provided the following technical condition is satisfied.
We say that a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of a polygonal domain $\Omega \subset \R^2$ is admissible if  $\#(\cT_N) \leq N$ and if 
\be
\label{defAdmiIntro}
\sup_{N \geq N_0} \left(\sqrt N \max_{T \in \cT_N} \diam(T)\right) <\infty.
\ee
For any admissible sequence $(\cT_N)_{N \geq N_0}$ of triangulations of a $\Omega$, one can establish the lower bound 
\be
\label{eqCSXOpt}
\liminf_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \geq c \left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)},
\ee
where the constant $c>0$ is universal, see also Theorem \ref{thLowerLPIntro} below. % Therefore \iref{eqCSX} is optimal if we restrict our attention to admissible 
Furthermore the admissibility condition is not too restrictive : for each $\ve>0$ there exists an admissible sequence of triangulations $(\cT_N)_{N \geq N_0}$ which satisfies the upper estimate \iref{eqCSX} up to the additive constant $\ve$.\\

Similar results to \iref{eqCSX} and \iref{eqCSXOpt} can be developed for isotropic meshes, in which the triangles may vary in size but are constrained to be isotropic in the sense that the measure of degeneracy $\rho(T) := \diam(T)^2/|T|$ is uniformly bounded by a constant $\rho_0$, see for instance \cite{CMi2}.
In that case one needs to replace 
$$
\left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)} \stext{ with } \|d^2f\|_{L^\tau(\Omega)}
$$
in \iref{eqCSX} and \iref{eqCSXOpt}, and the constants $c$ and $C$ depend on the bound $\rho_0$ on the measure of degeneracy, see for instance \cite{CMi2}.
%The improvement due to anisotropy is thus the replacement at each point $z\in \Omega$ of the norm $\|d^2 f(z)\|$ with the non-linear quantity $\sqrt{|\det (d^2f(z))|}$. 
In terms of the eigenvalues $\lambda_1(z), \lambda_2(z)$ of the symmetric matrix $d^2 f(z)$ we thus replace
$$
\sqrt{|\lambda_1(z) \lambda_2(z)|}  \stext{ with } \max \{|\lambda_1(z)|, |\lambda_2(z)|\}.
$$
The use of anisotropic triangulations is therefore particularly advised when the eigenvalues of $d^2 f(z)$ have different orders of magnitude. This is the case if the approximated function $f$ exhibit strongly anisotropic features. % in certain regions.

\subsection{Questions raised in this thesis and open questions}
The result \iref{eqCSX} gives a sharp account of the improvement that anisotropic triangulations can provide compared to isotropic triangulation, under certain conditions. 
We have attempted to list these restrictions and to eliminate them when possible.
The four conditions mentioned below are the object of an in depth study in this thesis and could be eliminated, at least partly.
\begin{enumerate}[I]
\item (Other degrees, other norms)
We extend in Chapter \ref{chapOptAniso} the estimate \iref{eqCSX} to finite elements of arbitrary degree $m-1$, and to the Sobolev $W^{1,p}$ norms.
 Comparatively, the original result only applies to piecewise linear finite elements $m-1= 1$ and to $L^p$ norms. We obtain asymptotical error estimates and optimality results which are similar to \iref{eqCSX} and \iref{eqCSXOpt}. The determinant of the hessian matrix $\det (d^2 f)$ appearing in the original estimate is replaced with an ``invariant polynomial'' applied to the collection $d^m f$ of the $m$-th derivatives of $f$.

\qquad The combination of the following properties guarantees that a triangulation $\cT$ satisfies the optimal error estimate up to a fixed multiplicative constant, see Chapter \ref{secW1P2} for more quantitative analysis of these properties. First the interpolation error needs to be equidistributed among all triangles $T\in \cT$. Second the triangles need to have an optimal shape, which is now dictated by the $m$-th order derivatives of $f$, instead of the hessian matrix. Third the triangulation needs to be sufficiently fine in such way that $f$ is well approximated on each triangle by a polynomial of degree $m$. In the case of Sobolev $W^{1,p}$ norms a fourth property needs to be satisfied : any angle $\theta$ of any triangle $T\in \cT$ should be sufficiently far away from the flat angle, in other words $\theta \leq\theta_{\rm max} < \cPi$.\\

\item (Non smooth functions) 
We consider in Chapter \ref{chapCartoon} the model of cartoon functions, which is popular in image processing. These function are smooth except along a finite collection of smooth curves where they have jump discontinuities.

\qquad Cartoon functions are not differentiable, and the quantity $\|\sqrt{|\det d^2f|}\|_{L^\tau}$ which appears in \iref{eqCSX} has therefore no a-priori meaning. We show nevertheless that for some values of $\tau$ this quantity has a natural extension to cartoon functions $f$, which includes a one-dimensional integral along the collection $\Gamma$ of curves where $f$ is discontinuous. This contribution takes into account the jump of $f$ across $\Gamma$ as well as the curvature of $\Gamma$. However the extension of the approximation result \iref{eqCSX} in that context remains so far a conjecture.\\

\item (Mesh generation)
The most popular methods for anisotropic mesh generation in applications are based on Riemannian metrics, as exposed in \iref{defHHessian}. These metrics encode at each point the desired size, aspect ratio and orientation of the triangles.

\qquad This raises the objective of defining and proving precise equivalence results between some classes of triangulations and of metrics. We answer this question in Chapter \ref{chapMeshMet}, which provides a translation of some geometrical properties of triangulations into regularity properties satisfied by the corresponding metrics. We pay a particular attention to the angle condition evoked in I for the approximation of function in the $W^{1,p}$ semi-norm, the fact that the angles appearing in the triangulation are uniformly bounded away from $\cPi$. These results are used in Chapter \ref{chapApproxMet} to reformulate, and solve in some cases, several optimization problems posed on triangulations.\\

\item (Combining hierarchy with anisotropy) 
A number of algorithms are based on hierarchical sequences of triangulations $(\cT_N)_{N \geq N_0}$, a property which guarantees % The fact that $\cT_{N+1}$ is a refinement of $\cT_N$ implies 
the inclusion of the associated finite element spaces $V_k(\cT_N)\subset V_k(\cT_{N+1})$. The property of hierarchy also allows for the definition of wavelet bases, and is a key in the analysis of some PDEs.

\qquad We define in Chapter \ref{chapCDHM} an algorithm producing sequences of (non conforming) anisotropic triangulations which satisfy this property of hierarchy, and in certain circumstances also satisfy the optimal error estimate \iref{eqCSX}. This algorithm strongly differs from the mesh generation methods presented previously, the local patching strategy and the approach based on riemannian metrics, since these are not adapted to hierarchical mesh refinement.\\
\end{enumerate}

Current results in anisotropic mesh adaptation for finite element approximation %, the study of $e_N(f)_X$, 
also suffer from two other important restrictions : they are only asymptotical, and they extend with difficulty to dimensions larger than two.
%The results presented in this section, which are more or less the state of the art in anisotropic mesh adaptation, also suffer from two other weaknesses. 
Removing these two restrictions raises difficult problems and remains mostly an open question at the time of writing.

\begin{enumerate}[i)]
\item (Non asymptotical results) 
The optimal error estimate \iref{eqCSX} involves a limit as the number $N$ of triangles constituting the mesh $\cT_N$ tends to infinity, see \iref{defLimSup}.
The asymptotic nature of this error estimate reveals that a sufficiently large number of triangles is needed to finely tune the triangulation $\cT_N$ to the local properties of the approximated function $f$. A smaller number of triangles raises the need for a compromise between the adaptation to the local features approximated function $f$ and the geometrical constraints involved in the production of a bi-dimensional triangulation.

\qquad We give in Chapter \ref{chapMeshMet} a translation of these geometrical constraints into the form of regularity properties satisfied by riemannian metrics, continuous objects which are equivalent to triangulations, see Theorem \ref{thMeshMetIntro}. In the case of isotropic triangulations we recover in Chapter \ref{chapApproxMet} some classical error estimates, expressed in terms of the Hardy-Littlewood maximal function of $|d^mf|$,  for the quantity 
$$
\sup_{N \geq 1} N^\frac m 2 e_{\cT_N} (f)_X %\left(\text{ instead of } \limsup_{N \to \infty} N^\frac m 2 e_{\cT_N} (f)_X\right).
$$
instead of the upper limit $\limsup_{N \to \infty} N^\frac m 2 e_{\cT_N} (f)_X$.
Obtaining a relevant estimate of this quantity in the case of anisotropic triangulations remains today an open question. \\

\item (Meshes in three or more dimensions) 
Throughout this introduction, we have yet only considered functions of two variables and bi-dimensional triangulations. 
Our discussion remains relevant in dimension three or higher, and three dimensional anisotropic mesh adaptation is already successfully used in applications, see for instance \cite{A}.

\qquad However a number of theoretical aspects of these methods remain unanswered. The key difficulty is the production of three dimensional anisotropic meshes, which is difficult from a practical point of view and not well understood from a theoretical point of view. We formulate in Chapter \ref{chapMeshMet} several conjectures which extend our bi-dimensional results on the equivalence of meshes and riemannian metrics.

\qquad We also consider dimensions larger than $2$ in parts I and II of this thesis, % (OptAniso??) and (Cartoon??),
which leads us to several types of difficulties. Some of these difficulties have an algebraic nature in Chapter \ref{chapOptAniso}, a geometric nature in Chapter \ref{chapCartoon}, or are related to mesh generation in Chapter\ref{chapW1P}. We formulate a precise conjecture each time that we cannot solve these difficulties.\\ 
\end{enumerate}

Last, the two following questions could be raised about the results \iref{eqCSX} and \iref{eqCSXOpt} on optimal mesh adaptation presented in this introduction. We regard them as more minor and they are not the subject of in depth discussion in this thesis.
\begin{enumerate}[i)]
\item (Interpolation instead of best approximation)
Some estimates presented in this introduction, such as \iref{eqCSX}, are based on the interpolation error instead of the best approximation error. In other words, for a given function $f$ and triangulation $\cT$ they provide an upper bound for 
\be
\label{eqInterp}
\|f-\interp_\cT^{m-1} f\|_{L^p} \stext{ or } \|\nabla (f - \interp_\cT^{m-1} f)\|_{L^p}
\ee
instead of 
\be
\label{eqBestApprox}
e_\cT(f)_{L^p} := \min_{g\in V_{m-1}(\cT)} \|f-g\|_{L^p} \stext{ or } e_\cT(f)_{W^{1,p}} := \min_{g\in V_{m-1}(\cT)} \|\nabla (f-g)\|_{L^p}.
\ee
\qquad The quantities \iref{eqInterp} correspond to the particular choice $g=\interp_\cT^{m-1} f$ and are therefore an upper bound for the corresponding quantities in \iref{eqBestApprox}. Is the difference so big that an estimate on \iref{eqInterp} is not relevant in the case \iref{eqBestApprox}?
The answer is generally ``no'' if the function $f$ is sufficiently smooth and if the triangulation $\cT$ is sufficiently fine, which is the case in the asymptotic setting considered in \iref{eqCSX}.
In contrast we consider in Chapter \ref{chapApproxMet} some functions of weaker regularity, and triangulations of fixed cardinality, which forbids the use of the standard Lagrange interpolation operator. The interpolation of $f$ is thus replaced with an quasi-interpolation of the local averages of $f$.\\

\item (The admissibility condition) 
The optimality results presented in this thesis, such as \iref{eqCSXOpt}, require the admissibility of the sequence $(\cT_N)_{N\geq N_0}$ of triangulations. This technical hypothesis can be removed in certain cases, such as the interpolation of a convex function by finite elements of degree one, see \cite{BBLS}.
We have not been able to remove this hypothesis in the general case, but we believe that the admissibility condition is rather a technical inelegancy than a weakness of the theory.
\end{enumerate}

\section{Outline of the thesis}
%\label{secIntro2}

This thesis is composed of four parts I to IV which correspond to four key questions in anisotropic finite element approximation : approximation using finite elements of arbitrary degree, or measured in Sobolev norms; the link between anisotropic smoothness classes and image models; the equivalence between certain classes of triangulations and of  riemannian metrics; and eventually the combination of hierarchy with anisotropy.

These four parts, as well as the nine chapters composing them, are mostly self consistent and can be read independently.

\subsection{Finite elements of arbitrary degree, and Sobolev norms} %Elements finis de plus haut degré, normes de Sobolev}%Premier objectif : que peut-on faire de mieux, asymptotiquement?}
\label{subsecOptAnisoIntro}

We have extended the optimal asymptotic estimate \iref{eqCSX} to finite elements of arbitrary degree. In order to present our results we need to introduce some notations.

We denote by $\H_m$ the space of homogeneous polynomials of degree $m$:
$$
\H_m := \Span\{x^k y^l \sep k+l = m\}.
$$
A key ingredient of our approach is the shape function $K_{m,p} : \H_m \to \R_+$, where $1\leq p\leq \infty$ is an exponent. 
This function is defined as an optimization of the $L^p$ interpolation error among the collection of triangles of unit area of all possible shapes: for all $\pi\in \H_m$,
\be
\label{defKMPIntro}
K_{m,p}(\pi) := \inf_{|T| = 1} \|\pi-\interp_T^{m-1} \pi\|_{L^p(T)}.
\ee
Our main result is the following asymptotic error estimate.
\begin{theoremIntro}
\label{thOptiLPIntro}
Let $\Omega\subset \R^2$ be a bounded polygonal domain, let $f\in C^m(\overline \Omega)$ and let  $1\leq p < \infty$.
There exists a sequence $(\cT_N)_{N \geq N_0}$ of conforming triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqLPIntro}
\limsup_{N \to \infty} N^{\frac m 2}\|f-\interp_{\cT_N}^{m-1} f\|_{L^p(\Omega)} \leq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)}, \stext{ where } \frac 1 \tau := \frac m 2 + \frac 1 p.
\ee
\end{theoremIntro}

In the error estimate \iref{eqLPIntro}, we identify the collection $d^m f(z)$ of derivatives of order $m$ of $f$ at the point $z\in \Omega$ to the corresponding homogeneous polynomial in the Taylor development of $f$ at $z$. In other words
$$
\frac {d^m f(z)}{m!} \sim \sum_{k+l = m} \frac{\partial^m f(z)}{\partial^k x\, \partial^l y} \, \frac {x^k}{k!} \frac {y^l}{l!}.
$$

Theorem \ref{thOptiLPIntro} extends the known result \iref{eqCSX} to finite elements of arbitrary degree $m-1$. The quality of the approximation of $f$ is similarly determined by a non-linear quantity of its derivatives: the shape function $K_{m,p}(d^m f(z))$ replaces $\sqrt{|\det (d^2f(z))|}$ appearing in \iref{eqCSX}. 
In the case of isotropic triangulations, in which the measure of non degeneracy $\rho(T) := \diam(T)^2/|T|$ is uniformly bounded among all triangles $T\in \cT_N$, $N \geq N_0$, by a given constant $\rho_0$, the nonlinear quantity $K_{m,p}(\frac {d^m f(z)} {m!})$ needs to be replaced by the larger quantity $\|d^mf(z)\|$. The improvement due to anisotropy is thus expressed through the shape function $K_{m,p}$, at least for an asymptotically large number of triangles.

This remark raises the need for an in depth study of the shape function $K_{m,p}$. For $m=2$ we have established that $K_{2,p}(\pi)$ is proportional to the square root of the determinant of the quadratic polynomial $\pi = a x^2 + 2 b xy + cy^2\in \H^2$:
$$
K_{2,p}(\pi) = c_{2,p}(\det \pi) \sqrt{|\det \pi|} = c_{2,p}(ac-b^2)\sqrt {|ac-b^2|},
$$
where the constant $c_{2,p}(s)>0$ only depends on the sign of $s$. We thus recover the earlier result \iref{eqCSX}.
For $m=3$, the shape function $K_{3,p}$ is the fourth root of the discriminant of the homogenous cubic polynomial $\pi = a x^3+3bx^2y+3cxy^2+dy^3\in \H_3$:
$$
K_{3,p}(\pi) = c_{3,p}(\disc \pi) \sqrt{|\disc \pi|} = c_{3,p}(\disc \pi)\sqrt {|4(ac-b^2)(bd-c^2) - (ad-bc)^2|},
$$
where the constant $c_{3,p}(s)>0$ only depends on the sign of $s$. For larger values $m\geq 4$ we have obtained an explicit quantity uniformly equivalent to the shape function $K_{m,p}$, but not an explicit expression of $K_{m,p}$. This equivalent has the following form : there exists a polynomial $Q_m(a_0, \cdots, a_m)$ of the $m+1$ variables $a_0, \cdots, a_m$ and a constant $C_m>0$ such that for all $\pi = a_0 x^m+ a_1 x^{m-1}y+ \cdots a_m y^m\in \H_m$ one has with $r_m := \deg Q_m$,
\be
\label{equivKQ}
C_m^{-1} \sqrt[r_m]{Q_m(a_0, \cdots , a_m)} \leq K_{m,p}(\pi) \leq  C_m\sqrt[r_m]{Q_m(a_0, \cdots , a_m)}.
\ee
The polynomial $Q_m$ is obtained using the theory of invariant polynomials developed by Hilbert in \cite{Hilbert}. We also characterise %the polynomials $\pi\in \H_m$ on which the function $K_{m,p}$ vanishes, and thus 
the possible cases of ``super-convergence'' : $K_{m,p}(\pi)=0$ if and only if $\pi$ has a linear factor $ax+by$ of multiplicity $s>m/2$, in other words the homogeneous polynomial $\pi$ is sufficiently degenerated.\\

The proof of theorem \ref{thOptiLPIntro} is based on a ``local patching strategy'', a two scale mesh generation procedure which proceeds as follows: we consider a first triangulation $\cR$ of the polygonal domain $\Omega$ which is sufficiently fine in such way that the derivatives of order $m$ of $f$ vary little on each triangle $R\in \cR$ around an average value denoted by $\pi_R\in \H_m$. To each polynomial $\pi_R$, $R\in \cR$, we then associate a triangle $T_R$ which is a minimizer, or a near minimizer, of the optimization problem defining $K_{m,p}(\pi_R)$. We then on each $R\in \cR$ using the triangle $T_R$ a properly scaled and its symmetric with respect to the origin. Eventually, as illustrated on Figure \ref{figLocPatch} the triangulation $\cT_N$ is obtained by gluing together the periodic tilings on each $R\in \cR$, with a few additional triangles in order obtain a globally conforming mesh.

\begin{figure}
	\centering
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/NonConformTiling.pdf}
		\hspace{1cm}
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/ConformTiling.pdf}
		\hspace{1cm}
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/TriangleClasses.pdf}
	\caption{\label{figLocPatch} Illustration of the local patching strategy : the elements of a macro triangulation $\cR$ are covered by periodic tilings, which are then glued together.}
\end{figure}

The next theorem establishes that the asymptotic error estimate \iref{eqLPIntro} is sharp, at least if we restrict our attention to admissible sequences of triangulations, see \iref{defAdmiIntro} for the definition of this condition. Furthermore \iref{eqLPEpsIntro} shows that the admissibility condition is not too restrictive.

\begin{theoremIntro}
\label{thLowerLPIntro}
Let  $\Omega\subset \R^2$ be a bounded polygonal domain, let $f\in C^m(\overline \Omega)$, and let $1\leq p\leq \infty$.
Let $(\cT_N)_{N \geq N_0}$, $\#(\cT_N) \leq N$, be an admissible sequence of triangulations of $\Omega$. Then
\be
\label{eqLPLowerIntro}
\liminf_{N \to \infty} N^{\frac m 2} \|f-\interp_{\cT_N}^{m-1} f\|_{L^p(\Omega)} \geq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)},
\ee
where  $\frac 1 \tau := \frac m 2 + \frac 1 p$. Furthermore for any $\ve>0$ there exists an admissible sequence $(\cT_N^\ve)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N^\ve) \leq N$, and such that: 
\be
\label{eqLPEpsIntro}
\limsup_{N \to \infty} N^{\frac m 2} \|f-\interp_{\cT^\ve_N}^{m-1} f\|_{L^p(\Omega)} \geq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)}.
\ee
\end{theoremIntro}

We extend in Chapter \ref{chapW1P} Theorems \ref{thOptiLPIntro} and \ref{thLowerLPIntro} to Sobolev $W^{1,p}$ semi-norms. For that purpose the shape function $K_{m,p}$ is be replaced by the analogous quantity for $W^{1,p}$ semi-norms $L_{m,p} : \H_m \to \R_+$ which is defined as follows: for all $\pi \in \H_m$ 
$$
L_{m,p}(\pi) := \inf_{|T|=1} \|\nabla (\pi-\interp_T^{m-1} \pi)\|_{L^p(T)},
$$
and the exponent $\tau$ becomes $\frac 1 \tau := \frac {m-1} 2+ \frac 1 p$.
Similarly to \iref{equivKQ} we have also found some explicit equivalents of $L_{m,p}(\pi)$ defined by an algebraic expression in the coefficients of $\pi\in \H_m$.
Our results for the $W^{1,p}$ semi-norm are thus extremely similar to the results obtained for the $L^p$ norm.
The extension of the proofs however is not straightforward, because of the following new phenomenon: the presence of flat angles in a triangulation deteriorates the interpolation in the $W^{1,p}$ semi-norm, which is not the case in the $L^p$ norm. 

Eventually we also extend in Chapter \ref{chapBlocks} Theorems \ref{thOptiLPIntro} and \ref{thLowerLPIntro}  to partitions of a rectangular domain into anisotropic rectangles aligned with the coordinate axes, instead of triangles, with the approximation error measured in the $L^p$ norm. %, which are again potentially highly anisotropic.
 Such partitions are relevant when the coordinate axes play a privileged role, in such way that the anisotropic features of the approximated function $f$ are likely to be aligned with the coordinate axes.
The proof of the results for partitions into blocks or into triangles uses the same key ideas, but the technicalities are greatly reduced in the first case due to the presence of privileged axes.

Part \ref{partAsymptApprox} is organized as follows. We first consider in Chapter \ref{chapBlocks} partitions of a domain into rectangles or blocks aligned with the coordinate axes, with the error measured in the $L^p$ norm. 
We take advantage of this simple setting to introduce and examine in detail the shape function and the local patching strategy.
We then turn in Chapter \ref{chapOptAniso} to finite element interpolation error on anisotropic triangulations measured in the $L^p$ norm, and we eventually consider in Chapter \ref{chapW1P} the $W^{1,p}$ interpolation error.
The three chapters composing Part \ref{partAsymptApprox} are self consistent and can be read independently.

\subsection{Anisotropic smoothness classes and image models}

There exists various ways of measuring the smoothness of functions on a domain $\Omega\subset \R^2$, generally through the definition of an {\it appropriate smoothness} space and an associated norm. Classical instances are Sobolev and Besov spaces. Such spaces  are of common use when describing the regularity of solutions to partial differential equations. From a numerical perspective they are also useful in order to sharply characterize at which rate a function $f$ may be approximated by simpler functions such as Fourier series, finite elements (on isotropic triangulations), splines or wavelets.

Functions arising in concrete applications, for instance in image processing or in the solution of hyperbolic PDEs, often %may have inhomogeneous smoothness properties, in the sense that they 
exhibit areas of smoothness separated by local discontinuities.
The smoothness space that is best taylored to take these features into account is the space $BV$ of functions of bounded variation. 
This space consists of those $f\in L^1(\Omega)$ such that $\nabla f$ is a bounded measure, i.e. such that their total variation 
$$
\TV(f) = |f|_{BV} := \max\left\{\int_\Omega f \diver \vp \sep \vp\in \cD(\Omega), \|\vp\|_{L^\infty} \leq 1\right\}.
$$
is finite. Assume that $\Omega := ]0,1[^2$ is the unit square, and denote by $f_N$ the approximation of $f$ by the $N$ terms of its development on the Haar basis which correspond to the largest coefficients. It is established in \cite{CDPX, CDDD2} that 
\be
\label{eqApproxTV}
\sup_{N \geq 0} \sqrt N \|f-f_N\|_{L^2(\Omega)} \leq C \TV(f).
\ee

The result \iref{eqCSX} and its generalisation Theorem \ref{thOptiLPIntro} establish that the quality of the approximation of a function $f$ by finite elements on anisotropic triangulations is governed by some non-linear quantities of the derivatives of $f$, at least from an asymptotical point of view.
In the case of finite elements of degree $1$, and of the approximation in $L^2$ norm, the relevant quantity is the following
$$
A(f) := \left\|\sqrt {|\det(d^2f)|}\right\|_{L^{2/3}(\Omega)}.
$$
For any bounded polygonal domain $\Omega$ and any $f\in C^2(\overline \Omega)$ there exists, see \iref{eqCSX}, a sequence $\cT_N$ of triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqApproxA}
\limsup_{N \to \infty} N \|f-\interp_{\cT_N}^1 f\|_{L^2(\Omega)} \leq C A(f).
\ee

The functional $A$ strongly differs from the total variation $\TV$, and also from the Sobolev, Holder or Besov norms, because of its nonlinear behavior: $A$ does not satisfy the triangle inequality, or any quasi-triangle inequality. In other words for any constant $C$ there exists $f,g\in C^2(\overline \Omega)$ such that 
\be
\label{eqNoTri}
A(f+g) \not \leq C(A(f)+A(g)).
\ee
%Contrary to the total variation $\TV$, the functional $A$ is not a priori attached to an smoothness space. If such a space exists then the \iref{eqNoTri} 
The lack of a triangular inequality forbids to use the classical techniques of linear analysis to define a smoothness space attached to the functional $A$. Another problem comes from the limit appearing in \iref{eqApproxA}, which not present in classical approximation theory, see for instance \iref{eqApproxTV}. (A naive attempt to define an approximation space associated to the functional $A$ is nevertheless presented in Chapter \ref{chapApproxMet}.)

Concrete applications require nevertheless that results of the type of \iref{eqApproxA} be extended to non smooth functions and in particular to the class of cartoon functions.
A heuristical analysis presented in Chapter \ref{chapCartoon} suggests that for any cartoon function $f$ defined on a bounded polygonal domain $\Omega$, there exists a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N)\leq N$, and such that 
\be
\label{eqApproxCartoon}
\sup_{N\geq N_0} N \|f-\interp_{\cT_N}^1 f\|_{L^2(\Omega)} < \infty. % \text{ est borné, \quad où } r_p := \min\left\{1, \frac 2 p\right\}.
\ee
The compact form of this estimate hides the balance between to different phenomena in the approximation of $f$, each of them requiring approximately half of the cardinality of $\cT_N$. First the function $f$ is approximated by the linear interpolant $\interp_{\cT_N}^1 f$ on the regions where $f$ is smooth. Second the collection $\Gamma$ of curves along which $f$ is discontinuous is approximated by the boundaries $\partial T$, of the triangles $T\in \cT_N$. The difference $f-\interp_{\cT_N}^1 f$ does not tend to zero on the neighborhood of $\Gamma$, but the width of this neighborhood tends to $0$.

The approximation result \iref{eqApproxCartoon} raises the hope that a precise and quantitative asymptotic estimate, similar to \iref{eqApproxA}, can be obtained for cartoon functions.
So far we have only fulfilled one part of this program: the extension of the functional $A$ to cartoon functions. More precisely, consider a radial and compactly supported function $\vp\in C^\infty(\R^2)$ of unit integral. 
For any $\delta>0$ we define $\vp_\delta(z) := \frac 1 {\delta^2} \vp\left(\frac z \delta\right)$ and we denote by $f_\delta := f*\vp_\delta$ the convolution of $f$ with $\vp_\delta$. 
We establish in Chapter \ref{chapCartoon} that $A(f_\delta)$ converges as $\delta \to 0$, to an explicit expression
\begin{eqnarray*}
\lim_{\delta \to 0} A(f_\delta)^{2/3} &=& \left\|\sqrt{|\det(d^2 f)|}\right\|_{L^{2/3}(\Omega\sm\Gamma)}^{2/3} + C(\vp) \left\|\sqrt{|\kappa|} \gamma\right\|_{L^{2/3}(\Gamma)}^{2/3}\\ %\left(\|\right)
&=& \int_{\Omega\sm\Gamma} \sqrt[3]{|\det (d^2 f(z))|}dz+ C(\vp)\int_\Gamma |\kappa(s)|^{1/3} |\gamma(s)|^{2/3}ds.
\end{eqnarray*} %\frac 1 3 \frac 2 3
In the previous equation, we denote by $\Gamma$ the collection of curves where the cartoon function $f$ is discontinuous, by $\gamma(s)$ the jump of $f$ at the point $s\in \Gamma$, and by $\kappa(s)$ the curvature of $\Gamma$ at $s$. The constant $C(\vp)$ is positive and explicit in terms of $\vp$.

\begin{figure}
\centering
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Sina.pdf}
\hspace{1cm}
\includegraphics[height=4cm,width=4cm]{\pathPic/Bayesien/Staira.pdf}
\hspace{1cm}
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Flowera.pdf}
\caption{\label{figTVA} Behavior of the functionals $\TV$ and $A$ on different types of images.}
\end{figure}

Comparatively, we have 
$$
\TV(f) = \int_{\Omega\sm\Gamma} |\nabla f(z)|dz+\int_\Gamma |\gamma(s)| ds.
$$

Part \ref{partCartoon} consists of the single chapter, Chapter \ref{chapCartoon}, containing in particular the above result. The rest of this chapter is organized as follows.
The extension of the nonlinear functional $A$ to cartoon functions puts in light a link, explored in section \S\ref{secCartoon4}, 
between anisotropic finite element approximation and several other mathematical fields. We think in particular of affine invariant image processing \cite{Ca} and of the definition in \cite{DPW} of smoothness spaces through the regularity of the level lines of a function.
The functional $A$ also can be thought of as a new quantitative image model : a monochromatic image, described by a brightness function $f: [0,1]^2 \to [0,1]$, is plausible if $A(f)$ is sufficiently small. Generalising the work \cite{LMo} we explore in section \S\ref{secCartoon5.5} an image recovery procedure using this model as a bayesian prior. 
Eventually we describe in section \S\ref{secCartoon6} the extension to cartoon functions of other non-linear quantities appearing in anisotropic finite element approximation such as the norm $\|K_{m,p}(d^m f)\|_{L^\tau}$ of the shape function for $m\geq 2$, or the counterpart of this quantitiy for functions $f$ of more than two variables.


\subsection{Mesh generation and riemannian metrics} %Génération de maillage et métriques riemanniennes} %Problèmes de génération de maillage}

Triangulations are discrete objects of combinatorial nature : they can be described by the collection of their vertices and of the edges between them. This description is fruitful for the demonstration of algebraic results such as the Euler formula, or for computer processing.

In the context of anisotropic mesh adaptation, several works \cite{Shew,Bois,A} choose in contrast to replace triangulations of a domain $\Omega$ with a continuous object during the optimisation procedure : a riemannian metric, in other words a continuous function $H$ from $\Omega$ to the set $S_2^+$ of symmetric positive definite matrices. Our purpose is to give a theoretical background to this replacement, through the formulation of precise equivalence results between some classes of triangulations and of riemannian metrics. In particular the geometrical properties of the triangulations need to be translated under the form regularity properties of the riemannian metrics.

In order to state our results we need to introduce some notations. We associate to each triangle $T$ its barycenter $z_T\in R^2$ and the symmetric positive definite matrix $\cH_T\in S_2^+$ such that the ellipse $\cE_T$ defined by 
$$
\cE_T := \{z\in \R^2 \sep (z-z_T)^\trans \cH_T (z-z_T)\},
$$
is the ellipse of minimal area containing $T$. The point $z_T$ thus encodes the position of $T$, while the matrix $\cH_T\in S_2^+$ encodes the area, the aspect ratio and the orientation (but not the angles) of the triangle $T$ .

We denote by $\bT$ the collection of triangulations of the infinite domain $\R^2$ - the choice to consider infinite triangulations is guided by simplicity, and further work will be devoted to triangulations of bounded domains.
We denote by $\bH := C^0(\R^2, S_2^+)$ the collection of riemannian metrics on $\R^2$. A metric $H\in \bH$ continuously associates to each point $z\in \R^2$ a symmetric positive matrix $H(z)\in S_2^+$.
We say that a triangulation $\cT\in \bT$ is $C$-equivalent to a metric $H \in \bH$ if for all $T\in \cT$ and for all $z\in T$ we have 
$$
C^{-2} H(z) \leq \cH_T \leq C^2 H(z). 
$$
We say that a class of triangulations $\bT_*\subset \bT$ is equivalent to a class of metrics $\bH_*\subset \bH$ if there exists a uniform constant $C>0$ such that 
\begin{itemize}
\item For any triangulation $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C$-équivalent.
\item For any metric $H\in \bH_*$ there exists a triangulation $\cT\in \bT_*$ such that $\cT$ and $H$ are $C$-équivalent.
\end{itemize}

%The full class $\bT$ of all triangulations is not equivalent to the full class $\bH$ of all metrics. 
We define below three particularly relevant classes of triangulation
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}
$$
which have a minor dependency on a parameter $C\geq 1$.
When $C$ is sufficiently large, these classes of triangulations are equivalent to three classes of metrics respectively 
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
We now turn to the description of these classes of triangulations and of metrics.
The class $\bT_{g,C}$ of \emph{graded} triangulations, is defined by the following condition which imposes a minimum of consistency among the shapes of neighbouring triangles. A triangulation $\cT$ belongs to $\bT_{g,C}$ if for all $T, T'\in \cT$ one has
$$
T \cap T' \neq \emptyset \quad \Ra \quad C^{-2} \cH_T \leq \cH_{T'} \leq C \cH_T.
$$
A triangulation $\cT$ belongs to the class $\bT_{i,C}$ of \emph{isotropic} triangulations if $\cT$ is graded : $\cT\in \bT_{g,C}$,
%(cette condition peut être supprimée, voir ??) 
and if the elements of $\cT$ are sufficiently close to the equilateral triangle, as expressed by the following condition: for all $T\in \cT$
$$
\|\cH_T\| \|\cH_T^{-1}\|\leq C^2.
$$
Eventually the class $\bT_{a,C}$ of \emph{quasi-acute} triangulations is defined by a slightly more technical condition on the maximal angles of the triangles, see Chapter \ref{chapMeshMet}. This condition guarantees the stability of the gradient of the interpolation of a function, but raises difficulties in terms of mesh generation which diminish the flexibility of use of quasi-acute triangulations in practical applications. One of our key results is the reformulation of this diminished flexibility under the form of a regularity assumption on an equivalent riemannian metric.

When the constant $C$ is sufficiently large, the class $\bT_{i,C}$ of isotropic triangulations is equivalent to the class $\bH_i$ of metrics $H$ which are proportional to the identity
$
H(z) = \Id /s(z)^2 ,
$
and such that the proportionality factor $s$ satisfies one of the following \emph{equivalent} properties
\begin{enumerate}[$\bullet$]
\item Euclidean Lipschitz Property: $|s(z) - s(z')| \leq |z-z'|$ for all $z,z'\in \R^2.$
\item Riemannian Lipschitz Property: $|\ln s(z) - \ln s(z')| \leq d_H(z,z')$ for all $z,z'\in \R^2.$
\end{enumerate}
We recall that the riemannian distance $d_H(z,z')$ measures the length, distorted by the metric $H$, of the smallest path joining $z$ and $z'$, see Chapter \label{chapMeshMet}.

The two lipschitz properties presented above have (non equivalent) natural extensions to general anisotropic riemannian metrics. They involve two distances $d_+$ and $d_\times$ on the collection $S_2^+$ of symmetric positive definite  riemannian metrics %, see ??
\begin{eqnarray}
\label{eqDPlusIntro}
d_+(H(z), H(z') ) & \leq & |z-z'| \stext{ for all } z,z'\in \R^2,\\
\label{eqDTimesIntro}
d_\times(H(z), H(z') ) & \leq &d_H(z,z') \stext{ for all } z,z'\in \R^2.
\end{eqnarray}

Our main result reformulates under the form of the above Lipschitz properties the flexibility offered by the class of graded triangulations $\bT_{g,C}$ and of quasi-acute triangulations $\bT_{a,C}$ - note that the latter is more rigid due to the angle constraint.
\begin{theoremIntro}
\label{thMeshMetIntro}
If the constant $C$ is sufficiently large, then the class $\bT_{g,C}$ of graded triangulations is equivalent to the class $\bH_g$ of metrics satisfying \iref{eqDTimesIntro}. The class $\bT_{a,C}$ of quasi-acute triangulations is equivalent to the class $\bH_a$ of metrics satisfying simultaneously \iref{eqDTimesIntro} and \iref{eqDPlusIntro}.
\end{theoremIntro}

%(*Séparation de deux ensembles, un mot sur l'approx Theory*)

\subsection{Hierarchical refinement  algorithms}

The last part of this thesis, Part \ref{partGreedy}, is devoted to the study an algorithm proposed by Cohen, Dyn and Hecht which produces hierarchical sequences $(\cT_N)_{N\geq N_0}$ of (non-conforming) anisotropic triangulations adapted to a given function $f$.
Given a triangulation $\cT$ of a domain $\Omega$ and a function $f\in L^p(\Omega)$, this algorithm creates in one step a triangulation $\cT'$ of $\Omega$, of cardinality $\#(\cT') = \#(\cT)+1$, proceeding as follows:
\begin{enumerate}
\item (Greedy triangle selection) A triangle $T\in \cT$ which has a maximal contribution to the error is selected 
$$
T := \argmax_{T'\in \cT} \|f-\cA_{T'} f\|_{L^p(T')},
$$
where $\cA_T : L^p(T) \to \P_1$ a projection operator, for instance the $L^2(T)$ orthogonal projection onto $\P_1$.
\item (Decision of a bisection)
The refinement procedure considers the three following bisection choices for the triangle $T$ : from the midpoint of an edge $e\in \{a,b,c\}$ of $T$ to the opposite vertex, creating the sub-triangles $T_e^1$ and $T_e^2$. The edge which minimizes a given decision function $d_T(e,f)$ is selected,  and we define 
$$
\cT' := \cT-\{T\} + \{T_e^1, T_e^2\}.
$$
\end{enumerate}
Starting from a triangulation $\cT_0$ of cardinality $N_0$ of the domain $\Omega$, the algorithm produces step after step a sequence $(\cT_N)_{N\geq N_0}$, see Figure \ref{figRefinement}, of triangulations ``adapted'' to a given function $f\in L^p(\Omega)$. The properties of these triangulations strongly depend on the approximated function $f$ and on the choice of the decision function $d_T(e,f)$, which guides the creation of anisotropy - in contrast the projection operator $\cA_T$ plays a rather minor role.

\begin{figure}
	\centering
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Algo1.pdf}
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Algo2.pdf}
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Algo3.pdf}
	\caption{\label{figRefinement}Refinement algorithm : selection of the triangle which maximizes the local approximation error (in blue), choice of a bisection among the three possibilities, repetition of these two steps until the refinement is sufficient.}
\end{figure}

We present this algorithm in more detail in Chapter \ref{chapCDHM}, and we prove the convergence of this algorithm
%a general convergence result for any bounded polygonal domain $\Omega$ and any $f\in L^p(\Omega)$, 
under some assumptions on the projection operator $\cA_T$ and the decision function $d_T(e,f)$.
Our main result, presented in Chapter \ref{chapBisecOpt}, states that when $f$ is a strictly convex $C^2$ function, for a particular choice \iref{eqDecisionL1} of the decision function, the sequence $(\cT_N)_{N\geq N_0}$ of triangulations generated by this algorithm satisfies the best possible asymptotic convergence estimate
$$
\limsup_{N \to \infty} N \| f-\cA_{\cT_N} f\|_{L^p(\Omega)} \leq C \|\sqrt{|\det (d^2f)|}\|_{L^\tau(\Omega)},
$$
where $\frac 1 \tau := 1+ \frac 1 p$ and where $\cA_\cT f$ denotes the piecewise linear function on $\Omega$ which coincides with $\cA_T f$ on each $T\in \cT$.\\

Eventually we study in Chapter \ref{chapVariations} some variants of the hierarchical refinement algorithm presented above. %, which is also referred to as the ``greedy algorithm''. 
More precisely we consider in section \S\ref{secAltDec} a decision function based on the $L^2$ approximation error, which is particularly well suited to the numerical implementation since it can be evaluated in small computing time.

We then focus in section \S\ref{secAltBi} on the approximation of cartoon functions. The original algorithm is not well suited to this context, and we therefore introduce and study some modifications of the bisection choices offered to the decision function.

Eventually we consider in section \S\ref{secGreedyRect} another variant of the algorithm, which is based on rectangles aligned with with the coordinate axes instead of triangles of arbitrary direction. This simplification leads to Theorem \ref{thRect} which guarantees the best possible convergence estimate for all $C^1$ functions, in the case of piecewise constant approximations on rectangles aligned with the coordinate axes.


==> Introduction/IntroEngTheseOld3.tex <==
%\title{Adaptive and anisotropic finite element approximation:\\Theory and Algorithms}
%%Approximation adaptative et anisotrope par éléments finis\\Théorie et Algorithmes}
%\maketitle
%\tableofcontents

%Important : this introduction is only draft, and is not ready to be reviewed.

\section{Anisotropic finite element approximation : why and how?} %Finite element approximation : Motivations, State of the art and Open questions}

This thesis is devoted to the problem of approximating functions by piecewise polynomial
finite elements over triangulations, and more general meshes. We are particularly
concerned with the setting where the mesh is {\it adaptively designed} depending 
on the function to be approximated. This mesh may therefore include elements 
of strongly varying size, aspect ratio and orientation.\\

Approximation by piecewise polynomial functions
is a procedure that occurs in numerous applications. 
In some of them such as 
terrain data simplification, surface or image compression,
the function $f$ to be approximated might be fully known.
In other applications such as denoising, statistical learning or 
in the finite element discretization of PDE's,
it might be only partially known or fully
unknown.
In all these applications, one usually makes the 
distinction between {\it uniform} and {\it adaptive} approximation.
In the uniform case, the domain of interest is decomposed into
a partition where all elements have comparable shape and size,
while these attributes are allowed to vary strongly in the adaptive case.
The partition may therefore be adapted to the local properties
of $f$, with the objective of 
optimizing the trade-off between accuracy and complexity of
the approximation.

From an approximation theoretic point of view, the trade-off between
accuracy and complexity if usually tied to the smoothness properties of the
function: typically one expects higher convergence rates for smoother functions.
Functions arising in concrete applications may however have inhomogeneous smoothness properties, in the sense that they exhibit areas of smoothness separated by localized discontinuities.
Two typical instances displayed in see Figure \ref{figEllTri0} 
and Figure \ref{figInria} are (i) edges in functions representing images, and (ii) shock profiles in the solutions to non-linear hyperbolic PDE's. 
%These functions often need to be processed numerically, for instance for image denoising or compression, or for the simulation of the evolution of a PDE. 
Numerical procedures for image processing, such as image denoising or compression, or for the simulation of PDE's  greatly benefit from economical and faithful approximations of such functions.
A piecewise polynomial approximation on a uniform partition of the domain is generally not sufficient for these purposes. A first step toward adaptivity is to vary the size of the elements forming the partition
according to the local smoothness properties of the function. A very similar procedure,
often used in image processing, consists in retaining the largest terms in a wavelet
decomposition, such as displayed on Figure \ref{figEllTri0} (iii). A second step is to observe that a higher resolution is needed in the direction orthogonal to the curve of discontinuity than in the tangential direction, and to take advantage of this property by using an {\it anisotropic} partition of the domain. In the two dimensional cases, such partitions
are typically built from triangles of high aspect ratio aligned with the discontinuities, 
as displayed Figure \ref{figEllTri0} (iv) and Figure \ref{figInria}.

\begin{figure}
\centering
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/Triangle.pdf}
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/TriangleUnif.pdf}\\
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/Haar.pdf}
\includegraphics[height = 4cm,width = 4cm]{\pathPic/Cartoon/TriangleMeshed.pdf}
\caption{A piecewise smooth function (i), Uniform partition of the domain (ii), Partition associated to the adaptive approximation based on the largest coefficients
in the Haar wavelet basis (iii), Partition associated to an adaptive anisotropic finite element approximation (iv). (credit : G. Peyr\'e)\label{figEllTri0}}
\end{figure}

In the context of numerical PDE's, adaptivity also refers to the fact that
the computational mesh is not fixed in advance, but instead is dynamically
updated based on the available information on the exact solution
gained through the solution process. From a numerical point of view, 
such methods require more complex algorithms and more intricate
 data structures than their non-adaptive counterparts. 
From a theoretical point of view the analysis of these adaptive
algorithms, when it is possible, is generally involved. As a matter of fact, 
the improvement brought by adaptivity in terms of convergence
rate is rigorously established only for few systems of PDE's,
and in the case of {\it isotropic} finite element meshes. 
We refer to the survey paper \cite{Nochetto} for a complete overview
on these aspects adaptive in the case of elliptic equations.
We need to mention that these difficulties are 
exacerbated when anisotropic elements are used.
Several numerical mesh generation software such as \cite{FreeFem, Inria, A}, nevertheless
successfully use anisotropic adaptativity for the numerical simulation of PDE's,
as displayed for instance on Figure \ref{figInria}. From a numerical point of view, the improvement brought by these methods seems obvious compared to non-adaptive or adaptive isotropic methods. However, many aspects of the theoretical analysis of anisotropic methods remain open questions.\\

\begin{figure}
	\centering		
	\includegraphics[width=4.5cm,height=3cm]{\pathPic/SimuExt/AlauzetPlane.pdf}
	\hspace{1cm}
	\includegraphics[width=3.5cm,height=3cm]{\pathPic/SimuExt/AlauzetShock.pdf}
	\caption{Airflow around a supersonic plane, computed using a three dimensional highly anisotropic mesh. (credit : F. Alauzet \cite{A}.\label{figInria})}
\end{figure}

This thesis studies the problem of anisotropic mesh adaptation for the approximation of a {\it known} function, which may be regarded as a preliminary step for the analysis of anisotropic mesh adaptation for the numerical simulation of PDE's, but may also serve in other applications such as terrain data, surface and image processing.\\

Given a triangulation $\cT$ of a bounded polygonal domain $\Omega\subset\R^2$, and a fixed integer $k\geq 1$, we denote by $V_k(\cT)$ the space of finite elements of degree $k$ on $\cT$. The space $V_k(\cT)$ consists of all
%, potentially discontinuous, %continuous % almost everywhere bounded 
functions which coincide on each triangle $T\in \cT$ with a polynomial of total degree $k$
$$
V_k( \cT) := \{g\; ; \; g_{|T} \in \P_k,\; T \in \cT\}.
$$
The dimension of $V_k(\cT)$ is of the order $\cO(k^2 \#(\cT))$. %, and the elements of $V_k(\cT)$ can be efficiently manipulated numerically.
Given a function $f : \Omega \to \R$ and a triangulation $\cT$ of $\Omega$, 
the best approximation error of $f$ in $V_k(\cT)$ is defined by
\be
\label{eqApproxG}
e_\cT(f)_X := \inf_{g\in V_k(\cT)} \|f-g\|_X.
\ee
The letter $X$ indicates the norm or semi-norm in which the approximation error $\|f-g\|_X$ is measured. In this thesis we restrict our attention to the $L^p$ norm and the $W^{1,p}$ semi-norm, where $1\leq p \leq \infty$. They are defined as follows: 
$$
\|h\|_{L^p(\Omega)} := \left(\int_\Omega |h|^p\right)^{\frac 1 p} \stext{ and } |h|_{W^{1,p}(\Omega)} := \left(\int_\Omega |\nabla h|^p\right)^{\frac 1 p},
$$
with the standard modification when $p=\infty$. Note that when using the $W^{1,p}$ semi-norm,
we need to impose global continuity of $g$ in the above definition of $V_k(\cT)$.

The best approximation $g\in V_k(\cT)$ of $f$ can be exactly computed in the case of the $L^2$ norm or the $W^{1,2}$ (or $H^1$) semi-norm: $g$ is the orthogonal projection of $f$ onto $V_k(\cT)$ with respect to the scalar product associated to the norm of interest. In the case $p\neq 2$ of non hilbertian norms the best approximation of $f$ is generally hard to compute, but ``satisfactory'' approximations can be obtained by different methods. If the function is smooth (at least continuous), one may
use the standard Lagrange interpolant, while for non-smooth functions a 
quasi-interpolant operator is preferred, see Chapter \ref{chapApproxMet}.
More generally, if $P_{\cT}$ is any continuous projection operator from $X$ to $\cT$, 
it is easily seen that
for any $f\in X$, one has
\be
\label{stableproj}
 \|f-P_\cT f\|_X \leq Ce_\cT(f)_X,
 \ee
where $C:=1+\|P_\cT\|_{X\to X}$. The problem of approximating a function $f$ on a {\it given} triangulation $\cT$, using finite elements of degree $k$, is thus solved in good part.\\
 
In the context of adaptive approximation, the triangulation $\cT$ of the domain $\Omega$ is not fixed, but can be freely chosen depending on the function $f$ (in contrast we always assume in this thesis 
that the integer $k$ is fixed although arbitrary). This naturally raises the objective of characterizing and constructing an optimal mesh for a given function $f$. Given a norm $X$ of interest
and a function $f$ to be approximated, we formulate the problem of {\it optimal mesh adaptation}, as 
minimizing the approximation error over all triangulations of {\it prescribed cardinality}. We therefore
define the adaptive best approximation error by
\be
\label{eqApproxT}
e_N(f)_X := \inf_{\#(\cT) \leq N} e_\cT(f)_X=\inf_{\#(\cT) \leq N}\inf_{g\in V_k(\cT)} \|f-g\|_X.
\ee
In contrast to the procedure of best finite element approximation on a fixed mesh, adaptive and anisotropic approximation is not yet well understood. In particular (i) {\it how does the optimal
mesh depend on the function} $f$ and (ii) {\it how does the optimal error $e_N(f)_X$ decay
as $N$ grows} ? These problems are well understood is the isotropic setting, 
for which the optimization is restricted to triangulations for which all triangles satisfy a uniform shape constraint
$$
\diam(T)^2\leq C |T|
$$
where $h_T$ and $|T|$ stand for the diameter and area of $T$ respectively, and $C>0$ is a fixed constant. In the general setting of potentially anisotropic triangulations, 
they are open problems.

Heuristically, the simplicity of \iref{eqApproxG} comparatively to \iref{eqApproxT} is due to the fact that the optimization is posed on the linear space $V_k(\cT)$,
and that a near best solution may therefore be obtained by applying to $f$ a 
stable projection operator as expressed by \iref{stableproj}.
In contrast the optimization problem \iref{eqApproxT} is posed on the {\it union} of
spaces $V_k(\cT)$ for all triangulations $\cT$ satisfying $\#(\cT)\leq N$, which is certainly not a linear space. This problem is therefore an instance of {\it nonlinear approximation}. Other instances
include best $N$-terms approximations in a dictionary of functions, best approximation by rational function. We refer to \cite{De} for a survey on nonlinear approximation.\\

The purpose of this thesis is to better understand optimal
mesh adaptation posed on the {\it full class of potentially anisotropic triangulations}. 
The four parts of the thesis are respectively devoted to the four questions below: 
%Each part 
%We discuss this problem through four different questions, which reflect four different point of views, a
%The four parts of this thesis are devoted the following questions, which are also discussed in more detail in the second half of this introduction. 
%We have addressed in particular the following questions:
%\begin{enumerate}[$\bullet$]
\begin{enumerate}[I.]
\item 
How does the approximation error $e_N(f)_X$ behaves in the asymptotic regime
when the number of triangles $N$ grows to $+\infty$, when $f$ is
a smooth function ? In that context, we establish mathematical characterization
of the optimal mesh, as well as sharp estimates of $e_N(f)_X$ by above and below
in terms of $N$ and quantities that depend {\it nonlinearly} on the derivatives of $f$.
\item 
Which classes of functions govern the rate of decay of $e_N(f)_X$ as $N$ grows,
and are in that sense naturally tied to the problem of optimal mesh adaptation? 
In particular, we have in mind the model of the so-called {\it cartoon functions},
which by definition are smooth except along a collection of smooth curves of discontinuity.
This is a popular image model in the image processing community (see for instance
Figure \ref{figEllTri0} for an instance of a cartoon image). We shall see that such a model 
naturally fits in a richer function class corresponding to a given rate of decay of $e_N(f)_X$ ?
\item 
Could the optimization problem \iref{eqApproxT} posed on triangulations 
$\cT$ of a given cardinality $N$, be replaced by an equivalent more tractable problem ?
Triangulations are indeed discrete combinatorial objects, described in terms of points and edges, 
which is not handy when solving optimization problems of the form \iref{eqApproxT}. 
We study the correspondence between certain classes of triangulations and of 
{\it riemanninan metrics} which in contrast are continuous objects. This allows us to reformulate 
and to solve the original optimization problem as a more tractable problem posed on the
set of riemannian metrics. %of the family of \iref{eqApproxT}.
\item 
Is it possible to produce a near-optimal sequence of triangulations $(\cT_N)_{N \geq _0}$ with
$\#(\cT_N)=N$, using a {\it hierarchical refinement procedure}? The property
of hierarchy guarantees the inclusion of the associated finite element spaces $V_k(\cT_N) \subset V_k(\cT_{N+1})$. It is required in applications such as progressive encoding or online
data processing. We provide with a simple and explicit algorithm 
which gives a positive answer to this question under some conditions.
\end{enumerate}

\subsection{State of the art}

Before detailing the content of the thesis, we
give in this section a short overview of the state of the art on both problems
of the study of $e_N(f)_X$ as $N$ grows,
and the construction of a near-optimal triangulation. For that purpose we need to introduce some notations.
We assume in the following that $f\in C^0(\overline \Omega)$, where $\Omega \subset \R^2$ is a bounded polygonal domain and $\overline \Omega$ denotes the closure of $\Omega$. For each triangulation $\cT$ of $\Omega$ we denote by $\interp^k_\cT$ the standard interpolation operator on Lagrange finite elements of degree $k$ on $\cT$: on each triangle $T\in\cT$
the interpolation $\interp^k_\cT f$ is the unique element of $\P_k$ which agrees with
$f$ on the points of barycentric coordinates in $\{0,\frac 1 k,\cdots,\frac {k-1} k,1\}$.
In the case $k=1$, these points are simply the three vertices of $T$.
If the triangulation $\cT$ is conforming (each edge of a triangle is either on the boundary
of $\Omega$ or coincides with the entire edge of another triangle), then $\interp_\cT^k f$ is continuous. In order to be consistent with the rest of this thesis we define $m := k+1\geq 2$, and we thus have 
$$
e_\cT(f)_{L^p} \leq \|f-\interp_\cT^{m-1} f\|_{L^p(\Omega)} \stext{ and } e_\cT(f)_{W^{1,p}} \leq  \|\nabla f-\nabla \interp_\cT^{m-1} f\|_{L^p(\Omega)}.
$$
Any estimate on the interpolation error thus automatically yields an upper estimate on the best approximation error $e_\cT(f)_X$. Furthermore if $f$ is sufficiently smooth and if $\cT$ is sufficiently fine, then these quantities are generally comparable.\\

One of the founding results of adaptive anisotropic finite element approximation deals with
the case of piecewise linear elements ($m=2$) with the error measured in the $L^p$ norm, see \cite{CSX} or Chapter \ref{chapOptAniso}. This result may be stated as follows: for any bounded polygonal domain $\Omega\subset \R^2$, for any $1 \leq p < \infty$, and for any function $f\in C^2(\overline \Omega)$ there exists a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N) \leq N$, and such that 
\be
\label{eqCSX}
\limsup_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \leq C \left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)},
\ee
where the exponent $\tau \in (0, \infty)$ is defined by 
$$
\frac 1 \tau := 1 + \frac 1 p\, ,
$$ 
and $C$ is a universal constant ($C$ is independent of $p$, $\Omega$ and $f$).
We recall that the upper limit of a sequence $(u_N)_{N \geq N_0}$ is defined by %one has
\be
\label{defLimSup}
\limsup_{N \to \infty} u_N := \lim_{N \to \infty} \sup_{n \geq N} u_n,
\ee
and is in general strictly smaller than the supremum $\sup_{N\geq N_0} u_n$. It is still an open question to find an appropriate upper bound for $\sup_{N\geq N_0} \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)}$ when optimally adapted anisotropic partitions are used.
The result \iref{eqCSX} can be extended to the exponent $p=\infty$, and to simplicial partitions
of domains $\Omega$ of higher dimension, but the meshes $\cT_N$ may then not be conforming.

The result \iref{eqCSX} reveals that the accuracy of the approximation to $f$ is governed by the quantity $\sqrt{|\det(d^2 f)|}$, which depends non-linearly on the hessian matrix $d^2 f$. This non-linear dependency is heavily tied to the fact that we authorize triangles of potentially highly anisotropic shape. The estimate \iref{eqCSX} is obtained by producing sufficiently fine triangulations which combine the two following heuristical properties:
\begin{enumerate}[a)]
\item {\it Error equidistribution:} the contribution 
$\|f-\interp_T^{m-1}f\|_{L^p(T)}$ of each triangle $T \in \cT_N$ to the global interpolation error $\|f-\interp_{\cT_N}^{m-1}f\|_{L^p(\Omega)}$ is approximately the same. This condition can be translated into a local constraint on the area of the triangles, which is dictated by the local behavior of $f$ and in particular by $\det(d^2f(z))$.
\item {\it Optimal shape of the triangles:} the aspect ratio and the orientation of a triangle $T$ 
is dictated by the ratio of eigenvalues and by the eigenvectors 
of the hessian matrix $d^2f(z)$ for $z\in T$.
\end{enumerate}

The simplest method for producing a sequence $(\cT_N)_{N \geq N_0}$ 
of triangulations satisfying \iref{eqCSX} is to use a ``local patching strategy'' 
that may be intuitively described as follows. In a first step the domain $\Omega$ is split into regions $\Omega_i$, $1\leq i \leq k$, sufficiently small so that the hessian matrix $d^2f(z)$ varies little
on each $\Omega_i$ around an average value $M_i$.
In other words $f$ is well approximated by a quadratic polynomial on each $\Omega_i$. 
Each region $\Omega_i$ is then tiled using a uniform triangulation $\cT_N^i$ with 
aspect ratio based on $M_i$, and the triangulations $\cT_N^i$ of $\Omega_i$ are glued together into a triangulation $\cT_N$ of $\Omega$, at the price of a few additional triangles at the interfaces between 
the $\Omega_i$. 

\begin{figure}
	\centering
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/NonConformTiling.pdf}
		\hspace{1cm}
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/ConformTiling.pdf}
		\hspace{1cm}
		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/TriangleClasses.pdf}
	\caption{\label{figLocPatch} Illustration of the local patching strategy : the elements of a macro triangulation $\cR$ are covered by periodic tilings, which are then glued together.}
\end{figure}

This construction, which is illustrated on Figure \ref{figLocPatch} is sufficient for the purpose of
proving the asymptotical result \iref{eqCSX} but not for practical applications since it only becomes efficient for a large number of triangles. The following approach, based on riemannian metrics, is often preferred in applications.
We assume for simplicity that the hessian matrix $M(z) := d^2f(z)$ is positive definite for each $z\in \Omega$, and we define 
\be
\label{defHHessian}
H(z) := \lambda^2 (\det M(z))^{-\frac 1 {2p+2}} M(z)
\ee
where $\lambda>0$ is a constant which role is to control the resolution of the
triangulation. Such a map $H$ is called a riemannian metric, and continuously associates to each point $z\in \Omega$ a symmetric positive definite matrix $H(z)$. Note that for each $z\in \Omega$ the matrix $H(z)$ defines an ellipse
$$
\cE_z := \{u \sep u^\trans H(z) u\leq 1\}.
$$ 
As illustrated on the left part of Figure \ref{figEllTri}, a metric encodes at each point $z\in \Omega$ an information of area, aspect ratio and orientation, under the form of a symmetric positive definite matrix $H(z)$, or equivalently of an ellipse $\cE_z$. 
Several mesh generation algorithms, such as \cite{FreeFem,Inria} are able to produce a triangulation adapted to a given metric $z\mapsto H(z)$ in the sense for each $z\in \Omega$ the triangle $T\in \cT$ containing $z$ has a shape ``similar'' to the ellipse $\cE_z$  as illustrated on the right part of Figure \ref{figEllTri}.
In mathematical terms, this means that one has for each triangle $T$ and $z\in T$,
\be
\label{triellipse}
b_T+c_1 \cE_z\subset T \subset b_T+c_2 \cE_z,
\ee
where $0<c_1<c_2$ are fixed constants and $b_T$ is the barycenter of $T$,
or equivalently that $T$ is ``close'' to an equilateral 
triangle of unit area in the metric $H(z)$,
If $\cT$ is such a triangulation and if $\lambda$ is sufficiently large, a heuristic argument 
(which will be recalled in Chapter \ref{chapOptAniso}) shows that 
$$
\#(\cT) \|f-\interp_{\cT}^1 f\|_{L^p(\Omega)} \leq C \|\sqrt{|\det (d^2f)|}\|_{L^\tau(\Omega)},
$$
where the constant $C$ depends on $c_1$ and $c_2$.

Varying the parameter $\lambda$ we obtain different triangulations $\cT_\lambda$, of cardinality proportional to $\lambda$, which leads to the error estimate \iref{eqCSX}.
The production of the mesh $\cT$ from the metric $H$ is not straightforward. In
addition,  there exists no rigorous proof that
the similarity condition \iref{triellipse} is achieved for most mesh generation algorithms,
to the notable exception of \cite{Shew} and \cite{Bois}.\\

\begin{figure}
\centering
\includegraphics[height = 4cm,width = 8cm]{\pathPic/Ellipses/EllShewChuk.pdf}
\caption{A metric and an adapted triangulation, (credit : J. Schoen)\label{figEllTri}}
\end{figure}

The approximation result \iref{eqCSX} is proved to be optimal if we restrict our attention to triangulations
which satisfy a technical condition defined as follows. %provided the following technical condition is satisfied.
We say that a sequence $(\cT_N)_{N \geq N_0}$ of triangulations of a polygonal domain $\Omega \subset \R^2$ is admissible if  $\#(\cT_N) \leq N$ and if 
\be
\label{defAdmiIntro}
\sup_{N \geq N_0} \left(\sqrt N \max_{T \in \cT_N} \diam(T)\right) <\infty.
\ee
For any admissible sequence $(\cT_N)_{N \geq N_0}$ of triangulations of a $\Omega$, one can establish the lower bound 
\be
\label{eqCSXOpt}
\liminf_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \geq c \left\| \sqrt{|\det (d^2f)|}\right\|_{L^\tau(\Omega)},
\ee
where the constant $c>0$ is universal (see also Theorem \ref{thLowerLPIntro} in the outline
of the thesis below). % Therefore \iref{eqCSX} is optimal if we restrict our attention to admissible 
Furthermore the admissibility condition is not too restrictive : for each $\ve>0$ there exists an admissible sequence of triangulations $(\cT_N)_{N \geq N_0}$ which satisfies the upper estimate \iref{eqCSX} up to the additive constant $\ve$ in the right hand side.\\

Similar results to \iref{eqCSX} and \iref{eqCSXOpt} can be developed for isotropic meshes, in which the triangles may vary in size but are constrained to be isotropic in the sense that the measure of degeneracy $\rho(T) := \diam(T)^2/|T|$ is uniformly bounded by a constant $\rho_0$, see for instance \cite{CMi2}. In that case the counterpart to  \iref{eqCSX} has the form
\be
\label{eqCSXiso}
\limsup_{N\to \infty} N \|f-\interp^1_{\cT_N} f\|_{L^p(\Omega)} \leq C \| d^2f\|_{L^\tau(\Omega)},
\ee
for the same value of $\tau$ and similarly for the counterpart to \iref{eqCSXOpt}, with
with constants $c$ and $C$ that depend on the bound $\rho_0$ on the measure of degeneracy, see for instance \cite{CMi2}. Therefore the 
nonlinear quantity
$\sqrt{|\det (d^2f)|}$ is replaced by
the linear $d^2f$ in the $L^\tau$ norm, and these results are now very similar
to those of best $N$-term wavelet approximation \cite{Co}.

In terms of the eigenvalues $\lambda_1(z), \lambda_2(z)$ of the symmetric matrix $d^2 f(z)$ we thus replace the geometric mean $\sqrt{|\lambda_1(z) \lambda_2(z)|}$ by $\max \{|\lambda_1(z)|, |\lambda_2(z)|\}$ which may be significantly larger when these eigenvalue have different order 
of magnitude. This is typically the case if the approximated function $f$ exhibit strongly anisotropic features, and therefore we may expect significant improvement when using anisotropic meshes
for such functions.\\ % in certain regions.

The result \iref{eqCSX} gives a sharp account of the improvement that anisotropic triangulations can provide compared to isotropic triangulation, under certain conditions. 
We have attempted to list these restrictions and to eliminate them when possible.
The four following conditions are the object of an in depth study in this thesis and could be eliminated, at least partly.
\begin{enumerate}[I.]
\item The original result only applies to piecewise linear interpolation error measured in the $L^p$ norm, while higher order finite elements and Sobolev $W^{1,p}$ norms are equally relevant.
\item The approximated function $f$ needs to be $C^2$, while the most interesting applications of adaptive approximation involve non smooth and even discontinuous functions, such as those appearing in Figures \ref{figEllTri0} and \ref{figInria}.
\item Most numerical applications of the this result use Riemannian metrics as an intermediate tool for mesh generation, but this approach lacks a precise equivalence result between these continuous objects and the different classes of anisotropic triangulations.
\item The known anisotropic mesh generation algorithms cannot be adapted to produce hierarchical sequences of triangles. % - either based on riemannian metrics, the local patching  are not compatible with The mesh generation algorithms gen
\end{enumerate}

We also need to mention two fundamental issues with this result which are discussed in this thesis but could not be eliminated. The suppression of these restrictions will be the subject of future research. First the error estimate \iref{eqCSX} only gives asymptotical information, as the number of triangles $N$ tends to $\infty$, while an error estimate valid for all values of $N$ is highly desirable. Second the extension of this result to functions defined on domains of dimension higher than two is hindered by a difficult problem of computational geometry : the production of {\it anisotropic and conforming meshes} in dimension $3$ or higher. This problem is addressed by some numerical methods such as \cite{Inria} but not solved from a theoretical point of view.



\section{Outline of the thesis}
%\label{secIntro2}

This thesis is composed of four parts which attempt to solve four key issues, numbered I to IV, encountered in earlier results on adaptive and anisotropic finite element approximation.
These four parts, as well as the nine chapters composing them, are mostly self consistent and can be read independently.

\subsection{Finite elements of arbitrary degree, and Sobolev norms} %Elements finis de plus haut degré, normes de Sobolev}%Premier objectif : que peut-on faire de mieux, asymptotiquement?}
\label{subsecOptAnisoIntro}

We extend in Part \ref{partAsymptApprox} the asymptotic estimate \iref{eqCSX} to finite elements of arbitrary degree, and to the family of Sobolev $W^{1,p}$ semi norms.\\

As a starter we consider in Chapter \ref{chapBlocks} partitions of a domain into rectangles aligned with the coordinate axes,  as illustrated on Figure \ref{figRectPart}, instead of triangles of arbitrary direction. Such partitions are relevant when the coordinate axes play a privileged role, in such way that the anisotropic features of the approximated function $f$ are likely to be aligned with the coordinate axes. 

The biggest advantage of this setting is that the mathematical technicalities required for the construction of an anisotropic partition of a domain, as well as the error analysis, is simplified by the presence of preferred directions. We thus take advantage of this simple setting to introduce and study two key concepts, named the {\it shape function} and the {\it local patching strategy} which are common to the analysis of the finite element approximation error on  triangulations. Our results apply to piecewise polynomials of arbitrary degree, when the approximation error is measured in the $L^p$ norm. We choose however in this introduction to insist on our results for adaptive anisotropic triangulations, since they are more striking in some sense and also more firmly tied to applications.\\

\begin{figure}
\centerline{
\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/CMrectsplit.pdf}
}
\caption{Anisotropic partitions of a domain into rectangles.\label{figRectPart}}
\end{figure}

Chapter \ref{chapOptAniso} is devoted to the extension of the asymptotically optimal error estimate \iref{eqCSX} to finite elements of arbitrary degree $m-1$, $m\geq 2$.
In order to present our results we need to introduce some notations.
We denote by $\H_m$ the space of homogeneous polynomials of degree $m$:
$$
\H_m := \Span\{x^k y^l \sep k+l = m\}.
$$
A key ingredient of our approach is the shape function $K_{m,p} : \H_m \to \R_+$, where $1\leq p\leq \infty$ is an exponent. 
This function is defined by an optimization of the $L^p$ interpolation error among the collection of triangles of unit area and of all possible shapes: for all $\pi\in \H_m$,
\be
\label{defKMPIntro}
K_{m,p}(\pi) := \inf_{|T| = 1} \|\pi-\interp_T^{m-1} \pi\|_{L^p(T)}.
\ee
Our main result is the following asymptotic error estimate.
\begin{theoremIntro}
\label{thOptiLPIntro}
Let $\Omega\subset \R^2$ be a bounded polygonal domain, let $f\in C^m(\overline \Omega)$ and let  $1\leq p < \infty$.
There exists a sequence $(\cT_N)_{N \geq N_0}$, $\#(\cT_N) \leq N$, of conforming triangulations of $\Omega$ such that 
\be
\label{eqLPIntro}
\limsup_{N \to \infty} N^{\frac m 2}\|f-\interp_{\cT_N}^{m-1} f\|_{L^p(\Omega)} \leq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)}
\ee
where the exponent $\tau \in (0, \infty)$ is defined by $\frac 1 \tau := \frac m 2 + \frac 1 p$.
\end{theoremIntro}

In the error estimate \iref{eqLPIntro}, we identify the collection $d^m f(z)$ of derivatives of order $m$ of $f$ at the point $z\in \Omega$ to the corresponding homogeneous polynomial in the Taylor development of $f$ at $z$. In mathematical form %other words
$$
\frac {d^m f(z)}{m!} \sim \sum_{k+l = m} \frac{\partial^m f}{\partial^k x\, \partial^l y}(z) \, \frac {x^k}{k!} \frac {y^l}{l!}.
$$

Theorem \ref{thOptiLPIntro} extends the known result \iref{eqCSX} to finite elements of arbitrary degree $m-1$. The quality of the adaptive and anisotropic approximation of $f$ is similarly determined by a non-linear quantity of its derivatives: the shape function $K_{m,p}(d^m f(z))$ is the ``generalization'' of the determinant $\sqrt{|\det (d^2f(z))|}$ appearing in \iref{eqCSX} to derivatives of arbitrary order.

%In the case of isotropic triangulations, in which the measure of non degeneracy $\rho(T) := \diam(T)^2/|T|$ is uniformly bounded among all triangles $T\in \cT_N$, $N \geq N_0$, by a given constant $\rho_0$, the nonlinear quantity $K_{m,p}(\frac {d^m f(z)} {m!})$ of the m-th derivatives needs to be replaced by the larger quantity $\|d^mf(z)\|$. The improvement due to anisotropy is thus expressed through the shape function $K_{m,p}$, at least for an asymptotically large number of triangles.

This remark raises the need for an in depth study of the shape function $K_{m,p}$. For $m=2$ we have established that $K_{2,p}(\pi)$ is proportional to the square root of the determinant of the quadratic polynomial $\pi = a x^2 + 2 b xy + cy^2\in \H^2$:
$$
K_{2,p}(\pi) = c_{2,p}(\det \pi) \sqrt{|\det \pi|} = c_{2,p}(ac-b^2)\sqrt {|ac-b^2|},
$$
where the constant $c_{2,p}(s)>0$ only depends on the sign of $s$. We thus recover the earlier result \iref{eqCSX}.
For $m=3$, the shape function $K_{3,p}$ is the fourth root of the discriminant of the homogenous cubic polynomial $\pi = a x^3+3bx^2y+3cxy^2+dy^3\in \H_3$:
$$
K_{3,p}(\pi) = c_{3,p}(\disc \pi) \sqrt{|\disc \pi|} = c_{3,p}(\disc \pi)\sqrt {|4(ac-b^2)(bd-c^2) - (ad-bc)^2|},
$$
where the constant $c_{3,p}(s)>0$ only depends on the sign of $s$. For larger values $m\geq 4$ we have not obtained an explicit expression of the shape function $K_{m,p}$, but an explicit quantity uniformly equivalent to this function. This equivalent has the following form : there exists a polynomial $Q_m(a_0, \cdots, a_m)$ of the $m+1$ variables $a_0, \cdots, a_m$ and a constant $C_m>0$ such that for all $\pi = a_0 x^m+ a_1 x^{m-1}y+ \cdots a_m y^m\in \H_m$ one has with $r_m := \deg Q_m$,
\be
\label{equivKQ}
C_m^{-1} \sqrt[r_m]{Q_m(a_0, \cdots , a_m)} \leq K_{m,p}(\pi) \leq  C_m\sqrt[r_m]{Q_m(a_0, \cdots , a_m)}.
\ee
The polynomial $Q_m$ is obtained using the theory of invariant polynomials developed by Hilbert in \cite{Hilbert}. We also characterise the vanishing of the shape function, and thus %the polynomials $\pi\in \H_m$ on which the function $K_{m,p}$ vanishes, and thus 
the possible cases of ``super-convergence'' : $K_{m,p}(\pi)=0$ if and only if $\pi$ has a linear factor $ax+by$ of multiplicity $s>m/2$, in other words the homogeneous polynomial $\pi$ is sufficiently degenerated.\\

The proof of theorem \ref{thOptiLPIntro} is based on a ``local patching strategy'', a two scale mesh generation procedure which proceeds as follows: we consider a first triangulation $\cR$ of the polygonal domain $\Omega$ which is sufficiently fine in such way that the derivatives of order $m$ of $f$ vary little on each triangle $R\in \cR$ around an average value denoted by $\pi_R\in \H_m$. To each polynomial $\pi_R$, $R\in \cR$, we then associate a triangle $T_R$ which is a minimizer, or a near minimizer, of the optimization problem defining $K_{m,p}(\pi_R)$. We then tile each $R\in \cR$ using the triangle $T_R$ a properly scaled and its symmetric with respect to the origin. Eventually, as illustrated on Figure \ref{figLocPatch} the triangulation $\cT_N$ is obtained by gluing together the periodic tilings on each $R\in \cR$, with a few additional triangles in order obtain a globally conforming mesh.\\

%\begin{figure}
%	\centering
%		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/NonConformTiling.pdf}
%		\hspace{1cm}
%		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/ConformTiling.pdf}
%		\hspace{1cm}
%		\includegraphics[width=4cm,height=4cm]{\pathPic/PaperOptAniso/TriangleClasses.pdf}
%	\caption{\label{figLocPatch} Illustration of the local patching strategy : the elements of a macro triangulation $\cR$ are covered by periodic tilings, which are then glued together.}
%\end{figure}

The next theorem establishes that the asymptotic error estimate \iref{eqLPIntro} is sharp, at least if we restrict our attention to admissible sequences of triangulations, a condition defined in \iref{defAdmiIntro}. The approximation result \iref{eqLPEpsIntro} establishes furthermore that the admissibility condition is not too restrictive.

\begin{theoremIntro}
\label{thLowerLPIntro}
Let  $\Omega\subset \R^2$ be a bounded polygonal domain, let $f\in C^m(\overline \Omega)$ and let $1\leq p\leq \infty$.
Let $(\cT_N)_{N \geq N_0}$, $\#(\cT_N) \leq N$, be an admissible sequence of triangulations of $\Omega$. Then
\be
\label{eqLPLowerIntro}
\liminf_{N \to \infty} N^{\frac m 2} \|f-\interp_{\cT_N}^{m-1} f\|_{L^p(\Omega)} \geq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)},
\ee
where  $\frac 1 \tau := \frac m 2 + \frac 1 p$. Furthermore for any $\ve>0$ there exists an admissible sequence $(\cT_N^\ve)_{N \geq N_0}$ of triangulations of $\Omega$, satisfying $\#(\cT_N^\ve) \leq N$, and such that: 
\be
\label{eqLPEpsIntro}
\limsup_{N \to \infty} N^{\frac m 2} \|f-\interp_{\cT^\ve_N}^{m-1} f\|_{L^p(\Omega)} \geq \left\|K_{m,p}\left(\frac{d^m f}{m!}\right) \right\|_{L^\tau(\Omega)}.
\ee
\end{theoremIntro}

Chapter \ref{chapW1P} is devoted to counterparts of Theorems \ref{thOptiLPIntro} and \ref{thLowerLPIntro} when the interpolation error is measured in the Sobolev $W^{1,p}$ semi-norms, $1\leq p < \infty$. These estimates involve the counterpart $L_{m,p} : \H_m \to \R_+$ of the shape function $K_{m,p}$ which is defined as follows: for all $\pi \in \H_m$ 
$$
L_{m,p}(\pi) := \inf_{|T|=1} \|\nabla (\pi-\interp_T^{m-1} \pi)\|_{L^p(T)}.
$$
%and the exponent $\tau$ becomes $\frac 1 \tau := \frac {m-1} 2+ \frac 1 p$.
We also provide some explicit equivalents of $L_{m,p}(\pi)$, defined similarly to \iref{equivKQ} by an algebraic expression in the coefficients of $\pi\in \H_m$.
Our results for the $W^{1,p}$ semi-norm are thus extremely similar to the results obtained for the $L^p$ norm.
The adaptation of the proofs however is not straightforward, due to the following new phenomenon: the presence of ``flat'', strongly obtuse, triangles in a meshes may cause the gradient of the interpolated function to oscillate, as illustrated in Figure \ref{figParaAO}. This phenomenon deteriorates the interpolation error in the $W^{1,p}$ semi-norm, but not in the $L^p$ norm, these ``flat'' triangles therefore need to be carefully avoided. 

Before turning to description of the rest of this thesis we recall to the reader that the three chapters composing Part \ref{partAsymptApprox} are self consistent and can be read independently.

\begin{figure}
\centerline{
\includegraphics[width=5cm,height=4cm]{\pathPic/Triangles/ParaboleAigue.pdf}
\includegraphics[width=5cm,height=4cm]{\pathPic/Triangles/ParaboleObtuse.pdf}
}
\caption{Interpolation of a bi-dimensional parabolic function on a mesh built of acute or ``flat'', strongly obtuse, triangles.\label{figParaAO}}
\end{figure}

\subsection{Anisotropic smoothness classes and image models}

There exists various ways of measuring the smoothness of functions on a domain $\Omega\subset \R^2$, generally through the definition of an {\it appropriate smoothness} space and an associated norm. Classical instances are Sobolev and Besov spaces. Such spaces  are of common use when describing the regularity of solutions to partial differential equations. From a numerical perspective they are also useful in order to sharply characterize at which rate a function $f$ may be approximated by simpler functions such as Fourier series, finite elements (on isotropic triangulations), splines or wavelets.

%Functions arising in concrete applications, for instance in image processing or in the solution of hyperbolic PDEs, often %may have inhomogeneous smoothness properties, in the sense that they 
%exhibit areas of smoothness separated by local discontinuities.
%The smoothness space that is best taylored to take these features into account is the space $BV$ of functions of bounded variation. 
%This space consists of those $f\in L^1(\Omega)$ such that $\nabla f$ is a bounded measure, i.e. such that their total variation 
%$$
%\TV(f) = |f|_{BV} := \max\left\{\int_\Omega f \diver \vp \sep \vp\in \cD(\Omega), \|\vp\|_{L^\infty} \leq 1\right\}.
%$$
%is finite. Assume that $\Omega := ]0,1[^2$ is the unit square, and denote by $f_N$ the approximation of $f$ by the $N$ terms of its development on the Haar basis which correspond to the largest coefficients. It is established in \cite{CDPX, CDDD2} that 
%\be
%\label{eqApproxTV}
%\sup_{N \geq 0} \sqrt N \|f-f_N\|_{L^2(\Omega)} \leq C \TV(f).
%\ee

The result of adaptive anisotropic approximation \iref{eqCSX} and its generalisation Theorem \ref{thOptiLPIntro} establish that the quality of the approximation of a function $f$ by finite elements on anisotropic triangulations is governed by a non-linear quantities of the derivatives of $f$, at least from an asymptotical point of view.
In the case of finite elements of degree $1$, and of the approximation in $L^2$ norm, the relevant quantity is the following
$$
A(f) := \left\|\sqrt {|\det(d^2f)|}\right\|_{L^{2/3}(\Omega)}.
$$
The functional $A$ strongly differs from the total variation $\TV$, and also from the Sobolev, Holder or Besov norms, because of its nonlinear behavior: $A$ does not satisfy the triangle inequality, or any quasi-triangle inequality. In other words for any constant $C$ there exists $f,g\in C^2(\overline \Omega)$ such that 
\be
\label{eqNoTri}
A(f+g) \not \leq C(A(f)+A(g)).
\ee
%Contrary to the total variation $\TV$, the functional $A$ is not a priori attached to an smoothness space. If such a space exists then the \iref{eqNoTri} 
The lack of a triangular inequality forbids to use the classical techniques of linear analysis to define a smoothness space attached to the functional $A$.\\ %Another problem comes from the limit appearing in \iref{eqApproxA}, which not present in classical approximation theory. %, see for instance \iref{eqApproxTV}. %(A naive attempt to define an approximation space associated to the functional $A$ is nevertheless presented in Chapter \ref{chapApproxMet}.)

Functions arising in concrete applications, for instance in image processing or in the solution of hyperbolic PDEs, often %may have inhomogeneous smoothness properties, in the sense that they 
exhibit areas of smoothness separated by local discontinuities.
%These applications therefore require that results of the type of \iref{eqApproxA} be extended to non smooth functions and in particular to the class of cartoon functions illustrated on Figure \ref{figEllTri0}, which are smooth except for a jump discontinuity accross collection of smooth curves.
A heuristical analysis presented in Chapter \ref{chapCartoon} suggests that for any cartoon function $f$ defined on a bounded polygonal domain $\Omega$, there exists a sequence $(\cT_N)_{N \geq N_0}$ of anisotropic triangulations of $\Omega$, satisfying $\#(\cT_N)\leq N$, and such that 
\be
\label{eqApproxCartoon}
\sup_{N\geq N_0} N \|f-\interp_{\cT_N}^1 f\|_{L^2(\Omega)} < \infty. % \text{ est borné, \quad où } r_p := \min\left\{1, \frac 2 p\right\}.
\ee
As illustrated on Figure \ref{figEllTri0}, the triangulations $(\cT_N)_{N \geq N_0}$ combine highly anisotropic triangles aligned with the discontinuities of $f$, and large triangles in the regions where $f$ is smooth.
%The compact form of this estimate hides the balance between to different phenomena in the approximation of $f$, each of them requiring approximately half of the cardinality of $\cT_N$. First the function $f$ is approximated by the linear interpolant $\interp_{\cT_N}^1 f$ on the regions where $f$ is smooth. Second the collection $\Gamma$ of curves along which $f$ is discontinuous is approximated by the boundaries $\partial T$, of the triangles $T\in \cT_N$. The difference $f-\interp_{\cT_N}^1 f$ does not tend to zero on the neighborhood of $\Gamma$, but the width of this neighborhood tends to $0$.
The approximation result \iref{eqApproxCartoon} raises the hope that a precise and quantitative asymptotic error estimate for the adaptive anisotropic approximation of cartoon functions extends the known result 
\be
\label{eqApproxA}
\limsup_{N \to \infty} N \|f-\interp_{\cT_N}^1 f\|_{L^2(\Omega)} \leq C A(f),
\ee
which holds for all $C^2$ functions.

So far we have only fulfilled one part of this program: the extension of the functional $A$ to cartoon functions. More precisely, consider a radial and compactly supported function $\vp\in C^\infty(\R^2)$ of unit integral. 
For any $\delta>0$ we define $\vp_\delta(z) := \frac 1 {\delta^2} \vp\left(\frac z \delta\right)$ and we denote by $f_\delta := f*\vp_\delta$ the convolution of $f$ with $\vp_\delta$. 
We establish in Chapter \ref{chapCartoon} that $A(f_\delta)$ converges as $\delta \to 0$, to an explicit expression
\begin{eqnarray*}
\lim_{\delta \to 0} A(f_\delta)^{2/3} &=& \left\|\sqrt{|\det(d^2 f)|}\right\|_{L^{2/3}(\Omega\sm\Gamma)}^{2/3} + C(\vp) \left\|\sqrt{|\kappa|} \gamma\right\|_{L^{2/3}(\Gamma)}^{2/3}\\ %\left(\|\right)
&=& \int_{\Omega\sm\Gamma} \sqrt[3]{|\det (d^2 f(z))|}dz+ C(\vp)\int_\Gamma |\kappa(s)|^{1/3} |\gamma(s)|^{2/3}ds.
\end{eqnarray*} %\frac 1 3 \frac 2 3
In the previous equation, we denote by $\Gamma$ the collection of curves where the cartoon function $f$ is discontinuous, by $\gamma(s)$ the jump of $f$ at the point $s\in \Gamma$, and by $\kappa(s)$ the curvature of $\Gamma$ at $s$. The constant $C(\vp)$ is positive and explicit in terms of $\vp$.\\

The extension of the nonlinear functional $A$ to cartoon functions puts in light a link, explored in section \S\ref{secCartoon4}, 
between anisotropic finite element approximation and several other mathematical fields. We think in particular of affine invariant image processing \cite{Ca} and of the definition in \cite{DPW} of smoothness spaces through the regularity of the level lines of a function.\\

\begin{figure}
\centering
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Sina.pdf}
\hspace{1cm}
\includegraphics[height=4cm,width=4cm]{\pathPic/Bayesien/Staira.pdf}
\hspace{1cm}
\includegraphics[height=3cm,width=4cm]{\pathPic/Bayesien/Flowera.pdf}
\caption{Behavior of the functionals $\TV$ and $A$ on different types of images.\label{figTVA}}
\end{figure}

We also regard the quantity $A$ as a ``second order'' counter part of the total variation semi-norm $\TV$, a measure of smoothness defined in terms of the first derivatives which is also finite for all cartoon functions. The total variation plays a central role in image processing and in the analysis of transport equations, two domains in which piecewise smooth functions naturally appear. For any cartoon function $f$, the total variation $\TV(f)$ is given by the following formula  
$$
\TV(f) = \int_{\Omega\sm\Gamma} |\nabla f(z)|dz+\int_\Gamma |\gamma(s)| ds.
$$
We explore in \S\ref{secCartoon5.5} the behavior of the two quantities $A(f)$ and $\TV(f)$ for different families of cartoon functions $f$. It appears that $A(f)$ and $D(f)$ are equivalent when $f$ is a smoothly oscillating function $f(z) := \cos(\omega |z|)$ with large $\omega$, see figure \ref{figTVA} (i). In contrast the discontinuities are penalized in a different manner by these two functionals. For a staircase-like function, as illustrated on Figure \ref{figTVA}, the total variation remains bounded while $A$ tends to infinity as the number of steps grows, due contribution $|\gamma(s)|^{2/3}$ of the jump term. Furthermore, due to the curvature term $|\kappa(s)|^\frac 1 3$, $A$ is much larger than $\TV$ for characteristic functions of sets with a complex or oscillating boundary as illustrated in Figure \ref{figTVA}. 

The functional $A$ can thus be thought of as a new quantitative image model : a monochromatic image, described by a brightness function $f: [0,1]^2 \to [0,1]$, is plausible if $A(f)$ is sufficiently small. Generalising the work \cite{LMo} we explore an image recovery procedure using this model as a bayesian prior. \\

%Part \ref{partCartoon} consists of the single chapter, Chapter \ref{chapCartoon}, containing in particular the above result. The rest of this chapter is organized as follows.
%The extension of the nonlinear functional $A$ to cartoon functions puts in light a link, explored in section \S\ref{secCartoon4}, 
%between anisotropic finite element approximation and several other mathematical fields. We think in particular of affine invariant image processing \cite{Ca} and of the definition in \cite{DPW} of smoothness spaces through the regularity of the level lines of a function.
%The functional $A$ also can be thought of as a new quantitative image model : a monochromatic image, described by a brightness function $f: [0,1]^2 \to [0,1]$, is plausible if $A(f)$ is sufficiently small. Generalising the work \cite{LMo} we explore in section \S\ref{secCartoon5.5} an image recovery procedure using this model as a bayesian prior. 
Eventually we describe in section \S\ref{secCartoon6} the extension to cartoon functions of other non-linear quantities appearing in anisotropic finite element approximation such as the norm $\|K_{m,p}(d^m f)\|_{L^\tau}$ of the shape function for $m\geq 2$, or the counterpart of this quantitiy for functions $f$ of more than two variables.


\subsection{Mesh generation and riemannian metrics} %Génération de maillage et métriques riemanniennes} %Problèmes de génération de maillage}

Triangulations are discrete objects of combinatorial nature : they can be described by the collection of their vertices and of the edges between them. This description is fruitful for the demonstration of algebraic results such as the Euler formula, or for computer processing.

In contrasts, several works \cite{Shew,Bois,A} on anisotropic mesh adaptation choose in some contexts to replace triangulations of a domain $\Omega$ with a continuous equivalent object : a riemannian metric, in other words a continuous function $H$ from $\Omega$ to the set $S_2^+$ of symmetric positive definite matrices. Our purpose in Part \ref{partRiemann} is to give a theoretical background to this replacement, through the formulation of precise equivalence results between some classes of triangulations and of riemannian metrics. 
This equivalence translates some geometrical constraints satisfied by the triangulations into the form regularity properties of the equivalent riemannian metrics.\\

In order to state our results we need to introduce some notations. We associate to each triangle $T$ its barycenter $z_T\in R^2$ and the symmetric positive definite matrix $\cH_T\in S_2^+$ such that the ellipse $\cE_T$ defined by 
$$
\cE_T := \{z\in \R^2 \sep (z-z_T)^\trans \cH_T (z-z_T)\},
$$
is the ellipse of minimal area containing $T$. The point $z_T$ thus encodes the position of $T$, while the matrix $\cH_T\in S_2^+$ encodes the area, the aspect ratio and the orientation (but not the angles) of the triangle $T$ .

We denote by $\bT$ the collection of triangulations of the infinite domain $\R^2$ - the choice to consider infinite triangulations is guided by simplicity, and further work will be devoted to triangulations of bounded domains.
We denote by $\bH := C^0(\R^2, S_2^+)$ the collection of riemannian metrics on $\R^2$. A metric $H\in \bH$ continuously associates to each point $z\in \R^2$ a symmetric positive matrix $H(z)\in S_2^+$.
We say that a triangulation $\cT\in \bT$ is $C$-equivalent to a metric $H \in \bH$ if for all $T\in \cT$ and for all $z\in T$ we have 
$$
C^{-2} H(z) \leq \cH_T \leq C^2 H(z). 
$$
We say that a class of triangulations $\bT_*\subset \bT$ is equivalent to a class of metrics $\bH_*\subset \bH$ if there exists a uniform constant $C>0$ such that 
\begin{itemize}
\item For any triangulation $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C$-équivalent.
\item For any metric $H\in \bH_*$ there exists a triangulation $\cT\in \bT_*$ such that $\cT$ and $H$ are $C$-équivalent.\\
\end{itemize}

%The full class $\bT$ of all triangulations is not equivalent to the full class $\bH$ of all metrics. 
We consider in Part \ref{partRiemann} three particularly relevant classes of triangulation of $\R^2$
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}
$$
which have a minor dependency on a parameter $C\geq 1$. The constraints satisfied by these classes of triangulations of $\R^2$ are illustrated by some bounded triangulations on Figure \ref{figDisk}.
When $C$ is sufficiently large, these classes of triangulations are equivalent to three classes of metrics respectively 
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
We now turn to the description of these classes of triangulations and of metrics.
The class $\bT_{g,C}$ of \emph{graded} triangulations, is defined by the following condition which imposes a minimum of consistency among the shapes of neighbouring triangles. A triangulation $\cT$ belongs to $\bT_{g,C}$ if for all $T, T'\in \cT$ one has
$$
T \cap T' \neq \emptyset \quad \Ra \quad C^{-2} \cH_T \leq \cH_{T'} \leq C \cH_T.
$$
A triangulation $\cT$ belongs to the class $\bT_{i,C}$ of \emph{isotropic} triangulations if $\cT$ is graded, $\cT\in \bT_{g,C}$,
%(cette condition peut être supprimée, voir ??) 
and if the elements of $\cT$ are sufficiently close to the equilateral triangle, as expressed by the following condition: for all $T\in \cT$
$$
\|\cH_T\| \|\cH_T^{-1}\|\leq C^2.
$$
Eventually the class $\bT_{a,C}$ of \emph{quasi-acute} triangulations is defined by a slightly more technical condition on the maximal angles of the triangles, see Chapter \ref{chapMeshMet}. This condition guarantees the stability of the gradient of the interpolation of a function, but raises difficulties in terms of mesh generation which diminish the flexibility of use of quasi-acute triangulations in practical applications. One of our key results is the reformulation of this diminished flexibility under the form of a regularity assumption on an equivalent riemannian metric.\\

We establish in Chapter \ref{chapMeshMet} that when the constant $C$ is sufficiently large, the class $\bT_{i,C}$ of isotropic triangulations is equivalent to the class $\bH_i$ of metrics $H$ which are proportional to the identity
$
H(z) = \Id /s(z)^2 ,
$
and such that the proportionality factor $s$ satisfies one of the following \emph{equivalent} properties
\begin{enumerate}[$\bullet$]
\item Euclidean Lipschitz Property: $|s(z) - s(z')| \leq |z-z'|$ for all $z,z'\in \R^2.$
\item Riemannian Lipschitz Property: $|\ln s(z) - \ln s(z')| \leq d_H(z,z')$ for all $z,z'\in \R^2.$
\end{enumerate}
We recall that the riemannian distance $d_H(z,z')$ measures the length, distorted by the metric $H$, of the smallest path joining $z$ and $z'$. %, see Chapter \ref{chapMeshMet}.
$$
d_H(z,z') := \inf_{\substack{\gamma(0) = z\\ \gamma(1) = z'}} \int_0^1 \|\gamma'(t) \|_{H(\gamma(t))} dt
$$
where $\|u\|_M := \sqrt {u^\trans M u}$ and where the infimum is taken among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$.

The two lipschitz properties presented above have (non equivalent) natural extensions to general anisotropic riemannian metrics. They involve two distances $d_+$ and $d_\times$ on the collection $S_2^+$ of symmetric positive definite  riemannian metrics %, see ??
\begin{eqnarray}
\label{eqDPlusIntro}
d_+(H(z), H(z') ) & \leq & |z-z'| \stext{ for all } z,z'\in \R^2,\\
\label{eqDTimesIntro}
d_\times(H(z), H(z') ) & \leq &d_H(z,z') \stext{ for all } z,z'\in \R^2.
\end{eqnarray}

The main result of Chapter \ref{chapMeshMet} reformulates under the form of the above Lipschitz properties the flexibility offered by the class of graded triangulations $\bT_{g,C}$ and of quasi-acute triangulations $\bT_{a,C}$ - note that the latter is more rigid due to the angle constraint.
\begin{theoremIntro}
\label{thMeshMetIntro}
If the constant $C$ is sufficiently large, then the class $\bT_{g,C}$ of graded triangulations is equivalent to the class $\bH_g$ of metrics satisfying \iref{eqDTimesIntro}, and the class $\bT_{a,C}$ of quasi-acute triangulations is equivalent to the class $\bH_a$ of metrics satisfying simultaneously \iref{eqDTimesIntro} and \iref{eqDPlusIntro}.
\end{theoremIntro}

\begin{figure}
	\centering
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskIso.pdf}
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskAigu.pdf}
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskGen.pdf}
		\includegraphics[width=6cm,height=3.2cm]{\pathPic/CoucheLimite/DiskNoReg.pdf}
	\caption{\label{figDisk} Production of a Layer of simplices of width $\delta$ along the unit circle using $\delta^{-1}$ isotropic triangles (i), $\delta^{-\frac 1 2} |\ln \delta|$ ``quasi-acute'' triangles (ii), $\delta^{-\frac 1 2}$ triangles triangles satisfying (iii) or not (iv) the grading condition.}
\end{figure}

We give in Chapter \ref{chapApproxMet} some applications of these results to a in the context of approximation theory and of constrained mesh generation. Let us describe the latter example. 
For any closed set $E\subset \R^2$ and any mesh $\cT\in \bT$ we denote by $V_\cT(E)$ the neighborhood of $E$ in the triangulation $\cT$, which is defined as follows
$$
V_\cT(E) := \bigcup_{\substack{T\in \cT\\ T \cap E \neq \emptyset}} T.
$$
We say that a mesh $\cT$ separates two disjoint closed sets $X$ and $Y$ if $V_\cT(X) \cap V_\cT(Y) = \emptyset$. The counterpart for metrics of this property is the following : a metric $H\in \bH$ separates $X$ and $Y$ if $d_H(x,y)\geq 1$ for all $x\in X$ and $y\in Y$. Chapter \ref{chapApproxMet} shows that these two properties are rigorously equivalent, and uses this reformulation to compute the smallest number of triangles (up to periodicity) required for the separation of some sets using a (periodic) isotropic, quasi-acute or graded triangulation. As illustrated on Figure \ref{figDisk} putting more constraints on the triangulation raises the need of using more triangles to separate the  same sets.

\subsection{Hierarchical refinement  algorithms}

The last part of this thesis, Part \ref{partGreedy}, is devoted to the study an algorithm proposed by Cohen, Dyn and Hecht which produces hierarchical sequences $(\cT_N)_{N\geq N_0}$ of (non-conforming) anisotropic triangulations adapted to a given function $f$.
Given a triangulation $\cT$ of a domain $\Omega$ and a function $f\in L^p(\Omega)$, this algorithm creates in one step a triangulation $\cT'$ of $\Omega$, of cardinality $\#(\cT') = \#(\cT)+1$, proceeding as follows:
\begin{enumerate}
\item (Greedy triangle selection) A triangle $T\in \cT$ which has a maximal contribution to the error is selected 
$$
T := \argmax_{T'\in \cT} \|f-\cA_{T'} f\|_{L^p(T')},
$$
where $\cA_T : L^p(T) \to \P_1$ a projection operator, for instance the $L^2(T)$ orthogonal projection onto $\P_1$.
\item (Decision of a bisection)
The refinement procedure considers the three following bisection choices for the triangle $T$ : from the midpoint of an edge $e\in \{a,b,c\}$ of $T$ to the opposite vertex, creating the sub-triangles $T_e^1$ and $T_e^2$. The edge which minimizes a given decision function $d_T(e,f)$ is selected,  and we define 
$$
\cT' := \cT-\{T\} + \{T_e^1, T_e^2\}.
$$
\end{enumerate}
Starting from a triangulation $\cT_0$ of cardinality $N_0$ of the domain $\Omega$, the algorithm produces step after step a sequence $(\cT_N)_{N\geq N_0}$, see Figure \ref{figRefinement}, of triangulations ``adapted'' to a given function $f\in L^p(\Omega)$. The properties of these triangulations strongly depend on the approximated function $f$ and on the choice of the decision function $d_T(e,f)$, which guides the creation of anisotropy - in contrast the projection operator $\cA_T$ plays a rather minor role.

\begin{figure}
	\centering
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Algo1.pdf}
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Algo2.pdf}
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Algo3.pdf}
	\caption{\label{figRefinement}Refinement algorithm : selection of the triangle which maximizes the local approximation error (in blue), choice of a bisection among the three possibilities, repetition of these two steps until the refinement is sufficient.}
\end{figure}

We present this algorithm in more detail in Chapter \ref{chapCDHM}, and we prove the convergence of this algorithm
%a general convergence result for any bounded polygonal domain $\Omega$ and any $f\in L^p(\Omega)$, 
under some assumptions on the projection operator $\cA_T$ and the decision function $d_T(e,f)$.
Our main result, presented in Chapter \ref{chapBisecOpt}, states that when $f$ is a strictly convex $C^2$ function, for a particular choice \iref{eqDecisionL1} of the decision function, the sequence $(\cT_N)_{N\geq N_0}$ of triangulations generated by this algorithm satisfies the best possible asymptotic convergence estimate
$$
\limsup_{N \to \infty} N \| f-\cA_{\cT_N} f\|_{L^p(\Omega)} \leq C \|\sqrt{|\det (d^2f)|}\|_{L^\tau(\Omega)},
$$
where $\frac 1 \tau := 1+ \frac 1 p$ and where $\cA_\cT f$ denotes the piecewise linear function on $\Omega$ which coincides with $\cA_T f$ on each $T\in \cT$.\\

Eventually we study in Chapter \ref{chapVariations} some variants of the hierarchical refinement algorithm presented above. %, which is also referred to as the ``greedy algorithm''. 
More precisely we consider in section \S\ref{secAltDec} a decision function based on the $L^2$ approximation error, which is particularly well suited to the numerical implementation since it can be evaluated in small computing time.

We then focus in section \S\ref{secAltBi} on the approximation of cartoon functions. The original algorithm is not well suited to this context, and we therefore introduce and study some modifications of the bisection choices offered to the decision function.

Eventually we consider in section \S\ref{secGreedyRect} another variant of the algorithm, which is based on rectangles aligned with with the coordinate axes instead of triangles of arbitrary direction. This simplification leads to Theorem \ref{thRect} which guarantees the best possible convergence estimate for all $C^1$ functions, in the case of piecewise constant approximations on rectangles aligned with the coordinate axes.


==> Introduction/QuestionsRaised.tex <==

\subsection{Questions raised in this thesis and open questions}
The result \iref{eqCSX} gives a sharp account of the improvement that anisotropic triangulations can provide compared to isotropic triangulation, under certain conditions. 
We have attempted to list these restrictions and to eliminate them when possible.
The four conditions mentioned below are the object of an in depth study in this thesis and could be eliminated, at least partly.
\begin{enumerate}[I]
\item (Other degrees, other norms)
We extend in Chapter \ref{chapOptAniso} the estimate \iref{eqCSX} to finite elements of arbitrary degree $m-1$, and to the Sobolev $W^{1,p}$ norms.
 Comparatively, the original result only applies to piecewise linear finite elements $m-1= 1$ and to $L^p$ norms. We obtain asymptotical error estimates and optimality results which are similar to \iref{eqCSX} and \iref{eqCSXOpt}. The determinant of the hessian matrix $\det (d^2 f)$ appearing in the original estimate is replaced with an ``invariant polynomial'' applied to the collection $d^m f$ of the $m$-th derivatives of $f$.

\qquad The combination of the following properties guarantees that a triangulation $\cT$ satisfies the optimal error estimate up to a fixed multiplicative constant, see Chapter \ref{secW1P2} for more quantitative analysis of these properties. First the interpolation error needs to be equidistributed among all triangles $T\in \cT$. Second the triangles need to have an optimal shape, which is now dictated by the $m$-th order derivatives of $f$, instead of the hessian matrix. Third the triangulation needs to be sufficiently fine in such way that $f$ is well approximated on each triangle by a polynomial of degree $m$. In the case of Sobolev $W^{1,p}$ norms a fourth property needs to be satisfied : any angle $\theta$ of any triangle $T\in \cT$ should be sufficiently far away from the flat angle, in other words $\theta \leq\theta_{\rm max} < \cPi$.\\

\item (Non smooth functions) 
We consider in Chapter \ref{chapCartoon} the model of cartoon functions, which is popular in image processing. These function are smooth except along a finite collection of smooth curves where they have jump discontinuities.

\qquad Cartoon functions are not differentiable, and the quantity $\|\sqrt{|\det d^2f|}\|_{L^\tau}$ which appears in \iref{eqCSX} has therefore no a-priori meaning. We show nevertheless that for some values of $\tau$ this quantity has a natural extension to cartoon functions $f$, which includes a one-dimensional integral along the collection $\Gamma$ of curves where $f$ is discontinuous. This contribution takes into account the jump of $f$ across $\Gamma$ as well as the curvature of $\Gamma$. However the extension of the approximation result \iref{eqCSX} in that context remains so far a conjecture.\\

\item (Mesh generation)
The most popular methods for anisotropic mesh generation in applications are based on Riemannian metrics, as exposed in \iref{defHHessian}. These metrics encode at each point the desired size, aspect ratio and orientation of the triangles.

\qquad This raises the objective of defining and proving precise equivalence results between some classes of triangulations and of metrics. We answer this question in Chapter \ref{chapMeshMet}, which provides a translation of some geometrical properties of triangulations into regularity properties satisfied by the corresponding metrics. We pay a particular attention to the angle condition evoked in I for the approximation of function in the $W^{1,p}$ semi-norm, the fact that the angles appearing in the triangulation are uniformly bounded away from $\cPi$. These results are used in Chapter \ref{chapApproxMet} to reformulate, and solve in some cases, several optimization problems posed on triangulations.\\

\item (Combining hierarchy with anisotropy) 
A number of algorithms are based on hierarchical sequences of triangulations $(\cT_N)_{N \geq N_0}$, a property which guarantees % The fact that $\cT_{N+1}$ is a refinement of $\cT_N$ implies 
the inclusion of the associated finite element spaces $V_k(\cT_N)\subset V_k(\cT_{N+1})$. The property of hierarchy also allows for the definition of wavelet bases, and is a key in the analysis of some PDEs.

\qquad We define in Chapter \ref{chapCDHM} an algorithm producing sequences of (non conforming) anisotropic triangulations which satisfy this property of hierarchy, and in certain circumstances also satisfy the optimal error estimate \iref{eqCSX}. This algorithm strongly differs from the mesh generation methods presented previously, the local patching strategy and the approach based on riemannian metrics, since these are not adapted to hierarchical mesh refinement.\\
\end{enumerate}

Current results in anisotropic mesh adaptation for finite element approximation %, the study of $e_N(f)_X$, 
also suffer from two other important restrictions : they are only asymptotical, and they extend with difficulty to dimensions larger than two.
%The results presented in this section, which are more or less the state of the art in anisotropic mesh adaptation, also suffer from two other weaknesses. 
Removing these two restrictions raises difficult problems and remains mostly an open question at the time of writing.

\begin{enumerate}[i)]
\item (Non asymptotical results) 
The optimal error estimate \iref{eqCSX} involves a limit as the number $N$ of triangles constituting the mesh $\cT_N$ tends to infinity, see \iref{defLimSup}.
The asymptotic nature of this error estimate reveals that a sufficiently large number of triangles is needed to finely tune the triangulation $\cT_N$ to the local properties of the approximated function $f$. A smaller number of triangles raises the need for a compromise between the adaptation to the local features approximated function $f$ and the geometrical constraints involved in the production of a bi-dimensional triangulation.

\qquad We give in Chapter \ref{chapMeshMet} a translation of these geometrical constraints into the form of regularity properties satisfied by riemannian metrics, continuous objects which are equivalent to triangulations, see Theorem \ref{thMeshMetIntro}. In the case of isotropic triangulations we recover in Chapter \ref{chapApproxMet} some classical error estimates, expressed in terms of the Hardy-Littlewood maximal function of $|d^mf|$,  for the quantity 
$$
\sup_{N \geq 1} N^\frac m 2 e_{\cT_N} (f)_X %\left(\text{ instead of } \limsup_{N \to \infty} N^\frac m 2 e_{\cT_N} (f)_X\right).
$$
instead of the upper limit $\limsup_{N \to \infty} N^\frac m 2 e_{\cT_N} (f)_X$.
Obtaining a relevant estimate of this quantity in the case of anisotropic triangulations remains today an open question. \\

\item (Meshes in three or more dimensions) 
Throughout this introduction, we have yet only considered functions of two variables and bi-dimensional triangulations. 
Our discussion remains relevant in dimension three or higher, and three dimensional anisotropic mesh adaptation is already successfully used in applications, see for instance \cite{A}.

\qquad However a number of theoretical aspects of these methods remain unanswered. The key difficulty is the production of three dimensional anisotropic meshes, which is difficult from a practical point of view and not well understood from a theoretical point of view. We formulate in Chapter \ref{chapMeshMet} several conjectures which extend our bi-dimensional results on the equivalence of meshes and riemannian metrics.

\qquad We also consider dimensions larger than $2$ in parts I and II of this thesis, % (OptAniso??) and (Cartoon??),
which leads us to several types of difficulties. Some of these difficulties have an algebraic nature in Chapter \ref{chapOptAniso}, a geometric nature in Chapter \ref{chapCartoon}, or are related to mesh generation in Chapter\ref{chapW1P}. We formulate a precise conjecture each time that we cannot solve these difficulties.\\ 
\end{enumerate}

Last, the two following questions could be raised about the results \iref{eqCSX} and \iref{eqCSXOpt} on optimal mesh adaptation presented in this introduction. We regard them as more minor and they are not the subject of in depth discussion in this thesis.
\begin{enumerate}[i)]
\item (Interpolation instead of best approximation)
Some estimates presented in this introduction, such as \iref{eqCSX}, are based on the interpolation error instead of the best approximation error. In other words, for a given function $f$ and triangulation $\cT$ they provide an upper bound for 
\be
\label{eqInterp}
\|f-\interp_\cT^{m-1} f\|_{L^p} \stext{ or } \|\nabla (f - \interp_\cT^{m-1} f)\|_{L^p}
\ee
instead of 
\be
\label{eqBestApprox}
e_\cT(f)_{L^p} := \min_{g\in V_{m-1}(\cT)} \|f-g\|_{L^p} \stext{ or } e_\cT(f)_{W^{1,p}} := \min_{g\in V_{m-1}(\cT)} \|\nabla (f-g)\|_{L^p}.
\ee
\qquad The quantities \iref{eqInterp} correspond to the particular choice $g=\interp_\cT^{m-1} f$ and are therefore an upper bound for the corresponding quantities in \iref{eqBestApprox}. Is the difference so big that an estimate on \iref{eqInterp} is not relevant in the case \iref{eqBestApprox}?
The answer is generally ``no'' if the function $f$ is sufficiently smooth and if the triangulation $\cT$ is sufficiently fine, which is the case in the asymptotic setting considered in \iref{eqCSX}.
In contrast we consider in Chapter \ref{chapApproxMet} some functions of weaker regularity, and triangulations of fixed cardinality, which forbids the use of the standard Lagrange interpolation operator. The interpolation of $f$ is thus replaced with an quasi-interpolation of the local averages of $f$.\\

\item (The admissibility condition) 
The optimality results presented in this thesis, such as \iref{eqCSXOpt}, require the admissibility of the sequence $(\cT_N)_{N\geq N_0}$ of triangulations. This technical hypothesis can be removed in certain cases, such as the interpolation of a convex function by finite elements of degree one, see \cite{BBLS}.
We have not been able to remove this hypothesis in the general case, but we believe that the admissibility condition is rather a technical inelegancy than a weakness of the theory.
\end{enumerate}

==> MeshMetric/MeshMetricTheseOld.tex <==
\input{../PreambleThese}

\section{Introduction}

Triangulations and meshes are finite objects of combinatorial nature: they can be described by a collection of vertices and of connection between these. This description is fruitful for the demonstration of algebraic results, such as the Euler formula, or for computer processing.
In contrast, many approaches towards anisotropic mesh generation are based on a continuous object, namely a riemannian metric $z\mapsto H(z)$, in other words a continuous function $H$ from the domain $\Omega\subset \R^d$ to the set $S_d^+$ of symmetric positive definite matrices. Once this metric has been properly designed, it is the task of a mesh generation algorithm such as \cite{Shew,Bois,FreeFem,Inria} to generate a triangulation that agrees with this metric, in a sense specified below \iref{defEquiv}.
The purpose of this chapter is to formulate precise equivalence results between some classes of triangulations and of riemannian metrics. This equivalence translates some geometrical constraints satisfied by the triangulations into the form of regularity properties of the equivalent riemannian metrics.\\

Our results are so far limited to meshes and metrics defined on the entire infinite domain $\R^d$, and the dimension $d\geq 2$ is fixed throughout this chapter. 
The choice of the unbounded domain $\R^d$ guided by simplicity, since the curvature and the singularities of
of the boundary $\partial\Omega$ induces additional difficulties 
from the point of view of computational mesh generation.
Bounded domains will be the object of future work.
We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$, and we introduce in \S\ref{subsecDefTStar} three embedded subsets of $\bT$ of particular interest 
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
where $C\geq 1$ is a parameter which plays a minor role.
The set $\bT_{i,C}$ collects all \emph{isotropic} meshes $\cT$ which are heuristically defined as follows: the simplices $T\in \cT$ may have strongly varying volumes, but their aspect ratio is uniformly bounded. 
The largest set $\bT_{g,C}$ collects \emph{graded} meshes, which only satisfy a condition of local consistency: all the  geometrical features of the simplices $T\in \cT$ may vary strongly, volume, aspect ratio and orientation, but two \emph{neighboring} simplices should not be excessively different.
The intermediate set $\bT_{a,C}$ collects \emph{quasi-acute} meshes, which definition involves the measure of sliverness $S(T)$ of a simplex $T$ introduced in Chapter \ref{chapW1P} and also discussed in Chapter \ref{chapApproxMet}. 
The measure of sliverness plays an important role in the finite element approximation of a function on a mesh $\cT$ when the error is measured in the Sobolev $W^{1,p}$ norm.\\

We associate to each simplex $T$ a symmetric positive definite matrix $\cH_T$ such that the ellipsoid
$$
\cE_T := \{z\in \R^d \sep (z-z_T) \cH_T (z-z_T)^\trans \leq 1\},
$$
which is centered at the barycenter $z_T$ of $T$,
is the ellipsoid of minimal volume containing $T$. The properties of the matrix $\cH_T$ are discussed in \S \ref{subsecIntroSimplex} of this introduction,  as well as its explicit expression in terms of the coordinates of the simplex $T$. The matrix $\cH_T\in S_d^+$ encodes the volume, the aspect ratio and the orientation (but not the angles) of the simplex $T$. Two triangles $T$ and their associated ellipses $\cE_T$ are illustrated on figure \ref{figET}.

\begin{figure}
\centering
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleAigu.pdf}
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleObtus.pdf}
	\caption{Two triangles $T$ and their associated ellipse $\cE_T$.\label{figET}}
\end{figure}

A riemannian metric on $\R^d$ is a continuous map $H$ which associates to any $z\in \R^d$ a symmetric positive definite matrix $H(z)\in S_d^+$. We denote by $\bH = C^0(\R^d,S_d^+)$ the collection of riemannian metrics.
The following definition introduce a notion of equivalence between meshes and metrics
\begin{definition}
\label{defEqHT}
We say that a mesh $\cT\in \bT$ is $C_0$-equivalent to a given metric $H\in \bH$, where $C_0\geq 1$ is a fixed constant, if for all $T \in \cT$ and all $z\in T$ one has 
\be
\label{defEquiv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
\ee
We say that a collection of simplicial meshes $\bT_*\subset \bT$ is equivalent to a collection $H_*$ of metrics if there exists a uniform constant $C_0\geq 1$ such that the following holds:
\begin{itemize}
\item For any mesh $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\item For any metric $H\in \bH_*$ there exists a mesh $\cT\in \bT_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\end{itemize}
\end{definition}
Our main result (Theorem \ref{thEquiv}) states that when the constant $C$ is sufficiently large, and if dimension is $d=2$, the three classes of meshes $\bT_{i,C}\subset \bT_{a,C} \subset \bT_{g,C}$ are respectively equivalent to three classes of metrics
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
that are defined by precise smoothness conditions on the function $z\mapsto H(z)$ in \S \ref{subsecDefHStar} of this introduction.
%Our main result Theorem \ref{thEquiv} states that when the parameter $C$ is large enough and the dimension is $d=2$, the collections $\bT_{\star,C}$ of triangulations are equivalent to the corresponding collections $H_\star$ of metrics for any symbol $\star \in \{i,a,g\}$. 
The most striking point of this result is that, although the matrix $\cH_T$ does not encode the angles of a simplex $T$, the fact that a mesh $\cT\in \bT_{a,C}$ is \emph{quasi-acute} can be translated in a precise regularity condition on the metric $H$ equivalent to $\cT$.

In order to state our results more precisely we need to introduce some notations. We first recall some notations of linear algebra. We denote by $\M_d$ the collection of $d\times d$ matrices with real entries. We denote by $\GL_d$ the standard linear group, by $\SL_d$ the special linear group and by $\cO_d$ the orthogonal group
\begin{eqnarray*}
\GL_d &:=& \{A\in \M_d\sep \det A\neq 0\}\\
\SL_d &:=& \{A\in \M_d\sep \det A=1\}\\
\cO_d &:=& \{U\in \M_d\sep U^\trans U = \Id\}.
\end{eqnarray*}
We denote by $S_d$ the collection of symmetric matrices, by $S_d^\oplus$ the subset of non-negative symmetric matrices, and by $S_d^+$ the collection of symmetric positive definite matrices.
\begin{eqnarray*}
S_d &:=& \{M\in \M_d\sep M = M^\trans\}\\
S_d^\oplus &:=& \{M\in S_d\sep z^\trans M z \geq 0 \text{ for all } z\in \R^d\}\\
S_d^+ &:=& S_d^\oplus \cap \GL_d.
\end{eqnarray*}
Let $M,M'\in S_d$, we write $M\leq M'$ if $M'-M\in S_d^\oplus$, and $M< M'$ if $M'-M\in S_d^+$. We recall that for any $M,M'\in S_d$ such that $M\leq M'$ and any $\phi\in \M_d$ we have $\phi^\trans M \phi \leq \phi^\trans M' \phi$. Furthermore if $M,M' \in S_d^+$ and $M\leq M'$ then $M'^{-1} \leq M^{-1}$. For each symmetric positive definite matrix $M\in S_d^+$ we define a norm $\|\cdot\|_M$ as follows: for all $u\in \R^d$
$$
\|u\|^2_M := u^\trans M u.
$$

\subsection{Geometry of the simplex}
\label{subsecIntroSimplex}
The basic geometrical object studied in this chapter is the $d$-dimensional simplex, which is defined as follows.
\begin{definition}
A $d$-dimensional simplex $T$ is the convex envelope of a set $V\subset \R^d$ of $d+1$ %non-coplanar 
vertices, not contained in a $d-1$ dimensional affine subspace of $\R^d$ : 
$$
T = \Cvx(V).
$$
We denote by $\cF(T)$ the collection of faces of $T$ of any dimension,
\be
\label{defFT}
\cF(T) := \{\Cvx(V') \sep V'\subset V\}.
\ee
\end{definition}
Observe that $\emptyset$ and $T$ are among the faces of a simplex $T$, since they respectively correspond to $V'=\emptyset$ and $V'=V$.
We denote by $z_T\in \R^d$ the barycenter of a simplex $T$ of vertices $V$
$$
z_T := \frac 1 {d+1} \sum_{v\in V} v,
$$
and we define a symmetric positive definite matrix $\cH_T\in S_d^+$ as follows
\be
\label{defcH}
\cH_T^{-1} = \frac d {d+1} \sum_{v\in V} (v-z_T) (v-z_T)^\trans. %\frac {2d}{(d+1)^2}\sum_{v,v'\in V} (v-v')(v-v')^\trans. 
\ee
Some of the key properties of the matrix $\cH_T$ are exposed in the next proposition.
Throughout this chapter, we denote by $\TEq$ a $d$-dimensional equilateral simplex, centered at the origin
i.e. such that $z_\TEq=0$, and having its vertices on the unit ball. One easily checks that 
$$
\cH_\TEq = \Id.
$$
% Note that 
%\be
%\label{eqBallTEq}
%%\{z\in \R^d \sep |z| \leq 1/d\} 
%B(0, 1/d) \subset \TEq \subset \overline B(0,1).
%\ee
%
%%We associate to any simplex $T$ its barycenter $z_T\in \R^d$, and a symmetric positive definite matrix
%We denote by $z_T$ the barycenter of a simplex $T$, and we also associate to $T$ a symmetric positive definite matrix $\cH_T\in S_d^+$ which encodes some of its geometrical properties, in particular the volume, the elongation and the orientation of $T$.
\begin{prop}
\label{propHT}
The following holds for any $d$-dimensional simplex $T$. 
\begin{itemize}
\item
For any an affine change of coordinates $\Phi$, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0$ in $\R^d$, we have 
\be
\label{invcH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
\item
There exists a rotation $U\in \cO_d$, depending on $T$, such that 
\be
\label{eqcHTEq}
\cH_T^\frac 1 2 (T-z_T) = U(\TEq),
\ee
hence 
\be
\label{eqVolTHT}
|T| \sqrt{\det \cH_T} = |\TEq|.
\ee
\item
We have the inclusions 
\be
\label{eqTET}
\{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1/d\} \subset T \subset \cE_T := \{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1\},
\ee
and the these two ellipsoids are respectively the one of largest volume included in $T$, and of smallest volume containing $T$.
\end{itemize}
\end{prop}
\proof
For any simplex $\Phi^{-1}(v)$ of the simplex $\Phi^{-1}(T)$, we have 
$$
\Phi^{-1}(v)-z_{\Phi^{-1}(T)} = \Phi^{-1}(v)-\Phi^{-1}(z_T) = \phi^{-1}(v-z_T).
$$
Injecting this relation in \iref{defcH} we obtain \iref{invcH}. 
We now turn to the proof of \iref{eqcHTEq} and for that purpose we remark that the simplices $\TEq$ and $T' := \cH_T^\frac 1 2 (T-z_T)$ have both their barycenter at zero, $z_\TEq = z_{T'} = 0$, hence there exists a linear map $\phi\in \GL_d$ such that $T' = \phi^{-1}(\TEq)$. We thus obtain, using the formula \iref{invcH} for the transformation of $\cH_T$ under affine change of coordinates 
$$
\begin{array}{ccccc}
\cH_{T'} &=& \cH_T^{-\frac 1 2} \cH_T \cH_T^{-\frac 1 2} &=& \Id \\ 
\cH_{\phi^{-1}(\TEq)} &=& \phi^\trans \cH_\TEq &=& \phi^\trans \phi.
\end{array}
$$
Hence $\phi^\trans \phi= \Id$ which establishes that $\phi\in \cO_d$ and concludes the proof of \iref{eqcHTEq}.
%One easily checks that 
%$$
%\overline B(0,1/d) \subset \TEq \subset \overline B(0,1),
%$$
%where
It is well known that the smallest ellipsoid containing $\TEq$ is the unit ball, and that the largest ellipsoid included in $\TEq$ is the ball of radius $1/d$. Combining this fact with the change of coordinates \iref{eqcHTEq} we obtain \iref{eqTET} which concludes the proof of this proposition.
\sq

Note that for any simplex $T$ and any $z,z'\in T$ we obtain using \iref{eqTET}
\be
\label{eqDiamTHT}
\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2.
\ee

We introduce a measure of degeneracy $\rho(T)$ of a $d$-dimensional simplex $T$
\be
\label{defRhoMM}
\rho(T) := \sqrt{\|\cH_T\| \|\cH_T^{-1}\|}.
\ee
%This measure of non degeneracy $\rho$ is slightly different from the measure of non degeneracy $\frac {\diam(T)^d} {|T|}$ used in some of the previous chapters. However these two measures play a similar role and can be compared. Indeed we obtain using \iref{eqVolTHT} and \iref{eqcTET}
%\be
%\label{eqRhoRhop}
%\frac{\rho(T)}{d^\frac d 2|\TEq|} \leq  \frac{(\|\cH_T^{-1}\|/d)^\frac d 2} {|\TEq| (\det \cH_T)^{-\frac 1 2}} \leq \frac{\diam(T)^d} {|T|} \leq \frac{\|\cH_T^{-1}\|^\frac d 2} {|\TEq|(\det \cH_T)^{-\frac 1 2}}\leq \frac{\rho(T)^{d-1}}{|\TEq|}.
%\ee
%Observing that $\|A\| \|A^{-1}\|^{-(d-1)} \leq |\det A| \leq \|A\|^{d-1} \|A^{-1}\|^{-1}$ for any $A\in \GL_d$
%it follows that 
Observe that $\rho(T)\geq 1$ for any simplex $T$, with equality if and only if $\cH_T$ is proportional to the identity, which implies in view of \iref{eqcHTEq} that $T$ is a displacement of the equilateral simplex $\TEq$:
$$
\rho(T) = 1 \stext{ if and only if }
%\ \Longleftrightarrow \ 
T = z_T+r U(\TEq) \text{ for some }  r>0 \text{ and } U \in \cO_d.
$$
The measure of degeneracy $\rho$ is slightly different from the measure of degeneracy $\frac {\diam(T)^d} {|T|}$ used in Chapters \ref{chapOptAniso} and \ref{chapW1P} but both have the same role: they are minimal for the equilateral simplex, and increase as the simplex becomes thinner.\\

The measure of sliverness $S(T)$ of a simplex $T$ is a quantity which plays an important role in the context of optimal mesh adaptation for the finite element approximation of a function in the Sobolev $W^{1,p}$ norm, see   \cite{Ba, Ja}, and Chapters \ref{chapW1P} and \ref{chapApproxMet}. 
This measure of sliverness is defined in Chapter \ref{chapW1P} and illustrated by several examples and equivalent quantities. We recall the definition of this quantity
\be
\label{defSMM}
S(T) := \inf \{ \|\phi\| \|\phi^{-1}\| \sep \phi \in \GL_d \text{ and } \phi(T) \text{ is acute } \},
\ee
a simplex is acute if the exterior normals $\n, \n'$ to any two distinct faces of $T$ have a negative scalar product $\<\n,\n'\>\leq 0$.
As observed in Chapter \ref{chapW1P}, the measure of sliverness $S(T)$ can be interpreted as the distance from $T$ to the collection of acute simplices.

The exterior normals $\n,\n'$ to any two $d-1$-dimensional faces of $\TEq$ satisfy $\<\n,\n'\> =-1/d$, hence this simplex is acute. Recalling \iref{eqcHTEq}
 we thus obtain for any simplex $T$
$$
S(T) \leq \rho(T).
$$
Apart from this upper bound, the matrix $\cH_T$ does not contain any direct information on the measure of sliverness $S(T)$.
%One of the key results of this chapter is that in a bidimensional triangulation $\cT$, and conjecturedly in higher dimension too, the variation of the matrix $\cH_T$ as $T$ varies in $\cT$ does encode the measure of sliverness in some sense.
For any bidimensional triangle $T$ of largest angle $\theta$, Proposition \ref{propSTan} of Chapter \ref{chapW1P} states that :
$$
S(T) = \max\left\{1, \tan \frac \theta 2 \right\}.
$$

\subsection{Simplicial meshes}
\label{subsecDefTStar}

As a starter, we recall the definition of a simplicial mesh of $\R^d$.
%We first briefly recall the defini
%Before introducing simplicial meshes, we briefly recall the definition of locally finite partitions of $\R^d$.

%In order to introduce q,xcl meshes 
\begin{definition}
\label{defSimplMesh}
A conforming simplicial mesh of $\R^d$ is a collection $\cT$ of simplices which satisfy the conformity axiom :  for all $T,T'\in \cT$
\be
\label{confAxiom}
T\cap T' \in \cF(T) \cap \cF(T'),
\ee
as well as the following properties
\begin{itemize}
\item (Covering) The simplices $T\in \cT$ cover the whole infinite domain $\R^d$:
$$
\bigcup_{T\in \cT} T = \R^d.
$$
\item (Partition) The interiors of the simplices $T\in \cT$ are pairwise disjoint: for any $T,T'\in \cT$,
$$
\interior (T) \cap \interior(T') \neq \emptyset\stext{ implies }  T=T'. %
$$
\item (Local finiteness) For any compact set $K \subset \R^d$, only a finite collection of simplices $T\in \cT$ intersect $K$:
$$
\{T \in \cQ \sep K \cap T \neq \emptyset \} \ \text{ is finite.}
$$
\end{itemize}
\end{definition}
The conformity axiom \iref{confAxiom} states that the intersection of any two simplices in $\cT$ needs to be a full common face.We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$.

For an optimal efficiency, numerous numerical simulation software use anisotropic meshes, in which the simplices may have an arbitrary shape. Anisotropic meshes are used for instance, to create a thin layer of simplices close to a geometric feature which is relevant in a numerical simulation.
In order to avoid excessively wild meshes, one often requires relevant  some consistency between the shapes of neighboring simplices.We therefore introduce for any constant $C \geq 1$ the class $\bT_{g,C} \subset \bT$ of \emph{graded} meshes, which is defined as follows.
A mesh $\cT$ belongs to $\bT_{g,C}$ if for any two simplices $T,T'\in \cT$ one has 
\be
\label{defTG}
T \cap T'\neq \emptyset \stext{ implies } C^{-2}\cH_T \leq \cH_{T'} \leq C^2 \cH_T.
\ee

For any $C\geq 1$ we also introduce the class $\bT_{i,C}$ of \emph{isotropic} meshes, by requiring that in addition to \iref{defTG} that the measure of degeneracy $\rho$ is uniformly bounded by $C$, which forbids any anisotropy.
A mesh $\cT$ belongs to $\bT_{i,C}$ if and only if $\cT\in \bT_{g,C}$ and for all $T \in \cT$
$$
\rho(T) \leq C. %C \geq 1? or 0? 
$$

%The next proposition shows that the definition of $\bT_{i,C}$ is slightly redundant, in the sense that condition \iref{defTG} could be avoided.
%\begin{prop}
%Denote by $\bT'_{i,C}$ the collection of meshes $\cT\in \bT$ satisfying $\rho(T) \leq C$ for all $T\in \cT$ (but perhaps not the gradedness condition \iref{defTG}). %We thus have $\bT_{i,C} \subset \bT'_{i,C}$.\\
%Then for all $C$ there exists $C' = C'(C)$ such that 
%$$
%\bT_{i,C} \subset \bT'_{i,C} \subset \bT_{i,C'}.
%$$
%\end{prop}
%
%\proof
%See appendix. 
%\sq

In order to introduce the intermediate collection $\bT_{a,C}$ of $C$-quasi-acute meshes, we first define the notion of refinement of a simplicial mesh.
\begin{definition}
Consider two meshes $\cT,\cT'\in \bT$ and a constant $C\geq 1$. We say that $\cT'$ is a $C$-refinement of $\cT$ if it satisfies the following properties.
\begin{itemize}
\item (Inclusion) Any simplex $T'\in \cT'$ is contained in a simplex $T\in \cT$. % such that $T'\subset T$.
\item (Bounded refinement) Any simplex  $T\in \cT$, contains most $C$ simplices $T'\in \cT$.
\end{itemize}
\end{definition}

A graded mesh $\cT \in \bT_{g,C}$ belongs to the collection $\bT_{a,C}$ of quasi-acute meshes if and only there exists a $C$-refinement $\cT'$ of $\cT$ which satisfies for all $T' \in \cT'$
$$
S(T') \leq C.
$$
In particular if $\cT\in \bT_{i,C}$, then choosing $\cT' = \cT$, which is a $C$-refinement since $C\geq 1$, and recalling that $S(T) \leq \rho(T)$ for any simplex $T$, we obtain that $\cT\in \bT_{a,C}$. Thus $\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}$ as announced.

The constraints defining graded, quasi-acute and isotropic meshes are illustrated on Figure \ref{figDisk}
in the main introduction of the thesis. 
Figure \ref{figAcuteGen} gives an example of a quasi-acute triangulation which 
by the above described refinement process leads to a slightly finer triangulation on
sliverness $S(T)$ is uniformly bounded.

\begin{figure}
\centering
%	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarGdeVap.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap1.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap2.pdf}
	\caption{\label{figAcuteGen}
Quasi-acute triangulation (left) and refined triangulation with uniformly bounded sliverness (right).
	}
\end{figure}

\subsection{Riemannian metrics}
\label{subsecDefHStar}

For any metric $H \in \bH$ and path $\gamma \in C^1([a,b],\R^d)$, we define the riemmannian length $l_H(\gamma)$ by the integral
$$
l_H(\gamma) := \int_a^b \|\gamma'\|_{H(\gamma(t))} dt.
$$
The riemmannian distance $d_H$ between two points  $z,z'\in \R^d$, is the infimum of the length of all paths joining $z$ and $z'$, 
\be
\label{defdH}
d_H(z,z') := \inf\left\{l_H(\gamma)\sep \gamma\in C^1\left([0,1],\R^d\right), \ \gamma(0) = z \text{ and } \gamma(1) = z'\right\}.
\ee
If $H, H'\in \bH$ are such that $H(z) \leq H'(z)$ for all $z\in \R^d$, then $d_H(z,z') \leq d_{H'}(z,z')$ for all $z,z'\in \R^d$.
By construction, the riemannian distance $d_H$ associated to a metric $H\in \bH$ is locally equivalent close to a point $z$ to the distance defined by the norm $\|\cdot \|_{H(z)}$: for all $z\in \R^d$
\be
\label{eqDistLoc}
\limsup_{\ve \to 0} \sup_{p,q\in B(z, \ve)} |\ln d_H(p,q) - \ln \|p-q\|_{H(z)}| = 0,
\ee
where $B(z,\ve)$ denotes the euclidean ball of radius $\ve$ around $z$.\\


\begin{remark}[Riemannian geodesics]
When a metric $H$ is sufficiently smooth, a special family of curves named Riemannian geodesics can be defined and studied. A riemannian geodesic is a curve $\gamma\in C^0(\R, \R^d)$ which satisfies a second order differential equation %written in terms of the second order derivatives of $H$, 
called the equation of geodesics. This equation implies that for any sufficiently close $t,t'\in \R$ the curve $\gamma_{|[t,t']}$ is the path of smallest possible length joining the points $\gamma(t)$ and $\gamma(t')$ : 
$d_H(\gamma(t), \gamma(t')) = l_H(\gamma_{|[t,t']})$.

Geodesics are not defined for general continuous or Lipschitz riemannian metrics, such as those constituting the sets $\bH$ and $\bH_i \subset \bH_a\subset \bH_g$, since the coefficients of the equation of geodesics involve the second derivatives of the metric. Notions related to geodesics, such as the injectivity radius of a metric, therefore have no meaning in our context.
This is not an issue for our purposes since, following the point of view of \cite{Gromov},
%[Gromov, Metric structures for Riemannian and non-Riemannian spaces, Birkhauser (1999)]
we study Riemannian distances and not Riemannian geodesics. 

%Note also that geodesics only exist when the metric $H$ has requires that $H$ has at least $C^2$ smoothness, while the metrics studied in this chapter generally only have $C^0$ or Lipschitz smoothness.

%Since we only assume that $H$ is a continuous metric, the infimum \iref{defdH} may or may not be attained, and in that later case possibly for several paths. The equation of geodesics associated to a riemannian metric involves the second order derivatives, which are not defined in our context.
%(* also the point of view of Gromov : we study distances and not geodesics*)
\end{remark}


We denote by $\bH_i$ the collection of metrics $H \in \bH$ which are proportionnal to the identity: for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2},
$$
and such that the proportionality factor $s$ satisfies one of the two following conditions conditions, which are surprisingly equivalent as shown in Proposition \ref{propEquivS}:
\begin{itemize}
\item (``Additive'' Lipschitz condition)  
\be
\label{eqLipSAdd}
|s(z) - s(z')| \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
\item (``Multiplicative'' Lipschitz condition)
\be
\label{eqLipSMult}
|\ln s(z) - \ln s(z')| \leq d_H(z,z') \stext{ for all } z,z'\in\R^d.
\ee
\end{itemize}

The two Lipschitz properties \iref{eqLipSAdd} and \iref{eqLipSMult} have a natural generalisation to general anisotropic metrics but are not equivalent in that context.
In order to introduce the regularity conditions defining the classes $\bH_i\subset \bH_a\subset \bH_g$ of metrics, we need to  two distances $d_\times$ and $d_+$ on the set $S_d^+$ of symmetric positive definite matrices. 
For any $M,M'\in S_d^+$ we define
\be
\label{defDTimes}
d_\times (M,M') := \min \{\delta \geq 0 \sep e^{-2\delta} M \leq M' \leq e^{2 \delta} M\}.
\ee
For instance, a mesh $\cT$ is $C$-equivalent to a metric $H$, as defined in \iref{defEquiv}, if and only if for all $T \in \cT$ and all $z\in \cT$ one has 
$$
d_\times (H(z), \cH_T) \leq \ln C.
$$
There exists various expressions of the distance $d_\times$ : for all $M,M'\in S_d^+$ one has 
\be
\label{eqDTimesLog}
d_\times (M,M') = \sup_{u\in \sR^d\sm \{0\}} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
\ee
and 
\be
\label{eqDTimesProd}
d_\times (M,M') = \ln \left(\max \{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\}\right).
\ee
The exponential of the distance $d_\times$ was used in the earlier paper \cite{Shew} %on anisotropic mesh generation
under the name ``relative deformation''. 
We define a second distance $d_+$ on $S_d^+$ as follows 
\be
\label{defDPlus}
d_+(M,M') := \|M^{-\frac 1 2} - M'^{-\frac 1 2}\|.
\ee
The expressions \iref{eqDTimesProd} and \iref{defDPlus} of the distances $d_\times$ and $d_+$ show that they are respectively tied to multiplicative or additive properties of matrices, which justifies their notations.
Note also that for any $s,s'>0$ one has
\be
\label{eqDIso}
d_\times (s^{-2} \Id, s'^{-2} \Id) = |\ln s - \ln s'| \stext{ and } d_+(s^{-2} \Id, s'^{-2} \Id) = |s-s'|.\\
\ee

We denote by $\bH_g$ the collection of metrics $H\in \bH$ which satisfy the natural extension of \iref{eqLipSMult} to general anisotropic metrics:
\be
\label{eqLipMult}
d_\times (H(z), H(z')) \leq d_H(z,z') \stext{ for all }z,z'\in\R^d.
\ee
This condition can be heuristically described as follows: a metric $H\in \bH$ defines close to each point $z\in\R^d$ a norm $\|\cdot\|_{H(z)}$ which encodes an anisotropic notion of scale. The equation \iref{eqLipMult} states that the metric $H$ itself is consistent a the scale that it encodes.\\

We denote by $\bH_a$ the collection of metrics $H\in \bH$ which satisfy both \iref{eqLipMult} and the natural extension of \iref{eqLipSAdd} to general anisotropic metrics:
\be
\label{eqLipAdd}
d_+ (H(z), H(z')) \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
In addition to the results of mesh generation presented in this chapter, we show in the next chapter, Chapter\ref{chapApproxMet}, that this condition is critical in order to define a local averaging operator compatible with Sobolev norms. 
%decrire le lien avec les angles aigus.
\begin{remark}
\label{remHomog}
Let $H\in \bH$, and let $\lambda>0$. Using the homogeneity properties of the distances $d_\times$, $d_+$ on $S_d^+$ and $d_H$ on $\R^d$ with respect to $H$, we obtain that $\lambda^2 H\in \bH_g$ if and only if 
\be
\label{eqLipTimesLambda}
d_\times (H(z), H(z')) \leq \lambda d_H(z,z') \stext{ for all } z,z'\in \R^d, 
\ee
and $\lambda^2 H\in \bH_a$ if and only if we have in addition to the previous property 
\be
\label{eqLipPlusLambda}
d_+ (H(z), H(z')) \leq \lambda |z-z'| \stext{ for all } z,z'\in \R^d.
\ee
In particular the collections $\bH_i \subset \bH_a \subset \bH_g$ of isotropic, quasi-acute and graded metrics are stable under multiplication by a constant larger than one : for any $\star \in \{a,b,c\}$, any $H\in \bH_\star$ and any $\lambda \geq 1$ we have $\lambda^2 H\in \bH_\star$.
%this operation corresponds to the uniform refinement of a triangulation...
\end{remark}

\subsection{Main results}

The main result of this chapter is the equivalence of the classes of meshes and metrics defined above, which is  announced in the first part of the introduction and proved in sections \S\ref{secMeshToMet} and  \S \ref{secMetToMesh}. In two cases we were only able to establish this equivalence when the dimension is $d=2$. 
\begin{theorem}
\label{thEquiv}
There exists $C_0 = C_0(d)$ such that for all $C\geq C_0$ the following holds.
\begin{enumerate}[i)]
\item The collections $\bT_{i,C}$ of triangulations and $\bH_i$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{a,C}$ of triangulations and $\bH_a$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{g,C}$ of triangulations and $\bH_g$ of metrics are equivalent.
\end{enumerate}
\end{theorem}

Let us comment on this result.
The theory of isotropic meshes is already well developed, and our result i) in this direction should be regarded as a reformulation of previous work, intended to put into perspective the results on anisotropic meshes. The main ingredient of the proof of i) is the mesh refinement procedure exposed in \cite{Nochetto}. 

In the case iii) of graded metrics the key ingredients used for the construction of a triangulation $\cT\in \bT_{g,C}$ equivalent to a metric $H \in \bH_g$ come from the paper of computational geometry \cite{Shew}. In contrast the arguments used to produce a metric $H \in \bH_g$ from a mesh $\cT \in \bH_{g,C}$ are new, to the knowledge of the author, and they hold in any dimension.

Last the author has not heard of any anterior results on the collection $\bT_{a,C}$ of quasi-acute meshes, and most of the techniques used in that context are new.

\begin{conjecture}
The author conjectures that the points ii) and iii) of Theorem \ref{thEquiv} holds without restriction on the dimension $d$.
\end{conjecture}

This chapter is organised as follows. We establish in section \S \ref{secMetProp} some general properties of metrics in $\bH_a$ or $\bH_g$. 
We first prove in \S\ref{subsecMetInv} a property of invariance of the collection $\bH_g$ of graded metrics with respect to affine changes of coordinates.
The regularity assumptions \iref{eqLipMult} and \iref{eqLipAdd} defining graded and quasi-acute metrics simply mean that the map $H : \R^d \to S_d^+$ is Lipschitz with respect to some distances on $\R^d$ and $S_d^+$. 
We therefore study metrics from this point of view in \S\ref{subsecMetLip}.
We focus in \S\ref{subsecMetGeom} on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. In particular we compare the $d_H$ with the euclidean distance and we estimate the volume of balls. 


Section \S\ref{secEigen} is devoted to the study of metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has  an eigenspace of dimension at least $d-1$ at each point. This condition clearly holds if the dimension is $d=2$ but is also relevant in some applications to higher dimension such as the creation of a this layer of simplices close to a $d-1$ dimensional surface. This situation is discussed in Chapter \ref{chapApproxMet}, and involves metric which have an eigenvalue much larger that the others in the orthogonal direction to the surface of interest.
We give an approximate translation of the regularity properties \iref{eqLipAdd} and \iref{eqLipMult} defining the collections $\bH_a$ and $\bH_g$ of metrics in terms of the two eigenvalues of $H$ and of the direction of the eigenspaces of such metrics. 

The last two sections \S\ref{secMeshToMet} and \S\ref{secMetToMesh} are devoted to the proof of Theorem \ref{thEquiv}. More precisely we adress in \S\ref{secMetToMesh} the production of an isotropic, quasi-acute or graded mesh equivalent to a given metric $H\in \bH_i$, $\bH_a$ or $\bH_g$. Conversely we depict in \S\ref{secMeshToMet} to construction of a metric which is equivalent to a given mesh.


\section{General properties of graded and quasi-acute metrics}
\label{secMetProp}

We study in this section the general properties of the  distinguished classes of metrics $\bH_i \subset \bH_a \subset \bH_g$. 
We first establish in \S\ref{subsecMetInv} some invariance properties of these collections of metrics with respect to affine changes of coordinates.
We then regard in \S\ref{subsecMetLip} metrics as Lipschitz functions $H : \R^d\to S_d^+$. %, and we recall some basic properties of these.
The last subsection \S\ref{subsecMetGeom} is devoted to the comparison of the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$, with respect to the standard euclidean distance and Lebesgue measure.

\subsection{Invariance properties and restriction of metrics}
\label{subsecMetInv}

We focus in this subsection on the properties of invariance of the collections of meshes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ and of metrics $\bH_i \subset \bH_a\subset \bH_g$ introduced in this chapter.

Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$.
We have for any simplex $T$, as previously observed in \iref{invcH},
\be
\label{eqInvH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
Mimicking this property we define for any $H \in \bH$ a transported version $H_\Phi\in \bH$ as follows: for all $z\in \R^d$
\be
\label{defHPhi}
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi.
\ee
In the language of differential geometry,
the metric $H_\Phi$ is generally referred to as the ``pull back'' of $H$ by $\Phi$. If a mesh $\cT\in \bT$ is $C$-equivalent to a metric $H\in \bH$, then \iref{eqInvH} and \iref{defHPhi} clearly imply that the mesh $\Phi^{-1}(\cT)$ is $C$-equivalent to the metric $H_\Phi$.

The next proposition studies the invariance of the collections $\bT_{\star,C}$ of meshes and $\bT_\star$ of metrics, $\star \in \{i,a,g\}$, under the transformations $\cT \mapsto \Phi^{-1}(\cT)$ or $H \mapsto H_\Phi$ induced by an affine change of coordinates $\Phi$.

\begin{prop}
\label{propInvT}
Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. 
The following holds for any constant $C\geq 1$.
\begin{enumerate}[i)]
\item If $\cT \in \bT_{g,C}$ then $\Phi^{-1}(\cT) \in \bT_{g,C}$. If $H \in \bH_g$ then $H_\Phi\in \bH_g$.
\item Assume that $\Phi$ is an isometry, in other words $\phi\in \cO_d$.\\
If $\cT\in \bT_{a,C}$ then $\Phi^{-1}(\cT)\in \bT_{a,C}$, and similarly if $\cT\in \bT_{i,C}$ then $\Phi^{-1}(\cT)\in \bT_{i,C}$.\\
If $H\in \bH_a$ then $H_\Phi\in \bH_a$, and similarly if $H\in \bH_i$ then $H_\Phi\in \bH_i$.
\end{enumerate}
\end{prop}

\proof
%We concentrate on the case of meshes, since the statements on metrics are a special case of the propositions (??) and (??) below (* no : state the result for iso and quasi acute metrics too*).
%We first consider the case of meshes, and then 
We first establish the properties announced for meshes, and we then focus on metrics.
Let $M,M'\in S_d^+$, let $C\geq 1$ and let $\phi\in \GL_d$. Clearly
$$
\text{ if } C^{-2} M \leq M' \leq C^2 M \stext{ then } C^{-2} \phi^\trans M\phi \leq \phi^\trans M'\phi  \leq C^2 \phi^\trans M\phi.
$$
%Consequently if a mesh $\cT$ satisfies the condition \iref{defTG} defining the elements of $\bT_{g,C}$
%
%satisfy $C^{-2} M \leq M' \leq C^2 M$, then we also ha
%For any $M,M'\in S_d^+$ we obtain using \iref{defDTimes} that 
%$$
%d_\times (\phi^\trans M \phi,\ \phi^\trans M' \phi) = d_\times (M,M').
%$$
%It follows using \iref{eqInvH} that for any  two simplices $T,T'$,
%$$
%d_\times (\cH_{\Phi^{-1}(T)}, \cH_{\Phi^{-1}(T')}) = d_\times (\cH_T,\cH_{T'}).
%$$ 
In view of the definition \iref{defTG} of $\bT_{g,C}$ we obtain that $\Phi^{-1}(\cT)\in \bT_{g,C}$ for any mesh $\cT\in\bT_{g,C}$ as announced in i).

If $\Phi$ is an isometry then for any simplex $T$ we obtain, using the definitions \iref{defRhoMM} and \iref{defSMM} of the measure of degeneracy $\rho$ and the measure of sliverness $S$, that
$$
\rho(\Phi^{-1}(T)) = \rho(T) \stext{ and } S(\Phi^{-1}(T)) = S(T).
$$
This implies the properties of $\bT_{a,C}$ and $\bT_{i,C}$ announced in b), which concludes the proof of the properties announced for meshes.

We therefore turn our attention to metrics. The fact that $H_\Phi\in \bH_g$ for any $H\in \bH_g$ and any affine change of coordinates $\Phi$ is a special case of Proposition \ref{propHG} below. We thus admit this property and we focus on isotropic and graded metrics and isometric changes of coordinates.

If $H\in \bH_i$, then $H = \Id/s(z)^2$ where $s: \R^d \to \R_+^*$ is a Lipschitz function. Since $\phi\in \cO^d$ we have $\phi^\trans \phi = \Id$ and therefore 
$$
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi = \Id/s(\Phi(z))^2.
$$
The map $s \circ \Phi : \R_d\to \R_+^*$ is Lipschitz since it is the composition of a Lipschitz function with an isometry, which establishes that $H_\Phi\in \bH_i$ as announced.

If $H\in \bH_a$ and $\Phi$ is an isometry, then for any $z,z'\in \R^d$
\begin{eqnarray*}
\|H_\Phi(z)-H_\Phi(z')\| &=& \|\phi^\trans \left(H(\Phi(z))-H(\Phi(z'))\right) \phi\| \\
&=& \|H(\Phi(z))-H(\Phi(z'))\|\\
& \leq& \|\Phi(z)-\Phi(z')\|\\
& =& \|\phi(z-z')\|= |z-z'|,
\end{eqnarray*}
which establishes that $H_\Phi$ satisfies the Lipschitz regularity condition \iref{eqLipAdd}. We already know from the case of graded metrics that the other regularity condition \iref{eqLipMult} is satisfied by $H_\Phi$, which establishes that $H_\Phi\in \bH_a$ and concludes the proof of this proposition.
\sq


In practical applications, one often needs to mesh simultaneously a domain $\Omega$ and a surface $\Gamma$ embedded in $\Omega$. In terms of metric this raises the following question: given a metric $H$ on $\Omega$ which satisfies certain properties of regularity %, corresponding do a certain class of meshes, 
what is the regularity of the restriction of this metric to $\Gamma$?

The next proposition answers this question is the simplified setting where $\Omega$ is the infinite domain $\R^d$, $\Gamma$ is an affine subspace of $\R^d$, and properties of regularity are those defining the collection $\bH_g$ of graded metrics. For any $1\leq k \leq d$ we denote by $\bH_g(\R^k)$ the collection of graded metrics on $\R^k$.

\begin{prop}
\label{propHG}
Let $1\leq k\leq d$, let $\Phi : \R^k\to \R^d$ be an affine injective map, $\Phi(z) = \phi z+z_0$ where $\phi\in M_{d,k}$ has rank $k$ and $z_0\in \R^d$. Let $H\in \bH$ and let for all $z\in \R^k$
$$%\be
%\label{defHPhi}
H_\Phi(z) := \phi^\trans H(\Phi(z)) \phi.
$$%\ee
If $H\in \bH_g$ then $H_\Phi\in \bH_g(\R^k)$. 
\end{prop}

\proof
For any $u\in \R^d$, one has 
\be
\label{chgNorm}
\|u\|_{H_\Phi(z)} = \|\phi(u)\|_{H(\Phi(z))}.
\ee
Hence for any $z,z'\in \R^k$ we obtain using \iref{eqDTimesLog},
\be
\label{dNHPhi}
\begin{array}{rcl}
d(H_\Phi(z), \ H_\Phi(z'))  &=&\displaystyle \sup_{u\in \sR^k\sm\{0\}} \left|\ln \left\|\phi(u)\right\|_{H(\Phi(z))} -\ln \left\|\phi(u)\right\|_{H(\Phi(z'))}\right| \\
& \leq& d(H(\Phi(z)), \  H(\Phi(z')))
\end{array}
\ee
For any path $\gamma\in C^1([0,1], \R^k)$, it follows from \iref{chgNorm} that % the distorted lengths tied to $H$ and $H_\phi$ are therefore linked by 
$$
l_H(\Phi\circ \gamma) = \int_0^1 \|\phi(\gamma'(t))\|_{H(\Phi(\gamma(t)))}dt =  l_{H_\Phi}(\gamma).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^k)$ joining two points $z,z'\in \R^k$, we obtain since $\Phi\circ \gamma\in C^1([0,1], \R^d)$ is a path joining $\Phi(z)$ and $\Phi(z')$
\be
\label{dHPhi}
d_H(\Phi(z), \Phi(z')) \leq d_{H_\Phi}(z,z')
\ee
Combining \iref{dNHPhi} and \iref{dHPhi}, we conclude the proof of this proposition.
\sq


\subsection{Metrics as Lipschitz functions}
\label{subsecMetLip}
Lipschitz functions play an important role in this chapter and in particular in this section. We recall here their basic properties.
If $(X,d_X)$ and $(Y,d_Y)$ are two metric spaces, and if $f \in C^0(X , Y)$, we define 
the dilatation $\dil(f) \in [0, \infty]$ of $f$ as follows
$$
\dil(f) := \sup_{\substack{x,x'\in X \\ x \neq x'}} \frac{d_Y(f(x),f(x'))}{d_X(x,x')}
$$

We say that $f$ is Lipschitz if $\dil(f) \leq 1$, and more generally that $f$ is $\lambda$-Lipschitz if $\dil(f) \leq \lambda$.
We define the local dilatation $\dil_x(f)$ of a function $f\in C^0(X,Y)$ at a point $x\in X$ as follows
\be
\label{defDilX}
\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
\lim_{\ve\to 0} \left(\sup_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
\ee
%\be
%\label{defDilX}
%\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
%\lim_{\ve\to 0} \left(\sup_{e,e'\in B(x,\ve)} \frac{d_Y(f(e),f(e'))}{d_X(e,e')}\right).
%\ee
We specify the distance function on $X$ or $Y$ if it is not the expected ``canonical one'', in particular if $X$ or $Y$ is a subset of $\R^k$ and if the associated distance is not the standard euclidean distance but the riemannian distance $d_H$ associated to a metric, or if $X$ or $Y$ is the collection $S_d^+$ of symmetric positive definite matrices since none of the two distances $d_+$ or $d_\times$ is canonical. The local dilatation is in that case denoted as follows
$$
\dil_x(f\sep d_X, d_Y), \quad \dil_x(f\sep d_X)  \stext{ or } \dil_x(f\sep d_Y).
$$

The local dilatation $\dil_x(f)$ only depends on the local properties of the metric spaces close to $x$ and $f(x)$. Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$. For any $f\in C^0(\R^d, Y)$ and any $z\in \R^d$ we obtain using \iref{eqDistLoc}
\be
\label{eqDilNorm}
\|H(z)^{-1}\|^{-\frac 1 2} \dil_z(f) \leq \dil_z(f\sep d_H) = \dil_z(f \sep \|\cdot \|_{H(z)}) \leq \sqrt{\|H(z)\|} \dil_z(f)
\ee
We also introduce the lower local dilatation $\dil_z^*(f)\leq \dil_z(f)$ which is defined as follows
$$
\dil_z^*(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
$$
The next proposition establishes that local dilatations are sub-multiplicative.
\begin{lemma}
\label{lemmaSubMult}
Let $(X,d_X)$, $(Y,d_Y)$ and $(Z,d_Z)$ be three metric spaces, and let $f\in C^0(X,Y)$ and $g\in C^0(Y,Z)$. 
For any $x\in X$ one has 
\be
\label{eqDilUpper1}
\dil_x(g \circ f) \leq \dil_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side. Similarly we have 
\be
\label{eqDilLower1}
\dil_x(g \circ f) \geq \dil^*_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side.
\end{lemma}

\proof
We first establish \iref{eqDilUpper1}.
If $\dil_x(f) = \infty$ or $\dil_{f(x)}(g) = \infty$, then there is nothing to prove. We may therefore assume that $\dil_x(f) < \infty$ and $\dil_{f(x)}(g) < \infty$.
For any $\ve>0$ we define 
$$
F(\ve) = \sup_{p,q\in B(x, \ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)} \stext{ and } G(\ve) := \sup_{p,q\in B(f(x), \ve)} \frac{d_Z(g(p),g(q))}{d_Y(p,q)}
$$
It follows that 
$$
\sup_{p,q\in B(x, \ve)} \frac{d_Z(g(f(p)),g(f(q)))}{d_X(p,q)} \leq F(\ve) \, G(F(\ve) \ve).
$$
Taking the limit as $\ve \to 0$ we obtain \iref{eqDilUpper1} which concludes the proof.
For the proof of \iref{eqDilLower1} we consider two sequences $(p_n)_{n \geq 0}$, $(q_n)_{n \geq 0}$ which both tend to $x$ and such that $d_Y(f(p_n),f(q_n))/d_X(p_n, q_n) \to \dil_x(f)$ as $n \to \infty$. We thus have 
$$
\frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_X(p_n,q_n)} = \frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_Y(f(p_n),f(q_n))} \times \frac{d_Y(f(p_n),g(f(q_n)))}{d_X(p_n,q_n)},
$$
and taking the limit as $n \to \infty$ we obtain \iref{eqDilLower1} which concludes the proof of this lemma.
\sq

Let $f: \Omega \to V$ be a $C^1$ function, where $\Omega\subset \R^d$ is an open set and $V$ is a Banach space. Then for any $z\in \Omega$ the local dilatation $\dil_z(f)$, and the lower dilatation $\dil_z^*(f)$ only depend on the differential $d_z f : \R^d \to V$ of $f$ at $z$
\be
\label{eqDilDiff}
\dil_z(f) = \sup_{|u|=1} \|d_z f(u)\| \stext{ and } \dil_z^*(f) = \inf_{|u|=1} \|d_z f(u)\|
\ee
Applying Lemma \ref{lemmaSubMult} and \iref{eqDilDiff} to the function $g=\ln$ we obtain for any metric space $(X,d_X)$, any $f\in C^0(X,\R_+^*)$ and any $x\in X$
\be
\label{eqDilLog}
\dil_x(\ln f) = \frac {\dil_x(f)} {f(x)} .
\ee

The following proposition shows that, under certain circumstances, the Lipschitz property is a local property.
\begin{prop}
\label{propDilLoc}
Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$.
For any $f\in C^0(\R^d, Y)$ and any path $\gamma\in C^1([0,1], \R^d)$, $\gamma(0) = z$, $\gamma(1) = z'$, one has
\be
\label{eqLipLocPath}
d_Y(f(z), f(z')) \leq l_H(\gamma) \sup_{0\leq t \leq 1} \dil_{\gamma(t)}(f).
\ee
It follows that %In particular 
\be
\label{eqDilLoc}
\dil(f) = \sup_{z\in \sR^d} \dil_z(f).
\ee
\end{prop}

\proof
%Consider $z,z'\in \R^d$, and a path $\gamma\in C^1([0,1],\R^d)$ such that $\gamma(0) = z$, $\gamma(1)=z'$ and $l_H(\gamma) \leq d_H(z,z')+\delta$ where $\delta>0$ is a constant that is devoted to tend to zero in the last step of the proof.
We equip the segment $[0,1]$ with the distance $d_\gamma$ defined for $0 \leq t\leq t'\leq 1$ by 
\be
\label{defDGamma}
d_\gamma(t,t') = d_\gamma(t',t) = l_H(\gamma_{|[t,t']}).
\ee
Note that for any $t\leq t_* \leq t'$ one has 
\be
\label{exactTri}
d_\gamma(t,t') = d_\gamma(t,t_*)+d_\gamma(t_*,t')
\ee
The map $\gamma : ([0,1], d_\gamma) \to (\R^d, d_H)$ is clearly Lipschitz.
It thus follows from Lemma \ref{lemmaSubMult} that $F := f\circ \gamma :[0,1] \to Y$ satisfies for all $t\in [0,1]$
$$
\dil_t(F) \leq \dil_{\gamma(t)}(f) \leq \lambda := \sup_{0\leq t'\leq 1} \dil_{\gamma(t')}(f).
$$
We assume that $\lambda<\infty$, otherwise there is nothing to prove, and we consider a fixed $\delta>0$. For each $t\in [0,1]$ there exists therefore an interval $V_t\subset [0,1]$ containing $t$, relatively open in $[0,1]$, and such that $F_{|V_t}$ is $(\lambda+\delta)$-Lipschitz. Since the segment $[0,1]$ is compact, there exists a finite set $I_0\subset [0,1]$ such that 
$$
[0,1] = \bigcup_{t\in I_0} V_t.
$$
Let $V,V'\subset [0,1]$ be two intersecting intervals, and assume that $F$ is $\lambda+\delta$ Lipschitz on $V$ and on $V'$. For any $t\in V$ and $t'\in V'$, there exists $t_*\in V\cap V'$ which satisfies $t\leq t_*\leq t'$ or $t\geq t_* \geq t'$. Recalling \iref{exactTri} we thus obtain  
\begin{eqnarray*}
d_Y(F(t),F(t')) &\leq& d_Y(F(t), F(t_*))+d_Y(F(t_*), F(t')) \\
&\leq& (\lambda+\delta) d_\gamma(t,t_*)+( \lambda+\delta)d_\gamma(t_*,t') \\
&=& (\lambda+\delta)d_\gamma(t,t').
\end{eqnarray*}
Thus $F$ is $\lambda+\delta$ Lipschitz on the interval $V\cup V'$. Since $[0,1]$ is covered by a finite collection of open intervals on which $F$ is $\lambda+\ve$ Lipschitz, we obtain proceeding by induction that $F$ is $(\lambda+\delta)$-Lipshitz on $[0,1]$ and therefore 
$$
d_Y(f(z),f(z')) = d_Y(F(0),F(1))\leq (\lambda+\delta) d_\gamma(0,1) = (\lambda+\delta)l_H(\gamma). %\leq (\lambda+\delta)(d_H(z,z')+\delta).
$$
Letting $\delta\to 0$ we obtain \iref{eqLipLocPath}. Taking the infimum of \iref{eqLipLocPath} among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_Y(f(z),f(z')) \leq  \lambda d_H(z,z')$. Therefore $f : (\R^d, d_H) \to (Y,d_Y)$ is $\lambda$-Lipschitz, which concludes the proof of this proposition.
%The upper inequality $\geq$ is a direct consequence of the definition \iref{defDilX} of the local dilatation, and we therefore turn to the lower inequality $\leq$.
\sq

The next corollary shows that the global dilatation is controlled by the local dilatation even if the latter is not known on a \emph{sufficiently thin} set $\Gamma$, such as the skeleton of a mesh.

\begin{corollary}
\label{corolLipNoGamma}
Let $\Gamma\subset \R^d$ be a set which has the following property : for any path $\gamma\in C^1([0,1], \R^d)$ there exists a sequence of path $(\gamma_n)_{n \geq 0}$ which converge to $\gamma$ in $C^1$ norm and such that  $\{t\in [0,1]\sep \gamma_n(t) \in \Gamma\}$ is finite for each $n$.\\
Let $H\in \bH$, let $(Y,d_Y)$ be an arbitrary metric space, and met let $f\in C^0(\R^d, Y)$.
Then 
$$
\dil(f) = \sup_{z\in \R^d \sm \Gamma} \dil_z(f).
$$
\end{corollary}

\proof
We denote $\lambda := \sup_{z\in \R^d \sm \Gamma} \dil_z(f)$.
We consider two points $z,z'\in \R^d$ and a path $\gamma\in C^1([0,1], \R^d)$ such that $\gamma(0) = z$ and $\gamma(1) = z'$. %, and a sequence $\gamma_n$ converging to $\gamma$ in $C^1$ norm.

We first assume that the set $\{t\in [0,1]\sep \gamma(t) \in \Gamma\}$ is finite, and we denote its elements by $t_1< \cdots < t_k$. We set by convention $t_0 = 0$ and $t_{k+1} = 1$.
For each $0\leq i \leq k$ and each $t,t'$ such that $t_i <t<t'<t_{i+1}$ we have $d_Y(f(\gamma(t)),f(\gamma(t'))) \leq \lambda l_H(\gamma_{|[t,t']})$. Letting $t\to t_i$ and $t'\to t_{i+1}$ we obtain $d_Y(f(\gamma(t_i)),f(\gamma(t_{i+1}))) \leq \lambda l_H(\gamma_{|[t_i,t_{i+1}]})$. Adding up we obtain 
$$
d_Y(f(z), f(z')) \leq \sum_{0\leq i \leq  k} d_Y(f(\gamma(t_i)), f(\gamma(t_{i+1}))) \leq \lambda
\sum_{0\leq i \leq k} l_H(\gamma_{[t_i, t_{i+1}]}) = \lambda l_H(\gamma).
$$

We now consider the case where $\gamma$ meets the set $\Gamma$ an infinite number of times, and we choose a sequence $\gamma_n$ as described above. We obtain $d_Y(f(\gamma_n(0)), f(\gamma_n(1))) \leq \lambda l_H(\gamma_n)$ for each $n\geq 0$. Since $\gamma_n \to \gamma$ in $C^1$ norm as $n \to \infty$ we obtain taking the limit $d_Y(f(z), f(z')) \leq \lambda l_H(\gamma)$.

Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ we obtain $d_Y(f(z), f(z')) \leq \lambda d_H(z,z')$, which concludes the proof of this proposition.
\sq


%Let $(Y, \|\cdot \|_Y)$ and $(Z, \|\cdot\|_Z)$ be two banach spaces. Let $y\in Y$, $g\in C^1(Y,Z)$, and $L = g'(f(x))$, then clearly 
%$$
%\dil_y(g) = \|L\|.
%$$
%Injecting this in \iref{eqDilUpper1} we obtain 
%\be
%\label{eqDilUpper2}
%\dil_x(g \circ f) \leq\|L\|  \dil_x (f).
%\ee
%We also need a lower bound in several cases. For that purpose we define 
%$$
%\dil^*_z(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(z,\ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)}\right),
%$$
%and we obtain proceeding similarly, but with the different convention $0\times \infty = \infty\times 0 = 0$
%$$
%\dil_z(g\circ f) \geq \dil^*_{f(z)}(g) \dil_z(f).
%$$

The next proposition establishes that the regularity conditions \iref{eqLipMult} and \iref{eqLipAdd} defining the collections of quasi-acute or graded metrics are equivalent in the case of a metric proportionnal to the identity. %$\bH_a$ $\bH_g$

\begin{prop}
\label{propEquivS}
Let $s\in C^0(\R^d, R_+^*)$ and let $H(z) := \Id/s(z)^2$ for all $z\in \R^d$. We have 
\be
\label{eqDilLnH}
\dil_z(\ln s\sep d_H) = \dil_z(s).
\ee
Hence the following properties are equivalent.
\begin{enumerate}
\item The map $s : \R^d \to \R$ is Lipschitz. (i.e. $H\in \bH_i$) %For all $z,z'\in \R^d$ one has $|s(z)-s(z')|\leq |z-z'|$.
\item (``Additive'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_+(H(z),H(z')) \leq |z-z'|$.
\item (``Multiplicative'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_\times(H(z),H(z'))\leq d_H(z,z')$.
\end{enumerate}
\end{prop}

\proof %reprendre preuve??
Combining \iref{eqDilNorm} and \iref{eqDilLog} we obtain for any $z\in \R^d$
$$
%\dil_z (H\sep  d_\times, d_H) = 
\dil_z(\ln s\sep d_H) = s(z) \dil_z(\ln s) = \dil_z(s),
$$
which establishes \iref{eqDilLnH}.
According to \iref{eqDIso} we have for any $z,z'\in \R^d$
$$
d_+(H(z),H(z')) = |s(z) - s(z')| \stext{ and } d_\times (H(z),H(z')) = |\ln s(z) - \ln s(z')|.
$$
The properties 1. and 2. are thus equivalent to $\dil(s)\leq 1$, and therefore also to 
\be
\label{eqDilsLoc}
\dil_z(s) \leq 1 \text{ for all } z\in \R^d.
\ee
according Proposition \ref{propDilLoc} applied to the constant metric $H_0 = \Id$ and to the function $f=s$.
On the other hand property 3. is equivalent to $\dil(\ln s \sep d_H) \leq 1$, and thus to 
$$
\dil_z(\ln s\sep d_H) \leq 1 \text{ for all } z\in \R^d
$$
according to Proposition \ref{propDilLoc} applied to the metric $H$ and to the function $f=\ln s$.
This property equivalent to \iref{eqDilsLoc} according to \iref{eqDilLnH}, which concludes the proof of this Proposition.
\sq

The next corollary uses Proposition \ref{propEquivS} to analyse the regularity of the first and last eigenvalue of a metric.
\begin{corollary}
\label{corolLipNorm}
\begin{itemize}
\item
For any $H\in \bH_g$, the map $z\mapsto \|H(z)\|^{-\frac 1 2}$ is Lipschitz.
\item
For any $H\in \bH_a$, the map $z\mapsto \|H(z)^{-\frac 1 2}\|$ is Lipschitz.
\end{itemize}
\end{corollary}
\proof
\begin{itemize}
\item 
%For any $M,M'\in S_d^+$ we have 
%\begin{eqnarray*}
%d_\times(M,M') &=& \ln \left(\max\left\{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\right\}\right) \\
%&\geq &\ln \left(\max \left\{\frac{\|M^\frac 1 2\|}{\|M'^{\frac 1 2}\|}, \, \frac{\|M'^{\frac 1 2}\|}{\|M^{\frac 1 2}\|}\right\}\right)\\
%& = & \frac 1 2 \left|\ln \|M\| - \ln \|M'\|\right|.
%\end{eqnarray*}
Consider $H\in \bH_g$, define $s(z) := \|H(z)\|^{-\frac 1 2}$ and 
$$
H'(z) := \frac \Id {s(z)^2} = \|H(z)\|\Id.
$$
Since $H(z) \leq H'(z)$ for all $z\in \R^d$, we have $d_H(z,z') \leq d_{H'} (z,z')$ for all $z, z'\in \R^d$.

Consider a pair $M,M'\in S_d^+$ of matrices and a real $\delta>0$. If $e^{-2\delta} M \leq M' \leq e^{2\delta} M$, then taking the norm we obtain $e^{-2\delta} \|M\| \leq \|M'\| \leq e^{2\delta} \|M\|$. It follows that 
$$
\frac 1 2 |\ln \|M\| - \ln \|M'\|| \leq d_\times (M,M').
$$
We thus have for any $z,z'\in \R^d$
\begin{eqnarray*}
|\ln s(z)-\ln s(z')| &=& \frac 1 2 \left|\ln \|H(z)\| - \ln \|H(z')\|\right| \\ %\left|\ln \left(\sqrt{\|H(z)\|}\right) -\ln \left(\sqrt{\|H(z')\|}\right)\right| \\%
%& \leq & \sup_{u\neq 0} |\ln \|u\|_{H(z)} - \ln \|u\|_{H(z')}|\\
&\leq & d_\times(H(z),H(z')) \\
&\leq& d_H(z,z')\\
&\leq& d_{H'}(z,z').
\end{eqnarray*}
Applying Proposition \ref{propEquivS} to the metric $H'$ we obtain that $H'\in \bH_i$, and therefore that $s$ is Lipschitz as announced.
\item
Consider $H\in \bH_a$. We have for any $z,z'\in \R^d$
$$
\left|\|H(z)^{-\frac 1 2}\| - \|H(z')^{-\frac 1 2}\| \right| \leq \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| \leq |z-z'|,
$$
which concludes the proof of this corollary.\sq
\end{itemize}

Our last proposition studies the local dilatation of the maximum and the minimum of two functions.
\begin{prop}
\label{propDilMax}
Let $(X,d_X)$ be a metric space and let $\lambda, \mu\in C^0(X, \R)$. Let $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda, \mu\}$. Then for all $x\in X$
\be
\label{eqDilMax1}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} \leq \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
If $(X,d_H) = (\R^d, d_H)$, where $H \in \bH$ is a riemannian metric, then equality holds
\be
\label{eqDilMax2}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} = \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
\end{prop}

\proof
We have for any $p,q\in X$,
\begin{eqnarray*}
|\gamma(p)-\gamma(q)| &=& |\min\{\lambda(p), \mu(p)\} - \min \{\lambda(q), \mu(q)\}|\\
& \leq & \max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}.
\end{eqnarray*}
For any $x\in X$ and any $\ve>0$ we thus obtain
\begin{eqnarray*}
\dil(\gamma_{|B(x,\ve)}) &=& \sup_{p,q\in B(x,\ve)} \frac{|\gamma(p)-\gamma(q)|}{d_X(p,q)} \\
&\leq& \sup_{p,q\in B(x,\ve)} \frac{\max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}}{d_X(p,q)}\\
& =& \max\left\{\sup_{p,q\in B(x,\ve)}  \frac{|\lambda(p)-\lambda(q)|}{d_X(p,q)}, \sup_{p,q\in B(x,\ve)}  \frac{|\mu(p)-\mu(q)|}{d_X(p,q)}\right\}\\
&=& \max\left\{\dil(\lambda_{|B(x, \ve)}), \dil(\mu_{|B(x,\ve)})\right\}.
\end{eqnarray*}
Letting $\ve \to 0$ we obtain $\dil_x(\gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$. Likewise $\dil_x(\Gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$ which concludes the proof of \iref{eqDilMax1}.

We now turn to the proof of \iref{eqDilMax2}. For that purpose we consider a fixed $\ve>0$ and we define
$$
r := \max \{\dil(\gamma_{|B(x,\ve)}\sep \|\cdot\|_{H(x)}), \ \dil(\Gamma_{|B(x,\ve)} \sep \|\cdot\|_{H(x)})\},
$$
where $B(x,\ve)$ stands for the euclidean unit ball of radius $\ve$ centered at $x$.
Consider two points $p,q\in B(x,\ve)$. If $\lambda(p) \geq \mu(p)$ and $\lambda(q)\geq \mu(q)$, or if $\lambda(p) \leq \mu(p)$ and $\lambda(q)\leq \mu(q)$, then 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)|&=& \max \{|\gamma(p)-\gamma(q)|, |\Gamma(p)-\Gamma(q)|\}\\
&\leq & \|p-q\|_{H(x)}
\end{eqnarray*}
Otherwise if  $\lambda(p) \geq \mu(p)$ and $\lambda(q)\leq \mu(q)$, or $\lambda(p) \leq \mu(p)$ and $\lambda(q)\geq \mu(q)$, then there exists a point $r$ on the segment $[p,q]$ such that $\lambda(r)=\mu(r)$. We thus have %$|p-r|+|r-q| = |p-q|$ and 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)| &\leq& \max \{|\gamma(p)-\gamma(r)|, |\Gamma(r)-\Gamma(q)|\}\\
& &+ \max \{|\gamma(r)-\gamma(q)|, |\Gamma(r)-\Gamma(q)|\}\\
& \leq & \|p-r\|_{H(x)} + \|r-q\|_{H(x)} = \|p-q\|_{H(x)}
\end{eqnarray*}
If follows that $\dil(\lambda_{|B(x,\ve)}\sep \|\cdot\|_{H(x)})\leq r$, and letting $\ve\to 0$ we obtain 
$$
\dil_x(\lambda\sep \|\cdot\|_{H(x)}) \leq \max\{\dil_x(\gamma\sep \|\cdot\|_{H(x)}), \ \dil_x(\Gamma \sep \|\cdot \|_{H(x)})\}.
$$ 
Recalling that $\dil_x(f\sep d_H) = \dil_x(f\sep \|\cdot\|_x)$ for any $f\in C^0(\R^d, \R)$ and any for all $x\in \R^d$, see \iref{eqDilNorm}, we obtain $\dil_x(\lambda) \leq \max\{\dil_x(\gamma), \ \dil_x(\Gamma)\}$. Proceeding likewise for $\mu$ we obtain \iref{eqDilMax2} which concludes the proof of this proposition.
\sq

\subsection{Geometric properties of the space $(\R^d, d_H)$} %Estimates of size}
\label{subsecMetGeom}

We focus in this subsection on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. The next proposition compares the riemannian distance $d_H$ between two points $z$ and $z+u$ with the norm $\|u\|_{H(z)}$ of their difference.

%with the euclidean distance and we estimate the volume of balls. 
%The next proposition compares the Riemannian distance associated to a graded metric, with 

\begin{prop}
\label{propEuclidRiemann}
Let $H \in \bH_g$ and let $z\in \R^d$. For all $u\in \R^d$ one has
\be
\label{eqEuclidRiemann}
\ln(1+\|u\|_{H(z)}) \leq d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention when $\|u\|_{H(z)}\geq 1$.
\end{prop}
\proof
%We first prove the left part of \iref{eqEuclidRiemann}, and for that purpose
We consider a path $\gamma\in C^1([0,1], \R^d)$, and we define for each $t\in [0,1]$
\be
\label{defLGamma}
l(t) := \int_0^t \|\gamma'(t)\|_{H(\gamma(t))}dt.
\ee
Since $H\in \bH_g$ we have for any $t\in [0,1]$
$$
\exp(-2\, d_H(z, \gamma(t))) \, H(z) \leq H(\gamma(t)) \leq  \exp(2 \, d_H(z, \gamma(t))) \, H(z)
$$
therefore, since $d_H(z, \gamma(t)) \leq l(t)$,
$$
\exp(-2l(t)) H(z)  \leq H(\gamma(t)) \leq  \exp(2l(t)) H(z).
$$
It follows that 
$$
\|\gamma'(t)\|_{H(z)} \exp(-l(t)) \leq l'(t) = \|\gamma'(t)\|_{H(\gamma(t))} \leq  \|\gamma'(t)\|_{H(z)} \exp(l(t)), %\exp(-l(t))
$$
hence 
\be
\label{eqGammapLp}
-\frac d {dt} \exp(-l(t)) \leq \|\gamma'(t)\|_{H(z)} \leq \frac d {dt} \exp(l(t)).
\ee
We have 
\be
\label{eqGammaGammap}
\|u\|_{H(z)} =  \|\gamma(1)-\gamma(0)\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt
\ee
with equality if $\gamma(t) = z+tu$ is the straight line.
%We now assume that $\gamma(t) \neq \gamma(0)$ for all $t\in (0,1]$, which is the case generically. The map $t\mapsto \|\gamma(t)-\gamma(0)\|_{H(z)}$ is therefore $C^1$ on $(0,1]$ and we have 
%$$
%\frac d {dt} \|\gamma(t)-\gamma(0)\|_{H(z)} \leq \|\gamma'(t)\|_{H(z)},
%$$
%with equality if $\gamma(t)-\gamma(0) = c \gamma'(t)$ for some $c>0$.
%In the special case of the straight line $\gamma(t)=z+tu$, \iref{eqGammaGammap} is an equality and we thus obtain 
In that case, integrating the left part of \iref{eqGammapLp} we obtain
$$
 1-\exp(-l_H(\gamma)) = -\int_0^1 \left(\frac d {dt} \exp(-l(t))\right)dt   \leq  \int_0^1 \|\gamma'(t)\|_{H(z)} dt %= \|\gamma(1)-\gamma(0)\|_{H(z)} \exp(-l(0)) - \exp(-l(1))
 = \|u\|_{H(z)}.
$$
Rearranging the terms we obtain the right part of \iref{eqEuclidRiemann}:
$$
d_H(z,z+u) \leq l_H(\gamma) \leq -\ln(1-\|u\|_{H(z)}).
$$
We now consider an arbitrary path $\gamma$ joining $z$ and $z+u$ and we obtain integrating the right part of \iref{eqGammapLp} and recalling \iref{eqGammaGammap}
$$
\exp(l_H(\gamma)) -1 = \int_0^1 \left(\frac d {dt} \exp(l(t))\right) dt  \geq \int_0^1 \|\gamma'(t)\|_{H(z)} dt \geq \|u\|_{H(z)},
$$
which is equivalent to
$$
l_H(\gamma) \geq \ln(1+\|u\|_{H(z)}).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ satisfying $\gamma(0) = z$ and $\gamma(1) = z+u$, we obtain the left part of \iref{eqEuclidRiemann}, which concludes the proof of this proposition.
\sq

We discuss in the rest of this section the consequences of the comparison \iref{eqEuclidRiemann} of the riemannian distance $d_H$ with the distance associated to the norm $\|\cdot\|_{H(z)}$ when $H\in \bH_g$. %is devoted to 
Combining the right part of \iref{eqEuclidRiemann} with the expression \iref{eqDTimesLog} of the distance $d_\times$ we obtain an estimate of the local variations of the norm $\|\cdot \|_{H(z)}$ associated to the metric $H$ at a point $z$: let $H\in \bH_g$, and let $z,u,v\in \R^d$ be such that $\|u\|_{H(z)} < 1$, then
\be
\label{eqLocalNorm}
(1-\|u\|_{H(z)}) \|v\|_{H(z)} \leq \|v\|_{H(z+u)} \leq (1-\|u\|_{H(z)})^{-1} \|v\|_{H(z)}. %\frac{\|v\|_{H(z)}}{1-\|u\|_{H(z)}}.
\ee
Note also that 
\be
\label{eqLocalDet}
(1-\|u\|_{H(z)})^d \sqrt{\det H(z)} \leq \sqrt{\det H(z)} \leq (1-\|u\|_{H(z)})^{-d} \sqrt{\det H(z)}.
\ee
Another important consequence of \iref{eqEuclidRiemann} is that the closed balls $\{z'\in \R^d \sep d_H(z,z')\leq r\}$ for the distance $d_H$, are closed and bounded subsets $\R^d$, hence are compact. %From this point a classical argument (??) shows that $(R^d,d_H)$ is a complete metric space.

The following example establishes that \iref{eqEuclidRiemann} is a sharp inequality. The metric $H$ defined by 
$$
H(z) := \frac \Id {(1+|z|)^2}
$$
belongs to $\bH_i$ since $z\mapsto 1+|z|$ is Lipschitz, hence $H$ also belongs to $\bH_a$ and $\bH_g$.
For any $v\in \R^d$, one easily checks that the path of minimal length joining $0$ to $v$ is the straight line, and that
$$
d_H(0, v) = \ln(1+|v|).
$$
Choosing $z=0$ and $u=v$ we obtain that the left part of \iref{eqEuclidRiemann} is sharp
$$
\ln (1+ \|u\|_{H(0)}) = \ln (1+ |u|) = d_H(0,0+u).
$$
Choosing $z=-v$ and $u = v$ we obtain that the right part of \iref{eqEuclidRiemann} is sharp
$$
-\ln\left(1-\|u\|_{H(-u)} \right) = -\ln \left(1-\frac {|u|}{1+|u|}\right) = \ln(1+|u|) = d_H(-u, -u+ u).
$$

The next corollary uses Proposition \ref{propEuclidRiemann} to obtain a lower bound for the mass of balls in the measure $z\mapsto \sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. %states a volume estimate Proposition \ref{propLength} implies a volume estimate. %also allows us to compare the vo
\begin{corollary}
\label{corolVol}
There exists $c=c(d)>0$ such that the following holds. Let $H \in \bH_g$,
let $L\geq 1$ and let $z_0\in \R^d$. Denoting $\cE$ the ellipse 
$$
\cE = \{z\in \R^d\sep \|z-z_0\|_{H(z_0)}\leq L\}.
$$ 
we have 
\be
\label{eqVolLog}
\int_\cE \sqrt{\det H} \geq c \ln L. %\max\{L,1\}.
\ee
%Then 
%$$
%\int_\cE \sqrt {\det H} \geq c \ln L -1
%$$
%where $c=...$
%In particular if $H(z)\geq \lambda^2\Id$ (*$\|u\|_{H(z)} \geq \lambda |u|$ for all $u\in \R^d$*) then 
%\be
%\label{volBR}
%\int_{B(z,r)} \sqrt{\det H} \geq c \ln \max\{\lambda r, 1\}
%\ee
\end{corollary}

\proof
It follows from Proposition \ref{propEuclidRiemann} that $d(z_0, z) \geq \ln (L+1)$ for all $z\in \partial \cE$. We define the integer 
$$
k = \left\lfloor \ln(L+1) -\frac 1 2\right\rfloor,
$$
and we consider $k$ points $z_1, \cdots , z_k \in E$ such that for all $0 \leq i \leq k$
$$
d_H(z_0, z_i)= i.
$$
We define 
$
r_0 := 1-e^{-\frac 1 2} = 0.39\cdots
$
in such way that 
$$
-\ln (1-r_0) = \frac 1 2.
$$
For all $0 \leq i \leq k$ we denote by $\cE_i$ the ellipse 
$$
\cE_i  := \left\{z\in \R^d \sep \|z-z_i\|_{H(z_i)} \leq r_0\right\}.
$$
We have $\cE_i \subset \cE$ for all $0 \leq i \leq k$, indeed for any $z\in \cE_i$ we have 
$$
d_H(z_0, z) \leq d_H(z_0, z_i) + d_H(z_i, z) \leq i- \ln (1-r_0) \leq k+\frac 1 2 \leq \ln (L+1),
$$
Denoting by $\interior(E)$ the interior of a set $E\subset \R^d$, we observe that for all $0 \leq i<j\leq k$, for all $z\in \interior(\cE_i)$ and $z'\in \interior(\cE_j)$, we have
$$
d_H(z,z') \geq d_H(z_i, z_j) -d_H(z_i, z) - d_H(z_j,z') > |d_H(z_0, z_i) - d(z_0, d_j)| + 2\ln(1 -r_0) =0, %\geq 1+ 2 \ln(1-\frac 1 3)>0.
$$
hence $\interior(\cE_i) \cap \interior(\cE_j) = \emptyset$.
It follows that 
$$
\int_\cE \sqrt{\det H} \geq \sum_{0 \leq i \leq k} \int_{\cE_i} \sqrt{\det H}.
$$
Furthermore we have for all $z\in \cE_i$
$$
H(z) \geq (1-\|z-z_i\|_{H(z_i)})^2 H(z_i)  \geq (1-r_0)^2 H(z_i),
$$
and therefore 
\be
\label{eqzzi}
\sqrt{\det H(z)} \geq (1-r_0)^d \sqrt{\det H(z_i)}.
\ee
We denote by $B(z,r)$ the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$, and we observe that 
$u\mapsto z_i + H(z_i)^{-\frac 1 2} u$ maps $B(0,r_0)$ onto $\cE_i$. Combining this remark with \iref{eqzzi} we obtain
\begin{eqnarray*}
\int_{\cE_i} \sqrt{\det H} &\geq& (1-r_0)^d \int_{\cE_i} \sqrt{\det H(z_i)} \\
&=& (1-r_0)^d \int_{B(0,r_0)} 1 \\
&=& c_0 := r_0^d (1-r_0)^d |B(0,1)|.
\end{eqnarray*}
%where $B(z,r)$ denotes the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$.
Eventually we obtain 
$$
\int_\cE \sqrt{\det H} \geq (k+1) c_0 \geq (\ln(L+1) - 1/2) c_0.
$$
In order to obtain \iref{eqVolLog} we simply recall that $L\geq 1$ and therefore that %Since Recalling that $L\geq 1$ we find that 
$$
\ln (L+1) = \frac{\ln(L+1)}{2 \ln 2} +  \left(1-\frac 1 {2 \ln 2}\right)\ln(L+1) \geq \frac 1 2 + \left(1-\frac 1 {2 \ln 2}\right)\ln L $$
which concludes the proof of \iref{eqVolLog} with $c=(1- 1/(2 \ln 2))c_0$.
%Applying \iref{eqVolLog} to $L = \lambda r$ we obtain \iref{volBR} which concludes the proof of this proposition.
\sq


\section{Metrics having an eigenspace of dimension $d-1$ at each point}
\label{secEigen}
We focus in this subsection on metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has an eigenspace of dimension at least $d-1$ at each point $z\in \R^d$. 
%If the dimension is $d=2$, then a metric $H\in \bH$ generically satisfies this condition on a dense subset of $\R^d$. %any metric $H\in \bH$ satisfies this condition. 
This condition clearly holds if the dimension is $d=2$, but is also relevant in higher dimension. 
Indeed, as discussed in \S\ref{secOptGeom} of Chapter \ref{chapApproxMet}, this type of metrics appears when one needs to create mesh containing a thin layer of simplices close to an hypersurface $\Gamma$. In that case the matrix $H(z)$ at a point $z\in \Gamma$ typically has an eigenspace of dimension $d-1$ which is tangent to $\Gamma$ and is associated to a small eigenvalue, and an eigenspace of dimension $1$ in the direction orthogonal to $\Gamma$ associated to a large eigenvalue. 

The main result of this section is Theorem \ref{th2Spaces} which characterises those of these metrics which belongs to $\bH_a$ or $\bH_g$ in terms of the regularity of their eigenvalues and of their eigenvectors.
Corollary \ref{corolHgToHa} to this theorem gives a simple procedure to obtain a quasi-acute metric from a graded metric $H$ such that $H(z)$ has an eigenspace of dimension $d-1$ at each point. \\

We denote by $\bbS := \{\theta\in \R^d \sep |\theta| = 1\}$ the unit sphere of $\R^d$, equipped with the distance 
$$
d_\bbS(\theta, \theta') := \arccos(\<\theta, \theta'\>).
$$
We denote by $\cA$ the space of parameters
$$
\cA := \R_+^*\times \R_+^*\times \bbS,
$$
and we define a map $\cS :\cA\to S_d^+$ as follows
\be
\label{defcS}
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
\ee
In any orthonormal basis $\cB$ of $\R^d$ which begins with the vector $\theta$ we have the following expression
$$
[\cS(\lambda, \mu, \theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda &0 & 0 & \cdots\\
0 & \mu & 0 & \cdots\\
0 & 0 & \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right).
$$
We also define for any $a = (\lambda, \mu, \theta)\in \cA$
$$
\cH(a) := \cS(a)^{-2} = \lambda^{-2} \theta \theta^\trans+ \mu^{-2}(1-\theta \theta^\trans).
$$
%If $M\in S_d^+$ has an eigenspace of dimension $d-1$ exactly, then 
%
%We denote by $S_{d*}^+$ the collection of symmetric positive definite matrices $M\in S_d^+$ which have an eigenspace of dimension exactly $d-1$.
%We also denote by $\cA^*$ the collection of $(\lambda, \mu, \pm\theta)\in \cA$ which satisfies $\lambda\neq \mu$ if $d>2$ (resp. $\lambda>\mu$ is the dimension is $d=2$).
%Then
%$$
%\cH : \cA^* \to S_{d*}^+
%$$
%is a one to one map.



%Such a metric $H$ can be parametrized using two eigenvalues $\lambda, \mu\in \R_+^*$  and a subspace of dimension $d-1$ of $\R^d$ defined through an un-oriented unit normal $\pm \theta$. Our purpose in this section is to translate the fact that $H\in \bH_\star$, for some $\star\in \{i,a,g\}$, into simpler properties satisfied by $\lambda,\mu$ and $\theta$.
%
%
%
%In order to state our results, we need to introduce the collection $\cP$ of all hyperplanes of $\R^d$, also called the projective space. An hy
%
%
%We define the space of parameters
%$$
%\cA :=  \R_+^* \times \R_+^* \times \cP,
%$$
%where $\cP$ is the $d-1$-dimensional real projective space.
%For all $(\theta, \lambda, \mu)\in \cA$ we define 
%$$
%S( \lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans),
%$$
%and $H(\theta, \lambda, \mu) := S^{-2}$.
%The space $\cA$ is a differential variety, and the tangent space to a triplet $(\theta, \lambda, \mu)\in \cA$ is 
%$$
%T_{(\theta, \lambda, \mu)} \cA =  \R \times \R \times \theta^\perp,
%$$
%where $\theta^\perp$ refers to the orthogonal hyperplane to $\theta$ in $\R^d$.

For any metric $H \in \bH$ and any $z\in \R^d$ we denote by $\dil_z(H)_\times$ and $\dil_z(H)_+$ the local dilatations at $z$ associated to the Lipschitz conditions \iref{eqLipMult} and \iref{eqLipAdd} defining $\bH_g$ and $\bH_a$:
\be
\label{defDilH}
\dil_z(H)_\times := \dil_z(H \sep d_\times, d_H) \stext{ and } \dil_z(H)_+ := \dil_z(H \sep d_+).
\ee
We recall that the local dilatation $\dil_z(f)$ of a function $f$ at a point $z$ is defined by \iref{defDilX}.
%We set $D_z(H) := \dil(\lambda)$ if $z\notin \Omega$
For any open set $\Omega\subset \R^d$ and any $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$,  we define for all $z\in \Omega$
\be
\label{eqDZA}
D_z(a)_\times := \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \frac 1 2 \left| \frac {\lambda(z)} {\mu(z)} - \frac {\mu(z)} {\lambda(z)} \right|\dil_z(\theta\sep  d_H)\right\}, %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
and 
\be
\label{eqDZAP}
D_z(a)_+ := \max\left\{\dil_z(\lambda), \ \dil_z(\mu),\ |\lambda(z)-\mu(z)| \dil_z(\theta)\right\}. %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
Note that these quantities are not defined if $\lambda(z) = \mu(z)$ and $\dil_z(\theta\sep  d_H)=\infty$ simultaneously, since an indeterminate form $0\times \infty$ appears in \iref{eqDZA} and \iref{eqDZAP}.
\begin{theorem}
\label{th2Spaces}
Let $H \in \bH$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, such that $H = \cH\circ a$ on $\Omega$.
Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$. Then 
\be
\label{eqDilTimes}
D_z(a)_\times \leq \dil_z(H)_\times \leq 2D_z(a)_\times
\ee
and%, with $\gamma := \|H^{-\frac 1 2}\| = \max\{\lambda, \mu\}$, 
\be
\label{eqDilPlus}
D_z(a)_+ \leq \dil_z(H)_+ \leq 2D_z(a)_+.
\ee
%In particular, defining $\gamma := \|H(z)^{-\frac 1 2}\| = \max \{\lambda, \mu\}$ we have 
%\be
%\label{eqDilMax}
%\max\{\dil_z(\gamma), \, D_z(a)_\times\} \leq \max \{D_z(a)_+, \, D_z(a)_\times\} \leq 2\max\{\dil_z(\gamma), \, D_z(a)_\times\}.
%\ee
\end{theorem}

%The estimate \iref{eqDilPlus} on $\dil_z(H)_+$ is not very sharp, but this is not an issue since one usually does not needs to control $ \dil_z(H)_+$ but rather $\max\{\dil_z(H)_\times,\dil_z(H)_+\}$, for which we obtain combining \iref{eqDilTimes} and \iref{eqDilPlus} the sharper estimate 
%$$
% \max\{\dil_z(\gamma), D_z(a)\} \leq \max\{\dil_z(H)_\times,\dil_z(H)_+\} \leq 2 \max\{\dil_z(\gamma), D_z(a)\}.
%$$
The rest of this section is devoted to the proof of this theorem and to Corollary \ref{corolHgToHa}. Our first lemma defines and estimates a quantity $\Delta(a,b,c)$ which appears repeatedly in the rest of the proof.


\begin{lemma}
\label{lemmaDelta}
We define for all $a,b,c\in \R$ the quantity $\Delta(a,b,c)\in \R_+$, as follows % which is the norm of a $d\times d$ matrix,
\be
\label{defDelta}
\Delta(a,b,c) := 
\left\| 
\left(
\begin{array}{cccc}
a & b & 0 & \cdots\\
b & c& 0 & \cdots\\
0 & 0 & c & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right)
\right\|.
\ee
We have 
\be
\label{eqEstimM}
\max\{|a|, |b|, |c|\} \leq \Delta(a,b,c) \leq 2 \max\{|a|, |b|, |c|\}.
\ee
\end{lemma}

\proof
We consider fixed values of $a,b,c\in \R$ and we denote by $M$ the matrix presented in \iref{defDelta}, in such way that $\Delta(a,b,c) = \|M\|$. We also define $\lambda := \max\{|a|,|b|,|c|\}$.
We have 
$$
\Delta(a,b,c) = \|M\|\geq \max_{1\leq i,j\leq d} |M_{ij}| = \lambda,
$$
which establishes the left part of \iref{eqEstimM}. For all $p\in [1,\infty]$ we denote by $l^p$ the usual norm on $\R^d$ of exponent $p$. We have 
$$
\|M\|_{l^\infty\to l^\infty} = \max_{1 \leq i \leq d} \sum_{1\leq j \leq d} |M_{ij}| \leq 2 \lambda \stext{ and } \|M\|_{l^1\to l^1} = \max_{1 \leq j \leq d} \sum_{1\leq 1 \leq d} |M_{ij}| \leq 2 \lambda.
$$
By interpolation we thus obtain  
$$
\|M\| = \|M\|_{l^2\to l^2} \leq \sqrt{\|M\|_{l^1\to l^1} \|M\|_{l^\infty\to l^\infty} } \leq 2 \lambda,
$$
which concludes the proof.
\sq

The parameter space $\cA = \bbS \times \R_+^* \times \R_+^*$ is a differential variety, and the regularity of functions defined on $\cA$ should be seen through local charts.
For each $a = (\lambda, \mu, \theta)\in \cA$ we define a local chart $\psi_a$ of a neigborhood of $a$ in $\cA$ as follows: 
\be
\label{defPsia}
\psi_a : (-\lambda, \infty)\times (-\mu , \infty) \times (B(0,\cPi) \cap \theta^\perp) \to \cA
\ee
is defined by 
$$
\psi_a(\Lambda, M, r\Theta) := (\lambda+ \Lambda,\, \mu+ M,\, \cos(r) \theta + \sin(r) \Theta),
$$
where $|\Theta| = 1$. Note that $\psi_a$ is one to one and that $d_\bbS(\theta, \, \cos(r) \theta + \sin(r) \Theta) = r$.
In \iref{defPsia} we denoted by $\theta^\perp := \{\Theta\in \R^d \sep \<\theta, \Theta\> = 0 \}$ the space orthogonal to $\theta$, and $B(0,\cPi)$ the open euclidean ball of radius $\cPi$.
%it preserves distances in the following sense: if $(\lambda', \mu', \theta') = \psi_a(\Lambda, M, r\Theta)$ then $\lambda'-\lambda = \Lambda$, $\mu'-\mu=M$ and $

Let $V$ be a banach space. We say that a function $\vp : \cA \to V$ is $C^1$ if for any $a\in \cA$ the function $\vp\circ \psi_a$ is $C^1$.
In that case for any $a\in \cA$ we define the differential 
%and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
$$
d_a\vp(A) : \R\times \R\times \theta^\perp \to V
$$
by the formula
$$
d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( tA) - \vp(a)} t. %\Lambda, t M, t r\Theta
$$
We then have
 $$
\dil_a(\vp) = \|d_a(\vp)\|.
$$
%where $d_0 (\vp\circ \psi_a) :  \R\times \R\times \theta^\perp \to V$ denotes the differential of function $\vp\circ \psi_a$ at the origin $(0,0,0) \in (-\lambda, \infty)\times (-\mu , \infty) \times (B(\pi) \cap \theta^\perp)$.
%In that case for any $a\in \cA$ and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
%$$
%d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( t\Lambda, t M, t r\Theta) - \vp(a)} t,
%$$
%and we have for any path $\gamma\in C^1([0,1], \cA)$ 
%$$
%\vp(\gamma(1)) - \vp(\gamma(0)) = \int_0^1 d \vp_{\gamma(t)} (\gamma'(t)) dt.
%$$

\begin{prop}
\label{propPhiPlus}
Define $V_+ := S_d$, equipped with the standard norm $\|\cdot\|$, and define $\vp_+ (a) := \cS(a)$.
Then for all $a,b\in \cA$ we have 
\be
\label{eqDPPhiP}
d_+(\cH(a), \cH(b)) = \|\vp_+(a)-\vp_+(b)\|.
\ee
Furthermore $\vp_+ \in C^1(\cA, V_+)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
$$
\|d_a \vp_+(A)\|_\infty= 
\Delta(\Lambda, \ (\lambda-\mu) r ,\ M).
$$
\end{prop}

\proof
The \iref{eqDPPhiP} directly follows from the fact that $\cH(a)^{-1} = \cS(a)^2 = \vp_+(a)^2$, and from the definition \iref{defDPlus} of $d_+$.
The function $\vp_+ = \cS$ is $C^1$, and even $C^\infty$, since it has a polynomial expression 
$$
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
$$
We have at the first order in $\lambda, \mu, r$
\begin{eqnarray*}
\cS(\lambda+ \Lambda, \, \mu+M, \, \theta+r\Theta) &=&
 (\lambda+ \Lambda) (\theta+ r\Theta) (\theta+r\Theta)^\trans \\
 & &+ (\mu+M)(\Id - (\theta+ r\Theta) (\theta+r\Theta)^\trans)\\
 &=& S(\lambda, \mu, \theta) \\
 & &+ \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans)\\
& &+  \cO((|\Lambda|+ |M|+ |r|)^2)
\end{eqnarray*}
Therefore %$\vp_+$ is $C^1$ and 
\be
\label{eqDiffS}
%d_a\vp_+(\Lambda, \,M, \,r\Theta) = 
d_a\cS(\Lambda, \,M, \,r\Theta) =  \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans).
\ee
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[d_a\cS(\Lambda, \,M, \,r\Theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda & r(\lambda-\mu) & 0 & \cdots\\
r(\lambda-\mu) & M & 0 & \cdots\\
0 & 0 & M & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
which concludes the proof of this proposition.
\sq


\begin{prop}
\label{propPhiTimes}
Define $V_\times := C^0(\bbS, \R)$, equipped with the $\|\cdot\|_\infty$ norm, and define $\vp_\times : \cA \to V_\times$ as follows: for any $a\in \cA$ and any $u\in \bbS$
%\be
%\label{eqDTPhiT}
$$
\vp_\times (a) := (u \mapsto \ln \|u\|_{\cH(a)}).
$$
%\vp_\times (a)(u) = \ln \|u\|_{\cH(a)}.
%\ee
Then for all $a,b\in \cA$ we have 
\be
\label{eqDTPhiT}
\|\vp_\times(a)-\vp_\times(b)\|_\infty = d_\times(\cH(a), \cH(b)).
\ee
Furthermore $\vp_\times \in C^1(\cA, V_\times)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
\be
\label{eqNormDPhiPlus}
\|d_a \vp_\times(A)\|_\infty= 
\Delta\left(\frac \Lambda \lambda ,\ \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) ,\ \frac M \mu\right).
\ee
\end{prop}

\proof
Using the expression \iref{eqDTimesLog} of the distance $d_\times$ and the homogeneity of norms we obtain for any $M,M'\in S_d^+$,
$$
d_\times (M,M') = \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
$$
which implies \iref{eqDTPhiT}.
%The inequality \iref{eqDTPhiT} follows from the expression \iref{eqDTimesLog} of the distance $d_\times$.

As observed in the proof of Proposition \ref{propPhiPlus} the function $\cS : \cA\to S_d^+$ is $C^1$, and $d_a\cS(A)$ has the explicit expression \iref{eqDiffS}.
It is well known that the inverse map ${\rm Inv} : \GL_d \to \GL_d$ is $C^1$ and has the the following differential : for any $\phi\in \GL_d$ and any $\Phi\in M_d$
$$
d_\phi {\rm Inv} (\Phi) = \phi^{-1} \Phi \phi^{-1}.
$$
By composition, $\cS^{-1} : \cA \to S_d^+$ is also $C^1$, and for any $a=(\lambda, \mu , \theta)\in \cA$ and any $A\in \R\times \R \times \theta^\perp$
$$
d_a(\cS^{-1})(A) = S(a)^{-1} (d_a S(A) ) S(a)^{-1}.
$$
For any $u\in \bbS$ we have 
$$
\ln \|u\|_{\cH(a)} = \ln \|\cS(a)^{-1}u\| = \frac 1 2 \ln \left(\<\cS(a)^{-1}u,\cS(a)^{-1}u\>\right).
$$
Therefore, again by composition, 
\begin{eqnarray*}
d_a (\ln \|u\|_{\cH})(A) &=&  \frac 1 {2\|\cS(a)^{-1}u\|^2} (\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>\\
& &\quad +\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>)\\% \frac {\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>+\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>}{2\|\cS(a)^{-1}u\|^2}\\
&=& \frac{\<G(a,A) v,v\>}{\|v\|^2}
\end{eqnarray*}
where $v = \cS^{-1}(a)u$. The function $G$ has the following expression : for any $a = (\lambda, \mu, \theta)\in \R_+^* \times \R_+^* \times \bbS$ and any $A = (\Lambda, M, r\Theta)\in \R\times \R \times \theta^\perp$
\begin{eqnarray*}
G(a,A) &=& \frac{\cS(a)^{-1} (d_a\cS(A)) + (d_a\cS(A)) \cS(a)^{-1}} 2\\
&=& \frac \Lambda \lambda \theta \theta^\trans +  \frac M \mu (\Id - \theta \theta^\trans) + \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right)(\theta \Theta^\trans + \Theta \theta^\trans),
\end{eqnarray*}
the last expression follows from the explicit expression \iref{eqDiffS} of $d_a\cS(A)$ establishes in the proof of the previous proposition, and from the fact that $\theta^\trans \Theta = 0$.
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[G(a,A)]_\cB = 
\left(
\begin{array}{cccc}
\frac \Lambda \lambda & \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & 0 & \cdots\\
\frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & \frac M \mu & 0 & \cdots\\
0 & 0 & \frac M \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
The map $\vp_\times$ is differentiable, as the composition of differentiable maps, and we thus have
\begin{eqnarray*}
\|d_a \vp_\times(A)\|_\infty &=& \sup \left\{ \frac{|\<G(a,A) v,v\>|}{\|v\|^2} \sep u\in \bbS, \, v=\cS(a)^{-1} u\right\}\\
&=& \|G(a,A)\|,
\end{eqnarray*}
which establishes \iref{eqNormDPhiPlus} and concludes the proof of this proposition.
\sq

We now consider a fixed $z\in \Omega$ and we remark that 
$$
\dil_z(H)_\times = \dil_z(\cH\circ a)_\times  = \dil_z(\vp_\times \circ a\sep d_H). %\leq \dil_{a(z)} (\vp_+\sep d_z) \dil_z(a\sep d_H, d_z)
$$
Therefore,  according to Lemma \ref{lemmaSubMult} for any norm $\|\cdot\|_{a(z)}$ defined on the tangent space $\R\times \R \times \theta(z)^\perp$ to $a(z)\in \cA$ we have 
\be
\label{eqDilPhiA}
\begin{array}{rcl}
& &\dil^*_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} a\sep d_H, \|\cdot \|_{a(z)})\\
& \leq& \dil_z(H)_\times\\
& \leq& \dil_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} \circ a\sep d_H, \|\cdot\|_{a(z)})
\end{array}
\ee
provided no indeterminate $0\times \infty$ or $\infty \times 0$ appears on the first and last term of this inequality.
%We recall that a neighborhood of $a(z)$ is parametrized by the local chart 
%\be
%\label{defPsiAZ}
%\psi_{a(z)} : (\Lambda, M, r\Theta) \to (\lambda(z) + \Lambda, \, \mu(z) + M, \, \cos(r)\theta(z)+ \sin(r) \Theta)
%\ee
%where $|\Theta| = 1$. 
We consider a fixed point $z\in \Omega$, and we distinguish the two cases $\lambda(z) \neq \mu(z)$ and $\lambda(z) = \mu(z)$.

\paragraph{Proof in the case $\lambda(z) \neq \mu(z)$.}
For each $a=(\lambda, \mu, \theta)\in \cA$ we define a norm $\|\cdot \|_a$ on the tangent space $\R\times \R \times \theta^\perp$ to $\cA$ at the point $a$ : for all $A = (\Lambda, M , \Theta)\in \R\times \R \times \theta^\perp$
$$
\|A\|_a = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \frac 1 2 \left| \frac \lambda \mu - \frac \mu \lambda\right| \|\Theta\|\right\}.
$$
We have by construction 
\be
\label{eqDilADZDH}
\dil_z(\psi_{a(z)}^{-1}\circ a\sep d_H, \|\cdot \|_{a(z)}) = D_z(a)_\times
\ee
According to Lemma \ref{lemmaDelta} and Proposition \ref{propPhiTimes} we have for any $a=(\lambda, \mu, \theta)\in \cA$ and any $A\in \R\times\R \times \theta^\perp$
$$
\|A\|_a \leq \|d_a \vp_\times(A)\|_\infty = \|d_0 (\vp_\times \circ \psi_a)\|_\infty \leq 2 \|A\|_a.
$$
Since $\vp_\times$ is $C^1$ it follows from \iref{eqDilDiff} that 
$$
1 \leq \dil^*_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq \dil_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq 2.
$$
Combining \iref{eqDilPhiA}, \iref{eqDilADZDH} and the last inequality we obtain
$$
D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times,
$$
which establishes the announced result \iref{eqDilTimes} in the case $\lambda(z)\neq \mu(z)$. A similar reasoning establishes the counterpart \iref{eqDilPlus} of this ineaquality for the distance $d_+$. 

\paragraph{Proof in the case $\lambda(z) = \mu(z)$.}
%We now turn to the case of equality $\lambda(z) = \mu(z)$.
For any $\ve>0$ and any $a=(\lambda, \mu, \theta)\in \cA$ such that $\lambda = \mu$ we define a norm $\|\cdot\|_{a,\ve}$ on the tangent space $\R\times \R\times \theta^\perp$ to $a$ in $\cA$ as follows : 
$$
\|A\|_{a, \ve} = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \ve \|\Theta\|\right\}.
$$
%$$
%d_z^\ve((\Lambda, M, r\Theta), (\Lambda', M', r'\Theta')) := \max \left\{\frac {|\Lambda-\Lambda'|} {\lambda(z)},\, \frac {|M-M'|} {\mu(z)}, \, \ve \|r\Theta - r'\Theta'\|\right\}.
%$$
This modification is required because the original norm $\|\cdot\|_a$ used in the case $\lambda\neq \mu$ is only a semi-norm when $\lambda = \mu$.
Reasoning similarly to the case $\lambda(z) \neq \mu(z)$ we obtain the upper bound
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H), \ \ve\dil_z(\theta\sep  d_H)\right\}.
$$
We now establish a lower bound on $\dil_z(H)_\times$.
We may assume that $\dil_z(\theta \sep d_H) < \infty$ otherwise there is nothing to prove. Since $\ve>0$ is arbitrary we thus obtain 
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H)\right\} = 2D_z(a)_\times.
$$
We now turn to the lower bound on $\dil_z(H)_\times$. 
For that purpose we define the functions $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda,\mu\}$  and we observe that for all $z,z'\in \Omega$
\begin{eqnarray*}
d_\times (H(z),H(z')) &=& \ln \max \{\|H(z)^\frac 1 2 H(z')^{-\frac 1 2}\|, \, \|H(z')^\frac 1 2 H(z)^{-\frac 1 2}\|\}\\
&\geq & \frac 1 2 \max \{|\ln \|H(z)\|- \ln \|H(z')\||, \, |\ln \|H(z)^{-1}\|- \ln \|H(z')^{-1}\||\\
&=& \max \{ |\ln\gamma(z) - \ln \gamma(z')|,\, |\ln \Gamma(z) - \ln \Gamma(z')|\}.
\end{eqnarray*}
We thus obtain
$$
\dil_z(H)_\times = \dil_z(H\sep d_\times, d_H) \geq \max \{ \dil_z(\ln \gamma\sep d_H), \, \dil_z(\ln \Gamma \sep d_H)\}.
$$
Hence according to Proposition \ref{propDilMax}
$$
\dil_z(H)_\times \geq \max \{\dil_z(\ln \lambda\sep d_H), \dil_z(\ln \mu\sep d_H)\} = D_z(a)_\times.
$$
Therefore $D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times$, and proceeding likewise we obtain $D_z(a)_+ \leq \dil_z(H)_+ \leq 2 D_z(a)_+$, which concludes the proof of Theorem \ref{th2Spaces}. \\

The next corollary shows how a quasi-acute metric can be obtained from a graded one.
We denote by $\diag(\lambda_1, \cdots, \lambda_d)$ the diagonal matrix of entries $\lambda_1, \cdots, \lambda_d$. 
Let $M\in S_d$ and let $U\in \cO_d$ and $\lambda_1, \cdots , \lambda_d\in\R$ be such that 
\be
\label{eqDiagSd}
M = U^\trans \diag(\lambda_1, \cdots , \lambda_d) U
\ee
For any $\alpha\in \R$ we define the matrix $\max \{\alpha, M\}\in S_d^+$ as follows
$$
\max\{\alpha, M\} := U^\trans \diag(\max\{\alpha, \lambda_1\}, \cdots, \max\{\alpha, \lambda_d\})U,
$$
and we observe that $\max\{\alpha, M\}$ does not depend on the choice of the matrix $U$ and on the order of the eigenvalues $\lambda_1, \cdots, \lambda_d$ in the decomposition \iref{eqDiagSd}.
For instance we have for any $(\lambda, \mu, \theta)\in \cA$ and any $s>0$  
$$ %\lambda^{-2} \theta\theta^\trans+ \mu^{-2} (\Id-\theta \theta^\trans)
\max \{s^{-2}, \cH(a)\} = \min\{s, \lambda\}^{-2} \theta \theta^\trans+ \min\{s, \mu\}^{-2} (\Id-\theta \theta^\trans).
$$

\begin{corollary}
\label{corolHgToHa}
Let $H\in \bH$ be such that $H(z)$ has an eigenvalue of multiplicity $\geq d-1$ for all $z\in \R^d$. We define $s:\R^d\to \R_+^*$ and $H'\in \bH$ as follows : for all $z\in \R^d$
$$
s(z) := \inf_{z'\in \sR^d} |z-z'|+ \|H(z')^{-\frac 1 2}\|,
$$
and 
$$
H'(z) := \max\{s(z)^{-2}, H(z)\}.
$$
If $H\in \bH_g$, then $4^2H'\in \bH_a$.
\end{corollary}

\proof
For each $\ve>0$ we define 
$$
H_\ve := \max\{e^{2 \ve} s(z)^{-2}, H(z)\}.
$$
The proof proceeds as follows: we first establish that for any $z\in \R^d$ one has 
\be
\label{eqDilHe}
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
\ee
We then use these properties to obtain that $4^2 H_\ve \in \bH_a$, and we conclude the proof using the convergence $H_\ve \to H$ as $\ve \to 0$.\\

We first observe that $s : \R^d \to \R_+^*$ is Lipschitz and that $s(z)\leq \|H(z)^{-\frac 1 2}\|$ for all $z\in \R^d$.

Consider a fixed point $z\in\R^d$. If $H(z)$ is proportional to $\Id$, which means that $\|H(z)\|^{-\frac 1 2} = \|H(z)^{-\frac 1 2}\| \geq s(z)$, then $H_\ve = e^{2 \ve} \Id/ s^2$ on a neighborhood of $z$. This implies according to \iref{eqDilLnH} %\ref{PropEquivS}
$$
\dil_z(H_\ve)_\times =\dil_z(H_\ve)_+ = \dil_z(e^{-\ve} s) \leq e^{-\ve}\leq 1,
$$
and therefore \iref{eqDilHe}.
On the other hand if $H(z)$ is not proportional to $\Id$ then there exists three continuous functions $\lambda, \mu \in C^0(\R^d, \R_+^*)$ and $\theta \in C^0(\R^d, \bbS)$ (where $\bbS := \{u\in \R^d \sep |u| = 1\}$) such that 
$
H = \lambda^{-2} \theta \theta^\trans+ \mu^{-2} (\Id - \theta \theta^\trans).
$
on a neighborhood of $z$.
Hence on the same neighborhood of $z$, 
$$
H_\ve = \min\{e^{-\ve} s,\lambda\}^{-2} \theta \theta^\trans+ \min\{e^{-\ve} s,\mu\}^{-2} (\Id - \theta \theta^\trans).
$$

\paragraph{Proof that $\dil_z(H_\ve)_\times \leq 2$.}
We define $H_\ve^i := e^{2\ve} \Id/ s^2$ and we observe that $H_\ve \geq H_\ve^i$ and $H_\ve \geq H$, hence for any $p,q\in \R^d$
$$
d_{H_\ve}(p,q) \geq \max \{d_H(p,q), \, d_{H_\ve^i}(p,q)\}.
$$
Using Proposition \ref{propDilLoc} we thus obtain  
\begin{eqnarray*}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\} \sep d_{H_\ve}) &\leq& \max \{\dil_z(\ln (e^{-\ve} s)\sep d_{H_\ve}), \,\dil_z(\ln \lambda\sep d_{H_\ve})\}\\
&\leq & \max \{\dil_z(\ln(e^{-\ve} s \sep d_{H_\ve^i})), \,\dil_z(\ln \lambda\sep d_H)\}\\
& \leq & \max \{\dil_z(e^{-\ve} s), \, \dil_z(H)_\times\}\\
& \leq & \max \{e^{-\ve}, 1\} =1,
\end{eqnarray*}
where we used Theorem \ref{th2Spaces} and Proposition \ref{propEquivS} in the third line.
Likewise $\dil_z(\ln \min\{e^{-\ve} s, \lambda\}\leq 1$. 
Since the function 
$$
t \mapsto \frac t \mu - \frac \mu t
$$
is increasing, we easily obtain that
$$
\left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right| \leq \left|\frac \lambda \mu - \frac \mu \lambda\right|.
$$
Therefore   
$$
\frac 1 2 \left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right|  \dil_z(\theta \sep d_{H_\ve}) \leq \frac 1 2\left|\frac \lambda \mu - \frac \mu \lambda\right| \dil_z(\theta\sep d_H) \leq 1,
$$
which implies that $D_z(a_\ve)_\times \leq 1$ where $a_\ve=(\min\{e^{-\ve}s, \lambda\}, \min\{e^{-\ve} s, \mu\}, \theta) \in C^0(\R^d,\cA)$. Hence
$$
\dil_z(H_\ve)_\times \leq 2 D_z(a_\ve)_\times \leq 2,
$$
which concludes this paragraph.
\paragraph{Proof that $\dil_z(H_\ve)_+ \leq 4$.}
As already observed in \iref{eqDilNorm}, for any metric space $(X,d_X)$ and any function $f\in C^0(\R^d, X)$ we have 
\be
\label{eqDilNormLM}
\dil_z(f) \leq \|H(z)\|^{\frac 1 2}\dil_z(f\sep d_H) = \frac{\dil_z(f\sep d_H)}{\min\{\lambda(z), \mu(z)\}}.
\ee
If $\lambda(z)<\mu(z)$ we therefore obtain 
\begin{eqnarray*}
\dil_z(\min\{e^{-\ve} s , \lambda\}) &\leq& \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)}\right\}\\
 &\leq& \max \{e^{-\ve}, \, \dil_z(\ln \lambda\sep  d_H)\}\\
 &\leq & \max \{e^{-\ve} , \, 1\} = 1.
\end{eqnarray*}
Still assuming that $\lambda(z)<\mu(z)$, we have $s(z)\leq \|H(z)^{-\frac 1 2}\| \leq \mu(z)$ by construction of $s$, and therefore $\min\{e^{-\ve} s, \mu\} = e^{-\ve} s$ on a neighborhood of $z$. It follows that 
$$
\dil_z(\min\{e^{-\ve} s, \mu\}) = \dil_z(e^{-\ve} s)\leq e^{-\ve} \leq 1.
$$
Proceeding similarly if $\lambda(z)>\mu(z)$ we also obtain $\dil_z(\min\{e^{-\ve} s, \lambda\})$ and $\dil_z(\min\{e^{-\ve} s, \mu\})$. 
We now focus on the local dilatation of the orientation $\theta$, and for that purpose we observe that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}|  \leq  |\lambda(z) - \mu(z)|.
$$
Furthermore we have according to \iref{eqDilNormLM}
\begin{eqnarray*}
 |\lambda(z) - \mu(z)| \dil_z(\theta)
&\leq& \frac {|\lambda(z) - \mu(z)|}{\min\{\lambda(z), \mu(z)\}} \dil_z(\theta\sep d_H)\\
&=& \left(\frac {\max \{\lambda(z), \mu(z)\}}{\min\{\lambda(z), \mu(z)\}}-1\right)\dil_z(\theta\sep d_H)\\
& \leq & \left|\frac {\lambda(z)} {\mu(z)}-\frac {\mu(z)} {\lambda(z)}\right|\dil_z(\theta\sep d_H) \\
&\leq & 2 D_z(a)_\times \leq 2.
\end{eqnarray*}
We conclude that $D_z(a_\ve)_+ \leq 2$, and therefore $\dil_z(H_\ve)_+ \leq 4$.

\paragraph{Conclusion.}
We have established that for all $z\in \R^d$ and all $\ve>0$
$$
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
$$
Therefore for any $z,z'\in \R^d$, since $H_\ve \leq e^{2\ve} H'$,
$$
d_\times(H_\ve(z), H_\ve(z')) \leq 2d_{H_\ve}(z,z') \leq 2e^\ve d_{H'}(z,z') \stext{ and } d_+(H_\ve(z), H_\ve(z')) \leq 4|z-z'|.
$$
Letting $\ve \to 0$ we obtain 
$$
d_\times(H'(z), H'(z')) \leq 2d_{H'}(z,z') \stext{ and } d_+(H'(z), H'(z')) \leq 4|z-z'|.
$$
According to Remark \ref{remHomog} this implies that $4^2 H\in \bH_a$, which concludes the proof of this corollary.
\sq


\section{From mesh to metric}
\label{secMeshToMet}
The techniques presented in this section show how to produce an metric $H\in \bH_i$, $\bH_a$ or $\bH_g$ from an isotropic, quasi-acute (in two dimensions), or graded mesh $\cT$.

Combining the next proposition with its counterpart Proposition \ref{propMeshGen}, on the generation of a mesh from a metric, yields the main result of this chapter: Theorem \ref{thEquiv} on the equivalence of the classes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ of meshes and $\bH_i \subset \bH_a \subset \bH_g$ of metrics which is announced in the introduction.
\begin{prop}
\label{propMetGen}
For any $C_0>0$ there exits $C = C(C_0,d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $\cT \in \bT_{i, C_0}$ there exists $H \in \bH_i$ which is $C$-adapted to $\cT$.
\item If $d=2$, then for any $\cT \in \bT_{a, C_0}$ there exists $H \in \bH_a$ which is $C$-adapted to $\cT$.
\item For any $\cT \in \bT_{g,C_0}$ there exists $H \in \bH_g$ which is $C$-adapted to $\cT$.
\end{enumerate}
\end{prop}

The rest of this section is devoted to the proof of this proposition.
For any mesh $\cT\in \bT$, and for any vertex $v$ of $\cT$, we denote by $n_\cT(v)$ the number of simplices in the mesh $\cT$ containing $v$:
$$
n_\cT(v) := \#\{T\in \cT \sep v\in T\}. %, %\text{s.t. } 
$$
We denote by $H_\cT^g\in \bH$ the piecewise linear metric on $\cT$ which satisfies for each vertex $v$ of $\cT$
\be
\label{eqHcTg}
H_\cT^g(v) := \frac 1 {n_\cT(v)} \sum_{\substack{T\in \cT\\\text{s.t. } v\in T}} \cH_T.
\ee
The metric $H_\cT^g$ on a simplex $T\in \cT$ is simply the linear interpolation of the averages of the matrices $\cH_T$ attached to the simplices containing a vertex $v$. 

The next lemma establishes a property of the barycentric coordinates on a simplex, which is useful for the analysis of  the regularity of a piecewise linear function on an anisotropic mesh, such as the metric $H_\cT^g$.
\begin{lemma}
\label{lemmaNormLambda}
Let $T$ be a simplex and let $V$ be the collection of vertices of $T$. Let $\lambda_v(z)$, $v\in V$ be the barycentric coordinates on $T$. Then for all $z,z'\in T$
\be
\label{eqNormLambda}
\|z-z'\|^2_{\cH_T} = \frac {d+1} d \sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2.
\ee
\end{lemma}

\proof
We first assume that $T$ is the reference equilateral simplex $\TEq$. %, and we recall that $\cH_\TEq = \Id$.
For any two vertices $v,v'$ in the collection $\VEq$ of vertices of $\TEq$ one easily checks that 
\be
\label{eqScalTEq}
\<v,v'\> = 
\left\{
\begin{array}{cl}
1 &\text{ if } v=v,'\\
-1/d &\text{ if } v \neq v'.
\end{array}
\right.
\ee
Indeed $|v|=1$ by construction for any vertex $v$ of $\TEq$, the scalar product $\<v,v'\>$ has a value $\alpha$ which is independent of the pair of distinct vertices $v,v'\in \VEq$. Since $\TEq$ is centered at the origin we obtain $0 = \<v,\sum_{v\in V} v\>  = |v|^2 + d \alpha$ which establishes \iref{eqScalTEq}.
We thus obtain for any $z,z'\in \TEq$ 
\begin{eqnarray*}
|z-z'|^2  &=& \left|\sum_{v\in \VEq} (\lambda_v(z) - \lambda_v(z'))v\right|^2 \\
&=& \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \sum_{v\neq v'} (\lambda_v(z)-\lambda_v(z'))(\lambda_{v'}(z)-\lambda_{v'}(z')).
\end{eqnarray*}
Therefore 
$$
|z-z'|^2 =  \left(1+\frac 1 d\right) \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \left(\sum_{v\in \VEq} \lambda_v(z)-\lambda_v(z')\right)^2,
$$
which concludes the proof in the case of $\TEq$ since $\cH_\TEq = \Id$ and since the barycentric coordinates of $z$ and of $z'$ sum to $1$.

We now consider an arbitrary simplex $T$, and an affine change change of coordinates $\Phi$ such that $\Phi(T) = \TEq$, $\Phi(z) = \phi z+ z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. We have $\cH_T = \phi^\trans \phi$ according to \iref{invcH}, hence for all $z,z'\in T$
$$
 |\Phi(z) - \Phi(z')| = |\phi(z-z')| = \|z-z'\|_{\cH_T}.
$$
Furthermore the barycentric coordinates of $z$ and $z'$ in $T$ are the same as those of $\Phi(z)$ and $\Phi(z')$ in $\Phi(T) = \TEq$, hence \iref{eqNormLambda} holds which concludes the proof of this lemma.
\sq



The next proposition establishes that the metric $H_\cT^g$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case iii) of graded meshes. More precisely for any mesh $\cT\in \bT_{g,C_0}$ the metric $d C_0^{10} H_\cT^g$ belongs to $\bH_g$ and is $C_0^6 \sqrt d$ equivalent to $\cT$.



\begin{prop}
\label{propHTG}
For any $\cT\in \bT_{g,C_0}$ the metric $H_\cT^g$ is $C_0$-adapted to $\cT$, and $d C_0^{10} H_\cT^g\in \bH_g$.
\end{prop}

\proof
We consider a simplex $T\in \cT$, and we recall that for any neighbor $T'$ of $T$ one has 
$$
C_0^{-2} \cH_T \leq \cH_{T'} \leq C_0^2 \cH_T.
$$
Averaging these matrices as in \iref{eqHcTg} we obtain for any vertex $v$ of $T$
\be
\label{eqHTHv}
C_0^{-2} \cH_T \leq H_\cT^g(v)\leq C_0^2 \cH_T.
\ee
Averaging with respect to the barycentric coordinates of a point $z\in T$ we eventually obtain 
\be
\label{eqHTHz}
C_0^{-2} \cH_T \leq H_\cT^g(z)\leq C_0^2 \cH_T,
\ee
which establishes as announced that the metric $H_\cT^g$ is $C_0$-adapted to $\cT$.

We now establish the regularity property of $H_\cT^g$, and for that purpose we consider two points $z,z'\in T$ and a vector $u\in \R^d\sm\{0\}$. We thus have 
\begin{eqnarray*}
\frac {\|u\|^2_{H_\cT^g(z)}} {\|u\|^2_{H_\cT^g(z')}} &=& \frac {\sum_{v\in V} \lambda_v(z) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2} \\
&=& 1+ \frac {\sum_{v\in V} (\lambda_v(z)-\lambda_v(z')) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2}\\
&\leq& 1+ C_0^4 \frac{\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|}{\sum_{v\in V} \lambda_v(z')}\\
& \leq & 1+C_0^4 \sqrt {(d+1)\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2}\\
&=& 1+C_0^4 \sqrt d \| z-z'\|_{\cH_T},
\end{eqnarray*}
where we used \iref{eqHTHv} in the third line, Cauchy-Schwartz inequality in the fourth line, and Lemma \iref{lemmaNormLambda} in the fifth line.
We consider a simplex $T\in \cT$ and we intend to give a uniform bound on $\dil_z(H_\cT^g)_\times$ for all $z\in \interior(T)$. It follows from our estimate on $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, and from the analog estimate for  $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, that 
\begin{eqnarray*}
d_\times (H_\cT^g(z), H_\cT^g(z')) &=& \max_{u\neq 0} \left|\ln \|u\|_{H_\cT^g(z)} - \ln \|u\|_{H_\cT^g(z')}\right|\\
&\leq& \frac 1 2\ln (1+C_0^4 \sqrt d \|z-z'\|_{\cH_T}) \\
&\leq& \frac {C_0^4 \sqrt d} 2 \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Hence according to \iref{eqHTHz} and \iref{eqDilNorm} we obtain for all $z\in \interior (T)$
$$
\dil_z(H_\cT^g)_\times \leq C_0^5 \sqrt d.
$$
The metric $H := d C_0^{10} H_\cT^g$ thus satisfies $\dil_z(H)_\times = (dC_0^{10})^{-1/2}\dil_z(H_\cT^g)_\times \leq 1$ for any point $z$ in the interior of any simplex $T\in \cT$.

Let $z,z'\in \R^d$ and let $\gamma\in C^1([0,1], \R^d)$ be such that $\gamma(0) = z$ and $\gamma(1) = z'$.
There exists a sequence $(\ve_n)_{n \geq 0}$, $\ve_n \in \R^d$, $\ve_n \to 0$, such that for all $n \geq 0$ the translated path $\gamma+\ve_n$ intersects the skeleton 
$
\cup_{T\in \cT} \partial T
$
of the mesh $\cT$ only a finite number of times $0\leq t_1^n < \cdots < t_{k(n)}^n\leq 1$. Defining $t_0^n := 0$ and $t^n_{k(n)+1} := 1$, Proposition \ref{propDilLoc} states that for all $0\leq i \leq k(n)$ one has 
$$
d_\times (H(\gamma(t^n_i)+\ve_n), \, H(\gamma(t_{i+1})+\ve_n)) \leq l_H(\gamma_{|[t_1,t_{i+1}]}+\ve_n).
$$
Adding up these inequalities we obtain $d_\times (H(z+\ve_n), \, H(z'+\ve_n)) \leq l_H(\gamma+\ve_n)$, and therefore $d_\times (H(z), \, H(z')) \leq l_H(\gamma)$ as $n \to \infty$. Taking the infimum among all paths $\gamma$ joining $z$ and $z'$ we obtain $d_\times(H(z), H(z')) \leq d_H(z,z')$, hence $H \in \bH_g$ as announced which concludes the proof. 
\sq

We associate to any mesh $\cT\in \bT$ a metric $H_\cT^i$ defined as follows : for all $z\in \R^d$, 
$$
H_\cT^i(z) := \|H_\cT^g(z)\| \Id.
$$
The next result shows that $H_\cT^i$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case of isotropic metrics. More precisely for any mesh $\cT\in \bT_{i,C_0}$ the metric $d C_0^{10} H_\cT^i$ belongs to $\bH_i$ and is $C_0^7 \sqrt d$ equivalent to the mesh $\cT$.

\begin{corollary}
For any mesh $\cT\in \bT_{i,C_0}$ the metric $H_\cT^i$ is $C_0^2$-adapted to the mesh $\cT$, and $d C_0^{10} H_\cT^i \in \bH_i$.
\end{corollary}

\proof
For any matrix $M\in S_d^+$ we have $\|M^{-1}\|^{-1} \Id \leq M \leq \|M\| \Id$. We therefore obtain for any simplex $T\in \cT$
\be
\label{eqcHNormcH}
C_0^{-2} \|\cH_T\| \Id\leq \frac{\|\cH_T\|} {\rho(T)^2} \Id = \|\cH_T^{-1}\|^{-1} \Id \leq \cH_T \leq \|\cH_T\|\Id.
\ee
Let $T\in \cT$ and let $z\in T$. Since $\rho(T) \leq C_0$ and $C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z)$ we obtain 
$$
C_0^{-2} H_\cT^i(z) := C_0^{-2} \|H_\cT^g(z)\| \Id \leq \|\cH_T\| \Id \leq C_0^2 H_\cT^i(z).
$$
Combining this with \iref{eqcHNormcH} we obtain
$$
C_0^{-4} H_\cT^i(z) \leq \cH_T \leq C_0^2 H_\cT^i(z),
$$
which establishes as announced that the metric $H_\cT^i$ is $C_0^2$ equivalent to the mesh $\cT$.

According to Proposition \ref{propHTG} we have $d C_0^{10} H_\cT^g\in \bH_g$. Corollary \ref{corolLipNorm} thus implies that $d C_0^{10} H_\cT^i\in \bH_i$, which concludes the proof of this proposition.
\sq

Before turning to the case of quasi-acute metrics we prove a lemma on the neighborhood of a simplex in a graded mesh. For any mesh $\cT\in \bT$ and any closed set $E\subset \R^d$ the neighborhood $V_\cT(E)$ of $E$ in $\cT$ is  defined as the union of all simplices $T\in \cT$ which intersect $E$: 
$$
V_\cT(E) := \cup_{\substack{T\in \cT\\T \cap E \neq \emptyset}} T.
$$

\begin{prop}
\label{propNeighborT}
Let $\cT\in \bT_{g,C_0}$ and let $T \in \cT$, then for all $x\in T$ and all $y \in \R^d \sm V_\cT(T)$ we have 
$$
\|x-y\|_{\cH_T} \geq (C_0\sqrt d)^{-1}.
$$
\end{prop}

\proof
The simplex $T\in \cT$ is fixed throughout this proof. We consider the function $\vp : \R^d \to \R$ which is piecewise linear on the mesh $\cT$, and which satisfies for any vertex $v$ of the mesh $\cT$
$$
\vp(v) = 
\left\{
\begin{array}{cl}
1 & \text{ if } v\in T,\\
0 & \text{ if } v \notin T.
\end{array}
\right.
$$
We denote by $V'$ the collection of vertices of a simplex $T'\in \cT$, and by $(\lambda_v(z))_{v\in V'}$ the barycentric coordinates of a point $z\in T'$.
We have for any $z,z'\in T'$
\begin{eqnarray*}
|\vp(z)- \vp(z')| &\leq& \sum_{v \in V'} |\lambda_v(z)-\lambda_v(z')| \vp(v)\\
& \leq &\sqrt{(d+1) \sum_{v\in V'} |\lambda_v(z)-\lambda_v(z')|^2} \\
&= &\sqrt d \|z-z'\|_{\cH_{T'}}.
\end{eqnarray*}
Recalling that $\vp$ is identically $0$ on $T'$ if $T\cap T' = \emptyset$, and that $\cH_{T'} \leq C_0^2 \cH_T$ otherwise, we obtain for any $z,z'\in T'$
$$
|\vp(z)- \vp(z')| \leq C_0\sqrt d \|z-z'\|_{\cH_{T}}.
$$
We claim that $\vp : (\R^d, \|\cdot \|_{\cH_T})  \to \R$ is $C_0\sqrt d$-Lipschitz. Indeed consider $z,z'\in \R^d$, and denote by $z_1, \cdots, z_k$ the intersections of the segment $[z,z']$ with the skeleton $\cup_{T'\in \cT} \partial T'$ of the mesh. Defining $z_0 := z$ and $z_{k+1} := z'$ we obtain 
% generically a finite number. 
$$
|\vp(z)-\vp(z')| \leq \sum_{0 \leq i \leq k} |\vp(z_i)-\vp(z_{i+1})| \leq C_0 \sqrt d \sum_{0 \leq i \leq k} \|z_i - z_{i+1}\|_{\cH_T} =C_0 \sqrt d \|z-z'\|_{\cH_T}.
$$
For any $x\in T$ and any $y\in \R^d\sm V_\cT(T)$ we have $\vp(x) = 1$, $\vp(y) = 0$, thus $1 \leq C_0\sqrt d \|x-y\|_{\cH_T}$ which concludes the proof of this proposition.
\sq

We assume from this point that the dimension is $d=2$. %, and we thus restrict our attention to the bi-dimensional triangulations.
For each triangulation $\cT\in \bT$ we define a function $s_\cT : \R^2 \to \R_+^*$ as follows 
$$
s_\cT(z) := \inf_{z'\in \sR^2} |z-z'| + \|H_\cT^g(z')^{-\frac 1 2}\|.
$$
We define a metric $H_\cT^a \in \bH$ as follows : for each $z\in \R^2$  
\be
\label{defHTA}
H_\cT^a(z) = \max\{s_\cT(z)^{-2} , \, H_\cT^g(z)\}.
\ee

The rest of this section is devoted to proof of the following proposition, on quasi-acute meshes, in two dimensions.
\begin{prop}
\label{propHTA}
For any $C_0 \geq 1$ there exists $C=C(C_0)$ such that the following holds.
For any $\cT\in \bT_{a,C_0}$ the metric $H_\cT^a$ is $C$-adapted to the mesh $\cT$, and $32 C_0^{10} H_\cT^a\in \bH_a$.
\end{prop}

The fact that $32 C_0^{10} H_\cT^a\in \bH_a$ directly follows from the fact that $2 C_0^{10} \bH_\cT^g\in \bH_g$ and from Corollary \ref{corolHgToHa}. 

For each $z\in \R^2$ define $d_\cT(z) := \|H_\cT^g(z)^{-\frac 1 2}\|$. This quantity should be heuristically regarded as the diameter of the triangle containing $z$. We establish below the following property : there exists $\delta = \delta(C_0) >0$ such that for all $z,z'\in \R^2$
\be
\label{eqRegDT}
\text{ if } |z'-z| \leq \delta d_\cT(z) \stext{ then }  d_\cT(z') \geq \delta d_\cT(z).
\ee
Before turning to the proof of \iref{eqRegDT} we show how this property leads to the proof of Proposition \ref{propHTA}.
For all $z\in \R^d$ we have 
$$
s_\cT(z) = \inf_{z\in \sR^2} |z-z'|+d_\cT(z)  \geq \inf_{z'\in \sR^2} \min \{|z-z'|, \, d_\cT(z')\} \geq \delta d_\cT(z'),
$$
indeed $|z-z'|\geq \delta d_\cT(z)$ or $d_\cT(z') \geq \delta d_\cT(z)$ for any $z'\in \R^d$ according to \iref{eqRegDT}.
Combining this with the definition \iref{defHTA} of $H_\cT^a$ we obtain for all $z\in \R^2$
$$
\delta^2 H_\cT^a(z) \leq H_\cT^g(z)\leq H_\cT^a(z). 
$$
Recalling that $H_\cT^g$ is $C_0$-adapted to the mesh $\cT$, see proposition \ref{propHTG}, we obtain for all $T\in \cT$ and all $z\in T$ 
$$
\delta^2 C_0^{-2} H_\cT^a(z) \leq C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z) \leq C_0^2 H_\cT^a(z)
$$
which establishes that the metric $H_\cT^a$ is $C_0/\delta$ adapted to the mesh $\cT$, and concludes the proof of Proposition \ref{propHTA}.\\

We now turn to the proof of \iref{eqRegDT}, and for that purpose we introduce some notations.
For each segment $e=[\omega-u, \omega+u]\subset \R^2$ we define the diamond $\lozenge(e)$ of $e$ as follows
$$
\lozenge(e) := \{z\in \R^2 \sep |\<z-\omega,u\>|+ C_0 |\det (z-\omega,u)| < |u|^2\}.
$$
The next lemma considers a triangulation $\cT'$ on which the measure of sliverness is uniformly bounded by $C_0$, and compares the length an edge $e$ of $\cT'$ with the diameter of the triangles in $\cT'$ which intersect $\lozenge(e)$.

\begin{lemma}
\label{lemmaUUp}
Let $\cT'\in \bT$ be a triangulation such that $S(T) \leq C_0$ for all $T\in \cT'$. Let  $e=[\omega-u, \omega+u]$ be an edge of $\cT'$.
Then there is no vertex in the diamond $\lozenge(e)$, and for all $z\in \lozenge(e)$ and any triangle $T\in \cT'$ containing $z$, there exists an edge $e'= [\omega'-u', \omega'+u']$ of $T$ satisfying  
$$
2 |u'| \geq |u| -C_0 |\det (z-\omega,u)|/ |u|
%2 |\<u,u'\>| \geq |u|^2 - C_0 |\det (z,u)|.
$$
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$, and we assume up to a translation and a rotation that $\omega = 0$ and $u = u_y$.
We recall that for any triangle $T$, with maximal angle $\theta$, the measure of sliverness $S(T)$ has the following expression
$$
S(T) = \max\{1, \tan(\theta/2)\}.
$$
We assume for contradiction that there exists a vertex $v_0 = (x_0,y_0)\in \lozenge(e)$, and we assume without loss of generality that $x_0<0$. We consider a vertex $v_1 = (x_1,y_1)$ of $\cT$ such that the angle 
$$
\theta_0 :=  \angle(v_1-v_0, \, u_x) \in [-\cPi, \cPi)
$$
has the smallest possible absolute value $|\theta_0|$ (the bold letter $\cPi$ denotes the numerical constant $\cPi = 3.14159\cdots$). By construction there exists a triangle $T\in \cT$ containing $v_0$ and $v_1$ which has an angle  larger or equal or equal than $2\theta_0$ at the vertex $v_0$. It follows that $|\tan \theta_0| \leq S(T) \leq C_0$, and therefore  
$$
|y_1-y_0| \leq |\tan \theta_0| (x_1 - x_0) \leq C_0 (x_1-x_0).
$$
Proceeding inductively we define a sequence $v_n = (x_n, y_n)$, $n\geq 0$, of vertices of $\cT$ satisfying 
$
|y_{n+1} - y_n| \leq C_0 (x_{n+1} - x_n). 
$
Adding these inequalities together we obtain 
$$
|y_n-y_0|  \leq C_0 (x_n-x_0).
$$
It follows that one of the edges $[v_n, v_{n+1}]$, $n \geq 0$, of the mesh $\cT'$ intersects the edge $e$, which is a contradiction. The diamond $\lozenge(e)$ therefore does not contain any vertex, which concludes the proof of the first part of this proposition. \\

We now consider a point $z_0 = (x_0,y_0)\in \lozenge(e)$ and we assume without loss of generality that $x_0 \geq 0$. We consider a triangle $T$ containing $z_0$, and an edge $e'= [\omega'-u', \omega'+u']$ of $T$ which is on the left of $z_0$ (in other words the edge $e'$ and the segment $[(0,y_0),(x_0, y_0)]$ joining the point $z_0$ to its orthogonal projection on the edge $e$ intersect).

Since there is no vertex of $\cT'$ in the diamond $\lozenge(e)$, the edge $e'$ intersects the boundary of $\lozenge(e)$ at two points. We denote these points by $(x,y)$ and $(x',y')$, and we assume that without loss of generality that $y\geq 0 \geq y'$.
Observing that $0 \leq x \leq C_0^{-1}$, $0 \leq x'\leq C_0^{-1}$ and $\min\{x,x'\} \leq x_0$ we obtain  
$$
y-y' = (1-C_0 x) - (-1+C_0 x') \geq 1-C_0 x_0.
$$
Since $u = u_y = (0,1)$ and $2 u' = \lambda (x-x', y-y')$ for some $|\lambda| \geq 1$, we obtain 
$$
2|\<u,u'\>| \geq  
y-y' \geq 1-C_0 x_0 = |u|^2 - C_0 |\det (z_0,u)|,
$$
which concludes the proof of this proposition.
\sq

We now consider a fixed quasi-acute mesh $\cT\in \bT_{a,C_0}$ and we denote by $\cT'$ a fixed $C_0$-refinement of $\cT$ which satisfies $S(T) \leq C_0$ for all $T\in \cT'$. The next proposition involves a rectangular set $\square(e)$ associated to an edge $e$ of $\cT'$ which contains $e$ in its interior, contrary to the set $\lozenge(e)$ appearing in the previous proposition.  

\begin{lemma}
\label{lemmaRect}
There exists a constant $\delta_0 = \delta_0(C_0, d)>0$ such that the following holds.
We define the rectangle $\square(e)$ associated to an edge $e = [\omega-u, \, \omega+u]$ of $\cT'$ as follows
$$
\square(e) = \{z\in \R^2 \sep |\<z-\omega, u\>|\leq (1+\delta_0)|u|^2 \text{ and } |\det (z-\omega,u )| \leq \delta_0 |u|^2\},
$$
%where $\delta_0 = \delta_0(C_0):= ??1/(2C_0) >0$ is a constant specified in the proof.
We have $d_\cT(z) \geq \delta_0|u|$ for all $z\in \square(e)$.
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$. 
Up to a rotation and a translation, we may again assume that $\omega = 0$ and $u = u_y=(0,1)$.
We consider a triangle $T\in \cT$ containing the edge $e$ (note that $e\subset T$ but that $e$ may not be an edge of $T$, since we only known that $e$ is an edge in $\cT'$).

We define $H := H_\cT^g$. Recalling that $H$ is $C_0$-equivalent to $\cT$ we obtain for all $z\in e$
$$
C_0^{-2} H(z)\leq \cH_T \leq C_0^2 H(z). 
$$
The inclusion $e\subset T \subset \cE_T$ implies the upper bound $\|u\|_{\cH_T} = \|u_y\|_{\cH_T} \leq 1$. Hence for all $z\in e$
$$
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq \|u_y\|_{H(z)}^{-1} \geq C_0^{-1}.
$$
Note also that for any $z,u \in \R^2$
$$
d_\times (H(z), H(z+u)) \geq \ln \|H(z)^\frac 1 2 H(z+u)^{-\frac 1 2}\| \geq |\ln d_\cT(z) -\ln d_\cT(z+u)|.
$$
We define $C_1 := \sqrt 2 C_0^5$, in such way that $C_1^2 H\in \bH_g$, and we thus have  according to \iref{eqLocalNorm} if $C_1\|u\|_{H(z)}<1$
$$
|\ln d_\cT(z) -\ln d_\cT(z+u)| \leq d_\times (H(z), H(z+u)) \leq -\ln (1-C_1\|u\|_{H(z)}).
$$
Therefore for all $z\in e$ and all $u\in \R^d$,
$$
d_\cT(z+u) \geq d_\cT(z) (1-C_1 \|u\|_{H(z)}) \geq C_0^{-1}(1-C_1C_0 \|u\|_{\cH_T}).
$$
We define $C_2 := 4C_0C_1$ and we observe that any point of the rectangle 
\be
\label{eqRectGrad}
\left[\frac {-1}{C_2 \|u_x\|_{\cH_T}}, \,\frac 1 {C_2 \|u_x\|_{\cH_T}}\right] \times \left[-(1+C_2^{-1}), \, 1+C_2^{-1}\right].
\ee
can be written under the form $z+u$ where $z\in e$ and $\|u\|_{\cH_T} \leq 1/(2C_0C_1)$. We thus have  
\be
\label{eqdGrad}
d_\cT(z') \geq 1/(2C_0)
\ee
 on this rectangle.

We introduce a small constant $\delta = \delta(C_0)>0$ which is specified later in the proof. It follows from \iref{eqRectGrad} and \iref{eqdGrad} that the proof of this lemma is complete if $\|\cH_T\| \leq \delta^{-2}$, with $\delta_0 := \min \{\delta/C_2, \, 1/(2C_0)\}$.
We thus assume from this point that $\|\cH_T\|\geq \delta^{-2}$.\\

We assume that $\delta< C_0^{-1}$ and we define the rectangle
$$
\square_\delta := [-\delta, \delta] \times [1-C_0 \delta, -1+C_0 \delta],
$$
which is included in $\overline \lozenge(e)$ by construction.
Since $C_1^2 H\in \bH_g$, the function $z\mapsto \|H(z)\|^{-\frac 1 2}$ is $C_1$-Lipschitz according to Corollary \ref{corolLipNorm}. We thus have for all $z = (x,y)\in \square_\delta$
\be
\label{defr0}
\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2}+C_1|x|\leq r_0(\delta) := (C_0+C_1)\delta.
%\|u_x\|_{H(z)} \geq \|u_x\|_{H(y,0)}(1-C_1 |x| \|u_x\|_{H(y,0)}) \geq C_*(1-C_1 C_0 \delta_* C_*),
%\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2} + C_1 |x|
\ee
On the other hand it follows from Lemma \ref{lemmaUUp} that any $z = (x,y)\in \square_\delta$ is contained in a triangle containing an edge $e' = [\omega'-u', \omega'+u']$ such that $|u'| \geq (1-C_0 \delta)/2$. We thus have 
$$
1 \geq \|u'\|_{\cH_{T'}} \geq \frac{|u'|}{ \|\cH_{T'}^{-\frac 1 2}\|} \geq \frac{1-C_0 \delta}{2 \|\cH_{T'}^{-\frac 1 2}\|} 
$$
and therefore 
%of length at least $T'\in \cT$ satisfying $\|\cH_{T'}^{-\frac 1 2}\| \geq (1-C_0 \delta_*)/2$, hence 
\be
\label{defR0}
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq C_0^{-1} \|\cH_{T'}^{-\frac 1 2}\|  \geq  R_0(\delta) := (1-C_0 \delta)/(2C_0). %\det (z,u_y)
\ee
For all $z\in \square_\delta$, we denote by $\theta(z) = (\cos \Theta(z), \sin \Theta(z))$, $\Theta(z)\in [0, \cPi]$, the direction of the eigenvector associated to the small eigenvalue of $H(z)$, in such way that 
\be
\label{eqNormTheta}
\|\theta(z)\|_{H(z)} = \|H(z)^{-\frac 1 2}\|^{-1} = d_\cT(z)^{-1}.
\ee
We thus have for any $(0,y)\in e$
$$
C_0 \geq C_0 \|u_y\|_{\cH_T} \geq \|u_y\|_{H(0,y)} \geq |\cos \Theta(0,y)| \sqrt{\|H(0,y)\|} = \delta^{-1} |\cos \Theta(0,y)| ,
$$
hence 
$$
|\cos \Theta(0,y)| \leq  C_0 \delta.
$$
For all $z\in \square_\delta$ we have according to Theorem \ref{th2Spaces} 
$$
(R_0(\delta)-r_0(\delta)) \dil_z(\Theta) \leq  (\|H(z)^{-\frac 1 2}\| - \|H(z)\|^{-\frac 1 2}) \dil_z(\Theta) \leq 2C_1.
$$
Hence we obtain for all $z= (x,y)\in \square_\delta$  
$$
(R_0(\delta)-r_0(\delta)) |\Theta(z) - \Theta(0,y)| \leq 2C_1 |x|\leq 2C_1 \delta,
$$
hence since $t \mapsto \cos t$ is a Lipschitz function %, since $\cos : [0, \cPi/2]\to \R$ is convex
\be
\label{defTheta0}
|\cos \Theta(z)| \leq \cos \Theta_0(\delta) := C_0 \delta + \frac{\delta}{R_0(\delta)-r_0(\delta)}.
\ee
We have according to \iref{eqLocalNorm} for all $z\in \square_\delta$ and all $r\geq 0$ such that $C_1r\|\theta\|_{H(z)}<1$,
\begin{eqnarray*}
|\ln d_\cT(z+r \theta(z)) - \ln d_\cT(z)| &\leq& d_\times (H(z+r\theta(z)),H(z))\\
&\leq& -\ln (1-C_1r\|\theta\|_{H(z)})\\
&=& -\ln (1-C_1r/d_\cT(z)),
\end{eqnarray*}
therefore 
$$
d_\cT(z+r \theta(z)) \geq  d_\cT(z) (1-|r| C_1 /d_\cT(z)).
$$
For all $z\in \square_\delta$ such that $|r|\leq R_1(\delta) := R_0(\delta)/(2C_1)$ we thus obtain
$$
d_\cT(z+r\theta(z)) \geq R_0(\delta)(1-|r|C_1/R_0(\delta))\geq R_0(\delta)/2.
$$
It follows that $d_\cT(z')\geq R_0(\delta)/2$ for all $z'$ in the set 
$$
\{z+r\theta(z) \sep z\in \square_\delta,\, |r|\leq R_1(\delta)\} \supset [-\delta_0,\delta_0]\times [-(1+\mu_0),1+\mu_0]
$$
where 
\be
\label{eqD0MU0}
\delta_0 := \delta - r \cos \Theta_0(\delta) \stext{ and }  \mu_0 := -C_0 \delta+ r \sin \Theta_0(\delta)
\ee
and where the constant $0 \leq r\leq R_1(\delta)$ can be freely chosen.
The rest of the proof consists in choosing appropriate constants $\delta$ and $r$.\\

As $\delta \to 0$ we have $r_0(\delta)\to 0$, $R_0(\delta) \to 1/(2C_0)$ and $\cos\Theta_0(\delta) \to 0$. We thus choose $\delta = \delta(C_0,d)>0$ sufficiently small in such way that 
\be
\label{eqRCS}
R_0 \geq 1/(4C_0)
, \quad
\cos \Theta_0 \leq 1/(8C_0)
, \quad
\sin \Theta_0 \geq 1/2
.
\ee
We then choose $r := 4C_0 \delta$, which is smaller than $R_1(\delta)= R_0(\delta)/(2C_1) \geq 1/(8C_1C_0)$ if $\delta$ is sufficiently small. Injecting this choice of $r$ and \iref{eqRCS} in \iref{eqD0MU0} we thus obtain 
$$
\delta_0 \geq \delta/2 \stext{ and }\mu_0 \geq C_0 \delta.
$$
We have thus established under the hypothesis $\|\cH_T\|\geq \delta^{-2}$ that 
hence $d_\cT(z) \geq 1/(8C_0)$ for all $z$ in the rectangle 
$$
[-\delta/2, \delta/2]\times [-(1+C_0\delta), 1+C_0 \delta].
$$
Since the case $\|\cH_T\|\leq \delta^{-2}$ is already established this concludes the proof of this proposition.
\sq

The next lemma establishes a technical property on the covering a one dimensional segment by smaller ones, which is a key to the end of this proof.

\begin{lemma}
\label{lemmaCoverSeg}
Let $x_1, \cdots , x_k\in [0,1]$ and let $h_1, \cdots, h_k >0$ be such that 
\be
\label{eqDefXiHi}
[0,1]\subset \bigcup_{1\leq i \leq k} [x_i-h_i, \, x_i+h_i].
\ee
Let $\delta>0$ and let $h_* = h_*(k,\delta) := \exp(1-2k/\delta)/\delta$. Then 
\be
\label{eqInclSeg}
[0,1]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_* \leq h_i}} [x_i-(1+\delta)h_i, \, x_i+(1+\delta)h_i].
\ee
\end{lemma}

\proof
For each $y\in [0,1]$ we denote by $h(y)$ the value $h_i$ associated to the segment $[x_i-h_i, x_i+h_i]$ of smallest length containing $y$.
We thus have 
$$
\int_{[0,1]} \frac {dy} {h(y)} \leq \sum_{1\leq i \leq k} \int_{x_i-h_i}^{x_i+h_i} \frac 1 {h_i} = 2k.
$$
We assume for contradiction that \iref{eqInclSeg} does not hold, and we consider a point $x\in [0,1]$ which does not belong to the right hand side of $[0,1]$. For each $y\in [0,1]$ one of the two following possibilities holds
$$
\delta h(y) < |x-y| \stext{ or } h(y) < h_*.
$$
Integrating we obtain 
$$
\int_0^1 \frac {dy} {h(y)}  \geq \int_0^1 \frac {dy} {\max\{|x-y|/\delta,\, h_*\}}.
$$
The minimum value of the right hand side is attained for $x=0$ or $1$ and equals 
$$
\int_0^1 \frac {dy}{\max \{|x-y|/\delta, h_*\}} = \int_0^{\delta h_*} \frac 1 h_* + \int_{\delta h_*}^1 \frac \delta ydy = \delta(1-\ln(\delta h_*))
$$
Thus $2k>\delta(1-\ln(\delta h_*))$, which contradicts the definition of $h_*$. This concludes the proof of this lemma.
\sq

Under the hypotheses of Lemma \ref{lemmaCoverSeg} we thus have
\be
\label{eqInclSegDouble}
[-h_*\delta,\, 1+h_*\delta]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_i \leq h_*}} [x_i-(1+2\delta)h_i, \, x_i+(1+2\delta)h_i].
\ee


We now conclude the proof of Proposition \ref{propHTA}.
We consider a point $z\in \R^2$ contained in a triangle $T\in \cT$, and we denote by $\cT$ the longest edge $e$ of $T$. Up to a rotation and a translation, we may assume that $e=[0, u_x]$ joins the origin of $\R^2$ to the the vector $u_x := (1,0)$.
Since the triangulation $\cT'$ is a $C_0$-refinement of $\cT$, the edge $e$ of $T$ is built of $k \leq C_0$ edges $(e_i)_{1 \leq i \leq k}$ of $\cT'$,
$$
e_i = [(x_i-h_i)u_x,\,  (x_i +h_i) u_x].
$$

We define $h_* := h_*(C_0, \delta_0/2) = 2\exp(1-4C_0/\delta_0)/\delta_0$, where $\delta_0$ is the constant from Lemma \ref{lemmaRect}, and we observe that 
\be
\label{eqRectHoDo}
\bigcup_{h_* \leq h_i} \square(e_i) \supset \left[-\frac{h_* \delta_0} 2, 1+ \frac{h_* \delta_0} 2\right] \times [-h_* \delta_0, h_* \delta_0],
\ee
(*details to do*)

Since $e$ is the longest edge of $T$, the angles of $T$ at the extremities of $e$ are acute.
Furthermore the height $h$ of $T$ orthogonal to the edge $e = [0,u_x]$ satisfies 
$$
h = 2 |T|  = \frac{\lambda} { \sqrt {\det \cH_T}} = \frac{\lambda}{\sqrt{\|\cH_T\| \|\cH_T^{-1}\|^{-1}}}  = \frac{\lambda \|\cH_T^{-1}\|}{\rho(T)} 
$$
where $\lambda := 3 \sqrt 3 /2$.
Upper bound on $\|\cH_T^{-1}\|$ remarking for instance that, denoting by $V$ the collection of vertices of $T$,
$$
\cH_T^{-1} = \frac d {2 (d+1)^2} \sum_{v, v'\in V} (v-v') (v-v')^\trans,
$$
and that the longest edge of $T$ has length $1$.
Hence the rectangle \iref{eqRectHoDo} forms a neighborhood of the triangle $T$, and thus of $z$ which concludes the proof.

\section{From metric to mesh}
\label{secMetToMesh}
%\subsection{Mesh generation}
\label{secMeshGen}

%We prove in this section Theorems \ref{thI}, \ref{thA} and \ref{thR} on the equivalence between certain classes of meshes and of metrics. %, which is divided in two parts.
%This proof is divided in two parts as follows. Proposition \ref{propMeshGen} in \S \ref{secMeshGen} we show how a mesh can be generated from a Riemannian metric, and Proposition \ref{propMetGen} in \S\ref{secMetGen} we show how a metric can be generated from a mesh.
%
This section is dedicated to the proof of the following result, on the generation of a mesh from a metric.
\begin{prop}
\label{propMeshGen}
There exists $C_0 = C_0(d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $H\in \bH_i$ there exists $\cT \in \bT_{i,C_0}$ which is $C_0$-adapted to $H$.
\item If $d=2$, then for any $H \in \bH_a$ there exists $\cT\in \bT_a$ which is $C_0$-adapted to $\cT$.
\item If $d=2$, then for any $H \in \bH_g$ there exists $\cT\in \bT_g$ which is $C_0$-adapted to $\cT$.\end{enumerate}
\end{prop}

Point {\it i)} is established in the \S\ref{secMeshGenI}, point {\it iii)} in \S \ref{secMeshGenG} an eventually {\it ii)} in \S \ref{secMeshGenA}.\\


We first introduce the notion of equispaced points in a metric space. Let $(X,d)$ be a metric space, we say that a subset $X_0 \subset X$ is $C_0$-equispaced if the following holds.
%We say that a point set $\cP\subset \R^2$ is $C_0$-equidistributed with respect to a metric $H\in \bH$ (*to a distance $d$?*) if the following holds :
\begin{enumerate}[a)]
\item (Covering) The open balls $B(x,C_0) := \{y\in X \sep d_X(x,y)<C_0\}$ centered at the points $x\in X_0$ cover $X$:
\be
\label{eqCover}
\bigcup_{x\in X_0}  B(x,C_0) = X.
\ee
%For all $z\in \R^2$, $d_H(z, \cP)\leq C_0$. 
\item (Separation) The open balls $B(x,C_0^{-1})$ are pairwise disjoint: for all $x,x'\in X_0$ such that $x\neq x'$,
\be
\label{eqSep}
B(x,C_0^{-1}) \cap B(x', C_0^{-1}) = \emptyset
\ee
%For all $p\in \cP$, $d_H(p, \cP\sm \{p\}) \geq C_0^{-1}$.
\end{enumerate}

The next lemma establishes the existence of such a set under certain assumptions. %shows that such sets exist in metric spaces 
\begin{lemma}
\label{lemmaEquiSpaced}
Let $(X,d_X)$ be a metric space in which the closed balls $B'(x,r) := \{y\in X \sep d_X(x,y) \leq r\}$ are compact for all $x\in X$ and $r\geq 0$. Then there exists a (finite or) countable subset $X_0\subset X$ which is $\sqrt 2$-equispaced.
\end{lemma}

\proof
We define inductively a finite or countable sequence $x_0, x_1, \cdots$ of points in $X$ as follows.
We choose $x_0$ arbitrarily.
Assuming that $x_0, \cdots, x_n$ are already defined we consider the closed set 
\be
\label{eqDefXn}
X^n := X\sm \left(\bigcup_{0\leq i \leq n} B(x_i, \sqrt 2)\right) = 
\{x\in X \sep d_X(x,x_i) \geq \sqrt 2 \text{ for all } 0 \leq i \leq n\}.
\ee
If the set $X^n$ is empty, then the sequence ends and we define $N = n+1$. Otherwise we choose $x_{n+1}$ arbitrarily among the minimisers of $d_X(x,x_0)$ on $X^n$:
\be
\label{defxn}
x_{n+1} \in \underset {x\in X_n} \argmin \,d(x,x_0).
\ee
Such a minimizer exists since $X^n$ is closed and since the closed balls in $X$ are compact.
%$$
%X^n \cap \overline B\left(x_0, \ 1+ \inf_{x\in X^n} d_X(x_0, x)\right)
%$$
%is compact.
We define $N = \infty$ if the sequence $(x_n)$ is infinite.

We denote by $X_0 := \{x_n \sep 0\leq n<N\}$ the collection of all points of this finite or countable sequence.
%
%We define $N := \infty$ if the sequence $x_0, x_1, \cdots$ is infinite, and we denote by $X_0$ the collection of all points of this finite or countable sequence,
%$$
%X_0 := \{x_n \sep 0 \leq n < N\}.
%$$ 
%%as the collection of all points $x_0, x_1, \cdots$ of this finite or countable sequence.
%, which clearly is finite or countable.
By construction, we thus have $d_X(x_i, x_j) \geq \sqrt 2$ for all $0 \leq i < j<N$, and therefore 
\be
\label{eqSep2}
B\left(x_i, \frac{\sqrt 2} 2\right) \cap B\left(x_j, \frac{\sqrt 2} 2\right) = \emptyset,
\ee
which establishes the separation property \iref{eqSep}, and shows that $X_0$ is a discrete set.

We now assume for contradiction that the covering property \iref{eqCover} does not hold, and we choose a point $x_*\in X$ such that $d(x_n,x_*)>\sqrt 2$ for all $n\geq 0$. The definition \iref{defxn} of $x_{n+1}$ implies that $d_X(x_0, x_n) \leq d_X(x_0, x_*)$ for all $n \geq 0$, which means that $X_0$ is included in a ball 
$$
X_0\subset B'(x_0, d_X(x_0, x_*)).
$$
The set $X_0$ is therefore both discrete and compact, hence finite, which means that $N<\infty$ and that the set $X^{N-1}$ defined on \iref{eqDefXn} is empty. This contradicts our hypothesis that the covering property does not hold, which concludes the proof of this proposition.
\sq


%The next lemma gives a simple (from a theoretical point of view) procedure which produces a point set equidistributed with respect to a metric.
%\begin{lemma}
%Let $H\in \bH$ and let $(p_n)_{n\geq 0}$ be a sequence of points obtained by choosing $p_0 = 0$ and then iteratively choosing $p_{n+1}$ among the minimizers of
%\be
%\label{defpn}
%\min\{\|p\| \sep d_H(p, \{p_0,\cdots , p_n\} \geq 1)
%\ee
%
%Then the point set $\cP := \{p_n \sep n \geq 0\}$ is $1$-equidistributed with respect to $H$.
%\end{lemma}
%
%\proof
%The separation holds by construction. It implies in particular that for any $M \geq 1$, $\cP\cap B(0,M)$ is finite. 
%
%%Since $H$ is continuous and positive definite, for each $M$ the set $\{n\geq 0 \sep \|p_n\| \leq M\}$ is finite.
%Indeed let $\Lambda^2 := \max \{\|H(z)\| \sep \|z\| \leq M\}$.
%The balls $B(p, \Lambda/2)$, $p\in \cP\cap B(M)$ are pairwise disjoint. It follows from a volume argument that $\cP\cap B(M)$ is finite.
%
%Let us assume by contradiction that there exists $z\in \R^2$ such that $d(z, \cP)>1$. Then for $n$ large enough we have $\|z\| < \| p_{n+1}\|$ which is incompatible with the construction of $p_{n+1}$ as a minimizer of \iref{defpn}.
%\sq


\subsection{Isotropic Mesh generation}
\label{secMeshGenI}
The survey paper \cite{Nochetto} describes a the construction of a hierarchical family of meshes of the rectangular domain 
$
[0,1]^d.
$ 
All these meshes are the refinement of a ``fundamental'' mesh $\cT_0 = \{T_\sigma \sep \sigma \in \Sigma_d\}$, where $\Sigma_d$ stands for the collection of permutations of the set $\{1,\cdots,d\}$, which is formed of the $d!$ Kuhn simplices 
$$
T_\sigma := \{z\in [0,1]^d \sep z_{\sigma(1)} \leq \cdots \leq z_{\sigma(d)}\}.
$$
%A sequence $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $A procedure, guided by the user 
%The ``fundamentalbasic mesh $\cT_0$ of $[0,1]^d$ 
Starting from $\cT_0$, the algorithm described in \cite{Nochetto} produces, guided by the user, a family $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $[0,1]^d$ proceeding as follows. 
Assume that the mesh $\cT_n$ has already been generated.
%Once the mesh $\cT_n$ is defined, the mesh $\cT_{n+1}$ is obtained as follows.
%\begin{enumerate}
%\item (Marking) The user selects
%\item (Refinement)
%\end{enumerate}
%The mesh $\cT_{n+1}$ is produced from $\cT_n$ as follows 
\begin{itemize}
\item (Marking)
The user selects a subset $\cM_n \subset \cT_n$.
\item (Refinement)
The algorithm generates a $2$-refinement $\cT_{n+1}$ of $\cT_n$,  
$$
\cT_{n+1} := \Refine(\cT_n, \cM_n).
$$
which does not contain any of the marked simplices : $\cT_{n+1} \cap \cM_n = \emptyset.$
\end{itemize}
\noindent

The elements of the meshes $(\cT_n)_{n \geq 0}$ have a very specific structure, which main features are described below.
\begin{property}
\label{propertyIso}
Any simplex $T$ produced by this algorithm possesses the following properties.
\begin{enumerate}[a)]
\item (Discrete Volumes) The volume of $T$ has the form
\be
\label{eqVolTG}
|T| = \frac {2^{-g(T)}}{d!},
\ee
where $g(T)\geq 0$ is an integer called the ``generation'' of $T$.
\item
(Finite number of classes)
The simplex 
$$
2^{\frac{g(T)} d} (T-z_T),
$$
which is centered at the origin and has volume $1/d!$, %$\frac 1 {d!}$, 
belongs to a finite family $\gT_0$ of simplices.
%\item
%(Vertices lie on a grid)
%The vertices of $T$ lie on the grid
%$$
%2^{-\left\lceil \frac {g(T)} d\right\rceil} \Z^d
%$$
\end{enumerate}
\end{property}
The survey paper \cite{Nochetto} also contains a result, Proposition 4.1, which establishes that $\cT_{n+1} := \Refine(\cT_n, \cM_n)$ is a \emph{local} refinement of $\cT_n$ in the following sense: for all $T'\in \cT_{n+1} \sm \cT_n$ there exists $T\in \cM_n$ such that 
\be
\label{eqDG}
g(T)\geq g(T') \stext{ and } d(T,T') \leq D \, 2^{-g(T')/d},
\ee
where $D = D(d)$ is a fixed constant and where 
$
d(T,T') := \min\{|z-z'| \sep z\in T, \, z'\in T'\}.\\
$

The next lemma shows that this refinement algorithm can be used to produce a conforming isotropic mesh $\cT$ of the unit cube $[0,1]^d$, such that the diameters $\diam(T)$, $T\in \cT$, are specified by a given Lipschitz function.

\begin{lemma}
\label{lemmaSCube}
There exists $C=C(d)$ such that the following holds.
Let $s:[0,1]^d\to  (0,\sqrt d]$ be a lipschitz function, and let $(\cT_n)_{n \geq 0}$ be the sequence of meshes produced by the algorithm when the collection $\cM_n\subset \cT_n$ of marked simplices is defined as follows
\be
\label{defMn}
\cM_n := \left\{T\in \cT_n \sep \min_T s < \diam(T)\right\}.
\ee
Then the sequence of meshes stabilizes : there exists $N\geq 0$ such that $\cT_n = \cT_N$ for all $n \geq N$. Furthermore we have for all $T\in \cT_N$ 
\be
\label{eqEquivCube}
\diam(T) \leq \min_T s \leq C \diam(T).
\ee
\end{lemma}

\proof
We recall that for each simplex $T$ produced by the algorithm, the simplex $2^{g(T)/d}(T-z_T)$ belongs to a finite family $\gT_0$ of simplices.
We define 
$$
D_0 := \max_{T \in \gT_0} \diam(T),
$$
and we observe that for any $n\in \N$ and any $T \in \cM_n$ one has 
\be
\label{eqMinDiam}
s_0 := \min_{[0,1]^d} s \leq \min_T s \leq \diam(T) \leq D_0 2^{\frac{-g(T)} d},
\ee
hence 
\be
\label{eqMaxGT}
g(T)\leq C_1 := d \frac{\ln (D_0/s_0)}{\ln 2}.
\ee
We first prove that the sequence $(\cT_n)_{n \geq 0}$ of meshes stabilizes. According to \iref{eqDG} for any  
$$
T' \in \cT_n = (\cT_n \sm \cT_{n-1}) \cup \cdots \cup (\cT_1 \sm \cT_0) \cup \cT_0
$$
there exists 
$$
T\in \cM_{n-1} \cup \cdots \cup \cM_0 \cup \cT_0
$$
such that $g(T') \leq g(T) \leq C_1$ according to \iref{eqMaxGT}. 
%Combining this with \iref{eqMaxG} we obtain 
%$$
%\sup_{T' \in \cT_n} g(T') \leq C_1.
%$$
This leads us to a uniform bound on $\#(\cT_n)$:
$$
1 = \sum_{T \in \cT_n} |T'| \geq \#(\cT_n) \min_{T \in \cT_n} |T'| = \#(\cT_n) \min_{T \in \cT_n} \frac{2^{-g(T)}}{d!} \geq \#(\cT_n) \frac{2^{-C_1} }{d!},
$$
hence $\#(\cT_n) \leq d! 2^{C_1}$. Since $\cT_{n+1}$ is a refinement of $\cT_n$ we have either $\#(\cT_{n+1}) \geq \#(\cT_n)+1$ or $\cT_{n+1} = \cT_n$, and in the latter case one has $\cT_n = \cT_{n+1} = \cT_{n+k}$ for all $k \geq 0$ by construction. This case eventually happens since $\#(\cT_n)$ is uniformly bounded, which shows that the sequence $(\cT_n)_{n\geq 0}$ of meshes stabilizes.\\

We now turn to the the proof of \iref{eqEquivCube}, and for that purpose we consider $N\geq 0$ such that $\cT_N=\cT_n$ for all $n \geq N$. 
We have for all $T\in \cT_N$
$$
\diam(T) \leq \min_T h,
$$
indeed otherwise $T\in \cM_N$ and therefore $\cT_{N+1}\neq \cT_N$ which is a contradiction.
This establishes the left part of \iref{eqEquivCube}, and we now focus on the right part.
For that purpose we consider $T'\in \cT_N$, and we define 
$$
n(T') := \min \{n \geq 0\sep T \in \cT_n\}.
$$
If $n(T') = 0$, then $T'$ is one of the $d!$ Kuhn simplices $(T_\sigma)_{\sigma\in \Sigma_d}$ that form $\cT_0$, and therefore 
$$
\diam(T') = \sqrt d \geq \min_T s
$$
since $s$ is uniformly bounded by $\sqrt d$.
Otherwise we have $T'\in \cT_{n(T)} \sm \cT_{n(T)-1}$, hence there exists $T\in \cM_{n(T)-1}$ such that \iref{eqDG} holds.
Denoting $d(T,T') := \min\{|z-z'| \sep z\in T,\, z'\in T'\}$, and recalling that $g(T') \leq g(T)$, we obtain 
\begin{eqnarray*}
\min_{T'} s &\leq& \min_T s+ \diam(T) +d(T,T')\\
& \leq & \diam(T) + \diam(T) + D 2^{-g(T')/d}\\
&\leq & 2D_0 2^{-g(T)/d}+D 2^{-g(T')/d}\\
& \leq & (2D_0+D) 2^{-g(T')/d}\\
& \leq & C \diam(T'),
\end{eqnarray*}
where 
$$
C := \frac{2D_0+D}{\min \{\diam(T)\sep T \in \gT_0\}},
$$
which concludes the proof of this proposition.
\sq

The rest of this section is devoted to the proof the point {\it i)} of Proposition \ref{propMeshGen}.
We thus consider a metric $H\in \bH_i$, and we recall there exists a Lipschitz function $s: \R^d \to \R_+^*$ such that for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2}.
$$
For each $n\geq 0$ we define a function $s_n : [0,1]^d \to \R_+^*$, which is clearly Lipschitz, as follows
\be
\label{defSn}
s_n(z) := 2^{-n} s(2^n (z-z_0))
\ee
where $z_0 = (1/2, \cdots , 1/2)$ is the barycenter of the cube $[0,1]^d$.
%The function $s_n$ is clearly Lipschitz, and 
For all $z\in [0,1]^d$ and all $n \geq 0$ we have 
$$
s_n(z) \leq s_n(z_0) + |z-z_0| \leq 2^{-n} s(0) + \frac {\sqrt d} 2.
$$
The function $s_n$ is therefore uniformly bounded by $\sqrt d$ on $[0,1]^d$ when $n$ is sufficiently large.
We denote by $\cT^n$ the mesh of the cube $[0,1]^d$ described by Lemma \ref{lemmaSCube} for the function $s_n$. We thus have %for all $T\in \cT^n$
\be
\label{eqDiamSn}
\diam(T) \leq \min_T s_n \leq C \diam(T) \stext{ for all } T \in \cT^n,
\ee
where $C=C(d)$ is the constant from Lemma \ref{lemmaSCube}.
We denote by $\cT_n$ the mesh of the cube $[-2^{n-1}, 2^{n-1}]^d$ obtained by translating the mesh $\cT^n$ by $-z_0$ and dilating it by $2^n$. In mathematical terms: % In condensed notations
$$
\cT_n := \{2^n(T-z_0)\sep T \in \cT^n\}.
$$
%$$
%\cT_n := 2^n (\cT^n -z_0).
%$$
In view of \iref{defSn} and \iref{eqDiamSn} we thus have 
\be
\label{eqMinSDiamT}
\diam(T) \leq \min_T s \leq C \diam(T) \stext{ for all } T \in \cT_n,
\ee
which implies for any $z\in T$
$$
\diam(T) \leq \min_T s \leq s(z) \leq \min_T s + \diam(T) \leq (C+1) \diam(T).
$$
We denote by $C_0$ the smallest constant such that for all $T$ in the finite set $\gT_0$ one has 
$$
 \frac{C_0^{-2} \Id}{\diam(T)^2} \leq \cH_T \leq \frac{C_0^2\Id}{(C+1)^2\diam(T)^2 },
$$
and we thus obtain for all $T\in \cT_n$ and all $z\in T$
\be
\label{eqHHTIso}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Unfortunately the mesh $\cT_n$ does not cover $\R^d$ but only the cube $[-2^{n-1}, 2^{n-1}]$. 
The next lemma allows to extract a global mesh $\cT$ of the infinite domain $\R^d$ from the sequence of meshes $(\cT_n)_{n\geq 0}$.

\begin{lemma}
Let $(\Omega_n)_{n \geq 0}$ be an increasing sequence of polygonal domains of $\R^d$, which exhausts $\R^d$ in the following sense:
$$
\bigcup_{n \geq 0} \Omega_n = \R^d \stext{ and } \Omega_n \subset \Omega_{n+1} \text{ for all } n\geq 0.
$$
Let $H \in \bH_g$, let $(\cT_n)_{n \geq 0}$ be a sequence of conforming simplicial meshes of the domains $\Omega_n$, and assume that for all $n \geq 0$, all $T\in \cT_n$ and all $z\in T$ one has 
\be
\label{eqHHTConv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Then there exists a mesh $\cT\in \bT$ such that 
$
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
$
for all $T\in \cT$ and all $z\in T$.
\end{lemma}

\proof
The heuristic idea of this proof is to ``extract a converging subsequence'' from the sequence $(\cT_n)_{n \geq 0}$ of meshes. Unfortunately meshes are discrete objects of combinatorial nature, and the convergence of meshes has no meaning a priori. We therefore use Lipschitz functions as an intermediate object, for which convergence is well defined and which benefit of a compactness property.\\

We associate a function $\phi_T : \R^d \to \R$ to each simplex $T$, which is defined as follows. The function $\phi_T$ is supported on $T$, and for all $z\in T$ we have in terms of the barycentric coordinates $\lambda_v(z)$ of $z$ with respect to the vertices $v\in V$ of $T$:
%To each simplex $T$ of vertices $V$, and barycentric coordinates $(\lambda_v)_{v\in V}$ we associate the function 
$$
\phi_T(z) := \min_{v\in V} \lambda_v(z).
$$
%The maximum of this function has value $1/d$ and is attained at the barycenter $z_T$ of $T$. Furthermore for each $z\in T$ and each $0\leq r \leq 1$ one easily checks that 
%$$
%\phi_T(z+r(z-z_T)) \geq r/d.
%$$
According to Lemma \ref{lemmaNormLambda}, we have for any $z,z'\in T$ and any $v\in V$
$$
|\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T},
$$
hence 
\be
\label{eqPhiLip}
|\phi_T(z) - \phi_T(z')| \leq \max_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T}.
\ee

For all $n \geq 0$ we define a function $\phi_n$ on $\R^d$ as follows
$$
\phi_n := \sum_{T \in \cT_n} \phi_T.
$$
It follows from \iref{eqHHTConv} and \iref{eqPhiLip} that for all $z\in \R^d$
$$
\dil_z(\phi_n\sep d_H) \leq C_0,
$$
hence $\phi_n : (\R^d,d_H) \to \R$ is $C_0$-Lipschitz according to Proposition \ref{propDilLoc}. Since the space $(\R^d, d_H)$ is locally compact, due to Proposition \ref{propEuclidRiemann}, Ascoli's compactness theorem states that there exists %a the sequence $(\phi_n)_{n \geq 0}$ of $C_0$-Lipschitz functions admits a 
subsequence $(\phi_{n_k})_{k \geq 0}$ which converges uniformly on all compact sets of $\R^d$ to a $C_0$-Lipschitz function $\phi$. 

We therefore assume, up to such an extraction, that 
$
\phi_n \to \phi
$
uniformly on all compact sets of $\R^d$.
We denote by $\cT$ the collection of closures of connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$:
$$
\cT := \left\{ \overline E \sep E \text{ is a connected component of } \{z\in \R^d \sep \phi(z)>0\} \right\}.
$$
For each $z\in \R^d$ and each $n \geq 0$, we denote by $T_n(z)$ the element of $\cT_n$ containing $z$ in its interior if it exists, and $T_n(z) = \emptyset$ otherwise.
If $\phi(z)>0$, then $T_n(z)\neq \emptyset$ for all $n$ sufficiently large, and one easily checks that 
\be
\label{eqTTnz}
T_n(z)\text{ converges in Hausdorff distance to the element }T(z)\in \cT
\ee
 containing $z$. Hence $\cT$ is a collection of simplices, and the convergence $T_n(z)\to T(z)$ in haussdorf distance, combined with the hypothesis $C_0^{-2} H(z) \leq T_n(z) \leq C_0^2 H(z)$, implies that  
\be
\label{eqHHTConv2}
C_0^{-2} H(z) \leq T(z) \leq C_0^2 H(z).
\ee
In order to conclude this proof we need to show that the collection $\cT$ of simplices is a conforming mesh of $\R^d$. We thus have to check the hypotheses of Definition \ref{defSimplMesh}.
The interiors $\interior(T)$, $T\in \cT$ are pairwise disjoint since they are the connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$.
We claim furthermore that $\cT$ covers $\R^d$. Indeed let $z\in \R^d$be arbitrary and for all $n$ let $T_n\in \cT_n$ be such that $z\in T_n$. Since $C_0^{-2} H(z) \leq \cH_{T_n}\leq C_0^2 H(z)$ there exists a subsequence $T_{n_k}$ which converges in the Haussdorf distance to a simplex $T$ containing $z$. We clearly have $T\in \cT$ which establishes as announced that $\cT$ covers $\R^d$.
The fact that $\cT$ is locally finite easily follows from \iref{eqHHTConv2}.\\


We now turn to the proof of the conformity property, and for that purpose we consider an arbitrary Lipschitz function $f : (\R^d, d_H) \to \R$ with compact support. 
Let $T$ be a simplex such that $C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)$. We have for any vertex $v$ of $T$
$$
|f(v) - f(z_T)| \leq d_H(z_T,v) \leq C_0 \|z_T - v\|_{\cH_T} = C_0.
$$
Denoting by $V$ the collection of vertices of $T$ we thus obtain for any $z,z'\in T$
$$
\interp_T^1 f(z) - \interp_T^1 f(z') = \sum_{v\in V} (\lambda_v(z) - \lambda_v(z')) (f(v) - f(z_T)) 
$$
hence using Lemma \ref{lemmaNormLambda}
\begin{eqnarray*}
|\interp_T^1 f(z) - \interp_T^1 f(z')| &\leq& C_0 \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')| \\
&\leq& C_0 \sqrt{(d+1)  \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|^2} \\
&=& C_0 \sqrt d \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Let $n_0 \geq 0$ be such that $\supp(f)\subset \Omega_{n_0}$. The last inequality implies that 
$$
\dil_z(\interp_{\cT_n}^1 f \sep d_H)\leq C_0^2 \sqrt d
$$
for any $z\in \R^d$ and all $n \geq n_0$, which shows according to Proposition \ref{propDilLoc} that $\interp_{\cT_n}^1 f : (\R^d, d_H) \to \R$ is $C_0^2\sqrt d$-Lipschitz.

We define 
$
D := \cup_{T \in \cT} \interior(T),
$
and we denote by $\interp_T^1 f : D \to \R$ the function which coincides with $\interp_T^1 f$ on the \emph{interior} of each $T\in \cT$. % (and which is possibly discontinuous at the interfaces between the simplices $T\in \cT$). 
For any $z\in D$ we obtain using \iref{eqTTnz} that $\interp_{\cT_n}^1 f(z) \to \interp_\cT^1 f(z)$, hence for any $z,z'\in D$
$$
|\interp_\cT^1 f(z) - \interp_\cT^1 f(z')| = \lim_{n \to \infty} |\interp_{\cT_n}^1 f(z)-\interp_{\cT_n}^1 f(z')| \leq \sqrt d C_0^2 \, d_H(z,z').
$$
The interpolant $\interp_T^1 f : D \to \R$ therefore extends to a $\sqrt d C_0^2$-Lipschitz function $\interp_T^1 f : (\R^d, d_H) \to \R$. It easily follows that $\interp_\cT^1 f$ is continuous for any compactly supported $C^1$ function $f$. This property characterizes conforming meshes, hence $\cT\in \bT$ which concludes the proof.
\sq

\subsection{Graded mesh generation}
\label{secMeshGenG}

We prove in this section a result of bi-dimensional mesh generation, Theorem \ref{thEquiMesh}, which implies Point (iii) of Proposition \ref{propMeshGen}. The key ingredients of this section come from the paper \cite{Shew}.
We assume throughout this section that the dimension is $d=2$.


We consider a fixed metric $H \in \bH$. For any $x,y\in \R^2$ we define 
$$
d_x(y) := \|x-y\|_{H(x)}.
$$
We also consider a fixed discrete collection of sites $V \subset \R^2$, and we define the anisotropic Voronoi cell of a site $v\in V$ as follows 
$$
\Vor(v) := \{z\in \R^2 \sep d_v(z) \leq d_w(z) \text{ for all } w \in V\}.
$$
The anisotropic Voronoi cell $\Vor(v)$ is thus the collection of points $z$ which are \emph{closer to the side $v$ than to any other site}.
The classical (isotropic) Voronoi is obtained by choosing $H = \Id$.
We refer to the paper \cite{Shew} Figure 3 for an illustration of the anisotropic Voronoi diagram $\{\Vor(v) \sep v\in V\}$ associated to a point set.

We denote by $V_z$ the collection of sites $v\in V$ which contain a given point $z\in \R^2$ in their Voronoi region:
$$
V_z := \{v \in V \sep z \in \Vor(v)\}.
$$
We define a collection $\cT_0(V,H)$ of convex sets attached to the metric $H$ and to the collection $V$ of sites
$$
\cT_0(V,H) := \{\Cvx(V_z) \sep z \in \R^2 \text{ and } \#(V_z) \geq 3\}.
$$

The next theorem establishes that, under certain conditions on the metric $H$ and the set $V$, the collection $\cT_0(V,H)$ of convex sets is a triangulation of $\R^2$ adapted to the metric $H$.

\begin{theorem}
\label{thEquiMesh}
For each $C_0$ there exists $C = C(C_0)\geq 1$ and $c=c(C_0)>0$ such that the following holds. \\
Let $H \in \bH$ and $V \subset \R^2$. 
Assume that $c^2 H \in \bH_g$ and that $V$ is $C_0$-equispaced with respect to the distance $d_H$. 
Then $\cT_0(V,H)$ is a partition of $\R^2$ and arbitrarily triangulating each polygon yields a triangulation $\cT$ which is $C$-adapted to $H$. Furthermore if the vertices $V$ are in general position the $\cT_0(V,H)$ is already a triangulation, named the Anisotropic Delaunay triangulation in \cite{Shew}.
\end{theorem}



Before turning to the proof of this theorem, we show how to conclude the proof of point  iii) of proposition \ref{propMeshGen}.
We denote by $C=C(\sqrt 2)$ the constant attached to $C_0 = \sqrt 2$ in theorem \ref{thEquiMesh}.
Let $H_0 \in \bH_g$, and let $H := C H_0$. It follows from Lemma \ref{lemmaEquiSpaced} that there exists a set $V \subset \R^2$ which is $\sqrt 2$- equispaced with respect to the distance $d_H$.
Theorem \ref{thEquiMesh} therefore states that there exists a triangulation $\cT$ of $\R^2$ which is $C$-adapted to $H$, and therefore $C^2$-adapted to $H_0$ which concludes the proof of point iii) of Proposition \ref{propMeshGen}.\\


We now turn to the proof of Theorem \ref{thEquiMesh}, which is based on three (??) theorems presented in \cite{Shew}. 
%These theorems are based on a property that needs to be 
For that purpose we recall some definitions of this paper. %introduce the following definitions.
\begin{definition}
%The wedge of $v,v'$ is 
\begin{itemize}
\item (Wedge of two points)
We define the wedge $\wed(v,w)$ of two distinct sites $v,w\in V$ as follows
$$
\wed(v,w) := \{z\in \R^2 \sep (z-v)^\trans H(v) (w-v) >0 \text{ and } (z-w)^\trans H(w) (v-w) >0\}
$$ 
\item (Wedge property)
We say that the Voronoi diagram of $V$ is wedged if for any two distinct $v,w \in V$ we have 
$$
\Vor(v) \cap \Vor(w) \subset \wed(v,w).
$$
\end{itemize}
\end{definition}

The wedge property expresses that the collection $\Vor(v) \cap \Vor(w)$ of points $q$ shared by the Voronoi regions of the sites $v$ and $w$ lie in a cone defined by two linear inequalities.
We refer to \cite{Shew} Figure 4 for an illustration of the wedge of two sites.

The next proposition, which is partly is based on Lemma 5 from \cite{Shew},
 shows that the wedge property is automatically satisfied in our context.
For any metric $H$ and constant $c>0$ such that $c^2H\in \bH_g$, it easily follows from Proposition \ref{propEuclidRiemann} that for all $x,y\in \R^2$
\be
\label{eqDHLog}
\ln (1+ c\, d_x(y)) \leq c \, d_H(x,y) \leq - \ln(1- c\, d_x(y)), 
\ee
which is equivalent to 
\be
\label{eqDHExp}
1-\exp(-c\, d_H(x,y)) \leq c \, d_x(y) \leq \exp(c \, d_H(x,y))-1.
\ee

\begin{prop}
\label{propWedge}
For each $C_0$ there exists $c=c(C_0)>0$ such that the following holds.\\
If $V$ is $C_0$ equispaced and if $c^2H\in \bH_g$ then the wedge property is satisfied.
\end{prop}

\proof
We assume for contradiction that there exists two distinct vertices $v,w \in V$, and a point $q\in \Vor(V) \cap \Vor(W)$ such that $z\notin \wed(v,w)$. We may assume, up to exchanging the roles of $v$ and $w$, that 
$$
(q-w)^\trans H(w) (v-w) \leq 0.
$$
Defining 
$
\tau := \exp d_\times (H(v), H(w))
$
we obtain using Lemma 5 from \cite{Shew} %(*$q$ instead of $z$??*)
\be
\label{eqShewWedge}
 d_w(v) \leq d_w(q) \sqrt{\tau^2-1}.
\ee
We now estimate the quantities $d_w(v)$, $d_w(q)$ and $\tau$ appearing in this estimate, in order to obtain a contradiction when $c$ is sufficiently small.

Since the set $V$ is $C_0$-equispaced, there exists $u\in V$ such that $d_H(u,q) \leq C_0$. Recalling that $z\in \Vor(v)\cap \Vor(w)$ we thus obtain using \iref{eqDHExp}
\be
\label{eqDiamVor}
d_v(q) = d_w(q) \leq d_u(q) \leq \frac{\exp(c \, d_H(u,q))-1} c \leq r_0(c) := \frac{\exp(c C_0)-1} c,
\ee
and therefore using \iref{eqDHLog} 
\be
\label{eqVordvw}
d_H(v,w) \leq d_H(v,q)+ d_H(q,w) \leq r_1(c) := \frac {-2\ln (1- c r_0(c))}  c,% \frac 1 {1-f(c)}.
\ee
hence 
\be
\label{eqTauWedge}
\ln \tau = d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
\ee
Since the collection $V$ of sites is $C_0$-equispaced the sets $\{z \sep d_H(z,v) <C_0^{-1}\}$ and $\{z \sep d_H(z,w) <C_0^{-1}\}$ are disjoint. Therefore 
\be
\label{eqSepdvw}
d_H(v,w) \geq 2C_0^{-1}
\ee
which implies that %and using \iref{eqDHLog}
\be
\label{eqdvwWedge}
c d_w(v) \geq 1-\exp(-c d_H(v,w)) \geq 1-\exp(-2cC_0)
\ee

%We thus obtain $d_w(v)\geq \frac{1-\exp(-2 c C_0^{-1} )} c$ using \iref{eqDHExp}, furthermore we have 
%$$
%\ln \tau \leq d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
%$$
%
%
%the fact that $V$ is $C_0$-equispaced and
%
Injecting \iref{eqDiamVor}, \iref{eqTauWedge} and \iref{eqdvwWedge} in \iref{eqShewWedge} we obtain
\be
\label{eqFinalWedge}
1-\exp(-2 c C_0^{-1} )\leq (\exp(cC_0)-1) \sqrt{\exp(2c r_1(c))-1}.
\ee
For any fixed $C_0$, we have $r_0(c) \to C_0$ and $r_1(c) \to 2C_0$ as $c\to 0$. Therefore the left hand side of \iref{eqFinalWedge} is equivalent to $2cC_0^{-1}$ and the right hand side to $2c^2 C_0^2$, thus the inequality \iref{eqFinal} does not hold when $c$ is sufficiently small. The wedge property is therefore satisfied which concludes the proof of this proposition.
\sq

The dual of the Voronoi diagram is the graph defined by the collection of edges
$$
\{ [v,v'] \sep v,v'\in V \text{ and } \Vor(v) \cap \Vor(v') \neq \emptyset\} = \{\Cvx(V_z) \sep z\in \R^2 \text{ and } \#(V_z) = 2\}.
$$
The next theorem, established in \cite{Shew} under the name ``dual triangulation theorem'' shows that this graph is a polygonalization of $\R^2$ with strictly convex polygons when the wedge property is satisfied.
Furthermore these polygons are given by 
$$
\cT_0(V,H) = \{\Cvx(V_z) \sep z\in \R^2 \text{ and } \#(V_z) = 3\}.
$$
which shows that $\cT_0(V,H)$ is a partition of $\R^2$ into strictly convex polygons

We need to mention that the original result is more general and also applies to bounded polygonal domains, but this is not needed in our context.

%(*note : applied to the whole domain $\R^2$*)
\begin{theorem}[Dual triangulation theorem. Labelle, Shewchuck, \cite{Shew}]
\label{thShew}
If the Voronoi diagram of the point set $V \subset \R^2$ is wedged, then the geometric dual of this diagram is a polygonalization of $\R^2$ with strictly convex polygons and is a triangulation if $V$ is in general position.
\end{theorem}


The next theorem, originally stated in \cite{Shew} as Corollary 10 to Theorem 9 of the same paper, allows to control the angles of a triangle in the anisotropic Delaunay triangulation.

\begin{theorem}[Labelle, Shewchuk, \cite{Shew}]
\label{thAngle}
Let $v_1,v_2,v_3\in V$ and let $q\in \Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)$. Let 
$$
r = d_{v_1}(q) = d_{v_2}(q) = d_{v_3}(q) \stext{ and }
l = \min\{d_{v_i}(v_j) \sep i,j \in \{1,2,3\}, i \neq j\}.
$$ 
Define $\beta := \max\{r/l,\, 1/\sqrt 2\}$, %and %$\gamma\in [1,\infty)$ by 
%Let $1\leq \gamma \leq \sqrt 2$ and $\beta \geq \frac 1 {\sqrt 2}$ satisfy
$$
\gamma := \exp \max \{d_\times (H(v_i), H(v_j)) \sep i,j \in \{1,2,3\}, i \neq j\},
$$
and
\be
\label{defChi}
\chi := \frac 1 {2 \beta} - \frac{(\gamma^2-1)\beta} 2.
\ee
If $\gamma \leq \sqrt 2$ and $\chi>0$ then any angle $\theta$ of the triangle of vertices $(\sqrt{H(v_1)} v_k)_{1 \leq k \leq 3}$ satisfies
$$
\arcsin ( \chi/ \gamma^2) \leq \theta \leq 2 \arccos(\chi/\gamma^2).
$$
%where $S = H(v_1)^{\frac 1 2}$.
\end{theorem}

\begin{corollary}
For each $C_0\geq 1$ there exists $c=c(C_0)>0$ such that the following holds.
If $V$ is $C_0$ equispaced, if $c^2H\in \bH_g$ and if $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$, then denoting by $T$ the triangle of vertices $v_1,v_2,v_3$ we have for all $z\in T$
$$
C^{-2} H(z) \leq \cH(z) \leq C^2 H(z).
$$
\end{corollary}
\proof
We use \iref{eqDHExp} and \iref{eqDHLog} and the fact that $V$ is $C_0$-equispaced to obtain explicit bounds on the quantities $r$, $l$, $\beta$, $\gamma$ and $\chi$ appearing in Theorem \ref{thAngle}.

Proceeding as in the proof of Proposition \ref{propWedge}, inequalities \iref{eqDiamVor}, \iref{eqVordvw} and \iref{eqSepdvw}, we obtain 
$$
r\leq r_0(c) := (\exp(c C_0)-1)/c \stext{ and } 2 C_0^{-1} \leq d_H(v_i,v_j) \leq r_1(c) := -2\ln(1-c r_0(c))/c.
$$
%We have for all 
%$2C_0^{-1}\leq d_H(v_i,v_j) \leq 2C_0$ for all $1\leq i< j\leq 3$, and 
Therefore 
$$
l := \min_{i\neq j} d_{v_i}(v_j)\geq \min_{i\neq j} \frac{1-\exp(-c d_H(v_i,v_j))} c \geq  r_2(c) := \frac{1-\exp(-2cC_0^{-1})} c,
$$
$$
L := \max_{i\neq j} d_{v_i}(v_j) \leq (\exp(c r_1(c))-1)/c
$$
and 
$$
\gamma \leq \max_{i\neq j} \exp(c \,d_H(v_i,v_j)) \leq \exp(c \,r_1(c)).
$$
In particular 
$
\beta \leq r_3(c) := \min\{r_0(c)/r_2(c),\, 1/\sqrt 2\}. % = \frac{\exp(cC_0)-1}{1-\exp(-2 cC_0^{-1})},
$
Injecting this into \iref{defChi} yields an explicit lower estimate 
$$
\chi\geq r_4(c) := \frac 1 {2r_3(c)} - \frac{ (\exp(2cr_1(c))-1) r_3(c)} 2,
$$ 
and $\chi/\gamma^2\geq r_5(c) := r_4(c) \exp(-2cr_1(c))$.

For a fixed $C_0$ we obtain as $c\to 0$ the limits $r_0(c) \to C_0$, $r_1(c)\to 2 C_0$, $r_2(c) \to 2C_0^{-1}$, $r_3(c) \to \min\{C_0^2/2, 1/\sqrt 2\}$.
We assume without loss of generality that $C_0\geq \sqrt 2$ and we thus obtain $r_3(c) \to C_0^2/2$, 
$r_4(c) \to 1/C_0^2$ and $r_5(c) \to 1/C_0^2$. 
We may therefore choose $c$ sufficiently small in such way that 
$l \geq r_2(c)\geq C_0^{-1}$, $L \leq (\exp(c r_1(c))-1)/c \leq 4 C_0$ and $\chi/\gamma^2 \geq r_5(c)\geq 1/(2C_0^2)$.

We denote by $T$ the triangle of vertices $v_1, v_2, v_3$. The length of any edge of $T' := \sqrt{H(v_1)}(T)$ is bounded above and below by $l \geq C_0^{-1}$ and $L \leq 4 C_0$ respectively, and the angles of $T'$ satisfy $\arcsin ( 1/(2 C_0^2) ) \leq \theta \leq 2 \arccos(1/(2 C_0^2))$. The collection of triangles which satisfy these inequalities is compact, thus there exists a constant $C_1 = C_1(C_0)$ such that 
$$
C_1^{-2} \Id \leq \cH_{T'} \leq C_1^2 \Id,
$$
hence $C_1^{-2} H(v_1) \leq \cH_{T'} \leq C_1^2 H(v_1)$. For any $z\in T$ we obtain, remarking that $\|z-v_1\|_{\cH_T} \leq 2$ for all $z\in T$ and using \iref{eqLocalNorm}, 
$$
C_1^{-2} (1-2cC_1)^2 H(z) \leq \cH_{T'} \leq C_1^2(1-2cC_1)^{-2} H(z)
$$
which concludes the proof of this proposition.
\sq

\input{../Bibliography/Bibliography.tex}
\end{document}



==> MeshMetric/MeshMetricTheseOld2.tex <==
\input{../PreambleThese}

\section{Introduction}

Triangulations and meshes are finite objects of combinatorial nature: they can be described by a collection of vertices and of connection between these. This description is fruitful for the demonstration of algebraic results, such as the Euler formula, or for computer processing.
In contrast, many approaches towards anisotropic mesh generation are based on a continuous object, namely a riemannian metric $z\mapsto H(z)$, in other words a continuous function $H$ from the domain $\Omega\subset \R^d$ to the set $S_d^+$ of symmetric positive definite matrices. Once this metric has been properly designed, it is the task of a mesh generation algorithm such as \cite{Shew,Bois,FreeFem,Inria} to generate a triangulation that agrees with this metric, in a sense specified below \iref{defEquiv}.
The purpose of this chapter is to formulate precise equivalence results between some classes of triangulations and of riemannian metrics. This equivalence translates some geometrical constraints satisfied by the triangulations into the form of regularity properties of the equivalent riemannian metrics.\\

Our results are so far limited to meshes and metrics defined on the entire infinite domain $\R^d$, and the dimension $d\geq 2$ is fixed throughout this chapter. 
The choice of the unbounded domain $\R^d$ guided by simplicity, since the curvature and the singularities of
of the boundary $\partial\Omega$ induces additional difficulties 
from the point of view of computational mesh generation.
Bounded domains will be the object of future work.
We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$, and we introduce in \S\ref{subsecDefTStar} three embedded subsets of $\bT$ of particular interest 
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
where $C\geq 1$ is a parameter which plays a minor role.
The set $\bT_{i,C}$ collects all \emph{isotropic} meshes $\cT$ which are heuristically defined as follows: the simplices $T\in \cT$ may have strongly varying volumes, but their aspect ratio is uniformly bounded. 
The largest set $\bT_{g,C}$ collects \emph{graded} meshes, which only satisfy a condition of local consistency: all the  geometrical features of the simplices $T\in \cT$ may vary strongly, volume, aspect ratio and orientation, but two \emph{neighboring} simplices should not be excessively different.
The intermediate set $\bT_{a,C}$ collects \emph{quasi-acute} meshes, which definition involves the measure of sliverness $S(T)$ of a simplex $T$ introduced in Chapter \ref{chapW1P} and also discussed in Chapter \ref{chapApproxMet}. 
The measure of sliverness plays an important role in the finite element approximation of a function on a mesh $\cT$ when the error is measured in the Sobolev $W^{1,p}$ norm.\\

We associate to each simplex $T$ a symmetric positive definite matrix $\cH_T$ such that the ellipsoid
$$
\cE_T := \{z\in \R^d \sep (z-z_T) \cH_T (z-z_T)^\trans \leq 1\},
$$
which is centered at the barycenter $z_T$ of $T$,
is the ellipsoid of minimal volume containing $T$. The properties of the matrix $\cH_T$ are discussed in \S \ref{subsecIntroSimplex} of this introduction,  as well as its explicit expression in terms of the coordinates of the simplex $T$. The matrix $\cH_T\in S_d^+$ encodes the volume, the aspect ratio and the orientation (but not the angles) of the simplex $T$. Two triangles $T$ and their associated ellipses $\cE_T$ are illustrated on figure \ref{figET}.

\begin{figure}
\centering
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleAigu.pdf}
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleObtus.pdf}
	\caption{Two triangles $T$ and their associated ellipse $\cE_T$.\label{figET}}
\end{figure}

A riemannian metric on $\R^d$ is a continuous map $H$ which associates to any $z\in \R^d$ a symmetric positive definite matrix $H(z)\in S_d^+$. We denote by $\bH = C^0(\R^d,S_d^+)$ the collection of riemannian metrics.
The following definition introduce a notion of equivalence between meshes and metrics
\begin{definition}
\label{defEqHT}
We say that a mesh $\cT\in \bT$ is $C_0$-equivalent to a given metric $H\in \bH$, where $C_0\geq 1$ is a fixed constant, if for all $T \in \cT$ and all $z\in T$ one has 
\be
\label{defEquiv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
\ee
We say that a collection of simplicial meshes $\bT_*\subset \bT$ is equivalent to a collection $H_*$ of metrics if there exists a uniform constant $C_0\geq 1$ such that the following holds:
\begin{itemize}
\item For any mesh $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\item For any metric $H\in \bH_*$ there exists a mesh $\cT\in \bT_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\end{itemize}
\end{definition}
Our main result (Theorem \ref{thEquiv}) states that when the constant $C$ is sufficiently large, and if dimension is $d=2$, the three classes of meshes $\bT_{i,C}\subset \bT_{a,C} \subset \bT_{g,C}$ are respectively equivalent to three classes of metrics
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
that are defined by precise smoothness conditions on the function $z\mapsto H(z)$ in \S \ref{subsecDefHStar} of this introduction.
%Our main result Theorem \ref{thEquiv} states that when the parameter $C$ is large enough and the dimension is $d=2$, the collections $\bT_{\star,C}$ of triangulations are equivalent to the corresponding collections $H_\star$ of metrics for any symbol $\star \in \{i,a,g\}$. 
The most striking point of this result is that, although the matrix $\cH_T$ does not encode the angles of a simplex $T$, the fact that a mesh $\cT\in \bT_{a,C}$ is \emph{quasi-acute} can be translated in a precise regularity condition on the metric $H$ equivalent to $\cT$.

In order to state our results more precisely we need to introduce some notations. We first recall some notations of linear algebra. We denote by $\M_d$ the collection of $d\times d$ matrices with real entries. We denote by $\GL_d$ the standard linear group, by $\SL_d$ the special linear group and by $\cO_d$ the orthogonal group
\begin{eqnarray*}
\GL_d &:=& \{A\in \M_d\sep \det A\neq 0\}\\
\SL_d &:=& \{A\in \M_d\sep \det A=1\}\\
\cO_d &:=& \{U\in \M_d\sep U^\trans U = \Id\}.
\end{eqnarray*}
We denote by $S_d$ the collection of symmetric matrices, by $S_d^\oplus$ the subset of non-negative symmetric matrices, and by $S_d^+$ the collection of symmetric positive definite matrices.
\begin{eqnarray*}
S_d &:=& \{M\in \M_d\sep M = M^\trans\}\\
S_d^\oplus &:=& \{M\in S_d\sep z^\trans M z \geq 0 \text{ for all } z\in \R^d\}\\
S_d^+ &:=& S_d^\oplus \cap \GL_d.
\end{eqnarray*}
Let $M,M'\in S_d$, we write $M\leq M'$ if $M'-M\in S_d^\oplus$, and $M< M'$ if $M'-M\in S_d^+$. We recall that for any $M,M'\in S_d$ such that $M\leq M'$ and any $\phi\in \M_d$ we have $\phi^\trans M \phi \leq \phi^\trans M' \phi$. Furthermore if $M,M' \in S_d^+$ and $M\leq M'$ then $M'^{-1} \leq M^{-1}$. For each symmetric positive definite matrix $M\in S_d^+$ we define a norm $\|\cdot\|_M$ as follows: for all $u\in \R^d$
$$
\|u\|^2_M := u^\trans M u.
$$

\subsection{Geometry of the simplex}
\label{subsecIntroSimplex}
The basic geometrical object studied in this chapter is the $d$-dimensional simplex, which is defined as follows.
\begin{definition}
A $d$-dimensional simplex $T$ is the convex envelope of a set $V\subset \R^d$ of $d+1$ %non-coplanar 
vertices, not contained in a $d-1$ dimensional affine subspace of $\R^d$ : 
$$
T = \Cvx(V).
$$
We denote by $\cF(T)$ the collection of faces of $T$ of any dimension,
\be
\label{defFT}
\cF(T) := \{\Cvx(V') \sep V'\subset V\}.
\ee
\end{definition}
Observe that $\emptyset$ and $T$ are among the faces of a simplex $T$, since they respectively correspond to $V'=\emptyset$ and $V'=V$.
We denote by $z_T\in \R^d$ the barycenter of a simplex $T$ of vertices $V$
$$
z_T := \frac 1 {d+1} \sum_{v\in V} v,
$$
and we define a symmetric positive definite matrix $\cH_T\in S_d^+$ as follows
\be
\label{defcH}
\cH_T^{-1} = \frac d {d+1} \sum_{v\in V} (v-z_T) (v-z_T)^\trans. %\frac {2d}{(d+1)^2}\sum_{v,v'\in V} (v-v')(v-v')^\trans. 
\ee
Some of the key properties of the matrix $\cH_T$ are exposed in the next proposition.
Throughout this chapter, we denote by $\TEq$ a $d$-dimensional equilateral simplex, centered at the origin
i.e. such that $z_\TEq=0$, and having its vertices on the unit ball. One easily checks that 
$$
\cH_\TEq = \Id.
$$
% Note that 
%\be
%\label{eqBallTEq}
%%\{z\in \R^d \sep |z| \leq 1/d\} 
%B(0, 1/d) \subset \TEq \subset \overline B(0,1).
%\ee
%
%%We associate to any simplex $T$ its barycenter $z_T\in \R^d$, and a symmetric positive definite matrix
%We denote by $z_T$ the barycenter of a simplex $T$, and we also associate to $T$ a symmetric positive definite matrix $\cH_T\in S_d^+$ which encodes some of its geometrical properties, in particular the volume, the elongation and the orientation of $T$.
\begin{prop}
\label{propHT}
The following holds for any $d$-dimensional simplex $T$. 
\begin{itemize}
\item
For any an affine change of coordinates $\Phi$, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0$ in $\R^d$, we have 
\be
\label{invcH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
\item
There exists a rotation $U\in \cO_d$, depending on $T$, such that 
\be
\label{eqcHTEq}
\cH_T^\frac 1 2 (T-z_T) = U(\TEq),
\ee
hence 
\be
\label{eqVolTHT}
|T| \sqrt{\det \cH_T} = |\TEq|.
\ee
\item
We have the inclusions 
\be
\label{eqTET}
\{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1/d\} \subset T \subset \cE_T := \{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1\},
\ee
and the these two ellipsoids are respectively the one of largest volume included in $T$, and of smallest volume containing $T$.
\end{itemize}
\end{prop}
\proof
For any simplex $\Phi^{-1}(v)$ of the simplex $\Phi^{-1}(T)$, we have 
$$
\Phi^{-1}(v)-z_{\Phi^{-1}(T)} = \Phi^{-1}(v)-\Phi^{-1}(z_T) = \phi^{-1}(v-z_T).
$$
Injecting this relation in \iref{defcH} we obtain \iref{invcH}. 
We now turn to the proof of \iref{eqcHTEq} and for that purpose we remark that the simplices $\TEq$ and $T' := \cH_T^\frac 1 2 (T-z_T)$ have both their barycenter at zero, $z_\TEq = z_{T'} = 0$, hence there exists a linear map $\phi\in \GL_d$ such that $T' = \phi^{-1}(\TEq)$. We thus obtain, using the formula \iref{invcH} for the transformation of $\cH_T$ under affine change of coordinates 
$$
\begin{array}{ccccc}
\cH_{T'} &=& \cH_T^{-\frac 1 2} \cH_T \cH_T^{-\frac 1 2} &=& \Id \\ 
\cH_{\phi^{-1}(\TEq)} &=& \phi^\trans \cH_\TEq &=& \phi^\trans \phi.
\end{array}
$$
Hence $\phi^\trans \phi= \Id$ which establishes that $\phi\in \cO_d$ and concludes the proof of \iref{eqcHTEq}.
%One easily checks that 
%$$
%\overline B(0,1/d) \subset \TEq \subset \overline B(0,1),
%$$
%where
It is well known that the smallest ellipsoid containing $\TEq$ is the unit ball, and that the largest ellipsoid included in $\TEq$ is the ball of radius $1/d$. Combining this fact with the change of coordinates \iref{eqcHTEq} we obtain \iref{eqTET} which concludes the proof of this proposition.
\sq

Note that for any simplex $T$ and any $z,z'\in T$ we obtain using \iref{eqTET}
\be
\label{eqDiamTHT}
\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2.
\ee

We introduce a measure of degeneracy $\rho(T)$ of a $d$-dimensional simplex $T$
\be
\label{defRhoMM}
\rho(T) := \sqrt{\|\cH_T\| \|\cH_T^{-1}\|}.
\ee
%This measure of non degeneracy $\rho$ is slightly different from the measure of non degeneracy $\frac {\diam(T)^d} {|T|}$ used in some of the previous chapters. However these two measures play a similar role and can be compared. Indeed we obtain using \iref{eqVolTHT} and \iref{eqcTET}
%\be
%\label{eqRhoRhop}
%\frac{\rho(T)}{d^\frac d 2|\TEq|} \leq  \frac{(\|\cH_T^{-1}\|/d)^\frac d 2} {|\TEq| (\det \cH_T)^{-\frac 1 2}} \leq \frac{\diam(T)^d} {|T|} \leq \frac{\|\cH_T^{-1}\|^\frac d 2} {|\TEq|(\det \cH_T)^{-\frac 1 2}}\leq \frac{\rho(T)^{d-1}}{|\TEq|}.
%\ee
%Observing that $\|A\| \|A^{-1}\|^{-(d-1)} \leq |\det A| \leq \|A\|^{d-1} \|A^{-1}\|^{-1}$ for any $A\in \GL_d$
%it follows that 
Observe that $\rho(T)\geq 1$ for any simplex $T$, with equality if and only if $\cH_T$ is proportional to the identity, which implies in view of \iref{eqcHTEq} that $T$ is a displacement of the equilateral simplex $\TEq$:
$$
\rho(T) = 1 \stext{ if and only if }
%\ \Longleftrightarrow \ 
T = z_T+r U(\TEq) \text{ for some }  r>0 \text{ and } U \in \cO_d.
$$
The measure of degeneracy $\rho$ is slightly different from the measure of degeneracy $\frac {\diam(T)^d} {|T|}$ used in Chapters \ref{chapOptAniso} and \ref{chapW1P} but both have the same role: they are minimal for the equilateral simplex, and increase as the simplex becomes thinner.\\

The measure of sliverness $S(T)$ of a simplex $T$ is a quantity which plays an important role in the context of optimal mesh adaptation for the finite element approximation of a function in the Sobolev $W^{1,p}$ norm, see   \cite{Ba, Ja}, and Chapters \ref{chapW1P} and \ref{chapApproxMet}. 
This measure of sliverness is defined in Chapter \ref{chapW1P} and illustrated by several examples and equivalent quantities. We recall the definition of this quantity
\be
\label{defSMM}
S(T) := \inf \{ \|\phi\| \|\phi^{-1}\| \sep \phi \in \GL_d \text{ and } \phi(T) \text{ is acute } \},
\ee
a simplex is acute if the exterior normals $\n, \n'$ to any two distinct faces of $T$ have a negative scalar product $\<\n,\n'\>\leq 0$.
As observed in Chapter \ref{chapW1P}, the measure of sliverness $S(T)$ can be interpreted as the distance from $T$ to the collection of acute simplices.

The exterior normals $\n,\n'$ to any two $d-1$-dimensional faces of $\TEq$ satisfy $\<\n,\n'\> =-1/d$, hence this simplex is acute. Recalling \iref{eqcHTEq}
 we thus obtain for any simplex $T$
$$
S(T) \leq \rho(T).
$$
Apart from this upper bound, the matrix $\cH_T$ does not contain any direct information on the measure of sliverness $S(T)$.
%One of the key results of this chapter is that in a bidimensional triangulation $\cT$, and conjecturedly in higher dimension too, the variation of the matrix $\cH_T$ as $T$ varies in $\cT$ does encode the measure of sliverness in some sense.
For any bidimensional triangle $T$ of largest angle $\theta$, Proposition \ref{propSTan} of Chapter \ref{chapW1P} states that :
$$
S(T) = \max\left\{1, \tan \frac \theta 2 \right\}.
$$

\subsection{Simplicial meshes}
\label{subsecDefTStar}

As a starter, we recall the definition of a simplicial mesh of $\R^d$.
%We first briefly recall the defini
%Before introducing simplicial meshes, we briefly recall the definition of locally finite partitions of $\R^d$.

%In order to introduce q,xcl meshes 
\begin{definition}
\label{defSimplMesh}
A conforming simplicial mesh of $\R^d$ is a collection $\cT$ of simplices which satisfy the conformity axiom :  for all $T,T'\in \cT$
\be
\label{confAxiom}
T\cap T' \in \cF(T) \cap \cF(T'),
\ee
as well as the following properties
\begin{itemize}
\item (Covering) The simplices $T\in \cT$ cover the whole infinite domain $\R^d$:
$$
\bigcup_{T\in \cT} T = \R^d.
$$
\item (Partition) The interiors of the simplices $T\in \cT$ are pairwise disjoint: for any $T,T'\in \cT$,
$$
\interior (T) \cap \interior(T') \neq \emptyset\stext{ implies }  T=T'. %
$$
\item (Local finiteness) For any compact set $K \subset \R^d$, only a finite collection of simplices $T\in \cT$ intersect $K$:
$$
\{T \in \cQ \sep K \cap T \neq \emptyset \} \ \text{ is finite.}
$$
\end{itemize}
\end{definition}
The conformity axiom \iref{confAxiom} states that the intersection of any two simplices in $\cT$ needs to be a full common face.We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$.

For an optimal efficiency, numerous numerical simulation software use anisotropic meshes, in which the simplices may have an arbitrary shape. Anisotropic meshes are used for instance, to create a thin layer of simplices close to a geometric feature which is relevant in a numerical simulation.
In order to avoid excessively wild meshes, one often requires relevant  some consistency between the shapes of neighboring simplices.We therefore introduce for any constant $C \geq 1$ the class $\bT_{g,C} \subset \bT$ of \emph{graded} meshes, which is defined as follows.
A mesh $\cT$ belongs to $\bT_{g,C}$ if for any two simplices $T,T'\in \cT$ one has 
\be
\label{defTG}
T \cap T'\neq \emptyset \stext{ implies } C^{-2}\cH_T \leq \cH_{T'} \leq C^2 \cH_T.
\ee

For any $C\geq 1$ we also introduce the class $\bT_{i,C}$ of \emph{isotropic} meshes, by requiring that in addition to \iref{defTG} that the measure of degeneracy $\rho$ is uniformly bounded by $C$, which forbids any anisotropy.
A mesh $\cT$ belongs to $\bT_{i,C}$ if and only if $\cT\in \bT_{g,C}$ and for all $T \in \cT$
$$
\rho(T) \leq C. %C \geq 1? or 0? 
$$

%The next proposition shows that the definition of $\bT_{i,C}$ is slightly redundant, in the sense that condition \iref{defTG} could be avoided.
%\begin{prop}
%Denote by $\bT'_{i,C}$ the collection of meshes $\cT\in \bT$ satisfying $\rho(T) \leq C$ for all $T\in \cT$ (but perhaps not the gradedness condition \iref{defTG}). %We thus have $\bT_{i,C} \subset \bT'_{i,C}$.\\
%Then for all $C$ there exists $C' = C'(C)$ such that 
%$$
%\bT_{i,C} \subset \bT'_{i,C} \subset \bT_{i,C'}.
%$$
%\end{prop}
%
%\proof
%See appendix. 
%\sq

In order to introduce the intermediate collection $\bT_{a,C}$ of $C$-quasi-acute meshes, we first define the notion of refinement of a simplicial mesh.
\begin{definition}
Consider two meshes $\cT,\cT'\in \bT$ and a constant $C\geq 1$. We say that $\cT'$ is a $C$-refinement of $\cT$ if it satisfies the following properties.
\begin{itemize}
\item (Inclusion) Any simplex $T'\in \cT'$ is contained in a simplex $T\in \cT$. % such that $T'\subset T$.
\item (Bounded refinement) Any simplex  $T\in \cT$, contains most $C$ simplices $T'\in \cT$.
\end{itemize}
\end{definition}

A graded mesh $\cT \in \bT_{g,C}$ belongs to the collection $\bT_{a,C}$ of quasi-acute meshes if and only there exists a $C$-refinement $\cT'$ of $\cT$ which satisfies for all $T' \in \cT'$
$$
S(T') \leq C.
$$
In particular if $\cT\in \bT_{i,C}$, then choosing $\cT' = \cT$, which is a $C$-refinement since $C\geq 1$, and recalling that $S(T) \leq \rho(T)$ for any simplex $T$, we obtain that $\cT\in \bT_{a,C}$. Thus $\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}$ as announced.

The constraints defining graded, quasi-acute and isotropic meshes are illustrated on Figure \ref{figDisk}
in the main introduction of the thesis. 
Figure \ref{figAcuteGen} gives an example of a quasi-acute triangulation which 
by the above described refinement process leads to a slightly finer triangulation on
sliverness $S(T)$ is uniformly bounded.

\begin{figure}
\centering
%	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarGdeVap.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap1.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap2.pdf}
	\caption{\label{figAcuteGen}
Quasi-acute triangulation (left) and refined triangulation with uniformly bounded sliverness (right).
	}
\end{figure}

\subsection{Riemannian metrics}
\label{subsecDefHStar}

For any metric $H \in \bH$ and path $\gamma \in C^1([a,b],\R^d)$, we define the riemmannian length $l_H(\gamma)$ by the integral
$$
l_H(\gamma) := \int_a^b \|\gamma'\|_{H(\gamma(t))} dt.
$$
The riemmannian distance $d_H$ between two points  $z,z'\in \R^d$, is the infimum of the length of all paths joining $z$ and $z'$, 
\be
\label{defdH}
d_H(z,z') := \inf\left\{l_H(\gamma)\sep \gamma\in C^1\left([0,1],\R^d\right), \ \gamma(0) = z \text{ and } \gamma(1) = z'\right\}.
\ee
If $H, H'\in \bH$ are such that $H(z) \leq H'(z)$ for all $z\in \R^d$, then $d_H(z,z') \leq d_{H'}(z,z')$ for all $z,z'\in \R^d$.
By construction, the riemannian distance $d_H$ associated to a metric $H\in \bH$ is locally equivalent close to a point $z$ to the distance defined by the norm $\|\cdot \|_{H(z)}$: for all $z\in \R^d$
\be
\label{eqDistLoc}
\limsup_{\ve \to 0} \sup_{p,q\in B(z, \ve)} |\ln d_H(p,q) - \ln \|p-q\|_{H(z)}| = 0,
\ee
where $B(z,\ve)$ denotes the euclidean ball of radius $\ve$ around $z$.\\


\begin{remark}[Riemannian geodesics]
When a metric $H$ is sufficiently smooth, a special family of curves named Riemannian geodesics can be defined and studied. A riemannian geodesic is a curve $\gamma\in C^0(\R, \R^d)$ which satisfies a second order differential equation %written in terms of the second order derivatives of $H$, 
called the equation of geodesics. This equation implies that for any sufficiently close $t,t'\in \R$ the curve $\gamma_{|[t,t']}$ is the path of smallest possible length joining the points $\gamma(t)$ and $\gamma(t')$ : 
$d_H(\gamma(t), \gamma(t')) = l_H(\gamma_{|[t,t']})$.

Geodesics are not defined for general continuous or Lipschitz riemannian metrics, such as those constituting the sets $\bH$ and $\bH_i \subset \bH_a\subset \bH_g$, since the coefficients of the equation of geodesics involve the second derivatives of the metric. Notions related to geodesics, such as the injectivity radius of a metric, therefore have no meaning in our context.
This is not an issue for our purposes since, following the point of view of \cite{Gromov},
%[Gromov, Metric structures for Riemannian and non-Riemannian spaces, Birkhauser (1999)]
we study Riemannian distances and not Riemannian geodesics. 

%Note also that geodesics only exist when the metric $H$ has requires that $H$ has at least $C^2$ smoothness, while the metrics studied in this chapter generally only have $C^0$ or Lipschitz smoothness.

%Since we only assume that $H$ is a continuous metric, the infimum \iref{defdH} may or may not be attained, and in that later case possibly for several paths. The equation of geodesics associated to a riemannian metric involves the second order derivatives, which are not defined in our context.
%(* also the point of view of Gromov : we study distances and not geodesics*)
\end{remark}


We denote by $\bH_i$ the collection of metrics $H \in \bH$ which are proportionnal to the identity: for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2},
$$
and such that the proportionality factor $s$ satisfies one of the two following conditions conditions, which are surprisingly equivalent as shown in Proposition \ref{propEquivS}:
\begin{itemize}
\item (``Additive'' Lipschitz condition)  
\be
\label{eqLipSAdd}
|s(z) - s(z')| \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
\item (``Multiplicative'' Lipschitz condition)
\be
\label{eqLipSMult}
|\ln s(z) - \ln s(z')| \leq d_H(z,z') \stext{ for all } z,z'\in\R^d.
\ee
\end{itemize}

The two Lipschitz properties \iref{eqLipSAdd} and \iref{eqLipSMult} have a natural generalisation to general anisotropic metrics but are not equivalent in that context.
In order to introduce the regularity conditions defining the classes $\bH_i\subset \bH_a\subset \bH_g$ of metrics, we need to  two distances $d_\times$ and $d_+$ on the set $S_d^+$ of symmetric positive definite matrices. 
For any $M,M'\in S_d^+$ we define
\be
\label{defDTimes}
d_\times (M,M') := \min \{\delta \geq 0 \sep e^{-2\delta} M \leq M' \leq e^{2 \delta} M\}.
\ee
For instance, a mesh $\cT$ is $C$-equivalent to a metric $H$, as defined in \iref{defEquiv}, if and only if for all $T \in \cT$ and all $z\in \cT$ one has 
$$
d_\times (H(z), \cH_T) \leq \ln C.
$$
There exists various expressions of the distance $d_\times$ : for all $M,M'\in S_d^+$ one has 
\be
\label{eqDTimesLog}
d_\times (M,M') = \sup_{u\in \sR^d\sm \{0\}} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
\ee
and 
\be
\label{eqDTimesProd}
d_\times (M,M') = \ln \left(\max \{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\}\right).
\ee
The exponential of the distance $d_\times$ was used in the earlier paper \cite{Shew} %on anisotropic mesh generation
under the name ``relative deformation''. 
We define a second distance $d_+$ on $S_d^+$ as follows 
\be
\label{defDPlus}
d_+(M,M') := \|M^{-\frac 1 2} - M'^{-\frac 1 2}\|.
\ee
The expressions \iref{eqDTimesProd} and \iref{defDPlus} of the distances $d_\times$ and $d_+$ show that they are respectively tied to multiplicative or additive properties of matrices, which justifies their notations.
Note also that for any $s,s'>0$ one has
\be
\label{eqDIso}
d_\times (s^{-2} \Id, s'^{-2} \Id) = |\ln s - \ln s'| \stext{ and } d_+(s^{-2} \Id, s'^{-2} \Id) = |s-s'|.\\
\ee

We denote by $\bH_g$ the collection of metrics $H\in \bH$ which satisfy the natural extension of \iref{eqLipSMult} to general anisotropic metrics:
\be
\label{eqLipMult}
d_\times (H(z), H(z')) \leq d_H(z,z') \stext{ for all }z,z'\in\R^d.
\ee
This condition can be heuristically described as follows: a metric $H\in \bH$ defines close to each point $z\in\R^d$ a norm $\|\cdot\|_{H(z)}$ which encodes an anisotropic notion of scale. The equation \iref{eqLipMult} states that the metric $H$ itself is consistent a the scale that it encodes.\\

We denote by $\bH_a$ the collection of metrics $H\in \bH$ which satisfy both \iref{eqLipMult} and the natural extension of \iref{eqLipSAdd} to general anisotropic metrics:
\be
\label{eqLipAdd}
d_+ (H(z), H(z')) \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
In addition to the results of mesh generation presented in this chapter, we show in the next chapter, Chapter\ref{chapApproxMet}, that this condition is critical in order to define a local averaging operator compatible with Sobolev norms. 
%decrire le lien avec les angles aigus.
\begin{remark}
\label{remHomog}
Let $H\in \bH$, and let $\lambda>0$. Using the homogeneity properties of the distances $d_\times$, $d_+$ on $S_d^+$ and $d_H$ on $\R^d$ with respect to $H$, we obtain that $\lambda^2 H\in \bH_g$ if and only if 
\be
\label{eqLipTimesLambda}
d_\times (H(z), H(z')) \leq \lambda d_H(z,z') \stext{ for all } z,z'\in \R^d, 
\ee
and $\lambda^2 H\in \bH_a$ if and only if we have in addition to the previous property 
\be
\label{eqLipPlusLambda}
d_+ (H(z), H(z')) \leq \lambda |z-z'| \stext{ for all } z,z'\in \R^d.
\ee
In particular the collections $\bH_i \subset \bH_a \subset \bH_g$ of isotropic, quasi-acute and graded metrics are stable under multiplication by a constant larger than one : for any $\star \in \{a,b,c\}$, any $H\in \bH_\star$ and any $\lambda \geq 1$ we have $\lambda^2 H\in \bH_\star$.
%this operation corresponds to the uniform refinement of a triangulation...
\end{remark}

\subsection{Main results}

The main result of this chapter is the equivalence of the classes of meshes and metrics defined above, which is  announced in the first part of the introduction and proved in sections \S\ref{secMeshToMet} and  \S \ref{secMetToMesh}. In two cases we were only able to establish this equivalence when the dimension is $d=2$. 
\begin{theorem}
\label{thEquiv}
There exists $C_0 = C_0(d)$ such that for all $C\geq C_0$ the following holds.
\begin{enumerate}[i)]
\item The collections $\bT_{i,C}$ of triangulations and $\bH_i$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{a,C}$ of triangulations and $\bH_a$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{g,C}$ of triangulations and $\bH_g$ of metrics are equivalent.
\end{enumerate}
\end{theorem}

Let us comment on this result.
The theory of isotropic meshes is already well developed, and our result i) in this direction should be regarded as a reformulation of previous work, intended to put into perspective the results on anisotropic meshes. The main ingredient of the proof of i) is the mesh refinement procedure exposed in \cite{Nochetto}. 

In the case iii) of graded metrics the key ingredients used for the construction of a triangulation $\cT\in \bT_{g,C}$ equivalent to a metric $H \in \bH_g$ come from the paper of computational geometry \cite{Shew}. In contrast the arguments used to produce a metric $H \in \bH_g$ from a mesh $\cT \in \bH_{g,C}$ are new, to the knowledge of the author, and they hold in any dimension.

Last the author has not heard of any anterior results on the collection $\bT_{a,C}$ of quasi-acute meshes, and most of the techniques used in that context are new.

\begin{conjecture}
The author conjectures that the points ii) and iii) of Theorem \ref{thEquiv} holds without restriction on the dimension $d$.
\end{conjecture}

This chapter is organised as follows. We establish in section \S \ref{secMetProp} some general properties of metrics in $\bH_a$ or $\bH_g$. 
We first prove in \S\ref{subsecMetInv} a property of invariance of the collection $\bH_g$ of graded metrics with respect to affine changes of coordinates.
The regularity assumptions \iref{eqLipMult} and \iref{eqLipAdd} defining graded and quasi-acute metrics simply mean that the map $H : \R^d \to S_d^+$ is Lipschitz with respect to some distances on $\R^d$ and $S_d^+$. 
We therefore study metrics from this point of view in \S\ref{subsecMetLip}.
We focus in \S\ref{subsecMetGeom} on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. In particular we compare the $d_H$ with the euclidean distance and we estimate the volume of balls. 


Section \S\ref{secEigen} is devoted to the study of metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has  an eigenspace of dimension at least $d-1$ at each point. This condition clearly holds if the dimension is $d=2$ but is also relevant in some applications to higher dimension such as the creation of a this layer of simplices close to a $d-1$ dimensional surface. This situation is discussed in Chapter \ref{chapApproxMet}, and involves metric which have an eigenvalue much larger that the others in the orthogonal direction to the surface of interest.
We give an approximate translation of the regularity properties \iref{eqLipAdd} and \iref{eqLipMult} defining the collections $\bH_a$ and $\bH_g$ of metrics in terms of the two eigenvalues of $H$ and of the direction of the eigenspaces of such metrics. 

The last two sections \S\ref{secMeshToMet} and \S\ref{secMetToMesh} are devoted to the proof of Theorem \ref{thEquiv}. More precisely we adress in \S\ref{secMetToMesh} the production of an isotropic, quasi-acute or graded mesh equivalent to a given metric $H\in \bH_i$, $\bH_a$ or $\bH_g$. Conversely we depict in \S\ref{secMeshToMet} to construction of a metric which is equivalent to a given mesh.


\section{General properties of graded and quasi-acute metrics}
\label{secMetProp}

We study in this section the general properties of the  distinguished classes of metrics $\bH_i \subset \bH_a \subset \bH_g$. 
We first establish in \S\ref{subsecMetInv} some invariance properties of these collections of metrics with respect to affine changes of coordinates.
We then regard in \S\ref{subsecMetLip} metrics as Lipschitz functions $H : \R^d\to S_d^+$. %, and we recall some basic properties of these.
The last subsection \S\ref{subsecMetGeom} is devoted to the comparison of the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$, with respect to the standard euclidean distance and Lebesgue measure.

\subsection{Invariance properties and restriction of metrics}
\label{subsecMetInv}

We focus in this subsection on the properties of invariance of the collections of meshes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ and of metrics $\bH_i \subset \bH_a\subset \bH_g$ introduced in this chapter.

Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$.
We have for any simplex $T$, as previously observed in \iref{invcH},
\be
\label{eqInvH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
Mimicking this property we define for any $H \in \bH$ a transported version $H_\Phi\in \bH$ as follows: for all $z\in \R^d$
\be
\label{defHPhi}
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi.
\ee
In the language of differential geometry,
the metric $H_\Phi$ is generally referred to as the ``pull back'' of $H$ by $\Phi$. If a mesh $\cT\in \bT$ is $C$-equivalent to a metric $H\in \bH$, then \iref{eqInvH} and \iref{defHPhi} clearly imply that the mesh $\Phi^{-1}(\cT)$ is $C$-equivalent to the metric $H_\Phi$.

The next proposition studies the invariance of the collections $\bT_{\star,C}$ of meshes and $\bT_\star$ of metrics, $\star \in \{i,a,g\}$, under the transformations $\cT \mapsto \Phi^{-1}(\cT)$ or $H \mapsto H_\Phi$ induced by an affine change of coordinates $\Phi$.

\begin{prop}
\label{propInvT}
Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. 
The following holds for any constant $C\geq 1$.
\begin{enumerate}[i)]
\item If $\cT \in \bT_{g,C}$ then $\Phi^{-1}(\cT) \in \bT_{g,C}$. If $H \in \bH_g$ then $H_\Phi\in \bH_g$.
\item Assume that $\Phi$ is an isometry, in other words $\phi\in \cO_d$.\\
If $\cT\in \bT_{a,C}$ then $\Phi^{-1}(\cT)\in \bT_{a,C}$, and similarly if $\cT\in \bT_{i,C}$ then $\Phi^{-1}(\cT)\in \bT_{i,C}$.\\
If $H\in \bH_a$ then $H_\Phi\in \bH_a$, and similarly if $H\in \bH_i$ then $H_\Phi\in \bH_i$.
\end{enumerate}
\end{prop}

\proof
%We concentrate on the case of meshes, since the statements on metrics are a special case of the propositions (??) and (??) below (* no : state the result for iso and quasi acute metrics too*).
%We first consider the case of meshes, and then 
We first establish the properties announced for meshes, and we then focus on metrics.
Let $M,M'\in S_d^+$, let $C\geq 1$ and let $\phi\in \GL_d$. Clearly
$$
\text{ if } C^{-2} M \leq M' \leq C^2 M \stext{ then } C^{-2} \phi^\trans M\phi \leq \phi^\trans M'\phi  \leq C^2 \phi^\trans M\phi.
$$
%Consequently if a mesh $\cT$ satisfies the condition \iref{defTG} defining the elements of $\bT_{g,C}$
%
%satisfy $C^{-2} M \leq M' \leq C^2 M$, then we also ha
%For any $M,M'\in S_d^+$ we obtain using \iref{defDTimes} that 
%$$
%d_\times (\phi^\trans M \phi,\ \phi^\trans M' \phi) = d_\times (M,M').
%$$
%It follows using \iref{eqInvH} that for any  two simplices $T,T'$,
%$$
%d_\times (\cH_{\Phi^{-1}(T)}, \cH_{\Phi^{-1}(T')}) = d_\times (\cH_T,\cH_{T'}).
%$$ 
In view of the definition \iref{defTG} of $\bT_{g,C}$ we obtain that $\Phi^{-1}(\cT)\in \bT_{g,C}$ for any mesh $\cT\in\bT_{g,C}$ as announced in i).

If $\Phi$ is an isometry then for any simplex $T$ we obtain, using the definitions \iref{defRhoMM} and \iref{defSMM} of the measure of degeneracy $\rho$ and the measure of sliverness $S$, that
$$
\rho(\Phi^{-1}(T)) = \rho(T) \stext{ and } S(\Phi^{-1}(T)) = S(T).
$$
This implies the properties of $\bT_{a,C}$ and $\bT_{i,C}$ announced in b), which concludes the proof of the properties announced for meshes.

We therefore turn our attention to metrics. The fact that $H_\Phi\in \bH_g$ for any $H\in \bH_g$ and any affine change of coordinates $\Phi$ is a special case of Proposition \ref{propHG} below. We thus admit this property and we focus on isotropic and graded metrics and isometric changes of coordinates.

If $H\in \bH_i$, then $H = \Id/s(z)^2$ where $s: \R^d \to \R_+^*$ is a Lipschitz function. Since $\phi\in \cO^d$ we have $\phi^\trans \phi = \Id$ and therefore 
$$
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi = \Id/s(\Phi(z))^2.
$$
The map $s \circ \Phi : \R_d\to \R_+^*$ is Lipschitz since it is the composition of a Lipschitz function with an isometry, which establishes that $H_\Phi\in \bH_i$ as announced.

If $H\in \bH_a$ and $\Phi$ is an isometry, then for any $z,z'\in \R^d$
\begin{eqnarray*}
\|H_\Phi(z)-H_\Phi(z')\| &=& \|\phi^\trans \left(H(\Phi(z))-H(\Phi(z'))\right) \phi\| \\
&=& \|H(\Phi(z))-H(\Phi(z'))\|\\
& \leq& \|\Phi(z)-\Phi(z')\|\\
& =& \|\phi(z-z')\|= |z-z'|,
\end{eqnarray*}
which establishes that $H_\Phi$ satisfies the Lipschitz regularity condition \iref{eqLipAdd}. We already know from the case of graded metrics that the other regularity condition \iref{eqLipMult} is satisfied by $H_\Phi$, which establishes that $H_\Phi\in \bH_a$ and concludes the proof of this proposition.
\sq


In practical applications, one often needs to mesh simultaneously a domain $\Omega$ and a surface $\Gamma$ embedded in $\Omega$. In terms of metric this raises the following question: given a metric $H$ on $\Omega$ which satisfies certain properties of regularity %, corresponding do a certain class of meshes, 
what is the regularity of the restriction of this metric to $\Gamma$?

The next proposition answers this question is the simplified setting where $\Omega$ is the infinite domain $\R^d$, $\Gamma$ is an affine subspace of $\R^d$, and properties of regularity are those defining the collection $\bH_g$ of graded metrics. For any $1\leq k \leq d$ we denote by $\bH_g(\R^k)$ the collection of graded metrics on $\R^k$.

\begin{prop}
\label{propHG}
Let $1\leq k\leq d$, let $\Phi : \R^k\to \R^d$ be an affine injective map, $\Phi(z) = \phi z+z_0$ where $\phi\in M_{d,k}$ has rank $k$ and $z_0\in \R^d$. Let $H\in \bH$ and let for all $z\in \R^k$
$$%\be
%\label{defHPhi}
H_\Phi(z) := \phi^\trans H(\Phi(z)) \phi.
$$%\ee
If $H\in \bH_g$ then $H_\Phi\in \bH_g(\R^k)$. 
\end{prop}

\proof
For any $u\in \R^d$, one has 
\be
\label{chgNorm}
\|u\|_{H_\Phi(z)} = \|\phi(u)\|_{H(\Phi(z))}.
\ee
Hence for any $z,z'\in \R^k$ we obtain using \iref{eqDTimesLog},
\be
\label{dNHPhi}
\begin{array}{rcl}
d(H_\Phi(z), \ H_\Phi(z'))  &=&\displaystyle \sup_{u\in \sR^k\sm\{0\}} \left|\ln \left\|\phi(u)\right\|_{H(\Phi(z))} -\ln \left\|\phi(u)\right\|_{H(\Phi(z'))}\right| \\
& \leq& d(H(\Phi(z)), \  H(\Phi(z')))
\end{array}
\ee
For any path $\gamma\in C^1([0,1], \R^k)$, it follows from \iref{chgNorm} that % the distorted lengths tied to $H$ and $H_\phi$ are therefore linked by 
$$
l_H(\Phi\circ \gamma) = \int_0^1 \|\phi(\gamma'(t))\|_{H(\Phi(\gamma(t)))}dt =  l_{H_\Phi}(\gamma).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^k)$ joining two points $z,z'\in \R^k$, we obtain since $\Phi\circ \gamma\in C^1([0,1], \R^d)$ is a path joining $\Phi(z)$ and $\Phi(z')$
\be
\label{dHPhi}
d_H(\Phi(z), \Phi(z')) \leq d_{H_\Phi}(z,z')
\ee
Combining \iref{dNHPhi} and \iref{dHPhi}, we conclude the proof of this proposition.
\sq


\subsection{Metrics as Lipschitz functions}
\label{subsecMetLip}
Lipschitz functions play an important role in this chapter and in particular in this section. We recall here their basic properties.
If $(X,d_X)$ and $(Y,d_Y)$ are two metric spaces, and if $f \in C^0(X , Y)$, we define 
the dilatation $\dil(f) \in [0, \infty]$ of $f$ as follows
$$
\dil(f) := \sup_{\substack{x,x'\in X \\ x \neq x'}} \frac{d_Y(f(x),f(x'))}{d_X(x,x')}
$$

We say that $f$ is Lipschitz if $\dil(f) \leq 1$, and more generally that $f$ is $\lambda$-Lipschitz if $\dil(f) \leq \lambda$.
We define the local dilatation $\dil_x(f)$ of a function $f\in C^0(X,Y)$ at a point $x\in X$ as follows
\be
\label{defDilX}
\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
\lim_{\ve\to 0} \left(\sup_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
\ee
%\be
%\label{defDilX}
%\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
%\lim_{\ve\to 0} \left(\sup_{e,e'\in B(x,\ve)} \frac{d_Y(f(e),f(e'))}{d_X(e,e')}\right).
%\ee
We specify the distance function on $X$ or $Y$ if it is not the expected ``canonical one'', in particular if $X$ or $Y$ is a subset of $\R^k$ and if the associated distance is not the standard euclidean distance but the riemannian distance $d_H$ associated to a metric, or if $X$ or $Y$ is the collection $S_d^+$ of symmetric positive definite matrices since none of the two distances $d_+$ or $d_\times$ is canonical. The local dilatation is in that case denoted as follows
$$
\dil_x(f\sep d_X, d_Y), \quad \dil_x(f\sep d_X)  \stext{ or } \dil_x(f\sep d_Y).
$$

The local dilatation $\dil_x(f)$ only depends on the local properties of the metric spaces close to $x$ and $f(x)$. Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$. For any $f\in C^0(\R^d, Y)$ and any $z\in \R^d$ we obtain using \iref{eqDistLoc}
\be
\label{eqDilNorm}
\|H(z)^{-1}\|^{-\frac 1 2} \dil_z(f) \leq \dil_z(f\sep d_H) = \dil_z(f \sep \|\cdot \|_{H(z)}) \leq \sqrt{\|H(z)\|} \dil_z(f)
\ee
We also introduce the lower local dilatation $\dil_z^*(f)\leq \dil_z(f)$ which is defined as follows
$$
\dil_z^*(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
$$
The next proposition establishes that local dilatations are sub-multiplicative.
\begin{lemma}
\label{lemmaSubMult}
Let $(X,d_X)$, $(Y,d_Y)$ and $(Z,d_Z)$ be three metric spaces, and let $f\in C^0(X,Y)$ and $g\in C^0(Y,Z)$. 
For any $x\in X$ one has 
\be
\label{eqDilUpper1}
\dil_x(g \circ f) \leq \dil_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side. Similarly we have 
\be
\label{eqDilLower1}
\dil_x(g \circ f) \geq \dil^*_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side.
\end{lemma}

\proof
We first establish \iref{eqDilUpper1}.
If $\dil_x(f) = \infty$ or $\dil_{f(x)}(g) = \infty$, then there is nothing to prove. We may therefore assume that $\dil_x(f) < \infty$ and $\dil_{f(x)}(g) < \infty$.
For any $\ve>0$ we define 
$$
F(\ve) = \sup_{p,q\in B(x, \ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)} \stext{ and } G(\ve) := \sup_{p,q\in B(f(x), \ve)} \frac{d_Z(g(p),g(q))}{d_Y(p,q)}
$$
It follows that 
$$
\sup_{p,q\in B(x, \ve)} \frac{d_Z(g(f(p)),g(f(q)))}{d_X(p,q)} \leq F(\ve) \, G(F(\ve) \ve).
$$
Taking the limit as $\ve \to 0$ we obtain \iref{eqDilUpper1} which concludes the proof.
For the proof of \iref{eqDilLower1} we consider two sequences $(p_n)_{n \geq 0}$, $(q_n)_{n \geq 0}$ which both tend to $x$ and such that $d_Y(f(p_n),f(q_n))/d_X(p_n, q_n) \to \dil_x(f)$ as $n \to \infty$. We thus have 
$$
\frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_X(p_n,q_n)} = \frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_Y(f(p_n),f(q_n))} \times \frac{d_Y(f(p_n),g(f(q_n)))}{d_X(p_n,q_n)},
$$
and taking the limit as $n \to \infty$ we obtain \iref{eqDilLower1} which concludes the proof of this lemma.
\sq

Let $f: \Omega \to V$ be a $C^1$ function, where $\Omega\subset \R^d$ is an open set and $V$ is a Banach space. Then for any $z\in \Omega$ the local dilatation $\dil_z(f)$, and the lower dilatation $\dil_z^*(f)$ only depend on the differential $d_z f : \R^d \to V$ of $f$ at $z$
\be
\label{eqDilDiff}
\dil_z(f) = \sup_{|u|=1} \|d_z f(u)\| \stext{ and } \dil_z^*(f) = \inf_{|u|=1} \|d_z f(u)\|
\ee
Applying Lemma \ref{lemmaSubMult} and \iref{eqDilDiff} to the function $g=\ln$ we obtain for any metric space $(X,d_X)$, any $f\in C^0(X,\R_+^*)$ and any $x\in X$
\be
\label{eqDilLog}
\dil_x(\ln f) = \frac {\dil_x(f)} {f(x)} .
\ee

The following proposition shows that, under certain circumstances, the Lipschitz property is a local property.
\begin{prop}
\label{propDilLoc}
Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$.
For any $f\in C^0(\R^d, Y)$ and any path $\gamma\in C^1([0,1], \R^d)$, $\gamma(0) = z$, $\gamma(1) = z'$, one has
\be
\label{eqLipLocPath}
d_Y(f(z), f(z')) \leq l_H(\gamma) \sup_{0\leq t \leq 1} \dil_{\gamma(t)}(f).
\ee
It follows that %In particular 
\be
\label{eqDilLoc}
\dil(f) = \sup_{z\in \sR^d} \dil_z(f).
\ee
\end{prop}

\proof
%Consider $z,z'\in \R^d$, and a path $\gamma\in C^1([0,1],\R^d)$ such that $\gamma(0) = z$, $\gamma(1)=z'$ and $l_H(\gamma) \leq d_H(z,z')+\delta$ where $\delta>0$ is a constant that is devoted to tend to zero in the last step of the proof.
We equip the segment $[0,1]$ with the distance $d_\gamma$ defined for $0 \leq t\leq t'\leq 1$ by 
\be
\label{defDGamma}
d_\gamma(t,t') = d_\gamma(t',t) = l_H(\gamma_{|[t,t']}).
\ee
Note that for any $t\leq t_* \leq t'$ one has 
\be
\label{exactTri}
d_\gamma(t,t') = d_\gamma(t,t_*)+d_\gamma(t_*,t')
\ee
The map $\gamma : ([0,1], d_\gamma) \to (\R^d, d_H)$ is clearly Lipschitz.
It thus follows from Lemma \ref{lemmaSubMult} that $F := f\circ \gamma :[0,1] \to Y$ satisfies for all $t\in [0,1]$
$$
\dil_t(F) \leq \dil_{\gamma(t)}(f) \leq \lambda := \sup_{0\leq t'\leq 1} \dil_{\gamma(t')}(f).
$$
We assume that $\lambda<\infty$, otherwise there is nothing to prove, and we consider a fixed $\delta>0$. For each $t\in [0,1]$ there exists therefore an interval $V_t\subset [0,1]$ containing $t$, relatively open in $[0,1]$, and such that $F_{|V_t}$ is $(\lambda+\delta)$-Lipschitz. Since the segment $[0,1]$ is compact, there exists a finite set $I_0\subset [0,1]$ such that 
$$
[0,1] = \bigcup_{t\in I_0} V_t.
$$
Let $V,V'\subset [0,1]$ be two intersecting intervals, and assume that $F$ is $\lambda+\delta$ Lipschitz on $V$ and on $V'$. For any $t\in V$ and $t'\in V'$, there exists $t_*\in V\cap V'$ which satisfies $t\leq t_*\leq t'$ or $t\geq t_* \geq t'$. Recalling \iref{exactTri} we thus obtain  
\begin{eqnarray*}
d_Y(F(t),F(t')) &\leq& d_Y(F(t), F(t_*))+d_Y(F(t_*), F(t')) \\
&\leq& (\lambda+\delta) d_\gamma(t,t_*)+( \lambda+\delta)d_\gamma(t_*,t') \\
&=& (\lambda+\delta)d_\gamma(t,t').
\end{eqnarray*}
Thus $F$ is $\lambda+\delta$ Lipschitz on the interval $V\cup V'$. Since $[0,1]$ is covered by a finite collection of open intervals on which $F$ is $\lambda+\ve$ Lipschitz, we obtain proceeding by induction that $F$ is $(\lambda+\delta)$-Lipshitz on $[0,1]$ and therefore 
$$
d_Y(f(z),f(z')) = d_Y(F(0),F(1))\leq (\lambda+\delta) d_\gamma(0,1) = (\lambda+\delta)l_H(\gamma). %\leq (\lambda+\delta)(d_H(z,z')+\delta).
$$
Letting $\delta\to 0$ we obtain \iref{eqLipLocPath}. Taking the infimum of \iref{eqLipLocPath} among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_Y(f(z),f(z')) \leq  \lambda d_H(z,z')$. Therefore $f : (\R^d, d_H) \to (Y,d_Y)$ is $\lambda$-Lipschitz, which concludes the proof of this proposition.
%The upper inequality $\geq$ is a direct consequence of the definition \iref{defDilX} of the local dilatation, and we therefore turn to the lower inequality $\leq$.
\sq

The next corollary shows that the global dilatation is controlled by the local dilatation even if the latter is not known on a \emph{sufficiently thin} set $\Gamma$, such as the skeleton of a mesh.

\begin{corollary}
\label{corolLipNoGamma}
Let $\Gamma\subset \R^d$ be a set which has the following property : for any path $\gamma\in C^1([0,1], \R^d)$ there exists a sequence of path $(\gamma_n)_{n \geq 0}$ which converge to $\gamma$ in $C^1$ norm and such that  $\{t\in [0,1]\sep \gamma_n(t) \in \Gamma\}$ is finite for each $n$.\\
Let $H\in \bH$, let $(Y,d_Y)$ be an arbitrary metric space, and met let $f\in C^0(\R^d, Y)$.
Then 
$$
\dil(f) = \sup_{z\in \R^d \sm \Gamma} \dil_z(f).
$$
\end{corollary}

\proof
We denote $\lambda := \sup_{z\in \R^d \sm \Gamma} \dil_z(f)$.
We consider two points $z,z'\in \R^d$ and a path $\gamma\in C^1([0,1], \R^d)$ such that $\gamma(0) = z$ and $\gamma(1) = z'$. %, and a sequence $\gamma_n$ converging to $\gamma$ in $C^1$ norm.

We first assume that the set $\{t\in [0,1]\sep \gamma(t) \in \Gamma\}$ is finite, and we denote its elements by $t_1< \cdots < t_k$. We set by convention $t_0 = 0$ and $t_{k+1} = 1$.
For each $0\leq i \leq k$ and each $t,t'$ such that $t_i <t<t'<t_{i+1}$ we have $d_Y(f(\gamma(t)),f(\gamma(t'))) \leq \lambda l_H(\gamma_{|[t,t']})$. Letting $t\to t_i$ and $t'\to t_{i+1}$ we obtain $d_Y(f(\gamma(t_i)),f(\gamma(t_{i+1}))) \leq \lambda l_H(\gamma_{|[t_i,t_{i+1}]})$. Adding up we obtain 
$$
d_Y(f(z), f(z')) \leq \sum_{0\leq i \leq  k} d_Y(f(\gamma(t_i)), f(\gamma(t_{i+1}))) \leq \lambda
\sum_{0\leq i \leq k} l_H(\gamma_{[t_i, t_{i+1}]}) = \lambda l_H(\gamma).
$$

We now consider the case where $\gamma$ meets the set $\Gamma$ an infinite number of times, and we choose a sequence $\gamma_n$ as described above. We obtain $d_Y(f(\gamma_n(0)), f(\gamma_n(1))) \leq \lambda l_H(\gamma_n)$ for each $n\geq 0$. Since $\gamma_n \to \gamma$ in $C^1$ norm as $n \to \infty$ we obtain taking the limit $d_Y(f(z), f(z')) \leq \lambda l_H(\gamma)$.

Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ we obtain $d_Y(f(z), f(z')) \leq \lambda d_H(z,z')$, which concludes the proof of this proposition.
\sq


%Let $(Y, \|\cdot \|_Y)$ and $(Z, \|\cdot\|_Z)$ be two banach spaces. Let $y\in Y$, $g\in C^1(Y,Z)$, and $L = g'(f(x))$, then clearly 
%$$
%\dil_y(g) = \|L\|.
%$$
%Injecting this in \iref{eqDilUpper1} we obtain 
%\be
%\label{eqDilUpper2}
%\dil_x(g \circ f) \leq\|L\|  \dil_x (f).
%\ee
%We also need a lower bound in several cases. For that purpose we define 
%$$
%\dil^*_z(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(z,\ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)}\right),
%$$
%and we obtain proceeding similarly, but with the different convention $0\times \infty = \infty\times 0 = 0$
%$$
%\dil_z(g\circ f) \geq \dil^*_{f(z)}(g) \dil_z(f).
%$$

The next proposition establishes that the regularity conditions \iref{eqLipMult} and \iref{eqLipAdd} defining the collections of quasi-acute or graded metrics are equivalent in the case of a metric proportionnal to the identity. %$\bH_a$ $\bH_g$

\begin{prop}
\label{propEquivS}
Let $s\in C^0(\R^d, R_+^*)$ and let $H(z) := \Id/s(z)^2$ for all $z\in \R^d$. We have 
\be
\label{eqDilLnH}
\dil_z(\ln s\sep d_H) = \dil_z(s).
\ee
Hence the following properties are equivalent.
\begin{enumerate}
\item The map $s : \R^d \to \R$ is Lipschitz. (i.e. $H\in \bH_i$) %For all $z,z'\in \R^d$ one has $|s(z)-s(z')|\leq |z-z'|$.
\item (``Additive'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_+(H(z),H(z')) \leq |z-z'|$.
\item (``Multiplicative'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_\times(H(z),H(z'))\leq d_H(z,z')$.
\end{enumerate}
\end{prop}

\proof %reprendre preuve??
Combining \iref{eqDilNorm} and \iref{eqDilLog} we obtain for any $z\in \R^d$
$$
%\dil_z (H\sep  d_\times, d_H) = 
\dil_z(\ln s\sep d_H) = s(z) \dil_z(\ln s) = \dil_z(s),
$$
which establishes \iref{eqDilLnH}.
According to \iref{eqDIso} we have for any $z,z'\in \R^d$
$$
d_+(H(z),H(z')) = |s(z) - s(z')| \stext{ and } d_\times (H(z),H(z')) = |\ln s(z) - \ln s(z')|.
$$
The properties 1. and 2. are thus equivalent to $\dil(s)\leq 1$, and therefore also to 
\be
\label{eqDilsLoc}
\dil_z(s) \leq 1 \text{ for all } z\in \R^d.
\ee
according Proposition \ref{propDilLoc} applied to the constant metric $H_0 = \Id$ and to the function $f=s$.
On the other hand property 3. is equivalent to $\dil(\ln s \sep d_H) \leq 1$, and thus to 
$$
\dil_z(\ln s\sep d_H) \leq 1 \text{ for all } z\in \R^d
$$
according to Proposition \ref{propDilLoc} applied to the metric $H$ and to the function $f=\ln s$.
This property equivalent to \iref{eqDilsLoc} according to \iref{eqDilLnH}, which concludes the proof of this Proposition.
\sq

The next corollary uses Proposition \ref{propEquivS} to analyse the regularity of the first and last eigenvalue of a metric.
\begin{corollary}
\label{corolLipNorm}
\begin{itemize}
\item
For any $H\in \bH_g$, the map $z\mapsto \|H(z)\|^{-\frac 1 2}$ is Lipschitz.
\item
For any $H\in \bH_a$, the map $z\mapsto \|H(z)^{-\frac 1 2}\|$ is Lipschitz.
\end{itemize}
\end{corollary}
\proof
\begin{itemize}
\item 
%For any $M,M'\in S_d^+$ we have 
%\begin{eqnarray*}
%d_\times(M,M') &=& \ln \left(\max\left\{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\right\}\right) \\
%&\geq &\ln \left(\max \left\{\frac{\|M^\frac 1 2\|}{\|M'^{\frac 1 2}\|}, \, \frac{\|M'^{\frac 1 2}\|}{\|M^{\frac 1 2}\|}\right\}\right)\\
%& = & \frac 1 2 \left|\ln \|M\| - \ln \|M'\|\right|.
%\end{eqnarray*}
Consider $H\in \bH_g$, define $s(z) := \|H(z)\|^{-\frac 1 2}$ and 
$$
H'(z) := \frac \Id {s(z)^2} = \|H(z)\|\Id.
$$
Since $H(z) \leq H'(z)$ for all $z\in \R^d$, we have $d_H(z,z') \leq d_{H'} (z,z')$ for all $z, z'\in \R^d$.

Consider a pair $M,M'\in S_d^+$ of matrices and a real $\delta>0$. If $e^{-2\delta} M \leq M' \leq e^{2\delta} M$, then taking the norm we obtain $e^{-2\delta} \|M\| \leq \|M'\| \leq e^{2\delta} \|M\|$. It follows that 
$$
\frac 1 2 |\ln \|M\| - \ln \|M'\|| \leq d_\times (M,M').
$$
We thus have for any $z,z'\in \R^d$
\begin{eqnarray*}
|\ln s(z)-\ln s(z')| &=& \frac 1 2 \left|\ln \|H(z)\| - \ln \|H(z')\|\right| \\ %\left|\ln \left(\sqrt{\|H(z)\|}\right) -\ln \left(\sqrt{\|H(z')\|}\right)\right| \\%
%& \leq & \sup_{u\neq 0} |\ln \|u\|_{H(z)} - \ln \|u\|_{H(z')}|\\
&\leq & d_\times(H(z),H(z')) \\
&\leq& d_H(z,z')\\
&\leq& d_{H'}(z,z').
\end{eqnarray*}
Applying Proposition \ref{propEquivS} to the metric $H'$ we obtain that $H'\in \bH_i$, and therefore that $s$ is Lipschitz as announced.
\item
Consider $H\in \bH_a$. We have for any $z,z'\in \R^d$
$$
\left|\|H(z)^{-\frac 1 2}\| - \|H(z')^{-\frac 1 2}\| \right| \leq \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| \leq |z-z'|,
$$
which concludes the proof of this corollary.\sq
\end{itemize}

Our last proposition studies the local dilatation of the maximum and the minimum of two functions.
\begin{prop}
\label{propDilMax}
Let $(X,d_X)$ be a metric space and let $\lambda, \mu\in C^0(X, \R)$. Let $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda, \mu\}$. Then for all $x\in X$
\be
\label{eqDilMax1}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} \leq \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
If $(X,d_H) = (\R^d, d_H)$, where $H \in \bH$ is a riemannian metric, then equality holds
\be
\label{eqDilMax2}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} = \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
\end{prop}

\proof
We have for any $p,q\in X$,
\begin{eqnarray*}
|\gamma(p)-\gamma(q)| &=& |\min\{\lambda(p), \mu(p)\} - \min \{\lambda(q), \mu(q)\}|\\
& \leq & \max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}.
\end{eqnarray*}
For any $x\in X$ and any $\ve>0$ we thus obtain
\begin{eqnarray*}
\dil(\gamma_{|B(x,\ve)}) &=& \sup_{p,q\in B(x,\ve)} \frac{|\gamma(p)-\gamma(q)|}{d_X(p,q)} \\
&\leq& \sup_{p,q\in B(x,\ve)} \frac{\max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}}{d_X(p,q)}\\
& =& \max\left\{\sup_{p,q\in B(x,\ve)}  \frac{|\lambda(p)-\lambda(q)|}{d_X(p,q)}, \sup_{p,q\in B(x,\ve)}  \frac{|\mu(p)-\mu(q)|}{d_X(p,q)}\right\}\\
&=& \max\left\{\dil(\lambda_{|B(x, \ve)}), \dil(\mu_{|B(x,\ve)})\right\}.
\end{eqnarray*}
Letting $\ve \to 0$ we obtain $\dil_x(\gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$. Likewise $\dil_x(\Gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$ which concludes the proof of \iref{eqDilMax1}.

We now turn to the proof of \iref{eqDilMax2}. For that purpose we consider a fixed $\ve>0$ and we define
$$
r := \max \{\dil(\gamma_{|B(x,\ve)}\sep \|\cdot\|_{H(x)}), \ \dil(\Gamma_{|B(x,\ve)} \sep \|\cdot\|_{H(x)})\},
$$
where $B(x,\ve)$ stands for the euclidean unit ball of radius $\ve$ centered at $x$.
Consider two points $p,q\in B(x,\ve)$. If $\lambda(p) \geq \mu(p)$ and $\lambda(q)\geq \mu(q)$, or if $\lambda(p) \leq \mu(p)$ and $\lambda(q)\leq \mu(q)$, then 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)|&=& \max \{|\gamma(p)-\gamma(q)|, |\Gamma(p)-\Gamma(q)|\}\\
&\leq & \|p-q\|_{H(x)}
\end{eqnarray*}
Otherwise if  $\lambda(p) \geq \mu(p)$ and $\lambda(q)\leq \mu(q)$, or $\lambda(p) \leq \mu(p)$ and $\lambda(q)\geq \mu(q)$, then there exists a point $r$ on the segment $[p,q]$ such that $\lambda(r)=\mu(r)$. We thus have %$|p-r|+|r-q| = |p-q|$ and 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)| &\leq& \max \{|\gamma(p)-\gamma(r)|, |\Gamma(r)-\Gamma(q)|\}\\
& &+ \max \{|\gamma(r)-\gamma(q)|, |\Gamma(r)-\Gamma(q)|\}\\
& \leq & \|p-r\|_{H(x)} + \|r-q\|_{H(x)} = \|p-q\|_{H(x)}
\end{eqnarray*}
If follows that $\dil(\lambda_{|B(x,\ve)}\sep \|\cdot\|_{H(x)})\leq r$, and letting $\ve\to 0$ we obtain 
$$
\dil_x(\lambda\sep \|\cdot\|_{H(x)}) \leq \max\{\dil_x(\gamma\sep \|\cdot\|_{H(x)}), \ \dil_x(\Gamma \sep \|\cdot \|_{H(x)})\}.
$$ 
Recalling that $\dil_x(f\sep d_H) = \dil_x(f\sep \|\cdot\|_x)$ for any $f\in C^0(\R^d, \R)$ and any for all $x\in \R^d$, see \iref{eqDilNorm}, we obtain $\dil_x(\lambda) \leq \max\{\dil_x(\gamma), \ \dil_x(\Gamma)\}$. Proceeding likewise for $\mu$ we obtain \iref{eqDilMax2} which concludes the proof of this proposition.
\sq

\subsection{Geometric properties of the space $(\R^d, d_H)$} %Estimates of size}
\label{subsecMetGeom}

We focus in this subsection on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. The next proposition compares the riemannian distance $d_H$ between two points $z$ and $z+u$ with the norm $\|u\|_{H(z)}$ of their difference.

%with the euclidean distance and we estimate the volume of balls. 
%The next proposition compares the Riemannian distance associated to a graded metric, with 

\begin{prop}
\label{propEuclidRiemann}
Let $H \in \bH_g$ and let $z\in \R^d$. For all $u\in \R^d$ one has
\be
\label{eqEuclidRiemann}
\ln(1+\|u\|_{H(z)}) \leq d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention when $\|u\|_{H(z)}\geq 1$.
\end{prop}
\proof
%We first prove the left part of \iref{eqEuclidRiemann}, and for that purpose
We consider a path $\gamma\in C^1([0,1], \R^d)$, and we define for each $t\in [0,1]$
\be
\label{defLGamma}
l(t) := \int_0^t \|\gamma'(t)\|_{H(\gamma(t))}dt.
\ee
Since $H\in \bH_g$ we have for any $t\in [0,1]$
$$
\exp(-2\, d_H(z, \gamma(t))) \, H(z) \leq H(\gamma(t)) \leq  \exp(2 \, d_H(z, \gamma(t))) \, H(z)
$$
therefore, since $d_H(z, \gamma(t)) \leq l(t)$,
$$
\exp(-2l(t)) H(z)  \leq H(\gamma(t)) \leq  \exp(2l(t)) H(z).
$$
It follows that 
$$
\|\gamma'(t)\|_{H(z)} \exp(-l(t)) \leq l'(t) = \|\gamma'(t)\|_{H(\gamma(t))} \leq  \|\gamma'(t)\|_{H(z)} \exp(l(t)), %\exp(-l(t))
$$
hence 
\be
\label{eqGammapLp}
-\frac d {dt} \exp(-l(t)) \leq \|\gamma'(t)\|_{H(z)} \leq \frac d {dt} \exp(l(t)).
\ee
We have 
\be
\label{eqGammaGammap}
\|u\|_{H(z)} =  \|\gamma(1)-\gamma(0)\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt
\ee
with equality if $\gamma(t) = z+tu$ is the straight line.
%We now assume that $\gamma(t) \neq \gamma(0)$ for all $t\in (0,1]$, which is the case generically. The map $t\mapsto \|\gamma(t)-\gamma(0)\|_{H(z)}$ is therefore $C^1$ on $(0,1]$ and we have 
%$$
%\frac d {dt} \|\gamma(t)-\gamma(0)\|_{H(z)} \leq \|\gamma'(t)\|_{H(z)},
%$$
%with equality if $\gamma(t)-\gamma(0) = c \gamma'(t)$ for some $c>0$.
%In the special case of the straight line $\gamma(t)=z+tu$, \iref{eqGammaGammap} is an equality and we thus obtain 
In that case, integrating the left part of \iref{eqGammapLp} we obtain
$$
 1-\exp(-l_H(\gamma)) = -\int_0^1 \left(\frac d {dt} \exp(-l(t))\right)dt   \leq  \int_0^1 \|\gamma'(t)\|_{H(z)} dt %= \|\gamma(1)-\gamma(0)\|_{H(z)} \exp(-l(0)) - \exp(-l(1))
 = \|u\|_{H(z)}.
$$
Rearranging the terms we obtain the right part of \iref{eqEuclidRiemann}:
$$
d_H(z,z+u) \leq l_H(\gamma) \leq -\ln(1-\|u\|_{H(z)}).
$$
We now consider an arbitrary path $\gamma$ joining $z$ and $z+u$ and we obtain integrating the right part of \iref{eqGammapLp} and recalling \iref{eqGammaGammap}
$$
\exp(l_H(\gamma)) -1 = \int_0^1 \left(\frac d {dt} \exp(l(t))\right) dt  \geq \int_0^1 \|\gamma'(t)\|_{H(z)} dt \geq \|u\|_{H(z)},
$$
which is equivalent to
$$
l_H(\gamma) \geq \ln(1+\|u\|_{H(z)}).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ satisfying $\gamma(0) = z$ and $\gamma(1) = z+u$, we obtain the left part of \iref{eqEuclidRiemann}, which concludes the proof of this proposition.
\sq

We discuss in the rest of this section the consequences of the comparison \iref{eqEuclidRiemann} of the riemannian distance $d_H$ with the distance associated to the norm $\|\cdot\|_{H(z)}$ when $H\in \bH_g$. %is devoted to 
Combining the right part of \iref{eqEuclidRiemann} with the expression \iref{eqDTimesLog} of the distance $d_\times$ we obtain an estimate of the local variations of the norm $\|\cdot \|_{H(z)}$ associated to the metric $H$ at a point $z$: let $H\in \bH_g$, and let $z,u,v\in \R^d$ be such that $\|u\|_{H(z)} < 1$, then
\be
\label{eqLocalNorm}
(1-\|u\|_{H(z)}) \|v\|_{H(z)} \leq \|v\|_{H(z+u)} \leq (1-\|u\|_{H(z)})^{-1} \|v\|_{H(z)}. %\frac{\|v\|_{H(z)}}{1-\|u\|_{H(z)}}.
\ee
Note also that 
\be
\label{eqLocalDet}
(1-\|u\|_{H(z)})^d \sqrt{\det H(z)} \leq \sqrt{\det H(z)} \leq (1-\|u\|_{H(z)})^{-d} \sqrt{\det H(z)}.
\ee
Another important consequence of \iref{eqEuclidRiemann} is that the closed balls $\{z'\in \R^d \sep d_H(z,z')\leq r\}$ for the distance $d_H$, are closed and bounded subsets $\R^d$, hence are compact. %From this point a classical argument (??) shows that $(R^d,d_H)$ is a complete metric space.

The following example establishes that \iref{eqEuclidRiemann} is a sharp inequality. The metric $H$ defined by 
$$
H(z) := \frac \Id {(1+|z|)^2}
$$
belongs to $\bH_i$ since $z\mapsto 1+|z|$ is Lipschitz, hence $H$ also belongs to $\bH_a$ and $\bH_g$.
For any $v\in \R^d$, one easily checks that the path of minimal length joining $0$ to $v$ is the straight line, and that
$$
d_H(0, v) = \ln(1+|v|).
$$
Choosing $z=0$ and $u=v$ we obtain that the left part of \iref{eqEuclidRiemann} is sharp
$$
\ln (1+ \|u\|_{H(0)}) = \ln (1+ |u|) = d_H(0,0+u).
$$
Choosing $z=-v$ and $u = v$ we obtain that the right part of \iref{eqEuclidRiemann} is sharp
$$
-\ln\left(1-\|u\|_{H(-u)} \right) = -\ln \left(1-\frac {|u|}{1+|u|}\right) = \ln(1+|u|) = d_H(-u, -u+ u).
$$

The next corollary uses Proposition \ref{propEuclidRiemann} to obtain a lower bound for the mass of balls in the measure $z\mapsto \sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. %states a volume estimate Proposition \ref{propLength} implies a volume estimate. %also allows us to compare the vo
\begin{corollary}
\label{corolVol}
There exists $c=c(d)>0$ such that the following holds. Let $H \in \bH_g$,
let $L\geq 1$ and let $z_0\in \R^d$. Denoting $\cE$ the ellipse 
$$
\cE = \{z\in \R^d\sep \|z-z_0\|_{H(z_0)}\leq L\}.
$$ 
we have 
\be
\label{eqVolLog}
\int_\cE \sqrt{\det H} \geq c \ln L. %\max\{L,1\}.
\ee
%Then 
%$$
%\int_\cE \sqrt {\det H} \geq c \ln L -1
%$$
%where $c=...$
%In particular if $H(z)\geq \lambda^2\Id$ (*$\|u\|_{H(z)} \geq \lambda |u|$ for all $u\in \R^d$*) then 
%\be
%\label{volBR}
%\int_{B(z,r)} \sqrt{\det H} \geq c \ln \max\{\lambda r, 1\}
%\ee
\end{corollary}

\proof
It follows from Proposition \ref{propEuclidRiemann} that $d(z_0, z) \geq \ln (L+1)$ for all $z\in \partial \cE$. We define the integer 
$$
k = \left\lfloor \ln(L+1) -\frac 1 2\right\rfloor,
$$
and we consider $k$ points $z_1, \cdots , z_k \in E$ such that for all $0 \leq i \leq k$
$$
d_H(z_0, z_i)= i.
$$
We define 
$
r_0 := 1-e^{-\frac 1 2} = 0.39\cdots
$
in such way that 
$$
-\ln (1-r_0) = \frac 1 2.
$$
For all $0 \leq i \leq k$ we denote by $\cE_i$ the ellipse 
$$
\cE_i  := \left\{z\in \R^d \sep \|z-z_i\|_{H(z_i)} \leq r_0\right\}.
$$
We have $\cE_i \subset \cE$ for all $0 \leq i \leq k$, indeed for any $z\in \cE_i$ we have 
$$
d_H(z_0, z) \leq d_H(z_0, z_i) + d_H(z_i, z) \leq i- \ln (1-r_0) \leq k+\frac 1 2 \leq \ln (L+1),
$$
Denoting by $\interior(E)$ the interior of a set $E\subset \R^d$, we observe that for all $0 \leq i<j\leq k$, for all $z\in \interior(\cE_i)$ and $z'\in \interior(\cE_j)$, we have
$$
d_H(z,z') \geq d_H(z_i, z_j) -d_H(z_i, z) - d_H(z_j,z') > |d_H(z_0, z_i) - d(z_0, d_j)| + 2\ln(1 -r_0) =0, %\geq 1+ 2 \ln(1-\frac 1 3)>0.
$$
hence $\interior(\cE_i) \cap \interior(\cE_j) = \emptyset$.
It follows that 
$$
\int_\cE \sqrt{\det H} \geq \sum_{0 \leq i \leq k} \int_{\cE_i} \sqrt{\det H}.
$$
Furthermore we have for all $z\in \cE_i$
$$
H(z) \geq (1-\|z-z_i\|_{H(z_i)})^2 H(z_i)  \geq (1-r_0)^2 H(z_i),
$$
and therefore 
\be
\label{eqzzi}
\sqrt{\det H(z)} \geq (1-r_0)^d \sqrt{\det H(z_i)}.
\ee
We denote by $B(z,r)$ the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$, and we observe that 
$u\mapsto z_i + H(z_i)^{-\frac 1 2} u$ maps $B(0,r_0)$ onto $\cE_i$. Combining this remark with \iref{eqzzi} we obtain
\begin{eqnarray*}
\int_{\cE_i} \sqrt{\det H} &\geq& (1-r_0)^d \int_{\cE_i} \sqrt{\det H(z_i)} \\
&=& (1-r_0)^d \int_{B(0,r_0)} 1 \\
&=& c_0 := r_0^d (1-r_0)^d |B(0,1)|.
\end{eqnarray*}
%where $B(z,r)$ denotes the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$.
Eventually we obtain 
$$
\int_\cE \sqrt{\det H} \geq (k+1) c_0 \geq (\ln(L+1) - 1/2) c_0.
$$
In order to obtain \iref{eqVolLog} we simply recall that $L\geq 1$ and therefore that %Since Recalling that $L\geq 1$ we find that 
$$
\ln (L+1) = \frac{\ln(L+1)}{2 \ln 2} +  \left(1-\frac 1 {2 \ln 2}\right)\ln(L+1) \geq \frac 1 2 + \left(1-\frac 1 {2 \ln 2}\right)\ln L $$
which concludes the proof of \iref{eqVolLog} with $c=(1- 1/(2 \ln 2))c_0$.
%Applying \iref{eqVolLog} to $L = \lambda r$ we obtain \iref{volBR} which concludes the proof of this proposition.
\sq


\section{Metrics having an eigenspace of dimension $d-1$ at each point}
\label{secEigen}
We focus in this subsection on metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has an eigenspace of dimension at least $d-1$ at each point $z\in \R^d$. 
%If the dimension is $d=2$, then a metric $H\in \bH$ generically satisfies this condition on a dense subset of $\R^d$. %any metric $H\in \bH$ satisfies this condition. 
This condition clearly holds if the dimension is $d=2$, but is also relevant in higher dimension. 
Indeed, as discussed in \S\ref{secOptGeom} of Chapter \ref{chapApproxMet}, this type of metrics appears when one needs to create mesh containing a thin layer of simplices close to an hypersurface $\Gamma$. In that case the matrix $H(z)$ at a point $z\in \Gamma$ typically has an eigenspace of dimension $d-1$ which is tangent to $\Gamma$ and is associated to a small eigenvalue, and an eigenspace of dimension $1$ in the direction orthogonal to $\Gamma$ associated to a large eigenvalue. 

The main result of this section is Theorem \ref{th2Spaces} which characterises those of these metrics which belongs to $\bH_a$ or $\bH_g$ in terms of the regularity of their eigenvalues and of their eigenvectors.
Corollary \ref{corolHgToHa} to this theorem gives a simple procedure to obtain a quasi-acute metric from a graded metric $H$ such that $H(z)$ has an eigenspace of dimension $d-1$ at each point. \\

We denote by $\bbS := \{\theta\in \R^d \sep |\theta| = 1\}$ the unit sphere of $\R^d$, equipped with the distance 
$$
d_\bbS(\theta, \theta') := \arccos(\<\theta, \theta'\>).
$$
We denote by $\cA$ the space of parameters
$$
\cA := \R_+^*\times \R_+^*\times \bbS,
$$
and we define a map $\cS :\cA\to S_d^+$ as follows
\be
\label{defcS}
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
\ee
In any orthonormal basis $\cB$ of $\R^d$ which begins with the vector $\theta$ we have the following expression
$$
[\cS(\lambda, \mu, \theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda &0 & 0 & \cdots\\
0 & \mu & 0 & \cdots\\
0 & 0 & \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right).
$$
We also define for any $a = (\lambda, \mu, \theta)\in \cA$
$$
\cH(a) := \cS(a)^{-2} = \lambda^{-2} \theta \theta^\trans+ \mu^{-2}(1-\theta \theta^\trans).
$$
%If $M\in S_d^+$ has an eigenspace of dimension $d-1$ exactly, then 
%
%We denote by $S_{d*}^+$ the collection of symmetric positive definite matrices $M\in S_d^+$ which have an eigenspace of dimension exactly $d-1$.
%We also denote by $\cA^*$ the collection of $(\lambda, \mu, \pm\theta)\in \cA$ which satisfies $\lambda\neq \mu$ if $d>2$ (resp. $\lambda>\mu$ is the dimension is $d=2$).
%Then
%$$
%\cH : \cA^* \to S_{d*}^+
%$$
%is a one to one map.



%Such a metric $H$ can be parametrized using two eigenvalues $\lambda, \mu\in \R_+^*$  and a subspace of dimension $d-1$ of $\R^d$ defined through an un-oriented unit normal $\pm \theta$. Our purpose in this section is to translate the fact that $H\in \bH_\star$, for some $\star\in \{i,a,g\}$, into simpler properties satisfied by $\lambda,\mu$ and $\theta$.
%
%
%
%In order to state our results, we need to introduce the collection $\cP$ of all hyperplanes of $\R^d$, also called the projective space. An hy
%
%
%We define the space of parameters
%$$
%\cA :=  \R_+^* \times \R_+^* \times \cP,
%$$
%where $\cP$ is the $d-1$-dimensional real projective space.
%For all $(\theta, \lambda, \mu)\in \cA$ we define 
%$$
%S( \lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans),
%$$
%and $H(\theta, \lambda, \mu) := S^{-2}$.
%The space $\cA$ is a differential variety, and the tangent space to a triplet $(\theta, \lambda, \mu)\in \cA$ is 
%$$
%T_{(\theta, \lambda, \mu)} \cA =  \R \times \R \times \theta^\perp,
%$$
%where $\theta^\perp$ refers to the orthogonal hyperplane to $\theta$ in $\R^d$.

For any metric $H \in \bH$ and any $z\in \R^d$ we denote by $\dil_z(H)_\times$ and $\dil_z(H)_+$ the local dilatations at $z$ associated to the Lipschitz conditions \iref{eqLipMult} and \iref{eqLipAdd} defining $\bH_g$ and $\bH_a$:
\be
\label{defDilH}
\dil_z(H)_\times := \dil_z(H \sep d_\times, d_H) \stext{ and } \dil_z(H)_+ := \dil_z(H \sep d_+).
\ee
We recall that the local dilatation $\dil_z(f)$ of a function $f$ at a point $z$ is defined by \iref{defDilX}.
%We set $D_z(H) := \dil(\lambda)$ if $z\notin \Omega$
For any open set $\Omega\subset \R^d$ and any $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$,  we define for all $z\in \Omega$
\be
\label{eqDZA}
D_z(a)_\times := \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \frac 1 2 \left| \frac {\lambda(z)} {\mu(z)} - \frac {\mu(z)} {\lambda(z)} \right|\dil_z(\theta\sep  d_H)\right\}, %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
and 
\be
\label{eqDZAP}
D_z(a)_+ := \max\left\{\dil_z(\lambda), \ \dil_z(\mu),\ |\lambda(z)-\mu(z)| \dil_z(\theta)\right\}. %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
Note that these quantities are not defined if $\lambda(z) = \mu(z)$ and $\dil_z(\theta\sep  d_H)=\infty$ simultaneously, since an indeterminate form $0\times \infty$ appears in \iref{eqDZA} and \iref{eqDZAP}.
\begin{theorem}
\label{th2Spaces}
Let $H \in \bH$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, such that $H = \cH\circ a$ on $\Omega$.
Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$. Then 
\be
\label{eqDilTimes}
D_z(a)_\times \leq \dil_z(H)_\times \leq 2D_z(a)_\times
\ee
and%, with $\gamma := \|H^{-\frac 1 2}\| = \max\{\lambda, \mu\}$, 
\be
\label{eqDilPlus}
D_z(a)_+ \leq \dil_z(H)_+ \leq 2D_z(a)_+.
\ee
%In particular, defining $\gamma := \|H(z)^{-\frac 1 2}\| = \max \{\lambda, \mu\}$ we have 
%\be
%\label{eqDilMax}
%\max\{\dil_z(\gamma), \, D_z(a)_\times\} \leq \max \{D_z(a)_+, \, D_z(a)_\times\} \leq 2\max\{\dil_z(\gamma), \, D_z(a)_\times\}.
%\ee
\end{theorem}

%The estimate \iref{eqDilPlus} on $\dil_z(H)_+$ is not very sharp, but this is not an issue since one usually does not needs to control $ \dil_z(H)_+$ but rather $\max\{\dil_z(H)_\times,\dil_z(H)_+\}$, for which we obtain combining \iref{eqDilTimes} and \iref{eqDilPlus} the sharper estimate 
%$$
% \max\{\dil_z(\gamma), D_z(a)\} \leq \max\{\dil_z(H)_\times,\dil_z(H)_+\} \leq 2 \max\{\dil_z(\gamma), D_z(a)\}.
%$$
The rest of this section is devoted to the proof of this theorem and to Corollary \ref{corolHgToHa}. Our first lemma defines and estimates a quantity $\Delta(a,b,c)$ which appears repeatedly in the rest of the proof.


\begin{lemma}
\label{lemmaDelta}
We define for all $a,b,c\in \R$ the quantity $\Delta(a,b,c)\in \R_+$, as follows % which is the norm of a $d\times d$ matrix,
\be
\label{defDelta}
\Delta(a,b,c) := 
\left\| 
\left(
\begin{array}{cccc}
a & b & 0 & \cdots\\
b & c& 0 & \cdots\\
0 & 0 & c & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right)
\right\|.
\ee
We have 
\be
\label{eqEstimM}
\max\{|a|, |b|, |c|\} \leq \Delta(a,b,c) \leq 2 \max\{|a|, |b|, |c|\}.
\ee
\end{lemma}

\proof
We consider fixed values of $a,b,c\in \R$ and we denote by $M$ the matrix presented in \iref{defDelta}, in such way that $\Delta(a,b,c) = \|M\|$. We also define $\lambda := \max\{|a|,|b|,|c|\}$.
We have 
$$
\Delta(a,b,c) = \|M\|\geq \max_{1\leq i,j\leq d} |M_{ij}| = \lambda,
$$
which establishes the left part of \iref{eqEstimM}. For all $p\in [1,\infty]$ we denote by $l^p$ the usual norm on $\R^d$ of exponent $p$. We have 
$$
\|M\|_{l^\infty\to l^\infty} = \max_{1 \leq i \leq d} \sum_{1\leq j \leq d} |M_{ij}| \leq 2 \lambda \stext{ and } \|M\|_{l^1\to l^1} = \max_{1 \leq j \leq d} \sum_{1\leq 1 \leq d} |M_{ij}| \leq 2 \lambda.
$$
By interpolation we thus obtain  
$$
\|M\| = \|M\|_{l^2\to l^2} \leq \sqrt{\|M\|_{l^1\to l^1} \|M\|_{l^\infty\to l^\infty} } \leq 2 \lambda,
$$
which concludes the proof.
\sq

The parameter space $\cA = \bbS \times \R_+^* \times \R_+^*$ is a differential variety, and the regularity of functions defined on $\cA$ should be seen through local charts.
For each $a = (\lambda, \mu, \theta)\in \cA$ we define a local chart $\psi_a$ of a neigborhood of $a$ in $\cA$ as follows: 
\be
\label{defPsia}
\psi_a : (-\lambda, \infty)\times (-\mu , \infty) \times (B(0,\cPi) \cap \theta^\perp) \to \cA
\ee
is defined by 
$$
\psi_a(\Lambda, M, r\Theta) := (\lambda+ \Lambda,\, \mu+ M,\, \cos(r) \theta + \sin(r) \Theta),
$$
where $|\Theta| = 1$. Note that $\psi_a$ is one to one and that $d_\bbS(\theta, \, \cos(r) \theta + \sin(r) \Theta) = r$.
In \iref{defPsia} we denoted by $\theta^\perp := \{\Theta\in \R^d \sep \<\theta, \Theta\> = 0 \}$ the space orthogonal to $\theta$, and $B(0,\cPi)$ the open euclidean ball of radius $\cPi$.
%it preserves distances in the following sense: if $(\lambda', \mu', \theta') = \psi_a(\Lambda, M, r\Theta)$ then $\lambda'-\lambda = \Lambda$, $\mu'-\mu=M$ and $

Let $V$ be a banach space. We say that a function $\vp : \cA \to V$ is $C^1$ if for any $a\in \cA$ the function $\vp\circ \psi_a$ is $C^1$.
In that case for any $a\in \cA$ we define the differential 
%and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
$$
d_a\vp(A) : \R\times \R\times \theta^\perp \to V
$$
by the formula
$$
d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( tA) - \vp(a)} t. %\Lambda, t M, t r\Theta
$$
We then have
 $$
\dil_a(\vp) = \|d_a(\vp)\|.
$$
%where $d_0 (\vp\circ \psi_a) :  \R\times \R\times \theta^\perp \to V$ denotes the differential of function $\vp\circ \psi_a$ at the origin $(0,0,0) \in (-\lambda, \infty)\times (-\mu , \infty) \times (B(\pi) \cap \theta^\perp)$.
%In that case for any $a\in \cA$ and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
%$$
%d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( t\Lambda, t M, t r\Theta) - \vp(a)} t,
%$$
%and we have for any path $\gamma\in C^1([0,1], \cA)$ 
%$$
%\vp(\gamma(1)) - \vp(\gamma(0)) = \int_0^1 d \vp_{\gamma(t)} (\gamma'(t)) dt.
%$$

\begin{prop}
\label{propPhiPlus}
Define $V_+ := S_d$, equipped with the standard norm $\|\cdot\|$, and define $\vp_+ (a) := \cS(a)$.
Then for all $a,b\in \cA$ we have 
\be
\label{eqDPPhiP}
d_+(\cH(a), \cH(b)) = \|\vp_+(a)-\vp_+(b)\|.
\ee
Furthermore $\vp_+ \in C^1(\cA, V_+)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
$$
\|d_a \vp_+(A)\|_\infty= 
\Delta(\Lambda, \ (\lambda-\mu) r ,\ M).
$$
\end{prop}

\proof
The \iref{eqDPPhiP} directly follows from the fact that $\cH(a)^{-1} = \cS(a)^2 = \vp_+(a)^2$, and from the definition \iref{defDPlus} of $d_+$.
The function $\vp_+ = \cS$ is $C^1$, and even $C^\infty$, since it has a polynomial expression 
$$
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
$$
We have at the first order in $\lambda, \mu, r$
\begin{eqnarray*}
\cS(\lambda+ \Lambda, \, \mu+M, \, \theta+r\Theta) &=&
 (\lambda+ \Lambda) (\theta+ r\Theta) (\theta+r\Theta)^\trans \\
 & &+ (\mu+M)(\Id - (\theta+ r\Theta) (\theta+r\Theta)^\trans)\\
 &=& S(\lambda, \mu, \theta) \\
 & &+ \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans)\\
& &+  \cO((|\Lambda|+ |M|+ |r|)^2)
\end{eqnarray*}
Therefore %$\vp_+$ is $C^1$ and 
\be
\label{eqDiffS}
%d_a\vp_+(\Lambda, \,M, \,r\Theta) = 
d_a\cS(\Lambda, \,M, \,r\Theta) =  \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans).
\ee
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[d_a\cS(\Lambda, \,M, \,r\Theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda & r(\lambda-\mu) & 0 & \cdots\\
r(\lambda-\mu) & M & 0 & \cdots\\
0 & 0 & M & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
which concludes the proof of this proposition.
\sq


\begin{prop}
\label{propPhiTimes}
Define $V_\times := C^0(\bbS, \R)$, equipped with the $\|\cdot\|_\infty$ norm, and define $\vp_\times : \cA \to V_\times$ as follows: for any $a\in \cA$ and any $u\in \bbS$
%\be
%\label{eqDTPhiT}
$$
\vp_\times (a) := (u \mapsto \ln \|u\|_{\cH(a)}).
$$
%\vp_\times (a)(u) = \ln \|u\|_{\cH(a)}.
%\ee
Then for all $a,b\in \cA$ we have 
\be
\label{eqDTPhiT}
\|\vp_\times(a)-\vp_\times(b)\|_\infty = d_\times(\cH(a), \cH(b)).
\ee
Furthermore $\vp_\times \in C^1(\cA, V_\times)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
\be
\label{eqNormDPhiPlus}
\|d_a \vp_\times(A)\|_\infty= 
\Delta\left(\frac \Lambda \lambda ,\ \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) ,\ \frac M \mu\right).
\ee
\end{prop}

\proof
Using the expression \iref{eqDTimesLog} of the distance $d_\times$ and the homogeneity of norms we obtain for any $M,M'\in S_d^+$,
$$
d_\times (M,M') = \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
$$
which implies \iref{eqDTPhiT}.
%The inequality \iref{eqDTPhiT} follows from the expression \iref{eqDTimesLog} of the distance $d_\times$.

As observed in the proof of Proposition \ref{propPhiPlus} the function $\cS : \cA\to S_d^+$ is $C^1$, and $d_a\cS(A)$ has the explicit expression \iref{eqDiffS}.
It is well known that the inverse map ${\rm Inv} : \GL_d \to \GL_d$ is $C^1$ and has the the following differential : for any $\phi\in \GL_d$ and any $\Phi\in M_d$
$$
d_\phi {\rm Inv} (\Phi) = \phi^{-1} \Phi \phi^{-1}.
$$
By composition, $\cS^{-1} : \cA \to S_d^+$ is also $C^1$, and for any $a=(\lambda, \mu , \theta)\in \cA$ and any $A\in \R\times \R \times \theta^\perp$
$$
d_a(\cS^{-1})(A) = S(a)^{-1} (d_a S(A) ) S(a)^{-1}.
$$
For any $u\in \bbS$ we have 
$$
\ln \|u\|_{\cH(a)} = \ln \|\cS(a)^{-1}u\| = \frac 1 2 \ln \left(\<\cS(a)^{-1}u,\cS(a)^{-1}u\>\right).
$$
Therefore, again by composition, 
\begin{eqnarray*}
d_a (\ln \|u\|_{\cH})(A) &=&  \frac 1 {2\|\cS(a)^{-1}u\|^2} (\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>\\
& &\quad +\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>)\\% \frac {\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>+\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>}{2\|\cS(a)^{-1}u\|^2}\\
&=& \frac{\<G(a,A) v,v\>}{\|v\|^2}
\end{eqnarray*}
where $v = \cS^{-1}(a)u$. The function $G$ has the following expression : for any $a = (\lambda, \mu, \theta)\in \R_+^* \times \R_+^* \times \bbS$ and any $A = (\Lambda, M, r\Theta)\in \R\times \R \times \theta^\perp$
\begin{eqnarray*}
G(a,A) &=& \frac{\cS(a)^{-1} (d_a\cS(A)) + (d_a\cS(A)) \cS(a)^{-1}} 2\\
&=& \frac \Lambda \lambda \theta \theta^\trans +  \frac M \mu (\Id - \theta \theta^\trans) + \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right)(\theta \Theta^\trans + \Theta \theta^\trans),
\end{eqnarray*}
the last expression follows from the explicit expression \iref{eqDiffS} of $d_a\cS(A)$ establishes in the proof of the previous proposition, and from the fact that $\theta^\trans \Theta = 0$.
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[G(a,A)]_\cB = 
\left(
\begin{array}{cccc}
\frac \Lambda \lambda & \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & 0 & \cdots\\
\frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & \frac M \mu & 0 & \cdots\\
0 & 0 & \frac M \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
The map $\vp_\times$ is differentiable, as the composition of differentiable maps, and we thus have
\begin{eqnarray*}
\|d_a \vp_\times(A)\|_\infty &=& \sup \left\{ \frac{|\<G(a,A) v,v\>|}{\|v\|^2} \sep u\in \bbS, \, v=\cS(a)^{-1} u\right\}\\
&=& \|G(a,A)\|,
\end{eqnarray*}
which establishes \iref{eqNormDPhiPlus} and concludes the proof of this proposition.
\sq

We now consider a fixed $z\in \Omega$ and we remark that 
$$
\dil_z(H)_\times = \dil_z(\cH\circ a)_\times  = \dil_z(\vp_\times \circ a\sep d_H). %\leq \dil_{a(z)} (\vp_+\sep d_z) \dil_z(a\sep d_H, d_z)
$$
Therefore,  according to Lemma \ref{lemmaSubMult} for any norm $\|\cdot\|_{a(z)}$ defined on the tangent space $\R\times \R \times \theta(z)^\perp$ to $a(z)\in \cA$ we have 
\be
\label{eqDilPhiA}
\begin{array}{rcl}
& &\dil^*_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} a\sep d_H, \|\cdot \|_{a(z)})\\
& \leq& \dil_z(H)_\times\\
& \leq& \dil_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} \circ a\sep d_H, \|\cdot\|_{a(z)})
\end{array}
\ee
provided no indeterminate $0\times \infty$ or $\infty \times 0$ appears on the first and last term of this inequality.
%We recall that a neighborhood of $a(z)$ is parametrized by the local chart 
%\be
%\label{defPsiAZ}
%\psi_{a(z)} : (\Lambda, M, r\Theta) \to (\lambda(z) + \Lambda, \, \mu(z) + M, \, \cos(r)\theta(z)+ \sin(r) \Theta)
%\ee
%where $|\Theta| = 1$. 
We consider a fixed point $z\in \Omega$, and we distinguish the two cases $\lambda(z) \neq \mu(z)$ and $\lambda(z) = \mu(z)$.

\paragraph{Proof in the case $\lambda(z) \neq \mu(z)$.}
For each $a=(\lambda, \mu, \theta)\in \cA$ we define a norm $\|\cdot \|_a$ on the tangent space $\R\times \R \times \theta^\perp$ to $\cA$ at the point $a$ : for all $A = (\Lambda, M , \Theta)\in \R\times \R \times \theta^\perp$
$$
\|A\|_a = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \frac 1 2 \left| \frac \lambda \mu - \frac \mu \lambda\right| \|\Theta\|\right\}.
$$
We have by construction 
\be
\label{eqDilADZDH}
\dil_z(\psi_{a(z)}^{-1}\circ a\sep d_H, \|\cdot \|_{a(z)}) = D_z(a)_\times
\ee
According to Lemma \ref{lemmaDelta} and Proposition \ref{propPhiTimes} we have for any $a=(\lambda, \mu, \theta)\in \cA$ and any $A\in \R\times\R \times \theta^\perp$
$$
\|A\|_a \leq \|d_a \vp_\times(A)\|_\infty = \|d_0 (\vp_\times \circ \psi_a)\|_\infty \leq 2 \|A\|_a.
$$
Since $\vp_\times$ is $C^1$ it follows from \iref{eqDilDiff} that 
$$
1 \leq \dil^*_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq \dil_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq 2.
$$
Combining \iref{eqDilPhiA}, \iref{eqDilADZDH} and the last inequality we obtain
$$
D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times,
$$
which establishes the announced result \iref{eqDilTimes} in the case $\lambda(z)\neq \mu(z)$. A similar reasoning establishes the counterpart \iref{eqDilPlus} of this ineaquality for the distance $d_+$. 

\paragraph{Proof in the case $\lambda(z) = \mu(z)$.}
%We now turn to the case of equality $\lambda(z) = \mu(z)$.
For any $\ve>0$ and any $a=(\lambda, \mu, \theta)\in \cA$ such that $\lambda = \mu$ we define a norm $\|\cdot\|_{a,\ve}$ on the tangent space $\R\times \R\times \theta^\perp$ to $a$ in $\cA$ as follows : 
$$
\|A\|_{a, \ve} = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \ve \|\Theta\|\right\}.
$$
%$$
%d_z^\ve((\Lambda, M, r\Theta), (\Lambda', M', r'\Theta')) := \max \left\{\frac {|\Lambda-\Lambda'|} {\lambda(z)},\, \frac {|M-M'|} {\mu(z)}, \, \ve \|r\Theta - r'\Theta'\|\right\}.
%$$
This modification is required because the original norm $\|\cdot\|_a$ used in the case $\lambda\neq \mu$ is only a semi-norm when $\lambda = \mu$.
Reasoning similarly to the case $\lambda(z) \neq \mu(z)$ we obtain the upper bound
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H), \ \ve\dil_z(\theta\sep  d_H)\right\}.
$$
We now establish a lower bound on $\dil_z(H)_\times$.
We may assume that $\dil_z(\theta \sep d_H) < \infty$ otherwise there is nothing to prove. Since $\ve>0$ is arbitrary we thus obtain 
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H)\right\} = 2D_z(a)_\times.
$$
We now turn to the lower bound on $\dil_z(H)_\times$. 
For that purpose we define the functions $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda,\mu\}$  and we observe that for all $z,z'\in \Omega$
\begin{eqnarray*}
d_\times (H(z),H(z')) &=& \ln \max \{\|H(z)^\frac 1 2 H(z')^{-\frac 1 2}\|, \, \|H(z')^\frac 1 2 H(z)^{-\frac 1 2}\|\}\\
&\geq & \frac 1 2 \max \{|\ln \|H(z)\|- \ln \|H(z')\||, \, |\ln \|H(z)^{-1}\|- \ln \|H(z')^{-1}\||\\
&=& \max \{ |\ln\gamma(z) - \ln \gamma(z')|,\, |\ln \Gamma(z) - \ln \Gamma(z')|\}.
\end{eqnarray*}
We thus obtain
$$
\dil_z(H)_\times = \dil_z(H\sep d_\times, d_H) \geq \max \{ \dil_z(\ln \gamma\sep d_H), \, \dil_z(\ln \Gamma \sep d_H)\}.
$$
Hence according to Proposition \ref{propDilMax}
$$
\dil_z(H)_\times \geq \max \{\dil_z(\ln \lambda\sep d_H), \dil_z(\ln \mu\sep d_H)\} = D_z(a)_\times.
$$
Therefore $D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times$, and proceeding likewise we obtain $D_z(a)_+ \leq \dil_z(H)_+ \leq 2 D_z(a)_+$, which concludes the proof of Theorem \ref{th2Spaces}. \\

The next corollary shows how a quasi-acute metric can be obtained from a graded one.
We denote by $\diag(\lambda_1, \cdots, \lambda_d)$ the diagonal matrix of entries $\lambda_1, \cdots, \lambda_d$. 
Let $M\in S_d$ and let $U\in \cO_d$ and $\lambda_1, \cdots , \lambda_d\in\R$ be such that 
\be
\label{eqDiagSd}
M = U^\trans \diag(\lambda_1, \cdots , \lambda_d) U
\ee
For any $\alpha\in \R$ we define the matrix $\max \{\alpha, M\}\in S_d^+$ as follows
$$
\max\{\alpha, M\} := U^\trans \diag(\max\{\alpha, \lambda_1\}, \cdots, \max\{\alpha, \lambda_d\})U,
$$
and we observe that $\max\{\alpha, M\}$ does not depend on the choice of the matrix $U$ and on the order of the eigenvalues $\lambda_1, \cdots, \lambda_d$ in the decomposition \iref{eqDiagSd}.
For instance we have for any $(\lambda, \mu, \theta)\in \cA$ and any $s>0$  
$$ %\lambda^{-2} \theta\theta^\trans+ \mu^{-2} (\Id-\theta \theta^\trans)
\max \{s^{-2}, \cH(a)\} = \min\{s, \lambda\}^{-2} \theta \theta^\trans+ \min\{s, \mu\}^{-2} (\Id-\theta \theta^\trans).
$$

\begin{corollary}
\label{corolHgToHa}
Let $H\in \bH$ be such that $H(z)$ has an eigenvalue of multiplicity $\geq d-1$ for all $z\in \R^d$. We define $s:\R^d\to \R_+^*$ and $H'\in \bH$ as follows : for all $z\in \R^d$
$$
s(z) := \inf_{z'\in \sR^d} |z-z'|+ \|H(z')^{-\frac 1 2}\|,
$$
and 
$$
H'(z) := \max\{s(z)^{-2}, H(z)\}.
$$
If $H\in \bH_g$, then $4^2H'\in \bH_a$.
\end{corollary}

\proof
For each $\ve>0$ we define 
$$
H_\ve := \max\{e^{2 \ve} s(z)^{-2}, H(z)\}.
$$
The proof proceeds as follows: we first establish that for any $z\in \R^d$ one has 
\be
\label{eqDilHe}
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
\ee
We then use these properties to obtain that $4^2 H_\ve \in \bH_a$, and we conclude the proof using the convergence $H_\ve \to H$ as $\ve \to 0$.\\

We first observe that $s : \R^d \to \R_+^*$ is Lipschitz and that $s(z)\leq \|H(z)^{-\frac 1 2}\|$ for all $z\in \R^d$.

Consider a fixed point $z\in\R^d$. If $H(z)$ is proportional to $\Id$, which means that $\|H(z)\|^{-\frac 1 2} = \|H(z)^{-\frac 1 2}\| \geq s(z)$, then $H_\ve = e^{2 \ve} \Id/ s^2$ on a neighborhood of $z$. This implies according to \iref{eqDilLnH} %\ref{PropEquivS}
$$
\dil_z(H_\ve)_\times =\dil_z(H_\ve)_+ = \dil_z(e^{-\ve} s) \leq e^{-\ve}\leq 1,
$$
and therefore \iref{eqDilHe}.
On the other hand if $H(z)$ is not proportional to $\Id$ then there exists three continuous functions $\lambda, \mu \in C^0(\R^d, \R_+^*)$ and $\theta \in C^0(\R^d, \bbS)$ (where $\bbS := \{u\in \R^d \sep |u| = 1\}$) such that 
$
H = \lambda^{-2} \theta \theta^\trans+ \mu^{-2} (\Id - \theta \theta^\trans).
$
on a neighborhood of $z$.
Hence on the same neighborhood of $z$, 
$$
H_\ve = \min\{e^{-\ve} s,\lambda\}^{-2} \theta \theta^\trans+ \min\{e^{-\ve} s,\mu\}^{-2} (\Id - \theta \theta^\trans).
$$

\paragraph{Proof that $\dil_z(H_\ve)_\times \leq 2$.}
We define $H_\ve^i := e^{2\ve} \Id/ s^2$ and we observe that $H_\ve \geq H_\ve^i$ and $H_\ve \geq H$, hence for any $p,q\in \R^d$
$$
d_{H_\ve}(p,q) \geq \max \{d_H(p,q), \, d_{H_\ve^i}(p,q)\}.
$$
Using Proposition \ref{propDilLoc} we thus obtain  
\begin{eqnarray*}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\} \sep d_{H_\ve}) &\leq& \max \{\dil_z(\ln (e^{-\ve} s)\sep d_{H_\ve}), \,\dil_z(\ln \lambda\sep d_{H_\ve})\}\\
&\leq & \max \{\dil_z(\ln(e^{-\ve} s \sep d_{H_\ve^i})), \,\dil_z(\ln \lambda\sep d_H)\}\\
& \leq & \max \{\dil_z(e^{-\ve} s), \, \dil_z(H)_\times\}\\
& \leq & \max \{e^{-\ve}, 1\} =1,
\end{eqnarray*}
where we used Theorem \ref{th2Spaces} and Proposition \ref{propEquivS} in the third line.
Likewise $\dil_z(\ln \min\{e^{-\ve} s, \lambda\}\leq 1$. 
Since the function 
$$
t \mapsto \frac t \mu - \frac \mu t
$$
is increasing, we easily obtain that
$$
\left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right| \leq \left|\frac \lambda \mu - \frac \mu \lambda\right|.
$$
Therefore   
$$
\frac 1 2 \left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right|  \dil_z(\theta \sep d_{H_\ve}) \leq \frac 1 2\left|\frac \lambda \mu - \frac \mu \lambda\right| \dil_z(\theta\sep d_H) \leq 1,
$$
which implies that $D_z(a_\ve)_\times \leq 1$ where $a_\ve=(\min\{e^{-\ve}s, \lambda\}, \min\{e^{-\ve} s, \mu\}, \theta) \in C^0(\R^d,\cA)$. Hence
$$
\dil_z(H_\ve)_\times \leq 2 D_z(a_\ve)_\times \leq 2,
$$
which concludes this paragraph.
\paragraph{Proof that $\dil_z(H_\ve)_+ \leq 4$.}
As already observed in \iref{eqDilNorm}, for any metric space $(X,d_X)$ and any function $f\in C^0(\R^d, X)$ we have 
\be
\label{eqDilNormLM}
\dil_z(f) \leq \|H(z)\|^{\frac 1 2}\dil_z(f\sep d_H) = \frac{\dil_z(f\sep d_H)}{\min\{\lambda(z), \mu(z)\}}.
\ee
If $\lambda(z)<\mu(z)$ we therefore obtain 
\begin{eqnarray*}
\dil_z(\min\{e^{-\ve} s , \lambda\}) &\leq& \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)}\right\}\\
 &\leq& \max \{e^{-\ve}, \, \dil_z(\ln \lambda\sep  d_H)\}\\
 &\leq & \max \{e^{-\ve} , \, 1\} = 1.
\end{eqnarray*}
Still assuming that $\lambda(z)<\mu(z)$, we have $s(z)\leq \|H(z)^{-\frac 1 2}\| \leq \mu(z)$ by construction of $s$, and therefore $\min\{e^{-\ve} s, \mu\} = e^{-\ve} s$ on a neighborhood of $z$. It follows that 
$$
\dil_z(\min\{e^{-\ve} s, \mu\}) = \dil_z(e^{-\ve} s)\leq e^{-\ve} \leq 1.
$$
Proceeding similarly if $\lambda(z)>\mu(z)$ we also obtain $\dil_z(\min\{e^{-\ve} s, \lambda\})$ and $\dil_z(\min\{e^{-\ve} s, \mu\})$. 
We now focus on the local dilatation of the orientation $\theta$, and for that purpose we observe that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}|  \leq  |\lambda(z) - \mu(z)|.
$$
Furthermore we have according to \iref{eqDilNormLM}
\begin{eqnarray*}
 |\lambda(z) - \mu(z)| \dil_z(\theta)
&\leq& \frac {|\lambda(z) - \mu(z)|}{\min\{\lambda(z), \mu(z)\}} \dil_z(\theta\sep d_H)\\
&=& \left(\frac {\max \{\lambda(z), \mu(z)\}}{\min\{\lambda(z), \mu(z)\}}-1\right)\dil_z(\theta\sep d_H)\\
& \leq & \left|\frac {\lambda(z)} {\mu(z)}-\frac {\mu(z)} {\lambda(z)}\right|\dil_z(\theta\sep d_H) \\
&\leq & 2 D_z(a)_\times \leq 2.
\end{eqnarray*}
We conclude that $D_z(a_\ve)_+ \leq 2$, and therefore $\dil_z(H_\ve)_+ \leq 4$.

\paragraph{Conclusion.}
We have established that for all $z\in \R^d$ and all $\ve>0$
$$
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
$$
Therefore for any $z,z'\in \R^d$, since $H_\ve \leq e^{2\ve} H'$,
$$
d_\times(H_\ve(z), H_\ve(z')) \leq 2d_{H_\ve}(z,z') \leq 2e^\ve d_{H'}(z,z') \stext{ and } d_+(H_\ve(z), H_\ve(z')) \leq 4|z-z'|.
$$
Letting $\ve \to 0$ we obtain 
$$
d_\times(H'(z), H'(z')) \leq 2d_{H'}(z,z') \stext{ and } d_+(H'(z), H'(z')) \leq 4|z-z'|.
$$
According to Remark \ref{remHomog} this implies that $4^2 H\in \bH_a$, which concludes the proof of this corollary.
\sq


\section{From mesh to metric}
\label{secMeshToMet}
The techniques presented in this section show how to produce an metric $H\in \bH_i$, $\bH_a$ or $\bH_g$ from an isotropic, quasi-acute (in two dimensions), or graded mesh $\cT$.

Combining the next proposition with its counterpart Proposition \ref{propMeshGen}, on the generation of a mesh from a metric, yields the main result of this chapter: Theorem \ref{thEquiv} on the equivalence of the classes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ of meshes and $\bH_i \subset \bH_a \subset \bH_g$ of metrics which is announced in the introduction.
\begin{prop}
\label{propMetGen}
For any $C_0>0$ there exits $C = C(C_0,d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $\cT \in \bT_{i, C_0}$ there exists $H \in \bH_i$ which is $C$-adapted to $\cT$.
\item If $d=2$, then for any $\cT \in \bT_{a, C_0}$ there exists $H \in \bH_a$ which is $C$-adapted to $\cT$.
\item For any $\cT \in \bT_{g,C_0}$ there exists $H \in \bH_g$ which is $C$-adapted to $\cT$.
\end{enumerate}
\end{prop}

The rest of this section is devoted to the proof of this proposition.
For any mesh $\cT\in \bT$, and for any vertex $v$ of $\cT$, we denote by $n_\cT(v)$ the number of simplices in the mesh $\cT$ containing $v$:
$$
n_\cT(v) := \#\{T\in \cT \sep v\in T\}. %, %\text{s.t. } 
$$
We denote by $H_\cT^g\in \bH$ the piecewise linear metric on $\cT$ which satisfies for each vertex $v$ of $\cT$
\be
\label{eqHcTg}
H_\cT^g(v) := \frac 1 {n_\cT(v)} \sum_{\substack{T\in \cT\\\text{s.t. } v\in T}} \cH_T.
\ee
The metric $H_\cT^g$ on a simplex $T\in \cT$ is simply the linear interpolation of the averages of the matrices $\cH_T$ attached to the simplices containing a vertex $v$. 

The next lemma establishes a property of the barycentric coordinates on a simplex, which is useful for the analysis of  the regularity of a piecewise linear function on an anisotropic mesh, such as the metric $H_\cT^g$.
\begin{lemma}
\label{lemmaNormLambda}
Let $T$ be a simplex and let $V$ be the collection of vertices of $T$. Let $\lambda_v(z)$, $v\in V$ be the barycentric coordinates on $T$. Then for all $z,z'\in T$
\be
\label{eqNormLambda}
\|z-z'\|^2_{\cH_T} = \frac {d+1} d \sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2.
\ee
\end{lemma}

\proof
We first assume that $T$ is the reference equilateral simplex $\TEq$. %, and we recall that $\cH_\TEq = \Id$.
For any two vertices $v,v'$ in the collection $\VEq$ of vertices of $\TEq$ one easily checks that 
\be
\label{eqScalTEq}
\<v,v'\> = 
\left\{
\begin{array}{cl}
1 &\text{ if } v=v,'\\
-1/d &\text{ if } v \neq v'.
\end{array}
\right.
\ee
Indeed $|v|=1$ by construction for any vertex $v$ of $\TEq$, the scalar product $\<v,v'\>$ has a value $\alpha$ which is independent of the pair of distinct vertices $v,v'\in \VEq$. Since $\TEq$ is centered at the origin we obtain $0 = \<v,\sum_{v\in V} v\>  = |v|^2 + d \alpha$ which establishes \iref{eqScalTEq}.
We thus obtain for any $z,z'\in \TEq$ 
\begin{eqnarray*}
|z-z'|^2  &=& \left|\sum_{v\in \VEq} (\lambda_v(z) - \lambda_v(z'))v\right|^2 \\
&=& \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \sum_{v\neq v'} (\lambda_v(z)-\lambda_v(z'))(\lambda_{v'}(z)-\lambda_{v'}(z')).
\end{eqnarray*}
Therefore 
$$
|z-z'|^2 =  \left(1+\frac 1 d\right) \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \left(\sum_{v\in \VEq} \lambda_v(z)-\lambda_v(z')\right)^2,
$$
which concludes the proof in the case of $\TEq$ since $\cH_\TEq = \Id$ and since the barycentric coordinates of $z$ and of $z'$ sum to $1$.

We now consider an arbitrary simplex $T$, and an affine change change of coordinates $\Phi$ such that $\Phi(T) = \TEq$, $\Phi(z) = \phi z+ z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. We have $\cH_T = \phi^\trans \phi$ according to \iref{invcH}, hence for all $z,z'\in T$
$$
 |\Phi(z) - \Phi(z')| = |\phi(z-z')| = \|z-z'\|_{\cH_T}.
$$
Furthermore the barycentric coordinates of $z$ and $z'$ in $T$ are the same as those of $\Phi(z)$ and $\Phi(z')$ in $\Phi(T) = \TEq$, hence \iref{eqNormLambda} holds which concludes the proof of this lemma.
\sq



The next proposition establishes that the metric $H_\cT^g$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case iii) of graded meshes. More precisely for any mesh $\cT\in \bT_{g,C_0}$ the metric $d C_0^{10} H_\cT^g$ belongs to $\bH_g$ and is $C_0^6 \sqrt d$ equivalent to $\cT$.



\begin{prop}
\label{propHTG}
For any $\cT\in \bT_{g,C_0}$ the metric $H_\cT^g$ is $C_0$-adapted to $\cT$, and $d C_0^{10} H_\cT^g\in \bH_g$.
\end{prop}

\proof
We consider a simplex $T\in \cT$, and we recall that for any neighbor $T'$ of $T$ one has 
$$
C_0^{-2} \cH_T \leq \cH_{T'} \leq C_0^2 \cH_T.
$$
Averaging these matrices as in \iref{eqHcTg} we obtain for any vertex $v$ of $T$
\be
\label{eqHTHv}
C_0^{-2} \cH_T \leq H_\cT^g(v)\leq C_0^2 \cH_T.
\ee
Averaging with respect to the barycentric coordinates of a point $z\in T$ we eventually obtain 
\be
\label{eqHTHz}
C_0^{-2} \cH_T \leq H_\cT^g(z)\leq C_0^2 \cH_T,
\ee
which establishes as announced that the metric $H_\cT^g$ is $C_0$-adapted to $\cT$.

We now establish the regularity property of $H_\cT^g$, and for that purpose we consider two points $z,z'\in T$ and a vector $u\in \R^d\sm\{0\}$. We thus have 
\begin{eqnarray*}
\frac {\|u\|^2_{H_\cT^g(z)}} {\|u\|^2_{H_\cT^g(z')}} &=& \frac {\sum_{v\in V} \lambda_v(z) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2} \\
&=& 1+ \frac {\sum_{v\in V} (\lambda_v(z)-\lambda_v(z')) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2}\\
&\leq& 1+ C_0^4 \frac{\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|}{\sum_{v\in V} \lambda_v(z')}\\
& \leq & 1+C_0^4 \sqrt {(d+1)\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2}\\
&=& 1+C_0^4 \sqrt d \| z-z'\|_{\cH_T},
\end{eqnarray*}
where we used \iref{eqHTHv} in the third line, Cauchy-Schwartz inequality in the fourth line, and Lemma \iref{lemmaNormLambda} in the fifth line.
We consider a simplex $T\in \cT$ and we intend to give a uniform bound on $\dil_z(H_\cT^g)_\times$ for all $z\in \interior(T)$. It follows from our estimate on $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, and from the analog estimate for  $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, that 
\begin{eqnarray*}
d_\times (H_\cT^g(z), H_\cT^g(z')) &=& \max_{u\neq 0} \left|\ln \|u\|_{H_\cT^g(z)} - \ln \|u\|_{H_\cT^g(z')}\right|\\
&\leq& \frac 1 2\ln (1+C_0^4 \sqrt d \|z-z'\|_{\cH_T}) \\
&\leq& \frac {C_0^4 \sqrt d} 2 \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Hence according to \iref{eqHTHz} and \iref{eqDilNorm} we obtain for all $z\in \interior (T)$
$$
\dil_z(H_\cT^g)_\times \leq C_0^5 \sqrt d.
$$
The metric $H := d C_0^{10} H_\cT^g$ thus satisfies $\dil_z(H)_\times = (dC_0^{10})^{-1/2}\dil_z(H_\cT^g)_\times \leq 1$ for any point $z$ in the interior of any simplex $T\in \cT$.

Let $z,z'\in \R^d$ and let $\gamma\in C^1([0,1], \R^d)$ be such that $\gamma(0) = z$ and $\gamma(1) = z'$.
There exists a sequence $(\ve_n)_{n \geq 0}$, $\ve_n \in \R^d$, $\ve_n \to 0$, such that for all $n \geq 0$ the translated path $\gamma+\ve_n$ intersects the skeleton 
$
\cup_{T\in \cT} \partial T
$
of the mesh $\cT$ only a finite number of times $0\leq t_1^n < \cdots < t_{k(n)}^n\leq 1$. Defining $t_0^n := 0$ and $t^n_{k(n)+1} := 1$, Proposition \ref{propDilLoc} states that for all $0\leq i \leq k(n)$ one has 
$$
d_\times (H(\gamma(t^n_i)+\ve_n), \, H(\gamma(t_{i+1})+\ve_n)) \leq l_H(\gamma_{|[t_1,t_{i+1}]}+\ve_n).
$$
Adding up these inequalities we obtain $d_\times (H(z+\ve_n), \, H(z'+\ve_n)) \leq l_H(\gamma+\ve_n)$, and therefore $d_\times (H(z), \, H(z')) \leq l_H(\gamma)$ as $n \to \infty$. Taking the infimum among all paths $\gamma$ joining $z$ and $z'$ we obtain $d_\times(H(z), H(z')) \leq d_H(z,z')$, hence $H \in \bH_g$ as announced which concludes the proof. 
\sq

We associate to any mesh $\cT\in \bT$ a metric $H_\cT^i$ defined as follows : for all $z\in \R^d$, 
$$
H_\cT^i(z) := \|H_\cT^g(z)\| \Id.
$$
The next result shows that $H_\cT^i$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case of isotropic metrics. More precisely for any mesh $\cT\in \bT_{i,C_0}$ the metric $d C_0^{10} H_\cT^i$ belongs to $\bH_i$ and is $C_0^7 \sqrt d$ equivalent to the mesh $\cT$.

\begin{corollary}
For any mesh $\cT\in \bT_{i,C_0}$ the metric $H_\cT^i$ is $C_0^2$-adapted to the mesh $\cT$, and $d C_0^{10} H_\cT^i \in \bH_i$.
\end{corollary}

\proof
For any matrix $M\in S_d^+$ we have $\|M^{-1}\|^{-1} \Id \leq M \leq \|M\| \Id$. We therefore obtain for any simplex $T\in \cT$
\be
\label{eqcHNormcH}
C_0^{-2} \|\cH_T\| \Id\leq \frac{\|\cH_T\|} {\rho(T)^2} \Id = \|\cH_T^{-1}\|^{-1} \Id \leq \cH_T \leq \|\cH_T\|\Id.
\ee
Let $T\in \cT$ and let $z\in T$. Since $\rho(T) \leq C_0$ and $C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z)$ we obtain 
$$
C_0^{-2} H_\cT^i(z) := C_0^{-2} \|H_\cT^g(z)\| \Id \leq \|\cH_T\| \Id \leq C_0^2 H_\cT^i(z).
$$
Combining this with \iref{eqcHNormcH} we obtain
$$
C_0^{-4} H_\cT^i(z) \leq \cH_T \leq C_0^2 H_\cT^i(z),
$$
which establishes as announced that the metric $H_\cT^i$ is $C_0^2$ equivalent to the mesh $\cT$.

According to Proposition \ref{propHTG} we have $d C_0^{10} H_\cT^g\in \bH_g$. Corollary \ref{corolLipNorm} thus implies that $d C_0^{10} H_\cT^i\in \bH_i$, which concludes the proof of this proposition.
\sq

Before turning to the case of quasi-acute metrics we prove a lemma on the neighborhood of a simplex in a graded mesh. For any mesh $\cT\in \bT$ and any closed set $E\subset \R^d$ the neighborhood $V_\cT(E)$ of $E$ in $\cT$ is  defined as the union of all simplices $T\in \cT$ which intersect $E$: 
$$
V_\cT(E) := \cup_{\substack{T\in \cT\\T \cap E \neq \emptyset}} T.
$$

\begin{prop}
\label{propNeighborT}
Let $\cT\in \bT_{g,C_0}$ and let $T \in \cT$, then for all $x\in T$ and all $y \in \R^d \sm V_\cT(T)$ we have 
$$
\|x-y\|_{\cH_T} \geq (C_0\sqrt d)^{-1}.
$$
\end{prop}

\proof
The simplex $T\in \cT$ is fixed throughout this proof. We consider the function $\vp : \R^d \to \R$ which is piecewise linear on the mesh $\cT$, and which satisfies for any vertex $v$ of the mesh $\cT$
$$
\vp(v) = 
\left\{
\begin{array}{cl}
1 & \text{ if } v\in T,\\
0 & \text{ if } v \notin T.
\end{array}
\right.
$$
We denote by $V'$ the collection of vertices of a simplex $T'\in \cT$, and by $(\lambda_v(z))_{v\in V'}$ the barycentric coordinates of a point $z\in T'$.
We have for any $z,z'\in T'$
\begin{eqnarray*}
|\vp(z)- \vp(z')| &\leq& \sum_{v \in V'} |\lambda_v(z)-\lambda_v(z')| \vp(v)\\
& \leq &\sqrt{(d+1) \sum_{v\in V'} |\lambda_v(z)-\lambda_v(z')|^2} \\
&= &\sqrt d \|z-z'\|_{\cH_{T'}}.
\end{eqnarray*}
Recalling that $\vp$ is identically $0$ on $T'$ if $T\cap T' = \emptyset$, and that $\cH_{T'} \leq C_0^2 \cH_T$ otherwise, we obtain for any $z,z'\in T'$
$$
|\vp(z)- \vp(z')| \leq C_0\sqrt d \|z-z'\|_{\cH_{T}}.
$$
We claim that $\vp : (\R^d, \|\cdot \|_{\cH_T})  \to \R$ is $C_0\sqrt d$-Lipschitz. Indeed consider $z,z'\in \R^d$, and denote by $z_1, \cdots, z_k$ the intersections of the segment $[z,z']$ with the skeleton $\cup_{T'\in \cT} \partial T'$ of the mesh. Defining $z_0 := z$ and $z_{k+1} := z'$ we obtain 
% generically a finite number. 
$$
|\vp(z)-\vp(z')| \leq \sum_{0 \leq i \leq k} |\vp(z_i)-\vp(z_{i+1})| \leq C_0 \sqrt d \sum_{0 \leq i \leq k} \|z_i - z_{i+1}\|_{\cH_T} =C_0 \sqrt d \|z-z'\|_{\cH_T}.
$$
For any $x\in T$ and any $y\in \R^d\sm V_\cT(T)$ we have $\vp(x) = 1$, $\vp(y) = 0$, thus $1 \leq C_0\sqrt d \|x-y\|_{\cH_T}$ which concludes the proof of this proposition.
\sq

We assume from this point that the dimension is $d=2$. %, and we thus restrict our attention to the bi-dimensional triangulations.
For each triangulation $\cT\in \bT$ we define a function $s_\cT : \R^2 \to \R_+^*$ as follows 
$$
s_\cT(z) := \inf_{z'\in \sR^2} |z-z'| + \|H_\cT^g(z')^{-\frac 1 2}\|.
$$
We define a metric $H_\cT^a \in \bH$ as follows : for each $z\in \R^2$  
\be
\label{defHTA}
H_\cT^a(z) = \max\{s_\cT(z)^{-2} , \, H_\cT^g(z)\}.
\ee

The rest of this section is devoted to proof of the following proposition, on quasi-acute meshes, in two dimensions.
\begin{prop}
\label{propHTA}
For any $C_0 \geq 1$ there exists $C=C(C_0)$ such that the following holds.
For any $\cT\in \bT_{a,C_0}$ the metric $H_\cT^a$ is $C$-adapted to the mesh $\cT$, and $32 C_0^{10} H_\cT^a\in \bH_a$.
\end{prop}

The fact that $32 C_0^{10} H_\cT^a\in \bH_a$ directly follows from the fact that $2 C_0^{10} \bH_\cT^g\in \bH_g$ and from Corollary \ref{corolHgToHa}. 

For each $z\in \R^2$ define $d_\cT(z) := \|H_\cT^g(z)^{-\frac 1 2}\|$. This quantity should be heuristically regarded as the diameter of the triangle containing $z$. We establish below the following property : there exists $\delta = \delta(C_0) >0$ such that for all $z,z'\in \R^2$
\be
\label{eqRegDT}
\text{ if } |z'-z| \leq \delta d_\cT(z) \stext{ then }  d_\cT(z') \geq \delta d_\cT(z).
\ee
Before turning to the proof of \iref{eqRegDT} we show how this property leads to the proof of Proposition \ref{propHTA}.
For all $z\in \R^d$ we have 
$$
s_\cT(z) = \inf_{z\in \sR^2} |z-z'|+d_\cT(z)  \geq \inf_{z'\in \sR^2} \min \{|z-z'|, \, d_\cT(z')\} \geq \delta d_\cT(z'),
$$
indeed $|z-z'|\geq \delta d_\cT(z)$ or $d_\cT(z') \geq \delta d_\cT(z)$ for any $z'\in \R^d$ according to \iref{eqRegDT}.
Combining this with the definition \iref{defHTA} of $H_\cT^a$ we obtain for all $z\in \R^2$
$$
\delta^2 H_\cT^a(z) \leq H_\cT^g(z)\leq H_\cT^a(z). 
$$
Recalling that $H_\cT^g$ is $C_0$-adapted to the mesh $\cT$, see proposition \ref{propHTG}, we obtain for all $T\in \cT$ and all $z\in T$ 
$$
\delta^2 C_0^{-2} H_\cT^a(z) \leq C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z) \leq C_0^2 H_\cT^a(z)
$$
which establishes that the metric $H_\cT^a$ is $C_0/\delta$ adapted to the mesh $\cT$, and concludes the proof of Proposition \ref{propHTA}.\\

We now turn to the proof of \iref{eqRegDT}, and for that purpose we introduce some notations.
For each segment $e=[\omega-u, \omega+u]\subset \R^2$ we define the diamond $\lozenge(e)$ of $e$ as follows
$$
\lozenge(e) := \{z\in \R^2 \sep |\<z-\omega,u\>|+ C_0 |\det (z-\omega,u)| < |u|^2\}.
$$
The next lemma considers a triangulation $\cT'$ on which the measure of sliverness is uniformly bounded by $C_0$, and compares the length an edge $e$ of $\cT'$ with the diameter of the triangles in $\cT'$ which intersect $\lozenge(e)$.

\begin{lemma}
\label{lemmaUUp}
Let $\cT'\in \bT$ be a triangulation such that $S(T) \leq C_0$ for all $T\in \cT'$. Let  $e=[\omega-u, \omega+u]$ be an edge of $\cT'$.
Then there is no vertex in the diamond $\lozenge(e)$, and for all $z\in \lozenge(e)$ and any triangle $T\in \cT'$ containing $z$, there exists an edge $e'= [\omega'-u', \omega'+u']$ of $T$ satisfying  
$$
2 |u'| \geq |u| -C_0 |\det (z-\omega,u)|/ |u|
%2 |\<u,u'\>| \geq |u|^2 - C_0 |\det (z,u)|.
$$
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$, and we assume up to a translation and a rotation that $\omega = 0$ and $u = u_y$.
We recall that for any triangle $T$, with maximal angle $\theta$, the measure of sliverness $S(T)$ has the following expression
$$
S(T) = \max\{1, \tan(\theta/2)\}.
$$
We assume for contradiction that there exists a vertex $v_0 = (x_0,y_0)\in \lozenge(e)$, and we assume without loss of generality that $x_0<0$. We consider a vertex $v_1 = (x_1,y_1)$ of $\cT$ such that the angle 
$$
\theta_0 :=  \angle(v_1-v_0, \, u_x) \in [-\cPi, \cPi)
$$
has the smallest possible absolute value $|\theta_0|$ (the bold letter $\cPi$ denotes the numerical constant $\cPi = 3.14159\cdots$). By construction there exists a triangle $T\in \cT$ containing $v_0$ and $v_1$ which has an angle  larger or equal or equal than $2\theta_0$ at the vertex $v_0$. It follows that $|\tan \theta_0| \leq S(T) \leq C_0$, and therefore  
$$
|y_1-y_0| \leq |\tan \theta_0| (x_1 - x_0) \leq C_0 (x_1-x_0).
$$
Proceeding inductively we define a sequence $v_n = (x_n, y_n)$, $n\geq 0$, of vertices of $\cT$ satisfying 
$
|y_{n+1} - y_n| \leq C_0 (x_{n+1} - x_n). 
$
Adding these inequalities together we obtain 
$$
|y_n-y_0|  \leq C_0 (x_n-x_0).
$$
It follows that one of the edges $[v_n, v_{n+1}]$, $n \geq 0$, of the mesh $\cT'$ intersects the edge $e$, which is a contradiction. The diamond $\lozenge(e)$ therefore does not contain any vertex, which concludes the proof of the first part of this proposition. \\

We now consider a point $z_0 = (x_0,y_0)\in \lozenge(e)$ and we assume without loss of generality that $x_0 \geq 0$. We consider a triangle $T$ containing $z_0$, and an edge $e'= [\omega'-u', \omega'+u']$ of $T$ which is on the left of $z_0$ (in other words the edge $e'$ and the segment $[(0,y_0),(x_0, y_0)]$ joining the point $z_0$ to its orthogonal projection on the edge $e$ intersect).

Since there is no vertex of $\cT'$ in the diamond $\lozenge(e)$, the edge $e'$ intersects the boundary of $\lozenge(e)$ at two points. We denote these points by $(x,y)$ and $(x',y')$, and we assume that without loss of generality that $y\geq 0 \geq y'$.
Observing that $0 \leq x \leq C_0^{-1}$, $0 \leq x'\leq C_0^{-1}$ and $\min\{x,x'\} \leq x_0$ we obtain  
$$
y-y' = (1-C_0 x) - (-1+C_0 x') \geq 1-C_0 x_0.
$$
Since $u = u_y = (0,1)$ and $2 u' = \lambda (x-x', y-y')$ for some $|\lambda| \geq 1$, we obtain 
$$
2|\<u,u'\>| \geq  
y-y' \geq 1-C_0 x_0 = |u|^2 - C_0 |\det (z_0,u)|,
$$
which concludes the proof of this proposition.
\sq

We now consider a fixed quasi-acute mesh $\cT\in \bT_{a,C_0}$ and we denote by $\cT'$ a fixed $C_0$-refinement of $\cT$ which satisfies $S(T) \leq C_0$ for all $T\in \cT'$. The next proposition involves a rectangular set $\square(e)$ associated to an edge $e$ of $\cT'$ which contains $e$ in its interior, contrary to the set $\lozenge(e)$ appearing in the previous proposition.  

\begin{lemma}
\label{lemmaRect}
There exists a constant $\delta_0 = \delta_0(C_0, d)>0$ such that the following holds.
We define the rectangle $\square(e)$ associated to an edge $e = [\omega-u, \, \omega+u]$ of $\cT'$ as follows
$$
\square(e) = \{z\in \R^2 \sep |\<z-\omega, u\>|\leq (1+\delta_0)|u|^2 \text{ and } |\det (z-\omega,u )| \leq \delta_0 |u|^2\},
$$
%where $\delta_0 = \delta_0(C_0):= ??1/(2C_0) >0$ is a constant specified in the proof.
We have $d_\cT(z) \geq \delta_0|u|$ for all $z\in \square(e)$.
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$. 
Up to a rotation and a translation, we may again assume that $\omega = 0$ and $u = u_y=(0,1)$.
We consider a triangle $T\in \cT$ containing the edge $e$ (note that $e\subset T$ but that $e$ may not be an edge of $T$, since we only known that $e$ is an edge in $\cT'$).

We define $H := H_\cT^g$. Recalling that $H$ is $C_0$-equivalent to $\cT$ we obtain for all $z\in e$
$$
C_0^{-2} H(z)\leq \cH_T \leq C_0^2 H(z). 
$$
The inclusion $e\subset T \subset \cE_T$ implies the upper bound $\|u\|_{\cH_T} = \|u_y\|_{\cH_T} \leq 1$. Hence for all $z\in e$
$$
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq \|u_y\|_{H(z)}^{-1} \geq C_0^{-1}.
$$
Note also that for any $z,u \in \R^2$
$$
d_\times (H(z), H(z+u)) \geq \ln \|H(z)^\frac 1 2 H(z+u)^{-\frac 1 2}\| \geq |\ln d_\cT(z) -\ln d_\cT(z+u)|.
$$
We define $C_1 := \sqrt 2 C_0^5$, in such way that $C_1^2 H\in \bH_g$, and we thus have  according to \iref{eqLocalNorm} if $C_1\|u\|_{H(z)}<1$
$$
|\ln d_\cT(z) -\ln d_\cT(z+u)| \leq d_\times (H(z), H(z+u)) \leq -\ln (1-C_1\|u\|_{H(z)}).
$$
Therefore for all $z\in e$ and all $u\in \R^d$,
$$
d_\cT(z+u) \geq d_\cT(z) (1-C_1 \|u\|_{H(z)}) \geq C_0^{-1}(1-C_1C_0 \|u\|_{\cH_T}).
$$
We define $C_2 := 4C_0C_1$ and we observe that any point of the rectangle 
\be
\label{eqRectGrad}
\left[\frac {-1}{C_2 \|u_x\|_{\cH_T}}, \,\frac 1 {C_2 \|u_x\|_{\cH_T}}\right] \times \left[-(1+C_2^{-1}), \, 1+C_2^{-1}\right].
\ee
can be written under the form $z+u$ where $z\in e$ and $\|u\|_{\cH_T} \leq 1/(2C_0C_1)$. We thus have  
\be
\label{eqdGrad}
d_\cT(z') \geq 1/(2C_0)
\ee
 on this rectangle.

We introduce a small constant $\delta = \delta(C_0)>0$ which is specified later in the proof. It follows from \iref{eqRectGrad} and \iref{eqdGrad} that the proof of this lemma is complete if $\|\cH_T\| \leq \delta^{-2}$, with $\delta_0 := \min \{\delta/C_2, \, 1/(2C_0)\}$.
We thus assume from this point that $\|\cH_T\|\geq \delta^{-2}$.\\

We assume that $\delta< C_0^{-1}$ and we define the rectangle
$$
\square_\delta := [-\delta, \delta] \times [1-C_0 \delta, -1+C_0 \delta],
$$
which is included in $\overline \lozenge(e)$ by construction.
Since $C_1^2 H\in \bH_g$, the function $z\mapsto \|H(z)\|^{-\frac 1 2}$ is $C_1$-Lipschitz according to Corollary \ref{corolLipNorm}. We thus have for all $z = (x,y)\in \square_\delta$
\be
\label{defr0}
\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2}+C_1|x|\leq r_0(\delta) := (C_0+C_1)\delta.
%\|u_x\|_{H(z)} \geq \|u_x\|_{H(y,0)}(1-C_1 |x| \|u_x\|_{H(y,0)}) \geq C_*(1-C_1 C_0 \delta_* C_*),
%\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2} + C_1 |x|
\ee
On the other hand it follows from Lemma \ref{lemmaUUp} that any $z = (x,y)\in \square_\delta$ is contained in a triangle containing an edge $e' = [\omega'-u', \omega'+u']$ such that $|u'| \geq (1-C_0 \delta)/2$. We thus have 
$$
1 \geq \|u'\|_{\cH_{T'}} \geq \frac{|u'|}{ \|\cH_{T'}^{-\frac 1 2}\|} \geq \frac{1-C_0 \delta}{2 \|\cH_{T'}^{-\frac 1 2}\|} 
$$
and therefore 
%of length at least $T'\in \cT$ satisfying $\|\cH_{T'}^{-\frac 1 2}\| \geq (1-C_0 \delta_*)/2$, hence 
\be
\label{defR0}
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq C_0^{-1} \|\cH_{T'}^{-\frac 1 2}\|  \geq  R_0(\delta) := (1-C_0 \delta)/(2C_0). %\det (z,u_y)
\ee
For all $z\in \square_\delta$, we denote by $\theta(z) = (\cos \Theta(z), \sin \Theta(z))$, $\Theta(z)\in [0, \cPi]$, the direction of the eigenvector associated to the small eigenvalue of $H(z)$, in such way that 
\be
\label{eqNormTheta}
\|\theta(z)\|_{H(z)} = \|H(z)^{-\frac 1 2}\|^{-1} = d_\cT(z)^{-1}.
\ee
We thus have for any $(0,y)\in e$
$$
C_0 \geq C_0 \|u_y\|_{\cH_T} \geq \|u_y\|_{H(0,y)} \geq |\cos \Theta(0,y)| \sqrt{\|H(0,y)\|} = \delta^{-1} |\cos \Theta(0,y)| ,
$$
hence 
$$
|\cos \Theta(0,y)| \leq  C_0 \delta.
$$
For all $z\in \square_\delta$ we have according to Theorem \ref{th2Spaces} 
$$
(R_0(\delta)-r_0(\delta)) \dil_z(\Theta) \leq  (\|H(z)^{-\frac 1 2}\| - \|H(z)\|^{-\frac 1 2}) \dil_z(\Theta) \leq 2C_1.
$$
Hence we obtain for all $z= (x,y)\in \square_\delta$  
$$
(R_0(\delta)-r_0(\delta)) |\Theta(z) - \Theta(0,y)| \leq 2C_1 |x|\leq 2C_1 \delta,
$$
hence since $t \mapsto \cos t$ is a Lipschitz function %, since $\cos : [0, \cPi/2]\to \R$ is convex
\be
\label{defTheta0}
|\cos \Theta(z)| \leq \cos \Theta_0(\delta) := C_0 \delta + \frac{\delta}{R_0(\delta)-r_0(\delta)}.
\ee
We have according to \iref{eqLocalNorm} for all $z\in \square_\delta$ and all $r\geq 0$ such that $C_1r\|\theta\|_{H(z)}<1$,
\begin{eqnarray*}
|\ln d_\cT(z+r \theta(z)) - \ln d_\cT(z)| &\leq& d_\times (H(z+r\theta(z)),H(z))\\
&\leq& -\ln (1-C_1r\|\theta\|_{H(z)})\\
&=& -\ln (1-C_1r/d_\cT(z)),
\end{eqnarray*}
therefore 
$$
d_\cT(z+r \theta(z)) \geq  d_\cT(z) (1-|r| C_1 /d_\cT(z)).
$$
For all $z\in \square_\delta$ such that $|r|\leq R_1(\delta) := R_0(\delta)/(2C_1)$ we thus obtain
$$
d_\cT(z+r\theta(z)) \geq R_0(\delta)(1-|r|C_1/R_0(\delta))\geq R_0(\delta)/2.
$$
It follows that $d_\cT(z')\geq R_0(\delta)/2$ for all $z'$ in the set 
$$
\{z+r\theta(z) \sep z\in \square_\delta,\, |r|\leq R_1(\delta)\} \supset [-\delta_0,\delta_0]\times [-(1+\mu_0),1+\mu_0]
$$
where 
\be
\label{eqD0MU0}
\delta_0 := \delta - r \cos \Theta_0(\delta) \stext{ and }  \mu_0 := -C_0 \delta+ r \sin \Theta_0(\delta)
\ee
and where the constant $0 \leq r\leq R_1(\delta)$ can be freely chosen.
The rest of the proof consists in choosing appropriate constants $\delta$ and $r$.\\

As $\delta \to 0$ we have $r_0(\delta)\to 0$, $R_0(\delta) \to 1/(2C_0)$ and $\cos\Theta_0(\delta) \to 0$. We thus choose $\delta = \delta(C_0,d)>0$ sufficiently small in such way that 
\be
\label{eqRCS}
R_0 \geq 1/(4C_0)
, \quad
\cos \Theta_0 \leq 1/(8C_0)
, \quad
\sin \Theta_0 \geq 1/2
.
\ee
We then choose $r := 4C_0 \delta$, which is smaller than $R_1(\delta)= R_0(\delta)/(2C_1) \geq 1/(8C_1C_0)$ if $\delta$ is sufficiently small. Injecting this choice of $r$ and \iref{eqRCS} in \iref{eqD0MU0} we thus obtain 
$$
\delta_0 \geq \delta/2 \stext{ and }\mu_0 \geq C_0 \delta.
$$
We have thus established under the hypothesis $\|\cH_T\|\geq \delta^{-2}$ that 
hence $d_\cT(z) \geq 1/(8C_0)$ for all $z$ in the rectangle 
$$
[-\delta/2, \delta/2]\times [-(1+C_0\delta), 1+C_0 \delta].
$$
Since the case $\|\cH_T\|\leq \delta^{-2}$ is already established this concludes the proof of this proposition.
\sq

The next lemma establishes a technical property on the covering a one dimensional segment by smaller ones, which is a key to the end of this proof.

\begin{lemma}
\label{lemmaCoverSeg}
Let $x_1, \cdots , x_k\in [0,1]$ and let $h_1, \cdots, h_k >0$ be such that 
\be
\label{eqDefXiHi}
[0,1]\subset \bigcup_{1\leq i \leq k} [x_i-h_i, \, x_i+h_i].
\ee
Let $\delta>0$ and let $h_* = h_*(k,\delta) := \exp(1-2k/\delta)/\delta$. Then 
\be
\label{eqInclSeg}
[0,1]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_* \leq h_i}} [x_i-(1+\delta)h_i, \, x_i+(1+\delta)h_i].
\ee
\end{lemma}

\proof
For each $y\in [0,1]$ we denote by $h(y)$ the value $h_i$ associated to the segment $[x_i-h_i, x_i+h_i]$ of smallest length containing $y$.
We thus have 
$$
\int_{[0,1]} \frac {dy} {h(y)} \leq \sum_{1\leq i \leq k} \int_{x_i-h_i}^{x_i+h_i} \frac 1 {h_i} = 2k.
$$
We assume for contradiction that \iref{eqInclSeg} does not hold, and we consider a point $x\in [0,1]$ which does not belong to the right hand side of $[0,1]$. For each $y\in [0,1]$ one of the two following possibilities holds
$$
\delta h(y) < |x-y| \stext{ or } h(y) < h_*.
$$
Integrating we obtain 
$$
\int_0^1 \frac {dy} {h(y)}  \geq \int_0^1 \frac {dy} {\max\{|x-y|/\delta,\, h_*\}}.
$$
The minimum value of the right hand side is attained for $x=0$ or $1$ and equals 
$$
\int_0^1 \frac {dy}{\max \{|x-y|/\delta, h_*\}} = \int_0^{\delta h_*} \frac 1 h_* + \int_{\delta h_*}^1 \frac \delta ydy = \delta(1-\ln(\delta h_*))
$$
Thus $2k>\delta(1-\ln(\delta h_*))$, which contradicts the definition of $h_*$. This concludes the proof of this lemma.
\sq

Under the hypotheses of Lemma \ref{lemmaCoverSeg} we thus have
\be
\label{eqInclSegDouble}
[-h_*\delta,\, 1+h_*\delta]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_i \leq h_*}} [x_i-(1+2\delta)h_i, \, x_i+(1+2\delta)h_i].
\ee


We now conclude the proof of Proposition \ref{propHTA}.
We consider a point $z\in \R^2$ contained in a triangle $T\in \cT$, and we denote by $\cT$ the longest edge $e$ of $T$. Up to a rotation and a translation, we may assume that $e=[0, u_x]$ joins the origin of $\R^2$ to the the vector $u_x := (1,0)$.
Note that 
\be
\label{eqNormHTInv}
2 \geq \|u_x\|_{\cH_T} \geq \|\cH_T^{-\frac 1 2}\|^{-1}.
\ee
Since the triangulation $\cT'$ is a $C_0$-refinement of $\cT$, the edge $e$ of $T$ is built of $k \leq C_0$ edges $(e_i)_{1 \leq i \leq k}$ of $\cT'$,
$$
e_i = [(x_i-h_i)u_x,\,  (x_i +h_i) u_x].
$$

We define $h_* := h_*(C_0, \delta_0/2) = 2\exp(1-4C_0/\delta_0)/\delta_0$, where $\delta_0$ is the constant from Lemma \ref{lemmaRect}, and we observe that 
\be
\label{eqRectHoDo}
\bigcup_{h_* \leq h_i} \square(e_i) \supset \left[-\frac{h_* \delta_0} 2, 1+ \frac{h_* \delta_0} 2\right] \times [-h_* \delta_0, h_* \delta_0],
\ee
Since $e$ is the longest edge of $T$, the angles of $T$ at the extremities of $e$ are acute.
Furthermore the height $h$ of $T$ orthogonal to the edge $e = [0,u_x]$ satisfies 
$$
h/2 = |T|  = \frac{|\TEq|} { \sqrt {\det \cH_T}} = \frac{|\TEq|}{\sqrt{\|\cH_T\| \|\cH_T^{-1}\|^{-1}}}  = \frac{|\TEq| \|\cH_T^{-1}\|}{\rho(T)} \geq \frac{|\TEq|}{4 \rho(T)} .
$$
Hence we obtain with $c := |\TEq|/8$ the inclusion
\be
\label{eqTRectRho}
T \subset [0,1] \times [-c/\rho(T), c/\rho(T)]
\ee
We distinguish two cases depending on the value of $\rho(T)$. If $c/\rho(T) \leq h_* \delta_0$, equivalently $\rho(T) \geq c/(h_* \delta_0)$ we obtain combining \iref{eqRectHoDo} and \iref{eqTRactRho} that $d_\cT\geq h_*\delta_0$ on the set 
$$
z+ \left[-\frac {h_*\delta_0} 2, \frac {h_*\delta_0} 2\right]^2
$$
which concludes the proof of this proposition.
One the other hand we have for any vector $u\in \R^2$
$$
\frac{d_\cT(z+u)}{d_\cT(z)} \geq  1-C_1 \|u\|_{H(z)} \geq 1-C_0C_1 \|u\|_{\cH_T} \geq  1-C_0C_1 \rho(T) |u| \|\cH_T^{-\frac 1 2}\|^{-1} \geq 1-2 C_0C_1 \rho(T) |u| 
$$
which concludes the proof if $\rho(T) \leq c/(h_*\delta_0)$.

\section{From metric to mesh}
\label{secMetToMesh}
%\subsection{Mesh generation}
\label{secMeshGen}

%We prove in this section Theorems \ref{thI}, \ref{thA} and \ref{thR} on the equivalence between certain classes of meshes and of metrics. %, which is divided in two parts.
%This proof is divided in two parts as follows. Proposition \ref{propMeshGen} in \S \ref{secMeshGen} we show how a mesh can be generated from a Riemannian metric, and Proposition \ref{propMetGen} in \S\ref{secMetGen} we show how a metric can be generated from a mesh.
%
This section is dedicated to the proof of the following result, on the generation of a mesh from a metric.
\begin{prop}
\label{propMeshGen}
There exists $C_0 = C_0(d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $H\in \bH_i$ there exists $\cT \in \bT_{i,C_0}$ which is $C_0$-adapted to $H$.
\item If $d=2$, then for any $H \in \bH_a$ there exists $\cT\in \bT_a$ which is $C_0$-adapted to $\cT$.
\item If $d=2$, then for any $H \in \bH_g$ there exists $\cT\in \bT_g$ which is $C_0$-adapted to $\cT$.\end{enumerate}
\end{prop}

Point {\it i)} is established in the \S\ref{secMeshGenI}, point {\it iii)} in \S \ref{secMeshGenG} an eventually {\it ii)} in \S \ref{secMeshGenA}.\\

\subsection{Isotropic Mesh generation}
\label{secMeshGenI}

\begin{figure}
\centering
\includegraphics[width = 5cm, height = 5cm]{\pathPic/Dessins/THalfSquareJenny.pdf}
\caption{A bidimensional triangulation generated by the isotropic refinement procedure}
\end{figure}

The survey paper \cite{Nochetto} describes a the construction of a hierarchical family of meshes of the rectangular domain 
$
[0,1]^d.
$ 
All these meshes are the refinement of a ``fundamental'' mesh $\cT_0 = \{T_\sigma \sep \sigma \in \Sigma_d\}$, where $\Sigma_d$ stands for the collection of permutations of the set $\{1,\cdots,d\}$, and $T_\sigma$ for the Kuhn simplex
$$
T_\sigma := \{z\in [0,1]^d \sep z_{\sigma(1)} \leq \cdots \leq z_{\sigma(d)}\}.
$$
%A sequence $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $A procedure, guided by the user 
%The ``fundamentalbasic mesh $\cT_0$ of $[0,1]^d$ 
Starting from $\cT_0$, the algorithm described in \cite{Nochetto} produces, guided by the user, a family $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $[0,1]^d$ proceeding as follows. 
Assume that the mesh $\cT_n$ has already been generated.
%Once the mesh $\cT_n$ is defined, the mesh $\cT_{n+1}$ is obtained as follows.
%\begin{enumerate}
%\item (Marking) The user selects
%\item (Refinement)
%\end{enumerate}
%The mesh $\cT_{n+1}$ is produced from $\cT_n$ as follows 
\begin{itemize}
\item (Marking)
The user selects a subset $\cM_n \subset \cT_n$.
\item (Refinement)
The algorithm generates a $2$-refinement $\cT_{n+1}$ of $\cT_n$,  
$$
\cT_{n+1} := \Refine(\cT_n, \cM_n).
$$
which does not contain any of the marked simplices : $\cT_{n+1} \cap \cM_n = \emptyset.$
\end{itemize}
\noindent

The elements of the meshes $(\cT_n)_{n \geq 0}$ have a very specific structure, which main features are described below.
\begin{property}
\label{propertyIso}
Any simplex $T$ produced by this algorithm possesses the following properties.
\begin{enumerate}[a)]
\item (Discrete Volumes) The volume of $T$ has the form
\be
\label{eqVolTG}
|T| = \frac {2^{-g(T)}}{d!},
\ee
where $g(T)\geq 0$ is an integer called the ``generation'' of $T$.
\item
(Finite number of classes)
The simplex 
$$
2^{\frac{g(T)} d} (T-z_T),
$$
which is centered at the origin and has volume $1/d!$, %$\frac 1 {d!}$, 
belongs to a finite family $\gT_0$ of simplices.
%\item
%(Vertices lie on a grid)
%The vertices of $T$ lie on the grid
%$$
%2^{-\left\lceil \frac {g(T)} d\right\rceil} \Z^d
%$$
\end{enumerate}
\end{property}
The survey paper \cite{Nochetto} also contains a result, Proposition 4.1, which establishes that $\cT_{n+1} := \Refine(\cT_n, \cM_n)$ is a \emph{local} refinement of $\cT_n$ in the following sense: for all $T'\in \cT_n \sm \cT_{n+1}$ there exists $T\in \cM_n$ such that 
\be
\label{eqDG}
g(T)\geq g(T') \stext{ and } d(T,T') \leq D \, 2^{-g(T')/d},
\ee
where $D = D(d)$ is a fixed constant and where 
$$
d(T,T') := \min\{|z-z'| \sep z\in T, \, z'\in T'\}.\\
$$

The next lemma shows that this refinement algorithm can be used to produce a conforming isotropic mesh $\cT$ of the unit cube $[0,1]^d$, such that the diameters $\diam(T)$, $T\in \cT$, are specified by a given Lipschitz function.

\begin{lemma}
\label{lemmaSCube}
%There exists $C=C(d)$ such that the following holds.
Let $s:[0,1]^d\to  (0,\sqrt d]$ be a $c$-lipschitz function, where $0<c\leq 1$. Let $(\cT_n)_{n \geq 0}$ be the sequence of meshes produced by the algorithm when the collection $\cM_n\subset \cT_n$ of marked simplices is defined as follows
\be
\label{defMn}
\cM_n := \left\{T\in \cT_n \sep \min_T s < \diam(T)\right\}.
\ee
Then the sequence of meshes stabilizes : there exists $N\geq 0$ such that $\cT_n = \cT_N$ for all $n \geq N$. Furthermore we have for all $T\in \cT_N$ and all $z\in T$
\be
\label{eqEquivCube}
\diam(T) \leq s(z) \leq C_s \diam(T).
\ee
where 
$$
C_s := 2^\frac 1 d \frac {D_+ (1+c) + c D}{D_-}
$$
where $D_+ := \max\{ \diam(T) \sep T \in \gT_0\}$ and $D_- := \min\{ \diam(T) \sep T \in \gT_0\}$.
\end{lemma}

\proof
%%We recall that for each simplex $T$ produced by the algorithm, the simplex $2^{g(T)/d}(T-z_T)$ belongs to a finite family $\gT_0$ of simplices.
%%We define 
%%$$
%%D_0 := \max_{T \in \gT_0} \diam(T),
%%$$
%For any $n\in \N$ and any $T \in \cM_n$ one has 
%\be
%\label{eqMinDiam}
%s_0 := \min_{[0,1]^d} s \leq \min_T s < \diam(T) \leq D_+ 2^{\frac{-g(T)} d},
%\ee
%hence 
%\be
%\label{eqMaxGT}
%g(T)\leq C_1 := d \frac{\ln (D_+/s_0)}{\ln 2}.
%\ee
%We first prove that the sequence $(\cT_n)_{n \geq 0}$ of meshes stabilizes. Let 
%$$
%T^* \in \cT_n = (\cT_n \sm \cT_{n-1}) \cup \cdots \cup (\cT_1 \sm \cT_0) \cup \cT_0.
%$$
%Either $T^* \in \cT_0$, or $T^*$ has a father $T'\in \cT_{n-1}$, and in that case there exists according to \iref{eqDG} 
%$$
%T\in \cM_{n-1} \cup \cdots \cup \cM_0 \cup \cT_0
%$$
%such that $g(T^*) = g(T') +1 \leq g(T)+1 \leq C_1+1$ according to \iref{eqMaxGT}. 
%%Combining this with \iref{eqMaxG} we obtain 
%%$$
%%\sup_{T' \in \cT_n} g(T') \leq C_1.
%%$$
%This leads us to a uniform bound on $\#(\cT_n)$:
%$$
%1 = \sum_{T \in \cT_n} |T'| \geq \#(\cT_n) \min_{T \in \cT_n} |T'| = \#(\cT_n) \min_{T \in \cT_n} \frac{2^{-g(T)}}{d!} \geq \#(\cT_n) \frac{2^{-C_1-1} }{d!},
%$$
%hence $\#(\cT_n) \leq d! 2^{C_1+1}$. Since $\cT_{n+1}$ is a refinement of $\cT_n$ we have either $\#(\cT_{n+1}) \geq \#(\cT_n)+1$ or $\cT_{n+1} = \cT_n$, and in the latter case one has $\cT_n = \cT_{n+1} = \cT_{n+k}$ for all $k \geq 0$ by construction. This case eventually happens since $\#(\cT_n)$ is uniformly bounded, which shows that the sequence $(\cT_n)_{n\geq 0}$ of meshes stabilizes.\\
%
We now turn to the the proof of \iref{eqEquivCube}, and for that purpose we consider $N\geq 0$ such that $\cT_N=\cT_n$ for all $n \geq N$. 
We have for all $T\in \cT_N$
$$
\diam(T) \leq \min_T h,
$$
indeed otherwise $T\in \cM_N$ and therefore $\cT_{N+1}\neq \cT_N$ which is a contradiction.

This establishes the left part of \iref{eqEquivCube}, and we now focus on the right part.
Consider a simplex $T^*\in \cT_N$. If $T^*$ is one of the $d!$ Kuhn simplices $(T_\sigma)_{\sigma\in \Sigma_d}$ that form $\cT_0$, then we have 
$$
\diam(T^*) = \sqrt d \geq  s(z)
$$
for any $z\in T$ since $s$ is uniformly bounded by $\sqrt d$.
Otherwise $T^*$ has a father $T'$, and there exists a simplex $T$ which was selected for bisection such, hence there exists $T\in \cM_{n(T)-1}$ such that \iref{eqDG} holds (* applies to the father of $T$*).
Denoting $d(T,T') := \min\{|z-z'| \sep z\in T,\, z'\in T'\}$, and recalling that $g(T') \leq g(T)$, we obtain 
\begin{eqnarray*}
\min_{T'} s &\leq& \min_T s+ \diam(T) +d(T,T')\\
& \leq & \diam(T) + \diam(T) + D 2^{-g(T')/d}\\
&\leq & 2D_0 2^{-g(T)/d}+D 2^{-g(T')/d}\\
& \leq & (2D_0+D) 2^{-g(T')/d}\\
& \leq & C \diam(T'),
\end{eqnarray*}
where 
$$
C := \frac{2D_0+D}{\min \{\diam(T)\sep T \in \gT_0\}},
$$
which concludes the proof of this proposition.
\sq

The rest of this section is devoted to the proof the point {\it i)} of Proposition \ref{propMeshGen}.
We thus consider a metric $H\in \bH_i$, and we recall there exists a Lipschitz function $s: \R^d \to \R_+^*$ such that for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2}.
$$
For each $n\geq 0$ we define a function $s_n : [0,1]^d \to \R_+^*$, which is clearly Lipschitz, as follows
\be
\label{defSn}
s_n(z) := 2^{-n} s(2^n (z-z_0))
\ee
where $z_0 = (1/2, \cdots , 1/2)$ is the barycenter of the cube $[0,1]^d$.
%The function $s_n$ is clearly Lipschitz, and 
For all $z\in [0,1]^d$ and all $n \geq 0$ we have 
$$
s_n(z) \leq s_n(z_0) + |z-z_0| \leq 2^{-n} s(0) + \frac {\sqrt d} 2.
$$
The function $s_n$ is therefore uniformly bounded by $\sqrt d$ on $[0,1]^d$ when $n$ is sufficiently large.
We denote by $\cT^n$ the mesh of the cube $[0,1]^d$ described by Lemma \ref{lemmaSCube} for the function $s_n$. We thus have %for all $T\in \cT^n$
\be
\label{eqDiamSn}
\diam(T) \leq \min_T s_n \leq C \diam(T) \stext{ for all } T \in \cT^n,
\ee
where $C=C(d)$ is the constant from Lemma \ref{lemmaSCube}.
We denote by $\cT_n$ the mesh of the cube $[-2^{n-1}, 2^{n-1}]^d$ obtained by translating the mesh $\cT^n$ by $-z_0$ and dilating it by $2^n$. In mathematical terms: % In condensed notations
$$
\cT_n := \{2^n(T-z_0)\sep T \in \cT^n\}.
$$
%$$
%\cT_n := 2^n (\cT^n -z_0).
%$$
In view of \iref{defSn} and \iref{eqDiamSn} we thus have 
\be
\label{eqMinSDiamT}
\diam(T) \leq \min_T s \leq C \diam(T) \stext{ for all } T \in \cT_n,
\ee
which implies for any $z\in T$
$$
\diam(T) \leq \min_T s \leq s(z) \leq \min_T s + \diam(T) \leq (C+1) \diam(T).
$$
We denote by $C_0$ the smallest constant such that for all $T$ in the finite set $\gT_0$ one has 
$$
 \frac{C_0^{-2} \Id}{\diam(T)^2} \leq \cH_T \leq \frac{C_0^2\Id}{(C+1)^2\diam(T)^2 },
$$
and we thus obtain for all $T\in \cT_n$ and all $z\in T$
\be
\label{eqHHTIso}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Unfortunately the mesh $\cT_n$ does not cover $\R^d$ but only the cube $[-2^{n-1}, 2^{n-1}]$. 
The next lemma allows to extract a global mesh $\cT$ of the infinite domain $\R^d$ from the sequence of meshes $(\cT_n)_{n\geq 0}$.

\begin{lemma}
Let $(\Omega_n)_{n \geq 0}$ be an increasing sequence of polygonal domains of $\R^d$, which exhausts $\R^d$ in the following sense:
$$
\bigcup_{n \geq 0} \Omega_n = \R^d \stext{ and } \Omega_n \subset \Omega_{n+1} \text{ for all } n\geq 0.
$$
Let $H \in \bH_g$, let $(\cT_n)_{n \geq 0}$ be a sequence of conforming simplicial meshes of the domains $\Omega_n$, and assume that for all $n \geq 0$, all $T\in \cT_n$ and all $z\in T$ one has 
\be
\label{eqHHTConv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Then there exists a mesh $\cT\in \bT$ such that 
$
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
$
for all $T\in \cT$ and all $z\in T$.
\end{lemma}

\proof
The heuristic idea of this proof is to ``extract a converging subsequence'' from the sequence $(\cT_n)_{n \geq 0}$ of meshes. Unfortunately meshes are discrete objects of combinatorial nature, and the convergence of meshes has no meaning a priori. We therefore use Lipschitz functions as an intermediate object, for which convergence is well defined and which benefit of a compactness property.\\

We associate a function $\phi_T : \R^d \to \R$ to each simplex $T$, which is defined as follows. The function $\phi_T$ is supported on $T$, and for all $z\in T$ we have in terms of the barycentric coordinates $\lambda_v(z)$ of $z$ with respect to the vertices $v\in V$ of $T$:
%To each simplex $T$ of vertices $V$, and barycentric coordinates $(\lambda_v)_{v\in V}$ we associate the function 
$$
\phi_T(z) := \min_{v\in V} \lambda_v(z).
$$
%The maximum of this function has value $1/d$ and is attained at the barycenter $z_T$ of $T$. Furthermore for each $z\in T$ and each $0\leq r \leq 1$ one easily checks that 
%$$
%\phi_T(z+r(z-z_T)) \geq r/d.
%$$
According to Lemma \ref{lemmaNormLambda}, we have for any $z,z'\in T$ and any $v\in V$
$$
|\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T},
$$
hence 
\be
\label{eqPhiLip}
|\phi_T(z) - \phi_T(z')| \leq \max_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T}.
\ee

For all $n \geq 0$ we define a function $\phi_n$ on $\R^d$ as follows
$$
\phi_n := \sum_{T \in \cT_n} \phi_T.
$$
It follows from \iref{eqHHTConv} and \iref{eqPhiLip} that for all $z\in \R^d$
$$
\dil_z(\phi_n\sep d_H) \leq C_0,
$$
hence $\phi_n : (\R^d,d_H) \to \R$ is $C_0$-Lipschitz according to Proposition \ref{propDilLoc}. Since the space $(\R^d, d_H)$ is locally compact, due to Proposition \ref{propEuclidRiemann}, Ascoli's compactness theorem states that there exists %a the sequence $(\phi_n)_{n \geq 0}$ of $C_0$-Lipschitz functions admits a 
subsequence $(\phi_{n_k})_{k \geq 0}$ which converges uniformly on all compact sets of $\R^d$ to a $C_0$-Lipschitz function $\phi$. 

We therefore assume, up to such an extraction, that 
$
\phi_n \to \phi
$
uniformly on all compact sets of $\R^d$.
We denote by $\cT$ the collection of closures of connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$:
$$
\cT := \left\{ \overline E \sep E \text{ is a connected component of } \{z\in \R^d \sep \phi(z)>0\} \right\}.
$$
For each $z\in \R^d$ and each $n \geq 0$, we denote by $T_n(z)$ the element of $\cT_n$ containing $z$ in its interior if it exists, and $T_n(z) = \emptyset$ otherwise.
If $\phi(z)>0$, then $T_n(z)\neq \emptyset$ for all $n$ sufficiently large, and one easily checks that 
\be
\label{eqTTnz}
T_n(z)\text{ converges in Hausdorff distance to the element }T(z)\in \cT
\ee
 containing $z$. Hence $\cT$ is a collection of simplices, and the convergence $T_n(z)\to T(z)$ in haussdorf distance, combined with the hypothesis $C_0^{-2} H(z) \leq T_n(z) \leq C_0^2 H(z)$, implies that  
\be
\label{eqHHTConv2}
C_0^{-2} H(z) \leq T(z) \leq C_0^2 H(z).
\ee
In order to conclude this proof we need to show that the collection $\cT$ of simplices is a conforming mesh of $\R^d$. We thus have to check the hypotheses of Definition \ref{defSimplMesh}.
The interiors $\interior(T)$, $T\in \cT$ are pairwise disjoint since they are the connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$.
We claim furthermore that $\cT$ covers $\R^d$. Indeed let $z\in \R^d$be arbitrary and for all $n$ let $T_n\in \cT_n$ be such that $z\in T_n$. Since $C_0^{-2} H(z) \leq \cH_{T_n}\leq C_0^2 H(z)$ there exists a subsequence $T_{n_k}$ which converges in the Haussdorf distance to a simplex $T$ containing $z$. We clearly have $T\in \cT$ which establishes as announced that $\cT$ covers $\R^d$.
The fact that $\cT$ is locally finite easily follows from \iref{eqHHTConv2}.\\


We now turn to the proof of the conformity property, and for that purpose we consider an arbitrary Lipschitz function $f : (\R^d, d_H) \to \R$ with compact support. 
Let $T$ be a simplex such that $C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)$. We have for any vertex $v$ of $T$
$$
|f(v) - f(z_T)| \leq d_H(z_T,v) \leq C_0 \|z_T - v\|_{\cH_T} = C_0.
$$
Denoting by $V$ the collection of vertices of $T$ we thus obtain for any $z,z'\in T$
$$
\interp_T^1 f(z) - \interp_T^1 f(z') = \sum_{v\in V} (\lambda_v(z) - \lambda_v(z')) (f(v) - f(z_T)) 
$$
hence using Lemma \ref{lemmaNormLambda}
$$
|\interp_T^1 f(z) - \interp_T^1 f(z')| \leq C_0 \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq C_0 \sqrt{(d+1)  \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|^2} = C_0 \sqrt d \|z-z'\|_{\cH_T}.
$$
Let $n_0 \geq 0$ be such that $\supp(f)\subset \Omega_{n_0}$. The last inequality implies that 
$$
\dil_z(\interp_{\cT_n}^1 f \sep d_H)\leq C_0^2 \sqrt d
$$
for any $z\in \R^d$ and all $n \geq n_0$, which shows according to Proposition \ref{propDilLoc} that $\interp_{\cT_n}^1 f : (\R^d, d_H) \to \R$ is $C_0^2\sqrt d$-Lipschitz.

We define 
$
D := \cup_{T \in \cT} \interior(T),
$
and we denote by $\interp_T^1 f : D \to \R$ the function which coincides with $\interp_T^1 f$ on the \emph{interior} of each $T\in \cT$. % (and which is possibly discontinuous at the interfaces between the simplices $T\in \cT$). 
For any $z\in D$ we obtain using \iref{eqTTnz} that $\interp_{\cT_n}^1 f(z) \to \interp_\cT^1 f(z)$, hence for any $z,z'\in D$
$$
|\interp_\cT^1 f(z) - \interp_\cT^1 f(z')| = \lim_{n \to \infty} |\interp_{\cT_n}^1 f(z)-\interp_{\cT_n}^1 f(z')| \leq \sqrt d C_0^2 \, d_H(z,z').
$$
The interpolant $\interp_T^1 f : D \to \R$ therefore extends to a $\sqrt d C_0^2$-Lipschitz function $\interp_T^1 f : (\R^d, d_H) \to \R$. It easily follows that $\interp_\cT^1 f$ is continuous for any compactly supported $C^1$ function $f$. This property characterizes conforming meshes, hence $\cT\in \bT$ which concludes the proof.
\sq



\begin{corollary}(Bidimensional triangulations)
\label{corolBidimIso}
Assume that the dimension is $d=2$. There exists $c>0$ such that the following holds: il $s: \R^2 \to \R_+^*$ is $c$-Lipschitz, then there exist a mesh $\cT$ of $\R^2$ built of half squares, and such that for all $T\in \cT$ and $z\in T$
$$
s(z)/2 \leq \diam(T) \leq s(z).
$$
\end{corollary}

\proof
When the dimension is $d=2$, the collection $\gT_0$ of triangles contains only half squares, of area $1/2$.
We thus have
$$
\diam(T) = 2^{\frac{1-g(T)} 2}
$$

We consider the triangulation $\cT$ of $[0,1]^2$ created by the procedure described in Lemma \ref{lemmaSCube}.
For any $T \in \cT_0$ we have $\diam(T) \leq \min_T s$ by construction.

Furthermore for any $T'\in \cT$, $T'$ is either one of the two initial half squares, hence $\diam(T') \geq \sqrt 2 \geq \lambda(z)$ for any $z\in T'$, or there exists a simplex $T$ such that \iref{eqDG} holds.

We thus obtain for any $z\in \cT'$
$$
s(z) \leq \min_T s + c(\diam(T)+ d(T,T'))  
\leq \diam(T)(1+ c)+ c D 2^{-g(T')/d} \leq   
$$

\sq


\subsection{Graded mesh generation}
\label{secMeshGenG}

We prove in this section a result of bi-dimensional mesh generation, Theorem \ref{thEquiMesh}, which implies Point (iii) of Proposition \ref{propMeshGen}. The key ingredients of this section come from the paper \cite{Shew}.
We assume throughout this section that the dimension is $d=2$.

For that purpose we introduce the notion of equispaced points in an abstract metric space.
 Let $(X,d_X)$ be a metric space and let $\delta>0$, we say that a subset $\cV \subset X$ is $\delta$-equispaced if the following holds.
\begin{enumerate}[a)]
\item (Covering) The distance from an arbitrary point $x\in X$ to $\cV$ is bounded by $1$ : for all $x\in X$
\be
\label{eqCover}
d_X(x, \cV) := \inf\{d_X(x,v) \sep v \in \cV\} \leq 1.
\ee
\item (Separation) The pairwise distances between the points of $\cV$ are larger than $\delta$ : for all $v, v'\in \cV$ such that $v \neq v'$
\be
\label{eqSep}
d_X(v,v') \geq \delta.
\ee
\end{enumerate}

The next lemma establishes the existence of such a set under certain assumptions. \begin{lemma}
\label{lemmaEquiSpaced}
Let $(X,d_X)$ be a metric space in which the closed balls $B'(x,r) := \{y\in X \sep d_X(x,y) \leq r\}$ are compact for all $x\in X$ and $r\geq 0$. 
Let $\cV_0$ subset $X$ be such that $d_X(v,v') \geq 1$ for all $v,v'\in \cV_0$ such that $v\neq v'$. Then there exists a $1$-equispaced set $\cV$ of the metric space $(X,d_X)$, containing $\cV_0$.
\end{lemma}

\proof
We may assume that $\cV_0 \neq \emptyset$, up to including an arbitrary point of $X$, and we choose an  arbitrary  $x_0\in \cV_0$.
We define inductively a sequence $(x_n)_{0 \leq n< N}$ of points and $(\cV_n)_{0 \leq n < N}$ of subsets of $X$, where $N\in \N \cup \{\infty\}$ is specified later, proceeding as follows.
Assuming that $\cV_n$ is already defined we consider the closer set 
\be
\label{eqDefXn}
X_n :=  
\{x\in X \sep d_X(x,\cV_n) \geq 1\}.
\ee
If the set $X_n$ is empty, then the sequence ends and we define $N := n+1$. Otherwise we choose $x_{n+1}$ arbitrarily among the minimisers of $d_X(x,x_0)$ on $X^n$:
\be
\label{defxn}
x_{n+1} \in \underset {x\in X_n} \argmin \,d_X(x,x_0),
\ee
and we define $\cV_{n+1} := \cV_n \cup\{x_{n+1}\}$.
Such a minimizer exists since $X_n$ is closed and since the closed balls in $X$ are compact.
%$$
%X^n \cap \overline B\left(x_0, \ 1+ \inf_{x\in X^n} d_X(x_0, x)\right)
%$$
%is compact.
We define $N := \infty$ none of the sets $(X_n)_{n \geq 0}$ is empty. %if the sequence $(x_n)$ is infinite.

We define $\cV := \cup_{0 \leq n <N} \cV_n$.
%We denote by $X_0 := \{x_n \sep 0\leq n<N\}$ the collection of all points of this finite or countable sequence.
%
%We define $N := \infty$ if the sequence $x_0, x_1, \cdots$ is infinite, and we denote by $X_0$ the collection of all points of this finite or countable sequence,
%$$
%X_0 := \{x_n \sep 0 \leq n < N\}.
%$$ 
%%as the collection of all points $x_0, x_1, \cdots$ of this finite or countable sequence.
%, which clearly is finite or countable.
By construction, we thus have $d_X(v, v') \geq 1$ for all $v,v'\in \cV$
which establishes the separation property \iref{eqSep}. %, and shows that $\cV$ is a discrete set.

We now assume for contradiction that the covering property \iref{eqCover} does not hold which implies that $N= \infty$. We choose a point $x_*\in X$ such that $d_X(x_*, \cV)>1$, and therefore $x_*\in X_n$ for all $n \geq 0$. The definition \iref{defxn} of $x_{n+1}$ implies that $d_X(x_0, x_n) \leq d_X(x_0, x_*)$ for all $n \geq 0$, hence the discrete collection of points
$
\{x_n \sep n \geq 0\}
$
in included in the closed ball $\{x\in X \sep d_X(x_0, x) \leq d_X(x_0, x_*)\}$ which is compact.
The sequence $(x_n)_{n \geq 0}$ therefore admits a converging subsequence, but this contradict the fact that the pairwise distances between these points are larger than $1$, which concludes the proof of this proposition.
\sq


%The next lemma gives a simple (from a theoretical point of view) procedure which produces a point set equidistributed with respect to a metric.
%\begin{lemma}
%Let $H\in \bH$ and let $(p_n)_{n\geq 0}$ be a sequence of points obtained by choosing $p_0 = 0$ and then iteratively choosing $p_{n+1}$ among the minimizers of
%\be
%\label{defpn}
%\min\{\|p\| \sep d_H(p, \{p_0,\cdots , p_n\} \geq 1)
%\ee
%
%Then the point set $\cP := \{p_n \sep n \geq 0\}$ is $1$-equidistributed with respect to $H$.
%\end{lemma}
%
%\proof
%The separation holds by construction. It implies in particular that for any $M \geq 1$, $\cP\cap B(0,M)$ is finite. 
%
%%Since $H$ is continuous and positive definite, for each $M$ the set $\{n\geq 0 \sep \|p_n\| \leq M\}$ is finite.
%Indeed let $\Lambda^2 := \max \{\|H(z)\| \sep \|z\| \leq M\}$.
%The balls $B(p, \Lambda/2)$, $p\in \cP\cap B(M)$ are pairwise disjoint. It follows from a volume argument that $\cP\cap B(M)$ is finite.
%
%Let us assume by contradiction that there exists $z\in \R^2$ such that $d(z, \cP)>1$. Then for $n$ large enough we have $\|z\| < \| p_{n+1}\|$ which is incompatible with the construction of $p_{n+1}$ as a minimizer of \iref{defpn}.
%\sq




We consider a fixed metric $H \in \bH$. For any $x,y\in \R^2$ we define 
$$
d_x(y) := \|x-y\|_{H(x)}.
$$
We also consider a fixed discrete collection of vertices, or ``sites'', $\cV \subset \R^2$, and we define the anisotropic Voronoi cell of a site $v\in V$ as follows 
\be
\label{defVorv}
\Vor(v) := \{z\in \R^2 \sep d_v(z) \leq d_w(z) \text{ for all } w \in V\}.
\ee
The anisotropic Voronoi cell $\Vor(v)$ is thus the collection of points $z$ which are \emph{closer to the vertex $v$ than to any other site}.
The classical (isotropic) Voronoi is obtained by choosing $H = \Id$.
We refer to the paper \cite{Shew} Figure 3 for an illustration of the anisotropic Voronoi diagram $\{\Vor(v) \sep v\in \cV\}$ associated to a point set.

For each $z\in \R^2$ we define $\cV_z$ the collection of vertices which contain $z$ in their Voronoi region:
$$
\cV_z := \{v \in \cV \sep z \in \Vor(v)\}.
$$
The geometric dual of the Voronoi diagram is the graph $\cG(\cV,H)$ defined as follows:
\be
\label{defGVH}
\cG(\cV,H) := \{[v,v'] \sep \text{there exists } z\in \R^2 \text{ such that } V_z = \{v,v'\}\}.
\ee

%We define a collection $\cT_0(V,H)$ of convex sets attached to the metric $H$ and to the collection $V$ of sites
%$$
%\cT_0(V,H) := \{\Cvx(V_z) \sep z \in \R^2 \text{ and } \#(V_z) \geq 3\}.
%$$
The next theorem establishes that $\cG(\cV,H)$ is, under certain conditions on the metric $H$ and the set $\cV$, the graph of a triangulation adapted to $H$.

\begin{theorem}
\label{thEquiMesh}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta)\geq 1$ such that the following holds.
Let $H$ be a metric such that $c^2 H\in \bH_g$, and let $\cV$ be a $\delta$-equispaced subset of $(\R^2, d_H)$.
Then the $\cG(\cV,H)$ is a planar graph which defines a partition of $\R^2$ into strictly convex polygons. Arbitrarily triangulating each polygon yields a triangulation $\cT$ which is $C$-adapted to $H$, called an anisotropic Delaunay triangulation. Furthermore if $\cV$ is in general position then $\cG(\cV,H)$ is already the graph of a triangulation.
\end{theorem}

This theorem implies point iii) of Proposition \ref{propMeshGen}, proceeding as follows: 
for any $H_0 \in \bH_g$, we construct using lemma \ref{lemmaEquiSpaced} a subset $\cV$ of the metric space $(\R^2, d_{H_0}/c(1))$ which is $1$-equispaced. According to Theorem \ref{thEquiMesh} there exists a triangulation $\cT$, of vertices $\cV$, which is $C(1)$-adapted to the metric $H := H_0/c(1)^2$, and therefore $C(1)/c(1)$-adapted to $H_0$.\\


We now turn to the proof of Theorem \ref{thEquiMesh}, which is based on three theorems presented in \cite{Shew}. 
%These theorems are based on a property that needs to be 
For that purpose we recall some definitions of this paper. %introduce the following definitions.
\begin{definition}
\label{defWedge}
%The wedge of $v,v'$ is 
\begin{itemize}
\item (Wedge of two points)
We define the wedge $\wed(v,w)$ of two distinct sites $v,w\in V$ as follows
$$
\wed(v,w) := \{z\in \R^2 \sep (z-v)^\trans H(v) (w-v) >0 \text{ and } (z-w)^\trans H(w) (v-w) >0\}
$$ 
\item (Wedge property)
We say that the Voronoi diagram of $V$ is wedged if for any two distinct $v,w \in V$ we have 
$$
\Vor(v) \cap \Vor(w) \subset \wed(v,w).
$$
\end{itemize}
\end{definition}

The wedge property expresses that the collection $\Vor(v) \cap \Vor(w)$ of points $q$ shared by the Voronoi regions of the sites $v$ and $w$ lie in a cone defined by two linear inequalities.
We refer to \cite{Shew} Figure 4 for an illustration of the wedge of two sites.

The next proposition, which is partly is based on Lemma 5 from \cite{Shew},
 shows that the wedge property is automatically satisfied in our context.
For any metric $H$ and any constant $c>0$ such that $c^2H\in \bH_g$, it easily follows from Proposition \ref{propEuclidRiemann} that for all $x,y\in \R^2$
\be
\label{eqDHLog}
\ln (1+ c\, d_x(y)) \leq c \, d_H(x,y) \leq - \ln(1- c\, d_x(y)), 
\ee
which is equivalent to 
\be
\label{eqDHExp}
1-\exp(-c\, d_H(x,y)) \leq c \, d_x(y) \leq \exp(c \, d_H(x,y))-1.
\ee

\begin{lemma}
\label{lemmaDiamVor}
If $c^2 H\in \bH_g$ %and $\cV$ is $\delta$-equispaced, 
then
for any $v\in \cV$ and any $q\in \Vor(v)$ we have 
\be
\label{eqDiamVor}
\|q-v\|_{H(v)} \leq r_0(c) := (e^c-1)/c.
\ee
If $v,w \in \cV$ satisfy $\Vor(v) \cap \Vor(w) \neq \emptyset$, then 
\be
\label{eqVordvw}
%\delta \leq 
d_H(v,w) \leq r_1(c) := -2\ln(2-e^c)/c.
\ee
Note that $r_0(c) \to 1$ and $r_1(c) \to 2$ as $c\to 0$. Note also that $d_H(v,w)\geq \delta$ if $\cV$ is $\delta$-equispaced.
\end{lemma}

\proof
For any $q\in \cV$ there exists $v_* \in \cV$ such that 
$
d_H(q,v_*) \leq 1,
$
and therefore 
$$
\|q-v_*\|_{H(v_*)} \leq r_0(c) := (e^c-1)/c,
$$
which implies \iref{eqDiamVor} using the definition \iref{defVorv} of the Voronoi diagram.
We thus turn to the proof of \iref{eqVordvw} and for that purpose we consider a point $q\in \Vor (v)\cap\Vor(w)$. We thus have
$
\max\{\|q-v\|_{H(v)} , \|q-w\|_{H(w)} \}\leq  v_c%-\ln(1-c v_c)/c
$
hence
$$
d_H(v,w) \leq r_1(c) :=-2\ln(1-c r_0(c))/c,
$$
which concludes the proof.
\sq

\begin{prop}
\label{propWedge}
For each $\delta$ there exists $c=c(\delta)>0$ such that the following holds.\\
If a metric $H$ satisfies $c^2H\in \bH_g$ and if $\cV$ is a $\delta$-equispaced subset of $(\R^2,d_H)$, then the wedge property is satisfied.
\end{prop}

\proof
We assume for contradiction that there exists two distinct vertices $v,w \in V$, and a point $q\in \Vor(V) \cap \Vor(W)$ such that $z\notin \wed(v,w)$. We may assume, up to exchanging the roles of $v$ and $w$, that 
$$
(q-w)^\trans H(w) (v-w) \leq 0.
$$
Defining the ``relative distortion''
$
\tau := \exp d_\times (H(v), H(w))
$
we obtain using Lemma 5 from \cite{Shew} %(*$q$ instead of $z$??*)
\be
\label{eqShewWedge}
 d_w(v) \leq d_w(q) \sqrt{\tau^2-1}.
\ee
We now estimate the quantities $d_w(v)$, $d_w(q)$ and $\tau$ appearing in this estimate, in order to obtain a contradiction when $c$ is sufficiently small.

%Since the set $V$ is $C_0$-equispaced, there exists $u\in V$ such that $d_H(u,q) \leq C_0$. Recalling that $z\in \Vor(v)\cap \Vor(w)$ we thus obtain using \iref{eqDHExp}
%\be
%\label{eqDiamVor}
%d_v(q) = d_w(q) \leq d_u(q) \leq \frac{\exp(c \, d_H(u,q))-1} c \leq r_0(c) := \frac{\exp(c C_0)-1} c,
%\ee
%and therefore using \iref{eqDHLog} 
%\be
%\label{eqVordvw}
%d_H(v,w) \leq d_H(v,q)+ d_H(q,w) \leq r_1(c) := \frac {-2\ln (1- c r_0(c))}  c,% \frac 1 {1-f(c)}.
%\ee
%hence 
We have 
\be
\label{eqTauWedge}
\ln \tau = d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
\ee
Since $\cV$ is $\delta$-equispaced we have 
$
d_H(v,w) \geq \delta
$
and therefore 
\be
\label{eqdvwWedge}
c \,d_w(v) \geq 1-\exp(-c d_H(v,w)) \geq 1-\exp(-c\delta)
\ee
Injecting \iref{eqDiamVor}, \iref{eqTauWedge} and \iref{eqdvwWedge} in \iref{eqShewWedge} we obtain
\be
\label{eqFinalWedge}
\frac{1-\exp(-c\delta )} c \leq \frac{\exp(c)-1} c \sqrt{\exp(2c r_1(c))-1}.
\ee
The left hand side tends to $\delta$ as $c\to 0$, while the right hand side tends to $0$. We thus obtain a contradiction when $c$ is sufficiently small which concludes the proof of this proposition.
\sq

\begin{theorem}[Dual triangulation theorem. Labelle, Shewchuck, \cite{Shew}]
\label{thShew}
If the Voronoi diagram of the point set $\cV \subset \R^2$ is wedged, then the geometric dual of this diagram is a polygonalization of $\R^2$ with strictly convex polygons and is a triangulation $\cT$ if $\cV$ is in general position.
\end{theorem}

Under the hypotheses of this theorem the vertices $v_1, \cdots, v_k$ of a polygon in the dual Voronoi diagram satisfy by construction $\Vor(v_1)\cap \cdots \cap \Vor(v_k) \neq \emptyset$, and therefore the vertices $v_1, v_2, v_3$ of a triangle $T\in \cT$ satisfy $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$.

The next theorem, originally stated in \cite{Shew} as Corollary 10 to Theorem 9 of the same paper, allows to control the angles of a triangle in the anisotropic Delaunay triangulation.

\begin{theorem}[Labelle, Shewchuk, \cite{Shew}]
\label{thAngle}
Let $v_1,v_2,v_3\in \cV$ and let $q\in \Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)$. Let 
$$
r = d_{v_1}(q) = d_{v_2}(q) = d_{v_3}(q) \stext{ and }
l = \min\{d_{v_i}(v_j) \sep i,j \in \{1,2,3\}, i \neq j\}.
$$ 
Define $\beta := \max\{r/l,\, 1/\sqrt 2\}$, %and %$\gamma\in [1,\infty)$ by 
%Let $1\leq \gamma \leq \sqrt 2$ and $\beta \geq \frac 1 {\sqrt 2}$ satisfy
$$
\gamma := \exp \max \{d_\times (H(v_i), H(v_j)) \sep i,j \in \{1,2,3\}, i \neq j\},
$$
and
\be
\label{defChi}
\chi := \frac 1 {2 \beta} - \frac{(\gamma^2-1)\beta} 2.
\ee
If $\gamma \leq \sqrt 2$ and $\chi>0$ then any angle $\theta$ of the triangle of vertices $(\sqrt{H(v_1)} v_k)_{1 \leq k \leq 3}$ satisfies
$$
\arcsin ( \chi/ \gamma^2) \leq \theta \leq 2 \arccos(\chi/\gamma^2).
$$
%where $S = H(v_1)^{\frac 1 2}$.
\end{theorem}

\begin{corollary}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta) \geq 1$ such that the following holds.
If $\cV$ is $\delta$-equispaced, if $c^2H\in \bH_g$ and if $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$, then denoting by $T$ the triangle of vertices $v_1,v_2,v_3$ we have for all $z\in T$
$$
C^{-2} H(z) \leq \cH(z) \leq C^2 H(z).
$$
\end{corollary}
\proof
We use \iref{eqDHExp} and \iref{eqDHLog} and the fact that $V$ is $\delta$-equispaced to obtain explicit bounds on the quantities $r$, $l$, $\beta$, $\gamma$ and $\chi$ appearing in Theorem \ref{thAngle}.
It follows from Lemma \ref{lemmaDiamVor} that 
$$
r\leq r_0(c) \stext{ and } \delta \leq d_H(v_i,v_j) \leq r_1(c).
$$
Therefore 
$$
l := \min_{i\neq j} d_{v_i}(v_j)\geq %\min_{i\neq j} \frac{1-\exp(-c d_H(v_i,v_j))} c \geq  
r_2(c) := (1-\exp(-c\delta))/ c,
$$
and 
$$
L := \max_{i\neq j} d_{v_i}(v_j) \leq (\exp(c r_1(c))-1)/c
$$
and 
$$
\gamma \leq \max_{i\neq j} \exp(c \,d_H(v_i,v_j)) \leq \exp(c \,r_1(c)).
$$
In particular 
$
\beta \leq r_3(c) := \min\{r_0(c)/r_2(c),\, 1/\sqrt 2\}. % = \frac{\exp(cC_0)-1}{1-\exp(-2 cC_0^{-1})},
$
Injecting this into \iref{defChi} yields an explicit lower estimate 
$$
\chi\geq r_4(c) := \frac 1 {2r_3(c)} - \frac{ (\exp(2cr_1(c))-1) r_3(c)} 2,
$$ 
and $\chi/\gamma^2\geq r_5(c) := r_4(c) \exp(-2cr_1(c))$.

For a fixed $\delta$ we obtain as $c\to 0$ the limits $r_0(c) \to 1$, $r_1(c)\to 2 $, $r_2(c) \to \delta$, $r_3(c) \to \min\{\delta, 1/\sqrt 2\}$ and $r_4(c) \to 1/(2\min\{\delta, 1/\sqrt 2\})$ and $r_5(c)$ as the same limit.

%We assume without loss of generality that $\delta \geq 1/\sqrt 2$ and we thus obtain $r_3(c) \to \delta$, 
%$r_4(c) \to 1/C_0^2$ and $r_5(c) \to 1/C_0^2$. 
We may therefore choose $c$ sufficiently small in such way that 
$$
l \geq l_0 := \delta/2, \ L  \leq L_0 := 4 \text{ and }\chi/\gamma^2 \geq \Chi_0 := 1/(4\min\{\delta, 1/\sqrt 2\}).
$$
We denote by $T$ the triangle of vertices $v_1, v_2, v_3$. The length of any edge of $T' := \sqrt{H(v_1)}(T)$ is bounded above by $L_0$ and below by $l_0$ respectively, and the angles of $T'$ satisfy $\arcsin (\Chi_0) \leq \theta \leq 2 \arccos(\Chi_0)$. The collection of triangles centered at the origin which satisfy these inequalities is compact, thus there exists a constant $C_1 = C_1(C_0)$ such that 
$$
C_1^{-2} \Id \leq \cH_{T'} \leq C_1^2 \Id,
$$
hence $C_1^{-2} H(v_1) \leq \cH_{T'} \leq C_1^2 H(v_1)$. For any $z\in T$ we obtain, remarking that $\|z-v_1\|_{\cH_T} \leq 2$ for all $z\in T$ and using \iref{eqLocalNorm}, 
$$
C_1^{-2} (1-2cC_1)^2 H(z) \leq \cH_{T'} \leq C_1^2(1-2cC_1)^{-2} H(z)
$$
which concludes the proof of this proposition, with $C = C_1(1-2cC_1)^{-1}$.
\sq

\subsection{Acute mesh generation}
\label{secMeshGenA}

This section is devoted to the proof of Point ii) of Proposition \ref{propMeshGen}, and we thus assume that the dimension is $d=2$. This proof combines the constructions of isotropic and graded meshes presented in \S\ref{secMeshGenI} and \S\ref{secMeshGenI} to produce a quasi-acute mesh.


We consider a metric $H$ such that $c^2 H\in \bH_a$, where $c$ is a constant specified later, such that $0<c\leq 1$. The constant $c$ needs to be \emph{sufficiently small} in the following sense :  some of the arguments presented in this proof require that $c\leq c_i$, where $c_0, \cdots c_k$ are a finite number of absolute numerical constants (independent of the quasi-acute metric $H$ in particular). We mention these requirements when they appear and we assume that they hold.\\

We define two functions $\lambda, \mu : \R^2 \to \R$ as follows : for all $z\in \R^2$
$$
\lambda(z) := \|H(z)^{-\frac 1 2}\| \stext{ and } \mu(z) = \|H(z)\|^{-\frac 1 2}.
$$
Note that $\lambda(z) \geq \mu(z)$.
The functions $\lambda, \mu$ are $c$-Lipschitz according to Corollary \ref{corolLipNorm} : for all $z,z'\in \R^d$
$$
|\lambda(z)-\lambda(z')| \leq c|z-z'| \text{ and } |\mu(z) - \mu(z') | \leq c|z-z'|.
$$
%We define the metric 
%$$
%H_0:= \|H^{-1}\|^{-1} \Id = \Id/\lambda^2,
%$$
%and observe that $cH_0 \in \bH_i$ since $\lambda$ is $c$-Lipschitz, which implies that $H_0 \in \bH_i$.
%Since $H \in \bH_i$, it follows from Point i) of Proposition \ref{propMeshGen}, that there exists an absolute numerical constant $\delta_0>0$ (independent of $H$) and a mesh $\cT_0 \in \bT$ such that for all $T\in \cT_0$ and all $z\in T$
If $c$ is sufficiently small, then there exists according to Corollary \ref{corolBidimIso} a mesh $\cT_0$ built of half squares and such that for all $T\in \cT_0$ and $z\in \cT$
\be
\label{ratioDiamLambda}
\frac 2 3  \lambda(z) \leq \diam(T)\leq \lambda(z). 
\ee
%(*this or $1/2$?? what is the simplest?*)
%Furthermore we assume that the triangles $T\in \cT_0$ are half squares, which is the case for the construction of such a triangulation presented in \S \ref{secMeshGenI}. 
We denote by $\cV_0$ the collection of vertices of $\cT_0$.\\

For each $u,u'\in \R^2 \sm\{0\}$ we define the (unoriented) angle
$$
\varangle (u,u') := \arccos \left(\frac{\<u,u'\>}{|u| |u'|}\right) \in [0,\cPi].
$$
For any $u,u'\in\bbS$, the angle $\varangle (u,u')$ coincides with the distance $d_\bbS(u,u')$ used in \S\ref{secEigen}. %Note that the angle coincides with the distance on 
For any triangle $T\in \cT_0$ of vertices $v,w,w'$ we thus have $\varangle(w-v,w'-v) \in \{\cPi/4, \cPi/2\}$. For each $u\in \R^2$ we denote by $u^\perp$ the vector obtained by rotating the vector $u$ by $\cPi/2$ is direct trigonometric sense.\\

We say that two vertices $v,w\in \cV_0$ are neighbors in $\cT_0$ if they belong to a common triangle $T\in \cT_0$.
In that case we have %Let $v,w$ be two vertices of a triangle $T\in \cT_0$, then 
\be
\label{edgeLambda}
\frac{\lambda(z)\sqrt 2}3 \leq \frac{\diam(T)}{\sqrt 2}\leq |v-w| \leq \diam(T)\leq \lambda(z)
\ee
Furthermore for any fixed $v\in \cV_0$ any vertex $w\in \cV_0$ which minimizes $|v-w|$ is clearly a neighbor of $v$ in $\cT_0$. It follows that for any $v,w\in \cV_0$,
\be
\label{pairwiseV0}
\lambda(z) \frac {\sqrt 2} 3 \leq |v-w| 
\ee
Note also that for any $T,T'\in \cT_0$ such that $T \cap T' \neq \emptyset$ it follows from \iref{ratioDiamLambda} that 
\be
\label{eqDiamRatio}
\diam(T)/\sqrt 2 \leq \diam(T') \leq \sqrt 2 \diam(T),
\ee
and for any two neighbors $w,w'$ of a vertex $v\in \cV_0$ we have 
\be
\label{eqEdgeRatio}
|v-w|/2 \leq |v-w'| \leq 2|v-w|.
\ee


%\begin{lemma}(useful??)
%\label{lemmaDV0}
%For each $v\in \cV_0$ the union $V_\cT(v)$ of the triangles containing $v$ is convex, and we have 
%\be
%\label{diamCellvT0}
%d_{H_0}(v, \R^2\sm V_\cT(v))\geq \delta_0.
%\ee
%Consequently we have for all $v,w\in \cV_0$ 
%\be
%\label{eqDH0vw}
%\delta_0 \leq d_{H_0}(v,w) .
%\ee
%\end{lemma}
%
%\proof
%Let $w_1,w_2,w_3$ be three consecutive vertices, in trigonometric order, on $\partial V_\cT(v)$. Since $\varangle (w_2-w_1, w_2-v)$ and $\varangle (w_2-w_3, w_2-v)$ both belong to $\in \{\cPi/4, \cPi/2\}$, we obtain that the interior angle of the polygon $V_\cT(v)$ belongs to $\{\cPi/2, 3\cPi/4, \cPi\}$, which implies that this polygon is convex.
%
%We denote by $f$ the piecewise linear function on $\cT_0$ such that $f(v)=1$ and $f(w)=0$ for all other vertices in $\cT_0$. For any triangle $T\in \cT_0$ containing $v$ the gradient of $f$ is constant on $T$, orthogonal to the edge $e$ of $T$ opposite to $v$, and for $z\in \interior(T)$ of modulus 
%$$
%|\nabla f(z)| = \frac 1 {d(v,e)} \leq \frac 2 {\diam(T)} \leq \frac 1 {\delta_0\lambda(z)}.
%$$
%It follows that $\dil_z(f\sep d_{H_0}) \leq 1/\delta_0$ and therefore that $f : (\R^2, d_{H_0}) \to \R$ is $1/\delta_0$-Lipschitz. If $z\in (\R^2 \sm V_\cT(v))$ then $|f(v)-f(z)| = 1 \leq d_{H_0}(v,z)/\delta_0$ which implies the announced result. 
%\sq
For each $z\in \R^2$ we define 
$$
\rho(z) = \lambda(z)/\mu(z) \in [1, \infty).
$$
We recall that the functions $\lambda$ and $\mu$ are $c$-Lipschitz, and that $\diam(T) \leq \lambda(z)$ for any $T\in \cT_0$. It follows that for any $T\in \cT_0$ and any $z,z'\in T$
\be
\label{eqLambdaT}
\lambda(z)(1-c) \leq \lambda(z') \leq \lambda(z)(1+c) \stext{ and } \mu(z)-c\lambda(z) \leq \mu(z') \leq \mu(z)+ \lambda(z),%\stext{ for all } T \in \cT_0, \ z,z'\in T
\ee
which implies 
$$
\rho(z') = \frac{\lambda(z')}{\mu(z')} \geq \frac{\lambda(z)(1-c)}{\mu(z)+c \lambda(z)} \geq \frac {1-c}{\rho(z)^{-1}+c}.
$$
This formula has an immediate corollary.
\begin{corollary}
\label{corolRho23}
If $c$ is sufficiently small, then the following holds. For any $T\in \cT_0$ and any $z,z'\in T$ : if $\rho(z) \geq 3$ then $\rho(z') \geq 2$, and if $\rho(z) \geq 4$ then $\rho(z') \geq 3$.
\end{corollary}
The pairs $(3,2)$ and $(4,3)$ appearing in this corollary can be replaced with $(n+1,n)$ where $n \geq 1$ is arbitrary, but the bound upper bound on $c$ depends on $n$.\\

%, and we observe that
%$$
%H_0(z) \leq H(z) \leq \rho(z)^2 H_0(z).
%$$
For each $z\in \R^2$ such that $\rho(z)>1$ we denote by $\theta(z)\in \bbS := \{u\in \R^2\sep |u| = 1\}$ a unit vector such that
\be
\label{defAngle}
H(z) = \lambda(z)^{-2} \theta(z) \theta(z)^\trans+ \mu(z)^{-2} (\Id-\theta(z) \theta(z)^\trans).
\ee
Note that there exists two, opposite, choices for the vector $\theta(z)$.
On any simply connected domain $\Omega\subset \R^2$ such that $\rho(z)>1$ for all $z\in \Omega$, there exists a continuous map $z\mapsto \theta_*(z)$ satisfying \iref{defAngle}. Since $c^2 H\in \bH_a$ we have for all $z\in \Omega$, according to Theorem \ref{th2Spaces}
%For each $z\in \R^2$ such that $\rho(z)$, the angle $z'\to \theta(z')$ can be defined in a neighborhood of $z$ and we have according to Theorem \ref{th2Spaces}, since $c^2H \in \bH_a$
\be
\label{eqDilThetaA}
(\lambda(z)-\mu(z) ) \dil_z(\theta_* \sep d_\bbS) \leq c.
\ee
For any two vectors $u,u'\in \R^2\sm\{0\}$ we define %the non-oriented, acute, angle
$$
\lhd(u,u') := \min \{\varangle(u,u'),\, \varangle(u,-u')\} = \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
$$
This quantity is used to measure the angle formed by two vectors with no clear orientation.
The formula \iref{eqDilThetaA} had an immediate corollary.
\begin{corollary}
\label{corolTheta2C}
Let $T\in \cT_0$ be such that $\rho\geq 2$ on $T$. Then for any $z,z'\in T$ and any $\theta(z), \theta(z')\in \bbS$ such that \iref{defAngle} holds, we have 
$$
\lhd(\theta(z), \theta(z')) \leq 2c.
$$ 
\end{corollary}

\proof
Since $T$ is a simply connected domain and $\rho \geq 2$ on $T$, there exists a continuous map $\theta_*\in C^0(T, \bbS)$ satisfying \iref{defAngle} at each point.
We thus have 
$$
\lhd(\theta(z), \theta(z')) = \lhd(\theta_*(z), \theta_*(z')) \leq \varangle(\theta_*(z), \theta_*(z')) = d_\bbS (\theta_*(z), \theta_*(z')) \leq \diam(T) \max_{x\in T} \dil_x(\theta_*),
$$
and for any $x\in T$
$$
\diam(T)\dil_x(\theta_*) \leq \lambda(x)\dil_x(\theta_*) \leq 2 (\lambda(x)-\mu(x)) \dil_x(\theta_*)  \leq 2c,
$$
which concludes the proof.
\sq

For each vertex $v\in \cV_0$ we define a set $\Gamma_v\subset \R^2$ as follows : $\Gamma_v := \{v\}$ if $\rho(v) <3$, and 
\be
\label{defGammav}
\Gamma_v := \left[v, \, \frac v 3+ \frac{2w_-} 3\right] \cup \left[v,\frac v 3 +\frac{2w_+} 3\right] 
\ee
if $\rho(v)\geq 3$, where $w_-,w_+\in \cV_0$ are two neighbors of $v$ in $\cT_0$ which respectively minimize and maximize the quantity $\<\theta(v)^\perp, w-v\>$. In mathematical terms for any neighbor $w\in \cV_0$ of $v$
\be
\label{defWmWp}
\<\theta(v)^\perp, w_- -v\> \leq \<\theta(v)^\perp, w-v\> \leq  \<\theta(v)^\perp, w_+ - v\>. 
\ee
We define $\Gamma := \cup_{v\in \cV_0} \Gamma_v$, and for each $z\in \Gamma\sm\cV_0$ we define 
\be
\label{defGammaz}
\Gamma_z := \bigcup_{\substack{v\in \cV_0 \\ z \in \Gamma_v}} \Gamma_v.
\ee
For any vertex $v\in \cV_0$ the set $\Gamma_v$ does not contain any vertex $w\in \cV_0$ distinct from $v$. It follows that \iref{defGammaz} agrees with \iref{defGammav} for any $z\in \cV_0$.\\ 

\begin{lemma}
\label{lemmaAngleWmWp}
let $v\in \cV_0$ be such that $\rho(v) \geq 3$, and let $w_+, w_-$ be two neighbors of $v$ satisfying \iref{defWmWp}.
We have 
\be
\label{eqAngleWmWp}
\varangle(\theta(v)^\perp, w_+ -v) \leq \cPi/4,
\stext{ and }
\varangle(\theta(v)^\perp, v-w_-) \leq \cPi/4.
\ee
\end{lemma}

\proof
We restrict without loss of generality our attention to the proof of the first inequality, and we assume for contradiction that $\vp := \varangle(\theta^\perp, w_+-v)>\cPi/4$. % in \iref{eqAngleWmWp}.
Among the two vertices $w\in \cV_0$ such that the triangle of vertices $v,w,w_+$ belongs to $\cT_0$, we choose the one such that $\varangle(\theta^\perp, w-v)$ is minimal.
We denote $\psi := \varangle(w-v, w_+-v) \in \{\cPi/4, \cPi/2\}$ and we obtain 
$$
\<\theta(v)^\perp, w_+-v\> = |w_+-v|\cos \vp \stext{ and } \<\theta(v)^\perp, w-v\> = |w-v|\cos (\vp-\psi).
$$
If $\psi = \cPi/2$ then $|w_+-v| = |w-v|$ since the triangles $T\in \cT_0$ are half squares, and $\cos (\vp-\psi) = \sin \vp$. We thus have $\cos \vp \geq \sin \vp$ according to \iref{defWmWp} which contradicts our assumption that $\vp>\cPi/4$.
If $\psi = \{\cPi/4\}$ then $|w_+-v| = \sqrt 2 |w-v|$ or $|w_+-v| =  |w-v|/\sqrt 2$. We thus have $\sqrt 2 \cos \vp \geq \cos (\vp-\cPi/4)$ which again contradicts our assumption that $\vp \leq \cPi/4$.
\sq
%
%$$
%\angle(u,u') := \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
%$$
%(Stricly speaking, $\angle(u,u')$ is the smallest of the two unoriented angles formed by $u,u'$ and $u,-u'$.)



%\begin{lemma}
%Let $T\in \cT_0$ and let $z,z'\in T$, then 
%\be
%\label{stabRho}
%\rho(z') \geq  \frac{1-c}{1/\rho(z)+c}.
%\ee
%Defining $\rho_c := \frac{1-c}{1/2+c}$, we have if $\rho(z) \geq 2$ that 
%%$$
%%\rho(z') \geq  \rho_c := \frac{1-c}{1/2+c}.
%%$$
%%and 
%\be
%\label{stabTheta}
%\angle(\theta(z), \theta(z')) \leq \vp_c := \frac c {1-1/\rho_c}.
%\ee
%\end{lemma}
%
%\proof
%Since the functions $\lambda$ and $\mu$ are Lipschitz, and since $|z-z'| \leq \lambda(z)$, we have
%$$
%\rho(z') = \frac {\lambda(z')}{\mu(z')} \geq \frac {\lambda(z)-c \lambda(z)}{\mu(z)-c \lambda(z)} = \frac{\lambda(z)(1-c)}{\lambda(z)(1/\rho(z)+c)} = \frac{1-c}{1/\rho(z)+c},
%$$
%which establishes \iref{stabRho}.
%We thus turn to the proof of \iref{stabTheta}, and for that purpose we recall that 
%$
%(\lambda(z') - \mu(z')) \dil_{z'}(\theta)\leq c
%$
%for any $z'\in T$.
%Observing that 
%$$
%\lambda(z')-\mu(z') = \lambda(z') (1-1/\rho(z')) \geq \diam(T) (1-1/\rho_c)
%$$
%we obtain 
%$$
%\angle(\theta(z), \theta(z')) \leq \diam(T) \max_{z'\in T} \dil_{z'}(\theta) \leq \frac c {1-1/\rho_c},
%$$
%which concludes the proof of \iref{stabTheta}.
%\sq

\begin{lemma}
For any $z\in \Gamma$ and any $z'\in \Gamma_z$ distinct from $z$
we have
\be
\label{eqAngleGammaz}
\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
\ee
and therefore if $c$ is sufficiently small
$$
\angle(\theta(z)^\perp ,z'-z) \leq \cPi/3, 
$$
and there exists a Lipschitz map $\gamma : [\alpha, \beta]\to \R$ such that the following is a bijection
$$
t\in [\alpha, \beta] \mapsto z+ t\theta(z)^\perp + \sqrt 3 \gamma(t) \theta(z) \in \Gamma_v.
$$
\end{lemma}

\proof
We consider a vertex $v\in \cT_0$ such that $z,z'\in \Gamma_v$, and we note that $\rho(v) \geq 3$ by construction of $\Gamma_v$, and therefore $\rho \geq 2$ on a triangle common to $v$ and $z$ according to Corollary \ref{corolRho23}.
It thus follows from Corollary \ref{corolTheta2C} that 
\begin{eqnarray*}
\angle(\theta(z), z-z')&\leq& 2c + \angle(\theta(v), z-z') \\
&\leq& 2c + \max \{ \angle(\theta(v), w_+-v), \angle(\theta(v), w_- -v)\}\\
& \leq & 2c + \cPi/4,
\end{eqnarray*}
which concludes the proof.
\sq

The next proposition gives some properties of the set $\Gamma$.
%We use the notation 
%$$
%d(z,E) := \inf \{|z-e| \sep e \in E\} \stext{ and } d_H(z,e) := \inf \{d_H(z,e)\sep e\in E\}.
%$$
\begin{prop}
\label{propDistUpLow}
If $c$ is sufficiently small, then the following holds.
For any $z\in \Gamma$,
\be
\label{eqDistzGH0}
 \min\{|z-e| \sep  e\in \Gamma\sm \Gamma_z\} \geq \frac {10}{91} \lambda(z) % >\frac 1 {10}
%(most appropriate bound??)
%\frac{\lambda(z)} {10} %\frac{\delta_0} 5 %:= \frac{(1-c)\delta_0}{3 \sqrt 2}\lambda(z), %(euclidean distance??) %d(z,\Gamma\sm \Gamma_z) 
\ee
%If $z\in \Gamma$ and $\rho(z) \geq 4$ then 
%in such way that 
%\be
%\label{assumPhic}
%\frac{1+\vp_c 4\sqrt 2}{1-\vp_c\sqrt 2}\leq \frac 4 3
%\ee
and for $z\in \R^2$
\be
\label{eqDistzGH}
\min\{\|z-e\|_{H(z)} \sep e \in \Gamma\} \leq 2 %1+ \frac {2\sqrt 2} 3 <2. 
\ee
\end{prop}

\proof
We first establish \iref{eqDistzGH0}. 
Let $z\in \Gamma$ and let $v\in \cV_0$ be such that $z\in \Gamma_v$. We have $z= (1-\alpha) v+\alpha w_*$ for some $\alpha\in [0,2/3]$ and some neighbor $w_*\in \{w_+,w_-\}$ of $v$.
Denoting by $V_{\cT_0}(v)$ the union of all triangles $T\in \cT_0$ containing $v$, and by $\cV_0(v)$ the collection of neighbors of $v$ in $\cT_0$, we have
$$
\Gamma\sm \Gamma(z) \subset \overline {\R^2 \sm V_{\cT_0}(v)} \bigcup_{w\in \cV_0(v)\sm\{w_*\}} \left[\frac{2v+w}3, w\right].
$$
Therefore (*picture needed*)
\begin{eqnarray*}
d(z,\Gamma\sm \Gamma(z)) &\geq & \min \left\{ d(z, \R^2 \sm V_\cT(v)), \ \min_{w\in \cV_0(v) \sm \{w_*\} } d\left(z,\left[\frac{2v+w}3, w\right]\right)\right\}\\
& \geq & \min \left\{ \frac{|w_*-z|}{\sqrt 2}, \ \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)\sm \{w_*\}} |v-w|\right\}\\
& = & \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)} |v-w|\\
& \geq & \frac{1}{3\sqrt 2} \lambda(v)\frac {\sqrt 2} 3 \\
&\geq&  \frac{\lambda(z)(1-c)}{9}.
\end{eqnarray*}
where we used \iref{edgeLambda} in the fourth line, and \iref{eqLambdaT} in the last line. This establishes \iref{eqDistzGH0} if $c$ is sufficiently small.\\

We now turn to the proof of \iref{eqDistzGH}. (*picture needed*)
Let $T \in \cT$ and let $z\in T$. Since $T$ is a half square there exists a vertex $v$ of $T$ such that $|z-v| \leq \diam(T)/2$, hence %For any vertex $v$ of $T$ we obtain %If $\rho(z)\leq 4$, then any vertex $v$ of $T$ satisfies 
$$
\|z-v\|_{H(z)} \leq  \frac{|z-v|}{\mu(z)}   \leq \frac{\diam(T)}{2 \mu(z)} \leq \frac{\lambda(z)}{2 \mu(z)} = \frac{\rho(z)} 2,
$$
which concludes the proof if $\rho(z) \leq 4$. If $\rho(z) \geq 4$ and $c$ is sufficiently small then $\rho(v) \geq 3$ for any vertex $v$ of the triangle $T$ according to Corollary \ref{corolRho23}.

We choose two vertices $v,w$ of $T$ such that the line $(z+ r \theta(z))_{r\in \sR}$ intersects $\partial T$ on the segment $[v,(v+w)/2]$.
We denote by $w_-$ and $w_+$ the neighbors of $v$ in $\cT_0$ which satisfy \iref{defWmWp}.
We have according to \iref{eqEdgeRatio}
$$
\<\theta(v)^\perp,w_+ - v\> \geq |w_+-v|\cos(\cPi/4) \geq \frac{|w-v|} 2 \frac 1 {\sqrt 2}. %/(2\sqrt 2).
$$
We assume without loss of generality that $\theta(v)$ and $\theta(z)$ are oriented in consistently, in such way that $\<\theta(z), \theta(v)\> \geq 0$, and we obtain using Corollary \ref{corolTheta2C}
$$
|\theta(z)-\theta(v)| \leq \varangle(\theta(z), \theta(v)) = \lhd(\theta(z), \theta(v))\leq 2c.
$$
It follows that 
\begin{eqnarray*}
\<\theta(z)^\perp, w-v\> &=& \<\theta(z)^\perp-\theta(v)^\perp, w-v\>+\<\theta(v)^\perp, w-v\>\\
& \leq & |\theta(z)-\theta(v)| |w-v| + \<\theta(v)^\perp, w_+-v\>\\
& \leq & (1+4c \sqrt 2 )\<\theta(v)^\perp, w_+-v\>.\\
%& \leq & (1+4 c\sqrt 2) }{1-\vp_c\sqrt 2} \<\theta(z)^\perp,w_+ - v\>.
%& \leq & \frac 4 3 \<\theta(z)^\perp,w_+ - v\>
\end{eqnarray*}
Denoting $\Theta := \varangle(\theta(v)^\perp, w_+-v)$ and $\Phi := \varangle(\theta(z)^\perp, w_+-v)$ we obtain 
$$
\frac{\<\theta(v)^\perp, w_+-v\>}{\<\theta(z)^\perp, w_+-v\>} = \frac{\cos(\Theta)}{\cos(\Phi)} \leq \frac{\cos(\Theta)}{\cos(\Theta) - |\Phi-\Theta|} =\left(1-\frac {|\Phi-\Theta|}{\cos\Theta}\right)^{-1}\leq (1-2 \sqrt 2 c)^{-1} % - 2c} = \frac 1 {1-2 \sqrt 2 c},
$$
hence 
$$
\<\theta(z)^\perp, w-v\>  \leq \frac{1+4c \sqrt 2}{1-2 \sqrt 2 c}\<\theta(z)^\perp, w_+-v\>
$$
Proceeding likewise for $w_-$, and assuming that $c$ is sufficiently small, we obtain 
%
%We assume that $c$ is sufficiently small in such way that 
%\be
%\label{assumPhic}
%\frac{1+\vp_c 4\sqrt 2}{1-\vp_c\sqrt 2}\leq \frac 4 3
%\ee
$$
\frac 4 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, w-v\> \leq  \frac 4 3\<\theta(z)^\perp, w_+ - v\>,
$$
and therefore since $z+r\theta(z)\in [v,(v+w)/2]$ for some $r\in \R$,
$$
\frac 2 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, z-v\> \leq  \frac 2 3\<\theta(z)^\perp, w_+ - v\>.
$$
It follows that the line $(z+r\theta(z))_{r\in \sR}$ intersects the set $\Gamma_v := [v, (v+2w_+)/3] \cup  [v, (v+2w_-)/3]$ at some point $z'$.
%hence there exists $r\in \R$ such that $z' := z+ r\theta(z) \in \Gamma_v$. 
The point $z'$ belongs to triangle $T'$ containing $v$, and we obtain using \iref{eqDiamRatio} 
\begin{eqnarray*}
\lambda(z) \|z'-z\|_{H(z)} &=& \lambda(z)\|r\theta(z)\|_{H(z)}\\
&=& |r|\\
&=& |z-z'|\\
&\leq& |z-v|+|v-z'|\\
&\leq& \diam(T)+ \frac 2 3\diam(T')\\
&\leq & \left(1+\frac 2 3 \sqrt 2\right) \diam(T)
 \leq  \left(1+\frac 2 3 \sqrt 2\right) \lambda(z),
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

%We assume from this point that $c>0$ is sufficiently small in such way that 
%\iref{assumPhic} holds, and that 
%$e_c \geq \delta_0/5$. 
We define 
\be
\label{defDelta1}
\delta_1 := \delta_0/10.
\ee
\begin{lemma}
\label{lemmaConstV}
The following holds if $c$ is sufficiently small.
There exists a discrete set $\cV \subset\Gamma$ containing $\cV_0$ and satisfying the following:
\begin{itemize}
\item (Separation) For all $v,w\in \cV$, $d_H(v,w) \geq 1/10$.
\item (Distance from $\Gamma$) For all $z\in \Gamma$, $d_H(z, \cV) \leq 1/10$.
\item (Distance from $\R^2$) For all $z\in \R^2$, $d_H(z,\cV) \leq 2+1/4$.
\end{itemize}
%We denote by $\cV$ a $1$-equispaced subset of the metric space $(\Gamma, d_H/\delta_1)$ containing $\cV_0$.
%The set $\cV$ is also a $\delta_1/5$-equispaced subset of the metric space $(\R^2, d_H/5)$.
\end{lemma}
\proof
For any $v,w\in \cV_0$ we obtain using \iref{pairwiseV0} and Proposition \ref{propEuclidRiemann}
\begin{eqnarray*}
d_H(v,w) &\geq& \ln(1+c\|v-w\|_{H(v)})/c\\
&\geq& \ln(1+c|v-w|/\lambda(v))/c\\
&\geq& \ln(1+c\sqrt 2 /3)/c \geq 1/10\\
\end{eqnarray*}
if $c$ is sufficiently small since $\sqrt 2 /3>1/10$.

According to Lemma \ref{lemmaEquiSpaced} there exists a $1$-equispaced subset $\cV$ of the metric space  $(\Gamma, 10 \:d_H)$ containing $\cV_0$, since the pairwise distanced between points of $\cV_0$ are larger than $1$ for the distance $10 \:d_H$.
Two first announced properties, separation and distance from $\Gamma$, simply state the fact that $\cV$ is a $1$-equispaced subset of $(\Gamma, d_H)$.

The third property, distance from $\R^2$, is obtained as follows: for any $z\in \R^2$ there exists according to Proposition \label{propDistUpLow} a point $e\in \Gamma$ such that $\|z-e\|_{H(z)}\leq 2$. Furthermore there exists a vertex $v\in \cV$ such that $d_H(e,v) \leq 1/10$, hence
$$
d_H(z,\cV) \leq d_H(z,e)+ d_H(e,v) \leq -\ln(1-c\|z-e\|_{H(z)})/c + 1/10 \leq -\ln(1-2c)/c + 1/10.
$$
Hence $d_H(z,\cV)<2+1/4$ if $c$ is sufficiently small.
\sq

\begin{lemma}
\label{lemmaRecallG}
There exists a absolute constant $C_0\geq 1$ such that the following holds if $c$ is sufficiently small.
The set $\cV$ is wedged with respect to the metric $H$, and the anisotropic Delaunay triangulation obtained by arbitrarily triangulating the cells of the graph $\cG(\cV,H)$ is $C_0$-adapted to $H$.

Furthermore for any edge $[v,w]$ of $\cT$ and any $z\in [v,w]$ we have 
$$
\|v-w\|_{H(z)} \leq 5.
$$
\end{lemma}

\proof
We denote $\alpha := (2+1/4)^{-1}$ throughout the proof of this lemma.
It follows from to Lemma \ref{lemmaConstV} that the set $\cV$ is a $\alpha/10$-equispaced subset of the metric space $(\R^2, \alpha d_H)$. 

Theorem \ref{thEquiMesh} applied to the metric $\alpha^2 H$, therefore implies that, if $c$ is sufficiently small, the set 
$\cV$ is wedged for the metric $\alpha^2 H$ and that arbitrarily triangulating the convex cells of the graph $\cG(\cV,\alpha^2 H)$, which are convex yields a triangulation $\cT$ which is $C$-adapted to the metric $\alpha^2H$ (hence $C_0 := C/\alpha$-adapted to $H$), where $C$ is an absolute constant.

The definition \iref{defGVH} of the graph $\cG(V,H)$ implies that $\cG(\cV,\alpha^2 H) = \cG(\cV,H)$, and Definition \ref{defWedge} of the wedge property shows that it holds for $H$ if and only if it holds for $\alpha^2 H$. 

For any edge $[v,w]$ of $\cT$ the Voronoi regions $\Vor(v)$ and $\Vor(w)$ intersect (by definition of the anisotropic Delaunay triangulation), and we thus have according to Lemma \ref{lemmaDiamVor} 
$$
\alpha d_H(v,w) = d_{\alpha^2 H} (v,w) \leq -2\ln (2-e^{c'})/c'
$$
where $c' := c/\alpha$. This implies the last property since $2 (1+1/4) <5$.

(*details*)
\sq


\begin{prop}
If $c$ is sufficiently small.
For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$ we have 
\be
\label{vpNotInGammav}
\sin \lhd (\theta(v),v-w) \leq \frac {50}{\rho(v)}.
\ee
%We define $\rho_0\in [1,\infty)$ by $\sin (\cPi/12) = 50/\rho_0$.
\end{prop}

\proof
If $c$ is sufficiently small, then Proposition \ref{propDistUpLow} implies that $|v-w| \geq \lambda(v)/10$, and Lemma \ref{lemmaRecallG} states that $\|v-w\|_{H(v)} \leq 5$.
Denoting $\vp := \lhd (\theta(v),v-v')$ we obtain 
$$
5\geq \|v-w\|_{H(v)} \geq \frac{|v-w|\sin \vp}{\mu(v)} \geq \frac{\lambda(v) \sin \vp}{10 \mu(v)}.
$$
which implies the announced result.
\sq

%\begin{lemma}
%If $c$ is sufficiently small, then the following holds.
%
%\end{lemma}

\begin{lemma}
\label{lemmaVorFar}
If $c$ is sufficiently small, then for any $v\in \cV$, $w\in \cV\sm \Gamma_v$ and $z\in \Vor(w)\cap \Gamma$ we have 
$$
|z-v|\geq \lambda(v)/100.
$$
\end{lemma}

\proof
For any $z\in \Gamma$, there exists $w\in \cV$ such that $d_H(z,w) \leq 1/10$, and therefore 
$
\|z-w\|_{H(w)} \leq (\exp(c/10)-1)/c.
$
By definition of the Voronoi diagram, for any $z\in \R^2$ and any $w\in \cV$ such that $z\in \Vor(v)$, we thus have 
\be
\label{diamVor10}
\|z-w\|_{H(w)} \leq (\exp(c/10)-1)/c.
\ee
Let $v\in \cV$ any $z\in \R^2$ be such that $|z-v|\leq |\lambda(v)/200$, and let $w\in \cV$ be such that $z\in \Vor(v)$. We claim that $w\in \Gamma_v$ if $c$ is sufficiently small.
Indeed \iref{diamVor10} implies that 
$$
c d_H(z,w) \leq -\ln (1-c\|z-w\|_{H(w)}) \leq -\ln(2-\exp(c/10)).
$$
On the other hand
\begin{eqnarray*}
c d_H(z,w) &\geq& \ln(1+c\|z-w\|_{H(z)})\\
& \geq & \ln(1+c |z-w|/\lambda(z))\\
& \geq & \ln\left(1+c \frac{|w-v|-|z-v|}{\lambda(v)+c|z-v|}\right)\\
&\geq & \ln\left(1+c \frac{10/91-1/100}{\lambda(v)(1+c/100)}\right)\\
\end{eqnarray*}
hence 
\be
\label{eq909}
\frac{-\ln(2-\exp(c/10))}c \leq \frac 1 c\ln\left(1+c \frac{10/91-1/100}{\lambda(v)(1+c/100)}\right)
\ee
As $c\to 0$, the left hand side tends to $1/10$, while the right hand side tends to $10/91-1/100 = 909/9100 < 1/10$. Hence \iref{eq909} is a contradiction if $c$ is sufficiently small.\\
\sq

\begin{lemma}
If $c$ is sufficiently small, then 
for any $v\in \cV$ we have 
$$
\Vor(v) \supset \{z\sep \|z-v\|_{H(v)} \leq 1/25\}.
$$
\end{lemma}

\proof
We consider $z\in \partial \Vor(v)$, hence $z\in \Vor(v) \cap \Vor(w)$.
Define $r:=\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$, hence using the separation property
\begin{eqnarray*}
1/10 &\leq& d_H(v,w)\\
&\leq& d_H(z,v)+d_H(z,w)\\
&\leq& -\ln (1-c\|z-v\|_{H(v)})/c - \ln (1-c\|z-v\|_{H(v)})/c\\
&=& -2 \ln (1-cr)/c.
\end{eqnarray*}
It follows that 
$$
r\geq (1-\exp(-c/20))/c,
$$
and therefore $r\geq 1/25$ if $c$ is sufficiently small, 
which concludes the proof.
\sq

The set $\Gamma$ is a union of polygonal lines (and of isolated points). If $v\in \Gamma$ is on a polygonal line, we say that the neighbors of $v$ on $\Gamma$ are the previous and next points on $\Gamma$ if they exist.

\begin{prop}
The following holds if $c$ is sufficiently small.
Let $v\in \cV$ be such that $\rho(v)\geq \rho_0$, where $\rho_0$ is a constant specified in the proof. Then $v$ forms an edge with each of its neighbors in $\Gamma$, no edge with any other point in $\Gamma_v$, and at least two edges with $w,w'\in \cV\sm\Gamma$ such that and in opposite directions in the sense that satisfying $\<w-v, w'-v\> <0$.
\end{prop}

\proof
If follows from \iref{eqAngleGammaz} that there exists an interval $[\alpha, \beta]$, and a Lipschitz map $\omega : [\alpha, \beta]\to \R$ such that 
$$
t\in [\alpha, \beta] \to z+ \gamma(t) := z+ t \theta(z)^\perp + \sqrt 3 \omega(t) \theta(z) \in \Gamma_v %\Gamma(t) :=
$$
is one to one. % ($\omega$ is piecewise affine)
We have 
$$
\frac {|t-t'|} {\mu(z)} \leq \|\gamma(t)-\gamma(t')\|_{H(z)} = \sqrt {\left(\frac{t-t'}{\mu(z)}\right)^2 + 3 \left(\frac{\omega(t)-\omega(t')}{\lambda(z)}\right)^2} \leq \frac {|t-t'|} {\mu(z)} \sqrt {1+3\rho(z)^{-2}}.
$$

Our purpose is now to establish that $v$ for any neighbor $w$ of $v$ on $\Gamma$ the segment $[v,w]$ is an edge of $\cT$.
We assume that $v$ has a neighbor $w$ corresponding to a positive value of $t$.
We define 
$$
\beta' := \max\{t\in [0,\beta]\sep v+\gamma(t') \in \Vor(v) \text{ for } 0 \leq t'\leq t\} 
$$
and we observe that 
$$
|\beta'|/\mu(v) \leq \|\gamma(\beta')\|_{H(v)} \leq (\exp(c/10)-1)/c.
$$
Note that $v+r\lambda\theta(v) \in \Vor(v)$ for $|r|\leq 1/25$.
Since the Voronoi regions are star shaped, it follows that $z:=v+\gamma(\beta')\notin \Vor(w)$ for $w\in \Gamma_v$ corresponding to negative values of $t$.
Furthermore $z\notin \Vor(w)$ for $w\in \Gamma\sm \Gamma_v$ due to Lemma \label{lemmaVorFar}.

Thus $z\in \Vor(w)$ for some $w\in \Gamma_v$ corresponding to a positive value of $t$. 
Upper bound on $t$ since $\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$ we obtain 
$$
\ln(1+c\|v-w\|_{H(v)})/c \leq  d_H(v,w) \leq d_H(v,z)+d_H(z,w) \leq -2\ln(1-c\|z-v\|_{H(v)})/c.
$$
Apply the argument that the Voronoi region is star shaped to the neighbor of $v$.

Denote by $T_0,T_1$ the two triangles containing $[v,w]$, and denote by $w_0, w_1$ the two third vertices.
the edges $[v,w_0]$ and $[v,w_1]$ are close to the direction of $\theta(v)$, using the fact that $\cH_{T_i} \simeq H(v)$. 
More precisely : 
Or area of $T_i$ -> length $|v-w_i|\simeq \lambda$ -> orientation since $\|v-w_i\|_{H(v)} \leq 5$.
Thus no connection with neighbors corresponding to positive $t$.


%
%Upper boun
%We have 
%$$
%\<\theta
%$$
%
%
%
%
%We recall that the Voronoi regions are star shaped (insufficient argument since not a strainght line), and we define 
%$$
%[\alpha', \beta'] := \{t\in [\alpha, \beta] \sep v+\gamma(t) \in \Vor(v)\}.
%$$
%We assume that $\beta'<\beta$, otherwise 
%We have 
%$$
%|\beta'|/\mu(v) \leq \|\gamma(\beta')\|_{H(v)} \leq (\exp(c/10)-1)/c.
%$$
%Let $w\in \cV$, $w\neq v$, be such that $v+\gamma(\beta') \in \Vor(w)$.
%We have $\|w-v+\gamma(\beta')\|_{H(w)} = \|\gamma(\beta')\|_{H(v)}$, hence 
%
%
%For any $w\in \cV$ we have $d_H(v,w) \geq 1/10$
%
%
%Let $w\in \cV$, $w\neq v$, be such that $v+\gamma(\beta') \in \Vor(w)$.
%We have $\|w-v+\gamma(\beta')\|_{H(w)} = \|\gamma(\beta')\|_{H(v)}$, hence 
%
%
%
%
%
%Note that 
%The index of 
%
%$$
%\alpha' := \min ([\alpha,\beta] \cap \Vor(v)) \text{ and } \beta' := \max ([\alpha, \beta] \cap \Vor(v)),
%$$
%
%If $\beta' = \beta$, then there is no 
%We define 
%
%
%We have 
%$$
%d_H(z,z+\gamma(t)) \geq \ln (1+c\|\gamma(t)\|_{H(z)}) = \ln(1+c 
%$$
%
%We parametrize the set $\Gamma_v$ by the map $\gamma :[\alpha, \beta]\to  \Gamma_v$ defined as follows : for all $x\in [\alpha, /\beta]$
%$$
%\gamma^{-1}(x)= \< \theta(v)^\perp , x-v\>.
%$$
%We have the estimates
%$$
%bjlxt
%$$
%
%(*big one*)
%We consider two successive points $v,w\in \cV$ on $\Gamma$, and we show that $[v,w]\subset \interior(\Vor(v) \cup \Vor(w))$ if $\rho(v)\geq ??$.
%
%Note that $\|v-w\|_{H(v)} \leq 2\delta_1(1+o_c(1))$.
%Indeed $B_H(v+\delta_1\bt(v)??, \delta_1(1+??))$ contains a point, which needs to be on $\Gamma_v$, hence neighbor not far.
%
%No problem from $\Gamma\sm \Gamma_z$.
%
%We have $v+r\lambda \theta(v)$ for $r\in [??\delta_1,??\delta_1]$, and likewise for $w$.
%Thus angle formed : 
%$$
%|\<\theta(v)^\perp, v+r \lambda\theta(v) - (\alpha v+(1-\alpha)w)\>| \leq |v-w| \leq 3\mu.
%$$
%and 
%$|v+r \lambda\theta(v) - (\alpha v+(1-\alpha)w)| \geq  |r|\lambda -|v-w|\geq |r|\lambda(v) - 3\mu(v)$
%Thus if $\rho(v)$ is sufficiently large,
%$$
%\angle(\theta(z)^\perp , ...) > \cPi/3,
%$$
%hence the point does not belong to $\Gamma_z$. Thus $z\notin \Vor(x)$, thus the $[v,w]$ belongs to the interior of $\Vor(v) \cup \Vor(w)$.
%
We next show that $v$ is not linked to other points on $\Gamma_v$.
Assume that this is the case for contradiction.
$w\in \Gamma_v$ is such that $[v,w]$ is an edge of $\cT$.
We introduce the vertex $v_0\in \cT_0$ in between $v$ and $w$.
The segments $[v,v_0]$ and $[v_0,w]$ are included in the edge set of $\cT$. The triangle of vertices $v,v_0,w$ contains an element of $\cT$, but this is a contradiction with the diameter which should be of the order $\lambda(v)$ and not $\mu(v)$.





%%First we remark that $
%Let $z=\alpha v+(1-\alpha) w$.
%We grow an ellipse around $z$, we first fall on $v,w$
%
%The collection $\cV$ of vertices is a $1$-equispaced subset of $(\Gamma, d_H/\delta_1)$, 
%For all $x\in \Gamma$
%By construction 
%
%For that purpose we remark that 
%
%Let $x\in \cV$.
%
%
%
%
%
%We thus turn to the proof of the second property. The fact that  the angle property appearing in \iref{vpInGammav} is a direct consequence of \iref{eqAngleGammaz} : we have $\angle (\theta(v)^\perp, v-w) \leq \cPi/3$ provided $\vp_c \leq \cPi/12$ which is the case if $c$ is sufficiently small.
%
%We thus have 
%$$
% \cos(\cPi/3)\frac{|v-v'|}{\mu(v)} \leq \|v-w\|_{H(v)}\leq 12.
%$$
%
%We now establish that $e\subset \Gamma$, if $\rho(v)$ is sufficiently large, and for that purpose we first show that two successive points on $\Gamma$ are always linked by an edge.
%
%
%Use star shaped.
%
%Then we consider the two triangles containing this edge, and we obtain a contradiction with the angle...
%
%We then assume that there exists another connection, and we obtain a contradiction with the diameter of the triangle.
%%we denote by $v_*$ the point of $\cV$ next to $v$ in $\Gamma$ and such that $\<v^*-v, \, v'-v\> \geq 0$.
%%The voronoi region of $v^*$ contains...
\sq

%\begin{corollary}
%\label{corolDirRho}
%If $c$ is sufficiently small.
%Let $T_0\in \cT_0$ and let $z\in T_0$. If $\rho(z) \geq \rho_0$, then any edge $e$ of $\cT$ intersecting $T_0$ satisfies $e\subset \Gamma$ or $\angle(\vec e, \theta) \leq \cPi/12$.
%\end{corollary}
%
%\proof
%
%\sq


%We say that a point $v\in \cV$ is extremal if $\Gamma_v\neq \{v\}$ and if at least one the two (opposite) tangent vectors $\bt(v)$ to $\Gamma$ at the point $v$, satisfies 
%$$
%\Gamma_v \cap \cV \cap (v +  \bt(v)\R_+) = \emptyset.
%$$

We define $\rho_* := \max\{\rho_0, \rho_1\}$.
If a triangle $T\in \cT$ contains a simplex $v\in \cV$ such that $\rho(v) \leq \rho_*$, then we obtain 
$$
S(T) \leq \rho(T) = \sqrt{\|\cH_T\| \|\cH_T^{-1}\|} \leq C_0^2 \rho(v) \leq C_0^2 \rho_*.
$$
The next lemma allows to control the angles at the points $v$ which satisfy $\rho(v) \geq \rho_*$.
\begin{lemma}
\label{lemmaAngles}
To each vertex $v\in \cV$ such that $\rho(v) \geq \rho_*$ we associate the collection $E(v)$ of all vectors $w-v$ where $w$ is a neighbor of $v$ in $\cT$, as well as the two tangents to $\Gamma$ at $v$.
%
% of vectors $w-v$ for all $w\in \cV_0(v)$, as well as $\bt(v)$ if $v$ is extremal.
The angle formed by two successive directions in $E(v)$, in trigonometric order, is smaller that $\vp_*$.
%is uniformly bounded by an absolute  constant independent of $H$.
\end{lemma}

\proof
At each vertex $v$ we have the four directions : close to $\theta$, $-\theta$, and not so far from $\theta^\perp$ and $-\theta^\perp$ (one of the two last ones being brought by $\bt(v)$ if $v$ is extremal).

%Such a vertex $v$ has an edge with a neighbor $w\in \Gamma$. Consider could be a corollary of the previous.
\sq

\begin{prop}
%Denote by $\cT^*$ the non-conforming triangulation obtained by cutting the triangles in $\cT$ containing an extremal vertex $v$ and such that $\rho(v) \geq \rho_0$ in the direction of $\bt(v)$.

Denote by $\cQ$ the partition into convex polygons obtained by cutting $\cT$ by all segments joining an extremal vextex $v\in \cV$ satisfying $\rho(v) \geq ??$ to the vertex $v'\in \cV_0$ in the direction of $\bt(v)$.

Then the interior angles in $\cQ$ are smaller than ??. %Each triangle $T\in \cT$ contains at most $??$ cells of $\cC$, which are at most hexagons (in other words they have $3$ to $6$ elements).

Denote $\cT'$ the triangulation obtained by randomly triangulating the convex cells of $\cQ$.

Then $\cT'$ is a $??$-refinement of $\cT$ and $S(T') \leq ??$ for all $T'\in \cT'$.
\end{prop}

\proof
The angles of the cells $Q\in \cQ$ fall into two categories.
The angles at the vertices of $\cT$ are bounded by ?? according to Lemma \ref{lemmaAngles}.
The angles which are not at the vertices are formed by the junction from an extremal vertex to $v\in \cV$ to the vertex $w\in \cT_0$ in front, and are bounded by ?? combining Lemma \ref{lemmaDirRho} and the direction of $\bt(v)$.\\

The triangulation $\cT'$ is obtained by triangulating the convex cells forming $\cQ$, and this operation reduces the angles. We thus have the same bound ??, and
$$
S(T) \leq \tan(??/2).
$$

We now prove that $\cT'$ is a bounded refinement of $\cT$, and for that purpose we consider and edge $e=[v,w]$ of $\cT$. %=[\omega-u, \omega+u]

We have by construction $|v-w|/\lambda(v) \leq \|v-w\|_{H(v)} \leq 12$.
The triangles $T\in \cT_0$ intersected by $[v,w]$ satisfy for some $z\in [v,w]$ the inequality 
$$
2 \delta_0 \lambda(v) (1-12c) \leq 2 \delta_0 \lambda(z) \leq \diam(T) \leq \lambda(v) \leq \lambda(u)(1+12c)
$$
Therefore they are contained in the ball $B(v,  \lambda(v)(12+1+12c))$ and have area 
$$
|T| = \diam(T)^2/4 \geq \delta_0^2 \lambda(v)^2 (1-12c)^2.
$$
Therefore there are at most 
$$
\cPi (13+12c)^2/ (1-12c)^2 \leq k := \cPi 14^2,
$$
such triangles, and the edge $e$ is thus cut in at most $k$ parts by the edges joining an extremal vertex in $\cV$ to the corresponding vertex in $\cV_0$.

Hence there are at most $3k$ vertices of $\cT'$ on the three edges of a triangle $T\in \cT$ (including the vertices of $T$).
Since any conforming triangulation of convex envelope of $n+2$ points uses $n$ triangles, we obtain that $\cT'$ is a $3k-2$ refinement of $\cT$.
\sq

\input{../Bibliography/Bibliography.tex}
\end{document}



==> MeshMetric/MeshMetricTheseOld3.tex <==
\input{../PreambleThese}

\section{Introduction}

Triangulations and meshes are finite objects of combinatorial nature: they can be described by a collection of vertices and of connection between these. This description is fruitful for the demonstration of algebraic results, such as the Euler formula, or for computer processing.
In contrast, many approaches towards anisotropic mesh generation are based on a continuous object, namely a riemannian metric $z\mapsto H(z)$, in other words a continuous function $H$ from the domain $\Omega\subset \R^d$ to the set $S_d^+$ of symmetric positive definite matrices. Once this metric has been properly designed, it is the task of a mesh generation algorithm such as \cite{Shew,Bois,FreeFem,Inria} to generate a triangulation that agrees with this metric, in a sense specified below \iref{defEquiv}.
The purpose of this chapter is to formulate precise equivalence results between some classes of triangulations and of riemannian metrics. This equivalence translates some geometrical constraints satisfied by the triangulations into the form of regularity properties of the equivalent riemannian metrics.\\

Our results are so far limited to meshes and metrics defined on the entire infinite domain $\R^d$, and the dimension $d\geq 2$ is fixed throughout this chapter. 
The choice of the unbounded domain $\R^d$ guided by simplicity, since the curvature and the singularities of
of the boundary $\partial\Omega$ induces additional difficulties 
from the point of view of computational mesh generation.
Bounded domains will be the object of future work.
We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$, and we introduce in \S\ref{subsecDefTStar} three embedded subsets of $\bT$ of particular interest 
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
where $C\geq 1$ is a parameter which plays a minor role.
The set $\bT_{i,C}$ collects all \emph{isotropic} meshes $\cT$ which are heuristically defined as follows: the simplices $T\in \cT$ may have strongly varying volumes, but their aspect ratio is uniformly bounded. 
The largest set $\bT_{g,C}$ collects \emph{graded} meshes, which only satisfy a condition of local consistency: all the  geometrical features of the simplices $T\in \cT$ may vary strongly, volume, aspect ratio and orientation, but two \emph{neighboring} simplices should not be excessively different.
The intermediate set $\bT_{a,C}$ collects \emph{quasi-acute} meshes, which definition involves the measure of sliverness $S(T)$ of a simplex $T$ introduced in Chapter \ref{chapW1P} and also discussed in Chapter \ref{chapApproxMet}. 
The measure of sliverness plays an important role in the finite element approximation of a function on a mesh $\cT$ when the error is measured in the Sobolev $W^{1,p}$ norm.\\

We associate to each simplex $T$ a symmetric positive definite matrix $\cH_T$ such that the ellipsoid
$$
\cE_T := \{z\in \R^d \sep (z-z_T) \cH_T (z-z_T)^\trans \leq 1\},
$$
which is centered at the barycenter $z_T$ of $T$,
is the ellipsoid of minimal volume containing $T$. The properties of the matrix $\cH_T$ are discussed in \S \ref{subsecIntroSimplex} of this introduction,  as well as its explicit expression in terms of the coordinates of the simplex $T$. The matrix $\cH_T\in S_d^+$ encodes the volume, the aspect ratio and the orientation (but not the angles) of the simplex $T$. Two triangles $T$ and their associated ellipses $\cE_T$ are illustrated on figure \ref{figET}.

\begin{figure}
\centering
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleAigu.pdf}
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleObtus.pdf}
	\caption{Two triangles $T$ and their associated ellipse $\cE_T$.\label{figET}}
\end{figure}

A riemannian metric on $\R^d$ is a continuous map $H$ which associates to any $z\in \R^d$ a symmetric positive definite matrix $H(z)\in S_d^+$. We denote by $\bH = C^0(\R^d,S_d^+)$ the collection of riemannian metrics.
The following definition introduce a notion of equivalence between meshes and metrics
\begin{definition}
\label{defEqHT}
We say that a mesh $\cT\in \bT$ is $C_0$-equivalent to a given metric $H\in \bH$, where $C_0\geq 1$ is a fixed constant, if for all $T \in \cT$ and all $z\in T$ one has 
\be
\label{defEquiv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
\ee
We say that a collection of simplicial meshes $\bT_*\subset \bT$ is equivalent to a collection $H_*$ of metrics if there exists a uniform constant $C_0\geq 1$ such that the following holds:
\begin{itemize}
\item For any mesh $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\item For any metric $H\in \bH_*$ there exists a mesh $\cT\in \bT_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\end{itemize}
\end{definition}
Our main result (Theorem \ref{thEquiv}) states that when the constant $C$ is sufficiently large, and if dimension is $d=2$, the three classes of meshes $\bT_{i,C}\subset \bT_{a,C} \subset \bT_{g,C}$ are respectively equivalent to three classes of metrics
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
that are defined by precise smoothness conditions on the function $z\mapsto H(z)$ in \S \ref{subsecDefHStar} of this introduction.
%Our main result Theorem \ref{thEquiv} states that when the parameter $C$ is large enough and the dimension is $d=2$, the collections $\bT_{\star,C}$ of triangulations are equivalent to the corresponding collections $H_\star$ of metrics for any symbol $\star \in \{i,a,g\}$. 
The most striking point of this result is that, although the matrix $\cH_T$ does not encode the angles of a simplex $T$, the fact that a mesh $\cT\in \bT_{a,C}$ is \emph{quasi-acute} can be translated in a precise regularity condition on the metric $H$ equivalent to $\cT$.

In order to state our results more precisely we need to introduce some notations. We first recall some notations of linear algebra. We denote by $\M_d$ the collection of $d\times d$ matrices with real entries. We denote by $\GL_d$ the standard linear group, by $\SL_d$ the special linear group and by $\cO_d$ the orthogonal group
\begin{eqnarray*}
\GL_d &:=& \{A\in \M_d\sep \det A\neq 0\}\\
\SL_d &:=& \{A\in \M_d\sep \det A=1\}\\
\cO_d &:=& \{U\in \M_d\sep U^\trans U = \Id\}.
\end{eqnarray*}
We denote by $S_d$ the collection of symmetric matrices, by $S_d^\oplus$ the subset of non-negative symmetric matrices, and by $S_d^+$ the collection of symmetric positive definite matrices.
\begin{eqnarray*}
S_d &:=& \{M\in \M_d\sep M = M^\trans\}\\
S_d^\oplus &:=& \{M\in S_d\sep z^\trans M z \geq 0 \text{ for all } z\in \R^d\}\\
S_d^+ &:=& S_d^\oplus \cap \GL_d.
\end{eqnarray*}
Let $M,M'\in S_d$, we write $M\leq M'$ if $M'-M\in S_d^\oplus$, and $M< M'$ if $M'-M\in S_d^+$. We recall that for any $M,M'\in S_d$ such that $M\leq M'$ and any $\phi\in \M_d$ we have $\phi^\trans M \phi \leq \phi^\trans M' \phi$. Furthermore if $M,M' \in S_d^+$ and $M\leq M'$ then $M'^{-1} \leq M^{-1}$. For each symmetric positive definite matrix $M\in S_d^+$ we define a norm $\|\cdot\|_M$ as follows: for all $u\in \R^d$
$$
\|u\|^2_M := u^\trans M u.
$$

\subsection{Geometry of the simplex}
\label{subsecIntroSimplex}
The basic geometrical object studied in this chapter is the $d$-dimensional simplex, which is defined as follows.
\begin{definition}
A $d$-dimensional simplex $T$ is the convex envelope of a set $V\subset \R^d$ of $d+1$ %non-coplanar 
vertices, not contained in a $d-1$ dimensional affine subspace of $\R^d$ : 
$$
T = \Cvx(V).
$$
We denote by $\cF(T)$ the collection of faces of $T$ of any dimension,
\be
\label{defFT}
\cF(T) := \{\Cvx(V') \sep V'\subset V\}.
\ee
\end{definition}
Observe that $\emptyset$ and $T$ are among the faces of a simplex $T$, since they respectively correspond to $V'=\emptyset$ and $V'=V$.
We denote by $z_T\in \R^d$ the barycenter of a simplex $T$ of vertices $V$
$$
z_T := \frac 1 {d+1} \sum_{v\in V} v,
$$
and we define a symmetric positive definite matrix $\cH_T\in S_d^+$ as follows
\be
\label{defcH}
\cH_T^{-1} = \frac d {d+1} \sum_{v\in V} (v-z_T) (v-z_T)^\trans. %\frac {2d}{(d+1)^2}\sum_{v,v'\in V} (v-v')(v-v')^\trans. 
\ee
Some of the key properties of the matrix $\cH_T$ are exposed in the next proposition.
Throughout this chapter, we denote by $\TEq$ a $d$-dimensional equilateral simplex, centered at the origin
i.e. such that $z_\TEq=0$, and having its vertices on the unit ball. One easily checks that 
$$
\cH_\TEq = \Id.
$$
% Note that 
%\be
%\label{eqBallTEq}
%%\{z\in \R^d \sep |z| \leq 1/d\} 
%B(0, 1/d) \subset \TEq \subset \overline B(0,1).
%\ee
%
%%We associate to any simplex $T$ its barycenter $z_T\in \R^d$, and a symmetric positive definite matrix
%We denote by $z_T$ the barycenter of a simplex $T$, and we also associate to $T$ a symmetric positive definite matrix $\cH_T\in S_d^+$ which encodes some of its geometrical properties, in particular the volume, the elongation and the orientation of $T$.
\begin{prop}
\label{propHT}
The following holds for any $d$-dimensional simplex $T$. 
\begin{itemize}
\item
For any an affine change of coordinates $\Phi$, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0$ in $\R^d$, we have 
\be
\label{invcH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
\item
There exists a rotation $U\in \cO_d$, depending on $T$, such that 
\be
\label{eqcHTEq}
\cH_T^\frac 1 2 (T-z_T) = U(\TEq),
\ee
hence 
\be
\label{eqVolTHT}
|T| \sqrt{\det \cH_T} = |\TEq|.
\ee
\item
We have the inclusions 
\be
\label{eqTET}
\{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1/d\} \subset T \subset \cE_T := \{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1\},
\ee
and the these two ellipsoids are respectively the one of largest volume included in $T$, and of smallest volume containing $T$.
\end{itemize}
\end{prop}
\proof
For any simplex $\Phi^{-1}(v)$ of the simplex $\Phi^{-1}(T)$, we have 
$$
\Phi^{-1}(v)-z_{\Phi^{-1}(T)} = \Phi^{-1}(v)-\Phi^{-1}(z_T) = \phi^{-1}(v-z_T).
$$
Injecting this relation in \iref{defcH} we obtain \iref{invcH}. 
We now turn to the proof of \iref{eqcHTEq} and for that purpose we remark that the simplices $\TEq$ and $T' := \cH_T^\frac 1 2 (T-z_T)$ have both their barycenter at zero, $z_\TEq = z_{T'} = 0$, hence there exists a linear map $\phi\in \GL_d$ such that $T' = \phi^{-1}(\TEq)$. We thus obtain, using the formula \iref{invcH} for the transformation of $\cH_T$ under affine change of coordinates 
$$
\begin{array}{ccccc}
\cH_{T'} &=& \cH_T^{-\frac 1 2} \cH_T \cH_T^{-\frac 1 2} &=& \Id \\ 
\cH_{\phi^{-1}(\TEq)} &=& \phi^\trans \cH_\TEq &=& \phi^\trans \phi.
\end{array}
$$
Hence $\phi^\trans \phi= \Id$ which establishes that $\phi\in \cO_d$ and concludes the proof of \iref{eqcHTEq}.
%One easily checks that 
%$$
%\overline B(0,1/d) \subset \TEq \subset \overline B(0,1),
%$$
%where
It is well known that the smallest ellipsoid containing $\TEq$ is the unit ball, and that the largest ellipsoid included in $\TEq$ is the ball of radius $1/d$. Combining this fact with the change of coordinates \iref{eqcHTEq} we obtain \iref{eqTET} which concludes the proof of this proposition.
\sq

Note that for any simplex $T$ and any $z,z'\in T$ we obtain using \iref{eqTET}
\be
\label{eqDiamTHT}
\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2.
\ee

We introduce a measure of degeneracy $\rho(T)$ of a $d$-dimensional simplex $T$
\be
\label{defRhoMM}
\rho(T) := \sqrt{\|\cH_T\| \|\cH_T^{-1}\|}.
\ee
%This measure of non degeneracy $\rho$ is slightly different from the measure of non degeneracy $\frac {\diam(T)^d} {|T|}$ used in some of the previous chapters. However these two measures play a similar role and can be compared. Indeed we obtain using \iref{eqVolTHT} and \iref{eqcTET}
%\be
%\label{eqRhoRhop}
%\frac{\rho(T)}{d^\frac d 2|\TEq|} \leq  \frac{(\|\cH_T^{-1}\|/d)^\frac d 2} {|\TEq| (\det \cH_T)^{-\frac 1 2}} \leq \frac{\diam(T)^d} {|T|} \leq \frac{\|\cH_T^{-1}\|^\frac d 2} {|\TEq|(\det \cH_T)^{-\frac 1 2}}\leq \frac{\rho(T)^{d-1}}{|\TEq|}.
%\ee
%Observing that $\|A\| \|A^{-1}\|^{-(d-1)} \leq |\det A| \leq \|A\|^{d-1} \|A^{-1}\|^{-1}$ for any $A\in \GL_d$
%it follows that 
Observe that $\rho(T)\geq 1$ for any simplex $T$, with equality if and only if $\cH_T$ is proportional to the identity, which implies in view of \iref{eqcHTEq} that $T$ is a displacement of the equilateral simplex $\TEq$:
$$
\rho(T) = 1 \stext{ if and only if }
%\ \Longleftrightarrow \ 
T = z_T+r U(\TEq) \text{ for some }  r>0 \text{ and } U \in \cO_d.
$$
The measure of degeneracy $\rho$ is slightly different from the measure of degeneracy $\frac {\diam(T)^d} {|T|}$ used in Chapters \ref{chapOptAniso} and \ref{chapW1P} but both have the same role: they are minimal for the equilateral simplex, and increase as the simplex becomes thinner.\\

The measure of sliverness $S(T)$ of a simplex $T$ is a quantity which plays an important role in the context of optimal mesh adaptation for the finite element approximation of a function in the Sobolev $W^{1,p}$ norm, see   \cite{Ba, Ja}, and Chapters \ref{chapW1P} and \ref{chapApproxMet}. 
This measure of sliverness is defined in Chapter \ref{chapW1P} and illustrated by several examples and equivalent quantities. We recall the definition of this quantity
\be
\label{defSMM}
S(T) := \inf \{ \|\phi\| \|\phi^{-1}\| \sep \phi \in \GL_d \text{ and } \phi(T) \text{ is acute } \},
\ee
a simplex is acute if the exterior normals $\n, \n'$ to any two distinct faces of $T$ have a negative scalar product $\<\n,\n'\>\leq 0$.
As observed in Chapter \ref{chapW1P}, the measure of sliverness $S(T)$ can be interpreted as the distance from $T$ to the collection of acute simplices.

The exterior normals $\n,\n'$ to any two $d-1$-dimensional faces of $\TEq$ satisfy $\<\n,\n'\> =-1/d$, hence this simplex is acute. Recalling \iref{eqcHTEq}
 we thus obtain for any simplex $T$
$$
S(T) \leq \rho(T).
$$
Apart from this upper bound, the matrix $\cH_T$ does not contain any direct information on the measure of sliverness $S(T)$.
%One of the key results of this chapter is that in a bidimensional triangulation $\cT$, and conjecturedly in higher dimension too, the variation of the matrix $\cH_T$ as $T$ varies in $\cT$ does encode the measure of sliverness in some sense.
For any bidimensional triangle $T$ of largest angle $\theta$, Proposition \ref{propSTan} of Chapter \ref{chapW1P} states that :
$$
S(T) = \max\left\{1, \tan \frac \theta 2 \right\}.
$$

\subsection{Simplicial meshes}
\label{subsecDefTStar}

As a starter, we recall the definition of a simplicial mesh of $\R^d$.
%We first briefly recall the defini
%Before introducing simplicial meshes, we briefly recall the definition of locally finite partitions of $\R^d$.

%In order to introduce q,xcl meshes 
\begin{definition}
\label{defSimplMesh}
A conforming simplicial mesh of $\R^d$ is a collection $\cT$ of simplices which satisfy the conformity axiom :  for all $T,T'\in \cT$
\be
\label{confAxiom}
T\cap T' \in \cF(T) \cap \cF(T'),
\ee
as well as the following properties
\begin{itemize}
\item (Covering) The simplices $T\in \cT$ cover the whole infinite domain $\R^d$:
$$
\bigcup_{T\in \cT} T = \R^d.
$$
\item (Partition) The interiors of the simplices $T\in \cT$ are pairwise disjoint: for any $T,T'\in \cT$,
$$
\interior (T) \cap \interior(T') \neq \emptyset\stext{ implies }  T=T'. %
$$
\item (Local finiteness) For any compact set $K \subset \R^d$, only a finite collection of simplices $T\in \cT$ intersect $K$:
$$
\{T \in \cQ \sep K \cap T \neq \emptyset \} \ \text{ is finite.}
$$
\end{itemize}
\end{definition}
The conformity axiom \iref{confAxiom} states that the intersection of any two simplices in $\cT$ needs to be a full common face.We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$.

For an optimal efficiency, numerous numerical simulation software use anisotropic meshes, in which the simplices may have an arbitrary shape. Anisotropic meshes are used for instance, to create a thin layer of simplices close to a geometric feature which is relevant in a numerical simulation.
In order to avoid excessively wild meshes, one often requires relevant  some consistency between the shapes of neighboring simplices.We therefore introduce for any constant $C \geq 1$ the class $\bT_{g,C} \subset \bT$ of \emph{graded} meshes, which is defined as follows.
A mesh $\cT$ belongs to $\bT_{g,C}$ if for any two simplices $T,T'\in \cT$ one has 
\be
\label{defTG}
T \cap T'\neq \emptyset \stext{ implies } C^{-2}\cH_T \leq \cH_{T'} \leq C^2 \cH_T.
\ee

For any $C\geq 1$ we also introduce the class $\bT_{i,C}$ of \emph{isotropic} meshes, by requiring that in addition to \iref{defTG} that the measure of degeneracy $\rho$ is uniformly bounded by $C$, which forbids any anisotropy.
A mesh $\cT$ belongs to $\bT_{i,C}$ if and only if $\cT\in \bT_{g,C}$ and for all $T \in \cT$
$$
\rho(T) \leq C. %C \geq 1? or 0? 
$$

%The next proposition shows that the definition of $\bT_{i,C}$ is slightly redundant, in the sense that condition \iref{defTG} could be avoided.
%\begin{prop}
%Denote by $\bT'_{i,C}$ the collection of meshes $\cT\in \bT$ satisfying $\rho(T) \leq C$ for all $T\in \cT$ (but perhaps not the gradedness condition \iref{defTG}). %We thus have $\bT_{i,C} \subset \bT'_{i,C}$.\\
%Then for all $C$ there exists $C' = C'(C)$ such that 
%$$
%\bT_{i,C} \subset \bT'_{i,C} \subset \bT_{i,C'}.
%$$
%\end{prop}
%
%\proof
%See appendix. 
%\sq

In order to introduce the intermediate collection $\bT_{a,C}$ of $C$-quasi-acute meshes, we first define the notion of refinement of a simplicial mesh.
\begin{definition}
Consider two meshes $\cT,\cT'\in \bT$ and a constant $C\geq 1$. We say that $\cT'$ is a $C$-refinement of $\cT$ if it satisfies the following properties.
\begin{itemize}
\item (Inclusion) Any simplex $T'\in \cT'$ is contained in a simplex $T\in \cT$. % such that $T'\subset T$.
\item (Bounded refinement) Any simplex  $T\in \cT$, contains most $C$ simplices $T'\in \cT$.
\end{itemize}
\end{definition}

A graded mesh $\cT \in \bT_{g,C}$ belongs to the collection $\bT_{a,C}$ of quasi-acute meshes if and only there exists a $C$-refinement $\cT'$ of $\cT$ which satisfies for all $T' \in \cT'$
$$
S(T') \leq C.
$$
In particular if $\cT\in \bT_{i,C}$, then choosing $\cT' = \cT$, which is a $C$-refinement since $C\geq 1$, and recalling that $S(T) \leq \rho(T)$ for any simplex $T$, we obtain that $\cT\in \bT_{a,C}$. Thus $\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}$ as announced.

The constraints defining graded, quasi-acute and isotropic meshes are illustrated on Figure \ref{figDisk}
in the main introduction of the thesis. 
Figure \ref{figAcuteGen} gives an example of a quasi-acute triangulation which 
by the above described refinement process leads to a slightly finer triangulation on
sliverness $S(T)$ is uniformly bounded.

\begin{figure}
\centering
%	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarGdeVap.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap1.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap2.pdf}
	\caption{\label{figAcuteGen}
Quasi-acute triangulation (left) and refined triangulation with uniformly bounded sliverness (right).
	}
\end{figure}

\subsection{Riemannian metrics}
\label{subsecDefHStar}

For any metric $H \in \bH$ and path $\gamma \in C^1([a,b],\R^d)$, we define the riemmannian length $l_H(\gamma)$ by the integral
$$
l_H(\gamma) := \int_a^b \|\gamma'\|_{H(\gamma(t))} dt.
$$
The riemmannian distance $d_H$ between two points  $z,z'\in \R^d$, is the infimum of the length of all paths joining $z$ and $z'$, 
\be
\label{defdH}
d_H(z,z') := \inf\left\{l_H(\gamma)\sep \gamma\in C^1\left([0,1],\R^d\right), \ \gamma(0) = z \text{ and } \gamma(1) = z'\right\}.
\ee
If $H, H'\in \bH$ are such that $H(z) \leq H'(z)$ for all $z\in \R^d$, then $d_H(z,z') \leq d_{H'}(z,z')$ for all $z,z'\in \R^d$.
By construction, the riemannian distance $d_H$ associated to a metric $H\in \bH$ is locally equivalent close to a point $z$ to the distance defined by the norm $\|\cdot \|_{H(z)}$: for all $z\in \R^d$
\be
\label{eqDistLoc}
\limsup_{\ve \to 0} \sup_{p,q\in B(z, \ve)} |\ln d_H(p,q) - \ln \|p-q\|_{H(z)}| = 0,
\ee
where $B(z,\ve)$ denotes the euclidean ball of radius $\ve$ around $z$.\\


\begin{remark}[Riemannian geodesics]
When a metric $H$ is sufficiently smooth, a special family of curves named Riemannian geodesics can be defined and studied. A riemannian geodesic is a curve $\gamma\in C^0(\R, \R^d)$ which satisfies a second order differential equation %written in terms of the second order derivatives of $H$, 
called the equation of geodesics. This equation implies that for any sufficiently close $t,t'\in \R$ the curve $\gamma_{|[t,t']}$ is the path of smallest possible length joining the points $\gamma(t)$ and $\gamma(t')$ : 
$d_H(\gamma(t), \gamma(t')) = l_H(\gamma_{|[t,t']})$.

Geodesics are not defined for general continuous or Lipschitz riemannian metrics, such as those constituting the sets $\bH$ and $\bH_i \subset \bH_a\subset \bH_g$, since the coefficients of the equation of geodesics involve the second derivatives of the metric. Notions related to geodesics, such as the injectivity radius of a metric, therefore have no meaning in our context.
This is not an issue for our purposes since, following the point of view of \cite{Gromov},
%[Gromov, Metric structures for Riemannian and non-Riemannian spaces, Birkhauser (1999)]
we study Riemannian distances and not Riemannian geodesics. 

%Note also that geodesics only exist when the metric $H$ has requires that $H$ has at least $C^2$ smoothness, while the metrics studied in this chapter generally only have $C^0$ or Lipschitz smoothness.

%Since we only assume that $H$ is a continuous metric, the infimum \iref{defdH} may or may not be attained, and in that later case possibly for several paths. The equation of geodesics associated to a riemannian metric involves the second order derivatives, which are not defined in our context.
%(* also the point of view of Gromov : we study distances and not geodesics*)
\end{remark}


We denote by $\bH_i$ the collection of metrics $H \in \bH$ which are proportionnal to the identity: for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2},
$$
and such that the proportionality factor $s$ satisfies one of the two following conditions conditions, which are surprisingly equivalent as shown in Proposition \ref{propEquivS}:
\begin{itemize}
\item (``Additive'' Lipschitz condition)  
\be
\label{eqLipSAdd}
|s(z) - s(z')| \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
\item (``Multiplicative'' Lipschitz condition)
\be
\label{eqLipSMult}
|\ln s(z) - \ln s(z')| \leq d_H(z,z') \stext{ for all } z,z'\in\R^d.
\ee
\end{itemize}

The two Lipschitz properties \iref{eqLipSAdd} and \iref{eqLipSMult} have a natural generalisation to general anisotropic metrics but are not equivalent in that context.
In order to introduce the regularity conditions defining the classes $\bH_i\subset \bH_a\subset \bH_g$ of metrics, we need to  two distances $d_\times$ and $d_+$ on the set $S_d^+$ of symmetric positive definite matrices. 
For any $M,M'\in S_d^+$ we define
\be
\label{defDTimes}
d_\times (M,M') := \min \{\delta \geq 0 \sep e^{-2\delta} M \leq M' \leq e^{2 \delta} M\}.
\ee
For instance, a mesh $\cT$ is $C$-equivalent to a metric $H$, as defined in \iref{defEquiv}, if and only if for all $T \in \cT$ and all $z\in \cT$ one has 
$$
d_\times (H(z), \cH_T) \leq \ln C.
$$
There exists various expressions of the distance $d_\times$ : for all $M,M'\in S_d^+$ one has 
\be
\label{eqDTimesLog}
d_\times (M,M') = \sup_{u\in \sR^d\sm \{0\}} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
\ee
and 
\be
\label{eqDTimesProd}
d_\times (M,M') = \ln \left(\max \{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\}\right).
\ee
The exponential of the distance $d_\times$ was used in the earlier paper \cite{Shew} %on anisotropic mesh generation
under the name ``relative deformation''. 
We define a second distance $d_+$ on $S_d^+$ as follows 
\be
\label{defDPlus}
d_+(M,M') := \|M^{-\frac 1 2} - M'^{-\frac 1 2}\|.
\ee
The expressions \iref{eqDTimesProd} and \iref{defDPlus} of the distances $d_\times$ and $d_+$ show that they are respectively tied to multiplicative or additive properties of matrices, which justifies their notations.
Note also that for any $s,s'>0$ one has
\be
\label{eqDIso}
d_\times (s^{-2} \Id, s'^{-2} \Id) = |\ln s - \ln s'| \stext{ and } d_+(s^{-2} \Id, s'^{-2} \Id) = |s-s'|.\\
\ee

We denote by $\bH_g$ the collection of metrics $H\in \bH$ which satisfy the natural extension of \iref{eqLipSMult} to general anisotropic metrics:
\be
\label{eqLipMult}
d_\times (H(z), H(z')) \leq d_H(z,z') \stext{ for all }z,z'\in\R^d.
\ee
This condition can be heuristically described as follows: a metric $H\in \bH$ defines close to each point $z\in\R^d$ a norm $\|\cdot\|_{H(z)}$ which encodes an anisotropic notion of scale. The equation \iref{eqLipMult} states that the metric $H$ itself is consistent a the scale that it encodes.\\

We denote by $\bH_a$ the collection of metrics $H\in \bH$ which satisfy both \iref{eqLipMult} and the natural extension of \iref{eqLipSAdd} to general anisotropic metrics:
\be
\label{eqLipAdd}
d_+ (H(z), H(z')) \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
In addition to the results of mesh generation presented in this chapter, we show in the next chapter, Chapter\ref{chapApproxMet}, that this condition is critical in order to define a local averaging operator compatible with Sobolev norms. 
%decrire le lien avec les angles aigus.
\begin{remark}
\label{remHomog}
Let $H\in \bH$, and let $\lambda>0$. Using the homogeneity properties of the distances $d_\times$, $d_+$ on $S_d^+$ and $d_H$ on $\R^d$ with respect to $H$, we obtain that $\lambda^2 H\in \bH_g$ if and only if 
\be
\label{eqLipTimesLambda}
d_\times (H(z), H(z')) \leq \lambda d_H(z,z') \stext{ for all } z,z'\in \R^d, 
\ee
and $\lambda^2 H\in \bH_a$ if and only if we have in addition to the previous property 
\be
\label{eqLipPlusLambda}
d_+ (H(z), H(z')) \leq \lambda |z-z'| \stext{ for all } z,z'\in \R^d.
\ee
In particular the collections $\bH_i \subset \bH_a \subset \bH_g$ of isotropic, quasi-acute and graded metrics are stable under multiplication by a constant larger than one : for any $\star \in \{a,b,c\}$, any $H\in \bH_\star$ and any $\lambda \geq 1$ we have $\lambda^2 H\in \bH_\star$.
%this operation corresponds to the uniform refinement of a triangulation...
\end{remark}

\subsection{Main results}

The main result of this chapter is the equivalence of the classes of meshes and metrics defined above, which is  announced in the first part of the introduction and proved in sections \S\ref{secMeshToMet} and  \S \ref{secMetToMesh}. In two cases we were only able to establish this equivalence when the dimension is $d=2$. 
\begin{theorem}
\label{thEquiv}
There exists $C_0 = C_0(d)$ such that for all $C\geq C_0$ the following holds.
\begin{enumerate}[i)]
\item The collections $\bT_{i,C}$ of triangulations and $\bH_i$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{a,C}$ of triangulations and $\bH_a$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{g,C}$ of triangulations and $\bH_g$ of metrics are equivalent.
\end{enumerate}
\end{theorem}

Let us comment on this result.
The theory of isotropic meshes is already well developed, and our result i) in this direction should be regarded as a reformulation of previous work, intended to put into perspective the results on anisotropic meshes. The main ingredient of the proof of i) is the mesh refinement procedure exposed in \cite{Nochetto}. 

In the case iii) of graded metrics the key ingredients used for the construction of a bidimensional triangulation $\cT\in \bT_{g,C}$ equivalent to a metric $H \in \bH_g$ come from the paper of computational geometry \cite{Shew}. In contrast the arguments used to produce a metric $H \in \bH_g$ from a mesh $\cT \in \bH_{g,C}$ hold in any dimension.

Last the author has not heard of any anterior results on the collection $\bT_{a,C}$ of quasi-acute meshes, and most of the techniques used in that context are new. 
The author is sorry to say that the proofs in that case are not yet as polished as the rest of the thesis, due to time constraints.

\begin{conjecture}
The author conjectures that the points ii) and iii) of Theorem \ref{thEquiv} holds without restriction on the dimension $d$.
\end{conjecture}

This chapter is organised as follows. We establish in section \S \ref{secMetProp} some general properties of metrics in $\bH_a$ or $\bH_g$. 
We first prove in \S\ref{subsecMetInv} a property of invariance of the collection $\bH_g$ of graded metrics with respect to affine changes of coordinates.
The regularity assumptions \iref{eqLipMult} and \iref{eqLipAdd} defining graded and quasi-acute metrics simply mean that the map $H : \R^d \to S_d^+$ is Lipschitz with respect to some distances on $\R^d$ and $S_d^+$. 
We therefore study metrics from this point of view in \S\ref{subsecMetLip}.
We focus in \S\ref{subsecMetGeom} on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. In particular we compare the $d_H$ with the euclidean distance and we estimate the volume of balls. 


Section \S\ref{secEigen} is devoted to the study of metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has  an eigenspace of dimension at least $d-1$ at each point. This condition clearly holds if the dimension is $d=2$ but is also relevant in some applications to higher dimension such as the creation of a this layer of simplices close to a $d-1$ dimensional surface. This situation is discussed in Chapter \ref{chapApproxMet}, and involves metric which have an eigenvalue much larger that the others in the orthogonal direction to the surface of interest.
We give an approximate translation of the regularity properties \iref{eqLipAdd} and \iref{eqLipMult} defining the collections $\bH_a$ and $\bH_g$ of metrics in terms of the two eigenvalues of $H$ and of the direction of the eigenspaces of such metrics. 

The last two sections \S\ref{secMeshToMet} and \S\ref{secMetToMesh} are devoted to the proof of Theorem \ref{thEquiv}. More precisely we adress in \S\ref{secMetToMesh} the production of an isotropic, quasi-acute or graded mesh equivalent to a given metric $H\in \bH_i$, $\bH_a$ or $\bH_g$. Conversely we depict in \S\ref{secMeshToMet} to construction of a metric which is equivalent to a given mesh.


\section{General properties of graded and quasi-acute metrics}
\label{secMetProp}

We study in this section the general properties of the  distinguished classes of metrics $\bH_i \subset \bH_a \subset \bH_g$. 
We first establish in \S\ref{subsecMetInv} some invariance properties of these collections of metrics with respect to affine changes of coordinates.
We then regard in \S\ref{subsecMetLip} metrics as Lipschitz functions $H : \R^d\to S_d^+$. %, and we recall some basic properties of these.
The last subsection \S\ref{subsecMetGeom} is devoted to the comparison of the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$, with respect to the standard euclidean distance and Lebesgue measure.

\subsection{Invariance properties and restriction of metrics}
\label{subsecMetInv}

We focus in this subsection on the properties of invariance of the collections of meshes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ and of metrics $\bH_i \subset \bH_a\subset \bH_g$ introduced in this chapter.

Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$.
We have for any simplex $T$, as previously observed in \iref{invcH},
\be
\label{eqInvH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
Mimicking this property we define for any $H \in \bH$ a transported version $H_\Phi\in \bH$ as follows: for all $z\in \R^d$
\be
\label{defHPhi}
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi.
\ee
In the language of differential geometry,
the metric $H_\Phi$ is generally referred to as the ``pull back'' of $H$ by $\Phi$. If a mesh $\cT\in \bT$ is $C$-equivalent to a metric $H\in \bH$, then \iref{eqInvH} and \iref{defHPhi} clearly imply that the mesh $\Phi^{-1}(\cT)$ is $C$-equivalent to the metric $H_\Phi$.

The next proposition studies the invariance of the collections $\bT_{\star,C}$ of meshes and $\bT_\star$ of metrics, $\star \in \{i,a,g\}$, under the transformations $\cT \mapsto \Phi^{-1}(\cT)$ or $H \mapsto H_\Phi$ induced by an affine change of coordinates $\Phi$.

\begin{prop}
\label{propInvT}
Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. 
The following holds for any constant $C\geq 1$.
\begin{enumerate}[i)]
\item If $\cT \in \bT_{g,C}$ then $\Phi^{-1}(\cT) \in \bT_{g,C}$. If $H \in \bH_g$ then $H_\Phi\in \bH_g$.
\item Assume that $\Phi$ is an isometry, in other words $\phi\in \cO_d$.\\
If $\cT\in \bT_{a,C}$ then $\Phi^{-1}(\cT)\in \bT_{a,C}$, and similarly if $\cT\in \bT_{i,C}$ then $\Phi^{-1}(\cT)\in \bT_{i,C}$.\\
If $H\in \bH_a$ then $H_\Phi\in \bH_a$, and similarly if $H\in \bH_i$ then $H_\Phi\in \bH_i$.
\end{enumerate}
\end{prop}

\proof
%We concentrate on the case of meshes, since the statements on metrics are a special case of the propositions (??) and (??) below (* no : state the result for iso and quasi acute metrics too*).
%We first consider the case of meshes, and then 
We first establish the properties announced for meshes, and we then focus on metrics.
Let $M,M'\in S_d^+$, let $C\geq 1$ and let $\phi\in \GL_d$. Clearly
$$
\text{ if } C^{-2} M \leq M' \leq C^2 M \stext{ then } C^{-2} \phi^\trans M\phi \leq \phi^\trans M'\phi  \leq C^2 \phi^\trans M\phi.
$$
%Consequently if a mesh $\cT$ satisfies the condition \iref{defTG} defining the elements of $\bT_{g,C}$
%
%satisfy $C^{-2} M \leq M' \leq C^2 M$, then we also ha
%For any $M,M'\in S_d^+$ we obtain using \iref{defDTimes} that 
%$$
%d_\times (\phi^\trans M \phi,\ \phi^\trans M' \phi) = d_\times (M,M').
%$$
%It follows using \iref{eqInvH} that for any  two simplices $T,T'$,
%$$
%d_\times (\cH_{\Phi^{-1}(T)}, \cH_{\Phi^{-1}(T')}) = d_\times (\cH_T,\cH_{T'}).
%$$ 
In view of the definition \iref{defTG} of $\bT_{g,C}$ we obtain that $\Phi^{-1}(\cT)\in \bT_{g,C}$ for any mesh $\cT\in\bT_{g,C}$ as announced in i).

If $\Phi$ is an isometry then for any simplex $T$ we obtain, using the definitions \iref{defRhoMM} and \iref{defSMM} of the measure of degeneracy $\rho$ and the measure of sliverness $S$, that
$$
\rho(\Phi^{-1}(T)) = \rho(T) \stext{ and } S(\Phi^{-1}(T)) = S(T).
$$
This implies the properties of $\bT_{a,C}$ and $\bT_{i,C}$ announced in b), which concludes the proof of the properties announced for meshes.

We therefore turn our attention to metrics. The fact that $H_\Phi\in \bH_g$ for any $H\in \bH_g$ and any affine change of coordinates $\Phi$ is a special case of Proposition \ref{propHG} below. We thus admit this property and we focus on isotropic and graded metrics and isometric changes of coordinates.

If $H\in \bH_i$, then $H = \Id/s(z)^2$ where $s: \R^d \to \R_+^*$ is a Lipschitz function. Since $\phi\in \cO^d$ we have $\phi^\trans \phi = \Id$ and therefore 
$$
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi = \Id/s(\Phi(z))^2.
$$
The map $s \circ \Phi : \R_d\to \R_+^*$ is Lipschitz since it is the composition of a Lipschitz function with an isometry, which establishes that $H_\Phi\in \bH_i$ as announced.

If $H\in \bH_a$ and $\Phi$ is an isometry, then for any $z,z'\in \R^d$
\begin{eqnarray*}
\|H_\Phi(z)-H_\Phi(z')\| &=& \|\phi^\trans \left(H(\Phi(z))-H(\Phi(z'))\right) \phi\| \\
&=& \|H(\Phi(z))-H(\Phi(z'))\|\\
& \leq& \|\Phi(z)-\Phi(z')\|\\
& =& \|\phi(z-z')\|= |z-z'|,
\end{eqnarray*}
which establishes that $H_\Phi$ satisfies the Lipschitz regularity condition \iref{eqLipAdd}. We already know from the case of graded metrics that the other regularity condition \iref{eqLipMult} is satisfied by $H_\Phi$, which establishes that $H_\Phi\in \bH_a$ and concludes the proof of this proposition.
\sq


In practical applications, one often needs to mesh simultaneously a domain $\Omega$ and a surface $\Gamma$ embedded in $\Omega$. In terms of metric this raises the following question: given a metric $H$ on $\Omega$ which satisfies certain properties of regularity %, corresponding do a certain class of meshes, 
what is the regularity of the restriction of this metric to $\Gamma$?

The next proposition answers this question is the simplified setting where $\Omega$ is the infinite domain $\R^d$, $\Gamma$ is an affine subspace of $\R^d$, and properties of regularity are those defining the collection $\bH_g$ of graded metrics. For any $1\leq k \leq d$ we denote by $\bH_g(\R^k)$ the collection of graded metrics on $\R^k$.

\begin{prop}
\label{propHG}
Let $1\leq k\leq d$, let $\Phi : \R^k\to \R^d$ be an affine injective map, $\Phi(z) = \phi z+z_0$ where $\phi\in M_{d,k}$ has rank $k$ and $z_0\in \R^d$. Let $H\in \bH$ and let for all $z\in \R^k$
$$%\be
%\label{defHPhi}
H_\Phi(z) := \phi^\trans H(\Phi(z)) \phi.
$$%\ee
If $H\in \bH_g$ then $H_\Phi\in \bH_g(\R^k)$. 
\end{prop}

\proof
For any $u\in \R^d$, one has 
\be
\label{chgNorm}
\|u\|_{H_\Phi(z)} = \|\phi(u)\|_{H(\Phi(z))}.
\ee
Hence for any $z,z'\in \R^k$ we obtain using \iref{eqDTimesLog},
\be
\label{dNHPhi}
\begin{array}{rcl}
d(H_\Phi(z), \ H_\Phi(z'))  &=&\displaystyle \sup_{u\in \sR^k\sm\{0\}} \left|\ln \left\|\phi(u)\right\|_{H(\Phi(z))} -\ln \left\|\phi(u)\right\|_{H(\Phi(z'))}\right| \\
& \leq& d(H(\Phi(z)), \  H(\Phi(z')))
\end{array}
\ee
For any path $\gamma\in C^1([0,1], \R^k)$, it follows from \iref{chgNorm} that % the distorted lengths tied to $H$ and $H_\phi$ are therefore linked by 
$$
l_H(\Phi\circ \gamma) = \int_0^1 \|\phi(\gamma'(t))\|_{H(\Phi(\gamma(t)))}dt =  l_{H_\Phi}(\gamma).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^k)$ joining two points $z,z'\in \R^k$, we obtain since $\Phi\circ \gamma\in C^1([0,1], \R^d)$ is a path joining $\Phi(z)$ and $\Phi(z')$
\be
\label{dHPhi}
d_H(\Phi(z), \Phi(z')) \leq d_{H_\Phi}(z,z')
\ee
Combining \iref{dNHPhi} and \iref{dHPhi}, we conclude the proof of this proposition.
\sq


\subsection{Metrics as Lipschitz functions}
\label{subsecMetLip}
Lipschitz functions play an important role in this chapter and in particular in this section. We recall here their basic properties.
If $(X,d_X)$ and $(Y,d_Y)$ are two metric spaces, and if $f \in C^0(X , Y)$, we define 
the dilatation $\dil(f) \in [0, \infty]$ of $f$ as follows
$$
\dil(f) := \sup_{\substack{x,x'\in X \\ x \neq x'}} \frac{d_Y(f(x),f(x'))}{d_X(x,x')}
$$

We say that $f$ is Lipschitz if $\dil(f) \leq 1$, and more generally that $f$ is $\lambda$-Lipschitz if $\dil(f) \leq \lambda$.
We define the local dilatation $\dil_x(f)$ of a function $f\in C^0(X,Y)$ at a point $x\in X$ as follows
\be
\label{defDilX}
\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
\lim_{\ve\to 0} \left(\sup_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
\ee
%\be
%\label{defDilX}
%\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
%\lim_{\ve\to 0} \left(\sup_{e,e'\in B(x,\ve)} \frac{d_Y(f(e),f(e'))}{d_X(e,e')}\right).
%\ee
We specify the distance function on $X$ or $Y$ if it is not the expected ``canonical one'', in particular if $X$ or $Y$ is a subset of $\R^k$ and if the associated distance is not the standard euclidean distance but the riemannian distance $d_H$ associated to a metric, or if $X$ or $Y$ is the collection $S_d^+$ of symmetric positive definite matrices since none of the two distances $d_+$ or $d_\times$ is canonical. The local dilatation is in that case denoted as follows
$$
\dil_x(f\sep d_X, d_Y), \quad \dil_x(f\sep d_X)  \stext{ or } \dil_x(f\sep d_Y).
$$

The local dilatation $\dil_x(f)$ only depends on the local properties of the metric spaces close to $x$ and $f(x)$. Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$. For any $f\in C^0(\R^d, Y)$ and any $z\in \R^d$ we obtain using \iref{eqDistLoc}
\be
\label{eqDilNorm}
\|H(z)^{-1}\|^{-\frac 1 2} \dil_z(f) \leq \dil_z(f\sep d_H) = \dil_z(f \sep \|\cdot \|_{H(z)}) \leq \sqrt{\|H(z)\|} \dil_z(f)
\ee
We also introduce the lower local dilatation $\dil_z^*(f)\leq \dil_z(f)$ which is defined as follows
$$
\dil_z^*(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
$$
The next proposition establishes that local dilatations are sub-multiplicative.
\begin{lemma}
\label{lemmaSubMult}
Let $(X,d_X)$, $(Y,d_Y)$ and $(Z,d_Z)$ be three metric spaces, and let $f\in C^0(X,Y)$ and $g\in C^0(Y,Z)$. 
For any $x\in X$ one has 
\be
\label{eqDilUpper1}
\dil_x(g \circ f) \leq \dil_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side. Similarly we have 
\be
\label{eqDilLower1}
\dil_x(g \circ f) \geq \dil^*_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side.
\end{lemma}

\proof
We first establish \iref{eqDilUpper1}.
If $\dil_x(f) = \infty$ or $\dil_{f(x)}(g) = \infty$, then there is nothing to prove. We may therefore assume that $\dil_x(f) < \infty$ and $\dil_{f(x)}(g) < \infty$.
For any $\ve>0$ we define 
$$
F(\ve) = \sup_{p,q\in B(x, \ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)} \stext{ and } G(\ve) := \sup_{p,q\in B(f(x), \ve)} \frac{d_Z(g(p),g(q))}{d_Y(p,q)}
$$
It follows that 
$$
\sup_{p,q\in B(x, \ve)} \frac{d_Z(g(f(p)),g(f(q)))}{d_X(p,q)} \leq F(\ve) \, G(F(\ve) \ve).
$$
Taking the limit as $\ve \to 0$ we obtain \iref{eqDilUpper1} which concludes the proof.
For the proof of \iref{eqDilLower1} we consider two sequences $(p_n)_{n \geq 0}$, $(q_n)_{n \geq 0}$ which both tend to $x$ and such that $d_Y(f(p_n),f(q_n))/d_X(p_n, q_n) \to \dil_x(f)$ as $n \to \infty$. We thus have 
$$
\frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_X(p_n,q_n)} = \frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_Y(f(p_n),f(q_n))} \times \frac{d_Y(f(p_n),g(f(q_n)))}{d_X(p_n,q_n)},
$$
and taking the limit as $n \to \infty$ we obtain \iref{eqDilLower1} which concludes the proof of this lemma.
\sq

Let $f: \Omega \to V$ be a $C^1$ function, where $\Omega\subset \R^d$ is an open set and $V$ is a Banach space. Then for any $z\in \Omega$ the local dilatation $\dil_z(f)$, and the lower dilatation $\dil_z^*(f)$ only depend on the differential $d_z f : \R^d \to V$ of $f$ at $z$
\be
\label{eqDilDiff}
\dil_z(f) = \sup_{|u|=1} \|d_z f(u)\| \stext{ and } \dil_z^*(f) = \inf_{|u|=1} \|d_z f(u)\|
\ee
Applying Lemma \ref{lemmaSubMult} and \iref{eqDilDiff} to the function $g=\ln$ we obtain for any metric space $(X,d_X)$, any $f\in C^0(X,\R_+^*)$ and any $x\in X$
\be
\label{eqDilLog}
\dil_x(\ln f) = \frac {\dil_x(f)} {f(x)} .
\ee

The following proposition shows that, under certain circumstances, the Lipschitz property is a local property.
\begin{prop}
\label{propDilLoc}
Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$.
For any $f\in C^0(\R^d, Y)$ and any path $\gamma\in C^1([0,1], \R^d)$, $\gamma(0) = z$, $\gamma(1) = z'$, one has
\be
\label{eqLipLocPath}
d_Y(f(z), f(z')) \leq l_H(\gamma) \sup_{0\leq t \leq 1} \dil_{\gamma(t)}(f).
\ee
It follows that %In particular 
\be
\label{eqDilLoc}
\dil(f) = \sup_{z\in \sR^d} \dil_z(f).
\ee
\end{prop}

\proof
%Consider $z,z'\in \R^d$, and a path $\gamma\in C^1([0,1],\R^d)$ such that $\gamma(0) = z$, $\gamma(1)=z'$ and $l_H(\gamma) \leq d_H(z,z')+\delta$ where $\delta>0$ is a constant that is devoted to tend to zero in the last step of the proof.
We equip the segment $[0,1]$ with the distance $d_\gamma$ defined for $0 \leq t\leq t'\leq 1$ by 
\be
\label{defDGamma}
d_\gamma(t,t') = d_\gamma(t',t) = l_H(\gamma_{|[t,t']}).
\ee
Note that for any $t\leq t_* \leq t'$ one has 
\be
\label{exactTri}
d_\gamma(t,t') = d_\gamma(t,t_*)+d_\gamma(t_*,t')
\ee
The map $\gamma : ([0,1], d_\gamma) \to (\R^d, d_H)$ is clearly Lipschitz.
It thus follows from Lemma \ref{lemmaSubMult} that $F := f\circ \gamma :[0,1] \to Y$ satisfies for all $t\in [0,1]$
$$
\dil_t(F) \leq \dil_{\gamma(t)}(f) \leq \lambda := \sup_{0\leq t'\leq 1} \dil_{\gamma(t')}(f).
$$
We assume that $\lambda<\infty$, otherwise there is nothing to prove, and we consider a fixed $\delta>0$. For each $t\in [0,1]$ there exists therefore an interval $V_t\subset [0,1]$ containing $t$, relatively open in $[0,1]$, and such that $F_{|V_t}$ is $(\lambda+\delta)$-Lipschitz. Since the segment $[0,1]$ is compact, there exists a finite set $I_0\subset [0,1]$ such that 
$$
[0,1] = \bigcup_{t\in I_0} V_t.
$$
Let $V,V'\subset [0,1]$ be two intersecting intervals, and assume that $F$ is $\lambda+\delta$ Lipschitz on $V$ and on $V'$. For any $t\in V$ and $t'\in V'$, there exists $t_*\in V\cap V'$ which satisfies $t\leq t_*\leq t'$ or $t\geq t_* \geq t'$. Recalling \iref{exactTri} we thus obtain  
\begin{eqnarray*}
d_Y(F(t),F(t')) &\leq& d_Y(F(t), F(t_*))+d_Y(F(t_*), F(t')) \\
&\leq& (\lambda+\delta) d_\gamma(t,t_*)+( \lambda+\delta)d_\gamma(t_*,t') \\
&=& (\lambda+\delta)d_\gamma(t,t').
\end{eqnarray*}
Thus $F$ is $\lambda+\delta$ Lipschitz on the interval $V\cup V'$. Since $[0,1]$ is covered by a finite collection of open intervals on which $F$ is $\lambda+\ve$ Lipschitz, we obtain proceeding by induction that $F$ is $(\lambda+\delta)$-Lipshitz on $[0,1]$ and therefore 
$$
d_Y(f(z),f(z')) = d_Y(F(0),F(1))\leq (\lambda+\delta) d_\gamma(0,1) = (\lambda+\delta)l_H(\gamma). %\leq (\lambda+\delta)(d_H(z,z')+\delta).
$$
Letting $\delta\to 0$ we obtain \iref{eqLipLocPath}. Taking the infimum of \iref{eqLipLocPath} among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_Y(f(z),f(z')) \leq  \lambda d_H(z,z')$. Therefore $f : (\R^d, d_H) \to (Y,d_Y)$ is $\lambda$-Lipschitz, which concludes the proof of this proposition.
%The upper inequality $\geq$ is a direct consequence of the definition \iref{defDilX} of the local dilatation, and we therefore turn to the lower inequality $\leq$.
\sq

The next corollary shows that the global dilatation is controlled by the local dilatation even if the latter is not known on a \emph{sufficiently thin} set $\Gamma$, such as the skeleton of a mesh.

\begin{corollary}
\label{corolLipNoGamma}
Let $\Gamma\subset \R^d$ be a set which has the following property : for any path $\gamma\in C^1([0,1], \R^d)$ there exists a sequence of path $(\gamma_n)_{n \geq 0}$ which converge to $\gamma$ in $C^1$ norm and such that  $\{t\in [0,1]\sep \gamma_n(t) \in \Gamma\}$ is finite for each $n$.\\
Let $H\in \bH$, let $(Y,d_Y)$ be an arbitrary metric space, and met let $f\in C^0(\R^d, Y)$.
Then 
$$
\dil(f) = \sup_{z\in \R^d \sm \Gamma} \dil_z(f).
$$
\end{corollary}

\proof
We denote $\lambda := \sup_{z\in \R^d \sm \Gamma} \dil_z(f)$.
We consider two points $z,z'\in \R^d$ and a path $\gamma\in C^1([0,1], \R^d)$ such that $\gamma(0) = z$ and $\gamma(1) = z'$. %, and a sequence $\gamma_n$ converging to $\gamma$ in $C^1$ norm.

We first assume that the set $\{t\in [0,1]\sep \gamma(t) \in \Gamma\}$ is finite, and we denote its elements by $t_1< \cdots < t_k$. We set by convention $t_0 = 0$ and $t_{k+1} = 1$.
For each $0\leq i \leq k$ and each $t,t'$ such that $t_i <t<t'<t_{i+1}$ we have $d_Y(f(\gamma(t)),f(\gamma(t'))) \leq \lambda l_H(\gamma_{|[t,t']})$. Letting $t\to t_i$ and $t'\to t_{i+1}$ we obtain $d_Y(f(\gamma(t_i)),f(\gamma(t_{i+1}))) \leq \lambda l_H(\gamma_{|[t_i,t_{i+1}]})$. Adding up we obtain 
$$
d_Y(f(z), f(z')) \leq \sum_{0\leq i \leq  k} d_Y(f(\gamma(t_i)), f(\gamma(t_{i+1}))) \leq \lambda
\sum_{0\leq i \leq k} l_H(\gamma_{[t_i, t_{i+1}]}) = \lambda l_H(\gamma).
$$

We now consider the case where $\gamma$ meets the set $\Gamma$ an infinite number of times, and we choose a sequence $\gamma_n$ as described above. We obtain $d_Y(f(\gamma_n(0)), f(\gamma_n(1))) \leq \lambda l_H(\gamma_n)$ for each $n\geq 0$. Since $\gamma_n \to \gamma$ in $C^1$ norm as $n \to \infty$ we obtain taking the limit $d_Y(f(z), f(z')) \leq \lambda l_H(\gamma)$.

Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ we obtain $d_Y(f(z), f(z')) \leq \lambda d_H(z,z')$, which concludes the proof of this proposition.
\sq


%Let $(Y, \|\cdot \|_Y)$ and $(Z, \|\cdot\|_Z)$ be two banach spaces. Let $y\in Y$, $g\in C^1(Y,Z)$, and $L = g'(f(x))$, then clearly 
%$$
%\dil_y(g) = \|L\|.
%$$
%Injecting this in \iref{eqDilUpper1} we obtain 
%\be
%\label{eqDilUpper2}
%\dil_x(g \circ f) \leq\|L\|  \dil_x (f).
%\ee
%We also need a lower bound in several cases. For that purpose we define 
%$$
%\dil^*_z(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(z,\ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)}\right),
%$$
%and we obtain proceeding similarly, but with the different convention $0\times \infty = \infty\times 0 = 0$
%$$
%\dil_z(g\circ f) \geq \dil^*_{f(z)}(g) \dil_z(f).
%$$

The next proposition establishes that the regularity conditions \iref{eqLipMult} and \iref{eqLipAdd} defining the collections of quasi-acute or graded metrics are equivalent in the case of a metric proportionnal to the identity. %$\bH_a$ $\bH_g$

\begin{prop}
\label{propEquivS}
Let $s\in C^0(\R^d, R_+^*)$ and let $H(z) := \Id/s(z)^2$ for all $z\in \R^d$. We have 
\be
\label{eqDilLnH}
\dil_z(\ln s\sep d_H) = \dil_z(s).
\ee
Hence the following properties are equivalent.
\begin{enumerate}
\item The map $s : \R^d \to \R$ is Lipschitz. (i.e. $H\in \bH_i$) %For all $z,z'\in \R^d$ one has $|s(z)-s(z')|\leq |z-z'|$.
\item (``Additive'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_+(H(z),H(z')) \leq |z-z'|$.
\item (``Multiplicative'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_\times(H(z),H(z'))\leq d_H(z,z')$.
\end{enumerate}
\end{prop}

\proof %reprendre preuve??
Combining \iref{eqDilNorm} and \iref{eqDilLog} we obtain for any $z\in \R^d$
$$
%\dil_z (H\sep  d_\times, d_H) = 
\dil_z(\ln s\sep d_H) = s(z) \dil_z(\ln s) = \dil_z(s),
$$
which establishes \iref{eqDilLnH}.
According to \iref{eqDIso} we have for any $z,z'\in \R^d$
$$
d_+(H(z),H(z')) = |s(z) - s(z')| \stext{ and } d_\times (H(z),H(z')) = |\ln s(z) - \ln s(z')|.
$$
The properties 1. and 2. are thus equivalent to $\dil(s)\leq 1$, and therefore also to 
\be
\label{eqDilsLoc}
\dil_z(s) \leq 1 \text{ for all } z\in \R^d.
\ee
according Proposition \ref{propDilLoc} applied to the constant metric $H_0 = \Id$ and to the function $f=s$.
On the other hand property 3. is equivalent to $\dil(\ln s \sep d_H) \leq 1$, and thus to 
$$
\dil_z(\ln s\sep d_H) \leq 1 \text{ for all } z\in \R^d
$$
according to Proposition \ref{propDilLoc} applied to the metric $H$ and to the function $f=\ln s$.
This property equivalent to \iref{eqDilsLoc} according to \iref{eqDilLnH}, which concludes the proof of this Proposition.
\sq

The next corollary uses Proposition \ref{propEquivS} to analyse the regularity of the first and last eigenvalue of a metric.
\begin{corollary}
\label{corolLipNorm}
\begin{itemize}
\item
For any $H\in \bH_g$, the map $z\mapsto \|H(z)\|^{-\frac 1 2}$ is Lipschitz.
\item
For any $H\in \bH_a$, the map $z\mapsto \|H(z)^{-\frac 1 2}\|$ is Lipschitz.
\end{itemize}
\end{corollary}
\proof
\begin{itemize}
\item 
%For any $M,M'\in S_d^+$ we have 
%\begin{eqnarray*}
%d_\times(M,M') &=& \ln \left(\max\left\{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\right\}\right) \\
%&\geq &\ln \left(\max \left\{\frac{\|M^\frac 1 2\|}{\|M'^{\frac 1 2}\|}, \, \frac{\|M'^{\frac 1 2}\|}{\|M^{\frac 1 2}\|}\right\}\right)\\
%& = & \frac 1 2 \left|\ln \|M\| - \ln \|M'\|\right|.
%\end{eqnarray*}
Consider $H\in \bH_g$, define $s(z) := \|H(z)\|^{-\frac 1 2}$ and 
$$
H'(z) := \frac \Id {s(z)^2} = \|H(z)\|\Id.
$$
Since $H(z) \leq H'(z)$ for all $z\in \R^d$, we have $d_H(z,z') \leq d_{H'} (z,z')$ for all $z, z'\in \R^d$.

Consider a pair $M,M'\in S_d^+$ of matrices and a real $\delta>0$. If $e^{-2\delta} M \leq M' \leq e^{2\delta} M$, then taking the norm we obtain $e^{-2\delta} \|M\| \leq \|M'\| \leq e^{2\delta} \|M\|$. It follows that 
$$
\frac 1 2 |\ln \|M\| - \ln \|M'\|| \leq d_\times (M,M').
$$
We thus have for any $z,z'\in \R^d$
\begin{eqnarray*}
|\ln s(z)-\ln s(z')| &=& \frac 1 2 \left|\ln \|H(z)\| - \ln \|H(z')\|\right| \\ %\left|\ln \left(\sqrt{\|H(z)\|}\right) -\ln \left(\sqrt{\|H(z')\|}\right)\right| \\%
%& \leq & \sup_{u\neq 0} |\ln \|u\|_{H(z)} - \ln \|u\|_{H(z')}|\\
&\leq & d_\times(H(z),H(z')) \\
&\leq& d_H(z,z')\\
&\leq& d_{H'}(z,z').
\end{eqnarray*}
Applying Proposition \ref{propEquivS} to the metric $H'$ we obtain that $H'\in \bH_i$, and therefore that $s$ is Lipschitz as announced.
\item
Consider $H\in \bH_a$. We have for any $z,z'\in \R^d$
$$
\left|\|H(z)^{-\frac 1 2}\| - \|H(z')^{-\frac 1 2}\| \right| \leq \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| \leq |z-z'|,
$$
which concludes the proof of this corollary.\sq
\end{itemize}

Our last proposition studies the local dilatation of the maximum and the minimum of two functions.
\begin{prop}
\label{propDilMax}
Let $(X,d_X)$ be a metric space and let $\lambda, \mu\in C^0(X, \R)$. Let $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda, \mu\}$. Then for all $x\in X$
\be
\label{eqDilMax1}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} \leq \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
If $(X,d_H) = (\R^d, d_H)$, where $H \in \bH$ is a riemannian metric, then equality holds
\be
\label{eqDilMax2}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} = \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
\end{prop}

\proof
We have for any $p,q\in X$,
\begin{eqnarray*}
|\gamma(p)-\gamma(q)| &=& |\min\{\lambda(p), \mu(p)\} - \min \{\lambda(q), \mu(q)\}|\\
& \leq & \max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}.
\end{eqnarray*}
For any $x\in X$ and any $\ve>0$ we thus obtain
\begin{eqnarray*}
\dil(\gamma_{|B(x,\ve)}) &=& \sup_{p,q\in B(x,\ve)} \frac{|\gamma(p)-\gamma(q)|}{d_X(p,q)} \\
&\leq& \sup_{p,q\in B(x,\ve)} \frac{\max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}}{d_X(p,q)}\\
& =& \max\left\{\sup_{p,q\in B(x,\ve)}  \frac{|\lambda(p)-\lambda(q)|}{d_X(p,q)}, \sup_{p,q\in B(x,\ve)}  \frac{|\mu(p)-\mu(q)|}{d_X(p,q)}\right\}\\
&=& \max\left\{\dil(\lambda_{|B(x, \ve)}), \dil(\mu_{|B(x,\ve)})\right\}.
\end{eqnarray*}
Letting $\ve \to 0$ we obtain $\dil_x(\gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$. Likewise $\dil_x(\Gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$ which concludes the proof of \iref{eqDilMax1}.

We now turn to the proof of \iref{eqDilMax2}. For that purpose we consider a fixed $\ve>0$ and we define
$$
r := \max \{\dil(\gamma_{|B(x,\ve)}\sep \|\cdot\|_{H(x)}), \ \dil(\Gamma_{|B(x,\ve)} \sep \|\cdot\|_{H(x)})\},
$$
where $B(x,\ve)$ stands for the euclidean unit ball of radius $\ve$ centered at $x$.
Consider two points $p,q\in B(x,\ve)$. If $\lambda(p) \geq \mu(p)$ and $\lambda(q)\geq \mu(q)$, or if $\lambda(p) \leq \mu(p)$ and $\lambda(q)\leq \mu(q)$, then 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)|&=& \max \{|\gamma(p)-\gamma(q)|, |\Gamma(p)-\Gamma(q)|\}\\
&\leq & \|p-q\|_{H(x)}
\end{eqnarray*}
Otherwise if  $\lambda(p) \geq \mu(p)$ and $\lambda(q)\leq \mu(q)$, or $\lambda(p) \leq \mu(p)$ and $\lambda(q)\geq \mu(q)$, then there exists a point $r$ on the segment $[p,q]$ such that $\lambda(r)=\mu(r)$. We thus have %$|p-r|+|r-q| = |p-q|$ and 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)| &\leq& \max \{|\gamma(p)-\gamma(r)|, |\Gamma(r)-\Gamma(q)|\}\\
& &+ \max \{|\gamma(r)-\gamma(q)|, |\Gamma(r)-\Gamma(q)|\}\\
& \leq & \|p-r\|_{H(x)} + \|r-q\|_{H(x)} = \|p-q\|_{H(x)}
\end{eqnarray*}
If follows that $\dil(\lambda_{|B(x,\ve)}\sep \|\cdot\|_{H(x)})\leq r$, and letting $\ve\to 0$ we obtain 
$$
\dil_x(\lambda\sep \|\cdot\|_{H(x)}) \leq \max\{\dil_x(\gamma\sep \|\cdot\|_{H(x)}), \ \dil_x(\Gamma \sep \|\cdot \|_{H(x)})\}.
$$ 
Recalling that $\dil_x(f\sep d_H) = \dil_x(f\sep \|\cdot\|_x)$ for any $f\in C^0(\R^d, \R)$ and any for all $x\in \R^d$, see \iref{eqDilNorm}, we obtain $\dil_x(\lambda) \leq \max\{\dil_x(\gamma), \ \dil_x(\Gamma)\}$. Proceeding likewise for $\mu$ we obtain \iref{eqDilMax2} which concludes the proof of this proposition.
\sq

\subsection{Geometric properties of the space $(\R^d, d_H)$} %Estimates of size}
\label{subsecMetGeom}

We focus in this subsection on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. The next proposition compares the riemannian distance $d_H$ between two points $z$ and $z+u$ with the norm $\|u\|_{H(z)}$ of their difference.

%with the euclidean distance and we estimate the volume of balls. 
%The next proposition compares the Riemannian distance associated to a graded metric, with 

\begin{prop}
\label{propEuclidRiemann}
Let $H \in \bH_g$ and let $z\in \R^d$. For all $u\in \R^d$ one has
\be
\label{eqEuclidRiemann}
\ln(1+\|u\|_{H(z)}) \leq d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention when $\|u\|_{H(z)}\geq 1$.
\end{prop}
\proof
%We first prove the left part of \iref{eqEuclidRiemann}, and for that purpose
We consider a path $\gamma\in C^1([0,1], \R^d)$, and we define for each $t\in [0,1]$
\be
\label{defLGamma}
l(t) := \int_0^t \|\gamma'(t)\|_{H(\gamma(t))}dt.
\ee
Since $H\in \bH_g$ we have for any $t\in [0,1]$
$$
\exp(-2\, d_H(z, \gamma(t))) \, H(z) \leq H(\gamma(t)) \leq  \exp(2 \, d_H(z, \gamma(t))) \, H(z)
$$
therefore, since $d_H(z, \gamma(t)) \leq l(t)$,
$$
\exp(-2l(t)) H(z)  \leq H(\gamma(t)) \leq  \exp(2l(t)) H(z).
$$
It follows that 
$$
\|\gamma'(t)\|_{H(z)} \exp(-l(t)) \leq l'(t) = \|\gamma'(t)\|_{H(\gamma(t))} \leq  \|\gamma'(t)\|_{H(z)} \exp(l(t)), %\exp(-l(t))
$$
hence 
\be
\label{eqGammapLp}
-\frac d {dt} \exp(-l(t)) \leq \|\gamma'(t)\|_{H(z)} \leq \frac d {dt} \exp(l(t)).
\ee
We have 
\be
\label{eqGammaGammap}
\|u\|_{H(z)} =  \|\gamma(1)-\gamma(0)\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt
\ee
with equality if $\gamma(t) = z+tu$ is the straight line.
%We now assume that $\gamma(t) \neq \gamma(0)$ for all $t\in (0,1]$, which is the case generically. The map $t\mapsto \|\gamma(t)-\gamma(0)\|_{H(z)}$ is therefore $C^1$ on $(0,1]$ and we have 
%$$
%\frac d {dt} \|\gamma(t)-\gamma(0)\|_{H(z)} \leq \|\gamma'(t)\|_{H(z)},
%$$
%with equality if $\gamma(t)-\gamma(0) = c \gamma'(t)$ for some $c>0$.
%In the special case of the straight line $\gamma(t)=z+tu$, \iref{eqGammaGammap} is an equality and we thus obtain 
In that case, integrating the left part of \iref{eqGammapLp} we obtain
$$
 1-\exp(-l_H(\gamma)) = -\int_0^1 \left(\frac d {dt} \exp(-l(t))\right)dt   \leq  \int_0^1 \|\gamma'(t)\|_{H(z)} dt %= \|\gamma(1)-\gamma(0)\|_{H(z)} \exp(-l(0)) - \exp(-l(1))
 = \|u\|_{H(z)}.
$$
Rearranging the terms we obtain the right part of \iref{eqEuclidRiemann}:
$$
d_H(z,z+u) \leq l_H(\gamma) \leq -\ln(1-\|u\|_{H(z)}).
$$
We now consider an arbitrary path $\gamma$ joining $z$ and $z+u$ and we obtain integrating the right part of \iref{eqGammapLp} and recalling \iref{eqGammaGammap}
$$
\exp(l_H(\gamma)) -1 = \int_0^1 \left(\frac d {dt} \exp(l(t))\right) dt  \geq \int_0^1 \|\gamma'(t)\|_{H(z)} dt \geq \|u\|_{H(z)},
$$
which is equivalent to
$$
l_H(\gamma) \geq \ln(1+\|u\|_{H(z)}).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ satisfying $\gamma(0) = z$ and $\gamma(1) = z+u$, we obtain the left part of \iref{eqEuclidRiemann}, which concludes the proof of this proposition.
\sq

We discuss in the rest of this section the consequences of the comparison \iref{eqEuclidRiemann} of the riemannian distance $d_H$ with the distance associated to the norm $\|\cdot\|_{H(z)}$ when $H\in \bH_g$. %is devoted to 
Combining the right part of \iref{eqEuclidRiemann} with the expression \iref{eqDTimesLog} of the distance $d_\times$ we obtain an estimate of the local variations of the norm $\|\cdot \|_{H(z)}$ associated to the metric $H$ at a point $z$: let $H\in \bH_g$, and let $z,u,v\in \R^d$ be such that $\|u\|_{H(z)} < 1$, then
\be
\label{eqLocalNorm}
(1-\|u\|_{H(z)}) \|v\|_{H(z)} \leq \|v\|_{H(z+u)} \leq (1-\|u\|_{H(z)})^{-1} \|v\|_{H(z)}. %\frac{\|v\|_{H(z)}}{1-\|u\|_{H(z)}}.
\ee
Note also that 
\be
\label{eqLocalDet}
(1-\|u\|_{H(z)})^d \sqrt{\det H(z)} \leq \sqrt{\det H(z)} \leq (1-\|u\|_{H(z)})^{-d} \sqrt{\det H(z)}.
\ee
Another important consequence of \iref{eqEuclidRiemann} is that the closed balls $\{z'\in \R^d \sep d_H(z,z')\leq r\}$ for the distance $d_H$, are closed and bounded subsets $\R^d$, hence are compact. %From this point a classical argument (??) shows that $(R^d,d_H)$ is a complete metric space.

The following example establishes that \iref{eqEuclidRiemann} is a sharp inequality. The metric $H$ defined by 
$$
H(z) := \frac \Id {(1+|z|)^2}
$$
belongs to $\bH_i$ since $z\mapsto 1+|z|$ is Lipschitz, hence $H$ also belongs to $\bH_a$ and $\bH_g$.
For any $v\in \R^d$, one easily checks that the path of minimal length joining $0$ to $v$ is the straight line, and that
$$
d_H(0, v) = \ln(1+|v|).
$$
Choosing $z=0$ and $u=v$ we obtain that the left part of \iref{eqEuclidRiemann} is sharp
$$
\ln (1+ \|u\|_{H(0)}) = \ln (1+ |u|) = d_H(0,0+u).
$$
Choosing $z=-v$ and $u = v$ we obtain that the right part of \iref{eqEuclidRiemann} is sharp
$$
-\ln\left(1-\|u\|_{H(-u)} \right) = -\ln \left(1-\frac {|u|}{1+|u|}\right) = \ln(1+|u|) = d_H(-u, -u+ u).
$$

The next corollary uses Proposition \ref{propEuclidRiemann} to obtain a lower bound for the mass of balls in the measure $z\mapsto \sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. %states a volume estimate Proposition \ref{propLength} implies a volume estimate. %also allows us to compare the vo
\begin{corollary}
\label{corolVol}
There exists $c=c(d)>0$ such that the following holds. Let $H \in \bH_g$,
let $L\geq 1$ and let $z_0\in \R^d$. Denoting $\cE$ the ellipse 
$$
\cE = \{z\in \R^d\sep \|z-z_0\|_{H(z_0)}\leq L\}.
$$ 
we have 
\be
\label{eqVolLog}
\int_\cE \sqrt{\det H} \geq c \ln L. %\max\{L,1\}.
\ee
%Then 
%$$
%\int_\cE \sqrt {\det H} \geq c \ln L -1
%$$
%where $c=...$
%In particular if $H(z)\geq \lambda^2\Id$ (*$\|u\|_{H(z)} \geq \lambda |u|$ for all $u\in \R^d$*) then 
%\be
%\label{volBR}
%\int_{B(z,r)} \sqrt{\det H} \geq c \ln \max\{\lambda r, 1\}
%\ee
\end{corollary}

\proof
It follows from Proposition \ref{propEuclidRiemann} that $d(z_0, z) \geq \ln (L+1)$ for all $z\in \partial \cE$. We define the integer 
$$
k = \left\lfloor \ln(L+1) -\frac 1 2\right\rfloor,
$$
and we consider $k$ points $z_1, \cdots , z_k \in E$ such that for all $0 \leq i \leq k$
$$
d_H(z_0, z_i)= i.
$$
We define 
$
r_0 := 1-e^{-\frac 1 2} = 0.39\cdots
$
in such way that 
$$
-\ln (1-r_0) = \frac 1 2.
$$
For all $0 \leq i \leq k$ we denote by $\cE_i$ the ellipse 
$$
\cE_i  := \left\{z\in \R^d \sep \|z-z_i\|_{H(z_i)} \leq r_0\right\}.
$$
We have $\cE_i \subset \cE$ for all $0 \leq i \leq k$, indeed for any $z\in \cE_i$ we have 
$$
d_H(z_0, z) \leq d_H(z_0, z_i) + d_H(z_i, z) \leq i- \ln (1-r_0) \leq k+\frac 1 2 \leq \ln (L+1),
$$
Denoting by $\interior(E)$ the interior of a set $E\subset \R^d$, we observe that for all $0 \leq i<j\leq k$, for all $z\in \interior(\cE_i)$ and $z'\in \interior(\cE_j)$, we have
$$
d_H(z,z') \geq d_H(z_i, z_j) -d_H(z_i, z) - d_H(z_j,z') > |d_H(z_0, z_i) - d(z_0, d_j)| + 2\ln(1 -r_0) =0, %\geq 1+ 2 \ln(1-\frac 1 3)>0.
$$
hence $\interior(\cE_i) \cap \interior(\cE_j) = \emptyset$.
It follows that 
$$
\int_\cE \sqrt{\det H} \geq \sum_{0 \leq i \leq k} \int_{\cE_i} \sqrt{\det H}.
$$
Furthermore we have for all $z\in \cE_i$
$$
H(z) \geq (1-\|z-z_i\|_{H(z_i)})^2 H(z_i)  \geq (1-r_0)^2 H(z_i),
$$
and therefore 
\be
\label{eqzzi}
\sqrt{\det H(z)} \geq (1-r_0)^d \sqrt{\det H(z_i)}.
\ee
We denote by $B(z,r)$ the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$, and we observe that 
$u\mapsto z_i + H(z_i)^{-\frac 1 2} u$ maps $B(0,r_0)$ onto $\cE_i$. Combining this remark with \iref{eqzzi} we obtain
\begin{eqnarray*}
\int_{\cE_i} \sqrt{\det H} &\geq& (1-r_0)^d \int_{\cE_i} \sqrt{\det H(z_i)} \\
&=& (1-r_0)^d \int_{B(0,r_0)} 1 \\
&=& c_0 := r_0^d (1-r_0)^d |B(0,1)|.
\end{eqnarray*}
%where $B(z,r)$ denotes the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$.
Eventually we obtain 
$$
\int_\cE \sqrt{\det H} \geq (k+1) c_0 \geq (\ln(L+1) - 1/2) c_0.
$$
In order to obtain \iref{eqVolLog} we simply recall that $L\geq 1$ and therefore that %Since Recalling that $L\geq 1$ we find that 
$$
\ln (L+1) = \frac{\ln(L+1)}{2 \ln 2} +  \left(1-\frac 1 {2 \ln 2}\right)\ln(L+1) \geq \frac 1 2 + \left(1-\frac 1 {2 \ln 2}\right)\ln L $$
which concludes the proof of \iref{eqVolLog} with $c=(1- 1/(2 \ln 2))c_0$.
%Applying \iref{eqVolLog} to $L = \lambda r$ we obtain \iref{volBR} which concludes the proof of this proposition.
\sq


\section{Metrics having an eigenspace of dimension $d-1$ at each point}
\label{secEigen}
We focus in this subsection on metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has an eigenspace of dimension at least $d-1$ at each point $z\in \R^d$. 
%If the dimension is $d=2$, then a metric $H\in \bH$ generically satisfies this condition on a dense subset of $\R^d$. %any metric $H\in \bH$ satisfies this condition. 
This condition clearly holds if the dimension is $d=2$, but is also relevant in higher dimension. 
Indeed, as discussed in \S\ref{secOptGeom} of Chapter \ref{chapApproxMet}, this type of metrics appears when one needs to create mesh containing a thin layer of simplices close to an hypersurface $\Gamma$. In that case the matrix $H(z)$ at a point $z\in \Gamma$ typically has an eigenspace of dimension $d-1$ which is tangent to $\Gamma$ and is associated to a small eigenvalue, and an eigenspace of dimension $1$ in the direction orthogonal to $\Gamma$ associated to a large eigenvalue. 

The main result of this section is Theorem \ref{th2Spaces} which characterises those of these metrics which belongs to $\bH_a$ or $\bH_g$ in terms of the regularity of their eigenvalues and of their eigenvectors.
Corollary \ref{corolHgToHa} to this theorem gives a simple procedure to obtain a quasi-acute metric from a graded metric $H$ such that $H(z)$ has an eigenspace of dimension $d-1$ at each point. \\

We denote by $\bbS := \{\theta\in \R^d \sep |\theta| = 1\}$ the unit sphere of $\R^d$, equipped with the distance 
$$
d_\bbS(\theta, \theta') := \arccos(\<\theta, \theta'\>).
$$
We denote by $\cA$ the space of parameters
$$
\cA := \R_+^*\times \R_+^*\times \bbS,
$$
and we define a map $\cS :\cA\to S_d^+$ as follows
\be
\label{defcS}
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
\ee
In any orthonormal basis $\cB$ of $\R^d$ which begins with the vector $\theta$ we have the following expression
$$
[\cS(\lambda, \mu, \theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda &0 & 0 & \cdots\\
0 & \mu & 0 & \cdots\\
0 & 0 & \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right).
$$
We also define for any $a = (\lambda, \mu, \theta)\in \cA$
$$
\cH(a) := \cS(a)^{-2} = \lambda^{-2} \theta \theta^\trans+ \mu^{-2}(1-\theta \theta^\trans).
$$
%If $M\in S_d^+$ has an eigenspace of dimension $d-1$ exactly, then 
%
%We denote by $S_{d*}^+$ the collection of symmetric positive definite matrices $M\in S_d^+$ which have an eigenspace of dimension exactly $d-1$.
%We also denote by $\cA^*$ the collection of $(\lambda, \mu, \pm\theta)\in \cA$ which satisfies $\lambda\neq \mu$ if $d>2$ (resp. $\lambda>\mu$ is the dimension is $d=2$).
%Then
%$$
%\cH : \cA^* \to S_{d*}^+
%$$
%is a one to one map.



%Such a metric $H$ can be parametrized using two eigenvalues $\lambda, \mu\in \R_+^*$  and a subspace of dimension $d-1$ of $\R^d$ defined through an un-oriented unit normal $\pm \theta$. Our purpose in this section is to translate the fact that $H\in \bH_\star$, for some $\star\in \{i,a,g\}$, into simpler properties satisfied by $\lambda,\mu$ and $\theta$.
%
%
%
%In order to state our results, we need to introduce the collection $\cP$ of all hyperplanes of $\R^d$, also called the projective space. An hy
%
%
%We define the space of parameters
%$$
%\cA :=  \R_+^* \times \R_+^* \times \cP,
%$$
%where $\cP$ is the $d-1$-dimensional real projective space.
%For all $(\theta, \lambda, \mu)\in \cA$ we define 
%$$
%S( \lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans),
%$$
%and $H(\theta, \lambda, \mu) := S^{-2}$.
%The space $\cA$ is a differential variety, and the tangent space to a triplet $(\theta, \lambda, \mu)\in \cA$ is 
%$$
%T_{(\theta, \lambda, \mu)} \cA =  \R \times \R \times \theta^\perp,
%$$
%where $\theta^\perp$ refers to the orthogonal hyperplane to $\theta$ in $\R^d$.

For any metric $H \in \bH$ and any $z\in \R^d$ we denote by $\dil_z(H)_\times$ and $\dil_z(H)_+$ the local dilatations at $z$ associated to the Lipschitz conditions \iref{eqLipMult} and \iref{eqLipAdd} defining $\bH_g$ and $\bH_a$:
\be
\label{defDilH}
\dil_z(H)_\times := \dil_z(H \sep d_\times, d_H) \stext{ and } \dil_z(H)_+ := \dil_z(H \sep d_+).
\ee
We recall that the local dilatation $\dil_z(f)$ of a function $f$ at a point $z$ is defined by \iref{defDilX}.
%We set $D_z(H) := \dil(\lambda)$ if $z\notin \Omega$
For any open set $\Omega\subset \R^d$ and any $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$,  we define for all $z\in \Omega$
\be
\label{eqDZA}
D_z(a)_\times := \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \frac 1 2 \left| \frac {\lambda(z)} {\mu(z)} - \frac {\mu(z)} {\lambda(z)} \right|\dil_z(\theta\sep  d_H)\right\}, %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
and 
\be
\label{eqDZAP}
D_z(a)_+ := \max\left\{\dil_z(\lambda), \ \dil_z(\mu),\ |\lambda(z)-\mu(z)| \dil_z(\theta)\right\}. %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
Note that these quantities are not defined if $\lambda(z) = \mu(z)$ and $\dil_z(\theta\sep  d_H)=\infty$ simultaneously, since an indeterminate form $0\times \infty$ appears in \iref{eqDZA} and \iref{eqDZAP}.
\begin{theorem}
\label{th2Spaces}
Let $H \in \bH$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, such that $H = \cH\circ a$ on $\Omega$.
Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$. Then 
\be
\label{eqDilTimes}
D_z(a)_\times \leq \dil_z(H)_\times \leq 2D_z(a)_\times
\ee
and%, with $\gamma := \|H^{-\frac 1 2}\| = \max\{\lambda, \mu\}$, 
\be
\label{eqDilPlus}
D_z(a)_+ \leq \dil_z(H)_+ \leq 2D_z(a)_+.
\ee
%In particular, defining $\gamma := \|H(z)^{-\frac 1 2}\| = \max \{\lambda, \mu\}$ we have 
%\be
%\label{eqDilMax}
%\max\{\dil_z(\gamma), \, D_z(a)_\times\} \leq \max \{D_z(a)_+, \, D_z(a)_\times\} \leq 2\max\{\dil_z(\gamma), \, D_z(a)_\times\}.
%\ee
\end{theorem}

%The estimate \iref{eqDilPlus} on $\dil_z(H)_+$ is not very sharp, but this is not an issue since one usually does not needs to control $ \dil_z(H)_+$ but rather $\max\{\dil_z(H)_\times,\dil_z(H)_+\}$, for which we obtain combining \iref{eqDilTimes} and \iref{eqDilPlus} the sharper estimate 
%$$
% \max\{\dil_z(\gamma), D_z(a)\} \leq \max\{\dil_z(H)_\times,\dil_z(H)_+\} \leq 2 \max\{\dil_z(\gamma), D_z(a)\}.
%$$
The rest of this section is devoted to the proof of this theorem and to Corollary \ref{corolHgToHa}. Our first lemma defines and estimates a quantity $\Delta(a,b,c)$ which appears repeatedly in the rest of the proof.


\begin{lemma}
\label{lemmaDelta}
We define for all $a,b,c\in \R$ the quantity $\Delta(a,b,c)\in \R_+$, as follows % which is the norm of a $d\times d$ matrix,
\be
\label{defDelta}
\Delta(a,b,c) := 
\left\| 
\left(
\begin{array}{cccc}
a & b & 0 & \cdots\\
b & c& 0 & \cdots\\
0 & 0 & c & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right)
\right\|.
\ee
We have 
\be
\label{eqEstimM}
\max\{|a|, |b|, |c|\} \leq \Delta(a,b,c) \leq 2 \max\{|a|, |b|, |c|\}.
\ee
\end{lemma}

\proof
We consider fixed values of $a,b,c\in \R$ and we denote by $M$ the matrix presented in \iref{defDelta}, in such way that $\Delta(a,b,c) = \|M\|$. We also define $\lambda := \max\{|a|,|b|,|c|\}$.
We have 
$$
\Delta(a,b,c) = \|M\|\geq \max_{1\leq i,j\leq d} |M_{ij}| = \lambda,
$$
which establishes the left part of \iref{eqEstimM}. For all $p\in [1,\infty]$ we denote by $l^p$ the usual norm on $\R^d$ of exponent $p$. We have 
$$
\|M\|_{l^\infty\to l^\infty} = \max_{1 \leq i \leq d} \sum_{1\leq j \leq d} |M_{ij}| \leq 2 \lambda \stext{ and } \|M\|_{l^1\to l^1} = \max_{1 \leq j \leq d} \sum_{1\leq 1 \leq d} |M_{ij}| \leq 2 \lambda.
$$
By interpolation we thus obtain  
$$
\|M\| = \|M\|_{l^2\to l^2} \leq \sqrt{\|M\|_{l^1\to l^1} \|M\|_{l^\infty\to l^\infty} } \leq 2 \lambda,
$$
which concludes the proof.
\sq

The parameter space $\cA = \bbS \times \R_+^* \times \R_+^*$ is a differential variety, and the regularity of functions defined on $\cA$ should be seen through local charts.
For each $a = (\lambda, \mu, \theta)\in \cA$ we define a local chart $\psi_a$ of a neigborhood of $a$ in $\cA$ as follows: 
\be
\label{defPsia}
\psi_a : (-\lambda, \infty)\times (-\mu , \infty) \times (B(0,\cPi) \cap \theta^\perp) \to \cA
\ee
is defined by 
$$
\psi_a(\Lambda, M, r\Theta) := (\lambda+ \Lambda,\, \mu+ M,\, \cos(r) \theta + \sin(r) \Theta),
$$
where $|\Theta| = 1$. Note that $\psi_a$ is one to one and that $d_\bbS(\theta, \, \cos(r) \theta + \sin(r) \Theta) = r$.
In \iref{defPsia} we denoted by $\theta^\perp := \{\Theta\in \R^d \sep \<\theta, \Theta\> = 0 \}$ the space orthogonal to $\theta$, and $B(0,\cPi)$ the open euclidean ball of radius $\cPi$.
%it preserves distances in the following sense: if $(\lambda', \mu', \theta') = \psi_a(\Lambda, M, r\Theta)$ then $\lambda'-\lambda = \Lambda$, $\mu'-\mu=M$ and $

Let $V$ be a banach space. We say that a function $\vp : \cA \to V$ is $C^1$ if for any $a\in \cA$ the function $\vp\circ \psi_a$ is $C^1$.
In that case for any $a\in \cA$ we define the differential 
%and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
$$
d_a\vp(A) : \R\times \R\times \theta^\perp \to V
$$
by the formula
$$
d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( tA) - \vp(a)} t. %\Lambda, t M, t r\Theta
$$
We then have
 $$
\dil_a(\vp) = \|d_a(\vp)\|.
$$
%where $d_0 (\vp\circ \psi_a) :  \R\times \R\times \theta^\perp \to V$ denotes the differential of function $\vp\circ \psi_a$ at the origin $(0,0,0) \in (-\lambda, \infty)\times (-\mu , \infty) \times (B(\pi) \cap \theta^\perp)$.
%In that case for any $a\in \cA$ and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
%$$
%d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( t\Lambda, t M, t r\Theta) - \vp(a)} t,
%$$
%and we have for any path $\gamma\in C^1([0,1], \cA)$ 
%$$
%\vp(\gamma(1)) - \vp(\gamma(0)) = \int_0^1 d \vp_{\gamma(t)} (\gamma'(t)) dt.
%$$

\begin{prop}
\label{propPhiPlus}
Define $V_+ := S_d$, equipped with the standard norm $\|\cdot\|$, and define $\vp_+ (a) := \cS(a)$.
Then for all $a,b\in \cA$ we have 
\be
\label{eqDPPhiP}
d_+(\cH(a), \cH(b)) = \|\vp_+(a)-\vp_+(b)\|.
\ee
Furthermore $\vp_+ \in C^1(\cA, V_+)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
$$
\|d_a \vp_+(A)\|_\infty= 
\Delta(\Lambda, \ (\lambda-\mu) r ,\ M).
$$
\end{prop}

\proof
The \iref{eqDPPhiP} directly follows from the fact that $\cH(a)^{-1} = \cS(a)^2 = \vp_+(a)^2$, and from the definition \iref{defDPlus} of $d_+$.
The function $\vp_+ = \cS$ is $C^1$, and even $C^\infty$, since it has a polynomial expression 
$$
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
$$
We have at the first order in $\lambda, \mu, r$
\begin{eqnarray*}
\cS(\lambda+ \Lambda, \, \mu+M, \, \theta+r\Theta) &=&
 (\lambda+ \Lambda) (\theta+ r\Theta) (\theta+r\Theta)^\trans \\
 & &+ (\mu+M)(\Id - (\theta+ r\Theta) (\theta+r\Theta)^\trans)\\
 &=& S(\lambda, \mu, \theta) \\
 & &+ \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans)\\
& &+  \cO((|\Lambda|+ |M|+ |r|)^2)
\end{eqnarray*}
Therefore %$\vp_+$ is $C^1$ and 
\be
\label{eqDiffS}
%d_a\vp_+(\Lambda, \,M, \,r\Theta) = 
d_a\cS(\Lambda, \,M, \,r\Theta) =  \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans).
\ee
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[d_a\cS(\Lambda, \,M, \,r\Theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda & r(\lambda-\mu) & 0 & \cdots\\
r(\lambda-\mu) & M & 0 & \cdots\\
0 & 0 & M & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
which concludes the proof of this proposition.
\sq


\begin{prop}
\label{propPhiTimes}
Define $V_\times := C^0(\bbS, \R)$, equipped with the $\|\cdot\|_\infty$ norm, and define $\vp_\times : \cA \to V_\times$ as follows: for any $a\in \cA$ and any $u\in \bbS$
%\be
%\label{eqDTPhiT}
$$
\vp_\times (a) := (u \mapsto \ln \|u\|_{\cH(a)}).
$$
%\vp_\times (a)(u) = \ln \|u\|_{\cH(a)}.
%\ee
Then for all $a,b\in \cA$ we have 
\be
\label{eqDTPhiT}
\|\vp_\times(a)-\vp_\times(b)\|_\infty = d_\times(\cH(a), \cH(b)).
\ee
Furthermore $\vp_\times \in C^1(\cA, V_\times)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
\be
\label{eqNormDPhiPlus}
\|d_a \vp_\times(A)\|_\infty= 
\Delta\left(\frac \Lambda \lambda ,\ \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) ,\ \frac M \mu\right).
\ee
\end{prop}

\proof
Using the expression \iref{eqDTimesLog} of the distance $d_\times$ and the homogeneity of norms we obtain for any $M,M'\in S_d^+$,
$$
d_\times (M,M') = \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
$$
which implies \iref{eqDTPhiT}.
%The inequality \iref{eqDTPhiT} follows from the expression \iref{eqDTimesLog} of the distance $d_\times$.

As observed in the proof of Proposition \ref{propPhiPlus} the function $\cS : \cA\to S_d^+$ is $C^1$, and $d_a\cS(A)$ has the explicit expression \iref{eqDiffS}.
It is well known that the inverse map ${\rm Inv} : \GL_d \to \GL_d$ is $C^1$ and has the the following differential : for any $\phi\in \GL_d$ and any $\Phi\in M_d$
$$
d_\phi {\rm Inv} (\Phi) = \phi^{-1} \Phi \phi^{-1}.
$$
By composition, $\cS^{-1} : \cA \to S_d^+$ is also $C^1$, and for any $a=(\lambda, \mu , \theta)\in \cA$ and any $A\in \R\times \R \times \theta^\perp$
$$
d_a(\cS^{-1})(A) = S(a)^{-1} (d_a S(A) ) S(a)^{-1}.
$$
For any $u\in \bbS$ we have 
$$
\ln \|u\|_{\cH(a)} = \ln \|\cS(a)^{-1}u\| = \frac 1 2 \ln \left(\<\cS(a)^{-1}u,\cS(a)^{-1}u\>\right).
$$
Therefore, again by composition, 
\begin{eqnarray*}
d_a (\ln \|u\|_{\cH})(A) &=&  \frac 1 {2\|\cS(a)^{-1}u\|^2} (\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>\\
& &\quad +\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>)\\% \frac {\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>+\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>}{2\|\cS(a)^{-1}u\|^2}\\
&=& \frac{\<G(a,A) v,v\>}{\|v\|^2}
\end{eqnarray*}
where $v = \cS^{-1}(a)u$. The function $G$ has the following expression : for any $a = (\lambda, \mu, \theta)\in \R_+^* \times \R_+^* \times \bbS$ and any $A = (\Lambda, M, r\Theta)\in \R\times \R \times \theta^\perp$
\begin{eqnarray*}
G(a,A) &=& \frac{\cS(a)^{-1} (d_a\cS(A)) + (d_a\cS(A)) \cS(a)^{-1}} 2\\
&=& \frac \Lambda \lambda \theta \theta^\trans +  \frac M \mu (\Id - \theta \theta^\trans) + \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right)(\theta \Theta^\trans + \Theta \theta^\trans),
\end{eqnarray*}
the last expression follows from the explicit expression \iref{eqDiffS} of $d_a\cS(A)$ establishes in the proof of the previous proposition, and from the fact that $\theta^\trans \Theta = 0$.
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[G(a,A)]_\cB = 
\left(
\begin{array}{cccc}
\frac \Lambda \lambda & \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & 0 & \cdots\\
\frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & \frac M \mu & 0 & \cdots\\
0 & 0 & \frac M \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
The map $\vp_\times$ is differentiable, as the composition of differentiable maps, and we thus have
\begin{eqnarray*}
\|d_a \vp_\times(A)\|_\infty &=& \sup \left\{ \frac{|\<G(a,A) v,v\>|}{\|v\|^2} \sep u\in \bbS, \, v=\cS(a)^{-1} u\right\}\\
&=& \|G(a,A)\|,
\end{eqnarray*}
which establishes \iref{eqNormDPhiPlus} and concludes the proof of this proposition.
\sq

We now consider a fixed $z\in \Omega$ and we remark that 
$$
\dil_z(H)_\times = \dil_z(\cH\circ a)_\times  = \dil_z(\vp_\times \circ a\sep d_H). %\leq \dil_{a(z)} (\vp_+\sep d_z) \dil_z(a\sep d_H, d_z)
$$
Therefore,  according to Lemma \ref{lemmaSubMult} for any norm $\|\cdot\|_{a(z)}$ defined on the tangent space $\R\times \R \times \theta(z)^\perp$ to $a(z)\in \cA$ we have 
\be
\label{eqDilPhiA}
\begin{array}{rcl}
& &\dil^*_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} a\sep d_H, \|\cdot \|_{a(z)})\\
& \leq& \dil_z(H)_\times\\
& \leq& \dil_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} \circ a\sep d_H, \|\cdot\|_{a(z)})
\end{array}
\ee
provided no indeterminate $0\times \infty$ or $\infty \times 0$ appears on the first and last term of this inequality.
%We recall that a neighborhood of $a(z)$ is parametrized by the local chart 
%\be
%\label{defPsiAZ}
%\psi_{a(z)} : (\Lambda, M, r\Theta) \to (\lambda(z) + \Lambda, \, \mu(z) + M, \, \cos(r)\theta(z)+ \sin(r) \Theta)
%\ee
%where $|\Theta| = 1$. 
We consider a fixed point $z\in \Omega$, and we distinguish the two cases $\lambda(z) \neq \mu(z)$ and $\lambda(z) = \mu(z)$.

\paragraph{Proof in the case $\lambda(z) \neq \mu(z)$.}
For each $a=(\lambda, \mu, \theta)\in \cA$ we define a norm $\|\cdot \|_a$ on the tangent space $\R\times \R \times \theta^\perp$ to $\cA$ at the point $a$ : for all $A = (\Lambda, M , \Theta)\in \R\times \R \times \theta^\perp$
$$
\|A\|_a = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \frac 1 2 \left| \frac \lambda \mu - \frac \mu \lambda\right| \|\Theta\|\right\}.
$$
We have by construction 
\be
\label{eqDilADZDH}
\dil_z(\psi_{a(z)}^{-1}\circ a\sep d_H, \|\cdot \|_{a(z)}) = D_z(a)_\times
\ee
According to Lemma \ref{lemmaDelta} and Proposition \ref{propPhiTimes} we have for any $a=(\lambda, \mu, \theta)\in \cA$ and any $A\in \R\times\R \times \theta^\perp$
$$
\|A\|_a \leq \|d_a \vp_\times(A)\|_\infty = \|d_0 (\vp_\times \circ \psi_a)\|_\infty \leq 2 \|A\|_a.
$$
Since $\vp_\times$ is $C^1$ it follows from \iref{eqDilDiff} that 
$$
1 \leq \dil^*_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq \dil_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq 2.
$$
Combining \iref{eqDilPhiA}, \iref{eqDilADZDH} and the last inequality we obtain
$$
D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times,
$$
which establishes the announced result \iref{eqDilTimes} in the case $\lambda(z)\neq \mu(z)$. A similar reasoning establishes the counterpart \iref{eqDilPlus} of this ineaquality for the distance $d_+$. 

\paragraph{Proof in the case $\lambda(z) = \mu(z)$.}
%We now turn to the case of equality $\lambda(z) = \mu(z)$.
For any $\ve>0$ and any $a=(\lambda, \mu, \theta)\in \cA$ such that $\lambda = \mu$ we define a norm $\|\cdot\|_{a,\ve}$ on the tangent space $\R\times \R\times \theta^\perp$ to $a$ in $\cA$ as follows : 
$$
\|A\|_{a, \ve} = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \ve \|\Theta\|\right\}.
$$
%$$
%d_z^\ve((\Lambda, M, r\Theta), (\Lambda', M', r'\Theta')) := \max \left\{\frac {|\Lambda-\Lambda'|} {\lambda(z)},\, \frac {|M-M'|} {\mu(z)}, \, \ve \|r\Theta - r'\Theta'\|\right\}.
%$$
This modification is required because the original norm $\|\cdot\|_a$ used in the case $\lambda\neq \mu$ is only a semi-norm when $\lambda = \mu$.
Reasoning similarly to the case $\lambda(z) \neq \mu(z)$ we obtain the upper bound
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H), \ \ve\dil_z(\theta\sep  d_H)\right\}.
$$
We now establish a lower bound on $\dil_z(H)_\times$.
We may assume that $\dil_z(\theta \sep d_H) < \infty$ otherwise there is nothing to prove. Since $\ve>0$ is arbitrary we thus obtain 
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H)\right\} = 2D_z(a)_\times.
$$
We now turn to the lower bound on $\dil_z(H)_\times$. 
For that purpose we define the functions $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda,\mu\}$  and we observe that for all $z,z'\in \Omega$
\begin{eqnarray*}
d_\times (H(z),H(z')) &=& \ln \max \{\|H(z)^\frac 1 2 H(z')^{-\frac 1 2}\|, \, \|H(z')^\frac 1 2 H(z)^{-\frac 1 2}\|\}\\
&\geq & \frac 1 2 \max \{|\ln \|H(z)\|- \ln \|H(z')\||, \, |\ln \|H(z)^{-1}\|- \ln \|H(z')^{-1}\||\\
&=& \max \{ |\ln\gamma(z) - \ln \gamma(z')|,\, |\ln \Gamma(z) - \ln \Gamma(z')|\}.
\end{eqnarray*}
We thus obtain
$$
\dil_z(H)_\times = \dil_z(H\sep d_\times, d_H) \geq \max \{ \dil_z(\ln \gamma\sep d_H), \, \dil_z(\ln \Gamma \sep d_H)\}.
$$
Hence according to Proposition \ref{propDilMax}
$$
\dil_z(H)_\times \geq \max \{\dil_z(\ln \lambda\sep d_H), \dil_z(\ln \mu\sep d_H)\} = D_z(a)_\times.
$$
Therefore $D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times$, and proceeding likewise we obtain $D_z(a)_+ \leq \dil_z(H)_+ \leq 2 D_z(a)_+$, which concludes the proof of Theorem \ref{th2Spaces}. \\

Our first corollary estimates the dilatation in with respect to the euclidean distance, instead of the riemanian distance, of the variable $\theta$ in a graded metric having an eigenspace of dimension $d-1$ at each point..

\begin{corollary}
\label{corolDilThetaG}
Under the hypotheses of Theorem \ref{th2Spaces} we have
%Let $H\in \bH_g$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$ such that $H = \cH\circ a$ on $\Omega$. Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$. Then
$$ 
|\lambda(z) - \mu(z)| \dil_z(\theta) \leq 2 D_z(a)_\times %\leq 2.
$$
\end{corollary}
\proof
Furthermore we have according to \iref{eqDilNormLM}
\begin{eqnarray*}
 |\lambda(z) - \mu(z)| \dil_z(\theta)
&\leq& \frac {|\lambda(z) - \mu(z)|}{\min\{\lambda(z), \mu(z)\}} \dil_z(\theta\sep d_H)\\
&=& \left(\frac {\max \{\lambda(z), \mu(z)\}}{\min\{\lambda(z), \mu(z)\}}-1\right)\dil_z(\theta\sep d_H)\\
& \leq & \left|\frac {\lambda(z)} {\mu(z)}-\frac {\mu(z)} {\lambda(z)}\right|\dil_z(\theta\sep d_H) \\
&\leq & 2 D_z(a)_\times% \leq 2.
\end{eqnarray*}
\sq


The next corollary shows how a quasi-acute metric can be obtained from a graded one.
We denote by $\diag(\lambda_1, \cdots, \lambda_d)$ the diagonal matrix of entries $\lambda_1, \cdots, \lambda_d$. 
Let $M\in S_d$ and let $U\in \cO_d$ and $\lambda_1, \cdots , \lambda_d\in\R$ be such that 
\be
\label{eqDiagSd}
M = U^\trans \diag(\lambda_1, \cdots , \lambda_d) U
\ee
For any $\alpha\in \R$ we define the matrix $\max \{\alpha, M\}\in S_d^+$ as follows
$$
\max\{\alpha, M\} := U^\trans \diag(\max\{\alpha, \lambda_1\}, \cdots, \max\{\alpha, \lambda_d\})U,
$$
and we observe that $\max\{\alpha, M\}$ does not depend on the choice of the matrix $U$ and on the order of the eigenvalues $\lambda_1, \cdots, \lambda_d$ in the decomposition \iref{eqDiagSd}.
For instance we have for any $(\lambda, \mu, \theta)\in \cA$ and any $s>0$  
$$ %\lambda^{-2} \theta\theta^\trans+ \mu^{-2} (\Id-\theta \theta^\trans)
\max \{s^{-2}, \cH(a)\} = \min\{s, \lambda\}^{-2} \theta \theta^\trans+ \min\{s, \mu\}^{-2} (\Id-\theta \theta^\trans).
$$

\begin{corollary}
\label{corolHgToHa}
Let $H\in \bH$ be such that $H(z)$ has an eigenvalue of multiplicity $\geq d-1$ for all $z\in \R^d$. We define $s:\R^d\to \R_+^*$ and $H'\in \bH$ as follows : for all $z\in \R^d$
$$
s(z) := \inf_{z'\in \sR^d} |z-z'|+ \|H(z')^{-\frac 1 2}\|,
$$
and 
$$
H'(z) := \max\{s(z)^{-2}, H(z)\}.
$$
If $H\in \bH_g$, then $4^2H'\in \bH_a$.
\end{corollary}

\proof
For each $\ve>0$ we define 
$$
H_\ve := \max\{e^{2 \ve} s(z)^{-2}, H(z)\}.
$$
The proof proceeds as follows: we first establish that for any $z\in \R^d$ one has 
\be
\label{eqDilHe}
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
\ee
We then use these properties to obtain that $4^2 H_\ve \in \bH_a$, and we conclude the proof using the convergence $H_\ve \to H$ as $\ve \to 0$.\\

We first observe that $s : \R^d \to \R_+^*$ is Lipschitz and that $s(z)\leq \|H(z)^{-\frac 1 2}\|$ for all $z\in \R^d$.

Consider a fixed point $z\in\R^d$. If $H(z)$ is proportional to $\Id$, which means that $\|H(z)\|^{-\frac 1 2} = \|H(z)^{-\frac 1 2}\| \geq s(z)$, then $H_\ve = e^{2 \ve} \Id/ s^2$ on a neighborhood of $z$. This implies according to \iref{eqDilLnH} %\ref{PropEquivS}
$$
\dil_z(H_\ve)_\times =\dil_z(H_\ve)_+ = \dil_z(e^{-\ve} s) \leq e^{-\ve}\leq 1,
$$
and therefore \iref{eqDilHe}.
On the other hand if $H(z)$ is not proportional to $\Id$ then there exists three continuous functions $\lambda, \mu \in C^0(\R^d, \R_+^*)$ and $\theta \in C^0(\R^d, \bbS)$ (where $\bbS := \{u\in \R^d \sep |u| = 1\}$) such that 
$
H = \lambda^{-2} \theta \theta^\trans+ \mu^{-2} (\Id - \theta \theta^\trans).
$
on a neighborhood of $z$.
Hence on the same neighborhood of $z$, 
$$
H_\ve = \min\{e^{-\ve} s,\lambda\}^{-2} \theta \theta^\trans+ \min\{e^{-\ve} s,\mu\}^{-2} (\Id - \theta \theta^\trans).
$$

We now establish that $\dil_z(H_\ve)_\times \leq 2$. 
We define $H_\ve^i := e^{2\ve} \Id/ s^2$ and we observe that $H_\ve \geq H_\ve^i$ and $H_\ve \geq H$, hence for any $p,q\in \R^d$
$$
d_{H_\ve}(p,q) \geq \max \{d_H(p,q), \, d_{H_\ve^i}(p,q)\}.
$$
Using Proposition \ref{propDilLoc} we thus obtain  
\begin{eqnarray*}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\} \sep d_{H_\ve}) &\leq& \max \{\dil_z(\ln (e^{-\ve} s)\sep d_{H_\ve}), \,\dil_z(\ln \lambda\sep d_{H_\ve})\}\\
&\leq & \max \{\dil_z(\ln(e^{-\ve} s \sep d_{H_\ve^i})), \,\dil_z(\ln \lambda\sep d_H)\}\\
& \leq & \max \{\dil_z(e^{-\ve} s), \, \dil_z(H)_\times\}\\
& \leq & \max \{e^{-\ve}, 1\} =1,
\end{eqnarray*}
where we used Theorem \ref{th2Spaces} and Proposition \ref{propEquivS} in the third line.
Likewise $\dil_z(\ln \min\{e^{-\ve} s, \lambda\}\leq 1$. 
Since the function 
$$
t \mapsto \frac t \mu - \frac \mu t
$$
is increasing, we easily obtain that
$$
\left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right| \leq \left|\frac \lambda \mu - \frac \mu \lambda\right|.
$$
Therefore   
$$
\frac 1 2 \left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right|  \dil_z(\theta \sep d_{H_\ve}) \leq \frac 1 2\left|\frac \lambda \mu - \frac \mu \lambda\right| \dil_z(\theta\sep d_H) \leq 1,
$$
which implies that $D_z(a_\ve)_\times \leq 1$ where $a_\ve=(\min\{e^{-\ve}s, \lambda\}, \min\{e^{-\ve} s, \mu\}, \theta) \in C^0(\R^d,\cA)$. Hence
$$
\dil_z(H_\ve)_\times \leq 2 D_z(a_\ve)_\times \leq 2.
$$

We now turn to the proof that $\dil_z(H_\ve)_+ \leq 4$.
As already observed in \iref{eqDilNorm}, for any metric space $(X,d_X)$ and any function $f\in C^0(\R^d, X)$ we have 
\be
\label{eqDilNormLM}
\dil_z(f) \leq \|H(z)\|^{\frac 1 2}\dil_z(f\sep d_H) = \frac{\dil_z(f\sep d_H)}{\min\{\lambda(z), \mu(z)\}}.
\ee
If $\lambda(z)<\mu(z)$ we therefore obtain 
\begin{eqnarray*}
\dil_z(\min\{e^{-\ve} s , \lambda\}) &\leq& \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)}\right\}\\
 &\leq& \max \{e^{-\ve}, \, \dil_z(\ln \lambda\sep  d_H)\}\\
 &\leq & \max \{e^{-\ve} , \, 1\} = 1.
\end{eqnarray*}
Still assuming that $\lambda(z)<\mu(z)$, we have $s(z)\leq \|H(z)^{-\frac 1 2}\| \leq \mu(z)$ by construction of $s$, and therefore $\min\{e^{-\ve} s, \mu\} = e^{-\ve} s$ on a neighborhood of $z$. It follows that 
$$
\dil_z(\min\{e^{-\ve} s, \mu\}) = \dil_z(e^{-\ve} s)\leq e^{-\ve} \leq 1.
$$
Proceeding similarly if $\lambda(z)>\mu(z)$ we also obtain $\dil_z(\min\{e^{-\ve} s, \lambda\})$ and $\dil_z(\min\{e^{-\ve} s, \mu\})$. 
We now focus on the local dilatation of the orientation $\theta$, and for that purpose we observe that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}|  \leq  |\lambda(z) - \mu(z)|.
$$
It follows from Corollary \ref{corolDilThetaG} that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}| \dil_z(\theta) \leq D_z(a)_+ \leq 2,
$$
and therefore $D_z(a_\ve)_+ \leq 2$, which implies $\dil_z(H_\ve)_+ \leq 4$.\\

We have established that for all $z\in \R^d$ and all $\ve>0$
$$
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
$$
Hence for any $z,z'\in \R^d$, since $H_\ve \leq e^{2\ve} H'$,
$$
d_\times(H_\ve(z), H_\ve(z')) \leq 2d_{H_\ve}(z,z') \leq 2e^\ve d_{H'}(z,z') \stext{ and } d_+(H_\ve(z), H_\ve(z')) \leq 4|z-z'|.
$$
Letting $\ve \to 0$ we obtain 
$$
d_\times(H'(z), H'(z')) \leq 2d_{H'}(z,z') \stext{ and } d_+(H'(z), H'(z')) \leq 4|z-z'|.
$$
According to Remark \ref{remHomog} this implies that $4^2 H\in \bH_a$, which concludes the proof of this corollary.
\sq


\section{From mesh to metric}
\label{secMeshToMet}
The techniques presented in this section show how to produce an metric $H\in \bH_i$, $\bH_a$ or $\bH_g$ from an isotropic, quasi-acute (in two dimensions), or graded mesh $\cT$.

Combining the next proposition with its counterpart Proposition \ref{propMeshGen}, on the generation of a mesh from a metric, yields the main result of this chapter: Theorem \ref{thEquiv} on the equivalence of the classes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ of meshes and $\bH_i \subset \bH_a \subset \bH_g$ of metrics which is announced in the introduction.
\begin{prop}
\label{propMetGen}
For any $C_0>0$ there exits $C = C(C_0,d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $\cT \in \bT_{i, C_0}$ there exists $H \in \bH_i$ which is $C$-adapted to $\cT$.
\item If $d=2$, then for any $\cT \in \bT_{a, C_0}$ there exists $H \in \bH_a$ which is $C$-adapted to $\cT$.
\item For any $\cT \in \bT_{g,C_0}$ there exists $H \in \bH_g$ which is $C$-adapted to $\cT$.
\end{enumerate}
\end{prop}

The rest of this section is devoted to the proof of this proposition.
For any mesh $\cT\in \bT$, and for any vertex $v$ of $\cT$, we denote by $n_\cT(v)$ the number of simplices in the mesh $\cT$ containing $v$:
$$
n_\cT(v) := \#\{T\in \cT \sep v\in T\}. %, %\text{s.t. } 
$$
We denote by $H_\cT^g\in \bH$ the piecewise linear metric on $\cT$ which satisfies for each vertex $v$ of $\cT$
\be
\label{eqHcTg}
H_\cT^g(v) := \frac 1 {n_\cT(v)} \sum_{\substack{T\in \cT\\\text{s.t. } v\in T}} \cH_T.
\ee
The metric $H_\cT^g$ on a simplex $T\in \cT$ is simply the linear interpolation of the averages of the matrices $\cH_T$ attached to the simplices containing a vertex $v$. 

The next lemma establishes a property of the barycentric coordinates on a simplex, which is useful for the analysis of  the regularity of a piecewise linear function on an anisotropic mesh, such as the metric $H_\cT^g$.
\begin{lemma}
\label{lemmaNormLambda}
Let $T$ be a simplex and let $V$ be the collection of vertices of $T$. Let $\lambda_v(z)$, $v\in V$ be the barycentric coordinates on $T$. Then for all $z,z'\in T$
\be
\label{eqNormLambda}
\|z-z'\|^2_{\cH_T} = \frac {d+1} d \sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2.
\ee
\end{lemma}

\proof
We first assume that $T$ is the reference equilateral simplex $\TEq$. %, and we recall that $\cH_\TEq = \Id$.
For any two vertices $v,v'$ in the collection $\VEq$ of vertices of $\TEq$ one easily checks that 
\be
\label{eqScalTEq}
\<v,v'\> = 
\left\{
\begin{array}{cl}
1 &\text{ if } v=v,'\\
-1/d &\text{ if } v \neq v'.
\end{array}
\right.
\ee
Indeed $|v|=1$ by construction for any vertex $v$ of $\TEq$, the scalar product $\<v,v'\>$ has a value $\alpha$ which is independent of the pair of distinct vertices $v,v'\in \VEq$. Since $\TEq$ is centered at the origin we obtain $0 = \<v,\sum_{v\in V} v\>  = |v|^2 + d \alpha$ which establishes \iref{eqScalTEq}.
We thus obtain for any $z,z'\in \TEq$ 
\begin{eqnarray*}
|z-z'|^2  &=& \left|\sum_{v\in \VEq} (\lambda_v(z) - \lambda_v(z'))v\right|^2 \\
&=& \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \sum_{v\neq v'} (\lambda_v(z)-\lambda_v(z'))(\lambda_{v'}(z)-\lambda_{v'}(z')).
\end{eqnarray*}
Therefore 
$$
|z-z'|^2 =  \left(1+\frac 1 d\right) \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \left(\sum_{v\in \VEq} \lambda_v(z)-\lambda_v(z')\right)^2,
$$
which concludes the proof in the case of $\TEq$ since $\cH_\TEq = \Id$ and since the barycentric coordinates of $z$ and of $z'$ sum to $1$.

We now consider an arbitrary simplex $T$, and an affine change change of coordinates $\Phi$ such that $\Phi(T) = \TEq$, $\Phi(z) = \phi z+ z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. We have $\cH_T = \phi^\trans \phi$ according to \iref{invcH}, hence for all $z,z'\in T$
$$
 |\Phi(z) - \Phi(z')| = |\phi(z-z')| = \|z-z'\|_{\cH_T}.
$$
Furthermore the barycentric coordinates of $z$ and $z'$ in $T$ are the same as those of $\Phi(z)$ and $\Phi(z')$ in $\Phi(T) = \TEq$, hence \iref{eqNormLambda} holds which concludes the proof of this lemma.
\sq



The next proposition establishes that the metric $H_\cT^g$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case iii) of graded meshes. More precisely for any mesh $\cT\in \bT_{g,C_0}$ the metric $d C_0^{10} H_\cT^g$ belongs to $\bH_g$ and is $C_0^6 \sqrt d$ equivalent to $\cT$.



\begin{prop}
\label{propHTG}
For any $\cT\in \bT_{g,C_0}$ the metric $H_\cT^g$ is $C_0$-adapted to $\cT$, and $d C_0^{10} H_\cT^g\in \bH_g$.
\end{prop}

\proof
We consider a simplex $T\in \cT$, and we recall that for any neighbor $T'$ of $T$ one has 
$$
C_0^{-2} \cH_T \leq \cH_{T'} \leq C_0^2 \cH_T.
$$
Averaging these matrices as in \iref{eqHcTg} we obtain for any vertex $v$ of $T$
\be
\label{eqHTHv}
C_0^{-2} \cH_T \leq H_\cT^g(v)\leq C_0^2 \cH_T.
\ee
Averaging with respect to the barycentric coordinates of a point $z\in T$ we eventually obtain 
\be
\label{eqHTHz}
C_0^{-2} \cH_T \leq H_\cT^g(z)\leq C_0^2 \cH_T,
\ee
which establishes as announced that the metric $H_\cT^g$ is $C_0$-adapted to $\cT$.

We now establish the regularity property of $H_\cT^g$, and for that purpose we consider two points $z,z'\in T$ and a vector $u\in \R^d\sm\{0\}$. We thus have 
\begin{eqnarray*}
\frac {\|u\|^2_{H_\cT^g(z)}} {\|u\|^2_{H_\cT^g(z')}} &=& \frac {\sum_{v\in V} \lambda_v(z) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2} \\
&=& 1+ \frac {\sum_{v\in V} (\lambda_v(z)-\lambda_v(z')) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2}\\
&\leq& 1+ C_0^4 \frac{\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|}{\sum_{v\in V} \lambda_v(z')}\\
& \leq & 1+C_0^4 \sqrt {(d+1)\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2}\\
&=& 1+C_0^4 \sqrt d \| z-z'\|_{\cH_T},
\end{eqnarray*}
where we used \iref{eqHTHv} in the third line, Cauchy-Schwartz inequality in the fourth line, and Lemma \iref{lemmaNormLambda} in the fifth line.
We consider a simplex $T\in \cT$ and we intend to give a uniform bound on $\dil_z(H_\cT^g)_\times$ for all $z\in \interior(T)$. It follows from our estimate on $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, and from the analog estimate for  $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, that 
\begin{eqnarray*}
d_\times (H_\cT^g(z), H_\cT^g(z')) &=& \max_{u\neq 0} \left|\ln \|u\|_{H_\cT^g(z)} - \ln \|u\|_{H_\cT^g(z')}\right|\\
&\leq& \frac 1 2\ln (1+C_0^4 \sqrt d \|z-z'\|_{\cH_T}) \\
&\leq& \frac {C_0^4 \sqrt d} 2 \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Hence according to \iref{eqHTHz} and \iref{eqDilNorm} we obtain for all $z\in \interior (T)$
$$
\dil_z(H_\cT^g)_\times \leq C_0^5 \sqrt d.
$$
The metric $H := d C_0^{10} H_\cT^g$ thus satisfies $\dil_z(H)_\times = (dC_0^{10})^{-1/2}\dil_z(H_\cT^g)_\times \leq 1$ for any point $z$ in the interior of any simplex $T\in \cT$.
If follows from Corollary \ref{corolLipNoGamma} that $H \in \bH_g$, which concludes the proof.
\sq

We associate to any mesh $\cT\in \bT$ a metric $H_\cT^i$ defined as follows : for all $z\in \R^d$, 
$$
H_\cT^i(z) := \|H_\cT^g(z)\| \Id.
$$
The next result shows that $H_\cT^i$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case of isotropic metrics. More precisely for any mesh $\cT\in \bT_{i,C_0}$ the metric $d C_0^{10} H_\cT^i$ belongs to $\bH_i$ and is $C_0^7 \sqrt d$ equivalent to the mesh $\cT$.

\begin{corollary}
For any mesh $\cT\in \bT_{i,C_0}$ the metric $H_\cT^i$ is $C_0^2$-adapted to the mesh $\cT$, and $d C_0^{10} H_\cT^i \in \bH_i$.
\end{corollary}

\proof
For any matrix $M\in S_d^+$ we have $\|M^{-1}\|^{-1} \Id \leq M \leq \|M\| \Id$. We therefore obtain for any simplex $T\in \cT$
\be
\label{eqcHNormcH}
C_0^{-2} \|\cH_T\| \Id\leq \frac{\|\cH_T\|} {\rho(T)^2} \Id = \|\cH_T^{-1}\|^{-1} \Id \leq \cH_T \leq \|\cH_T\|\Id.
\ee
Let $T\in \cT$ and let $z\in T$. Since $\rho(T) \leq C_0$ and $C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z)$ we obtain 
$$
C_0^{-2} H_\cT^i(z) := C_0^{-2} \|H_\cT^g(z)\| \Id \leq \|\cH_T\| \Id \leq C_0^2 H_\cT^i(z).
$$
Combining this with \iref{eqcHNormcH} we obtain
$$
C_0^{-4} H_\cT^i(z) \leq \cH_T \leq C_0^2 H_\cT^i(z),
$$
which establishes as announced that the metric $H_\cT^i$ is $C_0^2$ equivalent to the mesh $\cT$.

According to Proposition \ref{propHTG} we have $d C_0^{10} H_\cT^g\in \bH_g$. Corollary \ref{corolLipNorm} thus implies that $d C_0^{10} H_\cT^i\in \bH_i$, which concludes the proof of this proposition.
\sq

Before turning to the case of quasi-acute metrics we prove a lemma on the neighborhood of a simplex in a graded mesh. For any mesh $\cT\in \bT$ and any closed set $E\subset \R^d$ the neighborhood $V_\cT(E)$ of $E$ in $\cT$ is  defined as the union of all simplices $T\in \cT$ which intersect $E$: 
$$
V_\cT(E) := \cup_{\substack{T\in \cT\\T \cap E \neq \emptyset}} T.
$$

\begin{prop}
\label{propNeighborT}
Let $\cT\in \bT_{g,C_0}$ and let $T \in \cT$, then for all $x\in T$ and all $y \in \R^d \sm V_\cT(T)$ we have 
$$
\|x-y\|_{\cH_T} \geq (C_0\sqrt d)^{-1}.
$$
\end{prop}

\proof
The simplex $T\in \cT$ is fixed throughout this proof. We consider the function $\vp : \R^d \to \R$ which is piecewise linear on the mesh $\cT$, and which satisfies for any vertex $v$ of the mesh $\cT$
$$
\vp(v) = 
\left\{
\begin{array}{cl}
1 & \text{ if } v\in T,\\
0 & \text{ if } v \notin T.
\end{array}
\right.
$$
We denote by $V'$ the collection of vertices of a simplex $T'\in \cT$, and by $(\lambda_v(z))_{v\in V'}$ the barycentric coordinates of a point $z\in T'$.
We have for any $z,z'\in T'$
\begin{eqnarray*}
|\vp(z)- \vp(z')| &\leq& \sum_{v \in V'} |\lambda_v(z)-\lambda_v(z')| \vp(v)\\
& \leq &\sqrt{(d+1) \sum_{v\in V'} |\lambda_v(z)-\lambda_v(z')|^2} \\
&= &\sqrt d \|z-z'\|_{\cH_{T'}}.
\end{eqnarray*}
Recalling that $\vp$ is identically $0$ on $T'$ if $T\cap T' = \emptyset$, and that $\cH_{T'} \leq C_0^2 \cH_T$ otherwise, we obtain for any $z,z'\in T'$
$$
|\vp(z)- \vp(z')| \leq C_0\sqrt d \|z-z'\|_{\cH_{T}}.
$$
If follows from Corollary \ref{corolLipNoGamma} that $\vp : (\R^d, \|\cdot \|_{\cH_T})  \to \R$ is $C_0\sqrt d$-Lipschitz.
For any $x\in T$ and any $y\in \R^d\sm V_\cT(T)$ we have $\vp(x) = 1$, $\vp(y) = 0$, thus $1 \leq C_0\sqrt d \|x-y\|_{\cH_T}$ which concludes the proof of this proposition.
\sq

We assume from this point that the dimension is $d=2$. %, and we thus restrict our attention to the bi-dimensional triangulations.
For each triangulation $\cT\in \bT$ we define a function $s_\cT : \R^2 \to \R_+^*$ as follows 
$$
s_\cT(z) := \inf_{z'\in \sR^2} |z-z'| + \|H_\cT^g(z')^{-\frac 1 2}\|.
$$
We define a metric $H_\cT^a \in \bH$ as follows : for each $z\in \R^2$  
\be
\label{defHTA}
H_\cT^a(z) = \max\{s_\cT(z)^{-2} , \, H_\cT^g(z)\}.
\ee

The rest of this section is devoted to proof of the following proposition, on quasi-acute meshes, in two dimensions.
\begin{prop}
\label{propHTA}
For any $C_0 \geq 1$ there exists $C=C(C_0)$ such that the following holds.
For any $\cT\in \bT_{a,C_0}$ the metric $H_\cT^a$ is $C$-adapted to the mesh $\cT$, and $32 C_0^{10} H_\cT^a\in \bH_a$.
\end{prop}

The author is sorry to say that, due to time constraints, this proof is not as polished as the rest of the thesis.

The fact that $32 C_0^{10} H_\cT^a\in \bH_a$ directly follows from the fact that $2 C_0^{10} \bH_\cT^g\in \bH_g$ and from Corollary \ref{corolHgToHa}. 

For each $z\in \R^2$ define $d_\cT(z) := \|H_\cT^g(z)^{-\frac 1 2}\|$. This quantity should be heuristically regarded as the diameter of the triangle containing $z$. We establish below the following property : there exists $\delta = \delta(C_0) >0$ such that for all $z,z'\in \R^2$
\be
\label{eqRegDT}
\text{ if } |z'-z| \leq \delta d_\cT(z) \stext{ then }  d_\cT(z') \geq \delta d_\cT(z).
\ee
Before turning to the proof of \iref{eqRegDT} we show how this property leads to the proof of Proposition \ref{propHTA}.
For all $z\in \R^d$ we have 
$$
s_\cT(z) = \inf_{z\in \sR^2} |z-z'|+d_\cT(z)  \geq \inf_{z'\in \sR^2} \min \{|z-z'|, \, d_\cT(z')\} \geq \delta d_\cT(z'),
$$
indeed $|z-z'|\geq \delta d_\cT(z)$ or $d_\cT(z') \geq \delta d_\cT(z)$ for any $z'\in \R^d$ according to \iref{eqRegDT}.
Combining this with the definition \iref{defHTA} of $H_\cT^a$ we obtain for all $z\in \R^2$
$$
\delta^2 H_\cT^a(z) \leq H_\cT^g(z)\leq H_\cT^a(z). 
$$
Recalling that $H_\cT^g$ is $C_0$-adapted to the mesh $\cT$, see proposition \ref{propHTG}, we obtain for all $T\in \cT$ and all $z\in T$ 
$$
\delta^2 C_0^{-2} H_\cT^a(z) \leq C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z) \leq C_0^2 H_\cT^a(z)
$$
which establishes that the metric $H_\cT^a$ is $C_0/\delta$ adapted to the mesh $\cT$, and concludes the proof of Proposition \ref{propHTA}.\\

For each $u\in \R^2$, we denote by $u^\perp$ the vector obtained by rotating $u$ by $\cPi/2$ in direct trigonometric orientation sense.

We now turn to the proof of \iref{eqRegDT}, and for that purpose we introduce some notations.
For each segment $e=[\omega-u, \omega+u]\subset \R^2$ we define the diamond $\lozenge(e)$ of $e$ as follows
$$
\lozenge(e) := \{z\in \R^2 \sep |\<z-\omega,u\>|+ C_0 |\<z-\omega,u^\perp\>| < |u|^2\}.
$$
This set is illustrated on Figure \ref{figLozenge} (left).

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/LozengeJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/SeqZnJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/TRedJenny.pdf}
\caption{An edge $e$ and the set $\lozenge(e)$ (left), sequence $(z_n)_{n \geq 0}$ (center), diameter of a triangle intersecting $\lozenge(e)$ (right). \label{figLozenge}}
\end{figure}

The next lemma considers a triangulation $\cT'$ on which the measure of sliverness is uniformly bounded by $C_0$, and compares the length an edge $e$ of $\cT'$ with the diameter of the triangles in $\cT'$ which intersect $\lozenge(e)$.

\begin{lemma}
\label{lemmaUUp}
Let $\cT'\in \bT$ be a triangulation such that $S(T) \leq C_0$ for all $T\in \cT'$. Let  $e=[\omega-u, \omega+u]$ be an edge of $\cT'$.
Then there is no vertex in the diamond $\lozenge(e)$, and for all $z\in \lozenge(e)$ and any triangle $T\in \cT'$ containing $z$, there exists an edge $e'= [\omega'-u', \omega'+u']$ of $T$ satisfying  
$$
2 |u'| \geq |u| -C_0 |\<z-\omega,u^\perp\>|/ |u|
%2 |\<u,u'\>| \geq |u|^2 - C_0 |\det (z,u)|.
$$
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$, and we assume up to a translation and a rotation that $\omega = 0$ and $u = u_y$.
We recall that for any triangle $T$, with maximal angle $\theta$, the measure of sliverness $S(T)$ has the following expression
$$
S(T) = \max\{1, \tan(\theta/2)\}.
$$
We assume for contradiction that there exists a vertex $v_0 = (x_0,y_0)\in \lozenge(e)$, and we assume without loss of generality that $x_0<0$. We consider a vertex $v_1 = (x_1,y_1)$ of $\cT$ such that the angle 
$$
\theta_0 :=  \angle(v_1-v_0, \, u_x) \in [-\cPi, \cPi)
$$
has the smallest possible absolute value $|\theta_0|$ (the bold letter $\cPi$ denotes the numerical constant $\cPi = 3.14159\cdots$). By construction there exists a triangle $T\in \cT$ containing $v_0$ and $v_1$ which has an angle  larger or equal or equal than $2\theta_0$ at the vertex $v_0$. It follows that $|\tan \theta_0| \leq S(T) \leq C_0$, and therefore  
$$
|y_1-y_0| \leq |\tan \theta_0| (x_1 - x_0) \leq C_0 (x_1-x_0).
$$
Proceeding inductively, as illustrated on Figure \ref{figLozenge} (center), we define a sequence $z_n = (x_n, y_n)$, $n\geq 0$, of vertices of $\cT$ satisfying 
$
|y_{n+1} - y_n| \leq C_0 (x_{n+1} - x_n). 
$
Adding these inequalities together we obtain 
$$
|y_n-y_0|  \leq C_0 (x_n-x_0).
$$
It follows that one of the edges $[z_n, z_{n+1}]$, $n \geq 0$, of the mesh $\cT'$ intersects the edge $e$, which is a contradiction. The diamond $\lozenge(e)$ therefore does not contain any vertex, which concludes the proof of the first part of this proposition. \\

We now consider a point $z_0 = (x_0,y_0)\in \lozenge(e)$ and we assume without loss of generality that $x_0 \geq 0$. We consider a triangle $T$ containing $z_0$, and an edge $e'= [\omega'-u', \omega'+u']$ of $T$ which is on the left of $z_0$ (in other words the edge $e'$ and the segment $[(0,y_0),(x_0, y_0)]$ joining the point $z_0$ to its orthogonal projection on the edge $e$ intersect). The point $z_0$ and the triangle $T$ are illustrated on Figure \ref{figLozenge} (right).

Since there is no vertex of $\cT'$ in the diamond $\lozenge(e)$, the edge $e'$ intersects the boundary of $\lozenge(e)$ at two points. We denote these points by $(x,y)$ and $(x',y')$, and we assume that without loss of generality that $y\geq 0 \geq y'$.
Observing that $0 \leq x \leq C_0^{-1}$, $0 \leq x'\leq C_0^{-1}$ and $\min\{x,x'\} \leq x_0$ we obtain  
$$
y-y' = (1-C_0 x) - (-1+C_0 x') \geq 1-C_0 x_0.
$$
Since $u = u_y = (0,1)$, $\omega = 0$ and $2 u' = \lambda (x-x', y-y')$ for some $|\lambda| \geq 1$, we obtain 
$$
2|\<u,u'\>| \geq  
y-y' \geq 1-C_0 x_0 = |u|^2 - C_0 |\<z_0-\omega,u\>|,
$$
which concludes the proof of this proposition.
\sq

\begin{figure}
\centering
\includegraphics[width = 4.5cm, height = 4cm]{\pathPic/Dessins/Jenny/LozengeCarreDeltaJenny.pdf}
\includegraphics[width = 2.5cm, height = 4cm]{\pathPic/Dessins/Jenny/CarreDeltaCarreEJenny.pdf}
\caption{An edge $e$, the diamond $\lozenge(e)$ and the rectangle $\square_\delta$ involved in Lemma \ref{lemmaRect} (left), the rectangles $\square_e$ and $\square_\delta$.
\label{figSquare}
}
\end{figure}


We now consider a fixed quasi-acute mesh $\cT\in \bT_{a,C_0}$ and we denote by $\cT'$ a fixed $C_0$-refinement of $\cT$ which satisfies $S(T) \leq C_0$ for all $T\in \cT'$. The next proposition involves a rectangular set $\square(e)$ associated to an edge $e$ of $\cT'$ which contains $e$ in its interior, in contrast to the set $\lozenge(e)$ appearing in the previous proposition.  
This set is illustrated on Figure \ref{figSquare} (right).
\begin{lemma}
\label{lemmaRect}
There exists a constant $\delta_0 = \delta_0(C_0, d)>0$ such that the following holds.
We define the rectangle $\square(e)$ associated to an edge $e = [\omega-u, \, \omega+u]$ of $\cT'$ as follows
$$
\square(e) = \{z\in \R^2 \sep |\<z-\omega, u\>|\leq (1+\delta_0)|u|^2 \text{ and } |\<z-\omega,u^\perp \>| \leq \delta_0 |u|^2\},
$$
%where $\delta_0 = \delta_0(C_0):= ??1/(2C_0) >0$ is a constant specified in the proof.
We have $d_\cT(z) \geq \delta_0|u|$ for all $z\in \square(e)$.
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$. 
Up to a rotation and a translation, we may again assume that $\omega = 0$ and $u = u_y=(0,1)$.
We consider a triangle $T\in \cT$ containing the edge $e$ (note that $e\subset T$ but that $e$ may not be an edge of $T$, since we only known that $e$ is an edge in $\cT'$).

We define $H := H_\cT^g$. Recalling that $H$ is $C_0$-equivalent to $\cT$ we obtain for all $z\in e$
$$
C_0^{-2} H(z)\leq \cH_T \leq C_0^2 H(z). 
$$
The inclusion $e\subset T \subset \cE_T$ implies the upper bound $\|u\|_{\cH_T} = \|u_y\|_{\cH_T} \leq 1$. Hence for all $z\in e$
$$
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq \|u_y\|_{H(z)}^{-1} \geq C_0^{-1}.
$$
Note also that for any $z,u \in \R^2$
$$
d_\times (H(z), H(z+u)) \geq \ln \|H(z)^\frac 1 2 H(z+u)^{-\frac 1 2}\| \geq |\ln d_\cT(z) -\ln d_\cT(z+u)|.
$$
We define $C_1 := \sqrt 2 C_0^5$, in such way that $C_1^2 H\in \bH_g$, and we thus have  according to \iref{eqLocalNorm} if $C_1\|u\|_{H(z)}<1$
$$
|\ln d_\cT(z) -\ln d_\cT(z+u)| \leq d_\times (H(z), H(z+u)) \leq -\ln (1-C_1\|u\|_{H(z)}).
$$
Therefore for all $z\in e$ and all $u\in \R^d$,
$$
d_\cT(z+u) \geq d_\cT(z) (1-C_1 \|u\|_{H(z)}) \geq C_0^{-1}(1-C_1C_0 \|u\|_{\cH_T}).
$$
We define $C_2 := 4C_0C_1$ and we observe that any point of the rectangle 
\be
\label{eqRectGrad}
\left[\frac {-1}{C_2 \|u_x\|_{\cH_T}}, \,\frac 1 {C_2 \|u_x\|_{\cH_T}}\right] \times \left[-(1+C_2^{-1}), \, 1+C_2^{-1}\right].
\ee
can be written under the form $z+u$ where $z\in e$ and $\|u\|_{\cH_T} \leq 1/(2C_0C_1)$. We thus have  
\be
\label{eqdGrad}
d_\cT(z') \geq 1/(2C_0)
\ee
 on this rectangle.

We introduce a small constant $\delta = \delta(C_0)>0$ which is specified later in the proof. It follows from \iref{eqRectGrad} and \iref{eqdGrad} that the proof of this lemma is complete if $\|\cH_T\| \leq \delta^{-2}$, with $\delta_0 := \min \{\delta/C_2, \, 1/(2C_0)\}$.
We thus assume from this point that $\|\cH_T\|\geq \delta^{-2}$.\\

We assume that $\delta< C_0^{-1}$ and we define the rectangle
$$
\square_\delta := [-\delta, \delta] \times [1-C_0 \delta, -1+C_0 \delta],
$$
which is included in $\overline \lozenge(e)$ by construction.
Since $C_1^2 H\in \bH_g$, the function $z\mapsto \|H(z)\|^{-\frac 1 2}$ is $C_1$-Lipschitz according to Corollary \ref{corolLipNorm}. We thus have for all $z = (x,y)\in \square_\delta$
\be
\label{defr0}
\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2}+C_1|x|\leq r_0(\delta) := (C_0+C_1)\delta.
%\|u_x\|_{H(z)} \geq \|u_x\|_{H(y,0)}(1-C_1 |x| \|u_x\|_{H(y,0)}) \geq C_*(1-C_1 C_0 \delta_* C_*),
%\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2} + C_1 |x|
\ee
On the other hand it follows from Lemma \ref{lemmaUUp} that any $z = (x,y)\in \square_\delta$ is contained in a triangle containing an edge $e' = [\omega'-u', \omega'+u']$ such that $|u'| \geq (1-C_0 \delta)/2$. We thus have 
$$
1 \geq \|u'\|_{\cH_{T'}} \geq \frac{|u'|}{ \|\cH_{T'}^{-\frac 1 2}\|} \geq \frac{1-C_0 \delta}{2 \|\cH_{T'}^{-\frac 1 2}\|} 
$$
and therefore 
%of length at least $T'\in \cT$ satisfying $\|\cH_{T'}^{-\frac 1 2}\| \geq (1-C_0 \delta_*)/2$, hence 
\be
\label{defR0}
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq C_0^{-1} \|\cH_{T'}^{-\frac 1 2}\|  \geq  R_0(\delta) := (1-C_0 \delta)/(2C_0). %\det (z,u_y)
\ee
For all $z\in \square_\delta$, we denote by $\theta(z) = (\cos \Theta(z), \sin \Theta(z))$, $\Theta(z)\in [0, \cPi]$, the direction of the eigenvector associated to the small eigenvalue of $H(z)$, in such way that 
\be
\label{eqNormTheta}
\|\theta(z)\|_{H(z)} = \|H(z)^{-\frac 1 2}\|^{-1} = d_\cT(z)^{-1}.
\ee
We thus have for any $(0,y)\in e$
$$
C_0 \geq C_0 \|u_y\|_{\cH_T} \geq \|u_y\|_{H(0,y)} \geq |\cos \Theta(0,y)| \sqrt{\|H(0,y)\|} = \delta^{-1} |\cos \Theta(0,y)| ,
$$
hence 
$$
|\cos \Theta(0,y)| \leq  C_0 \delta.
$$
For all $z\in \square_\delta$ we have according to Corollary \ref{corolDilThetaG} %Theorem \ref{th2Spaces} 
$$
(R_0(\delta)-r_0(\delta)) \dil_z(\Theta) \leq  (\|H(z)^{-\frac 1 2}\| - \|H(z)\|^{-\frac 1 2}) \dil_z(\Theta) \leq 2C_1.
$$
Hence we obtain for all $z= (x,y)\in \square_\delta$  
$$
(R_0(\delta)-r_0(\delta)) |\Theta(z) - \Theta(0,y)| \leq 2C_1 |x|\leq 2C_1 \delta,
$$
hence since $t \mapsto \cos t$ is a Lipschitz function %, since $\cos : [0, \cPi/2]\to \R$ is convex
\be
\label{defTheta0}
|\cos \Theta(z)| \leq \cos \Theta_0(\delta) := C_0 \delta + \frac{\delta}{R_0(\delta)-r_0(\delta)}.
\ee
We have according to \iref{eqLocalNorm} for all $z\in \square_\delta$ and all $r\geq 0$ such that $C_1r\|\theta\|_{H(z)}<1$,
\begin{eqnarray*}
|\ln d_\cT(z+r \theta(z)) - \ln d_\cT(z)| &\leq& d_\times (H(z+r\theta(z)),H(z))\\
&\leq& -\ln (1-C_1r\|\theta\|_{H(z)})\\
&=& -\ln (1-C_1r/d_\cT(z)),
\end{eqnarray*}
therefore 
$$
d_\cT(z+r \theta(z)) \geq  d_\cT(z) (1-|r| C_1 /d_\cT(z)).
$$
For all $z\in \square_\delta$ such that $|r|\leq R_1(\delta) := R_0(\delta)/(2C_1)$ we thus obtain
$$
d_\cT(z+r\theta(z)) \geq R_0(\delta)(1-|r|C_1/R_0(\delta))\geq R_0(\delta)/2.
$$
It follows that $d_\cT(z')\geq R_0(\delta)/2$ for all $z'$ in the set 
$$
\{z+r\theta(z) \sep z\in \square_\delta,\, |r|\leq R_1(\delta)\} \supset [-\delta_0,\delta_0]\times [-(1+\mu_0),1+\mu_0]
$$
where 
\be
\label{eqD0MU0}
\delta_0 := \delta - r \cos \Theta_0(\delta) \stext{ and }  \mu_0 := -C_0 \delta+ r \sin \Theta_0(\delta)
\ee
and where the constant $0 \leq r\leq R_1(\delta)$ can be freely chosen.
The rest of the proof consists in choosing appropriate constants $\delta$ and $r$.\\

As $\delta \to 0$ we have $r_0(\delta)\to 0$, $R_0(\delta) \to 1/(2C_0)$ and $\cos\Theta_0(\delta) \to 0$. We thus choose $\delta = \delta(C_0,d)>0$ sufficiently small in such way that 
\be
\label{eqRCS}
R_0 \geq 1/(4C_0)
, \quad
\cos \Theta_0 \leq 1/(8C_0)
, \quad
\sin \Theta_0 \geq 1/2
.
\ee
We then choose $r := 4C_0 \delta$, which is smaller than $R_1(\delta)= R_0(\delta)/(2C_1) \geq 1/(8C_1C_0)$ if $\delta$ is sufficiently small. Injecting this choice of $r$ and \iref{eqRCS} in \iref{eqD0MU0} we thus obtain 
$$
\delta_0 \geq \delta/2 \stext{ and }\mu_0 \geq C_0 \delta.
$$
We have thus established under the hypothesis $\|\cH_T\|\geq \delta^{-2}$ that 
hence $d_\cT(z) \geq 1/(8C_0)$ for all $z$ in the rectangle 
$$
[-\delta/2, \delta/2]\times [-(1+C_0\delta), 1+C_0 \delta].
$$
Since the case $\|\cH_T\|\leq \delta^{-2}$ is already established this concludes the proof of this proposition.
\sq

The next lemma establishes a technical property on the covering a one dimensional segment by smaller ones, which is a key to the end of this proof.

\begin{lemma}
\label{lemmaCoverSeg}
Let $x_1, \cdots , x_k\in [0,1]$ and let $h_1, \cdots, h_k >0$ be such that 
\be
\label{eqDefXiHi}
[0,1]\subset \bigcup_{1\leq i \leq k} [x_i-h_i, \, x_i+h_i].
\ee
Let $\delta>0$ and let $h_* = h_*(k,\delta) := \exp(1-2k/\delta)/\delta$. Then 
\be
\label{eqInclSeg}
[0,1]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_* \leq h_i}} [x_i-(1+\delta)h_i, \, x_i+(1+\delta)h_i].
\ee
\end{lemma}

\proof
For each $y\in [0,1]$ we denote by $h(y)$ the value $h_i$ associated to the segment $[x_i-h_i, x_i+h_i]$ of smallest length containing $y$.
We thus have 
$$
\int_{[0,1]} \frac {dy} {h(y)} \leq \sum_{1\leq i \leq k} \int_{x_i-h_i}^{x_i+h_i} \frac 1 {h_i} = 2k.
$$
We assume for contradiction that \iref{eqInclSeg} does not hold, and we consider a point $x\in [0,1]$ which does not belong to the right hand side of $[0,1]$. For each $y\in [0,1]$ one of the two following possibilities holds
$$
\delta h(y) < |x-y| \stext{ or } h(y) < h_*.
$$
Integrating we obtain 
$$
\int_0^1 \frac {dy} {h(y)}  \geq \int_0^1 \frac {dy} {\max\{|x-y|/\delta,\, h_*\}}.
$$
The minimum value of the right hand side is attained for $x=0$ or $1$ and equals 
$$
\int_0^1 \frac {dy}{\max \{|x-y|/\delta, h_*\}} = \int_0^{\delta h_*} \frac 1 h_* + \int_{\delta h_*}^1 \frac \delta ydy = \delta(1-\ln(\delta h_*))
$$
Thus $2k>\delta(1-\ln(\delta h_*))$, which contradicts the definition of $h_*$. This concludes the proof of this lemma.
\sq

Under the hypotheses of Lemma \ref{lemmaCoverSeg} we thus have
\be
\label{eqInclSegDouble}
[-h_*\delta,\, 1+h_*\delta]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_i \leq h_*}} [x_i-(1+2\delta)h_i, \, x_i+(1+2\delta)h_i].
\ee


We now conclude the proof of Proposition \ref{propHTA}.
We consider a point $z\in \R^2$ contained in a triangle $T\in \cT$, and we denote by $\cT$ the longest edge $e$ of $T$. Up to a rotation and a translation, we may assume that $e=[0, u_x]$ joins the origin of $\R^2$ to the the vector $u_x := (1,0)$.
Note that 
\be
\label{eqNormHTInv}
2 \geq \|u_x\|_{\cH_T} \geq \|\cH_T^{-\frac 1 2}\|^{-1}.
\ee
Since the triangulation $\cT'$ is a $C_0$-refinement of $\cT$, the edge $e$ of $T$ is built of $k \leq C_0$ edges $(e_i)_{1 \leq i \leq k}$ of $\cT'$,
$$
e_i = [(x_i-h_i)u_x,\,  (x_i +h_i) u_x].
$$
The triangle $T$ and the edges $(e_i)_{1\leq i\leq k}$ are illustrated on Figure \ref{figTFlat} (left).

\begin{figure}
\centering
\includegraphics[width = 7cm, height = 1.5cm]{\pathPic/Dessins/Jenny/TFlatJenny.pdf}
\includegraphics[width = 8cm, height = 2.5cm]{\pathPic/Dessins/Jenny/cupCarresJenny.pdf}
\caption{
A triangle $T\in \cT$ and the edges $(e_i)_{1\leq i \leq k}$ of $\cT'$ contained in $T$ (left), the set \iref{eqRectHoDo} (right). 
\label{figTFlat}}
\end{figure}

We define $h_* := h_*(C_0, \delta_0/2) = 2\exp(1-4C_0/\delta_0)/\delta_0$, where $\delta_0$ is the constant from Lemma \ref{lemmaRect}, and we observe that 
\be
\label{eqRectHoDo}
\bigcup_{h_* \leq h_i} \square(e_i) \supset \left[-\frac{h_* \delta_0} 2, 1+ \frac{h_* \delta_0} 2\right] \times [-h_* \delta_0, h_* \delta_0],
\ee
This set is illustrated on Figure \ref{figTFlat} (right).
Since $e$ is the longest edge of $T$, the angles of $T$ at the extremities of $e$ are acute.
Furthermore the height $h$ of $T$ orthogonal to the edge $e = [0,u_x]$ satisfies 
$$
h/2 = |T|  = \frac{|\TEq|} { \sqrt {\det \cH_T}} = \frac{|\TEq|}{\sqrt{\|\cH_T\| \|\cH_T^{-1}\|^{-1}}}  = \frac{|\TEq| \|\cH_T^{-1}\|}{\rho(T)} \geq \frac{|\TEq|}{4 \rho(T)} .
$$
Hence we obtain with $c := |\TEq|/8$ the inclusion
\be
\label{eqTRectRho}
T \subset [0,1] \times [-c/\rho(T), c/\rho(T)]
\ee
We distinguish two cases depending on the value of $\rho(T)$. If $c/\rho(T) \leq h_* \delta_0$, equivalently $\rho(T) \geq c/(h_* \delta_0)$ we obtain combining \iref{eqRectHoDo} and \iref{eqTRactRho} that $d_\cT\geq h_*\delta_0$ on the set 
$$
z+ \left[-\frac {h_*\delta_0} 2, \frac {h_*\delta_0} 2\right]^2
$$
which concludes the proof of this proposition.
One the other hand we have for any vector $u\in \R^2$
$$
\frac{d_\cT(z+u)}{d_\cT(z)} \geq  1-C_1 \|u\|_{H(z)} \geq 1-C_0C_1 \|u\|_{\cH_T} \geq  1-C_0C_1 \rho(T) |u| \|\cH_T^{-\frac 1 2}\|^{-1} \geq 1-2 C_0C_1 \rho(T) |u| 
$$
which concludes the proof if $\rho(T) \leq c/(h_*\delta_0)$.

\section{From metric to mesh}
\label{secMetToMesh}
%\subsection{Mesh generation}
\label{secMeshGen}

%We prove in this section Theorems \ref{thI}, \ref{thA} and \ref{thR} on the equivalence between certain classes of meshes and of metrics. %, which is divided in two parts.
%This proof is divided in two parts as follows. Proposition \ref{propMeshGen} in \S \ref{secMeshGen} we show how a mesh can be generated from a Riemannian metric, and Proposition \ref{propMetGen} in \S\ref{secMetGen} we show how a metric can be generated from a mesh.
%
This section is dedicated to the proof of the following result, on the generation of a mesh from a metric.
\begin{prop}
\label{propMeshGen}
There exists $C_0 = C_0(d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $H\in \bH_i$ there exists $\cT \in \bT_{i,C_0}$ which is $C_0$-adapted to $H$.
\item If $d=2$, then for any $H \in \bH_a$ there exists $\cT\in \bT_a$ which is $C_0$-adapted to $\cT$.
\item If $d=2$, then for any $H \in \bH_g$ there exists $\cT\in \bT_g$ which is $C_0$-adapted to $\cT$.\end{enumerate}
\end{prop}

Point {\it i)} is established in the \S\ref{secMeshGenI}, point {\it iii)} in \S \ref{secMeshGenG} an eventually {\it ii)} in \S \ref{secMeshGenA}.\\

\subsection{Isotropic Mesh generation}
\label{secMeshGenI}

\begin{figure}
\centering
\includegraphics[width = 5cm, height = 5cm]{\pathPic/Dessins/Jenny/THalfSquareJenny.pdf}
\caption{A bidimensional triangulation generated by the isotropic refinement procedure
\label{figHalfSquares}}
\end{figure}

The survey paper \cite{Nochetto} describes a the construction of a hierarchical family of meshes of the rectangular domain 
$
[0,1]^d.
$ 
All these meshes are the refinement of a ``fundamental'' mesh $\cT_0 = \{T_\sigma \sep \sigma \in \Sigma_d\}$, where $\Sigma_d$ stands for the collection of permutations of the set $\{1,\cdots,d\}$, and $T_\sigma$ for the Kuhn simplex
$$
T_\sigma := \{z\in [0,1]^d \sep z_{\sigma(1)} \leq \cdots \leq z_{\sigma(d)}\}.
$$
%A sequence $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $A procedure, guided by the user 
%The ``fundamentalbasic mesh $\cT_0$ of $[0,1]^d$ 
Starting from $\cT_0$, the algorithm described in \cite{Nochetto} produces, guided by the user, a family $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $[0,1]^d$ proceeding as follows. 
Assume that the mesh $\cT_n$ has already been generated.
%Once the mesh $\cT_n$ is defined, the mesh $\cT_{n+1}$ is obtained as follows.
%\begin{enumerate}
%\item (Marking) The user selects
%\item (Refinement)
%\end{enumerate}
%The mesh $\cT_{n+1}$ is produced from $\cT_n$ as follows 
\begin{itemize}
\item (Marking)
The user selects a subset $\cM_n \subset \cT_n$.
\item (Refinement)
The algorithm generates a $2$-refinement $\cT_{n+1}$ of $\cT_n$,  
$$
\cT_{n+1} := \Refine(\cT_n, \cM_n).
$$
which does not contain any of the marked simplices : $\cT_{n+1} \cap \cM_n = \emptyset.$
\end{itemize}
\noindent

The elements of the meshes $(\cT_n)_{n \geq 0}$ have a very specific structure, which main features are described below.
\begin{property}
\label{propertyIso}
Any simplex $T$ produced by this algorithm possesses the following properties.
\begin{enumerate}[a)]
\item (Discrete Volumes) The volume of $T$ has the form
\be
\label{eqVolTG}
|T| = \frac {2^{-g(T)}}{d!},
\ee
where $g(T)\geq 0$ is an integer called the ``generation'' of $T$.
\item
(Finite number of classes)
The simplex 
$$
2^{\frac{g(T)} d} (T-z_T),
$$
which is centered at the origin and has volume $1/d!$, %$\frac 1 {d!}$, 
belongs to a finite family $\gT_0$ of simplices.
%\item
%(Vertices lie on a grid)
%The vertices of $T$ lie on the grid
%$$
%2^{-\left\lceil \frac {g(T)} d\right\rceil} \Z^d
%$$
\end{enumerate}
\end{property}
The survey paper \cite{Nochetto} also contains a result, Proposition 4.1, which establishes that $\cT_{n+1} := \Refine(\cT_n, \cM_n)$ is a \emph{local} refinement of $\cT_n$ in the following sense: for all $T'\in \cT_n \sm \cT_{n+1}$ there exists $T\in \cM_n$ such that 
\be
\label{eqDG}
g(T)\geq g(T') \stext{ and } d(T,T') \leq D \, 2^{-g(T')/d},
\ee
where $D = D(d)$ is a fixed constant and where 
$$
d(T,T') := \min\{|z-z'| \sep z\in T, \, z'\in T'\}.\\
$$

The next lemma shows that this refinement algorithm can be used to produce a conforming isotropic mesh $\cT$ of the unit cube $[0,1]^d$, such that the diameters $\diam(T)$, $T\in \cT$, are specified by a given Lipschitz function.

\begin{lemma}
\label{lemmaSCube}
%There exists $C=C(d)$ such that the following holds.
Let $s:[0,1]^d\to  (0,\sqrt d]$ be a $c$-lipschitz function, where $0<c\leq 1$. Let $(\cT_n)_{n \geq 0}$ be the sequence of meshes produced by the algorithm when the collection $\cM_n\subset \cT_n$ of marked simplices is defined as follows
\be
\label{defMn}
\cM_n := \left\{T\in \cT_n \sep \min_T s < \diam(T)\right\}.
\ee
Then the sequence of meshes stabilizes : there exists $N\geq 0$ such that $\cT_n = \cT_N$ for all $n \geq N$. Furthermore we have for all $T\in \cT_N$ and all $z\in T$
\be
\label{eqEquivCube}
\diam(T) \leq s(z) \leq C_s \diam(T).
\ee
where 
\be
\label{defCs}
C_s := 2^\frac 1 d \frac {D_+ (1+c) + c D}{D_-}
\ee
where $D_+ := \max\{ \diam(T) \sep T \in \gT_0\}$ and $D_- := \min\{ \diam(T) \sep T \in \gT_0\}$.
\end{lemma}

\proof
We first show that for any $n \geq 0$ any $T_*\in \cT_n$ and any $z\in T_*$ we have $s(z) \leq C_s \diam(T_*)$.

Indeed if $T_*\in \cT_0$ then 
$$
s(z) \leq \sqrt d =  \diam(T_*) \leq C_s \diam(T_*)
$$
since $C_s\geq 1$ and since $s$ is uniformly bounded by $\sqrt d$.

Otherwise $T_*$ has a father $T'$ which was bisected in the refinement process, hence there exists a simplex $T$ such that \iref{eqDG} holds and which was selected for bisection, hence $\min_T s < \diam(T)$.

We thus obtain for any $z\in T$
\begin{eqnarray*}
s(z) &\leq& \min_T s+ c(\diam(T') + d(T,T'))\\
& \leq & \diam(T)+c(\diam(T') + d(T,T'))\\
& \leq & D_+ 2^{-g(T)/d} + c(D_+2^{-g(T')/d} + D 2^{-g(T')/d})\\
& \leq &  2^{-(g(T_*)-1)} (D_+(1+c)+cD)\\
& \leq & C_s \diam(T_*),
\end{eqnarray*}
which concludes the proof of the right part of \iref{eqEquivCube}.

From the fourth line of this inequality we also obtain an uniform lower bound on the volume of the simplices generated by the refinement procedure
$$
|T_*| = \frac{2^{-g(T_*)}}{d!} \geq c_0 := \frac{\min\{ s(z) \sep z\in [0,1]^d\}}{d! 2^\frac 1 d  (D_+(1+c)+cD)}.
$$
It follows that $\#(\cT_n)$ is uniformly bounded by $1/c_0$, which immediately implies that the sequence $(\cT_n)_{n \geq 0}$ of meshes stabilizes.

Let $N$ be such that $\cT_n = \cT_N$ for all $n \geq N$. We thus have $\cM_N = \emptyset$ and therefore $\diam(T) \leq \min_T s$ for all $T\in \cT_N$, which implies the left part of \iref{eqEquivCube}.
\sq

The rest of this section is devoted to the proof the point i) of Proposition \ref{propMeshGen}.
We thus consider a metric $H\in \bH_i$, and we recall there exists a Lipschitz function $s: \R^d \to \R_+^*$ such that for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2}.
$$
For each $n\geq 0$ we define a function $s_n : [0,1]^d \to \R_+^*$, which is clearly Lipschitz, as follows
\be
\label{defSn}
s_n(z) := 2^{-n} s(2^n (z-z_0))
\ee
where $z_0 = (1/2, \cdots , 1/2)$ is the barycenter of the cube $[0,1]^d$.
%The function $s_n$ is clearly Lipschitz, and 
For all $z\in [0,1]^d$ and all $n \geq 0$ we have 
$$
s_n(z) \leq s_n(z_0) + |z-z_0| \leq 2^{-n} s(0) + \frac {\sqrt d} 2.
$$
The function $s_n$ is therefore uniformly bounded by $\sqrt d$ on $[0,1]^d$ when $n$ is sufficiently large.
We denote by $\cT^n$ the mesh of the cube $[0,1]^d$ described by Lemma \ref{lemmaSCube} for the function $s_n$. We thus have %for all $T\in \cT^n$
\be
\label{eqDiamSn}
\diam(T) \leq s_n(z) \leq C \diam(T) \stext{ for all } T \in \cT^n, \, z\in T.
\ee
where $C=C(d)$ is the constant from Lemma \ref{lemmaSCube}.
We denote by $\cT_n$ the mesh of the cube $[-2^{n-1}, 2^{n-1}]^d$ obtained by translating the mesh $\cT^n$ by $-z_0$ and dilating it by $2^n$. In mathematical terms: % In condensed notations
$$
\cT_n := \{2^n(T-z_0)\sep T \in \cT^n\}.
$$
%$$
%\cT_n := 2^n (\cT^n -z_0).
%$$
In view of \iref{defSn} and \iref{eqDiamSn} we thus have 
\be
\label{eqMinSDiamT}
\diam(T) \leq s(z) \leq C \diam(T) \stext{ for all } T \in \cT_n,\, z\in T,
\ee
We denote by $C_0$ the smallest constant such that for all $T$ in the finite set $\gT_0$ one has 
$$
 \frac{C_0^{-2} \Id}{\diam(T)^2} \leq \cH_T \leq \frac{C_0^2\Id}{C^2\diam(T)^2 },
$$
and we thus obtain for all $T\in \cT_n$ and all $z\in T$
\be
\label{eqHHTIso}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Unfortunately the mesh $\cT_n$ does not cover $\R^d$ but only the cube $[-2^{n-1}, 2^{n-1}]$. 
The next lemma shows that a global mesh $\cT$ of the infinite domain $\R^d$ can be extracted from the sequence of meshes $(\cT_n)_{n\geq 0}$.

\begin{lemma}
\label{lemmaExtractMesh}
Let $(\Omega_n)_{n \geq 0}$ be an increasing sequence of polygonal domains of $\R^d$, which exhausts $\R^d$ in the following sense:
$$
\bigcup_{n \geq 0} \Omega_n = \R^d \stext{ and } \Omega_n \subset \Omega_{n+1} \text{ for all } n\geq 0.
$$
Let $H \in \bH_g$, let $(\cT_n)_{n \geq 0}$ be a sequence of conforming simplicial meshes of the domains $\Omega_n$, and assume that for all $n \geq 0$, all $T\in \cT_n$ and all $z\in T$ one has 
\be
\label{eqHHTConv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Then there exists a mesh $\cT\in \bT$ such that 
$
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
$
for all $T\in \cT$ and all $z\in T$.
\end{lemma}

\proof
The heuristic idea of this proof is to ``extract a converging subsequence'' from the sequence $(\cT_n)_{n \geq 0}$ of meshes. Unfortunately meshes are discrete objects of combinatorial nature, and the convergence of meshes has no meaning a priori. We therefore use Lipschitz functions as an intermediate object, for which convergence is well defined and which benefit of a compactness property.\\

We associate a function $\phi_T : \R^d \to \R$ to each simplex $T$, which is defined as follows. The function $\phi_T$ is supported on $T$, and for all $z\in T$ we have in terms of the barycentric coordinates $\lambda_v(z)$ of $z$ with respect to the vertices $v\in V$ of $T$:
%To each simplex $T$ of vertices $V$, and barycentric coordinates $(\lambda_v)_{v\in V}$ we associate the function 
$$
\phi_T(z) := \min_{v\in V} \lambda_v(z).
$$
%The maximum of this function has value $1/d$ and is attained at the barycenter $z_T$ of $T$. Furthermore for each $z\in T$ and each $0\leq r \leq 1$ one easily checks that 
%$$
%\phi_T(z+r(z-z_T)) \geq r/d.
%$$
According to Lemma \ref{lemmaNormLambda}, we have for any $z,z'\in T$ and any $v\in V$
$$
|\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T},
$$
hence 
\be
\label{eqPhiLip}
|\phi_T(z) - \phi_T(z')| \leq \max_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T}.
\ee

For all $n \geq 0$ we define a function $\phi_n$ on $\R^d$ as follows
$$
\phi_n := \sum_{T \in \cT_n} \phi_T.
$$
It follows from \iref{eqHHTConv} and \iref{eqPhiLip} that for all $T\in \cT_n$ and all $z\in \interior(T)$
$$
\dil_z(\phi_n\sep d_H) \leq C_0.
$$
Since in addition $\phi_n = 0$ on $\R^d \sm \Omega_n$ it follows from corollary \ref{corolLipNoGamma} that $\phi_n : (\R^d,d_H) \to \R$ is $C_0$-Lipschitz. Since the space $(\R^d, d_H)$ is locally compact, due to Proposition \ref{propEuclidRiemann}, Ascoli's compactness theorem states that there exists 
subsequence $(\phi_{n_k})_{k \geq 0}$ which converges uniformly on all compact sets of $\R^d$ to a $C_0$-Lipschitz function $\phi$. 

We therefore assume, up to such an extraction, that 
$
\phi_n \to \phi
$
uniformly on all compact sets of $\R^d$.
We denote by $\cT$ the collection of closures of connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$:
$$
\cT := \left\{ \overline E \sep E \text{ is a connected component of } \{z\in \R^d \sep \phi(z)>0\} \right\}.
$$
For each $z\in \R^d$ and each $n \geq 0$, we denote by $T_n(z)$ the element of $\cT_n$ containing $z$ in its interior if it exists, and $T_n(z) = \emptyset$ otherwise.
If $\phi(z)>0$, then $T_n(z)\neq \emptyset$ for all $n$ sufficiently large, and one easily checks that 
\be
\label{eqTTnz}
T_n(z)\text{ converges in Hausdorff distance to the element }T(z)\in \cT
\ee
 containing $z$. Hence $\cT$ is a collection of simplices, and the convergence $T_n(z)\to T(z)$ in haussdorf distance, combined with the hypothesis $C_0^{-2} H(z) \leq T_n(z) \leq C_0^2 H(z)$, implies that  
\be
\label{eqHHTConv2}
C_0^{-2} H(z) \leq T(z) \leq C_0^2 H(z).
\ee
In order to conclude this proof we need to show that the collection $\cT$ of simplices is a conforming mesh of $\R^d$. We thus have to check the hypotheses of Definition \ref{defSimplMesh}.
The interiors $\interior(T)$, $T\in \cT$ are pairwise disjoint since they are the connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$.
We claim furthermore that $\cT$ covers $\R^d$. Indeed let $z\in \R^d$be arbitrary and for all $n$ let $T_n\in \cT_n$ be such that $z\in T_n$. Since $C_0^{-2} H(z) \leq \cH_{T_n}\leq C_0^2 H(z)$ there exists a subsequence $T_{n_k}$ which converges in the Haussdorf distance to a simplex $T$ containing $z$. We clearly have $T\in \cT$ which establishes as announced that $\cT$ covers $\R^d$.
The fact that $\cT$ is locally finite easily follows from \iref{eqHHTConv2}.\\


We now turn to the proof of the conformity property, and for that purpose we consider an arbitrary Lipschitz function $f : (\R^d, d_H) \to \R$ with compact support. 
Let $T$ be a simplex such that $C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)$. We have for any vertex $v$ of $T$
$$
|f(v) - f(z_T)| \leq d_H(z_T,v) \leq C_0 \|z_T - v\|_{\cH_T} = C_0.
$$
Denoting by $V$ the collection of vertices of $T$ we thus obtain for any $z,z'\in T$
$$
\interp_T f(z) - \interp_T f(z') = \sum_{v\in V} (\lambda_v(z) - \lambda_v(z')) (f(v) - f(z_T)).
$$
Where $\interp_T$ denotes the $\P_1$ (piecewise affine) interpolation on a simplex $T$, and $\interp_\cT$ the $\P_1$ interpolation on a mesh $\cT$.
hence using Lemma \ref{lemmaNormLambda}
\begin{eqnarray*}
|\interp_T f(z) - \interp_T f(z')| &\leq& C_0 \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|\\
 &\leq& C_0 \sqrt{(d+1)  \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|^2} \\
 &=& C_0 \sqrt d \|z-z'\|_{\cH_T}.
\end{eqnarray*}
The last inequality implies that 
$$
\dil_z(\interp_{\cT_n} f \sep d_H)\leq C_0^2 \sqrt d
$$
for all $T\in \cT_n$ and $z\in \interior(T)$.
Let $n_0 \geq 0$ be such that $\supp(f)\subset \Omega_{n_0}$, which implies that $\interp_{\cT_n} f$ is continuous. It follows from Corollary \ref{corolLipNoGamma} that $\interp_{\cT_n} f : (\R^d, d_H) \to \R$ is $C_0^2\sqrt d$-Lipschitz.

We define 
$
D := \cup_{T \in \cT} \interior(T),
$
and we denote by $\interp_T f : D \to \R$ the function which coincides with $\interp_T f$ on the \emph{interior} of each $T\in \cT$. % (and which is possibly discontinuous at the interfaces between the simplices $T\in \cT$). 
For any $z\in D$ we obtain using \iref{eqTTnz} that $\interp_{\cT_n} f(z) \to \interp_\cT f(z)$, hence for any $z,z'\in D$
$$
|\interp_\cT f(z) - \interp_\cT f(z')| = \lim_{n \to \infty} |\interp_{\cT_n} f(z)-\interp_{\cT_n} f(z')| \leq \sqrt d C_0^2 \, d_H(z,z').
$$
The piecewise interpolant $\interp_T f : D \to \R$ therefore extends to a $\sqrt d C_0^2$-Lipschitz function $\interp_T f : (\R^d, d_H) \to \R$. It easily follows that $\interp_\cT f$ is continuous for any compactly supported $C^1$ function $f$. This property characterizes conforming meshes, hence $\cT\in \bT$ which concludes the proof.
\sq



\begin{corollary}(Bidimensional triangulations)
\label{corolBidimIso}
Assume that the dimension is $d=2$. There exists $c>0$ such that the following holds: if $s: \R^2 \to \R_+^*$ is $c$-Lipschitz, then there exist a mesh $\cT$ of $\R^2$ built of half squares, and such that for all $T\in \cT$ and $z\in T$
\be
\label{eqDT32}
\diam(T) \leq s(z) \leq 3 \diam(T)/2.
\ee
\end{corollary}

\proof
When the dimension is $d=2$, the collection $\gT_0$ of triangles contains only half squares, of area $1/2$, hence  $D_+ = D_- = \sqrt 2$. 

As $s \to 0$ the constant $C_s$ defined by \iref{defCs} tends to $\sqrt 2$. Hence $C_s\leq 3/2$ when $s$ is sufficiently small.
If $s$ is bounded by $\sqrt 2$ on $[0,1]^2$ one may therefore produce a mesh $\cT_*$ of $[0,1]^2$ such that \iref{eqDT32} holds for all $T\in \cT_*$, $z\in T$.

From this point construct as before a sequence of meshes $\cT_n$ of the squares $[-2^{n-1}, 2^{n-1}]$ which satisfies \iref{eqDT32}, and we extract a global mesh $\cT$ of $\R^2$ using Lemma \ref{lemmaExtractMesh}. The triangles $T\in \cT$ still satisfy the inequality \iref{eqDT32} since they are limits in the Haussdorff distance of triangles from the triangulations $\cT_n$.
\sq


\subsection{Graded mesh generation}
\label{secMeshGenG}

We prove in this section a result of bi-dimensional mesh generation, Theorem \ref{thEquiMesh}, which implies Point (iii) of Proposition \ref{propMeshGen}. The key ingredients of this section come from the paper \cite{Shew}.
We assume throughout this section that the dimension is $d=2$.

For that purpose we introduce the notion of equispaced points in an abstract metric space.
 Let $(X,d_X)$ be a metric space and let $\delta>0$, we say that a subset $\cV \subset X$ is $\delta$-equispaced if the following holds.
\begin{enumerate}[a)]
\item (Covering) The distance from an arbitrary point $x\in X$ to $\cV$ is bounded by $1$ : for all $x\in X$
\be
\label{eqCover}
d_X(x, \cV) := \inf\{d_X(x,v) \sep v \in \cV\} \leq 1.
\ee
\item (Separation) The pairwise distances between the points of $\cV$ are larger than $\delta$ : for all $v, v'\in \cV$ such that $v \neq v'$
\be
\label{eqSep}
d_X(v,v') \geq \delta.
\ee
\end{enumerate}

The next lemma establishes the existence of such a set under certain assumptions. \begin{lemma}
\label{lemmaEquiSpaced}
Let $(X,d_X)$ be a metric space in which the closed balls $B'(x,r) := \{y\in X \sep d_X(x,y) \leq r\}$ are compact for all $x\in X$ and $r\geq 0$. 
Let $\cV_0$ subset $X$ be such that $d_X(v,v') \geq 1$ for all $v,v'\in \cV_0$ such that $v\neq v'$. Then there exists a $1$-equispaced set $\cV$ of the metric space $(X,d_X)$, containing $\cV_0$.
\end{lemma}

\proof
We may assume that $\cV_0 \neq \emptyset$, up to including an arbitrary point of $X$, and we choose an  arbitrary  $x_0\in \cV_0$.
We define inductively a sequence $(x_n)_{0 \leq n< N}$ of points and $(\cV_n)_{0 \leq n < N}$ of subsets of $X$, where $N\in \N \cup \{\infty\}$ is specified later, proceeding as follows.
Assuming that $\cV_n$ is already defined we consider the closer set 
\be
\label{eqDefXn}
X_n :=  
\{x\in X \sep d_X(x,\cV_n) \geq 1\}.
\ee
If the set $X_n$ is empty, then the sequence ends and we define $N := n+1$. Otherwise we choose $x_{n+1}$ arbitrarily among the minimisers of $d_X(x,x_0)$ on $X^n$:
\be
\label{defxn}
x_{n+1} \in \underset {x\in X_n} \argmin \,d_X(x,x_0),
\ee
and we define $\cV_{n+1} := \cV_n \cup\{x_{n+1}\}$.
Such a minimizer exists since $X_n$ is closed and since the closed balls in $X$ are compact.
%$$
%X^n \cap \overline B\left(x_0, \ 1+ \inf_{x\in X^n} d_X(x_0, x)\right)
%$$
%is compact.
We define $N := \infty$ none of the sets $(X_n)_{n \geq 0}$ is empty. %if the sequence $(x_n)$ is infinite.

We define $\cV := \cup_{0 \leq n <N} \cV_n$.
%We denote by $X_0 := \{x_n \sep 0\leq n<N\}$ the collection of all points of this finite or countable sequence.
%
%We define $N := \infty$ if the sequence $x_0, x_1, \cdots$ is infinite, and we denote by $X_0$ the collection of all points of this finite or countable sequence,
%$$
%X_0 := \{x_n \sep 0 \leq n < N\}.
%$$ 
%%as the collection of all points $x_0, x_1, \cdots$ of this finite or countable sequence.
%, which clearly is finite or countable.
By construction, we thus have $d_X(v, v') \geq 1$ for all $v,v'\in \cV$
which establishes the separation property \iref{eqSep}. %, and shows that $\cV$ is a discrete set.

We now assume for contradiction that the covering property \iref{eqCover} does not hold which implies that $N= \infty$. We choose a point $x_*\in X$ such that $d_X(x_*, \cV)>1$, and therefore $x_*\in X_n$ for all $n \geq 0$. The definition \iref{defxn} of $x_{n+1}$ implies that $d_X(x_0, x_n) \leq d_X(x_0, x_*)$ for all $n \geq 0$, hence the discrete collection of points
$
\{x_n \sep n \geq 0\}
$
in included in the closed ball $\{x\in X \sep d_X(x_0, x) \leq d_X(x_0, x_*)\}$ which is compact.
The sequence $(x_n)_{n \geq 0}$ therefore admits a converging subsequence, but this contradict the fact that the pairwise distances between these points are larger than $1$, which concludes the proof of this proposition.
\sq


%The next lemma gives a simple (from a theoretical point of view) procedure which produces a point set equidistributed with respect to a metric.
%\begin{lemma}
%Let $H\in \bH$ and let $(p_n)_{n\geq 0}$ be a sequence of points obtained by choosing $p_0 = 0$ and then iteratively choosing $p_{n+1}$ among the minimizers of
%\be
%\label{defpn}
%\min\{\|p\| \sep d_H(p, \{p_0,\cdots , p_n\} \geq 1)
%\ee
%
%Then the point set $\cP := \{p_n \sep n \geq 0\}$ is $1$-equidistributed with respect to $H$.
%\end{lemma}
%
%\proof
%The separation holds by construction. It implies in particular that for any $M \geq 1$, $\cP\cap B(0,M)$ is finite. 
%
%%Since $H$ is continuous and positive definite, for each $M$ the set $\{n\geq 0 \sep \|p_n\| \leq M\}$ is finite.
%Indeed let $\Lambda^2 := \max \{\|H(z)\| \sep \|z\| \leq M\}$.
%The balls $B(p, \Lambda/2)$, $p\in \cP\cap B(M)$ are pairwise disjoint. It follows from a volume argument that $\cP\cap B(M)$ is finite.
%
%Let us assume by contradiction that there exists $z\in \R^2$ such that $d(z, \cP)>1$. Then for $n$ large enough we have $\|z\| < \| p_{n+1}\|$ which is incompatible with the construction of $p_{n+1}$ as a minimizer of \iref{defpn}.
%\sq




We consider a fixed metric $H \in \bH$. For any $x,y\in \R^2$ we define 
$$
d_x(y) := \|x-y\|_{H(x)}.
$$
We also consider a fixed discrete collection of vertices, or ``sites'', $\cV \subset \R^2$, and we define the anisotropic Voronoi cell of a site $v\in V$ as follows 
\be
\label{defVorv}
\Vor(v) := \{z\in \R^2 \sep d_v(z) \leq d_w(z) \text{ for all } w \in V\}.
\ee
The anisotropic Voronoi cell $\Vor(v)$ is thus the collection of points $z$ which are \emph{closer to the vertex $v$ than to any other site}.
The classical (isotropic) Voronoi is obtained by choosing $H = \Id$.
We refer to the paper \cite{Shew} Figure 3 for an illustration of the anisotropic Voronoi diagram $\{\Vor(v) \sep v\in \cV\}$ associated to a point set.

For each $z\in \R^2$ we define $\cV_z$ the collection of vertices which contain $z$ in their Voronoi region:
$$
\cV_z := \{v \in \cV \sep z \in \Vor(v)\}.
$$
The geometric dual of the Voronoi diagram is the graph $\cG(\cV,H)$ defined as follows:
\be
\label{defGVH}
\cG(\cV,H) := \{[v,v'] \sep \text{there exists } z\in \R^2 \text{ such that } V_z = \{v,v'\}\}.
\ee

%We define a collection $\cT_0(V,H)$ of convex sets attached to the metric $H$ and to the collection $V$ of sites
%$$
%\cT_0(V,H) := \{\Cvx(V_z) \sep z \in \R^2 \text{ and } \#(V_z) \geq 3\}.
%$$
The next theorem establishes that $\cG(\cV,H)$ is, under certain conditions on the metric $H$ and the set $\cV$, the graph of a triangulation adapted to $H$.

\begin{theorem}
\label{thEquiMesh}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta)\geq 1$ such that the following holds.
Let $H$ be a metric such that $c^2 H\in \bH_g$, and let $\cV$ be a $\delta$-equispaced subset of $(\R^2, d_H)$.
Then the $\cG(\cV,H)$ is a planar graph which defines a partition of $\R^2$ into strictly convex polygons. Arbitrarily triangulating each polygon yields a triangulation $\cT$ which is $C$-adapted to $H$, called an anisotropic Delaunay triangulation. Furthermore if $\cV$ is in general position then $\cG(\cV,H)$ is already the graph of a triangulation.
\end{theorem}

This theorem implies point iii) of Proposition \ref{propMeshGen}, proceeding as follows: 
for any $H_0 \in \bH_g$, we construct using lemma \ref{lemmaEquiSpaced} a subset $\cV$ of the metric space $(\R^2, d_{H_0}/c(1))$ which is $1$-equispaced. According to Theorem \ref{thEquiMesh} there exists a triangulation $\cT$, of vertices $\cV$, which is $C(1)$-adapted to the metric $H := H_0/c(1)^2$, and therefore $C(1)/c(1)$-adapted to $H_0$.\\


We now turn to the proof of Theorem \ref{thEquiMesh}, which is based on three theorems presented in \cite{Shew}. 
%These theorems are based on a property that needs to be 
For that purpose we recall some definitions of this paper. %introduce the following definitions.
\begin{definition}
\label{defWedge}
%The wedge of $v,v'$ is 
\begin{itemize}
\item (Wedge of two points)
We define the wedge $\wed(v,w)$ of two distinct sites $v,w\in V$ as follows
$$
\wed(v,w) := \{z\in \R^2 \sep (z-v)^\trans H(v) (w-v) >0 \text{ and } (z-w)^\trans H(w) (v-w) >0\}
$$ 
\item (Wedge property)
We say that the Voronoi diagram of $V$ is wedged if for any two distinct $v,w \in V$ we have 
$$
\Vor(v) \cap \Vor(w) \subset \wed(v,w).
$$
\end{itemize}
\end{definition}

The wedge property expresses that the collection $\Vor(v) \cap \Vor(w)$ of points $q$ shared by the Voronoi regions of the sites $v$ and $w$ lie in a cone defined by two linear inequalities.
We refer to \cite{Shew} Figure 4 for an illustration of the wedge of two sites.

The next proposition, which is partly is based on Lemma 5 from \cite{Shew},
 shows that the wedge property is automatically satisfied in our context.
For any metric $H$ and any constant $c>0$ such that $c^2H\in \bH_g$, it easily follows from Proposition \ref{propEuclidRiemann} that for all $x,y\in \R^2$
\be
\label{eqDHLog}
\ln (1+ c\, d_x(y)) \leq c \, d_H(x,y) \leq - \ln(1- c\, d_x(y)), 
\ee
which is equivalent to 
\be
\label{eqDHExp}
1-\exp(-c\, d_H(x,y)) \leq c \, d_x(y) \leq \exp(c \, d_H(x,y))-1.
\ee

\begin{lemma}
\label{lemmaDiamVor}
If $c^2 H\in \bH_g$ %and $\cV$ is $\delta$-equispaced, 
then
for any $v\in \cV$ and any $q\in \Vor(v)$ we have 
\be
\label{eqDiamVor}
\|q-v\|_{H(v)} \leq r_0(c) := (e^c-1)/c.
\ee
If $v,w \in \cV$ satisfy $\Vor(v) \cap \Vor(w) \neq \emptyset$, then 
\be
\label{eqVordvw}
%\delta \leq 
d_H(v,w) \leq r_1(c) := -2\ln(2-e^c)/c.
\ee
Note that $r_0(c) \to 1$ and $r_1(c) \to 2$ as $c\to 0$. Note also that $d_H(v,w)\geq \delta$ if $\cV$ is $\delta$-equispaced.
\end{lemma}

\proof
For any $q\in \cV$ there exists $v_* \in \cV$ such that 
$
d_H(q,v_*) \leq 1,
$
and therefore 
$$
\|q-v_*\|_{H(v_*)} \leq r_0(c) := (e^c-1)/c,
$$
which implies \iref{eqDiamVor} using the definition \iref{defVorv} of the Voronoi diagram.
We thus turn to the proof of \iref{eqVordvw} and for that purpose we consider a point $q\in \Vor (v)\cap\Vor(w)$. We thus have
$
\max\{\|q-v\|_{H(v)} , \|q-w\|_{H(w)} \}\leq  v_c%-\ln(1-c v_c)/c
$
hence
$$
d_H(v,w) \leq r_1(c) :=-2\ln(1-c r_0(c))/c,
$$
which concludes the proof.
\sq

\begin{prop}
\label{propWedge}
For each $\delta$ there exists $c=c(\delta)>0$ such that the following holds.\\
If a metric $H$ satisfies $c^2H\in \bH_g$ and if $\cV$ is a $\delta$-equispaced subset of $(\R^2,d_H)$, then the wedge property is satisfied.
\end{prop}

\proof
We assume for contradiction that there exists two distinct vertices $v,w \in V$, and a point $q\in \Vor(V) \cap \Vor(W)$ such that $z\notin \wed(v,w)$. We may assume, up to exchanging the roles of $v$ and $w$, that 
$$
(q-w)^\trans H(w) (v-w) \leq 0.
$$
Defining the ``relative distortion''
$
\tau := \exp d_\times (H(v), H(w))
$
we obtain using Lemma 5 from \cite{Shew} %(*$q$ instead of $z$??*)
\be
\label{eqShewWedge}
 d_w(v) \leq d_w(q) \sqrt{\tau^2-1}.
\ee
We now estimate the quantities $d_w(v)$, $d_w(q)$ and $\tau$ appearing in this estimate, in order to obtain a contradiction when $c$ is sufficiently small.

%Since the set $V$ is $C_0$-equispaced, there exists $u\in V$ such that $d_H(u,q) \leq C_0$. Recalling that $z\in \Vor(v)\cap \Vor(w)$ we thus obtain using \iref{eqDHExp}
%\be
%\label{eqDiamVor}
%d_v(q) = d_w(q) \leq d_u(q) \leq \frac{\exp(c \, d_H(u,q))-1} c \leq r_0(c) := \frac{\exp(c C_0)-1} c,
%\ee
%and therefore using \iref{eqDHLog} 
%\be
%\label{eqVordvw}
%d_H(v,w) \leq d_H(v,q)+ d_H(q,w) \leq r_1(c) := \frac {-2\ln (1- c r_0(c))}  c,% \frac 1 {1-f(c)}.
%\ee
%hence 
We have 
\be
\label{eqTauWedge}
\ln \tau = d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
\ee
Since $\cV$ is $\delta$-equispaced we have 
$
d_H(v,w) \geq \delta
$
and therefore 
\be
\label{eqdvwWedge}
c \,d_w(v) \geq 1-\exp(-c d_H(v,w)) \geq 1-\exp(-c\delta)
\ee
Injecting \iref{eqDiamVor}, \iref{eqTauWedge} and \iref{eqdvwWedge} in \iref{eqShewWedge} we obtain
\be
\label{eqFinalWedge}
\frac{1-\exp(-c\delta )} c \leq \frac{\exp(c)-1} c \sqrt{\exp(2c r_1(c))-1}.
\ee
The left hand side tends to $\delta$ as $c\to 0$, while the right hand side tends to $0$. We thus obtain a contradiction when $c$ is sufficiently small which concludes the proof of this proposition.
\sq

\begin{theorem}[Dual triangulation theorem. Labelle, Shewchuck, \cite{Shew}]
\label{thShew}
If the Voronoi diagram of the point set $\cV \subset \R^2$ is wedged, then the geometric dual of this diagram is a polygonalization of $\R^2$ with strictly convex polygons and is a triangulation $\cT$ if $\cV$ is in general position.
\end{theorem}

Under the hypotheses of this theorem the vertices $v_1, \cdots, v_k$ of a polygon in the dual Voronoi diagram satisfy by construction $\Vor(v_1)\cap \cdots \cap \Vor(v_k) \neq \emptyset$, and therefore the vertices $v_1, v_2, v_3$ of a triangle $T\in \cT$ satisfy $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$.

The next theorem, originally stated in \cite{Shew} as Corollary 10 to Theorem 9 of the same paper, allows to control the angles of a triangle in the anisotropic Delaunay triangulation.

\begin{theorem}[Labelle, Shewchuk, \cite{Shew}]
\label{thAngle}
Let $v_1,v_2,v_3\in \cV$ and let $q\in \Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)$. Let 
$$
r = d_{v_1}(q) = d_{v_2}(q) = d_{v_3}(q) \stext{ and }
l = \min\{d_{v_i}(v_j) \sep i,j \in \{1,2,3\}, i \neq j\}.
$$ 
Define $\beta := \max\{r/l,\, 1/\sqrt 2\}$, %and %$\gamma\in [1,\infty)$ by 
%Let $1\leq \gamma \leq \sqrt 2$ and $\beta \geq \frac 1 {\sqrt 2}$ satisfy
$$
\gamma := \exp \max \{d_\times (H(v_i), H(v_j)) \sep i,j \in \{1,2,3\}, i \neq j\},
$$
and
\be
\label{defChi}
\chi := \frac 1 {2 \beta} - \frac{(\gamma^2-1)\beta} 2.
\ee
If $\gamma \leq \sqrt 2$ and $\chi>0$ then any angle $\theta$ of the triangle of vertices $(\sqrt{H(v_1)} v_k)_{1 \leq k \leq 3}$ satisfies
$$
\arcsin ( \chi/ \gamma^2) \leq \theta \leq 2 \arccos(\chi/\gamma^2).
$$
%where $S = H(v_1)^{\frac 1 2}$.
\end{theorem}

\begin{corollary}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta) \geq 1$ such that the following holds.
If $\cV$ is $\delta$-equispaced, if $c^2H\in \bH_g$ and if $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$, then denoting by $T$ the triangle of vertices $v_1,v_2,v_3$ we have for all $z\in T$
$$
C^{-2} H(z) \leq \cH(z) \leq C^2 H(z).
$$
\end{corollary}
\proof
We use \iref{eqDHExp} and \iref{eqDHLog} and the fact that $V$ is $\delta$-equispaced to obtain explicit bounds on the quantities $r$, $l$, $\beta$, $\gamma$ and $\chi$ appearing in Theorem \ref{thAngle}.
It follows from Lemma \ref{lemmaDiamVor} that 
$$
r\leq r_0(c) \stext{ and } \delta \leq d_H(v_i,v_j) \leq r_1(c).
$$
Therefore 
$$
l := \min_{i\neq j} d_{v_i}(v_j)\geq %\min_{i\neq j} \frac{1-\exp(-c d_H(v_i,v_j))} c \geq  
r_2(c) := (1-\exp(-c\delta))/ c,
$$
and 
$$
L := \max_{i\neq j} d_{v_i}(v_j) \leq (\exp(c r_1(c))-1)/c
$$
and 
$$
\gamma \leq \max_{i\neq j} \exp(c \,d_H(v_i,v_j)) \leq \exp(c \,r_1(c)).
$$
In particular 
$
\beta \leq r_3(c) := \min\{r_0(c)/r_2(c),\, 1/\sqrt 2\}. % = \frac{\exp(cC_0)-1}{1-\exp(-2 cC_0^{-1})},
$
Injecting this into \iref{defChi} yields an explicit lower estimate 
$$
\chi\geq r_4(c) := \frac 1 {2r_3(c)} - \frac{ (\exp(2cr_1(c))-1) r_3(c)} 2,
$$ 
and $\chi/\gamma^2\geq r_5(c) := r_4(c) \exp(-2cr_1(c))$.

For a fixed $\delta$ we obtain as $c\to 0$ the limits $r_0(c) \to 1$, $r_1(c)\to 2 $, $r_2(c) \to \delta$, $r_3(c) \to \min\{\delta, 1/\sqrt 2\}$ and $r_4(c) \to 1/(2\min\{\delta, 1/\sqrt 2\})$ and $r_5(c)$ as the same limit.

%We assume without loss of generality that $\delta \geq 1/\sqrt 2$ and we thus obtain $r_3(c) \to \delta$, 
%$r_4(c) \to 1/C_0^2$ and $r_5(c) \to 1/C_0^2$. 
We may therefore choose $c$ sufficiently small in such way that 
$$
l \geq l_0 := \delta/2, \ L  \leq L_0 := 4 \text{ and }\chi/\gamma^2 \geq \Chi_0 := 1/(4\min\{\delta, 1/\sqrt 2\}).
$$
We denote by $T$ the triangle of vertices $v_1, v_2, v_3$. The length of any edge of $T' := \sqrt{H(v_1)}(T)$ is bounded above by $L_0$ and below by $l_0$ respectively, and the angles of $T'$ satisfy $\arcsin (\Chi_0) \leq \theta \leq 2 \arccos(\Chi_0)$. The collection of triangles centered at the origin which satisfy these inequalities is compact, thus there exists a constant $C_1 = C_1(C_0)$ such that 
$$
C_1^{-2} \Id \leq \cH_{T'} \leq C_1^2 \Id,
$$
hence $C_1^{-2} H(v_1) \leq \cH_{T'} \leq C_1^2 H(v_1)$. For any $z\in T$ we obtain, remarking that $\|z-v_1\|_{\cH_T} \leq 2$ for all $z\in T$ and using \iref{eqLocalNorm}, 
$$
C_1^{-2} (1-2cC_1)^2 H(z) \leq \cH_{T'} \leq C_1^2(1-2cC_1)^{-2} H(z)
$$
which concludes the proof of this proposition, with $C = C_1(1-2cC_1)^{-1}$.
\sq

\subsection{Acute mesh generation}
\label{secMeshGenA}

This section is devoted to the proof of Point ii) of Proposition \ref{propMeshGen}. We thus assume that the dimension is $d=2$. This proof combines the constructions of isotropic and graded meshes presented in \S\ref{secMeshGenI} and \S\ref{secMeshGenI} to produce a quasi-acute mesh. 
The key idea of this proof if that the anisotropic Delaunay triangulation described in the previous subsection contains only \emph{few} strongly obtuse angles if the set $\cV$ of vertices is structured along lines which are \emph{transverse to the direction of anisotropy}, as illustrated on Figure \ref{figAcuteGen}. 

The author is sorry to say that this proof is not yet as polished as the rest of the thesis, due to time constraints.

The arguments below establish that there exists absolute constants $1 \geq c>0$, $C$ such that for each metric $H$ satisfying $c^2 H\in \bH_a$ there exists a mesh $\cT\in \bT_{a,C}$ which is $C$-adapted to $H$. It immediately follows that for each $H'\in \bH_a$ there exists a mesh $\cT\in \bT_{a,C}$ which is $C/c$ adapted to $H'$ (applying the above to $H := H'/c^2$) , which concludes the proof of Proposition \ref{propMeshGen}.

We consider a metric $H$ such that $c^2 H\in \bH_a$, where $c$ is a constant specified later, such that $0<c\leq 1$. The constant $c$ needs to be \emph{sufficiently small} in the following sense :  some of the arguments presented in this proof require that $c\leq c_i$, where $c_0, \cdots c_k$ are a finite number of absolute numerical constants (independent of the quasi-acute metric $H$). We mention these requirements when they appear and we assume that they hold.\\


We define two functions $\lambda, \mu : \R^2 \to \R$ as follows : for all $z\in \R^2$
$$
\lambda(z) := \|H(z)^{-\frac 1 2}\| \stext{ and } \mu(z) = \|H(z)\|^{-\frac 1 2}.
$$
Note that $\lambda(z) \geq \mu(z)$.
The functions $\lambda, \mu$ are $c$-Lipschitz according to Corollary \ref{corolLipNorm} : for all $z,z'\in \R^d$
$$
|\lambda(z)-\lambda(z')| \leq c|z-z'| \text{ and } |\mu(z) - \mu(z') | \leq c|z-z'|.
$$
%We define the metric 
%$$
%H_0:= \|H^{-1}\|^{-1} \Id = \Id/\lambda^2,
%$$
%and observe that $cH_0 \in \bH_i$ since $\lambda$ is $c$-Lipschitz, which implies that $H_0 \in \bH_i$.
%Since $H \in \bH_i$, it follows from Point i) of Proposition \ref{propMeshGen}, that there exists an absolute numerical constant $\delta_0>0$ (independent of $H$) and a mesh $\cT_0 \in \bT$ such that for all $T\in \cT_0$ and all $z\in T$
If $c$ is sufficiently small, then there exists according to Corollary \ref{corolBidimIso} a mesh $\cT_0$ built of half squares (as illustrated on Figure \ref{figHalfSquares}) and such that for all $T\in \cT_0$ and all $z\in T$
\be
\label{ratioDiamLambda}
\frac 2 3  \lambda(z) \leq \diam(T)\leq \lambda(z). 
\ee
%(*this or $1/2$?? what is the simplest?*)
%Furthermore we assume that the triangles $T\in \cT_0$ are half squares, which is the case for the construction of such a triangulation presented in \S \ref{secMeshGenI}. 
We denote by $\cV_0$ the collection of vertices of $\cT_0$.\\

For each $u,u'\in \R^2 \sm\{0\}$ we define the (unoriented) angle
$$
\varangle (u,u') := \arccos \left(\frac{\<u,u'\>}{|u| |u'|}\right) \in [0,\cPi].
$$
For any $u,u'\in\bbS := \{v\in \R^2 \sep |v|=1\}$, the angle $\varangle (u,u')$ coincides with the distance $d_\bbS(u,u')$ used in \S\ref{secEigen}. %Note that the angle coincides with the distance on 
For any triangle $T\in \cT_0$ of vertices $v,w,w'$ we thus have $\varangle(w-v,w'-v) \in \{\cPi/4, \cPi/2\}$. For each $u\in \R^2$ we denote by $u^\perp$ the vector obtained by rotating the vector $u$ by $\cPi/2$ is direct trigonometric sense.\\

We say that two vertices $v,w\in \cV_0$ are neighbors in $\cT_0$ if they belong to a common triangle $T\in \cT_0$.
In that case we have %Let $v,w$ be two vertices of a triangle $T\in \cT_0$, then 
\be
\label{edgeLambda}
\frac{\lambda(z)\sqrt 2}3 \leq \frac{\diam(T)}{\sqrt 2}\leq |v-w| \leq \diam(T)\leq \lambda(z)
\ee
Furthermore for any fixed $v\in \cV_0$ any vertex $w\in \cV_0$ which minimizes $|v-w|$ is clearly a neighbor of $v$ in $\cT_0$. It follows that for any distinct $v,w\in \cV_0$
\be
\label{pairwiseV0}
\lambda(z) \frac {\sqrt 2} 3 \leq |v-w| .
\ee
The diameter of any triangle $T\in \cT_0$ is a power of $\sqrt 2$ by construction. Therefore if two triangles $T,T'\in \cT_0$ share a vertex $v$, then it follows from \iref{ratioDiamLambda} that 
\be
\label{eqDiamRatio}
\diam(T)/\sqrt 2 \leq \diam(T') \leq \sqrt 2 \diam(T),
\ee
hence for any two neighbors $w,w'$ of a vertex $v\in \cV_0$ we have 
\be
\label{eqEdgeRatio}
|v-w|/2 \leq |v-w'| \leq 2|v-w|.
\ee


%\begin{lemma}(useful??)
%\label{lemmaDV0}
%For each $v\in \cV_0$ the union $V_\cT(v)$ of the triangles containing $v$ is convex, and we have 
%\be
%\label{diamCellvT0}
%d_{H_0}(v, \R^2\sm V_\cT(v))\geq \delta_0.
%\ee
%Consequently we have for all $v,w\in \cV_0$ 
%\be
%\label{eqDH0vw}
%\delta_0 \leq d_{H_0}(v,w) .
%\ee
%\end{lemma}
%
%\proof
%Let $w_1,w_2,w_3$ be three consecutive vertices, in trigonometric order, on $\partial V_\cT(v)$. Since $\varangle (w_2-w_1, w_2-v)$ and $\varangle (w_2-w_3, w_2-v)$ both belong to $\in \{\cPi/4, \cPi/2\}$, we obtain that the interior angle of the polygon $V_\cT(v)$ belongs to $\{\cPi/2, 3\cPi/4, \cPi\}$, which implies that this polygon is convex.
%
%We denote by $f$ the piecewise linear function on $\cT_0$ such that $f(v)=1$ and $f(w)=0$ for all other vertices in $\cT_0$. For any triangle $T\in \cT_0$ containing $v$ the gradient of $f$ is constant on $T$, orthogonal to the edge $e$ of $T$ opposite to $v$, and for $z\in \interior(T)$ of modulus 
%$$
%|\nabla f(z)| = \frac 1 {d(v,e)} \leq \frac 2 {\diam(T)} \leq \frac 1 {\delta_0\lambda(z)}.
%$$
%It follows that $\dil_z(f\sep d_{H_0}) \leq 1/\delta_0$ and therefore that $f : (\R^2, d_{H_0}) \to \R$ is $1/\delta_0$-Lipschitz. If $z\in (\R^2 \sm V_\cT(v))$ then $|f(v)-f(z)| = 1 \leq d_{H_0}(v,z)/\delta_0$ which implies the announced result. 
%\sq
For each $z\in \R^2$ we define 
$$
\rho(z) = \lambda(z)/\mu(z) \in [1, \infty).
$$
Since the functions $\lambda$ and $\mu$ are $c$-Lipschitz, and since $\diam(T) \leq \lambda(z)$ for any $T\in \cT_0$,  it follows that for any $T\in \cT_0$ and any $z,z'\in T$
\be
\label{eqLambdaT}
\lambda(z)(1-c) \leq \lambda(z') \leq \lambda(z)(1+c) \stext{ and } \mu(z)-c\lambda(z) \leq \mu(z') \leq \mu(z)+ \lambda(z),%\stext{ for all } T \in \cT_0, \ z,z'\in T
\ee
which implies 
\be
\label{eqrhozzp}
\rho(z') = \frac{\lambda(z')}{\mu(z')} \geq \frac{\lambda(z)(1-c)}{\mu(z)+c \lambda(z)} \geq \frac {1-c}{\rho(z)^{-1}+c}.
\ee
This formula has an immediate corollary.
\begin{corollary}
\label{corolRho23}
If $c$ is sufficiently small, then the following holds. For any $T\in \cT_0$ and any $z,z'\in T$ one has : if $\rho(z) \geq 3$ then $\rho(z') \geq 2$, and if $\rho(z) \geq 4$ then $\rho(z') \geq 3$.
\end{corollary}

%The pairs $(3,2)$ and $(4,3)$ of integers appearing in this corollary can be replaced with $(n+1,n)$ where $n \geq 1$ is arbitrary, but the bound upper bound on $c$ depends on $n$.\\


%, and we observe that
%$$
%H_0(z) \leq H(z) \leq \rho(z)^2 H_0(z).
%$$
For each $z\in \R^2$ such that $\rho(z)>1$ we denote by $\theta(z)\in \bbS := \{u\in \R^2\sep |u| = 1\}$ a unit vector such that
\be
\label{defAngle}
H(z) = \lambda(z)^{-2} \theta(z) \theta(z)^\trans+ \mu(z)^{-2} (\Id-\theta(z) \theta(z)^\trans).
\ee
Note that there exists two, opposite, choices for the vector $\theta(z)$.
Consider a simply connected domain $\Omega\subset \R^2$ such that $\rho(z)>1$ for all $z\in \Omega$. Then there exists a \emph{continuous} map $z\mapsto \theta_*(z)$ satisfying \iref{defAngle}, hence $\theta_*(z) = \pm \theta(z)$ for all $z\in \Omega$. Since $c^2 H\in \bH_a$ we have for all $z\in \Omega$, according to Theorem \ref{th2Spaces}
%For each $z\in \R^2$ such that $\rho(z)$, the angle $z'\to \theta(z')$ can be defined in a neighborhood of $z$ and we have according to Theorem \ref{th2Spaces}, since $c^2H \in \bH_a$
\be
\label{eqDilThetaA}
(\lambda(z)-\mu(z) ) \dil_z(\theta_*) \leq c. %\sep d_\bbS
\ee
For any two vectors $u,u'\in \R^2\sm\{0\}$ we define %the non-oriented, acute, angle
$$
\lhd(u,u') := \min \{\varangle(u,u'),\, \varangle(u,-u')\} = \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
$$
%This quantity is used to measure the angle formed by two vectors with no clear orientation.
Formula \iref{eqDilThetaA} had an immediate corollary.
\begin{corollary}
\label{corolTheta2C}
Let $T\in \cT_0$ be such that $\rho\geq 2$ on $T$. Then for any $z,z'\in T$ and any $\theta(z), \theta(z')\in \bbS$ such that \iref{defAngle} holds, we have 
$$
\lhd(\theta(z), \theta(z')) \leq 2c.
$$ 
\end{corollary}

\proof
Since $T$ is a simply connected domain and $\rho \geq 2$ on $T$, there exists a continuous map $\theta_*\in C^0(T, \bbS)$ satisfying \iref{defAngle} at each point.
We thus have 
$$
\lhd(\theta(z), \theta(z')) = \lhd(\theta_*(z), \theta_*(z')) \leq \varangle(\theta_*(z), \theta_*(z'))  \leq \diam(T) \max_{x\in T} \dil_x(\theta_*),
$$
and for any $x\in T$, since $\rho(x)\geq 2$,
$$
\diam(T)\dil_x(\theta_*) \leq \lambda(x)\dil_x(\theta_*) \leq 2 (\lambda(x)-\mu(x)) \dil_x(\theta_*)  \leq 2c,
$$
which concludes the proof.
\sq

For each vertex $v\in \cV_0$ we define a set $\Gamma_v\subset \R^2$ as follows : $\Gamma_v := \{v\}$ if $\rho(v) <3$, and 
\be
\label{defGammav}
\Gamma_v := \left[v, \, \frac v 3+ \frac{2w_-} 3\right] \cup \left[v,\frac v 3 +\frac{2w_+} 3\right] 
\ee
if $\rho(v)\geq 3$, where $w_-,w_+\in \cV_0$ are two neighbors of $v$ in $\cT_0$ which respectively minimize and maximize the quantity $\<\theta(v)^\perp, w-v\>$. In mathematical terms for any neighbor $w\in \cV_0$ of $v$
\be
\label{defWmWp}
\<\theta(v)^\perp, w_- -v\> \leq \<\theta(v)^\perp, w-v\> \leq  \<\theta(v)^\perp, w_+ - v\>. 
\ee
This property is illustrated on Figure \ref{figWmWp}.

\begin{figure}
\centering
\includegraphics[width=4cm, height=4cm]{\pathPic/Dessins/Jenny/VT0vJenny.pdf}\hspace{0.5cm}
\includegraphics[width=6cm, height=4cm]{\pathPic/Dessins/Jenny/DirThetaJenny.pdf}
\caption{Neighborhood $V_{\cT_0}(v)$ of a simplex $v$ in the triangulation $\cT_0$ (left), the neighbors $w_+$ and $w_-$ of a vertex $v$ in $\cT_0$.
\label{figWmWp}}
\end{figure}

We define $\Gamma := \cup_{v\in \cV_0} \Gamma_v$, and for each $z\in \Gamma\sm\cV_0$ we define 
\be
\label{defGammaz}
\Gamma_z := \bigcup_{\substack{v\in \cV_0 \\ z \in \Gamma_v}} \Gamma_v.
\ee
Note that for any vertex $v\in \cV_0$ the set $\Gamma_v$ does not contain any vertex $w\in \cV_0$ distinct from $v$, hence \iref{defGammaz} agrees with \iref{defGammav} for any $z\in \cV_0$.\\ 

\begin{lemma}
\label{lemmaAngleWmWp}
let $v\in \cV_0$ be such that $\rho(v) \geq 3$, and let $w_+, w_-$ be two neighbors of $v$ satisfying \iref{defWmWp}.
We have 
\be
\label{eqAngleWmWp}
\varangle(\theta(v)^\perp, w_+ -v) \leq \cPi/4,
\stext{ and }
\varangle(\theta(v)^\perp, v-w_-) \leq \cPi/4.
\ee
\end{lemma}

\proof
We restrict without loss of generality our attention to the proof of the first inequality, and we assume for contradiction that $\vp := \varangle(\theta^\perp, w_+-v)>\cPi/4$. % in \iref{eqAngleWmWp}.
Among the two vertices $w\in \cV_0$ such that the triangle of vertices $v,w,w_+$ belongs to $\cT_0$, we choose the one such that $\varangle(\theta^\perp, w-v)$ is minimal.
We denote $\psi := \varangle(w-v, w_+-v) \in \{\cPi/4, \cPi/2\}$ and we obtain 
$$
\<\theta(v)^\perp, w_+-v\> = |w_+-v|\cos \vp \stext{ and } \<\theta(v)^\perp, w-v\> = |w-v|\cos (\vp-\psi).
$$
If $\psi = \cPi/2$ then $|w_+-v| = |w-v|$ since the triangles $T\in \cT_0$ are half squares, and $\cos (\vp-\psi) = \sin \vp$. We thus have $\cos \vp \geq \sin \vp$ according to \iref{defWmWp} which contradicts our assumption that $\vp>\cPi/4$.
If $\psi = \{\cPi/4\}$ then $|w_+-v| = \sqrt 2 |w-v|$ or $|w_+-v| =  |w-v|/\sqrt 2$. We thus have $\sqrt 2 \cos \vp \geq \cos (\vp-\cPi/4)$ which again contradicts our assumption that $\vp \leq \cPi/4$.
\sq
%
%$$
%\angle(u,u') := \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
%$$
%(Stricly speaking, $\angle(u,u')$ is the smallest of the two unoriented angles formed by $u,u'$ and $u,-u'$.)



%\begin{lemma}
%Let $T\in \cT_0$ and let $z,z'\in T$, then 
%\be
%\label{stabRho}
%\rho(z') \geq  \frac{1-c}{1/\rho(z)+c}.
%\ee
%Defining $\rho_c := \frac{1-c}{1/2+c}$, we have if $\rho(z) \geq 2$ that 
%%$$
%%\rho(z') \geq  \rho_c := \frac{1-c}{1/2+c}.
%%$$
%%and 
%\be
%\label{stabTheta}
%\angle(\theta(z), \theta(z')) \leq \vp_c := \frac c {1-1/\rho_c}.
%\ee
%\end{lemma}
%
%\proof
%Since the functions $\lambda$ and $\mu$ are Lipschitz, and since $|z-z'| \leq \lambda(z)$, we have
%$$
%\rho(z') = \frac {\lambda(z')}{\mu(z')} \geq \frac {\lambda(z)-c \lambda(z)}{\mu(z)-c \lambda(z)} = \frac{\lambda(z)(1-c)}{\lambda(z)(1/\rho(z)+c)} = \frac{1-c}{1/\rho(z)+c},
%$$
%which establishes \iref{stabRho}.
%We thus turn to the proof of \iref{stabTheta}, and for that purpose we recall that 
%$
%(\lambda(z') - \mu(z')) \dil_{z'}(\theta)\leq c
%$
%for any $z'\in T$.
%Observing that 
%$$
%\lambda(z')-\mu(z') = \lambda(z') (1-1/\rho(z')) \geq \diam(T) (1-1/\rho_c)
%$$
%we obtain 
%$$
%\angle(\theta(z), \theta(z')) \leq \diam(T) \max_{z'\in T} \dil_{z'}(\theta) \leq \frac c {1-1/\rho_c},
%$$
%which concludes the proof of \iref{stabTheta}.
%\sq

\begin{lemma}
For any $z\in \Gamma$ and any $z'\in \Gamma_z$ distinct from $z$
we have
\be
\label{eqAngleGammaz}
\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
\ee
and therefore if $c$ is sufficiently small
$$
\angle(\theta(z)^\perp ,z'-z) \leq \cPi/3, 
$$
and there exists a piecewise affine Lipschitz map $\gamma : [\alpha, \beta]\to \R$ such that the following is a bijection
$$
t\in [\alpha, \beta] \mapsto z+ t\theta(z)^\perp + \sqrt 3 \gamma(t) \theta(z) \in \Gamma_v.
$$
\end{lemma}

\proof
We consider a vertex $v\in \cT_0$ such that $z,z'\in \Gamma_v$, and we note that $\rho(v) \geq 3$ by construction of $\Gamma_v$, and therefore $\rho \geq 2$ on a triangle common to $v$ and $z$ according to Corollary \ref{corolRho23}.
It thus follows from Corollary \ref{corolTheta2C} that 
\begin{eqnarray*}
\angle(\theta(z), z-z')&\leq& 2c + \angle(\theta(v), z-z') \\
&\leq& 2c + \max \{ \angle(\theta(v), w_+-v), \angle(\theta(v), w_- -v)\}\\
& \leq & 2c + \cPi/4,
\end{eqnarray*}
which concludes the proof.
\sq

The next proposition gives some properties of the set $\Gamma$.
\begin{prop}
\label{propDistUpLow}
If $c$ is sufficiently small, then the following holds.
For any $z\in \Gamma$,
\be
\label{eqDistzGH0}
 \min\{|z-e| \sep  e\in \Gamma\sm \Gamma_z\} \geq \frac {10}{91} \lambda(z) % >\frac 1 {10}
\ee
and for $z\in \R^2$
\be
\label{eqDistzGH}
\min\{\|z-e\|_{H(z)} \sep e \in \Gamma\} \leq 2 %1+ \frac {2\sqrt 2} 3 <2. 
\ee
\end{prop}

\begin{figure}
\centering
\includegraphics[width = 4cm, height = 4cm]{\pathPic/Dessins/Jenny/DistZGJenny.pdf}
\caption{Illustration of the proof of Proposition \ref{propDistUpLow} \label{figDistZG}}
\end{figure}

\proof
We first establish \iref{eqDistzGH0}. 
Let $z\in \Gamma$ and let $v\in \cV_0$ be such that $z\in \Gamma_v$. We have $z= (1-\alpha) v+\alpha w_*$ for some $\alpha\in [0,2/3]$ and some neighbor $w_*\in \{w_+,w_-\}$ of $v$.
Denoting by $V_{\cT_0}(v)$ the union of all triangles $T\in \cT_0$ containing $v$, and by $\cV_0(v)$ the collection of neighbors of $v$ in $\cT_0$, we have
$$
\Gamma\sm \Gamma(z) \subset \overline {\R^2 \sm V_{\cT_0}(v)} \bigcup_{w\in \cV_0(v)\sm\{w_*\}} \left[\frac{2v+w}3, w\right].
$$
The set appearing in the right hand side is illustrated on Figure \ref{figDistZG}.
It follows that 
\begin{eqnarray*}
d(z,\Gamma\sm \Gamma(z)) &\geq & \min \left\{ d(z, \R^2 \sm V_\cT(v)), \ \min_{w\in \cV_0(v) \sm \{w_*\} } d\left(z,\left[\frac{2v+w}3, w\right]\right)\right\}\\
& \geq & \min \left\{ \frac{|w_*-z|}{\sqrt 2}, \ \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)\sm \{w_*\}} |v-w|\right\}\\
& = & \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)} |v-w|\\
& \geq & \frac{1}{3\sqrt 2} \lambda(v)\frac {\sqrt 2} 3 \\
&\geq&  \frac{\lambda(z)(1-c)}{9}.
\end{eqnarray*}
where we used \iref{edgeLambda} in the fourth line, and \iref{eqLambdaT} in the last line. This establishes \iref{eqDistzGH0} if $c$ is sufficiently small.\\

We now turn to the proof of \iref{eqDistzGH}. 
Let $T \in \cT$ and let $z\in T$. Since $T$ is a half square there exists a vertex $v$ of $T$ such that $|z-v| \leq \diam(T)/2$, hence %For any vertex $v$ of $T$ we obtain %If $\rho(z)\leq 4$, then any vertex $v$ of $T$ satisfies 
$$
\|z-v\|_{H(z)} \leq  \frac{|z-v|}{\mu(z)}   \leq \frac{\diam(T)}{2 \mu(z)} \leq \frac{\lambda(z)}{2 \mu(z)} = \frac{\rho(z)} 2,
$$
which concludes the proof if $\rho(z) \leq 4$. If $\rho(z) \geq 4$ and $c$ is sufficiently small then $\rho(v) \geq 3$ for any vertex $v$ of the triangle $T$ according to Corollary \ref{corolRho23}.

We choose two vertices $v,w$ of $T$ such that the line $(z+ r \theta(z))_{r\in \sR}$ intersects $\partial T$ on the segment $[v,(v+w)/2]$.
We denote by $w_-$ and $w_+$ the neighbors of $v$ in $\cT_0$ which satisfy \iref{defWmWp}.
Our first step is to establish that the line $(z+ r \theta(z))_{r\in \sR}$ intersects the set $\Gamma_v$ : this is heuristically due to the fact that the angle $\lhd(\theta(z), \theta(v))$ is small and that the vertices $w_-$ and $w_+$ are the \emph{fathest} from $v$ in the direction of $\theta(v)^\perp$ as illustrated on Figure \ref{figWmWp} (right).

We have according to \iref{eqEdgeRatio}
$$
\<\theta(v)^\perp,w_+ - v\> \geq |w_+-v|\cos(\cPi/4) \geq \frac{|w-v|} 2 \frac 1 {\sqrt 2}. %/(2\sqrt 2).
$$
We assume without loss of generality that %$\theta(v)$ and $\theta(z)$ are oriented in consistently, in such way that 
$\<\theta(z), \theta(v)\> \geq 0$, and we obtain using Corollary \ref{corolTheta2C}
$$
|\theta(z)-\theta(v)| \leq \varangle(\theta(z), \theta(v)) = \lhd(\theta(z), \theta(v))\leq 2c.
$$
It follows that 
\begin{eqnarray*}
\<\theta(z)^\perp, w-v\> &=& \<\theta(z)^\perp-\theta(v)^\perp, w-v\>+\<\theta(v)^\perp, w-v\>\\
& \leq & |\theta(z)-\theta(v)| |w-v| + \<\theta(v)^\perp, w_+-v\>\\
& \leq & (1+4c \sqrt 2 )\<\theta(v)^\perp, w_+-v\>.\\
%& \leq & (1+4 c\sqrt 2) }{1-\vp_c\sqrt 2} \<\theta(z)^\perp,w_+ - v\>.
%& \leq & \frac 4 3 \<\theta(z)^\perp,w_+ - v\>
\end{eqnarray*}
Denoting $\Theta := \varangle(\theta(v)^\perp, w_+-v)$ and $\Phi := \varangle(\theta(z)^\perp, w_+-v)$ we obtain 
$$
\frac{\<\theta(v)^\perp, w_+-v\>}{\<\theta(z)^\perp, w_+-v\>} = \frac{\cos(\Theta)}{\cos(\Phi)} \leq \frac{\cos(\Theta)}{\cos(\Theta) - |\Phi-\Theta|} =\left(1-\frac {|\Phi-\Theta|}{\cos\Theta}\right)^{-1}\leq (1-2 \sqrt 2 c)^{-1} % - 2c} = \frac 1 {1-2 \sqrt 2 c},
$$
hence 
$$
\<\theta(z)^\perp, w-v\>  \leq \frac{1+4c \sqrt 2}{1-2 \sqrt 2 c}\<\theta(z)^\perp, w_+-v\>
$$
Proceeding likewise for $w_-$, and assuming that $c$ is sufficiently small, we obtain 
%
%We assume that $c$ is sufficiently small in such way that 
%\be
%\label{assumPhic}
%\frac{1+\vp_c 4\sqrt 2}{1-\vp_c\sqrt 2}\leq \frac 4 3
%\ee
$$
\frac 4 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, w-v\> \leq  \frac 4 3\<\theta(z)^\perp, w_+ - v\>,
$$
and therefore since $z+r\theta(z)\in [v,(v+w)/2]$ for some $r\in \R$,
$$
\frac 2 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, z-v\> \leq  \frac 2 3\<\theta(z)^\perp, w_+ - v\>.
$$
It follows that the line $(z+r\theta(z))_{r\in \sR}$ intersects the set $\Gamma_v := [v, (v+2w_+)/3] \cup  [v, (v+2w_-)/3]$ at some point $z'$.
%hence there exists $r\in \R$ such that $z' := z+ r\theta(z) \in \Gamma_v$. 
The point $z'$ belongs to triangle $T'$ containing $v$, and we obtain using \iref{eqDiamRatio} 
\begin{eqnarray*}
\lambda(z) \|z'-z\|_{H(z)} &=& \lambda(z)\|r\theta(z)\|_{H(z)}\\
&=& |r|\\
&=& |z-z'|\\
&\leq& |z-v|+|v-z'|\\
&\leq& \diam(T)+ \frac 2 3\diam(T')\\
&\leq & \left(1+\frac 2 3 \sqrt 2\right) \diam(T)
 \leq  \left(1+\frac 2 3 \sqrt 2\right) \lambda(z),
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

We construct in the next lemma the set of vertices $\cV$ of the quasi-acute triangulation $\cT$ to be constructed by sampling the set $\Gamma$.

\begin{lemma}
\label{lemmaConstV}
The following holds if $c$ is sufficiently small.
There exists a discrete set $\cV \subset\Gamma$ containing $\cV_0$ and satisfying the following:
\begin{enumerate}[i)]
\item (Separation) For all $v,w\in \cV$, $d_H(v,w) \geq 1/10$.
\item (Distance from $\Gamma$) For all $z\in \Gamma$, $d_H(z, \cV) \leq 1/10$.
\item (Distance from $\R^2$) For all $z\in \R^2$, $d_H(z,\cV) \leq 2+1/4$.
\end{enumerate}
\end{lemma}
\proof
For any distinct $v,w\in \cV_0$ we obtain using \iref{pairwiseV0} and Proposition \ref{propEuclidRiemann}
\begin{eqnarray*}
d_H(v,w) &\geq& \ln(1+c\|v-w\|_{H(v)})/c\\
&\geq& \ln(1+c|v-w|/\lambda(v))/c\\
&\geq& \ln(1+c\sqrt 2 /3)/c 
\end{eqnarray*}
which is larger than $1/10$ if $c$ is sufficiently small. % since $\sqrt 2 /3>1/10$.

We denote by $\cV$ a $1$-equispaced subset of the metric space $(\Gamma, 10\:d_H)$ containing $\cV_0$, which exists according to Lemma \ref{lemmaEquiSpaced}. The two first announced properties, separation and distance from $\Gamma$, follow directly from this construction.

The third property is obtained as follows: for any $z\in \R^2$ there exists according to Proposition \label{propDistUpLow} a point $e\in \Gamma$ such that $\|z-e\|_{H(z)}\leq 2$. Furthermore there exists a vertex $v\in \cV$ such that $d_H(e,v) \leq 1/10$, hence
$$
d_H(z,\cV) \leq d_H(z,e)+ d_H(e,v) \leq -\ln(1-c\|z-e\|_{H(z)})/c + 1/10 \leq -\ln(1-2c)/c + 1/10.
$$
which is smaller than $2+1/4$ if $c$ is sufficiently small.
\sq


\begin{lemma}
\label{lemmaDiamVorGamma}
For any $v\in \cV$ we have 
$$
\max\{\|z-v\|_{H(v)} \sep z\in \Gamma\cap \Vor(v)\} \leq r_0(c) := (e^{c/10}-1)/c.
$$
(and $r_0(c) \to 1/10$ as $c\to 0$).
Furthermore $c$ is sufficiently small and if $v,w\in \cV$ are such that $\Vor(v) \cap \Vor(w) \cap \Gamma \neq \emptyset$, then 
$$
\|v-w\|_{H(v)} \leq 1/4.
$$
\end{lemma}

\proof
According to point ii) of Lemma \ref{lemmaConstV} there exists $w\in \cV$ such that $d_H(z,w) \leq 1/10$. It thus follows from the definition of the Voronoi diagram that 
\begin{eqnarray*}
\|z-w\|_{H(w)} &\leq& \|z-w'\|_{H(w')}\\
&\leq& (\exp(c d_H(z,w'))-1)/c\\
&\leq&  (\exp(c/10)-1)/c.
\end{eqnarray*}

We now turn to the second point of the proposition, and we consider a point $z\in \Vor(v) \cap \Vor(w) \cap \Gamma$.
We thus have $\|z-v\|_{H(v)} = \|z-w\|_{H(w)} \leq r_0(c)$ which implies 
$$
\ln(1+c\|v-w\|_{H(v)})/c \leq d_H(v,w) \leq d_H(v,z)+d_H(z,w) \leq -2 \ln(1-c r_0(c))/c
$$
hence $\|v-w\|_{H(v)} \leq ((1-cr_0(c))^{-2}-1)/c$ which tends to $1/4$ as $c\to 0$. This concludes the proof of this proposition.
\sq


\begin{lemma}
\label{lemmaRecallG}
There exists a absolute constant $C_0\geq 1$ such that the following holds if $c$ is sufficiently small.
The set $\cV$ is wedged with respect to the metric $H$, and the anisotropic Delaunay triangulation obtained by arbitrarily triangulating the cells of the graph $\cG(\cV,H)$ is $C_0$-adapted to $H$.

Furthermore for any edge $[v,w]$ of $\cT$ and any $z\in [v,w]$ we have 
$$
\|v-w\|_{H(z)} \leq 5.
$$
\end{lemma}

\proof
We denote $\alpha := (2+1/4)^{-1}$ throughout the proof of this lemma.
It follows from to Lemma \ref{lemmaConstV} that the set $\cV$ is a $\alpha/10$-equispaced subset of the metric space $(\R^2, \alpha d_H)$. 

Theorem \ref{thEquiMesh} applied to the metric $\alpha^2 H$, therefore implies that, if $c$ is sufficiently small, the set 
$\cV$ is wedged for the metric $\alpha^2 H$ and that arbitrarily triangulating the convex cells of the graph $\cG(\cV,\alpha^2 H)$, which are convex yields a triangulation $\cT$ which is $C$-adapted to the metric $\alpha^2H$ (hence $C_0 := C/\alpha$-adapted to $H$), where $C$ is an absolute constant.

The definition \iref{defGVH} of the graph $\cG(V,H)$ implies that $\cG(\cV,\alpha^2 H) = \cG(\cV,H)$, and Definition \ref{defWedge} of the wedge property shows that it holds for $H$ if and only if it holds for $\alpha^2 H$. 

For any edge $[v,w]$ of $\cT$ the Voronoi regions $\Vor(v)$ and $\Vor(w)$ intersect (by definition of the anisotropic Delaunay triangulation), and we thus have according to Lemma \ref{lemmaDiamVor} 
$$
\alpha d_H(v,w) = d_{\alpha^2 H} (v,w) \leq -2\ln (2-e^{c'})/c'
$$
where $c' := c/\alpha$. Hence 
$$
d_H(v,w) \leq r_0(c) := -2 \ln (2-e^{c/\alpha})/c.
$$
If follows that 
$
\|v-w\|_{H(v)} \leq r_1(c) := (e^{c r_0(c))}-1)/c,
$
hence \iref{eqLocalNorm}
$
\|v-w\|_{H(z)} \leq \|v-w\|_{H(v)} (1-c \|v-z\|_{H(v)})^{-1} \leq r_2(c) := r_1(c) (1-c r_1(c))^{-1}
$
for any $z\in [v,w]$.
As $c\to 0$ the functions $r_0$, $r_1$ and $r_2$ all tend to $2 (1+1/4) <5$. Choosing $c$ sufficiently small concludes the proof of this proposition.
\sq


\begin{lemma}
If $c$ is sufficiently small, then the following holds.
For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$ we have 
\be
\label{vpNotInGammav}
\sin \lhd (\theta(v),v-w) \leq \frac {50}{\rho(v)}.
\ee
%We define $\rho_0\in [1,\infty)$ by $\sin (\cPi/12) = 50/\rho_0$.
\end{lemma}

\proof
If $c$ is sufficiently small, then Proposition \ref{propDistUpLow} implies that $|v-w| \geq \lambda(v)/10$, and Lemma \ref{lemmaRecallG} states that $\|v-w\|_{H(v)} \leq 5$.
Denoting $\vp := \lhd (\theta(v),v-v')$ we obtain 
$$
5\geq \|v-w\|_{H(v)} \geq \frac{|v-w|\sin \vp}{\mu(v)} \geq \frac{\lambda(v) \sin \vp}{10 \mu(v)}.
$$
which implies the announced result.
\sq

%\begin{lemma}
%If $c$ is sufficiently small, then the following holds.
%
%\end{lemma}

The next lemma gives a lower bound on the distance from a vertex $v\in \cV$ to the Voronoi region of a vertex $w\in \cV\sm\Gamma$.

\begin{lemma}
\label{lemmaVorFar}
If $c$ is sufficiently small, then for any $v\in \cV$, $w\in \cV\sm \Gamma_v$ 
$$
\inf\{|v-z|\sep z\in \Vor(w) \cap \Gamma\} \geq \lambda(v)/100.
$$

%and $z\in \Vor(w)\cap \Gamma$ we have 
%$$
%|z-v|\geq \lambda(v)/100.
%$$
\end{lemma}

\proof
We have for any $z\in \Vor(w) \cap \Gamma$, according to Lemma \ref{lemmaDiamVorGamma} 
\begin{eqnarray*}
|v-z| &\geq& |v-w|-|z-w|\\
& \geq & |v-w| - \|z-w\|_{H(w)} \lambda(w)\\
& \geq & |v-w| - r_0(c) (\lambda(v)+c|v-w|)\\
& = & |v-w| (1-c r_0(c)) -r_0(c) \lambda(v)\\
& \geq & \frac {10} {91}\lambda(v) (1-cr_0(c)) - r_0(c) \lambda(v)\\
&=& r_1(c) \lambda(v),
\end{eqnarray*}
where we used \iref{eqDistzGH0} in the fifth line, and where $r_1(c) := 10(1-cr_0(c))/91 - r_0(c)$.
As $c\to 0$ we have $r_0(c) \to 1/10$ and $r_1(c) \to 10/91-1/10 >1/100$. If $c$ is sufficiently small we therefore have $r_1(c) \geq 1/100$ which concludes the proof.
\sq

The next proposition shows that the Voronoi cell of a vertex $v$ contains a ball of fixed radius for the distance $\|\cdot\|_{H(v)}$ (hence an ellipse).

\begin{lemma}
\label{lemmaVorBall}
If $c$ is sufficiently small, then 
for any $v\in \cV$ we have 
$$
\Vor(v) \supset \{z\in \R^2 \sep \|z-v\|_{H(v)} \leq 1/25\},
$$
\end{lemma}

\proof
We consider $z\in \partial \Vor(v)$, hence $z\in \Vor(v) \cap \Vor(w)$ for some vertex $w\in \cV$.
We define $r:=\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$ and we obtain using Point i) of Lemma \ref{lemmaConstV}
\begin{eqnarray*}
1/10 &\leq& d_H(v,w)\\
&\leq& d_H(z,v)+d_H(z,w)\\
&\leq& -\ln (1-c\|z-v\|_{H(v)})/c - \ln (1-c\|z-v\|_{H(v)})/c\\
&=& -2 \ln (1-cr)/c.
\end{eqnarray*}
It follows that 
$$
r\geq (1-\exp(-c/20))/c,
$$
and therefore $r\geq 1/25$ if $c$ is sufficiently small, 
which concludes the proof.
\sq

%The set $\Gamma$ is a union of polygonal lines (and of isolated points). If $v\in \Gamma$ is on a polygonal line, we say that the neighbors of $v$ on $\Gamma$ (if they exist) are the previous and next points on $\Gamma$.

%The set $\Gamma$ is a union of polygonal lines (and of isolated points). We say that two points $v,w\in \Gamma$ are neighbors on $\Gamma$ if 

We say that two points $v,w\in \cV$ are neighbors on $\Gamma$ if 
$$
(v,w) \subset \Gamma\sm \cV.
$$
Note that $\Gamma\sm\cV$ is a collection of straight open intervals, since $\cV_0\subset \cV$.
Note also that two neighbors on $\Gamma$ belong to the same element of $\cT_0$.

\begin{lemma}
\label{lemmaSegVor}
If $c$ is sufficiently small, then the following holds.
For any $v\in \cV$ such that $\rho(v) \geq \rho_0 = 22$ the vector $v$ has at least a neighbor on $\Gamma$. Furthermore for any neighbor $w$ of $v$ on $\Gamma$ we have 
$$
|v-w|\leq \mu(v)/2
$$
and 
\be
\label{eqNeighborEdge}
[v,w] \subset \interior(\Vor(v) \cup \Vor(w)).
\ee
and consequently $[v,w]$ is an edge of $\cT$. 
\end{lemma}

\proof
We first remark that according to Lemma \ref{lemmaDiamVorGamma} 
\be
\label{dzvmu}
r_0(c) \geq \|z-v\|_{H(v)} \geq \cos\left(\cPi/ 3 \right) \frac {|z-v|}{\mu(v)}  = \frac {|z-v|}{2 \mu(v)}
\ee
We assume for contradiction that the inclusion \iref{eqNeighborEdge} does not hold, and we thus consider two points $z\in [v,w]\cap \Vor(v)$ and $w'\in \cV$ such that $z\in \Vor(w')$.



If $w'\notin \Gamma_v$, then $|z-v| \geq  \lambda(v)/100$ according to Lemma \ref{lemmaVorFar}.
Combining this with \iref{dzvmu} we obtain 
$$
\rho_0 \leq \rho(v) = \lambda(v)/\mu(v) \leq 200 r_0(c).
$$
If $c$ is sufficiently small then $200r_0(c) < 21 < 22$ which gives a contradiction (recall that $r_0(c) \to 1/10$ as $c\to 0$).

We now consider the case $w'\in \Gamma_v$, and we first assume that $w'$ is not on the same side as $w$ on $\Gamma$, in the sense that $\<w-v, \theta(v)^\perp \>>0$ and $\<w'-v, \theta(v)\> <0$.
Hence there exists $\alpha\in [0,1]$ and $r\in \R$ such that 
$$
v + r \theta(v) = z+ \alpha(w'-z).
$$
%Consider a vector $u$ orthogonal to $w-z'$. 
We thus have 
$
r\<\theta(v),(w'-z)^\perp \> = \<z-v , (w'-z)^\perp\>
$
hence
$$
r/2\leq  |r| \cos \lhd(\theta(v)^\perp, w'-v) \leq  |z-v| \leq 2 \mu(v) r_0(c).
$$
According to \cite{Shew} Lemma 3 (Visibility Lemma) the Voronoi regions of a wedged Voronoi diagram are star-shaped. Since the Voronoi diagram is wedged according to Lemma \ref{lemmaRecallG} we obtain using Lemma \ref{lemmaVorBall} that 
$$
\frac {\lambda(v)} {25} = \|r\theta(v)\|_{H(v)} \leq r \leq 4 \mu(v) r_0(c),
$$
hence $\rho_0 \leq \rho(v) \leq 100 r_0(c)$. This is a contradiction if $c$ is sufficiently small since $100 r_0(c) <11 <22 = \rho_0(c)$.

It follows that $w'$ is on the same side as $w$ on $\Gamma$, with respect to $v$, in the sense that  $\<w-v, \theta(v)^\perp \>>0$ and $\<w'-v, \theta(v)^\perp\> >0$.

We now remark that the vertices $v,w$ belong to the same element of $\cT_0$ since they are neighbors on $\Gamma$. Hence $\rho(w) \geq \rho_0 - 1=21$ if $c$ is sufficiently small.
Way may therefore apply this proof to $w$, and we obtain that $w'$ is on the same side as $v$ with respect to $w$, in the sense that  $\<w'-w, \theta(w)^\perp \><0$ and $\<w'-v, \theta(w)\> <0$ (if $\<\theta(w), \theta(v)\> >0$).

It follows that $w'\in (v,w)$ which is a contradiction.


Finally, we remark that according to Lemma \ref{lemmaDiamVorGamma}
$$
1/4 \geq \|v-w\|_{H(v)} \geq \frac{|v-w| \cos (\cPi/3)}{\mu(v)} = \frac{|v-w|}{2\mu(v)}
$$
hence $|v-w|\leq \mu(v)/2$ which concludes the proof.
\sq


\begin{prop}
The following holds if $c$ is sufficiently small.
For any $v\in \cV$ be such that $\rho(v)\geq \rho_1$, where $\rho_1$ is a constant specified in the proof, the following holds.
\begin{enumerate}
\item The vertex $v$ has two neighbors $w,w'$ on $\cT$ such that 
\be
\label{eqAnglesUpDown}
\varangle(w-v, \theta(v)) \leq \cPi/12 \stext{ and } \varangle(w'-v, -\theta(v)) \leq \cPi/12.
\ee
\item A vertex $w\in \cT\cap \Gamma_v$ is a neighbor of $v$ on $\cT$ if and only if it is a neighbor of $v$ on $\Gamma$.
\end{enumerate}
\end{prop}

\proof
Consider a neighbor $w_*$ of $v$ on $\Gamma$. Then according to Lemma \ref{lemmaSegVor} the segment $[v,w]$ is an edge of $\cT$, hence $w_*$ is a neighbor of $v$ on $\cT$ by definition.
Let $T,T'\in \cT$ be the two triangles containing the edge $[v,w_*]$, and let $w,w'\in \cV$ be the third vertex of these triangles respectively.

Since $\cT$ is $C_0$-adapted to the metric $H$, we obtain 
$$
|T| = |\TEq| (\det \cH_T)^{-\frac 1 2} \geq |\TEq|  C_0^{-2} (\det H(v))^{-\frac 1 2} =  |\TEq|  C_0^{-2} \lambda(v) \mu(v).
$$
On the other hand $|w_*-v| \leq \mu(v)/2$ according to Lemma \ref{lemmaSegVor}, and 
$$
\mu(v)\sin \lhd(w-v,\theta(v))  |w-v|\leq \|v-w\|_{H(v)} \leq C_0 \|v-w\|_{\cH_T} \leq 2C_0.
$$
Combining these inequalities we obtain  
$$
|\TEq|  C_0^{-2} \lambda(v) \mu(v) \leq  |T| \leq \frac 1 2 |w-v| |w_*-v| \leq \frac{2C_0\mu(v) }{\sin \lhd(w-v,\theta(v))} \mu(v)/2.
$$
hence 
$$
\sin \lhd(w-v,\theta(v)) \leq \frac{C_0^3}{|\TEq| \rho(v)}. 
$$
We define 
$$
\rho_1 := \frac{C_0^3}{|\TEq|\sin (\cPi/12)}
$$
and we thus obtain $\lhd(w-v,\theta(v)) \leq \cPi/2$. Likewise $\lhd(w'-v,\theta(v)) \leq \cPi/2$. 

Since $\varangle (w_* - v, \theta(v)) \in [\cPi/3,2 \cPi/3]$, and since the triangles $T,T'$ contain the edge $[v,w_*]$, thus implies \iref{eqAnglesUpDown}.

Let $v'\in \cV \cap \Gamma_v$ be a vertex on the side of the neighbor $w_*$.
Then $\lhd(v'-v, \theta(v)^\perp) \leq \cPi/3$ which implies that the segment $[v,v']$ intersects one of the triangles $T$ or $T'$. 
Therefore $v'$ is not a neighbor of $v$ in $\cT$.

Likewise, if $v$ has a second neighbor $w_{**}$ on $\Gamma$ (on the other side than $w_*$ with respect to $w$), then $[v,w_{**}]$ is an edge of $\cT$. Similarly we obtain that for any point $v''\in \Gamma_v$ on the side of $w_{**}$, the segment $[v,v'']$ is not an edge of $\cT$.

This implies Point 2. and concludes the proof of this proposition.


This is a contradiction, hence no point on the side of the neighbor


we obtain the announced result.
We define $\rho_1$ by the equation $\cos (\cPi/12) = C_0^3 / |\TEq| \rho_1$ and we obtain 

It follows that 
$$
|u-v| \geq 
$$
Consider a neighbor $w$ of $v$ on $\Gamma$. Then 


If follows from \iref{eqAngleGammaz} that there exists an interval $[\alpha, \beta]$, and a Lipschitz map $\omega : [\alpha, \beta]\to \R$ such that 
$$
t\in [\alpha, \beta] \to z+ \gamma(t) := z+ t \theta(z)^\perp + \sqrt 3 \omega(t) \theta(z) \in \Gamma_v %\Gamma(t) :=
$$
is one to one. % ($\omega$ is piecewise affine)
We have 
$$
\frac {|t-t'|} {\mu(z)} \leq \|\gamma(t)-\gamma(t')\|_{H(z)} = \sqrt {\left(\frac{t-t'}{\mu(z)}\right)^2 + 3 \left(\frac{\omega(t)-\omega(t')}{\lambda(z)}\right)^2} \leq \frac {|t-t'|} {\mu(z)} \sqrt {1+3\rho(z)^{-2}}.
$$

Our purpose is now to establish that $v$ for any neighbor $w$ of $v$ on $\Gamma$ the segment $[v,w]$ is an edge of $\cT$.
We assume that $v$ has a neighbor $w$ corresponding to a positive value of $t$.
We define 
$$
\beta' := \max\{t\in [0,\beta]\sep v+\gamma(t') \in \Vor(v) \text{ for } 0 \leq t'\leq t\} 
$$
and we observe that 
$$
|\beta'|/\mu(v) \leq \|\gamma(\beta')\|_{H(v)} \leq (\exp(c/10)-1)/c.
$$
Note that $v+r\lambda\theta(v) \in \Vor(v)$ for $|r|\leq 1/25$.
Since the Voronoi regions are star shaped, it follows that $z:=v+\gamma(\beta')\notin \Vor(w)$ for $w\in \Gamma_v$ corresponding to negative values of $t$.
Furthermore $z\notin \Vor(w)$ for $w\in \Gamma\sm \Gamma_v$ due to Lemma \label{lemmaVorFar}.

Thus $z\in \Vor(w)$ for some $w\in \Gamma_v$ corresponding to a positive value of $t$. 
Upper bound on $t$ since $\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$ we obtain 
$$
\ln(1+c\|v-w\|_{H(v)})/c \leq  d_H(v,w) \leq d_H(v,z)+d_H(z,w) \leq -2\ln(1-c\|z-v\|_{H(v)})/c.
$$
Apply the argument that the Voronoi region is star shaped to the neighbor of $v$.

Denote by $T_0,T_1$ the two triangles containing $[v,w]$, and denote by $w_0, w_1$ the two third vertices.
the edges $[v,w_0]$ and $[v,w_1]$ are close to the direction of $\theta(v)$, using the fact that $\cH_{T_i} \simeq H(v)$. 
More precisely : 
Or area of $T_i$ -> length $|v-w_i|\simeq \lambda$ -> orientation since $\|v-w_i\|_{H(v)} \leq 5$.
Thus no connection with neighbors corresponding to positive $t$.


%
%Upper boun
%We have 
%$$
%\<\theta
%$$
%
%
%
%
%We recall that the Voronoi regions are star shaped (insufficient argument since not a strainght line), and we define 
%$$
%[\alpha', \beta'] := \{t\in [\alpha, \beta] \sep v+\gamma(t) \in \Vor(v)\}.
%$$
%We assume that $\beta'<\beta$, otherwise 
%We have 
%$$
%|\beta'|/\mu(v) \leq \|\gamma(\beta')\|_{H(v)} \leq (\exp(c/10)-1)/c.
%$$
%Let $w\in \cV$, $w\neq v$, be such that $v+\gamma(\beta') \in \Vor(w)$.
%We have $\|w-v+\gamma(\beta')\|_{H(w)} = \|\gamma(\beta')\|_{H(v)}$, hence 
%
%
%For any $w\in \cV$ we have $d_H(v,w) \geq 1/10$
%
%
%Let $w\in \cV$, $w\neq v$, be such that $v+\gamma(\beta') \in \Vor(w)$.
%We have $\|w-v+\gamma(\beta')\|_{H(w)} = \|\gamma(\beta')\|_{H(v)}$, hence 
%
%
%
%
%
%Note that 
%The index of 
%
%$$
%\alpha' := \min ([\alpha,\beta] \cap \Vor(v)) \text{ and } \beta' := \max ([\alpha, \beta] \cap \Vor(v)),
%$$
%
%If $\beta' = \beta$, then there is no 
%We define 
%
%
%We have 
%$$
%d_H(z,z+\gamma(t)) \geq \ln (1+c\|\gamma(t)\|_{H(z)}) = \ln(1+c 
%$$
%
%We parametrize the set $\Gamma_v$ by the map $\gamma :[\alpha, \beta]\to  \Gamma_v$ defined as follows : for all $x\in [\alpha, /\beta]$
%$$
%\gamma^{-1}(x)= \< \theta(v)^\perp , x-v\>.
%$$
%We have the estimates
%$$
%bjlxt
%$$
%
%(*big one*)
%We consider two successive points $v,w\in \cV$ on $\Gamma$, and we show that $[v,w]\subset \interior(\Vor(v) \cup \Vor(w))$ if $\rho(v)\geq ??$.
%
%Note that $\|v-w\|_{H(v)} \leq 2\delta_1(1+o_c(1))$.
%Indeed $B_H(v+\delta_1\bt(v)??, \delta_1(1+??))$ contains a point, which needs to be on $\Gamma_v$, hence neighbor not far.
%
%No problem from $\Gamma\sm \Gamma_z$.
%
%We have $v+r\lambda \theta(v)$ for $r\in [??\delta_1,??\delta_1]$, and likewise for $w$.
%Thus angle formed : 
%$$
%|\<\theta(v)^\perp, v+r \lambda\theta(v) - (\alpha v+(1-\alpha)w)\>| \leq |v-w| \leq 3\mu.
%$$
%and 
%$|v+r \lambda\theta(v) - (\alpha v+(1-\alpha)w)| \geq  |r|\lambda -|v-w|\geq |r|\lambda(v) - 3\mu(v)$
%Thus if $\rho(v)$ is sufficiently large,
%$$
%\angle(\theta(z)^\perp , ...) > \cPi/3,
%$$
%hence the point does not belong to $\Gamma_z$. Thus $z\notin \Vor(x)$, thus the $[v,w]$ belongs to the interior of $\Vor(v) \cup \Vor(w)$.
%
We next show that $v$ is not linked to other points on $\Gamma_v$.
Assume that this is the case for contradiction.
$w\in \Gamma_v$ is such that $[v,w]$ is an edge of $\cT$.
We introduce the vertex $v_0\in \cT_0$ in between $v$ and $w$.
The segments $[v,v_0]$ and $[v_0,w]$ are included in the edge set of $\cT$. The triangle of vertices $v,v_0,w$ contains an element of $\cT$, but this is a contradiction with the diameter which should be of the order $\lambda(v)$ and not $\mu(v)$.





%%First we remark that $
%Let $z=\alpha v+(1-\alpha) w$.
%We grow an ellipse around $z$, we first fall on $v,w$
%
%The collection $\cV$ of vertices is a $1$-equispaced subset of $(\Gamma, d_H/\delta_1)$, 
%For all $x\in \Gamma$
%By construction 
%
%For that purpose we remark that 
%
%Let $x\in \cV$.
%
%
%
%
%
%We thus turn to the proof of the second property. The fact that  the angle property appearing in \iref{vpInGammav} is a direct consequence of \iref{eqAngleGammaz} : we have $\angle (\theta(v)^\perp, v-w) \leq \cPi/3$ provided $\vp_c \leq \cPi/12$ which is the case if $c$ is sufficiently small.
%
%We thus have 
%$$
% \cos(\cPi/3)\frac{|v-v'|}{\mu(v)} \leq \|v-w\|_{H(v)}\leq 12.
%$$
%
%We now establish that $e\subset \Gamma$, if $\rho(v)$ is sufficiently large, and for that purpose we first show that two successive points on $\Gamma$ are always linked by an edge.
%
%
%Use star shaped.
%
%Then we consider the two triangles containing this edge, and we obtain a contradiction with the angle...
%
%We then assume that there exists another connection, and we obtain a contradiction with the diameter of the triangle.
%%we denote by $v_*$ the point of $\cV$ next to $v$ in $\Gamma$ and such that $\<v^*-v, \, v'-v\> \geq 0$.
%%The voronoi region of $v^*$ contains...
\sq

%\begin{corollary}
%\label{corolDirRho}
%If $c$ is sufficiently small.
%Let $T_0\in \cT_0$ and let $z\in T_0$. If $\rho(z) \geq \rho_0$, then any edge $e$ of $\cT$ intersecting $T_0$ satisfies $e\subset \Gamma$ or $\angle(\vec e, \theta) \leq \cPi/12$.
%\end{corollary}
%
%\proof
%
%\sq


%We say that a point $v\in \cV$ is extremal if $\Gamma_v\neq \{v\}$ and if at least one the two (opposite) tangent vectors $\bt(v)$ to $\Gamma$ at the point $v$, satisfies 
%$$
%\Gamma_v \cap \cV \cap (v +  \bt(v)\R_+) = \emptyset.
%$$

We define $\rho_* := \max\{\rho_0, \rho_1\}$.
If a triangle $T\in \cT$ contains a simplex $v\in \cV$ such that $\rho(v) \leq \rho_*$, then we obtain 
$$
S(T) \leq \rho(T) = \sqrt{\|\cH_T\| \|\cH_T^{-1}\|} \leq C_0^2 \rho(v) \leq C_0^2 \rho_*.
$$
The next lemma allows to control the angles at the points $v$ which satisfy $\rho(v) \geq \rho_*$.
\begin{lemma}
\label{lemmaAngles}
To each vertex $v\in \cV$ such that $\rho(v) \geq \rho_*$ we associate the collection $E(v)$ of all vectors $w-v$ where $w$ is a neighbor of $v$ in $\cT$, as well as the two tangents to $\Gamma$ at $v$.
%
% of vectors $w-v$ for all $w\in \cV_0(v)$, as well as $\bt(v)$ if $v$ is extremal.
The angle formed by two successive directions in $E(v)$, in trigonometric order, is smaller that $\vp_*$.
%is uniformly bounded by an absolute  constant independent of $H$.
\end{lemma}

\proof
At each vertex $v$ we have the four directions : close to $\theta$, $-\theta$, and not so far from $\theta^\perp$ and $-\theta^\perp$ (one of the two last ones being brought by $\bt(v)$ if $v$ is extremal).

%Such a vertex $v$ has an edge with a neighbor $w\in \Gamma$. Consider could be a corollary of the previous.
\sq

\begin{prop}
%Denote by $\cT^*$ the non-conforming triangulation obtained by cutting the triangles in $\cT$ containing an extremal vertex $v$ and such that $\rho(v) \geq \rho_0$ in the direction of $\bt(v)$.

Denote by $\cQ$ the partition into convex polygons obtained by cutting $\cT$ by all segments joining an extremal vextex $v\in \cV$ satisfying $\rho(v) \geq ??$ to the vertex $v'\in \cV_0$ in the direction of $\bt(v)$.

Then the interior angles in $\cQ$ are smaller than ??. %Each triangle $T\in \cT$ contains at most $??$ cells of $\cC$, which are at most hexagons (in other words they have $3$ to $6$ elements).

Denote $\cT'$ the triangulation obtained by randomly triangulating the convex cells of $\cQ$.

Then $\cT'$ is a $??$-refinement of $\cT$ and $S(T') \leq ??$ for all $T'\in \cT'$.
\end{prop}

\proof
The angles of the cells $Q\in \cQ$ fall into two categories.
The angles at the vertices of $\cT$ are bounded by ?? according to Lemma \ref{lemmaAngles}.
The angles which are not at the vertices are formed by the junction from an extremal vertex to $v\in \cV$ to the vertex $w\in \cT_0$ in front, and are bounded by ?? combining Lemma \ref{lemmaDirRho} and the direction of $\bt(v)$.\\

The triangulation $\cT'$ is obtained by triangulating the convex cells forming $\cQ$, and this operation reduces the angles. We thus have the same bound ??, and
$$
S(T) \leq \tan(??/2).
$$

We now prove that $\cT'$ is a bounded refinement of $\cT$, and for that purpose we consider and edge $e=[v,w]$ of $\cT$. %=[\omega-u, \omega+u]

We have by construction $|v-w|/\lambda(v) \leq \|v-w\|_{H(v)} \leq 12$.
The triangles $T\in \cT_0$ intersected by $[v,w]$ satisfy for some $z\in [v,w]$ the inequality 
$$
2 \delta_0 \lambda(v) (1-12c) \leq 2 \delta_0 \lambda(z) \leq \diam(T) \leq \lambda(v) \leq \lambda(u)(1+12c)
$$
Therefore they are contained in the ball $B(v,  \lambda(v)(12+1+12c))$ and have area 
$$
|T| = \diam(T)^2/4 \geq \delta_0^2 \lambda(v)^2 (1-12c)^2.
$$
Therefore there are at most 
$$
\cPi (13+12c)^2/ (1-12c)^2 \leq k := \cPi 14^2,
$$
such triangles, and the edge $e$ is thus cut in at most $k$ parts by the edges joining an extremal vertex in $\cV$ to the corresponding vertex in $\cV_0$.

Hence there are at most $3k$ vertices of $\cT'$ on the three edges of a triangle $T\in \cT$ (including the vertices of $T$).
Since any conforming triangulation of convex envelope of $n+2$ points uses $n$ triangles, we obtain that $\cT'$ is a $3k-2$ refinement of $\cT$.
\sq

\input{../Bibliography/Bibliography.tex}
\end{document}



==> MeshMetric/MeshMetricTheseOld4.tex <==
\input{../PreambleThese}

\section{Introduction}

Triangulations and meshes are finite objects of combinatorial nature: they can be described by a collection of vertices and of connection between these. This description is fruitful for the demonstration of algebraic results, such as the Euler formula, or for computer processing.
In contrast, many approaches towards anisotropic mesh generation are based on a continuous object, namely a riemannian metric $z\mapsto H(z)$, in other words a continuous function $H$ from the domain $\Omega\subset \R^d$ to the set $S_d^+$ of symmetric positive definite matrices. Once this metric has been properly designed, it is the task of a mesh generation algorithm such as \cite{Shew,Bois,FreeFem,Inria} to generate a triangulation that agrees with this metric, in a sense specified below \iref{defEquiv}.
The purpose of this chapter is to formulate precise equivalence results between some classes of triangulations and of riemannian metrics. This equivalence translates some geometrical constraints satisfied by the triangulations into the form of regularity properties of the equivalent riemannian metrics.\\

Our results are so far limited to meshes and metrics defined on the entire infinite domain $\R^d$, and the dimension $d\geq 2$ is fixed throughout this chapter. 
The choice of the unbounded domain $\R^d$ guided by simplicity, since the curvature and the singularities of
of the boundary $\partial\Omega$ induces additional difficulties 
from the point of view of computational mesh generation.
Bounded domains will be the object of future work.
We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$, and we introduce in \S\ref{subsecDefTStar} three embedded subsets of $\bT$ of particular interest 
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
where $C\geq 1$ is a parameter which plays a minor role.
The set $\bT_{i,C}$ collects all \emph{isotropic} meshes $\cT$ which are heuristically defined as follows: the simplices $T\in \cT$ may have strongly varying volumes, but their aspect ratio is uniformly bounded. 
The largest set $\bT_{g,C}$ collects \emph{graded} meshes, which only satisfy a condition of local consistency: all the  geometrical features of the simplices $T\in \cT$ may vary strongly, volume, aspect ratio and orientation, but two \emph{neighboring} simplices should not be excessively different.
The intermediate set $\bT_{a,C}$ collects \emph{quasi-acute} meshes, which definition involves the measure of sliverness $S(T)$ of a simplex $T$ introduced in Chapter \ref{chapW1P} and also discussed in Chapter \ref{chapApproxMet}. 
The measure of sliverness plays an important role in the finite element approximation of a function on a mesh $\cT$ when the error is measured in the Sobolev $W^{1,p}$ norm.\\

We associate to each simplex $T$ a symmetric positive definite matrix $\cH_T$ such that the ellipsoid
$$
\cE_T := \{z\in \R^d \sep (z-z_T) \cH_T (z-z_T)^\trans \leq 1\},
$$
which is centered at the barycenter $z_T$ of $T$,
is the ellipsoid of minimal volume containing $T$. The properties of the matrix $\cH_T$ are discussed in \S \ref{subsecIntroSimplex} of this introduction,  as well as its explicit expression in terms of the coordinates of the simplex $T$. The matrix $\cH_T\in S_d^+$ encodes the volume, the aspect ratio and the orientation (but not the angles) of the simplex $T$. Two triangles $T$ and their associated ellipses $\cE_T$ are illustrated on figure \ref{figET}.

\begin{figure}
\centering
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleAigu.pdf}
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleObtus.pdf}
	\caption{Two triangles $T$ and their associated ellipse $\cE_T$.\label{figET}}
\end{figure}

A riemannian metric on $\R^d$ is a continuous map $H$ which associates to any $z\in \R^d$ a symmetric positive definite matrix $H(z)\in S_d^+$. We denote by $\bH = C^0(\R^d,S_d^+)$ the collection of riemannian metrics.
The following definition introduce a notion of equivalence between meshes and metrics
\begin{definition}
\label{defEqHT}
We say that a mesh $\cT\in \bT$ is $C_0$-equivalent to a given metric $H\in \bH$, where $C_0\geq 1$ is a fixed constant, if for all $T \in \cT$ and all $z\in T$ one has 
\be
\label{defEquiv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
\ee
We say that a collection of simplicial meshes $\bT_*\subset \bT$ is equivalent to a collection $H_*$ of metrics if there exists a uniform constant $C_0\geq 1$ such that the following holds:
\begin{itemize}
\item For any mesh $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\item For any metric $H\in \bH_*$ there exists a mesh $\cT\in \bT_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\end{itemize}
\end{definition}
Our main result (Theorem \ref{thEquiv}) states that when the constant $C$ is sufficiently large, and if dimension is $d=2$, the three classes of meshes $\bT_{i,C}\subset \bT_{a,C} \subset \bT_{g,C}$ are respectively equivalent to three classes of metrics
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
that are defined by precise smoothness conditions on the function $z\mapsto H(z)$ in \S \ref{subsecDefHStar} of this introduction.
%Our main result Theorem \ref{thEquiv} states that when the parameter $C$ is large enough and the dimension is $d=2$, the collections $\bT_{\star,C}$ of triangulations are equivalent to the corresponding collections $H_\star$ of metrics for any symbol $\star \in \{i,a,g\}$. 
The most striking point of this result is that, although the matrix $\cH_T$ does not encode the angles of a simplex $T$, the fact that a mesh $\cT\in \bT_{a,C}$ is \emph{quasi-acute} can be translated in a precise regularity condition on the metric $H$ equivalent to $\cT$.

In order to state our results more precisely we need to introduce some notations. We first recall some notations of linear algebra. We denote by $\M_d$ the collection of $d\times d$ matrices with real entries. We denote by $\GL_d$ the standard linear group, by $\SL_d$ the special linear group and by $\cO_d$ the orthogonal group
\begin{eqnarray*}
\GL_d &:=& \{A\in \M_d\sep \det A\neq 0\}\\
\SL_d &:=& \{A\in \M_d\sep \det A=1\}\\
\cO_d &:=& \{U\in \M_d\sep U^\trans U = \Id\}.
\end{eqnarray*}
We denote by $S_d$ the collection of symmetric matrices, by $S_d^\oplus$ the subset of non-negative symmetric matrices, and by $S_d^+$ the collection of symmetric positive definite matrices.
\begin{eqnarray*}
S_d &:=& \{M\in \M_d\sep M = M^\trans\}\\
S_d^\oplus &:=& \{M\in S_d\sep z^\trans M z \geq 0 \text{ for all } z\in \R^d\}\\
S_d^+ &:=& S_d^\oplus \cap \GL_d.
\end{eqnarray*}
Let $M,M'\in S_d$, we write $M\leq M'$ if $M'-M\in S_d^\oplus$, and $M< M'$ if $M'-M\in S_d^+$. We recall that for any $M,M'\in S_d$ such that $M\leq M'$ and any $\phi\in \M_d$ we have $\phi^\trans M \phi \leq \phi^\trans M' \phi$. Furthermore if $M,M' \in S_d^+$ and $M\leq M'$ then $M'^{-1} \leq M^{-1}$. For each symmetric positive definite matrix $M\in S_d^+$ we define a norm $\|\cdot\|_M$ as follows: for all $u\in \R^d$
$$
\|u\|^2_M := u^\trans M u.
$$

\subsection{Geometry of the simplex}
\label{subsecIntroSimplex}
The basic geometrical object studied in this chapter is the $d$-dimensional simplex, which is defined as follows.
\begin{definition}
A $d$-dimensional simplex $T$ is the convex envelope of a set $V\subset \R^d$ of $d+1$ %non-coplanar 
vertices, not contained in a $d-1$ dimensional affine subspace of $\R^d$ : 
$$
T = \Cvx(V).
$$
We denote by $\cF(T)$ the collection of faces of $T$ of any dimension,
\be
\label{defFT}
\cF(T) := \{\Cvx(V') \sep V'\subset V\}.
\ee
\end{definition}
Observe that $\emptyset$ and $T$ are among the faces of a simplex $T$, since they respectively correspond to $V'=\emptyset$ and $V'=V$.
We denote by $z_T\in \R^d$ the barycenter of a simplex $T$ of vertices $V$
$$
z_T := \frac 1 {d+1} \sum_{v\in V} v,
$$
and we define a symmetric positive definite matrix $\cH_T\in S_d^+$ as follows
\be
\label{defcH}
\cH_T^{-1} = \frac d {d+1} \sum_{v\in V} (v-z_T) (v-z_T)^\trans. %\frac {2d}{(d+1)^2}\sum_{v,v'\in V} (v-v')(v-v')^\trans. 
\ee
Some of the key properties of the matrix $\cH_T$ are exposed in the next proposition.
Throughout this chapter, we denote by $\TEq$ a $d$-dimensional equilateral simplex, centered at the origin
i.e. such that $z_\TEq=0$, and having its vertices on the unit ball. One easily checks that 
$$
\cH_\TEq = \Id.
$$
% Note that 
%\be
%\label{eqBallTEq}
%%\{z\in \R^d \sep |z| \leq 1/d\} 
%B(0, 1/d) \subset \TEq \subset \overline B(0,1).
%\ee
%
%%We associate to any simplex $T$ its barycenter $z_T\in \R^d$, and a symmetric positive definite matrix
%We denote by $z_T$ the barycenter of a simplex $T$, and we also associate to $T$ a symmetric positive definite matrix $\cH_T\in S_d^+$ which encodes some of its geometrical properties, in particular the volume, the elongation and the orientation of $T$.
\begin{prop}
\label{propHT}
The following holds for any $d$-dimensional simplex $T$. 
\begin{itemize}
\item
For any an affine change of coordinates $\Phi$, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0$ in $\R^d$, we have 
\be
\label{invcH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
\item
There exists a rotation $U\in \cO_d$, depending on $T$, such that 
\be
\label{eqcHTEq}
\cH_T^\frac 1 2 (T-z_T) = U(\TEq),
\ee
hence 
\be
\label{eqVolTHT}
|T| \sqrt{\det \cH_T} = |\TEq|.
\ee
\item
We have the inclusions 
\be
\label{eqTET}
\{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1/d\} \subset T \subset \cE_T := \{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1\},
\ee
and the these two ellipsoids are respectively the one of largest volume included in $T$, and of smallest volume containing $T$.
\end{itemize}
\end{prop}
\proof
For any simplex $\Phi^{-1}(v)$ of the simplex $\Phi^{-1}(T)$, we have 
$$
\Phi^{-1}(v)-z_{\Phi^{-1}(T)} = \Phi^{-1}(v)-\Phi^{-1}(z_T) = \phi^{-1}(v-z_T).
$$
Injecting this relation in \iref{defcH} we obtain \iref{invcH}. 
We now turn to the proof of \iref{eqcHTEq} and for that purpose we remark that the simplices $\TEq$ and $T' := \cH_T^\frac 1 2 (T-z_T)$ have both their barycenter at zero, $z_\TEq = z_{T'} = 0$, hence there exists a linear map $\phi\in \GL_d$ such that $T' = \phi^{-1}(\TEq)$. We thus obtain, using the formula \iref{invcH} for the transformation of $\cH_T$ under affine change of coordinates 
$$
\begin{array}{ccccc}
\cH_{T'} &=& \cH_T^{-\frac 1 2} \cH_T \cH_T^{-\frac 1 2} &=& \Id \\ 
\cH_{\phi^{-1}(\TEq)} &=& \phi^\trans \cH_\TEq &=& \phi^\trans \phi.
\end{array}
$$
Hence $\phi^\trans \phi= \Id$ which establishes that $\phi\in \cO_d$ and concludes the proof of \iref{eqcHTEq}.
%One easily checks that 
%$$
%\overline B(0,1/d) \subset \TEq \subset \overline B(0,1),
%$$
%where
It is well known that the smallest ellipsoid containing $\TEq$ is the unit ball, and that the largest ellipsoid included in $\TEq$ is the ball of radius $1/d$. Combining this fact with the change of coordinates \iref{eqcHTEq} we obtain \iref{eqTET} which concludes the proof of this proposition.
\sq

Note that for any simplex $T$ and any $z,z'\in T$ we obtain using \iref{eqTET}
\be
\label{eqDiamTHT}
\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2.
\ee

We introduce a measure of degeneracy $\rho(T)$ of a $d$-dimensional simplex $T$
\be
\label{defRhoMM}
\rho(T) := \sqrt{\|\cH_T\| \|\cH_T^{-1}\|}.
\ee
%This measure of non degeneracy $\rho$ is slightly different from the measure of non degeneracy $\frac {\diam(T)^d} {|T|}$ used in some of the previous chapters. However these two measures play a similar role and can be compared. Indeed we obtain using \iref{eqVolTHT} and \iref{eqcTET}
%\be
%\label{eqRhoRhop}
%\frac{\rho(T)}{d^\frac d 2|\TEq|} \leq  \frac{(\|\cH_T^{-1}\|/d)^\frac d 2} {|\TEq| (\det \cH_T)^{-\frac 1 2}} \leq \frac{\diam(T)^d} {|T|} \leq \frac{\|\cH_T^{-1}\|^\frac d 2} {|\TEq|(\det \cH_T)^{-\frac 1 2}}\leq \frac{\rho(T)^{d-1}}{|\TEq|}.
%\ee
%Observing that $\|A\| \|A^{-1}\|^{-(d-1)} \leq |\det A| \leq \|A\|^{d-1} \|A^{-1}\|^{-1}$ for any $A\in \GL_d$
%it follows that 
Observe that $\rho(T)\geq 1$ for any simplex $T$, with equality if and only if $\cH_T$ is proportional to the identity, which implies in view of \iref{eqcHTEq} that $T$ is a displacement of the equilateral simplex $\TEq$:
$$
\rho(T) = 1 \stext{ if and only if }
%\ \Longleftrightarrow \ 
T = z_T+r U(\TEq) \text{ for some }  r>0 \text{ and } U \in \cO_d.
$$
The measure of degeneracy $\rho$ is slightly different from the measure of degeneracy $\frac {\diam(T)^d} {|T|}$ used in Chapters \ref{chapOptAniso} and \ref{chapW1P} but both have the same role: they are minimal for the equilateral simplex, and increase as the simplex becomes thinner.\\

The measure of sliverness $S(T)$ of a simplex $T$ is a quantity which plays an important role in the context of optimal mesh adaptation for the finite element approximation of a function in the Sobolev $W^{1,p}$ norm, see   \cite{Ba, Ja}, and Chapters \ref{chapW1P} and \ref{chapApproxMet}. 
This measure of sliverness is defined in Chapter \ref{chapW1P} and illustrated by several examples and equivalent quantities. We recall the definition of this quantity
\be
\label{defSMM}
S(T) := \inf \{ \|\phi\| \|\phi^{-1}\| \sep \phi \in \GL_d \text{ and } \phi(T) \text{ is acute } \},
\ee
a simplex is acute if the exterior normals $\n, \n'$ to any two distinct faces of $T$ have a negative scalar product $\<\n,\n'\>\leq 0$.
As observed in Chapter \ref{chapW1P}, the measure of sliverness $S(T)$ can be interpreted as the distance from $T$ to the collection of acute simplices.

The exterior normals $\n,\n'$ to any two $d-1$-dimensional faces of $\TEq$ satisfy $\<\n,\n'\> =-1/d$, hence this simplex is acute. Recalling \iref{eqcHTEq}
 we thus obtain for any simplex $T$
$$
S(T) \leq \rho(T).
$$
Apart from this upper bound, the matrix $\cH_T$ does not contain any direct information on the measure of sliverness $S(T)$.
%One of the key results of this chapter is that in a bidimensional triangulation $\cT$, and conjecturedly in higher dimension too, the variation of the matrix $\cH_T$ as $T$ varies in $\cT$ does encode the measure of sliverness in some sense.
For any bidimensional triangle $T$ of largest angle $\theta$, Proposition \ref{propSTan} of Chapter \ref{chapW1P} states that :
$$
S(T) = \max\left\{1, \tan \frac \theta 2 \right\}.
$$

\subsection{Simplicial meshes}
\label{subsecDefTStar}

As a starter, we recall the definition of a simplicial mesh of $\R^d$.
%We first briefly recall the defini
%Before introducing simplicial meshes, we briefly recall the definition of locally finite partitions of $\R^d$.

%In order to introduce q,xcl meshes 
\begin{definition}
\label{defSimplMesh}
A conforming simplicial mesh of $\R^d$ is a collection $\cT$ of simplices which satisfy the conformity axiom :  for all $T,T'\in \cT$
\be
\label{confAxiom}
T\cap T' \in \cF(T) \cap \cF(T'),
\ee
as well as the following properties
\begin{itemize}
\item (Covering) The simplices $T\in \cT$ cover the whole infinite domain $\R^d$:
$$
\bigcup_{T\in \cT} T = \R^d.
$$
\item (Partition) The interiors of the simplices $T\in \cT$ are pairwise disjoint: for any $T,T'\in \cT$,
$$
\interior (T) \cap \interior(T') \neq \emptyset\stext{ implies }  T=T'. %
$$
\item (Local finiteness) For any compact set $K \subset \R^d$, only a finite collection of simplices $T\in \cT$ intersect $K$:
$$
\{T \in \cQ \sep K \cap T \neq \emptyset \} \ \text{ is finite.}
$$
\end{itemize}
\end{definition}
The conformity axiom \iref{confAxiom} states that the intersection of any two simplices in $\cT$ needs to be a full common face.We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$.

For an optimal efficiency, numerous numerical simulation software use anisotropic meshes, in which the simplices may have an arbitrary shape. Anisotropic meshes are used for instance, to create a thin layer of simplices close to a geometric feature which is relevant in a numerical simulation.
In order to avoid excessively wild meshes, one often requires relevant  some consistency between the shapes of neighboring simplices.We therefore introduce for any constant $C \geq 1$ the class $\bT_{g,C} \subset \bT$ of \emph{graded} meshes, which is defined as follows.
A mesh $\cT$ belongs to $\bT_{g,C}$ if for any two simplices $T,T'\in \cT$ one has 
\be
\label{defTG}
T \cap T'\neq \emptyset \stext{ implies } C^{-2}\cH_T \leq \cH_{T'} \leq C^2 \cH_T.
\ee

For any $C\geq 1$ we also introduce the class $\bT_{i,C}$ of \emph{isotropic} meshes, by requiring that in addition to \iref{defTG} that the measure of degeneracy $\rho$ is uniformly bounded by $C$, which forbids any anisotropy.
A mesh $\cT$ belongs to $\bT_{i,C}$ if and only if $\cT\in \bT_{g,C}$ and for all $T \in \cT$
$$
\rho(T) \leq C. %C \geq 1? or 0? 
$$

%The next proposition shows that the definition of $\bT_{i,C}$ is slightly redundant, in the sense that condition \iref{defTG} could be avoided.
%\begin{prop}
%Denote by $\bT'_{i,C}$ the collection of meshes $\cT\in \bT$ satisfying $\rho(T) \leq C$ for all $T\in \cT$ (but perhaps not the gradedness condition \iref{defTG}). %We thus have $\bT_{i,C} \subset \bT'_{i,C}$.\\
%Then for all $C$ there exists $C' = C'(C)$ such that 
%$$
%\bT_{i,C} \subset \bT'_{i,C} \subset \bT_{i,C'}.
%$$
%\end{prop}
%
%\proof
%See appendix. 
%\sq

In order to introduce the intermediate collection $\bT_{a,C}$ of $C$-quasi-acute meshes, we first define the notion of refinement of a simplicial mesh.
\begin{definition}
Consider two meshes $\cT,\cT'\in \bT$ and a constant $C\geq 1$. We say that $\cT'$ is a $C$-refinement of $\cT$ if it satisfies the following properties.
\begin{itemize}
\item (Inclusion) Any simplex $T'\in \cT'$ is contained in a simplex $T\in \cT$. % such that $T'\subset T$.
\item (Bounded refinement) Any simplex  $T\in \cT$, contains most $C$ simplices $T'\in \cT$.
\end{itemize}
\end{definition}

A graded mesh $\cT \in \bT_{g,C}$ belongs to the collection $\bT_{a,C}$ of quasi-acute meshes if and only there exists a $C$-refinement $\cT'$ of $\cT$ which satisfies for all $T' \in \cT'$
$$
S(T') \leq C.
$$
In particular if $\cT\in \bT_{i,C}$, then choosing $\cT' = \cT$, which is a $C$-refinement since $C\geq 1$, and recalling that $S(T) \leq \rho(T)$ for any simplex $T$, we obtain that $\cT\in \bT_{a,C}$. Thus $\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}$ as announced.

The constraints defining graded, quasi-acute and isotropic meshes are illustrated on Figure \ref{figDisk}
in the main introduction of the thesis. 
Figure \ref{figAcuteGen} gives an example of a quasi-acute triangulation which 
by the above described refinement process leads to a slightly finer triangulation on
sliverness $S(T)$ is uniformly bounded.

\begin{figure}
\centering
%	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarGdeVap.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap1.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap2.pdf}
	\caption{\label{figAcuteGen}
Quasi-acute triangulation (left) and refined triangulation with uniformly bounded sliverness (right).
	}
\end{figure}

\subsection{Riemannian metrics}
\label{subsecDefHStar}

For any metric $H \in \bH$ and path $\gamma \in C^1([a,b],\R^d)$, we define the riemmannian length $l_H(\gamma)$ by the integral
$$
l_H(\gamma) := \int_a^b \|\gamma'\|_{H(\gamma(t))} dt.
$$
The riemmannian distance $d_H$ between two points  $z,z'\in \R^d$, is the infimum of the length of all paths joining $z$ and $z'$, 
\be
\label{defdH}
d_H(z,z') := \inf\left\{l_H(\gamma)\sep \gamma\in C^1\left([0,1],\R^d\right), \ \gamma(0) = z \text{ and } \gamma(1) = z'\right\}.
\ee
If $H, H'\in \bH$ are such that $H(z) \leq H'(z)$ for all $z\in \R^d$, then $d_H(z,z') \leq d_{H'}(z,z')$ for all $z,z'\in \R^d$.
By construction, the riemannian distance $d_H$ associated to a metric $H\in \bH$ is locally equivalent close to a point $z$ to the distance defined by the norm $\|\cdot \|_{H(z)}$: for all $z\in \R^d$
\be
\label{eqDistLoc}
\limsup_{\ve \to 0} \sup_{p,q\in B(z, \ve)} |\ln d_H(p,q) - \ln \|p-q\|_{H(z)}| = 0,
\ee
where $B(z,\ve)$ denotes the euclidean ball of radius $\ve$ around $z$.\\


\begin{remark}[Riemannian geodesics]
When a metric $H$ is sufficiently smooth, a special family of curves named Riemannian geodesics can be defined and studied. A riemannian geodesic is a curve $\gamma\in C^0(\R, \R^d)$ which satisfies a second order differential equation %written in terms of the second order derivatives of $H$, 
called the equation of geodesics. This equation implies that for any sufficiently close $t,t'\in \R$ the curve $\gamma_{|[t,t']}$ is the path of smallest possible length joining the points $\gamma(t)$ and $\gamma(t')$ : 
$d_H(\gamma(t), \gamma(t')) = l_H(\gamma_{|[t,t']})$.

Geodesics are not defined for general continuous or Lipschitz riemannian metrics, such as those constituting the sets $\bH$ and $\bH_i \subset \bH_a\subset \bH_g$, since the coefficients of the equation of geodesics involve the second derivatives of the metric. Notions related to geodesics, such as the injectivity radius of a metric, therefore have no meaning in our context.
This is not an issue for our purposes since, following the point of view of \cite{Gromov},
%[Gromov, Metric structures for Riemannian and non-Riemannian spaces, Birkhauser (1999)]
we study Riemannian distances and not Riemannian geodesics. 

%Note also that geodesics only exist when the metric $H$ has requires that $H$ has at least $C^2$ smoothness, while the metrics studied in this chapter generally only have $C^0$ or Lipschitz smoothness.

%Since we only assume that $H$ is a continuous metric, the infimum \iref{defdH} may or may not be attained, and in that later case possibly for several paths. The equation of geodesics associated to a riemannian metric involves the second order derivatives, which are not defined in our context.
%(* also the point of view of Gromov : we study distances and not geodesics*)
\end{remark}


We denote by $\bH_i$ the collection of metrics $H \in \bH$ which are proportionnal to the identity: for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2},
$$
and such that the proportionality factor $s$ satisfies one of the two following conditions conditions, which are surprisingly equivalent as shown in Proposition \ref{propEquivS}:
\begin{itemize}
\item (``Additive'' Lipschitz condition)  
\be
\label{eqLipSAdd}
|s(z) - s(z')| \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
\item (``Multiplicative'' Lipschitz condition)
\be
\label{eqLipSMult}
|\ln s(z) - \ln s(z')| \leq d_H(z,z') \stext{ for all } z,z'\in\R^d.
\ee
\end{itemize}

The two Lipschitz properties \iref{eqLipSAdd} and \iref{eqLipSMult} have a natural generalisation to general anisotropic metrics but are not equivalent in that context.
In order to introduce the regularity conditions defining the classes $\bH_i\subset \bH_a\subset \bH_g$ of metrics, we need to  two distances $d_\times$ and $d_+$ on the set $S_d^+$ of symmetric positive definite matrices. 
For any $M,M'\in S_d^+$ we define
\be
\label{defDTimes}
d_\times (M,M') := \min \{\delta \geq 0 \sep e^{-2\delta} M \leq M' \leq e^{2 \delta} M\}.
\ee
For instance, a mesh $\cT$ is $C$-equivalent to a metric $H$, as defined in \iref{defEquiv}, if and only if for all $T \in \cT$ and all $z\in \cT$ one has 
$$
d_\times (H(z), \cH_T) \leq \ln C.
$$
There exists various expressions of the distance $d_\times$ : for all $M,M'\in S_d^+$ one has 
\be
\label{eqDTimesLog}
d_\times (M,M') = \sup_{u\in \sR^d\sm \{0\}} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
\ee
and 
\be
\label{eqDTimesProd}
d_\times (M,M') = \ln \left(\max \{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\}\right).
\ee
The exponential of the distance $d_\times$ was used in the earlier paper \cite{Shew} %on anisotropic mesh generation
under the name ``relative deformation''. 
We define a second distance $d_+$ on $S_d^+$ as follows 
\be
\label{defDPlus}
d_+(M,M') := \|M^{-\frac 1 2} - M'^{-\frac 1 2}\|.
\ee
The expressions \iref{eqDTimesProd} and \iref{defDPlus} of the distances $d_\times$ and $d_+$ show that they are respectively tied to multiplicative or additive properties of matrices, which justifies their notations.
Note also that for any $s,s'>0$ one has
\be
\label{eqDIso}
d_\times (s^{-2} \Id, s'^{-2} \Id) = |\ln s - \ln s'| \stext{ and } d_+(s^{-2} \Id, s'^{-2} \Id) = |s-s'|.\\
\ee

We denote by $\bH_g$ the collection of metrics $H\in \bH$ which satisfy the natural extension of \iref{eqLipSMult} to general anisotropic metrics:
\be
\label{eqLipMult}
d_\times (H(z), H(z')) \leq d_H(z,z') \stext{ for all }z,z'\in\R^d.
\ee
This condition can be heuristically described as follows: a metric $H\in \bH$ defines close to each point $z\in\R^d$ a norm $\|\cdot\|_{H(z)}$ which encodes an anisotropic notion of scale. The equation \iref{eqLipMult} states that the metric $H$ itself is consistent a the scale that it encodes.\\

We denote by $\bH_a$ the collection of metrics $H\in \bH$ which satisfy both \iref{eqLipMult} and the natural extension of \iref{eqLipSAdd} to general anisotropic metrics:
\be
\label{eqLipAdd}
d_+ (H(z), H(z')) \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
In addition to the results of mesh generation presented in this chapter, we show in the next chapter, Chapter\ref{chapApproxMet}, that this condition is critical in order to define a local averaging operator compatible with Sobolev norms. 
%decrire le lien avec les angles aigus.
\begin{remark}
\label{remHomog}
Let $H\in \bH$, and let $\lambda>0$. Using the homogeneity properties of the distances $d_\times$, $d_+$ on $S_d^+$ and $d_H$ on $\R^d$ with respect to $H$, we obtain that $\lambda^2 H\in \bH_g$ if and only if 
\be
\label{eqLipTimesLambda}
d_\times (H(z), H(z')) \leq \lambda d_H(z,z') \stext{ for all } z,z'\in \R^d, 
\ee
and $\lambda^2 H\in \bH_a$ if and only if we have in addition to the previous property 
\be
\label{eqLipPlusLambda}
d_+ (H(z), H(z')) \leq \lambda |z-z'| \stext{ for all } z,z'\in \R^d.
\ee
In particular the collections $\bH_i \subset \bH_a \subset \bH_g$ of isotropic, quasi-acute and graded metrics are stable under multiplication by a constant larger than one : for any $\star \in \{a,b,c\}$, any $H\in \bH_\star$ and any $\lambda \geq 1$ we have $\lambda^2 H\in \bH_\star$.
%this operation corresponds to the uniform refinement of a triangulation...
\end{remark}

\subsection{Main results}

The main result of this chapter is the equivalence of the classes of meshes and metrics defined above, which is  announced in the first part of the introduction and proved in sections \S\ref{secMeshToMet} and  \S \ref{secMetToMesh}. In two cases we were only able to establish this equivalence when the dimension is $d=2$. 
\begin{theorem}
\label{thEquiv}
There exists $C_0 = C_0(d)$ such that for all $C\geq C_0$ the following holds.
\begin{enumerate}[i)]
\item The collections $\bT_{i,C}$ of triangulations and $\bH_i$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{a,C}$ of triangulations and $\bH_a$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{g,C}$ of triangulations and $\bH_g$ of metrics are equivalent.
\end{enumerate}
\end{theorem}

Let us comment on this result.
The theory of isotropic meshes is already well developed, and our result i) in this direction should be regarded as a reformulation of previous work, intended to put into perspective the results on anisotropic meshes. The main ingredient of the proof of i) is the mesh refinement procedure exposed in \cite{Nochetto}. 

In the case iii) of graded metrics the key ingredients used for the construction of a bidimensional triangulation $\cT\in \bT_{g,C}$ equivalent to a metric $H \in \bH_g$ come from the paper of computational geometry \cite{Shew}. In contrast the arguments used to produce a metric $H \in \bH_g$ from a mesh $\cT \in \bH_{g,C}$ hold in any dimension.

Last the author has not heard of any anterior results on the collection $\bT_{a,C}$ of quasi-acute meshes, and most of the techniques used in that context are new. 
The author is sorry to say that the proofs in that case are not yet as polished as the rest of the thesis, due to time constraints.

\begin{conjecture}
The author conjectures that the points ii) and iii) of Theorem \ref{thEquiv} holds without restriction on the dimension $d$.
\end{conjecture}

This chapter is organised as follows. We establish in section \S \ref{secMetProp} some general properties of metrics in $\bH_a$ or $\bH_g$. 
We first prove in \S\ref{subsecMetInv} a property of invariance of the collection $\bH_g$ of graded metrics with respect to affine changes of coordinates.
The regularity assumptions \iref{eqLipMult} and \iref{eqLipAdd} defining graded and quasi-acute metrics simply mean that the map $H : \R^d \to S_d^+$ is Lipschitz with respect to some distances on $\R^d$ and $S_d^+$. 
We therefore study metrics from this point of view in \S\ref{subsecMetLip}.
We focus in \S\ref{subsecMetGeom} on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. In particular we compare the $d_H$ with the euclidean distance and we estimate the volume of balls. 


Section \S\ref{secEigen} is devoted to the study of metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has  an eigenspace of dimension at least $d-1$ at each point. This condition clearly holds if the dimension is $d=2$ but is also relevant in some applications to higher dimension such as the creation of a this layer of simplices close to a $d-1$ dimensional surface. This situation is discussed in Chapter \ref{chapApproxMet}, and involves metric which have an eigenvalue much larger that the others in the orthogonal direction to the surface of interest.
We give an approximate translation of the regularity properties \iref{eqLipAdd} and \iref{eqLipMult} defining the collections $\bH_a$ and $\bH_g$ of metrics in terms of the two eigenvalues of $H$ and of the direction of the eigenspaces of such metrics. 

The last two sections \S\ref{secMeshToMet} and \S\ref{secMetToMesh} are devoted to the proof of Theorem \ref{thEquiv}. More precisely we adress in \S\ref{secMetToMesh} the production of an isotropic, quasi-acute or graded mesh equivalent to a given metric $H\in \bH_i$, $\bH_a$ or $\bH_g$. Conversely we depict in \S\ref{secMeshToMet} to construction of a metric which is equivalent to a given mesh.


\section{General properties of graded and quasi-acute metrics}
\label{secMetProp}

We study in this section the general properties of the  distinguished classes of metrics $\bH_i \subset \bH_a \subset \bH_g$. 
We first establish in \S\ref{subsecMetInv} some invariance properties of these collections of metrics with respect to affine changes of coordinates.
We then regard in \S\ref{subsecMetLip} metrics as Lipschitz functions $H : \R^d\to S_d^+$. %, and we recall some basic properties of these.
The last subsection \S\ref{subsecMetGeom} is devoted to the comparison of the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$, with respect to the standard euclidean distance and Lebesgue measure.

\subsection{Invariance properties and restriction of metrics}
\label{subsecMetInv}

We focus in this subsection on the properties of invariance of the collections of meshes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ and of metrics $\bH_i \subset \bH_a\subset \bH_g$ introduced in this chapter.

Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$.
We have for any simplex $T$, as previously observed in \iref{invcH},
\be
\label{eqInvH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
Mimicking this property we define for any $H \in \bH$ a transported version $H_\Phi\in \bH$ as follows: for all $z\in \R^d$
\be
\label{defHPhi}
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi.
\ee
In the language of differential geometry,
the metric $H_\Phi$ is generally referred to as the ``pull back'' of $H$ by $\Phi$. If a mesh $\cT\in \bT$ is $C$-equivalent to a metric $H\in \bH$, then \iref{eqInvH} and \iref{defHPhi} clearly imply that the mesh $\Phi^{-1}(\cT)$ is $C$-equivalent to the metric $H_\Phi$.

The next proposition studies the invariance of the collections $\bT_{\star,C}$ of meshes and $\bT_\star$ of metrics, $\star \in \{i,a,g\}$, under the transformations $\cT \mapsto \Phi^{-1}(\cT)$ or $H \mapsto H_\Phi$ induced by an affine change of coordinates $\Phi$.

\begin{prop}
\label{propInvT}
Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. 
The following holds for any constant $C\geq 1$.
\begin{enumerate}[i)]
\item If $\cT \in \bT_{g,C}$ then $\Phi^{-1}(\cT) \in \bT_{g,C}$. If $H \in \bH_g$ then $H_\Phi\in \bH_g$.
\item Assume that $\Phi$ is an isometry, in other words $\phi\in \cO_d$.\\
If $\cT\in \bT_{a,C}$ then $\Phi^{-1}(\cT)\in \bT_{a,C}$, and similarly if $\cT\in \bT_{i,C}$ then $\Phi^{-1}(\cT)\in \bT_{i,C}$.\\
If $H\in \bH_a$ then $H_\Phi\in \bH_a$, and similarly if $H\in \bH_i$ then $H_\Phi\in \bH_i$.
\end{enumerate}
\end{prop}

\proof
%We concentrate on the case of meshes, since the statements on metrics are a special case of the propositions (??) and (??) below (* no : state the result for iso and quasi acute metrics too*).
%We first consider the case of meshes, and then 
We first establish the properties announced for meshes, and we then focus on metrics.
Let $M,M'\in S_d^+$, let $C\geq 1$ and let $\phi\in \GL_d$. Clearly
$$
\text{ if } C^{-2} M \leq M' \leq C^2 M \stext{ then } C^{-2} \phi^\trans M\phi \leq \phi^\trans M'\phi  \leq C^2 \phi^\trans M\phi.
$$
%Consequently if a mesh $\cT$ satisfies the condition \iref{defTG} defining the elements of $\bT_{g,C}$
%
%satisfy $C^{-2} M \leq M' \leq C^2 M$, then we also ha
%For any $M,M'\in S_d^+$ we obtain using \iref{defDTimes} that 
%$$
%d_\times (\phi^\trans M \phi,\ \phi^\trans M' \phi) = d_\times (M,M').
%$$
%It follows using \iref{eqInvH} that for any  two simplices $T,T'$,
%$$
%d_\times (\cH_{\Phi^{-1}(T)}, \cH_{\Phi^{-1}(T')}) = d_\times (\cH_T,\cH_{T'}).
%$$ 
In view of the definition \iref{defTG} of $\bT_{g,C}$ we obtain that $\Phi^{-1}(\cT)\in \bT_{g,C}$ for any mesh $\cT\in\bT_{g,C}$ as announced in i).

If $\Phi$ is an isometry then for any simplex $T$ we obtain, using the definitions \iref{defRhoMM} and \iref{defSMM} of the measure of degeneracy $\rho$ and the measure of sliverness $S$, that
$$
\rho(\Phi^{-1}(T)) = \rho(T) \stext{ and } S(\Phi^{-1}(T)) = S(T).
$$
This implies the properties of $\bT_{a,C}$ and $\bT_{i,C}$ announced in b), which concludes the proof of the properties announced for meshes.

We therefore turn our attention to metrics. The fact that $H_\Phi\in \bH_g$ for any $H\in \bH_g$ and any affine change of coordinates $\Phi$ is a special case of Proposition \ref{propHG} below. We thus admit this property and we focus on isotropic and graded metrics and isometric changes of coordinates.

If $H\in \bH_i$, then $H = \Id/s(z)^2$ where $s: \R^d \to \R_+^*$ is a Lipschitz function. Since $\phi\in \cO^d$ we have $\phi^\trans \phi = \Id$ and therefore 
$$
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi = \Id/s(\Phi(z))^2.
$$
The map $s \circ \Phi : \R_d\to \R_+^*$ is Lipschitz since it is the composition of a Lipschitz function with an isometry, which establishes that $H_\Phi\in \bH_i$ as announced.

If $H\in \bH_a$ and $\Phi$ is an isometry, then for any $z,z'\in \R^d$
\begin{eqnarray*}
\|H_\Phi(z)-H_\Phi(z')\| &=& \|\phi^\trans \left(H(\Phi(z))-H(\Phi(z'))\right) \phi\| \\
&=& \|H(\Phi(z))-H(\Phi(z'))\|\\
& \leq& \|\Phi(z)-\Phi(z')\|\\
& =& \|\phi(z-z')\|= |z-z'|,
\end{eqnarray*}
which establishes that $H_\Phi$ satisfies the Lipschitz regularity condition \iref{eqLipAdd}. We already know from the case of graded metrics that the other regularity condition \iref{eqLipMult} is satisfied by $H_\Phi$, which establishes that $H_\Phi\in \bH_a$ and concludes the proof of this proposition.
\sq


In practical applications, one often needs to mesh simultaneously a domain $\Omega$ and a surface $\Gamma$ embedded in $\Omega$. In terms of metric this raises the following question: given a metric $H$ on $\Omega$ which satisfies certain properties of regularity %, corresponding do a certain class of meshes, 
what is the regularity of the restriction of this metric to $\Gamma$?

The next proposition answers this question is the simplified setting where $\Omega$ is the infinite domain $\R^d$, $\Gamma$ is an affine subspace of $\R^d$, and properties of regularity are those defining the collection $\bH_g$ of graded metrics. For any $1\leq k \leq d$ we denote by $\bH_g(\R^k)$ the collection of graded metrics on $\R^k$.

\begin{prop}
\label{propHG}
Let $1\leq k\leq d$, let $\Phi : \R^k\to \R^d$ be an affine injective map, $\Phi(z) = \phi z+z_0$ where $\phi\in M_{d,k}$ has rank $k$ and $z_0\in \R^d$. Let $H\in \bH$ and let for all $z\in \R^k$
$$%\be
%\label{defHPhi}
H_\Phi(z) := \phi^\trans H(\Phi(z)) \phi.
$$%\ee
If $H\in \bH_g$ then $H_\Phi\in \bH_g(\R^k)$. 
\end{prop}

\proof
For any $u\in \R^d$, one has 
\be
\label{chgNorm}
\|u\|_{H_\Phi(z)} = \|\phi(u)\|_{H(\Phi(z))}.
\ee
Hence for any $z,z'\in \R^k$ we obtain using \iref{eqDTimesLog},
\be
\label{dNHPhi}
\begin{array}{rcl}
d(H_\Phi(z), \ H_\Phi(z'))  &=&\displaystyle \sup_{u\in \sR^k\sm\{0\}} \left|\ln \left\|\phi(u)\right\|_{H(\Phi(z))} -\ln \left\|\phi(u)\right\|_{H(\Phi(z'))}\right| \\
& \leq& d(H(\Phi(z)), \  H(\Phi(z')))
\end{array}
\ee
For any path $\gamma\in C^1([0,1], \R^k)$, it follows from \iref{chgNorm} that % the distorted lengths tied to $H$ and $H_\phi$ are therefore linked by 
$$
l_H(\Phi\circ \gamma) = \int_0^1 \|\phi(\gamma'(t))\|_{H(\Phi(\gamma(t)))}dt =  l_{H_\Phi}(\gamma).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^k)$ joining two points $z,z'\in \R^k$, we obtain since $\Phi\circ \gamma\in C^1([0,1], \R^d)$ is a path joining $\Phi(z)$ and $\Phi(z')$
\be
\label{dHPhi}
d_H(\Phi(z), \Phi(z')) \leq d_{H_\Phi}(z,z')
\ee
Combining \iref{dNHPhi} and \iref{dHPhi}, we conclude the proof of this proposition.
\sq


\subsection{Metrics as Lipschitz functions}
\label{subsecMetLip}
Lipschitz functions play an important role in this chapter and in particular in this section. We recall here their basic properties.
If $(X,d_X)$ and $(Y,d_Y)$ are two metric spaces, and if $f \in C^0(X , Y)$, we define 
the dilatation $\dil(f) \in [0, \infty]$ of $f$ as follows
$$
\dil(f) := \sup_{\substack{x,x'\in X \\ x \neq x'}} \frac{d_Y(f(x),f(x'))}{d_X(x,x')}
$$

We say that $f$ is Lipschitz if $\dil(f) \leq 1$, and more generally that $f$ is $\lambda$-Lipschitz if $\dil(f) \leq \lambda$.
We define the local dilatation $\dil_x(f)$ of a function $f\in C^0(X,Y)$ at a point $x\in X$ as follows
\be
\label{defDilX}
\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
\lim_{\ve\to 0} \left(\sup_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
\ee
%\be
%\label{defDilX}
%\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
%\lim_{\ve\to 0} \left(\sup_{e,e'\in B(x,\ve)} \frac{d_Y(f(e),f(e'))}{d_X(e,e')}\right).
%\ee
We specify the distance function on $X$ or $Y$ if it is not the expected ``canonical one'', in particular if $X$ or $Y$ is a subset of $\R^k$ and if the associated distance is not the standard euclidean distance but the riemannian distance $d_H$ associated to a metric, or if $X$ or $Y$ is the collection $S_d^+$ of symmetric positive definite matrices since none of the two distances $d_+$ or $d_\times$ is canonical. The local dilatation is in that case denoted as follows
$$
\dil_x(f\sep d_X, d_Y), \quad \dil_x(f\sep d_X)  \stext{ or } \dil_x(f\sep d_Y).
$$

The local dilatation $\dil_x(f)$ only depends on the local properties of the metric spaces close to $x$ and $f(x)$. Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$. For any $f\in C^0(\R^d, Y)$ and any $z\in \R^d$ we obtain using \iref{eqDistLoc}
\be
\label{eqDilNorm}
\|H(z)^{-1}\|^{-\frac 1 2} \dil_z(f) \leq \dil_z(f\sep d_H) = \dil_z(f \sep \|\cdot \|_{H(z)}) \leq \sqrt{\|H(z)\|} \dil_z(f)
\ee
We also introduce the lower local dilatation $\dil_z^*(f)\leq \dil_z(f)$ which is defined as follows
$$
\dil_z^*(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
$$
The next proposition establishes that local dilatations are sub-multiplicative.
\begin{lemma}
\label{lemmaSubMult}
Let $(X,d_X)$, $(Y,d_Y)$ and $(Z,d_Z)$ be three metric spaces, and let $f\in C^0(X,Y)$ and $g\in C^0(Y,Z)$. 
For any $x\in X$ one has 
\be
\label{eqDilUpper1}
\dil_x(g \circ f) \leq \dil_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side. Similarly we have 
\be
\label{eqDilLower1}
\dil_x(g \circ f) \geq \dil^*_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side.
\end{lemma}

\proof
We first establish \iref{eqDilUpper1}.
If $\dil_x(f) = \infty$ or $\dil_{f(x)}(g) = \infty$, then there is nothing to prove. We may therefore assume that $\dil_x(f) < \infty$ and $\dil_{f(x)}(g) < \infty$.
For any $\ve>0$ we define 
$$
F(\ve) = \sup_{p,q\in B(x, \ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)} \stext{ and } G(\ve) := \sup_{p,q\in B(f(x), \ve)} \frac{d_Z(g(p),g(q))}{d_Y(p,q)}
$$
It follows that 
$$
\sup_{p,q\in B(x, \ve)} \frac{d_Z(g(f(p)),g(f(q)))}{d_X(p,q)} \leq F(\ve) \, G(F(\ve) \ve).
$$
Taking the limit as $\ve \to 0$ we obtain \iref{eqDilUpper1} which concludes the proof.
For the proof of \iref{eqDilLower1} we consider two sequences $(p_n)_{n \geq 0}$, $(q_n)_{n \geq 0}$ which both tend to $x$ and such that $d_Y(f(p_n),f(q_n))/d_X(p_n, q_n) \to \dil_x(f)$ as $n \to \infty$. We thus have 
$$
\frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_X(p_n,q_n)} = \frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_Y(f(p_n),f(q_n))} \times \frac{d_Y(f(p_n),g(f(q_n)))}{d_X(p_n,q_n)},
$$
and taking the limit as $n \to \infty$ we obtain \iref{eqDilLower1} which concludes the proof of this lemma.
\sq

Let $f: \Omega \to V$ be a $C^1$ function, where $\Omega\subset \R^d$ is an open set and $V$ is a Banach space. Then for any $z\in \Omega$ the local dilatation $\dil_z(f)$, and the lower dilatation $\dil_z^*(f)$ only depend on the differential $d_z f : \R^d \to V$ of $f$ at $z$
\be
\label{eqDilDiff}
\dil_z(f) = \sup_{|u|=1} \|d_z f(u)\| \stext{ and } \dil_z^*(f) = \inf_{|u|=1} \|d_z f(u)\|
\ee
Applying Lemma \ref{lemmaSubMult} and \iref{eqDilDiff} to the function $g=\ln$ we obtain for any metric space $(X,d_X)$, any $f\in C^0(X,\R_+^*)$ and any $x\in X$
\be
\label{eqDilLog}
\dil_x(\ln f) = \frac {\dil_x(f)} {f(x)} .
\ee

The following proposition shows that, under certain circumstances, the Lipschitz property is a local property.
\begin{prop}
\label{propDilLoc}
Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$.
For any $f\in C^0(\R^d, Y)$ and any path $\gamma\in C^1([0,1], \R^d)$, $\gamma(0) = z$, $\gamma(1) = z'$, one has
\be
\label{eqLipLocPath}
d_Y(f(z), f(z')) \leq l_H(\gamma) \sup_{0\leq t \leq 1} \dil_{\gamma(t)}(f).
\ee
It follows that %In particular 
\be
\label{eqDilLoc}
\dil(f) = \sup_{z\in \sR^d} \dil_z(f).
\ee
\end{prop}

\proof
%Consider $z,z'\in \R^d$, and a path $\gamma\in C^1([0,1],\R^d)$ such that $\gamma(0) = z$, $\gamma(1)=z'$ and $l_H(\gamma) \leq d_H(z,z')+\delta$ where $\delta>0$ is a constant that is devoted to tend to zero in the last step of the proof.
We equip the segment $[0,1]$ with the distance $d_\gamma$ defined for $0 \leq t\leq t'\leq 1$ by 
\be
\label{defDGamma}
d_\gamma(t,t') = d_\gamma(t',t) = l_H(\gamma_{|[t,t']}).
\ee
Note that for any $t\leq t_* \leq t'$ one has 
\be
\label{exactTri}
d_\gamma(t,t') = d_\gamma(t,t_*)+d_\gamma(t_*,t')
\ee
The map $\gamma : ([0,1], d_\gamma) \to (\R^d, d_H)$ is clearly Lipschitz.
It thus follows from Lemma \ref{lemmaSubMult} that $F := f\circ \gamma :[0,1] \to Y$ satisfies for all $t\in [0,1]$
$$
\dil_t(F) \leq \dil_{\gamma(t)}(f) \leq \lambda := \sup_{0\leq t'\leq 1} \dil_{\gamma(t')}(f).
$$
We assume that $\lambda<\infty$, otherwise there is nothing to prove, and we consider a fixed $\delta>0$. For each $t\in [0,1]$ there exists therefore an interval $V_t\subset [0,1]$ containing $t$, relatively open in $[0,1]$, and such that $F_{|V_t}$ is $(\lambda+\delta)$-Lipschitz. Since the segment $[0,1]$ is compact, there exists a finite set $I_0\subset [0,1]$ such that 
$$
[0,1] = \bigcup_{t\in I_0} V_t.
$$
Let $V,V'\subset [0,1]$ be two intersecting intervals, and assume that $F$ is $\lambda+\delta$ Lipschitz on $V$ and on $V'$. For any $t\in V$ and $t'\in V'$, there exists $t_*\in V\cap V'$ which satisfies $t\leq t_*\leq t'$ or $t\geq t_* \geq t'$. Recalling \iref{exactTri} we thus obtain  
\begin{eqnarray*}
d_Y(F(t),F(t')) &\leq& d_Y(F(t), F(t_*))+d_Y(F(t_*), F(t')) \\
&\leq& (\lambda+\delta) d_\gamma(t,t_*)+( \lambda+\delta)d_\gamma(t_*,t') \\
&=& (\lambda+\delta)d_\gamma(t,t').
\end{eqnarray*}
Thus $F$ is $\lambda+\delta$ Lipschitz on the interval $V\cup V'$. Since $[0,1]$ is covered by a finite collection of open intervals on which $F$ is $\lambda+\ve$ Lipschitz, we obtain proceeding by induction that $F$ is $(\lambda+\delta)$-Lipshitz on $[0,1]$ and therefore 
$$
d_Y(f(z),f(z')) = d_Y(F(0),F(1))\leq (\lambda+\delta) d_\gamma(0,1) = (\lambda+\delta)l_H(\gamma). %\leq (\lambda+\delta)(d_H(z,z')+\delta).
$$
Letting $\delta\to 0$ we obtain \iref{eqLipLocPath}. Taking the infimum of \iref{eqLipLocPath} among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_Y(f(z),f(z')) \leq  \lambda d_H(z,z')$. Therefore $f : (\R^d, d_H) \to (Y,d_Y)$ is $\lambda$-Lipschitz, which concludes the proof of this proposition.
%The upper inequality $\geq$ is a direct consequence of the definition \iref{defDilX} of the local dilatation, and we therefore turn to the lower inequality $\leq$.
\sq

The next corollary shows that the global dilatation is controlled by the local dilatation even if the latter is not known on a \emph{sufficiently thin} set $\Gamma$, such as the skeleton of a mesh.

\begin{corollary}
\label{corolLipNoGamma}
Let $\Gamma\subset \R^d$ be a set which has the following property : for any path $\gamma\in C^1([0,1], \R^d)$ there exists a sequence of path $(\gamma_n)_{n \geq 0}$ which converge to $\gamma$ in $C^1$ norm and such that  $\{t\in [0,1]\sep \gamma_n(t) \in \Gamma\}$ is finite for each $n$.\\
Let $H\in \bH$, let $(Y,d_Y)$ be an arbitrary metric space, and met let $f\in C^0(\R^d, Y)$.
Then 
$$
\dil(f) = \sup_{z\in \R^d \sm \Gamma} \dil_z(f).
$$
\end{corollary}

\proof
We denote $\lambda := \sup_{z\in \R^d \sm \Gamma} \dil_z(f)$.
We consider two points $z,z'\in \R^d$ and a path $\gamma\in C^1([0,1], \R^d)$ such that $\gamma(0) = z$ and $\gamma(1) = z'$. %, and a sequence $\gamma_n$ converging to $\gamma$ in $C^1$ norm.

We first assume that the set $\{t\in [0,1]\sep \gamma(t) \in \Gamma\}$ is finite, and we denote its elements by $t_1< \cdots < t_k$. We set by convention $t_0 = 0$ and $t_{k+1} = 1$.
For each $0\leq i \leq k$ and each $t,t'$ such that $t_i <t<t'<t_{i+1}$ we have $d_Y(f(\gamma(t)),f(\gamma(t'))) \leq \lambda l_H(\gamma_{|[t,t']})$. Letting $t\to t_i$ and $t'\to t_{i+1}$ we obtain $d_Y(f(\gamma(t_i)),f(\gamma(t_{i+1}))) \leq \lambda l_H(\gamma_{|[t_i,t_{i+1}]})$. Adding up we obtain 
$$
d_Y(f(z), f(z')) \leq \sum_{0\leq i \leq  k} d_Y(f(\gamma(t_i)), f(\gamma(t_{i+1}))) \leq \lambda
\sum_{0\leq i \leq k} l_H(\gamma_{[t_i, t_{i+1}]}) = \lambda l_H(\gamma).
$$

We now consider the case where $\gamma$ meets the set $\Gamma$ an infinite number of times, and we choose a sequence $\gamma_n$ as described above. We obtain $d_Y(f(\gamma_n(0)), f(\gamma_n(1))) \leq \lambda l_H(\gamma_n)$ for each $n\geq 0$. Since $\gamma_n \to \gamma$ in $C^1$ norm as $n \to \infty$ we obtain taking the limit $d_Y(f(z), f(z')) \leq \lambda l_H(\gamma)$.

Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ we obtain $d_Y(f(z), f(z')) \leq \lambda d_H(z,z')$, which concludes the proof of this proposition.
\sq


%Let $(Y, \|\cdot \|_Y)$ and $(Z, \|\cdot\|_Z)$ be two banach spaces. Let $y\in Y$, $g\in C^1(Y,Z)$, and $L = g'(f(x))$, then clearly 
%$$
%\dil_y(g) = \|L\|.
%$$
%Injecting this in \iref{eqDilUpper1} we obtain 
%\be
%\label{eqDilUpper2}
%\dil_x(g \circ f) \leq\|L\|  \dil_x (f).
%\ee
%We also need a lower bound in several cases. For that purpose we define 
%$$
%\dil^*_z(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(z,\ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)}\right),
%$$
%and we obtain proceeding similarly, but with the different convention $0\times \infty = \infty\times 0 = 0$
%$$
%\dil_z(g\circ f) \geq \dil^*_{f(z)}(g) \dil_z(f).
%$$

The next proposition establishes that the regularity conditions \iref{eqLipMult} and \iref{eqLipAdd} defining the collections of quasi-acute or graded metrics are equivalent in the case of a metric proportionnal to the identity. %$\bH_a$ $\bH_g$

\begin{prop}
\label{propEquivS}
Let $s\in C^0(\R^d, R_+^*)$ and let $H(z) := \Id/s(z)^2$ for all $z\in \R^d$. We have 
\be
\label{eqDilLnH}
\dil_z(\ln s\sep d_H) = \dil_z(s).
\ee
Hence the following properties are equivalent.
\begin{enumerate}
\item The map $s : \R^d \to \R$ is Lipschitz. (i.e. $H\in \bH_i$) %For all $z,z'\in \R^d$ one has $|s(z)-s(z')|\leq |z-z'|$.
\item (``Additive'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_+(H(z),H(z')) \leq |z-z'|$.
\item (``Multiplicative'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_\times(H(z),H(z'))\leq d_H(z,z')$.
\end{enumerate}
\end{prop}

\proof %reprendre preuve??
Combining \iref{eqDilNorm} and \iref{eqDilLog} we obtain for any $z\in \R^d$
$$
%\dil_z (H\sep  d_\times, d_H) = 
\dil_z(\ln s\sep d_H) = s(z) \dil_z(\ln s) = \dil_z(s),
$$
which establishes \iref{eqDilLnH}.
According to \iref{eqDIso} we have for any $z,z'\in \R^d$
$$
d_+(H(z),H(z')) = |s(z) - s(z')| \stext{ and } d_\times (H(z),H(z')) = |\ln s(z) - \ln s(z')|.
$$
The properties 1. and 2. are thus equivalent to $\dil(s)\leq 1$, and therefore also to 
\be
\label{eqDilsLoc}
\dil_z(s) \leq 1 \text{ for all } z\in \R^d.
\ee
according Proposition \ref{propDilLoc} applied to the constant metric $H_0 = \Id$ and to the function $f=s$.
On the other hand property 3. is equivalent to $\dil(\ln s \sep d_H) \leq 1$, and thus to 
$$
\dil_z(\ln s\sep d_H) \leq 1 \text{ for all } z\in \R^d
$$
according to Proposition \ref{propDilLoc} applied to the metric $H$ and to the function $f=\ln s$.
This property equivalent to \iref{eqDilsLoc} according to \iref{eqDilLnH}, which concludes the proof of this Proposition.
\sq

The next corollary uses Proposition \ref{propEquivS} to analyse the regularity of the first and last eigenvalue of a metric.
\begin{corollary}
\label{corolLipNorm}
\begin{itemize}
\item
For any $H\in \bH_g$, the map $z\mapsto \|H(z)\|^{-\frac 1 2}$ is Lipschitz.
\item
For any $H\in \bH_a$, the map $z\mapsto \|H(z)^{-\frac 1 2}\|$ is Lipschitz.
\end{itemize}
\end{corollary}
\proof
\begin{itemize}
\item 
%For any $M,M'\in S_d^+$ we have 
%\begin{eqnarray*}
%d_\times(M,M') &=& \ln \left(\max\left\{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\right\}\right) \\
%&\geq &\ln \left(\max \left\{\frac{\|M^\frac 1 2\|}{\|M'^{\frac 1 2}\|}, \, \frac{\|M'^{\frac 1 2}\|}{\|M^{\frac 1 2}\|}\right\}\right)\\
%& = & \frac 1 2 \left|\ln \|M\| - \ln \|M'\|\right|.
%\end{eqnarray*}
Consider $H\in \bH_g$, define $s(z) := \|H(z)\|^{-\frac 1 2}$ and 
$$
H'(z) := \frac \Id {s(z)^2} = \|H(z)\|\Id.
$$
Since $H(z) \leq H'(z)$ for all $z\in \R^d$, we have $d_H(z,z') \leq d_{H'} (z,z')$ for all $z, z'\in \R^d$.

Consider a pair $M,M'\in S_d^+$ of matrices and a real $\delta>0$. If $e^{-2\delta} M \leq M' \leq e^{2\delta} M$, then taking the norm we obtain $e^{-2\delta} \|M\| \leq \|M'\| \leq e^{2\delta} \|M\|$. It follows that 
$$
\frac 1 2 |\ln \|M\| - \ln \|M'\|| \leq d_\times (M,M').
$$
We thus have for any $z,z'\in \R^d$
\begin{eqnarray*}
|\ln s(z)-\ln s(z')| &=& \frac 1 2 \left|\ln \|H(z)\| - \ln \|H(z')\|\right| \\ %\left|\ln \left(\sqrt{\|H(z)\|}\right) -\ln \left(\sqrt{\|H(z')\|}\right)\right| \\%
%& \leq & \sup_{u\neq 0} |\ln \|u\|_{H(z)} - \ln \|u\|_{H(z')}|\\
&\leq & d_\times(H(z),H(z')) \\
&\leq& d_H(z,z')\\
&\leq& d_{H'}(z,z').
\end{eqnarray*}
Applying Proposition \ref{propEquivS} to the metric $H'$ we obtain that $H'\in \bH_i$, and therefore that $s$ is Lipschitz as announced.
\item
Consider $H\in \bH_a$. We have for any $z,z'\in \R^d$
$$
\left|\|H(z)^{-\frac 1 2}\| - \|H(z')^{-\frac 1 2}\| \right| \leq \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| \leq |z-z'|,
$$
which concludes the proof of this corollary.\sq
\end{itemize}

Our last proposition studies the local dilatation of the maximum and the minimum of two functions.
\begin{prop}
\label{propDilMax}
Let $(X,d_X)$ be a metric space and let $\lambda, \mu\in C^0(X, \R)$. Let $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda, \mu\}$. Then for all $x\in X$
\be
\label{eqDilMax1}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} \leq \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
If $(X,d_H) = (\R^d, d_H)$, where $H \in \bH$ is a riemannian metric, then equality holds
\be
\label{eqDilMax2}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} = \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
\end{prop}

\proof
We have for any $p,q\in X$,
\begin{eqnarray*}
|\gamma(p)-\gamma(q)| &=& |\min\{\lambda(p), \mu(p)\} - \min \{\lambda(q), \mu(q)\}|\\
& \leq & \max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}.
\end{eqnarray*}
For any $x\in X$ and any $\ve>0$ we thus obtain
\begin{eqnarray*}
\dil(\gamma_{|B(x,\ve)}) &=& \sup_{p,q\in B(x,\ve)} \frac{|\gamma(p)-\gamma(q)|}{d_X(p,q)} \\
&\leq& \sup_{p,q\in B(x,\ve)} \frac{\max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}}{d_X(p,q)}\\
& =& \max\left\{\sup_{p,q\in B(x,\ve)}  \frac{|\lambda(p)-\lambda(q)|}{d_X(p,q)}, \sup_{p,q\in B(x,\ve)}  \frac{|\mu(p)-\mu(q)|}{d_X(p,q)}\right\}\\
&=& \max\left\{\dil(\lambda_{|B(x, \ve)}), \dil(\mu_{|B(x,\ve)})\right\}.
\end{eqnarray*}
Letting $\ve \to 0$ we obtain $\dil_x(\gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$. Likewise $\dil_x(\Gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$ which concludes the proof of \iref{eqDilMax1}.

We now turn to the proof of \iref{eqDilMax2}. For that purpose we consider a fixed $\ve>0$ and we define
$$
r := \max \{\dil(\gamma_{|B(x,\ve)}\sep \|\cdot\|_{H(x)}), \ \dil(\Gamma_{|B(x,\ve)} \sep \|\cdot\|_{H(x)})\},
$$
where $B(x,\ve)$ stands for the euclidean unit ball of radius $\ve$ centered at $x$.
Consider two points $p,q\in B(x,\ve)$. If $\lambda(p) \geq \mu(p)$ and $\lambda(q)\geq \mu(q)$, or if $\lambda(p) \leq \mu(p)$ and $\lambda(q)\leq \mu(q)$, then 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)|&=& \max \{|\gamma(p)-\gamma(q)|, |\Gamma(p)-\Gamma(q)|\}\\
&\leq & \|p-q\|_{H(x)}
\end{eqnarray*}
Otherwise if  $\lambda(p) \geq \mu(p)$ and $\lambda(q)\leq \mu(q)$, or $\lambda(p) \leq \mu(p)$ and $\lambda(q)\geq \mu(q)$, then there exists a point $r$ on the segment $[p,q]$ such that $\lambda(r)=\mu(r)$. We thus have %$|p-r|+|r-q| = |p-q|$ and 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)| &\leq& \max \{|\gamma(p)-\gamma(r)|, |\Gamma(r)-\Gamma(q)|\}\\
& &+ \max \{|\gamma(r)-\gamma(q)|, |\Gamma(r)-\Gamma(q)|\}\\
& \leq & \|p-r\|_{H(x)} + \|r-q\|_{H(x)} = \|p-q\|_{H(x)}
\end{eqnarray*}
If follows that $\dil(\lambda_{|B(x,\ve)}\sep \|\cdot\|_{H(x)})\leq r$, and letting $\ve\to 0$ we obtain 
$$
\dil_x(\lambda\sep \|\cdot\|_{H(x)}) \leq \max\{\dil_x(\gamma\sep \|\cdot\|_{H(x)}), \ \dil_x(\Gamma \sep \|\cdot \|_{H(x)})\}.
$$ 
Recalling that $\dil_x(f\sep d_H) = \dil_x(f\sep \|\cdot\|_x)$ for any $f\in C^0(\R^d, \R)$ and any for all $x\in \R^d$, see \iref{eqDilNorm}, we obtain $\dil_x(\lambda) \leq \max\{\dil_x(\gamma), \ \dil_x(\Gamma)\}$. Proceeding likewise for $\mu$ we obtain \iref{eqDilMax2} which concludes the proof of this proposition.
\sq

\subsection{Geometric properties of the space $(\R^d, d_H)$} %Estimates of size}
\label{subsecMetGeom}

We focus in this subsection on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. The next proposition compares the riemannian distance $d_H$ between two points $z$ and $z+u$ with the norm $\|u\|_{H(z)}$ of their difference.

%with the euclidean distance and we estimate the volume of balls. 
%The next proposition compares the Riemannian distance associated to a graded metric, with 

\begin{prop}
\label{propEuclidRiemann}
Let $H \in \bH_g$ and let $z\in \R^d$. For all $u\in \R^d$ one has
\be
\label{eqEuclidRiemann}
\ln(1+\|u\|_{H(z)}) \leq d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention when $\|u\|_{H(z)}\geq 1$.
\end{prop}
\proof
%We first prove the left part of \iref{eqEuclidRiemann}, and for that purpose
We consider a path $\gamma\in C^1([0,1], \R^d)$, and we define for each $t\in [0,1]$
\be
\label{defLGamma}
l(t) := \int_0^t \|\gamma'(t)\|_{H(\gamma(t))}dt.
\ee
Since $H\in \bH_g$ we have for any $t\in [0,1]$
$$
\exp(-2\, d_H(z, \gamma(t))) \, H(z) \leq H(\gamma(t)) \leq  \exp(2 \, d_H(z, \gamma(t))) \, H(z)
$$
therefore, since $d_H(z, \gamma(t)) \leq l(t)$,
$$
\exp(-2l(t)) H(z)  \leq H(\gamma(t)) \leq  \exp(2l(t)) H(z).
$$
It follows that 
$$
\|\gamma'(t)\|_{H(z)} \exp(-l(t)) \leq l'(t) = \|\gamma'(t)\|_{H(\gamma(t))} \leq  \|\gamma'(t)\|_{H(z)} \exp(l(t)), %\exp(-l(t))
$$
hence 
\be
\label{eqGammapLp}
-\frac d {dt} \exp(-l(t)) \leq \|\gamma'(t)\|_{H(z)} \leq \frac d {dt} \exp(l(t)).
\ee
We have 
\be
\label{eqGammaGammap}
\|u\|_{H(z)} =  \|\gamma(1)-\gamma(0)\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt
\ee
with equality if $\gamma(t) = z+tu$ is the straight line.
%We now assume that $\gamma(t) \neq \gamma(0)$ for all $t\in (0,1]$, which is the case generically. The map $t\mapsto \|\gamma(t)-\gamma(0)\|_{H(z)}$ is therefore $C^1$ on $(0,1]$ and we have 
%$$
%\frac d {dt} \|\gamma(t)-\gamma(0)\|_{H(z)} \leq \|\gamma'(t)\|_{H(z)},
%$$
%with equality if $\gamma(t)-\gamma(0) = c \gamma'(t)$ for some $c>0$.
%In the special case of the straight line $\gamma(t)=z+tu$, \iref{eqGammaGammap} is an equality and we thus obtain 
In that case, integrating the left part of \iref{eqGammapLp} we obtain
$$
 1-\exp(-l_H(\gamma)) = -\int_0^1 \left(\frac d {dt} \exp(-l(t))\right)dt   \leq  \int_0^1 \|\gamma'(t)\|_{H(z)} dt %= \|\gamma(1)-\gamma(0)\|_{H(z)} \exp(-l(0)) - \exp(-l(1))
 = \|u\|_{H(z)}.
$$
Rearranging the terms we obtain the right part of \iref{eqEuclidRiemann}:
$$
d_H(z,z+u) \leq l_H(\gamma) \leq -\ln(1-\|u\|_{H(z)}).
$$
We now consider an arbitrary path $\gamma$ joining $z$ and $z+u$ and we obtain integrating the right part of \iref{eqGammapLp} and recalling \iref{eqGammaGammap}
$$
\exp(l_H(\gamma)) -1 = \int_0^1 \left(\frac d {dt} \exp(l(t))\right) dt  \geq \int_0^1 \|\gamma'(t)\|_{H(z)} dt \geq \|u\|_{H(z)},
$$
which is equivalent to
$$
l_H(\gamma) \geq \ln(1+\|u\|_{H(z)}).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ satisfying $\gamma(0) = z$ and $\gamma(1) = z+u$, we obtain the left part of \iref{eqEuclidRiemann}, which concludes the proof of this proposition.
\sq

We discuss in the rest of this section the consequences of the comparison \iref{eqEuclidRiemann} of the riemannian distance $d_H$ with the distance associated to the norm $\|\cdot\|_{H(z)}$ when $H\in \bH_g$. %is devoted to 
Combining the right part of \iref{eqEuclidRiemann} with the expression \iref{eqDTimesLog} of the distance $d_\times$ we obtain an estimate of the local variations of the norm $\|\cdot \|_{H(z)}$ associated to the metric $H$ at a point $z$: let $H\in \bH_g$, and let $z,u,v\in \R^d$ be such that $\|u\|_{H(z)} < 1$, then
\be
\label{eqLocalNorm}
(1-\|u\|_{H(z)}) \|v\|_{H(z)} \leq \|v\|_{H(z+u)} \leq (1-\|u\|_{H(z)})^{-1} \|v\|_{H(z)}. %\frac{\|v\|_{H(z)}}{1-\|u\|_{H(z)}}.
\ee
Note also that 
\be
\label{eqLocalDet}
(1-\|u\|_{H(z)})^d \sqrt{\det H(z)} \leq \sqrt{\det H(z)} \leq (1-\|u\|_{H(z)})^{-d} \sqrt{\det H(z)}.
\ee
Another important consequence of \iref{eqEuclidRiemann} is that the closed balls $\{z'\in \R^d \sep d_H(z,z')\leq r\}$ for the distance $d_H$, are closed and bounded subsets $\R^d$, hence are compact. %From this point a classical argument (??) shows that $(R^d,d_H)$ is a complete metric space.

The following example establishes that \iref{eqEuclidRiemann} is a sharp inequality. The metric $H$ defined by 
$$
H(z) := \frac \Id {(1+|z|)^2}
$$
belongs to $\bH_i$ since $z\mapsto 1+|z|$ is Lipschitz, hence $H$ also belongs to $\bH_a$ and $\bH_g$.
For any $v\in \R^d$, one easily checks that the path of minimal length joining $0$ to $v$ is the straight line, and that
$$
d_H(0, v) = \ln(1+|v|).
$$
Choosing $z=0$ and $u=v$ we obtain that the left part of \iref{eqEuclidRiemann} is sharp
$$
\ln (1+ \|u\|_{H(0)}) = \ln (1+ |u|) = d_H(0,0+u).
$$
Choosing $z=-v$ and $u = v$ we obtain that the right part of \iref{eqEuclidRiemann} is sharp
$$
-\ln\left(1-\|u\|_{H(-u)} \right) = -\ln \left(1-\frac {|u|}{1+|u|}\right) = \ln(1+|u|) = d_H(-u, -u+ u).
$$

The next corollary uses Proposition \ref{propEuclidRiemann} to obtain a lower bound for the mass of balls in the measure $z\mapsto \sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. %states a volume estimate Proposition \ref{propLength} implies a volume estimate. %also allows us to compare the vo
\begin{corollary}
\label{corolVol}
There exists $c=c(d)>0$ such that the following holds. Let $H \in \bH_g$,
let $L\geq 1$ and let $z_0\in \R^d$. Denoting $\cE$ the ellipse 
$$
\cE = \{z\in \R^d\sep \|z-z_0\|_{H(z_0)}\leq L\}.
$$ 
we have 
\be
\label{eqVolLog}
\int_\cE \sqrt{\det H} \geq c \ln L. %\max\{L,1\}.
\ee
%Then 
%$$
%\int_\cE \sqrt {\det H} \geq c \ln L -1
%$$
%where $c=...$
%In particular if $H(z)\geq \lambda^2\Id$ (*$\|u\|_{H(z)} \geq \lambda |u|$ for all $u\in \R^d$*) then 
%\be
%\label{volBR}
%\int_{B(z,r)} \sqrt{\det H} \geq c \ln \max\{\lambda r, 1\}
%\ee
\end{corollary}

\proof
It follows from Proposition \ref{propEuclidRiemann} that $d(z_0, z) \geq \ln (L+1)$ for all $z\in \partial \cE$. We define the integer 
$$
k = \left\lfloor \ln(L+1) -\frac 1 2\right\rfloor,
$$
and we consider $k$ points $z_1, \cdots , z_k \in E$ such that for all $0 \leq i \leq k$
$$
d_H(z_0, z_i)= i.
$$
We define 
$
r_0 := 1-e^{-\frac 1 2} = 0.39\cdots
$
in such way that 
$$
-\ln (1-r_0) = \frac 1 2.
$$
For all $0 \leq i \leq k$ we denote by $\cE_i$ the ellipse 
$$
\cE_i  := \left\{z\in \R^d \sep \|z-z_i\|_{H(z_i)} \leq r_0\right\}.
$$
We have $\cE_i \subset \cE$ for all $0 \leq i \leq k$, indeed for any $z\in \cE_i$ we have 
$$
d_H(z_0, z) \leq d_H(z_0, z_i) + d_H(z_i, z) \leq i- \ln (1-r_0) \leq k+\frac 1 2 \leq \ln (L+1),
$$
Denoting by $\interior(E)$ the interior of a set $E\subset \R^d$, we observe that for all $0 \leq i<j\leq k$, for all $z\in \interior(\cE_i)$ and $z'\in \interior(\cE_j)$, we have
$$
d_H(z,z') \geq d_H(z_i, z_j) -d_H(z_i, z) - d_H(z_j,z') > |d_H(z_0, z_i) - d(z_0, d_j)| + 2\ln(1 -r_0) =0, %\geq 1+ 2 \ln(1-\frac 1 3)>0.
$$
hence $\interior(\cE_i) \cap \interior(\cE_j) = \emptyset$.
It follows that 
$$
\int_\cE \sqrt{\det H} \geq \sum_{0 \leq i \leq k} \int_{\cE_i} \sqrt{\det H}.
$$
Furthermore we have for all $z\in \cE_i$
$$
H(z) \geq (1-\|z-z_i\|_{H(z_i)})^2 H(z_i)  \geq (1-r_0)^2 H(z_i),
$$
and therefore 
\be
\label{eqzzi}
\sqrt{\det H(z)} \geq (1-r_0)^d \sqrt{\det H(z_i)}.
\ee
We denote by $B(z,r)$ the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$, and we observe that 
$u\mapsto z_i + H(z_i)^{-\frac 1 2} u$ maps $B(0,r_0)$ onto $\cE_i$. Combining this remark with \iref{eqzzi} we obtain
\begin{eqnarray*}
\int_{\cE_i} \sqrt{\det H} &\geq& (1-r_0)^d \int_{\cE_i} \sqrt{\det H(z_i)} \\
&=& (1-r_0)^d \int_{B(0,r_0)} 1 \\
&=& c_0 := r_0^d (1-r_0)^d |B(0,1)|.
\end{eqnarray*}
%where $B(z,r)$ denotes the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$.
Eventually we obtain 
$$
\int_\cE \sqrt{\det H} \geq (k+1) c_0 \geq (\ln(L+1) - 1/2) c_0.
$$
In order to obtain \iref{eqVolLog} we simply recall that $L\geq 1$ and therefore that %Since Recalling that $L\geq 1$ we find that 
$$
\ln (L+1) = \frac{\ln(L+1)}{2 \ln 2} +  \left(1-\frac 1 {2 \ln 2}\right)\ln(L+1) \geq \frac 1 2 + \left(1-\frac 1 {2 \ln 2}\right)\ln L $$
which concludes the proof of \iref{eqVolLog} with $c=(1- 1/(2 \ln 2))c_0$.
%Applying \iref{eqVolLog} to $L = \lambda r$ we obtain \iref{volBR} which concludes the proof of this proposition.
\sq


\section{Metrics having an eigenspace of dimension $d-1$ at each point}
\label{secEigen}
We focus in this subsection on metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has an eigenspace of dimension at least $d-1$ at each point $z\in \R^d$. 
%If the dimension is $d=2$, then a metric $H\in \bH$ generically satisfies this condition on a dense subset of $\R^d$. %any metric $H\in \bH$ satisfies this condition. 
This condition clearly holds if the dimension is $d=2$, but is also relevant in higher dimension. 
Indeed, as discussed in \S\ref{secOptGeom} of Chapter \ref{chapApproxMet}, this type of metrics appears when one needs to create mesh containing a thin layer of simplices close to an hypersurface $\Gamma$. In that case the matrix $H(z)$ at a point $z\in \Gamma$ typically has an eigenspace of dimension $d-1$ which is tangent to $\Gamma$ and is associated to a small eigenvalue, and an eigenspace of dimension $1$ in the direction orthogonal to $\Gamma$ associated to a large eigenvalue. 

The main result of this section is Theorem \ref{th2Spaces} which characterises those of these metrics which belongs to $\bH_a$ or $\bH_g$ in terms of the regularity of their eigenvalues and of their eigenvectors.
Corollary \ref{corolHgToHa} to this theorem gives a simple procedure to obtain a quasi-acute metric from a graded metric $H$ such that $H(z)$ has an eigenspace of dimension $d-1$ at each point. \\

We denote by $\bbS := \{\theta\in \R^d \sep |\theta| = 1\}$ the unit sphere of $\R^d$, equipped with the distance 
$$
d_\bbS(\theta, \theta') := \arccos(\<\theta, \theta'\>).
$$
We denote by $\cA$ the space of parameters
$$
\cA := \R_+^*\times \R_+^*\times \bbS,
$$
and we define a map $\cS :\cA\to S_d^+$ as follows
\be
\label{defcS}
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
\ee
In any orthonormal basis $\cB$ of $\R^d$ which begins with the vector $\theta$ we have the following expression
$$
[\cS(\lambda, \mu, \theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda &0 & 0 & \cdots\\
0 & \mu & 0 & \cdots\\
0 & 0 & \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right).
$$
We also define for any $a = (\lambda, \mu, \theta)\in \cA$
$$
\cH(a) := \cS(a)^{-2} = \lambda^{-2} \theta \theta^\trans+ \mu^{-2}(1-\theta \theta^\trans).
$$
%If $M\in S_d^+$ has an eigenspace of dimension $d-1$ exactly, then 
%
%We denote by $S_{d*}^+$ the collection of symmetric positive definite matrices $M\in S_d^+$ which have an eigenspace of dimension exactly $d-1$.
%We also denote by $\cA^*$ the collection of $(\lambda, \mu, \pm\theta)\in \cA$ which satisfies $\lambda\neq \mu$ if $d>2$ (resp. $\lambda>\mu$ is the dimension is $d=2$).
%Then
%$$
%\cH : \cA^* \to S_{d*}^+
%$$
%is a one to one map.



%Such a metric $H$ can be parametrized using two eigenvalues $\lambda, \mu\in \R_+^*$  and a subspace of dimension $d-1$ of $\R^d$ defined through an un-oriented unit normal $\pm \theta$. Our purpose in this section is to translate the fact that $H\in \bH_\star$, for some $\star\in \{i,a,g\}$, into simpler properties satisfied by $\lambda,\mu$ and $\theta$.
%
%
%
%In order to state our results, we need to introduce the collection $\cP$ of all hyperplanes of $\R^d$, also called the projective space. An hy
%
%
%We define the space of parameters
%$$
%\cA :=  \R_+^* \times \R_+^* \times \cP,
%$$
%where $\cP$ is the $d-1$-dimensional real projective space.
%For all $(\theta, \lambda, \mu)\in \cA$ we define 
%$$
%S( \lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans),
%$$
%and $H(\theta, \lambda, \mu) := S^{-2}$.
%The space $\cA$ is a differential variety, and the tangent space to a triplet $(\theta, \lambda, \mu)\in \cA$ is 
%$$
%T_{(\theta, \lambda, \mu)} \cA =  \R \times \R \times \theta^\perp,
%$$
%where $\theta^\perp$ refers to the orthogonal hyperplane to $\theta$ in $\R^d$.

For any metric $H \in \bH$ and any $z\in \R^d$ we denote by $\dil_z(H)_\times$ and $\dil_z(H)_+$ the local dilatations at $z$ associated to the Lipschitz conditions \iref{eqLipMult} and \iref{eqLipAdd} defining $\bH_g$ and $\bH_a$:
\be
\label{defDilH}
\dil_z(H)_\times := \dil_z(H \sep d_\times, d_H) \stext{ and } \dil_z(H)_+ := \dil_z(H \sep d_+).
\ee
We recall that the local dilatation $\dil_z(f)$ of a function $f$ at a point $z$ is defined by \iref{defDilX}.
%We set $D_z(H) := \dil(\lambda)$ if $z\notin \Omega$
For any open set $\Omega\subset \R^d$ and any $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$,  we define for all $z\in \Omega$
\be
\label{eqDZA}
D_z(a)_\times := \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \frac 1 2 \left| \frac {\lambda(z)} {\mu(z)} - \frac {\mu(z)} {\lambda(z)} \right|\dil_z(\theta\sep  d_H)\right\}, %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
and 
\be
\label{eqDZAP}
D_z(a)_+ := \max\left\{\dil_z(\lambda), \ \dil_z(\mu),\ |\lambda(z)-\mu(z)| \dil_z(\theta)\right\}. %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
Note that these quantities are not defined if $\lambda(z) = \mu(z)$ and $\dil_z(\theta\sep  d_H)=\infty$ simultaneously, since an indeterminate form $0\times \infty$ appears in \iref{eqDZA} and \iref{eqDZAP}.
\begin{theorem}
\label{th2Spaces}
Let $H \in \bH$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, such that $H = \cH\circ a$ on $\Omega$.
Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$. Then 
\be
\label{eqDilTimes}
D_z(a)_\times \leq \dil_z(H)_\times \leq 2D_z(a)_\times
\ee
and%, with $\gamma := \|H^{-\frac 1 2}\| = \max\{\lambda, \mu\}$, 
\be
\label{eqDilPlus}
D_z(a)_+ \leq \dil_z(H)_+ \leq 2D_z(a)_+.
\ee
%In particular, defining $\gamma := \|H(z)^{-\frac 1 2}\| = \max \{\lambda, \mu\}$ we have 
%\be
%\label{eqDilMax}
%\max\{\dil_z(\gamma), \, D_z(a)_\times\} \leq \max \{D_z(a)_+, \, D_z(a)_\times\} \leq 2\max\{\dil_z(\gamma), \, D_z(a)_\times\}.
%\ee
\end{theorem}

%The estimate \iref{eqDilPlus} on $\dil_z(H)_+$ is not very sharp, but this is not an issue since one usually does not needs to control $ \dil_z(H)_+$ but rather $\max\{\dil_z(H)_\times,\dil_z(H)_+\}$, for which we obtain combining \iref{eqDilTimes} and \iref{eqDilPlus} the sharper estimate 
%$$
% \max\{\dil_z(\gamma), D_z(a)\} \leq \max\{\dil_z(H)_\times,\dil_z(H)_+\} \leq 2 \max\{\dil_z(\gamma), D_z(a)\}.
%$$
The rest of this section is devoted to the proof of this theorem and to Corollary \ref{corolHgToHa}. Our first lemma defines and estimates a quantity $\Delta(a,b,c)$ which appears repeatedly in the rest of the proof.


\begin{lemma}
\label{lemmaDelta}
We define for all $a,b,c\in \R$ the quantity $\Delta(a,b,c)\in \R_+$, as follows % which is the norm of a $d\times d$ matrix,
\be
\label{defDelta}
\Delta(a,b,c) := 
\left\| 
\left(
\begin{array}{cccc}
a & b & 0 & \cdots\\
b & c& 0 & \cdots\\
0 & 0 & c & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right)
\right\|.
\ee
We have 
\be
\label{eqEstimM}
\max\{|a|, |b|, |c|\} \leq \Delta(a,b,c) \leq 2 \max\{|a|, |b|, |c|\}.
\ee
\end{lemma}

\proof
We consider fixed values of $a,b,c\in \R$ and we denote by $M$ the matrix presented in \iref{defDelta}, in such way that $\Delta(a,b,c) = \|M\|$. We also define $\lambda := \max\{|a|,|b|,|c|\}$.
We have 
$$
\Delta(a,b,c) = \|M\|\geq \max_{1\leq i,j\leq d} |M_{ij}| = \lambda,
$$
which establishes the left part of \iref{eqEstimM}. For all $p\in [1,\infty]$ we denote by $l^p$ the usual norm on $\R^d$ of exponent $p$. We have 
$$
\|M\|_{l^\infty\to l^\infty} = \max_{1 \leq i \leq d} \sum_{1\leq j \leq d} |M_{ij}| \leq 2 \lambda \stext{ and } \|M\|_{l^1\to l^1} = \max_{1 \leq j \leq d} \sum_{1\leq 1 \leq d} |M_{ij}| \leq 2 \lambda.
$$
By interpolation we thus obtain  
$$
\|M\| = \|M\|_{l^2\to l^2} \leq \sqrt{\|M\|_{l^1\to l^1} \|M\|_{l^\infty\to l^\infty} } \leq 2 \lambda,
$$
which concludes the proof.
\sq

The parameter space $\cA = \bbS \times \R_+^* \times \R_+^*$ is a differential variety, and the regularity of functions defined on $\cA$ should be seen through local charts.
For each $a = (\lambda, \mu, \theta)\in \cA$ we define a local chart $\psi_a$ of a neigborhood of $a$ in $\cA$ as follows: 
\be
\label{defPsia}
\psi_a : (-\lambda, \infty)\times (-\mu , \infty) \times (B(0,\cPi) \cap \theta^\perp) \to \cA
\ee
is defined by 
$$
\psi_a(\Lambda, M, r\Theta) := (\lambda+ \Lambda,\, \mu+ M,\, \cos(r) \theta + \sin(r) \Theta),
$$
where $|\Theta| = 1$. Note that $\psi_a$ is one to one and that $d_\bbS(\theta, \, \cos(r) \theta + \sin(r) \Theta) = r$.
In \iref{defPsia} we denoted by $\theta^\perp := \{\Theta\in \R^d \sep \<\theta, \Theta\> = 0 \}$ the space orthogonal to $\theta$, and $B(0,\cPi)$ the open euclidean ball of radius $\cPi$.
%it preserves distances in the following sense: if $(\lambda', \mu', \theta') = \psi_a(\Lambda, M, r\Theta)$ then $\lambda'-\lambda = \Lambda$, $\mu'-\mu=M$ and $

Let $V$ be a banach space. We say that a function $\vp : \cA \to V$ is $C^1$ if for any $a\in \cA$ the function $\vp\circ \psi_a$ is $C^1$.
In that case for any $a\in \cA$ we define the differential 
%and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
$$
d_a\vp(A) : \R\times \R\times \theta^\perp \to V
$$
by the formula
$$
d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( tA) - \vp(a)} t. %\Lambda, t M, t r\Theta
$$
We then have
 $$
\dil_a(\vp) = \|d_a(\vp)\|.
$$
%where $d_0 (\vp\circ \psi_a) :  \R\times \R\times \theta^\perp \to V$ denotes the differential of function $\vp\circ \psi_a$ at the origin $(0,0,0) \in (-\lambda, \infty)\times (-\mu , \infty) \times (B(\pi) \cap \theta^\perp)$.
%In that case for any $a\in \cA$ and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
%$$
%d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( t\Lambda, t M, t r\Theta) - \vp(a)} t,
%$$
%and we have for any path $\gamma\in C^1([0,1], \cA)$ 
%$$
%\vp(\gamma(1)) - \vp(\gamma(0)) = \int_0^1 d \vp_{\gamma(t)} (\gamma'(t)) dt.
%$$

\begin{prop}
\label{propPhiPlus}
Define $V_+ := S_d$, equipped with the standard norm $\|\cdot\|$, and define $\vp_+ (a) := \cS(a)$.
Then for all $a,b\in \cA$ we have 
\be
\label{eqDPPhiP}
d_+(\cH(a), \cH(b)) = \|\vp_+(a)-\vp_+(b)\|.
\ee
Furthermore $\vp_+ \in C^1(\cA, V_+)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
$$
\|d_a \vp_+(A)\|_\infty= 
\Delta(\Lambda, \ (\lambda-\mu) r ,\ M).
$$
\end{prop}

\proof
The \iref{eqDPPhiP} directly follows from the fact that $\cH(a)^{-1} = \cS(a)^2 = \vp_+(a)^2$, and from the definition \iref{defDPlus} of $d_+$.
The function $\vp_+ = \cS$ is $C^1$, and even $C^\infty$, since it has a polynomial expression 
$$
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
$$
We have at the first order in $\lambda, \mu, r$
\begin{eqnarray*}
\cS(\lambda+ \Lambda, \, \mu+M, \, \theta+r\Theta) &=&
 (\lambda+ \Lambda) (\theta+ r\Theta) (\theta+r\Theta)^\trans \\
 & &+ (\mu+M)(\Id - (\theta+ r\Theta) (\theta+r\Theta)^\trans)\\
 &=& S(\lambda, \mu, \theta) \\
 & &+ \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans)\\
& &+  \cO((|\Lambda|+ |M|+ |r|)^2)
\end{eqnarray*}
Therefore %$\vp_+$ is $C^1$ and 
\be
\label{eqDiffS}
%d_a\vp_+(\Lambda, \,M, \,r\Theta) = 
d_a\cS(\Lambda, \,M, \,r\Theta) =  \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans).
\ee
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[d_a\cS(\Lambda, \,M, \,r\Theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda & r(\lambda-\mu) & 0 & \cdots\\
r(\lambda-\mu) & M & 0 & \cdots\\
0 & 0 & M & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
which concludes the proof of this proposition.
\sq


\begin{prop}
\label{propPhiTimes}
Define $V_\times := C^0(\bbS, \R)$, equipped with the $\|\cdot\|_\infty$ norm, and define $\vp_\times : \cA \to V_\times$ as follows: for any $a\in \cA$ and any $u\in \bbS$
%\be
%\label{eqDTPhiT}
$$
\vp_\times (a) := (u \mapsto \ln \|u\|_{\cH(a)}).
$$
%\vp_\times (a)(u) = \ln \|u\|_{\cH(a)}.
%\ee
Then for all $a,b\in \cA$ we have 
\be
\label{eqDTPhiT}
\|\vp_\times(a)-\vp_\times(b)\|_\infty = d_\times(\cH(a), \cH(b)).
\ee
Furthermore $\vp_\times \in C^1(\cA, V_\times)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
\be
\label{eqNormDPhiPlus}
\|d_a \vp_\times(A)\|_\infty= 
\Delta\left(\frac \Lambda \lambda ,\ \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) ,\ \frac M \mu\right).
\ee
\end{prop}

\proof
Using the expression \iref{eqDTimesLog} of the distance $d_\times$ and the homogeneity of norms we obtain for any $M,M'\in S_d^+$,
$$
d_\times (M,M') = \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
$$
which implies \iref{eqDTPhiT}.
%The inequality \iref{eqDTPhiT} follows from the expression \iref{eqDTimesLog} of the distance $d_\times$.

As observed in the proof of Proposition \ref{propPhiPlus} the function $\cS : \cA\to S_d^+$ is $C^1$, and $d_a\cS(A)$ has the explicit expression \iref{eqDiffS}.
It is well known that the inverse map ${\rm Inv} : \GL_d \to \GL_d$ is $C^1$ and has the the following differential : for any $\phi\in \GL_d$ and any $\Phi\in M_d$
$$
d_\phi {\rm Inv} (\Phi) = \phi^{-1} \Phi \phi^{-1}.
$$
By composition, $\cS^{-1} : \cA \to S_d^+$ is also $C^1$, and for any $a=(\lambda, \mu , \theta)\in \cA$ and any $A\in \R\times \R \times \theta^\perp$
$$
d_a(\cS^{-1})(A) = S(a)^{-1} (d_a S(A) ) S(a)^{-1}.
$$
For any $u\in \bbS$ we have 
$$
\ln \|u\|_{\cH(a)} = \ln \|\cS(a)^{-1}u\| = \frac 1 2 \ln \left(\<\cS(a)^{-1}u,\cS(a)^{-1}u\>\right).
$$
Therefore, again by composition, 
\begin{eqnarray*}
d_a (\ln \|u\|_{\cH})(A) &=&  \frac 1 {2\|\cS(a)^{-1}u\|^2} (\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>\\
& &\quad +\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>)\\% \frac {\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>+\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>}{2\|\cS(a)^{-1}u\|^2}\\
&=& \frac{\<G(a,A) v,v\>}{\|v\|^2}
\end{eqnarray*}
where $v = \cS^{-1}(a)u$. The function $G$ has the following expression : for any $a = (\lambda, \mu, \theta)\in \R_+^* \times \R_+^* \times \bbS$ and any $A = (\Lambda, M, r\Theta)\in \R\times \R \times \theta^\perp$
\begin{eqnarray*}
G(a,A) &=& \frac{\cS(a)^{-1} (d_a\cS(A)) + (d_a\cS(A)) \cS(a)^{-1}} 2\\
&=& \frac \Lambda \lambda \theta \theta^\trans +  \frac M \mu (\Id - \theta \theta^\trans) + \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right)(\theta \Theta^\trans + \Theta \theta^\trans),
\end{eqnarray*}
the last expression follows from the explicit expression \iref{eqDiffS} of $d_a\cS(A)$ establishes in the proof of the previous proposition, and from the fact that $\theta^\trans \Theta = 0$.
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[G(a,A)]_\cB = 
\left(
\begin{array}{cccc}
\frac \Lambda \lambda & \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & 0 & \cdots\\
\frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & \frac M \mu & 0 & \cdots\\
0 & 0 & \frac M \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
The map $\vp_\times$ is differentiable, as the composition of differentiable maps, and we thus have
\begin{eqnarray*}
\|d_a \vp_\times(A)\|_\infty &=& \sup \left\{ \frac{|\<G(a,A) v,v\>|}{\|v\|^2} \sep u\in \bbS, \, v=\cS(a)^{-1} u\right\}\\
&=& \|G(a,A)\|,
\end{eqnarray*}
which establishes \iref{eqNormDPhiPlus} and concludes the proof of this proposition.
\sq

We now consider a fixed $z\in \Omega$ and we remark that 
$$
\dil_z(H)_\times = \dil_z(\cH\circ a)_\times  = \dil_z(\vp_\times \circ a\sep d_H). %\leq \dil_{a(z)} (\vp_+\sep d_z) \dil_z(a\sep d_H, d_z)
$$
Therefore,  according to Lemma \ref{lemmaSubMult} for any norm $\|\cdot\|_{a(z)}$ defined on the tangent space $\R\times \R \times \theta(z)^\perp$ to $a(z)\in \cA$ we have 
\be
\label{eqDilPhiA}
\begin{array}{rcl}
& &\dil^*_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} a\sep d_H, \|\cdot \|_{a(z)})\\
& \leq& \dil_z(H)_\times\\
& \leq& \dil_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} \circ a\sep d_H, \|\cdot\|_{a(z)})
\end{array}
\ee
provided no indeterminate $0\times \infty$ or $\infty \times 0$ appears on the first and last term of this inequality.
%We recall that a neighborhood of $a(z)$ is parametrized by the local chart 
%\be
%\label{defPsiAZ}
%\psi_{a(z)} : (\Lambda, M, r\Theta) \to (\lambda(z) + \Lambda, \, \mu(z) + M, \, \cos(r)\theta(z)+ \sin(r) \Theta)
%\ee
%where $|\Theta| = 1$. 
We consider a fixed point $z\in \Omega$, and we distinguish the two cases $\lambda(z) \neq \mu(z)$ and $\lambda(z) = \mu(z)$.

\paragraph{Proof in the case $\lambda(z) \neq \mu(z)$.}
For each $a=(\lambda, \mu, \theta)\in \cA$ we define a norm $\|\cdot \|_a$ on the tangent space $\R\times \R \times \theta^\perp$ to $\cA$ at the point $a$ : for all $A = (\Lambda, M , \Theta)\in \R\times \R \times \theta^\perp$
$$
\|A\|_a = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \frac 1 2 \left| \frac \lambda \mu - \frac \mu \lambda\right| \|\Theta\|\right\}.
$$
We have by construction 
\be
\label{eqDilADZDH}
\dil_z(\psi_{a(z)}^{-1}\circ a\sep d_H, \|\cdot \|_{a(z)}) = D_z(a)_\times
\ee
According to Lemma \ref{lemmaDelta} and Proposition \ref{propPhiTimes} we have for any $a=(\lambda, \mu, \theta)\in \cA$ and any $A\in \R\times\R \times \theta^\perp$
$$
\|A\|_a \leq \|d_a \vp_\times(A)\|_\infty = \|d_0 (\vp_\times \circ \psi_a)\|_\infty \leq 2 \|A\|_a.
$$
Since $\vp_\times$ is $C^1$ it follows from \iref{eqDilDiff} that 
$$
1 \leq \dil^*_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq \dil_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq 2.
$$
Combining \iref{eqDilPhiA}, \iref{eqDilADZDH} and the last inequality we obtain
$$
D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times,
$$
which establishes the announced result \iref{eqDilTimes} in the case $\lambda(z)\neq \mu(z)$. A similar reasoning establishes the counterpart \iref{eqDilPlus} of this ineaquality for the distance $d_+$. 

\paragraph{Proof in the case $\lambda(z) = \mu(z)$.}
%We now turn to the case of equality $\lambda(z) = \mu(z)$.
For any $\ve>0$ and any $a=(\lambda, \mu, \theta)\in \cA$ such that $\lambda = \mu$ we define a norm $\|\cdot\|_{a,\ve}$ on the tangent space $\R\times \R\times \theta^\perp$ to $a$ in $\cA$ as follows : 
$$
\|A\|_{a, \ve} = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \ve \|\Theta\|\right\}.
$$
%$$
%d_z^\ve((\Lambda, M, r\Theta), (\Lambda', M', r'\Theta')) := \max \left\{\frac {|\Lambda-\Lambda'|} {\lambda(z)},\, \frac {|M-M'|} {\mu(z)}, \, \ve \|r\Theta - r'\Theta'\|\right\}.
%$$
This modification is required because the original norm $\|\cdot\|_a$ used in the case $\lambda\neq \mu$ is only a semi-norm when $\lambda = \mu$.
Reasoning similarly to the case $\lambda(z) \neq \mu(z)$ we obtain the upper bound
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H), \ \ve\dil_z(\theta\sep  d_H)\right\}.
$$
We now establish a lower bound on $\dil_z(H)_\times$.
We may assume that $\dil_z(\theta \sep d_H) < \infty$ otherwise there is nothing to prove. Since $\ve>0$ is arbitrary we thus obtain 
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda, d_H), \ \dil_z(\ln \mu, d_H)\right\} = 2D_z(a)_\times.
$$
We now turn to the lower bound on $\dil_z(H)_\times$. 
For that purpose we define the functions $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda,\mu\}$  and we observe that for all $z,z'\in \Omega$
\begin{eqnarray*}
d_\times (H(z),H(z')) &=& \ln \max \{\|H(z)^\frac 1 2 H(z')^{-\frac 1 2}\|, \, \|H(z')^\frac 1 2 H(z)^{-\frac 1 2}\|\}\\
&\geq & \frac 1 2 \max \{|\ln \|H(z)\|- \ln \|H(z')\||, \, |\ln \|H(z)^{-1}\|- \ln \|H(z')^{-1}\||\\
&=& \max \{ |\ln\gamma(z) - \ln \gamma(z')|,\, |\ln \Gamma(z) - \ln \Gamma(z')|\}.
\end{eqnarray*}
We thus obtain
$$
\dil_z(H)_\times = \dil_z(H\sep d_\times, d_H) \geq \max \{ \dil_z(\ln \gamma\sep d_H), \, \dil_z(\ln \Gamma \sep d_H)\}.
$$
Hence according to Proposition \ref{propDilMax}
$$
\dil_z(H)_\times \geq \max \{\dil_z(\ln \lambda\sep d_H), \dil_z(\ln \mu\sep d_H)\} = D_z(a)_\times.
$$
Therefore $D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times$, and proceeding likewise we obtain $D_z(a)_+ \leq \dil_z(H)_+ \leq 2 D_z(a)_+$, which concludes the proof of Theorem \ref{th2Spaces}. \\

Our first corollary estimates the dilatation in with respect to the euclidean distance, instead of the riemanian distance, of the variable $\theta$ in a graded metric having an eigenspace of dimension $d-1$ at each point..

\begin{corollary}
\label{corolDilThetaG}
Under the hypotheses of Theorem \ref{th2Spaces} we have
%Let $H\in \bH_g$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$ such that $H = \cH\circ a$ on $\Omega$. Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$. Then
$$ 
|\lambda(z) - \mu(z)| \dil_z(\theta) \leq 2 D_z(a)_\times %\leq 2.
$$
\end{corollary}
\proof
Furthermore we have according to \iref{eqDilNormLM}
\begin{eqnarray*}
 |\lambda(z) - \mu(z)| \dil_z(\theta)
&\leq& \frac {|\lambda(z) - \mu(z)|}{\min\{\lambda(z), \mu(z)\}} \dil_z(\theta\sep d_H)\\
&=& \left(\frac {\max \{\lambda(z), \mu(z)\}}{\min\{\lambda(z), \mu(z)\}}-1\right)\dil_z(\theta\sep d_H)\\
& \leq & \left|\frac {\lambda(z)} {\mu(z)}-\frac {\mu(z)} {\lambda(z)}\right|\dil_z(\theta\sep d_H) \\
&\leq & 2 D_z(a)_\times% \leq 2.
\end{eqnarray*}
\sq


The next corollary shows how a quasi-acute metric can be obtained from a graded one.
We denote by $\diag(\lambda_1, \cdots, \lambda_d)$ the diagonal matrix of entries $\lambda_1, \cdots, \lambda_d$. 
Let $M\in S_d$ and let $U\in \cO_d$ and $\lambda_1, \cdots , \lambda_d\in\R$ be such that 
\be
\label{eqDiagSd}
M = U^\trans \diag(\lambda_1, \cdots , \lambda_d) U
\ee
For any $\alpha\in \R$ we define the matrix $\max \{\alpha, M\}\in S_d^+$ as follows
$$
\max\{\alpha, M\} := U^\trans \diag(\max\{\alpha, \lambda_1\}, \cdots, \max\{\alpha, \lambda_d\})U,
$$
and we observe that $\max\{\alpha, M\}$ does not depend on the choice of the matrix $U$ and on the order of the eigenvalues $\lambda_1, \cdots, \lambda_d$ in the decomposition \iref{eqDiagSd}.
For instance we have for any $(\lambda, \mu, \theta)\in \cA$ and any $s>0$  
$$ %\lambda^{-2} \theta\theta^\trans+ \mu^{-2} (\Id-\theta \theta^\trans)
\max \{s^{-2}, \cH(a)\} = \min\{s, \lambda\}^{-2} \theta \theta^\trans+ \min\{s, \mu\}^{-2} (\Id-\theta \theta^\trans).
$$

\begin{corollary}
\label{corolHgToHa}
Let $H\in \bH$ be such that $H(z)$ has an eigenvalue of multiplicity $\geq d-1$ for all $z\in \R^d$. We define $s:\R^d\to \R_+^*$ and $H'\in \bH$ as follows : for all $z\in \R^d$
$$
s(z) := \inf_{z'\in \sR^d} |z-z'|+ \|H(z')^{-\frac 1 2}\|,
$$
and 
$$
H'(z) := \max\{s(z)^{-2}, H(z)\}.
$$
If $H\in \bH_g$, then $4^2H'\in \bH_a$.
\end{corollary}

\proof
For each $\ve>0$ we define 
$$
H_\ve := \max\{e^{2 \ve} s(z)^{-2}, H(z)\}.
$$
The proof proceeds as follows: we first establish that for any $z\in \R^d$ one has 
\be
\label{eqDilHe}
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
\ee
We then use these properties to obtain that $4^2 H_\ve \in \bH_a$, and we conclude the proof using the convergence $H_\ve \to H$ as $\ve \to 0$.\\

We first observe that $s : \R^d \to \R_+^*$ is Lipschitz and that $s(z)\leq \|H(z)^{-\frac 1 2}\|$ for all $z\in \R^d$.

Consider a fixed point $z\in\R^d$. If $H(z)$ is proportional to $\Id$, which means that $\|H(z)\|^{-\frac 1 2} = \|H(z)^{-\frac 1 2}\| \geq s(z)$, then $H_\ve = e^{2 \ve} \Id/ s^2$ on a neighborhood of $z$. This implies according to \iref{eqDilLnH} %\ref{PropEquivS}
$$
\dil_z(H_\ve)_\times =\dil_z(H_\ve)_+ = \dil_z(e^{-\ve} s) \leq e^{-\ve}\leq 1,
$$
and therefore \iref{eqDilHe}.
On the other hand if $H(z)$ is not proportional to $\Id$ then there exists three continuous functions $\lambda, \mu \in C^0(\R^d, \R_+^*)$ and $\theta \in C^0(\R^d, \bbS)$ (where $\bbS := \{u\in \R^d \sep |u| = 1\}$) such that 
$
H = \lambda^{-2} \theta \theta^\trans+ \mu^{-2} (\Id - \theta \theta^\trans).
$
on a neighborhood of $z$.
Hence on the same neighborhood of $z$, 
$$
H_\ve = \min\{e^{-\ve} s,\lambda\}^{-2} \theta \theta^\trans+ \min\{e^{-\ve} s,\mu\}^{-2} (\Id - \theta \theta^\trans).
$$

We now establish that $\dil_z(H_\ve)_\times \leq 2$. 
We define $H_\ve^i := e^{2\ve} \Id/ s^2$ and we observe that $H_\ve \geq H_\ve^i$ and $H_\ve \geq H$, hence for any $p,q\in \R^d$
$$
d_{H_\ve}(p,q) \geq \max \{d_H(p,q), \, d_{H_\ve^i}(p,q)\}.
$$
Using Proposition \ref{propDilLoc} we thus obtain  
\begin{eqnarray*}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\} \sep d_{H_\ve}) &\leq& \max \{\dil_z(\ln (e^{-\ve} s)\sep d_{H_\ve}), \,\dil_z(\ln \lambda\sep d_{H_\ve})\}\\
&\leq & \max \{\dil_z(\ln(e^{-\ve} s \sep d_{H_\ve^i})), \,\dil_z(\ln \lambda\sep d_H)\}\\
& \leq & \max \{\dil_z(e^{-\ve} s), \, \dil_z(H)_\times\}\\
& \leq & \max \{e^{-\ve}, 1\} =1,
\end{eqnarray*}
where we used Theorem \ref{th2Spaces} and Proposition \ref{propEquivS} in the third line.
Likewise $\dil_z(\ln \min\{e^{-\ve} s, \lambda\}\leq 1$. 
Since the function 
$$
t \mapsto \frac t \mu - \frac \mu t
$$
is increasing, we easily obtain that
$$
\left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right| \leq \left|\frac \lambda \mu - \frac \mu \lambda\right|.
$$
Therefore   
$$
\frac 1 2 \left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right|  \dil_z(\theta \sep d_{H_\ve}) \leq \frac 1 2\left|\frac \lambda \mu - \frac \mu \lambda\right| \dil_z(\theta\sep d_H) \leq 1,
$$
which implies that $D_z(a_\ve)_\times \leq 1$ where $a_\ve=(\min\{e^{-\ve}s, \lambda\}, \min\{e^{-\ve} s, \mu\}, \theta) \in C^0(\R^d,\cA)$. Hence
$$
\dil_z(H_\ve)_\times \leq 2 D_z(a_\ve)_\times \leq 2.
$$

We now turn to the proof that $\dil_z(H_\ve)_+ \leq 4$.
As already observed in \iref{eqDilNorm}, for any metric space $(X,d_X)$ and any function $f\in C^0(\R^d, X)$ we have 
\be
\label{eqDilNormLM}
\dil_z(f) \leq \|H(z)\|^{\frac 1 2}\dil_z(f\sep d_H) = \frac{\dil_z(f\sep d_H)}{\min\{\lambda(z), \mu(z)\}}.
\ee
If $\lambda(z)<\mu(z)$ we therefore obtain 
\begin{eqnarray*}
\dil_z(\min\{e^{-\ve} s , \lambda\}) &\leq& \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)}\right\}\\
 &\leq& \max \{e^{-\ve}, \, \dil_z(\ln \lambda\sep  d_H)\}\\
 &\leq & \max \{e^{-\ve} , \, 1\} = 1.
\end{eqnarray*}
Still assuming that $\lambda(z)<\mu(z)$, we have $s(z)\leq \|H(z)^{-\frac 1 2}\| \leq \mu(z)$ by construction of $s$, and therefore $\min\{e^{-\ve} s, \mu\} = e^{-\ve} s$ on a neighborhood of $z$. It follows that 
$$
\dil_z(\min\{e^{-\ve} s, \mu\}) = \dil_z(e^{-\ve} s)\leq e^{-\ve} \leq 1.
$$
Proceeding similarly if $\lambda(z)>\mu(z)$ we also obtain $\dil_z(\min\{e^{-\ve} s, \lambda\})$ and $\dil_z(\min\{e^{-\ve} s, \mu\})$. 
We now focus on the local dilatation of the orientation $\theta$, and for that purpose we observe that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}|  \leq  |\lambda(z) - \mu(z)|.
$$
It follows from Corollary \ref{corolDilThetaG} that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}| \dil_z(\theta) \leq D_z(a)_+ \leq 2,
$$
and therefore $D_z(a_\ve)_+ \leq 2$, which implies $\dil_z(H_\ve)_+ \leq 4$.\\

We have established that for all $z\in \R^d$ and all $\ve>0$
$$
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
$$
Hence for any $z,z'\in \R^d$, since $H_\ve \leq e^{2\ve} H'$,
$$
d_\times(H_\ve(z), H_\ve(z')) \leq 2d_{H_\ve}(z,z') \leq 2e^\ve d_{H'}(z,z') \stext{ and } d_+(H_\ve(z), H_\ve(z')) \leq 4|z-z'|.
$$
Letting $\ve \to 0$ we obtain 
$$
d_\times(H'(z), H'(z')) \leq 2d_{H'}(z,z') \stext{ and } d_+(H'(z), H'(z')) \leq 4|z-z'|.
$$
According to Remark \ref{remHomog} this implies that $4^2 H\in \bH_a$, which concludes the proof of this corollary.
\sq


\section{From mesh to metric}
\label{secMeshToMet}
The techniques presented in this section show how to produce an metric $H\in \bH_i$, $\bH_a$ or $\bH_g$ from an isotropic, quasi-acute (in two dimensions), or graded mesh $\cT$.

Combining the next proposition with its counterpart Proposition \ref{propMeshGen}, on the generation of a mesh from a metric, yields the main result of this chapter: Theorem \ref{thEquiv} on the equivalence of the classes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ of meshes and $\bH_i \subset \bH_a \subset \bH_g$ of metrics which is announced in the introduction.
\begin{prop}
\label{propMetGen}
For any $C_0>0$ there exits $C = C(C_0,d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $\cT \in \bT_{i, C_0}$ there exists $H \in \bH_i$ which is $C$-adapted to $\cT$.
\item If $d=2$, then for any $\cT \in \bT_{a, C_0}$ there exists $H \in \bH_a$ which is $C$-adapted to $\cT$.
\item For any $\cT \in \bT_{g,C_0}$ there exists $H \in \bH_g$ which is $C$-adapted to $\cT$.
\end{enumerate}
\end{prop}

The rest of this section is devoted to the proof of this proposition.
For any mesh $\cT\in \bT$, and for any vertex $v$ of $\cT$, we denote by $n_\cT(v)$ the number of simplices in the mesh $\cT$ containing $v$:
$$
n_\cT(v) := \#\{T\in \cT \sep v\in T\}. %, %\text{s.t. } 
$$
We denote by $H_\cT^g\in \bH$ the piecewise linear metric on $\cT$ which satisfies for each vertex $v$ of $\cT$
\be
\label{eqHcTg}
H_\cT^g(v) := \frac 1 {n_\cT(v)} \sum_{\substack{T\in \cT\\\text{s.t. } v\in T}} \cH_T.
\ee
The metric $H_\cT^g$ on a simplex $T\in \cT$ is simply the linear interpolation of the averages of the matrices $\cH_T$ attached to the simplices containing a vertex $v$. 

The next lemma establishes a property of the barycentric coordinates on a simplex, which is useful for the analysis of  the regularity of a piecewise linear function on an anisotropic mesh, such as the metric $H_\cT^g$.
\begin{lemma}
\label{lemmaNormLambda}
Let $T$ be a simplex and let $V$ be the collection of vertices of $T$. Let $\lambda_v(z)$, $v\in V$ be the barycentric coordinates on $T$. Then for all $z,z'\in T$
\be
\label{eqNormLambda}
\|z-z'\|^2_{\cH_T} = \frac {d+1} d \sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2.
\ee
\end{lemma}

\proof
We first assume that $T$ is the reference equilateral simplex $\TEq$. %, and we recall that $\cH_\TEq = \Id$.
For any two vertices $v,v'$ in the collection $\VEq$ of vertices of $\TEq$ one easily checks that 
\be
\label{eqScalTEq}
\<v,v'\> = 
\left\{
\begin{array}{cl}
1 &\text{ if } v=v,'\\
-1/d &\text{ if } v \neq v'.
\end{array}
\right.
\ee
Indeed $|v|=1$ by construction for any vertex $v$ of $\TEq$, the scalar product $\<v,v'\>$ has a value $\alpha$ which is independent of the pair of distinct vertices $v,v'\in \VEq$. Since $\TEq$ is centered at the origin we obtain $0 = \<v,\sum_{v\in V} v\>  = |v|^2 + d \alpha$ which establishes \iref{eqScalTEq}.
We thus obtain for any $z,z'\in \TEq$ 
\begin{eqnarray*}
|z-z'|^2  &=& \left|\sum_{v\in \VEq} (\lambda_v(z) - \lambda_v(z'))v\right|^2 \\
&=& \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \sum_{v\neq v'} (\lambda_v(z)-\lambda_v(z'))(\lambda_{v'}(z)-\lambda_{v'}(z')).
\end{eqnarray*}
Therefore 
$$
|z-z'|^2 =  \left(1+\frac 1 d\right) \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \left(\sum_{v\in \VEq} \lambda_v(z)-\lambda_v(z')\right)^2,
$$
which concludes the proof in the case of $\TEq$ since $\cH_\TEq = \Id$ and since the barycentric coordinates of $z$ and of $z'$ sum to $1$.

We now consider an arbitrary simplex $T$, and an affine change change of coordinates $\Phi$ such that $\Phi(T) = \TEq$, $\Phi(z) = \phi z+ z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. We have $\cH_T = \phi^\trans \phi$ according to \iref{invcH}, hence for all $z,z'\in T$
$$
 |\Phi(z) - \Phi(z')| = |\phi(z-z')| = \|z-z'\|_{\cH_T}.
$$
Furthermore the barycentric coordinates of $z$ and $z'$ in $T$ are the same as those of $\Phi(z)$ and $\Phi(z')$ in $\Phi(T) = \TEq$, hence \iref{eqNormLambda} holds which concludes the proof of this lemma.
\sq



The next proposition establishes that the metric $H_\cT^g$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case iii) of graded meshes. More precisely for any mesh $\cT\in \bT_{g,C_0}$ the metric $d C_0^{10} H_\cT^g$ belongs to $\bH_g$ and is $C_0^6 \sqrt d$ equivalent to $\cT$.



\begin{prop}
\label{propHTG}
For any $\cT\in \bT_{g,C_0}$ the metric $H_\cT^g$ is $C_0$-adapted to $\cT$, and $d C_0^{10} H_\cT^g\in \bH_g$.
\end{prop}

\proof
We consider a simplex $T\in \cT$, and we recall that for any neighbor $T'$ of $T$ one has 
$$
C_0^{-2} \cH_T \leq \cH_{T'} \leq C_0^2 \cH_T.
$$
Averaging these matrices as in \iref{eqHcTg} we obtain for any vertex $v$ of $T$
\be
\label{eqHTHv}
C_0^{-2} \cH_T \leq H_\cT^g(v)\leq C_0^2 \cH_T.
\ee
Averaging with respect to the barycentric coordinates of a point $z\in T$ we eventually obtain 
\be
\label{eqHTHz}
C_0^{-2} \cH_T \leq H_\cT^g(z)\leq C_0^2 \cH_T,
\ee
which establishes as announced that the metric $H_\cT^g$ is $C_0$-adapted to $\cT$.

We now establish the regularity property of $H_\cT^g$, and for that purpose we consider two points $z,z'\in T$ and a vector $u\in \R^d\sm\{0\}$. We thus have 
\begin{eqnarray*}
\frac {\|u\|^2_{H_\cT^g(z)}} {\|u\|^2_{H_\cT^g(z')}} &=& \frac {\sum_{v\in V} \lambda_v(z) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2} \\
&=& 1+ \frac {\sum_{v\in V} (\lambda_v(z)-\lambda_v(z')) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2}\\
&\leq& 1+ C_0^4 \frac{\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|}{\sum_{v\in V} \lambda_v(z')}\\
& \leq & 1+C_0^4 \sqrt {(d+1)\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2}\\
&=& 1+C_0^4 \sqrt d \| z-z'\|_{\cH_T},
\end{eqnarray*}
where we used \iref{eqHTHv} in the third line, Cauchy-Schwartz inequality in the fourth line, and Lemma \iref{lemmaNormLambda} in the fifth line.
We consider a simplex $T\in \cT$ and we intend to give a uniform bound on $\dil_z(H_\cT^g)_\times$ for all $z\in \interior(T)$. It follows from our estimate on $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, and from the analog estimate for  $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, that 
\begin{eqnarray*}
d_\times (H_\cT^g(z), H_\cT^g(z')) &=& \max_{u\neq 0} \left|\ln \|u\|_{H_\cT^g(z)} - \ln \|u\|_{H_\cT^g(z')}\right|\\
&\leq& \frac 1 2\ln (1+C_0^4 \sqrt d \|z-z'\|_{\cH_T}) \\
&\leq& \frac {C_0^4 \sqrt d} 2 \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Hence according to \iref{eqHTHz} and \iref{eqDilNorm} we obtain for all $z\in \interior (T)$
$$
\dil_z(H_\cT^g)_\times \leq C_0^5 \sqrt d.
$$
The metric $H := d C_0^{10} H_\cT^g$ thus satisfies $\dil_z(H)_\times = (dC_0^{10})^{-1/2}\dil_z(H_\cT^g)_\times \leq 1$ for any point $z$ in the interior of any simplex $T\in \cT$.
If follows from Corollary \ref{corolLipNoGamma} that $H \in \bH_g$, which concludes the proof.
\sq

We associate to any mesh $\cT\in \bT$ a metric $H_\cT^i$ defined as follows : for all $z\in \R^d$, 
$$
H_\cT^i(z) := \|H_\cT^g(z)\| \Id.
$$
The next result shows that $H_\cT^i$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case of isotropic metrics. More precisely for any mesh $\cT\in \bT_{i,C_0}$ the metric $d C_0^{10} H_\cT^i$ belongs to $\bH_i$ and is $C_0^7 \sqrt d$ equivalent to the mesh $\cT$.

\begin{corollary}
For any mesh $\cT\in \bT_{i,C_0}$ the metric $H_\cT^i$ is $C_0^2$-adapted to the mesh $\cT$, and $d C_0^{10} H_\cT^i \in \bH_i$.
\end{corollary}

\proof
For any matrix $M\in S_d^+$ we have $\|M^{-1}\|^{-1} \Id \leq M \leq \|M\| \Id$. We therefore obtain for any simplex $T\in \cT$
\be
\label{eqcHNormcH}
C_0^{-2} \|\cH_T\| \Id\leq \frac{\|\cH_T\|} {\rho(T)^2} \Id = \|\cH_T^{-1}\|^{-1} \Id \leq \cH_T \leq \|\cH_T\|\Id.
\ee
Let $T\in \cT$ and let $z\in T$. Since $\rho(T) \leq C_0$ and $C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z)$ we obtain 
$$
C_0^{-2} H_\cT^i(z) := C_0^{-2} \|H_\cT^g(z)\| \Id \leq \|\cH_T\| \Id \leq C_0^2 H_\cT^i(z).
$$
Combining this with \iref{eqcHNormcH} we obtain
$$
C_0^{-4} H_\cT^i(z) \leq \cH_T \leq C_0^2 H_\cT^i(z),
$$
which establishes as announced that the metric $H_\cT^i$ is $C_0^2$ equivalent to the mesh $\cT$.

According to Proposition \ref{propHTG} we have $d C_0^{10} H_\cT^g\in \bH_g$. Corollary \ref{corolLipNorm} thus implies that $d C_0^{10} H_\cT^i\in \bH_i$, which concludes the proof of this proposition.
\sq

Before turning to the case of quasi-acute metrics we prove a lemma on the neighborhood of a simplex in a graded mesh. For any mesh $\cT\in \bT$ and any closed set $E\subset \R^d$ the neighborhood $V_\cT(E)$ of $E$ in $\cT$ is  defined as the union of all simplices $T\in \cT$ which intersect $E$: 
$$
V_\cT(E) := \cup_{\substack{T\in \cT\\T \cap E \neq \emptyset}} T.
$$

\begin{prop}
\label{propNeighborT}
Let $\cT\in \bT_{g,C_0}$ and let $T \in \cT$, then for all $x\in T$ and all $y \in \R^d \sm V_\cT(T)$ we have 
$$
\|x-y\|_{\cH_T} \geq (C_0\sqrt d)^{-1}.
$$
\end{prop}

\proof
The simplex $T\in \cT$ is fixed throughout this proof. We consider the function $\vp : \R^d \to \R$ which is piecewise linear on the mesh $\cT$, and which satisfies for any vertex $v$ of the mesh $\cT$
$$
\vp(v) = 
\left\{
\begin{array}{cl}
1 & \text{ if } v\in T,\\
0 & \text{ if } v \notin T.
\end{array}
\right.
$$
We denote by $V'$ the collection of vertices of a simplex $T'\in \cT$, and by $(\lambda_v(z))_{v\in V'}$ the barycentric coordinates of a point $z\in T'$.
We have for any $z,z'\in T'$
\begin{eqnarray*}
|\vp(z)- \vp(z')| &\leq& \sum_{v \in V'} |\lambda_v(z)-\lambda_v(z')| \vp(v)\\
& \leq &\sqrt{(d+1) \sum_{v\in V'} |\lambda_v(z)-\lambda_v(z')|^2} \\
&= &\sqrt d \|z-z'\|_{\cH_{T'}}.
\end{eqnarray*}
Recalling that $\vp$ is identically $0$ on $T'$ if $T\cap T' = \emptyset$, and that $\cH_{T'} \leq C_0^2 \cH_T$ otherwise, we obtain for any $z,z'\in T'$
$$
|\vp(z)- \vp(z')| \leq C_0\sqrt d \|z-z'\|_{\cH_{T}}.
$$
If follows from Corollary \ref{corolLipNoGamma} that $\vp : (\R^d, \|\cdot \|_{\cH_T})  \to \R$ is $C_0\sqrt d$-Lipschitz.
For any $x\in T$ and any $y\in \R^d\sm V_\cT(T)$ we have $\vp(x) = 1$, $\vp(y) = 0$, thus $1 \leq C_0\sqrt d \|x-y\|_{\cH_T}$ which concludes the proof of this proposition.
\sq

We assume from this point that the dimension is $d=2$. %, and we thus restrict our attention to the bi-dimensional triangulations.
For each triangulation $\cT\in \bT$ we define a function $s_\cT : \R^2 \to \R_+^*$ as follows 
$$
s_\cT(z) := \inf_{z'\in \sR^2} |z-z'| + \|H_\cT^g(z')^{-\frac 1 2}\|.
$$
We define a metric $H_\cT^a \in \bH$ as follows : for each $z\in \R^2$  
\be
\label{defHTA}
H_\cT^a(z) = \max\{s_\cT(z)^{-2} , \, H_\cT^g(z)\}.
\ee

The rest of this section is devoted to proof of the following proposition, on quasi-acute meshes, in two dimensions.
\begin{prop}
\label{propHTA}
For any $C_0 \geq 1$ there exists $C=C(C_0)$ such that the following holds.
For any $\cT\in \bT_{a,C_0}$ the metric $H_\cT^a$ is $C$-adapted to the mesh $\cT$, and $32 C_0^{10} H_\cT^a\in \bH_a$.
\end{prop}

The author is sorry to say that, due to time constraints, this proof is not as polished as the rest of the thesis.

The fact that $32 C_0^{10} H_\cT^a\in \bH_a$ directly follows from the fact that $2 C_0^{10} \bH_\cT^g\in \bH_g$ and from Corollary \ref{corolHgToHa}. 

For each $z\in \R^2$ define $d_\cT(z) := \|H_\cT^g(z)^{-\frac 1 2}\|$. This quantity should be heuristically regarded as the diameter of the triangle containing $z$. We establish below the following property : there exists $\delta = \delta(C_0) >0$ such that for all $z,z'\in \R^2$
\be
\label{eqRegDT}
\text{ if } |z'-z| \leq \delta d_\cT(z) \stext{ then }  d_\cT(z') \geq \delta d_\cT(z).
\ee
Before turning to the proof of \iref{eqRegDT} we show how this property leads to the proof of Proposition \ref{propHTA}.
For all $z\in \R^d$ we have 
$$
s_\cT(z) = \inf_{z\in \sR^2} |z-z'|+d_\cT(z)  \geq \inf_{z'\in \sR^2} \min \{|z-z'|, \, d_\cT(z')\} \geq \delta d_\cT(z'),
$$
indeed $|z-z'|\geq \delta d_\cT(z)$ or $d_\cT(z') \geq \delta d_\cT(z)$ for any $z'\in \R^d$ according to \iref{eqRegDT}.
Combining this with the definition \iref{defHTA} of $H_\cT^a$ we obtain for all $z\in \R^2$
$$
\delta^2 H_\cT^a(z) \leq H_\cT^g(z)\leq H_\cT^a(z). 
$$
Recalling that $H_\cT^g$ is $C_0$-adapted to the mesh $\cT$, see proposition \ref{propHTG}, we obtain for all $T\in \cT$ and all $z\in T$ 
$$
\delta^2 C_0^{-2} H_\cT^a(z) \leq C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z) \leq C_0^2 H_\cT^a(z)
$$
which establishes that the metric $H_\cT^a$ is $C_0/\delta$ adapted to the mesh $\cT$, and concludes the proof of Proposition \ref{propHTA}.\\

For each $u\in \R^2$, we denote by $u^\perp$ the vector obtained by rotating $u$ by $\cPi/2$ in direct trigonometric orientation sense.

We now turn to the proof of \iref{eqRegDT}, and for that purpose we introduce some notations.
For each segment $e=[\omega-u, \omega+u]\subset \R^2$ we define the diamond $\lozenge(e)$ of $e$ as follows
$$
\lozenge(e) := \{z\in \R^2 \sep |\<z-\omega,u\>|+ C_0 |\<z-\omega,u^\perp\>| < |u|^2\}.
$$
This set is illustrated on Figure \ref{figLozenge} (left).

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/LozengeJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/SeqZnJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/TRedJenny.pdf}
\caption{An edge $e$ and the set $\lozenge(e)$ (left), sequence $(z_n)_{n \geq 0}$ (center), diameter of a triangle intersecting $\lozenge(e)$ (right). \label{figLozenge}}
\end{figure}

The next lemma considers a triangulation $\cT'$ on which the measure of sliverness is uniformly bounded by $C_0$, and compares the length an edge $e$ of $\cT'$ with the diameter of the triangles in $\cT'$ which intersect $\lozenge(e)$.

\begin{lemma}
\label{lemmaUUp}
Let $\cT'\in \bT$ be a triangulation such that $S(T) \leq C_0$ for all $T\in \cT'$. Let  $e=[\omega-u, \omega+u]$ be an edge of $\cT'$.
Then there is no vertex in the diamond $\lozenge(e)$, and for all $z\in \lozenge(e)$ and any triangle $T\in \cT'$ containing $z$, there exists an edge $e'= [\omega'-u', \omega'+u']$ of $T$ satisfying  
$$
2 |u'| \geq |u| -C_0 |\<z-\omega,u^\perp\>|/ |u|
%2 |\<u,u'\>| \geq |u|^2 - C_0 |\det (z,u)|.
$$
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$, and we assume up to a translation and a rotation that $\omega = 0$ and $u = u_y$.
We recall that for any triangle $T$, with maximal angle $\theta$, the measure of sliverness $S(T)$ has the following expression
$$
S(T) = \max\{1, \tan(\theta/2)\}.
$$
We assume for contradiction that there exists a vertex $v_0 = (x_0,y_0)\in \lozenge(e)$, and we assume without loss of generality that $x_0<0$. We consider a vertex $v_1 = (x_1,y_1)$ of $\cT$ such that the angle 
$$
\theta_0 :=  \angle(v_1-v_0, \, u_x) \in [-\cPi, \cPi)
$$
has the smallest possible absolute value $|\theta_0|$ (the bold letter $\cPi$ denotes the numerical constant $\cPi = 3.14159\cdots$). By construction there exists a triangle $T\in \cT$ containing $v_0$ and $v_1$ which has an angle  larger or equal or equal than $2\theta_0$ at the vertex $v_0$. It follows that $|\tan \theta_0| \leq S(T) \leq C_0$, and therefore  
$$
|y_1-y_0| \leq |\tan \theta_0| (x_1 - x_0) \leq C_0 (x_1-x_0).
$$
Proceeding inductively, as illustrated on Figure \ref{figLozenge} (center), we define a sequence $z_n = (x_n, y_n)$, $n\geq 0$, of vertices of $\cT$ satisfying 
$
|y_{n+1} - y_n| \leq C_0 (x_{n+1} - x_n). 
$
Adding these inequalities together we obtain 
$$
|y_n-y_0|  \leq C_0 (x_n-x_0).
$$
It follows that one of the edges $[z_n, z_{n+1}]$, $n \geq 0$, of the mesh $\cT'$ intersects the edge $e$, which is a contradiction. The diamond $\lozenge(e)$ therefore does not contain any vertex, which concludes the proof of the first part of this proposition. \\

We now consider a point $z_0 = (x_0,y_0)\in \lozenge(e)$ and we assume without loss of generality that $x_0 \geq 0$. We consider a triangle $T$ containing $z_0$, and an edge $e'= [\omega'-u', \omega'+u']$ of $T$ which is on the left of $z_0$ (in other words the edge $e'$ and the segment $[(0,y_0),(x_0, y_0)]$ joining the point $z_0$ to its orthogonal projection on the edge $e$ intersect). The point $z_0$ and the triangle $T$ are illustrated on Figure \ref{figLozenge} (right).

Since there is no vertex of $\cT'$ in the diamond $\lozenge(e)$, the edge $e'$ intersects the boundary of $\lozenge(e)$ at two points. We denote these points by $(x,y)$ and $(x',y')$, and we assume that without loss of generality that $y\geq 0 \geq y'$.
Observing that $0 \leq x \leq C_0^{-1}$, $0 \leq x'\leq C_0^{-1}$ and $\min\{x,x'\} \leq x_0$ we obtain  
$$
y-y' = (1-C_0 x) - (-1+C_0 x') \geq 1-C_0 x_0.
$$
Since $u = u_y = (0,1)$, $\omega = 0$ and $2 u' = \lambda (x-x', y-y')$ for some $|\lambda| \geq 1$, we obtain 
$$
2|\<u,u'\>| \geq  
y-y' \geq 1-C_0 x_0 = |u|^2 - C_0 |\<z_0-\omega,u\>|,
$$
which concludes the proof of this proposition.
\sq

\begin{figure}
\centering
\includegraphics[width = 4.5cm, height = 4cm]{\pathPic/Dessins/Jenny/LozengeCarreDeltaJenny.pdf}
\includegraphics[width = 2.5cm, height = 4cm]{\pathPic/Dessins/Jenny/CarreDeltaCarreEJenny.pdf}
\caption{An edge $e$, the diamond $\lozenge(e)$ and the rectangle $\square_\delta$ involved in Lemma \ref{lemmaRect} (left), the rectangles $\square_e$ and $\square_\delta$.
\label{figSquare}
}
\end{figure}


We now consider a fixed quasi-acute mesh $\cT\in \bT_{a,C_0}$ and we denote by $\cT'$ a fixed $C_0$-refinement of $\cT$ which satisfies $S(T) \leq C_0$ for all $T\in \cT'$. The next proposition involves a rectangular set $\square(e)$ associated to an edge $e$ of $\cT'$ which contains $e$ in its interior, in contrast to the set $\lozenge(e)$ appearing in the previous proposition.  
This set is illustrated on Figure \ref{figSquare} (right).
\begin{lemma}
\label{lemmaRect}
There exists a constant $\delta_0 = \delta_0(C_0, d)>0$ such that the following holds.
We define the rectangle $\square(e)$ associated to an edge $e = [\omega-u, \, \omega+u]$ of $\cT'$ as follows
$$
\square(e) = \{z\in \R^2 \sep |\<z-\omega, u\>|\leq (1+\delta_0)|u|^2 \text{ and } |\<z-\omega,u^\perp \>| \leq \delta_0 |u|^2\},
$$
%where $\delta_0 = \delta_0(C_0):= ??1/(2C_0) >0$ is a constant specified in the proof.
We have $d_\cT(z) \geq \delta_0|u|$ for all $z\in \square(e)$.
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$. 
Up to a rotation and a translation, we may again assume that $\omega = 0$ and $u = u_y=(0,1)$.
We consider a triangle $T\in \cT$ containing the edge $e$ (note that $e\subset T$ but that $e$ may not be an edge of $T$, since we only known that $e$ is an edge in $\cT'$).

We define $H := H_\cT^g$. Recalling that $H$ is $C_0$-equivalent to $\cT$ we obtain for all $z\in e$
$$
C_0^{-2} H(z)\leq \cH_T \leq C_0^2 H(z). 
$$
The inclusion $e\subset T \subset \cE_T$ implies the upper bound $\|u\|_{\cH_T} = \|u_y\|_{\cH_T} \leq 1$. Hence for all $z\in e$
$$
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq \|u_y\|_{H(z)}^{-1} \geq C_0^{-1}.
$$
Note also that for any $z,u \in \R^2$
$$
d_\times (H(z), H(z+u)) \geq \ln \|H(z)^\frac 1 2 H(z+u)^{-\frac 1 2}\| \geq |\ln d_\cT(z) -\ln d_\cT(z+u)|.
$$
We define $C_1 := \sqrt 2 C_0^5$, in such way that $C_1^2 H\in \bH_g$, and we thus have  according to \iref{eqLocalNorm} if $C_1\|u\|_{H(z)}<1$
$$
|\ln d_\cT(z) -\ln d_\cT(z+u)| \leq d_\times (H(z), H(z+u)) \leq -\ln (1-C_1\|u\|_{H(z)}).
$$
Therefore for all $z\in e$ and all $u\in \R^d$,
$$
d_\cT(z+u) \geq d_\cT(z) (1-C_1 \|u\|_{H(z)}) \geq C_0^{-1}(1-C_1C_0 \|u\|_{\cH_T}).
$$
We define $C_2 := 4C_0C_1$ and we observe that any point of the rectangle 
\be
\label{eqRectGrad}
\left[\frac {-1}{C_2 \|u_x\|_{\cH_T}}, \,\frac 1 {C_2 \|u_x\|_{\cH_T}}\right] \times \left[-(1+C_2^{-1}), \, 1+C_2^{-1}\right].
\ee
can be written under the form $z+u$ where $z\in e$ and $\|u\|_{\cH_T} \leq 1/(2C_0C_1)$. We thus have  
\be
\label{eqdGrad}
d_\cT(z') \geq 1/(2C_0)
\ee
 on this rectangle.

We introduce a small constant $\delta = \delta(C_0)>0$ which is specified later in the proof. It follows from \iref{eqRectGrad} and \iref{eqdGrad} that the proof of this lemma is complete if $\|\cH_T\| \leq \delta^{-2}$, with $\delta_0 := \min \{\delta/C_2, \, 1/(2C_0)\}$.
We thus assume from this point that $\|\cH_T\|\geq \delta^{-2}$.\\

We assume that $\delta< C_0^{-1}$ and we define the rectangle
$$
\square_\delta := [-\delta, \delta] \times [1-C_0 \delta, -1+C_0 \delta],
$$
which is included in $\overline \lozenge(e)$ by construction.
Since $C_1^2 H\in \bH_g$, the function $z\mapsto \|H(z)\|^{-\frac 1 2}$ is $C_1$-Lipschitz according to Corollary \ref{corolLipNorm}. We thus have for all $z = (x,y)\in \square_\delta$
\be
\label{defr0}
\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2}+C_1|x|\leq r_0(\delta) := (C_0+C_1)\delta.
%\|u_x\|_{H(z)} \geq \|u_x\|_{H(y,0)}(1-C_1 |x| \|u_x\|_{H(y,0)}) \geq C_*(1-C_1 C_0 \delta_* C_*),
%\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2} + C_1 |x|
\ee
On the other hand it follows from Lemma \ref{lemmaUUp} that any $z = (x,y)\in \square_\delta$ is contained in a triangle containing an edge $e' = [\omega'-u', \omega'+u']$ such that $|u'| \geq (1-C_0 \delta)/2$. We thus have 
$$
1 \geq \|u'\|_{\cH_{T'}} \geq \frac{|u'|}{ \|\cH_{T'}^{-\frac 1 2}\|} \geq \frac{1-C_0 \delta}{2 \|\cH_{T'}^{-\frac 1 2}\|} 
$$
and therefore 
%of length at least $T'\in \cT$ satisfying $\|\cH_{T'}^{-\frac 1 2}\| \geq (1-C_0 \delta_*)/2$, hence 
\be
\label{defR0}
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq C_0^{-1} \|\cH_{T'}^{-\frac 1 2}\|  \geq  R_0(\delta) := (1-C_0 \delta)/(2C_0). %\det (z,u_y)
\ee
For all $z\in \square_\delta$, we denote by $\theta(z) = (\cos \Theta(z), \sin \Theta(z))$, $\Theta(z)\in [0, \cPi]$, the direction of the eigenvector associated to the small eigenvalue of $H(z)$, in such way that 
\be
\label{eqNormTheta}
\|\theta(z)\|_{H(z)} = \|H(z)^{-\frac 1 2}\|^{-1} = d_\cT(z)^{-1}.
\ee
We thus have for any $(0,y)\in e$
$$
C_0 \geq C_0 \|u_y\|_{\cH_T} \geq \|u_y\|_{H(0,y)} \geq |\cos \Theta(0,y)| \sqrt{\|H(0,y)\|} = \delta^{-1} |\cos \Theta(0,y)| ,
$$
hence 
$$
|\cos \Theta(0,y)| \leq  C_0 \delta.
$$
For all $z\in \square_\delta$ we have according to Corollary \ref{corolDilThetaG} %Theorem \ref{th2Spaces} 
$$
(R_0(\delta)-r_0(\delta)) \dil_z(\Theta) \leq  (\|H(z)^{-\frac 1 2}\| - \|H(z)\|^{-\frac 1 2}) \dil_z(\Theta) \leq 2C_1.
$$
Hence we obtain for all $z= (x,y)\in \square_\delta$  
$$
(R_0(\delta)-r_0(\delta)) |\Theta(z) - \Theta(0,y)| \leq 2C_1 |x|\leq 2C_1 \delta,
$$
hence since $t \mapsto \cos t$ is a Lipschitz function %, since $\cos : [0, \cPi/2]\to \R$ is convex
\be
\label{defTheta0}
|\cos \Theta(z)| \leq \cos \Theta_0(\delta) := C_0 \delta + \frac{\delta}{R_0(\delta)-r_0(\delta)}.
\ee
We have according to \iref{eqLocalNorm} for all $z\in \square_\delta$ and all $r\geq 0$ such that $C_1r\|\theta\|_{H(z)}<1$,
\begin{eqnarray*}
|\ln d_\cT(z+r \theta(z)) - \ln d_\cT(z)| &\leq& d_\times (H(z+r\theta(z)),H(z))\\
&\leq& -\ln (1-C_1r\|\theta\|_{H(z)})\\
&=& -\ln (1-C_1r/d_\cT(z)),
\end{eqnarray*}
therefore 
$$
d_\cT(z+r \theta(z)) \geq  d_\cT(z) (1-|r| C_1 /d_\cT(z)).
$$
For all $z\in \square_\delta$ such that $|r|\leq R_1(\delta) := R_0(\delta)/(2C_1)$ we thus obtain
$$
d_\cT(z+r\theta(z)) \geq R_0(\delta)(1-|r|C_1/R_0(\delta))\geq R_0(\delta)/2.
$$
It follows that $d_\cT(z')\geq R_0(\delta)/2$ for all $z'$ in the set 
$$
\{z+r\theta(z) \sep z\in \square_\delta,\, |r|\leq R_1(\delta)\} \supset [-\delta_0,\delta_0]\times [-(1+\mu_0),1+\mu_0]
$$
where 
\be
\label{eqD0MU0}
\delta_0 := \delta - r \cos \Theta_0(\delta) \stext{ and }  \mu_0 := -C_0 \delta+ r \sin \Theta_0(\delta)
\ee
and where the constant $0 \leq r\leq R_1(\delta)$ can be freely chosen.
The rest of the proof consists in choosing appropriate constants $\delta$ and $r$.\\

As $\delta \to 0$ we have $r_0(\delta)\to 0$, $R_0(\delta) \to 1/(2C_0)$ and $\cos\Theta_0(\delta) \to 0$. We thus choose $\delta = \delta(C_0,d)>0$ sufficiently small in such way that 
\be
\label{eqRCS}
R_0 \geq 1/(4C_0)
, \quad
\cos \Theta_0 \leq 1/(8C_0)
, \quad
\sin \Theta_0 \geq 1/2
.
\ee
We then choose $r := 4C_0 \delta$, which is smaller than $R_1(\delta)= R_0(\delta)/(2C_1) \geq 1/(8C_1C_0)$ if $\delta$ is sufficiently small. Injecting this choice of $r$ and \iref{eqRCS} in \iref{eqD0MU0} we thus obtain 
$$
\delta_0 \geq \delta/2 \stext{ and }\mu_0 \geq C_0 \delta.
$$
We have thus established under the hypothesis $\|\cH_T\|\geq \delta^{-2}$ that 
hence $d_\cT(z) \geq 1/(8C_0)$ for all $z$ in the rectangle 
$$
[-\delta/2, \delta/2]\times [-(1+C_0\delta), 1+C_0 \delta].
$$
Since the case $\|\cH_T\|\leq \delta^{-2}$ is already established this concludes the proof of this proposition.
\sq

The next lemma establishes a technical property on the covering a one dimensional segment by smaller ones, which is a key to the end of this proof.

\begin{lemma}
\label{lemmaCoverSeg}
Let $x_1, \cdots , x_k\in [0,1]$ and let $h_1, \cdots, h_k >0$ be such that 
\be
\label{eqDefXiHi}
[0,1]\subset \bigcup_{1\leq i \leq k} [x_i-h_i, \, x_i+h_i].
\ee
Let $\delta>0$ and let $h_* = h_*(k,\delta) := \exp(1-2k/\delta)/\delta$. Then 
\be
\label{eqInclSeg}
[0,1]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_* \leq h_i}} [x_i-(1+\delta)h_i, \, x_i+(1+\delta)h_i].
\ee
\end{lemma}

\proof
For each $y\in [0,1]$ we denote by $h(y)$ the value $h_i$ associated to the segment $[x_i-h_i, x_i+h_i]$ of smallest length containing $y$.
We thus have 
$$
\int_{[0,1]} \frac {dy} {h(y)} \leq \sum_{1\leq i \leq k} \int_{x_i-h_i}^{x_i+h_i} \frac 1 {h_i} = 2k.
$$
We assume for contradiction that \iref{eqInclSeg} does not hold, and we consider a point $x\in [0,1]$ which does not belong to the right hand side of $[0,1]$. For each $y\in [0,1]$ one of the two following possibilities holds
$$
\delta h(y) < |x-y| \stext{ or } h(y) < h_*.
$$
Integrating we obtain 
$$
\int_0^1 \frac {dy} {h(y)}  \geq \int_0^1 \frac {dy} {\max\{|x-y|/\delta,\, h_*\}}.
$$
The minimum value of the right hand side is attained for $x=0$ or $1$ and equals 
$$
\int_0^1 \frac {dy}{\max \{|x-y|/\delta, h_*\}} = \int_0^{\delta h_*} \frac 1 h_* + \int_{\delta h_*}^1 \frac \delta ydy = \delta(1-\ln(\delta h_*))
$$
Thus $2k>\delta(1-\ln(\delta h_*))$, which contradicts the definition of $h_*$. This concludes the proof of this lemma.
\sq

Under the hypotheses of Lemma \ref{lemmaCoverSeg} we thus have
\be
\label{eqInclSegDouble}
[-h_*\delta,\, 1+h_*\delta]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_i \leq h_*}} [x_i-(1+2\delta)h_i, \, x_i+(1+2\delta)h_i].
\ee


We now conclude the proof of Proposition \ref{propHTA}.
We consider a point $z\in \R^2$ contained in a triangle $T\in \cT$, and we denote by $\cT$ the longest edge $e$ of $T$. Up to a rotation and a translation, we may assume that $e=[0, u_x]$ joins the origin of $\R^2$ to the the vector $u_x := (1,0)$.
Note that 
\be
\label{eqNormHTInv}
2 \geq \|u_x\|_{\cH_T} \geq \|\cH_T^{-\frac 1 2}\|^{-1}.
\ee
Since the triangulation $\cT'$ is a $C_0$-refinement of $\cT$, the edge $e$ of $T$ is built of $k \leq C_0$ edges $(e_i)_{1 \leq i \leq k}$ of $\cT'$,
$$
e_i = [(x_i-h_i)u_x,\,  (x_i +h_i) u_x].
$$
The triangle $T$ and the edges $(e_i)_{1\leq i\leq k}$ are illustrated on Figure \ref{figTFlat} (left).

\begin{figure}
\centering
\includegraphics[width = 7cm, height = 1.5cm]{\pathPic/Dessins/Jenny/TFlatJenny.pdf}
\includegraphics[width = 8cm, height = 2.5cm]{\pathPic/Dessins/Jenny/cupCarresJenny.pdf}
\caption{
A triangle $T\in \cT$ and the edges $(e_i)_{1\leq i \leq k}$ of $\cT'$ contained in $T$ (left), the set \iref{eqRectHoDo} (right). 
\label{figTFlat}}
\end{figure}

We define $h_* := h_*(C_0, \delta_0/2) = 2\exp(1-4C_0/\delta_0)/\delta_0$, where $\delta_0$ is the constant from Lemma \ref{lemmaRect}, and we observe that 
\be
\label{eqRectHoDo}
\bigcup_{h_* \leq h_i} \square(e_i) \supset \left[-\frac{h_* \delta_0} 2, 1+ \frac{h_* \delta_0} 2\right] \times [-h_* \delta_0, h_* \delta_0],
\ee
This set is illustrated on Figure \ref{figTFlat} (right).
Since $e$ is the longest edge of $T$, the angles of $T$ at the extremities of $e$ are acute.
Furthermore the height $h$ of $T$ orthogonal to the edge $e = [0,u_x]$ satisfies 
$$
h/2 = |T|  = \frac{|\TEq|} { \sqrt {\det \cH_T}} = \frac{|\TEq|}{\sqrt{\|\cH_T\| \|\cH_T^{-1}\|^{-1}}}  = \frac{|\TEq| \|\cH_T^{-1}\|}{\rho(T)} \geq \frac{|\TEq|}{4 \rho(T)} .
$$
Hence we obtain with $c := |\TEq|/8$ the inclusion
\be
\label{eqTRectRho}
T \subset [0,1] \times [-c/\rho(T), c/\rho(T)]
\ee
We distinguish two cases depending on the value of $\rho(T)$. If $c/\rho(T) \leq h_* \delta_0$, equivalently $\rho(T) \geq c/(h_* \delta_0)$ we obtain combining \iref{eqRectHoDo} and \iref{eqTRectRho} that $d_\cT\geq h_*\delta_0$ on the set 
$$
z+ \left[-\frac {h_*\delta_0} 2, \frac {h_*\delta_0} 2\right]^2
$$
which concludes the proof of this proposition.
One the other hand we have for any vector $u\in \R^2$
$$
\frac{d_\cT(z+u)}{d_\cT(z)} \geq  1-C_1 \|u\|_{H(z)} \geq 1-C_0C_1 \|u\|_{\cH_T} \geq  1-C_0C_1 \rho(T) |u| \|\cH_T^{-\frac 1 2}\|^{-1} \geq 1-2 C_0C_1 \rho(T) |u| 
$$
which concludes the proof if $\rho(T) \leq c/(h_*\delta_0)$.

\section{From metric to mesh}
\label{secMetToMesh}
%\subsection{Mesh generation}
\label{secMeshGen}

%We prove in this section Theorems \ref{thI}, \ref{thA} and \ref{thR} on the equivalence between certain classes of meshes and of metrics. %, which is divided in two parts.
%This proof is divided in two parts as follows. Proposition \ref{propMeshGen} in \S \ref{secMeshGen} we show how a mesh can be generated from a Riemannian metric, and Proposition \ref{propMetGen} in \S\ref{secMetGen} we show how a metric can be generated from a mesh.
%
This section is dedicated to the proof of the following result, on the generation of a mesh from a metric.
\begin{prop}
\label{propMeshGen}
There exists $C_0 = C_0(d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $H\in \bH_i$ there exists $\cT \in \bT_{i,C_0}$ which is $C_0$-adapted to $H$.
\item If $d=2$, then for any $H \in \bH_a$ there exists $\cT\in \bT_a$ which is $C_0$-adapted to $\cT$.
\item If $d=2$, then for any $H \in \bH_g$ there exists $\cT\in \bT_g$ which is $C_0$-adapted to $\cT$.\end{enumerate}
\end{prop}

Point {\it i)} is established in the \S\ref{secMeshGenI}, point {\it iii)} in \S \ref{secMeshGenG} an eventually {\it ii)} in \S \ref{secMeshGenA}.

%We consider in these proofs a metric $H$ such that $c^2H \in \bH_{\star}$ where $0<c\leq 1$ is a numerical constant and $\star \in \{i,a,g\}$ is a symbol. 

\begin{remark}
\label{remcC}
Let $\star \in \{i,a,g\}$ and let $1\geq c>0$, $C\geq 1$ be numerical constants. 
Assume that for any metric $H$ such that $c^2 H\in \bH_\star$ there exists a mesh $\cT\in \bT_{\star, C}$ which is $C$ adapted to $H$.
Then for any metric $H'\in \bH_\star$ there exists a mesh $\cT' \in \bT_{\star, C}$ which is $C/c$-adapted to $H'$.
(Indeed, choose a mesh $\cT'$ which is $C$-equivalent to the metric $H'/c^2$, and observe that $\cT'$ is $C/c$-equivalent to $H'$)
\end{remark}


\subsection{Isotropic Mesh generation}
\label{secMeshGenI}

\begin{figure}
\centering
\includegraphics[width = 5cm, height = 5cm]{\pathPic/Dessins/Jenny/THalfSquareJenny.pdf}
\caption{A bidimensional triangulation generated by the isotropic refinement procedure
\label{figHalfSquares}}
\end{figure}

The survey paper \cite{Nochetto} describes a the construction of a hierarchical family of meshes of the rectangular domain 
$
[0,1]^d.
$ 
All these meshes are the refinement of a ``fundamental'' mesh $\cT_0 = \{T_\sigma \sep \sigma \in \Sigma_d\}$, where $\Sigma_d$ stands for the collection of permutations of the set $\{1,\cdots,d\}$, and $T_\sigma$ for the Kuhn simplex
$$
T_\sigma := \{z\in [0,1]^d \sep z_{\sigma(1)} \leq \cdots \leq z_{\sigma(d)}\}.
$$
%A sequence $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $A procedure, guided by the user 
%The ``fundamentalbasic mesh $\cT_0$ of $[0,1]^d$ 
Starting from $\cT_0$, the algorithm described in \cite{Nochetto} produces, guided by the user, a family $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $[0,1]^d$ proceeding as follows. 
Assume that the mesh $\cT_n$ has already been generated.
%Once the mesh $\cT_n$ is defined, the mesh $\cT_{n+1}$ is obtained as follows.
%\begin{enumerate}
%\item (Marking) The user selects
%\item (Refinement)
%\end{enumerate}
%The mesh $\cT_{n+1}$ is produced from $\cT_n$ as follows 
\begin{itemize}
\item (Marking)
The user selects a subset $\cM_n \subset \cT_n$.
\item (Refinement)
The algorithm generates a $2$-refinement $\cT_{n+1}$ of $\cT_n$,  
$$
\cT_{n+1} := \Refine(\cT_n, \cM_n).
$$
which does not contain any of the marked simplices : $\cT_{n+1} \cap \cM_n = \emptyset.$
\end{itemize}
\noindent

The elements of the meshes $(\cT_n)_{n \geq 0}$ have a very specific structure, which main features are described below.
\begin{property}
\label{propertyIso}
Any simplex $T$ produced by this algorithm possesses the following properties.
\begin{enumerate}[a)]
\item (Discrete Volumes) The volume of $T$ has the form
\be
\label{eqVolTG}
|T| = \frac {2^{-g(T)}}{d!},
\ee
where $g(T)\geq 0$ is an integer called the ``generation'' of $T$.
\item
(Finite number of classes)
The simplex 
$$
2^{\frac{g(T)} d} (T-z_T),
$$
which is centered at the origin and has volume $1/d!$, %$\frac 1 {d!}$, 
belongs to a finite family $\gT_0$ of simplices.
%\item
%(Vertices lie on a grid)
%The vertices of $T$ lie on the grid
%$$
%2^{-\left\lceil \frac {g(T)} d\right\rceil} \Z^d
%$$
\end{enumerate}
\end{property}
The survey paper \cite{Nochetto} also contains a result, Proposition 4.1, which establishes that $\cT_{n+1} := \Refine(\cT_n, \cM_n)$ is a \emph{local} refinement of $\cT_n$ in the following sense: for all $T'\in \cT_n \sm \cT_{n+1}$ there exists $T\in \cM_n$ such that 
\be
\label{eqDG}
g(T)\geq g(T') \stext{ and } d(T,T') \leq D \, 2^{-g(T')/d},
\ee
where $D = D(d)$ is a fixed constant and where 
$$
d(T,T') := \min\{|z-z'| \sep z\in T, \, z'\in T'\}.\\
$$

The next lemma shows that this refinement algorithm can be used to produce a conforming isotropic mesh $\cT$ of the unit cube $[0,1]^d$, such that the diameters $\diam(T)$, $T\in \cT$, are specified by a given Lipschitz function.

\begin{lemma}
\label{lemmaSCube}
%There exists $C=C(d)$ such that the following holds.
Let $s:[0,1]^d\to  (0,\sqrt d]$ be a $c$-lipschitz function, where $0<c\leq 1$. Let $(\cT_n)_{n \geq 0}$ be the sequence of meshes produced by the algorithm when the collection $\cM_n\subset \cT_n$ of marked simplices is defined as follows
\be
\label{defMn}
\cM_n := \left\{T\in \cT_n \sep \min_T s < \diam(T)\right\}.
\ee
Then the sequence of meshes stabilizes : there exists $N\geq 0$ such that $\cT_n = \cT_N$ for all $n \geq N$. Furthermore we have for all $T\in \cT_N$ and all $z\in T$
\be
\label{eqEquivCube}
\diam(T) \leq s(z) \leq C_s \diam(T).
\ee
where 
\be
\label{defCs}
C_s := 2^\frac 1 d \frac {D_+ (1+c) + c D}{D_-}
\ee
where $D_+ := \max\{ \diam(T) \sep T \in \gT_0\}$ and $D_- := \min\{ \diam(T) \sep T \in \gT_0\}$.
\end{lemma}

\proof
We first show that for any $n \geq 0$ any $T_*\in \cT_n$ and any $z\in T_*$ we have $s(z) \leq C_s \diam(T_*)$.

Indeed if $T_*\in \cT_0$ then 
$$
s(z) \leq \sqrt d =  \diam(T_*) \leq C_s \diam(T_*)
$$
since $C_s\geq 1$ and since $s$ is uniformly bounded by $\sqrt d$.

Otherwise $T_*$ has a father $T'$ which was bisected in the refinement process, hence there exists a simplex $T$ such that \iref{eqDG} holds and which was selected for bisection, hence $\min_T s < \diam(T)$.

We thus obtain for any $z\in T$
\begin{eqnarray*}
s(z) &\leq& \min_T s+ c(\diam(T') + d(T,T'))\\
& \leq & \diam(T)+c(\diam(T') + d(T,T'))\\
& \leq & D_+ 2^{-g(T)/d} + c(D_+2^{-g(T')/d} + D 2^{-g(T')/d})\\
& \leq &  2^{-(g(T_*)-1)} (D_+(1+c)+cD)\\
& \leq & C_s \diam(T_*),
\end{eqnarray*}
which concludes the proof of the right part of \iref{eqEquivCube}.

From the fourth line of this inequality we also obtain an uniform lower bound on the volume of the simplices generated by the refinement procedure
$$
|T_*| = \frac{2^{-g(T_*)}}{d!} \geq c_0 := \frac{\min\{ s(z) \sep z\in [0,1]^d\}}{d! 2^\frac 1 d  (D_+(1+c)+cD)}.
$$
It follows that $\#(\cT_n)$ is uniformly bounded by $1/c_0$, which immediately implies that the sequence $(\cT_n)_{n \geq 0}$ of meshes stabilizes.

Let $N$ be such that $\cT_n = \cT_N$ for all $n \geq N$. We thus have $\cM_N = \emptyset$ and therefore $\diam(T) \leq \min_T s$ for all $T\in \cT_N$, which implies the left part of \iref{eqEquivCube}.
\sq

The rest of this section is devoted to the proof the point i) of Proposition \ref{propMeshGen}.
We thus consider a metric $H\in \bH_i$, and we recall there exists a Lipschitz function $s: \R^d \to \R_+^*$ such that for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2}.
$$
For each $n\geq 0$ we define a function $s_n : [0,1]^d \to \R_+^*$, which is clearly Lipschitz, as follows
\be
\label{defSn}
s_n(z) := 2^{-n} s(2^n (z-z_0))
\ee
where $z_0 = (1/2, \cdots , 1/2)$ is the barycenter of the cube $[0,1]^d$.
%The function $s_n$ is clearly Lipschitz, and 
For all $z\in [0,1]^d$ and all $n \geq 0$ we have 
$$
s_n(z) \leq s_n(z_0) + |z-z_0| \leq 2^{-n} s(0) + \frac {\sqrt d} 2.
$$
The function $s_n$ is therefore uniformly bounded by $\sqrt d$ on $[0,1]^d$ when $n$ is sufficiently large.
We denote by $\cT^n$ the mesh of the cube $[0,1]^d$ described by Lemma \ref{lemmaSCube} for the function $s_n$. We thus have %for all $T\in \cT^n$
\be
\label{eqDiamSn}
\diam(T) \leq s_n(z) \leq C \diam(T) \stext{ for all } T \in \cT^n, \, z\in T.
\ee
where $C=C(d)$ is the constant from Lemma \ref{lemmaSCube}.
We denote by $\cT_n$ the mesh of the cube $[-2^{n-1}, 2^{n-1}]^d$ obtained by translating the mesh $\cT^n$ by $-z_0$ and dilating it by $2^n$. In mathematical terms: % In condensed notations
$$
\cT_n := \{2^n(T-z_0)\sep T \in \cT^n\}.
$$
%$$
%\cT_n := 2^n (\cT^n -z_0).
%$$
In view of \iref{defSn} and \iref{eqDiamSn} we thus have 
\be
\label{eqMinSDiamT}
\diam(T) \leq s(z) \leq C \diam(T) \stext{ for all } T \in \cT_n,\, z\in T,
\ee
We denote by $C_0$ the smallest constant such that for all $T$ in the finite set $\gT_0$ one has 
$$
 \frac{C_0^{-2} \Id}{\diam(T)^2} \leq \cH_T \leq \frac{C_0^2\Id}{C^2\diam(T)^2 },
$$
and we thus obtain for all $T\in \cT_n$ and all $z\in T$
\be
\label{eqHHTIso}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Unfortunately the mesh $\cT_n$ does not cover $\R^d$ but only the cube $[-2^{n-1}, 2^{n-1}]$. 
The next lemma shows that a global mesh $\cT$ of the infinite domain $\R^d$ can be extracted from the sequence of meshes $(\cT_n)_{n\geq 0}$.

\begin{lemma}
\label{lemmaExtractMesh}
Let $(\Omega_n)_{n \geq 0}$ be an increasing sequence of polygonal domains of $\R^d$, which exhausts $\R^d$ in the following sense:
$$
\bigcup_{n \geq 0} \Omega_n = \R^d \stext{ and } \Omega_n \subset \Omega_{n+1} \text{ for all } n\geq 0.
$$
Let $H \in \bH_g$, let $(\cT_n)_{n \geq 0}$ be a sequence of conforming simplicial meshes of the domains $\Omega_n$, and assume that for all $n \geq 0$, all $T\in \cT_n$ and all $z\in T$ one has 
\be
\label{eqHHTConv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Then there exists a mesh $\cT\in \bT$ such that 
$
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
$
for all $T\in \cT$ and all $z\in T$.
\end{lemma}

\proof
The heuristic idea of this proof is to ``extract a converging subsequence'' from the sequence $(\cT_n)_{n \geq 0}$ of meshes. Unfortunately meshes are discrete objects of combinatorial nature, and the convergence of meshes has no meaning a priori. We therefore use Lipschitz functions as an intermediate object, for which convergence is well defined and which benefit of a compactness property.\\

We associate a function $\phi_T : \R^d \to \R$ to each simplex $T$, which is defined as follows. The function $\phi_T$ is supported on $T$, and for all $z\in T$ we have in terms of the barycentric coordinates $\lambda_v(z)$ of $z$ with respect to the vertices $v\in V$ of $T$:
%To each simplex $T$ of vertices $V$, and barycentric coordinates $(\lambda_v)_{v\in V}$ we associate the function 
$$
\phi_T(z) := \min_{v\in V} \lambda_v(z).
$$
%The maximum of this function has value $1/d$ and is attained at the barycenter $z_T$ of $T$. Furthermore for each $z\in T$ and each $0\leq r \leq 1$ one easily checks that 
%$$
%\phi_T(z+r(z-z_T)) \geq r/d.
%$$
According to Lemma \ref{lemmaNormLambda}, we have for any $z,z'\in T$ and any $v\in V$
$$
|\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T},
$$
hence 
\be
\label{eqPhiLip}
|\phi_T(z) - \phi_T(z')| \leq \max_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T}.
\ee

For all $n \geq 0$ we define a function $\phi_n$ on $\R^d$ as follows
$$
\phi_n := \sum_{T \in \cT_n} \phi_T.
$$
It follows from \iref{eqHHTConv} and \iref{eqPhiLip} that for all $T\in \cT_n$ and all $z\in \interior(T)$
$$
\dil_z(\phi_n\sep d_H) \leq C_0.
$$
Since in addition $\phi_n = 0$ on $\R^d \sm \Omega_n$ it follows from corollary \ref{corolLipNoGamma} that $\phi_n : (\R^d,d_H) \to \R$ is $C_0$-Lipschitz. Since the space $(\R^d, d_H)$ is locally compact, due to Proposition \ref{propEuclidRiemann}, Ascoli's compactness theorem states that there exists 
subsequence $(\phi_{n_k})_{k \geq 0}$ which converges uniformly on all compact sets of $\R^d$ to a $C_0$-Lipschitz function $\phi$. 

We therefore assume, up to such an extraction, that 
$
\phi_n \to \phi
$
uniformly on all compact sets of $\R^d$.
We denote by $\cT$ the collection of closures of connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$:
$$
\cT := \left\{ \overline E \sep E \text{ is a connected component of } \{z\in \R^d \sep \phi(z)>0\} \right\}.
$$
For each $z\in \R^d$ and each $n \geq 0$, we denote by $T_n(z)$ the element of $\cT_n$ containing $z$ in its interior if it exists, and $T_n(z) = \emptyset$ otherwise.
If $\phi(z)>0$, then $T_n(z)\neq \emptyset$ for all $n$ sufficiently large, and one easily checks that 
\be
\label{eqTTnz}
T_n(z)\text{ converges in Hausdorff distance to the element }T(z)\in \cT
\ee
 containing $z$. Hence $\cT$ is a collection of simplices, and the convergence $T_n(z)\to T(z)$ in haussdorf distance, combined with the hypothesis $C_0^{-2} H(z) \leq T_n(z) \leq C_0^2 H(z)$, implies that  
\be
\label{eqHHTConv2}
C_0^{-2} H(z) \leq T(z) \leq C_0^2 H(z).
\ee
In order to conclude this proof we need to show that the collection $\cT$ of simplices is a conforming mesh of $\R^d$. We thus have to check the hypotheses of Definition \ref{defSimplMesh}.
The interiors $\interior(T)$, $T\in \cT$ are pairwise disjoint since they are the connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$.
We claim furthermore that $\cT$ covers $\R^d$. Indeed let $z\in \R^d$be arbitrary and for all $n$ let $T_n\in \cT_n$ be such that $z\in T_n$. Since $C_0^{-2} H(z) \leq \cH_{T_n}\leq C_0^2 H(z)$ there exists a subsequence $T_{n_k}$ which converges in the Haussdorf distance to a simplex $T$ containing $z$. We clearly have $T\in \cT$ which establishes as announced that $\cT$ covers $\R^d$.
The fact that $\cT$ is locally finite easily follows from \iref{eqHHTConv2}.\\


We now turn to the proof of the conformity property, and for that purpose we consider an arbitrary Lipschitz function $f : (\R^d, d_H) \to \R$ with compact support. 
Let $T$ be a simplex such that $C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)$. We have for any vertex $v$ of $T$
$$
|f(v) - f(z_T)| \leq d_H(z_T,v) \leq C_0 \|z_T - v\|_{\cH_T} = C_0.
$$
Denoting by $V$ the collection of vertices of $T$ we thus obtain for any $z,z'\in T$
$$
\interp_T f(z) - \interp_T f(z') = \sum_{v\in V} (\lambda_v(z) - \lambda_v(z')) (f(v) - f(z_T)).
$$
Where $\interp_T$ denotes the $\P_1$ (piecewise affine) interpolation on a simplex $T$, and $\interp_\cT$ the $\P_1$ interpolation on a mesh $\cT$.
hence using Lemma \ref{lemmaNormLambda}
\begin{eqnarray*}
|\interp_T f(z) - \interp_T f(z')| &\leq& C_0 \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|\\
 &\leq& C_0 \sqrt{(d+1)  \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|^2} \\
 &=& C_0 \sqrt d \|z-z'\|_{\cH_T}.
\end{eqnarray*}
The last inequality implies that 
$$
\dil_z(\interp_{\cT_n} f \sep d_H)\leq C_0^2 \sqrt d
$$
for all $T\in \cT_n$ and $z\in \interior(T)$.
Let $n_0 \geq 0$ be such that $\supp(f)\subset \Omega_{n_0}$, which implies that $\interp_{\cT_n} f$ is continuous. It follows from Corollary \ref{corolLipNoGamma} that $\interp_{\cT_n} f : (\R^d, d_H) \to \R$ is $C_0^2\sqrt d$-Lipschitz.

We define 
$
D := \cup_{T \in \cT} \interior(T),
$
and we denote by $\interp_T f : D \to \R$ the function which coincides with $\interp_T f$ on the \emph{interior} of each $T\in \cT$. % (and which is possibly discontinuous at the interfaces between the simplices $T\in \cT$). 
For any $z\in D$ we obtain using \iref{eqTTnz} that $\interp_{\cT_n} f(z) \to \interp_\cT f(z)$, hence for any $z,z'\in D$
$$
|\interp_\cT f(z) - \interp_\cT f(z')| = \lim_{n \to \infty} |\interp_{\cT_n} f(z)-\interp_{\cT_n} f(z')| \leq \sqrt d C_0^2 \, d_H(z,z').
$$
The piecewise interpolant $\interp_T f : D \to \R$ therefore extends to a $\sqrt d C_0^2$-Lipschitz function $\interp_T f : (\R^d, d_H) \to \R$. It easily follows that $\interp_\cT f$ is continuous for any compactly supported $C^1$ function $f$. This property characterizes conforming meshes, hence $\cT\in \bT$ which concludes the proof.
\sq



\begin{corollary}(Bidimensional triangulations)
\label{corolBidimIso}
Assume that the dimension is $d=2$. There exists $c>0$ such that the following holds: if $s: \R^2 \to \R_+^*$ is $c$-Lipschitz, then there exist a mesh $\cT$ of $\R^2$ built of half squares, and such that for all $T\in \cT$ and $z\in T$
\be
\label{eqDT32}
\diam(T) \leq s(z) \leq 3 \diam(T)/2.
\ee
\end{corollary}

\proof
When the dimension is $d=2$, the collection $\gT_0$ of triangles contains only half squares, of area $1/2$, hence  $D_+ = D_- = \sqrt 2$. 

As $s \to 0$ the constant $C_s$ defined by \iref{defCs} tends to $\sqrt 2$. Hence $C_s\leq 3/2$ when $s$ is sufficiently small.
If $s$ is bounded by $\sqrt 2$ on $[0,1]^2$ one may therefore produce a mesh $\cT_*$ of $[0,1]^2$ such that \iref{eqDT32} holds for all $T\in \cT_*$, $z\in T$.

From this point construct as before a sequence of meshes $\cT_n$ of the squares $[-2^{n-1}, 2^{n-1}]$ which satisfies \iref{eqDT32}, and we extract a global mesh $\cT$ of $\R^2$ using Lemma \ref{lemmaExtractMesh}. The triangles $T\in \cT$ still satisfy the inequality \iref{eqDT32} since they are limits in the Haussdorff distance of triangles from the triangulations $\cT_n$.
\sq


\subsection{Graded mesh generation}
\label{secMeshGenG}

We prove in this section a result of bi-dimensional mesh generation, Theorem \ref{thEquiMesh}, which implies Point (iii) of Proposition \ref{propMeshGen}. The key ingredients of this section come from the paper \cite{Shew}.
We assume throughout this section that the dimension is $d=2$.

For that purpose we introduce the notion of equispaced points in an abstract metric space.
 Let $(X,d_X)$ be a metric space and let $\delta>0$, we say that a subset $\cV \subset X$ is $\delta$-equispaced if the following holds.
\begin{enumerate}[a)]
\item (Covering) The distance from an arbitrary point $x\in X$ to $\cV$ is bounded by $1$ : for all $x\in X$
\be
\label{eqCover}
d_X(x, \cV) := \inf\{d_X(x,v) \sep v \in \cV\} \leq 1.
\ee
\item (Separation) The pairwise distances between the points of $\cV$ are larger than $\delta$ : for all $v, v'\in \cV$ such that $v \neq v'$
\be
\label{eqSep}
d_X(v,v') \geq \delta.
\ee
\end{enumerate}

The next lemma establishes the existence of such a set under certain assumptions. \begin{lemma}
\label{lemmaEquiSpaced}
Let $(X,d_X)$ be a metric space in which the closed balls $B'(x,r) := \{y\in X \sep d_X(x,y) \leq r\}$ are compact for all $x\in X$ and $r\geq 0$. 
Let $\cV_0$ subset $X$ be such that $d_X(v,v') \geq 1$ for all $v,v'\in \cV_0$ such that $v\neq v'$. Then there exists a $1$-equispaced set $\cV$ of the metric space $(X,d_X)$, containing $\cV_0$.
\end{lemma}

\proof
We may assume that $\cV_0 \neq \emptyset$, up to including an arbitrary point of $X$, and we choose an  arbitrary  $x_0\in \cV_0$.
We define inductively a sequence $(x_n)_{0 \leq n< N}$ of points and $(\cV_n)_{0 \leq n < N}$ of subsets of $X$, where $N\in \N \cup \{\infty\}$ is specified later, proceeding as follows.
Assuming that $\cV_n$ is already defined we consider the closer set 
\be
\label{eqDefXn}
X_n :=  
\{x\in X \sep d_X(x,\cV_n) \geq 1\}.
\ee
If the set $X_n$ is empty, then the sequence ends and we define $N := n+1$. Otherwise we choose $x_{n+1}$ arbitrarily among the minimisers of $d_X(x,x_0)$ on $X^n$:
\be
\label{defxn}
x_{n+1} \in \underset {x\in X_n} \argmin \,d_X(x,x_0),
\ee
and we define $\cV_{n+1} := \cV_n \cup\{x_{n+1}\}$.
Such a minimizer exists since $X_n$ is closed and since the closed balls in $X$ are compact.
%$$
%X^n \cap \overline B\left(x_0, \ 1+ \inf_{x\in X^n} d_X(x_0, x)\right)
%$$
%is compact.
We define $N := \infty$ none of the sets $(X_n)_{n \geq 0}$ is empty. %if the sequence $(x_n)$ is infinite.

We define $\cV := \cup_{0 \leq n <N} \cV_n$.
%We denote by $X_0 := \{x_n \sep 0\leq n<N\}$ the collection of all points of this finite or countable sequence.
%
%We define $N := \infty$ if the sequence $x_0, x_1, \cdots$ is infinite, and we denote by $X_0$ the collection of all points of this finite or countable sequence,
%$$
%X_0 := \{x_n \sep 0 \leq n < N\}.
%$$ 
%%as the collection of all points $x_0, x_1, \cdots$ of this finite or countable sequence.
%, which clearly is finite or countable.
By construction, we thus have $d_X(v, v') \geq 1$ for all $v,v'\in \cV$
which establishes the separation property \iref{eqSep}. %, and shows that $\cV$ is a discrete set.

We now assume for contradiction that the covering property \iref{eqCover} does not hold which implies that $N= \infty$. We choose a point $x_*\in X$ such that $d_X(x_*, \cV)>1$, and therefore $x_*\in X_n$ for all $n \geq 0$. The definition \iref{defxn} of $x_{n+1}$ implies that $d_X(x_0, x_n) \leq d_X(x_0, x_*)$ for all $n \geq 0$, hence the discrete collection of points
$
\{x_n \sep n \geq 0\}
$
in included in the closed ball $\{x\in X \sep d_X(x_0, x) \leq d_X(x_0, x_*)\}$ which is compact.
The sequence $(x_n)_{n \geq 0}$ therefore admits a converging subsequence, but this contradict the fact that the pairwise distances between these points are larger than $1$, which concludes the proof of this proposition.
\sq


%The next lemma gives a simple (from a theoretical point of view) procedure which produces a point set equidistributed with respect to a metric.
%\begin{lemma}
%Let $H\in \bH$ and let $(p_n)_{n\geq 0}$ be a sequence of points obtained by choosing $p_0 = 0$ and then iteratively choosing $p_{n+1}$ among the minimizers of
%\be
%\label{defpn}
%\min\{\|p\| \sep d_H(p, \{p_0,\cdots , p_n\} \geq 1)
%\ee
%
%Then the point set $\cP := \{p_n \sep n \geq 0\}$ is $1$-equidistributed with respect to $H$.
%\end{lemma}
%
%\proof
%The separation holds by construction. It implies in particular that for any $M \geq 1$, $\cP\cap B(0,M)$ is finite. 
%
%%Since $H$ is continuous and positive definite, for each $M$ the set $\{n\geq 0 \sep \|p_n\| \leq M\}$ is finite.
%Indeed let $\Lambda^2 := \max \{\|H(z)\| \sep \|z\| \leq M\}$.
%The balls $B(p, \Lambda/2)$, $p\in \cP\cap B(M)$ are pairwise disjoint. It follows from a volume argument that $\cP\cap B(M)$ is finite.
%
%Let us assume by contradiction that there exists $z\in \R^2$ such that $d(z, \cP)>1$. Then for $n$ large enough we have $\|z\| < \| p_{n+1}\|$ which is incompatible with the construction of $p_{n+1}$ as a minimizer of \iref{defpn}.
%\sq




We consider a fixed metric $H \in \bH$. For any $x,y\in \R^2$ we define 
$$
d_x(y) := \|x-y\|_{H(x)}.
$$
We also consider a fixed discrete collection of vertices, or ``sites'', $\cV \subset \R^2$, and we define the anisotropic Voronoi cell of a site $v\in V$ as follows 
\be
\label{defVorv}
\Vor(v) := \{z\in \R^2 \sep d_v(z) \leq d_w(z) \text{ for all } w \in V\}.
\ee
The anisotropic Voronoi cell $\Vor(v)$ is thus the collection of points $z$ which are \emph{closer to the vertex $v$ than to any other site}.
The classical (isotropic) Voronoi is obtained by choosing $H = \Id$.
We refer to the paper \cite{Shew} Figure 3 for an illustration of the anisotropic Voronoi diagram $\{\Vor(v) \sep v\in \cV\}$ associated to a point set.

For each $z\in \R^2$ we define $\cV_z$ the collection of vertices which contain $z$ in their Voronoi region:
$$
\cV_z := \{v \in \cV \sep z \in \Vor(v)\}.
$$
The geometric dual of the Voronoi diagram is the graph $\cG(\cV,H)$ defined as follows:
\be
\label{defGVH}
\cG(\cV,H) := \{[v,v'] \sep \text{there exists } z\in \R^2 \text{ such that } V_z = \{v,v'\}\}.
\ee

%We define a collection $\cT_0(V,H)$ of convex sets attached to the metric $H$ and to the collection $V$ of sites
%$$
%\cT_0(V,H) := \{\Cvx(V_z) \sep z \in \R^2 \text{ and } \#(V_z) \geq 3\}.
%$$
The next theorem establishes that $\cG(\cV,H)$ is, under certain conditions on the metric $H$ and the set $\cV$, the graph of a triangulation adapted to $H$.

\begin{theorem}
\label{thEquiMesh}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta)\geq 1$ such that the following holds.
Let $H$ be a metric such that $c^2 H\in \bH_g$, and let $\cV$ be a $\delta$-equispaced subset of $(\R^2, d_H)$.
Then the $\cG(\cV,H)$ is a planar graph which defines a partition of $\R^2$ into strictly convex polygons. Arbitrarily triangulating each polygon yields a triangulation $\cT\in \bT_{g,C}$ which is $C$-adapted to $H$, called an anisotropic Delaunay triangulation. Furthermore if $\cV$ is in general position then $\cG(\cV,H)$ is already the graph of a triangulation.
\end{theorem}

Denote by $c$ and $C$ the constants attached to $\delta=1$ in this theorem.
It follows that for any metric $H$ such that $c^2 H \in \bH_g$, there exists a mesh $\cT\in \bT_{g,C}$ which is $C$-adapted to $H$, obtained as the Delaunay triangulation of a $1$-equispaced set of points $\cV\subset (\R^2, d_H)$. 
This immediately implies Point iii) of Proposition \ref{propMeshGen} according to Remark \ref{remcC}.


The rest of this section is devoted to the proof of Theorem \ref{thEquiMesh}, which is based on the methods and results presented in \cite{Shew}. 
%These theorems are based on a property that needs to be 
For that purpose we recall some definitions of this paper. %introduce the following definitions.
\begin{definition}
\label{defWedge}
%The wedge of $v,v'$ is 
\begin{itemize}
\item (Wedge of two points)
We define the wedge $\wed(v,w)$ of two distinct sites $v,w\in V$ as follows
$$
\wed(v,w) := \{z\in \R^2 \sep (z-v)^\trans H(v) (w-v) >0 \text{ and } (z-w)^\trans H(w) (v-w) >0\}
$$ 
\item (Wedge property)
We say that the Voronoi diagram of $V$ is wedged if for any two distinct $v,w \in V$ we have 
$$
\Vor(v) \cap \Vor(w) \subset \wed(v,w).
$$
\end{itemize}
\end{definition}

The wedge property expresses that the collection $\Vor(v) \cap \Vor(w)$ of points $q$ shared by the Voronoi regions of the sites $v$ and $w$ lie in a cone defined by two linear inequalities.
We refer to \cite{Shew} Figure 4 for an illustration of the wedge of two sites.

The next proposition, which is partly is based on Lemma 5 from \cite{Shew},
 shows that the wedge property is automatically satisfied in our context.
For any metric $H$ and any constant $c>0$ such that $c^2H\in \bH_g$, it easily follows from Proposition \ref{propEuclidRiemann} that for all $x,y\in \R^2$
\be
\label{eqDHLog}
\ln (1+ c\, d_x(y)) \leq c \, d_H(x,y) \leq - \ln(1- c\, d_x(y)), 
\ee
which is equivalent to 
\be
\label{eqDHExp}
1-\exp(-c\, d_H(x,y)) \leq c \, d_x(y) \leq \exp(c \, d_H(x,y))-1.
\ee

\begin{lemma}
\label{lemmaDiamVor}
If $c^2 H\in \bH_g$ %and $\cV$ is $\delta$-equispaced, 
then
for any $v\in \cV$ and any $q\in \Vor(v)$ we have 
\be
\label{eqDiamVor}
\|q-v\|_{H(v)} \leq r_0(c) := (e^c-1)/c.
\ee
If $v,w \in \cV$ satisfy $\Vor(v) \cap \Vor(w) \neq \emptyset$, then 
\be
\label{eqVordvw}
%\delta \leq 
d_H(v,w) \leq r_1(c) := -2\ln(2-e^c)/c.
\ee
Note that $r_0(c) \to 1$ and $r_1(c) \to 2$ as $c\to 0$. Note also that $d_H(v,w)\geq \delta$ if $\cV$ is $\delta$-equispaced.
\end{lemma}

\proof
For any $q\in \cV$ there exists $v_* \in \cV$ such that 
$
d_H(q,v_*) \leq 1,
$
and therefore 
$$
\|q-v_*\|_{H(v_*)} \leq r_0(c) := (e^c-1)/c,
$$
which implies \iref{eqDiamVor} using the definition \iref{defVorv} of the Voronoi diagram.
We thus turn to the proof of \iref{eqVordvw} and for that purpose we consider a point $q\in \Vor (v)\cap\Vor(w)$. We thus have
$
\max\{\|q-v\|_{H(v)} , \|q-w\|_{H(w)} \}\leq  v_c%-\ln(1-c v_c)/c
$
hence
$$
d_H(v,w) \leq r_1(c) :=-2\ln(1-c r_0(c))/c,
$$
which concludes the proof.
\sq

\begin{prop}
\label{propWedge}
For each $\delta$ there exists $c=c(\delta)>0$ such that the following holds.\\
If a metric $H$ satisfies $c^2H\in \bH_g$ and if $\cV$ is a $\delta$-equispaced subset of $(\R^2,d_H)$, then the wedge property is satisfied.
\end{prop}

\proof
We assume for contradiction that there exists two distinct vertices $v,w \in V$, and a point $q\in \Vor(V) \cap \Vor(W)$ such that $z\notin \wed(v,w)$. We may assume, up to exchanging the roles of $v$ and $w$, that 
$$
(q-w)^\trans H(w) (v-w) \leq 0.
$$
Defining the ``relative distortion''
$
\tau := \exp d_\times (H(v), H(w))
$
we obtain using Lemma 5 from \cite{Shew} %(*$q$ instead of $z$??*)
\be
\label{eqShewWedge}
 d_w(v) \leq d_w(q) \sqrt{\tau^2-1}.
\ee
We now estimate the quantities $d_w(v)$, $d_w(q)$ and $\tau$ appearing in this estimate, in order to obtain a contradiction when $c$ is sufficiently small.

%Since the set $V$ is $C_0$-equispaced, there exists $u\in V$ such that $d_H(u,q) \leq C_0$. Recalling that $z\in \Vor(v)\cap \Vor(w)$ we thus obtain using \iref{eqDHExp}
%\be
%\label{eqDiamVor}
%d_v(q) = d_w(q) \leq d_u(q) \leq \frac{\exp(c \, d_H(u,q))-1} c \leq r_0(c) := \frac{\exp(c C_0)-1} c,
%\ee
%and therefore using \iref{eqDHLog} 
%\be
%\label{eqVordvw}
%d_H(v,w) \leq d_H(v,q)+ d_H(q,w) \leq r_1(c) := \frac {-2\ln (1- c r_0(c))}  c,% \frac 1 {1-f(c)}.
%\ee
%hence 
We have 
\be
\label{eqTauWedge}
\ln \tau = d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
\ee
Since $\cV$ is $\delta$-equispaced we have 
$
d_H(v,w) \geq \delta
$
and therefore 
\be
\label{eqdvwWedge}
c \,d_w(v) \geq 1-\exp(-c d_H(v,w)) \geq 1-\exp(-c\delta)
\ee
Injecting \iref{eqDiamVor}, \iref{eqTauWedge} and \iref{eqdvwWedge} in \iref{eqShewWedge} we obtain
\be
\label{eqFinalWedge}
\frac{1-\exp(-c\delta )} c \leq \frac{\exp(c)-1} c \sqrt{\exp(2c r_1(c))-1}.
\ee
The left hand side tends to $\delta$ as $c\to 0$, while the right hand side tends to $0$. We thus obtain a contradiction when $c$ is sufficiently small which concludes the proof of this proposition.
\sq

\begin{theorem}[Dual triangulation theorem. Labelle, Shewchuck, \cite{Shew}]
\label{thShew}
If the Voronoi diagram of the point set $\cV \subset \R^2$ is wedged, then the geometric dual of this diagram is a polygonalization of $\R^2$ with strictly convex polygons and is a triangulation $\cT$ if $\cV$ is in general position.
\end{theorem}

Under the hypotheses of this theorem the vertices $v_1, \cdots, v_k$ of a polygon in the dual Voronoi diagram satisfy by construction $\Vor(v_1)\cap \cdots \cap \Vor(v_k) \neq \emptyset$, and therefore the vertices $v_1, v_2, v_3$ of a triangle $T\in \cT$ satisfy $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$.

The next theorem, originally stated in \cite{Shew} as Corollary 10 to Theorem 9 of the same paper, allows to control the angles of a triangle in the anisotropic Delaunay triangulation.

\begin{theorem}[Labelle, Shewchuk, \cite{Shew}]
\label{thAngle}
Let $v_1,v_2,v_3\in \cV$ and let $q\in \Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)$. Let 
$$
r = d_{v_1}(q) = d_{v_2}(q) = d_{v_3}(q) \stext{ and }
l = \min\{d_{v_i}(v_j) \sep i,j \in \{1,2,3\}, i \neq j\}.
$$ 
Define $\beta := \max\{r/l,\, 1/\sqrt 2\}$, %and %$\gamma\in [1,\infty)$ by 
%Let $1\leq \gamma \leq \sqrt 2$ and $\beta \geq \frac 1 {\sqrt 2}$ satisfy
$$
\gamma := \exp \max \{d_\times (H(v_i), H(v_j)) \sep i,j \in \{1,2,3\}, i \neq j\},
$$
and
\be
\label{defChi}
\chi := \frac 1 {2 \beta} - \frac{(\gamma^2-1)\beta} 2.
\ee
If $\gamma \leq \sqrt 2$ and $\chi>0$ then any angle $\theta$ of the triangle of vertices $(\sqrt{H(v_1)} v_k)_{1 \leq k \leq 3}$ satisfies
$$
\arcsin ( \chi/ \gamma^2) \leq \theta \leq 2 \arccos(\chi/\gamma^2).
$$
\end{theorem}

\begin{corollary}
\label{corolAdaptG}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta) \geq 1$ such that the following holds.
If $\cV$ is $\delta$-equispaced, if $c^2H\in \bH_g$ and if $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$, then denoting by $T$ the triangle of vertices $v_1,v_2,v_3$ we have for all $z\in T$
$$
C^{-2} H(z) \leq \cH(z) \leq C^2 H(z).
$$
\end{corollary}
\proof
We use \iref{eqDHExp} and \iref{eqDHLog} and the fact that $V$ is $\delta$-equispaced to obtain explicit bounds on the quantities $r$, $l$, $\beta$, $\gamma$ and $\chi$ appearing in Theorem \ref{thAngle}.
It follows from Lemma \ref{lemmaDiamVor} that 
$$
r\leq r_0(c) \stext{ and } \delta \leq d_H(v_i,v_j) \leq r_1(c).
$$
Therefore 
$$
l := \min_{i\neq j} d_{v_i}(v_j)\geq %\min_{i\neq j} \frac{1-\exp(-c d_H(v_i,v_j))} c \geq  
r_2(c) := (1-\exp(-c\delta))/ c,
$$
and 
$$
L := \max_{i\neq j} d_{v_i}(v_j) \leq (\exp(c r_1(c))-1)/c
$$
and 
$$
\gamma \leq \max_{i\neq j} \exp(c \,d_H(v_i,v_j)) \leq \exp(c \,r_1(c)).
$$
In particular 
$
\beta \leq r_3(c) := \min\{r_0(c)/r_2(c),\, 1/\sqrt 2\}. % = \frac{\exp(cC_0)-1}{1-\exp(-2 cC_0^{-1})},
$
Injecting this into \iref{defChi} yields an explicit lower estimate 
$$
\chi\geq r_4(c) := \frac 1 {2r_3(c)} - \frac{ (\exp(2cr_1(c))-1) r_3(c)} 2,
$$ 
and $\chi/\gamma^2\geq r_5(c) := r_4(c) \exp(-2cr_1(c))$.

For a fixed $\delta$ we obtain as $c\to 0$ the limits $r_0(c) \to 1$, $r_1(c)\to 2 $, $r_2(c) \to \delta$, $r_3(c) \to \min\{\delta, 1/\sqrt 2\}$ and $r_4(c) \to 1/(2\min\{\delta, 1/\sqrt 2\})$ and $r_5(c)$ as the same limit.

%We assume without loss of generality that $\delta \geq 1/\sqrt 2$ and we thus obtain $r_3(c) \to \delta$, 
%$r_4(c) \to 1/C_0^2$ and $r_5(c) \to 1/C_0^2$. 
We may therefore choose $c$ sufficiently small in such way that 
$$
l \geq l_0 := \delta/2, \ L  \leq L_0 := 4 \text{ and }\chi/\gamma^2 \geq \Chi_0 := 1/(4\min\{\delta, 1/\sqrt 2\}).
$$
We denote by $T$ the triangle of vertices $v_1, v_2, v_3$. The length of any edge of $T' := \sqrt{H(v_1)}(T)$ is bounded above by $L_0$ and below by $l_0$ respectively, and the angles of $T'$ satisfy $\arcsin (\Chi_0) \leq \theta \leq 2 \arccos(\Chi_0)$. The collection of triangles centered at the origin which satisfy these inequalities is compact, thus there exists a constant $C_1 = C_1(C_0)$ such that 
$$
C_1^{-2} \Id \leq \cH_{T'} \leq C_1^2 \Id,
$$
hence $C_1^{-2} H(v_1) \leq \cH_{T'} \leq C_1^2 H(v_1)$. For any $z\in T$ we obtain, remarking that $\|z-v_1\|_{\cH_T} \leq 2$ for all $z\in T$ and using \iref{eqLocalNorm}, 
$$
C_1^{-2} (1-2cC_1)^2 H(z) \leq \cH_{T'} \leq C_1^2(1-2cC_1)^{-2} H(z)
$$
which concludes the proof of this proposition, with $C = C_1(1-2cC_1)^{-1}$.
\sq

We now prove of Theorem \ref{thEquiMesh}.
According to the above results for any $\delta>0$ there exists $c = c(\delta)$ and $C=C(\delta)$ such that the following holds. 
For any set $\cV \subset (\R^2, d_H)$ which is $\delta$-equispaced, the Voronoi diagram associated to $\cV$ and $H$ is wedged according to Proposition \ref{propWedge}. The dual of this diagram is therefore a polygonalization of $\R^2$ with strictly convex polygons according to Theorem \ref{thShew}.
Randomly triangulating these cells yields a triangulation $\cT\in \bT$ which is $C$-adapted to $H$ according to Corollary \ref{corolAdaptG}. 

Furthermore consider to simplices $T,T'\in \cT$ such that $T \cap T'\neq \emptyset$, and a point $z\in T \cap T'$.
Then 
$$
C^{-2} \cH_T \leq H(z) \leq C^2 \cH_{T'},
$$
which shows that $\cT\in \bT_{g,C^2}$ and concludes the proof of Theorem \ref{thEquiMesh}.

\subsection{Quasi-Acute mesh generation}
\label{secMeshGenA}

This section is devoted to the proof of Point ii) of Proposition \ref{propMeshGen}, which is obtained by combining the  constructions of isotropic and graded triangulations presented in \S\ref{secMeshGenI} and \S\ref{secMeshGenI} to produce a quasi-acute triangulation. 
The key idea of this proof if that the anisotropic Delaunay triangulation described in the previous subsection contains only \emph{few} strongly obtuse angles if the set $\cV$ of vertices is structured along lines which are \emph{transverse to the direction of anisotropy}, as illustrated on Figure \ref{figAcuteGen} (in the introduction of this chapter). 

The author is sorry to say that this proof is not yet as polished as the rest of the thesis, due to time constraints.

We consider a fixed metric $H$ such that $c^2 H\in \bH_a$, where $c$ is an absolute constant specified in the proof and such that $0<c\leq 1$. This subsection is devoted to the construction of a mesh $\cT\in \bT_{a,C}$ which is $C$-adapted to $H$, where $C$ is an absolute constant also specified in the proof.
This construction immediately implies Proposition \ref{propMeshGen} according to Remark \ref{remcC}. 


For each $z\in \R^2$ we define %We define two functions $\lambda, \mu : \R^2 \to \R$ as follows : for all $z\in \R^2$
$$
\lambda(z) := \|H(z)^{-\frac 1 2}\| \stext{ and } \mu(z) = \|H(z)\|^{-\frac 1 2},
$$
and we observe that $\lambda(z) \geq \mu(z)$.
The functions $\lambda$ and $\mu$ are $c$-Lipschitz according to Corollary \ref{corolLipNorm}.
% : for all $z,z'\in \R^d$
%$$
%|\lambda(z)-\lambda(z')| \leq c|z-z'| \text{ and } |\mu(z) - \mu(z') | \leq c|z-z'|.
%$$
If $c$ is sufficiently small, then there exists according to Corollary \ref{corolBidimIso} a mesh $\cT_0$ such that for all $T\in \cT_0$ and all $z\in T$
\be
\label{ratioDiamLambda}
\frac 2 3  \lambda(z) \leq \diam(T)\leq \lambda(z). 
\ee
The mesh $\cT_0$ is built of half squares by construction (as illustrated on Figure \ref{figHalfSquares}) hence  for any edge $[v,w]$ of any triangle $T\in \cT_0$ we have $\diam(T)/\sqrt 2 \leq |v-w|\leq \diam(T)$, and the diameter of any triangle $T\in \cT_0$ is a power of $\sqrt 2$. Therefore if two triangles $T,T'\in \cT_0$ share a vertex $v$ we obtain 
\be
\label{eqDiamRatio}
\diam(T)/\sqrt 2 \leq \diam(T') \leq \sqrt 2 \diam(T),
\ee
which implies for any edges $[v,w]$ and $[v,w']$ (sharing the vertex $v$) of the triangulation $\cT_0$ 
\be
\label{eqEdgeRatio}
|v-w|/2 \leq |v-w'| \leq 2|v-w|.
\ee
Inequality \iref{ratioDiamLambda} also implies that for any edge $[v,w]$ of $\cT_0$
%We say that two vertices $v,w\in \cV_0$ are neighbors in $\cT_0$ if they belong to a common triangle $T\in \cT_0$.
%In that case we have %Let $v,w$ be two vertices of a triangle $T\in \cT_0$, then 
\be
\label{edgeLambda}
\frac{\lambda(z)\sqrt 2}3 \leq \frac{\diam(T)}{\sqrt 2}\leq |v-w| \leq \diam(T)\leq \lambda(z)
\ee
We denote by $\cV_0$ the collection of vertices of $\cT_0$. 
Consider a fixed $v\in \cV_0$ any vertex $w\in \cV_0$ such that $|v-w|$ is minimal. Then $[v,w]$ is clearly an edge of $\cT_0$. This implies for any distinct $v,w\in \cV_0$
\be
\label{pairwiseV0}
\lambda(v) \frac {\sqrt 2} 3 \leq |v-w| .
\ee


For each $z\in \R^2$ we define 
$$
\rho(z) := \lambda(z)/\mu(z)  = \sqrt{\|H(z)\| \|H(z)^{-1}\|} \in [1, \infty).
$$
Consider $z,z'\in \R^2$ such that $|z-z'| \leq r\lambda(z)$, where $r\geq 0$ is a constant. Then since $\lambda$ and $\mu$ are $c$-Lipschitz we obtain 
\be
\label{eqrhozzp}
\rho(z') = \frac{\lambda(z')}{\mu(z')} \geq \frac{\lambda(z)(1-r c)}{\mu(z)+ r c \lambda(z)} \geq \frac {1-r c}{\rho(z)^{-1}+r c}.
\ee
For each $\rho_0, r_0$ we denote by $c_\rho(\rho_0, r_0)>0$ the constant such that $\rho_0 = \frac {1-r_0 c_\rho(\rho_0, r_0)}{(\rho_0+1)^{-1}+r_0 c_\rho(\rho_0, c_0)}$.
For any $z,z'\in \R^2$ we thus have
$$
\left\{
\begin{array}{c}
|z-z'| \leq r_0\lambda(z)\\ 
\rho(z) \geq \rho_0+1\\
c\leq c_\rho(\rho_0, r_0)
\end{array}
\right.
%\Big(|z-z'| \leq r_0\lambda(z) , \ \rho(z) \geq \rho_0+1 \text{ and } c\leq c_\rho(\rho_0, r_0)\Big) 
\stext{ implies } \rho(z') \geq \rho_0
$$
For instance if $z,z'$ belong to the same triangle $T\in \cT_0$, if $\rho(z) \geq n+1$ and $c\leq c_\rho(n,1)$ then $\rho(z') \geq n$ according to \iref{edgeLambda}. 
%Throughout this proof we shall make a finite number of assumptions of the type $c \leq c_\rho(r_0,\rho_0)$ for some absolute constants $r_0, \rho_0$. They hold if $c$ if sufficiently small.

For each $z\in \R^2$ such that $\rho(z)>1$ we denote by $\theta(z)\in \bbS := \{u\in \R^2\sep |u| = 1\}$ a unit vector such that
\be
\label{defAngle}
H(z) = \lambda(z)^{-2} \theta(z) \theta(z)^\trans+ \mu(z)^{-2} (\Id-\theta(z) \theta(z)^\trans).
\ee
Note that there exists two, opposite, choices for the vector $\theta(z)$.
For each $u,u'\in \R^2 \sm\{0\}$ we define the (unoriented) angle
$$
\varangle (u,u') := \arccos \left(\frac{\<u,u'\>}{|u| |u'|}\right) \in [0,\cPi].
$$
and 
%For any two vectors $u,u'\in \R^2\sm\{0\}$ we define %the non-oriented, acute, angle
$$
\lhd(u,u') := \min \{\varangle(u,u'),\, \varangle(u,-u')\} = \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
$$
\begin{lemma}
If $c$ is sufficiently small, then the following holds.
For any $z,z'\in \R^2$ 
$$
\left\{
\begin{array}{c}
\rho(z) \geq 2\\
|z'-z|\leq 10 \lambda(z) 
\end{array}
\right.
\stext{ implies }
\lhd(\theta(z), \theta(z')) \leq \cPi/12.
$$
\end{lemma}

\proof
We consider a fixed point $z$ such that $\rho(z) \geq 3$ and we denote by $B$ the ball $\{z'\in \R^2\sep |z'-z| \leq 10 \lambda(z)\}$.
For each $z'\in B$ we have
\begin{eqnarray*}
\lambda(z') - \mu(z') &\geq& (\lambda(z)-c|z-z'|) - (\mu(z)+ c |z-z'|) \\
&=& \lambda(z) -\mu(z) -2 c |z-z'| \\
&\geq& \lambda(z) -\lambda(z)/ 3 - 20 c\lambda(z)\\
&=& \lambda(z)(2/3 -20 c),
\end{eqnarray*}
hence $\lambda(z') - \mu(z')\geq \lambda(z)/2$ if $c \leq 1/120$ which we assume from this point.

Furthermore since $B$ is simply connected there exists a continuous function $\theta_* : B \to \bbS$ (where $\bbS := \{u\in \R^2 \sep |u|=1\}$ denotes the unit circle) such that $\theta_*(z')  = \pm \theta(z')$ for all $z'\in B$.
According to Theorem \ref{th2Spaces} we have for all $z'\in B$
$$
\lambda(z)\dil_{z'}(\theta_*) \leq 2(\lambda(z')-\mu(z')) \dil_{z'}(\theta_*) \leq 2c.
$$
Therefore 
$$
\lhd(\theta(z), \theta(z'))\leq \varangle(\theta_*(z), \theta_*(z')) \leq |z-z'| \max_{\ti z \in [z,z']} \dil_{\ti z}(\theta_*) \leq 20c 
$$
which concludes the proof if $20c \leq \cPi/12$.
\sq

%For any $u,u'\in\bbS := \{v\in \R^2 \sep |v|=1\}$, the angle $\varangle (u,u')$ coincides with the distance $d_\bbS(u,u')$ used in \S\ref{secEigen}. %Note that the angle coincides with the distance on 
%For any triangle $T\in \cT_0$ of vertices $v,w,w'$ we thus have $\varangle(w-v,w'-v) \in \{\cPi/4, \cPi/2\}$. For each $u\in \R^2$ we denote by $u^\perp$ the vector obtained by rotating the vector $u$ by $\cPi/2$ is direct trigonometric sense.\\

%This quantity is used to measure the angle formed by two vectors with no clear orientation.
Formula \iref{eqDilThetaA} had an immediate corollary.
\begin{corollary}
\label{corolTheta2C}
Let $T\in \cT_0$ be such that $\rho\geq 2$ on $T$. Then for any $z,z'\in T$ and any $\theta(z), \theta(z')\in \bbS$ such that \iref{defAngle} holds, we have 
$$
\lhd(\theta(z), \theta(z')) \leq 2c.
$$ 
\end{corollary}

\proof
Since $T$ is a simply connected domain and $\rho \geq 2$ on $T$, there exists a continuous map $\theta_*\in C^0(T, \bbS)$ satisfying \iref{defAngle} at each point.
We thus have 
$$
\lhd(\theta(z), \theta(z')) = \lhd(\theta_*(z), \theta_*(z')) \leq \varangle(\theta_*(z), \theta_*(z'))  \leq \diam(T) \max_{x\in T} \dil_x(\theta_*),
$$
and for any $x\in T$, since $\rho(x)\geq 2$,
$$
\diam(T)\dil_x(\theta_*) \leq \lambda(x)\dil_x(\theta_*) \leq 2 (\lambda(x)-\mu(x)) \dil_x(\theta_*)  \leq 2c,
$$
which concludes the proof.
\sq

For each vertex $v\in \cV_0$ we define a set $\Gamma_v\subset \R^2$ as follows : $\Gamma_v := \{v\}$ if $\rho(v) <3$, and 
\be
\label{defGammav}
\Gamma_v := \left[v, \, \frac v 3+ \frac{2w_-} 3\right] \cup \left[v,\frac v 3 +\frac{2w_+} 3\right] 
\ee
if $\rho(v)\geq 3$, where $w_-,w_+\in \cV_0$ are two neighbors of $v$ in $\cT_0$ which respectively minimize and maximize the quantity $\<\theta(v)^\perp, w-v\>$. In mathematical terms for any neighbor $w\in \cV_0$ of $v$
\be
\label{defWmWp}
\<\theta(v)^\perp, w_- -v\> \leq \<\theta(v)^\perp, w-v\> \leq  \<\theta(v)^\perp, w_+ - v\>. 
\ee
This property is illustrated on Figure \ref{figWmWp}.

\begin{figure}
\centering
\includegraphics[width=4cm, height=4cm]{\pathPic/Dessins/Jenny/VT0vJenny.pdf}\hspace{0.5cm}
\includegraphics[width=6cm, height=4cm]{\pathPic/Dessins/Jenny/DirThetaJenny.pdf}
\caption{Neighborhood $V_{\cT_0}(v)$ of a simplex $v$ in the triangulation $\cT_0$ (left), the neighbors $w_+$ and $w_-$ of a vertex $v$ in $\cT_0$.
\label{figWmWp}}
\end{figure}

We define $\Gamma := \cup_{v\in \cV_0} \Gamma_v$, and for each $z\in \Gamma\sm\cV_0$ we define 
\be
\label{defGammaz}
\Gamma_z := \bigcup_{\substack{v\in \cV_0 \\ z \in \Gamma_v}} \Gamma_v.
\ee
Note that for any vertex $v\in \cV_0$ the set $\Gamma_v$ does not contain any vertex $w\in \cV_0$ distinct from $v$, hence \iref{defGammaz} agrees with \iref{defGammav} for any $z\in \cV_0$.\\ 

\begin{lemma}
\label{lemmaAngleWmWp}
let $v\in \cV_0$ be such that $\rho(v) \geq 3$, and let $w_+, w_-$ be two neighbors of $v$ satisfying \iref{defWmWp}.
We have 
\be
\label{eqAngleWmWp}
\varangle(\theta(v)^\perp, w_+ -v) \leq \cPi/4,
\stext{ and }
\varangle(\theta(v)^\perp, v-w_-) \leq \cPi/4.
\ee
\end{lemma}

\proof
We restrict without loss of generality our attention to the proof of the first inequality, and we assume for contradiction that $\vp := \varangle(\theta^\perp, w_+-v)>\cPi/4$. % in \iref{eqAngleWmWp}.
Among the two vertices $w\in \cV_0$ such that the triangle of vertices $v,w,w_+$ belongs to $\cT_0$, we choose the one such that $\varangle(\theta^\perp, w-v)$ is minimal.
We denote $\psi := \varangle(w-v, w_+-v) \in \{\cPi/4, \cPi/2\}$ and we obtain 
$$
\<\theta(v)^\perp, w_+-v\> = |w_+-v|\cos \vp \stext{ and } \<\theta(v)^\perp, w-v\> = |w-v|\cos (\vp-\psi).
$$
If $\psi = \cPi/2$ then $|w_+-v| = |w-v|$ since the triangles $T\in \cT_0$ are half squares, and $\cos (\vp-\psi) = \sin \vp$. We thus have $\cos \vp \geq \sin \vp$ according to \iref{defWmWp} which contradicts our assumption that $\vp>\cPi/4$.
If $\psi = \{\cPi/4\}$ then $|w_+-v| = \sqrt 2 |w-v|$ or $|w_+-v| =  |w-v|/\sqrt 2$. We thus have $\sqrt 2 \cos \vp \geq \cos (\vp-\cPi/4)$ which again contradicts our assumption that $\vp \leq \cPi/4$.
\sq
%
%$$
%\angle(u,u') := \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
%$$
%(Stricly speaking, $\angle(u,u')$ is the smallest of the two unoriented angles formed by $u,u'$ and $u,-u'$.)



%\begin{lemma}
%Let $T\in \cT_0$ and let $z,z'\in T$, then 
%\be
%\label{stabRho}
%\rho(z') \geq  \frac{1-c}{1/\rho(z)+c}.
%\ee
%Defining $\rho_c := \frac{1-c}{1/2+c}$, we have if $\rho(z) \geq 2$ that 
%%$$
%%\rho(z') \geq  \rho_c := \frac{1-c}{1/2+c}.
%%$$
%%and 
%\be
%\label{stabTheta}
%\angle(\theta(z), \theta(z')) \leq \vp_c := \frac c {1-1/\rho_c}.
%\ee
%\end{lemma}
%
%\proof
%Since the functions $\lambda$ and $\mu$ are Lipschitz, and since $|z-z'| \leq \lambda(z)$, we have
%$$
%\rho(z') = \frac {\lambda(z')}{\mu(z')} \geq \frac {\lambda(z)-c \lambda(z)}{\mu(z)-c \lambda(z)} = \frac{\lambda(z)(1-c)}{\lambda(z)(1/\rho(z)+c)} = \frac{1-c}{1/\rho(z)+c},
%$$
%which establishes \iref{stabRho}.
%We thus turn to the proof of \iref{stabTheta}, and for that purpose we recall that 
%$
%(\lambda(z') - \mu(z')) \dil_{z'}(\theta)\leq c
%$
%for any $z'\in T$.
%Observing that 
%$$
%\lambda(z')-\mu(z') = \lambda(z') (1-1/\rho(z')) \geq \diam(T) (1-1/\rho_c)
%$$
%we obtain 
%$$
%\angle(\theta(z), \theta(z')) \leq \diam(T) \max_{z'\in T} \dil_{z'}(\theta) \leq \frac c {1-1/\rho_c},
%$$
%which concludes the proof of \iref{stabTheta}.
%\sq

\begin{lemma}
For any $z\in \Gamma$ and any $z'\in \Gamma_z$ distinct from $z$
we have
\be
\label{eqAngleGammaz}
\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
\ee
and therefore if $c$ is sufficiently small
$$
\angle(\theta(z)^\perp ,z'-z) \leq \cPi/3, 
$$
and there exists a piecewise affine Lipschitz map $\gamma : [\alpha, \beta]\to \R$ such that the following is a bijection
$$
t\in [\alpha, \beta] \mapsto z+ t\theta(z)^\perp + \sqrt 3 \gamma(t) \theta(z) \in \Gamma_v.
$$
\end{lemma}

\proof
We consider a vertex $v\in \cT_0$ such that $z,z'\in \Gamma_v$, and we note that $\rho(v) \geq 3$ by construction of $\Gamma_v$, and therefore $\rho \geq 2$ on a triangle common to $v$ and $z$ according to Corollary \ref{corolRho23}.
It thus follows from Corollary \ref{corolTheta2C} that 
\begin{eqnarray*}
\angle(\theta(z), z-z')&\leq& 2c + \angle(\theta(v), z-z') \\
&\leq& 2c + \max \{ \angle(\theta(v), w_+-v), \angle(\theta(v), w_- -v)\}\\
& \leq & 2c + \cPi/4,
\end{eqnarray*}
which concludes the proof.
\sq

The next proposition gives some properties of the set $\Gamma$.
\begin{prop}
\label{propDistUpLow}
If $c$ is sufficiently small, then the following holds.
For any $z\in \Gamma$,
\be
\label{eqDistzGH0}
 \min\{|z-e| \sep  e\in \Gamma\sm \Gamma_z\} \geq \frac {10}{91} \lambda(z) % >\frac 1 {10}
\ee
and for $z\in \R^2$
\be
\label{eqDistzGH}
\min\{\|z-e\|_{H(z)} \sep e \in \Gamma\} \leq 2 %1+ \frac {2\sqrt 2} 3 <2. 
\ee
\end{prop}

\begin{figure}
\centering
\includegraphics[width = 4cm, height = 4cm]{\pathPic/Dessins/Jenny/DistZGJenny.pdf}
\caption{Illustration of the proof of Proposition \ref{propDistUpLow} \label{figDistZG}}
\end{figure}

\proof
We first establish \iref{eqDistzGH0}. 
Let $z\in \Gamma$ and let $v\in \cV_0$ be such that $z\in \Gamma_v$. We have $z= (1-\alpha) v+\alpha w_*$ for some $\alpha\in [0,2/3]$ and some neighbor $w_*\in \{w_+,w_-\}$ of $v$.
Denoting by $V_{\cT_0}(v)$ the union of all triangles $T\in \cT_0$ containing $v$, and by $\cV_0(v)$ the collection of neighbors of $v$ in $\cT_0$, we have
$$
\Gamma\sm \Gamma(z) \subset \overline {\R^2 \sm V_{\cT_0}(v)} \bigcup_{w\in \cV_0(v)\sm\{w_*\}} \left[\frac{2v+w}3, w\right].
$$
The set appearing in the right hand side is illustrated on Figure \ref{figDistZG}.
It follows that 
\begin{eqnarray*}
d(z,\Gamma\sm \Gamma(z)) &\geq & \min \left\{ d(z, \R^2 \sm V_\cT(v)), \ \min_{w\in \cV_0(v) \sm \{w_*\} } d\left(z,\left[\frac{2v+w}3, w\right]\right)\right\}\\
& \geq & \min \left\{ \frac{|w_*-z|}{\sqrt 2}, \ \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)\sm \{w_*\}} |v-w|\right\}\\
& = & \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)} |v-w|\\
& \geq & \frac{1}{3\sqrt 2} \lambda(v)\frac {\sqrt 2} 3 \\
&\geq&  \frac{\lambda(z)(1-c)}{9}.
\end{eqnarray*}
where we used \iref{edgeLambda} in the fourth line, and \iref{eqLambdaT} in the last line. This establishes \iref{eqDistzGH0} if $c$ is sufficiently small.\\

We now turn to the proof of \iref{eqDistzGH}. 
Let $T \in \cT$ and let $z\in T$. Since $T$ is a half square there exists a vertex $v$ of $T$ such that $|z-v| \leq \diam(T)/2$, hence %For any vertex $v$ of $T$ we obtain %If $\rho(z)\leq 4$, then any vertex $v$ of $T$ satisfies 
$$
\|z-v\|_{H(z)} \leq  \frac{|z-v|}{\mu(z)}   \leq \frac{\diam(T)}{2 \mu(z)} \leq \frac{\lambda(z)}{2 \mu(z)} = \frac{\rho(z)} 2,
$$
which concludes the proof if $\rho(z) \leq 4$. If $\rho(z) \geq 4$ and $c$ is sufficiently small then $\rho(v) \geq 3$ for any vertex $v$ of the triangle $T$ according to Corollary \ref{corolRho23}.

We choose two vertices $v,w$ of $T$ such that the line $(z+ r \theta(z))_{r\in \sR}$ intersects $\partial T$ on the segment $[v,(v+w)/2]$.
We denote by $w_-$ and $w_+$ the neighbors of $v$ in $\cT_0$ which satisfy \iref{defWmWp}.
Our first step is to establish that the line $(z+ r \theta(z))_{r\in \sR}$ intersects the set $\Gamma_v$ : this is heuristically due to the fact that the angle $\lhd(\theta(z), \theta(v))$ is small and that the vertices $w_-$ and $w_+$ are the \emph{fathest} from $v$ in the direction of $\theta(v)^\perp$ as illustrated on Figure \ref{figWmWp} (right).

We have according to \iref{eqEdgeRatio}
$$
\<\theta(v)^\perp,w_+ - v\> \geq |w_+-v|\cos(\cPi/4) \geq \frac{|w-v|} 2 \frac 1 {\sqrt 2}. %/(2\sqrt 2).
$$
We assume without loss of generality that %$\theta(v)$ and $\theta(z)$ are oriented in consistently, in such way that 
$\<\theta(z), \theta(v)\> \geq 0$, and we obtain using Corollary \ref{corolTheta2C}
$$
|\theta(z)-\theta(v)| \leq \varangle(\theta(z), \theta(v)) = \lhd(\theta(z), \theta(v))\leq 2c.
$$
It follows that 
\begin{eqnarray*}
\<\theta(z)^\perp, w-v\> &=& \<\theta(z)^\perp-\theta(v)^\perp, w-v\>+\<\theta(v)^\perp, w-v\>\\
& \leq & |\theta(z)-\theta(v)| |w-v| + \<\theta(v)^\perp, w_+-v\>\\
& \leq & (1+4c \sqrt 2 )\<\theta(v)^\perp, w_+-v\>.\\
%& \leq & (1+4 c\sqrt 2) }{1-\vp_c\sqrt 2} \<\theta(z)^\perp,w_+ - v\>.
%& \leq & \frac 4 3 \<\theta(z)^\perp,w_+ - v\>
\end{eqnarray*}
Denoting $\Theta := \varangle(\theta(v)^\perp, w_+-v)$ and $\Phi := \varangle(\theta(z)^\perp, w_+-v)$ we obtain 
$$
\frac{\<\theta(v)^\perp, w_+-v\>}{\<\theta(z)^\perp, w_+-v\>} = \frac{\cos(\Theta)}{\cos(\Phi)} \leq \frac{\cos(\Theta)}{\cos(\Theta) - |\Phi-\Theta|} =\left(1-\frac {|\Phi-\Theta|}{\cos\Theta}\right)^{-1}\leq (1-2 \sqrt 2 c)^{-1} % - 2c} = \frac 1 {1-2 \sqrt 2 c},
$$
hence 
$$
\<\theta(z)^\perp, w-v\>  \leq \frac{1+4c \sqrt 2}{1-2 \sqrt 2 c}\<\theta(z)^\perp, w_+-v\>
$$
Proceeding likewise for $w_-$, and assuming that $c$ is sufficiently small, we obtain 
%
%We assume that $c$ is sufficiently small in such way that 
%\be
%\label{assumPhic}
%\frac{1+\vp_c 4\sqrt 2}{1-\vp_c\sqrt 2}\leq \frac 4 3
%\ee
$$
\frac 4 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, w-v\> \leq  \frac 4 3\<\theta(z)^\perp, w_+ - v\>,
$$
and therefore since $z+r\theta(z)\in [v,(v+w)/2]$ for some $r\in \R$,
$$
\frac 2 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, z-v\> \leq  \frac 2 3\<\theta(z)^\perp, w_+ - v\>.
$$
It follows that the line $(z+r\theta(z))_{r\in \sR}$ intersects the set $\Gamma_v := [v, (v+2w_+)/3] \cup  [v, (v+2w_-)/3]$ at some point $z'$.
%hence there exists $r\in \R$ such that $z' := z+ r\theta(z) \in \Gamma_v$. 
The point $z'$ belongs to triangle $T'$ containing $v$, and we obtain using \iref{eqDiamRatio} 
\begin{eqnarray*}
\lambda(z) \|z'-z\|_{H(z)} &=& \lambda(z)\|r\theta(z)\|_{H(z)}\\
&=& |r|\\
&=& |z-z'|\\
&\leq& |z-v|+|v-z'|\\
&\leq& \diam(T)+ \frac 2 3\diam(T')\\
&\leq & \left(1+\frac 2 3 \sqrt 2\right) \diam(T)
 \leq  \left(1+\frac 2 3 \sqrt 2\right) \lambda(z),
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

We construct in the next lemma the set of vertices $\cV$ of the quasi-acute triangulation $\cT$ to be constructed by sampling the set $\Gamma$.

\begin{lemma}
\label{lemmaConstV}
The following holds if $c$ is sufficiently small.
There exists a discrete set $\cV \subset\Gamma$ containing $\cV_0$ and satisfying the following:
\begin{enumerate}[i)]
\item (Separation) For all $v,w\in \cV$, $d_H(v,w) \geq 1/10$.
\item (Distance from $\Gamma$) For all $z\in \Gamma$, $d_H(z, \cV) \leq 1/10$.
\item (Distance from $\R^2$) For all $z\in \R^2$, $d_H(z,\cV) \leq 2+1/4$.
\end{enumerate}
\end{lemma}
\proof
For any distinct $v,w\in \cV_0$ we obtain using \iref{pairwiseV0} and Proposition \ref{propEuclidRiemann}
\begin{eqnarray*}
d_H(v,w) &\geq& \ln(1+c\|v-w\|_{H(v)})/c\\
&\geq& \ln(1+c|v-w|/\lambda(v))/c\\
&\geq& \ln(1+c\sqrt 2 /3)/c 
\end{eqnarray*}
which is larger than $1/10$ if $c$ is sufficiently small. % since $\sqrt 2 /3>1/10$.

We denote by $\cV$ a $1$-equispaced subset of the metric space $(\Gamma, 10\:d_H)$ containing $\cV_0$, which exists according to Lemma \ref{lemmaEquiSpaced}. The two first announced properties, separation and distance from $\Gamma$, follow directly from this construction.

The third property is obtained as follows: for any $z\in \R^2$ there exists according to Proposition \ref{propDistUpLow} a point $e\in \Gamma$ such that $\|z-e\|_{H(z)}\leq 2$. Furthermore there exists a vertex $v\in \cV$ such that $d_H(e,v) \leq 1/10$, hence
$$
d_H(z,\cV) \leq d_H(z,e)+ d_H(e,v) \leq -\ln(1-c\|z-e\|_{H(z)})/c + 1/10 \leq -\ln(1-2c)/c + 1/10.
$$
which is smaller than $2+1/4$ if $c$ is sufficiently small.
\sq


\begin{lemma}
\label{lemmaDiamVorGamma}
For any $v\in \cV$ we have 
$$
\max\{\|z-v\|_{H(v)} \sep z\in \Gamma\cap \Vor(v)\} \leq r_0(c) := (e^{c/10}-1)/c.
$$
(and $r_0(c) \to 1/10$ as $c\to 0$).
Furthermore $c$ is sufficiently small and if $v,w\in \cV$ are such that $\Vor(v) \cap \Vor(w) \cap \Gamma \neq \emptyset$, then 
$$
\|v-w\|_{H(v)} \leq 1/4.
$$
\end{lemma}

\proof
According to point ii) of Lemma \ref{lemmaConstV} there exists $w\in \cV$ such that $d_H(z,w) \leq 1/10$. It thus follows from the definition of the Voronoi diagram that 
\begin{eqnarray*}
\|z-w\|_{H(w)} &\leq& \|z-w'\|_{H(w')}\\
&\leq& (\exp(c d_H(z,w'))-1)/c\\
&\leq&  (\exp(c/10)-1)/c.
\end{eqnarray*}

We now turn to the second point of the proposition, and we consider a point $z\in \Vor(v) \cap \Vor(w) \cap \Gamma$.
We thus have $\|z-v\|_{H(v)} = \|z-w\|_{H(w)} \leq r_0(c)$ which implies 
$$
\ln(1+c\|v-w\|_{H(v)})/c \leq d_H(v,w) \leq d_H(v,z)+d_H(z,w) \leq -2 \ln(1-c r_0(c))/c
$$
hence $\|v-w\|_{H(v)} \leq ((1-cr_0(c))^{-2}-1)/c$ which tends to $1/4$ as $c\to 0$. This concludes the proof of this proposition.
\sq


\begin{lemma}
\label{lemmaRecallG}
There exists a absolute constant $C_0\geq 1$ such that the following holds if $c$ is sufficiently small.
The set $\cV$ is wedged with respect to the metric $H$, and the anisotropic Delaunay triangulation obtained by arbitrarily triangulating the cells of the graph $\cG(\cV,H)$ is $C_0$-adapted to $H$.

Furthermore for any edge $[v,w]$ of $\cT$ and any $z\in [v,w]$ we have 
$$
\|v-w\|_{H(z)} \leq 5.
$$
\end{lemma}

\proof
We denote $\alpha := (2+1/4)^{-1}$ throughout the proof of this lemma.
It follows from to Lemma \ref{lemmaConstV} that the set $\cV$ is a $\alpha/10$-equispaced subset of the metric space $(\R^2, \alpha d_H)$. 

Theorem \ref{thEquiMesh} applied to the metric $\alpha^2 H$, therefore implies that, if $c$ is sufficiently small, the set 
$\cV$ is wedged for the metric $\alpha^2 H$ and that arbitrarily triangulating the convex cells of the graph $\cG(\cV,\alpha^2 H)$, which are convex yields a triangulation $\cT$ which is $C$-adapted to the metric $\alpha^2H$ (hence $C_0 := C/\alpha$-adapted to $H$), where $C$ is an absolute constant.

The definition \iref{defGVH} of the graph $\cG(V,H)$ implies that $\cG(\cV,\alpha^2 H) = \cG(\cV,H)$, and Definition \ref{defWedge} of the wedge property shows that it holds for $H$ if and only if it holds for $\alpha^2 H$. 

For any edge $[v,w]$ of $\cT$ the Voronoi regions $\Vor(v)$ and $\Vor(w)$ intersect (by definition of the anisotropic Delaunay triangulation), and we thus have according to Lemma \ref{lemmaDiamVor} 
$$
\alpha d_H(v,w) = d_{\alpha^2 H} (v,w) \leq -2\ln (2-e^{c'})/c'
$$
where $c' := c/\alpha$. Hence 
$$
d_H(v,w) \leq r_0(c) := -2 \ln (2-e^{c/\alpha})/c.
$$
If follows that 
$
\|v-w\|_{H(v)} \leq r_1(c) := (e^{c r_0(c))}-1)/c,
$
hence \iref{eqLocalNorm}
$
\|v-w\|_{H(z)} \leq \|v-w\|_{H(v)} (1-c \|v-z\|_{H(v)})^{-1} \leq r_2(c) := r_1(c) (1-c r_1(c))^{-1}
$
for any $z\in [v,w]$.
As $c\to 0$ the functions $r_0$, $r_1$ and $r_2$ all tend to $2 (1+1/4) <5$. Choosing $c$ sufficiently small concludes the proof of this proposition.
\sq


\begin{lemma}
If $c$ is sufficiently small, then the following holds.
For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$ we have 
\be
\label{vpNotInGammav}
\sin \lhd (\theta(v),v-w) \leq \frac {50}{\rho(v)}.
\ee
%We define $\rho_0\in [1,\infty)$ by $\sin (\cPi/12) = 50/\rho_0$.
\end{lemma}

\proof
If $c$ is sufficiently small, then Proposition \ref{propDistUpLow} implies that $|v-w| \geq \lambda(v)/10$, and Lemma \ref{lemmaRecallG} states that $\|v-w\|_{H(v)} \leq 5$.
Denoting $\vp := \lhd (\theta(v),v-v')$ we obtain 
$$
5\geq \|v-w\|_{H(v)} \geq \frac{|v-w|\sin \vp}{\mu(v)} \geq \frac{\lambda(v) \sin \vp}{10 \mu(v)}.
$$
which implies the announced result.
\sq

%\begin{lemma}
%If $c$ is sufficiently small, then the following holds.
%
%\end{lemma}

The next lemma gives a lower bound on the distance from a vertex $v\in \cV$ to the Voronoi region of a vertex $w\in \cV\sm\Gamma$.

\begin{lemma}
\label{lemmaVorFar}
If $c$ is sufficiently small, then for any $v\in \cV$, $w\in \cV\sm \Gamma_v$ 
$$
\inf\{|v-z|\sep z\in \Vor(w) \cap \Gamma\} \geq \lambda(v)/100.
$$

%and $z\in \Vor(w)\cap \Gamma$ we have 
%$$
%|z-v|\geq \lambda(v)/100.
%$$
\end{lemma}

\proof
We have for any $z\in \Vor(w) \cap \Gamma$, according to Lemma \ref{lemmaDiamVorGamma} 
\begin{eqnarray*}
|v-z| &\geq& |v-w|-|z-w|\\
& \geq & |v-w| - \|z-w\|_{H(w)} \lambda(w)\\
& \geq & |v-w| - r_0(c) (\lambda(v)+c|v-w|)\\
& = & |v-w| (1-c r_0(c)) -r_0(c) \lambda(v)\\
& \geq & \frac {10} {91}\lambda(v) (1-cr_0(c)) - r_0(c) \lambda(v)\\
&=& r_1(c) \lambda(v),
\end{eqnarray*}
where we used \iref{eqDistzGH0} in the fifth line, and where $r_1(c) := 10(1-cr_0(c))/91 - r_0(c)$.
As $c\to 0$ we have $r_0(c) \to 1/10$ and $r_1(c) \to 10/91-1/10 >1/100$. If $c$ is sufficiently small we therefore have $r_1(c) \geq 1/100$ which concludes the proof.
\sq

The next proposition shows that the Voronoi cell of a vertex $v$ contains a ball of fixed radius for the distance $\|\cdot\|_{H(v)}$ (hence an ellipse).

\begin{lemma}
\label{lemmaVorBall}
If $c$ is sufficiently small, then 
for any $v\in \cV$ we have 
$$
\Vor(v) \supset \{z\in \R^2 \sep \|z-v\|_{H(v)} \leq 1/25\},
$$
\end{lemma}

\proof
We consider $z\in \partial \Vor(v)$, hence $z\in \Vor(v) \cap \Vor(w)$ for some vertex $w\in \cV$.
We define $r:=\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$ and we obtain using Point i) of Lemma \ref{lemmaConstV}
\begin{eqnarray*}
1/10 &\leq& d_H(v,w)\\
&\leq& d_H(z,v)+d_H(z,w)\\
&\leq& -\ln (1-c\|z-v\|_{H(v)})/c - \ln (1-c\|z-v\|_{H(v)})/c\\
&=& -2 \ln (1-cr)/c.
\end{eqnarray*}
It follows that 
$$
r\geq (1-\exp(-c/20))/c,
$$
and therefore $r\geq 1/25$ if $c$ is sufficiently small, 
which concludes the proof.
\sq

%The set $\Gamma$ is a union of polygonal lines (and of isolated points). If $v\in \Gamma$ is on a polygonal line, we say that the neighbors of $v$ on $\Gamma$ (if they exist) are the previous and next points on $\Gamma$.

%The set $\Gamma$ is a union of polygonal lines (and of isolated points). We say that two points $v,w\in \Gamma$ are neighbors on $\Gamma$ if 

We say that two points $v,w\in \cV$ are neighbors on $\Gamma$ if 
$$
(v,w) \subset \Gamma\sm \cV.
$$
Note that $\Gamma\sm\cV$ is a collection of straight open intervals, since $\cV_0\subset \cV$.
Note also that two neighbors on $\Gamma$ belong to the same element of $\cT_0$.

\begin{lemma}
\label{lemmaSegVor}
If $c$ is sufficiently small, then the following holds.
For any $v\in \cV$ such that $\rho(v) \geq \rho_0 = 22$ the vector $v$ has at least a neighbor on $\Gamma$. Furthermore for any neighbor $w$ of $v$ on $\Gamma$ we have 
$$
|v-w|\leq \mu(v)/2
$$
and 
\be
\label{eqNeighborEdge}
[v,w] \subset \interior(\Vor(v) \cup \Vor(w)).
\ee
and consequently $[v,w]$ is an edge of $\cT$. 
\end{lemma}

\proof
We first remark that according to Lemma \ref{lemmaDiamVorGamma} 
\be
\label{dzvmu}
r_0(c) \geq \|z-v\|_{H(v)} \geq \cos\left(\cPi/ 3 \right) \frac {|z-v|}{\mu(v)}  = \frac {|z-v|}{2 \mu(v)}
\ee
We assume for contradiction that the inclusion \iref{eqNeighborEdge} does not hold, and we thus consider two points $z\in [v,w]\cap \Vor(v)$ and $w'\in \cV$ such that $z\in \Vor(w')$.



If $w'\notin \Gamma_v$, then $|z-v| \geq  \lambda(v)/100$ according to Lemma \ref{lemmaVorFar}.
Combining this with \iref{dzvmu} we obtain 
$$
\rho_0 \leq \rho(v) = \lambda(v)/\mu(v) \leq 200 r_0(c).
$$
If $c$ is sufficiently small then $200r_0(c) < 21 < 22$ which gives a contradiction (recall that $r_0(c) \to 1/10$ as $c\to 0$).

We now consider the case $w'\in \Gamma_v$, and we first assume that $w'$ is not on the same side as $w$ on $\Gamma$, in the sense that $\<w-v, \theta(v)^\perp \>>0$ and $\<w'-v, \theta(v)\> <0$.
Hence there exists $\alpha\in [0,1]$ and $r\in \R$ such that 
$$
v + r \theta(v) = z+ \alpha(w'-z).
$$
%Consider a vector $u$ orthogonal to $w-z'$. 
We thus have 
$
r\<\theta(v),(w'-z)^\perp \> = \<z-v , (w'-z)^\perp\>
$
hence
$$
r/2\leq  |r| \cos \lhd(\theta(v)^\perp, w'-v) \leq  |z-v| \leq 2 \mu(v) r_0(c).
$$
According to \cite{Shew} Lemma 3 (Visibility Lemma) the Voronoi regions of a wedged Voronoi diagram are star-shaped. Since the Voronoi diagram is wedged according to Lemma \ref{lemmaRecallG} we obtain using Lemma \ref{lemmaVorBall} that 
$$
\frac {\lambda(v)} {25} = \|r\theta(v)\|_{H(v)} \leq r \leq 4 \mu(v) r_0(c),
$$
hence $\rho_0 \leq \rho(v) \leq 100 r_0(c)$. This is a contradiction if $c$ is sufficiently small since $100 r_0(c) <11 <22 = \rho_0(c)$.

It follows that $w'$ is on the same side as $w$ on $\Gamma$, with respect to $v$, in the sense that  $\<w-v, \theta(v)^\perp \>>0$ and $\<w'-v, \theta(v)^\perp\> >0$.

We now remark that the vertices $v,w$ belong to the same element of $\cT_0$ since they are neighbors on $\Gamma$. Hence $\rho(w) \geq \rho_0 - 1=21$ if $c$ is sufficiently small.
Way may therefore apply this proof to $w$, and we obtain that $w'$ is on the same side as $v$ with respect to $w$, in the sense that  $\<w'-w, \theta(w)^\perp \><0$ and $\<w'-v, \theta(w)\> <0$ (if $\<\theta(w), \theta(v)\> >0$).

It follows that $w'\in (v,w)$ which is a contradiction.


Finally, we remark that according to Lemma \ref{lemmaDiamVorGamma}
$$
1/4 \geq \|v-w\|_{H(v)} \geq \frac{|v-w| \cos (\cPi/3)}{\mu(v)} = \frac{|v-w|}{2\mu(v)}
$$
hence $|v-w|\leq \mu(v)/2$ which concludes the proof.
\sq


\begin{prop}
The following holds if $c$ is sufficiently small.
For any $v\in \cV$ be such that $\rho(v)\geq \rho_1$, where $\rho_1$ is a constant specified in the proof, the following holds.
\begin{enumerate}
\item The vertex $v$ has two neighbors $w,w'$ on $\cT$ such that 
\be
\label{eqAnglesUpDown}
\varangle(w-v, \theta(v)) \leq \cPi/12 \stext{ and } \varangle(w'-v, -\theta(v)) \leq \cPi/12.
\ee
\item A vertex $w\in \cT\cap \Gamma_v$ is a neighbor of $v$ on $\cT$ if and only if it is a neighbor of $v$ on $\Gamma$.
\end{enumerate}
\end{prop}

\proof
Consider a neighbor $w_*$ of $v$ on $\Gamma$. Then according to Lemma \ref{lemmaSegVor} the segment $[v,w]$ is an edge of $\cT$, hence $w_*$ is a neighbor of $v$ on $\cT$ by definition.
Let $T,T'\in \cT$ be the two triangles containing the edge $[v,w_*]$, and let $w,w'\in \cV$ be the third vertex of these triangles respectively.

Since $\cT$ is $C_0$-adapted to the metric $H$, we obtain 
$$
|T| = |\TEq| (\det \cH_T)^{-\frac 1 2} \geq |\TEq|  C_0^{-2} (\det H(v))^{-\frac 1 2} =  |\TEq|  C_0^{-2} \lambda(v) \mu(v).
$$
On the other hand $|w_*-v| \leq \mu(v)/2$ according to Lemma \ref{lemmaSegVor}, and 
$$
\mu(v)\sin \lhd(w-v,\theta(v))  |w-v|\leq \|v-w\|_{H(v)} \leq C_0 \|v-w\|_{\cH_T} \leq 2C_0.
$$
Combining these inequalities we obtain  
$$
|\TEq|  C_0^{-2} \lambda(v) \mu(v) \leq  |T| \leq \frac 1 2 |w-v| |w_*-v| \leq \frac{2C_0\mu(v) }{\sin \lhd(w-v,\theta(v))} \mu(v)/2.
$$
hence 
$$
\sin \lhd(w-v,\theta(v)) \leq \frac{C_0^3}{|\TEq| \rho(v)}. 
$$
We define 
$$
\rho_1 := \frac{C_0^3}{|\TEq|\sin (\cPi/12)}
$$
and we thus obtain $\lhd(w-v,\theta(v)) \leq \cPi/2$. Likewise $\lhd(w'-v,\theta(v)) \leq \cPi/2$. 

Since $\varangle (w_* - v, \theta(v)) \in [\cPi/3,2 \cPi/3]$, and since the triangles $T,T'$ contain the edge $[v,w_*]$, thus implies \iref{eqAnglesUpDown}.

Let $v'\in \cV \cap \Gamma_v$ be a vertex on the side of the neighbor $w_*$.
Then $\lhd(v'-v, \theta(v)^\perp) \leq \cPi/3$ which implies that the segment $[v,v']$ intersects one of the triangles $T$ or $T'$. 
Therefore $v'$ is not a neighbor of $v$ in $\cT$.

Likewise, if $v$ has a second neighbor $w_{**}$ on $\Gamma$ (on the other side than $w_*$ with respect to $w$), then $[v,w_{**}]$ is an edge of $\cT$. Similarly we obtain that for any point $v''\in \Gamma_v$ on the side of $w_{**}$, the segment $[v,v'']$ is not an edge of $\cT$.

This implies Point 2. and concludes the proof of this proposition.
\sq

For each $v\in \cV_0$ we define $\Gamma'_v := [v,w_-] \cup[v,w_+]$ where $w_-$ and $w_+$ are defined by \iref{defWmWp}.
We then set 
$$
\Gamma' := \bigcup_{\substack{v\in \cT_0\\ \rho(v) \geq 1+\rho_1}} \Gamma'_v.
$$


\begin{prop}
If $c$ is sufficiently small, then the following holds.
Denote by $\cQ$ the partition into convex polygons of $\R^2$ obtained by the overlay of $\cT$ and $\Gamma'$.
We denote by $\cT'$ the partition obtained by randomly triangulating the convex cells of $\cQ$.


%Denote by $\cT'$ the triangulation obtained by randomly triangulating the 
%
%Denote by $\cQ$ the partition into convex polygons obtained by cutting $\cT$ by all segments joining an extremal vextex $v\in \cV$ satisfying $\rho(v) \geq ??$ to the vertex $v'\in \cV_0$ in the direction of $\bt(v)$.
%
%Then the interior angles in $\cQ$ are smaller than ??. %Each triangle $T\in \cT$ contains at most $??$ cells of $\cC$, which are at most hexagons (in other words they have $3$ to $6$ elements).
%
%Denote $\cT'$ the triangulation obtained by randomly triangulating the convex cells of $\cQ$.

Then $\cT'$ is a $??$-refinement of $\cT$ and $S(T') \leq ??$ for all $T'\in \cT'$.
\end{prop}

\proof
Since the collection $\cV$ of vertices of $\cT$ contains $\cV_0$ and since the segments in $\Gamma$ join some points of $\cV_0$, we find that the overlay of $\cT$ and $\Gamma$ is indeed a partition of $\R^2$ into convex polygons.

Our first objective is to give a uniform bound on the measure of sliverness in $\cT'$.
For that purpose we consider a cell $Q \in \cQ$ and a vertex $z$ of $Q$.

We first assume that $z\notin \cV$, hence $z$ is a vertex created by the overlay of $\Gamma$ on $\cT$.
We denote by $v_0$ the vertex in $\cV_0$ such that $z\in \Gamma'_{v_0}$, and we observe that $\rho(v_0) \geq \rho_0+1$.
Let $[w,w']$ be the edge of $\cT$ containing $z$. We have 
$$
|z-w| \leq \lambda(z) \|z-w\|_{H(z)} \leq \lambda(z) \|w-w'\|_{H(z)} \leq 5 \lambda(z)\leq 5 \lambda(v_0)(1+c). 
$$
hence
$$
|v_0 - w| \leq |v_0 - v| + |v-w| \leq \lambda(v_0) (6+5c).
$$
If $c$ is sufficiently small, then we obtain $\rho(w) \geq \rho_1$.
Therefore $w' \notin \Gamma_w$, otherwise $w'$ would be a neighbor of $w$, $[w,w'] \subset \Gamma$ which contradicts the fact that this edge was bisected by the overlay.

Hence $\sin \lhd(\theta(v),v-w) \leq 50/\rho(v)$. Hence $\lhd(\theta(v),v-w) < \cPi/24$. On the other hand $\lhd(\theta(v), \theta(z)) \leq 2 \times 5 c \leq \cPi/24$ if $c$ is sufficiently small. We conclude that $\lhd(v-v_0, w,w') \geq \cPi/12$.\\

We may therefore assume that $v\in \cV$.
If $\rho(v) \leq 2+\rho_1$ then 
$$
S(T) \leq \rho(T) = \sqrt {\|\cH_T\| \|\cH_T^{-1}\|} \leq C_0^2 \rho(v) \leq C_0^2 (2+\rho_1).
$$
The angle $\vp$ of $\cQ$ at $v$ is bounded by the angle of $T$ at $v$, hence by
$$
\tan \vp \leq C_0^2 (2+\rho_1),
$$
which gives a uniform bound.\\


If $\rho(v)\geq 2+\rho_1$, then there exists two neighbors $w,w'$ of $v$ satisfying \iref{eqAnglesUpDown}. Let $v_0\in \cT_0$ be such that $v \in \Gamma_{v_0}$. 
If $c$ is sufficiently small, then $\rho(v_0) \geq 1+\rho_1$. 
Therefore $v\in \Gamma'_v$, and the tangent $\bt, \bt'$ vectors to $\Gamma'_v$ in the two directions satisfy $\lhd(\theta(v)^\perp, \bt) \leq \cPi/3$ and $\lhd(\theta(v)^\perp, \bt') \leq \cPi/3$.

It follows that the angle of $Q$ at $v$ is bounded by $5 \cPi/6$.\\


We now prove that $\cT'$ is a bounded refinement of $\cT$, and for that purpose we consider and edge $e=[v,w]$ of $\cT$. %=[\omega-u, \omega+u]

We have by construction $|v-w|/\lambda(v) \leq \|v-w\|_{H(v)} \leq 12$.
The triangles $T\in \cT_0$ intersected by $[v,w]$ satisfy for some $z\in [v,w]$ the inequality 
$$
2 \delta_0 \lambda(v) (1-12c) \leq 2 \delta_0 \lambda(z) \leq \diam(T) \leq \lambda(v) \leq \lambda(u)(1+12c)
$$
Therefore they are contained in the ball $B(v,  \lambda(v)(12+1+12c))$ and have area 
$$
|T| = \diam(T)^2/4 \geq \delta_0^2 \lambda(v)^2 (1-12c)^2.
$$
Therefore there are at most 
$$
\cPi (13+12c)^2/ (1-12c)^2 \leq k := \cPi 14^2,
$$
such triangles, and the edge $e$ is thus cut in at most $k$ parts by the edges joining an extremal vertex in $\cV$ to the corresponding vertex in $\cV_0$.

Hence there are at most $3k$ vertices of $\cT'$ on the three edges of a triangle $T\in \cT$ (including the vertices of $T$).
Since any conforming triangulation of convex envelope of $n+2$ points uses $n$ triangles, we obtain that $\cT'$ is a $3k-2$ refinement of $\cT$.
\sq

\input{../Bibliography/Bibliography.tex}
\end{document}



==> MeshMetric/MeshMetricTheseOld5.tex <==
\input{../PreambleThese}

\section{Introduction}

Triangulations and meshes are finite objects of combinatorial nature: they can be described by a collection of vertices and of connection between these. This description is fruitful for the demonstration of algebraic results, such as the Euler formula, or for computer processing.
In contrast, many approaches towards anisotropic mesh generation are based on a continuous object, namely a riemannian metric $z\mapsto H(z)$, in other words a continuous function $H$ from the domain $\Omega\subset \R^d$ to the set $S_d^+$ of symmetric positive definite matrices. Once this metric has been properly designed, it is the task of a mesh generation algorithm such as \cite{Shew,Bois,FreeFem,Inria} to generate a triangulation that agrees with this metric, in a sense specified below \iref{defEquiv}.
The purpose of this chapter is to formulate precise equivalence results between some classes of triangulations and of riemannian metrics. This equivalence translates some geometrical constraints satisfied by the triangulations into the form of regularity properties of the equivalent riemannian metrics.\\

Our results are so far limited to meshes and metrics defined on the entire infinite domain $\R^d$, and the dimension $d\geq 2$ is fixed throughout this chapter. 
The choice of the unbounded domain $\R^d$ guided by simplicity, since the curvature and the singularities of
of the boundary $\partial\Omega$ induces additional difficulties 
from the point of view of computational mesh generation.
Bounded domains will be the object of future work.
We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$, and we introduce in \S\ref{subsecDefTStar} three embedded subsets of $\bT$ of particular interest 
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
where $C\geq 1$ is a parameter which plays a minor role.
The set $\bT_{i,C}$ collects all \emph{isotropic} meshes $\cT$ which are heuristically defined as follows: the simplices $T\in \cT$ may have strongly varying volumes, but their aspect ratio is uniformly bounded. 
The largest set $\bT_{g,C}$ collects \emph{graded} meshes, which only satisfy a condition of local consistency: all the  geometrical features of the simplices $T\in \cT$ may vary strongly, volume, aspect ratio and orientation, but two \emph{neighboring} simplices should not be excessively different.
The intermediate set $\bT_{a,C}$ collects \emph{quasi-acute} meshes, which definition involves the measure of sliverness $S(T)$ of a simplex $T$ introduced in Chapter \ref{chapW1P} and also discussed in Chapter \ref{chapApproxMet}. 
The measure of sliverness plays an important role in the finite element approximation of a function on a mesh $\cT$ when the error is measured in the Sobolev $W^{1,p}$ norm.\\

We associate to each simplex $T$ a symmetric positive definite matrix $\cH_T$ such that the ellipsoid
$$
\cE_T := \{z\in \R^d \sep (z-z_T) \cH_T (z-z_T)^\trans \leq 1\},
$$
which is centered at the barycenter $z_T$ of $T$,
is the ellipsoid of minimal volume containing $T$. The properties of the matrix $\cH_T$ are discussed in \S \ref{subsecIntroSimplex} of this introduction,  as well as its explicit expression in terms of the coordinates of the simplex $T$. The matrix $\cH_T\in S_d^+$ encodes the volume, the aspect ratio and the orientation (but not the angles) of the simplex $T$. Two triangles $T$ and their associated ellipses $\cE_T$ are illustrated on figure \ref{figET}.

\begin{figure}
\centering
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleAigu.pdf}
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleObtus.pdf}
	\caption{Two triangles $T$ and their associated ellipse $\cE_T$.\label{figET}}
\end{figure}

A riemannian metric on $\R^d$ is a continuous map $H$ which associates to any $z\in \R^d$ a symmetric positive definite matrix $H(z)\in S_d^+$. We denote by $\bH = C^0(\R^d,S_d^+)$ the collection of riemannian metrics.
The following definition introduce a notion of equivalence between meshes and metrics
\begin{definition}
\label{defEqHT}
We say that a mesh $\cT\in \bT$ is $C_0$-equivalent to a given metric $H\in \bH$, where $C_0\geq 1$ is a fixed constant, if for all $T \in \cT$ and all $z\in T$ one has 
\be
\label{defEquiv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
\ee
We say that a collection of simplicial meshes $\bT_*\subset \bT$ is equivalent to a collection $H_*$ of metrics if there exists a uniform constant $C_0\geq 1$ such that the following holds:
\begin{itemize}
\item For any mesh $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\item For any metric $H\in \bH_*$ there exists a mesh $\cT\in \bT_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\end{itemize}
\end{definition}
Our main result (Theorem \ref{thEquiv}) states that when the constant $C$ is sufficiently large, and if dimension is $d=2$, the three classes of meshes $\bT_{i,C}\subset \bT_{a,C} \subset \bT_{g,C}$ are respectively equivalent to three classes of metrics
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
that are defined by precise smoothness conditions on the function $z\mapsto H(z)$ in \S \ref{subsecDefHStar} of this introduction.
%Our main result Theorem \ref{thEquiv} states that when the parameter $C$ is large enough and the dimension is $d=2$, the collections $\bT_{\star,C}$ of triangulations are equivalent to the corresponding collections $H_\star$ of metrics for any symbol $\star \in \{i,a,g\}$. 
The most striking point of this result is that, although the matrix $\cH_T$ does not encode the angles of a simplex $T$, the fact that a mesh $\cT\in \bT_{a,C}$ is \emph{quasi-acute} can be translated in a precise regularity condition on the metric $H$ equivalent to $\cT$.

In order to state our results more precisely we need to introduce some notations. We first recall some notations of linear algebra. We denote by $\M_d$ the collection of $d\times d$ matrices with real entries. We denote by $\GL_d$ the standard linear group, by $\SL_d$ the special linear group and by $\cO_d$ the orthogonal group
\begin{eqnarray*}
\GL_d &:=& \{A\in \M_d\sep \det A\neq 0\}\\
\SL_d &:=& \{A\in \M_d\sep \det A=1\}\\
\cO_d &:=& \{U\in \M_d\sep U^\trans U = \Id\}.
\end{eqnarray*}
We denote by $S_d$ the collection of symmetric matrices, by $S_d^\oplus$ the subset of non-negative symmetric matrices, and by $S_d^+$ the collection of symmetric positive definite matrices.
\begin{eqnarray*}
S_d &:=& \{M\in \M_d\sep M = M^\trans\}\\
S_d^\oplus &:=& \{M\in S_d\sep z^\trans M z \geq 0 \text{ for all } z\in \R^d\}\\
S_d^+ &:=& S_d^\oplus \cap \GL_d.
\end{eqnarray*}
Let $M,M'\in S_d$, we write $M\leq M'$ if $M'-M\in S_d^\oplus$, and $M< M'$ if $M'-M\in S_d^+$. We recall that for any $M,M'\in S_d$ such that $M\leq M'$ and any $\phi\in \M_d$ we have $\phi^\trans M \phi \leq \phi^\trans M' \phi$. Furthermore if $M,M' \in S_d^+$ and $M\leq M'$ then $M'^{-1} \leq M^{-1}$. For each symmetric positive definite matrix $M\in S_d^+$ we define a norm $\|\cdot\|_M$ as follows: for all $u\in \R^d$
$$
\|u\|^2_M := u^\trans M u.
$$

\subsection{Geometry of the simplex}
\label{subsecIntroSimplex}
The basic geometrical object studied in this chapter is the $d$-dimensional simplex, which is defined as follows.
\begin{definition}
A $d$-dimensional simplex $T$ is the convex envelope of a set $V\subset \R^d$ of $d+1$ %non-coplanar 
vertices, not contained in a $d-1$ dimensional affine subspace of $\R^d$ : 
$$
T = \Cvx(V).
$$
We denote by $\cF(T)$ the collection of faces of $T$ of any dimension,
\be
\label{defFT}
\cF(T) := \{\Cvx(V') \sep V'\subset V\}.
\ee
\end{definition}
Observe that $\emptyset$ and $T$ are among the faces of a simplex $T$, since they respectively correspond to $V'=\emptyset$ and $V'=V$.
We denote by $z_T\in \R^d$ the barycenter of a simplex $T$ of vertices $V$
$$
z_T := \frac 1 {d+1} \sum_{v\in V} v,
$$
and we define a symmetric positive definite matrix $\cH_T\in S_d^+$ as follows
\be
\label{defcH}
\cH_T^{-1} = \frac d {d+1} \sum_{v\in V} (v-z_T) (v-z_T)^\trans. %\frac {2d}{(d+1)^2}\sum_{v,v'\in V} (v-v')(v-v')^\trans. 
\ee
Some of the key properties of the matrix $\cH_T$ are exposed in the next proposition.
Throughout this chapter, we denote by $\TEq$ a $d$-dimensional equilateral simplex, centered at the origin
i.e. such that $z_\TEq=0$, and having its vertices on the unit ball. One easily checks that 
$$
\cH_\TEq = \Id.
$$
% Note that 
%\be
%\label{eqBallTEq}
%%\{z\in \R^d \sep |z| \leq 1/d\} 
%B(0, 1/d) \subset \TEq \subset \overline B(0,1).
%\ee
%
%%We associate to any simplex $T$ its barycenter $z_T\in \R^d$, and a symmetric positive definite matrix
%We denote by $z_T$ the barycenter of a simplex $T$, and we also associate to $T$ a symmetric positive definite matrix $\cH_T\in S_d^+$ which encodes some of its geometrical properties, in particular the volume, the elongation and the orientation of $T$.
\begin{prop}
\label{propHT}
The following holds for any $d$-dimensional simplex $T$. 
\begin{itemize}
\item
For any an affine change of coordinates $\Phi$, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0$ in $\R^d$, we have 
\be
\label{invcH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
\item
There exists a rotation $U\in \cO_d$, depending on $T$, such that 
\be
\label{eqcHTEq}
\cH_T^\frac 1 2 (T-z_T) = U(\TEq),
\ee
hence 
\be
\label{eqVolTHT}
|T| \sqrt{\det \cH_T} = |\TEq|.
\ee
\item
We have the inclusions 
\be
\label{eqTET}
\{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1/d\} \subset T \subset \cE_T := \{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1\},
\ee
and the these two ellipsoids are respectively the one of largest volume included in $T$, and of smallest volume containing $T$.
\end{itemize}
\end{prop}
\proof
For any simplex $\Phi^{-1}(v)$ of the simplex $\Phi^{-1}(T)$, we have 
$$
\Phi^{-1}(v)-z_{\Phi^{-1}(T)} = \Phi^{-1}(v)-\Phi^{-1}(z_T) = \phi^{-1}(v-z_T).
$$
Injecting this relation in \iref{defcH} we obtain \iref{invcH}. 
We now turn to the proof of \iref{eqcHTEq} and for that purpose we remark that the simplices $\TEq$ and $T' := \cH_T^\frac 1 2 (T-z_T)$ have both their barycenter at zero, $z_\TEq = z_{T'} = 0$, hence there exists a linear map $\phi\in \GL_d$ such that $T' = \phi^{-1}(\TEq)$. We thus obtain, using the formula \iref{invcH} for the transformation of $\cH_T$ under affine change of coordinates 
$$
\begin{array}{ccccc}
\cH_{T'} &=& \cH_T^{-\frac 1 2} \cH_T \cH_T^{-\frac 1 2} &=& \Id \\ 
\cH_{\phi^{-1}(\TEq)} &=& \phi^\trans \cH_\TEq &=& \phi^\trans \phi.
\end{array}
$$
Hence $\phi^\trans \phi= \Id$ which establishes that $\phi\in \cO_d$ and concludes the proof of \iref{eqcHTEq}.
%One easily checks that 
%$$
%\overline B(0,1/d) \subset \TEq \subset \overline B(0,1),
%$$
%where
It is well known that the smallest ellipsoid containing $\TEq$ is the unit ball, and that the largest ellipsoid included in $\TEq$ is the ball of radius $1/d$. Combining this fact with the change of coordinates \iref{eqcHTEq} we obtain \iref{eqTET} which concludes the proof of this proposition.
\sq

Note that for any simplex $T$ and any $z,z'\in T$ we obtain using \iref{eqTET}
\be
\label{eqDiamTHT}
\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2.
\ee

We introduce a measure of degeneracy $\rho(T)$ of a $d$-dimensional simplex $T$
\be
\label{defRhoMM}
\rho(T) := \sqrt{\|\cH_T\| \|\cH_T^{-1}\|}.
\ee
%This measure of non degeneracy $\rho$ is slightly different from the measure of non degeneracy $\frac {\diam(T)^d} {|T|}$ used in some of the previous chapters. However these two measures play a similar role and can be compared. Indeed we obtain using \iref{eqVolTHT} and \iref{eqcTET}
%\be
%\label{eqRhoRhop}
%\frac{\rho(T)}{d^\frac d 2|\TEq|} \leq  \frac{(\|\cH_T^{-1}\|/d)^\frac d 2} {|\TEq| (\det \cH_T)^{-\frac 1 2}} \leq \frac{\diam(T)^d} {|T|} \leq \frac{\|\cH_T^{-1}\|^\frac d 2} {|\TEq|(\det \cH_T)^{-\frac 1 2}}\leq \frac{\rho(T)^{d-1}}{|\TEq|}.
%\ee
%Observing that $\|A\| \|A^{-1}\|^{-(d-1)} \leq |\det A| \leq \|A\|^{d-1} \|A^{-1}\|^{-1}$ for any $A\in \GL_d$
%it follows that 
Observe that $\rho(T)\geq 1$ for any simplex $T$, with equality if and only if $\cH_T$ is proportional to the identity, which implies in view of \iref{eqcHTEq} that $T$ is a displacement of the equilateral simplex $\TEq$:
$$
\rho(T) = 1 \stext{ if and only if }
%\ \Longleftrightarrow \ 
T = z_T+r U(\TEq) \text{ for some }  r>0 \text{ and } U \in \cO_d.
$$
The measure of degeneracy $\rho$ is slightly different from the measure of degeneracy $\frac {\diam(T)^d} {|T|}$ used in Chapters \ref{chapOptAniso} and \ref{chapW1P} but both have the same role: they are minimal for the equilateral simplex, and increase as the simplex becomes thinner.\\

The measure of sliverness $S(T)$ of a simplex $T$ is a quantity which plays an important role in the context of optimal mesh adaptation for the finite element approximation of a function in the Sobolev $W^{1,p}$ norm, see   \cite{Ba, Ja}, and Chapters \ref{chapW1P} and \ref{chapApproxMet}. 
This measure of sliverness is defined in Chapter \ref{chapW1P} and illustrated by several examples and equivalent quantities. We recall the definition of this quantity
\be
\label{defSMM}
S(T) := \inf \{ \|\phi\| \|\phi^{-1}\| \sep \phi \in \GL_d \text{ and } \phi(T) \text{ is acute } \},
\ee
a simplex is acute if the exterior normals $\n, \n'$ to any two distinct faces of $T$ have a negative scalar product $\<\n,\n'\>\leq 0$.
As observed in Chapter \ref{chapW1P}, the measure of sliverness $S(T)$ can be interpreted as the distance from $T$ to the collection of acute simplices.

The exterior normals $\n,\n'$ to any two $d-1$-dimensional faces of $\TEq$ satisfy $\<\n,\n'\> =-1/d$, hence this simplex is acute. Recalling \iref{eqcHTEq}
 we thus obtain for any simplex $T$
$$
S(T) \leq \rho(T).
$$
Apart from this upper bound, the matrix $\cH_T$ does not contain any direct information on the measure of sliverness $S(T)$.
%One of the key results of this chapter is that in a bidimensional triangulation $\cT$, and conjecturedly in higher dimension too, the variation of the matrix $\cH_T$ as $T$ varies in $\cT$ does encode the measure of sliverness in some sense.
For any bidimensional triangle $T$ of largest angle $\theta$, Proposition \ref{propSTan} of Chapter \ref{chapW1P} states that :
$$
S(T) = \max\left\{1, \tan \frac \theta 2 \right\}.
$$

\subsection{Simplicial meshes}
\label{subsecDefTStar}

As a starter, we recall the definition of a simplicial mesh of $\R^d$.
%We first briefly recall the defini
%Before introducing simplicial meshes, we briefly recall the definition of locally finite partitions of $\R^d$.

%In order to introduce q,xcl meshes 
\begin{definition}
\label{defSimplMesh}
A conforming simplicial mesh of $\R^d$ is a collection $\cT$ of simplices which satisfy the conformity axiom :  for all $T,T'\in \cT$
\be
\label{confAxiom}
T\cap T' \in \cF(T) \cap \cF(T'),
\ee
as well as the following properties
\begin{itemize}
\item (Covering) The simplices $T\in \cT$ cover the whole infinite domain $\R^d$:
$$
\bigcup_{T\in \cT} T = \R^d.
$$
\item (Partition) The interiors of the simplices $T\in \cT$ are pairwise disjoint: for any $T,T'\in \cT$,
$$
\interior (T) \cap \interior(T') \neq \emptyset\stext{ implies }  T=T'. %
$$
\item (Local finiteness) For any compact set $K \subset \R^d$, only a finite collection of simplices $T\in \cT$ intersect $K$:
$$
\{T \in \cQ \sep K \cap T \neq \emptyset \} \ \text{ is finite.}
$$
\end{itemize}
\end{definition}
The conformity axiom \iref{confAxiom} states that the intersection of any two simplices in $\cT$ needs to be a full common face.We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$.

For an optimal efficiency, numerous numerical simulation software use anisotropic meshes, in which the simplices may have an arbitrary shape. Anisotropic meshes are used for instance, to create a thin layer of simplices close to a geometric feature which is relevant in a numerical simulation.
In order to avoid excessively wild meshes, one often requires relevant  some consistency between the shapes of neighboring simplices.We therefore introduce for any constant $C \geq 1$ the class $\bT_{g,C} \subset \bT$ of \emph{graded} meshes, which is defined as follows.
A mesh $\cT$ belongs to $\bT_{g,C}$ if for any two simplices $T,T'\in \cT$ one has 
\be
\label{defTG}
T \cap T'\neq \emptyset \stext{ implies } C^{-2}\cH_T \leq \cH_{T'} \leq C^2 \cH_T.
\ee

For any $C\geq 1$ we also introduce the class $\bT_{i,C}$ of \emph{isotropic} meshes, by requiring that in addition to \iref{defTG} that the measure of degeneracy $\rho$ is uniformly bounded by $C$, which forbids any anisotropy.
A mesh $\cT$ belongs to $\bT_{i,C}$ if and only if $\cT\in \bT_{g,C}$ and for all $T \in \cT$
$$
\rho(T) \leq C. %C \geq 1? or 0? 
$$

%The next proposition shows that the definition of $\bT_{i,C}$ is slightly redundant, in the sense that condition \iref{defTG} could be avoided.
%\begin{prop}
%Denote by $\bT'_{i,C}$ the collection of meshes $\cT\in \bT$ satisfying $\rho(T) \leq C$ for all $T\in \cT$ (but perhaps not the gradedness condition \iref{defTG}). %We thus have $\bT_{i,C} \subset \bT'_{i,C}$.\\
%Then for all $C$ there exists $C' = C'(C)$ such that 
%$$
%\bT_{i,C} \subset \bT'_{i,C} \subset \bT_{i,C'}.
%$$
%\end{prop}
%
%\proof
%See appendix. 
%\sq

In order to introduce the intermediate collection $\bT_{a,C}$ of $C$-quasi-acute meshes, we first define the notion of refinement of a simplicial mesh.
\begin{definition}
Consider two meshes $\cT,\cT'\in \bT$ and a constant $C\geq 1$. We say that $\cT'$ is a $C$-refinement of $\cT$ if it satisfies the following properties.
\begin{itemize}
\item (Inclusion) Any simplex $T'\in \cT'$ is contained in a simplex $T\in \cT$. % such that $T'\subset T$.
\item (Bounded refinement) Any simplex  $T\in \cT$, contains most $C$ simplices $T'\in \cT$.
\end{itemize}
\end{definition}

A graded mesh $\cT \in \bT_{g,C}$ belongs to the collection $\bT_{a,C}$ of quasi-acute meshes if and only there exists a $C$-refinement $\cT'$ of $\cT$ which satisfies for all $T' \in \cT'$
$$
S(T') \leq C.
$$
In particular if $\cT\in \bT_{i,C}$, then choosing $\cT' = \cT$, which is a $C$-refinement since $C\geq 1$, and recalling that $S(T) \leq \rho(T)$ for any simplex $T$, we obtain that $\cT\in \bT_{a,C}$. Thus $\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}$ as announced.

The constraints defining graded, quasi-acute and isotropic meshes are illustrated on Figure \ref{figDisk}
in the main introduction of the thesis. 
Figure \ref{figAcuteGen} gives an example of a quasi-acute triangulation which 
by the above described refinement process leads to a slightly finer triangulation on
sliverness $S(T)$ is uniformly bounded.

\begin{figure}
\centering
%	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarGdeVap.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap1.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap2.pdf}
	\caption{\label{figAcuteGen}
Quasi-acute triangulation (left) and refined triangulation with uniformly bounded sliverness (right).
	}
\end{figure}

\subsection{Riemannian metrics}
\label{subsecDefHStar}

For any metric $H \in \bH$ and path $\gamma \in C^1([a,b],\R^d)$, we define the riemmannian length $l_H(\gamma)$ by the integral
$$
l_H(\gamma) := \int_a^b \|\gamma'\|_{H(\gamma(t))} dt.
$$
The riemmannian distance $d_H$ between two points  $z,z'\in \R^d$, is the infimum of the length of all paths joining $z$ and $z'$, 
\be
\label{defdH}
d_H(z,z') := \inf\left\{l_H(\gamma)\sep \gamma\in C^1\left([0,1],\R^d\right), \ \gamma(0) = z \text{ and } \gamma(1) = z'\right\}.
\ee
If $H, H'\in \bH$ are such that $H(z) \leq H'(z)$ for all $z\in \R^d$, then $d_H(z,z') \leq d_{H'}(z,z')$ for all $z,z'\in \R^d$.
By construction, the riemannian distance $d_H$ associated to a metric $H\in \bH$ is locally equivalent close to a point $z$ to the distance defined by the norm $\|\cdot \|_{H(z)}$: for all $z\in \R^d$
\be
\label{eqDistLoc}
\limsup_{\ve \to 0} \sup_{p,q\in B(z, \ve)} |\ln d_H(p,q) - \ln \|p-q\|_{H(z)}| = 0,
\ee
where $B(z,\ve)$ denotes the euclidean ball of radius $\ve$ around $z$.\\


\begin{remark}[Riemannian geodesics]
When a metric $H$ is sufficiently smooth, a special family of curves named Riemannian geodesics can be defined and studied. A riemannian geodesic is a curve $\gamma\in C^0(\R, \R^d)$ which satisfies a second order differential equation %written in terms of the second order derivatives of $H$, 
called the equation of geodesics. This equation implies that for any sufficiently close $t,t'\in \R$ the curve $\gamma_{|[t,t']}$ is the path of smallest possible length joining the points $\gamma(t)$ and $\gamma(t')$ : 
$d_H(\gamma(t), \gamma(t')) = l_H(\gamma_{|[t,t']})$.

Geodesics are not defined for general continuous or Lipschitz riemannian metrics, such as those constituting the sets $\bH$ and $\bH_i \subset \bH_a\subset \bH_g$, since the coefficients of the equation of geodesics involve the second derivatives of the metric. Notions related to geodesics, such as the injectivity radius of a metric, therefore have no meaning in our context.
This is not an issue for our purposes since, following the point of view of \cite{Gromov},
%[Gromov, Metric structures for Riemannian and non-Riemannian spaces, Birkhauser (1999)]
we study Riemannian distances and not Riemannian geodesics. 

%Note also that geodesics only exist when the metric $H$ has requires that $H$ has at least $C^2$ smoothness, while the metrics studied in this chapter generally only have $C^0$ or Lipschitz smoothness.

%Since we only assume that $H$ is a continuous metric, the infimum \iref{defdH} may or may not be attained, and in that later case possibly for several paths. The equation of geodesics associated to a riemannian metric involves the second order derivatives, which are not defined in our context.
%(* also the point of view of Gromov : we study distances and not geodesics*)
\end{remark}


We denote by $\bH_i$ the collection of metrics $H \in \bH$ which are proportionnal to the identity: for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2},
$$
and such that the proportionality factor $s$ satisfies one of the two following conditions conditions, which are surprisingly equivalent as shown in Proposition \ref{propEquivS}:
\begin{itemize}
\item (``Additive'' Lipschitz condition)  
\be
\label{eqLipSAdd}
|s(z) - s(z')| \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
\item (``Multiplicative'' Lipschitz condition)
\be
\label{eqLipSMult}
|\ln s(z) - \ln s(z')| \leq d_H(z,z') \stext{ for all } z,z'\in\R^d.
\ee
\end{itemize}

The two Lipschitz properties \iref{eqLipSAdd} and \iref{eqLipSMult} have a natural generalisation to general anisotropic metrics but are not equivalent in that context.
In order to introduce the regularity conditions defining the classes $\bH_i\subset \bH_a\subset \bH_g$ of metrics, we need to  two distances $d_\times$ and $d_+$ on the set $S_d^+$ of symmetric positive definite matrices. 
For any $M,M'\in S_d^+$ we define
\be
\label{defDTimes}
d_\times (M,M') := \min \{\delta \geq 0 \sep e^{-2\delta} M \leq M' \leq e^{2 \delta} M\}.
\ee
For instance, a mesh $\cT$ is $C$-equivalent to a metric $H$, as defined in \iref{defEquiv}, if and only if for all $T \in \cT$ and all $z\in \cT$ one has 
$$
d_\times (H(z), \cH_T) \leq \ln C.
$$
There exists various expressions of the distance $d_\times$ : for all $M,M'\in S_d^+$ one has 
\be
\label{eqDTimesLog}
\begin{array}{rcl}
d_\times (M,M') &=& \displaystyle\sup_{u\in \sR^d\sm \{0\}} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|\vspace{2mm}\\
&=&\displaystyle \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|
\end{array}
\ee
and 
\be
\label{eqDTimesProd}
d_\times (M,M') = \ln \left(\max \{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\}\right).
\ee
The exponential of the distance $d_\times$ was used in the earlier paper \cite{Shew} %on anisotropic mesh generation
under the name ``relative deformation''. 
We define a second distance $d_+$ on $S_d^+$ as follows 
\be
\label{defDPlus}
d_+(M,M') := \|M^{-\frac 1 2} - M'^{-\frac 1 2}\|.
\ee
The expressions \iref{eqDTimesProd} and \iref{defDPlus} of the distances $d_\times$ and $d_+$ show that they are respectively tied to multiplicative or additive properties of matrices, which justifies their notations.
Note also that for any $s,s'>0$ one has
\be
\label{eqDIso}
d_\times (s^{-2} \Id, s'^{-2} \Id) = |\ln s - \ln s'| \stext{ and } d_+(s^{-2} \Id, s'^{-2} \Id) = |s-s'|.\\
\ee

We denote by $\bH_g$ the collection of metrics $H\in \bH$ which satisfy the natural extension of \iref{eqLipSMult} to general anisotropic metrics:
\be
\label{eqLipMult}
d_\times (H(z), H(z')) \leq d_H(z,z') \stext{ for all }z,z'\in\R^d.
\ee
This condition can be heuristically described as follows: a metric $H\in \bH$ defines close to each point $z\in\R^d$ a norm $\|\cdot\|_{H(z)}$ which encodes an anisotropic notion of scale. The equation \iref{eqLipMult} states that the metric $H$ itself is consistent a the scale that it encodes.\\

We denote by $\bH_a$ the collection of metrics $H\in \bH$ which satisfy both \iref{eqLipMult} and the natural extension of \iref{eqLipSAdd} to general anisotropic metrics:
\be
\label{eqLipAdd}
d_+ (H(z), H(z')) \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
In addition to the results of mesh generation presented in this chapter, we show in the next chapter, Chapter\ref{chapApproxMet}, that this condition is critical in order to define a local averaging operator compatible with Sobolev norms. 
%decrire le lien avec les angles aigus.
\begin{remark}
\label{remHomog}
Let $H\in \bH$, and let $\lambda>0$. Using the homogeneity properties of the distances $d_\times$, $d_+$ on $S_d^+$ and $d_H$ on $\R^d$ with respect to $H$, we obtain that $\lambda^2 H\in \bH_g$ if and only if 
\be
\label{eqLipTimesLambda}
d_\times (H(z), H(z')) \leq \lambda d_H(z,z') \stext{ for all } z,z'\in \R^d, 
\ee
and $\lambda^2 H\in \bH_a$ if and only if we have in addition to the previous property 
\be
\label{eqLipPlusLambda}
d_+ (H(z), H(z')) \leq \lambda |z-z'| \stext{ for all } z,z'\in \R^d.
\ee
In particular the collections $\bH_i \subset \bH_a \subset \bH_g$ of isotropic, quasi-acute and graded metrics are stable under multiplication by a constant larger than one : for any $\star \in \{a,b,c\}$, any $H\in \bH_\star$ and any $\lambda \geq 1$ we have $\lambda^2 H\in \bH_\star$.
%this operation corresponds to the uniform refinement of a triangulation...
\end{remark}

\subsection{Main results}

The main result of this chapter is the equivalence of the classes of meshes and metrics defined above, which is  announced in the first part of the introduction and proved in sections \S\ref{secMeshToMet} and  \S \ref{secMetToMesh}. In two cases we were only able to establish this equivalence when the dimension is $d=2$. 
\begin{theorem}
\label{thEquiv}
There exists $C_0 = C_0(d)$ such that for all $C\geq C_0$ the following holds.
\begin{enumerate}[i)]
\item The collections $\bT_{i,C}$ of triangulations and $\bH_i$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{a,C}$ of triangulations and $\bH_a$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{g,C}$ of triangulations and $\bH_g$ of metrics are equivalent.
\end{enumerate}
\end{theorem}

Let us comment on this result.
The theory of isotropic meshes is already well developed, and our result i) in this direction should be regarded as a reformulation of previous work, intended to put into perspective the results on anisotropic meshes. The main ingredient of the proof of i) is the mesh refinement procedure exposed in \cite{Nochetto}. 

In the case iii) of graded metrics the key ingredients used for the construction of a bidimensional triangulation $\cT\in \bT_{g,C}$ equivalent to a metric $H \in \bH_g$ come from the paper of computational geometry \cite{Shew}. In contrast the arguments used to produce a metric $H \in \bH_g$ from a mesh $\cT \in \bH_{g,C}$ hold in any dimension.

Last the author has not heard of any anterior results on the collection $\bT_{a,C}$ of quasi-acute meshes, and most of the techniques used in that context are new. 
The author is sorry to say that the proofs in that case are not yet as polished as the rest of the thesis, due to time constraints.

\begin{conjecture}
The author conjectures that the points ii) and iii) of Theorem \ref{thEquiv} holds without restriction on the dimension $d$.
\end{conjecture}

This chapter is organised as follows. We establish in section \S \ref{secMetProp} some general properties of metrics in $\bH_a$ or $\bH_g$. 
We first prove in \S\ref{subsecMetInv} a property of invariance of the collection $\bH_g$ of graded metrics with respect to affine changes of coordinates.
The regularity assumptions \iref{eqLipMult} and \iref{eqLipAdd} defining graded and quasi-acute metrics simply mean that the map $H : \R^d \to S_d^+$ is Lipschitz with respect to some distances on $\R^d$ and $S_d^+$. 
We therefore study metrics from this point of view in \S\ref{subsecMetLip}.
We focus in \S\ref{subsecMetGeom} on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. In particular we compare the $d_H$ with the euclidean distance and we estimate the volume of balls. 


Section \S\ref{secEigen} is devoted to the study of metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has  an eigenspace of dimension at least $d-1$ at each point. This condition clearly holds if the dimension is $d=2$ but is also relevant in some applications to higher dimension such as the creation of a this layer of simplices close to a $d-1$ dimensional surface. This situation is discussed in Chapter \ref{chapApproxMet}, and involves metric which have an eigenvalue much larger that the others in the orthogonal direction to the surface of interest.
We give an approximate translation of the regularity properties \iref{eqLipAdd} and \iref{eqLipMult} defining the collections $\bH_a$ and $\bH_g$ of metrics in terms of the two eigenvalues of $H$ and of the direction of the eigenspaces of such metrics. 

The last two sections \S\ref{secMeshToMet} and \S\ref{secMetToMesh} are devoted to the proof of Theorem \ref{thEquiv}. More precisely we adress in \S\ref{secMetToMesh} the production of an isotropic, quasi-acute or graded mesh equivalent to a given metric $H\in \bH_i$, $\bH_a$ or $\bH_g$. Conversely we depict in \S\ref{secMeshToMet} to construction of a metric which is equivalent to a given mesh.


\section{General properties of graded and quasi-acute metrics}
\label{secMetProp}

We study in this section the general properties of the  distinguished classes of metrics $\bH_i \subset \bH_a \subset \bH_g$. 
We first establish in \S\ref{subsecMetInv} some invariance properties of these collections of metrics with respect to affine changes of coordinates.
We then regard in \S\ref{subsecMetLip} metrics as Lipschitz functions $H : \R^d\to S_d^+$. %, and we recall some basic properties of these.
The last subsection \S\ref{subsecMetGeom} is devoted to the comparison of the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$, with respect to the standard euclidean distance and Lebesgue measure.

\subsection{Invariance properties and restriction of metrics}
\label{subsecMetInv}

We focus in this subsection on the properties of invariance of the collections of meshes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ and of metrics $\bH_i \subset \bH_a\subset \bH_g$ introduced in this chapter.

Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$.
We have for any simplex $T$, as previously observed in \iref{invcH},
\be
\label{eqInvH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
Mimicking this property we define for any $H \in \bH$ a transported version $H_\Phi\in \bH$ as follows: for all $z\in \R^d$
\be
\label{defHPhi}
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi.
\ee
In the language of differential geometry,
the metric $H_\Phi$ is generally referred to as the ``pull back'' of $H$ by $\Phi$. If a mesh $\cT\in \bT$ is $C$-equivalent to a metric $H\in \bH$, then \iref{eqInvH} and \iref{defHPhi} clearly imply that the mesh $\Phi^{-1}(\cT)$ is $C$-equivalent to the metric $H_\Phi$.

The next proposition studies the invariance of the collections $\bT_{\star,C}$ of meshes and $\bT_\star$ of metrics, $\star \in \{i,a,g\}$, under the transformations $\cT \mapsto \Phi^{-1}(\cT)$ or $H \mapsto H_\Phi$ induced by an affine change of coordinates $\Phi$.

\begin{prop}
\label{propInvT}
Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. 
The following holds for any constant $C\geq 1$.
\begin{enumerate}[i)]
\item If $\cT \in \bT_{g,C}$ then $\Phi^{-1}(\cT) \in \bT_{g,C}$. If $H \in \bH_g$ then $H_\Phi\in \bH_g$.
\item Assume that $\Phi$ is an isometry, in other words $\phi\in \cO_d$.\\
If $\cT\in \bT_{a,C}$ then $\Phi^{-1}(\cT)\in \bT_{a,C}$, and similarly if $\cT\in \bT_{i,C}$ then $\Phi^{-1}(\cT)\in \bT_{i,C}$.\\
If $H\in \bH_a$ then $H_\Phi\in \bH_a$, and similarly if $H\in \bH_i$ then $H_\Phi\in \bH_i$.
\end{enumerate}
\end{prop}

\proof
%We concentrate on the case of meshes, since the statements on metrics are a special case of the propositions (??) and (??) below (* no : state the result for iso and quasi acute metrics too*).
%We first consider the case of meshes, and then 
We first establish the properties announced for meshes, and we then focus on metrics.
Let $M,M'\in S_d^+$, let $C\geq 1$ and let $\phi\in \GL_d$. Clearly
$$
\text{ if } C^{-2} M \leq M' \leq C^2 M \stext{ then } C^{-2} \phi^\trans M\phi \leq \phi^\trans M'\phi  \leq C^2 \phi^\trans M\phi.
$$
%Consequently if a mesh $\cT$ satisfies the condition \iref{defTG} defining the elements of $\bT_{g,C}$
%
%satisfy $C^{-2} M \leq M' \leq C^2 M$, then we also ha
%For any $M,M'\in S_d^+$ we obtain using \iref{defDTimes} that 
%$$
%d_\times (\phi^\trans M \phi,\ \phi^\trans M' \phi) = d_\times (M,M').
%$$
%It follows using \iref{eqInvH} that for any  two simplices $T,T'$,
%$$
%d_\times (\cH_{\Phi^{-1}(T)}, \cH_{\Phi^{-1}(T')}) = d_\times (\cH_T,\cH_{T'}).
%$$ 
In view of the definition \iref{defTG} of $\bT_{g,C}$ we obtain that $\Phi^{-1}(\cT)\in \bT_{g,C}$ for any mesh $\cT\in\bT_{g,C}$ as announced in i).

If $\Phi$ is an isometry then for any simplex $T$ we obtain, using the definitions \iref{defRhoMM} and \iref{defSMM} of the measure of degeneracy $\rho$ and the measure of sliverness $S$, that
$$
\rho(\Phi^{-1}(T)) = \rho(T) \stext{ and } S(\Phi^{-1}(T)) = S(T).
$$
This implies the properties of $\bT_{a,C}$ and $\bT_{i,C}$ announced in b), which concludes the proof of the properties announced for meshes.

We therefore turn our attention to metrics. The fact that $H_\Phi\in \bH_g$ for any $H\in \bH_g$ and any affine change of coordinates $\Phi$ is a special case of Proposition \ref{propHG} below. We thus admit this property and we focus on isotropic and quasi-acute metrics and \emph{isometric} changes of coordinates.

If $H\in \bH_i$, then $H = \Id/s(z)^2$ where $s: \R^d \to \R_+^*$ is a Lipschitz function. Since $\phi\in \cO^d$ we have $\phi^\trans \phi = \Id$ and therefore 
$$
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi = \Id/s(\Phi(z))^2.
$$
The map $s \circ \Phi : \R_d\to \R_+^*$ is Lipschitz since it is the composition of a Lipschitz function with an isometry, which establishes that $H_\Phi\in \bH_i$ as announced.

Since $\phi\in \cO_d$ we have for any symmetric matrix $M\in S_d^+$ and any exponent $\alpha\in \R^d$
$$
(\phi^\trans M \phi)^\alpha = \phi M^\alpha \phi.
$$
Consider $H\in \bH_a$, then for any $z,z'\in \R^d$
\begin{eqnarray*}
\|H_\Phi(z)^{-\frac 1 2}-H_\Phi(z')^{-\frac 1 2}\| &=& \|\phi^\trans \left(H(\Phi(z))^{-\frac 1 2}-H(\Phi(z'))^{-\frac 1 2}\right) \phi\| \\
&=& \|H(\Phi(z))^{-\frac 1 2}-H(\Phi(z'))^{-\frac 1 2}\|\\
& \leq& \|\Phi(z)-\Phi(z')\|\\
& =& \|\phi(z-z')\|= |z-z'|,
\end{eqnarray*}
which establishes that $H_\Phi$ satisfies the Lipschitz regularity condition \iref{eqLipAdd}. We already know from the case of graded metrics that the other regularity condition \iref{eqLipMult} is satisfied by $H_\Phi$, which establishes that $H_\Phi\in \bH_a$ and concludes the proof of this proposition.
\sq


In practical applications, one often needs to mesh simultaneously a domain $\Omega$ and a surface $\Gamma$ embedded in $\Omega$. In terms of metric this raises the following question: given a metric $H$ on $\Omega$ which satisfies certain properties of regularity %, corresponding do a certain class of meshes, 
what is the regularity of the restriction of this metric to $\Gamma$?

The next proposition answers this question is the simplified setting where $\Omega$ is the infinite domain $\R^d$, $\Gamma$ is an affine subspace of $\R^d$, and properties of regularity are those defining the collection $\bH_g$ of graded metrics. For any $1\leq k \leq d$ we denote by $\bH_g(\R^k)$ the collection of graded metrics on $\R^k$.

\begin{prop}
\label{propHG}
Let $1\leq k\leq d$, let $\Phi : \R^k\to \R^d$ be an affine injective map, $\Phi(z) = \phi z+z_0$ where $\phi\in M_{d,k}$ has rank $k$ and $z_0\in \R^d$. Let $H\in \bH$ and let for all $z\in \R^k$
$$%\be
%\label{defHPhi}
H_\Phi(z) := \phi^\trans H(\Phi(z)) \phi.
$$%\ee
If $H\in \bH_g$ then $H_\Phi\in \bH_g(\R^k)$. 
\end{prop}

\proof
For any $u\in \R^d$, one has 
\be
\label{chgNorm}
\|u\|_{H_\Phi(z)} = \|\phi(u)\|_{H(\Phi(z))}.
\ee
Hence for any $z,z'\in \R^k$ we obtain using \iref{eqDTimesLog},
\be
\label{dNHPhi}
\begin{array}{rcl}
d(H_\Phi(z), \ H_\Phi(z'))  &=&\displaystyle \sup_{u\in \sR^k\sm\{0\}} \left|\ln \left\|\phi(u)\right\|_{H(\Phi(z))} -\ln \left\|\phi(u)\right\|_{H(\Phi(z'))}\right| \\
& \leq& d(H(\Phi(z)), \  H(\Phi(z')))
\end{array}
\ee
For any path $\gamma\in C^1([0,1], \R^k)$, it follows from \iref{chgNorm} that % the distorted lengths tied to $H$ and $H_\phi$ are therefore linked by 
$$
l_H(\Phi\circ \gamma) = \int_0^1 \|\phi(\gamma'(t))\|_{H(\Phi(\gamma(t)))}dt =  l_{H_\Phi}(\gamma).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^k)$ joining two points $z,z'\in \R^k$, we obtain since $\Phi\circ \gamma\in C^1([0,1], \R^d)$ is a path joining $\Phi(z)$ and $\Phi(z')$
\be
\label{dHPhi}
d_H(\Phi(z), \Phi(z')) \leq d_{H_\Phi}(z,z')
\ee
Combining \iref{dNHPhi} and \iref{dHPhi}, we conclude the proof of this proposition.
\sq


\subsection{Metrics as Lipschitz functions}
\label{subsecMetLip}
%Lipschitz functions play an important role in this chapter and in particular in this section. We recall here their basic properties.
Consider to abstract metric spaces $(X,d_X)$ and $(Y,d_Y)$ and a continuous function $f \in C^0(X , Y)$. We define 
the dilatation $\dil(f) \in [0, \infty]$ of $f$ as follows
$$
\dil(f) := \sup_{\substack{x,x'\in X \\ x \neq x'}} \frac{d_Y(f(x),f(x'))}{d_X(x,x')}
$$

We say that $f$ is Lipschitz if $\dil(f) \leq 1$, and more generally that $f$ is $\lambda$-Lipschitz if $\dil(f) \leq \lambda$.
We define the local dilatation $\dil_x(f)$ of a function $f\in C^0(X,Y)$ at a point $x\in X$ as follows
\be
\label{defDilX}
\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
\lim_{\ve\to 0} \left(\sup_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
\ee
%\be
%\label{defDilX}
%\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
%\lim_{\ve\to 0} \left(\sup_{e,e'\in B(x,\ve)} \frac{d_Y(f(e),f(e'))}{d_X(e,e')}\right).
%\ee
We specify the distance function on $X$ or $Y$ if it is not the expected ``canonical one'', for instance if $X$ or $Y$ is a subset of $\R^k$ and if the associated distance is not the standard euclidean distance but the riemannian distance $d_H$ associated to a metric, or if $X$ or $Y$ is the collection $S_d^+$ of symmetric positive definite matrices since none of the two distances $d_+$ or $d_\times$ is canonical. The local dilatation is in that case denoted as follows
$$
\dil_x(f\sep d_X, d_Y), \quad \dil_x(f\sep d_X)  \stext{ or } \dil_x(f\sep d_Y).
$$

The local dilatation $\dil_x(f)$ only depends on the local properties of the metric spaces close to $x$ and $f(x)$. Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$. For any $f\in C^0(\R^d, Y)$ and any $z\in \R^d$ we obtain using \iref{eqDistLoc}
\be
\label{eqDilNorm}
\|H(z)^{-1}\|^{-\frac 1 2} \dil_z(f) \leq \dil_z(f\sep d_H) = \dil_z(f \sep \|\cdot \|_{H(z)}) \leq \sqrt{\|H(z)\|} \dil_z(f)
\ee
We also introduce the lower local dilatation $\dil_z^*(f)\leq \dil_z(f)$ which is defined as follows
$$
\dil_z^*(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
$$
The next proposition establishes that local dilatations are sub-multiplicative.
\begin{lemma}
\label{lemmaSubMult}
Let $(X,d_X)$, $(Y,d_Y)$ and $(Z,d_Z)$ be three metric spaces, and let $f\in C^0(X,Y)$ and $g\in C^0(Y,Z)$. 
For any $x\in X$ one has 
\be
\label{eqDilUpper1}
\dil_x(g \circ f) \leq \dil_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side. Similarly we have 
\be
\label{eqDilLower1}
\dil_x(g \circ f) \geq \dil^*_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side.
\end{lemma}

\proof
We first establish \iref{eqDilUpper1}.
If $\dil_x(f) = \infty$ or $\dil_{f(x)}(g) = \infty$, then there is nothing to prove. We may therefore assume that $\dil_x(f) < \infty$ and $\dil_{f(x)}(g) < \infty$.
For any $\ve>0$ we define 
$$
F(\ve) = \sup_{p,q\in B(x, \ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)} \stext{ and } G(\ve) := \sup_{p,q\in B(f(x), \ve)} \frac{d_Z(g(p),g(q))}{d_Y(p,q)}
$$
It follows that 
$$
\sup_{p,q\in B(x, \ve)} \frac{d_Z(g(f(p)),g(f(q)))}{d_X(p,q)} \leq F(\ve) \, G(F(\ve) \ve).
$$
Taking the limit as $\ve \to 0$ we obtain \iref{eqDilUpper1} which concludes the proof.
For the proof of \iref{eqDilLower1} we consider two sequences $(p_n)_{n \geq 0}$, $(q_n)_{n \geq 0}$ which both tend to $x$ and such that $d_Y(f(p_n),f(q_n))/d_X(p_n, q_n) \to \dil_x(f)$ as $n \to \infty$. We thus have 
$$
\frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_X(p_n,q_n)} = \frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_Y(f(p_n),f(q_n))} \times \frac{d_Y(f(p_n),g(f(q_n)))}{d_X(p_n,q_n)},
$$
and taking the limit as $n \to \infty$ we obtain \iref{eqDilLower1} which concludes the proof of this lemma.
\sq

Let $f: \Omega \to V$ be a $C^1$ function, where $\Omega\subset \R^d$ is an open set and $V$ is a Banach space. Then for any $z\in \Omega$ the local dilatation $\dil_z(f)$, and the lower dilatation $\dil_z^*(f)$ have an explicit expression in terms of the differential $d_z f : \R^d \to V$ of $f$ at $z$
\be
\label{eqDilDiff}
\dil_z(f) = \sup_{|u|=1} \|d_z f(u)\| \stext{ and } \dil_z^*(f) = \inf_{|u|=1} \|d_z f(u)\|
\ee
Applying Lemma \ref{lemmaSubMult} and \iref{eqDilDiff} to the function $g=\ln$ we obtain for any metric space $(X,d_X)$, any $f\in C^0(X,\R_+^*)$ and any $x\in X$
\be
\label{eqDilLog}
\dil_x(\ln f) = \frac {\dil_x(f)} {f(x)} .
\ee

The following proposition shows that, under certain circumstances, the Lipschitz property is a local property.
\begin{prop}
\label{propDilLoc}
Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$.
For any $f\in C^0(\R^d, Y)$ and any path $\gamma\in C^1([0,1], \R^d)$, $\gamma(0) = z$, $\gamma(1) = z'$, one has
\be
\label{eqLipLocPath}
d_Y(f(z), f(z')) \leq l_H(\gamma) \sup_{0\leq t \leq 1} \dil_{\gamma(t)}(f\sep d_H).
\ee
It follows that %In particular 
\be
\label{eqDilLoc}
\dil(f\sep d_H) = \sup_{z\in \sR^d} \dil_z(f\sep d_H).
\ee
\end{prop}

\proof
%Consider $z,z'\in \R^d$, and a path $\gamma\in C^1([0,1],\R^d)$ such that $\gamma(0) = z$, $\gamma(1)=z'$ and $l_H(\gamma) \leq d_H(z,z')+\delta$ where $\delta>0$ is a constant that is devoted to tend to zero in the last step of the proof.
We equip the segment $[0,1]$ with the distance $d_\gamma$ defined for $0 \leq t\leq t'\leq 1$ by 
\be
\label{defDGamma}
d_\gamma(t,t') = d_\gamma(t',t) = l_H(\gamma_{|[t,t']}).
\ee
Note that for any $t\leq t_* \leq t'$ one has 
\be
\label{exactTri}
d_\gamma(t,t') = d_\gamma(t,t_*)+d_\gamma(t_*,t')
\ee
The map $\gamma : ([0,1], d_\gamma) \to (\R^d, d_H)$ is clearly Lipschitz.
It thus follows from Lemma \ref{lemmaSubMult} that $F := f\circ \gamma :[0,1] \to Y$ satisfies for all $t\in [0,1]$
$$
\dil_t(F) \leq \dil_{\gamma(t)}(f) \leq \lambda := \sup_{0\leq t'\leq 1} \dil_{\gamma(t')}(f).
$$
We assume that $\lambda<\infty$, otherwise there is nothing to prove, and we consider a fixed $\delta>0$. For each $t\in [0,1]$ there exists therefore an interval $V_t\subset [0,1]$ containing $t$, relatively open in $[0,1]$, and such that $F_{|V_t}$ is $(\lambda+\delta)$-Lipschitz. Since the segment $[0,1]$ is compact, there exists a finite set $I_0\subset [0,1]$ such that 
\be
\label{finiteCover01}
[0,1] = \bigcup_{t\in I_0} V_t.
\ee
Let $V,V'\subset [0,1]$ be two intersecting intervals, and assume that $F$ is $\lambda+\delta$ Lipschitz on $V$ and on $V'$. For any $t\in V$ and $t'\in V'$, there exists $t_*\in V\cap V'$ which satisfies $t\leq t_*\leq t'$ or $t\geq t_* \geq t'$. Recalling \iref{exactTri} we thus obtain  
\begin{eqnarray*}
d_Y(F(t),F(t')) &\leq& d_Y(F(t), F(t_*))+d_Y(F(t_*), F(t')) \\
&\leq& (\lambda+\delta) d_\gamma(t,t_*)+( \lambda+\delta)d_\gamma(t_*,t') \\
&=& (\lambda+\delta)d_\gamma(t,t').
\end{eqnarray*}
Thus $F$ is $\lambda+\delta$ Lipschitz on the interval $V\cup V'$. Since $[0,1]$ is covered by the finite collection of open intervals \iref{finiteCover01} on which $F$ is $\lambda+\delta$ Lipschitz, we obtain proceeding by induction that $F$ is $(\lambda+\delta)$-Lipshitz on $[0,1]$ and therefore 
$$
d_Y(f(z),f(z')) = d_Y(F(0),F(1))\leq (\lambda+\delta) d_\gamma(0,1) = (\lambda+\delta)l_H(\gamma). %\leq (\lambda+\delta)(d_H(z,z')+\delta).
$$
Letting $\delta\to 0$ we obtain \iref{eqLipLocPath}. Taking the infimum of \iref{eqLipLocPath} among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_Y(f(z),f(z')) \leq  \lambda d_H(z,z')$. Therefore $\dil(f\sep d_H) \leq \lambda$. Conversely we have $\dil_z(f\sep d_H) \leq \dil(f\sep d_H)$ for any $z\in \R^d$, which establishes \iref{eqDilLoc} and concludes the proof of this proposition.\sq

The next corollary shows that the global dilatation of a function is controlled by the local dilatation on $\R^d\sm \Gamma$, if $\Gamma$ is a \emph{sufficiently thin} set. For instance the skeleton $\cup_{T\in \cT} \partial T$ of a mesh $\cT\in \bT$.

\begin{corollary}
\label{corolLipNoGamma}
Let $\Gamma\subset \R^d$ be a set which has the following property : for any path $\gamma\in C^1([0,1], \R^d)$ there exists a sequence of paths $(\gamma_n)_{n \geq 0}$ which converge to $\gamma$ in $C^1$ norm and such that  $\{t\in [0,1]\sep \gamma_n(t) \in \Gamma\}$ is finite for each $n$.\\
Let $H\in \bH$, let $(Y,d_Y)$ be an arbitrary metric space, and met let $f\in C^0(\R^d, Y)$.
Then 
$$
\dil(f\sep d_H) = \sup_{z\in \R^d \sm \Gamma} \dil_z(f\sep d_H).
$$
\end{corollary}

\proof
We denote $\lambda := \sup_{z\in \R^d \sm \Gamma} \dil_z(f)$.
We consider two points $z,z'\in \R^d$ and a path $\gamma\in C^1([0,1], \R^d)$ such that $\gamma(0) = z$ and $\gamma(1) = z'$. %, and a sequence $\gamma_n$ converging to $\gamma$ in $C^1$ norm.

We first assume that the set $\{t\in [0,1]\sep \gamma(t) \in \Gamma\}$ is finite, and we denote its elements by $t_1< \cdots < t_k$. We set by convention $t_0 = 0$ and $t_{k+1} = 1$.
For each $0\leq i \leq k$ and each $t,t'$ such that $t_i <t<t'<t_{i+1}$ we have $d_Y(f(\gamma(t)),f(\gamma(t'))) \leq \lambda l_H(\gamma_{|[t,t']})$ according to Proposition \ref{propDilLoc}. Letting $t\to t_i$ and $t'\to t_{i+1}$ we obtain $d_Y(f(\gamma(t_i)),f(\gamma(t_{i+1}))) \leq \lambda l_H(\gamma_{|[t_i,t_{i+1}]})$. Adding up we obtain 
$$
d_Y(f(z), f(z')) \leq \sum_{0\leq i \leq  k} d_Y(f(\gamma(t_i)), f(\gamma(t_{i+1}))) \leq \lambda
\sum_{0\leq i \leq k} l_H(\gamma_{[t_i, t_{i+1}]}) = \lambda l_H(\gamma).
$$

We now consider the case where $\gamma$ meets the set $\Gamma$ an infinite number of times, and we choose a sequence $(\gamma_n)_{n \geq 0}$ as described is the statement of the corollary. We obtain $d_Y(f(\gamma_n(0)), f(\gamma_n(1))) \leq \lambda l_H(\gamma_n)$ for each $n\geq 0$. Taking the limit as $n \to \infty$ we obtain $d_Y(f(z), f(z')) \leq \lambda l_H(\gamma)$ since $\gamma_n$ converges to $\gamma$ is $C^1$ norm.

Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ we obtain $d_Y(f(z), f(z')) \leq \lambda d_H(z,z')$, which concludes the proof of this proposition.
\sq


%Let $(Y, \|\cdot \|_Y)$ and $(Z, \|\cdot\|_Z)$ be two banach spaces. Let $y\in Y$, $g\in C^1(Y,Z)$, and $L = g'(f(x))$, then clearly 
%$$
%\dil_y(g) = \|L\|.
%$$
%Injecting this in \iref{eqDilUpper1} we obtain 
%\be
%\label{eqDilUpper2}
%\dil_x(g \circ f) \leq\|L\|  \dil_x (f).
%\ee
%We also need a lower bound in several cases. For that purpose we define 
%$$
%\dil^*_z(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(z,\ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)}\right),
%$$
%and we obtain proceeding similarly, but with the different convention $0\times \infty = \infty\times 0 = 0$
%$$
%\dil_z(g\circ f) \geq \dil^*_{f(z)}(g) \dil_z(f).
%$$

The next proposition establishes that the regularity conditions \iref{eqLipMult} and \iref{eqLipAdd} defining the collections of quasi-acute or graded metrics are equivalent in the case of a metric proportionnal to the identity. %$\bH_a$ $\bH_g$

\begin{prop}
\label{propEquivS}
Let $s\in C^0(\R^d, \R_+^*)$ and let $H := \Id/s^2$. We have for all $z\in \R^d$
\be
\label{eqDilLnH}
\dil_z(\ln s\sep d_H) = \dil_z(s).
\ee
Furthermore the following properties are equivalent.
\begin{enumerate}
\item The map $s : \R^d \to \R$ is Lipschitz. (i.e. $H\in \bH_i$) %For all $z,z'\in \R^d$ one has $|s(z)-s(z')|\leq |z-z'|$.
\item (``Additive'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_+(H(z),H(z')) \leq |z-z'|$.
\item (``Multiplicative'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_\times(H(z),H(z'))\leq d_H(z,z')$.
\end{enumerate}
\end{prop}

\proof %reprendre preuve??
Combining \iref{eqDilNorm} and \iref{eqDilLog} we obtain for any $z\in \R^d$
$$
%\dil_z (H\sep  d_\times, d_H) = 
\dil_z(\ln s\sep d_H) = s(z) \dil_z(\ln s) = \dil_z(s),
$$
which establishes \iref{eqDilLnH}.
According to \iref{eqDIso} we have for any $z,z'\in \R^d$
$$
d_+(H(z),H(z')) = |s(z) - s(z')| \stext{ and } d_\times (H(z),H(z')) = |\ln s(z) - \ln s(z')|.
$$
The properties 1. and 2. are thus equivalent to $\dil(s)\leq 1$, and therefore also to :
\be
\label{eqDilsLoc}
\dil_z(s) \leq 1 \text{ for all } z\in \R^d,
\ee
according Proposition \ref{propDilLoc} applied to the constant metric $H_0 = \Id$ and to the function $f=s$.
On the other hand property 3. is equivalent to $\dil(\ln s \sep d_H) \leq 1$, and thus to :
$$
\dil_z(\ln s\sep d_H) \leq 1 \text{ for all } z\in \R^d,
$$
according to Proposition \ref{propDilLoc} applied to the metric $H$ and to the function $f=\ln s$.
This property equivalent to \iref{eqDilsLoc} according to \iref{eqDilLnH}, which concludes the proof of this Proposition.
\sq

The next corollary uses Proposition \ref{propEquivS} to analyse the regularity of the first and last eigenvalue of a metric.
\begin{corollary}
\label{corolLipNorm}
\begin{enumerate}
\item
For any $H\in \bH_g$, the map $z\mapsto \|H(z)\|^{-\frac 1 2}$ is Lipschitz.
\item
For any $H\in \bH_a$, the map $z\mapsto \|H(z)^{-\frac 1 2}\|$ is Lipschitz.
\end{enumerate}
\end{corollary}
\proof
We first establish Point 1.
We consider $H\in \bH_g$, and we define $s(z) := \|H(z)\|^{-\frac 1 2}$ and 
$$
H'(z) := \frac \Id {s(z)^2} = \|H(z)\|\Id,
$$
for each $z\in \R^d$.
Since $H(z) \leq H'(z)$ for all $z\in \R^d$, we have $d_H(z,z') \leq d_{H'} (z,z')$ for all $z, z'\in \R^d$.

Consider a pair $M,M'\in S_d^+$ of matrices and a real $\delta>0$. If $e^{-2\delta} M \leq M' \leq e^{2\delta} M$, then taking the norm we obtain $e^{-2\delta} \|M\| \leq \|M'\| \leq e^{2\delta} \|M\|$. It follows that 
$$
\frac 1 2 |\ln \|M\| - \ln \|M'\|| \leq d_\times (M,M').
$$
We thus have for any $z,z'\in \R^d$
\begin{eqnarray*}
|\ln s(z)-\ln s(z')| &=& \frac 1 2 \left|\ln \|H(z)\| - \ln \|H(z')\|\right| \\ %\left|\ln \left(\sqrt{\|H(z)\|}\right) -\ln \left(\sqrt{\|H(z')\|}\right)\right| \\%
%& \leq & \sup_{u\neq 0} |\ln \|u\|_{H(z)} - \ln \|u\|_{H(z')}|\\
&\leq & d_\times(H(z),H(z')) \\
&\leq& d_H(z,z')\\
&\leq& d_{H'}(z,z').
\end{eqnarray*}
Applying Proposition \ref{propEquivS} to the metric $H'$ we obtain that $H'\in \bH_i$, and therefore that $s$ is Lipschitz as announced.\\

We now turn to the proof of Point 2. For any metric $H\in \bH_a$ we have 
$$
\left|\|H(z)^{-\frac 1 2}\| - \|H(z')^{-\frac 1 2}\| \right| \leq \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| \leq |z-z'|
$$
for all $z,z'\in \R^d$,
which concludes the proof of this corollary.\sq

Our last proposition studies the local dilatation of the maximum and the minimum of two functions.
\begin{prop}
\label{propDilMax}
Let $(X,d_X)$ be a metric space and let $\lambda, \mu\in C^0(X, \R)$. Let $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda, \mu\}$. Then for all $x\in X$
\be
\label{eqDilMax1}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} \leq \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
If $(X,d_H) = (\R^d, d_H)$, where $H \in \bH$ is a riemannian metric, then equality holds
\be
\label{eqDilMax2}
\max\{\dil_x(\gamma\sep d_H), \dil_x(\Gamma\sep d_H)\} = \max\{\dil_x(\lambda\sep d_H), \dil_x(\mu\sep d_H)\}.
\ee
\end{prop}

\proof
We have for any $p,q\in X$,
\begin{eqnarray*}
|\gamma(p)-\gamma(q)| &=& |\min\{\lambda(p), \mu(p)\} - \min \{\lambda(q), \mu(q)\}|\\
& \leq & \max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}.
\end{eqnarray*}
For any $x\in X$ and any $\ve>0$ we thus obtain
\begin{eqnarray*}
\dil(\gamma_{|B(x,\ve)}) &=& \sup_{p,q\in B(x,\ve)} \frac{|\gamma(p)-\gamma(q)|}{d_X(p,q)} \\
&\leq& \sup_{p,q\in B(x,\ve)} \frac{\max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}}{d_X(p,q)}\\
& =& \max\left\{\sup_{p,q\in B(x,\ve)}  \frac{|\lambda(p)-\lambda(q)|}{d_X(p,q)}, \sup_{p,q\in B(x,\ve)}  \frac{|\mu(p)-\mu(q)|}{d_X(p,q)}\right\}\\
&=& \max\left\{\dil(\lambda_{|B(x, \ve)}), \dil(\mu_{|B(x,\ve)})\right\}.
\end{eqnarray*}
Letting $\ve \to 0$ we obtain $\dil_x(\gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$. Proceeding likewise for $\Gamma$ we conclude the proof of \iref{eqDilMax1}.\\


We now turn to the proof of \iref{eqDilMax2}. For that purpose we consider a fixed $\ve>0$ and we define
$$
K := \max \{\dil(\gamma_{|B(x,\ve)}\sep \|\cdot\|_{H(x)}), \ \dil(\Gamma_{|B(x,\ve)} \sep \|\cdot\|_{H(x)})\},
$$
where $B(x,\ve)$ stands for the euclidean unit ball of radius $\ve$ centered at $x$.
Consider two points $p,q\in B(x,\ve)$. If $\lambda(p) \geq \mu(p)$ and $\lambda(q)\geq \mu(q)$, or if $\lambda(p) \leq \mu(p)$ and $\lambda(q)\leq \mu(q)$, then 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)|&=& \max \{|\gamma(p)-\gamma(q)|, |\Gamma(p)-\Gamma(q)|\}\\
&\leq & K\|p-q\|_{H(x)}
\end{eqnarray*}
Otherwise if  $\lambda(p) \geq \mu(p)$ and $\lambda(q)\leq \mu(q)$, or $\lambda(p) \leq \mu(p)$ and $\lambda(q)\geq \mu(q)$, then there exists a point $r$ on the segment $[p,q]$ such that $\lambda(r)=\mu(r)$. We thus have %$|p-r|+|r-q| = |p-q|$ and 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)| &\leq& \max \{|\gamma(p)-\gamma(r)|, |\Gamma(r)-\Gamma(q)|\}\\
& &+ \max \{|\gamma(r)-\gamma(q)|, |\Gamma(r)-\Gamma(q)|\}\\
& \leq & K\|p-r\|_{H(x)} + K\|r-q\|_{H(x)} = K\|p-q\|_{H(x)}
\end{eqnarray*}
If follows that $\dil(\lambda_{|B(x,\ve)}\sep \|\cdot\|_{H(x)})\leq K$, and letting $\ve\to 0$ we obtain 
$$
\dil_x(\lambda\sep \|\cdot\|_{H(x)}) \leq \max\{\dil_x(\gamma\sep \|\cdot\|_{H(x)}), \ \dil_x(\Gamma \sep \|\cdot \|_{H(x)})\}.
$$ 
Recalling that $\dil_x(f\sep d_H) = \dil_x(f\sep \|\cdot\|_x)$ for any $f\in C^0(\R^d, \R)$ and any $x\in \R^d$, see \iref{eqDilNorm}, we obtain $\dil_x(\lambda\sep d_H) \leq \max\{\dil_x(\gamma\sep d_H), \ \dil_x(\Gamma\sep d_H)\}$. Proceeding likewise for $\mu$ we obtain \iref{eqDilMax2} which concludes the proof of this proposition.
\sq

\subsection{Geometric properties of the space $(\R^d, d_H)$} %Estimates of size}
\label{subsecMetGeom}

We focus in this subsection on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. The next proposition compares the riemannian distance $d_H$ between two points $z$ and $z+u$ with the norm $\|u\|_{H(z)}$ of their difference.

%with the euclidean distance and we estimate the volume of balls. 
%The next proposition compares the Riemannian distance associated to a graded metric, with 

\begin{prop}
\label{propEuclidRiemann}
Let $H \in \bH_g$ and let $z\in \R^d$. For all $u\in \R^d$ one has
\be
\label{eqEuclidRiemann}
\ln(1+\|u\|_{H(z)}) \leq d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention when $\|u\|_{H(z)}\geq 1$.
\end{prop}
\proof
%We first prove the left part of \iref{eqEuclidRiemann}, and for that purpose
We consider a path $\gamma\in C^1([0,1], \R^d)$, and we define for each $t\in [0,1]$
\be
\label{defLGamma}
l(t) := \int_0^t \|\gamma'(t)\|_{H(\gamma(t))}dt.
\ee
Since $H\in \bH_g$ we have for any $t\in [0,1]$
$$
\exp(-2\, d_H(z, \gamma(t))) \, H(z) \leq H(\gamma(t)) \leq  \exp(2 \, d_H(z, \gamma(t))) \, H(z)
$$
therefore, since $d_H(z, \gamma(t)) \leq l(t)$,
$$
\exp(-2l(t)) H(z)  \leq H(\gamma(t)) \leq  \exp(2l(t)) H(z).
$$
It follows that 
$$
\|\gamma'(t)\|_{H(z)} \exp(-l(t)) \leq l'(t) = \|\gamma'(t)\|_{H(\gamma(t))} \leq  \|\gamma'(t)\|_{H(z)} \exp(l(t)), %\exp(-l(t))
$$
hence 
\be
\label{eqGammapLp}
-\frac d {dt} \exp(-l(t)) \leq \|\gamma'(t)\|_{H(z)} \leq \frac d {dt} \exp(l(t)).
\ee
We have 
\be
\label{eqGammaGammap}
\|u\|_{H(z)} =  \|\gamma(1)-\gamma(0)\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt
\ee
with equality if $\gamma(t) = z+tu$ is the straight line.
%We now assume that $\gamma(t) \neq \gamma(0)$ for all $t\in (0,1]$, which is the case generically. The map $t\mapsto \|\gamma(t)-\gamma(0)\|_{H(z)}$ is therefore $C^1$ on $(0,1]$ and we have 
%$$
%\frac d {dt} \|\gamma(t)-\gamma(0)\|_{H(z)} \leq \|\gamma'(t)\|_{H(z)},
%$$
%with equality if $\gamma(t)-\gamma(0) = c \gamma'(t)$ for some $c>0$.
%In the special case of the straight line $\gamma(t)=z+tu$, \iref{eqGammaGammap} is an equality and we thus obtain 
For that specific path $\gamma$ we obtain %In that case, integrating the left part of \iref{eqGammapLp} we obtain
$$
\|u\|_{H(z)} = \int_0^1 \|\gamma'(t)\|_{H(z)} dt \geq -\int_0^1 \left(\frac d {dt} \exp(-l(t))\right)dt = 1-\exp(-l_H(\gamma)).
$$
Rearranging the terms we obtain the right part of \iref{eqEuclidRiemann}:
$$
d_H(z,z+u) \leq l_H(\gamma) \leq -\ln(1-\|u\|_{H(z)}).
$$
We now consider an arbitrary path $\gamma$ joining $z$ and $z+u$ and we obtain integrating the right part of \iref{eqGammapLp} and recalling \iref{eqGammaGammap}
$$
\|u\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt \leq \int_0^1 \left(\frac d {dt} \exp(l(t))\right) dt = \exp(l_H(\gamma)) -1,
$$
which is equivalent to
$$
l_H(\gamma) \geq \ln(1+\|u\|_{H(z)}).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ satisfying $\gamma(0) = z$ and $\gamma(1) = z+u$, we obtain the left part of \iref{eqEuclidRiemann}, which concludes the proof of this proposition.
\sq

We discuss in the rest of this section the consequences of the comparison \iref{eqEuclidRiemann} of the riemannian distance $d_H$ with the distance associated to the norm $\|\cdot\|_{H(z)}$ when $H\in \bH_g$. %is devoted to 
Combining the right part of \iref{eqEuclidRiemann} with the expression \iref{eqDTimesLog} of the distance $d_\times$ we obtain an estimate of the local variations of the norm $\|\cdot \|_{H(z)}$ associated to the metric $H$ at a point $z$: let $H\in \bH_g$, and let $z,u,v\in \R^d$ be such that $\|u\|_{H(z)} < 1$, then
\be
\label{eqLocalNorm}
(1-\|u\|_{H(z)}) \|v\|_{H(z)} \leq \|v\|_{H(z+u)} \leq (1-\|u\|_{H(z)})^{-1} \|v\|_{H(z)}. %\frac{\|v\|_{H(z)}}{1-\|u\|_{H(z)}}.
\ee
Note also that 
\be
\label{eqLocalDet}
(1-\|u\|_{H(z)})^d \sqrt{\det H(z)} \leq \sqrt{\det H(z)} \leq (1-\|u\|_{H(z)})^{-d} \sqrt{\det H(z)}.
\ee
Another important consequence of \iref{eqEuclidRiemann} is that for any $z\in \R^d$ and $r\geq 0$ the closed ball $\{z'\in \R^d \sep d_H(z,z')\leq r\}$ for the distance $d_H$, is a closed and bounded subset $\R^d$, hence is compact. %From this point a classical argument (??) shows that $(R^d,d_H)$ is a complete metric space.

The following example establishes that \iref{eqEuclidRiemann} is a sharp inequality. The metric $H$ defined by 
$$
H(z) := \frac \Id {(1+|z|)^2}
$$
belongs to $\bH_i$ since $z\mapsto 1+|z|$ is Lipschitz, hence $H$ also belongs to $\bH_a$ and $\bH_g$.
For any $v\in \R^d$, one easily checks that the path of minimal length joining $0$ to $v$ is the straight line, and that
$$
d_H(0, v) = \ln(1+|v|).
$$
Choosing $z=0$ and $u=v$ we obtain that the left part of \iref{eqEuclidRiemann} is sharp
$$
\ln (1+ \|u\|_{H(0)}) = \ln (1+ |u|) = d_H(0,0+u).
$$
Choosing $z=-v$ and $u = v$ we obtain that the right part of \iref{eqEuclidRiemann} is sharp
$$
-\ln\left(1-\|u\|_{H(-u)} \right) = -\ln \left(1-\frac {|u|}{1+|u|}\right) = \ln(1+|u|) = d_H(-u, -u+ u).
$$

The next corollary uses Proposition \ref{propEuclidRiemann} to obtain a lower bound for the mass of balls in the measure $z\mapsto \sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. %states a volume estimate Proposition \ref{propLength} implies a volume estimate. %also allows us to compare the vo
\begin{corollary}
\label{corolVol}
There exists $c=c(d)>0$ such that the following holds. Let $H \in \bH_g$,
let $L\geq 1$ and let $z_0\in \R^d$. Denoting by $\cE$ the ellipse 
$$
\cE = \{z\in \R^d\sep \|z-z_0\|_{H(z_0)}\leq L\}.
$$ 
we have 
\be
\label{eqVolLog}
\int_\cE \sqrt{\det H} \geq c \ln L. %\max\{L,1\}.
\ee
\end{corollary}

\proof
It follows from Proposition \ref{propEuclidRiemann} that $d(z_0, z) \geq \ln (L+1)$ for all $z\in \partial \cE$. We define the integer 
$$
k = \left\lfloor \ln(L+1) -\frac 1 2\right\rfloor,
$$
and we consider $k$ points $z_1, \cdots , z_k \in E$ such that 
$
d_H(z_0, z_i)= i
$ 
for all $0 \leq i \leq k$.
We define 
$
r_0 := 1-e^{-\frac 1 2} = 0.39\cdots
$
in such way that 
$
-\ln (1-r_0) = 1/2.
$
For all $0 \leq i \leq k$ we denote by $\cE_i$ the ellipse 
$$
\cE_i  := \left\{z\in \R^d \sep \|z-z_i\|_{H(z_i)} \leq r_0\right\}.
$$
We claim that $\cE_i \subset \cE$ for all $0 \leq i \leq k$. Indeed for any $z\in \cE_i$ we have 
$$
d_H(z_0, z) \leq d_H(z_0, z_i) + d_H(z_i, z) \leq i- \ln (1-r_0) \leq k+\frac 1 2 \leq \ln (L+1),
$$
Denoting by $\interior(E)$ the interior of a set $E\subset \R^d$, we observe that for all $0 \leq i<j\leq k$, for all $z\in \interior(\cE_i)$ and $z'\in \interior(\cE_j)$, we have
$$
d_H(z,z') \geq d_H(z_i, z_j) -d_H(z_i, z) - d_H(z_j,z') > |d_H(z_0, z_i) - d(z_0, z_j)| + 2\ln(1 -r_0) =0, %\geq 1+ 2 \ln(1-\frac 1 3)>0.
$$
hence $\interior(\cE_i) \cap \interior(\cE_j) = \emptyset$.
It follows that 
$$
\int_\cE \sqrt{\det H} \geq \sum_{0 \leq i \leq k} \int_{\cE_i} \sqrt{\det H}.
$$
Furthermore we have for all $z\in \cE_i$
$$
H(z) \geq (1-\|z-z_i\|_{H(z_i)})^2 H(z_i)  \geq (1-r_0)^2 H(z_i),
$$
and therefore 
\be
\label{eqzzi}
\sqrt{\det H(z)} \geq (1-r_0)^d \sqrt{\det H(z_i)}.
\ee
We denote by $B(z,r)$ the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$, and we observe that 
$u\mapsto z_i + H(z_i)^{-\frac 1 2} u$ maps $B(0,r_0)$ onto $\cE_i$. Combining this remark with \iref{eqzzi} we obtain
\begin{eqnarray*}
\int_{\cE_i} \sqrt{\det H} &\geq& (1-r_0)^d \int_{\cE_i} \sqrt{\det H(z_i)} \\
&=& (1-r_0)^d \int_{B(0,r_0)} 1 \\
&=& c_0 := r_0^d (1-r_0)^d |B(0,1)|.
\end{eqnarray*}
%where $B(z,r)$ denotes the euclidean unit ball $\{z'\in \R^d \sep |z'-z|\leq r\}$.
Eventually we obtain 
$$
\int_\cE \sqrt{\det H} \geq (k+1) c_0 \geq (\ln(L+1) - 1/2) c_0.
$$
In order to obtain \iref{eqVolLog} we simply recall that $L\geq 1$ and therefore that %Since Recalling that $L\geq 1$ we find that 
$$
\ln (L+1) = \frac{\ln(L+1)}{2 \ln 2} +  \left(1-\frac 1 {2 \ln 2}\right)\ln(L+1) \geq \frac 1 2 + \left(1-\frac 1 {2 \ln 2}\right)\ln L $$
which concludes the proof of \iref{eqVolLog} with $c=(1- 1/(2 \ln 2))c_0$.
%Applying \iref{eqVolLog} to $L = \lambda r$ we obtain \iref{volBR} which concludes the proof of this proposition.
\sq


\section{Metrics having an eigenspace of dimension $d-1$ at each point}
\label{secEigen}
We focus in this subsection on metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has an eigenspace of dimension at least $d-1$ at each point $z\in \R^d$. 
%If the dimension is $d=2$, then a metric $H\in \bH$ generically satisfies this condition on a dense subset of $\R^d$. %any metric $H\in \bH$ satisfies this condition. 
This condition clearly holds if the dimension is $d=2$, but is also relevant in higher dimension. 
Indeed, as discussed in \S\ref{secOptGeom} of Chapter \ref{chapApproxMet}, this type of metrics appears when one needs to create mesh containing a thin layer of simplices close to an hypersurface $\Gamma$. In that case the matrix $H(z)$ at a point $z\in \Gamma$ typically has an eigenspace of dimension $d-1$ which is tangent to $\Gamma$ and is associated to a small eigenvalue, and an eigenspace of dimension $1$ in the direction orthogonal to $\Gamma$ associated to a large eigenvalue. 

The main result of this section is Theorem \ref{th2Spaces} which characterises those of these metrics which belongs to $\bH_a$ or $\bH_g$ in terms of the regularity of their eigenvalues and of their eigenvectors.
Corollary \ref{corolHgToHa} to this theorem gives a simple procedure to obtain a quasi-acute metric from a graded metric $H$ such that $H(z)$ has an eigenspace of dimension $d-1$ at each point. \\

We denote by $\bbS := \{\theta\in \R^d \sep |\theta| = 1\}$ the unit sphere of $\R^d$, equipped with the distance 
$$
d_\bbS(\theta, \theta') := \arccos(\<\theta, \theta'\>).
$$
We denote by $\cA$ the space of parameters
$$
\cA := \R_+^*\times \R_+^*\times \bbS,
$$
and we define a map $\cS :\cA\to S_d^+$ as follows
\be
\label{defcS}
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
\ee
In any orthonormal basis $\cB$ of $\R^d$ which begins with the vector $\theta$ we have the following expression
$$
[\cS(\lambda, \mu, \theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda &0 & 0 & \cdots\\
0 & \mu & 0 & \cdots\\
0 & 0 & \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right).
$$
We also define for any $a = (\lambda, \mu, \theta)\in \cA$
$$
\cH(a) := \cS(a)^{-2} = \lambda^{-2} \theta \theta^\trans+ \mu^{-2}(1-\theta \theta^\trans).
$$
%If $M\in S_d^+$ has an eigenspace of dimension $d-1$ exactly, then 
%
%We denote by $S_{d*}^+$ the collection of symmetric positive definite matrices $M\in S_d^+$ which have an eigenspace of dimension exactly $d-1$.
%We also denote by $\cA^*$ the collection of $(\lambda, \mu, \pm\theta)\in \cA$ which satisfies $\lambda\neq \mu$ if $d>2$ (resp. $\lambda>\mu$ is the dimension is $d=2$).
%Then
%$$
%\cH : \cA^* \to S_{d*}^+
%$$
%is a one to one map.



%Such a metric $H$ can be parametrized using two eigenvalues $\lambda, \mu\in \R_+^*$  and a subspace of dimension $d-1$ of $\R^d$ defined through an un-oriented unit normal $\pm \theta$. Our purpose in this section is to translate the fact that $H\in \bH_\star$, for some $\star\in \{i,a,g\}$, into simpler properties satisfied by $\lambda,\mu$ and $\theta$.
%
%
%
%In order to state our results, we need to introduce the collection $\cP$ of all hyperplanes of $\R^d$, also called the projective space. An hy
%
%
%We define the space of parameters
%$$
%\cA :=  \R_+^* \times \R_+^* \times \cP,
%$$
%where $\cP$ is the $d-1$-dimensional real projective space.
%For all $(\theta, \lambda, \mu)\in \cA$ we define 
%$$
%S( \lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans),
%$$
%and $H(\theta, \lambda, \mu) := S^{-2}$.
%The space $\cA$ is a differential variety, and the tangent space to a triplet $(\theta, \lambda, \mu)\in \cA$ is 
%$$
%T_{(\theta, \lambda, \mu)} \cA =  \R \times \R \times \theta^\perp,
%$$
%where $\theta^\perp$ refers to the orthogonal hyperplane to $\theta$ in $\R^d$.

For any metric $H \in \bH$ and any $z\in \R^d$ we denote by $\dil_z(H)_\times$ and $\dil_z(H)_+$ the local dilatations at $z$ associated to the Lipschitz conditions \iref{eqLipMult} and \iref{eqLipAdd} defining $\bH_g$ and $\bH_a$:
\be
\label{defDilH}
\dil_z(H)_\times := \dil_z(H \sep d_\times, d_H) \stext{ and } \dil_z(H)_+ := \dil_z(H \sep d_+).
\ee
We recall that the local dilatation $\dil_z(f)$ of a function $f$ at a point $z$ is defined by \iref{defDilX}.
%We set $D_z(H) := \dil(\lambda)$ if $z\notin \Omega$
For any open set $\Omega\subset \R^d$ and any $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$,  we define for all $z\in \Omega$
\be
\label{eqDZA}
D_z(a)_\times := \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \frac 1 2 \left| \frac {\lambda(z)} {\mu(z)} - \frac {\mu(z)} {\lambda(z)} \right|\dil_z(\theta\sep  d_H)\right\}, %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
and 
\be
\label{eqDZAP}
D_z(a)_+ := \max\left\{\dil_z(\lambda), \ \dil_z(\mu),\ |\lambda(z)-\mu(z)| \dil_z(\theta)\right\}. %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
Note that these quantities are not defined if $\lambda(z) = \mu(z)$ and $\dil_z(\theta\sep  d_H)=\infty$ simultaneously, since an indeterminate form $0\times \infty$ appears in \iref{eqDZA} and \iref{eqDZAP}.
\begin{theorem}
\label{th2Spaces}
Let $H \in \bH$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, such that $H = \cH\circ a$ on $\Omega$.
Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$. Then 
\be
\label{eqDilTimes}
D_z(a)_\times \leq \dil_z(H)_\times \leq 2D_z(a)_\times
\ee
and%, with $\gamma := \|H^{-\frac 1 2}\| = \max\{\lambda, \mu\}$, 
\be
\label{eqDilPlus}
D_z(a)_+ \leq \dil_z(H)_+ \leq 2D_z(a)_+.
\ee
%In particular, defining $\gamma := \|H(z)^{-\frac 1 2}\| = \max \{\lambda, \mu\}$ we have 
%\be
%\label{eqDilMax}
%\max\{\dil_z(\gamma), \, D_z(a)_\times\} \leq \max \{D_z(a)_+, \, D_z(a)_\times\} \leq 2\max\{\dil_z(\gamma), \, D_z(a)_\times\}.
%\ee
\end{theorem}

%The estimate \iref{eqDilPlus} on $\dil_z(H)_+$ is not very sharp, but this is not an issue since one usually does not needs to control $ \dil_z(H)_+$ but rather $\max\{\dil_z(H)_\times,\dil_z(H)_+\}$, for which we obtain combining \iref{eqDilTimes} and \iref{eqDilPlus} the sharper estimate 
%$$
% \max\{\dil_z(\gamma), D_z(a)\} \leq \max\{\dil_z(H)_\times,\dil_z(H)_+\} \leq 2 \max\{\dil_z(\gamma), D_z(a)\}.
%$$
The rest of this section is devoted to the proof of this theorem and to Corollary \ref{corolHgToHa}. Our first lemma defines and estimates a quantity $\Delta(a,b,c)$ which appears repeatedly in the rest of the proof.


\begin{lemma}
\label{lemmaDelta}
We define for all $a,b,c\in \R$ the quantity $\Delta(a,b,c)\in \R_+$, as follows % which is the norm of a $d\times d$ matrix,
\be
\label{defDelta}
\Delta(a,b,c) := 
\left\| 
\left(
\begin{array}{cccc}
a & b & 0 & \cdots\\
b & c& 0 & \cdots\\
0 & 0 & c & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right)
\right\|.
\ee
We have 
\be
\label{eqEstimM}
\max\{|a|, |b|, |c|\} \leq \Delta(a,b,c) \leq 2 \max\{|a|, |b|, |c|\}.
\ee
\end{lemma}

\proof
We consider fixed values of $a,b,c\in \R$ and we denote by $M$ the matrix presented in \iref{defDelta}, in such way that $\Delta(a,b,c) = \|M\|$. We also define $\lambda := \max\{|a|,|b|,|c|\}$.
We have 
$$
\Delta(a,b,c) = \|M\|\geq \max_{1\leq i,j\leq d} |M_{ij}| = \lambda,
$$
which establishes the left part of \iref{eqEstimM}. For all $p\in [1,\infty]$ we denote by $l^p$ the usual norm on $\R^d$ of exponent $p$. We have 
$$
\|M\|_{l^\infty\to l^\infty} = \max_{1 \leq i \leq d} \sum_{1\leq j \leq d} |M_{ij}| \leq 2 \lambda \stext{ and } \|M\|_{l^1\to l^1} = \max_{1 \leq j \leq d} \sum_{1\leq 1 \leq d} |M_{ij}| \leq 2 \lambda.
$$
By interpolation we thus obtain  
$$
\|M\| = \|M\|_{l^2\to l^2} \leq \sqrt{\|M\|_{l^1\to l^1} \|M\|_{l^\infty\to l^\infty} } \leq 2 \lambda,
$$
which concludes the proof.
\sq

The parameter space $\cA = \bbS \times \R_+^* \times \R_+^*$ is a differential variety, and the regularity of functions defined on $\cA$ should be seen through local charts.
For each $a = (\lambda, \mu, \theta)\in \cA$ we define a local chart $\psi_a$ of a neigborhood of $a$ in $\cA$ as follows: 
\be
\label{defPsia}
\psi_a : (-\lambda, \infty)\times (-\mu , \infty) \times (B(0,\cPi) \cap \theta^\perp) \to \cA
\ee
is defined by 
$$
\psi_a(\Lambda, M, r\Theta) := (\lambda+ \Lambda,\, \mu+ M,\, \cos(r) \theta + \sin(r) \Theta),
$$
where $|\Theta| = 1$. Note that $\psi_a$ is one to one and that $d_\bbS(\theta, \, \cos(r) \theta + \sin(r) \Theta) = r$.
In \iref{defPsia} we denoted by $\theta^\perp := \{\Theta\in \R^d \sep \<\theta, \Theta\> = 0 \}$ the space orthogonal to $\theta$, and $B(0,\cPi)$ the open euclidean ball of radius $\cPi$.
%it preserves distances in the following sense: if $(\lambda', \mu', \theta') = \psi_a(\Lambda, M, r\Theta)$ then $\lambda'-\lambda = \Lambda$, $\mu'-\mu=M$ and $

Let $V$ be a banach space. We say that a function $\vp : \cA \to V$ is $C^1$ if for any $a\in \cA$ the function $\vp\circ \psi_a$ is $C^1$.
In that case for any $a\in \cA$ we define the differential 
%and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
$$
d_a\vp(A) : \R\times \R\times \theta^\perp \to V
$$
by the formula
$$
d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( tA) - \vp(a)} t. %\Lambda, t M, t r\Theta
$$
We then have
 $$
\dil_a(\vp) = \|d_a(\vp)\|.
$$
%where $d_0 (\vp\circ \psi_a) :  \R\times \R\times \theta^\perp \to V$ denotes the differential of function $\vp\circ \psi_a$ at the origin $(0,0,0) \in (-\lambda, \infty)\times (-\mu , \infty) \times (B(\pi) \cap \theta^\perp)$.
%In that case for any $a\in \cA$ and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
%$$
%d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( t\Lambda, t M, t r\Theta) - \vp(a)} t,
%$$
%and we have for any path $\gamma\in C^1([0,1], \cA)$ 
%$$
%\vp(\gamma(1)) - \vp(\gamma(0)) = \int_0^1 d \vp_{\gamma(t)} (\gamma'(t)) dt.
%$$

\begin{prop}
\label{propPhiPlus}
Define $V_+ := S_d$, equipped with the standard norm $\|\cdot\|$, and define $\vp_+ (a) := \cS(a)$.
Then for all $a,b\in \cA$ we have 
\be
\label{eqDPPhiP}
d_+(\cH(a), \cH(b)) = \|\vp_+(a)-\vp_+(b)\|.
\ee
Furthermore $\vp_+ \in C^1(\cA, V_+)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
$$
\|d_a \vp_+(A)\|_\infty= 
\Delta(\Lambda, \ (\lambda-\mu) r ,\ M).
$$
\end{prop}

\proof
The \iref{eqDPPhiP} directly follows from the fact that $\cH(a)^{-1} = \cS(a)^2 = \vp_+(a)^2$, and from the definition \iref{defDPlus} of $d_+$.
The function $\vp_+ = \cS$ is $C^1$, and even $C^\infty$, since it has a polynomial expression 
$$
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
$$
We have at the first order in $\lambda, \mu, r$
\begin{eqnarray*}
\cS(\lambda+ \Lambda, \, \mu+M, \, \theta+r\Theta) &=&
 (\lambda+ \Lambda) (\theta+ r\Theta) (\theta+r\Theta)^\trans \\
 & &+ (\mu+M)(\Id - (\theta+ r\Theta) (\theta+r\Theta)^\trans)\\
 &=& S(\lambda, \mu, \theta) \\
 & &+ \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans)\\
& &+  \cO((|\Lambda|+ |M|+ |r|)^2)
\end{eqnarray*}
Therefore %$\vp_+$ is $C^1$ and 
\be
\label{eqDiffS}
%d_a\vp_+(\Lambda, \,M, \,r\Theta) = 
d_a\cS(\Lambda, \,M, \,r\Theta) =  \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans).
\ee
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[d_a\cS(\Lambda, \,M, \,r\Theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda & r(\lambda-\mu) & 0 & \cdots\\
r(\lambda-\mu) & M & 0 & \cdots\\
0 & 0 & M & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
which concludes the proof of this proposition.
\sq


\begin{prop}
\label{propPhiTimes}
Define $V_\times := C^0(\bbS, \R)$, equipped with the $\|\cdot\|_\infty$ norm, and define $\vp_\times : \cA \to V_\times$ as follows: for any $a\in \cA$ and any $u\in \bbS$
%\be
%\label{eqDTPhiT}
$$
\vp_\times (a) := (u \mapsto \ln \|u\|_{\cH(a)}).
$$
%\vp_\times (a)(u) = \ln \|u\|_{\cH(a)}.
%\ee
Then for all $a,b\in \cA$ we have 
\be
\label{eqDTPhiT}
\|\vp_\times(a)-\vp_\times(b)\|_\infty = d_\times(\cH(a), \cH(b)).
\ee
Furthermore $\vp_\times \in C^1(\cA, V_\times)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
\be
\label{eqNormDPhiPlus}
\|d_a \vp_\times(A)\|_\infty= 
\Delta\left(\frac \Lambda \lambda ,\ \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) ,\ \frac M \mu\right).
\ee
\end{prop}

\proof
Using the expression \iref{eqDTimesLog} of the distance $d_\times$ and the homogeneity of norms we obtain for any $M,M'\in S_d^+$,
$$
d_\times (M,M') = \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|,
$$
which implies \iref{eqDTPhiT}.
%The inequality \iref{eqDTPhiT} follows from the expression \iref{eqDTimesLog} of the distance $d_\times$.

As observed in the proof of Proposition \ref{propPhiPlus} the function $\cS : \cA\to S_d^+$ is $C^1$, and $d_a\cS(A)$ has the explicit expression \iref{eqDiffS}.
It is well known that the inverse map ${\rm Inv} : \GL_d \to \GL_d$ is $C^1$ and has the the following differential : for any $\phi\in \GL_d$ and any $\Phi\in M_d$
$$
d_\phi {\rm Inv} (\Phi) = \phi^{-1} \Phi \phi^{-1}.
$$
By composition, $\cS^{-1} : \cA \to S_d^+$ is also $C^1$, and for any $a=(\lambda, \mu , \theta)\in \cA$ and any $A\in \R\times \R \times \theta^\perp$
$$
d_a(\cS^{-1})(A) = S(a)^{-1} (d_a S(A) ) S(a)^{-1}.
$$
For any $u\in \bbS$ we have 
$$
\ln \|u\|_{\cH(a)} = \ln \|\cS(a)^{-1}u\| = \frac 1 2 \ln \left(\<\cS(a)^{-1}u,\cS(a)^{-1}u\>\right).
$$
Therefore, again by composition, 
\begin{eqnarray*}
d_a (\ln \|u\|_{\cH})(A) &=&  \frac 1 {2\|\cS(a)^{-1}u\|^2} (\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>\\
& &\quad +\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>)\\% \frac {\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>+\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>}{2\|\cS(a)^{-1}u\|^2}\\
&=& \frac{\<G(a,A) v,v\>}{\|v\|^2}
\end{eqnarray*}
where $v = \cS^{-1}(a)u$. The function $G$ has the following expression : for any $a = (\lambda, \mu, \theta)\in \R_+^* \times \R_+^* \times \bbS$ and any $A = (\Lambda, M, r\Theta)\in \R\times \R \times \theta^\perp$
\begin{eqnarray*}
G(a,A) &=& \frac{\cS(a)^{-1} (d_a\cS(A)) + (d_a\cS(A)) \cS(a)^{-1}} 2\\
&=& \frac \Lambda \lambda \theta \theta^\trans +  \frac M \mu (\Id - \theta \theta^\trans) + \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right)(\theta \Theta^\trans + \Theta \theta^\trans),
\end{eqnarray*}
the last expression follows from the explicit expression \iref{eqDiffS} of $d_a\cS(A)$ establishes in the proof of the previous proposition, and from the fact that $\theta^\trans \Theta = 0$.
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[G(a,A)]_\cB = 
\left(
\begin{array}{cccc}
\frac \Lambda \lambda & \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & 0 & \cdots\\
\frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & \frac M \mu & 0 & \cdots\\
0 & 0 & \frac M \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
The map $\vp_\times$ is differentiable, as the composition of differentiable maps, and we thus have
\begin{eqnarray*}
\|d_a \vp_\times(A)\|_\infty &=& \sup \left\{ \frac{|\<G(a,A) v,v\>|}{\|v\|^2} \sep u\in \bbS, \, v=\cS(a)^{-1} u\right\}\\
&=& \|G(a,A)\|,
\end{eqnarray*}
which establishes \iref{eqNormDPhiPlus} and concludes the proof of this proposition.
\sq

We now consider a fixed $z\in \Omega$ and we remark that 
$$
\dil_z(H)_\times = \dil_z(\cH\circ a)_\times  = \dil_z(\vp_\times \circ a\sep d_H). %\leq \dil_{a(z)} (\vp_+\sep d_z) \dil_z(a\sep d_H, d_z)
$$
Therefore,  according to Lemma \ref{lemmaSubMult} for any norm $\|\cdot\|_{a(z)}$ defined on the tangent space $\R\times \R \times \theta(z)^\perp$ to $a(z)\in \cA$ we have 
\be
\label{eqDilPhiA}
\begin{array}{rcl}
& &\dil^*_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} a\sep d_H, \|\cdot \|_{a(z)})\\
& \leq& \dil_z(H)_\times\\
& \leq& \dil_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} \circ a\sep d_H, \|\cdot\|_{a(z)})
\end{array}
\ee
provided no indeterminate $0\times \infty$ or $\infty \times 0$ appears on the first and last term of this inequality.
%We recall that a neighborhood of $a(z)$ is parametrized by the local chart 
%\be
%\label{defPsiAZ}
%\psi_{a(z)} : (\Lambda, M, r\Theta) \to (\lambda(z) + \Lambda, \, \mu(z) + M, \, \cos(r)\theta(z)+ \sin(r) \Theta)
%\ee
%where $|\Theta| = 1$. 
We consider a fixed point $z\in \Omega$, and we distinguish the two cases $\lambda(z) \neq \mu(z)$ and $\lambda(z) = \mu(z)$.

\paragraph{Proof in the case $\lambda(z) \neq \mu(z)$.}
For each $a=(\lambda, \mu, \theta)\in \cA$ we define a norm $\|\cdot \|_a$ on the tangent space $\R\times \R \times \theta^\perp$ to $\cA$ at the point $a$ : for all $A = (\Lambda, M , \Theta)\in \R\times \R \times \theta^\perp$
$$
\|A\|_a = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \frac 1 2 \left| \frac \lambda \mu - \frac \mu \lambda\right| \|\Theta\|\right\}.
$$
We have by construction 
\be
\label{eqDilADZDH}
\dil_z(\psi_{a(z)}^{-1}\circ a\sep d_H, \|\cdot \|_{a(z)}) = D_z(a)_\times
\ee
According to Lemma \ref{lemmaDelta} and Proposition \ref{propPhiTimes} we have for any $a=(\lambda, \mu, \theta)\in \cA$ and any $A\in \R\times\R \times \theta^\perp$
$$
\|A\|_a \leq \|d_a \vp_\times(A)\|_\infty = \|d_0 (\vp_\times \circ \psi_a)\|_\infty \leq 2 \|A\|_a.
$$
Since $\vp_\times$ is $C^1$ it follows from \iref{eqDilDiff} that 
$$
1 \leq \dil^*_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq \dil_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq 2.
$$
Combining \iref{eqDilPhiA}, \iref{eqDilADZDH} and the last inequality we obtain
$$
D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times,
$$
which establishes the announced result \iref{eqDilTimes} in the case $\lambda(z)\neq \mu(z)$. A similar reasoning establishes the counterpart \iref{eqDilPlus} of this ineaquality for the distance $d_+$. 

\paragraph{Proof in the case $\lambda(z) = \mu(z)$.}
%We now turn to the case of equality $\lambda(z) = \mu(z)$.
For any $\ve>0$ and any $a=(\lambda, \mu, \theta)\in \cA$ such that $\lambda = \mu$ we define a norm $\|\cdot\|_{a,\ve}$ on the tangent space $\R\times \R\times \theta^\perp$ to $a$ in $\cA$ as follows : 
$$
\|A\|_{a, \ve} = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \ve \|\Theta\|\right\}.
$$
%$$
%d_z^\ve((\Lambda, M, r\Theta), (\Lambda', M', r'\Theta')) := \max \left\{\frac {|\Lambda-\Lambda'|} {\lambda(z)},\, \frac {|M-M'|} {\mu(z)}, \, \ve \|r\Theta - r'\Theta'\|\right\}.
%$$
This modification is required because the original norm $\|\cdot\|_a$ used in the case $\lambda\neq \mu$ is only a semi-norm when $\lambda = \mu$.
Reasoning similarly to the case $\lambda(z) \neq \mu(z)$ we obtain the upper bound
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \ve\dil_z(\theta\sep  d_H)\right\}.
$$
We now establish a lower bound on $\dil_z(H)_\times$.
We may assume that $\dil_z(\theta \sep d_H) < \infty$ otherwise there is nothing to prove. Since $\ve>0$ is arbitrary we thus obtain 
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H)\right\} = 2D_z(a)_\times.
$$
We now turn to the lower bound on $\dil_z(H)_\times$. 
For that purpose we define the functions $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda,\mu\}$  and we observe that for all $z,z'\in \Omega$
\begin{eqnarray*}
d_\times (H(z),H(z')) &=& \ln \max \{\|H(z)^\frac 1 2 H(z')^{-\frac 1 2}\|, \, \|H(z')^\frac 1 2 H(z)^{-\frac 1 2}\|\}\\
&\geq & \frac 1 2 \max \{|\ln \|H(z)\|- \ln \|H(z')\||, \, |\ln \|H(z)^{-1}\|- \ln \|H(z')^{-1}\||\\
&=& \max \{ |\ln\gamma(z) - \ln \gamma(z')|,\, |\ln \Gamma(z) - \ln \Gamma(z')|\}.
\end{eqnarray*}
We thus obtain
$$
\dil_z(H)_\times = \dil_z(H\sep d_\times, d_H) \geq \max \{ \dil_z(\ln \gamma\sep d_H), \, \dil_z(\ln \Gamma \sep d_H)\}.
$$
Hence according to Proposition \ref{propDilMax}
$$
\dil_z(H)_\times \geq \max \{\dil_z(\ln \lambda\sep d_H), \dil_z(\ln \mu\sep d_H)\} = D_z(a)_\times.
$$
Therefore $D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times$, and proceeding likewise we obtain $D_z(a)_+ \leq \dil_z(H)_+ \leq 2 D_z(a)_+$, which concludes the proof of Theorem \ref{th2Spaces}. \\

Our first corollary estimates the dilatation in with respect to the euclidean distance, instead of the riemanian distance, of the variable $\theta$ in a graded metric having an eigenspace of dimension $d-1$ at each point..

\begin{corollary}
\label{corolDilThetaG}
Under the hypotheses of Theorem \ref{th2Spaces} we have
%Let $H\in \bH_g$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$ such that $H = \cH\circ a$ on $\Omega$. Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$. Then
$$ 
|\lambda(z) - \mu(z)| \dil_z(\theta) \leq 2 D_z(a)_\times %\leq 2.
$$
\end{corollary}
\proof
Furthermore we have according to \iref{eqDilNormLM}
\begin{eqnarray*}
 |\lambda(z) - \mu(z)| \dil_z(\theta)
&\leq& \frac {|\lambda(z) - \mu(z)|}{\min\{\lambda(z), \mu(z)\}} \dil_z(\theta\sep d_H)\\
&=& \left(\frac {\max \{\lambda(z), \mu(z)\}}{\min\{\lambda(z), \mu(z)\}}-1\right)\dil_z(\theta\sep d_H)\\
& \leq & \left|\frac {\lambda(z)} {\mu(z)}-\frac {\mu(z)} {\lambda(z)}\right|\dil_z(\theta\sep d_H) \\
&\leq & 2 D_z(a)_\times% \leq 2.
\end{eqnarray*}
\sq


The next corollary shows how a quasi-acute metric can be obtained from a graded one.
We denote by $\diag(\lambda_1, \cdots, \lambda_d)$ the diagonal matrix of entries $\lambda_1, \cdots, \lambda_d$. 
Let $M\in S_d$ and let $U\in \cO_d$ and $\lambda_1, \cdots , \lambda_d\in\R$ be such that 
\be
\label{eqDiagSd}
M = U^\trans \diag(\lambda_1, \cdots , \lambda_d) U
\ee
For any $\alpha\in \R$ we define the matrix $\max \{\alpha, M\}\in S_d^+$ as follows
$$
\max\{\alpha, M\} := U^\trans \diag(\max\{\alpha, \lambda_1\}, \cdots, \max\{\alpha, \lambda_d\})U,
$$
and we observe that $\max\{\alpha, M\}$ does not depend on the choice of the matrix $U$ and on the order of the eigenvalues $\lambda_1, \cdots, \lambda_d$ in the decomposition \iref{eqDiagSd}.
For instance we have for any $(\lambda, \mu, \theta)\in \cA$ and any $s>0$  
$$ %\lambda^{-2} \theta\theta^\trans+ \mu^{-2} (\Id-\theta \theta^\trans)
\max \{s^{-2}, \cH(a)\} = \min\{s, \lambda\}^{-2} \theta \theta^\trans+ \min\{s, \mu\}^{-2} (\Id-\theta \theta^\trans).
$$

\begin{corollary}
\label{corolHgToHa}
Let $H\in \bH$ be such that $H(z)$ has an eigenvalue of multiplicity $\geq d-1$ for all $z\in \R^d$. We define $s:\R^d\to \R_+^*$ and $H'\in \bH$ as follows : for all $z\in \R^d$
$$
s(z) := \inf_{z'\in \sR^d} |z-z'|+ \|H(z')^{-\frac 1 2}\|,
$$
and 
$$
H'(z) := \max\{s(z)^{-2}, H(z)\}.
$$
If $H\in \bH_g$, then $4^2H'\in \bH_a$.
\end{corollary}

\proof
For each $\ve>0$ we define 
$$
H_\ve := \max\{e^{2 \ve} s(z)^{-2}, H(z)\}.
$$
The proof proceeds as follows: we first establish that for any $z\in \R^d$ one has 
\be
\label{eqDilHe}
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
\ee
We then use these properties to obtain that $4^2 H_\ve \in \bH_a$, and we conclude the proof using the convergence $H_\ve \to H$ as $\ve \to 0$.\\

We first observe that $s : \R^d \to \R_+^*$ is Lipschitz and that $s(z)\leq \|H(z)^{-\frac 1 2}\|$ for all $z\in \R^d$.

Consider a fixed point $z\in\R^d$. If $H(z)$ is proportional to $\Id$, which means that $\|H(z)\|^{-\frac 1 2} = \|H(z)^{-\frac 1 2}\| \geq s(z)$, then $H_\ve = e^{2 \ve} \Id/ s^2$ on a neighborhood of $z$. This implies according to \iref{eqDilLnH} %\ref{PropEquivS}
$$
\dil_z(H_\ve)_\times =\dil_z(H_\ve)_+ = \dil_z(e^{-\ve} s) \leq e^{-\ve}\leq 1,
$$
and therefore \iref{eqDilHe}.
On the other hand if $H(z)$ is not proportional to $\Id$ then there exists three continuous functions $\lambda, \mu \in C^0(\R^d, \R_+^*)$ and $\theta \in C^0(\R^d, \bbS)$ (where $\bbS := \{u\in \R^d \sep |u| = 1\}$) such that 
$
H = \lambda^{-2} \theta \theta^\trans+ \mu^{-2} (\Id - \theta \theta^\trans).
$
on a neighborhood of $z$.
Hence on the same neighborhood of $z$, 
$$
H_\ve = \min\{e^{-\ve} s,\lambda\}^{-2} \theta \theta^\trans+ \min\{e^{-\ve} s,\mu\}^{-2} (\Id - \theta \theta^\trans).
$$

We now establish that $\dil_z(H_\ve)_\times \leq 2$. 
We define $H_\ve^i := e^{2\ve} \Id/ s^2$ and we observe that $H_\ve \geq H_\ve^i$ and $H_\ve \geq H$, hence for any $p,q\in \R^d$
$$
d_{H_\ve}(p,q) \geq \max \{d_H(p,q), \, d_{H_\ve^i}(p,q)\}.
$$
Using Proposition \ref{propDilLoc} we thus obtain  
\begin{eqnarray*}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\} \sep d_{H_\ve}) &\leq& \max \{\dil_z(\ln (e^{-\ve} s)\sep d_{H_\ve}), \,\dil_z(\ln \lambda\sep d_{H_\ve})\}\\
&\leq & \max \{\dil_z(\ln(e^{-\ve} s \sep d_{H_\ve^i})), \,\dil_z(\ln \lambda\sep d_H)\}\\
& \leq & \max \{\dil_z(e^{-\ve} s), \, \dil_z(H)_\times\}\\
& \leq & \max \{e^{-\ve}, 1\} =1,
\end{eqnarray*}
where we used Theorem \ref{th2Spaces} and Proposition \ref{propEquivS} in the third line.
Likewise $\dil_z(\ln \min\{e^{-\ve} s, \lambda\}\leq 1$. 
Since the function 
$$
t \mapsto \frac t \mu - \frac \mu t
$$
is increasing, we easily obtain that
$$
\left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right| \leq \left|\frac \lambda \mu - \frac \mu \lambda\right|.
$$
Therefore   
$$
\frac 1 2 \left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right|  \dil_z(\theta \sep d_{H_\ve}) \leq \frac 1 2\left|\frac \lambda \mu - \frac \mu \lambda\right| \dil_z(\theta\sep d_H) \leq 1,
$$
which implies that $D_z(a_\ve)_\times \leq 1$ where $a_\ve=(\min\{e^{-\ve}s, \lambda\}, \min\{e^{-\ve} s, \mu\}, \theta) \in C^0(\R^d,\cA)$. Hence
$$
\dil_z(H_\ve)_\times \leq 2 D_z(a_\ve)_\times \leq 2.
$$

We now turn to the proof that $\dil_z(H_\ve)_+ \leq 4$.
As already observed in \iref{eqDilNorm}, for any metric space $(X,d_X)$ and any function $f\in C^0(\R^d, X)$ we have 
\be
\label{eqDilNormLM}
\dil_z(f) \leq \|H(z)\|^{\frac 1 2}\dil_z(f\sep d_H) = \frac{\dil_z(f\sep d_H)}{\min\{\lambda(z), \mu(z)\}}.
\ee
If $\lambda(z)<\mu(z)$ we therefore obtain 
\begin{eqnarray*}
\dil_z(\min\{e^{-\ve} s , \lambda\}) &\leq& \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)}\right\}\\
 &\leq& \max \{e^{-\ve}, \, \dil_z(\ln \lambda\sep  d_H)\}\\
 &\leq & \max \{e^{-\ve} , \, 1\} = 1.
\end{eqnarray*}
Still assuming that $\lambda(z)<\mu(z)$, we have $s(z)\leq \|H(z)^{-\frac 1 2}\| \leq \mu(z)$ by construction of $s$, and therefore $\min\{e^{-\ve} s, \mu\} = e^{-\ve} s$ on a neighborhood of $z$. It follows that 
$$
\dil_z(\min\{e^{-\ve} s, \mu\}) = \dil_z(e^{-\ve} s)\leq e^{-\ve} \leq 1.
$$
Proceeding similarly if $\lambda(z)>\mu(z)$ we also obtain $\dil_z(\min\{e^{-\ve} s, \lambda\})$ and $\dil_z(\min\{e^{-\ve} s, \mu\})$. 
We now focus on the local dilatation of the orientation $\theta$, and for that purpose we observe that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}|  \leq  |\lambda(z) - \mu(z)|.
$$
It follows from Corollary \ref{corolDilThetaG} that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}| \dil_z(\theta) \leq D_z(a)_+ \leq 2,
$$
and therefore $D_z(a_\ve)_+ \leq 2$, which implies $\dil_z(H_\ve)_+ \leq 4$.\\

We have established that for all $z\in \R^d$ and all $\ve>0$
$$
\dil_z(H_\ve)_\times \leq 2 \stext{ and } \dil_z(H_\ve)_+ \leq 4.
$$
Hence for any $z,z'\in \R^d$, since $H_\ve \leq e^{2\ve} H'$,
$$
d_\times(H_\ve(z), H_\ve(z')) \leq 2d_{H_\ve}(z,z') \leq 2e^\ve d_{H'}(z,z') \stext{ and } d_+(H_\ve(z), H_\ve(z')) \leq 4|z-z'|.
$$
Letting $\ve \to 0$ we obtain 
$$
d_\times(H'(z), H'(z')) \leq 2d_{H'}(z,z') \stext{ and } d_+(H'(z), H'(z')) \leq 4|z-z'|.
$$
According to Remark \ref{remHomog} this implies that $4^2 H\in \bH_a$, which concludes the proof of this corollary.
\sq


\section{From mesh to metric}
\label{secMeshToMet}
The techniques presented in this section show how to produce an metric $H\in \bH_i$, $\bH_a$ or $\bH_g$ from an isotropic, quasi-acute (in two dimensions), or graded mesh $\cT$.

Combining the next proposition with its counterpart Proposition \ref{propMeshGen}, on the generation of a mesh from a metric, yields the main result of this chapter: Theorem \ref{thEquiv} on the equivalence of the classes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ of meshes and $\bH_i \subset \bH_a \subset \bH_g$ of metrics which is announced in the introduction.
\begin{prop}
\label{propMetGen}
For any $C_0>0$ there exits $C = C(C_0,d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $\cT \in \bT_{i, C_0}$ there exists $H \in \bH_i$ which is $C$-adapted to $\cT$.
\item If $d=2$, then for any $\cT \in \bT_{a, C_0}$ there exists $H \in \bH_a$ which is $C$-adapted to $\cT$.
\item For any $\cT \in \bT_{g,C_0}$ there exists $H \in \bH_g$ which is $C$-adapted to $\cT$.
\end{enumerate}
\end{prop}

The rest of this section is devoted to the proof of this proposition.
For any mesh $\cT\in \bT$, and for any vertex $v$ of $\cT$, we denote by $n_\cT(v)$ the number of simplices in the mesh $\cT$ containing $v$:
$$
n_\cT(v) := \#\{T\in \cT \sep v\in T\}. %, %\text{s.t. } 
$$
We denote by $H_\cT^g\in \bH$ the piecewise linear metric on $\cT$ which satisfies for each vertex $v$ of $\cT$
\be
\label{eqHcTg}
H_\cT^g(v) := \frac 1 {n_\cT(v)} \sum_{\substack{T\in \cT\\\text{s.t. } v\in T}} \cH_T.
\ee
The metric $H_\cT^g$ on a simplex $T\in \cT$ is simply the linear interpolation of the averages of the matrices $\cH_T$ attached to the simplices containing a vertex $v$. 

The next lemma establishes a property of the barycentric coordinates on a simplex, which is useful for the analysis of  the regularity of a piecewise linear function on an anisotropic mesh, such as the metric $H_\cT^g$.
\begin{lemma}
\label{lemmaNormLambda}
Let $T$ be a simplex and let $V$ be the collection of vertices of $T$. Let $\lambda_v(z)$, $v\in V$ be the barycentric coordinates on $T$. Then for all $z,z'\in T$
\be
\label{eqNormLambda}
\|z-z'\|^2_{\cH_T} = \frac {d+1} d \sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2.
\ee
\end{lemma}

\proof
We first assume that $T$ is the reference equilateral simplex $\TEq$. %, and we recall that $\cH_\TEq = \Id$.
For any two vertices $v,v'$ in the collection $\VEq$ of vertices of $\TEq$ one easily checks that 
\be
\label{eqScalTEq}
\<v,v'\> = 
\left\{
\begin{array}{cl}
1 &\text{ if } v=v,'\\
-1/d &\text{ if } v \neq v'.
\end{array}
\right.
\ee
Indeed $|v|=1$ by construction for any vertex $v$ of $\TEq$, the scalar product $\<v,v'\>$ has a value $\alpha$ which is independent of the pair of distinct vertices $v,v'\in \VEq$. Since $\TEq$ is centered at the origin we obtain $0 = \<v,\sum_{v\in V} v\>  = |v|^2 + d \alpha$ which establishes \iref{eqScalTEq}.
We thus obtain for any $z,z'\in \TEq$ 
\begin{eqnarray*}
|z-z'|^2  &=& \left|\sum_{v\in \VEq} (\lambda_v(z) - \lambda_v(z'))v\right|^2 \\
&=& \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \sum_{v\neq v'} (\lambda_v(z)-\lambda_v(z'))(\lambda_{v'}(z)-\lambda_{v'}(z')).
\end{eqnarray*}
Therefore 
$$
|z-z'|^2 =  \left(1+\frac 1 d\right) \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \left(\sum_{v\in \VEq} \lambda_v(z)-\lambda_v(z')\right)^2,
$$
which concludes the proof in the case of $\TEq$ since $\cH_\TEq = \Id$ and since the barycentric coordinates of $z$ and of $z'$ sum to $1$.

We now consider an arbitrary simplex $T$, and an affine change change of coordinates $\Phi$ such that $\Phi(T) = \TEq$, $\Phi(z) = \phi z+ z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. We have $\cH_T = \phi^\trans \phi$ according to \iref{invcH}, hence for all $z,z'\in T$
$$
 |\Phi(z) - \Phi(z')| = |\phi(z-z')| = \|z-z'\|_{\cH_T}.
$$
Furthermore the barycentric coordinates of $z$ and $z'$ in $T$ are the same as those of $\Phi(z)$ and $\Phi(z')$ in $\Phi(T) = \TEq$, hence \iref{eqNormLambda} holds which concludes the proof of this lemma.
\sq



The next proposition establishes that the metric $H_\cT^g$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case iii) of graded meshes. More precisely for any mesh $\cT\in \bT_{g,C_0}$ the metric $d C_0^{10} H_\cT^g$ belongs to $\bH_g$ and is $C_0^6 \sqrt d$ equivalent to $\cT$.



\begin{prop}
\label{propHTG}
For any $\cT\in \bT_{g,C_0}$ the metric $H_\cT^g$ is $C_0$-adapted to $\cT$, and $d C_0^{10} H_\cT^g\in \bH_g$.
\end{prop}

\proof
We consider a simplex $T\in \cT$, and we recall that for any neighbor $T'$ of $T$ one has 
$$
C_0^{-2} \cH_T \leq \cH_{T'} \leq C_0^2 \cH_T.
$$
Averaging these matrices as in \iref{eqHcTg} we obtain for any vertex $v$ of $T$
\be
\label{eqHTHv}
C_0^{-2} \cH_T \leq H_\cT^g(v)\leq C_0^2 \cH_T.
\ee
Averaging with respect to the barycentric coordinates of a point $z\in T$ we eventually obtain 
\be
\label{eqHTHz}
C_0^{-2} \cH_T \leq H_\cT^g(z)\leq C_0^2 \cH_T,
\ee
which establishes as announced that the metric $H_\cT^g$ is $C_0$-adapted to $\cT$.

We now establish the regularity property of $H_\cT^g$, and for that purpose we consider two points $z,z'\in T$ and a vector $u\in \R^d\sm\{0\}$. We thus have 
\begin{eqnarray*}
\frac {\|u\|^2_{H_\cT^g(z)}} {\|u\|^2_{H_\cT^g(z')}} &=& \frac {\sum_{v\in V} \lambda_v(z) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2} \\
&=& 1+ \frac {\sum_{v\in V} (\lambda_v(z)-\lambda_v(z')) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2}\\
&\leq& 1+ C_0^4 \frac{\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|}{\sum_{v\in V} \lambda_v(z')}\\
& \leq & 1+C_0^4 \sqrt {(d+1)\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2}\\
&=& 1+C_0^4 \sqrt d \| z-z'\|_{\cH_T},
\end{eqnarray*}
where we used \iref{eqHTHv} in the third line, Cauchy-Schwartz inequality in the fourth line, and Lemma \iref{lemmaNormLambda} in the fifth line.
We consider a simplex $T\in \cT$ and we intend to give a uniform bound on $\dil_z(H_\cT^g)_\times$ for all $z\in \interior(T)$. It follows from our estimate on $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, and from the analog estimate for  $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$, that 
\begin{eqnarray*}
d_\times (H_\cT^g(z), H_\cT^g(z')) &=& \max_{u\neq 0} \left|\ln \|u\|_{H_\cT^g(z)} - \ln \|u\|_{H_\cT^g(z')}\right|\\
&\leq& \frac 1 2\ln (1+C_0^4 \sqrt d \|z-z'\|_{\cH_T}) \\
&\leq& \frac {C_0^4 \sqrt d} 2 \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Hence according to \iref{eqHTHz} and \iref{eqDilNorm} we obtain for all $z\in \interior (T)$
$$
\dil_z(H_\cT^g)_\times \leq C_0^5 \sqrt d.
$$
The metric $H := d C_0^{10} H_\cT^g$ thus satisfies $\dil_z(H)_\times = (dC_0^{10})^{-1/2}\dil_z(H_\cT^g)_\times \leq 1$ for any point $z$ in the interior of any simplex $T\in \cT$.
If follows from Corollary \ref{corolLipNoGamma} that $H \in \bH_g$, which concludes the proof.
\sq

We associate to any mesh $\cT\in \bT$ a metric $H_\cT^i$ defined as follows : for all $z\in \R^d$, 
$$
H_\cT^i(z) := \|H_\cT^g(z)\| \Id.
$$
The next result shows that $H_\cT^i$ is, up to a fixed multiplicative constant, a solution to Proposition \ref{propMetGen} in the case of isotropic metrics. More precisely for any mesh $\cT\in \bT_{i,C_0}$ the metric $d C_0^{10} H_\cT^i$ belongs to $\bH_i$ and is $C_0^7 \sqrt d$ equivalent to the mesh $\cT$.

\begin{corollary}
For any mesh $\cT\in \bT_{i,C_0}$ the metric $H_\cT^i$ is $C_0^2$-adapted to the mesh $\cT$, and $d C_0^{10} H_\cT^i \in \bH_i$.
\end{corollary}

\proof
For any matrix $M\in S_d^+$ we have $\|M^{-1}\|^{-1} \Id \leq M \leq \|M\| \Id$. We therefore obtain for any simplex $T\in \cT$
\be
\label{eqcHNormcH}
C_0^{-2} \|\cH_T\| \Id\leq \frac{\|\cH_T\|} {\rho(T)^2} \Id = \|\cH_T^{-1}\|^{-1} \Id \leq \cH_T \leq \|\cH_T\|\Id.
\ee
Let $T\in \cT$ and let $z\in T$. Since $\rho(T) \leq C_0$ and $C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z)$ we obtain 
$$
C_0^{-2} H_\cT^i(z) := C_0^{-2} \|H_\cT^g(z)\| \Id \leq \|\cH_T\| \Id \leq C_0^2 H_\cT^i(z).
$$
Combining this with \iref{eqcHNormcH} we obtain
$$
C_0^{-4} H_\cT^i(z) \leq \cH_T \leq C_0^2 H_\cT^i(z),
$$
which establishes as announced that the metric $H_\cT^i$ is $C_0^2$ equivalent to the mesh $\cT$.

According to Proposition \ref{propHTG} we have $d C_0^{10} H_\cT^g\in \bH_g$. Corollary \ref{corolLipNorm} thus implies that $d C_0^{10} H_\cT^i\in \bH_i$, which concludes the proof of this proposition.
\sq

Before turning to the case of quasi-acute metrics we prove a lemma on the neighborhood of a simplex in a graded mesh. For any mesh $\cT\in \bT$ and any closed set $E\subset \R^d$ the neighborhood $V_\cT(E)$ of $E$ in $\cT$ is  defined as the union of all simplices $T\in \cT$ which intersect $E$: 
$$
V_\cT(E) := \cup_{\substack{T\in \cT\\T \cap E \neq \emptyset}} T.
$$

\begin{prop}
\label{propNeighborT}
Let $\cT\in \bT_{g,C_0}$ and let $T \in \cT$, then for all $x\in T$ and all $y \in \R^d \sm V_\cT(T)$ we have 
$$
\|x-y\|_{\cH_T} \geq (C_0\sqrt d)^{-1}.
$$
\end{prop}

\proof
The simplex $T\in \cT$ is fixed throughout this proof. We consider the function $\vp : \R^d \to \R$ which is piecewise linear on the mesh $\cT$, and which satisfies for any vertex $v$ of the mesh $\cT$
$$
\vp(v) = 
\left\{
\begin{array}{cl}
1 & \text{ if } v\in T,\\
0 & \text{ if } v \notin T.
\end{array}
\right.
$$
We denote by $V'$ the collection of vertices of a simplex $T'\in \cT$, and by $(\lambda_v(z))_{v\in V'}$ the barycentric coordinates of a point $z\in T'$.
We have for any $z,z'\in T'$
\begin{eqnarray*}
|\vp(z)- \vp(z')| &\leq& \sum_{v \in V'} |\lambda_v(z)-\lambda_v(z')| \vp(v)\\
& \leq &\sqrt{(d+1) \sum_{v\in V'} |\lambda_v(z)-\lambda_v(z')|^2} \\
&= &\sqrt d \|z-z'\|_{\cH_{T'}}.
\end{eqnarray*}
Recalling that $\vp$ is identically $0$ on $T'$ if $T\cap T' = \emptyset$, and that $\cH_{T'} \leq C_0^2 \cH_T$ otherwise, we obtain for any $z,z'\in T'$
$$
|\vp(z)- \vp(z')| \leq C_0\sqrt d \|z-z'\|_{\cH_{T}}.
$$
If follows from Corollary \ref{corolLipNoGamma} that $\vp : (\R^d, \|\cdot \|_{\cH_T})  \to \R$ is $C_0\sqrt d$-Lipschitz.
For any $x\in T$ and any $y\in \R^d\sm V_\cT(T)$ we have $\vp(x) = 1$, $\vp(y) = 0$, thus $1 \leq C_0\sqrt d \|x-y\|_{\cH_T}$ which concludes the proof of this proposition.
\sq

We assume from this point that the dimension is $d=2$. %, and we thus restrict our attention to the bi-dimensional triangulations.
For each triangulation $\cT\in \bT$ we define a function $s_\cT : \R^2 \to \R_+^*$ as follows 
$$
s_\cT(z) := \inf_{z'\in \sR^2} |z-z'| + \|H_\cT^g(z')^{-\frac 1 2}\|.
$$
We define a metric $H_\cT^a \in \bH$ as follows : for each $z\in \R^2$  
\be
\label{defHTA}
H_\cT^a(z) = \max\{s_\cT(z)^{-2} , \, H_\cT^g(z)\}.
\ee

The rest of this section is devoted to proof of the following proposition, on quasi-acute meshes, in two dimensions.
\begin{prop}
\label{propHTA}
For any $C_0 \geq 1$ there exists $C=C(C_0)$ such that the following holds.
For any $\cT\in \bT_{a,C_0}$ the metric $H_\cT^a$ is $C$-adapted to the mesh $\cT$, and $32 C_0^{10} H_\cT^a\in \bH_a$.
\end{prop}

The author is sorry to say that, due to time constraints, this proof is not as polished as the rest of the thesis.

The fact that $32 C_0^{10} H_\cT^a\in \bH_a$ directly follows from the fact that $2 C_0^{10} \bH_\cT^g\in \bH_g$ and from Corollary \ref{corolHgToHa}. 

For each $z\in \R^2$ define $d_\cT(z) := \|H_\cT^g(z)^{-\frac 1 2}\|$. This quantity should be heuristically regarded as the diameter of the triangle containing $z$. We establish below the following property : there exists $\delta = \delta(C_0) >0$ such that for all $z,z'\in \R^2$
\be
\label{eqRegDT}
\text{ if } |z'-z| \leq \delta d_\cT(z) \stext{ then }  d_\cT(z') \geq \delta d_\cT(z).
\ee
Before turning to the proof of \iref{eqRegDT} we show how this property leads to the proof of Proposition \ref{propHTA}.
For all $z\in \R^d$ we have 
$$
s_\cT(z) = \inf_{z\in \sR^2} |z-z'|+d_\cT(z)  \geq \inf_{z'\in \sR^2} \min \{|z-z'|, \, d_\cT(z')\} \geq \delta d_\cT(z'),
$$
indeed $|z-z'|\geq \delta d_\cT(z)$ or $d_\cT(z') \geq \delta d_\cT(z)$ for any $z'\in \R^d$ according to \iref{eqRegDT}.
Combining this with the definition \iref{defHTA} of $H_\cT^a$ we obtain for all $z\in \R^2$
$$
\delta^2 H_\cT^a(z) \leq H_\cT^g(z)\leq H_\cT^a(z). 
$$
Recalling that $H_\cT^g$ is $C_0$-adapted to the mesh $\cT$, see proposition \ref{propHTG}, we obtain for all $T\in \cT$ and all $z\in T$ 
$$
\delta^2 C_0^{-2} H_\cT^a(z) \leq C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z) \leq C_0^2 H_\cT^a(z)
$$
which establishes that the metric $H_\cT^a$ is $C_0/\delta$ adapted to the mesh $\cT$, and concludes the proof of Proposition \ref{propHTA}.\\

For each $u\in \R^2$, we denote by $u^\perp$ the vector obtained by rotating $u$ by $\cPi/2$ in direct trigonometric orientation sense.

We now turn to the proof of \iref{eqRegDT}, and for that purpose we introduce some notations.
For each segment $e=[\omega-u, \omega+u]\subset \R^2$ we define the diamond $\lozenge(e)$ of $e$ as follows
$$
\lozenge(e) := \{z\in \R^2 \sep |\<z-\omega,u\>|+ C_0 |\<z-\omega,u^\perp\>| < |u|^2\}.
$$
This set is illustrated on Figure \ref{figLozenge} (left).

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/LozengeJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/SeqZnJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/TRedJenny.pdf}
\caption{An edge $e$ and the set $\lozenge(e)$ (left), sequence $(z_n)_{n \geq 0}$ (center), diameter of a triangle intersecting $\lozenge(e)$ (right). \label{figLozenge}}
\end{figure}

The next lemma considers a triangulation $\cT'$ on which the measure of sliverness is uniformly bounded by $C_0$, and compares the length an edge $e$ of $\cT'$ with the diameter of the triangles in $\cT'$ which intersect $\lozenge(e)$.

\begin{lemma}
\label{lemmaUUp}
Let $\cT'\in \bT$ be a triangulation such that $S(T) \leq C_0$ for all $T\in \cT'$. Let  $e=[\omega-u, \omega+u]$ be an edge of $\cT'$.
Then there is no vertex in the diamond $\lozenge(e)$, and for all $z\in \lozenge(e)$ and any triangle $T\in \cT'$ containing $z$, there exists an edge $e'= [\omega'-u', \omega'+u']$ of $T$ satisfying  
$$
2 |u'| \geq |u| -C_0 |\<z-\omega,u^\perp\>|/ |u|
%2 |\<u,u'\>| \geq |u|^2 - C_0 |\det (z,u)|.
$$
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$, and we assume up to a translation and a rotation that $\omega = 0$ and $u = u_y$.
We recall that for any triangle $T$, with maximal angle $\theta$, the measure of sliverness $S(T)$ has the following expression
$$
S(T) = \max\{1, \tan(\theta/2)\}.
$$
We assume for contradiction that there exists a vertex $v_0 = (x_0,y_0)\in \lozenge(e)$, and we assume without loss of generality that $x_0<0$. We consider a vertex $v_1 = (x_1,y_1)$ of $\cT$ such that the angle 
$$
\theta_0 :=  \angle(v_1-v_0, \, u_x) \in [-\cPi, \cPi)
$$
has the smallest possible absolute value $|\theta_0|$ (the bold letter $\cPi$ denotes the numerical constant $\cPi = 3.14159\cdots$). By construction there exists a triangle $T\in \cT$ containing $v_0$ and $v_1$ which has an angle  larger or equal or equal than $2\theta_0$ at the vertex $v_0$. It follows that $|\tan \theta_0| \leq S(T) \leq C_0$, and therefore  
$$
|y_1-y_0| \leq |\tan \theta_0| (x_1 - x_0) \leq C_0 (x_1-x_0).
$$
Proceeding inductively, as illustrated on Figure \ref{figLozenge} (center), we define a sequence $z_n = (x_n, y_n)$, $n\geq 0$, of vertices of $\cT$ satisfying 
$
|y_{n+1} - y_n| \leq C_0 (x_{n+1} - x_n). 
$
Adding these inequalities together we obtain 
$$
|y_n-y_0|  \leq C_0 (x_n-x_0).
$$
It follows that one of the edges $[z_n, z_{n+1}]$, $n \geq 0$, of the mesh $\cT'$ intersects the edge $e$, which is a contradiction. The diamond $\lozenge(e)$ therefore does not contain any vertex, which concludes the proof of the first part of this proposition. \\

We now consider a point $z_0 = (x_0,y_0)\in \lozenge(e)$ and we assume without loss of generality that $x_0 \geq 0$. We consider a triangle $T$ containing $z_0$, and an edge $e'= [\omega'-u', \omega'+u']$ of $T$ which is on the left of $z_0$ (in other words the edge $e'$ and the segment $[(0,y_0),(x_0, y_0)]$ joining the point $z_0$ to its orthogonal projection on the edge $e$ intersect). The point $z_0$ and the triangle $T$ are illustrated on Figure \ref{figLozenge} (right).

Since there is no vertex of $\cT'$ in the diamond $\lozenge(e)$, the edge $e'$ intersects the boundary of $\lozenge(e)$ at two points. We denote these points by $(x,y)$ and $(x',y')$, and we assume that without loss of generality that $y\geq 0 \geq y'$.
Observing that $0 \leq x \leq C_0^{-1}$, $0 \leq x'\leq C_0^{-1}$ and $\min\{x,x'\} \leq x_0$ we obtain  
$$
y-y' = (1-C_0 x) - (-1+C_0 x') \geq 1-C_0 x_0.
$$
Since $u = u_y = (0,1)$, $\omega = 0$ and $2 u' = \lambda (x-x', y-y')$ for some $|\lambda| \geq 1$, we obtain 
$$
2|\<u,u'\>| \geq  
y-y' \geq 1-C_0 x_0 = |u|^2 - C_0 |\<z_0-\omega,u\>|,
$$
which concludes the proof of this proposition.
\sq

\begin{figure}
\centering
\includegraphics[width = 4.5cm, height = 4cm]{\pathPic/Dessins/Jenny/LozengeCarreDeltaJenny.pdf}
\includegraphics[width = 2.5cm, height = 4cm]{\pathPic/Dessins/Jenny/CarreDeltaCarreEJenny.pdf}
\caption{An edge $e$, the diamond $\lozenge(e)$ and the rectangle $\square_\delta$ involved in Lemma \ref{lemmaRect} (left), the rectangles $\square_e$ and $\square_\delta$.
\label{figSquare}
}
\end{figure}


We now consider a fixed quasi-acute mesh $\cT\in \bT_{a,C_0}$ and we denote by $\cT'$ a fixed $C_0$-refinement of $\cT$ which satisfies $S(T) \leq C_0$ for all $T\in \cT'$. The next proposition involves a rectangular set $\square(e)$ associated to an edge $e$ of $\cT'$ which contains $e$ in its interior, in contrast to the set $\lozenge(e)$ appearing in the previous proposition.  
This set is illustrated on Figure \ref{figSquare} (right).
\begin{lemma}
\label{lemmaRect}
There exists a constant $\delta_0 = \delta_0(C_0, d)>0$ such that the following holds.
We define the rectangle $\square(e)$ associated to an edge $e = [\omega-u, \, \omega+u]$ of $\cT'$ as follows
$$
\square(e) = \{z\in \R^2 \sep |\<z-\omega, u\>|\leq (1+\delta_0)|u|^2 \text{ and } |\<z-\omega,u^\perp \>| \leq \delta_0 |u|^2\},
$$
%where $\delta_0 = \delta_0(C_0):= ??1/(2C_0) >0$ is a constant specified in the proof.
We have $d_\cT(z) \geq \delta_0|u|$ for all $z\in \square(e)$.
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$. 
Up to a rotation and a translation, we may again assume that $\omega = 0$ and $u = u_y=(0,1)$.
We consider a triangle $T\in \cT$ containing the edge $e$ (note that $e\subset T$ but that $e$ may not be an edge of $T$, since we only known that $e$ is an edge in $\cT'$).

We define $H := H_\cT^g$. Recalling that $H$ is $C_0$-equivalent to $\cT$ we obtain for all $z\in e$
$$
C_0^{-2} H(z)\leq \cH_T \leq C_0^2 H(z). 
$$
The inclusion $e\subset T \subset \cE_T$ implies the upper bound $\|u\|_{\cH_T} = \|u_y\|_{\cH_T} \leq 1$. Hence for all $z\in e$
$$
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq \|u_y\|_{H(z)}^{-1} \geq C_0^{-1}.
$$
Note also that for any $z,u \in \R^2$
$$
d_\times (H(z), H(z+u)) \geq \ln \|H(z)^\frac 1 2 H(z+u)^{-\frac 1 2}\| \geq |\ln d_\cT(z) -\ln d_\cT(z+u)|.
$$
We define $C_1 := \sqrt 2 C_0^5$, in such way that $C_1^2 H\in \bH_g$, and we thus have  according to \iref{eqLocalNorm} if $C_1\|u\|_{H(z)}<1$
$$
|\ln d_\cT(z) -\ln d_\cT(z+u)| \leq d_\times (H(z), H(z+u)) \leq -\ln (1-C_1\|u\|_{H(z)}).
$$
Therefore for all $z\in e$ and all $u\in \R^d$,
$$
d_\cT(z+u) \geq d_\cT(z) (1-C_1 \|u\|_{H(z)}) \geq C_0^{-1}(1-C_1C_0 \|u\|_{\cH_T}).
$$
We define $C_2 := 4C_0C_1$ and we observe that any point of the rectangle 
\be
\label{eqRectGrad}
\left[\frac {-1}{C_2 \|u_x\|_{\cH_T}}, \,\frac 1 {C_2 \|u_x\|_{\cH_T}}\right] \times \left[-(1+C_2^{-1}), \, 1+C_2^{-1}\right].
\ee
can be written under the form $z+u$ where $z\in e$ and $\|u\|_{\cH_T} \leq 1/(2C_0C_1)$. We thus have  
\be
\label{eqdGrad}
d_\cT(z') \geq 1/(2C_0)
\ee
 on this rectangle.

We introduce a small constant $\delta = \delta(C_0)>0$ which is specified later in the proof. It follows from \iref{eqRectGrad} and \iref{eqdGrad} that the proof of this lemma is complete if $\|\cH_T\| \leq \delta^{-2}$, with $\delta_0 := \min \{\delta/C_2, \, 1/(2C_0)\}$.
We thus assume from this point that $\|\cH_T\|\geq \delta^{-2}$.\\

We assume that $\delta< C_0^{-1}$ and we define the rectangle
$$
\square_\delta := [-\delta, \delta] \times [1-C_0 \delta, -1+C_0 \delta],
$$
which is included in $\overline \lozenge(e)$ by construction.
Since $C_1^2 H\in \bH_g$, the function $z\mapsto \|H(z)\|^{-\frac 1 2}$ is $C_1$-Lipschitz according to Corollary \ref{corolLipNorm}. We thus have for all $z = (x,y)\in \square_\delta$
\be
\label{defr0}
\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2}+C_1|x|\leq r_0(\delta) := (C_0+C_1)\delta.
%\|u_x\|_{H(z)} \geq \|u_x\|_{H(y,0)}(1-C_1 |x| \|u_x\|_{H(y,0)}) \geq C_*(1-C_1 C_0 \delta_* C_*),
%\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2} + C_1 |x|
\ee
On the other hand it follows from Lemma \ref{lemmaUUp} that any $z = (x,y)\in \square_\delta$ is contained in a triangle containing an edge $e' = [\omega'-u', \omega'+u']$ such that $|u'| \geq (1-C_0 \delta)/2$. We thus have 
$$
1 \geq \|u'\|_{\cH_{T'}} \geq \frac{|u'|}{ \|\cH_{T'}^{-\frac 1 2}\|} \geq \frac{1-C_0 \delta}{2 \|\cH_{T'}^{-\frac 1 2}\|} 
$$
and therefore 
%of length at least $T'\in \cT$ satisfying $\|\cH_{T'}^{-\frac 1 2}\| \geq (1-C_0 \delta_*)/2$, hence 
\be
\label{defR0}
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq C_0^{-1} \|\cH_{T'}^{-\frac 1 2}\|  \geq  R_0(\delta) := (1-C_0 \delta)/(2C_0). %\det (z,u_y)
\ee
For all $z\in \square_\delta$, we denote by $\theta(z) = (\cos \Theta(z), \sin \Theta(z))$, $\Theta(z)\in [0, \cPi]$, the direction of the eigenvector associated to the small eigenvalue of $H(z)$, in such way that 
\be
\label{eqNormTheta}
\|\theta(z)\|_{H(z)} = \|H(z)^{-\frac 1 2}\|^{-1} = d_\cT(z)^{-1}.
\ee
We thus have for any $(0,y)\in e$
$$
C_0 \geq C_0 \|u_y\|_{\cH_T} \geq \|u_y\|_{H(0,y)} \geq |\cos \Theta(0,y)| \sqrt{\|H(0,y)\|} = \delta^{-1} |\cos \Theta(0,y)| ,
$$
hence 
$$
|\cos \Theta(0,y)| \leq  C_0 \delta.
$$
For all $z\in \square_\delta$ we have according to Corollary \ref{corolDilThetaG} %Theorem \ref{th2Spaces} 
$$
(R_0(\delta)-r_0(\delta)) \dil_z(\Theta) \leq  (\|H(z)^{-\frac 1 2}\| - \|H(z)\|^{-\frac 1 2}) \dil_z(\Theta) \leq 2C_1.
$$
Hence we obtain for all $z= (x,y)\in \square_\delta$  
$$
(R_0(\delta)-r_0(\delta)) |\Theta(z) - \Theta(0,y)| \leq 2C_1 |x|\leq 2C_1 \delta,
$$
hence since $t \mapsto \cos t$ is a Lipschitz function %, since $\cos : [0, \cPi/2]\to \R$ is convex
\be
\label{defTheta0}
|\cos \Theta(z)| \leq \cos \Theta_0(\delta) := C_0 \delta + \frac{\delta}{R_0(\delta)-r_0(\delta)}.
\ee
We have according to \iref{eqLocalNorm} for all $z\in \square_\delta$ and all $r\geq 0$ such that $C_1r\|\theta\|_{H(z)}<1$,
\begin{eqnarray*}
|\ln d_\cT(z+r \theta(z)) - \ln d_\cT(z)| &\leq& d_\times (H(z+r\theta(z)),H(z))\\
&\leq& -\ln (1-C_1r\|\theta\|_{H(z)})\\
&=& -\ln (1-C_1r/d_\cT(z)),
\end{eqnarray*}
therefore 
$$
d_\cT(z+r \theta(z)) \geq  d_\cT(z) (1-|r| C_1 /d_\cT(z)).
$$
For all $z\in \square_\delta$ such that $|r|\leq R_1(\delta) := R_0(\delta)/(2C_1)$ we thus obtain
$$
d_\cT(z+r\theta(z)) \geq R_0(\delta)(1-|r|C_1/R_0(\delta))\geq R_0(\delta)/2.
$$
It follows that $d_\cT(z')\geq R_0(\delta)/2$ for all $z'$ in the set 
$$
\{z+r\theta(z) \sep z\in \square_\delta,\, |r|\leq R_1(\delta)\} \supset [-\delta_0,\delta_0]\times [-(1+\mu_0),1+\mu_0]
$$
where 
\be
\label{eqD0MU0}
\delta_0 := \delta - r \cos \Theta_0(\delta) \stext{ and }  \mu_0 := -C_0 \delta+ r \sin \Theta_0(\delta)
\ee
and where the constant $0 \leq r\leq R_1(\delta)$ can be freely chosen.
The rest of the proof consists in choosing appropriate constants $\delta$ and $r$.\\

As $\delta \to 0$ we have $r_0(\delta)\to 0$, $R_0(\delta) \to 1/(2C_0)$ and $\cos\Theta_0(\delta) \to 0$. We thus choose $\delta = \delta(C_0,d)>0$ sufficiently small in such way that 
\be
\label{eqRCS}
R_0 \geq 1/(4C_0)
, \quad
\cos \Theta_0 \leq 1/(8C_0)
, \quad
\sin \Theta_0 \geq 1/2
.
\ee
We then choose $r := 4C_0 \delta$, which is smaller than $R_1(\delta)= R_0(\delta)/(2C_1) \geq 1/(8C_1C_0)$ if $\delta$ is sufficiently small. Injecting this choice of $r$ and \iref{eqRCS} in \iref{eqD0MU0} we thus obtain 
$$
\delta_0 \geq \delta/2 \stext{ and }\mu_0 \geq C_0 \delta.
$$
We have thus established under the hypothesis $\|\cH_T\|\geq \delta^{-2}$ that 
hence $d_\cT(z) \geq 1/(8C_0)$ for all $z$ in the rectangle 
$$
[-\delta/2, \delta/2]\times [-(1+C_0\delta), 1+C_0 \delta].
$$
Since the case $\|\cH_T\|\leq \delta^{-2}$ is already established this concludes the proof of this proposition.
\sq

The next lemma establishes a technical property on the covering a one dimensional segment by smaller ones, which is a key to the end of this proof.

\begin{lemma}
\label{lemmaCoverSeg}
Let $x_1, \cdots , x_k\in [0,1]$ and let $h_1, \cdots, h_k >0$ be such that 
\be
\label{eqDefXiHi}
[0,1]\subset \bigcup_{1\leq i \leq k} [x_i-h_i, \, x_i+h_i].
\ee
Let $\delta>0$ and let $h_* = h_*(k,\delta) := \exp(1-2k/\delta)/\delta$. Then 
\be
\label{eqInclSeg}
[0,1]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_* \leq h_i}} [x_i-(1+\delta)h_i, \, x_i+(1+\delta)h_i].
\ee
\end{lemma}

\proof
For each $y\in [0,1]$ we denote by $h(y)$ the value $h_i$ associated to the segment $[x_i-h_i, x_i+h_i]$ of smallest length containing $y$.
We thus have 
$$
\int_{[0,1]} \frac {dy} {h(y)} \leq \sum_{1\leq i \leq k} \int_{x_i-h_i}^{x_i+h_i} \frac 1 {h_i} = 2k.
$$
We assume for contradiction that \iref{eqInclSeg} does not hold, and we consider a point $x\in [0,1]$ which does not belong to the right hand side of $[0,1]$. For each $y\in [0,1]$ one of the two following possibilities holds
$$
\delta h(y) < |x-y| \stext{ or } h(y) < h_*.
$$
Integrating we obtain 
$$
\int_0^1 \frac {dy} {h(y)}  \geq \int_0^1 \frac {dy} {\max\{|x-y|/\delta,\, h_*\}}.
$$
The minimum value of the right hand side is attained for $x=0$ or $1$ and equals 
$$
\int_0^1 \frac {dy}{\max \{|x-y|/\delta, h_*\}} = \int_0^{\delta h_*} \frac 1 h_* + \int_{\delta h_*}^1 \frac \delta ydy = \delta(1-\ln(\delta h_*))
$$
Thus $2k>\delta(1-\ln(\delta h_*))$, which contradicts the definition of $h_*$. This concludes the proof of this lemma.
\sq

Under the hypotheses of Lemma \ref{lemmaCoverSeg} we thus have
\be
\label{eqInclSegDouble}
[-h_*\delta,\, 1+h_*\delta]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_i \leq h_*}} [x_i-(1+2\delta)h_i, \, x_i+(1+2\delta)h_i].
\ee


We now conclude the proof of Proposition \ref{propHTA}.
We consider a point $z\in \R^2$ contained in a triangle $T\in \cT$, and we denote by $\cT$ the longest edge $e$ of $T$. Up to a rotation and a translation, we may assume that $e=[0, u_x]$ joins the origin of $\R^2$ to the the vector $u_x := (1,0)$.
Note that 
\be
\label{eqNormHTInv}
2 \geq \|u_x\|_{\cH_T} \geq \|\cH_T^{-\frac 1 2}\|^{-1}.
\ee
Since the triangulation $\cT'$ is a $C_0$-refinement of $\cT$, the edge $e$ of $T$ is built of $k \leq C_0$ edges $(e_i)_{1 \leq i \leq k}$ of $\cT'$,
$$
e_i = [(x_i-h_i)u_x,\,  (x_i +h_i) u_x].
$$
The triangle $T$ and the edges $(e_i)_{1\leq i\leq k}$ are illustrated on Figure \ref{figTFlat} (left).

\begin{figure}
\centering
\includegraphics[width = 7cm, height = 1.5cm]{\pathPic/Dessins/Jenny/TFlatJenny.pdf}
\includegraphics[width = 8cm, height = 2.5cm]{\pathPic/Dessins/Jenny/cupCarresJenny.pdf}
\caption{
A triangle $T\in \cT$ and the edges $(e_i)_{1\leq i \leq k}$ of $\cT'$ contained in $T$ (left), the set \iref{eqRectHoDo} (right). 
\label{figTFlat}}
\end{figure}

We define $h_* := h_*(C_0, \delta_0/2) = 2\exp(1-4C_0/\delta_0)/\delta_0$, where $\delta_0$ is the constant from Lemma \ref{lemmaRect}, and we observe that 
\be
\label{eqRectHoDo}
\bigcup_{h_* \leq h_i} \square(e_i) \supset \left[-\frac{h_* \delta_0} 2, 1+ \frac{h_* \delta_0} 2\right] \times [-h_* \delta_0, h_* \delta_0],
\ee
This set is illustrated on Figure \ref{figTFlat} (right).
Since $e$ is the longest edge of $T$, the angles of $T$ at the extremities of $e$ are acute.
Furthermore the height $h$ of $T$ orthogonal to the edge $e = [0,u_x]$ satisfies 
$$
h/2 = |T|  = \frac{|\TEq|} { \sqrt {\det \cH_T}} = \frac{|\TEq|}{\sqrt{\|\cH_T\| \|\cH_T^{-1}\|^{-1}}}  = \frac{|\TEq| \|\cH_T^{-1}\|}{\rho(T)} \geq \frac{|\TEq|}{4 \rho(T)} .
$$
Hence we obtain with $c := |\TEq|/8$ the inclusion
\be
\label{eqTRectRho}
T \subset [0,1] \times [-c/\rho(T), c/\rho(T)]
\ee
We distinguish two cases depending on the value of $\rho(T)$. If $c/\rho(T) \leq h_* \delta_0$, equivalently $\rho(T) \geq c/(h_* \delta_0)$ we obtain combining \iref{eqRectHoDo} and \iref{eqTRectRho} that $d_\cT\geq h_*\delta_0$ on the set 
$$
z+ \left[-\frac {h_*\delta_0} 2, \frac {h_*\delta_0} 2\right]^2
$$
which concludes the proof of this proposition.
One the other hand we have for any vector $u\in \R^2$
$$
\frac{d_\cT(z+u)}{d_\cT(z)} \geq  1-C_1 \|u\|_{H(z)} \geq 1-C_0C_1 \|u\|_{\cH_T} \geq  1-C_0C_1 \rho(T) |u| \|\cH_T^{-\frac 1 2}\|^{-1} \geq 1-2 C_0C_1 \rho(T) |u| 
$$
which concludes the proof if $\rho(T) \leq c/(h_*\delta_0)$.

\section{From metric to mesh}
\label{secMetToMesh}
%\subsection{Mesh generation}
\label{secMeshGen}

%We prove in this section Theorems \ref{thI}, \ref{thA} and \ref{thR} on the equivalence between certain classes of meshes and of metrics. %, which is divided in two parts.
%This proof is divided in two parts as follows. Proposition \ref{propMeshGen} in \S \ref{secMeshGen} we show how a mesh can be generated from a Riemannian metric, and Proposition \ref{propMetGen} in \S\ref{secMetGen} we show how a metric can be generated from a mesh.
%
This section is dedicated to the proof of the following result, on the generation of a mesh from a metric.
\begin{prop}
\label{propMeshGen}
There exists $C_0 = C_0(d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $H\in \bH_i$ there exists $\cT \in \bT_{i,C_0}$ which is $C_0$-adapted to $H$.
\item If $d=2$, then for any $H \in \bH_a$ there exists $\cT\in \bT_a$ which is $C_0$-adapted to $\cT$.
\item If $d=2$, then for any $H \in \bH_g$ there exists $\cT\in \bT_g$ which is $C_0$-adapted to $\cT$.\end{enumerate}
\end{prop}

Point {\it i)} is established in the \S\ref{secMeshGenI}, point {\it iii)} in \S \ref{secMeshGenG} an eventually {\it ii)} in \S \ref{secMeshGenA}.

%We consider in these proofs a metric $H$ such that $c^2H \in \bH_{\star}$ where $0<c\leq 1$ is a numerical constant and $\star \in \{i,a,g\}$ is a symbol. 

\begin{remark}
\label{remcC}
Let $\star \in \{i,a,g\}$ and let $1\geq c>0$, $C\geq 1$ be numerical constants. 
Assume that for any metric $H$ such that $c^2 H\in \bH_\star$ there exists a mesh $\cT\in \bT_{\star, C}$ which is $C$ adapted to $H$.
Then for any metric $H'\in \bH_\star$ there exists a mesh $\cT' \in \bT_{\star, C}$ which is $C/c$-adapted to $H'$.
(Indeed, choose a mesh $\cT'$ which is $C$-equivalent to the metric $H'/c^2$, and observe that $\cT'$ is $C/c$-equivalent to $H'$)
\end{remark}


\subsection{Isotropic Mesh generation}
\label{secMeshGenI}

\begin{figure}
\centering
\includegraphics[width = 5cm, height = 5cm]{\pathPic/Dessins/Jenny/THalfSquareJenny.pdf}
\caption{A bidimensional triangulation generated by the isotropic refinement procedure
\label{figHalfSquares}}
\end{figure}

The survey paper \cite{Nochetto} describes a the construction of a hierarchical family of meshes of the rectangular domain 
$
[0,1]^d.
$ 
All these meshes are the refinement of a ``fundamental'' mesh $\cT_0 = \{T_\sigma \sep \sigma \in \Sigma_d\}$, where $\Sigma_d$ stands for the collection of permutations of the set $\{1,\cdots,d\}$, and $T_\sigma$ for the Kuhn simplex
$$
T_\sigma := \{z\in [0,1]^d \sep z_{\sigma(1)} \leq \cdots \leq z_{\sigma(d)}\}.
$$
%A sequence $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $A procedure, guided by the user 
%The ``fundamentalbasic mesh $\cT_0$ of $[0,1]^d$ 
Starting from $\cT_0$, the algorithm described in \cite{Nochetto} produces, guided by the user, a family $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $[0,1]^d$ proceeding as follows. 
Assume that the mesh $\cT_n$ has already been generated.
%Once the mesh $\cT_n$ is defined, the mesh $\cT_{n+1}$ is obtained as follows.
%\begin{enumerate}
%\item (Marking) The user selects
%\item (Refinement)
%\end{enumerate}
%The mesh $\cT_{n+1}$ is produced from $\cT_n$ as follows 
\begin{itemize}
\item (Marking)
The user selects a subset $\cM_n \subset \cT_n$.
\item (Refinement)
The algorithm generates a $2$-refinement $\cT_{n+1}$ of $\cT_n$,  
$$
\cT_{n+1} := \Refine(\cT_n, \cM_n).
$$
which does not contain any of the marked simplices : $\cT_{n+1} \cap \cM_n = \emptyset.$
\end{itemize}
\noindent

The elements of the meshes $(\cT_n)_{n \geq 0}$ have a very specific structure, which main features are described below.
\begin{property}
\label{propertyIso}
Any simplex $T$ produced by this algorithm possesses the following properties.
\begin{enumerate}[a)]
\item (Discrete Volumes) The volume of $T$ has the form
\be
\label{eqVolTG}
|T| = \frac {2^{-g(T)}}{d!},
\ee
where $g(T)\geq 0$ is an integer called the ``generation'' of $T$.
\item
(Finite number of classes)
The simplex 
$$
2^{\frac{g(T)} d} (T-z_T),
$$
which is centered at the origin and has volume $1/d!$, %$\frac 1 {d!}$, 
belongs to a finite family $\gT_0$ of simplices.
%\item
%(Vertices lie on a grid)
%The vertices of $T$ lie on the grid
%$$
%2^{-\left\lceil \frac {g(T)} d\right\rceil} \Z^d
%$$
\end{enumerate}
\end{property}
The survey paper \cite{Nochetto} also contains a result, Proposition 4.1, which establishes that $\cT_{n+1} := \Refine(\cT_n, \cM_n)$ is a \emph{local} refinement of $\cT_n$ in the following sense: for all $T'\in \cT_n \sm \cT_{n+1}$ there exists $T\in \cM_n$ such that 
\be
\label{eqDG}
g(T)\geq g(T') \stext{ and } d(T,T') \leq D \, 2^{-g(T')/d},
\ee
where $D = D(d)$ is a fixed constant and where 
$$
d(T,T') := \min\{|z-z'| \sep z\in T, \, z'\in T'\}.\\
$$

The next lemma shows that this refinement algorithm can be used to produce a conforming isotropic mesh $\cT$ of the unit cube $[0,1]^d$, such that the diameters $\diam(T)$, $T\in \cT$, are specified by a given Lipschitz function.

\begin{lemma}
\label{lemmaSCube}
%There exists $C=C(d)$ such that the following holds.
Let $s:[0,1]^d\to  (0,\sqrt d]$ be a $c$-lipschitz function, where $0<c\leq 1$. Let $(\cT_n)_{n \geq 0}$ be the sequence of meshes produced by the algorithm when the collection $\cM_n\subset \cT_n$ of marked simplices is defined as follows
\be
\label{defMn}
\cM_n := \left\{T\in \cT_n \sep \min_T s < \diam(T)\right\}.
\ee
Then the sequence of meshes stabilizes : there exists $N\geq 0$ such that $\cT_n = \cT_N$ for all $n \geq N$. Furthermore we have for all $T\in \cT_N$ and all $z\in T$
\be
\label{eqEquivCube}
\diam(T) \leq s(z) \leq C_s \diam(T).
\ee
where 
\be
\label{defCs}
C_s := 2^\frac 1 d \frac {D_+ (1+c) + c D}{D_-}
\ee
where $D_+ := \max\{ \diam(T) \sep T \in \gT_0\}$ and $D_- := \min\{ \diam(T) \sep T \in \gT_0\}$.
\end{lemma}

\proof
We first show that for any $n \geq 0$ any $T_*\in \cT_n$ and any $z\in T_*$ we have $s(z) \leq C_s \diam(T_*)$.

Indeed if $T_*\in \cT_0$ then 
$$
s(z) \leq \sqrt d =  \diam(T_*) \leq C_s \diam(T_*)
$$
since $C_s\geq 1$ and since $s$ is uniformly bounded by $\sqrt d$.

Otherwise $T_*$ has a father $T'$ which was bisected in the refinement process, hence there exists a simplex $T$ such that \iref{eqDG} holds and which was selected for bisection, hence $\min_T s < \diam(T)$.

We thus obtain for any $z\in T$
\begin{eqnarray*}
s(z) &\leq& \min_T s+ c(\diam(T') + d(T,T'))\\
& \leq & \diam(T)+c(\diam(T') + d(T,T'))\\
& \leq & D_+ 2^{-g(T)/d} + c(D_+2^{-g(T')/d} + D 2^{-g(T')/d})\\
& \leq &  2^{-(g(T_*)-1)} (D_+(1+c)+cD)\\
& \leq & C_s \diam(T_*),
\end{eqnarray*}
which concludes the proof of the right part of \iref{eqEquivCube}.

From the fourth line of this inequality we also obtain an uniform lower bound on the volume of the simplices generated by the refinement procedure
$$
|T_*| = \frac{2^{-g(T_*)}}{d!} \geq c_0 := \frac{\min\{ s(z) \sep z\in [0,1]^d\}}{d! 2^\frac 1 d  (D_+(1+c)+cD)}.
$$
It follows that $\#(\cT_n)$ is uniformly bounded by $1/c_0$, which immediately implies that the sequence $(\cT_n)_{n \geq 0}$ of meshes stabilizes.

Let $N$ be such that $\cT_n = \cT_N$ for all $n \geq N$. We thus have $\cM_N = \emptyset$ and therefore $\diam(T) \leq \min_T s$ for all $T\in \cT_N$, which implies the left part of \iref{eqEquivCube}.
\sq

The rest of this section is devoted to the proof the point i) of Proposition \ref{propMeshGen}.
We thus consider a metric $H\in \bH_i$, and we recall there exists a Lipschitz function $s: \R^d \to \R_+^*$ such that for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2}.
$$
For each $n\geq 0$ we define a function $s_n : [0,1]^d \to \R_+^*$, which is clearly Lipschitz, as follows
\be
\label{defSn}
s_n(z) := 2^{-n} s(2^n (z-z_0))
\ee
where $z_0 = (1/2, \cdots , 1/2)$ is the barycenter of the cube $[0,1]^d$.
%The function $s_n$ is clearly Lipschitz, and 
For all $z\in [0,1]^d$ and all $n \geq 0$ we have 
$$
s_n(z) \leq s_n(z_0) + |z-z_0| \leq 2^{-n} s(0) + \frac {\sqrt d} 2.
$$
The function $s_n$ is therefore uniformly bounded by $\sqrt d$ on $[0,1]^d$ when $n$ is sufficiently large.
We denote by $\cT^n$ the mesh of the cube $[0,1]^d$ described by Lemma \ref{lemmaSCube} for the function $s_n$. We thus have %for all $T\in \cT^n$
\be
\label{eqDiamSn}
\diam(T) \leq s_n(z) \leq C \diam(T) \stext{ for all } T \in \cT^n, \, z\in T.
\ee
where $C=C(d)$ is the constant from Lemma \ref{lemmaSCube}.
We denote by $\cT_n$ the mesh of the cube $[-2^{n-1}, 2^{n-1}]^d$ obtained by translating the mesh $\cT^n$ by $-z_0$ and dilating it by $2^n$. In mathematical terms: % In condensed notations
$$
\cT_n := \{2^n(T-z_0)\sep T \in \cT^n\}.
$$
%$$
%\cT_n := 2^n (\cT^n -z_0).
%$$
In view of \iref{defSn} and \iref{eqDiamSn} we thus have 
\be
\label{eqMinSDiamT}
\diam(T) \leq s(z) \leq C \diam(T) \stext{ for all } T \in \cT_n,\, z\in T,
\ee
We denote by $C_0$ the smallest constant such that for all $T$ in the finite set $\gT_0$ one has 
$$
 \frac{C_0^{-2} \Id}{\diam(T)^2} \leq \cH_T \leq \frac{C_0^2\Id}{C^2\diam(T)^2 },
$$
and we thus obtain for all $T\in \cT_n$ and all $z\in T$
\be
\label{eqHHTIso}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Unfortunately the mesh $\cT_n$ does not cover $\R^d$ but only the cube $[-2^{n-1}, 2^{n-1}]$. 
The next lemma shows that a global mesh $\cT$ of the infinite domain $\R^d$ can be extracted from the sequence of meshes $(\cT_n)_{n\geq 0}$.

\begin{lemma}
\label{lemmaExtractMesh}
Let $(\Omega_n)_{n \geq 0}$ be an increasing sequence of polygonal domains of $\R^d$, which exhausts $\R^d$ in the following sense:
$$
\bigcup_{n \geq 0} \Omega_n = \R^d \stext{ and } \Omega_n \subset \Omega_{n+1} \text{ for all } n\geq 0.
$$
Let $H \in \bH_g$, let $(\cT_n)_{n \geq 0}$ be a sequence of conforming simplicial meshes of the domains $\Omega_n$, and assume that for all $n \geq 0$, all $T\in \cT_n$ and all $z\in T$ one has 
\be
\label{eqHHTConv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Then there exists a mesh $\cT\in \bT$ such that 
$
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
$
for all $T\in \cT$ and all $z\in T$.
\end{lemma}

\proof
The heuristic idea of this proof is to ``extract a converging subsequence'' from the sequence $(\cT_n)_{n \geq 0}$ of meshes. Unfortunately meshes are discrete objects of combinatorial nature, and the convergence of meshes has no meaning a priori. We therefore use Lipschitz functions as an intermediate object, for which convergence is well defined and which benefit of a compactness property.\\

We associate a function $\phi_T : \R^d \to \R$ to each simplex $T$, which is defined as follows. The function $\phi_T$ is supported on $T$, and for all $z\in T$ we have in terms of the barycentric coordinates $\lambda_v(z)$ of $z$ with respect to the vertices $v\in V$ of $T$:
%To each simplex $T$ of vertices $V$, and barycentric coordinates $(\lambda_v)_{v\in V}$ we associate the function 
$$
\phi_T(z) := \min_{v\in V} \lambda_v(z).
$$
%The maximum of this function has value $1/d$ and is attained at the barycenter $z_T$ of $T$. Furthermore for each $z\in T$ and each $0\leq r \leq 1$ one easily checks that 
%$$
%\phi_T(z+r(z-z_T)) \geq r/d.
%$$
According to Lemma \ref{lemmaNormLambda}, we have for any $z,z'\in T$ and any $v\in V$
$$
|\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T},
$$
hence 
\be
\label{eqPhiLip}
|\phi_T(z) - \phi_T(z')| \leq \max_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T}.
\ee

For all $n \geq 0$ we define a function $\phi_n$ on $\R^d$ as follows
$$
\phi_n := \sum_{T \in \cT_n} \phi_T.
$$
It follows from \iref{eqHHTConv} and \iref{eqPhiLip} that for all $T\in \cT_n$ and all $z\in \interior(T)$
$$
\dil_z(\phi_n\sep d_H) \leq C_0.
$$
Since in addition $\phi_n = 0$ on $\R^d \sm \Omega_n$ it follows from corollary \ref{corolLipNoGamma} that $\phi_n : (\R^d,d_H) \to \R$ is $C_0$-Lipschitz. Since the space $(\R^d, d_H)$ is locally compact, due to Proposition \ref{propEuclidRiemann}, Ascoli's compactness theorem states that there exists 
subsequence $(\phi_{n_k})_{k \geq 0}$ which converges uniformly on all compact sets of $\R^d$ to a $C_0$-Lipschitz function $\phi$. 

We therefore assume, up to such an extraction, that 
$
\phi_n \to \phi
$
uniformly on all compact sets of $\R^d$.
We denote by $\cT$ the collection of closures of connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$:
$$
\cT := \left\{ \overline E \sep E \text{ is a connected component of } \{z\in \R^d \sep \phi(z)>0\} \right\}.
$$
For each $z\in \R^d$ and each $n \geq 0$, we denote by $T_n(z)$ the element of $\cT_n$ containing $z$ in its interior if it exists, and $T_n(z) = \emptyset$ otherwise.
If $\phi(z)>0$, then $T_n(z)\neq \emptyset$ for all $n$ sufficiently large, and one easily checks that 
\be
\label{eqTTnz}
T_n(z)\text{ converges in Hausdorff distance to the element }T(z)\in \cT
\ee
 containing $z$. Hence $\cT$ is a collection of simplices, and the convergence $T_n(z)\to T(z)$ in haussdorf distance, combined with the hypothesis $C_0^{-2} H(z) \leq T_n(z) \leq C_0^2 H(z)$, implies that  
\be
\label{eqHHTConv2}
C_0^{-2} H(z) \leq T(z) \leq C_0^2 H(z).
\ee
In order to conclude this proof we need to show that the collection $\cT$ of simplices is a conforming mesh of $\R^d$. We thus have to check the hypotheses of Definition \ref{defSimplMesh}.
The interiors $\interior(T)$, $T\in \cT$ are pairwise disjoint since they are the connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$.
We claim furthermore that $\cT$ covers $\R^d$. Indeed let $z\in \R^d$be arbitrary and for all $n$ let $T_n\in \cT_n$ be such that $z\in T_n$. Since $C_0^{-2} H(z) \leq \cH_{T_n}\leq C_0^2 H(z)$ there exists a subsequence $T_{n_k}$ which converges in the Haussdorf distance to a simplex $T$ containing $z$. We clearly have $T\in \cT$ which establishes as announced that $\cT$ covers $\R^d$.
The fact that $\cT$ is locally finite easily follows from \iref{eqHHTConv2}.\\


We now turn to the proof of the conformity property, and for that purpose we consider an arbitrary Lipschitz function $f : (\R^d, d_H) \to \R$ with compact support. 
Let $T$ be a simplex such that $C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)$. We have for any vertex $v$ of $T$
$$
|f(v) - f(z_T)| \leq d_H(z_T,v) \leq C_0 \|z_T - v\|_{\cH_T} = C_0.
$$
Denoting by $V$ the collection of vertices of $T$ we thus obtain for any $z,z'\in T$
$$
\interp_T f(z) - \interp_T f(z') = \sum_{v\in V} (\lambda_v(z) - \lambda_v(z')) (f(v) - f(z_T)).
$$
Where $\interp_T$ denotes the $\P_1$ (piecewise affine) interpolation on a simplex $T$, and $\interp_\cT$ the $\P_1$ interpolation on a mesh $\cT$.
hence using Lemma \ref{lemmaNormLambda}
\begin{eqnarray*}
|\interp_T f(z) - \interp_T f(z')| &\leq& C_0 \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|\\
 &\leq& C_0 \sqrt{(d+1)  \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|^2} \\
 &=& C_0 \sqrt d \|z-z'\|_{\cH_T}.
\end{eqnarray*}
The last inequality implies that 
$$
\dil_z(\interp_{\cT_n} f \sep d_H)\leq C_0^2 \sqrt d
$$
for all $T\in \cT_n$ and $z\in \interior(T)$.
Let $n_0 \geq 0$ be such that $\supp(f)\subset \Omega_{n_0}$, which implies that $\interp_{\cT_n} f$ is continuous. It follows from Corollary \ref{corolLipNoGamma} that $\interp_{\cT_n} f : (\R^d, d_H) \to \R$ is $C_0^2\sqrt d$-Lipschitz.

We define 
$
D := \cup_{T \in \cT} \interior(T),
$
and we denote by $\interp_T f : D \to \R$ the function which coincides with $\interp_T f$ on the \emph{interior} of each $T\in \cT$. % (and which is possibly discontinuous at the interfaces between the simplices $T\in \cT$). 
For any $z\in D$ we obtain using \iref{eqTTnz} that $\interp_{\cT_n} f(z) \to \interp_\cT f(z)$, hence for any $z,z'\in D$
$$
|\interp_\cT f(z) - \interp_\cT f(z')| = \lim_{n \to \infty} |\interp_{\cT_n} f(z)-\interp_{\cT_n} f(z')| \leq \sqrt d C_0^2 \, d_H(z,z').
$$
The piecewise interpolant $\interp_T f : D \to \R$ therefore extends to a $\sqrt d C_0^2$-Lipschitz function $\interp_T f : (\R^d, d_H) \to \R$. It easily follows that $\interp_\cT f$ is continuous for any compactly supported $C^1$ function $f$. This property characterizes conforming meshes, hence $\cT\in \bT$ which concludes the proof.
\sq



\begin{corollary}(Bidimensional triangulations)
\label{corolBidimIso}
Assume that the dimension is $d=2$. There exists $c>0$ such that the following holds: if $s: \R^2 \to \R_+^*$ is $c$-Lipschitz, then there exist a mesh $\cT$ of $\R^2$ built of half squares, and such that for all $T\in \cT$ and $z\in T$
\be
\label{eqDT32}
\diam(T) \leq s(z) \leq 3 \diam(T)/2.
\ee
\end{corollary}

\proof
When the dimension is $d=2$, the collection $\gT_0$ of triangles contains only half squares, of area $1/2$, hence  $D_+ = D_- = \sqrt 2$. 

As $s \to 0$ the constant $C_s$ defined by \iref{defCs} tends to $\sqrt 2$. Hence $C_s\leq 3/2$ when $s$ is sufficiently small.
If $s$ is bounded by $\sqrt 2$ on $[0,1]^2$ one may therefore produce a mesh $\cT_*$ of $[0,1]^2$ such that \iref{eqDT32} holds for all $T\in \cT_*$, $z\in T$.

From this point construct as before a sequence of meshes $\cT_n$ of the squares $[-2^{n-1}, 2^{n-1}]$ which satisfies \iref{eqDT32}, and we extract a global mesh $\cT$ of $\R^2$ using Lemma \ref{lemmaExtractMesh}. The triangles $T\in \cT$ still satisfy the inequality \iref{eqDT32} since they are limits in the Haussdorff distance of triangles from the triangulations $\cT_n$.
\sq


\subsection{Graded mesh generation}
\label{secMeshGenG}

We prove in this section a result of bi-dimensional mesh generation, Theorem \ref{thEquiMesh}, which implies Point (iii) of Proposition \ref{propMeshGen}. The key ingredients of this section come from the paper \cite{Shew}.
We assume throughout this section that the dimension is $d=2$.

For that purpose we introduce the notion of equispaced points in an abstract metric space.
 Let $(X,d_X)$ be a metric space and let $\delta>0$, we say that a subset $\cV \subset X$ is $\delta$-equispaced if the following holds.
\begin{enumerate}[a)]
\item (Covering) The distance from an arbitrary point $x\in X$ to $\cV$ is bounded by $1$ : for all $x\in X$
\be
\label{eqCover}
d_X(x, \cV) := \inf\{d_X(x,v) \sep v \in \cV\} \leq 1.
\ee
\item (Separation) The pairwise distances between the points of $\cV$ are larger than $\delta$ : for all $v, v'\in \cV$ such that $v \neq v'$
\be
\label{eqSep}
d_X(v,v') \geq \delta.
\ee
\end{enumerate}

The next lemma establishes the existence of such a set under certain assumptions. \begin{lemma}
\label{lemmaEquiSpaced}
Let $(X,d_X)$ be a metric space in which the closed balls $B'(x,r) := \{y\in X \sep d_X(x,y) \leq r\}$ are compact for all $x\in X$ and $r\geq 0$. 
Let $\cV_0$ subset $X$ be such that $d_X(v,v') \geq 1$ for all $v,v'\in \cV_0$ such that $v\neq v'$. Then there exists a $1$-equispaced set $\cV$ of the metric space $(X,d_X)$, containing $\cV_0$.
\end{lemma}

\proof
We may assume that $\cV_0 \neq \emptyset$, up to including an arbitrary point of $X$, and we choose an  arbitrary  $x_0\in \cV_0$.
We define inductively a sequence $(x_n)_{0 \leq n< N}$ of points and $(\cV_n)_{0 \leq n < N}$ of subsets of $X$, where $N\in \N \cup \{\infty\}$ is specified later, proceeding as follows.
Assuming that $\cV_n$ is already defined we consider the closer set 
\be
\label{eqDefXn}
X_n :=  
\{x\in X \sep d_X(x,\cV_n) \geq 1\}.
\ee
If the set $X_n$ is empty, then the sequence ends and we define $N := n+1$. Otherwise we choose $x_{n+1}$ arbitrarily among the minimisers of $d_X(x,x_0)$ on $X^n$:
\be
\label{defxn}
x_{n+1} \in \underset {x\in X_n} \argmin \,d_X(x,x_0),
\ee
and we define $\cV_{n+1} := \cV_n \cup\{x_{n+1}\}$.
Such a minimizer exists since $X_n$ is closed and since the closed balls in $X$ are compact.
%$$
%X^n \cap \overline B\left(x_0, \ 1+ \inf_{x\in X^n} d_X(x_0, x)\right)
%$$
%is compact.
We define $N := \infty$ none of the sets $(X_n)_{n \geq 0}$ is empty. %if the sequence $(x_n)$ is infinite.

We define $\cV := \cup_{0 \leq n <N} \cV_n$.
%We denote by $X_0 := \{x_n \sep 0\leq n<N\}$ the collection of all points of this finite or countable sequence.
%
%We define $N := \infty$ if the sequence $x_0, x_1, \cdots$ is infinite, and we denote by $X_0$ the collection of all points of this finite or countable sequence,
%$$
%X_0 := \{x_n \sep 0 \leq n < N\}.
%$$ 
%%as the collection of all points $x_0, x_1, \cdots$ of this finite or countable sequence.
%, which clearly is finite or countable.
By construction, we thus have $d_X(v, v') \geq 1$ for all $v,v'\in \cV$
which establishes the separation property \iref{eqSep}. %, and shows that $\cV$ is a discrete set.

We now assume for contradiction that the covering property \iref{eqCover} does not hold which implies that $N= \infty$. We choose a point $x_*\in X$ such that $d_X(x_*, \cV)>1$, and therefore $x_*\in X_n$ for all $n \geq 0$. The definition \iref{defxn} of $x_{n+1}$ implies that $d_X(x_0, x_n) \leq d_X(x_0, x_*)$ for all $n \geq 0$, hence the discrete collection of points
$
\{x_n \sep n \geq 0\}
$
in included in the closed ball $\{x\in X \sep d_X(x_0, x) \leq d_X(x_0, x_*)\}$ which is compact.
The sequence $(x_n)_{n \geq 0}$ therefore admits a converging subsequence, but this contradict the fact that the pairwise distances between these points are larger than $1$, which concludes the proof of this proposition.
\sq


%The next lemma gives a simple (from a theoretical point of view) procedure which produces a point set equidistributed with respect to a metric.
%\begin{lemma}
%Let $H\in \bH$ and let $(p_n)_{n\geq 0}$ be a sequence of points obtained by choosing $p_0 = 0$ and then iteratively choosing $p_{n+1}$ among the minimizers of
%\be
%\label{defpn}
%\min\{\|p\| \sep d_H(p, \{p_0,\cdots , p_n\} \geq 1)
%\ee
%
%Then the point set $\cP := \{p_n \sep n \geq 0\}$ is $1$-equidistributed with respect to $H$.
%\end{lemma}
%
%\proof
%The separation holds by construction. It implies in particular that for any $M \geq 1$, $\cP\cap B(0,M)$ is finite. 
%
%%Since $H$ is continuous and positive definite, for each $M$ the set $\{n\geq 0 \sep \|p_n\| \leq M\}$ is finite.
%Indeed let $\Lambda^2 := \max \{\|H(z)\| \sep \|z\| \leq M\}$.
%The balls $B(p, \Lambda/2)$, $p\in \cP\cap B(M)$ are pairwise disjoint. It follows from a volume argument that $\cP\cap B(M)$ is finite.
%
%Let us assume by contradiction that there exists $z\in \R^2$ such that $d(z, \cP)>1$. Then for $n$ large enough we have $\|z\| < \| p_{n+1}\|$ which is incompatible with the construction of $p_{n+1}$ as a minimizer of \iref{defpn}.
%\sq




We consider a fixed metric $H \in \bH$. For any $x,y\in \R^2$ we define 
$$
d_x(y) := \|x-y\|_{H(x)}.
$$
We also consider a fixed discrete collection of vertices, or ``sites'', $\cV \subset \R^2$, and we define the anisotropic Voronoi cell of a site $v\in V$ as follows 
\be
\label{defVorv}
\Vor(v) := \{z\in \R^2 \sep d_v(z) \leq d_w(z) \text{ for all } w \in V\}.
\ee
The anisotropic Voronoi cell $\Vor(v)$ is thus the collection of points $z$ which are \emph{closer to the vertex $v$ than to any other site}.
The classical (isotropic) Voronoi is obtained by choosing $H = \Id$.
We refer to the paper \cite{Shew} Figure 3 for an illustration of the anisotropic Voronoi diagram $\{\Vor(v) \sep v\in \cV\}$ associated to a point set.

For each $z\in \R^2$ we define $\cV_z$ the collection of vertices which contain $z$ in their Voronoi region:
$$
\cV_z := \{v \in \cV \sep z \in \Vor(v)\}.
$$
The geometric dual of the Voronoi diagram is the graph $\cG(\cV,H)$ defined as follows:
\be
\label{defGVH}
\cG(\cV,H) := \{[v,v'] \sep \text{there exists } z\in \R^2 \text{ such that } V_z = \{v,v'\}\}.
\ee

%We define a collection $\cT_0(V,H)$ of convex sets attached to the metric $H$ and to the collection $V$ of sites
%$$
%\cT_0(V,H) := \{\Cvx(V_z) \sep z \in \R^2 \text{ and } \#(V_z) \geq 3\}.
%$$
The next theorem establishes that $\cG(\cV,H)$ is, under certain conditions on the metric $H$ and the set $\cV$, the graph of a triangulation adapted to $H$.

\begin{theorem}
\label{thEquiMesh}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta)\geq 1$ such that the following holds.
Let $H$ be a metric such that $c^2 H\in \bH_g$, and let $\cV$ be a $\delta$-equispaced subset of $(\R^2, d_H)$.
Then the $\cG(\cV,H)$ is a planar graph which defines a partition of $\R^2$ into strictly convex polygons. Arbitrarily triangulating each polygon yields a triangulation $\cT\in \bT_{g,C}$ which is $C$-adapted to $H$, called an anisotropic Delaunay triangulation. Furthermore if $\cV$ is in general position then $\cG(\cV,H)$ is already the graph of a triangulation.
\end{theorem}

Denote by $c$ and $C$ the constants attached to $\delta=1$ in this theorem.
It follows that for any metric $H$ such that $c^2 H \in \bH_g$, there exists a mesh $\cT\in \bT_{g,C}$ which is $C$-adapted to $H$, obtained as the Delaunay triangulation of a $1$-equispaced set of points $\cV\subset (\R^2, d_H)$. 
This immediately implies Point iii) of Proposition \ref{propMeshGen} according to Remark \ref{remcC}.


The rest of this section is devoted to the proof of Theorem \ref{thEquiMesh}, which is based on the methods and results presented in \cite{Shew}. 
%These theorems are based on a property that needs to be 
For that purpose we recall some definitions of this paper. %introduce the following definitions.
\begin{definition}
\label{defWedge}
%The wedge of $v,v'$ is 
\begin{itemize}
\item (Wedge of two points)
We define the wedge $\wed(v,w)$ of two distinct sites $v,w\in V$ as follows
$$
\wed(v,w) := \{z\in \R^2 \sep (z-v)^\trans H(v) (w-v) >0 \text{ and } (z-w)^\trans H(w) (v-w) >0\}
$$ 
\item (Wedge property)
We say that the Voronoi diagram of $V$ is wedged if for any two distinct $v,w \in V$ we have 
$$
\Vor(v) \cap \Vor(w) \subset \wed(v,w).
$$
\end{itemize}
\end{definition}

The wedge property expresses that the collection $\Vor(v) \cap \Vor(w)$ of points $q$ shared by the Voronoi regions of the sites $v$ and $w$ lie in a cone defined by two linear inequalities.
We refer to \cite{Shew} Figure 4 for an illustration of the wedge of two sites.

The next proposition, which is partly is based on Lemma 5 from \cite{Shew},
 shows that the wedge property is automatically satisfied in our context.
For any metric $H$ and any constant $c>0$ such that $c^2H\in \bH_g$, it easily follows from Proposition \ref{propEuclidRiemann} that for all $x,y\in \R^2$
\be
\label{eqDHLog}
\ln (1+ c\, d_x(y)) \leq c \, d_H(x,y) \leq - \ln(1- c\, d_x(y)), 
\ee
which is equivalent to 
\be
\label{eqDHExp}
1-\exp(-c\, d_H(x,y)) \leq c \, d_x(y) \leq \exp(c \, d_H(x,y))-1.
\ee

\begin{lemma}
\label{lemmaDiamVor}
If $c^2 H\in \bH_g$ %and $\cV$ is $\delta$-equispaced, 
then
for any $v\in \cV$ and any $q\in \Vor(v)$ we have 
\be
\label{eqDiamVor}
\|q-v\|_{H(v)} \leq r_0(c) := (e^c-1)/c.
\ee
If $v,w \in \cV$ satisfy $\Vor(v) \cap \Vor(w) \neq \emptyset$, then 
\be
\label{eqVordvw}
%\delta \leq 
d_H(v,w) \leq r_1(c) := -2\ln(2-e^c)/c.
\ee
Note that $r_0(c) \to 1$ and $r_1(c) \to 2$ as $c\to 0$. Note also that $d_H(v,w)\geq \delta$ if $\cV$ is $\delta$-equispaced.
\end{lemma}

\proof
For any $q\in \cV$ there exists $v_* \in \cV$ such that 
$
d_H(q,v_*) \leq 1,
$
and therefore 
$$
\|q-v_*\|_{H(v_*)} \leq r_0(c) := (e^c-1)/c,
$$
which implies \iref{eqDiamVor} using the definition \iref{defVorv} of the Voronoi diagram.
We thus turn to the proof of \iref{eqVordvw} and for that purpose we consider a point $q\in \Vor (v)\cap\Vor(w)$. We thus have
$
\max\{\|q-v\|_{H(v)} , \|q-w\|_{H(w)} \}\leq  v_c%-\ln(1-c v_c)/c
$
hence
$$
d_H(v,w) \leq r_1(c) :=-2\ln(1-c r_0(c))/c,
$$
which concludes the proof.
\sq

\begin{prop}
\label{propWedge}
For each $\delta$ there exists $c=c(\delta)>0$ such that the following holds.\\
If a metric $H$ satisfies $c^2H\in \bH_g$ and if $\cV$ is a $\delta$-equispaced subset of $(\R^2,d_H)$, then the wedge property is satisfied.
\end{prop}

\proof
We assume for contradiction that there exists two distinct vertices $v,w \in V$, and a point $q\in \Vor(V) \cap \Vor(W)$ such that $z\notin \wed(v,w)$. We may assume, up to exchanging the roles of $v$ and $w$, that 
$$
(q-w)^\trans H(w) (v-w) \leq 0.
$$
Defining the ``relative distortion''
$
\tau := \exp d_\times (H(v), H(w))
$
we obtain using Lemma 5 from \cite{Shew} %(*$q$ instead of $z$??*)
\be
\label{eqShewWedge}
 d_w(v) \leq d_w(q) \sqrt{\tau^2-1}.
\ee
We now estimate the quantities $d_w(v)$, $d_w(q)$ and $\tau$ appearing in this estimate, in order to obtain a contradiction when $c$ is sufficiently small.

%Since the set $V$ is $C_0$-equispaced, there exists $u\in V$ such that $d_H(u,q) \leq C_0$. Recalling that $z\in \Vor(v)\cap \Vor(w)$ we thus obtain using \iref{eqDHExp}
%\be
%\label{eqDiamVor}
%d_v(q) = d_w(q) \leq d_u(q) \leq \frac{\exp(c \, d_H(u,q))-1} c \leq r_0(c) := \frac{\exp(c C_0)-1} c,
%\ee
%and therefore using \iref{eqDHLog} 
%\be
%\label{eqVordvw}
%d_H(v,w) \leq d_H(v,q)+ d_H(q,w) \leq r_1(c) := \frac {-2\ln (1- c r_0(c))}  c,% \frac 1 {1-f(c)}.
%\ee
%hence 
We have 
\be
\label{eqTauWedge}
\ln \tau = d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
\ee
Since $\cV$ is $\delta$-equispaced we have 
$
d_H(v,w) \geq \delta
$
and therefore 
\be
\label{eqdvwWedge}
c \,d_w(v) \geq 1-\exp(-c d_H(v,w)) \geq 1-\exp(-c\delta)
\ee
Injecting \iref{eqDiamVor}, \iref{eqTauWedge} and \iref{eqdvwWedge} in \iref{eqShewWedge} we obtain
\be
\label{eqFinalWedge}
\frac{1-\exp(-c\delta )} c \leq \frac{\exp(c)-1} c \sqrt{\exp(2c r_1(c))-1}.
\ee
The left hand side tends to $\delta$ as $c\to 0$, while the right hand side tends to $0$. We thus obtain a contradiction when $c$ is sufficiently small which concludes the proof of this proposition.
\sq

\begin{theorem}[Dual triangulation theorem. Labelle, Shewchuck, \cite{Shew}]
\label{thShew}
If the Voronoi diagram of the point set $\cV \subset \R^2$ is wedged, then the geometric dual of this diagram is a polygonalization of $\R^2$ with strictly convex polygons and is a triangulation $\cT$ if $\cV$ is in general position.
\end{theorem}

Under the hypotheses of this theorem the vertices $v_1, \cdots, v_k$ of a polygon in the dual Voronoi diagram satisfy by construction $\Vor(v_1)\cap \cdots \cap \Vor(v_k) \neq \emptyset$, and therefore the vertices $v_1, v_2, v_3$ of a triangle $T\in \cT$ satisfy $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$.

The next theorem, originally stated in \cite{Shew} as Corollary 10 to Theorem 9 of the same paper, allows to control the angles of a triangle in the anisotropic Delaunay triangulation.

\begin{theorem}[Labelle, Shewchuk, \cite{Shew}]
\label{thAngle}
Let $v_1,v_2,v_3\in \cV$ and let $q\in \Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)$. Let 
$$
r = d_{v_1}(q) = d_{v_2}(q) = d_{v_3}(q) \stext{ and }
l = \min\{d_{v_i}(v_j) \sep i,j \in \{1,2,3\}, i \neq j\}.
$$ 
Define $\beta := \max\{r/l,\, 1/\sqrt 2\}$, %and %$\gamma\in [1,\infty)$ by 
%Let $1\leq \gamma \leq \sqrt 2$ and $\beta \geq \frac 1 {\sqrt 2}$ satisfy
$$
\gamma := \exp \max \{d_\times (H(v_i), H(v_j)) \sep i,j \in \{1,2,3\}, i \neq j\},
$$
and
\be
\label{defChi}
\chi := \frac 1 {2 \beta} - \frac{(\gamma^2-1)\beta} 2.
\ee
If $\gamma \leq \sqrt 2$ and $\chi>0$ then any angle $\theta$ of the triangle of vertices $(\sqrt{H(v_1)} v_k)_{1 \leq k \leq 3}$ satisfies
$$
\arcsin ( \chi/ \gamma^2) \leq \theta \leq 2 \arccos(\chi/\gamma^2).
$$
\end{theorem}

\begin{corollary}
\label{corolAdaptG}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta) \geq 1$ such that the following holds.
If $\cV$ is $\delta$-equispaced, if $c^2H\in \bH_g$ and if $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$, then denoting by $T$ the triangle of vertices $v_1,v_2,v_3$ we have for all $z\in T$
$$
C^{-2} H(z) \leq \cH(z) \leq C^2 H(z).
$$
\end{corollary}
\proof
We use \iref{eqDHExp} and \iref{eqDHLog} and the fact that $V$ is $\delta$-equispaced to obtain explicit bounds on the quantities $r$, $l$, $\beta$, $\gamma$ and $\chi$ appearing in Theorem \ref{thAngle}.
It follows from Lemma \ref{lemmaDiamVor} that 
$$
r\leq r_0(c) \stext{ and } \delta \leq d_H(v_i,v_j) \leq r_1(c).
$$
Therefore 
$$
l := \min_{i\neq j} d_{v_i}(v_j)\geq %\min_{i\neq j} \frac{1-\exp(-c d_H(v_i,v_j))} c \geq  
r_2(c) := (1-\exp(-c\delta))/ c,
$$
and 
$$
L := \max_{i\neq j} d_{v_i}(v_j) \leq (\exp(c r_1(c))-1)/c
$$
and 
$$
\gamma \leq \max_{i\neq j} \exp(c \,d_H(v_i,v_j)) \leq \exp(c \,r_1(c)).
$$
In particular 
$
\beta \leq r_3(c) := \min\{r_0(c)/r_2(c),\, 1/\sqrt 2\}. % = \frac{\exp(cC_0)-1}{1-\exp(-2 cC_0^{-1})},
$
Injecting this into \iref{defChi} yields an explicit lower estimate 
$$
\chi\geq r_4(c) := \frac 1 {2r_3(c)} - \frac{ (\exp(2cr_1(c))-1) r_3(c)} 2,
$$ 
and $\chi/\gamma^2\geq r_5(c) := r_4(c) \exp(-2cr_1(c))$.

For a fixed $\delta$ we obtain as $c\to 0$ the limits $r_0(c) \to 1$, $r_1(c)\to 2 $, $r_2(c) \to \delta$, $r_3(c) \to \min\{\delta, 1/\sqrt 2\}$ and $r_4(c) \to 1/(2\min\{\delta, 1/\sqrt 2\})$ and $r_5(c)$ as the same limit.

%We assume without loss of generality that $\delta \geq 1/\sqrt 2$ and we thus obtain $r_3(c) \to \delta$, 
%$r_4(c) \to 1/C_0^2$ and $r_5(c) \to 1/C_0^2$. 
We may therefore choose $c$ sufficiently small in such way that 
$$
l \geq l_0 := \delta/2, \ L  \leq L_0 := 4 \text{ and }\chi/\gamma^2 \geq \Chi_0 := 1/(4\min\{\delta, 1/\sqrt 2\}).
$$
We denote by $T$ the triangle of vertices $v_1, v_2, v_3$. The length of any edge of $T' := \sqrt{H(v_1)}(T)$ is bounded above by $L_0$ and below by $l_0$ respectively, and the angles of $T'$ satisfy $\arcsin (\Chi_0) \leq \theta \leq 2 \arccos(\Chi_0)$. The collection of triangles centered at the origin which satisfy these inequalities is compact, thus there exists a constant $C_1 = C_1(C_0)$ such that 
$$
C_1^{-2} \Id \leq \cH_{T'} \leq C_1^2 \Id,
$$
hence $C_1^{-2} H(v_1) \leq \cH_{T'} \leq C_1^2 H(v_1)$. For any $z\in T$ we obtain, remarking that $\|z-v_1\|_{\cH_T} \leq 2$ for all $z\in T$ and using \iref{eqLocalNorm}, 
$$
C_1^{-2} (1-2cC_1)^2 H(z) \leq \cH_{T'} \leq C_1^2(1-2cC_1)^{-2} H(z)
$$
which concludes the proof of this proposition, with $C = C_1(1-2cC_1)^{-1}$.
\sq

We now prove of Theorem \ref{thEquiMesh}.
According to the above results for any $\delta>0$ there exists $c = c(\delta)$ and $C=C(\delta)$ such that the following holds. 
For any set $\cV \subset (\R^2, d_H)$ which is $\delta$-equispaced, the Voronoi diagram associated to $\cV$ and $H$ is wedged according to Proposition \ref{propWedge}. The dual of this diagram is therefore a polygonalization of $\R^2$ with strictly convex polygons according to Theorem \ref{thShew}.
Randomly triangulating these cells yields a triangulation $\cT\in \bT$ which is $C$-adapted to $H$ according to Corollary \ref{corolAdaptG}. 

Furthermore consider to simplices $T,T'\in \cT$ such that $T \cap T'\neq \emptyset$, and a point $z\in T \cap T'$.
Then 
$$
C^{-2} \cH_T \leq H(z) \leq C^2 \cH_{T'},
$$
which shows that $\cT\in \bT_{g,C^2}$ and concludes the proof of Theorem \ref{thEquiMesh}.

\subsection{Quasi-Acute mesh generation}
\label{secMeshGenA}

This section is devoted to the proof of Point ii) of Proposition \ref{propMeshGen}, which is obtained by combining the  constructions of isotropic and graded triangulations presented in \S\ref{secMeshGenI} and \S\ref{secMeshGenI} to produce a quasi-acute triangulation. 
The key idea of this proof if that the anisotropic Delaunay triangulation described in the previous subsection contains only \emph{few} strongly obtuse angles if the set $\cV$ of vertices is structured along lines which are \emph{transverse to the direction of anisotropy}, as illustrated on Figure \ref{figAcuteGen} (in the introduction of this chapter). 

The author is sorry to say that this proof is not yet as polished as the rest of the thesis, due to time constraints. This proof involves from instance a number of numerical constants which are far from optimal.

We consider a fixed metric $H$ such that $c^2 H\in \bH_a$, where $c$ is an absolute constant specified in the proof and such that $0<c\leq 1$. This subsection is devoted to the construction of a mesh $\cT\in \bT_{a,C}$ which is $C$-adapted to $H$, where $C$ is an absolute constant also specified in the proof.
This construction immediately implies Proposition \ref{propMeshGen} according to Remark \ref{remcC}. 


For each $z\in \R^2$ we define %We define two functions $\lambda, \mu : \R^2 \to \R$ as follows : for all $z\in \R^2$
$$
\lambda(z) := \|H(z)^{-\frac 1 2}\| \stext{ and } \mu(z) = \|H(z)\|^{-\frac 1 2},
$$
and we observe that $\lambda(z) \geq \mu(z)$.
The functions $\lambda$ and $\mu$ are $c$-Lipschitz according to Corollary \ref{corolLipNorm}.
% : for all $z,z'\in \R^d$
%$$
%|\lambda(z)-\lambda(z')| \leq c|z-z'| \text{ and } |\mu(z) - \mu(z') | \leq c|z-z'|.
%$$
If $c$ is sufficiently small, then there exists according to Corollary \ref{corolBidimIso} a mesh $\cT_0$ such that for all $T\in \cT_0$ and all $z\in T$
\be
\label{ratioDiamLambda}
\frac 2 3  \lambda(z) \leq \diam(T)\leq \lambda(z). 
\ee
The mesh $\cT_0$ is built of half squares by construction (as illustrated on Figure \ref{figHalfSquares}) hence  for any edge $[v,w]$ of any triangle $T\in \cT_0$ we have $\diam(T)/\sqrt 2 \leq |v-w|\leq \diam(T)$, and the diameter of any triangle $T\in \cT_0$ is a power of $\sqrt 2$. Therefore if two triangles $T,T'\in \cT_0$ share a vertex $v$ we obtain 
\be
\label{eqDiamRatio}
\diam(T)/\sqrt 2 \leq \diam(T') \leq \sqrt 2 \diam(T),
\ee
which implies for any edges $[v,w]$ and $[v,w']$ (sharing the vertex $v$) of the triangulation $\cT_0$ 
\be
\label{eqEdgeRatio}
|v-w|/2 \leq |v-w'| \leq 2|v-w|.
\ee
Inequality \iref{ratioDiamLambda} also implies that for any edge $[v,w]$ of $\cT_0$
%We say that two vertices $v,w\in \cV_0$ are neighbors in $\cT_0$ if they belong to a common triangle $T\in \cT_0$.
%In that case we have %Let $v,w$ be two vertices of a triangle $T\in \cT_0$, then 
\be
\label{edgeLambda}
\frac{\lambda(z)\sqrt 2}3 \leq \frac{\diam(T)}{\sqrt 2}\leq |v-w| \leq \diam(T)\leq \lambda(z)
\ee
We denote by $\cV_0$ the collection of vertices of $\cT_0$. 
Consider a fixed $v\in \cV_0$ any vertex $w\in \cV_0$ such that $|v-w|$ is minimal. Then $[v,w]$ is clearly an edge of $\cT_0$. This implies for any distinct $v,w\in \cV_0$
\be
\label{pairwiseV0}
\lambda(v) \frac {\sqrt 2} 3 \leq |v-w| .
\ee


For each $z\in \R^2$ we define 
$$
\rho(z) := \lambda(z)/\mu(z)  = \sqrt{\|H(z)\| \|H(z)^{-1}\|} \in [1, \infty).
$$
Consider $z,z'\in \R^2$ such that $|z-z'| \leq r\lambda(z)$, where $r\geq 0$ is a constant. Then since $\lambda$ and $\mu$ are $c$-Lipschitz we obtain 
\be
\label{eqrhozzp}
\rho(z') = \frac{\lambda(z')}{\mu(z')} \geq \frac{\lambda(z)(1-r c)}{\mu(z)+ r c \lambda(z)} \geq \frac {1-r c}{\rho(z)^{-1}+r c}.
\ee
For each $\rho_0, r_0$ we denote by $c_\rho(\rho_0, r_0)>0$ the constant such that $\rho_0 = \frac {1-r_0 c_\rho(\rho_0, r_0)}{(\rho_0+1)^{-1}+r_0 c_\rho(\rho_0, c_0)}$.
For any $z,z'\in \R^2$ we thus have
$$
\left\{
\begin{array}{c}
|z-z'| \leq r_0\lambda(z)\\ 
\rho(z) \geq \rho_0+1\\
c\leq c_\rho(\rho_0, r_0)
\end{array}
\right.
%\Big(|z-z'| \leq r_0\lambda(z) , \ \rho(z) \geq \rho_0+1 \text{ and } c\leq c_\rho(\rho_0, r_0)\Big) 
\stext{ implies } \rho(z') \geq \rho_0
$$
For instance if $z,z'$ belong to the same triangle $T\in \cT_0$, if $\rho(z) \geq n+1$ and $c\leq c_\rho(n,1)$ then $\rho(z') \geq n$ according to \iref{edgeLambda}. 
%Throughout this proof we shall make a finite number of assumptions of the type $c \leq c_\rho(r_0,\rho_0)$ for some absolute constants $r_0, \rho_0$. They hold if $c$ if sufficiently small.

For each $z\in \R^2$ such that $\rho(z)>1$ we denote by $\theta(z)\in \bbS := \{u\in \R^2\sep |u| = 1\}$ a unit vector such that
\be
\label{defAngle}
H(z) = \lambda(z)^{-2} \theta(z) \theta(z)^\trans+ \mu(z)^{-2} (\Id-\theta(z) \theta(z)^\trans).
\ee
Note that there exists two, opposite, choices for the vector $\theta(z)$.
For each $u,u'\in \R^2 \sm\{0\}$ we define the (unoriented) angle
$$
\varangle (u,u') := \arccos \left(\frac{\<u,u'\>}{|u| |u'|}\right) \in [0,\cPi].
$$
and 
%For any two vectors $u,u'\in \R^2\sm\{0\}$ we define %the non-oriented, acute, angle
$$
\lhd(u,u') := \min \{\varangle(u,u'),\, \varangle(u,-u')\} = \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
$$
\begin{lemma}
\label{lemmaAngle12}
If $c$ is sufficiently small, then the following holds.
For any $z,z'\in \R^2$ 
$$
\left\{
\begin{array}{c}
\rho(z) \geq 2\\
|z'-z|\leq 10 \lambda(z) 
\end{array}
\right.
\stext{ implies }
\lhd(\theta(z), \theta(z')) \leq \cPi/12,
$$
and likewise $\rho(z) \geq 4$ and $|z-z'| \leq \lambda(z)$ implies $\lhd(\theta(z), \theta(z')) \leq 1/(10 \sqrt 2)$.
\end{lemma}

\proof
We consider a fixed point $z$ such that $\rho(z) \geq 2$ and we denote by $B$ the ball $\{z'\in \R^2\sep |z'-z| \leq 10 \lambda(z)\}$.
For each $z'\in B$ we have
\begin{eqnarray*}
\lambda(z') - \mu(z') &\geq& (\lambda(z)-c|z-z'|) - (\mu(z)+ c |z-z'|) \\
&=& \lambda(z) -\mu(z) -2 c |z-z'| \\
&\geq& \lambda(z) -\lambda(z)/ 2 - 20 c\lambda(z)\\
&=& \lambda(z)(1/2 -20 c),
\end{eqnarray*}
hence $\lambda(z') - \mu(z')\geq \lambda(z)/3$ if $c \leq 1/120$, which we assume from this point.

Furthermore since $B$ is simply connected there exists a continuous function $\theta_* : B \to \bbS$ (where $\bbS := \{u\in \R^2 \sep |u|=1\}$ denotes the unit circle) such that $\theta_*(z')  = \pm \theta(z')$ for all $z'\in B$.
According to Theorem \ref{th2Spaces} we have for all $z'\in B$
$$
\lambda(z)\dil_{z'}(\theta_*) \leq 3(\lambda(z')-\mu(z')) \dil_{z'}(\theta_*) \leq 3c.
$$
Therefore, since the distance $d_\bbS$ on $\bbS$ involved in Theorem \ref{th2Spaces} coincides with the angle $\varangle$ we obtain
$$
\lhd(\theta(z), \theta(z'))\leq \varangle(\theta_*(z), \theta_*(z')) \leq |z-z'| \max_{\ti z \in [z,z']} \dil_{\ti z}(\theta_*) \leq 30c 
$$
which concludes the proof if $30c \leq \cPi/12$.
\sq


For each vertex $v\in \cV_0$ we define a set $\Gamma_v\subset \R^2$ as follows : $\Gamma_v := \{v\}$ if $\rho(v) <3$, and 
\be
\label{defGammav}
\Gamma_v := \left[v, \, \frac v 3+ \frac{2w_-} 3\right] \cup \left[v,\frac v 3 +\frac{2w_+} 3\right] 
\ee
if $\rho(v)\geq 3$, where $[v,w_-]$ and $[v,w_+]$ are two edges of $\cT_0$ which respectively minimize and maximize the quantity $\<\theta(v)^\perp, w-v\>$ (among the edges containing $v$).
In other words for any edge of $\cT_0$ of the form $[v,w]$ we have
\be
\label{defWmWp}
\<\theta(v)^\perp, w_- -v\> \leq \<\theta(v)^\perp, w-v\> \leq  \<\theta(v)^\perp, w_+ - v\>. 
\ee
This property is illustrated on Figure \ref{figWmWp}.

\begin{figure}
\centering
\includegraphics[width=4cm, height=4cm]{\pathPic/Dessins/Jenny/VT0vJenny.pdf}\hspace{1cm}
\includegraphics[width=6cm, height=4cm]{\pathPic/Dessins/Jenny/DirThetaJenny.pdf}
\caption{Neighborhood $V_{\cT_0}(v)$ of a simplex $v$ in the triangulation $\cT_0$ (left), the neighbors $w_+$ and $w_-$ of a vertex $v$ in $\cT_0$.
\label{figWmWp}}
\end{figure}

\begin{lemma}
\label{lemmaAngleWmWp}
let $v\in \cV_0$ be such that $\rho(v) \geq 3$, and let $[v,w_+]$, $[v,w_-]$ be two edges of $\cT_0$ satisfying \iref{defWmWp}.
We have 
\be
\label{eqAngleWmWp}
\varangle(\theta(v)^\perp, w_+ -v) \leq \cPi/4,
\stext{ and }
\varangle(\theta(v)^\perp, v-w_-) \leq \cPi/4.
\ee
\end{lemma}

\proof
We restrict without loss of generality our attention to the proof of the first inequality, and we assume for contradiction that $\vp := \varangle(\theta(v)^\perp, w_+-v)>\cPi/4$. % in \iref{eqAngleWmWp}.
Among the two vertices $w\in \cV_0$ such that the triangle of vertices $v,w,w_+$ belongs to $\cT_0$, we choose the one such that $\varangle(\theta^\perp, w-v)$ is minimal.
We denote $\psi := \varangle(w-v, w_+-v) \in \{\cPi/4, \cPi/2\}$ and we obtain 
$$
\<\theta(v)^\perp, w_+-v\> = |w_+-v|\cos \vp \stext{ and } \<\theta(v)^\perp, w-v\> = |w-v|\cos (\vp-\psi).
$$
If $\psi = \cPi/2$ then $|w_+-v| = |w-v|$ since the triangles $T\in \cT_0$ are half squares, and $\cos (\vp-\psi) = \sin \vp$. We thus have $\cos \vp \geq \sin \vp$ according to \iref{defWmWp} which contradicts our assumption that $\vp>\cPi/4$.
If $\psi = \{\cPi/4\}$ then $|w_+-v| = \sqrt 2 |w-v|$ or $|w_+-v| =  |w-v|/\sqrt 2$. We thus have $\sqrt 2 \cos \vp \geq \cos (\vp-\cPi/4)$ which again contradicts our assumption that $\vp > \cPi/4$.
\sq

We define $\Gamma := \cup_{v\in \cV_0} \Gamma_v$, and for each $z\in \Gamma\sm\cV_0$ we define 
\be
\label{defGammaz}
\Gamma_z := \bigcup_{\substack{v\in \cV_0 \\ z \in \Gamma_v}} \Gamma_v.
\ee
Note that for any vertex $v\in \cV_0$ the set $\Gamma_v$ does not contain any vertex $w\in \cV_0$ distinct from $v$, hence \iref{defGammaz} agrees with \iref{defGammav} for any $z\in \cV_0$.\\ 

\begin{lemma}
\label{lemmaPi3}
For any $z\in \Gamma$ and any $z'\in \Gamma_z$ 
distinct from $z$
%we have
%\be
%\label{eqAngleGammaz}
%\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
%\ee
%and therefore if $c$ is sufficiently small
we have 
$$
\angle(\theta(z)^\perp ,z'-z) \leq \cPi/3, 
$$
%and there exists a piecewise affine Lipschitz map $\gamma : [\alpha, \beta]\to \R$ such that the following is a bijection
%$$
%t\in [\alpha, \beta] \mapsto z+ t\theta(z)^\perp + \sqrt 3 \gamma(t) \theta(z) \in \Gamma_v.
%$$

(*alternative version*)
For any $z\in \Gamma$, any $z'\in \Gamma_z \sm \{z\}$ and any $\ti z \in [z, z']$ we have 
%we have
%\be
%\label{eqAngleGammaz}
%\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
%\ee
%and therefore if $c$ is sufficiently small
we have 
$$
\angle(\theta(\ti z)^\perp ,z'-z) \leq \cPi/3, 
$$


\end{lemma}

\proof
According to the definition \iref{defGammaz} of $\Gamma_z$ there exists a vertex $v\in \cT_0$ such that $z,z'\in \Gamma_v$. Therefore $|z-v| \leq \lambda(v)$ and $\rho(v) \geq 3$.
It follows from Lemma \ref{lemmaAngleWmWp} and Lemma \ref{lemmaAngle12} that 
$$
\lhd(\theta(z)^\perp, z'-z) \leq \lhd(\theta(v), \theta(z)) + \lhd(\theta(v),z'-z) \leq \cPi/12 + \cPi/4 = \cPi/3,
$$
which concludes the proof.
\sq

The next proposition gives some upper and lower bounds on the distance from a point to the set $\Gamma$.
\begin{prop}
\label{propDistUpLow}
If $c$ is sufficiently small, then the following holds.
For any $z\in \Gamma$,
\be
\label{eqDistzGH0}
 \min\{|z-e| \sep  e\in \Gamma\sm \Gamma_z\} \geq \frac {10}{91} \lambda(z) % >\frac 1 {10}
\ee
and for any $z\in \R^2$
\be
\label{eqDistzGH}
\min\{\|z-e\|_{H(z)} \sep e \in \Gamma\} \leq 2 %1+ \frac {2\sqrt 2} 3 <2. 
\ee
\end{prop}

\begin{figure}
\centering
\includegraphics[width = 4cm, height = 4cm]{\pathPic/Dessins/Jenny/DistZGJenny.pdf}
\caption{Illustration of the proof of Proposition \ref{propDistUpLow} \label{figDistZG}}
\end{figure}

\proof
We first establish \iref{eqDistzGH0}. 
Let $z\in \Gamma$ and let $v\in \cV_0$ be such that $z\in \Gamma_v$. There exists an edge $[v,w_*]$ of $\cT_0$ and a parameter $\alpha\in [0,2/3]$ such that $z= (1-\alpha) v+\alpha w_*$.
We denote by $V_{\cT_0}(v)$ the union of all triangles $T\in \cT_0$ containing $v$, and by $\cV_0(v)$ the collection of vertices $w$ such that $[v,w]$ is an edge of $\cT$. We thus have
$$
\Gamma\sm \Gamma(z) \subset \overline {\R^2 \sm V_{\cT_0}(v)} \bigcup_{w\in \cV_0(v)\sm\{w_*\}} \left[\frac{2v+w}3, w\right].
$$
The set appearing in the right hand side is illustrated on Figure \ref{figDistZG}.
Denoting $d(z,E) := \inf\{ |z-e|\sep e\in E\}$ we obtain 
\begin{eqnarray*}
d(z,\Gamma\sm \Gamma(z)) &\geq & \min \left\{ d(z, \R^2 \sm V_\cT(v)), \ \min_{w\in \cV_0(v) \sm \{w_*\} } d\left(z,\left[\frac{2v+w}3, w\right]\right)\right\}\\
& \geq & \min \left\{ \frac{|w_*-z|}{\sqrt 2}, \ \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)\sm \{w_*\}} |v-w|\right\}\\
& = & \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)} |v-w|\\
& \geq & \frac{1}{3\sqrt 2} \lambda(v)\frac {\sqrt 2} 3 \\
&\geq&  \frac{\lambda(z)(1-c|z-v|)}{9} \geq \frac{\lambda(z)(1-c)}{9},
\end{eqnarray*}
where we used \iref{edgeLambda} in the fourth line, and the fact that $\lambda$ is $c$-Lipschitz in the last line. This establishes \iref{eqDistzGH0} if $c$ is sufficiently small.\\

We now turn to the proof of \iref{eqDistzGH}. 
Let $T \in \cT_0$ and let $z\in T$. Since $T$ is a half square there exists a vertex $v$ of $T$ such that $|z-v| \leq \diam(T)/2$, hence %For any vertex $v$ of $T$ we obtain %If $\rho(z)\leq 4$, then any vertex $v$ of $T$ satisfies 
$$
\|z-v\|_{H(z)} \leq  \frac{|z-v|}{\mu(z)}   \leq \frac{\diam(T)}{2 \mu(z)} \leq \frac{\lambda(z)}{2 \mu(z)} = \frac{\rho(z)} 2,
$$
which concludes the proof if $\rho(z) \leq 4$. If $\rho(z) \geq 4$ and $c\leq c_\rho(3,1)$ then $\rho(v) \geq 3$ for any vertex $v$ of the triangle $T$.

We choose two vertices $v,w$ of $T$ such that the line $(z+ r \theta(z))_{r\in \sR}$ intersects $\partial T$ on the segment $[v,(v+w)/2]$.
We denote by $w_-,w_+\in \cV_0$ the neighbors of $v$ in $\cT_0$ which satisfy \iref{defWmWp}.
Our first step is to establish that the line $(z+ r \theta(z))_{r\in \sR}$ intersects the set $\Gamma_v$ : this is heuristically due to the fact that the angle $\lhd(\theta(z), \theta(v))$ is small and that the vertices $w_-$ and $w_+$ are the \emph{farthest} from $v$ in the direction of $\theta(v)^\perp$ as illustrated on Figure \ref{figWmWp} (right).

We have according to \iref{eqEdgeRatio}
$$
\<\theta(v)^\perp,w_+ - v\> \geq |w_+-v|\cos(\cPi/4) \geq \frac{|w-v|} 2 \frac 1 {\sqrt 2}. %/(2\sqrt 2).
$$
We assume without loss of generality that %$\theta(v)$ and $\theta(z)$ are oriented in consistently, in such way that 
$\<\theta(z), \theta(v)\> \geq 0$ which implies % and we obtain using Corollary \ref{corolTheta2C}
$$
|\theta(z)-\theta(v)| \leq \varangle(\theta(z), \theta(v)) = \lhd(\theta(z), \theta(v)) \leq \delta := 1/(10 \sqrt 2).
$$
It follows that 
\begin{eqnarray*}
\<\theta(z)^\perp, w-v\> &=& \<\theta(z)^\perp-\theta(v)^\perp, w-v\>+\<\theta(v)^\perp, w-v\>\\
& \leq & |\theta(z)-\theta(v)| |w-v| + \<\theta(v)^\perp, w_+-v\>\\
& \leq & (1+2\delta \sqrt 2 )\<\theta(v)^\perp, w_+-v\>.\\
%& \leq & (1+4 c\sqrt 2) }{1-\vp_c\sqrt 2} \<\theta(z)^\perp,w_+ - v\>.
%& \leq & \frac 4 3 \<\theta(z)^\perp,w_+ - v\>
\end{eqnarray*}
Denoting $\Theta := \varangle(\theta(v)^\perp, w_+-v)$ and $\Phi := \varangle(\theta(z)^\perp, w_+-v)$ we obtain 
$$
\frac{\<\theta(v)^\perp, w_+-v\>}{\<\theta(z)^\perp, w_+-v\>} = \frac{\cos(\Theta)}{\cos(\Phi)} \leq \frac{\cos(\Theta)}{\cos(\Theta) - |\Phi-\Theta|} =\left(1-\frac {|\Phi-\Theta|}{\cos\Theta}\right)^{-1}\leq (1-\delta \sqrt 2)^{-1} % - 2c} = \frac 1 {1-2 \sqrt 2 c},
$$
hence 
$$
\<\theta(z)^\perp, w-v\>  \leq \frac{1+2\delta \sqrt 2}{1-\delta \sqrt 2 c}\<\theta(z)^\perp, w_+-v\> \leq \frac 4 3 \<\theta(z)^\perp, w_+-v\>.
$$
Proceeding likewise for $w_-$, and assuming that $c$ is sufficiently small, we obtain 
%
%We assume that $c$ is sufficiently small in such way that 
%\be
%\label{assumPhic}
%\frac{1+\vp_c 4\sqrt 2}{1-\vp_c\sqrt 2}\leq \frac 4 3
%\ee
$$
\frac 4 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, w-v\> \leq  \frac 4 3\<\theta(z)^\perp, w_+ - v\>,
$$
and therefore since $z+r\theta(z)\in [v,(v+w)/2]$ for some $r\in \R$,
$$
\frac 2 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, z-v\> \leq  \frac 2 3\<\theta(z)^\perp, w_+ - v\>.
$$
It follows that the line $(z+r\theta(z))_{r\in \sR}$ intersects the set $\Gamma_v := [v, (v+2w_+)/3] \cup  [v, (v+2w_-)/3]$ at some point $z'$.
%hence there exists $r\in \R$ such that $z' := z+ r\theta(z) \in \Gamma_v$. 
The point $z'$ belongs to a triangle $T'$ containing $v$, which implies using \iref{eqDiamRatio} 
\begin{eqnarray*}
\lambda(z) \|z'-z\|_{H(z)} &=& \lambda(z)\|r\theta(z)\|_{H(z)}\\
&=& |r|\\
&=& |z-z'|\\
&\leq& |z-v|+|v-z'|\\
&\leq& \diam(T)+ \frac 2 3\diam(T')\\
&\leq & \left(1+\frac 2 3 \sqrt 2\right) \diam(T)
 \leq  \left(1+\frac 2 3 \sqrt 2\right) \lambda(z),
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

We construct in the next lemma the set of vertices $\cV$ of the quasi-acute triangulation $\cT$ to be constructed, by sampling the set $\Gamma$.

\begin{lemma}
\label{lemmaConstV}
The following holds if $c$ is sufficiently small.
There exists a discrete set $\cV \subset\Gamma$ containing $\cV_0$ and satisfying the following:
\begin{enumerate}[i)]
\item (Separation) For all $v,w\in \cV$, $d_H(v,w) \geq 1/10$.
\item (Distance from $\Gamma$) For all $z\in \Gamma$, $d_H(z, \cV) \leq 1/10$.
\item (Distance from $\R^2$) For all $z\in \R^2$, $d_H(z,\cV) \leq 2+1/4$.
\end{enumerate}
\end{lemma}
\proof
For any distinct $v,w\in \cV_0$ we obtain using \iref{pairwiseV0} and Proposition \ref{propEuclidRiemann}
\begin{eqnarray*}
d_H(v,w) &\geq& \ln(1+c\|v-w\|_{H(v)})/c\\
&\geq& \ln(1+c|v-w|/\lambda(v))/c\\
&\geq& \ln(1+c\sqrt 2 /3)/c 
\end{eqnarray*}
which is larger than $1/10$ if $c$ is sufficiently small. % since $\sqrt 2 /3>1/10$.

We denote by $\cV$ a $1$-equispaced subset of the metric space $(\Gamma, 10\:d_H)$ containing $\cV_0$, which exists according to Lemma \ref{lemmaEquiSpaced}. The two first announced properties, separation and distance from $\Gamma$, follow directly from this construction.

The third property is obtained as follows: for any $z\in \R^2$ there exists according to Proposition \ref{propDistUpLow} a point $e\in \Gamma$ such that $\|z-e\|_{H(z)}\leq 2$. Furthermore there exists a vertex $v\in \cV$ such that $d_H(e,v) \leq 1/10$, hence
$$
d_H(z,\cV) \leq d_H(z,e)+ d_H(e,v) \leq -\ln(1-c\|z-e\|_{H(z)})/c + 1/10 \leq -\ln(1-2c)/c + 1/10.
$$
which is smaller than $2+1/4$ if $c$ is sufficiently small.
\sq

The next lemma introduces the anisotropic Delaunay triangulation $\cT$ associated to the metric $H$ and the set of points $\cV$. 

\begin{lemma}
\label{lemmaRecallG}
There exists a absolute constant $C_0\geq 1$ such that the following holds if $c$ is sufficiently small.
The set $\cV$ is wedged with respect to the metric $H$, and the anisotropic Delaunay triangulation $\cT_0$ obtained by arbitrarily triangulating the cells of the graph $\cG(\cV,H)$ is $C_0$-adapted to $H$ and belongs to $\bT_{g,C_0}$.

Furthermore for any edge $[v,w]$ of $\cT$ and any $z\in [v,w]$ we have 
$$
\|v-w\|_{H(z)} \leq 5.
$$
\end{lemma}

\proof
We denote $\alpha := (2+1/4)^{-1}$ throughout the proof of this lemma.
It follows from to Lemma \ref{lemmaConstV} that the set $\cV$ is a $\alpha/10$-equispaced subset of the metric space $(\R^2, \alpha d_H)$. 

Theorem \ref{thEquiMesh} applied to the metric $\alpha^2 H$, therefore implies that, if $c$ is sufficiently small, the set 
$\cV$ is wedged for the metric $\alpha^2 H$ and that arbitrarily triangulating the convex cells of the graph $\cG(\cV,\alpha^2 H)$, which are convex yields a triangulation $\cT$ which is $C$-adapted to the metric $\alpha^2H$ (hence $C_0 := C/\alpha$-adapted to $H$), where $C$ is an absolute constant.

The definition \iref{defGVH} of the graph $\cG(V,H)$ implies that $\cG(\cV,\alpha^2 H) = \cG(\cV,H)$, and Definition \ref{defWedge} of the wedge property shows that it holds for $H$ if and only if it holds for $\alpha^2 H$. 

For any edge $[v,w]$ of $\cT$ the Voronoi regions $\Vor(v)$ and $\Vor(w)$ intersect (by definition of the anisotropic Delaunay triangulation), and we thus have according to Lemma \ref{lemmaDiamVor} 
$$
\alpha d_H(v,w) = d_{\alpha^2 H} (v,w) \leq -2\ln (2-e^{c'})/c'
$$
where $c' := c/\alpha$. Hence 
$$
d_H(v,w) \leq r_0(c) := -2 \ln (2-e^{c/\alpha})/c.
$$
If follows that 
$
\|v-w\|_{H(v)} \leq r_1(c) := (e^{c r_0(c))}-1)/c,
$
hence \iref{eqLocalNorm}
$
\|v-w\|_{H(z)} \leq \|v-w\|_{H(v)} (1-c \|v-z\|_{H(v)})^{-1} \leq r_2(c) := r_1(c) (1-c r_1(c))^{-1}
$
for any $z\in [v,w]$.
As $c\to 0$ the functions $r_0$, $r_1$ and $r_2$ all tend to $2 (1+1/4) <5$. Choosing $c$ sufficiently small concludes the proof of this proposition.
\sq

Triangulation $\cT$ introduced in the previous lemma is $C_0$ adapted to $H$, and belongs to $\bT_{g,C_0}$. The rest of this chapter is devoted to the proof that, if $c$ is sufficiently small, then $\cT$ is a quasi-acute triangulation : $\cT\in \bT_{a,C}$ where $C$ is an absolute constant.

The next lemma 
%is a first step in this direction. It 
states that the edges of $\cT$ fall into two well separated categories : the edges aligned with the direction $\theta$ of anisotropy, and the edges transverse to that direction.
%It heuristically expresses that the long edges of $\cT$ are aligned with the direction $\theta$ of anisotropy.

\begin{lemma}
%If $c$ is sufficiently small, then the following holds.
%For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$ we have 
%\be
%\label{vpNotInGammav}
%\sin \lhd (\theta(v),v-w) \leq \frac {50}{\rho(v)}.
%\ee
%
%(*alternative version*)
%For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$, and any $z\in [v,w]$ such that $\rho(z) \geq \rho_l$ we have 
%\be
%\label{vpNotInGammav2}
%\lhd(\theta(z), v-w) \leq \cPi/12,
%\ee
%where $\rho_l$ is a constant specified in the proof.
%
%
%(*alternative version*)
The following holds if $c$ is sufficiently small.
Let $[v,w]$ be an edge of $\cT$ and let $z\in \cT$ be such that $\rho(z) \geq \rho_l$, where $\rho_l$ is an absolute constant specified in the proof. Then 
\be
\label{twoDir}
\lhd(\theta(z) , w-v) \leq \cPi/12 \text{ or } \lhd(\theta(z)^\perp, w-v) \leq \cPi/3.
\ee

\end{lemma}

\proof
If $w\in \Gamma_v$ then the estimate $\lhd(\theta(z)^\perp, w-v) \leq \cPi/3$ immediately follows from lemma \ref{lemmaPi3}.
On the other hand if $w\notin \Gamma_v$Lemma \ref{lemmaRecallG} states that $\|v-w\|_{H(v)} \leq 5$.
$$
 \frac{|w-v|}{\mu(z)} \sin \lhd(\theta(z) , w-v) \leq \|w-v\|_{H(z)} \leq 5.
$$
Proposition \ref{propDistUpLow} implies that 
$$
\frac{|w-v|}{\lambda(z)} \geq \frac{|v-w|}{\lambda(v)(1+5c)} \geq \frac {10}{91(1+5c)}
$$
Hence $|w-v|\geq \lambda(z)/10$ if $c$ is sufficiently small.

It follows that 
$$
\sin \lhd(\theta(z) , w-v) \leq \frac{50}{\rho(z)},
$$
which concludes the proof choosing $\rho_l := 50 / \sin (\cPi/12)$.
\sq

The next lemma is devoted to the comparison of the Voronoi cell of a vertex $v\in \cV$ with closed balls $\overline B_H(v,r)$ around $v$ for the norm $\|\cdot \|_{H(z)}$ (which are therefore some ellipses)
$$
\overline B_H(v,r) := \{z\in \R^d \sep \|z-v\|_{H(v)} \leq r\}.
$$


%The next lemma shows that the Voronoi regions associated to a vertex $v\in \cV$ contain an ellipse of controlled size.

\begin{lemma}
\label{lemmaVorBall}
If $c$ is sufficiently small, then the following holds.
For any $v\in \cV$ we have 
$$
\overline B_H(v,1/25)  \subset \Vor(v), %:= \{z\in \R^2 \sep \|z-v\|_{H(v)} \leq 1/25\}
$$
and 
$$
\overline B_H(v,\alpha(c) /10) \supset \Vor(v) \cap \Gamma
$$
where $\alpha(c) := (e^{c/10} - 1)/(c/10)$ which tends to $1$ as $c \to 0$.
It follows that $\|v-w\| \leq 1/4$ for all $v,w\in \cV$ such that $\Vor(v) \cap \Vor(w) \cap \Gamma \neq \emptyset$.
\end{lemma}

\proof
We consider $z\in \partial \Vor(v)$, hence $z\in \Vor(v) \cap \Vor(w)$ for some vertex $w\in \cV$.
We define $r:=\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$ and we obtain using Point i) of Lemma \ref{lemmaConstV}
\begin{eqnarray*}
1/10 &\leq& d_H(v,w)\\
&\leq& d_H(z,v)+d_H(z,w)\\
&\leq& -\ln (1-c\|z-v\|_{H(v)})/c - \ln (1-c\|z-v\|_{H(v)})/c\\
&=& -2 \ln (1-cr)/c.
\end{eqnarray*}
It follows that 
$$
r\geq (1-\exp(-c/20))/c,
$$
and therefore $r\geq 1/25$ if $c$ is sufficiently small, 
which concludes the proof.
\sq


\begin{lemma}
\label{lemmaDiamVorGamma}
For any $v\in \cV$ we have 
$$
\max\{\|z-v\|_{H(v)} \sep z\in \Gamma\cap \Vor(v)\} \leq r_0(c) := (e^{c/10}-1)/c.
$$
(and $r_0(c) \to 1/10$ as $c\to 0$).
Furthermore $c$ is sufficiently small and if $v,w\in \cV$ are such that $\Vor(v) \cap \Vor(w) \cap \Gamma \neq \emptyset$, then 
$$
\|v-w\|_{H(v)} \leq 1/4.
$$
\end{lemma}

\proof
According to point ii) of Lemma \ref{lemmaConstV} there exists $w\in \cV$ such that $d_H(z,w) \leq 1/10$. It thus follows from the definition of the Voronoi diagram that 
\begin{eqnarray*}
\|z-w\|_{H(w)} &\leq& \|z-w'\|_{H(w')}\\
&\leq& (\exp(c d_H(z,w'))-1)/c\\
&\leq&  (\exp(c/10)-1)/c.
\end{eqnarray*}

We now turn to the second point of the proposition, and we consider a point $z\in \Vor(v) \cap \Vor(w) \cap \Gamma$.
We thus have $\|z-v\|_{H(v)} = \|z-w\|_{H(w)} \leq r_0(c)$ which implies 
$$
\ln(1+c\|v-w\|_{H(v)})/c \leq d_H(v,w) \leq d_H(v,z)+d_H(z,w) \leq -2 \ln(1-c r_0(c))/c
$$
hence $\|v-w\|_{H(v)} \leq ((1-cr_0(c))^{-2}-1)/c$ which tends to $1/4$ as $c\to 0$. This concludes the proof of this proposition.
\sq

%\begin{lemma}
%If $c$ is sufficiently small, then the following holds.
%
%\end{lemma}

The next lemma gives a lower bound on the distance from a vertex $v\in \cV$ to the Voronoi region of a vertex $w\in \cV\sm\Gamma$.

\begin{lemma}
\label{lemmaVorFar}
If $c$ is sufficiently small, then for any $v\in \cV$, $w\in \cV\sm \Gamma_v$ 
$$
\inf\{|v-z|\sep z\in \Vor(w) \cap \Gamma\} \geq \lambda(v)/100.
$$

%and $z\in \Vor(w)\cap \Gamma$ we have 
%$$
%|z-v|\geq \lambda(v)/100.
%$$
\end{lemma}

\proof
We have for any $z\in \Vor(w) \cap \Gamma$, according to Lemma \ref{lemmaDiamVorGamma} 
\begin{eqnarray*}
|v-z| &\geq& |v-w|-|z-w|\\
& \geq & |v-w| - \|z-w\|_{H(w)} \lambda(w)\\
& \geq & |v-w| - r_0(c) (\lambda(v)+c|v-w|)\\
& = & |v-w| (1-c r_0(c)) -r_0(c) \lambda(v)\\
& \geq & \frac {10} {91}\lambda(v) (1-cr_0(c)) - r_0(c) \lambda(v)\\
&=& r_1(c) \lambda(v),
\end{eqnarray*}
where we used \iref{eqDistzGH0} in the fifth line, and where $r_1(c) := 10(1-cr_0(c))/91 - r_0(c)$.
As $c\to 0$ we have $r_0(c) \to 1/10$ and $r_1(c) \to 10/91-1/10 >1/100$. If $c$ is sufficiently small we therefore have $r_1(c) \geq 1/100$ which concludes the proof.
\sq

The next proposition shows that the Voronoi cell of a vertex $v$ contains a ball of fixed radius for the distance $\|\cdot\|_{H(v)}$ (hence an ellipse).


%The set $\Gamma$ is a union of polygonal lines (and of isolated points). If $v\in \Gamma$ is on a polygonal line, we say that the neighbors of $v$ on $\Gamma$ (if they exist) are the previous and next points on $\Gamma$.

%The set $\Gamma$ is a union of polygonal lines (and of isolated points). We say that two points $v,w\in \Gamma$ are neighbors on $\Gamma$ if 

We say that two points $v,w\in \cV$ are neighbors on $\Gamma$ if 
$$
(v,w) \subset \Gamma\sm \cV.
$$
Note that $\Gamma\sm\cV$ is a collection of straight open intervals, since $\cV_0\subset \cV$.
Note also that two neighbors on $\Gamma$ belong to the same element of $\cT_0$.

\begin{lemma}
\label{lemmaSegVor}
If $c$ is sufficiently small, then the following holds.
For any $v\in \cV$ such that $\rho(v) \geq \rho_0 = 22$ the vector $v$ has at least a neighbor on $\Gamma$. Furthermore for any neighbor $w$ of $v$ on $\Gamma$ we have 
$$
|v-w|\leq \mu(v)/2
$$
and 
\be
\label{eqNeighborEdge}
[v,w] \subset \interior(\Vor(v) \cup \Vor(w)).
\ee
and consequently $[v,w]$ is an edge of $\cT$. 
\end{lemma}

\proof
We first remark that according to Lemma \ref{lemmaDiamVorGamma} 
\be
\label{dzvmu}
r_0(c) \geq \|z-v\|_{H(v)} \geq \cos\left(\cPi/ 3 \right) \frac {|z-v|}{\mu(v)}  = \frac {|z-v|}{2 \mu(v)}
\ee
We assume for contradiction that the inclusion \iref{eqNeighborEdge} does not hold, and we thus consider two points $z\in [v,w]\cap \Vor(v)$ and $w'\in \cV$ such that $z\in \Vor(w')$.



If $w'\notin \Gamma_v$, then $|z-v| \geq  \lambda(v)/100$ according to Lemma \ref{lemmaVorFar}.
Combining this with \iref{dzvmu} we obtain 
$$
\rho_0 \leq \rho(v) = \lambda(v)/\mu(v) \leq 200 r_0(c).
$$
If $c$ is sufficiently small then $200r_0(c) < 21 < 22$ which gives a contradiction (recall that $r_0(c) \to 1/10$ as $c\to 0$).

We now consider the case $w'\in \Gamma_v$, and we first assume that $w'$ is not on the same side as $w$ on $\Gamma$, in the sense that $\<w-v, \theta(v)^\perp \>>0$ and $\<w'-v, \theta(v)\> <0$.
Hence there exists $\alpha\in [0,1]$ and $r\in \R$ such that 
$$
v + r \theta(v) = z+ \alpha(w'-z).
$$
%Consider a vector $u$ orthogonal to $w-z'$. 
We thus have 
$
r\<\theta(v),(w'-z)^\perp \> = \<z-v , (w'-z)^\perp\>
$
hence
$$
r/2\leq  |r| \cos \lhd(\theta(v)^\perp, w'-v) \leq  |z-v| \leq 2 \mu(v) r_0(c).
$$
According to \cite{Shew} Lemma 3 (Visibility Lemma) the Voronoi regions of a wedged Voronoi diagram are star-shaped. Since the Voronoi diagram is wedged according to Lemma \ref{lemmaRecallG} we obtain using Lemma \ref{lemmaVorBall} that 
$$
\frac {\lambda(v)} {25} = \|r\theta(v)\|_{H(v)} \leq r \leq 4 \mu(v) r_0(c),
$$
hence $\rho_0 \leq \rho(v) \leq 100 r_0(c)$. This is a contradiction if $c$ is sufficiently small since $100 r_0(c) <11 <22 = \rho_0(c)$.

It follows that $w'$ is on the same side as $w$ on $\Gamma$, with respect to $v$, in the sense that  $\<w-v, \theta(v)^\perp \>>0$ and $\<w'-v, \theta(v)^\perp\> >0$.

We now remark that the vertices $v,w$ belong to the same element of $\cT_0$ since they are neighbors on $\Gamma$. Hence $\rho(w) \geq \rho_0 - 1=21$ if $c$ is sufficiently small.
Way may therefore apply this proof to $w$, and we obtain that $w'$ is on the same side as $v$ with respect to $w$, in the sense that  $\<w'-w, \theta(w)^\perp \><0$ and $\<w'-v, \theta(w)\> <0$ (if $\<\theta(w), \theta(v)\> >0$).

It follows that $w'\in (v,w)$ which is a contradiction.


Finally, we remark that according to Lemma \ref{lemmaDiamVorGamma}
$$
1/4 \geq \|v-w\|_{H(v)} \geq \frac{|v-w| \cos (\cPi/3)}{\mu(v)} = \frac{|v-w|}{2\mu(v)}
$$
hence $|v-w|\leq \mu(v)/2$ which concludes the proof.
\sq


\begin{prop}
The following holds if $c$ is sufficiently small.
For any $v\in \cV$ be such that $\rho(v)\geq \rho_1$, where $\rho_1$ is a constant specified in the proof, the following holds.
\begin{enumerate}
\item The vertex $v$ has two neighbors $w,w'$ on $\cT$ such that 
\be
\label{eqAnglesUpDown}
\varangle(w-v, \theta(v)) \leq \cPi/12 \stext{ and } \varangle(w'-v, -\theta(v)) \leq \cPi/12.
\ee
\item A vertex $w\in \cT\cap \Gamma_v$ is a neighbor of $v$ on $\cT$ if and only if it is a neighbor of $v$ on $\Gamma$.
\end{enumerate}
\end{prop}

\proof
Consider a neighbor $w_*$ of $v$ on $\Gamma$. Then according to Lemma \ref{lemmaSegVor} the segment $[v,w]$ is an edge of $\cT$, hence $w_*$ is a neighbor of $v$ on $\cT$ by definition.
Let $T,T'\in \cT$ be the two triangles containing the edge $[v,w_*]$, and let $w,w'\in \cV$ be the third vertex of these triangles respectively.

Since $\cT$ is $C_0$-adapted to the metric $H$, we obtain 
$$
|T| = |\TEq| (\det \cH_T)^{-\frac 1 2} \geq |\TEq|  C_0^{-2} (\det H(v))^{-\frac 1 2} =  |\TEq|  C_0^{-2} \lambda(v) \mu(v).
$$
On the other hand $|w_*-v| \leq \mu(v)/2$ according to Lemma \ref{lemmaSegVor}, and 
$$
\mu(v)\sin \lhd(w-v,\theta(v))  |w-v|\leq \|v-w\|_{H(v)} \leq C_0 \|v-w\|_{\cH_T} \leq 2C_0.
$$
Combining these inequalities we obtain  
$$
|\TEq|  C_0^{-2} \lambda(v) \mu(v) \leq  |T| \leq \frac 1 2 |w-v| |w_*-v| \leq \frac{2C_0\mu(v) }{\sin \lhd(w-v,\theta(v))} \mu(v)/2.
$$
hence 
$$
\sin \lhd(w-v,\theta(v)) \leq \frac{C_0^3}{|\TEq| \rho(v)}. 
$$
We define 
$$
\rho_1 := \frac{C_0^3}{|\TEq|\sin (\cPi/12)}
$$
and we thus obtain $\lhd(w-v,\theta(v)) \leq \cPi/2$. Likewise $\lhd(w'-v,\theta(v)) \leq \cPi/2$. 

Since $\varangle (w_* - v, \theta(v)) \in [\cPi/3,2 \cPi/3]$, and since the triangles $T,T'$ contain the edge $[v,w_*]$, thus implies \iref{eqAnglesUpDown}.

Let $v'\in \cV \cap \Gamma_v$ be a vertex on the side of the neighbor $w_*$.
Then $\lhd(v'-v, \theta(v)^\perp) \leq \cPi/3$ which implies that the segment $[v,v']$ intersects one of the triangles $T$ or $T'$. 
Therefore $v'$ is not a neighbor of $v$ in $\cT$.

Likewise, if $v$ has a second neighbor $w_{**}$ on $\Gamma$ (on the other side than $w_*$ with respect to $w$), then $[v,w_{**}]$ is an edge of $\cT$. Similarly we obtain that for any point $v''\in \Gamma_v$ on the side of $w_{**}$, the segment $[v,v'']$ is not an edge of $\cT$.

This implies Point 2. and concludes the proof of this proposition.
\sq

For each $v\in \cV_0$ we define $\Gamma'_v := [v,w_-] \cup[v,w_+]$ where $w_-$ and $w_+$ are defined by \iref{defWmWp}.
We then set 
$$
\Gamma' := \bigcup_{\substack{v\in \cT_0\\ \rho(v) \geq 1+\rho_1}} \Gamma'_v.
$$


\begin{prop}
If $c$ is sufficiently small, then the following holds.
Denote by $\cQ$ the partition into convex polygons of $\R^2$ obtained by the overlay of $\cT$ and $\Gamma'$.
We denote by $\cT'$ the partition obtained by randomly triangulating the convex cells of $\cQ$.


%Denote by $\cT'$ the triangulation obtained by randomly triangulating the 
%
%Denote by $\cQ$ the partition into convex polygons obtained by cutting $\cT$ by all segments joining an extremal vextex $v\in \cV$ satisfying $\rho(v) \geq ??$ to the vertex $v'\in \cV_0$ in the direction of $\bt(v)$.
%
%Then the interior angles in $\cQ$ are smaller than ??. %Each triangle $T\in \cT$ contains at most $??$ cells of $\cC$, which are at most hexagons (in other words they have $3$ to $6$ elements).
%
%Denote $\cT'$ the triangulation obtained by randomly triangulating the convex cells of $\cQ$.

Then $\cT'$ is a $??$-refinement of $\cT$ and $S(T') \leq ??$ for all $T'\in \cT'$.
\end{prop}

\proof
Since the collection $\cV$ of vertices of $\cT$ contains $\cV_0$ and since the segments in $\Gamma$ join some points of $\cV_0$, we find that the overlay of $\cT$ and $\Gamma$ is indeed a partition of $\R^2$ into convex polygons.

Our first objective is to give a uniform bound on the measure of sliverness in $\cT'$.
For that purpose we consider a cell $Q \in \cQ$ and a vertex $z$ of $Q$.

We first assume that $z\notin \cV$, hence $z$ is a vertex created by the overlay of $\Gamma$ on $\cT$.
We denote by $v_0$ the vertex in $\cV_0$ such that $z\in \Gamma'_{v_0}$, and we observe that $\rho(v_0) \geq \rho_0+1$.
Let $[w,w']$ be the edge of $\cT$ containing $z$. We have 
$$
|z-w| \leq \lambda(z) \|z-w\|_{H(z)} \leq \lambda(z) \|w-w'\|_{H(z)} \leq 5 \lambda(z)\leq 5 \lambda(v_0)(1+c). 
$$
hence
$$
|v_0 - w| \leq |v_0 - v| + |v-w| \leq \lambda(v_0) (6+5c).
$$
If $c$ is sufficiently small, then we obtain $\rho(w) \geq \rho_1$.
Therefore $w' \notin \Gamma_w$, otherwise $w'$ would be a neighbor of $w$, $[w,w'] \subset \Gamma$ which contradicts the fact that this edge was bisected by the overlay.

Hence $\sin \lhd(\theta(v),v-w) \leq 50/\rho(v)$. Hence $\lhd(\theta(v),v-w) < \cPi/24$. On the other hand $\lhd(\theta(v), \theta(z)) \leq 2 \times 5 c \leq \cPi/24$ if $c$ is sufficiently small. We conclude that $\lhd(v-v_0, w,w') \geq \cPi/12$.\\

We may therefore assume that $v\in \cV$.
If $\rho(v) \leq 2+\rho_1$ then 
$$
S(T) \leq \rho(T) = \sqrt {\|\cH_T\| \|\cH_T^{-1}\|} \leq C_0^2 \rho(v) \leq C_0^2 (2+\rho_1).
$$
The angle $\vp$ of $\cQ$ at $v$ is bounded by the angle of $T$ at $v$, hence by
$$
\tan \vp \leq C_0^2 (2+\rho_1),
$$
which gives a uniform bound.\\


If $\rho(v)\geq 2+\rho_1$, then there exists two neighbors $w,w'$ of $v$ satisfying \iref{eqAnglesUpDown}. Let $v_0\in \cT_0$ be such that $v \in \Gamma_{v_0}$. 
If $c$ is sufficiently small, then $\rho(v_0) \geq 1+\rho_1$. 
Therefore $v\in \Gamma'_v$, and the tangent $\bt, \bt'$ vectors to $\Gamma'_v$ in the two directions satisfy $\lhd(\theta(v)^\perp, \bt) \leq \cPi/3$ and $\lhd(\theta(v)^\perp, \bt') \leq \cPi/3$.

It follows that the angle of $Q$ at $v$ is bounded by $5 \cPi/6$.\\


We now prove that $\cT'$ is a bounded refinement of $\cT$, and for that purpose we consider and edge $e=[v,w]$ of $\cT$. %=[\omega-u, \omega+u]

We have by construction $|v-w|/\lambda(v) \leq \|v-w\|_{H(v)} \leq 12$.
The triangles $T\in \cT_0$ intersected by $[v,w]$ satisfy for some $z\in [v,w]$ the inequality 
$$
2 \delta_0 \lambda(v) (1-12c) \leq 2 \delta_0 \lambda(z) \leq \diam(T) \leq \lambda(v) \leq \lambda(u)(1+12c)
$$
Therefore they are contained in the ball $B(v,  \lambda(v)(12+1+12c))$ and have area 
$$
|T| = \diam(T)^2/4 \geq \delta_0^2 \lambda(v)^2 (1-12c)^2.
$$
Therefore there are at most 
$$
\cPi (13+12c)^2/ (1-12c)^2 \leq k := \cPi 14^2,
$$
such triangles, and the edge $e$ is thus cut in at most $k$ parts by the edges joining an extremal vertex in $\cV$ to the corresponding vertex in $\cV_0$.

Hence there are at most $3k$ vertices of $\cT'$ on the three edges of a triangle $T\in \cT$ (including the vertices of $T$).
Since any conforming triangulation of convex envelope of $n+2$ points uses $n$ triangles, we obtain that $\cT'$ is a $3k-2$ refinement of $\cT$.
\sq

%\input{../Bibliography/Bibliography.tex}
\end{document}



==> MeshMetric/MeshMetricTheseOld6.tex <==
\input{../PreambleThese}

\section{Introduction}

Triangulations and meshes are finite objects of combinatorial nature: they can be described by a collection of vertices and of connection between these. This description is fruitful for the demonstration of algebraic results, such as the Euler formula, or for computer processing.
In contrast, many approaches towards anisotropic mesh generation are based on a continuous object, namely a riemannian metric $z\mapsto H(z)$, in other words a continuous function $H$ from the domain $\Omega\subset \R^d$ to the set $S_d^+$ of symmetric positive definite matrices. Once this metric has been properly designed, it is the task of a mesh generation algorithm such as \cite{Shew,Bois,FreeFem,Inria} to generate a triangulation that agrees with this metric, in a sense specified below \iref{defEquiv}.
The purpose of this chapter is to formulate precise equivalence results between some classes of triangulations and of riemannian metrics. This equivalence translates some geometrical constraints satisfied by the triangulations into the form of regularity properties of the equivalent riemannian metrics.\\

Our results are so far limited to meshes and metrics defined on the entire infinite domain $\R^d$, and the dimension $d\geq 2$ is fixed throughout this chapter. 
The choice of the unbounded domain $\R^d$ guided by simplicity, since the curvature and the singularities of
of the boundary $\partial\Omega$ induces additional difficulties 
from the point of view of computational mesh generation.
Bounded domains will be the object of future work.
We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$, and we introduce in \S\ref{subsecDefTStar} three embedded subsets of $\bT$ of particular interest 
$$
\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C},
$$
where $C\geq 1$ is a parameter which plays a minor role.
The set $\bT_{i,C}$ collects all \emph{isotropic} meshes $\cT$ which are heuristically defined as follows: the simplices $T\in \cT$ may have strongly varying volumes, but their aspect ratio is uniformly bounded. 
The largest set $\bT_{g,C}$ collects \emph{graded} meshes, which only satisfy a condition of local consistency: all the  geometrical features of the simplices $T\in \cT$ may vary strongly, volume, aspect ratio and orientation, but two \emph{neighboring} simplices should not be excessively different.
The intermediate set $\bT_{a,C}$ collects \emph{quasi-acute} meshes, which definition involves the measure of sliverness $S(T)$ of a simplex $T$ introduced in Chapter \ref{chapW1P} and also discussed in Chapter \ref{chapApproxMet}. 
The measure of sliverness plays an important role in the finite element approximation of a function on a mesh $\cT$ when the error is measured in the Sobolev $W^{1,p}$ norm.\\

We associate to each simplex $T$ a symmetric positive definite matrix $\cH_T$ such that the ellipsoid
$$
\cE_T := \{z\in \R^d \sep (z-z_T) \cH_T (z-z_T)^\trans \leq 1\},
$$
which is centered at the barycenter $z_T$ of $T$,
is the ellipsoid of minimal volume containing $T$. The properties of the matrix $\cH_T$ are discussed in \S \ref{subsecIntroSimplex} of this introduction,  as well as its explicit expression in terms of the coordinates of the simplex $T$. The matrix $\cH_T\in S_d^+$ encodes the volume, the aspect ratio and the orientation (but not the angles) of the simplex $T$. Two triangles $T$ and their associated ellipses $\cE_T$ are illustrated on figure \ref{figET}.

\begin{figure}
\centering
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleAigu.pdf}
	\includegraphics[width = 4cm, height=1.5cm]{\pathPic/Triangles/TriangleObtus.pdf}
	\caption{Two triangles $T$ and their associated ellipse $\cE_T$.\label{figET}}
\end{figure}

A riemannian metric on $\R^d$ is a continuous map $H$ which associates to any $z\in \R^d$ a symmetric positive definite matrix $H(z)\in S_d^+$. We denote by $\bH = C^0(\R^d,S_d^+)$ the collection of riemannian metrics.
The following definition introduce a notion of equivalence between meshes and metrics
\begin{definition}
\label{defEqHT}
We say that a mesh $\cT\in \bT$ is $C_0$-equivalent to a given metric $H\in \bH$, where $C_0\geq 1$ is a fixed constant, if for all $T \in \cT$ and all $z\in T$ one has 
\be
\label{defEquiv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
\ee
We say that a collection of simplicial meshes $\bT_*\subset \bT$ is equivalent to a collection $H_*$ of metrics if there exists a uniform constant $C_0\geq 1$ such that the following holds:
\begin{itemize}
\item For any mesh $\cT\in \bT_*$ there exists a metric $H\in \bH_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\item For any metric $H\in \bH_*$ there exists a mesh $\cT\in \bT_*$ such that $\cT$ and $H$ are $C_0$ equivalent.
\end{itemize}
\end{definition}
Our main result (Theorem \ref{thEquiv}) states that when the constant $C$ is sufficiently large, and if dimension is $d=2$, the three classes of meshes $\bT_{i,C}\subset \bT_{a,C} \subset \bT_{g,C}$ are respectively equivalent to three classes of metrics
$$
\bH_i \subset \bH_a \subset \bH_g.
$$
that are defined by precise smoothness conditions on the function $z\mapsto H(z)$ in \S \ref{subsecDefHStar} of this introduction.
%Our main result Theorem \ref{thEquiv} states that when the parameter $C$ is large enough and the dimension is $d=2$, the collections $\bT_{\star,C}$ of triangulations are equivalent to the corresponding collections $H_\star$ of metrics for any symbol $\star \in \{i,a,g\}$. 
The most striking point of this result is that, although the matrix $\cH_T$ does not encode the angles of a simplex $T$, the fact that a mesh $\cT\in \bT_{a,C}$ is \emph{quasi-acute} can be translated in a precise regularity condition on the metric $H$ equivalent to $\cT$.

In order to state our results more precisely we need to introduce some notations. We first recall some notations of linear algebra. We denote by $\M_d$ the collection of $d\times d$ matrices with real entries. We denote by $\GL_d$ the standard linear group, by $\SL_d$ the special linear group and by $\cO_d$ the orthogonal group
\begin{eqnarray*}
\GL_d &:=& \{A\in \M_d\sep \det A\neq 0\}\\
\SL_d &:=& \{A\in \M_d\sep \det A=1\}\\
\cO_d &:=& \{U\in \M_d\sep U^\trans U = \Id\}.
\end{eqnarray*}
We denote by $S_d$ the collection of symmetric matrices, by $S_d^\oplus$ the subset of non-negative symmetric matrices, and by $S_d^+$ the collection of symmetric positive definite matrices.
\begin{eqnarray*}
S_d &:=& \{M\in \M_d\sep M = M^\trans\}\\
S_d^\oplus &:=& \{M\in S_d\sep z^\trans M z \geq 0 \text{ for all } z\in \R^d\}\\
S_d^+ &:=& S_d^\oplus \cap \GL_d.
\end{eqnarray*}
Let $M,M'\in S_d$, we write $M\leq M'$ if $M'-M\in S_d^\oplus$, and $M< M'$ if $M'-M\in S_d^+$. We recall that for any $M,M'\in S_d$ such that $M\leq M'$ and any $\phi\in \M_d$ we have $\phi^\trans M \phi \leq \phi^\trans M' \phi$. Furthermore if $M,M' \in S_d^+$ and $M\leq M'$ then $M'^{-1} \leq M^{-1}$. For each symmetric positive definite matrix $M\in S_d^+$ we define a norm $\|\cdot\|_M$ as follows: for all $u\in \R^d$
$$
\|u\|^2_M := u^\trans M u.
$$

\subsection{Geometry of the simplex}
\label{subsecIntroSimplex}
The basic geometrical object studied in this chapter is the $d$-dimensional simplex, which is defined as follows.
\begin{definition}
A $d$-dimensional simplex $T$ is the convex envelope of a set $V\subset \R^d$ of $d+1$ %non-coplanar 
vertices, not contained in a $d-1$ dimensional affine subspace of $\R^d$ : 
$$
T = \Cvx(V).
$$
We denote by $\cF(T)$ the collection of faces of $T$ of any dimension,
\be
\label{defFT}
\cF(T) := \{\Cvx(V') \sep V'\subset V\}.
\ee
\end{definition}
Observe that $\emptyset$ and $T$ are among the faces of a simplex $T$, since they respectively correspond to $V'=\emptyset$ and $V'=V$.
We denote by $z_T\in \R^d$ the barycenter of a simplex $T$ of vertices $V$
$$
z_T := \frac 1 {d+1} \sum_{v\in V} v,
$$
and we define a symmetric positive definite matrix $\cH_T\in S_d^+$ as follows
\be
\label{defcH}
\cH_T^{-1} = \frac d {d+1} \sum_{v\in V} (v-z_T) (v-z_T)^\trans. %\frac {2d}{(d+1)^2}\sum_{v,v'\in V} (v-v')(v-v')^\trans. 
\ee
Some of the key properties of the matrix $\cH_T$ are exposed in the next proposition.
Throughout this chapter, we denote by $\TEq$ a $d$-dimensional equilateral simplex, centered at the origin
i.e. such that $z_\TEq=0$, and having its vertices on the unit ball. One easily checks that 
$$
\cH_\TEq = \Id.
$$
% Note that 
%\be
%\label{eqBallTEq}
%%\{z\in \R^d \sep |z| \leq 1/d\} 
%B(0, 1/d) \subset \TEq \subset \overline B(0,1).
%\ee
%
%%We associate to any simplex $T$ its barycenter $z_T\in \R^d$, and a symmetric positive definite matrix
%We denote by $z_T$ the barycenter of a simplex $T$, and we also associate to $T$ a symmetric positive definite matrix $\cH_T\in S_d^+$ which encodes some of its geometrical properties, in particular the volume, the elongation and the orientation of $T$.
\begin{prop}
\label{propHT}
The following holds for any $d$-dimensional simplex $T$. 
\begin{itemize}
\item
For any an affine change of coordinates $\Phi$, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0$ in $\R^d$, we have 
\be
\label{invcH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
\item
There exists a rotation $U\in \cO_d$, depending on $T$, such that 
\be
\label{eqcHTEq}
\cH_T^\frac 1 2 (T-z_T) = U(\TEq),
\ee
hence 
\be
\label{eqVolTHT}
|T| \sqrt{\det \cH_T} = |\TEq|.
\ee
\item
We have the inclusions 
\be
\label{eqTET}
\{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1/d\} \subset T \subset \cE_T := \{z\in \R^d \sep \|z-z_T\|_{\cH_T}\leq 1\},
\ee
and the these two ellipsoids are respectively the one of largest volume included in $T$, and of smallest volume containing $T$.
\end{itemize}
\end{prop}
\proof
For any simplex $\Phi^{-1}(v)$ of the simplex $\Phi^{-1}(T)$, we have 
$$
\Phi^{-1}(v)-z_{\Phi^{-1}(T)} = \Phi^{-1}(v)-\Phi^{-1}(z_T) = \phi^{-1}(v-z_T).
$$
Injecting this relation in \iref{defcH} we obtain \iref{invcH}. 
We now turn to the proof of \iref{eqcHTEq} and for that purpose we remark that the simplices $\TEq$ and $T' := \cH_T^\frac 1 2 (T-z_T)$ have both their barycenter at zero, $z_\TEq = z_{T'} = 0$, hence there exists a linear map $\phi\in \GL_d$ such that $T' = \phi^{-1}(\TEq)$. We thus obtain, using the formula \iref{invcH} for the transformation of $\cH_T$ under affine change of coordinates 
$$
\begin{array}{ccccc}
\cH_{T'} &=& \cH_T^{-\frac 1 2} \cH_T \cH_T^{-\frac 1 2} &=& \Id \\ 
\cH_{\phi^{-1}(\TEq)} &=& \phi^\trans \cH_\TEq &=& \phi^\trans \phi.
\end{array}
$$
Hence $\phi^\trans \phi= \Id$ which establishes that $\phi\in \cO_d$ and concludes the proof of \iref{eqcHTEq}.
%One easily checks that 
%$$
%\overline B(0,1/d) \subset \TEq \subset \overline B(0,1),
%$$
%where
It is well known that the smallest ellipsoid containing $\TEq$ is the unit ball, and that the largest ellipsoid included in $\TEq$ is the ball of radius $1/d$. Combining this fact with the change of coordinates \iref{eqcHTEq} we obtain \iref{eqTET} which concludes the proof of this proposition.
\sq

Note that for any simplex $T$ and any $z,z'\in T$ we obtain using \iref{eqTET}
\be
\label{eqDiamTHT}
\|z-z'\|_{\cH_T} \leq \|z-z_T\|_{\cH_T} + \|z'-z_T\|_{\cH_T} \leq 1+1= 2.
\ee

We introduce a measure of degeneracy $\rho(T)$ of a $d$-dimensional simplex $T$
\be
\label{defRhoMM}
\rho(T) := \sqrt{\|\cH_T\| \|\cH_T^{-1}\|}.
\ee
%This measure of non degeneracy $\rho$ is slightly different from the measure of non degeneracy $\frac {\diam(T)^d} {|T|}$ used in some of the previous chapters. However these two measures play a similar role and can be compared. Indeed we obtain using \iref{eqVolTHT} and \iref{eqcTET}
%\be
%\label{eqRhoRhop}
%\frac{\rho(T)}{d^\frac d 2|\TEq|} \leq  \frac{(\|\cH_T^{-1}\|/d)^\frac d 2} {|\TEq| (\det \cH_T)^{-\frac 1 2}} \leq \frac{\diam(T)^d} {|T|} \leq \frac{\|\cH_T^{-1}\|^\frac d 2} {|\TEq|(\det \cH_T)^{-\frac 1 2}}\leq \frac{\rho(T)^{d-1}}{|\TEq|}.
%\ee
%Observing that $\|A\| \|A^{-1}\|^{-(d-1)} \leq |\det A| \leq \|A\|^{d-1} \|A^{-1}\|^{-1}$ for any $A\in \GL_d$
%it follows that 
Observe that $\rho(T)\geq 1$ for any simplex $T$, with equality if and only if $\cH_T$ is proportional to the identity, which implies in view of \iref{eqcHTEq} that $T$ is a displacement of the equilateral simplex $\TEq$:
$$
\rho(T) = 1 \stext{ if and only if }
%\ \Longleftrightarrow \ 
T = z_T+r U(\TEq) \text{ for some }  r>0 \text{ and } U \in \cO_d.
$$
The measure of degeneracy $\rho$ is slightly different from the measure of degeneracy $\frac {\diam(T)^d} {|T|}$ used in Chapters \ref{chapOptAniso} and \ref{chapW1P} but both have the same role: they are minimal for the equilateral simplex, and increase as the simplex becomes thinner.\\

The measure of sliverness $S(T)$ of a simplex $T$ is a quantity which plays an important role in the context of optimal mesh adaptation for the finite element approximation of a function in the Sobolev $W^{1,p}$ norm, see   \cite{Ba, Ja}, and Chapters \ref{chapW1P} and \ref{chapApproxMet}. 
This measure of sliverness is defined in Chapter \ref{chapW1P} and illustrated by several examples and equivalent quantities. We recall the definition of this quantity
\be
\label{defSMM}
S(T) := \inf \{ \|\phi\| \|\phi^{-1}\| \sep \phi \in \GL_d \text{ and } \phi(T) \text{ is acute } \},
\ee
a simplex is acute if the exterior normals $\n, \n'$ to any two distinct faces of $T$ have a negative scalar product $\<\n,\n'\>\leq 0$.
As observed in Chapter \ref{chapW1P}, the measure of sliverness $S(T)$ can be interpreted as the distance from $T$ to the collection of acute simplices.

The exterior normals $\n,\n'$ to any two $d-1$-dimensional faces of $\TEq$ satisfy $\<\n,\n'\> =-1/d$, hence this simplex is acute. Recalling \iref{eqcHTEq}
 we thus obtain for any simplex $T$
$$
S(T) \leq \rho(T).
$$
Apart from this upper bound, the matrix $\cH_T$ does not contain any direct information on the measure of sliverness $S(T)$.
%One of the key results of this chapter is that in a bidimensional triangulation $\cT$, and conjecturedly in higher dimension too, the variation of the matrix $\cH_T$ as $T$ varies in $\cT$ does encode the measure of sliverness in some sense.
For any bidimensional triangle $T$ of largest angle $\theta$, Proposition \ref{propSTan} of Chapter \ref{chapW1P} states that :
$$
S(T) = \max\left\{1, \tan \frac \theta 2 \right\}.
$$

\subsection{Simplicial meshes}
\label{subsecDefTStar}

As a starter, we recall the definition of a simplicial mesh of $\R^d$.
%We first briefly recall the defini
%Before introducing simplicial meshes, we briefly recall the definition of locally finite partitions of $\R^d$.

%In order to introduce q,xcl meshes 
\begin{definition}
\label{defSimplMesh}
A conforming simplicial mesh of $\R^d$ is a collection $\cT$ of simplices which satisfy the conformity axiom :  for all $T,T'\in \cT$
\be
\label{confAxiom}
T\cap T' \in \cF(T) \cap \cF(T'),
\ee
as well as the following properties
\begin{itemize}
\item (Covering) The simplices $T\in \cT$ cover the whole infinite domain $\R^d$:
$$
\bigcup_{T\in \cT} T = \R^d.
$$
\item (Partition) The interiors of the simplices $T\in \cT$ are pairwise disjoint: for any $T,T'\in \cT$,
$$
\interior (T) \cap \interior(T') \neq \emptyset\stext{ implies }  T=T'. %
$$
\item (Local finiteness) For any compact set $K \subset \R^d$, only a finite collection of simplices $T\in \cT$ intersect $K$:
$$
\{T \in \cQ \sep K \cap T \neq \emptyset \} \ \text{ is finite.}
$$
\end{itemize}
\end{definition}
The conformity axiom \iref{confAxiom} states that the intersection of any two simplices in $\cT$ needs to be a full common face.We denote by $\bT$ the collection of conforming simplicial meshes of $\R^d$.

For an optimal efficiency, numerous numerical simulation software use anisotropic meshes, in which the simplices may have an arbitrary shape. Anisotropic meshes are used for instance, to create a thin layer of simplices close to a geometric feature which is relevant in a numerical simulation.
In order to avoid excessively wild meshes, one often requires relevant  some consistency between the shapes of neighboring simplices.We therefore introduce for any constant $C \geq 1$ the class $\bT_{g,C} \subset \bT$ of \emph{graded} meshes, which is defined as follows.
A mesh $\cT$ belongs to $\bT_{g,C}$ if for any two simplices $T,T'\in \cT$ one has 
\be
\label{defTG}
T \cap T'\neq \emptyset \stext{ implies } C^{-2}\cH_T \leq \cH_{T'} \leq C^2 \cH_T.
\ee

For any $C\geq 1$ we also introduce the class $\bT_{i,C}$ of \emph{isotropic} meshes, by requiring that in addition to \iref{defTG} that the measure of degeneracy $\rho$ is uniformly bounded by $C$, which forbids any anisotropy.
A mesh $\cT$ belongs to $\bT_{i,C}$ if and only if $\cT\in \bT_{g,C}$ and for all $T \in \cT$
$$
\rho(T) \leq C. %C \geq 1? or 0? 
$$

%The next proposition shows that the definition of $\bT_{i,C}$ is slightly redundant, in the sense that condition \iref{defTG} could be avoided.
%\begin{prop}
%Denote by $\bT'_{i,C}$ the collection of meshes $\cT\in \bT$ satisfying $\rho(T) \leq C$ for all $T\in \cT$ (but perhaps not the gradedness condition \iref{defTG}). %We thus have $\bT_{i,C} \subset \bT'_{i,C}$.\\
%Then for all $C$ there exists $C' = C'(C)$ such that 
%$$
%\bT_{i,C} \subset \bT'_{i,C} \subset \bT_{i,C'}.
%$$
%\end{prop}
%
%\proof
%See appendix. 
%\sq

In order to introduce the intermediate collection $\bT_{a,C}$ of $C$-quasi-acute meshes, we first define the notion of refinement of a simplicial mesh.
\begin{definition}
Consider two meshes $\cT,\cT'\in \bT$ and a constant $C\geq 1$. We say that $\cT'$ is a $C$-refinement of $\cT$ if it satisfies the following properties.
\begin{itemize}
\item (Inclusion) Any simplex $T'\in \cT'$ is contained in a simplex $T\in \cT$. % such that $T'\subset T$.
\item (Bounded refinement) Any simplex  $T\in \cT$, contains most $C$ simplices $T'\in \cT$.
\end{itemize}
\end{definition}

A graded mesh $\cT \in \bT_{g,C}$ belongs to the collection $\bT_{a,C}$ of quasi-acute meshes if and only there exists a $C$-refinement $\cT'$ of $\cT$ which satisfies for all $T' \in \cT'$
$$
S(T') \leq C.
$$
In particular if $\cT\in \bT_{i,C}$, then choosing $\cT' = \cT$, which is a $C$-refinement since $C\geq 1$, and recalling that $S(T) \leq \rho(T)$ for any simplex $T$, we obtain that $\cT\in \bT_{a,C}$. Thus $\bT_{i,C} \subset \bT_{a,C} \subset \bT_{g,C}$ as announced.

The constraints defining graded, quasi-acute and isotropic meshes are illustrated on Figure \ref{figDisk}
in the main introduction of the thesis. 
Figure \ref{figAcuteGen} gives an example of a quasi-acute triangulation which 
by the above described refinement process leads to a slightly finer triangulation on
sliverness $S(T)$ is uniformly bounded.

\begin{figure}
\centering
%	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarGdeVap.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap1.pdf}
	\includegraphics[height = 4.5cm, width = 6cm]{\pathPic/Maillages/VarPteVap2.pdf}
	\caption{\label{figAcuteGen}
Quasi-acute triangulation (left) and refined triangulation with uniformly bounded sliverness (right).
	}
\end{figure}

\subsection{Riemannian metrics}
\label{subsecDefHStar}

For any metric $H \in \bH$ and path $\gamma \in C^1([a,b],\R^d)$, we define the riemmannian length $l_H(\gamma)$ by the integral
$$
l_H(\gamma) := \int_a^b \|\gamma'\|_{H(\gamma(t))} dt.
$$
The riemmannian distance $d_H$ between two points  $z,z'\in \R^d$, is the infimum of the length of all paths joining $z$ and $z'$, 
\be
\label{defdH}
d_H(z,z') := \inf\left\{l_H(\gamma)\sep \gamma\in C^1\left([0,1],\R^d\right), \ \gamma(0) = z \text{ and } \gamma(1) = z'\right\}.
\ee
If $H, H'\in \bH$ are such that $H(z) \leq H'(z)$ for all $z\in \R^d$, then $d_H(z,z') \leq d_{H'}(z,z')$ for all $z,z'\in \R^d$.
By construction, the riemannian distance $d_H$ associated to a metric $H\in \bH$ is locally equivalent close to a point $z$ to the distance defined by the norm $\|\cdot \|_{H(z)}$: for all $z\in \R^d$
\be
\label{eqDistLoc}
\limsup_{\ve \to 0} \sup_{p,q\in B(z, \ve)} |\ln d_H(p,q) - \ln \|p-q\|_{H(z)}| = 0,
\ee
where $B(z,\ve)$ denotes the euclidean ball of radius $\ve$ around $z$.\\


\begin{remark}[Riemannian geodesics]
When a metric $H$ is sufficiently smooth, a special family of curves named Riemannian geodesics can be defined and studied. A riemannian geodesic is a curve $\gamma\in C^0(\R, \R^d)$ which satisfies a second order differential equation %written in terms of the second order derivatives of $H$, 
called the equation of geodesics. This equation implies that for any sufficiently close $t,t'\in \R$ the curve $\gamma_{|[t,t']}$ is the path of smallest possible length joining the points $\gamma(t)$ and $\gamma(t')$ : 
$d_H(\gamma(t), \gamma(t')) = l_H(\gamma_{|[t,t']})$.

Geodesics are not defined for general continuous or Lipschitz riemannian metrics, such as those constituting the sets $\bH$ and $\bH_i \subset \bH_a\subset \bH_g$, since the coefficients of the equation of geodesics involve the second derivatives of the metric. Notions related to geodesics, such as the injectivity radius of a metric, therefore have no meaning in our context.
This is not an issue for our purposes since, following the point of view of \cite{Gromov},
%[Gromov, Metric structures for Riemannian and non-Riemannian spaces, Birkhauser (1999)]
we study Riemannian distances and not Riemannian geodesics. 

%Note also that geodesics only exist when the metric $H$ has requires that $H$ has at least $C^2$ smoothness, while the metrics studied in this chapter generally only have $C^0$ or Lipschitz smoothness.

%Since we only assume that $H$ is a continuous metric, the infimum \iref{defdH} may or may not be attained, and in that later case possibly for several paths. The equation of geodesics associated to a riemannian metric involves the second order derivatives, which are not defined in our context.
%(* also the point of view of Gromov : we study distances and not geodesics*)
\end{remark}


We denote by $\bH_i$ the collection of metrics $H \in \bH$ which are proportionnal to the identity: for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2},
$$
and such that the proportionality factor $s$ satisfies one of the two following conditions conditions, which are surprisingly equivalent as shown in Proposition \ref{propEquivS}:
\begin{itemize}
\item (``Additive'' Lipschitz condition)  
\be
\label{eqLipSAdd}
|s(z) - s(z')| \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
\item (``Multiplicative'' Lipschitz condition)
\be
\label{eqLipSMult}
|\ln s(z) - \ln s(z')| \leq d_H(z,z') \stext{ for all } z,z'\in\R^d.
\ee
\end{itemize}

The two Lipschitz properties \iref{eqLipSAdd} and \iref{eqLipSMult} have a natural generalisation to general anisotropic metrics but are not equivalent in that context.
In order to introduce the regularity conditions defining the classes $\bH_i\subset \bH_a\subset \bH_g$ of metrics, we need to  two distances $d_\times$ and $d_+$ on the set $S_d^+$ of symmetric positive definite matrices. 
For any $M,M'\in S_d^+$ we define
\be
\label{defDTimes}
d_\times (M,M') := \min \{\delta \geq 0 \sep e^{-2\delta} M \leq M' \leq e^{2 \delta} M\}.
\ee
For instance, a mesh $\cT$ is $C$-equivalent to a metric $H$, as defined in \iref{defEquiv}, if and only if for all $T \in \cT$ and all $z\in \cT$ one has 
$$
d_\times (H(z), \cH_T) \leq \ln C.
$$
There exists various expressions of the distance $d_\times$ : for all $M,M'\in S_d^+$ one easily checks that  
\be
\label{eqDTimesLog}
\begin{array}{rcl}
d_\times (M,M') &=& \displaystyle\sup_{u\in \sR^d\sm \{0\}} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|\vspace{2mm}\\
&=&\displaystyle \sup_{|u|=1} \left|\ln \|u\|_M - \ln \|u\|_{M'}\right|
\end{array}
\ee
and 
\be
\label{eqDTimesProd}
d_\times (M,M') = \ln \left(\max \{\|M^{-\frac 1 2} M'^{\frac 1 2}\|, \, \|M'^{-\frac 1 2} M^\frac 1 2\|\}\right).
\ee
This last expression implies that 
\be
\label{eqDTimesDiffLog}
d_\times (M,M') \geq \frac 1 2 \max\{ |\ln \|M\|-\ln\|M'\| |, \, |\ln \|M^{-1}\| - \ln \|M'^{-1}\| | \}
\ee
The exponential of the distance $d_\times$ was used in the earlier paper \cite{Shew} %on anisotropic mesh generation
under the name ``relative deformation''. 
We define a second distance $d_+$ on $S_d^+$ as follows 
\be
\label{defDPlus}
d_+(M,M') := \|M^{-\frac 1 2} - M'^{-\frac 1 2}\|.
\ee
The expressions \iref{eqDTimesProd} and \iref{defDPlus} of the distances $d_\times$ and $d_+$ show that they are respectively tied to multiplicative or additive properties of matrices, which justifies their notations.
Note also that for any $s,s'>0$ one has
\be
\label{eqDIso}
d_\times (s^{-2} \Id, s'^{-2} \Id) = |\ln s - \ln s'| \stext{ and } d_+(s^{-2} \Id, s'^{-2} \Id) = |s-s'|.\\
\ee

We denote by $\bH_g$ the collection of metrics $H\in \bH$ which satisfy the natural extension of \iref{eqLipSMult} to general anisotropic metrics:
\be
\label{eqLipMult}
d_\times (H(z), H(z')) \leq d_H(z,z') \stext{ for all }z,z'\in\R^d.
\ee
This condition can be heuristically described as follows: a metric $H\in \bH$ defines close to each point $z\in\R^d$ a norm $\|\cdot\|_{H(z)}$ which encodes an anisotropic notion of scale. The equation \iref{eqLipMult} states that the metric $H$ itself is consistent a the scale that it encodes.\\

We denote by $\bH_a$ the collection of metrics $H\in \bH$ which satisfy both \iref{eqLipMult} and the natural extension of \iref{eqLipSAdd} to general anisotropic metrics:
\be
\label{eqLipAdd}
d_+ (H(z), H(z')) \leq |z-z'| \stext{ for all }z,z'\in\R^d.
\ee
In addition to the results of mesh generation presented in this chapter, we show in the next chapter, Chapter\ref{chapApproxMet}, that this condition is critical in order to define a local averaging operator compatible with Sobolev norms. 
%decrire le lien avec les angles aigus.
\begin{remark}
\label{remHomog}
Let $H\in \bH$, and let $\lambda>0$. Using the homogeneity properties of the distances $d_\times$, $d_+$ on $S_d^+$ and $d_H$ on $\R^d$ with respect to $H$, we obtain that $\lambda^2 H\in \bH_g$ if and only if 
\be
\label{eqLipTimesLambda}
d_\times (H(z), H(z')) \leq \lambda d_H(z,z') \stext{ for all } z,z'\in \R^d, 
\ee
and $\lambda^2 H\in \bH_a$ if and only if we have in addition to the previous property 
\be
\label{eqLipPlusLambda}
d_+ (H(z), H(z')) \leq \lambda |z-z'| \stext{ for all } z,z'\in \R^d.
\ee
In particular the collections $\bH_i \subset \bH_a \subset \bH_g$ of isotropic, quasi-acute and graded metrics are stable under multiplication by a constant larger than one : for any $\star \in \{a,b,c\}$, any $H\in \bH_\star$ and any $\lambda \geq 1$ we have $\lambda^2 H\in \bH_\star$.
%this operation corresponds to the uniform refinement of a triangulation...
\end{remark}

\subsection{Main results}

The main result of this chapter is the equivalence of the classes of meshes and metrics defined above, which is  announced in the first part of the introduction and proved in sections \S\ref{secMeshToMet} and  \S \ref{secMetToMesh}. In two cases we were only able to establish this equivalence when the dimension is $d=2$. 
\begin{theorem}
\label{thEquiv}
There exists $C_0 = C_0(d)$ such that for all $C\geq C_0$ the following holds.
\begin{enumerate}[i)]
\item The collections $\bT_{i,C}$ of triangulations and $\bH_i$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{a,C}$ of triangulations and $\bH_a$ of metrics are equivalent.
\item If $d=2$, then the collections $\bT_{g,C}$ of triangulations and $\bH_g$ of metrics are equivalent.
\end{enumerate}
\end{theorem}

Let us comment on this result.
The theory of isotropic meshes is already well developed, and our result i) in this direction should be regarded as a reformulation of previous work, intended to put into perspective the results on anisotropic meshes. The main ingredient of the proof of i) is the mesh refinement procedure exposed in \cite{Nochetto}. 

In the case iii) of graded metrics the key ingredients used for the construction of a bidimensional triangulation $\cT\in \bT_{g,C}$ equivalent to a metric $H \in \bH_g$ come from the paper of computational geometry \cite{Shew}. In contrast the arguments used to produce a metric $H \in \bH_g$ from a mesh $\cT \in \bH_{g,C}$ hold in any dimension.

Last the author has not heard of any anterior results on the collection $\bT_{a,C}$ of quasi-acute meshes, and most of the techniques used in that context are new. 
The author is sorry to say that the proofs in that case are not yet as polished as the rest of the thesis, due to time constraints.

\begin{conjecture}
The author conjectures that the points ii) and iii) of Theorem \ref{thEquiv} holds without restriction on the dimension $d$.
\end{conjecture}

This chapter is organised as follows. We establish in section \S \ref{secMetProp} some general properties of metrics in $\bH_a$ or $\bH_g$. 
We first prove in \S\ref{subsecMetInv} a property of invariance of the collection $\bH_g$ of graded metrics with respect to affine changes of coordinates.
The regularity assumptions \iref{eqLipMult} and \iref{eqLipAdd} defining graded and quasi-acute metrics simply mean that the map $H : \R^d \to S_d^+$ is Lipschitz with respect to some distances on $\R^d$ and $S_d^+$. 
We therefore study metrics from this point of view in \S\ref{subsecMetLip}.
We focus in \S\ref{subsecMetGeom} on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. In particular we compare the $d_H$ with the euclidean distance and we estimate the volume of balls. 


Section \S\ref{secEigen} is devoted to the study of metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has  an eigenspace of dimension at least $d-1$ at each point. This condition clearly holds if the dimension is $d=2$ but is also relevant in some applications to higher dimension such as the creation of a this layer of simplices close to a $d-1$ dimensional surface. This situation is discussed in Chapter \ref{chapApproxMet}, and involves metric which have an eigenvalue much larger that the others in the orthogonal direction to the surface of interest.
We give an approximate translation of the regularity properties \iref{eqLipAdd} and \iref{eqLipMult} defining the collections $\bH_a$ and $\bH_g$ of metrics in terms of the two eigenvalues of $H$ and of the direction of the eigenspaces of such metrics. 

The last two sections \S\ref{secMeshToMet} and \S\ref{secMetToMesh} are devoted to the proof of Theorem \ref{thEquiv}. More precisely we adress in \S\ref{secMetToMesh} the production of an isotropic, quasi-acute or graded mesh equivalent to a given metric $H\in \bH_i$, $\bH_a$ or $\bH_g$. Conversely we depict in \S\ref{secMeshToMet} to construction of a metric which is equivalent to a given mesh.


\section{General properties of graded and quasi-acute metrics}
\label{secMetProp}

We study in this section the general properties of the  distinguished classes of metrics $\bH_i \subset \bH_a \subset \bH_g$. 
We first establish in \S\ref{subsecMetInv} some invariance properties of these collections of metrics with respect to affine changes of coordinates.
We then regard in \S\ref{subsecMetLip} metrics as Lipschitz functions $H : \R^d\to S_d^+$. %, and we recall some basic properties of these.
The last subsection \S\ref{subsecMetGeom} is devoted to the comparison of the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$, with respect to the standard euclidean distance and Lebesgue measure.

\subsection{Invariance properties and restriction of metrics}
\label{subsecMetInv}

We focus in this subsection on the properties of invariance of the collections of meshes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ and of metrics $\bH_i \subset \bH_a\subset \bH_g$ introduced in this chapter.

Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$.
We have for any simplex $T$, as previously observed in \iref{invcH},
\be
\label{eqInvH}
\cH_{\Phi^{-1}(T)} = \phi^\trans \cH_T \phi.
\ee
Mimicking this property we define for any $H \in \bH$ a transported version $H_\Phi\in \bH$ as follows: for all $z\in \R^d$
\be
\label{defHPhi}
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi.
\ee
In the language of differential geometry,
the metric $H_\Phi$ is generally referred to as the ``pull back'' of $H$ by $\Phi$. If a mesh $\cT\in \bT$ is $C$-equivalent to a metric $H\in \bH$, then \iref{eqInvH} and \iref{defHPhi} clearly imply that the mesh $\Phi^{-1}(\cT)$ is $C$-equivalent to the metric $H_\Phi$.

The next proposition studies the invariance of the collections $\bT_{\star,C}$ of meshes and $\bT_\star$ of metrics, $\star \in \{i,a,g\}$, under the transformations $\cT \mapsto \Phi^{-1}(\cT)$ or $H \mapsto H_\Phi$ induced by an affine change of coordinates $\Phi$.

\begin{prop}
\label{propInvT}
Let $\Phi : \R^d \to \R^d$ be an affine change of coordinates, $\Phi(z) := \phi z+z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. 
The following holds for any constant $C\geq 1$.
\begin{enumerate}[i)]
\item If $\cT \in \bT_{g,C}$ then $\Phi^{-1}(\cT) \in \bT_{g,C}$. If $H \in \bH_g$ then $H_\Phi\in \bH_g$.
\item Assume that $\Phi$ is an isometry, in other words $\phi\in \cO_d$.\\
If $\cT\in \bT_{a,C}$ then $\Phi^{-1}(\cT)\in \bT_{a,C}$, and similarly if $\cT\in \bT_{i,C}$ then $\Phi^{-1}(\cT)\in \bT_{i,C}$.\\
If $H\in \bH_a$ then $H_\Phi\in \bH_a$, and similarly if $H\in \bH_i$ then $H_\Phi\in \bH_i$.
\end{enumerate}
\end{prop}

\proof
%We concentrate on the case of meshes, since the statements on metrics are a special case of the propositions (??) and (??) below (* no : state the result for iso and quasi acute metrics too*).
%We first consider the case of meshes, and then 
We first establish the properties announced for meshes, and we then focus on metrics.
Let $M,M'\in S_d^+$, let $C\geq 1$ and let $\phi\in \GL_d$. Clearly
$$
\text{ if } C^{-2} M \leq M' \leq C^2 M \stext{ then } C^{-2} \phi^\trans M\phi \leq \phi^\trans M'\phi  \leq C^2 \phi^\trans M\phi.
$$
%Consequently if a mesh $\cT$ satisfies the condition \iref{defTG} defining the elements of $\bT_{g,C}$
%
%satisfy $C^{-2} M \leq M' \leq C^2 M$, then we also ha
%For any $M,M'\in S_d^+$ we obtain using \iref{defDTimes} that 
%$$
%d_\times (\phi^\trans M \phi,\ \phi^\trans M' \phi) = d_\times (M,M').
%$$
%It follows using \iref{eqInvH} that for any  two simplices $T,T'$,
%$$
%d_\times (\cH_{\Phi^{-1}(T)}, \cH_{\Phi^{-1}(T')}) = d_\times (\cH_T,\cH_{T'}).
%$$ 
In view of the definition \iref{defTG} of $\bT_{g,C}$ we obtain that $\Phi^{-1}(\cT)\in \bT_{g,C}$ for any mesh $\cT\in\bT_{g,C}$ as announced in i).

If $\Phi$ is an isometry then for any simplex $T$ we obtain, using the definitions \iref{defRhoMM} and \iref{defSMM} of the measure of degeneracy $\rho$ and the measure of sliverness $S$, that
$$
\rho(\Phi^{-1}(T)) = \rho(T) \stext{ and } S(\Phi^{-1}(T)) = S(T).
$$
This implies the properties of $\bT_{a,C}$ and $\bT_{i,C}$ announced in b), which concludes the proof of the properties announced for meshes.

We therefore turn our attention to metrics. The fact that $H_\Phi\in \bH_g$ for any $H\in \bH_g$ and any affine change of coordinates $\Phi$ is a special case of Proposition \ref{propHG} below. We thus admit this property and we focus on isotropic and quasi-acute metrics and \emph{isometric} changes of coordinates.

If $H\in \bH_i$, then $H = \Id/s(z)^2$ where $s: \R^d \to \R_+^*$ is a Lipschitz function. Since $\phi\in \cO^d$ we have $\phi^\trans \phi = \Id$ and therefore 
$$
H_\Phi(z) = \phi^\trans H(\Phi(z)) \phi = \Id/s(\Phi(z))^2.
$$
The map $s \circ \Phi : \R_d\to \R_+^*$ is Lipschitz since it is the composition of a Lipschitz function with an isometry, which establishes that $H_\Phi\in \bH_i$ as announced.

Since $\phi\in \cO_d$ we have for any symmetric matrix $M\in S_d^+$ and any exponent $\alpha\in \R$
$$
(\phi^\trans M \phi)^\alpha = \phi M^\alpha \phi.
$$
Consider $H\in \bH_a$, then for any $z,z'\in \R^d$
\begin{eqnarray*}
\|H_\Phi(z)^{-\frac 1 2}-H_\Phi(z')^{-\frac 1 2}\| &=& \|\phi^\trans \left(H(\Phi(z))^{-\frac 1 2}-H(\Phi(z'))^{-\frac 1 2}\right) \phi\| \\
&=& \|H(\Phi(z))^{-\frac 1 2}-H(\Phi(z'))^{-\frac 1 2}\|\\
& \leq& \|\Phi(z)-\Phi(z')\|\\
& =& \|\phi(z-z')\|= |z-z'|,
\end{eqnarray*}
which establishes that $H_\Phi$ satisfies the Lipschitz regularity condition \iref{eqLipAdd}. We already know from the case of graded metrics that the other regularity condition \iref{eqLipMult} is satisfied by $H_\Phi$, which establishes that $H_\Phi\in \bH_a$ and concludes the proof of this proposition.
\sq


In practical applications, one often needs to mesh simultaneously a domain $\Omega$ and a surface $\Gamma$ embedded in $\Omega$. In terms of metric this raises the following question: given a metric $H$ on $\Omega$ which satisfies certain properties of regularity %, corresponding do a certain class of meshes, 
what is the regularity of the restriction of this metric to $\Gamma$?

The next proposition answers this question is the simplified setting where $\Omega$ is the infinite domain $\R^d$, $\Gamma$ is an affine subspace of $\R^d$, and properties of regularity are those defining the collection $\bH_g$ of graded metrics. For any $1\leq k \leq d$ we denote by $\bH_g(\R^k)$ the collection of graded metrics on $\R^k$.

\begin{prop}
\label{propHG}
Let $1\leq k\leq d$, let $\Phi : \R^k\to \R^d$ be an affine injective map, $\Phi(z) = \phi z+z_0$ where $\phi\in M_{d,k}$ has rank $k$ and $z_0\in \R^d$. Let $H\in \bH$ and let for all $z\in \R^k$
$$%\be
%\label{defHPhi}
H_\Phi(z) := \phi^\trans H(\Phi(z)) \phi.
$$%\ee
If $H\in \bH_g$ then $H_\Phi\in \bH_g(\R^k)$. 
\end{prop}

\proof
For any $u\in \R^d$, one has 
\be
\label{chgNorm}
\|u\|_{H_\Phi(z)} = \|\phi(u)\|_{H(\Phi(z))}.
\ee
Hence for any $z,z'\in \R^k$ we obtain using \iref{eqDTimesLog},
\be
\label{dNHPhi}
\begin{array}{rcl}
d(H_\Phi(z), \ H_\Phi(z'))  &=&\displaystyle \sup_{u\in \sR^k\sm\{0\}} \left|\ln \left\|\phi(u)\right\|_{H(\Phi(z))} -\ln \left\|\phi(u)\right\|_{H(\Phi(z'))}\right| \\
& \leq& d(H(\Phi(z)), \  H(\Phi(z')))
\end{array}
\ee
For any path $\gamma\in C^1([0,1], \R^k)$, it follows from \iref{chgNorm} that % the distorted lengths tied to $H$ and $H_\phi$ are therefore linked by 
$$
l_H(\Phi\circ \gamma) = \int_0^1 \|\phi(\gamma'(t))\|_{H(\Phi(\gamma(t)))}dt =  l_{H_\Phi}(\gamma).
$$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^k)$ joining two points $z,z'\in \R^k$, we obtain since $\Phi\circ \gamma\in C^1([0,1], \R^d)$ is a path joining $\Phi(z)$ and $\Phi(z')$
\be
\label{dHPhi}
d_H(\Phi(z), \Phi(z')) \leq d_{H_\Phi}(z,z')
\ee
Combining \iref{dNHPhi} and \iref{dHPhi}, we conclude the proof of this proposition.
\sq


\subsection{Metrics as Lipschitz functions}
\label{subsecMetLip}
%Lipschitz functions play an important role in this chapter and in particular in this section. We recall here their basic properties.
Consider to abstract metric spaces $(X,d_X)$ and $(Y,d_Y)$ and a continuous function $f \in C^0(X , Y)$. We define 
the dilatation $\dil(f) \in [0, \infty]$ of $f$ as follows
$$
\dil(f) := \sup_{\substack{x,x'\in X \\ x \neq x'}} \frac{d_Y(f(x),f(x'))}{d_X(x,x')}
$$

We say that $f$ is Lipschitz if $\dil(f) \leq 1$, and more generally that $f$ is $\lambda$-Lipschitz if $\dil(f) \leq \lambda$.
We define the local dilatation $\dil_x(f)$ of a function $f\in C^0(X,Y)$ at a point $x\in X$ as follows
\be
\label{defDilX}
\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
\lim_{\ve\to 0} \left(\sup_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
\ee
%\be
%\label{defDilX}
%\dil_x(f) := \lim_{\ve\to 0} \dil \left(f_{|B(x,\ve)}\right) = 
%\lim_{\ve\to 0} \left(\sup_{e,e'\in B(x,\ve)} \frac{d_Y(f(e),f(e'))}{d_X(e,e')}\right).
%\ee
We specify the distance function on $X$ or $Y$ if it is not the expected ``canonical one'', for instance if $X$ or $Y$ is a subset of $\R^k$ and if the associated distance is not the standard euclidean distance but the riemannian distance $d_H$ associated to a metric, or if $X$ or $Y$ is the collection $S_d^+$ of symmetric positive definite matrices since none of the two distances $d_+$ or $d_\times$ is canonical. The local dilatation is in that case denoted as follows
$$
\dil_x(f\sep d_X, d_Y), \quad \dil_x(f\sep d_X)  \stext{ or } \dil_x(f\sep d_Y).
$$

The local dilatation $\dil_x(f)$ only depends on the local properties of the metric spaces close to $x$ and $f(x)$. Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$. For any $f\in C^0(\R^d, Y)$ and any $z\in \R^d$ we obtain using \iref{eqDistLoc}
\be
\label{eqDilNorm}
\|H(z)^{-1}\|^{-\frac 1 2} \dil_z(f) \leq \dil_z(f\sep d_H) = \dil_z(f \sep \|\cdot \|_{H(z)}) \leq \sqrt{\|H(z)\|} \dil_z(f)
\ee
We also introduce the lower local dilatation $\dil_z^*(f)\leq \dil_z(f)$ which is defined as follows
$$
\dil_z^*(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(x,\ve)} \frac{d_Y(f(q),f(q))}{d_X(p,q)}\right).
$$
The next proposition establishes that local dilatations are sub-multiplicative.
\begin{lemma}
\label{lemmaSubMult}
Let $(X,d_X)$, $(Y,d_Y)$ and $(Z,d_Z)$ be three metric spaces, and let $f\in C^0(X,Y)$ and $g\in C^0(Y,Z)$. 
For any $x\in X$ one has 
\be
\label{eqDilUpper1}
\dil_x(g \circ f) \leq \dil_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side. Similarly we have 
\be
\label{eqDilLower1}
\dil_x(g \circ f) \geq \dil^*_{f(x)}(g) \, \dil_x (f),
\ee
provided no indeterminate product $0\times \infty$ or $\infty \times 0$ appears in the right hand side.
\end{lemma}

\proof
We first establish \iref{eqDilUpper1}.
If $\dil_x(f) = \infty$ or $\dil_{f(x)}(g) = \infty$, then there is nothing to prove. We may therefore assume that $\dil_x(f) < \infty$ and $\dil_{f(x)}(g) < \infty$.
For any $\ve>0$ we define 
$$
F(\ve) = \sup_{p,q\in B(x, \ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)} \stext{ and } G(\ve) := \sup_{p,q\in B(f(x), \ve)} \frac{d_Z(g(p),g(q))}{d_Y(p,q)}
$$
It follows that 
$$
\sup_{p,q\in B(x, \ve)} \frac{d_Z(g(f(p)),g(f(q)))}{d_X(p,q)} \leq F(\ve) \, G(F(\ve) \ve).
$$
Taking the limit as $\ve \to 0$ we obtain \iref{eqDilUpper1} which concludes the proof.
For the proof of \iref{eqDilLower1} we consider two sequences $(p_n)_{n \geq 0}$, $(q_n)_{n \geq 0}$ which both tend to $x$ and such that $d_Y(f(p_n),f(q_n))/d_X(p_n, q_n) \to \dil_x(f)$ as $n \to \infty$. We thus have 
$$
\frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_X(p_n,q_n)} = \frac{d_Z(g(f(p_n)),g(f(q_n)))}{d_Y(f(p_n),f(q_n))} \times \frac{d_Y(f(p_n),g(f(q_n)))}{d_X(p_n,q_n)},
$$
and taking the limit as $n \to \infty$ we obtain \iref{eqDilLower1} which concludes the proof of this lemma.
\sq

Let $f: \Omega \to V$ be a $C^1$ function, where $\Omega\subset \R^d$ is an open set and $V$ is a Banach space. Then for any $z\in \Omega$ the local dilatation $\dil_z(f)$, and the lower dilatation $\dil_z^*(f)$ have an explicit expression in terms of the differential $d_z f : \R^d \to V$ of $f$ at $z$
\be
\label{eqDilDiff}
\dil_z(f) = \sup_{|u|=1} \|d_z f(u)\| \stext{ and } \dil_z^*(f) = \inf_{|u|=1} \|d_z f(u)\|
\ee
Applying Lemma \ref{lemmaSubMult} and \iref{eqDilDiff} to the function $g=\ln$ we obtain for any metric space $(X,d_X)$, any $f\in C^0(X,\R_+^*)$ and any $x\in X$
\be
\label{eqDilLog}
\dil_x(\ln f) = \frac {\dil_x(f)} {f(x)} .
\ee

The following proposition shows that, under certain circumstances, the Lipschitz property is a local property.
\begin{prop}
\label{propDilLoc}
Consider the metric space $(\R^d, d_H)$, where $H \in \bH$ is a fixed riemannian metric, and an arbitrary metric space $(Y,d_Y)$.
For any $f\in C^0(\R^d, Y)$ and any path $\gamma\in C^1([0,1], \R^d)$, $\gamma(0) = z$, $\gamma(1) = z'$, one has
\be
\label{eqLipLocPath}
d_Y(f(z), f(z')) \leq l_H(\gamma) \sup_{0\leq t \leq 1} \dil_{\gamma(t)}(f\sep d_H).
\ee
It follows that %In particular 
\be
\label{eqDilLoc}
\dil(f\sep d_H) = \sup_{z\in \sR^d} \dil_z(f\sep d_H).
\ee
\end{prop}

\proof
%Consider $z,z'\in \R^d$, and a path $\gamma\in C^1([0,1],\R^d)$ such that $\gamma(0) = z$, $\gamma(1)=z'$ and $l_H(\gamma) \leq d_H(z,z')+\delta$ where $\delta>0$ is a constant that is devoted to tend to zero in the last step of the proof.
We equip the segment $[0,1]$ with the distance $d_\gamma$ defined for $0 \leq t\leq t'\leq 1$ by 
\be
\label{defDGamma}
d_\gamma(t,t') = d_\gamma(t',t) = l_H(\gamma_{|[t,t']}).
\ee
Note that for any $t\leq t_* \leq t'$ one has 
\be
\label{exactTri}
d_\gamma(t,t') = d_\gamma(t,t_*)+d_\gamma(t_*,t')
\ee
The map $\gamma : ([0,1], d_\gamma) \to (\R^d, d_H)$ is clearly Lipschitz.
It thus follows from Lemma \ref{lemmaSubMult} that $F := f\circ \gamma :[0,1] \to Y$ satisfies for all $t\in [0,1]$
$$
\dil_t(F) \leq \dil_{\gamma(t)}(f) \leq \lambda := \sup_{0\leq t'\leq 1} \dil_{\gamma(t')}(f).
$$
We assume that $\lambda<\infty$, otherwise there is nothing to prove, and we consider a fixed $\delta>0$. For each $t\in [0,1]$ there exists therefore an interval $V_t\subset [0,1]$ containing $t$, relatively open in $[0,1]$, and such that $F_{|V_t}$ is $(\lambda+\delta)$-Lipschitz. Since the segment $[0,1]$ is compact, there exists a finite set $I_0\subset [0,1]$ such that 
\be
\label{finiteCover01}
[0,1] = \bigcup_{t\in I_0} V_t.
\ee
Let $V,V'\subset [0,1]$ be two intersecting intervals, and assume that $F$ is $\lambda+\delta$ Lipschitz on $V$ and on $V'$. For any $t\in V$ and $t'\in V'$, there exists $t_*\in V\cap V'$ which satisfies $t\leq t_*\leq t'$ or $t\geq t_* \geq t'$. Recalling \iref{exactTri} we thus obtain  
\begin{eqnarray*}
d_Y(F(t),F(t')) &\leq& d_Y(F(t), F(t_*))+d_Y(F(t_*), F(t')) \\
&\leq& (\lambda+\delta) d_\gamma(t,t_*)+( \lambda+\delta)d_\gamma(t_*,t') \\
&=& (\lambda+\delta)d_\gamma(t,t').
\end{eqnarray*}
Thus $F$ is $\lambda+\delta$ Lipschitz on the interval $V\cup V'$. Since $[0,1]$ is covered by the finite collection of open intervals \iref{finiteCover01} on which $F$ is $\lambda+\delta$ Lipschitz, we obtain proceeding by induction that $F$ is $(\lambda+\delta)$-Lipshitz on $[0,1]$ and therefore 
$$
d_Y(f(z),f(z')) = d_Y(F(0),F(1))\leq (\lambda+\delta) d_\gamma(0,1) = (\lambda+\delta)l_H(\gamma). %\leq (\lambda+\delta)(d_H(z,z')+\delta).
$$
Letting $\delta\to 0$ we obtain \iref{eqLipLocPath}. Taking the infimum of \iref{eqLipLocPath} among all paths $\gamma\in C^1([0,1], \R^d)$ joining $z$ and $z'$ we obtain $d_Y(f(z),f(z')) \leq  \lambda d_H(z,z')$. Therefore $\dil(f\sep d_H) \leq \lambda$. Conversely we have $\dil_z(f\sep d_H) \leq \dil(f\sep d_H)$ for any $z\in \R^d$, which establishes \iref{eqDilLoc} and concludes the proof of this proposition.\sq

The next corollary shows that the global dilatation of a function is controlled by the local dilatation on $\R^d\sm \Gamma$, if $\Gamma$ is a \emph{sufficiently thin} set. For instance the skeleton $\cup_{T\in \cT} \partial T$ of a mesh $\cT\in \bT$.

\begin{corollary}
\label{corolLipNoGamma}
Let $\Gamma\subset \R^d$ be a set which has the following property : for any path $\gamma\in C^1([0,1], \R^d)$ there exists a sequence of paths $(\gamma_n)_{n \geq 0}$ which converges to $\gamma$ in $C^1$ norm and such that  $\{t\in [0,1]\sep \gamma_n(t) \in \Gamma\}$ is finite for each $n$.\\
Let $H\in \bH$, let $(Y,d_Y)$ be an arbitrary metric space, and met let $f\in C^0(\R^d, Y)$.
Then 
$$
\dil(f\sep d_H) = \sup_{z\in \R^d \sm \Gamma} \dil_z(f\sep d_H).
$$
\end{corollary}

\proof
We denote $\lambda := \sup_{z\in \R^d \sm \Gamma} \dil_z(f)$.
We consider two points $z,z'\in \R^d$ and a path $\gamma\in C^1([0,1], \R^d)$ such that $\gamma(0) = z$ and $\gamma(1) = z'$. %, and a sequence $\gamma_n$ converging to $\gamma$ in $C^1$ norm.

We first assume that the set $\{t\in [0,1]\sep \gamma(t) \in \Gamma\}$ is finite, and we denote its elements by $t_1< \cdots < t_k$. We set by convention $t_0 = 0$ and $t_{k+1} = 1$.
For each $0\leq i \leq k$ and each $t,t'$ such that $t_i <t<t'<t_{i+1}$ we have $d_Y(f(\gamma(t)),f(\gamma(t'))) \leq \lambda l_H(\gamma_{|[t,t']})$ according to Proposition \ref{propDilLoc}. Letting $t\to t_i$ and $t'\to t_{i+1}$ we obtain $d_Y(f(\gamma(t_i)),f(\gamma(t_{i+1}))) \leq \lambda l_H(\gamma_{|[t_i,t_{i+1}]})$. Adding up we obtain 
$$
d_Y(f(z), f(z')) \leq \sum_{0\leq i \leq  k} d_Y(f(\gamma(t_i)), f(\gamma(t_{i+1}))) \leq \lambda
\sum_{0\leq i \leq k} l_H(\gamma_{[t_i, t_{i+1}]}) = \lambda l_H(\gamma).
$$

We now consider the case where $\gamma$ meets the set $\Gamma$ an infinite number of times, and we choose a sequence $(\gamma_n)_{n \geq 0}$ as described is the statement of the corollary. We obtain $d_Y(f(\gamma_n(0)), f(\gamma_n(1))) \leq \lambda l_H(\gamma_n)$ for each $n\geq 0$. Taking the limit as $n \to \infty$ we obtain $d_Y(f(z), f(z')) \leq \lambda l_H(\gamma)$ since $\gamma_n$ converges to $\gamma$ is $C^1$ norm as $n \to \infty$.

Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ we obtain $d_Y(f(z), f(z')) \leq \lambda d_H(z,z')$, which concludes the proof of this proposition.
\sq


%Let $(Y, \|\cdot \|_Y)$ and $(Z, \|\cdot\|_Z)$ be two banach spaces. Let $y\in Y$, $g\in C^1(Y,Z)$, and $L = g'(f(x))$, then clearly 
%$$
%\dil_y(g) = \|L\|.
%$$
%Injecting this in \iref{eqDilUpper1} we obtain 
%\be
%\label{eqDilUpper2}
%\dil_x(g \circ f) \leq\|L\|  \dil_x (f).
%\ee
%We also need a lower bound in several cases. For that purpose we define 
%$$
%\dil^*_z(f) := \lim_{\ve \to 0} \left(\inf_{p,q\in B(z,\ve)} \frac{d_Y(f(p),f(q))}{d_X(p,q)}\right),
%$$
%and we obtain proceeding similarly, but with the different convention $0\times \infty = \infty\times 0 = 0$
%$$
%\dil_z(g\circ f) \geq \dil^*_{f(z)}(g) \dil_z(f).
%$$

The next proposition establishes that the regularity conditions \iref{eqLipMult} and \iref{eqLipAdd} defining the collections of quasi-acute or graded metrics are equivalent in the case of a metric proportionnal to the identity. %$\bH_a$ $\bH_g$

\begin{prop}
\label{propEquivS}
Let $s\in C^0(\R^d, \R_+^*)$ and let $H := \Id/s^2$. We have for all $z\in \R^d$
\be
\label{eqDilLnH}
\dil_z(\ln s\sep d_H) = \dil_z(s).
\ee
Furthermore the following properties are equivalent.
\begin{enumerate}
\item The map $s : \R^d \to \R$ is Lipschitz. (i.e. $H\in \bH_i$) %For all $z,z'\in \R^d$ one has $|s(z)-s(z')|\leq |z-z'|$.
\item (``Additive'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_+(H(z),H(z')) \leq |z-z'|$.
\item (``Multiplicative'' Lipschitz property) For all $z,z'\in \R^d$ one has $d_\times(H(z),H(z'))\leq d_H(z,z')$.
\end{enumerate}
\end{prop}

\proof %reprendre preuve??
Combining \iref{eqDilNorm} and \iref{eqDilLog} we obtain for any $z\in \R^d$
$$
%\dil_z (H\sep  d_\times, d_H) = 
\dil_z(\ln s\sep d_H) = s(z) \dil_z(\ln s) = \dil_z(s),
$$
which establishes \iref{eqDilLnH}.
According to \iref{eqDIso} we have for any $z,z'\in \R^d$
$$
d_+(H(z),H(z')) = |s(z) - s(z')| \stext{ and } d_\times (H(z),H(z')) = |\ln s(z) - \ln s(z')|.
$$
The properties 1. and 2. are thus equivalent to $\dil(s)\leq 1$, and therefore also to :
\be
\label{eqDilsLoc}
\dil_z(s) \leq 1 \text{ for all } z\in \R^d,
\ee
according Proposition \ref{propDilLoc} applied to the constant metric $H_0 = \Id$ and to the function $f=s$.
On the other hand property 3. is equivalent to $\dil(\ln s \sep d_H) \leq 1$, and thus to :
$$
\dil_z(\ln s\sep d_H) \leq 1 \text{ for all } z\in \R^d,
$$
according to Proposition \ref{propDilLoc} applied to the metric $H$ and to the function $f=\ln s$.
This property equivalent to \iref{eqDilsLoc} according to \iref{eqDilLnH}, which concludes the proof of this Proposition.
\sq

The next corollary uses Proposition \ref{propEquivS} to analyse the regularity of the first and last eigenvalue of a metric.
\begin{corollary}
\label{corolLipNorm}
\begin{enumerate}
\item
For any $H\in \bH_g$, the map $z\mapsto \|H(z)\|^{-\frac 1 2}$ is Lipschitz.
\item
For any $H\in \bH_a$, the map $z\mapsto \|H(z)^{-\frac 1 2}\|$ is Lipschitz.
\end{enumerate}
\end{corollary}
\proof
We first establish Point 1.
We consider $H\in \bH_g$, and we define $s(z) := \|H(z)\|^{-\frac 1 2}$ and 
$$
H'(z) := \frac \Id {s(z)^2} = \|H(z)\|\Id,
$$
for each $z\in \R^d$.
Since $H(z) \leq H'(z)$ for all $z\in \R^d$, we have $d_H(z,z') \leq d_{H'} (z,z')$ for all $z, z'\in \R^d$.
%Consider a pair $M,M'\in S_d^+$ of matrices and a real $\delta>0$. If $e^{-2\delta} M \leq M' \leq e^{2\delta} M$, then taking the norm we obtain $e^{-2\delta} \|M\| \leq \|M'\| \leq e^{2\delta} \|M\|$. It follows that 
%$$
%\frac 1 2 |\ln \|M\| - \ln \|M'\|| \leq d_\times (M,M').
%$$
%We thus have for any $z,z'\in \R^d$
It follows that, using \iref{eqDTimesDiffLog},
\begin{eqnarray*}
|\ln s(z)-\ln s(z')| &=& \frac 1 2 \left|\ln \|H(z)\| - \ln \|H(z')\|\right| \\ %\left|\ln \left(\sqrt{\|H(z)\|}\right) -\ln \left(\sqrt{\|H(z')\|}\right)\right| \\%
%& \leq & \sup_{u\neq 0} |\ln \|u\|_{H(z)} - \ln \|u\|_{H(z')}|\\
&\leq & d_\times(H(z),H(z')) \\
&\leq& d_H(z,z')\\
&\leq& d_{H'}(z,z').
\end{eqnarray*}
Applying Proposition \ref{propEquivS} to the metric $H'$ we obtain that $H'\in \bH_i$, and therefore that $s$ is Lipschitz as announced.\\

The proof of Point 2. is more straightforward, since for any metric $H\in \bH_a$ we have 
$$
\left|\|H(z)^{-\frac 1 2}\| - \|H(z')^{-\frac 1 2}\| \right| \leq \|H(z)^{-\frac 1 2}-H(z')^{-\frac 1 2}\| \leq |z-z'|
$$
for all $z,z'\in \R^d$,
which concludes the proof of this corollary.\sq

Our last proposition studies the local dilatation of the maximum and the minimum of two functions.
\begin{prop}
\label{propDilMax}
Let $(X,d_X)$ be a metric space and let $\lambda, \mu\in C^0(X, \R)$. Let $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda, \mu\}$. Then for all $x\in X$
\be
\label{eqDilMax1}
\max\{\dil_x(\gamma), \dil_x(\Gamma)\} \leq \max\{\dil_x(\lambda), \dil_x(\mu)\}.
\ee
If $(X,d_X) = (\R^d, d_H)$, where $H \in \bH$ is a riemannian metric, then the above inequality becomes an equality 
\be
\label{eqDilMax2}
\max\{\dil_x(\gamma\sep d_H),\, \dil_x(\Gamma\sep d_H)\} = \max\{\dil_x(\lambda\sep d_H),\, \dil_x(\mu\sep d_H)\}.
\ee
\end{prop}

\proof
We have for any $p,q\in X$,
\begin{eqnarray*}
|\gamma(p)-\gamma(q)| &=& |\min\{\lambda(p), \mu(p)\} - \min \{\lambda(q), \mu(q)\}|\\
& \leq & \max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}.
\end{eqnarray*}
For any $x\in X$ and any $\ve>0$ we thus obtain
\begin{eqnarray*}
\dil(\gamma_{|B(x,\ve)}) &=& \sup_{p,q\in B(x,\ve)} \frac{|\gamma(p)-\gamma(q)|}{d_X(p,q)} \\
&\leq& \sup_{p,q\in B(x,\ve)} \frac{\max\{|\lambda(p)-\lambda(q)|,\, |\mu(p)-\mu(q)|\}}{d_X(p,q)}\\
& =& \max\left\{\sup_{p,q\in B(x,\ve)}  \frac{|\lambda(p)-\lambda(q)|}{d_X(p,q)}, \sup_{p,q\in B(x,\ve)}  \frac{|\mu(p)-\mu(q)|}{d_X(p,q)}\right\}\\
&=& \max\left\{\dil(\lambda_{|B(x, \ve)}), \dil(\mu_{|B(x,\ve)})\right\}.
\end{eqnarray*}
Letting $\ve \to 0$ we obtain $\dil_x(\gamma) \leq \max \{\dil_x(\lambda), \dil_x(\mu)\}$. Proceeding likewise for $\Gamma$ we conclude the proof of \iref{eqDilMax1}.\\


We now turn to the proof of \iref{eqDilMax2}. For that purpose we consider a fixed $\ve>0$ and we define
$$
K := \max \{\dil(\gamma_{|B(x,\ve)}\sep \|\cdot\|_{H(x)}), \ \dil(\Gamma_{|B(x,\ve)} \sep \|\cdot\|_{H(x)})\},
$$
where $B(x,\ve)$ stands for the euclidean unit ball of radius $\ve$ centered at $x$.
Consider two points $p,q\in B(x,\ve)$. If $\lambda(p) \geq \mu(p)$ and $\lambda(q)\geq \mu(q)$, or if $\lambda(p) \leq \mu(p)$ and $\lambda(q)\leq \mu(q)$, then 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)|&=& \max \{|\gamma(p)-\gamma(q)|, |\Gamma(p)-\Gamma(q)|\}\\
&\leq & K\|p-q\|_{H(x)}
\end{eqnarray*}
Otherwise if  $\lambda(p) \geq \mu(p)$ and $\lambda(q)\leq \mu(q)$, or $\lambda(p) \leq \mu(p)$ and $\lambda(q)\geq \mu(q)$, then there exists a point $r$ on the segment $[p,q]$ such that $\lambda(r)=\mu(r)$. We thus have %$|p-r|+|r-q| = |p-q|$ and 
\begin{eqnarray*}
|\lambda(p) -\lambda(q)| &\leq& \max \{|\gamma(p)-\gamma(r)|, |\Gamma(r)-\Gamma(q)|\}\\
& &+ \max \{|\gamma(r)-\gamma(q)|, |\Gamma(r)-\Gamma(q)|\}\\
& \leq & K\|p-r\|_{H(x)} + K\|r-q\|_{H(x)} = K\|p-q\|_{H(x)}
\end{eqnarray*}
If follows that $\dil(\lambda_{|B(x,\ve)}\sep \|\cdot\|_{H(x)})\leq K$, and letting $\ve\to 0$ we obtain 
$$
\dil_x(\lambda\sep \|\cdot\|_{H(x)}) \leq \max\{\dil_x(\gamma\sep \|\cdot\|_{H(x)}), \ \dil_x(\Gamma \sep \|\cdot \|_{H(x)})\}.
$$ 
Recalling that $\dil_x(f\sep d_H) = \dil_x(f\sep \|\cdot\|_{H(x)})$ for any $f\in C^0(\R^d, \R)$ and any $x\in \R^d$, see \iref{eqDilNorm}, we obtain $\dil_x(\lambda\sep d_H) \leq \max\{\dil_x(\gamma\sep d_H), \ \dil_x(\Gamma\sep d_H)\}$. Proceeding likewise for $\mu$ we obtain \iref{eqDilMax2} which concludes the proof of this proposition.
\sq

\subsection{Geometric properties of the space $(\R^d, d_H)$} %Estimates of size}
\label{subsecMetGeom}

We focus in this subsection on the ``geometrical properties'' of the space $\R^d$ equipped with the distance $d_H$ and the measure $\sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. The next proposition compares the riemannian distance $d_H$ between two points $z$ and $z+u$ with the norm $\|u\|_{H(z)}$ of their difference.

%with the euclidean distance and we estimate the volume of balls. 
%The next proposition compares the Riemannian distance associated to a graded metric, with 

\begin{prop}
\label{propEuclidRiemann}
Let $H \in \bH_g$ and let $z\in \R^d$. For all $u\in \R^d$ one has
\be
\label{eqEuclidRiemann}
\ln(1+\|u\|_{H(z)}) \leq d_H(z,z+u) \leq -\ln(1-\|u\|_{H(z)}),
\ee
where the right hand side equals $\infty$ by convention when $\|u\|_{H(z)}\geq 1$.
\end{prop}
\proof
%We first prove the left part of \iref{eqEuclidRiemann}, and for that purpose
We consider a path $\gamma\in C^1([0,1], \R^d)$, and we define for each $t\in [0,1]$
\be
\label{defLGamma}
l(t) := \int_0^t \|\gamma'(t)\|_{H(\gamma(t))}dt.
\ee
Since $H\in \bH_g$ we have for any $t\in [0,1]$
$$
\exp(-2\, d_H(z, \gamma(t))) \, H(z) \leq H(\gamma(t)) \leq  \exp(2 \, d_H(z, \gamma(t))) \, H(z)
$$
therefore, since $d_H(z, \gamma(t)) \leq l(t)$,
$$
\exp(-2l(t)) H(z)  \leq H(\gamma(t)) \leq  \exp(2l(t)) H(z).
$$
It follows that 
$$
\|\gamma'(t)\|_{H(z)} \exp(-l(t)) \leq l'(t) = \|\gamma'(t)\|_{H(\gamma(t))} \leq  \|\gamma'(t)\|_{H(z)} \exp(l(t)), %\exp(-l(t))
$$
hence 
\be
\label{eqGammapLp}
-\frac d {dt} \exp(-l(t)) \leq \|\gamma'(t)\|_{H(z)} \leq \frac d {dt} \exp(l(t)).
\ee
We have 
\be
\label{eqGammaGammap}
\|u\|_{H(z)} =  \|\gamma(1)-\gamma(0)\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt
\ee
with equality if $\gamma(t) = z+tu$ is the straight line.
%We now assume that $\gamma(t) \neq \gamma(0)$ for all $t\in (0,1]$, which is the case generically. The map $t\mapsto \|\gamma(t)-\gamma(0)\|_{H(z)}$ is therefore $C^1$ on $(0,1]$ and we have 
%$$
%\frac d {dt} \|\gamma(t)-\gamma(0)\|_{H(z)} \leq \|\gamma'(t)\|_{H(z)},
%$$
%with equality if $\gamma(t)-\gamma(0) = c \gamma'(t)$ for some $c>0$.
%In the special case of the straight line $\gamma(t)=z+tu$, \iref{eqGammaGammap} is an equality and we thus obtain 
For that specific path $\gamma$ we obtain %In that case, integrating the left part of \iref{eqGammapLp} we obtain
$$
\|u\|_{H(z)} = \int_0^1 \|\gamma'(t)\|_{H(z)} dt \geq -\int_0^1 \left(\frac d {dt} \exp(-l(t))\right)dt = 1-\exp(-l_H(\gamma)).
$$
Rearranging the terms we obtain the right part of \iref{eqEuclidRiemann}:
$$
d_H(z,z+u) \leq l_H(\gamma) \leq -\ln(1-\|u\|_{H(z)}).
$$
We now consider an arbitrary path $\gamma$ joining $z$ and $z+u$ and we obtain integrating the right part of \iref{eqGammapLp} and recalling \iref{eqGammaGammap}
$$
\|u\|_{H(z)} \leq \int_0^1 \|\gamma'(t)\|_{H(z)} dt \leq \int_0^1 \left(\frac d {dt} \exp(l(t))\right) dt = \exp(l_H(\gamma)) -1,
$$
which is equivalent to
$
l_H(\gamma) \geq \ln(1+\|u\|_{H(z)}).
$
Taking the infimum among all paths $\gamma\in C^1([0,1], \R^d)$ satisfying $\gamma(0) = z$ and $\gamma(1) = z+u$, we obtain the left part of \iref{eqEuclidRiemann}, which concludes the proof of this proposition.
\sq

We discuss in the rest of this section the consequences of the comparison \iref{eqEuclidRiemann} of the riemannian distance $d_H$ with the distance associated to the norm $\|\cdot\|_{H(z)}$ when $H\in \bH_g$. %is devoted to 
Combining the right part of \iref{eqEuclidRiemann} with the expression \iref{eqDTimesLog} of the distance $d_\times$ we obtain an estimate of the local variations of the norm $\|\cdot \|_{H(z)}$ associated to the metric $H$ at a point $z$: let $H\in \bH_g$, and let $z,u,v\in \R^d$ be such that $\|u\|_{H(z)} < 1$, then
\be
\label{eqLocalNorm}
(1-\|u\|_{H(z)}) \|v\|_{H(z)} \leq \|v\|_{H(z+u)} \leq (1-\|u\|_{H(z)})^{-1} \|v\|_{H(z)}. %\frac{\|v\|_{H(z)}}{1-\|u\|_{H(z)}}.
\ee
Note also that 
\be
\label{eqLocalDet}
(1-\|u\|_{H(z)})^d \sqrt{\det H(z)} \leq \sqrt{\det H(z)} \leq (1-\|u\|_{H(z)})^{-d} \sqrt{\det H(z)}.
\ee
Another important consequence of \iref{eqEuclidRiemann} is that for any $z\in \R^d$ and any $r\geq 0$ the closed ball $\{z'\in \R^d \sep d_H(z,z')\leq r\}$ for the distance $d_H$, is a closed and bounded subset $\R^d$, hence is compact. %From this point a classical argument (??) shows that $(R^d,d_H)$ is a complete metric space.

The following example establishes that \iref{eqEuclidRiemann} is a sharp inequality. The metric $H$ defined by 
$$
H(z) := \frac \Id {(1+|z|)^2}
$$
belongs to $\bH_i$ since $z\mapsto 1+|z|$ is Lipschitz, hence $H$ also belongs to $\bH_a$ and $\bH_g$.
For any $v\in \R^d$, one easily checks that the path of minimal length joining $0$ to $v$ is the straight line, and that
$$
d_H(0, v) = \ln(1+|v|).
$$
Choosing $z=0$ and $u=v$ we obtain that the left part of \iref{eqEuclidRiemann} is sharp
$$
\ln (1+ \|u\|_{H(0)}) = \ln (1+ |u|) = d_H(0,0+u).
$$
Choosing $z=-v$ and $u = v$ we obtain that the right part of \iref{eqEuclidRiemann} is sharp
$$
-\ln\left(1-\|u\|_{H(-u)} \right) = -\ln \left(1-\frac {|u|}{1+|u|}\right) = \ln(1+|u|) = d_H(-u, -u+ u).
$$

The next corollary uses Proposition \ref{propEuclidRiemann} to obtain a lower bound for the mass of balls in the measure $z\mapsto \sqrt{\det H(z)} dz$ associated to a graded metric $H\in \bH_g$. %states a volume estimate Proposition \ref{propLength} implies a volume estimate. %also allows us to compare the vo
For any metric $H\in \bH$, any $z\in \R^d$ and any $r>0$ we define the ellipse
$$
B_H(z) := \{ z+u\sep \|u\|_{H(z)} < r\},
$$
and we observe that 
$$
|B_H(z,r)| = \omega (\det H(z))^{-\frac 1 2}
$$
where $\omega$ denotes the volume of the standard euclidean ball.
\begin{corollary}
\label{corolVol}
There exists $c=c(d)>0$ such that the following holds. For any $H \in \bH_g$, any $r\geq 1$ and any $z\in \R^d$ we have 
\be
\label{eqVolLog}
\int_{B_H(z,r)} \sqrt{\det H} \geq c \ln r. 
\ee
\end{corollary}

\proof
It follows from Proposition \ref{propEuclidRiemann} that $d_H(z_0, z) \geq \ln (r+1)$ for all $z\in \partial B_H(z,r)$. We define the integer 
$$
k = \left\lfloor \ln(r+1) -\frac 1 2\right\rfloor,
$$
and we consider $k$ points $z_1, \cdots , z_k \in E$ such that 
$
d_H(z_0, z_i)= i
$ 
for all $0 \leq i \leq k$.
We define 
$
r_0 := 1-e^{-\frac 1 2} = 0.39\cdots
$
in such way that 
$
-\ln (1-r_0) = 1/2.
$
We have according to \iref{eqLocalDet} for all $z\in B_H(z_i,r_0)$
\be
\label{eqzzi}
\sqrt{\det H(z)} \geq (1-\|z-z_i\|_{H(z_i)})^d  \sqrt{\det H(z_i)} \geq (1-r_0)^d \sqrt{\det H(z_i)}.
\ee
For any $z\in B(z_i,r_0)$ we have 
$$
d_H(z_0, z) \leq d_H(z_0, z_i) + d_H(z_i, z) \leq i- \ln (1-r_0) \leq k+\frac 1 2 \leq \ln (r+1),
$$
which implies that $B(z_i,r_0) \subset B(z,r)$ for all $0 \leq i \leq k$.
Furthermore if $0\leq i<j\leq k$, $z\in B(z_i,r_0)$ and $z'\in B(z_j,r_0)$ then
$$
d_H(z,z') \geq d_H(z_i, z_j) -d_H(z_i, z) - d_H(z_j,z') > |d_H(z_0, z_i) - d(z_0, z_j)| + 2\ln(1 -r_0) =0, %\geq 1+ 2 \ln(1-\frac 1 3)>0.
$$
hence $B(z_i,r_0) \cap B(z_j,r_0) = \emptyset$.
It follows that 
\begin{eqnarray*}
\int_{B(z,r)} \sqrt{\det H} &\geq& \sum_{0 \leq i \leq k} \int_{B(z_i,r_0)} \sqrt{\det H}\\
&\geq& \sum_{0 \leq i \leq k} (1-r_0)^d \sqrt{\det H(z_i)} |B_H(z_i,r_0)|\\
&=& \omega r_0^d (1-r_0)^d (k+1)\\
& \geq & c_0 (\ln (r+1) - 1/2),
\end{eqnarray*}
where $c_0 :=  \omega r_0^d (1-r_0)^d$.
Since $r\geq 1$ we have 
$$
\ln(r+1) - \frac 1 2 \geq \left(\frac{\ln(r+1)}{2 \ln 2} -\frac 1 2\right)+  \left(1-\frac 1 {2 \ln 2}\right)\ln(r+1) \geq  \left(1-\frac 1 {2 \ln 2}\right)\ln r
$$
which concludes the proof with $c=(1- 1/(2 \ln 2))c_0$.
\sq


\section{Metrics having an eigenspace of dimension $d-1$ at each point}
\label{secEigen}
We focus in this subsection on metrics $H\in \bH$ such that the symmetric matrix $H(z)$ has an eigenspace of dimension at least $d-1$ at each point $z\in \R^d$. Note that this condition clearly holds if the dimension is $d=2$, but is also relevant in some applications to higher dimension as illustrated in \S \ref{secOptGeom} of the next chapter.
%, and is also used in \S \ref{secOptGeom} of the next chapter. 
%If the dimension is $d=2$, then a metric $H\in \bH$ generically satisfies this condition on a dense subset of $\R^d$. %any metric $H\in \bH$ satisfies this condition. 
%This condition clearly holds if the dimension is $d=2$,  is also used in \S \ref{secOptGeom} of the next chapter. 
%Indeed, as discussed in \S\ref{secOptGeom} of Chapter \ref{chapApproxMet}, this type of metrics appears when one needs to create mesh containing a thin layer of simplices close to an hypersurface $\Gamma$. In that case the matrix $H(z)$ at a point $z\in \Gamma$ typically has an eigenspace of dimension $d-1$ which is tangent to $\Gamma$ and is associated to a small eigenvalue, and an eigenspace of dimension $1$ in the direction orthogonal to $\Gamma$ associated to a large eigenvalue. 
The main result of this section is Theorem \ref{th2Spaces} which characterises those of these metrics which belongs to $\bH_a$ or $\bH_g$ in terms of the regularity of their eigenvalues and of their eigenvectors.
%Corollary \ref{corolHgToHa} to this theorem gives a simple procedure to obtain a quasi-acute metric from a graded metric $H$ such that $H(z)$ has an eigenspace of dimension $d-1$ at each point. \\

We denote by $\bbS := \{\theta\in \R^d \sep |\theta| = 1\}$ the unit sphere of $\R^d$, equipped with the distance 
$$
d_\bbS(\theta, \theta') := \arccos(\<\theta, \theta'\>).
$$
We denote by $\cA$ the space of parameters
$$
\cA := \R_+^*\times \R_+^*\times \bbS,
$$
and we define a map $\cS :\cA\to S_d^+$ as follows
\be
\label{defcS}
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
\ee
In any orthonormal basis $\cB$ of $\R^d$ which begins with the vector $\theta$ we have the following expression
$$
[\cS(\lambda, \mu, \theta)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda &0 & 0 & \cdots\\
0 & \mu & 0 & \cdots\\
0 & 0 & \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right).
$$
We also define for any $a = (\lambda, \mu, \theta)\in \cA$
$$
\cH(a) := \cS(a)^{-2} = \lambda^{-2} \theta \theta^\trans+ \mu^{-2}(1-\theta \theta^\trans).
$$
%If $M\in S_d^+$ has an eigenspace of dimension $d-1$ exactly, then 
%
%We denote by $S_{d*}^+$ the collection of symmetric positive definite matrices $M\in S_d^+$ which have an eigenspace of dimension exactly $d-1$.
%We also denote by $\cA^*$ the collection of $(\lambda, \mu, \pm\theta)\in \cA$ which satisfies $\lambda\neq \mu$ if $d>2$ (resp. $\lambda>\mu$ is the dimension is $d=2$).
%Then
%$$
%\cH : \cA^* \to S_{d*}^+
%$$
%is a one to one map.



%Such a metric $H$ can be parametrized using two eigenvalues $\lambda, \mu\in \R_+^*$  and a subspace of dimension $d-1$ of $\R^d$ defined through an un-oriented unit normal $\pm \theta$. Our purpose in this section is to translate the fact that $H\in \bH_\star$, for some $\star\in \{i,a,g\}$, into simpler properties satisfied by $\lambda,\mu$ and $\theta$.
%
%
%
%In order to state our results, we need to introduce the collection $\cP$ of all hyperplanes of $\R^d$, also called the projective space. An hy
%
%
%We define the space of parameters
%$$
%\cA :=  \R_+^* \times \R_+^* \times \cP,
%$$
%where $\cP$ is the $d-1$-dimensional real projective space.
%For all $(\theta, \lambda, \mu)\in \cA$ we define 
%$$
%S( \lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans),
%$$
%and $H(\theta, \lambda, \mu) := S^{-2}$.
%The space $\cA$ is a differential variety, and the tangent space to a triplet $(\theta, \lambda, \mu)\in \cA$ is 
%$$
%T_{(\theta, \lambda, \mu)} \cA =  \R \times \R \times \theta^\perp,
%$$
%where $\theta^\perp$ refers to the orthogonal hyperplane to $\theta$ in $\R^d$.

For any metric $H \in \bH$ and any $z\in \R^d$ we denote by $\dil_z(H)_\times$ and $\dil_z(H)_+$ the local dilatations at $z$ associated to the Lipschitz conditions \iref{eqLipMult} and \iref{eqLipAdd} defining $\bH_g$ and $\bH_a$:
\be
\label{defDilH}
\dil_z(H)_\times := \dil_z(H \sep d_\times, d_H) \stext{ and } \dil_z(H)_+ := \dil_z(H \sep d_+).
\ee
%We recall that the local dilatation $\dil_z(f)$ of a function $f$ at a point $z$ is defined by \iref{defDilX}.
%We set $D_z(H) := \dil(\lambda)$ if $z\notin \Omega$
Let $\Omega\subset \R^d$ be an open set, let $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, and let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$. We define
\be
\label{eqDZA}
D_z(a)_\times := \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \frac 1 2 \left| \frac {\lambda(z)} {\mu(z)} - \frac {\mu(z)} {\lambda(z)} \right|\dil_z(\theta\sep  d_H)\right\}, %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
and 
\be
\label{eqDZAP}
D_z(a)_+ := \max\left\{\dil_z(\lambda), \ \dil_z(\mu),\ |\lambda(z)-\mu(z)| \dil_z(\theta)\right\}. %\frac{\rho(z)-\rho(z)^{-1}} 2 
\ee
Note that these quantities are not defined if $\lambda(z) = \mu(z)$ and $\dil_z(\theta\sep  d_H)=\infty$ simultaneously, since an indeterminate product $0\times \infty$ appears in \iref{eqDZA} and \iref{eqDZAP}.
\begin{theorem}
\label{th2Spaces}
Let $H \in \bH$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$, such that $H = \cH\circ a$ on $\Omega$.
For each $z\in \Omega$ such that $\lambda(z) \neq \mu(z)$ or $\dil_z (\theta) < \infty$ one has  
%\be
%\label{eqDilTimes}
%D_z(a)_\times \leq \dil_z(H)_\times \leq 2D_z(a)_\times
%\ee
%and%, with $\gamma := \|H^{-\frac 1 2}\| = \max\{\lambda, \mu\}$, 
%\be
%\label{eqDilPlus}
%D_z(a)_+ \leq \dil_z(H)_+ \leq 2D_z(a)_+.
%\ee
\begin{eqnarray}
\label{eqDilTimes}
D_z(a)_\times &\leq \dil_z(H)_\times \leq& 2D_z(a)_\times\\
\label{eqDilPlus}
D_z(a)_+ &\leq \dil_z(H)_+ \leq& 2D_z(a)_+.
\end{eqnarray}
%In particular, defining $\gamma := \|H(z)^{-\frac 1 2}\| = \max \{\lambda, \mu\}$ we have 
%\be
%\label{eqDilMax}
%\max\{\dil_z(\gamma), \, D_z(a)_\times\} \leq \max \{D_z(a)_+, \, D_z(a)_\times\} \leq 2\max\{\dil_z(\gamma), \, D_z(a)_\times\}.
%\ee
\end{theorem}

%The estimate \iref{eqDilPlus} on $\dil_z(H)_+$ is not very sharp, but this is not an issue since one usually does not needs to control $ \dil_z(H)_+$ but rather $\max\{\dil_z(H)_\times,\dil_z(H)_+\}$, for which we obtain combining \iref{eqDilTimes} and \iref{eqDilPlus} the sharper estimate 
%$$
% \max\{\dil_z(\gamma), D_z(a)\} \leq \max\{\dil_z(H)_\times,\dil_z(H)_+\} \leq 2 \max\{\dil_z(\gamma), D_z(a)\}.
%$$
The rest of this section is devoted to the proof of this theorem and to the Corollaries \ref{corolDilThetaG} and  \ref{corolHgToHa}. Our intermediate result in the proof of Theorem \ref{th2Spaces} defines and estimates a quantity $\Delta(a,b,c)$ which appears repeatedly in the rest of the proof.


\begin{lemma}
\label{lemmaDelta}
For each $a,b,c\in \R$ we define %the quantity $\Delta(a,b,c)\in \R_+$, as follows % which is the norm of a $d\times d$ matrix,
\be
\label{defDelta}
\Delta(a,b,c) := 
\left\| 
\left(
\begin{array}{cccc}
a & b & 0 & \cdots\\
b & c& 0 & \cdots\\
0 & 0 & c & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right)
\right\|.
\ee
Then 
\be
\label{eqEstimM}
\max\{|a|, |b|, |c|\} \leq \Delta(a,b,c) \leq 2 \max\{|a|, |b|, |c|\}.
\ee
\end{lemma}

\proof
We consider fixed values of $a,b,c\in \R$ and we denote by $M$ the matrix appearing in \iref{defDelta}, in such way that $\Delta(a,b,c) = \|M\|$. We also define $\lambda := \max\{|a|,|b|,|c|\}$.
We have 
$$
\Delta(a,b,c) = \|M\|\geq \max_{1\leq i,j\leq d} |M_{ij}| = \lambda,
$$
which establishes the left part of \iref{eqEstimM}. For all $p\in [1,\infty]$ we denote by $l^p$ the usual norm on $\R^d$ of exponent $p$. We have 
$$
\|M\|_{l^\infty\to l^\infty} = \max_{1 \leq i \leq d} \sum_{1\leq j \leq d} |M_{ij}| \leq 2 \lambda \stext{ and } \|M\|_{l^1\to l^1} = \max_{1 \leq j \leq d} \sum_{1\leq 1 \leq d} |M_{ij}| \leq 2 \lambda.
$$
By interpolation we thus obtain  
$$
\|M\| = \|M\|_{l^2\to l^2} \leq \sqrt{\|M\|_{l^1\to l^1} \|M\|_{l^\infty\to l^\infty} } \leq 2 \lambda,
$$
which concludes the proof.
\sq

The parameter space $\cA = \bbS \times \R_+^* \times \R_+^*$ is a differential variety, and the regularity of functions defined on $\cA$ should be seen through local charts.
For each $a = (\lambda, \mu, \theta)\in \cA$ we define a local chart $\psi_a$ of a neigborhood of $a$ in $\cA$.
\be
\label{defPsia}
\psi_a : (-\lambda, \infty)\times (-\mu , \infty) \times (B(0,\cPi) \cap \theta^\perp) \to \cA,
\ee
where $\theta^\perp := \{\Theta\in \R^d \sep \<\theta, \Theta\> = 0 \}$ denotes the space orthogonal to $\theta$, and $B(0,\cPi)$ the open euclidean ball of radius $\cPi$.
We define 
$$
\psi_a(\Lambda, M, r\Theta) := (\lambda+ \Lambda,\, \mu+ M,\, \cos(r) \theta + \sin(r) \Theta),
$$
where $|\Theta| = 1$.
Note that $\psi_a$ is one to one and that $d_\bbS(\theta, \, \cos(r) \theta + \sin(r) \Theta) = r$.

Let $V$ be a banach space. We say that a function $\vp : \cA \to V$ is $C^1$ if for any $a\in \cA$ the function $\vp\circ \psi_a$ is $C^1$.
In that case for any $a\in \cA$ we define the differential 
%and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
$$
d_a\vp(A) : \R\times \R\times \theta^\perp \to V
$$
by the formula
$$
d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( tA) - \vp(a)} t. %\Lambda, t M, t r\Theta
$$
We then have
 $$
\dil_a(\vp) = \|d_a(\vp)\|.
$$
%where $d_0 (\vp\circ \psi_a) :  \R\times \R\times \theta^\perp \to V$ denotes the differential of function $\vp\circ \psi_a$ at the origin $(0,0,0) \in (-\lambda, \infty)\times (-\mu , \infty) \times (B(\pi) \cap \theta^\perp)$.
%In that case for any $a\in \cA$ and any $A = (\Lambda, M, r\Theta)\in T_a \cA := \R\times \R\times \theta^\perp$ we define
%$$
%d_a\vp(A) := d_0(\vp\circ \psi_a)(A) = \lim_{t\to 0} \frac{\vp\circ \psi_a( t\Lambda, t M, t r\Theta) - \vp(a)} t,
%$$
%and we have for any path $\gamma\in C^1([0,1], \cA)$ 
%$$
%\vp(\gamma(1)) - \vp(\gamma(0)) = \int_0^1 d \vp_{\gamma(t)} (\gamma'(t)) dt.
%$$

\begin{prop}
\label{propPhiPlus}
Define $V_+ := S_d$, equipped with the standard norm $\|\cdot\|$, and define $\vp_+ (a) := \cS(a)$.
Then for all $a,b\in \cA$ we have 
\be
\label{eqDPPhiP}
d_+(\cH(a), \cH(b)) = \|\vp_+(a)-\vp_+(b)\|.
\ee
Furthermore $\vp_+ \in C^1(\cA, V_+)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
$$
\|d_a \vp_+(A)\|_\infty= 
\Delta(\Lambda, \ (\lambda-\mu) r ,\ M).
$$
\end{prop}

\proof
The \iref{eqDPPhiP} directly follows from the fact that $\cH(a)^{-1} = \cS(a)^2 = \vp_+(a)^2$, and from the definition \iref{defDPlus} of $d_+$.
The function $\vp_+ = \cS$ is $C^1$ ( in fact  $C^\infty$), since it has a polynomial expression 
$$
\cS(\lambda, \mu, \theta) := \lambda \theta \theta^\trans+ \mu(1-\theta \theta^\trans).
$$
We consider a fixed point $a = (\lambda,\mu,\theta)\in \cA$, and $A=(\Lambda, M, r\Theta) \in T_a\cA$, where $|\Theta|=1$. 
We thus have for $t\in \R$
\begin{eqnarray*}
\cS(\psi_a(tA))  &=& %= \lambda+ \Lambda, \, \mu+M, \, \theta+r\Theta)
 (\lambda+ t\Lambda) (\theta+ tr\Theta) (\theta+tr\Theta)^\trans \\
 & &+ (\mu+tM)(\Id - (\theta+ tr\Theta) (\theta+tr\Theta)^\trans) +\cO(t^2)\\
 &=& S(\lambda, \mu, \theta) + \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans)+\cO(t^2)
\end{eqnarray*}
Therefore %$\vp_+$ is $C^1$ and 
\be
\label{eqDiffS}
%d_a\vp_+(\Lambda, \,M, \,r\Theta) = 
d_a\cS(A) =  \Lambda \theta \theta^\trans + M(\Id - \theta \theta^\trans) + r(\lambda-\mu) (\theta \Theta^\trans + \Theta \theta^\trans).
\ee
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[d_a\cS(A)]_\cB = 
\left(
\begin{array}{cccc}
\Lambda & r(\lambda-\mu) & 0 & \cdots\\
r(\lambda-\mu) & M & 0 & \cdots\\
0 & 0 & M & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
which concludes the proof of this proposition.
\sq


\begin{prop}
\label{propPhiTimes}
Define $V_\times := C^0(\bbS, \R)$, equipped with the $\|\cdot\|_\infty$ norm, and define $\vp_\times : \cA \to V_\times$ as follows: for any $a\in \cA$ and any $u\in \bbS$
$$
\vp_\times (a) := (u \mapsto \ln \|u\|_{\cH(a)}).
$$
Then for all $a,b\in \cA$ we have 
\be
\label{eqDTPhiT}
\|\vp_\times(a)-\vp_\times(b)\|_\infty = d_\times(\cH(a), \cH(b)).
\ee
Furthermore $\vp_\times \in C^1(\cA, V_\times)$ and for all $a=(\lambda, \mu, \theta)\in \cA$ and all $A = (\Lambda, M, r\Theta)\in T_a\cA$, with $|\Theta| = 1$, we have 
\be
\label{eqNormDPhiPlus}
\|d_a \vp_\times(A)\|_\infty= 
\Delta\left(\frac \Lambda \lambda ,\ \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) ,\ \frac M \mu\right).
\ee
\end{prop}

\proof
The expression \iref{eqDTPhiT} immediately follows from the expression \iref{eqDTimesLog} of the distance $d_\times$.
It is well known that the inverse map ${\rm Inv} : \GL_d \to \GL_d$ is $C^1$ and has the the following differential : for any $\phi\in \GL_d$ and any $\Phi\in M_d$
$$
d_\phi \Inv (\Phi) = \phi^{-1} \Phi \phi^{-1}.
$$
Since $\cS : \cA\to S_d^+$ is $C^1$, as observed in the proof of Proposition \ref{propPhiPlus}, the composition $\Inv \circ\, \cS : \cA \to S_d^+$ is also $C^1$, and for any $a=(\lambda, \mu , \theta)\in \cA$ and any $A\in \R\times \R \times \theta^\perp$
$$
d_a(\Inv \circ \, \cS)(A) = S(a)^{-1} (d_a S(A) ) S(a)^{-1}.
$$
For any $u\in \bbS$ we have 
$$
\ln \|u\|_{\cH(a)} = \ln \|\cS(a)^{-1}u\| = \frac 1 2 \ln \left(\<\cS(a)^{-1}u,\cS(a)^{-1}u\>\right).
$$
Therefore, again by composition, 
\begin{eqnarray*}
d_a (\ln \|u\|_{\cH})(A) &=&  \frac 1 {2\|\cS(a)^{-1}u\|^2} (\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>\\
& &\quad +\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>)\\% \frac {\<\cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u,\ \cS^{-1}(a)u\>+\<\cS^{-1}(a)u,\ \cS(a)^{-1} (d_a\cS(A))\cS^{-1}(a)u\>}{2\|\cS(a)^{-1}u\|^2}\\
&=& \frac{\<G(a,A) v,v\>}{\|v\|^2}
\end{eqnarray*}
where $v = \cS^{-1}(a)u$. The function $G$ has the following expression : for any $a = (\lambda, \mu, \theta)\in \R_+^* \times \R_+^* \times \bbS$ and any $A = (\Lambda, M, r\Theta)\in \R\times \R \times \theta^\perp$
\begin{eqnarray*}
G(a,A) &=& \frac{\cS(a)^{-1} (d_a\cS(A)) + (d_a\cS(A)) \cS(a)^{-1}} 2\\
&=& \frac \Lambda \lambda \theta \theta^\trans +  \frac M \mu (\Id - \theta \theta^\trans) + \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right)(\theta \Theta^\trans + \Theta \theta^\trans),
\end{eqnarray*}
where we used the explicit expression \iref{eqDiffS} of $d_a\cS(A)$, and the fact that $\theta^\trans \Theta = 0$.
Choosing an orthonormal basis $\cB$ of $\R^d$ which begins with the unit orthogonal vectors $\theta$ and $\Theta$, we obtain
$$
[G(a,A)]_\cB = 
\left(
\begin{array}{cccc}
\frac \Lambda \lambda & \frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & 0 & \cdots\\
\frac r 2\left(\frac \lambda \mu - \frac \mu \lambda\right) & \frac M \mu & 0 & \cdots\\
0 & 0 & \frac M \mu & 0\\
\vdots & \vdots & 0 &\ddots
\end{array}
\right),
$$
The map $\vp_\times$ is differentiable, as the composition of differentiable maps, and $d_a(\vp_\times(A))$ is the element of $V_\times  := C^0(\bbS, \R)$ defined by 
$
u \mapsto d_a (\ln \|u\|_\cH)(A).
$
Therefore 
\begin{eqnarray*}
\|d_a \vp_\times(A)\|_\infty &=& \sup \left\{ \frac{|\<G(a,A) v,v\>|}{\|v\|^2} \sep u\in \bbS, \, v=\cS(a)^{-1} u\right\}\\
&=& \|G(a,A)\|,
\end{eqnarray*}
which establishes \iref{eqNormDPhiPlus} and concludes the proof of this proposition.
\sq

We now consider a fixed $z\in \Omega$ and we remark that 
$$
\dil_z(H)_\times = \dil_z(\cH\circ a)_\times  = \dil_z(\vp_\times \circ a\sep d_H). %\leq \dil_{a(z)} (\vp_+\sep d_z) \dil_z(a\sep d_H, d_z)
$$
Therefore,  according to Lemma \ref{lemmaSubMult} for any norm $\|\cdot\|_{a(z)}$ defined on the tangent space $\R\times \R \times \theta(z)^\perp$ to $a(z)\in \cA$ we have 
\be
\label{eqDilPhiA}
\begin{array}{rcl}
& &\dil^*_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} a\sep d_H, \|\cdot \|_{a(z)})\\
& \leq& \dil_z(H)_\times\\
& \leq& \dil_0 (\vp_+\circ \psi_{a(z)} \sep \|\cdot\|_{a(z)}) \dil_z(\psi_{a(z)}^{-1} \circ a\sep d_H, \|\cdot\|_{a(z)})
\end{array}
\ee
provided no indeterminate $0\times \infty$ or $\infty \times 0$ appears on the first and last term of this inequality.
%We recall that a neighborhood of $a(z)$ is parametrized by the local chart 
%\be
%\label{defPsiAZ}
%\psi_{a(z)} : (\Lambda, M, r\Theta) \to (\lambda(z) + \Lambda, \, \mu(z) + M, \, \cos(r)\theta(z)+ \sin(r) \Theta)
%\ee
%where $|\Theta| = 1$. 
%We consider a fixed point $z\in \Omega$, and we distinguish the two cases $\lambda(z) \neq \mu(z)$ and $\lambda(z) = \mu(z)$.

We first consider the case where $\lambda(z) \neq \mu(z)$.
For each $a=(\lambda, \mu, \theta)\in \cA$ we define a norm $\|\cdot \|_a$ on the tangent space $\R\times \R \times \theta^\perp$ to $\cA$ at the point $a$ : for all $A = (\Lambda, M , \Theta)\in \R\times \R \times \theta^\perp$
$$
\|A\|_a = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \frac 1 2 \left| \frac \lambda \mu - \frac \mu \lambda\right| \|\Theta\|\right\}.
$$
We have by construction 
\be
\label{eqDilADZDH}
\dil_z(\psi_{a(z)}^{-1}\circ a\sep d_H, \|\cdot \|_{a(z)}) = D_z(a)_\times
\ee
According to Lemma \ref{lemmaDelta} and Proposition \ref{propPhiTimes} we have for any $a=(\lambda, \mu, \theta)\in \cA$ and any $A\in \R\times\R \times \theta^\perp$
$$
\|A\|_a \leq \|d_a \vp_\times(A)\|_\infty = \|d_0 (\vp_\times \circ \psi_a)\|_\infty \leq 2 \|A\|_a.
$$
Since $\vp_\times$ is $C^1$ it follows from \iref{eqDilDiff} that 
$$
1 \leq \dil^*_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq \dil_0 (\vp_\times\circ \psi_a\sep \|\cdot \|_a) \leq 2.
$$
Combining \iref{eqDilPhiA}, \iref{eqDilADZDH} and the last inequality we obtain
$$
D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times,
$$
which establishes the announced result \iref{eqDilTimes} in the case $\lambda(z)\neq \mu(z)$. A similar reasoning establishes the counterpart \iref{eqDilPlus} of this inequality for the distance $d_+$.\\

%\paragraph{Proof in the case $\lambda(z) = \mu(z)$.}
%We now turn to the case of equality $\lambda(z) = \mu(z)$.
We now consider the case $\lambda(z) = \mu(z)$.
For any $\ve>0$ and any $a=(\lambda, \mu, \theta)\in \cA$ such that $\lambda = \mu$ we define a norm $\|\cdot\|_{a,\ve}$ on the tangent space $\R\times \R\times \theta^\perp$ to $a$ in $\cA$ as follows : 
$$
\|A\|_{a, \ve} = \max \left\{\frac {|\Lambda|} \lambda , \, \frac {|M|} \mu, \, \ve \|\Theta\|\right\}.
$$
%$$
%d_z^\ve((\Lambda, M, r\Theta), (\Lambda', M', r'\Theta')) := \max \left\{\frac {|\Lambda-\Lambda'|} {\lambda(z)},\, \frac {|M-M'|} {\mu(z)}, \, \ve \|r\Theta - r'\Theta'\|\right\}.
%$$
This modification is required because the original norm $\|\cdot\|_a$ used in the case $\lambda\neq \mu$ is only a semi-norm when $\lambda = \mu$.
Reasoning similarly to the case $\lambda(z) \neq \mu(z)$ we obtain the upper bound
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H), \ \ve\dil_z(\theta\sep  d_H)\right\}.
$$
Since $\lambda(z) = \mu(z)$, the assumptions of the theorem state that $\dil_z(\theta \sep d_H) < \infty$. Since $\ve>0$ is arbitrary we thus obtain 
$$
\dil_z(H)_\times \leq 2 \max\left\{\dil_z(\ln \lambda\sep d_H), \ \dil_z(\ln \mu\sep d_H)\right\} = 2D_z(a)_\times.
$$
We now turn to the lower bound on $\dil_z(H)_\times$. 
For that purpose we define the functions $\gamma := \min \{\lambda, \mu\}$ and $\Gamma := \max\{\lambda,\mu\}$. For all $z,z'\in \Omega$ we have according to \iref{eqDTimesDiffLog} 
$$
d_\times (H(z),H(z')) \geq \max \{ |\ln\gamma(z) - \ln \gamma(z')|,\, |\ln \Gamma(z) - \ln \Gamma(z')|\}.
$$
Therefore 
$$
\dil_z(H)_\times = \dil_z(H\sep d_\times, d_H) \geq \max \{ \dil_z(\ln \gamma\sep d_H), \, \dil_z(\ln \Gamma \sep d_H)\}.
$$
Hence according to Proposition \ref{propDilMax}
$$
\dil_z(H)_\times \geq \max \{\dil_z(\ln \lambda\sep d_H), \dil_z(\ln \mu\sep d_H)\} = D_z(a)_\times.
$$
We have thus obtained $D_z(a)_\times \leq \dil_z(H)_\times \leq 2 D_z(a)_\times$, and proceeding likewise we obtain $D_z(a)_+ \leq \dil_z(H)_+ \leq 2 D_z(a)_+$, which concludes the proof of Theorem \ref{th2Spaces}. \\


Our first corollary compares $D_z(a)_\times$ with the dilatation $\dil_z(\theta)$, instead of $\dil_z(\theta\sep d_H)$ in Theorem \ref{th2Spaces}.
%We recall, see \iref{eqDilNorm}, that for any metric $H\in \bH$, any metric space $(Y,d_Y)$ and any function $f\in C^0(\R^d, Y)$ we have for all $z\in \R^d$
%\be
%\label{eqDilNormLM}
%\dil_z(f) \leq \|H(z)\|^{\frac 1 2}\dil_z(f\sep d_H)
%\ee

\begin{corollary}
\label{corolDilThetaG}
Under the hypotheses of Theorem \ref{th2Spaces} we have
%Let $H\in \bH_g$. Assume that there exists an open set $\Omega\subset \R^d$ and a continuous function $a\in C^0(\Omega, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$ such that $H = \cH\circ a$ on $\Omega$. Let $z\in \Omega$ be such that $\lambda(z) \neq \mu(z)$. Then
$$ 
|\lambda(z) - \mu(z)| \dil_z(\theta) \leq 2 D_z(a)_\times %\leq 2.
$$
\end{corollary}
\proof
Furthermore we have according to \iref{eqDilNorm} %\iref{eqDilNormLM}
\begin{eqnarray*}
 |\lambda(z) - \mu(z)| \dil_z(\theta)
&\leq& \frac {|\lambda(z) - \mu(z)|}{\min\{\lambda(z), \mu(z)\}} \dil_z(\theta\sep d_H)\\
&=& \left(\frac {\max \{\lambda(z), \mu(z)\}}{\min\{\lambda(z), \mu(z)\}}-1\right)\dil_z(\theta\sep d_H)\\
& \leq & \left|\frac {\lambda(z)} {\mu(z)}-\frac {\mu(z)} {\lambda(z)}\right|\dil_z(\theta\sep d_H) \\
&\leq & 2 D_z(a)_\times% \leq 2.
\end{eqnarray*}
which concludes the proof.
\sq


The next corollary shows how to construct a quasi-acute metric from a graded one.
Let $M\in S_d$ and let $U\in \cO_d$ and $\lambda_1, \cdots , \lambda_d\in\R$ be such that 
\be
\label{eqDiagSd}
M = U^\trans \diag(\lambda_1, \cdots , \lambda_d) U,
\ee
where $\diag(\lambda_1, \cdots, \lambda_d)$ denotes the diagonal matrix of entries $\lambda_1, \cdots, \lambda_d$. 
For any $\alpha\in \R$ we define the matrix $\max \{\alpha, M\}\in S_d$ as follows
$$
\max\{\alpha, M\} := U^\trans \diag(\max\{\alpha, \lambda_1\}, \cdots, \max\{\alpha, \lambda_d\})U,
$$
and we observe that $\max\{\alpha, M\}$ does not depend on the choice of the matrix $U$ and on the order of the eigenvalues $\lambda_1, \cdots, \lambda_d$ in the decomposition \iref{eqDiagSd}.
For any $(\lambda, \mu, \theta)\in \cA$ and any $s>0$ one has
\be
\label{maxsHa}
\max \{s^{-2}, \cH(a)\} = \min\{s, \lambda\}^{-2} \theta \theta^\trans+ \min\{s, \mu\}^{-2} (\Id-\theta \theta^\trans).
\ee

\begin{corollary}
\label{corolHgToHa}
Let $H\in \bH$ be such that $H(z)$ has an eigenvalue of multiplicity at least $d-1$ for all $z\in \R^d$. We define $s:\R^d\to \R_+^*$ and $H'\in \bH$ as follows : for all $z\in \R^d$
\begin{eqnarray*}
s(z) &:=& \inf_{z'\in \sR^d} |z-z'|+ \|H(z')^{-\frac 1 2}\|,\\
H'(z) &:=& \max\{s(z)^{-2}, H(z)\}.
\end{eqnarray*}
If $H\in \bH_g$, then $4^2H'\in \bH_a$.
\end{corollary}

\proof
We first observe that $s : \R^d \to \R_+^*$ is Lipschitz and that $s(z)\leq \|H(z)^{-\frac 1 2}\|$ for all $z\in \R^d$.
For each $\ve>0$ and each $z\in \R^d$ we define 
$$
H_\ve := \max\{e^{2 \ve} s(z)^{-2}, H(z)\}.
$$

Consider a fixed point $z\in\R^d$. If $H(z)$ is proportional to $\Id$, which means that $\|H(z)\|^{-\frac 1 2} = \|H(z)^{-\frac 1 2}\| \geq s(z)$, then $H_\ve = e^{2 \ve} \Id/ s^2$ on a neighborhood of $z$. This implies according to \iref{eqDilLnH} %\ref{PropEquivS}
$$
\dil_z(H_\ve)_\times =\dil_z(H_\ve)_+ = \dil_z(e^{-\ve} s) \leq e^{-\ve}\leq 1.
$$
%and therefore \iref{eqDilHe}.
On the other hand if $H(z)$ is not proportional to $\Id$ then there exists $a\in C^0(\R^d, \cA)$, $a(z) = (\lambda(z), \mu(z), \theta(z))$ such that $H = \cH\circ a$ on a neighborhood of $z$, and $D_z(a)_\times \leq 1$ according to Theorem \ref{th2Spaces}. 
We have according to \iref{maxsHa} on the same neighborhood of $z$, 
$$
H_\ve = \cH\circ a_\ve = \min\{e^{-\ve} s,\lambda\}^{-2} \theta \theta^\trans+ \min\{e^{-\ve} s,\mu\}^{-2} (\Id - \theta \theta^\trans),
$$
where $a_\ve=(\min\{e^{-\ve}s, \lambda\}, \min\{e^{-\ve} s, \mu\}, \theta) \in C^0(\R^d,\cA)$.

We define $H_\ve^i := e^{2\ve} \Id/ s^2$ and we observe that $H_\ve \geq H_\ve^i$ and $H_\ve \geq H$, hence for any $p,q\in \R^d$
$$
d_{H_\ve}(p,q) \geq \max \{d_H(p,q), \, d_{H_\ve^i}(p,q)\}.
$$
Using Proposition \ref{propDilLoc} we thus obtain  
\begin{eqnarray*}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\} \sep d_{H_\ve}) &\leq& \max \{\dil_z(\ln (e^{-\ve} s)\sep d_{H_\ve}), \,\dil_z(\ln \lambda\sep d_{H_\ve})\}\\
&\leq & \max \{\dil_z(\ln(e^{-\ve} s) \sep d_{H_\ve^i})), \,\dil_z(\ln \lambda\sep d_H)\}\\
& \leq & \max \{\dil_z(e^{-\ve} s), \, \dil_z(H)_\times\}\\
& \leq & \max \{e^{-\ve}, 1\} =1,
\end{eqnarray*}
where we used Theorem \ref{th2Spaces} and Proposition \ref{propEquivS} in the third line.
Proceeding likewise for the other eigenvalue of $H_\ve$ we conclude that 
\be
\label{eqDilAeVal}
\dil_z(\ln \min\{e^{-\ve} s, \lambda\}\sep d_{H_\ve}) \leq 1 \text{ and }
\dil_z(\ln \min\{e^{-\ve} s, \mu\}\sep d_{H_\ve}) \leq 1.
\ee
One easily checks that
$$
\left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right| \leq \left|\frac \lambda \mu - \frac \mu \lambda\right|,
$$
using that 
$
t \mapsto t/\mu - \mu/t %\frac t \mu - \frac \mu t
$
is increasing on $\R_+^*$.
Therefore   
$$
\frac 1 2 \left|\frac {\min\{e^{-\ve} s, \lambda\}}{\min\{e^{-\ve} s, \mu\}} - \frac {\min\{e^{-\ve} s, \mu\}}{\min\{e^{-\ve} s, \lambda\}}\right|  \dil_z(\theta \sep d_{H_\ve}) \leq \frac 1 2\left|\frac \lambda \mu - \frac \mu \lambda\right| \dil_z(\theta\sep d_H) \leq 1.
$$
Combining the last estimate with \iref{eqDilAeVal} we conclude that $D_z(a_\ve)_\times \leq 1$ and therefore $\dil_z(H_\ve)_\times \leq 2$ according to Theorem \ref{th2Spaces}.

Our next objective is to estimate $\dil_z(H_\ve)_+$.
Let us assume that $\lambda(z)<\mu(z)$, then
\begin{eqnarray*}
\dil_z(\min\{e^{-\ve} s , \lambda\}) &\leq& \max \left\{\dil_z(e^{-\ve} s), \, \dil_z(\lambda)\right\}\\
& \leq & \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\min\{\lambda(z), \mu(z)\}}\right\}\\
& = & \max \left\{\dil_z(e^{-\ve} s), \, \frac{\dil_z(\lambda \sep d_H)}{\lambda(z)}\right\}\\
&\leq& \max \{e^{-\ve}, \, \dil_z(\ln \lambda\sep  d_H)\}\\
&\leq & \max \{e^{-\ve} , \, 1\} = 1,
\end{eqnarray*}
where we used \iref{eqDilNorm} in the second line.
Still assuming that $\lambda(z)<\mu(z)$, we have $s(z)\leq \|H(z)^{-\frac 1 2}\| \leq \mu(z)$ by construction of $s$, and therefore $\min\{e^{-\ve} s, \mu\} = e^{-\ve} s$ on a neighborhood of $z$, and therefore
$
\dil_z(\min\{e^{-\ve} s, \mu\}) = \dil_z(e^{-\ve} s)\leq e^{-\ve} \leq 1.
$
Proceeding similarly if $\lambda(z)>\mu(z)$ we also obtain 
\be
\label{eqDilPVal}
\dil_z(\min\{e^{-\ve} s, \lambda\})\leq 1 \stext{ and } \dil_z(\min\{e^{-\ve} s, \mu\}).
\ee
We now focus on the local dilatation of the orientation $\theta$, and for that purpose we observe that 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}|  \leq  |\lambda(z) - \mu(z)|.
$$
Therefore according to Corollary \ref{corolDilThetaG} 
$$
|\min\{e^{-\ve}s(z),\lambda(z)\} - \min \{e^{-\ve}s(z), \mu(z)\}| \dil_z(\theta) \leq 2D_z(a)_\times \leq 2
$$
Combining this with \iref{eqDilPVal} we obtain $D_z(a_\ve)_+ \leq 2$ and therefore $\dil_z(H_\ve)_+ \leq 4$.\\

The above arguments show that 
$
\dil_z(H_\ve)_\times \leq 2
$
and 
$
\dil_z(H_\ve)_+ \leq 4,
$
which implies that $2^2H_\ve \in \bH_g$ and $4^2 H_\ve \in \bH_a$ according to Proposition \ref{propDilLoc} and Remark \ref{remHomog}.
Hence for any $z,z'\in \R^d$, since $H_\ve \leq e^{2\ve} H'$,
$$
d_\times(H_\ve(z), H_\ve(z')) \leq 2d_{H_\ve}(z,z') \leq 2e^\ve d_{H'}(z,z') \stext{ and } d_+(H_\ve(z), H_\ve(z')) \leq 4|z-z'|.
$$
Letting $\ve \to 0$ we obtain 
$$
d_\times(H'(z), H'(z')) \leq 2d_{H'}(z,z') \stext{ and } d_+(H'(z), H'(z')) \leq 4|z-z'|.
$$
Therefore $4^2 H\in \bH_a$, which concludes the proof of this corollary.
\sq


\section{From mesh to metric}
\label{secMeshToMet}
The techniques presented in this section show how to produce an metric $H\in \bH_i$, $\bH_a$ or $\bH_g$ from an isotropic, quasi-acute (in two dimensions), or graded mesh $\cT$.

Combining the next proposition with its counterpart Proposition \ref{propMeshGen}, on the generation of a mesh from a metric, yields the main result of this chapter: Theorem \ref{thEquiv} which states the equivalence of the classes $\bT_{i,C} \subset \bT_{a,C}\subset \bT_{g,C}$ of meshes and $\bH_i \subset \bH_a \subset \bH_g$ of metrics.
\begin{prop}
\label{propMetGen}
For any $C_0>0$ there exits $C = C(C_0,d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $\cT \in \bT_{i, C_0}$ there exists $H \in \bH_i$ which is $C$-adapted to $\cT$.
\item If $d=2$, then for any $\cT \in \bT_{a, C_0}$ there exists $H \in \bH_a$ which is $C$-adapted to $\cT$.
\item For any $\cT \in \bT_{g,C_0}$ there exists $H \in \bH_g$ which is $C$-adapted to $\cT$.
\end{enumerate}
\end{prop}

The rest of this section is devoted to the proof of this proposition.
For any mesh $\cT\in \bT$, and for any vertex $v$ of $\cT$, we denote by $n_\cT(v)$ the number of simplices in the mesh $\cT$ containing $v$:
$$
n_\cT(v) := \#\{T\in \cT \sep v\in T\}. %, %\text{s.t. } 
$$
We denote by $H_\cT^g\in \bH$ the piecewise linear metric on the mesh $\cT$ which satisfies for each vertex $v$ of $\cT$
\be
\label{eqHcTg}
H_\cT^g(v) := \frac 1 {n_\cT(v)} \sum_{\substack{T\in \cT\\\text{s.t. } v\in T}} \cH_T.
\ee
%The metric $H_\cT^g$ on a simplex $T\in \cT$ is simply the linear interpolation of the averages of the matrices $\cH_T$ attached to the simplices containing a vertex $v$. 

The next lemma establishes a property of the barycentric coordinates on a simplex, which is useful for the analysis of  the regularity of a piecewise linear function on an anisotropic mesh, such as the metric $H_\cT^g$.
\begin{lemma}
\label{lemmaNormLambda}
Let $T$ be a simplex and let $V$ be the collection of vertices of $T$. Let $(\lambda_v)_{v\in V}$ be the barycentric coordinates on $T$. Then for all $z,z'\in T$
\be
\label{eqNormLambda}
\|z-z'\|^2_{\cH_T} = \frac {d+1} d \sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2.
\ee
\end{lemma}

\proof
We first assume that $T$ is the reference equilateral simplex $\TEq$. %, and we recall that $\cH_\TEq = \Id$.
For any two vertices $v,v'$ in the collection $\VEq$ of vertices of $\TEq$ one has 
\be
\label{eqScalTEq}
\<v,v'\> = 
\left\{
\begin{array}{cl}
1 &\text{ if } v=v,'\\
-1/d &\text{ if } v \neq v'.
\end{array}
\right.
\ee
Indeed $|v|=1$ by construction for any vertex $v$ of $\TEq$, and for any $v'\in \VEq$ distinct from $v$ the scalar product $\<v,v'\>$ has a value $\alpha$ independent of $v$ and $v'$ by symmetry. Since $\TEq$ is centered at the origin we obtain $0 = \<v,\sum_{v\in V} v\>  = |v|^2 + d \alpha$ which establishes \iref{eqScalTEq}.
We thus obtain for any $z,z'\in \TEq$ 
\begin{eqnarray*}
|z-z'|^2  &=& \left|\sum_{v\in \VEq} (\lambda_v(z) - \lambda_v(z'))v\right|^2 \\
&=& \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \sum_{v\neq v'} (\lambda_v(z)-\lambda_v(z'))(\lambda_{v'}(z)-\lambda_{v'}(z')).
\end{eqnarray*}
Therefore 
$$
|z-z'|^2 =  \left(1+\frac 1 d\right) \sum_{v\in \VEq} |\lambda_v(z)-\lambda_v(z')|^2 -\frac 1 d \left(\sum_{v\in \VEq} \lambda_v(z)-\lambda_v(z')\right)^2,
$$
which concludes the proof in the case of $\TEq$ since $\cH_\TEq = \Id$ and since the barycentric coordinates of $z$ and of $z'$ sum to $1$.

We now consider an arbitrary simplex $T$, and an affine change change of coordinates $\Phi$ such that $\Phi(T) = \TEq$, $\Phi(z) = \phi z+ z_0$ where $\phi\in \GL_d$ and $z_0\in \R^d$. We have $\cH_T = \phi^\trans \phi$ according to \iref{invcH}, hence for all $z,z'\in T$
$$
 |\Phi(z) - \Phi(z')| = |\phi(z-z')| = \|z-z'\|_{\cH_T}.
$$
Furthermore the barycentric coordinates of $z$ and $z'$ in $T$ are the same as those of $\Phi(z)$ and $\Phi(z')$ in $\Phi(T) = \TEq$. This implies \iref{eqNormLambda} and concludes the proof of this lemma.
\sq

The next proposition immediately implies Point iii) of Proposition \ref{propMetGen}. Indeed for any mesh $\cT\in \bT_{g,C_0}$ the metric $d C_0^{10} H_\cT^g$ belongs to $\bH_g$ and is $C_0^6 \sqrt d$ equivalent to $\cT$.

\begin{prop}
\label{propHTG}
For any $\cT\in \bT_{g,C_0}$ the metric $H_\cT^g$ is $C_0$-adapted to $\cT$, and $d C_0^{10} H_\cT^g\in \bH_g$.
\end{prop}

\proof
We consider a simplex $T\in \cT$, and we recall that for any neighbor $T'$ of $T$ one has 
$$
C_0^{-2} \cH_T \leq \cH_{T'} \leq C_0^2 \cH_T.
$$
Averaging these matrices as in \iref{eqHcTg} we obtain for any vertex $v$ of $T$
\be
\label{eqHTHv}
C_0^{-2} \cH_T \leq H_\cT^g(v)\leq C_0^2 \cH_T.
\ee
Averaging with respect to the barycentric coordinates of a point $z\in T$ we eventually obtain 
\be
\label{eqHTHz}
C_0^{-2} \cH_T \leq H_\cT^g(z)\leq C_0^2 \cH_T,
\ee
which establishes as announced that the metric $H_\cT^g$ is $C_0$-adapted to $\cT$.

We now establish the regularity property of $H_\cT^g$, and for that purpose we consider two points $z,z'\in T$ and a vector $u\in \R^d\sm\{0\}$. We thus have 
\begin{eqnarray*}
\frac {\|u\|^2_{H_\cT^g(z)}} {\|u\|^2_{H_\cT^g(z')}} &=& \frac {\sum_{v\in V} \lambda_v(z) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2} \\
&=& 1+ \frac {\sum_{v\in V} (\lambda_v(z)-\lambda_v(z')) \|u\|_{H_\cT^g(v)}^2}{\sum_{v\in V} \lambda_v(z') \|u\|_{H_\cT^g(v)}^2}\\
&\leq& 1+ C_0^4 \frac{\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|}{\sum_{v\in V} \lambda_v(z')}\\
& \leq & 1+C_0^4 \sqrt {(d+1)\sum_{v\in V} |\lambda_v(z)-\lambda_v(z')|^2}\\
&=& 1+C_0^4 \sqrt d \| z-z'\|_{\cH_T},
\end{eqnarray*}
where we used \iref{eqHTHv} in the third line, Cauchy-Schwartz inequality in the fourth line, and Lemma \iref{lemmaNormLambda} in the fifth line.
Proceeding similarly for  $\|u\|_{H_\cT^g(z')}/\|u\|^2_{H_\cT^g(z)}$ we obtain
\begin{eqnarray*}
d_\times (H_\cT^g(z), H_\cT^g(z')) &=& \max_{u\neq 0} \left|\ln \|u\|_{H_\cT^g(z)} - \ln \|u\|_{H_\cT^g(z')}\right|\\
&\leq& \frac 1 2\ln (1+C_0^4 \sqrt d \|z-z'\|_{\cH_T}) \\
&\leq& \frac {C_0^4 \sqrt d} 2 \|z-z'\|_{\cH_T}.
\end{eqnarray*}
Hence according to \iref{eqHTHz} and \iref{eqDilNorm} for all $z\in \interior (T)$
$$
\dil_z(H_\cT^g)_\times = \dil_z(H_\cT^g\sep d_\times, \|\cdot \|_{H(z)}) \leq C_0 \dil_z(H_\cT^g\sep d_\times, \|\cdot \|_{\cH_T})  \leq C_0^5 \sqrt d.
$$
The metric $H := d C_0^{10} H_\cT^g$ thus satisfies $\dil_z(H)_\times = (dC_0^{10})^{-1/2}\dil_z(H_\cT^g)_\times \leq 1$ for any point $z$ in the interior of any simplex $T\in \cT$.
If follows from Corollary \ref{corolLipNoGamma} that $H \in \bH_g$, which concludes the proof.
\sq

We associate to any mesh $\cT\in \bT$ a metric $H_\cT^i$ defined as follows : for all $z\in \R^d$, 
$$
H_\cT^i(z) := \|H_\cT^g(z)\| \Id.
$$
The next result immediately implies Point i) of Proposition \ref{propMetGen}. Indeed for any mesh $\cT\in \bT_{i,C_0}$ the metric $d C_0^{10} H_\cT^i$ belongs to $\bH_i$ and is $C_0^7 \sqrt d$ equivalent to the mesh $\cT$.

\begin{corollary}
For any mesh $\cT\in \bT_{i,C_0}$ the metric $H_\cT^i$ is $C_0^2$-adapted to the mesh $\cT$, and $d C_0^{10} H_\cT^i \in \bH_i$.
\end{corollary}

\proof
We have for any simplex $T\in \cT$ %For any matrix $M\in S_d^+$ we have $\|M^{-1}\|^{-1} \Id \leq M \leq \|M\| \Id$. We therefore obtain for any simplex $T\in \cT$
\be
\label{eqcHNormcH}
C_0^{-2} \|\cH_T\| \Id\leq \frac{\|\cH_T\|} {\rho(T)^2} \Id = \|\cH_T^{-1}\|^{-1} \Id \leq \cH_T \leq \|\cH_T\|\Id.
\ee
For any point $z\in T$ we obtain since $C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z)$
$$
C_0^{-2} H_\cT^i(z) = C_0^{-2} \|H_\cT^g(z)\| \Id \leq \|\cH_T\| \Id \leq C_0^2 \|H_\cT^g(z)\| =C_0^2 H_\cT^i(z).
$$
Combining this with \iref{eqcHNormcH} we obtain
$$
C_0^{-4} H_\cT^i(z) \leq \cH_T \leq C_0^2 H_\cT^i(z),
$$
which establishes as announced that the metric $H_\cT^i$ is $C_0^2$ equivalent to the mesh $\cT$.

According to Proposition \ref{propHTG} we have $d C_0^{10} H_\cT^g\in \bH_g$. Corollary \ref{corolLipNorm} thus implies that $d C_0^{10} H_\cT^i\in \bH_i$, which concludes the proof of this proposition.
\sq

Before turning to the case of quasi-acute metrics we prove a lemma on the neighborhood of a simplex in a graded mesh. For any mesh $\cT\in \bT$ and any closed set $E\subset \R^d$ the neighborhood $V_\cT(E)$ of $E$ in $\cT$ is  defined as the union of all simplices $T\in \cT$ which intersect $E$: 
$$
V_\cT(E) := \cup_{\substack{T\in \cT\\T \cap E \neq \emptyset}} T.
$$

\begin{prop}
\label{propNeighborT}
Let $\cT\in \bT_{g,C_0}$ and let $T \in \cT$, then for all $x\in T$ and all $y \in \R^d \sm V_\cT(T)$ we have 
$$
\|x-y\|_{\cH_T} \geq (C_0\sqrt d)^{-1}.
$$
\end{prop}

\proof
We consider the function $\vp : \R^d \to \R$ which is piecewise linear on the mesh $\cT$, and which satisfies for any vertex $v$ of the mesh $\cT$
$$
\vp(v) = 
\left\{
\begin{array}{cl}
1 & \text{ if } v\in T,\\
0 & \text{ if } v \notin T.
\end{array}
\right.
$$
We denote by $V'$ the collection of vertices of a simplex $T'\in \cT$, and by $(\lambda_v(z))_{v\in V'}$ the barycentric coordinates of a point $z\in T'$.
We have for any $z,z'\in T'$
\begin{eqnarray*}
|\vp(z)- \vp(z')| &\leq& \sum_{v \in V'} |\lambda_v(z)-\lambda_v(z')| \vp(v)\\
& \leq &\sqrt{(d+1) \sum_{v\in V'} |\lambda_v(z)-\lambda_v(z')|^2} \\
&= &\sqrt d \|z-z'\|_{\cH_{T'}}.
\end{eqnarray*}
Since $\vp$ is identically $0$ on $T'$ if $T\cap T' = \emptyset$, and since $\cH_{T'} \leq C_0^2 \cH_T$ otherwise, we obtain for any $z,z'\in T'$
$$
|\vp(z)- \vp(z')| \leq C_0\sqrt d \|z-z'\|_{\cH_{T}}.
$$
Therefore $\dil_z(\vp, \|\cdot\|_{\cH_T})$ for any $T'\in \cT$ and any $z\in T'$, which implies that $\vp : (\R^d, \|\cdot \|_{\cH_T})  \to \R$ is $C_0\sqrt d$-Lipschitz according to Corollary \ref{corolLipNoGamma}.
For any $x\in T$ and any $y\in \R^d\sm V_\cT(T)$ we have $\vp(x) = 1$, $\vp(y) = 0$, thus $1 \leq C_0\sqrt d \|x-y\|_{\cH_T}$ which concludes the proof of this proposition.
\sq

We assume from this point that the dimension is $d=2$. %, and we thus restrict our attention to the bi-dimensional triangulations.
For each triangulation $\cT\in \bT$ we define a function $s_\cT : \R^2 \to \R_+^*$ and a metric $H_\cT^a\in \bH$ as follows : for all $z\in \R^2$
\begin{eqnarray}
s_\cT(z) &:=& \inf_{z'\in \sR^2} |z-z'| + \|H_\cT^g(z')^{-\frac 1 2}\|\\
\label{defHTA}
H_\cT^a(z) &:=& \max\{s_\cT(z)^{-2} , \, H_\cT^g(z)\}.
\end{eqnarray}

We assume from this point that the dimension is $d=2$.
The next proposition immediately implies Point ii) of Proposition \ref{propMetGen}. Indeed the metric $32 C_0^{10} H_\cT^a$ belongs to $\bH_a$ and is $32 C C_0^{10}$ adapted to the mesh $\cT$.
\begin{prop}
\label{propHTA}
For any $C_0 \geq 1$ there exists $C=C(C_0)$ such that the following holds.
For any $\cT\in \bT_{a,C_0}$ the metric $H_\cT^a$ is $C$-adapted to the mesh $\cT$, and $32 C_0^{10} H_\cT^a\in \bH_a$.
\end{prop}

The fact that $32 C_0^{10} H_\cT^a\in \bH_a$ directly follows from the fact that $2 C_0^{10} \bH_\cT^g\in \bH_g$ and from Corollary \ref{corolHgToHa}. 

We define $d_\cT(z) := \|H_\cT^g(z)^{-\frac 1 2}\|$ for each $z\in \R^2$. We establish below that there exists a constant $\delta = \delta(C_0)$, $0< \delta\leq 1$, such that for all $z,z'\in \R^2$
\be
\label{eqRegDT}
\text{ if } |z'-z| \leq \delta d_\cT(z) \stext{ then }  d_\cT(z') \geq \delta d_\cT(z).
\ee
Before turning to the proof of this property we show how it leads to the proof of Proposition \ref{propHTA}.
For all $z\in \R^d$ we have 
$$
s_\cT(z) = \inf_{z\in \sR^2} |z-z'|+d_\cT(z)  \geq \inf_{z'\in \sR^2} \min \{|z-z'|, \, d_\cT(z')\} \geq \delta d_\cT(z'),
$$
indeed $|z-z'|\geq \delta d_\cT(z)$ or $d_\cT(z') \geq \delta d_\cT(z)$ for any $z'\in \R^d$ according to \iref{eqRegDT}.
Combining this with the definition \iref{defHTA} of $H_\cT^a$ we obtain for all $z\in \R^2$
$$
\delta^2 H_\cT^a(z) \leq H_\cT^g(z)\leq H_\cT^a(z). 
$$
Recalling that $H_\cT^g$ is $C_0$-adapted to the mesh $\cT$, see proposition \ref{propHTG}, we obtain for all $T\in \cT$ and all $z\in T$ 
$$
\delta^2 C_0^{-2} H_\cT^a(z) \leq C_0^{-2} H_\cT^g(z) \leq \cH_T \leq C_0^2 H_\cT^g(z) \leq C_0^2 H_\cT^a(z)
$$
which establishes that the metric $H_\cT^a$ is $C_0/\delta$ adapted to the mesh $\cT$, and concludes the proof of Proposition \ref{propHTA}.\\

For notational simplicity we denote from this point $H := H_\cT^g$ and $C_1 := \sqrt 2 C_0^5$, hence $C_1^2 H \in \bH_g$ and $\cT$ is $C_0$ adapted to $H$. 
It follows from the inclusion \iref{eqTET} that 
$$
C_0^{-1} \|H(z)^{-\frac 1 2}\| \leq \| \cH_T^{-\frac 1 2}\| \leq \diam(T) \leq 2\| \cH_T^{-\frac 1 2}\| = \diam(\cE_T) \leq 2C_0 \|H(z)^{-\frac 1 2}\|,
$$
for any $T\in \cT$ and $z\in T$, which implies 
$$
\diam(T)/(2C_0)\leq d_\cT(z) \leq C_0\diam(T).
$$
The quantity $d_\cT(z)$ should therefore be heuristically regarded as the diameter of the triangle $T\in \cT$ containing $z$, and property \iref{eqRegDT} states that the diameters are constrained to vary in a Lipschitz manner in a quasi-acute triangulation.


We now turn to the proof of \iref{eqRegDT}, and for that purpose we introduce some notations.
For each $u\in \R^2$, we denote by $u^\perp$ the vector obtained by rotating $u$ by $\cPi/2$ in direct trigonometric orientation.
For each segment $e=[\omega-u, \omega+u]\subset \R^2$ we define the diamond $\lozenge(e)$ of $e$ as follows
$$
\lozenge(e) := \{z\in \R^2 \sep |\<z-\omega,u\>|+ C_0 |\<z-\omega,u^\perp\>| < |u|^2\}.
$$
This set is illustrated on Figure \ref{figLozenge} (left).

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/LozengeJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/SeqZnJenny.pdf}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Dessins/Jenny/TRedJenny.pdf}
\caption{An edge $e$ and the set $\lozenge(e)$ (left), sequence $(z_n)_{n \geq 0}$ (center), diameter of a triangle intersecting $\lozenge(e)$ (right). \label{figLozenge}}
\end{figure}

The next lemma considers a triangulation $\cT'$ on which the measure of sliverness is uniformly bounded by $C_0$, and compares the length an edge $e$ of $\cT'$ with the diameter of the triangles in $\cT'$ which intersect $\lozenge(e)$.

\begin{lemma}
\label{lemmaUUp}
Let $\cT'\in \bT$ be a triangulation such that $S(T) \leq C_0$ for all $T\in \cT'$. Let  $e=[\omega-u, \omega+u]$ be an edge of $\cT'$.
Then there is no vertex in the diamond $\lozenge(e)$, and for all $z\in \lozenge(e)$ and any triangle $T\in \cT'$ containing $z$, there exists an edge $e'= [\omega'-u', \omega'+u']$ of $T$ satisfying  
$$
2 |u'| \geq |u| -C_0 |\<z-\omega,u^\perp/ |u|\>
%2 |\<u,u'\>| \geq |u|^2 - C_0 |\det (z,u)|.
$$
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$, and we assume up to a translation and a rotation that $\omega = 0$ and $u = u_y$.
We recall that for any triangle $T$, with maximal angle $\theta$, the measure of sliverness $S(T)$ has the following expression
$$
S(T) = \max\{1, \tan(\theta/2)\}.
$$
We assume for contradiction that there exists a vertex $v_0 = (x_0,y_0)\in \lozenge(e)$, and we assume without loss of generality that $x_0<0$. We consider a vertex $v_1 = (x_1,y_1)$ of $\cT'$ such that $\<v_1-v_0,  u_x\> \geq 0$ and such that the angle
$$
\theta_0 :=  \varangle (v_1-v_0, \, u_x) = \arccos\left(\frac{\<v_1-v_0,  u_x\>}{|v_1-v_0| |u_x|} \right)
$$
has the smallest possible value. By construction there exists a triangle $T\in \cT$ containing $v_0$ and $v_1$ which has an angle  larger or equal or equal than $2\theta_0$ at the vertex $v_0$. It follows that $\tan \theta_0 \leq S(T) \leq C_0$, and therefore  
$$
|y_1-y_0| \leq  (x_1 - x_0)\tan \theta_0\leq C_0 (x_1-x_0).
$$
Proceeding inductively, as illustrated on Figure \ref{figLozenge} (center), we define a sequence $v_n = (x_n, y_n)$, $n\geq 0$, of vertices of $\cT$ satisfying 
$
|y_{n+1} - y_n| \leq C_0 (x_{n+1} - x_n). 
$
Adding these inequalities together we obtain 
$$
|y_n-y_0|  \leq C_0 (x_n-x_0).
$$
It follows that one of the edges $[v_n, v_{n+1}]$, $n \geq 0$, of the mesh $\cT'$ intersects the edge $e$, which is a contradiction. As announced the diamond $\lozenge(e)$ therefore does not contain any vertex. \\

We now consider a point $z_0 = (x_0,y_0)\in \lozenge(e)$ and we assume without loss of generality that $x_0 \geq 0$. We consider a triangle $T$ containing $z_0$, and an edge $e'= [\omega'-u', \omega'+u']$ of $T$ which is on the left of $z_0$ (in other words the edge $e'$ and the segment $[(0,y_0),(x_0, y_0)]$ joining the point $z_0$ to its orthogonal projection on the edge $e$ intersect). The point $z_0$ and the triangle $T$ are illustrated on Figure \ref{figLozenge} (right).

Since there is no vertex of $\cT'$ in the diamond $\lozenge(e)$, the edge $e'$ intersects the boundary of $\lozenge(e)$ at two points. We denote these points by $(x,y)$ and $(x',y')$, and we assume that without loss of generality that $y\geq 0 \geq y'$.
Observing that $0 \leq x \leq C_0^{-1}$, $0 \leq x'\leq C_0^{-1}$ and $\min\{x,x'\} \leq x_0$ we obtain  
$$
y-y' = (1-C_0 x) - (-1+C_0 x') \geq 1-C_0 x_0.
$$
Since $u = u_y = (0,1)$, $\omega = 0$ and $2 u' = \lambda (x-x', y-y')$ for some $|\lambda| \geq 1$, we obtain 
$$
2|\<u,u'\>| \geq  
y-y' \geq 1-C_0 x_0 = |u|^2 - C_0 |\<z_0-\omega,u\>|,
$$
which concludes the proof of this proposition.
\sq

\begin{figure}
\centering
\includegraphics[width = 4.5cm, height = 4cm]{\pathPic/Dessins/Jenny/LozengeCarreDeltaJenny.pdf}
\includegraphics[width = 2.5cm, height = 4cm]{\pathPic/Dessins/Jenny/CarreDeltaCarreEJenny.pdf}
\caption{An edge $e$, the diamond $\lozenge(e)$ and the rectangle $\square_\delta$ involved in Lemma \ref{lemmaRect} (left), the rectangles $\square(e)$ and $\square_\delta$.
\label{figSquare}
}
\end{figure}

From this point $\cT'$ denotes a $C_0$-refinement of the quasi-acute mesh $\cT\in \bT_{a,C_0}$, which satisfies $S(T) \leq C_0$ for all $T\in \cT'$. The next lemma involves a rectangular set $\square(e)$ associated to an edge $e$ of $\cT'$, illustrated on Figure \ref{figSquare} (right), which contains $e$ in its interior, in contrast to the set $\lozenge(e)$ appearing in the previous proposition.  

We have according to \iref{eqLocalNorm} for all $z,u\in \R^d$
\be
\label{eqRegDT}
d_\cT(z+u) \geq (1-C_1 \|u\|_{H(z)} ) d_\cT(z).
\ee

\begin{lemma}
\label{lemmaRect}
There exists a constant $\delta_0 = \delta_0(C_0, d)>0$ such that the following holds.
We define the rectangle $\square(e)$ associated to an edge $e = [\omega-u, \, \omega+u]$ of $\cT'$ as follows
$$
\square(e) = \{z\in \R^2 \sep |\<z-\omega, u\>|\leq (1+\delta_0)|u|^2 \text{ and } |\<z-\omega,u^\perp \>| \leq \delta_0 |u|^2\},
$$
%where $\delta_0 = \delta_0(C_0):= ??1/(2C_0) >0$ is a constant specified in the proof.
We have $d_\cT(z) \geq \delta_0|u|$ for all $z\in \square(e)$.
\end{lemma}

\proof
We denote by $u_x := (1,0)$ and $u_y := (0,1)$ the canonical basis of $\R^2$. 
Up to a rotation and a translation, we may again assume that $\omega = 0$ and $u = u_y=(0,1)$.
We consider a triangle $T\in \cT$ containing the edge $e$ (note that $e\subset T$ but that $e$ may not be an edge of $T$, since we only known that $e$ is an edge in $\cT'$).

The inclusion $e\subset T \subset \cE_T$ implies that $d_\cT(z) \geq C_0^{-1}$ for all $z\in e$. Hence for all $z\in e$ and all $u\in \R^d$, using \iref{eqRegDT},
$$
d_\cT(z+u) \geq  (1-C_1 \|u\|_{H(z)}) C_0^{-1}\geq (1-C_1C_0 \|u\|_{\cH_T})C_0^{-1}.
$$
We define $C_2 := 4C_0C_1$ and we observe that, since $\|u_y\|_{\cH_T} \leq 1$, any point of the rectangle 
\be
\label{eqRectGrad}
\left[\frac {-1}{C_2 \|u_x\|_{\cH_T}}, \,\frac 1 {C_2 \|u_x\|_{\cH_T}}\right] \times \left[-(1+C_2^{-1}), \, 1+C_2^{-1}\right].
\ee
can be written under the form $z+u$ where $z\in e$ and $\|u\|_{\cH_T} \leq 1/(2C_0C_1)$. We thus have  
$
d_\cT(z') \geq 1/(2C_0)
$
 on this rectangle.

We introduce a small constant $\delta = \delta(C_0)>0$ which is specified later in the proof. It follows from the above argument that the proof of this lemma is complete if $\|\cH_T\| \leq \delta^{-2}$, with $\delta_0 := \min \{\delta/C_2, \, 1/(2C_0)\}$.
We thus assume from this point that $\|\cH_T\|\geq \delta^{-2}$.\\

We assume that $\delta< C_0^{-1}$ and we define the rectangle
$$
\square_\delta := [-\delta, \delta] \times [1-C_0 \delta, -1+C_0 \delta],
$$
which is included in $\overline \lozenge(e)$ by construction.
Since $C_1^2 H\in \bH_g$, the function $z\mapsto \|H(z)\|^{-\frac 1 2}$ is $C_1$-Lipschitz according to Corollary \ref{corolLipNorm}. We thus have for all $z = (x,y)\in \square_\delta$
\be
\label{defr0}
\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2}+C_1|x|\leq r_0(\delta) := (C_0+C_1)\delta.
%\|u_x\|_{H(z)} \geq \|u_x\|_{H(y,0)}(1-C_1 |x| \|u_x\|_{H(y,0)}) \geq C_*(1-C_1 C_0 \delta_* C_*),
%\|H(z)\|^{-\frac 1 2} \leq \|H(0,y)\|^{-\frac 1 2} + C_1 |x|
\ee
On the other hand it follows from Lemma \ref{lemmaUUp} that any $z = (x,y)\in \square_\delta$ is contained in a triangle containing an edge $e' = [\omega'-u', \omega'+u']$ such that $|u'| \geq (1-C_0 \delta)/2$. We thus have 
$$
1 \geq \|u'\|_{\cH_{T'}} \geq \frac{|u'|}{ \|\cH_{T'}^{-\frac 1 2}\|} \geq \frac{1-C_0 \delta}{2 \|\cH_{T'}^{-\frac 1 2}\|} 
$$
and therefore 
%of length at least $T'\in \cT$ satisfying $\|\cH_{T'}^{-\frac 1 2}\| \geq (1-C_0 \delta_*)/2$, hence 
\be
\label{defR0}
d_\cT(z) = \|H(z)^{-\frac 1 2}\| \geq C_0^{-1} \|\cH_{T'}^{-\frac 1 2}\|  \geq  R_0(\delta) := (1-C_0 \delta)/(2C_0). %\det (z,u_y)
\ee
For all $z\in \square_\delta$, we denote by $\theta(z) = (\cos \Theta(z), \sin \Theta(z))$, $\Theta(z)\in [0, \cPi]$, the direction of the eigenvector associated to the small eigenvalue of $H(z)$, in such way that 
\be
\label{eqNormTheta}
\|\theta(z)\|_{H(z)} = \|H(z)^{-\frac 1 2}\|^{-1} = d_\cT(z)^{-1}.
\ee
According to \iref{eqRegDT} we have for all $z\in \square_\delta$ and all $r\in \R$
$$
d_\cT(z+r \theta(z)) \geq  d_\cT(z) (1-|r| C_1 /d_\cT(z)).
$$
For all $z\in \square_\delta$ and all $r\in \R$ such that $|r|\leq R_1(\delta) := R_0(\delta)/(2C_1)$ we thus obtain
\be
\label{DegDTR0}
d_\cT(z+r\theta(z)) \geq R_0(\delta)(1-|r|C_1/R_0(\delta))\geq R_0(\delta)/2.
\ee

We have for any $(0,y)\in e$
$$
C_0 \geq C_0 \|u_y\|_{\cH_T} \geq \|u_y\|_{H(0,y)} \geq |\cos \Theta(0,y)| \sqrt{\|H(0,y)\|} \geq |\cos \Theta(0,y)| /(\delta C_0) ,
$$
hence 
$
|\cos \Theta(0,y)| \leq  C_0^2 \delta.
$
For all $z\in \square_\delta$ we have according to Corollary \ref{corolDilThetaG} %Theorem \ref{th2Spaces} 
$$
(R_0(\delta)-r_0(\delta)) \dil_z(\Theta) \leq  (\|H(z)^{-\frac 1 2}\| - \|H(z)\|^{-\frac 1 2}) \dil_z(\Theta) \leq 2C_1.
$$
Hence we obtain for all $z= (x,y)\in \square_\delta$  
$$
(R_0(\delta)-r_0(\delta)) |\Theta(z) - \Theta(0,y)| \leq 2C_1 |x|\leq 2C_1 \delta,
$$
hence since $t \mapsto \cos t$ is a Lipschitz function %, since $\cos : [0, \cPi/2]\to \R$ is convex
\be
\label{defTheta0}
|\cos \Theta(z)| \leq \cos \Theta_0(\delta) := C_0^2 \delta + \frac{2C_1\delta}{R_0(\delta)-r_0(\delta)}.
\ee
%We have according to \iref{eqLocalNorm} for all $z\in \square_\delta$ and all $r\geq 0$ such that $C_1r\|\theta\|_{H(z)}<1$,
%\begin{eqnarray*}
%|\ln d_\cT(z+r \theta(z)) - \ln d_\cT(z)| &\leq& d_\times (H(z+r\theta(z)),H(z))\\
%&\leq& -\ln (1-C_1r\|\theta\|_{H(z)})\\
%&=& -\ln (1-C_1r/d_\cT(z)),
%\end{eqnarray*}
%therefore 
%$$
%
%$$
It follows that $d_\cT(z')\geq R_0(\delta)/2$ for all $z'$ in the set 
$$
\{z+r\theta(z) \sep z\in \square_\delta,\, |r|\leq R_1(\delta)\} \supset [-\delta_0,\delta_0]\times [-(1+\mu_0),1+\mu_0]
$$
where 
\be
\label{eqD0MU0}
\delta_0 := \delta - r \cos \Theta_0(\delta) \stext{ and }  \mu_0 := -C_0 \delta+ r \sin \Theta_0(\delta)
\ee
and where the constant $0 \leq r\leq R_1(\delta)$ can be freely chosen.
The rest of the proof consists in choosing appropriate constants $\delta$ and $r$.\\

As $\delta \to 0$ we have $r_0(\delta)\to 0$, $R_0(\delta) \to 1/(2C_0)$ and $\cos\Theta_0(\delta) \to 0$. We thus choose $\delta = \delta(C_0,d)>0$ sufficiently small in such way that 
\be
\label{eqRCS}
R_0 \geq 1/(4C_0)
, \quad
\cos \Theta_0 \leq 1/(8C_0)
, \quad
\sin \Theta_0 \geq 1/2
.
\ee
and such that $r := 4C_0 \delta$, is smaller than $R_1(\delta)= R_0(\delta)/(2C_1)$. Injecting this choice of $r$ and \iref{eqRCS} in \iref{eqD0MU0} we thus obtain 
$$
\delta_0 \geq \delta/2 \stext{ and }\mu_0 \geq C_0 \delta.
$$
This establishes under the hypothesis $\|\cH_T\|\geq \delta^{-2}$ that  $d_\cT(z) \geq 1/(8C_0)$ for all $z$ in the rectangle 
$$
[-\delta/2, \delta/2]\times [-(1+C_0\delta), 1+C_0 \delta],
$$
which concludes the proof of the proposition.
\sq

Our next intermediate result establishes a technical property on the covering a one dimensional segment by smaller ones.

\begin{lemma}
\label{lemmaCoverSeg}
Let $x_1, \cdots , x_k\in [0,1]$ and let $h_1, \cdots, h_k >0$ be such that 
\be
\label{eqDefXiHi}
[0,1]\subset \bigcup_{1\leq i \leq k} [x_i-h_i, \, x_i+h_i].
\ee
Let $\delta>0$ and let $h_* = h_*(k,\delta) := \exp(1-2k/\delta)/\delta$. Then 
\be
\label{eqInclSeg}
[0,1]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_* \leq h_i}} [x_i-(1+\delta)h_i, \, x_i+(1+\delta)h_i].
\ee
\end{lemma}

\proof
For each $y\in [0,1]$ we denote by $h(y)$ the value $h_i$ associated to the segment $[x_i-h_i, x_i+h_i]$ of smallest length containing $y$.
We thus have 
$$
\int_{[0,1]} \frac {dy} {h(y)} \leq \sum_{1\leq i \leq k} \int_{x_i-h_i}^{x_i+h_i} \frac 1 {h_i} = 2k.
$$
We assume for contradiction that \iref{eqInclSeg} does not hold, and we consider a point $x\in [0,1]$ which does not belong to the right hand side of $[0,1]$. For each $y\in [0,1]$ one of the two following possibilities holds
$$
\delta h(y) < |x-y| \stext{ or } h(y) < h_*.
$$
Integrating we obtain 
$$
\int_0^1 \frac {dy} {h(y)}  \geq \int_0^1 \frac {dy} {\max\{|x-y|/\delta,\, h_*\}}.
$$
The minimum value of the right hand side is attained for $x=0$ or $1$ and equals 
$$
\int_0^1 \frac {dy}{\max \{|x-y|/\delta, h_*\}} = \int_0^{\delta h_*} \frac 1 h_* + \int_{\delta h_*}^1 \frac \delta ydy = \delta(1-\ln(\delta h_*))
$$
Thus $2k>\delta(1-\ln(\delta h_*))$, which contradicts the definition of $h_*$. This concludes the proof of this lemma.
\sq

Under the hypotheses of Lemma \ref{lemmaCoverSeg} we thus have
\be
\label{eqInclSegDouble}
[-h_*\delta,\, 1+h_*\delta]\subset \bigcup_{\substack{1\leq i \leq k\\ \text{s.t. } h_i \leq h_*}} [x_i-(1+2\delta)h_i, \, x_i+(1+2\delta)h_i].
\ee


We now conclude the proof of Proposition \ref{propHTA}.
We consider a point $z\in \R^2$ contained in a triangle $T\in \cT$, and we denote by $\cT$ the longest edge $e$ of $T$. Up to a rotation and a translation, we may assume that $e=[0, u_x]$ joins the origin of $\R^2$ to the the vector $u_x := (1,0)$.
Since the triangulation $\cT'$ is a $C_0$-refinement of $\cT$, the edge $e$ of $T$ is built of $k \leq C_0$ edges $(e_i)_{1 \leq i \leq k}$ of $\cT'$,
$$
e_i = [(x_i-h_i)u_x,\,  (x_i +h_i) u_x].
$$
The triangle $T$ and the edges $(e_i)_{1\leq i\leq k}$ are illustrated on Figure \ref{figTFlat} (left).

\begin{figure}
\centering
\includegraphics[width = 7cm, height = 1.5cm]{\pathPic/Dessins/Jenny/TFlatJenny.pdf}
\includegraphics[width = 8cm, height = 2.5cm]{\pathPic/Dessins/Jenny/cupCarresJenny.pdf}
\caption{
A triangle $T\in \cT$ and the edges $(e_i)_{1\leq i \leq k}$ of $\cT'$ contained in $T$ (left), the set \iref{eqRectHoDo} (right). 
\label{figTFlat}}
\end{figure}

We define $h_* := h_*(C_0, \delta_0/2) = 2\exp(1-4C_0/\delta_0)/\delta_0$, where $\delta_0$ is the constant from Lemma \ref{lemmaRect}, and we obtain using \iref{eqInclSegDouble} that 
\be
\label{eqRectHoDo}
\bigcup_{h_* \leq h_i} \square(e_i) \supset \left[-\frac{h_* \delta_0} 2, 1+ \frac{h_* \delta_0} 2\right] \times [-h_* \delta_0, h_* \delta_0],
\ee
This set is illustrated on Figure \ref{figTFlat} (right).
Since $e$ is the longest edge of $T$, the angles of $T$ at the extremities of $e$ are acute.
Furthermore the height $h$ of $T$ orthogonal to the edge $e = [0,u_x]$ satisfies 
$$
h/2 = |T|  = \frac{|\TEq|} { \sqrt {\det \cH_T}} = \frac{|\TEq|}{\sqrt{\|\cH_T\| \|\cH_T^{-1}\|^{-1}}}  = \frac{|\TEq| \|\cH_T^{-1}\|}{\rho(T)} \geq \frac{|\TEq|}{4 \rho(T)} .
$$
Hence we obtain with $c := |\TEq|/8$ the inclusion
\be
\label{eqTRectRho}
T \subset [0,1] \times [-c/\rho(T), c/\rho(T)]
\ee
We distinguish two cases depending on the value of $\rho(T)$. If $\rho(T) \geq 2 c/(h_* \delta_0)$ we obtain combining \iref{eqRectHoDo} and \iref{eqTRectRho} that $d_\cT\geq h_*\delta_0$ on the set 
$$
z+ \left[-\frac {h_*\delta_0} 2, \frac {h_*\delta_0} 2\right]^2.
$$
Since $d_\cT(z) \leq C_0 \diam(T) = C_0$ this implies \iref{eqRegDT} with $\delta = h_* \delta_0 /(2C_0)$.
One the other hand if $\rho(T) \leq  \rho_0 := 2c/(h_*\delta_0)$, then 
$$
\|H(z)\|^\frac 1 2 \leq C_0 \|\cH_T\|^\frac 1 2 \leq \rho_0 C_0 \|\cH_T^{-\frac 1 2}\|^{-1} \leq \rho_0 C_0^2 \|H(z)^{-\frac 1 2}\|^{-1} \leq \frac{C_0^2 \rho_0}{d_\cT(z)}
$$
which implies for any vector $u\in \R^2$
$$
\frac{d_\cT(z+u)}{d_\cT(z)} \geq  1-C_1 \|u\|_{H(z)} \geq 1-\frac{C_* |u|}{d_\cT(z)}, 
$$
where $C_* := C_1 \rho_0 C_0^2$, which implies \iref{eqRegDT} with the constant $\delta := 1/(2C_*)$. This concludes the proof of Proposition \ref{propHTA}.

\section{From metric to mesh}
\label{secMetToMesh}
\label{secMeshGen}

This section is devoted to the proof of the following result, on the generation of a mesh from a metric.
\begin{prop}
\label{propMeshGen}
There exists $C_0 = C_0(d)$ such that the following holds: 
\begin{enumerate}[i)]
\item For any $H\in \bH_i$ there exists $\cT \in \bT_{i,C_0}$ which is $C_0$-adapted to $H$.
\item If $d=2$, then for any $H \in \bH_a$ there exists $\cT\in \bT_a$ which is $C_0$-adapted to $\cT$.
\item If $d=2$, then for any $H \in \bH_g$ there exists $\cT\in \bT_g$ which is $C_0$-adapted to $\cT$.\end{enumerate}
\end{prop}

Point {\it i)} is established in the \S\ref{secMeshGenI}, Point {\it iii)} in \S \ref{secMeshGenG} an eventually Point {\it ii)} in \S \ref{secMeshGenA}.

%We consider in these proofs a metric $H$ such that $c^2H \in \bH_{\star}$ where $0<c\leq 1$ is a numerical constant and $\star \in \{i,a,g\}$ is a symbol. 

\begin{remark}
\label{remcC}
Let $\star \in \{i,a,g\}$ and let $1\geq c>0$, $C\geq 1$ be numerical constants. 
Assume that for any metric $H$ such that $c^2 H\in \bH_\star$ there exists a mesh $\cT\in \bT_{\star, C}$ which is $C$ adapted to $H$.
Then for any metric $H'\in \bH_\star$ there exists a mesh $\cT' \in \bT_{\star, C}$ which is $C/c$-adapted to $H'$.
(Indeed, choose a mesh $\cT'$ which is $C$-equivalent to the metric $H'/c^2$, and observe that $\cT'$ is $C/c$-equivalent to $H'$)
\end{remark}


\subsection{Isotropic Mesh generation}
\label{secMeshGenI}

\begin{figure}
\centering
\includegraphics[width = 5cm, height = 5cm]{\pathPic/Dessins/Jenny/THalfSquareJenny.pdf}
\caption{A bidimensional triangulation generated by the isotropic refinement procedure
\label{figHalfSquares}}
\end{figure}

The survey paper \cite{Nochetto} describes a the construction of a hierarchical family of meshes of the rectangular domain 
$
[0,1]^d.
$ 
All these meshes are the refinement of a ``fundamental'' mesh $\cT_0 = \{T_\sigma \sep \sigma \in \Sigma_d\}$, where $\Sigma_d$ stands for the collection of permutations of the set $\{1,\cdots,d\}$, and $T_\sigma$ for the Kuhn simplex
$$
T_\sigma := \{z\in [0,1]^d \sep z_{\sigma(1)} \leq \cdots \leq z_{\sigma(d)}\}.
$$
%A sequence $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $A procedure, guided by the user 
%The ``fundamentalbasic mesh $\cT_0$ of $[0,1]^d$ 
Starting from $\cT_0$, the algorithm described in \cite{Nochetto} produces, guided by the user, a family $(\cT_n)_{n \geq 0}$ of conforming meshes of the cube $[0,1]^d$ proceeding as follows. 
Assume that the mesh $\cT_n$ has already been generated.
%Once the mesh $\cT_n$ is defined, the mesh $\cT_{n+1}$ is obtained as follows.
%\begin{enumerate}
%\item (Marking) The user selects
%\item (Refinement)
%\end{enumerate}
%The mesh $\cT_{n+1}$ is produced from $\cT_n$ as follows 
\begin{itemize}
\item (Marking)
The user selects a subset $\cM_n \subset \cT_n$.
\item (Refinement)
The algorithm generates a $2$-refinement $\cT_{n+1}$ of $\cT_n$,  
$$
\cT_{n+1} := \Refine(\cT_n, \cM_n).
$$
which does not contain any of the marked simplices : $\cT_{n+1} \cap \cM_n = \emptyset.$
\end{itemize}
\noindent

The elements of the meshes $(\cT_n)_{n \geq 0}$ have a very specific structure, which main features are described below.
\begin{property}
\label{propertyIso}
Any simplex $T$ produced by this algorithm possesses the following properties.
\begin{enumerate}[a)]
\item (Discrete Volumes) The volume of $T$ has the form
\be
\label{eqVolTG}
|T| = \frac {2^{-g(T)}}{d!},
\ee
where $g(T)\geq 0$ is an integer called the ``generation'' of $T$.
\item
(Finite number of classes)
The simplex 
$$
2^{\frac{g(T)} d} (T-z_T),
$$
%$\frac 1 {d!}$, 
belongs to a finite family $\gT_0$ of simplices.
%\item
%(Vertices lie on a grid)
%The vertices of $T$ lie on the grid
%$$
%2^{-\left\lceil \frac {g(T)} d\right\rceil} \Z^d
%$$
\end{enumerate}
\end{property}
The survey paper \cite{Nochetto} also contains a result, Proposition 4.1, which establishes that $\cT_{n+1} := \Refine(\cT_n, \cM_n)$ is a \emph{local} refinement of $\cT_n$ in the following sense: for all $T'\in \cT_n \sm \cT_{n+1}$ there exists $T\in \cM_n$ such that 
\be
\label{eqDG}
g(T)\geq g(T') \stext{ and } d(T,T') \leq D \, 2^{-g(T')/d},
\ee
where $D = D(d)$ is a fixed constant and where 
$$
d(T,T') := \min\{|z-z'| \sep z\in T, \, z'\in T'\}.\\
$$

The next lemma shows that this refinement algorithm can be used to produce a conforming isotropic mesh $\cT$ of the unit cube $[0,1]^d$, such that the diameters $\diam(T)$, $T\in \cT$, are specified by a given Lipschitz function.

\begin{lemma}
\label{lemmaSCube}
%There exists $C=C(d)$ such that the following holds.
Let $s:[0,1]^d\to  (0,\sqrt d]$ be a $c$-lipschitz function, where $0<c\leq 1$. Let $(\cT_n)_{n \geq 0}$ be the sequence of meshes produced by the algorithm when the collection $\cM_n\subset \cT_n$ of marked simplices is defined as follows:
\be
\label{defMn}
\cM_n := \left\{T\in \cT_n \sep \min_T s < \diam(T)\right\}.
\ee
Then the sequence of meshes stabilizes : there exists $N\geq 0$ such that $\cT_n = \cT_N$ for all $n \geq N$. Furthermore we have for all $T\in \cT_N$ and all $z\in T$
\be
\label{eqEquivCube}
\diam(T) \leq s(z) \leq K_c \diam(T).
\ee
where 
\be
\label{defKc}
K_c := 2^\frac 1 d \frac {D_+ (1+c) + c D}{D_-}
\ee
in which $D_+ := \max\{ \diam(T) \sep T \in \gT_0\}$ and $D_- := \min\{ \diam(T) \sep T \in \gT_0\}$.
\end{lemma}

\proof
We first show that for any $n \geq 0$ any $T_*\in \cT_n$ and any $z\in T_*$ we have $s(z) \leq K_c \diam(T_*)$.
Indeed if $T_*\in \cT_0$ then 
$$
s(z) \leq \sqrt d =  \diam(T_*) \leq K_c \diam(T_*)
$$
since $K_c\geq 1$ and since $s$ is uniformly bounded by $\sqrt d$.

Otherwise $T_*$ has a father $T'$ which was bisected in the refinement process, hence there exists a simplex $T$ such that \iref{eqDG} holds and which was selected for bisection, hence satisfies $\min_T s < \diam(T)$.

We thus obtain for any $z\in T$
\begin{eqnarray*}
s(z) &\leq& \min_T s+ c(\diam(T') + d(T,T'))\\
& \leq & \diam(T)+c(\diam(T') + d(T,T'))\\
& \leq & D_+ 2^{-g(T)/d} + c(D_+2^{-g(T')/d} + D 2^{-g(T')/d})\\
& \leq &  2^{-(g(T_*)-1)} (D_+(1+c)+cD)\\
& \leq & K_c \diam(T_*),
\end{eqnarray*}
which concludes the proof of the right part of \iref{eqEquivCube}.

From the fourth line of this inequality we also obtain an uniform lower bound on the volume of the simplices generated by the refinement procedure
$$
|T_*| = \frac{2^{-g(T_*)}}{d!} \geq c_0 := \frac{\min\{ s(z) \sep z\in [0,1]^d\}}{d! 2^\frac 1 d  (D_+(1+c)+cD)}.
$$
It follows that $\#(\cT_n)$ is uniformly bounded by $1/c_0$, which immediately implies that the sequence $(\cT_n)_{n \geq 0}$ of meshes stabilizes.

Let $N$ be such that $\cT_n = \cT_N$ for all $n \geq N$. We thus have $\cM_N = \emptyset$ and therefore $\diam(T) \leq \min_T s$ for all $T\in \cT_N$, which implies the left part of \iref{eqEquivCube}.
\sq

The rest of this section is devoted to the proof the point i) of Proposition \ref{propMeshGen}.
We thus consider a metric $H\in \bH_i$, and we recall there exists a Lipschitz function $s: \R^d \to \R_+^*$ such that for all $z\in \R^d$
$$
H(z) = \frac \Id {s(z)^2}.
$$
For each $n\geq 0$ we define a function $s_n : [0,1]^d \to \R_+^*$, which is clearly Lipschitz, as follows
\be
\label{defSn}
s_n(z) := 2^{-n} s(2^n (z-z_0))
\ee
where $z_0 = (1/2, \cdots , 1/2)$ is the barycenter of the cube $[0,1]^d$.
%The function $s_n$ is clearly Lipschitz, and 
For all $z\in [0,1]^d$ and all $n \geq 0$ we have 
$$
s_n(z) \leq s_n(z_0) + |z-z_0| \leq 2^{-n} s(0) + \frac {\sqrt d} 2.
$$
The function $s_n$ is therefore uniformly bounded by $\sqrt d$ on $[0,1]^d$ when $n$ is sufficiently large.
We denote by $\cT^n$ the mesh of the cube $[0,1]^d$ described by Lemma \ref{lemmaSCube} for the function $s_n$. We thus have %for all $T\in \cT^n$
\be
\label{eqDiamSn}
\diam(T) \leq s_n(z) \leq C \diam(T) \stext{ for all } T \in \cT^n, \, z\in T.
\ee
where $C=C(d)$ is the constant from Lemma \ref{lemmaSCube}.
We denote by $\cT_n$ the mesh of the cube $[-2^{n-1}, 2^{n-1}]^d$ obtained by translating the mesh $\cT^n$ by $-z_0$ and dilating it by $2^n$. In mathematical terms: % In condensed notations
$$
\cT_n := \{2^n(T-z_0)\sep T \in \cT^n\}.
$$
%$$
%\cT_n := 2^n (\cT^n -z_0).
%$$
In view of \iref{defSn} and \iref{eqDiamSn} we thus have 
\be
\label{eqMinSDiamT}
\diam(T) \leq s(z) \leq C \diam(T) \stext{ for all } T \in \cT_n,\, z\in T,
\ee
We denote by $C_0$ the smallest constant such that for all $T$ in the finite set $\gT_0$ one has 
$$
 \frac{C_0^{-2} \Id}{\diam(T)^2} \leq \cH_T \leq \frac{C_0^2\Id}{C^2\diam(T)^2 },
$$
and we thus obtain for all $T\in \cT_n$ and all $z\in T$
\be
\label{eqHHTIso}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Unfortunately the mesh $\cT_n$ does not cover $\R^d$ but only the cube $[-2^{n-1}, 2^{n-1}]$. 
The next lemma shows that a global mesh $\cT$ of the infinite domain $\R^d$ can be extracted from the sequence of meshes $(\cT_n)_{n\geq 0}$.

\begin{lemma}
\label{lemmaExtractMesh}
Let $(\Omega_n)_{n \geq 0}$ be an increasing sequence of polygonal domains of $\R^d$, which exhausts $\R^d$ in the following sense:
$$
\bigcup_{n \geq 0} \Omega_n = \R^d \stext{ and } \Omega_n \subset \Omega_{n+1} \text{ for all } n\geq 0.
$$
Let $H \in \bH_g$, let $(\cT_n)_{n \geq 0}$ be a sequence of conforming simplicial meshes of the domains $\Omega_n$, and assume that for all $n \geq 0$, all $T\in \cT_n$ and all $z\in T$ one has 
\be
\label{eqHHTConv}
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z).
\ee
Then there exists a mesh $\cT\in \bT$ such that 
$
C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)
$
for all $T\in \cT$ and all $z\in T$.
\end{lemma}

\proof
The heuristic idea of this proof is to ``extract a converging subsequence'' from the sequence $(\cT_n)_{n \geq 0}$ of meshes. Unfortunately meshes are discrete objects of combinatorial nature, and the convergence of meshes has no meaning a priori. We therefore use Lipschitz functions as an intermediate object, for which convergence is well defined and which benefit of a compactness property.\\

We associate a function $\phi_T : \R^d \to \R$ to each simplex $T$, which is defined as follows. The function $\phi_T$ is supported on $T$, and for all $z\in T$ we have in terms of the barycentric coordinates $\lambda_v(z)$ of $z$ with respect to the vertices $v\in V$ of $T$:
%To each simplex $T$ of vertices $V$, and barycentric coordinates $(\lambda_v)_{v\in V}$ we associate the function 
$$
\phi_T(z) := \min_{v\in V} \lambda_v(z).
$$
%The maximum of this function has value $1/d$ and is attained at the barycenter $z_T$ of $T$. Furthermore for each $z\in T$ and each $0\leq r \leq 1$ one easily checks that 
%$$
%\phi_T(z+r(z-z_T)) \geq r/d.
%$$
According to Lemma \ref{lemmaNormLambda}, we have for any $z,z'\in T$ and any $v\in V$
$$
|\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T},
$$
hence 
\be
\label{eqPhiLip}
|\phi_T(z) - \phi_T(z')| \leq \max_{v\in V} |\lambda_v(z) - \lambda_v(z')| \leq \|z-z'\|_{\cH_T}.
\ee

For all $n \geq 0$ we define a function $\phi_n$ on $\R^d$ as follows
$$
\phi_n := \sum_{T \in \cT_n} \phi_T.
$$
It follows from \iref{eqHHTConv} and \iref{eqPhiLip} that for all $T\in \cT_n$ and all $z\in \interior(T)$
$$
\dil_z(\phi_n\sep d_H) \leq C_0.
$$
Since in addition $\phi_n = 0$ on $\R^d \sm \Omega_n$ it follows from corollary \ref{corolLipNoGamma} that $\phi_n : (\R^d,d_H) \to \R$ is $C_0$-Lipschitz. Since the space $(\R^d, d_H)$ is locally compact, due to Proposition \ref{propEuclidRiemann}, Ascoli's compactness theorem states that there exists 
subsequence $(\phi_{n_k})_{k \geq 0}$ which converges uniformly on all compact sets of $\R^d$ to a $C_0$-Lipschitz function $\phi$. 

We therefore assume, up to such an extraction, that 
$
\phi_n \to \phi
$
uniformly on all compact sets of $\R^d$.
We denote by $\cT$ the collection of closures of connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$:
$$
\cT := \left\{ \overline E \sep E \text{ is a connected component of } \{z\in \R^d \sep \phi(z)>0\} \right\}.
$$
For each $z\in \R^d$ and each $n \geq 0$, we denote by $T_n(z)$ the element of $\cT_n$ containing $z$ in its interior if it exists, and $T_n(z) = \emptyset$ otherwise.
If $\phi(z)>0$, then $T_n(z)\neq \emptyset$ for all $n$ sufficiently large, and one easily checks that 
\be
\label{eqTTnz}
T_n(z)\text{ converges in Hausdorff distance to the element }T(z)\in \cT
\ee
 containing $z$. Hence $\cT$ is a collection of simplices, and the convergence $T_n(z)\to T(z)$ in haussdorf distance, combined with the hypothesis $C_0^{-2} H(z) \leq T_n(z) \leq C_0^2 H(z)$, implies that  
\be
\label{eqHHTConv2}
C_0^{-2} H(z) \leq T(z) \leq C_0^2 H(z).
\ee
In order to conclude this proof we need to show that the collection $\cT$ of simplices is a conforming mesh of $\R^d$. We thus have to check the hypotheses of Definition \ref{defSimplMesh}.
The interiors $\interior(T)$, $T\in \cT$ are pairwise disjoint since they are the connected components of the set $\{z\in \R^d \sep \phi(z)>0\}$.
We claim furthermore that $\cT$ covers $\R^d$. Indeed let $z\in \R^d$be arbitrary and for all $n$ let $T_n\in \cT_n$ be such that $z\in T_n$. Since $C_0^{-2} H(z) \leq \cH_{T_n}\leq C_0^2 H(z)$ there exists a subsequence $T_{n_k}$ which converges in the Haussdorf distance to a simplex $T$ containing $z$. We clearly have $T\in \cT$ which establishes as announced that $\cT$ covers $\R^d$.
The fact that $\cT$ is locally finite easily follows from \iref{eqHHTConv2}.\\


We now turn to the proof of the conformity property, and for that purpose we consider an arbitrary Lipschitz function $f : (\R^d, d_H) \to \R$ with compact support. 
Let $T$ be a simplex such that $C_0^{-2} H(z) \leq \cH_T \leq C_0^2 H(z)$. We have for any vertex $v$ of $T$
$$
|f(v) - f(z_T)| \leq d_H(z_T,v) \leq C_0 \|z_T - v\|_{\cH_T} = C_0.
$$
Denoting by $V$ the collection of vertices of $T$ we thus obtain for any $z,z'\in T$
$$
\interp_T f(z) - \interp_T f(z') = \sum_{v\in V} (\lambda_v(z) - \lambda_v(z')) (f(v) - f(z_T)).
$$
Where $\interp_T$ denotes the $\P_1$ (piecewise affine) interpolation on a simplex $T$, and $\interp_\cT$ the $\P_1$ interpolation on a mesh $\cT$.
hence using Lemma \ref{lemmaNormLambda}
\begin{eqnarray*}
|\interp_T f(z) - \interp_T f(z')| &\leq& C_0 \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|\\
 &\leq& C_0 \sqrt{(d+1)  \sum_{v\in V} |\lambda_v(z) - \lambda_v(z')|^2} \\
 &=& C_0 \sqrt d \|z-z'\|_{\cH_T}.
\end{eqnarray*}
The last inequality implies that 
$$
\dil_z(\interp_{\cT_n} f \sep d_H)\leq C_0^2 \sqrt d
$$
for all $T\in \cT_n$ and $z\in \interior(T)$.
Let $n_0 \geq 0$ be such that $\supp(f)\subset \Omega_{n_0}$, which implies that $\interp_{\cT_n} f$ is continuous. It follows from Corollary \ref{corolLipNoGamma} that $\interp_{\cT_n} f : (\R^d, d_H) \to \R$ is $C_0^2\sqrt d$-Lipschitz.

We define 
$
D := \cup_{T \in \cT} \interior(T),
$
and we denote by $\interp_T f : D \to \R$ the function which coincides with $\interp_T f$ on the \emph{interior} of each $T\in \cT$. % (and which is possibly discontinuous at the interfaces between the simplices $T\in \cT$). 
For any $z\in D$ we obtain using \iref{eqTTnz} that $\interp_{\cT_n} f(z) \to \interp_\cT f(z)$, hence for any $z,z'\in D$
$$
|\interp_\cT f(z) - \interp_\cT f(z')| = \lim_{n \to \infty} |\interp_{\cT_n} f(z)-\interp_{\cT_n} f(z')| \leq \sqrt d C_0^2 \, d_H(z,z').
$$
The piecewise interpolant $\interp_T f : D \to \R$ therefore extends to a $\sqrt d C_0^2$-Lipschitz function $\interp_T f : (\R^d, d_H) \to \R$. It easily follows that $\interp_\cT f$ is continuous for any compactly supported $C^1$ function $f$. This property characterizes conforming meshes, hence $\cT\in \bT$ which concludes the proof.
\sq



\begin{corollary}(Bidimensional triangulations)
\label{corolBidimIso}
Assume that the dimension is $d=2$. There exists $c>0$ such that the following holds: if $s: \R^2 \to \R_+^*$ is $c$-Lipschitz, then there exist a mesh $\cT$ of $\R^2$ built of half squares, and such that for all $T\in \cT$ and $z\in T$
\be
\label{eqDT32}
\diam(T) \leq s(z) \leq 3 \diam(T)/2.
\ee
\end{corollary}

\proof
When the dimension is $d=2$, the collection $\gT_0$ of triangles contains only half squares, of area $1/2$, hence  $D_+ = D_- = \sqrt 2$. 

As $s \to 0$ the constant $K_c$ defined by \iref{defKc} tends to $\sqrt 2$. Hence $K_c\leq 3/2$ when $s$ is sufficiently small.
If $s$ is bounded by $\sqrt 2$ on $[0,1]^2$ one may therefore produce a mesh $\cT_*$ of $[0,1]^2$ such that \iref{eqDT32} holds for all $T\in \cT_*$, $z\in T$.

From this point construct as before a sequence of meshes $\cT_n$ of the squares $[-2^{n-1}, 2^{n-1}]$ which satisfies \iref{eqDT32}, and we extract a global mesh $\cT$ of $\R^2$ using Lemma \ref{lemmaExtractMesh}. The triangles $T\in \cT$ still satisfy the inequality \iref{eqDT32} since they are limits in the Haussdorff distance of triangles from the triangulations $\cT_n$.
\sq


\subsection{Graded mesh generation}
\label{secMeshGenG}

We prove in this section a result of bi-dimensional mesh generation, Theorem \ref{thEquiMesh}, which implies Point (iii) of Proposition \ref{propMeshGen}. The key ingredients of this section come from the paper \cite{Shew}.
We assume throughout this section that the dimension is $d=2$.

For that purpose we introduce the notion of equispaced points in an abstract metric space.
 Let $(X,d_X)$ be a metric space and let $\delta>0$, we say that a subset $\cV \subset X$ is $\delta$-equispaced if the following holds.
\begin{enumerate}[a)]
\item (Covering) The distance from an arbitrary point $x\in X$ to $\cV$ is bounded by $1$ : for all $x\in X$
\be
\label{eqCover}
d_X(x, \cV) := \inf\{d_X(x,v) \sep v \in \cV\} \leq 1.
\ee
\item (Separation) The pairwise distances between the points of $\cV$ are larger than $\delta$ : for all $v, v'\in \cV$ such that $v \neq v'$
\be
\label{eqSep}
d_X(v,v') \geq \delta.
\ee
\end{enumerate}

The next lemma establishes the existence of such a set under certain assumptions. \begin{lemma}
\label{lemmaEquiSpaced}
Let $(X,d_X)$ be a metric space in which the closed balls $B'(x,r) := \{y\in X \sep d_X(x,y) \leq r\}$ are compact for all $x\in X$ and $r\geq 0$. 
Let $\cV_0$ subset $X$ be such that $d_X(v,v') \geq 1$ for all $v,v'\in \cV_0$ such that $v\neq v'$. Then there exists a $1$-equispaced set $\cV$ of the metric space $(X,d_X)$, containing $\cV_0$.
\end{lemma}

\proof
We may assume that $\cV_0 \neq \emptyset$, up to including an arbitrary point of $X$, and we choose an  arbitrary  $x_0\in \cV_0$.
We define inductively a sequence $(x_n)_{0 \leq n< N}$ of points and $(\cV_n)_{0 \leq n < N}$ of subsets of $X$, where $N\in \N \cup \{\infty\}$ is specified later, proceeding as follows.
Assuming that $\cV_n$ is already defined we consider the closer set 
\be
\label{eqDefXn}
X_n :=  
\{x\in X \sep d_X(x,\cV_n) \geq 1\}.
\ee
If the set $X_n$ is empty, then the sequence ends and we define $N := n+1$. Otherwise we choose $x_{n+1}$ arbitrarily among the minimisers of $d_X(x,x_0)$ on $X^n$:
\be
\label{defxn}
x_{n+1} \in \underset {x\in X_n} \argmin \,d_X(x,x_0),
\ee
and we define $\cV_{n+1} := \cV_n \cup\{x_{n+1}\}$.
Such a minimizer exists since $X_n$ is closed and since the closed balls in $X$ are compact.
%$$
%X^n \cap \overline B\left(x_0, \ 1+ \inf_{x\in X^n} d_X(x_0, x)\right)
%$$
%is compact.
We define $N := \infty$ none of the sets $(X_n)_{n \geq 0}$ is empty. %if the sequence $(x_n)$ is infinite.

We define $\cV := \cup_{0 \leq n <N} \cV_n$.
%We denote by $X_0 := \{x_n \sep 0\leq n<N\}$ the collection of all points of this finite or countable sequence.
%
%We define $N := \infty$ if the sequence $x_0, x_1, \cdots$ is infinite, and we denote by $X_0$ the collection of all points of this finite or countable sequence,
%$$
%X_0 := \{x_n \sep 0 \leq n < N\}.
%$$ 
%%as the collection of all points $x_0, x_1, \cdots$ of this finite or countable sequence.
%, which clearly is finite or countable.
By construction, we thus have $d_X(v, v') \geq 1$ for all $v,v'\in \cV$
which establishes the separation property \iref{eqSep}. %, and shows that $\cV$ is a discrete set.

We now assume for contradiction that the covering property \iref{eqCover} does not hold which implies that $N= \infty$. We choose a point $x_*\in X$ such that $d_X(x_*, \cV)>1$, and therefore $x_*\in X_n$ for all $n \geq 0$. The definition \iref{defxn} of $x_{n+1}$ implies that $d_X(x_0, x_n) \leq d_X(x_0, x_*)$ for all $n \geq 0$, hence the discrete collection of points
$
\{x_n \sep n \geq 0\}
$
in included in the closed ball $\{x\in X \sep d_X(x_0, x) \leq d_X(x_0, x_*)\}$ which is compact.
The sequence $(x_n)_{n \geq 0}$ therefore admits a converging subsequence, but this contradict the fact that the pairwise distances between these points are larger than $1$, which concludes the proof of this proposition.
\sq


%The next lemma gives a simple (from a theoretical point of view) procedure which produces a point set equidistributed with respect to a metric.
%\begin{lemma}
%Let $H\in \bH$ and let $(p_n)_{n\geq 0}$ be a sequence of points obtained by choosing $p_0 = 0$ and then iteratively choosing $p_{n+1}$ among the minimizers of
%\be
%\label{defpn}
%\min\{\|p\| \sep d_H(p, \{p_0,\cdots , p_n\} \geq 1)
%\ee
%
%Then the point set $\cP := \{p_n \sep n \geq 0\}$ is $1$-equidistributed with respect to $H$.
%\end{lemma}
%
%\proof
%The separation holds by construction. It implies in particular that for any $M \geq 1$, $\cP\cap B(0,M)$ is finite. 
%
%%Since $H$ is continuous and positive definite, for each $M$ the set $\{n\geq 0 \sep \|p_n\| \leq M\}$ is finite.
%Indeed let $\Lambda^2 := \max \{\|H(z)\| \sep \|z\| \leq M\}$.
%The balls $B(p, \Lambda/2)$, $p\in \cP\cap B(M)$ are pairwise disjoint. It follows from a volume argument that $\cP\cap B(M)$ is finite.
%
%Let us assume by contradiction that there exists $z\in \R^2$ such that $d(z, \cP)>1$. Then for $n$ large enough we have $\|z\| < \| p_{n+1}\|$ which is incompatible with the construction of $p_{n+1}$ as a minimizer of \iref{defpn}.
%\sq




We consider a fixed metric $H \in \bH$. For any $x,y\in \R^2$ we define 
$$
d_x(y) := \|x-y\|_{H(x)}.
$$
We also consider a fixed discrete collection of vertices, or ``sites'', $\cV \subset \R^2$, and we define the anisotropic Voronoi cell of a site $v\in V$ as follows 
\be
\label{defVorv}
\Vor(v) := \{z\in \R^2 \sep d_v(z) \leq d_w(z) \text{ for all } w \in V\}.
\ee
The anisotropic Voronoi cell $\Vor(v)$ is thus the collection of points $z$ which are \emph{closer to the vertex $v$ than to any other site}.
The classical (isotropic) Voronoi is obtained by choosing $H = \Id$.
We refer to the paper \cite{Shew} Figure 3 for an illustration of the anisotropic Voronoi diagram $\{\Vor(v) \sep v\in \cV\}$ associated to a point set.

For each $z\in \R^2$ we define $\cV_z$ the collection of vertices which contain $z$ in their Voronoi region:
$$
\cV_z := \{v \in \cV \sep z \in \Vor(v)\}.
$$
The geometric dual of the Voronoi diagram is the graph $\cG(\cV,H)$ defined as follows:
\be
\label{defGVH}
\cG(\cV,H) := \{[v,v'] \sep \text{there exists } z\in \R^2 \text{ such that } V_z = \{v,v'\}\}.
\ee

%We define a collection $\cT_0(V,H)$ of convex sets attached to the metric $H$ and to the collection $V$ of sites
%$$
%\cT_0(V,H) := \{\Cvx(V_z) \sep z \in \R^2 \text{ and } \#(V_z) \geq 3\}.
%$$
The next theorem establishes that $\cG(\cV,H)$ is, under certain conditions on the metric $H$ and the set $\cV$, the graph of a triangulation adapted to $H$.

\begin{theorem}
\label{thEquiMesh}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta)\geq 1$ such that the following holds.
Let $H$ be a metric such that $c^2 H\in \bH_g$, and let $\cV$ be a $\delta$-equispaced subset of $(\R^2, d_H)$.
Then the $\cG(\cV,H)$ is a planar graph which defines a partition of $\R^2$ into strictly convex polygons. Arbitrarily triangulating each polygon yields a triangulation $\cT\in \bT_{g,C}$ which is $C$-adapted to $H$, called an anisotropic Delaunay triangulation. Furthermore if $\cV$ is in general position then $\cG(\cV,H)$ is already the graph of a triangulation.
\end{theorem}

Denote by $c$ and $C$ the constants attached to $\delta=1$ in this theorem.
It follows that for any metric $H$ such that $c^2 H \in \bH_g$, there exists a mesh $\cT\in \bT_{g,C}$ which is $C$-adapted to $H$, obtained as the Delaunay triangulation of a $1$-equispaced set of points $\cV\subset (\R^2, d_H)$. 
This immediately implies Point iii) of Proposition \ref{propMeshGen} according to Remark \ref{remcC}.


The rest of this section is devoted to the proof of Theorem \ref{thEquiMesh}, which is based on the methods and results presented in \cite{Shew}. 
%These theorems are based on a property that needs to be 
For that purpose we recall some definitions of this paper. %introduce the following definitions.
\begin{definition}
\label{defWedge}
%The wedge of $v,v'$ is 
\begin{itemize}
\item (Wedge of two points)
We define the wedge $\wed(v,w)$ of two distinct sites $v,w\in V$ as follows
$$
\wed(v,w) := \{z\in \R^2 \sep (z-v)^\trans H(v) (w-v) >0 \text{ and } (z-w)^\trans H(w) (v-w) >0\}
$$ 
\item (Wedge property)
We say that the Voronoi diagram of $V$ is wedged if for any two distinct $v,w \in V$ we have 
$$
\Vor(v) \cap \Vor(w) \subset \wed(v,w).
$$
\end{itemize}
\end{definition}

The wedge property expresses that the collection $\Vor(v) \cap \Vor(w)$ of points $q$ shared by the Voronoi regions of the sites $v$ and $w$ lie in a cone defined by two linear inequalities.
We refer to \cite{Shew} Figure 4 for an illustration of the wedge of two sites.

The next proposition, which is partly is based on Lemma 5 from \cite{Shew},
 shows that the wedge property is automatically satisfied in our context.
For any metric $H$ and any constant $c>0$ such that $c^2H\in \bH_g$, it easily follows from Proposition \ref{propEuclidRiemann} that for all $x,y\in \R^2$
\be
\label{eqDHLog}
\ln (1+ c\, d_x(y)) \leq c \, d_H(x,y) \leq - \ln(1- c\, d_x(y)), 
\ee
which is equivalent to 
\be
\label{eqDHExp}
1-\exp(-c\, d_H(x,y)) \leq c \, d_x(y) \leq \exp(c \, d_H(x,y))-1.
\ee

\begin{lemma}
\label{lemmaDiamVor}
If $c^2 H\in \bH_g$ %and $\cV$ is $\delta$-equispaced, 
then
for any $v\in \cV$ and any $q\in \Vor(v)$ we have 
\be
\label{eqDiamVor}
\|q-v\|_{H(v)} \leq r_0(c) := (e^c-1)/c.
\ee
If $v,w \in \cV$ satisfy $\Vor(v) \cap \Vor(w) \neq \emptyset$, then 
\be
\label{eqVordvw}
%\delta \leq 
d_H(v,w) \leq r_1(c) := -2\ln(2-e^c)/c.
\ee
Note that $r_0(c) \to 1$ and $r_1(c) \to 2$ as $c\to 0$. Note also that $d_H(v,w)\geq \delta$ if $\cV$ is $\delta$-equispaced.
\end{lemma}

\proof
For any $q\in \cV$ there exists $v_* \in \cV$ such that 
$
d_H(q,v_*) \leq 1,
$
and therefore 
$$
\|q-v_*\|_{H(v_*)} \leq r_0(c) := (e^c-1)/c,
$$
which implies \iref{eqDiamVor} using the definition \iref{defVorv} of the Voronoi diagram.
We thus turn to the proof of \iref{eqVordvw} and for that purpose we consider a point $q\in \Vor (v)\cap\Vor(w)$. We thus have
$
\max\{\|q-v\|_{H(v)} , \|q-w\|_{H(w)} \}\leq  v_c%-\ln(1-c v_c)/c
$
hence
$$
d_H(v,w) \leq r_1(c) :=-2\ln(1-c r_0(c))/c,
$$
which concludes the proof.
\sq

\begin{prop}
\label{propWedge}
For each $\delta$ there exists $c=c(\delta)>0$ such that the following holds.\\
If a metric $H$ satisfies $c^2H\in \bH_g$ and if $\cV$ is a $\delta$-equispaced subset of $(\R^2,d_H)$, then the wedge property is satisfied.
\end{prop}

\proof
We assume for contradiction that there exists two distinct vertices $v,w \in V$, and a point $q\in \Vor(V) \cap \Vor(W)$ such that $z\notin \wed(v,w)$. We may assume, up to exchanging the roles of $v$ and $w$, that 
$$
(q-w)^\trans H(w) (v-w) \leq 0.
$$
Defining the ``relative distortion''
$
\tau := \exp d_\times (H(v), H(w))
$
we obtain using Lemma 5 from \cite{Shew} %(*$q$ instead of $z$??*)
\be
\label{eqShewWedge}
 d_w(v) \leq d_w(q) \sqrt{\tau^2-1}.
\ee
We now estimate the quantities $d_w(v)$, $d_w(q)$ and $\tau$ appearing in this estimate, in order to obtain a contradiction when $c$ is sufficiently small.

%Since the set $V$ is $C_0$-equispaced, there exists $u\in V$ such that $d_H(u,q) \leq C_0$. Recalling that $z\in \Vor(v)\cap \Vor(w)$ we thus obtain using \iref{eqDHExp}
%\be
%\label{eqDiamVor}
%d_v(q) = d_w(q) \leq d_u(q) \leq \frac{\exp(c \, d_H(u,q))-1} c \leq r_0(c) := \frac{\exp(c C_0)-1} c,
%\ee
%and therefore using \iref{eqDHLog} 
%\be
%\label{eqVordvw}
%d_H(v,w) \leq d_H(v,q)+ d_H(q,w) \leq r_1(c) := \frac {-2\ln (1- c r_0(c))}  c,% \frac 1 {1-f(c)}.
%\ee
%hence 
We have 
\be
\label{eqTauWedge}
\ln \tau = d_\times (H(v), H(w)) \leq c d_H(v,w) \leq c r_1(c).
\ee
Since $\cV$ is $\delta$-equispaced we have 
$
d_H(v,w) \geq \delta
$
and therefore 
\be
\label{eqdvwWedge}
c \,d_w(v) \geq 1-\exp(-c d_H(v,w)) \geq 1-\exp(-c\delta)
\ee
Injecting \iref{eqDiamVor}, \iref{eqTauWedge} and \iref{eqdvwWedge} in \iref{eqShewWedge} we obtain
\be
\label{eqFinalWedge}
\frac{1-\exp(-c\delta )} c \leq \frac{\exp(c)-1} c \sqrt{\exp(2c r_1(c))-1}.
\ee
The left hand side tends to $\delta$ as $c\to 0$, while the right hand side tends to $0$. We thus obtain a contradiction when $c$ is sufficiently small which concludes the proof of this proposition.
\sq

\begin{theorem}[Dual triangulation theorem. Labelle, Shewchuck, \cite{Shew}]
\label{thShew}
If the Voronoi diagram of the point set $\cV \subset \R^2$ is wedged, then the geometric dual of this diagram is a polygonalization of $\R^2$ with strictly convex polygons and is a triangulation $\cT$ if $\cV$ is in general position.
\end{theorem}

Under the hypotheses of this theorem the vertices $v_1, \cdots, v_k$ of a polygon in the dual Voronoi diagram satisfy by construction $\Vor(v_1)\cap \cdots \cap \Vor(v_k) \neq \emptyset$, and therefore the vertices $v_1, v_2, v_3$ of a triangle $T\in \cT$ satisfy $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$.

The next theorem, originally stated in \cite{Shew} as Corollary 10 to Theorem 9 of the same paper, allows to control the angles of a triangle in the anisotropic Delaunay triangulation.

\begin{theorem}[Labelle, Shewchuk, \cite{Shew}]
\label{thAngle}
Let $v_1,v_2,v_3\in \cV$ and let $q\in \Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)$. Let 
$$
r = d_{v_1}(q) = d_{v_2}(q) = d_{v_3}(q) \stext{ and }
l = \min\{d_{v_i}(v_j) \sep i,j \in \{1,2,3\}, i \neq j\}.
$$ 
Define $\beta := \max\{r/l,\, 1/\sqrt 2\}$, %and %$\gamma\in [1,\infty)$ by 
%Let $1\leq \gamma \leq \sqrt 2$ and $\beta \geq \frac 1 {\sqrt 2}$ satisfy
$$
\gamma := \exp \max \{d_\times (H(v_i), H(v_j)) \sep i,j \in \{1,2,3\}, i \neq j\},
$$
and
\be
\label{defChi}
\chi := \frac 1 {2 \beta} - \frac{(\gamma^2-1)\beta} 2.
\ee
If $\gamma \leq \sqrt 2$ and $\chi>0$ then any angle $\theta$ of the triangle of vertices $(\sqrt{H(v_1)} v_k)_{1 \leq k \leq 3}$ satisfies
$$
\arcsin ( \chi/ \gamma^2) \leq \theta \leq 2 \arccos(\chi/\gamma^2).
$$
\end{theorem}

\begin{corollary}
\label{corolAdaptG}
For each $\delta>0$ there exists $c=c(\delta)>0$ and $C=C(\delta) \geq 1$ such that the following holds.
If $\cV$ is $\delta$-equispaced, if $c^2H\in \bH_g$ and if $\Vor(v_1) \cap \Vor(v_2) \cap \Vor(v_3)\neq \emptyset$, then denoting by $T$ the triangle of vertices $v_1,v_2,v_3$ we have for all $z\in T$
$$
C^{-2} H(z) \leq \cH(z) \leq C^2 H(z).
$$
\end{corollary}
\proof
We use \iref{eqDHExp} and \iref{eqDHLog} and the fact that $V$ is $\delta$-equispaced to obtain explicit bounds on the quantities $r$, $l$, $\beta$, $\gamma$ and $\chi$ appearing in Theorem \ref{thAngle}.
It follows from Lemma \ref{lemmaDiamVor} that 
$$
r\leq r_0(c) \stext{ and } \delta \leq d_H(v_i,v_j) \leq r_1(c).
$$
Therefore 
$$
l := \min_{i\neq j} d_{v_i}(v_j)\geq %\min_{i\neq j} \frac{1-\exp(-c d_H(v_i,v_j))} c \geq  
r_2(c) := (1-\exp(-c\delta))/ c,
$$
and 
$$
L := \max_{i\neq j} d_{v_i}(v_j) \leq (\exp(c r_1(c))-1)/c
$$
and 
$$
\gamma \leq \max_{i\neq j} \exp(c \,d_H(v_i,v_j)) \leq \exp(c \,r_1(c)).
$$
In particular 
$
\beta \leq r_3(c) := \min\{r_0(c)/r_2(c),\, 1/\sqrt 2\}. % = \frac{\exp(cC_0)-1}{1-\exp(-2 cC_0^{-1})},
$
Injecting this into \iref{defChi} yields an explicit lower estimate 
$$
\chi\geq r_4(c) := \frac 1 {2r_3(c)} - \frac{ (\exp(2cr_1(c))-1) r_3(c)} 2,
$$ 
and $\chi/\gamma^2\geq r_5(c) := r_4(c) \exp(-2cr_1(c))$.

For a fixed $\delta$ we obtain as $c\to 0$ the limits $r_0(c) \to 1$, $r_1(c)\to 2 $, $r_2(c) \to \delta$, $r_3(c) \to \min\{\delta, 1/\sqrt 2\}$ and $r_4(c) \to 1/(2\min\{\delta, 1/\sqrt 2\})$ and $r_5(c)$ as the same limit.

%We assume without loss of generality that $\delta \geq 1/\sqrt 2$ and we thus obtain $r_3(c) \to \delta$, 
%$r_4(c) \to 1/C_0^2$ and $r_5(c) \to 1/C_0^2$. 
We may therefore choose $c$ sufficiently small in such way that 
$$
l \geq l_0 := \delta/2, \ L  \leq L_0 := 4 \text{ and }\chi/\gamma^2 \geq \Chi_0 := 1/(4\min\{\delta, 1/\sqrt 2\}).
$$
We denote by $T$ the triangle of vertices $v_1, v_2, v_3$. The length of any edge of $T' := \sqrt{H(v_1)}(T)$ is bounded above by $L_0$ and below by $l_0$ respectively, and the angles of $T'$ satisfy $\arcsin (\Chi_0) \leq \theta \leq 2 \arccos(\Chi_0)$. The collection of triangles centered at the origin which satisfy these inequalities is compact, thus there exists a constant $C_1 = C_1(C_0)$ such that 
$$
C_1^{-2} \Id \leq \cH_{T'} \leq C_1^2 \Id,
$$
hence $C_1^{-2} H(v_1) \leq \cH_{T'} \leq C_1^2 H(v_1)$. For any $z\in T$ we obtain, remarking that $\|z-v_1\|_{\cH_T} \leq 2$ for all $z\in T$ and using \iref{eqLocalNorm}, 
$$
C_1^{-2} (1-2cC_1)^2 H(z) \leq \cH_{T'} \leq C_1^2(1-2cC_1)^{-2} H(z)
$$
which concludes the proof of this proposition, with $C = C_1(1-2cC_1)^{-1}$.
\sq

We now prove of Theorem \ref{thEquiMesh}.
According to the above results for any $\delta>0$ there exists $c = c(\delta)$ and $C=C(\delta)$ such that the following holds. 
For any set $\cV \subset (\R^2, d_H)$ which is $\delta$-equispaced, the Voronoi diagram associated to $\cV$ and $H$ is wedged according to Proposition \ref{propWedge}. The dual of this diagram is therefore a polygonalization of $\R^2$ with strictly convex polygons according to Theorem \ref{thShew}.
Randomly triangulating these cells yields a triangulation $\cT\in \bT$ which is $C$-adapted to $H$ according to Corollary \ref{corolAdaptG}. 

Furthermore consider to simplices $T,T'\in \cT$ such that $T \cap T'\neq \emptyset$, and a point $z\in T \cap T'$.
Then 
$$
C^{-2} \cH_T \leq H(z) \leq C^2 \cH_{T'},
$$
which shows that $\cT\in \bT_{g,C^2}$ and concludes the proof of Theorem \ref{thEquiMesh}.

\subsection{Quasi-Acute mesh generation}
\label{secMeshGenA}

This section is devoted to the proof of Point ii) of Proposition \ref{propMeshGen}, which is obtained by combining the  constructions of isotropic and graded triangulations presented in \S\ref{secMeshGenI} and \S\ref{secMeshGenI} to produce a quasi-acute triangulation. 
The key idea of this proof if that the anisotropic Delaunay triangulation described in the previous subsection contains only \emph{few} strongly obtuse angles if the set $\cV$ of vertices is structured along lines which are \emph{transverse to the direction of anisotropy}, as illustrated on Figure \ref{figAcuteGen} (in the introduction of this chapter). 

The author is sorry to say that this proof is not yet as polished as the rest of the thesis, due to time constraints. This proof involves from instance a number of numerical constants which are far from optimal.

We consider a fixed metric $H$ such that $c^2 H\in \bH_a$, where $c$ is an absolute constant specified in the proof and such that $0<c\leq 1$. This subsection is devoted to the construction of a mesh $\cT\in \bT_{a,C}$ which is $C$-adapted to $H$, where $C$ is an absolute constant also specified in the proof.
This construction immediately implies Proposition \ref{propMeshGen} according to Remark \ref{remcC}. 


For each $z\in \R^2$ we define %We define two functions $\lambda, \mu : \R^2 \to \R$ as follows : for all $z\in \R^2$
$$
\lambda(z) := \|H(z)^{-\frac 1 2}\| \stext{ and } \mu(z) = \|H(z)\|^{-\frac 1 2},
$$
and we observe that $\lambda(z) \geq \mu(z)$.
The functions $\lambda$ and $\mu$ are $c$-Lipschitz according to Corollary \ref{corolLipNorm}.
% : for all $z,z'\in \R^d$
%$$
%|\lambda(z)-\lambda(z')| \leq c|z-z'| \text{ and } |\mu(z) - \mu(z') | \leq c|z-z'|.
%$$
If $c$ is sufficiently small, then there exists according to Corollary \ref{corolBidimIso} a mesh $\cT_0$ such that for all $T\in \cT_0$ and all $z\in T$
\be
\label{ratioDiamLambda}
\frac 2 3  \lambda(z) \leq \diam(T)\leq \lambda(z). 
\ee
The mesh $\cT_0$ is built of half squares by construction (as illustrated on Figure \ref{figHalfSquares}) hence  for any edge $[v,w]$ of any triangle $T\in \cT_0$ we have $\diam(T)/\sqrt 2 \leq |v-w|\leq \diam(T)$, and the diameter of any triangle $T\in \cT_0$ is a power of $\sqrt 2$. Therefore if two triangles $T,T'\in \cT_0$ share a vertex $v$ we obtain 
\be
\label{eqDiamRatio}
\diam(T)/\sqrt 2 \leq \diam(T') \leq \sqrt 2 \diam(T),
\ee
which implies for any edges $[v,w]$ and $[v,w']$ (sharing the vertex $v$) of the triangulation $\cT_0$ 
\be
\label{eqEdgeRatio}
|v-w|/2 \leq |v-w'| \leq 2|v-w|.
\ee
Inequality \iref{ratioDiamLambda} also implies that for any edge $[v,w]$ of $\cT_0$
%We say that two vertices $v,w\in \cV_0$ are neighbors in $\cT_0$ if they belong to a common triangle $T\in \cT_0$.
%In that case we have %Let $v,w$ be two vertices of a triangle $T\in \cT_0$, then 
\be
\label{edgeLambda}
\frac{\lambda(z)\sqrt 2}3 \leq \frac{\diam(T)}{\sqrt 2}\leq |v-w| \leq \diam(T)\leq \lambda(z)
\ee
We denote by $\cV_0$ the collection of vertices of $\cT_0$. 
Consider a fixed $v\in \cV_0$ any vertex $w\in \cV_0$ such that $|v-w|$ is minimal. Then $[v,w]$ is clearly an edge of $\cT_0$. This implies for any distinct $v,w\in \cV_0$
\be
\label{pairwiseV0}
\lambda(v) \frac {\sqrt 2} 3 \leq |v-w| .
\ee


For each $z\in \R^2$ we define 
$$
\rho(z) := \lambda(z)/\mu(z)  = \sqrt{\|H(z)\| \|H(z)^{-1}\|} \in [1, \infty).
$$
Consider $z,z'\in \R^2$ such that $|z-z'| \leq r\lambda(z)$, where $r\geq 0$ is a constant. Then since $\lambda$ and $\mu$ are $c$-Lipschitz we obtain 
\be
\label{eqrhozzp}
\rho(z') = \frac{\lambda(z')}{\mu(z')} \geq \frac{\lambda(z)(1-r c)}{\mu(z)+ r c \lambda(z)} \geq \frac {1-r c}{\rho(z)^{-1}+r c}.
\ee
For each $\rho_0, r_0$ we denote by $c_\rho(\rho_0, r_0)>0$ the constant such that $\rho_0 = \frac {1-r_0 c_\rho(\rho_0, r_0)}{(\rho_0+1)^{-1}+r_0 c_\rho(\rho_0, c_0)}$.
Hence for all $z,z'\in \R^2$ 
$$
\left\{
\begin{array}{c}
|z-z'| \leq r_0\lambda(z)\\ 
\rho(z) \geq \rho_0+1\\
c\leq c_\rho(\rho_0, r_0)
\end{array}
\right.
%\Big(|z-z'| \leq r_0\lambda(z) , \ \rho(z) \geq \rho_0+1 \text{ and } c\leq c_\rho(\rho_0, r_0)\Big) 
\stext{ implies } \rho(z') \geq \rho_0
$$
For instance if $z,z'$ belong to the same triangle $T\in \cT_0$, if $\rho(z) \geq n+1$ and if $c\leq c_\rho(n,1)$, then $\rho(z') \geq n$ according to \iref{edgeLambda}. 
%Throughout this proof we shall make a finite number of assumptions of the type $c \leq c_\rho(r_0,\rho_0)$ for some absolute constants $r_0, \rho_0$. They hold if $c$ if sufficiently small.

For each $z\in \R^2$ such that $\rho(z)>1$ we denote by $\theta(z)\in \bbS := \{u\in \R^2\sep |u| = 1\}$ a unit vector such that
\be
\label{defAngle}
H(z) = \lambda(z)^{-2} \theta(z) \theta(z)^\trans+ \mu(z)^{-2} (\Id-\theta(z) \theta(z)^\trans).
\ee
Note that there exists two, opposite, choices for the vector $\theta(z)$.
For each $u,u'\in \R^2 \sm\{0\}$ we define the (unoriented) angle
$$
\varangle (u,u') := \arccos \left(\frac{\<u,u'\>}{|u| |u'|}\right) \in [0,\cPi].
$$
and 
%For any two vectors $u,u'\in \R^2\sm\{0\}$ we define %the non-oriented, acute, angle
$$
\lhd(u,u') := \min \{\varangle(u,u'),\, \varangle(u,-u')\} = \arccos\left(\frac {|\<u,u'\>|}{|u| |u'|}\right) \in [0, \cPi/2].
$$
\begin{lemma}
\label{lemmaAngle12}
If $c$ is sufficiently small, then the following holds.
For any $z,z'\in \R^2$ 
$$
\left\{
\begin{array}{c}
\rho(z) \geq 2\\
|z'-z|\leq 10 \lambda(z) 
\end{array}
\right.
\stext{ implies }
\lhd(\theta(z), \theta(z')) \leq \cPi/12,
$$
and likewise $\rho(z) \geq 4$ and $|z-z'| \leq \lambda(z)$ implies $\lhd(\theta(z), \theta(z')) \leq 1/(10 \sqrt 2)$.
\end{lemma}

\proof
We consider a fixed point $z$ such that $\rho(z) \geq 2$ and we denote by $B$ the ball $\{z'\in \R^2\sep |z'-z| \leq 10 \lambda(z)\}$.
For each $z'\in B$ we have
\begin{eqnarray*}
\lambda(z') - \mu(z') &\geq& (\lambda(z)-c|z-z'|) - (\mu(z)+ c |z-z'|) \\
&=& \lambda(z) -\mu(z) -2 c |z-z'| \\
&\geq& \lambda(z) -\lambda(z)/ 2 - 20 c\lambda(z)\\
&=& \lambda(z)(1/2 -20 c),
\end{eqnarray*}
hence $\lambda(z') - \mu(z')\geq \lambda(z)/3$ if $c \leq 1/120$, which we assume from this point.

Furthermore since $B$ is simply connected there exists a continuous function $\theta_* : B \to \bbS$ (where $\bbS := \{u\in \R^2 \sep |u|=1\}$ denotes the unit circle) such that $\theta_*(z')  = \pm \theta(z')$ for all $z'\in B$.
According to Theorem \ref{th2Spaces} we have for all $z'\in B$
$$
\lambda(z)\dil_{z'}(\theta_*) \leq 3(\lambda(z')-\mu(z')) \dil_{z'}(\theta_*) \leq 3c.
$$
Therefore, since the distance $d_\bbS$ on $\bbS$ involved in Theorem \ref{th2Spaces} coincides with the angle $\varangle$ we obtain
$$
\lhd(\theta(z), \theta(z'))\leq \varangle(\theta_*(z), \theta_*(z')) \leq |z-z'| \max_{\ti z \in [z,z']} \dil_{\ti z}(\theta_*) \leq 30c 
$$
which concludes the proof if $30c \leq \cPi/12$.
\sq


For each vertex $v\in \cV_0$ we define a set $\Gamma_v\subset \R^2$ as follows : $\Gamma_v := \{v\}$ if $\rho(v) <3$, and 
\be
\label{defGammav}
\Gamma_v := \left[v, \, \frac v 3+ \frac{2w_-} 3\right] \cup \left[v,\frac v 3 +\frac{2w_+} 3\right] 
\ee
if $\rho(v)\geq 3$, where $[v,w_-]$ and $[v,w_+]$ are two edges of $\cT_0$ which respectively minimize and maximize the quantity $\<\theta(v)^\perp, w-v\>$ (among the edges containing $v$).
In other words for any edge of $\cT_0$ of the form $[v,w]$ we have
\be
\label{defWmWp}
\<\theta(v)^\perp, w_- -v\> \leq \<\theta(v)^\perp, w-v\> \leq  \<\theta(v)^\perp, w_+ - v\>. 
\ee
This property is illustrated on Figure \ref{figWmWp}.

\begin{figure}
\centering
\includegraphics[width=4cm, height=4cm]{\pathPic/Dessins/Jenny/VT0vJenny.pdf}\hspace{1cm}
\includegraphics[width=6cm, height=4cm]{\pathPic/Dessins/Jenny/DirThetaJenny.pdf}
\caption{Neighborhood $V_{\cT_0}(v)$ of a simplex $v$ in the triangulation $\cT_0$ (left), the neighbors $w_+$ and $w_-$ of a vertex $v$ in $\cT_0$.
\label{figWmWp}}
\end{figure}

\begin{lemma}
\label{lemmaAngleWmWp}
let $v\in \cV_0$ be such that $\rho(v) \geq 3$, and let $[v,w_+]$, $[v,w_-]$ be two edges of $\cT_0$ satisfying \iref{defWmWp}.
We have 
\be
\label{eqAngleWmWp}
\varangle(\theta(v)^\perp, w_+ -v) \leq \cPi/4,
\stext{ and }
\varangle(\theta(v)^\perp, v-w_-) \leq \cPi/4.
\ee
\end{lemma}

\proof
We restrict without loss of generality our attention to the proof of the first inequality, and we assume for contradiction that $\vp := \varangle(\theta(v)^\perp, w_+-v)>\cPi/4$. % in \iref{eqAngleWmWp}.
Among the two vertices $w\in \cV_0$ such that the triangle of vertices $v,w,w_+$ belongs to $\cT_0$, we choose the one such that $\varangle(\theta^\perp, w-v)$ is minimal.
We denote $\psi := \varangle(w-v, w_+-v) \in \{\cPi/4, \cPi/2\}$ and we obtain 
$$
\<\theta(v)^\perp, w_+-v\> = |w_+-v|\cos \vp \stext{ and } \<\theta(v)^\perp, w-v\> = |w-v|\cos (\vp-\psi).
$$
If $\psi = \cPi/2$ then $|w_+-v| = |w-v|$ since the triangles $T\in \cT_0$ are half squares, and $\cos (\vp-\psi) = \sin \vp$. We thus have $\cos \vp \geq \sin \vp$ according to \iref{defWmWp} which contradicts our assumption that $\vp>\cPi/4$.
If $\psi = \{\cPi/4\}$ then $|w_+-v| = \sqrt 2 |w-v|$ or $|w_+-v| =  |w-v|/\sqrt 2$. We thus have $\sqrt 2 \cos \vp \geq \cos (\vp-\cPi/4)$ which again contradicts our assumption that $\vp > \cPi/4$.
\sq

We define $\Gamma := \cup_{v\in \cV_0} \Gamma_v$, and for each $z\in \Gamma\sm\cV_0$ we define 
\be
\label{defGammaz}
\Gamma_z := \bigcup_{\substack{v\in \cV_0 \\ z \in \Gamma_v}} \Gamma_v.
\ee
Note that for any vertex $v\in \cV_0$ the set $\Gamma_v$ does not contain any vertex $w\in \cV_0$ distinct from $v$, hence \iref{defGammaz} agrees with \iref{defGammav} for any $z\in \cV_0$.\\ 

\begin{lemma}
\label{lemmaPi3}
For any $z\in \Gamma$ and any $z'\in \Gamma_z$ 
distinct from $z$
%we have
%\be
%\label{eqAngleGammaz}
%\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
%\ee
%and therefore if $c$ is sufficiently small
we have 
$$
\angle(\theta(z)^\perp ,z'-z) \leq \cPi/3, 
$$
%and there exists a piecewise affine Lipschitz map $\gamma : [\alpha, \beta]\to \R$ such that the following is a bijection
%$$
%t\in [\alpha, \beta] \mapsto z+ t\theta(z)^\perp + \sqrt 3 \gamma(t) \theta(z) \in \Gamma_v.
%$$

(*alternative version*)
For any $z\in \Gamma$, any $z'\in \Gamma_z \sm \{z\}$ and any $\ti z \in [z, z']$ we have 
%we have
%\be
%\label{eqAngleGammaz}
%\angle(\theta(z)^\perp ,z'-z) \leq 2c+\cPi/4, 
%\ee
%and therefore if $c$ is sufficiently small
$$
\angle(\theta(\ti z)^\perp ,z'-z) \leq \cPi/3, 
$$


\end{lemma}

\proof
According to the definition \iref{defGammaz} of $\Gamma_z$ there exists a vertex $v\in \cT_0$ such that $z,z'\in \Gamma_v$. Therefore $|z-v| \leq \lambda(v)$ and $\rho(v) \geq 3$.
It follows from Lemma \ref{lemmaAngleWmWp} and Lemma \ref{lemmaAngle12} that 
$$
\lhd(\theta(z)^\perp, z'-z) \leq \lhd(\theta(v), \theta(z)) + \lhd(\theta(v),z'-z) \leq \cPi/12 + \cPi/4 = \cPi/3,
$$
which concludes the proof.
\sq

The next proposition gives some upper and lower bounds on the distance from a point to the set $\Gamma$.
\begin{prop}
\label{propDistUpLow}
If $c$ is sufficiently small, then the following holds.
For any $z\in \Gamma$,
\be
\label{eqDistzGH0}
 \min\{|z-e| \sep  e\in \Gamma\sm \Gamma_z\} \geq \frac {10}{91} \lambda(z) % >\frac 1 {10}
\ee
and for any $z\in \R^2$
\be
\label{eqDistzGH}
\min\{\|z-e\|_{H(z)} \sep e \in \Gamma\} \leq 2 %1+ \frac {2\sqrt 2} 3 <2. 
\ee
\end{prop}

\begin{figure}
\centering
\includegraphics[width = 4cm, height = 4cm]{\pathPic/Dessins/Jenny/DistZGJenny.pdf}
\caption{Illustration of the proof of Proposition \ref{propDistUpLow} \label{figDistZG}}
\end{figure}

\proof
We first establish \iref{eqDistzGH0}. 
Let $z\in \Gamma$ and let $v\in \cV_0$ be such that $z\in \Gamma_v$. There exists an edge $[v,w_*]$ of $\cT_0$ and a parameter $\alpha\in [0,2/3]$ such that $z= (1-\alpha) v+\alpha w_*$.
We denote by $V_{\cT_0}(v)$ the union of all triangles $T\in \cT_0$ containing $v$, and by $\cV_0(v)$ the collection of vertices $w$ such that $[v,w]$ is an edge of $\cT$. We thus have
$$
\Gamma\sm \Gamma(z) \subset \overline {\R^2 \sm V_{\cT_0}(v)} \bigcup_{w\in \cV_0(v)\sm\{w_*\}} \left[\frac{2v+w}3, w\right].
$$
The set appearing in the right hand side is illustrated on Figure \ref{figDistZG}.
Denoting $d(z,E) := \inf\{ |z-e|\sep e\in E\}$ we obtain 
\begin{eqnarray*}
d(z,\Gamma\sm \Gamma(z)) &\geq & \min \left\{ d(z, \R^2 \sm V_\cT(v)), \ \min_{w\in \cV_0(v) \sm \{w_*\} } d\left(z,\left[\frac{2v+w}3, w\right]\right)\right\}\\
& \geq & \min \left\{ \frac{|w_*-z|}{\sqrt 2}, \ \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)\sm \{w_*\}} |v-w|\right\}\\
& = & \frac 1 {3\sqrt 2} \min_{w\in \cV_0(v)} |v-w|\\
& \geq & \frac{1}{3\sqrt 2} \lambda(v)\frac {\sqrt 2} 3 \\
&\geq&  \frac{\lambda(z)(1-c|z-v|)}{9} \geq \frac{\lambda(z)(1-c)}{9},
\end{eqnarray*}
where we used \iref{edgeLambda} in the fourth line, and the fact that $\lambda$ is $c$-Lipschitz in the last line. This establishes \iref{eqDistzGH0} if $c$ is sufficiently small.\\

We now turn to the proof of \iref{eqDistzGH}. 
Let $T \in \cT_0$ and let $z\in T$. Since $T$ is a half square there exists a vertex $v$ of $T$ such that $|z-v| \leq \diam(T)/2$, hence %For any vertex $v$ of $T$ we obtain %If $\rho(z)\leq 4$, then any vertex $v$ of $T$ satisfies 
$$
\|z-v\|_{H(z)} \leq  \frac{|z-v|}{\mu(z)}   \leq \frac{\diam(T)}{2 \mu(z)} \leq \frac{\lambda(z)}{2 \mu(z)} = \frac{\rho(z)} 2,
$$
which concludes the proof if $\rho(z) \leq 4$. If $\rho(z) \geq 4$ and $c\leq c_\rho(3,1)$ then $\rho(v) \geq 3$ for any vertex $v$ of the triangle $T$.

We choose two vertices $v,w$ of $T$ such that the line $(z+ r \theta(z))_{r\in \sR}$ intersects $\partial T$ on the segment $[v,(v+w)/2]$.
We denote by $w_-,w_+\in \cV_0$ the neighbors of $v$ in $\cT_0$ which satisfy \iref{defWmWp}.
Our first step is to establish that the line $(z+ r \theta(z))_{r\in \sR}$ intersects the set $\Gamma_v$ : this is heuristically due to the fact that the angle $\lhd(\theta(z), \theta(v))$ is small and that the vertices $w_-$ and $w_+$ are the \emph{farthest} from $v$ in the direction of $\theta(v)^\perp$ as illustrated on Figure \ref{figWmWp} (right).

We have according to \iref{eqEdgeRatio}
$$
\<\theta(v)^\perp,w_+ - v\> \geq |w_+-v|\cos(\cPi/4) \geq \frac{|w-v|} 2 \frac 1 {\sqrt 2}. %/(2\sqrt 2).
$$
We assume without loss of generality that %$\theta(v)$ and $\theta(z)$ are oriented in consistently, in such way that 
$\<\theta(z), \theta(v)\> \geq 0$ which implies % and we obtain using Corollary \ref{corolTheta2C}
$$
|\theta(z)-\theta(v)| \leq \varangle(\theta(z), \theta(v)) = \lhd(\theta(z), \theta(v)) \leq \delta := 1/(10 \sqrt 2).
$$
It follows that 
\begin{eqnarray*}
\<\theta(z)^\perp, w-v\> &=& \<\theta(z)^\perp-\theta(v)^\perp, w-v\>+\<\theta(v)^\perp, w-v\>\\
& \leq & |\theta(z)-\theta(v)| |w-v| + \<\theta(v)^\perp, w_+-v\>\\
& \leq & (1+2\delta \sqrt 2 )\<\theta(v)^\perp, w_+-v\>.\\
%& \leq & (1+4 c\sqrt 2) }{1-\vp_c\sqrt 2} \<\theta(z)^\perp,w_+ - v\>.
%& \leq & \frac 4 3 \<\theta(z)^\perp,w_+ - v\>
\end{eqnarray*}
Denoting $\Theta := \varangle(\theta(v)^\perp, w_+-v)$ and $\Phi := \varangle(\theta(z)^\perp, w_+-v)$ we obtain 
$$
\frac{\<\theta(v)^\perp, w_+-v\>}{\<\theta(z)^\perp, w_+-v\>} = \frac{\cos(\Theta)}{\cos(\Phi)} \leq \frac{\cos(\Theta)}{\cos(\Theta) - |\Phi-\Theta|} =\left(1-\frac {|\Phi-\Theta|}{\cos\Theta}\right)^{-1}\leq (1-\delta \sqrt 2)^{-1} % - 2c} = \frac 1 {1-2 \sqrt 2 c},
$$
hence 
$$
\<\theta(z)^\perp, w-v\>  \leq \frac{1+2\delta \sqrt 2}{1-\delta \sqrt 2 c}\<\theta(z)^\perp, w_+-v\> \leq \frac 4 3 \<\theta(z)^\perp, w_+-v\>.
$$
Proceeding likewise for $w_-$, and assuming that $c$ is sufficiently small, we obtain 
%
%We assume that $c$ is sufficiently small in such way that 
%\be
%\label{assumPhic}
%\frac{1+\vp_c 4\sqrt 2}{1-\vp_c\sqrt 2}\leq \frac 4 3
%\ee
$$
\frac 4 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, w-v\> \leq  \frac 4 3\<\theta(z)^\perp, w_+ - v\>,
$$
and therefore since $z+r\theta(z)\in [v,(v+w)/2]$ for some $r\in \R$,
$$
\frac 2 3\<\theta(z)^\perp, w_- -v\> \leq \<\theta(z)^\perp, z-v\> \leq  \frac 2 3\<\theta(z)^\perp, w_+ - v\>.
$$
It follows that the line $(z+r\theta(z))_{r\in \sR}$ intersects the set $\Gamma_v := [v, (v+2w_+)/3] \cup  [v, (v+2w_-)/3]$ at some point $z'$.
%hence there exists $r\in \R$ such that $z' := z+ r\theta(z) \in \Gamma_v$. 
The point $z'$ belongs to a triangle $T'$ containing $v$, which implies using \iref{eqDiamRatio} 
\begin{eqnarray*}
\lambda(z) \|z'-z\|_{H(z)} &=& \lambda(z)\|r\theta(z)\|_{H(z)}\\
&=& |r|\\
&=& |z-z'|\\
&\leq& |z-v|+|v-z'|\\
&\leq& \diam(T)+ \frac 2 3\diam(T')\\
&\leq & \left(1+\frac 2 3 \sqrt 2\right) \diam(T)
 \leq  \left(1+\frac 2 3 \sqrt 2\right) \lambda(z),
\end{eqnarray*}
which concludes the proof of this proposition.
\sq

We construct in the next lemma the set of vertices $\cV$ of the quasi-acute triangulation $\cT$ to be constructed, by sampling the set $\Gamma$.

\begin{lemma}
\label{lemmaConstV}
The following holds if $c$ is sufficiently small.
There exists a discrete set $\cV \subset\Gamma$ containing $\cV_0$ and satisfying the following:
\begin{enumerate}[i)]
\item (Separation) For all $v,w\in \cV$, $d_H(v,w) \geq 1/10$.
\item (Distance from $\Gamma$) For all $z\in \Gamma$, $d_H(z, \cV) \leq 1/10$.
\item (Distance from $\R^2$) For all $z\in \R^2$, $d_H(z,\cV) \leq 2+1/4$.
\end{enumerate}
\end{lemma}
\proof
For any distinct $v,w\in \cV_0$ we obtain using \iref{pairwiseV0} and Proposition \ref{propEuclidRiemann}
\begin{eqnarray*}
d_H(v,w) &\geq& \ln(1+c\|v-w\|_{H(v)})/c\\
&\geq& \ln(1+c|v-w|/\lambda(v))/c\\
&\geq& \ln(1+c\sqrt 2 /3)/c 
\end{eqnarray*}
which is larger than $1/10$ if $c$ is sufficiently small. % since $\sqrt 2 /3>1/10$.

We denote by $\cV$ a $1$-equispaced subset of the metric space $(\Gamma, 10\:d_H)$ containing $\cV_0$, which exists according to Lemma \ref{lemmaEquiSpaced}. The two first announced properties, separation and distance from $\Gamma$, follow directly from this construction.

The third property is obtained as follows: for any $z\in \R^2$ there exists according to Proposition \ref{propDistUpLow} a point $e\in \Gamma$ such that $\|z-e\|_{H(z)}\leq 2$. Furthermore there exists a vertex $v\in \cV$ such that $d_H(e,v) \leq 1/10$, hence
$$
d_H(z,\cV) \leq d_H(z,e)+ d_H(e,v) \leq -\ln(1-c\|z-e\|_{H(z)})/c + 1/10 \leq -\ln(1-2c)/c + 1/10.
$$
which is smaller than $2+1/4$ if $c$ is sufficiently small.
\sq

The next lemma introduces the anisotropic Delaunay triangulation $\cT$ associated to the metric $H$ and the set of points $\cV$. 

\begin{lemma}
\label{lemmaRecallG}
There exists a absolute constant $C_0\geq 1$ such that the following holds if $c$ is sufficiently small.
The set $\cV$ is wedged with respect to the metric $H$, and the anisotropic Delaunay triangulation $\cT_0$ obtained by arbitrarily triangulating the cells of the graph $\cG(\cV,H)$ is $C_0$-adapted to $H$ and belongs to $\bT_{g,C_0}$.

Furthermore for any edge $[v,w]$ of $\cT$ and any $z\in [v,w]$ we have 
$$
\|v-w\|_{H(z)} \leq 5.
$$
\end{lemma}

\proof
We denote $\alpha := (2+1/4)^{-1}$ throughout the proof of this lemma.
It follows from to Lemma \ref{lemmaConstV} that the set $\cV$ is a $\alpha/10$-equispaced subset of the metric space $(\R^2, \alpha d_H)$. 

Theorem \ref{thEquiMesh} applied to the metric $\alpha^2 H$, therefore implies that, if $c$ is sufficiently small, the set 
$\cV$ is wedged for the metric $\alpha^2 H$ and that arbitrarily triangulating the convex cells of the graph $\cG(\cV,\alpha^2 H)$, which are convex yields a triangulation $\cT$ which is $C$-adapted to the metric $\alpha^2H$ (hence $C_0 := C/\alpha$-adapted to $H$), where $C$ is an absolute constant.

The definition \iref{defGVH} of the graph $\cG(V,H)$ implies that $\cG(\cV,\alpha^2 H) = \cG(\cV,H)$, and Definition \ref{defWedge} of the wedge property shows that it holds for $H$ if and only if it holds for $\alpha^2 H$. 

For any edge $[v,w]$ of $\cT$ the Voronoi regions $\Vor(v)$ and $\Vor(w)$ intersect (by definition of the anisotropic Delaunay triangulation), and we thus have according to Lemma \ref{lemmaDiamVor} 
$$
\alpha d_H(v,w) = d_{\alpha^2 H} (v,w) \leq -2\ln (2-e^{c'})/c'
$$
where $c' := c/\alpha$. Hence 
$$
d_H(v,w) \leq r_0(c) := -2 \ln (2-e^{c/\alpha})/c.
$$
If follows that 
$
\|v-w\|_{H(v)} \leq r_1(c) := (e^{c r_0(c))}-1)/c,
$
hence \iref{eqLocalNorm}
$
\|v-w\|_{H(z)} \leq \|v-w\|_{H(v)} (1-c \|v-z\|_{H(v)})^{-1} \leq r_2(c) := r_1(c) (1-c r_1(c))^{-1}
$
for any $z\in [v,w]$.
As $c\to 0$ the functions $r_0$, $r_1$ and $r_2$ all tend to $2 (1+1/4) <5$. Choosing $c$ sufficiently small we  conclude the proof of this proposition.
\sq

Triangulation $\cT$ introduced in the previous lemma is $C_0$ adapted to $H$, and belongs to $\bT_{g,C_0}$. The rest of this chapter is devoted to the proof that, if $c$ is sufficiently small, then $\cT$ is a quasi-acute triangulation : $\cT\in \bT_{a,C}$ where $C$ is an absolute constant.

The next lemma 
%is a first step in this direction. It 
states that the edges of $\cT$ fall into three categories : the edges aligned with the direction $\theta$ of anisotropy, and the edges transverse to that direction.
%It heuristically expresses that the long edges of $\cT$ are aligned with the direction $\theta$ of anisotropy.

\begin{lemma}
\label{lemmaThreeTypes}
%If $c$ is sufficiently small, then the following holds.
%For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$ we have 
%\be
%\label{vpNotInGammav}
%\sin \lhd (\theta(v),v-w) \leq \frac {50}{\rho(v)}.
%\ee
%
%(*alternative version*)
%For any edge $[v,w]$ of $\cT$ such that $w\notin \Gamma_v$, and any $z\in [v,w]$ such that $\rho(z) \geq \rho_l$ we have 
%\be
%\label{vpNotInGammav2}
%\lhd(\theta(z), v-w) \leq \cPi/12,
%\ee
%where $\rho_l$ is a constant specified in the proof.
%
%
%(*alternative version*)
The following holds if $c$ is sufficiently small.
Let $[v,w]$ be an edge of $\cT$ and let $z\in [v,w]$. Then at least one of the following alternatives hold
\begin{enumerate}
\item $\rho(z) \leq \rho_l := 50 / \sin (\cPi/12)$, where $\rho_l$ is an absolute constant specified in the proof.
\item $w\in \Gamma_v$ and $\lhd(\theta(z)^\perp, w-v) \leq \cPi/3$
\item $w\notin \Gamma_v$ and $\lhd(\theta(z) , w-v) \leq \cPi/12$
\end{enumerate}
%\be
%\label{twoDir}
%\lhd(\theta(z) , w-v) \leq \cPi/12 \text{ or } \lhd(\theta(z)^\perp, w-v) \leq \cPi/3.
%\ee

\end{lemma}

\proof
If $w\in \Gamma_v$ then the estimate $\lhd(\theta(z)^\perp, w-v) \leq \cPi/3$ immediately follows from lemma \ref{lemmaPi3}.
On the other hand if $w\notin \Gamma_v$ Lemma \ref{lemmaRecallG} states that $\|v-w\|_{H(v)} \leq 5$.
$$
 \frac{|w-v|}{\mu(z)} \sin \lhd(\theta(z) , w-v) \leq \|w-v\|_{H(z)} \leq 5.
$$
Proposition \ref{propDistUpLow} implies that 
$$
\frac{|w-v|}{\lambda(z)} \geq \frac{|v-w|}{\lambda(v)(1+5c)} \geq \frac {10}{91(1+5c)}
$$
Hence $|w-v|\geq \lambda(z)/10$ if $c$ is sufficiently small.

It follows that 
$$
\sin \lhd(\theta(z) , w-v) \leq \frac{50}{\rho(z)},
$$
which concludes the proof choosing $\rho_l := 50 / \sin (\cPi/12)$.
\sq

The next lemma is devoted to the comparison of the Voronoi cell of a vertex $v\in \cV$ with closed balls $\overline B_H(v,r)$ around $v$ for the norm $\|\cdot \|_{H(z)}$ (which are therefore some ellipses)
$$
\overline B_H(v,r) := \{z\in \R^d \sep \|z-v\|_{H(v)} \leq r\}.
$$

\begin{lemma}
\label{lemmaVorBall}
If $c$ is sufficiently small, then the following holds.
For any $v\in \cV$
\begin{eqnarray*}
\overline B_H(v,1/25)  &\subset& \Vor(v)\\
\overline B_H(v,\alpha(c) /10) &\supset& \Vor(v) \cap \Gamma\\
\overline B(v,\alpha(c) \mu(v)/5) &\supset& \Vor(v) \cap \Gamma_v 
\end{eqnarray*}


%\begin{enumerate}
%\item
%$$
%\overline B_H(v,1/25)  \subset \Vor(v), %:= \{z\in \R^2 \sep \|z-v\|_{H(v)} \leq 1/25\}
%$$
%%\item
%$$
%\overline B_H(v,\alpha(c) /10) \supset \Vor(v) \cap \Gamma
%$$
where $\alpha(c) := (e^{c/10} - 1)/(c/10)$ which tends to $1$ as $c \to 0$.
%\end{enumerate}
\end{lemma}

\proof
We consider $z\in \partial \Vor(v)$, hence $z\in \Vor(v) \cap \Vor(w)$ for some vertex $w\in \cV$.
We define $r:=\|z-v\|_{H(v)} = \|z-w\|_{H(w)}$ and we obtain using Point i) of Lemma \ref{lemmaConstV}
\begin{eqnarray*}
1/10 &\leq& d_H(v,w)\\
&\leq& d_H(z,v)+d_H(z,w)\\
&\leq& -\ln (1-c\|z-v\|_{H(v)})/c - \ln (1-c\|z-v\|_{H(v)})/c\\
&=& -2 \ln (1-cr)/c.
\end{eqnarray*}
It follows that 
$$
r\geq (1-\exp(-c/20))/c,
$$
and therefore $r\geq 1/25$ if $c$ is sufficiently small, 
which concludes the proof.\\

According to point ii) of Lemma \ref{lemmaConstV} there exists $w\in \cV$ such that $d_H(z,w) \leq 1/10$. It thus follows from the definition of the Voronoi diagram that 
\begin{eqnarray*}
\|z-w\|_{H(w)} &\leq& \|z-w'\|_{H(w')}\\
&\leq& (\exp(c d_H(z,w'))-1)/c\\
&\leq&  (\exp(c/10)-1)/c,
\end{eqnarray*}
which concludes the proof.
\sq



\begin{lemma}
\label{lemmaInGammav}
The following holds if $c$ is sufficiently small.
Let $v,w\in \cV$ be such that $\Vor(v) \cap \Vor(w) \cap \Gamma_v \neq \emptyset$.
If $\rho(v) \geq 20$ then $w\in \Gamma_v$.
\end{lemma}

\proof
%We now turn to the third point of the proposition, and we consider a point $z\in \Vor(v) \cap \Vor(w) \cap \Gamma$.
We consider $z\in \Vor(v) \cap \Vor(w) \cap \Gamma_v$. %, and we denote $r := \|z-v\|_{H(v)} = \|z-w\|_{H(w)} \leq \alpha(c)$.
%We thus have $\|z-v\|_{H(v)} = \|z-w\|_{H(w)} \leq r_0(c)$ which implies 
%$$
%\ln(1+c\|v-w\|_{H(v)})/c \leq d_H(v,w) \leq d_H(v,z)+d_H(z,w) \leq -2 \ln(1-c r_0(c))/c
%$$
%hence $\|v-w\|_{H(v)} \leq ((1-cr_0(c))^{-2}-1)/c$ which tends to $1/5$ as $c\to 0$. 
%If $c$ is sufficiently small
According to Lemma \ref{lemmaVorBall} we thus have 
$
|z-v| \leq \mu(v) \alpha(c)/5%\|z-v\|_{H(v)} \leq \alpha(c)/10.
$
On the other hand 
$$
\frac{|z-w|}{\lambda(v)(1+5c)} \leq \frac{|z-w|}{\lambda(w)} \leq \|z-w\|_{H(w)} \leq \frac{\alpha(c)}{10}.
$$
Therefore injecting Proposition \ref{propDistUpLow}
$$
\frac {10}{91} \lambda(v)\leq |v-w| \leq  (2\mu(v) + (1+5c) \lambda(v)) \alpha(c) \leq \lambda(v) \left(1+5c+\frac 2 {\rho(v)}\right) \frac{\alpha(c)} {10}
$$
which implies 
$$
\frac {10}{91} \leq \left(1+5c+\frac 2{20}\right) \frac{\alpha(c)}{10}
$$
As $c\to 0$ the right hand side tends to $11/100<10/91$. Hence we obtain a contradiction if $c$ is sufficiently small.
\sq


Note that $\Gamma\sm\cV$ is a collection of straight open intervals, since $\cV_0\subset \cV$.
We define 
\begin{eqnarray*}
\Gamma_z^+ &:=& \{z'\in \Gamma_z \sep \<\theta(z)^\perp , z'-z\> \geq 0\} \\
\Gamma_z^- &:=& \{z'\in \Gamma_z \sep \<\theta(z)^\perp , z'-z\> \leq 0\}
\end{eqnarray*}
For instance if $\Gamma_{v_0}^+ = [v_0,(v+2w_+)/3$ and $\Gamma_{v_0}^- = [v_0,(v+2w_-)/3$ for any $v_0\in \cV_0$.

\begin{lemma}
If 
\end{lemma}



For any two vertices $v,w\in \cV$, we say that $[v,w]$ is an edge of $\Gamma$ if 
$$
(v,w) \subset \Gamma\sm \cV.
$$




\begin{lemma}
\label{lemmaSegVor}
The following holds if $c$ is sufficiently small.
If $v\in \cV$ and $\Gamma_v^+ \sm \Vor(v) \neq \emptyset$, then there exists $w\in \Gamma_v^+$ such that $[v,w]$ is an edge of both $\Gamma$ and $\cT$.
Furthermore $|v-w|\leq \mu(v)/2$. 
A similar property holds for $\Gamma_v^-$.


%If $[v,w]$ is an edge of $\Gamma$ and $\rho(v) \geq \rho_0 := 22$, then $[v,w]$ is an edge of $\cT$.
%If $c$ is sufficiently small, then the following holds.
%For any $v\in \cV$ such that $\rho(v) \geq \rho_0 = 22$ the vector $v$ has at least a neighbor on $\Gamma$. Furthermore for any neighbor $w$ of $v$ on $\Gamma$ we have 
%$$
%|v-w|\leq \mu(v)/2
%$$
%and 
%\be
%\label{eqNeighborEdge}
%[v,w] \subset \interior(\Vor(v) \cup \Vor(w)).
%\ee
%and consequently $[v,w]$ is an edge of $\cT$. 
\end{lemma}

\proof
We consider $v\in \cV$ such that $\rho(v) \geq 20$, a point $z\in \partial\Vor(v) \cap \Gamma_v^+$, and another vertex $w\in \cV$ such that $z\in \Vor(v)$.
According to Lemma \ref{lemmaInGammav} we have $w\in \Gamma_v$.

Remark that according to Lemma \ref{lemmaDiamVorGamma}
$$
1/4 \geq \|v-w\|_{H(v)} \geq \frac{|v-w| \cos (\cPi/3)}{\mu(v)} = \frac{|v-w|}{2\mu(v)}
$$
hence $|v-w|\leq \mu(v)/2$ which establishes the size estimate.


Let us assume for contradiction that $w\in \Gamma_v^-$.
Hence there exists $\alpha\in [0,1]$ and $r\in \R$ such that 
$$
v + r \theta(v) = z+ \alpha(w-z).
$$
Denoting by $u$ a unit vector orthogonal to $w-z$ we obtain 
$$
r\<\theta(v),u \> = \<z-v , u\>
$$
hence according to Lemma \ref{lemmaVorBall}
\be
\label{eqCutVor}
|r|/2\leq |r| \cos \lhd(\theta(v)^\perp, w-v) = |r|\cos\lhd(\theta(v), u)  \leq  |z-v| \leq \mu(v) \alpha(c)/5.
\ee
According to \cite{Shew} Lemma 3 (Visibility Lemma) the Voronoi regions of a wedged Voronoi diagram are star-shaped. 
%Since the Voronoi diagram is wedged according to Lemma \ref{lemmaRecallG} we obtain using 
We thus obtain from Lemma \ref{lemmaVorBall} that 
$$
|r| = \|r\theta(v)\|_{H(v)} \geq \frac {\lambda(v)} {25}.
$$
Combining the last equation with \iref{eqCutVor} we obtain $\rho_0 \leq \rho(v) \leq 10 \alpha(c)$. If $c$ is sufficiently small we have $10 \alpha(c) <11$ which gives a contradiction.

It follows that $w\in \Gamma_v^+$, and therefore there exists $v'\in \Gamma_v^+$ such that $[v,v']$ is an edge of $\Gamma$. 
Our purpose is now to establish that $v' = w$.
Assume for contradiction that this is not the case.
There exists $\alpha\in [0,1]$ and $r\in \R$ such that 
$$
v'+r \theta(v') = z + \alpha(w-z).
$$
denoting by $u$ a unit vector orthogonal to $w-z$ we obtain as previously 
$
r \<\theta(v'),u\> = \<z-v', u\>
$
and therefore as previously
$$
|r|/2 \leq  |r|\cos\lhd(\theta(v'), u) \leq |z-v'| \leq |z-w| \leq |v-w|\leq \mu(v) \alpha(c)/2.
$$
On the other hand since the Voronoi regions are star shaped
$
|r| \geq  \lambda(v')/25 \geq \lambda(v)(1-c)
$
which implies $\rho(v) \leq 25/(1-c)$ which is a contradiction if $c$ is sufficiently small.

%We have 
%$$
%|v-v'|\leq |v-w|\leq \mu(v)/2.
%$$
%Assume for contradictio
%
%We have $\rho(v') \geq \rho(v)-1\geq 20$ if $c\leq c_\rho(20,1)$. Without loss of generality we may assume that $\<\theta(v), \theta(v')\> \geq 0$. Hence $v$ and $z$ belong to $\Gamma_v^{-}$
%
%
%
%Without loss of generality we may assume that the orientations
%Without loss of generality 
%
%
%
%
%
%
%
%It follows that $w'\in \Gamma_v^+$.
%
%Since $[v,w]$ is an edge of $\Gamma$, we thus have 
%$$
%|z-w| \leq |v-w| \leq |v-w'| \leq ??\sim 2\mu(v) \alpha(c)/5
%$$
%Furthermore there exist
%we apply the same reasoning to $w$, again with star shaped.
%%We now remark that the vertices $v,w$ belong to the same element of $\cT_0$ since they are neighbors on $\Gamma$. Hence $\rho(w) \geq \rho_0 - 1=21$ if $c$ is sufficiently small.
%Way may therefore apply this proof to $w$, and we obtain that $w'$ is on the same side as $v$ with respect to $w$, in the sense that  $\<w'-w, \theta(w)^\perp \><0$ and $\<w'-v, \theta(w)\> <0$ (if $\<\theta(w), \theta(v)\> >0$).
%
%It follows that $w'\in (v,w)$ which is a contradiction.
%
%
%Finally, we remark that according to Lemma \ref{lemmaDiamVorGamma}
%$$
%1/4 \geq \|v-w\|_{H(v)} \geq \frac{|v-w| \cos (\cPi/3)}{\mu(v)} = \frac{|v-w|}{2\mu(v)}
%$$
%hence $|v-w|\leq \mu(v)/2$ which concludes the proof.
\sq

We introduce a new constant 
$$
\rho_0 := \max\{\rho_l, 2C_0\}.
$$
The next proposition states that the edges attached to a simplex $v$ such that $\rho(v) \geq \rho_0$ are of two types : either included in $\Gamma$, or aligned with the direction $\theta(v)$ of anisotropy.

\begin{prop}
The following holds if $c$ is sufficiently small.
Let $v\in \cV$ be such that $\rho(v)\geq \rho_0$. %, where $\rho_1$ is a constant specified in the proof, then 
\begin{enumerate}
\item There exists two edges $[v,w]$, $[v,w']$ of $\cT$ such that 
\be
\label{eqAnglesUpDown}
\varangle(w-v, \theta(v)) \leq \cPi/12 \stext{ and } \varangle(w'-v, -\theta(v)) \leq \cPi/12.
\ee
\item For any $w\in \cT\cap \Gamma_v$, the segment $[v,w]$ is an edge of $\cT$ if and only if it is an edge of $\Gamma$.
\end{enumerate}
\end{prop}

\proof
We first remark that $\Gamma_v \sm\Vor(v)\neq \emptyset$. Indeed there exists an edge $[v_0,w_0]$ of $\cT_0$ such that $v\in [v_0, (v_0+2w_0)/3] \subset \Gamma_v$.
Therefore according to \iref{edgeLambda}
$$
\max \{|v-v_0|, |v-w_0| \} \geq |v_0-w_0|/3 \geq \lambda(v)\sqrt 2/9.
$$
On the other hand $|z-v| \leq \mu(v)/4$ for all $z\in \Vor(v)\cap \Gamma_v$. Since $\rho(v) \geq \rho_0 > 9/(4\sqrt 2)$ we find that $v_0$ or $w_0$ does not belong to $\Vor(v)$.

Assume that $\Gamma_v^+\sm\Vor(v)\neq \emptyset$. Then according to the previous lemma there exists $w_*\in \Gamma_v^+$ such that $[v,w_*]$ is an edge of both $\Gamma$ and $\cT$.
Let $T,T'\in \cT$ be the two triangles containing the edge $[v,w_*]$, and let $w,w'\in \cV$ be the third vertex of these triangles respectively.

Since $\cT$ is $C_0$-adapted to the metric $H$, we obtain (*argument : inclusion of ellipse*)
$$
|v-w_*|+|v-w| > \diam(T) \geq \|\cH_T^{-\frac 1 2}\|/2 \geq \|H(v)^{-\frac 1 2}\|/(2C_0) = \lambda(v)/(2C_0).
$$
If both $w$ and $w_*$ belong to $\Gamma_v$, then we obtain $\rho(v) < 2C_0$ which is a contradiction.

Therefore $w\notin \Gamma_v$ which implies $\lhd(\theta(v), w-v) \leq \cPi/12$ according to Lemma \ref{lemmaThreeTypes}, which implies $\lhd(\theta(v), w-v)\in [0\cPi/12]\cup[11\cPi/12, \cPi]$. Likewise $\lhd(\theta(v), w'-v)\in [0\cPi/12]\cup[11\cPi/12, \cPi]$.
Since $\varangle (\theta(v), w_*-v) \in [\cPi/6, 5\cPi/6]$ according to Lemma ??, and since the triangles $T$ and $T'$ are on opposite sides of the edge $[v,w_*]$ we obtain  \iref{eqAnglesUpDown}.

For any vertex $v'\in \Gamma_v^+$ we also have $\varangle (\theta(v), v'-v) \in [\cPi/6, 5\cPi/6]$, which implies that the segment $[v,v']$ intersects one of the triangles $T$ or $T'$. Therefore $[v,v']$ is not an edge of $\cT$.\\

We proceed likewise for $\Gamma_v^-$ : either $\Gamma_v^-\sm \Vor(v)$ is empty, and therefore $\Gamma_v^{-} \cap \cV= \emptyset$, or $\Gamma_v^{-}\sm\Vor(v)\neq \emptyset$ and similarly we obtain that there exists $w_{**}\in \Gamma_v^{-}$ such that $[v,w_*]$ is an edge of both $\Gamma$ and $\cT$, and that for any $v''\in \Gamma_v\cap \cV$ distinct from $w_{**}$ the segment $[v,v'']$ is not an edge of $\cT$.

This implies Point 2. and concludes the proof of this proposition.
\sq

For each $v\in \cV_0$ we define $\Gamma'_v := [v,w_-] \cup[v,w_+]$ where $w_-$ and $w_+$ are defined by \iref{defWmWp}.
We then set 
$$
\Gamma' := \bigcup_{\substack{v\in \cT_0\\ \rho(v) \geq 1+\rho_1}} \Gamma'_v.
$$


\begin{prop}
If $c$ is sufficiently small, then the following holds.
Denote by $\cQ$ the partition into convex polygons of $\R^2$ obtained by the overlay of $\cT$ and $\Gamma'$.
Denote by $\cT'$ the partition obtained by randomly triangulating the convex cells of $\cQ$.


%Denote by $\cT'$ the triangulation obtained by randomly triangulating the 
%
%Denote by $\cQ$ the partition into convex polygons obtained by cutting $\cT$ by all segments joining an extremal vextex $v\in \cV$ satisfying $\rho(v) \geq ??$ to the vertex $v'\in \cV_0$ in the direction of $\bt(v)$.
%
%Then the interior angles in $\cQ$ are smaller than ??. %Each triangle $T\in \cT$ contains at most $??$ cells of $\cC$, which are at most hexagons (in other words they have $3$ to $6$ elements).
%
%Denote $\cT'$ the triangulation obtained by randomly triangulating the convex cells of $\cQ$.

Then $\cT'$ is a $??$-refinement of $\cT$ and $S(T') \leq ??$ for all $T'\in \cT'$.
\end{prop}

\proof
Since the collection $\cV$ of vertices of $\cT$ contains $\cV_0$ and since the segments in $\Gamma$ join some points of $\cV_0$, we find that the overlay of $\cT$ and $\Gamma$ is indeed a partition of $\R^2$ into convex polygons.

Our first objective is to give a uniform bound on the measure of sliverness in $\cT'$.
For that purpose we consider a cell $Q \in \cQ$, hence a convex polygon, and a vertex $z$ of $Q$.

We first assume that $z\notin \cV$, hence $z$ is a vertex created by the overlay of $\Gamma$ on $\cT$.
We denote by $v_0$ the vertex in $\cV_0$ such that $z\in \Gamma'_{v_0}$, and we observe that $\rho(v_0) \geq \rho_0+1$.
Let $[w,w']$ be the edge of $\cT$ containing $z$. We have 
$$
|z-w| \leq \lambda(z) \|z-w\|_{H(z)} \leq \lambda(z) \|w-w'\|_{H(z)} \leq 5 \lambda(z)\leq 5 \lambda(v_0)(1+c). 
$$
hence
$$
|v_0 - w| \leq |v_0 - v| + |v-w| \leq \lambda(v_0) (6+5c).
$$
If $c$ is sufficiently small, then we obtain $\rho(w) \geq \rho_1$.
Therefore $w' \notin \Gamma_w$, otherwise $w'$ would be a neighbor of $w$, $[w,w'] \subset \Gamma$ which contradicts the fact that this edge was bisected by the overlay.

Hence $\sin \lhd(\theta(v),v-w) \leq 50/\rho(v)$. Hence $\lhd(\theta(v),v-w) < \cPi/24$. On the other hand $\lhd(\theta(v), \theta(z)) \leq 2 \times 5 c \leq \cPi/24$ if $c$ is sufficiently small. We conclude that $\lhd(v-v_0, w,w') \geq \cPi/12$.\\

We may therefore assume that $v\in \cV$.
If $\rho(v) \leq 2+\rho_1$ then 
$$
S(T) \leq \rho(T) = \sqrt {\|\cH_T\| \|\cH_T^{-1}\|} \leq C_0^2 \rho(v) \leq C_0^2 (2+\rho_1).
$$
The angle $\vp$ of $\cQ$ at $v$ is bounded by the angle of $T$ at $v$, hence by
$$
\tan \vp \leq C_0^2 (2+\rho_1),
$$
which gives a uniform bound.\\


If $\rho(v)\geq 2+\rho_1$, then there exists two neighbors $w,w'$ of $v$ satisfying \iref{eqAnglesUpDown}. Let $v_0\in \cT_0$ be such that $v \in \Gamma_{v_0}$. 
If $c$ is sufficiently small, then $\rho(v_0) \geq 1+\rho_1$. 
Therefore $v\in \Gamma'_v$, and the tangent $\bt, \bt'$ vectors to $\Gamma'_v$ in the two directions satisfy $\lhd(\theta(v)^\perp, \bt) \leq \cPi/3$ and $\lhd(\theta(v)^\perp, \bt') \leq \cPi/3$.

It follows that the angle of $Q$ at $v$ is bounded by $5 \cPi/6$.\\


We now prove that $\cT'$ is a bounded refinement of $\cT$, and for that purpose we consider and edge $e=[v,w]$ of $\cT$. %=[\omega-u, \omega+u]

We have by construction $|v-w|/\lambda(v) \leq \|v-w\|_{H(v)} \leq 12$.
The triangles $T\in \cT_0$ intersected by $[v,w]$ satisfy for some $z\in [v,w]$ the inequality 
$$
2 \delta_0 \lambda(v) (1-12c) \leq 2 \delta_0 \lambda(z) \leq \diam(T) \leq \lambda(v) \leq \lambda(u)(1+12c)
$$
Therefore they are contained in the ball $B(v,  \lambda(v)(12+1+12c))$ and have area 
$$
|T| = \diam(T)^2/4 \geq \delta_0^2 \lambda(v)^2 (1-12c)^2.
$$
Therefore there are at most 
$$
\cPi (13+12c)^2/ (1-12c)^2 \leq k := \cPi 14^2,
$$
such triangles, and the edge $e$ is thus cut in at most $k$ parts by the edges joining an extremal vertex in $\cV$ to the corresponding vertex in $\cV_0$.

Hence there are at most $3k$ vertices of $\cT'$ on the three edges of a triangle $T\in \cT$ (including the vertices of $T$).
Since any conforming triangulation of convex envelope of $n+2$ points uses $n$ triangles, we obtain that $\cT'$ is a $3k-2$ refinement of $\cT$.
\sq

%\input{../Bibliography/Bibliography.tex}
\end{document}



==> Variations/VariationsTheseOld.tex <==
We study in this section some variations on the greedy algorithm. 

We consider in \S \ref{secAltDec} two decision functions, based on the $L^2$ approximation error or the $L^\infty$ interpolation error, which offer an alternative choice to the decision function \iref{eqDecisionL1} based on the $L^1$ interpolation error used in the previous chapter. The study of these decision functions is guided by the following reasons. The $L^2$ based decision function can be computed at a significantly smaller numerical cost than the $L^1$ based or $L^\infty$ based decision functions, and is therefore the method of choice in numerical applications. The $L^\infty$ based decision function, in contrast, allows us to obtain the most general convergence results. % from the theoretical point of view.


We then turn our attention in \S \ref{secAltBi} to the approximation of cartoon functions. % using the greedy algorithm. 
Unfortunately, it turns out in \S \ref{secNegRes} that the greedy algorithm fails to produce satisfying approximations of these functions. 
We then consider in \S\ref{secTriSec} and \S \ref{secConvexCut} some modifications of the greedy algorithm which partially solve this problem using alternative bisection choices. Instead of bisecting a triangle from a vertex to the midpoint of the opposite edge, we offer different possibilities which lead to more directional selectivity. In turn we obtain a satisfying convergence rate for a simple cartoon function, the characteristic function $f=\chi_P$ of the half plane $P=\{(x,y) \sep y \geq 0\}$. The behavior of the greedy algorithm on general cartoon functions remains an open question.

Eventually we consider in \S \ref{secGreedyRect} a variation of the greedy algorithm which is in some sense much simpler. 
It is based on piecewise constant approximation, instead of piecewise linear, and it produces partitions of the original domain into rectangles aligned with the coordinate axes, instead of triangles of arbitrary direction. 
Thanks these simplifications we were able to analyze this algorithm in a rather general setting, and we establish in Theorem \ref{thRect} a result of optimal convergence which applies to any $C^1$ function.


% extremely simplified version of the 
%Our motivation for studying these alternative choices are the following
%A
%
%Let us recall its main features.
%Given a function triangulation $\cT_{N_0}$ of a polygonal domain $\Omega$, of cardinality $\#(\cT_{N_0})$, and a function $f$ defined on $\Omega$, this algorithm generates a sequence $(\cT_N)_{N\geq N_0}$ of anisotropic triangulations, of cardinality $\#(\cT_N) = N$. Under some assumptions on the function $f$, it can be proved that asymptotically the approximation error of $f$ on these triangulations is optimally small.

\section{Alternative decision functions}
\label{secAltDec}

%At the heart of this algorithm there is a decision function $d_T(e,f)$, where $T\subset \Omega$ is any triangle and $e$ is an edge of $T$, which drives the creation of anisotropy. 
The purpose of this section is to investigate two alternative choices to the decision function \iref{eqDecisionL1} used in the previous chapter \S \ref{chapBisecOpt}.
In order to make these statements precise and to justify the study of these alternative decision functions, we need to introduce some notations. Most of those are simply recalled from the previous chapter.

We consider a fixed exponent $p$, $1\leq p\leq \infty$. %, and we measure the approximation errors in $L^p$ norm. %in which the approximation errors are measured.
For any triangle $T$ and any function $f\in C^0(T)$ we denote by $e_T(f)_p$ the approximation error of $f$ on $T$,
$$
e_T(f)_p := \|f-\cA_T f\|_p,
$$
where $\cA_T : C^0(T) \to \P_1$ is a linear operator which satisfies some assumptions given in \S\ref{subsecAssumAT}.
For any triangulation $\cT$ of a domain $\Omega$ and any $f\in C^0(\Omega)$ we denote by $e_\cT(f)_p$ the approximation error of $f$ on $\cT$ by piecewise linear elements, 
$$
e_\cT(f)_p^p := \sum_{T\in \cT} e_T(f)_p^p.
$$

%For any sequence $(\cT_N)_{N \geq N_0}$, of  of a polygonal domain $\Omega$
Let us briefly recall the definition of the greedy algorithm. % studied in this part of the thesis.
Let $\cT$ be a triangulation of a domain $\Omega$ and let $f\in C^0(\Omega)$.
The greedy algorithm creates in one step a triangulation $\cT'$ of $\Omega$, of cardinality $\#(\cT') = \#(\cT)+1$, proceeding as follows : 
\begin{enumerate}[a)]
\item A triangle $T\in \cT$ which maximizes the approximation error is selected.
$$
T = \underset {T'\in \cT} \argmax \ e_{T'}(f)_p.
$$
%where $e_T(f)_p$ is defined in [???].
\item %The refinement procedure considers the three edges $a,b,c$ of $T$. 
For each edge $e\in \{a,b,c\}$ of the triangle $T$ the bisection of $T$ from the midpoint of $e$ to the opposite vertex defines two children $T_e^1$ and $T_e^2$.
The edge $e$ which minimizes a given decision function $d_T(e,f)$ is selected
%, and selects the one which minimizes a given decision function $d_T(e,f)$,
$$
e := \underset {e'\in \{a,b,c\}} \argmin \ d_T(e',f).
$$
and we define the triangulation $\cT'$ by 
%The triangle $T$ is then bisected along the segment joining the midpoint of the edge $e$ to the opposite vertex. We denote by $T_e^1, T_e^2$ its children and we define the triangulation $\cT'$ by 
$$
\cT' := \cT - \{T\} + \{T_e^1, T_e^1\}.
$$
\end{enumerate}
Starting from a triangulation $\cT_{N_0}$ of the polygonal domain $\Omega$ , with $\#(\cT_{N_0}) = N_0$, the greedy algorithm creates step after step a sequence $\cT_{N_0+1}, \, \cT_{N_0+2}, \, \cdots$ of triangulations of $\Omega$ satisfying $\#(\cT_N) = N$. 

%In the previous part \S?? we considered the decision function defined by 
A possible choice for the decision function $d_T(e,f)$ %used in b) 
is the following, which is based on the $L^1$ interpolation error
\be
\label{eqDecisionL1}
d_T(e,f) := \|f-\interp_{T_e^1} f \|_{L^1(T_e^1)}+  \|f-\interp_{T_e^2} f \|_{L^1(T_e^2)},
\ee
where we denoted by $\interp_T f$ is the interpolation of a continuous function $f$ on a triangle $T$.

Theorem \ref{optitheo} states that if the function $f$ to be approximated is $C^2$ and strictly convex, and if the decision function is given by \iref{eqDecisionL1} then the sequence of triangulations generated by the greedy algorithm satisfies the asymptotical error estimate
\be
\label{eqOptiConv}
\limsup_{N\to \infty} N e_{\cT_N}(f) \leq C \left \| \sqrt{|\det(d^2 f)|} \right\|_{L^p(\Omega)}.
\ee
This theorem convergence estimate is the best that one can hope to achieve, and Theorem \ref{optitheorem} shows that it is optimal under some minor technical assumptions.
%According to  this error estimate is optimal among admissible sequences of triangulations (admissibility is a technical assumption, defined in (??)) .

%The parts 
%As observed in Remark \ref{remDiffRoles} the parts 1. and 2. of one step of the greedy algorithm have distinct purposes. In a few words, the purpose of the first part is to equidistribute the local $L^p$ error, while the second part drives the creation of anisotropy by selecting the splitting direction of the triangles.
%
%If $f$ is a $C^2$ and stricly convex function, then it is established in the previous chapter that the greedy algorithm generates an asymptotically optimal sequence of triangulations for the approximation of $f$ in $L^p$ norm, provided that the decision function is defined by 
%\be
%\label{eqDecisionL1}
%d_T(e,f) := \|f-\interp_{T_e^1} f \|_{L^1(T_e^1)}+  \|f-\interp_{T_e^2} f \|_{L^1(T_e^2)}.
%\ee
%In the previous expression, $e\in \{a,b,c\}$ is one of the edges of the triangle $T$, and $T_e^1, T_e^2$ are the two triangles obtained by splitting $T$ along the segment joining the midpoint of $e$ to the opposite vertex.

The purpose of this chapter is to investigate two alternative choices, replacing \iref{eqDecisionL1}, for the decision function $d_T(e,f)$. 
The first of these choices is based on the $L^2$ approximation error 
\be
\label{eqDecisionL2}
d_T(e,f) := \|f-P_{T_e^1} f \|_{L^2(T_e^1)}^2+  \|f-P_{T_e^2} f \|_{L^2(T_e^2)}^2,
\ee
where, for any triangle $T$, we denote by $P_T$ the $L^2(T)$ orthogonal projection onto the space $\P_1$ of affine functions. The second choice is based on the $L^\infty$ interpolation error,
\be
\label{eqDecisionLInf}
d_T(e,f) := \|f-\interp_{T_e^1} f \|_{L^\infty(T_e^1)}+  \|f-\interp_{T_e^2} f \|_{L^\infty(T_e^2)}.
\ee
Our motivations for studying these alternative decision functions %, and therefore the two corresponding modified greedy 
are the following.
\begin{itemize}
\item \emph{Decision function based on the $L^2$ error  \iref{eqDecisionL2}.}\\
From the point of view of computer run time, the biggest cost of the greedy algorithm comes from the evaluation of the decision function. As exposed below, a trick allows to evaluate the (discretized) $L^2$ based decision function \iref{eqDecisionL2} much faster than the $L^1$ based or $L^\infty$ based decision functions \iref{eqDecisionL1} and \iref{eqDecisionLInf}. 

The greedy algorithm has been implemented in C++ by Pr Lihua Yang.
For an image of realistic resolution, say $512 \times 512$, the (discretized) greedy algorithm takes only a few seconds to generate $5000$ triangles using the $L^2$ based decision function if it is efficiently evaluated. In contrast it may take up to a minute to generate the same number of triangles based on a brute force evaluation of the $L^2$ based decision function, or the $L^1$ based or $L^\infty$ based decision functions. 
As a result the $L^2$ based decision function \iref{eqDecisionL2} is the only one used in numerical experiments.

Theorem \ref{thOptiL2LInf} shows that the greedy algorithm based on the $L^2$ decision function \iref{eqDecisionL2} generates a sequence of triangulations satisfying the optimal estimate \iref{eqOptiConv} when it is applied to any quadratic function $f=q$ such that the quadratic form $\bq$ is non-degenerate.
In particular $q$ may be either stricly convex, concave or of hyperbolic type. 
The latter case, which corresponds to a mixed signature $(1,1)$ of the quadratic form $\bq$, is not treated in the  study in the previous chapter \S \ref{chapBisecOpt} of the $L^1$ based decision function \iref{eqDecisionL1}.\\

\item \emph{Decision function based on the $L^\infty$ error  \iref{eqDecisionLInf}.}\\
So far our most complete theoretical results are for the $L^\infty$ based decision function \iref{eqDecisionLInf}. 
Indeed Theorem \ref{thOptiL2LInf} shows that the optimal convergence estimate \iref{eqOptiConv} is achieved for any quadratic function $f=q$ such that the quadratic form $\bq$ is non degenerate.
Furthermore, it follows from Proposition \ref{propDiamZeroLInf} that the optimal estimate \iref{eqOptiConv} is also achieved for functions which are $C^2$ and stricly convex. The latter case is treated in Theorem \ref{optitheo} for the $L^1$ based decision function, but is not established for the $L^2$ based decision function.\\
%We were able to establish that the greedy algorithm generates an asymptotically optimal sequence of triangulations when the function $f$ to be approximated is a quadratic function of non degenerate associated quadratic form, either convex, concave or of hyperbolic type, and when $f$ is a $C^2$ and strictly convex function.
\end{itemize}

This chapter is organized as follows. We expose in \S \ref{secPosQuad} a detailed study 
of the different decision functions for a strictly convex quadratic function $f=q\in \P_2$.
We show in particular that among the three edges $e\in\{a,b,c\}$ of a triangle $T$ each of the three decision functions  $d_T(e,q)$, defined by \iref{eqDecisionL1}, \iref{eqDecisionL2} or \iref{eqDecisionLInf}, is minimal for the longest edge of $T$ measured in the $\bq$-metric $|\cdot|_q$. 
These results lead in \S \ref{subsecRatioConvex} to the proof that the greedy algorithm achieves the optimal asymptotic estimate \iref{eqOptiConv} when $f$ is such a quadratic function, but also when $f$ is a strictly convex $C^2$ function and the decision function is \iref{eqDecisionLInf}.

We then turn in \S \ref{secNegQuad} to quadratic functions $f=q$ of hyperbolic type, or mixed signature, a case that is not investigated in the previous chapter \S\ref{chapBisecOpt}. In other words such that the quadratic form $\bq$ has signature $(1,1)$. 
We identify the choice of the decision functions \iref{eqDecisionL2} and \iref{eqDecisionLInf} and we prove that the greedy algorithm achieves the optimal asymptotic error estimate \iref{eqOptiConv}. 


Before turning to the detailed study of the different decision functions, %\iref{eqDecisionL2} and \iref{eqDecisionLInf},
we expose as announced why the (discretized) $L^2$ based decision function \iref{eqDecisionL2} is much less expensive to compute than the $L^1$ based or $L^\infty$ based decision functions, in terms of computer run time.

Let $T$ be a triangle, and let $M_T$ be the following $3\times 3$ symmetric positive definite matrix, the Grammian matrix of the basis $(1,x,y)$ of the subspace $\P_1$ of $L^2(T)$,
$$
M_T := \int_T \left( 
\begin{array}{ccc}
1 & x & y\\
x & x^2 & xy\\
y & xy & y^2
\end{array}
\right)
dx\, dy
= 
\int_T
 (1,x,y)(1,x,y)^\trans
dx\,dy.
$$
Let also $V_T(f)\in \R^3$ be the vector of the first order moments of the function $f$ on $T$, 
$$
V_T(f) := \int_T (1,x,y)^\trans f(x,y) \, dx\, dy.
$$
The $L^2(T)$ orthogonal projection of $f$ onto $\P_1$ has the expression %One easily shows that 
$$
P_T(f) = (1,x,y)M_T^{-1} V_T.
$$
Therefore, denoting by $\<\cdot, \cdot\>$ the $L^2(T)$ scalar product,
\begin{eqnarray*}
\|f-P_T f\|_{L^2(T)}^2 &=& \|f\|_{L^2(T)}^2 - 2 \<f, P_T(f)\> + \|P_T(f)\|_{L^2(T)}^2\\
&=&  \|f\|_{L^2(T)}^2 - \|P_T(f)\|_{L^2(T)}^2\\
&=& \int_T f(x,y)^2 dx\, dy - V_T(f)^\trans M_T^{-1} V_T(f).
\end{eqnarray*}
Hence the $L^2(T)$ approximation error of $f$ on $T$ has an expression in terms of the integrals on $T$ of the functions $1,\, x,\, y,\, x^2, \, xy, \, y^2$, and $f, xf, yf, f^2$.
We now recall that the Fubini formula which transforms an integration on a bidimensional domain into two successive one dimensional  integrations. Indeed for any triangle $T$ and any $g\in L^1(T)$,
\be
\label{eqFubiniG}
\int_T g(x,y) \, dx \, dy = \int_{y_*(T)}^{y^*(T)} \left(\int_{x_*(T,y)}^{x^*(T,y)} g(x,y) dx \right) dy = \int_{y_*(T)}^{y^*(T)} \(G(x^*(T,y),y) - G(x_*(T,y),y) \)dy.
\ee
Where we have used the notations 
\begin{eqnarray*}
G(x,y)    &:=& \int_{-\infty}^x g(x,y) dy,\\
y_*(T)    &:=& \min\{ y\in \R \sep \exists x \in \R \text{ such that } (x,y) \in T\},\\
x_*(T,y) &:=& \min\{ x\in \R \sep (x,y) \in T\},
\end{eqnarray*}
and where $y^*(T)$ and $x^*(T,y)$ are obtained by taking the maximum instead of the minimum in the definitions of $y_*(T)$ and $x_*(T,y)$ respectively. The important point in \iref{eqFubiniG} is that the function $G$ does not depend on the triangle $T$. If this function is known, then \iref{eqFubiniG} transforms the bidimensional integration of $g$ into a one dimensional integration.
%The point that allows to drastically reduce The point that will be particularly useful to


The previous analysis extends to the discrete setting with the following modification : the Lebesgue measure on $T$ needs to be replaced with the sum of Diracs centered at the points of integer coordinates in $T$.
%$$
%\chi_T \, dx dy \quad \Rightarrow \quad \sum_{(i,j) \in T \cap \Z^2} \delta_{(i,j)}.
%$$ 
Indeed, the function $f$ that needs to be approximated is only sampled at the points of integer coordinates. The integrals appearing in the previous equations are therefore replaced by discrete sums.
%We now turn to the discrete setting. The function $g$ is replaced with a matrix $(g_{i,j})_{1\leq i,j \leq N}$, and the integral $\int_T g$ with 
\be
\label{eqIntDiscrete}
\int_T g(x,y) dx dy \quad \Rightarrow \quad
\sum_{(i,j)\in T} g_{i,j}.
\ee
In particular the quantity $\|f-P_T f\|_2^2$ appearing in the definition \iref{eqDecisionL2} of the $L^2$ based decision function is replaced with 
\be
\iref{eqErrorDiscrete}
\inf_{\pi \in \P_1} \sum_{(i,j)\in T} |f(i,j) -\pi(i,j)|^2.
\ee
Again, this quantity can be expressed in terms of the (discrete) integrals of the functions $1,x,y, \cdots, xf,yf,f^2,$ which do not depend on $T$.
The Fubini formula \iref{eqFubiniG} is replaced with 
\be
\label{eqFubiniDiscrete}
\sum_{(i,j)\in T} g_{i,j} = \sum_{j_*(T)\leq j \leq j^*(T)} G_{i_*(T,j), \, j} - G_{i^*(T,j), \, j}
\ee
where 
\begin{eqnarray*}
G_{i,j} &=& \sum_{0\leq i'\leq i} g_{i',j},\\
j_*(T) &=& \lfloor y_*(T) \rfloor\\
i_*(T,j) &=&  \lfloor x_*(T,j) \rfloor,
\end{eqnarray*}
and similarly  $j^*(T) = \lfloor y^*(T) \rfloor$ and $i^*(T,j) =  \lfloor x^*(T,j) \rfloor$. The points $(i_*(T,j),\, j)$, for all $j_*(T)\leq j \leq j^*(T)$, are illustrated on the right of Figure \ref{figFastIntegration} and surrounded by grayed  squares. On the same figure the points $(i^*(T,j),\, j)$, for all $j_*(T)\leq j \leq j^*(T)$, are surrounded by white squares.

Consider a fixed function $g$, such as $1,x,y,x^2,xy, y^2$ or $f,xf,yf,f^2$ which are needed for the evaluation of \iref{eqErrorDiscrete}, for which the sum \iref{eqIntDiscrete} needs to be evaluated for a large number of distinct triangles. The matrix $(G_{i,j})_{0\leq i,j \leq N}$ is evaluated once and for all and the sum \iref{eqIntDiscrete} is computed using \iref{eqFubiniG}, which involves a much smaller collection of points, see Figure \ref{figFastIntegration}.
%Let us assume that $g\in L^1(\Omega)$, and that $\int_T g$ needs to be computed for many different triangles $T\subset \Omega$.
%
%Let us assume that the function $g$ is defined domain $\Omega$ containing $T$, and that 
%Let $\Omega$ be a domain, and let $f\in L^1(\Omega)$
%If a given function 
%The dicretized computation of the integral of a function $g$ on a triangle $T$ can be partly precomputed as follows. 
This method greatly accelerates the numerical implementation of the greedy algorithm, in particular for the large and isotropic triangles that occur in its first steps.

\begin{figure}
	\centering
	\includegraphics[height = 4cm, width = 5cm]{\pathPic/Triangles/AllPts.pdf}
	\includegraphics[height = 4cm, width = 5cm]{\pathPic/Triangles/FewPts.pdf}
	\caption{\label{figFastIntegration}The cost of evaluating the interpolation error of a function $f$ on a triangle $T$  in the $L^1$ or $L^\infty$ norm is proportional to the number of points with integer coordinates on $T$ (left). Fewer points need to be considered to compute the $L^2$ projection error (right).} 
\end{figure}


\subsection{Positive quadratic functions}
\label{secPosQuad}

In this section, we study the algorithm 
when applied to a quadratic polynomial $q$ such that $\det(\b q)>0$. 
We shall assume without loss of generality that
$\b q$ is positive definite, since all our results
extend in a trivial manner to the negative definite case.

We first establish that 
the refinement procedure, either based on the 
decision functions \iref{eqDecisionL2} or \iref{eqDecisionLInf},
always selects for bisection the longest edge in the sense of the $\bq$-metric $|\cdot|_{\bq}$.
This is used to prove that the refinement procedure
produces triangles which tend to adopt an
optimal aspect ratio. 

\subsubsection{The $L^\infty$-based split}
\noindent
Let us denote by
$$
\alpha_T(f) = \|f-I_Tf\|_{L^\infty(T)},
$$
the interpolation error in the sup norm.
The decision function \iref{eqDecisionLInf} can be re-expressed
as
\be
d_T(e,f) = \alpha_{T_e^1}(f) + \alpha_{T_e^2}(f).
\label{optilinfedge}
\ee

\begin{theorem} \label{longestedgelinf}
If $|a|_{\bq}> \max\{|b|_{\bq},|c|_{\bq}\}$,
then $d_T(a,q) <\min\{d_T(b,q),d_T(c,q)\}$. Therefore the refinement
procedure based on {\rm \iref{optilinfedge}} selects the longest edge in the sense of the $\bq$-metric.
\end{theorem}

%This theorem means that for the quadratic function 
%$q(x,y) = x^2+y^2$, our refinement procedure is equivalent to the 
%{\it longest edge bisection} algorithm which has been extensively
%studied, see e.g. \cite{Ri}, and which is known to promote
%isotropic triangles. This gives us a
%first insight on why our algorithm might 
%generate triangles which are locally adapted to the hessian
%without computing this quantity. 
In order to prove this result, we need to study the interpolation
error in detail.

\begin{prop} \label{PropAlgErLInf}
Let T be a triangle with edges $a,b,c$ such that $|a|_\bq\geq |b|_\bq\geq |c|_\bq$,
and let $w\in \R^2$ and $r>0$ be the center and radius of 
the circumscribed circle for the $\bq$-metric,
i.e. such that $|v-w|_\bq=r$ for all the vertices $v$ of $T$. 
Then
$$
\frac{|a|_\bq^2} 4 \leq \alpha_T(q) \leq r^2.
$$ 
Right equality holds if $T$ is acute, i.e. $\< Q b, c\>\leq 0$, where $Q$ is the symmetric matrix associated to the quadratic form $\bq$. %$\b q(b,c)\leq 0$.
Left equality holds if $T$ is obtuse, i.e. $\< Q b, c\>\geq 0$. %$\b q(b,c)\geq 0$.
\end{prop}

\proof At any point $u\in \RR^2$, we have 
$$
(q - I_T q)(u) = |u-w|_\bq^2 - r^2.
$$
Indeed, the difference $(q - I_T q)(u) - (|u-w|_\bq^2 - r^2)$ is an affine function of $u$, which vanishes at the three vertices of $T$. Hence this difference is zero.

The function $|u-w|_\bq^2 - r^2$ is negative on $T$ with maximal value $0$ at the
vertices. If $T$ is acute, then its minimal value on $T$ is $-r^2$
and is attained at $w\in T$. If $T$ is not acute, 
then the minimum is attained at $m_a$, the midpoint of $a$, 
and if we choose a vertex $v$ at one end of $a$, 
we obtain the value at the minimum by 
Pythagoras' identity which gives
$$
\begin{array}{ll}
(q - I_T q)(m_a) &= |m_a-w|_\bq^2 - r^2= |m_a-w|_\bq^2 -|v-w|_\bq^2\\
& =-|v-m_a|_\bq^2 =-|a|_\bq^2/4.
\end{array}
$$ \sq 

The dichotomy in the above result is illustrated in the case of the
euclidean metric on figure 4. Note that it would be
sufficient to establish the above proof in this particular case,
since we can perform an affine coordinate change $\phi=Q^{-\frac 1 2}$ 
such that $\b q\circ \phi$ is the standard euclidean form
and that the $L^\infty$ interpolation error is left invariant
by this coordinate change.

\begin{figure}[htbp]
\centerline{
\includegraphics[width=8cm]{\pathPic/PaperCM/maxpoint.pdf}
}
\centerline{Figure 4: maximum point for the $L^\infty$ interpolation error}
\label{figerrorlinf}
\end{figure}

\noindent
We now prove the following result which clearly implies Theorem
\ref{longestedgelinf}.

\begin{prop} \label{ErLInf} Let T be a triangle with edges $|a|_\bq\geq |b|_\bq\geq |c|_\bq$.
We then have :
\begin{eqnarray*}
d_T(b,q)-d_T(a,q)&\geq & \frac 1 4 (\b q(a)-\b q(b)) \\
d_T(c,q)-d_T(a,q)&\geq & \frac 1 4 \left(\b q(a)-\left(\frac{|b|_\bq+|c|_\bq} 2\right)^2\right).
\end{eqnarray*}
\end{prop}

\begin{figure}[htbp]
\centerline{
\includegraphics[width=15cm,height=4cm]{\pathPic/PaperCM/cutabc.pdf}
}
\centerline{Figure 5: Notations in the proof of Proposition \iref{ErLInf}}
	\label{fig:cuts}
\end{figure}

\proof  
We introduce sub-triangles $T^i_e$, $i=1,2$ and $e=a,b,c$,
as defined in Figure 5, which correspond 
to the three refinement scenarios. With such definitions, the
following inequalities are easily derived from
Proposition \iref{PropAlgErLInf}
\begin{eqnarray*}
4\alpha_{T^2_a}(q) &=& \b q(b) \text{ (since } T^2_a \text{ is obtuse)}\\
4\alpha_{T^1_b}(q) &\geq& \b q(a)\\
4\alpha_{T^1_c}(q) &\geq& \b q(a)\\
4\alpha_{T^2_c}(q) &\geq& \b q(b)
\end{eqnarray*}
On the other hand, we shall prove 
\be
\alpha_{T^1_a}(q) \leq \alpha_{T^2_b}(q),
\label{estim1}
\ee
and
\be
4\alpha_{T^1_a}(q) \leq \left(\frac{|b|_\bq+|c|_\bq} 2\right)^2.
\label{estim2}
\ee
The proof of \iref{estim1} follows from elementary geometric observations.
Let $L$ be a line which is parallel to $c$ but does not contain it, and for $x\in L$
denote by $T_x$ the triangle of vertices $x$ and the end points of $c$.
Denoting respectively by $u(x)$ and $v(x)$ the diameter of $T_x$ 
and of its circumscribed circle for the $\bq$-metric, we remark that these functions 
decrease monotonously as $x$ tends to a point $x_c$ which is the orthogonal
projection (also for the $\bq$-metric) of the mid-point of $c$ onto $L$. Since
the function $x\mapsto \alpha_{T_x}(q)$ is continuous in $x$ and
equal to $u(x)$ or $v(x)$ at all $x$, we conclude that this
function also decreases monotonously as $x$ tends to $x_c$.
Applying this observation to the line that contains $m_a$ and $m_b$
the mid-points of $a$ and $b$, and remarking that
$m_a$ is closer to $x_c$ than $m_b$, we conclude that \iref{estim1} holds.

From \iref{estim1} and the first set of inequalities, we obtain
the first statement of the theorem since
$$
\begin{array}{ll}
d_T(b,q)-d_T(a,q)&=\alpha_{T^1_b}(q)+\alpha_{T^2_b}(q)-\alpha_{T^2_a}(q)-\alpha_{T^1_a}(q)\\
& \geq \alpha_{T^1_b}(q)-\alpha_{T^2_a}(q)
\geq  \frac 1 4(\b q(a)-\b q(b)).
\end{array}
$$

The proof of \iref{estim2} also follows from elementary geometric observations.
In the case where $T^1_a$ is obtuse, one of its edges $e$ is such
that $4\alpha_{T^1_a}=\b q(e)$, and \iref{estim2} follows since
$|e|_\bq\leq \frac 1 2 (|b|_\bq+|c|_\bq)$ for all $e$, using triangle inequality.
In the case where $T^1_a$ is acute, the center $w$ of its circumscribed
circle for the $\bq$-metric is inside $T^1_a$, and its diameter
is not larger than $\frac 1 2 (|b|_\bq+|c|_\bq)$ by convexity, as illustrated
on Figure 6 when $\bq$ is the euclidean metric.

From \iref{estim2} and the first set of inequalities, we obtain
the second statement of the theorem since
$$
\begin{array}{ll}
d_T(c,q)-d_T(a,q)&=\alpha_{T^2_c}(q)+\alpha_{T^1_c}(q)-\alpha_{T^2_a}(q)-\alpha_{T^1_a}(q) \\
&\geq \frac 1 4\left(\b q(b)+\b q(a)-\b q(b)-\left(\frac{|b|_\bq+|c|_\bq} 2\right)^2\right)\\
&=\frac 1 4 \left(\b q(a)-\left(\frac{|b|_\bq+|c|_\bq} 2\right)^2\right).
\end{array}
$$
\sq

\begin{figure}[htbp]
\centerline{
\includegraphics[width=4cm]{\pathPic/PaperCM/acutecase.pdf}
}
\centerline{Figure 6: The case where $T^1_a$ is acute.}
	\label{fig:bcD}
\end{figure}


\subsubsection{The $L^2$-based split}

We now denote by
$$
\beta_T(f) = \|f-P_Tf\|_{L^2(T)},
$$
the orthogonal projection error in the $L^2$ norm.
The decision function \iref{eqDecisionL2} now writes
\be
d_T(e,f) =\beta_{T_e^1}(f) ^2+ \beta_{T_e^2}(f)^2.
\label{optil2edge}
\ee
We shall prove that the refinement procedure
based on \iref{optil2edge} behaves in a similar way
as \iref{optilinfedge}.

\begin{theorem} \label{longestedgel2}
If $d,e\in \{a,b,c\}$ are two edges such that $|d|_\bq<|e|_\bq$, then
$d_T(e,q) <d_T(d,q)$. Therefore the refinement
procedure based on {\rm \iref{optil2edge}} selects 
the longest edge in the sense of $|\cdot|_\bq$.
\end{theorem}

In order to prove this result, we first provide with an algebraic expression
of $\beta_T(q)$ which is valid for any quadratic function $q$.

\begin{prop} \label{PropAlgEr}
Let $T$ be a triangle with edges $a,b,c$ and area $|T|$, 
and let $q$ be a quadratic function.
Then
\be
\beta_T^2(q) = |T| \left(c_1 (\b q(a)+\b q(b)+\b q(c))^2 - c_2 \det(\b q) |T|^2\right).
\label{localprojqerror}
\ee
with constants $c_1 = \frac 1{1200}$
and $c_2 = c_1  \frac {64} 3  = \frac {4}{225}$.
\end{prop}

\proof 
We first prove \iref{localprojqerror}
on the triangle $R$ of vertices $\{(0,0),(0,1),(1,0)\}$.
It is easy to compute the integrals on $R$
of monomials $x^ky^l$, $k+l\leq 4$.
Using these quantities, we can derive the orthogonal 
projection of a quadratic function thanks to a formal computing program,
which gives us
$$
\bq = ux^2+vy^2+2wxy \quad \Ra \quad P_R \bq = -\frac{u+v+w}{10} + \frac{2x} 5 (2u+w)+\frac{2y} 5 (2v+w).
$$
This yields the following expression
for the $L^2$-squared error between $q$ and its projection  
$$
\int_{R} (q-P_R q)^2 = 
\frac 1 {300} \left(u^2 + \frac{2 u v} 3 + v^2 - 2 u w - 2 v w + \frac{7 w^2} 3\right),
$$
which is equivalent to \iref{localprojqerror}.

For an arbitrary triangle $T$, using an affine bijective transformation
$\phi$ from $R$ to $T$, we have
$$
\beta_T(q)^2=J_\phi \beta_R(\ti q)^2,
$$
where $\ti q=q\circ \phi$ and $J_\phi$ is the constant jacobian of $\phi$. 
Using the validity of \iref{localprojqerror} on $R$
and the fact that $|T|=J_\phi |R|$, we thus obtain 
$$
\beta_T(q)^2=|T| \left(c_1 (\b {\ti q}(\ti a)+\b {\ti q}(\ti b)+\b {\ti q}(\ti c))^2 - c_2 \det(\b {\ti q}) |R|^2\right),
$$
where $\b {\ti q}$ is the quadratic form associated to $\ti q$ and 
$\ti e$ denotes the edge segment of $R$ mapped onto $e$ by $\phi$.
Since $\b {\ti q}(\ti e)=\b q(e)$ and $\det(\b {\ti q})=J_\phi^2\det(\b q)$,
we obtain \iref{localprojqerror} for $T$.
\sq
\nl
We now prove the following result which clearly implies Theorem
\ref{longestedgel2}.

\begin{corollary} \label{PropErrorChildren} Let $T$ be a triangle with edges $a,b,c$ and area $|T|$, 
with $|a|_\bq\geq |b|_\bq$
and $|a|_\bq\geq  |c|_\bq$. Then,
\begin{eqnarray}
\label{eqDecisionL2PosAB}
	d_T(b,q)-d_T(a,q) &\geq & \frac 5 4 c_1 |T| (\b q(a)^2-\b q(b)^2)\\
\label{eqDecisionL2PosAC}
	d_T(c,q)-d_T(a,q) &\geq & \frac 5 4 c_1 |T| (\b q(a)^2-\b q(c)^2)\\
\end{eqnarray}
\end{corollary}

\proof
The children triangles all have area $|T|/2$, and 
take their edges among $a,b,c$, 
$a/2,b/2,c/2$ and $\frac{a-b} 2,\frac{b-c} 2,\frac{c-a} 2$ (recall that $a+b+c=0$).
%on which the quadratic form $\b q$ can be expressed only in
%terms of $\b q(a),\b q(b), \b q(c)$. In particular, for the last group 
%$\frac{a-b} 2,\frac{b-c} 2,\frac{c-a} 2$, 
We use the identity
$$
\b q(u+v)+\b q(u-v) = 2\b q(u)+2\b q(v),
$$
which is valid for all quadratic forms, and implies
$$
\bq\left(\frac{b-c} 2\right) = \frac{\bq(b)+\bq(c)} 2-\frac{\bq(a)} 4.
$$
Using \iref{localprojqerror}, this allows us to compute the local projection 
errors for the children of $T$.
For example bisecting the edge $a$ creates two children $T'$ 
and $T''$ with edges $\frac a 2,b,\frac{c-b} 2$ and $\frac a 2,c,\frac{b-c} 2$, and therefore
\begin{eqnarray*}
\beta_{T'}^2(q) &=& |T'| \left(c_1 \left(\b q\left(\frac a 2\right)+\b q(b)+\b q\left(\frac{c-b} 2\right)\right)^2 - c_2 \det(\b q) |T'|^2\right)\\
&=& \frac{|T|} 2 \left(c_1 \left(\frac{3 \b q(b)+\b q(c)} 2\right)^2 - c_2 \det(\b q) \frac{|T|^2} 4\right)
\end{eqnarray*}
and similarly 
$$
\beta_{T''}^2(q) = \frac{|T|} 2 \left(c_1 \left(\frac{3 \b q(c)+\b q(b)} 2\right)^2 - c_2 \det(\b q) \frac{|T|^2} 4\right).
$$
Adding up, we thus obtain
\be
d_T(a,q) =\frac{|T|} 8 \left(c_1 (3 \b q(b)+\b q(c))^2 + c_1 (\b q(b)+3 \b q(c))^2 - 2 c_2 \det(\b q) |T|^2 \right).
\label{dtaq}
\ee
Subtracting this from the analogous expression for $d_T(b,q)$
we obtain 
$$
d_T(b,q) - d_T(a,q) = \frac{c_1 |T|} 4 \left(5 \left(\bq(a)^2 - \bq(c)^2\right) + 6 \bq(c) (\bq(a)-\bq(b)\right)
$$
which implies \iref{eqDecisionL2PosAB}.
Exchanging $b$ with $c$ we obtain \iref{eqDecisionL2PosAC} which concludes the proof.
% and $d_T(c,q)$, 
%we obtain the announced inequalities. 
\sq

\subsubsection{Convergence towards to optimal aspect ratio}
\label{subsecRatioConvex}

We have established is Theorems \ref{longestedgelinf} and \ref{longestedgel2} that for any triangle $T$ and any quadratic function $q\in \P_2$ such that the homogeneous component $\bq\in \H_2$ is positive definite, the decision functions \iref{eqDecisionL2} and \iref{eqDecisionLInf} based on the $L^2$ or $L^\infty$ error lead to the bisection of the same edge of $T$ : the longest edge of the $\bq$-metric.

Similarly it is established in Lemma \ref{lemmaLongestEdgeL1} in the previous chapter that the decision function \iref{eqDecisionL1} based on the $L^1$ interpolation error leads to the bisection of the same edge. As a result, the decision functions can be exchanged without affecting the greedy algorithm %when the function $f$ to be approximated is quadratic, 
and Corollary \ref{corolQuadApprox} can be extended.

\begin{theorem}
\label{thOptiL2LInf}
Let $\Omega$ be a triangle, and let $q$ be a quadratic function with positive definite associated quadratic form $\bq$. 
Let $q_N$ be the approximant of $q$ on $\Omega$ obtained by the greedy algorithm 
for the $L^p$ metric, using the $L^1$, $L^2$ or $L^\infty$ decision function  \iref{eqDecisionL1},  \iref{eqDecisionL2}, \iref{eqDecisionLInf}.
Then 
\be
%\label{eqOptiEstimQ}
\limsup_{N\to \infty} N \|q-q_N\|_{L^p(\Omega)}  \leq C \|\sqrt{\det(\bq)}\|_{L^\tau(\Omega)},
\ee
where $\frac 1 \tau=\frac 1 p +1$ and where the constant $C$ depends only on 
on the choice of the approximation operator $\cA_T$ used in the definition of the approximant.  
\end{theorem}

The local perturbation analysis exposed in the previous chapter \S \ref{section:OptQuad} for the $L^1$ based decision function extends without difficulties to the $L^2$ and $L^\infty$ based decision functions. 
From this point, it is not difficult to extend Theorem \ref{thOptiL2LInf} %Therefore the asymptotically optimal error estimate \iref{eqOptiConv} can be extended 
to functions $f$ which are close enough to a positive definite quadratic function $q$, in the sense that 
\be
\label{eqFApproxQuad}
d^2 q \leq d^2 f\leq (1+\mu) d^2 q
\ee
for a constant $\mu>0$ small enough.

Let us consider a $C^2$ and strictly convex function $f$ defined on a polygonal domain $\Omega$. In order to establish an asymptotical error estimate, %to obtain the asymptotically optimal error estimate \iref{eqOptiConv}
%\be
%\label{eqGlobalGreedy}
%\limsup_{N\to \infty} N \|f-f_N\|_{L^p(\Omega)}  \leq C \|\sqrt{\det(d^2f)}\|_{L^\tau(\Omega)},
%\ee
we need to be ensured that after sufficiently many steps of the greedy algorithm, 
the target function $f$ can be well approximated by a quadratic function $q=q_T$ 
on each triangle $T$, in the sense of \iref{eqFApproxQuad}, so that our local results will apply on such triangles.
This property follows from the next proposition, which is an extension of Proposition \ref{PropDiamZero} in which the $L^1$ based decision function \iref{eqDecisionL1} is replaced with the $L^\infty$ based decision function.
We postpone its proof to the appendix \S\ref{secPropDiamZero}.

\begin{prop} \label{propDiamZeroLInf}
Let $f$ be a $C^2$ function such that 
$d^2 f(x)\geq m I $ 
for some arbitrary but fixed $m >0$ independent of $x$. 
Let $\cT_N$ be the triangulation generated by the greedy algorithm
applied to $f$ using the $L^\infty$ decision function given by \iref{eqDecisionLInf}.
Then
$$
\lim_{N\to +\infty} \max_{T\in\cT_N}\diam(T)=0,
$$
i.e. the diameter of all triangles tends to $0$. As a result the optimal estimate \ref{eqOptiConv} holds for $f$.
\end{prop}

As a result, theorem \ref{optitheo} extends to the $L^\infty$ based decision function.
%Using a reasoning completely similar to the one presented
\begin{theorem}
\label{optitheoLInf}
Let $\Omega$ be a polygonal domain and let $f\in C^2(\Omega)$ be such that 
$
d^2f(x)\geq m I
$ 
for all $x\in \Omega$,
for some arbitrary but fixed $m >0$ independent of $x$. Let $f_N$
be the approximant obtained by the greedy algorithm 
for the $L^p$ metric, using the $L^1$ decision function \iref{eqDecisionL1} or the $L^\infty$ decision function \iref{eqDecisionLInf} (but not the $L^2$ decision function \iref{eqDecisionL2}).
Then 
$$
\limsup_{N\to \infty} N \|f-f_N\|_{L^p}  \leq C \|\sqrt{\det(d^2f)}\|_{L^\tau},
$$
where $\frac 1 \tau=\frac 1 p +1$ and where $C$
is an absolute constant (i.e. independent of $p$, $f$ and $\alpha$).  
\end{theorem}


%Unfortunately, we were not able to extend the proof of this result to the $L^2$ based decision function. 

\subsection{Quadratic functions of mixed sign}
\label{secNegQuad}

In this section, we study the algorithm 
when applied to a quadratic polynomial $q$ such that $\det(\b q)<0$. 
We shall follow the same steps, and reach similar conclusions, as in the positive definite case, using
a measure of non-degeneracy which is equivalent to $\rho_{\bq}(T)$.
If a triangle $T$ has edges $a,b,c$ such that $|\bq(a)|\geq |\bq(b)|\geq |\bq(c)|$, we will still refer to $a$ as the ``longest'' edge in the sense of $\bq$, although $\bq$ does not define a proper metric anymore.

The following inequalities that will be repeatedly used in this section can be derived when $\rho_\bq(T)$ is large enough. We postpone their proof to the appendix.
\begin{prop}
\label{rho48}
Let $T$ be a triangle such that $|\bq(a)|\geq |\bq(b)|\geq |\bq(c)|$, and define
$d= \frac{b-c} 2$.
\be 
\label{rho4}
\text{If }\rho_\bq(T) \geq 4, \text{ then } \bq(a)\bq(b)\geq 0, \ |\bq(a)|\geq 4 |\bq(c)| \text{ and } |\bq(a)|\geq 4 |\bq(d)|.
\ee
\be
\label{rho8}
\text{If }\rho_\bq(T) \geq 8, \text{ then } |\bq(a)|\leq \frac 3 8 |\bq(b)+\bq(c)|.
\ee
\end{prop}

\subsubsection{The $L^\infty$-based split}

\begin{theorem} %\label{longestedgelinf}
\label{thLInfSplitNeg}
If $|\bq(a)|> \max\{|\bq(b)|,|\bq(c)|\}$ and $\rho_\bq(T)\geq 4$,
then $d_T(a,q) <\min\{d_T(b,q),d_T(c,q)\}$. Therefore the refinement
procedure based on {\rm \iref{optilinfedge}} selects the longest edge in the sense of $\bq$.
\end{theorem}

This theorem is very similar to the one for positive quadratic functions. In order to prove it, we first study the interpolation error which has a simple form in this context.

\begin{prop}
Let $T$ be a triangle with edges $a,b,c$. Then
$$
\alpha_T(q) = \frac 1 4 \max\{|\bq(a)|,|\bq(b)|,|\bq(c)|\}.
$$
\end{prop}

\proof
Let $x_0$ be the point of $T$ at which the interpolation error is attained: $x_0 = \argmax_T |q-I_Tq|$. If $x_0$ is in the interior of $T$, then it must be a local extremum of $q-I_Tq$. However this function has only one critical point on $\R^2$, which is not an extremum since $\bq$ has mixed signature. Therefore $x_0$ must lie on an edge.
On each edge of $T$, the function $q-I_Tq$ is a one dimensional quadratic function vanishing at the endpoints. It follows that $x_0$ must lie in the middle of an edge
and the result follows.
\sq

\begin{prop}
Let $T$ be a triangle with edges $|\bq(a)|\geq |\bq(b)| \geq |\bq(c)|$ and verifying $\rho_\bq(T)\geq 4$. Then
\begin{eqnarray*}
d_T(b,q)-d_T(a,q) &\geq& \frac{|\bq(a)|-|\bq(b)|} 8\\
d_T(c,q)-d_T(a,q) &\geq& \frac{|\bq(a)|} 8
\end{eqnarray*}
\end{prop}

\proof
The bisection through the edge $a$ creates two sub-triangles $T^1_a,T^2_a$ of edges respectively $\frac a 2, b,d$ and $\frac a 2, c, d$. Using the last two inequalities in \iref{rho4} we obtain that $4 \alpha_{T^1_a} = \max\{|\bq(a/2)|,|\bq(b)|\}$ and $4 \alpha_{T^2_a} = |\bq(a/2)|$.
Therefore 
%$$%and the preceding proposition
%4 d_T(a,q) =|\bq(a/2)|+\max\{|\bq(a/2)|,|\bq(b)|\}.
%$$
$$
4 d_T(a,q) =\frac{|\bq(a)|} 4 +\max\left\{\frac{|\bq(a)|} 4,|\bq(b)|\right\}.
$$
On the other hand, the choice of bisecting the edge $b$ creates two subtriangles respectively containing  the edges $a$ and $\frac b 2$, and 
the choice of bisecting the edge $c$ creates two subtriangles respectively containing  the edges $a$ and $b$. This provides us with the lower bounds
\begin{eqnarray*}
4 d_T(b,q) &\geq & |\bq(a)|+\frac{|\bq(b)|} 4,\\
4 d_T(c,q) &\geq & |\bq(a)|+|\bq(b)|.
\end{eqnarray*}
The proposition follows easily, distinguishing between the two cases $|\bq(a)|\leq 4 |\bq(b)|$
and $|\bq(a)|\geq 4 |\bq(b)|$.
\sq

\subsubsection{The $L^2$-based split}

The same conclusions can be reached for the refinement procedure based on \iref{optil2edge}.

\begin{theorem} %\label{longestedgelinf}
\label{thL2SplitNeg}
If $|\bq(a)|> \max\{|\bq(b)|,|\bq(c)|\}$ and $\rho_\bq(T)\geq 4$,
then $d_T(a,q) <\min\{d_T(b,q),d_T(c,q)\}$. Therefore the refinement
procedure based on {\rm \iref{optil2edge}} selects the longest edge in the sense of $\bq$.
\end{theorem}

\proof
The expression found in \iref{dtaq} remains valid when $\det(\bq)<0$.
Substituting $a$ by $b$ or $c$ and subtracting, we obtain
\begin{eqnarray*}
d_T(b,q)-d_T(a,q) &=& \frac{5 c_1} 2 |T| (\bq(a)-\bq(b))\left(s+\frac{\bq(b)} 5\right),\\ %valeur de C?
d_T(c,q)-d_T(a,q) &=& \frac{5 c_1} 2 |T| (\bq(a)-\bq(c))\left(s+\frac{\bq(c)} 5\right),
\end{eqnarray*}
where $s=\bq(a)+\bq(b)+\bq(c)$.
Using \iref{rho4}, we see that the quantities 
$$
s+\frac{\bq(b)} 5, \quad s+\frac{\bq(c)} 5, \quad \bq(a)-\bq(b) \stext{ and } \bq(a)-\bq(c)
$$
all have the same sign as $\bq(a)$
and are non-zero. It follows that $d_T(a,q) <\min\{d_T(b,q),d_T(c,q)\}$.
\sq
%Let us rename the edges in such way that $|\bq(a)|\geq |\bq(b)|\geq |\bq(c)|$.

\subsubsection{Convergence toward the optimal aspect ratio.}


We have proved that the refinement procedure - either based on the
$L^\infty$ or $L^2$ decision function - systematically picks the longest
edge in the sense of $\bq$. Similarly to the positive definite
case, we now study the iteration of several refinement steps and
show that the generated triangles tend to adopt an optimal ``aspect ratio''
in the sense of the measure of non-degeneracy $\rho_{\bq}(T)$
introduced in \S 2.

As in \S 3.3, we introduce a close variant to 
$\rho_{\bq}(T)$. If $T$ is a triangle with edges $a,b,c$, we define
\be
\sigma_\bq(T) := \frac{\min\left\{|\b q(a)+\b q(b)|,\, |\b q(b)+\b q(c)|,\, |\b q(c)+\b q(a)|\right\}}{4|T|\sqrt{|\det \b q|}}.
\ee
Note that if $\bq$ was a positive quadratic form, this definition is
consistent with \iref{sigmaq}. We define our measure of non-degeneracy $\kappa_\bq$ by
\be
\kappa_\bq(T) := \max\{\sigma_\bq(T), 5/ 2\}.
\ee
We first show that the quantities $\kappa_\bq$ and $\rho_\bq$ are equivalent.
\begin{prop}
\label{rhosigma}
For any triangle $T$, one has
\be
2\sigma_\bq(T) \leq \rho_\bq(T),
\label{sigmarho}
\ee
and
\be
\frac 4 5\kappa_\bq(T) \leq \rho_\bq(T) \leq \frac{32} 3 \kappa_\bq(T).
\label{rhokappa}
\ee
\end{prop} 

\proof
We denote by $a,b,c$ the edges of $T$, and we assume that $|\bq(a)|\geq |\bq(b)| \geq |\bq(c)|$.
The inequality \iref{sigmarho} follows directly from the triangle inequality:
$$
2 |T| \sqrt{|\det \bq|} \sigma_\bq(T) \leq \frac{|\bq(b)+\bq(c)|} 2 \leq |\bq(a)| \leq |T| \sqrt{|\det \bq|} \rho_\bq(T).
$$
As mentioned earlier, $\rho_\bq(T)$ is always larger than $2$
and therefore \iref{sigmarho} implies the left inequality in \iref{rhokappa}.

It remains to prove the right inequality in \iref{rhokappa}.
If $\rho_\bq(T)\leq 8$, it is immediate
since $\sigma_\bq(T)\geq \frac 5 2$ and $\frac{32} 3 \frac 5 2 \geq 8$.
If $\rho_\bq(T)\geq 8$ then $\bq(a)\bq(b)\geq 0$ according to \iref{rho4} and therefore 
$$
|\bq(b)+\bq(c)|\leq |\bq(a)+\bq(c)|\leq |\bq(a)+\bq(b)|.
$$
%and from \iref{rho8} that $|\bq(a)|\leq \frac 8 3|\bq(b)+\bq(c)|$.
We obtain using \iref{rho8} that %It follows that 
$$
\rho_\bq(T)=\frac{|\bq(a)|}{|T| \sqrt{|\det \bq|}} \leq \frac 8 3 \frac{|\bq(b)+\bq(c)|}{|T| \sqrt{|\det \bq|}}
= \frac{32} 3 \sigma_\bq(T)\leq \frac{32} 3 \kappa_\bq(T),
$$
which concludes the proof.
\sq

Similar to $\rho_\bq$, the quantity $\kappa_\bq$ is invariant by a linear coordinate changes $\phi$,
in the sense that
$$
\kappa_{\bq\circ \phi}(T) = \kappa_\bq (\phi(T)).
$$
Our next result shows that $\kappa_\bq(T)$ is always reduced by 
the refinement procedure.

\begin{prop} 
\label{PropSigmaDecmixed}
If $T$ is a triangle with children $T_1$ and $T_2$ obtained by the
refinement procedure for the quadratic function $q$, using the $L^2$ based or $L^\infty$ based decision function, then
$$
\max\{\kappa_\bq(T_1), \kappa_\bq(T_2)\}\leq \kappa_\bq(T).
$$
\end{prop}

\proof
Let us assume that $a$ is the longest edge in the sense of $\bq$.
In the case where $\rho_\bq(T)\geq 4$, we already noticed
in the proof of Proposition \ref{rhosigma} 
that 
$$
\sigma_\bq(T) = \frac{|\b q(b)+\b q(c)|}{4|T|\sqrt{|\det \b q|}}.
$$
Moreover, according Theorems \ref{thLInfSplitNeg} and \ref{thL2SplitNeg} %to the results established in \S 4.1 and 4.2, 
the edge $a$ is selected by both decision functions.
It follows that the children $T_i$ have edges $a/2,b,(c-b)/2$ and $a/2, (b-c)/2,c$ 
(recall that $a+b+c=0$). We thus have
\begin{eqnarray*}
	2 |T| \sqrt{|\det \bq|}\ \sigma_\bq(T_i) & \leq & \left|\bq\left(\frac a 2 \right)+\bq\left(\frac{b-c}{2}\right)\right|\\
	& = & \left|\bq\left(\frac{b+c}{2}\right)+\bq\left(\frac{b-c}{2}\right)\right|\\
	& = & \frac{|\b q(b)+\b q(c)|}{2}\\
	& = & 2 |T|  \sqrt{|\det \b q|}\ \sigma_\bq(T).
\end{eqnarray*}
We have proved that $\sigma_\bq(T_i)\leq \sigma_\bq(T)$, and it readily follows that $\kappa_\bq(T_i)\leq \kappa_\bq(T)$.

In the case where $\rho_\bq(T)\leq 4$, we remark that $T_i$
contains at least one edge from $T$, say $s\in\{a,b,c\}$ 
and one half-edge $t\in \{\frac a 2,\frac b 2,\frac c 2\}$.
This provides an upper bound for $\sigma_\bq$ : 
\be
\label{rho4sigma}
\sigma_\bq(T_i) \leq \frac{|\bq(s)+ \bq(t)|}{2 |T| \sqrt{|\det \bq|}} \leq \frac{|\bq(a)|+ |\bq(\frac a 2)|}{2 |T| \sqrt{|\det \b q|}} = \frac 5 8 \rho_\bq(T) \leq \frac 5 2.
\ee
Therefore $\kappa_\bq(T_i) = \frac 5 2 \leq \kappa_\bq(T)$.
\sq

Our next objective is to show that as we iterate the refinement process,
the value of $\kappa_\bq(T)$ 
becomes bounded independently of $q$
for almost all generated triangles.
If $T$ is a triangle such that 
$|\bq(a)|\geq |\bq(b)|\geq |\bq(c)|$ and 
if the edge $a$ is cut (which is the case as soon as $\rho_\bq(T)\geq 4$, using the $L^2$ or $L^\infty$ based decision functions) 
we define $\psi_\bq(T)$ as the subtriangle containing the edge $c$.
We first prove a result which is analogous to Proposition \ref{PropFSigmaDec}.

\begin{prop} 
\label{PropFSigmaDecmixed} 
If $T$ is a triangle such that $\kappa_\bq(\psi_\bq^3(T))>\frac 5 2$, then 
$\kappa_\bq(\psi_\bq^3(T))\leq \frac 2 3 \kappa_\bq(T)$.
\end{prop}

\proof
Let $S$ be a triangle such that $\kappa_\bq(\psi_\bq(S))>\frac 5 2$. According to \iref{rho4sigma}, one must have $\rho_\bq(S)> 4$.
We assume that the edges of $S$ satisfy $|\bq(a)|\geq|\bq(b)|\geq|\bq(c)|$.
Since the three edges of $\psi_\bq(S)$ are $\frac a 2$, $c$ and $d=\frac{b-c} 2$, it follows 
from \iref{rho4} that the longest edge of $\psi_\bq(S)$ in the sense of 
$\bq$ is $\frac a 2$.

Since 
$$
\kappa_\bq(\psi_\bq(T)) \geq \kappa_\bq(\psi_\bq^2(T))\geq \kappa_\bq(\psi_\bq^3(T))>\frac 5 2,
$$
we can apply this observation to the triangles $T$, $\psi_\bq(T)$ and $\psi_\bq^2(T)$.
Therefore, denoting
by $a$ the longest edge of $T$ in the sense of $\bq$, 
we find that $\frac a 8$ is the longest edge of $\psi_\bq^3(T)$.
Since $|\psi_\bq^3(T)| = |T|/8$, we obtain that $\rho_\bq(\psi_\bq^3(T)) = \rho_\bq(T)/8$.
Using the results of Proposition \ref{rhosigma}, we thus have
$$
\kappa_\bq(\psi_\bq^3(T)) = \sigma_\bq(\psi_\bq^3(T))\leq \frac 1 2 \rho_\bq(\psi_\bq^3(T)) = \frac 1 {16} \rho_\bq(T) \leq \frac 2 3 \kappa_\bq(T),
$$
which concludes the proof.
\sq

An immediate consequence of Propositions \ref{PropSigmaDecmixed} and \ref{PropFSigmaDecmixed} is the following.

\begin{corollary} 
If $(T_i)_{i=1}^{8}$ are the 8 children obtained from 3 successive refinement procedures 
from $T$ for the function $q$, then
\begin{itemize}
	\item $\text{for all } i, \kappa_\bq(T_i)\leq \kappa_\bq(T)$
	\item $\text{there exists } i \text{ such that }, \kappa_\bq(T_i)\leq \frac{2}{3}\kappa_\bq(T)$ or $\kappa_\bq(T_i)=\frac 5 2$.\\
\end{itemize}
\end{corollary}

\noindent
We eventually obtain
the two following results which proof are exactly similar to
the ones of Theorem \ref{CorolStabilise} and Corollary \ref{corolQuadApprox}.

\begin{theorem}
Let $T$ be a triangle, and let $\bq$ a 
quadratic function of mixed type. Let  $k = \frac{\ln (2\kappa_\bq(T)/5)}{\ln3-\ln 2}$.
Then after $n$ applications of the refinement procedure starting from $T$,
at most $C n^k 7^{n/3}$ of the $2^n$ generated triangles are such
that $\kappa_\bq(S)>\frac 5 2$ where $C$ is an absolute constant. Therefore the proportion 
of such triangles tends exponentially to $0$ as $n\to +\infty$.\\
\end{theorem}


\begin{theorem}
\label{thOptiL2LInfNeg}
Let $\Omega$ be a triangle, and let $q$ be a quadratic function such that $\det \bq<0$.
Let $q_N$ be the approximant of $q$ on $\Omega$ obtained by the greedy algorithm 
for the $L^p$ metric, using the $L^2$ or $L^\infty$ decision function \iref{eqDecisionL2}, \iref{eqDecisionLInf}.
Then 
$$
\limsup_{N\to \infty} N \|q-q_N\|_{L^p(\Omega)}  \leq C \|\sqrt{\det(\bq)}\|_{L^\tau(\Omega)},
$$
where $\frac 1 \tau=\frac 1 p +1$ and where the constant $C$ depends only on 
on the choice of the approximation operator $\cA_T$ used in the definition of the approximant.  
\end{theorem}

\section{Alternative bisection choices, and the approximation of cartoon functions}
\label{secAltBi}

%\section{Cartoon functions} 

A popular, although simplistic, model for images is the set of cartoon functions, see Definition \ref{defcartoon}. 
In summary a function $f$ defined on a domain $\Omega$ is a cartoon function if it is piecewise $C^2$ on a partition of $\Omega$ into sub-domains $\Omega_i$ which have a piecewise $C^2$ boundary.
For any cartoon function $f$ on a bi-dimensional bounded domain $\Omega \subset \R^2$, the approximations  $(f_N)_{N\geq 0}$ obtained by retaining the $N$ largest coefficients in the wavelet expansion of $f$ satisfy, as observed in % [part II] 
\iref{wavN},
\be
\label{eqWav}
\|f-f_N\|_{L^2(\Omega)}\leq C N^{-\frac 1 2}. %\TV(f) 
\ee
One of the purposes of mesh adaptation is to improve on this estimate.
We therefore focus in this section on the $L^2$ approximation error.
For any triangle $T$ and any function $f\in L^2(T)$, we define 
\be
\label{defErrTL2}
e_T(f) := \inf_{\pi \in \sP_1} \|f-\pi\|_{L^2(T)} = \|f-P_T(f)\|_{L^2(T)},
\ee
where $P_T$ is the operator of $L^2(T)$ orthogonal projection onto the space $\P_1$ of affine functions.
For any triangulation $\cT$ of a polygonal domain $\Omega$, and any $f\in L^2(\Omega)$, we denote by $e_\cT(f)$ the error of approximation of $f$ in the $L^2(\Omega)$ norm by discontinuous piecewise affine functions on $\cT$. This quantity is defined by 
\be
\label{defErrCTL2}
e_\cT(f)^2 := \sum_{T\in \cT} e_T(f)^2 = \|f- P_\cT(f)\|_{L^2(\Omega)}^2,
\ee
where $P_\cT$ is the $L^2(\Omega)$ orthogonal projection onto the space of discontinuous piecewise affine functions on the triangulation $\cT$.
The heuristic analysis led in \iref{heurist} suggests that, if $f$ is a cartoon function on a polygonal domain $\Omega$, then  there exists a sequence $(\cT_N)_{N\geq N_0}$ of anisotropic triangulations of $\Omega$, satisfying $\#(\cT_N)\leq N$, and such that 
\be
\label{estimC}
e_{\cT_N}(f)\leq C N^{-1}. 
\ee

\begin{figure}
\centering
\includegraphics[width=3.5cm,height=3.5cm]{\pathPic/Subdivision/Bisec.pdf}
\hspace{1cm}
\includegraphics[width=3.5cm,height=3.5cm]{\pathPic/Subdivision/TriSec.pdf}
\caption{(left) Three bisection choices $S_T^3$, (right) Six bisection choices $S_T^6$.\label{figTriSec}}
\end{figure}

We make in this section an attempt, not totally conclusive, to answer the following question : is it possible to produce a sequence $(\cT_N)_{N \geq N_0}$ of triangulations satisfying the \iref{estimC} using a hierarchical refinement algorithm?
The analysis presented in \S\ref{secNegRes} shows that unfortunately the refinement algorithm studied in the previous chapters does \emph{not} satisfy \iref{estimC}. However, there is some hope that modifications of this algorithm  may achieve it, perhaps using the ideas presented in \S \ref{secTriSec} and \S \ref{secConvexCut}.

We briefly recall the definition of the greedy algorithm studied in this part of the thesis, slightly modified in this chapter in order to focus on the $L^2$ norm and to allow for more diverse possibilities of refinement.
Given a triangulation $\cT$ of a domain $\Omega$ and a function $f\in L^2(\Omega)$, the greedy algorithm creates in one step a triangulation $\cT'$ of $\Omega$, of cardinality $\#(\cT') = \#(\cT)+1$, proceeding as follows : %. One step of the refinement procedure%, the refinement procedure
\begin{enumerate}
\item A triangle $T\in \cT$ which maximizes the approximation error is selected.
$$
T = \underset {T'\in \cT} \argmax \ e_{T'}(f).
$$
\item The refinement procedure considers a finite set $S_T$ of segments $s$ along which the triangle $T$ may be split into two, thus creating two children $T_s^1$ and $T_s^2$. The segment $s\in S_T$ which minimizes a given decision function $d_T(s,f)$ is selected and we define 
$$
\cT' := \cT - \{T\} + \{T_s^1, T_s^1\}.
$$
\end{enumerate}
Please note that the set $S_T$ is defined in advance and independent of the function $f$ to be approximated, only the choice of $s\in S_T$ depends on $f$.
Two possible choices for the set $S_T$, denoted by $S_T^3$ and $S_T^6$,
are illustrated on Figure \ref{figTriSec}. 
The set $S_T^3$ contains three segments, which join one of the three vertices of $T$ to the midpoint of the opposite edge. It corresponds to the three bisection choices studied in the previous chapters.
The set $S_T^6$ contains a larger choice, namely six segments joining
 a vertex $v_1$ of $T$ to the barycenter $\frac 1 3 v_2+ \frac 2 3 v_3$ of the other vertices $v_2$ and $v_3$.

The choice of the decision function $d_T(s,f)$ is crucial since it guides the bisection process and the creation of anisotropy. 
We often consider the following decision function : if a triangle $T$ can be bisected along a segment $s$, creating two smaller triangles $T_s^1$ and $T_s^2$, then 
\be
\label{eqDecisionL2Bi}
d_T(s,f) := e_{T_s^1}(f)^2+e_{T_s^2}(f)^2.
\ee

Starting from a triangulation $\cT_{N_0}$ of the polygonal domain $\Omega$ on which the function $f$ needs to be approximated, with $\#(\cT_{N_0}) = N_0$, the greedy algorithm creates step after step a sequence $\cT_{N_0+1}, \, \cT_{N_0+2}, \, \cdots$ of triangulations of $\Omega$ satisfying $\#(\cT_N) = N$.
At the time of writing, unfortunately, the author does not know how to choose the set of segments $S_T$ and the decision function $d_T(s,f)$ such that given any cartoon function $f$, the sequence $(\cT_N)_{N\geq N_0}$ of triangulations produced by the greedy algorithm satisfies the desired estimate \iref{estimC}.
As an intermediate objective, we choose to study the behavior of the refinement procedure when $f$ is a particularly simple cartoon function, the characteristic function $f=\chi_P$ of the half plane $P\subset \R^2$ defined by 
$$
P := \{(x,y)\in \R^2 \sep y\geq 0\}.
$$
We denote by $D$ the line 
\be
\label{defD}
D = \partial P = \{(x,0) \sep x\in \R\},
\ee
and we observe that, denoting by $\mathring T$ the interior of a triangle $T$, one has % and we observe that 
\be
\label{eqErrorZero}
e_T(\chi_P) = 0 \quad \stext{ if and only if } \quad \mathring T \cap D = \emptyset.
\ee


We establish in \S \ref{secNegRes}, Proposition \ref{propNegResult}, a negative result : the refinement procedure previously studied, using the three bisection choices illustrated on the left of Figure \ref{figTriSec} may produce a sequence of triangulations $(\cT_N)_{N\geq 1}$ that \emph{does not} satisfy 
\be
\label{eqEstimChi}
e_{\cT_N}(\chi_P) \leq CN^{-1}.
\ee
We then prove in \S \ref{secTriSec} that if the six bisection choices $S_T^6$ illustrated on Figure \iref{figTriSec} are allowed, and if an appropriate decision function is used, then \iref{eqEstimChi} is satisfied. Eventually, we consider in \S \ref{secConvexCut} yet another modification of the refinement procedure, which only involves three bisection choices at each step, and for which \iref{eqEstimChi} is again satisfied.
%Unfortunately, the author cannot prove that these modifications of the algorithm still satisfy the results established in the previous chapters for convex or quadratic functions.

\begin{remark}[Constrained triangulations] 

Let us mention that the estimate \iref{estimC} can also be achieved with a different mesh adaptation method, 
%named constrained triangulations, 
which does not use anisotropic triangles.

In that approach the first step is to identify precisely the collection $E$ of curves where the cartoon function $f$ to be approximated is discontinuous. These curves are then discretized and a collection $\cE$ of piecewise linear approximations of the curves in $E$ is built. The second step is to build a triangulation $\cT$ of the domain $\Omega$ of definition of $f$ which is ``constrained'' to contain the collection $\cE$ of piecewise linear curves in its edge set.

This method is out of the scope of this thesis, and seems to be incompatible with hierachical mesh refinement. We refer the interested reader to \cite{Shew3}.
\end{remark}

\subsection{Three bisection choices : A negative result}
\label{secNegRes}

%As a result, the anisotropic triangulations created by the refinement 
%These results show that the piecewise This is a negative result since the desired estimate \iref{eqEstimChi} is \emph{not} achieved. 

We show in this section that the greedy algorithm studied in the previous chapters beats the error estimate \iref{eqWav} associated to wavelet expansions when $f=\chi_P$. However it fails to achieve the desired error estimate \iref{eqEstimChi}.
More precisely, Proposition \ref{propSpeedBi} shows that, if the decision function $d_T(s,f)$ satisfies Assumptions \ref{assumBi},
then the greedy refinement procedure for the function $f=\chi_P$, starting from 
an arbitrary triangulation $\cT_{N_0}$, $\#(\cT_{N_0}) = N_0$,
produces a sequence $(\cT_N)_{N\geq N_0}$ of triangulations, $\#(\cT_N) = N$, such that 
\be
\label{eqUpperBi}
e_{\cT_N}(\chi_P) \leq C N^{-\lambda/2},
\ee
where $\lambda/2 = 0.732\cdots$. 
This estimate cannot be improved since we establish in Proposition \ref{propNegResult} that there exists a triangle $\TRef$ such that the sequence $(\cT_N)_{N\geq 1}$ produced by the greedy refinement procedure for the function $f=\chi_P$ starting from $\cT_1 = \{\TRef\}$  satisfies 
\be
\label{eqBelowBi}
e_{\cT_N}(\chi_P) \geq c N^{-\lambda/2}
\ee
where $c>0$.

We say that two triangles $T$, $T'$ are $D$-affine equivalent
% with respect to the line $D$ 
if there exists an affine change of coordinates $\phi : \R^2\to \R^2$, that transforms $T$ into $T'$ and leaves the line $D$ defined at \iref{defD} invariant :  
$$
\phi(T) = T' \stext{ and } \phi(D) = D.
$$
%For any triangle $T$ there exists $-1\leq a \leq b$ such that $T$ is equivalent to the triangle of vertices
%$$
%(0,-1), (1,a), (0,b).
%$$
If $T$ and $T'$ are $D$-affine equivalent, then it follows from a change of variables that 
\be
\label{eqErrorAffEq}
|T|^{-\frac 1 2} e_T(\chi_P) = |T'|^{-\frac 1 2}e_{T'}(\chi_P).
\ee

\begin{figure}
\centering
\includegraphics[height = 2.6cm, width = 5cm]{\pathPic/Subdivision/Cut2_4.pdf}
\hspace{1cm}
\includegraphics[height = 2.6cm, width = 5cm]{\pathPic/Subdivision/Cut2_1.pdf}
\caption{\label{figCut2} Illustrations of Assumptions \ref{assumBi}, a) left and b) right. The line $D$ (Thick), forbidden bisection choices (dashed), authorized bisection choices (full).}
\end{figure}

The following assumptions on the decision function are illustrated on Figure \iref{figCut2}. Their purpose is to create, through the refinement process, a thin layer of triangles along the line $D$.
\begin{assumptions}
\label{assumBi}
Let $T$ be a triangle such that $e_T(\chi_P) \neq 0$. 
In the following we work under the assumption that 
segment $s\in S_T^3$ which minimizes the decision function $d_T(s,\chi_P)$ satisfies the following properties.
\begin{enumerate}[a)]
\item If there is such a possibility in $S_T^3$, the bisection of $T$ along $s$ creates a child $T'$ such that $e_{T'}(\chi_P) = 0$. 
\item If a) is impossible then the decision function selects a segment $s\in S_T^3$ joining a vertex of the triangle $T$ to the midpoint of an edge which is intersected by the line $D$.
\end{enumerate}
\end{assumptions}

These two properties are illustrated in figure \ref{figCut2}. Numerical experiments strongly suggest that they are satisfied for the decision function based on the $L^2$ error which is defined by \iref{eqDecisionL2Bi}.

We first prove the lower error bound \iref{eqBelowBi}, and for that purpose we denote by $\TRef$ the triangle of vertices
$$
(0,-1), (3,-1), (0,2).
$$
$\TRef$ is the large triangle enclosing the others on Figure \ref{figSmallTree}.
The refinement procedure applied to the triangle $\TRef$ and the function $f=\chi_P$ creates an infinite master tree $\cPRef$ of triangles. 
If $\cP$ is a finite subtree of $\cPRef$, (in other words $\cP$ contains $\TRef$ and the nodes of $\cP$ have either two or no children), then the leaves of $\cP$ define a triangulation $\cT$ of $\TRef$. 

\begin{prop}
\label{propNegResult}
There exists a constant $c>0$ such that : 
for any triangulation $\cT$ associated to a finite subtree of $\cPRef$, we have 
\be
\label{eqErrorChiNeg}
e_\cT(\chi_P) \geq c \#(\cT)^{-\lambda/2}
\ee
where $c>0$ is a positive constant and $\lambda = 1.464\cdots$ is the solution of 
\be
\label{defLambdaNeg}
\left(\frac 1 4\right)^{\frac1{1+\lambda}} +  \left(\frac 1 8\right)^{\frac1{1+\lambda}}=1.
\ee
In particular let $(\cT_N)_{N\geq 1}$ be the sequence of triangulations  generated by the greedy algorithm applied to the function $f=\chi_P$ and starting from $\cT_1 = \{\TRef\}$. If the decision function satisfies Assumptions \ref{assumBi}, then for all $N \geq 1$ one has 
$$
e_{\cT_N}(\chi_P) \geq c N^{-\lambda/2}.
$$
\end{prop}

\begin{figure}
\centering
\includegraphics[height = 3cm, width = 4cm]{\pathPic/Subdivision/Tree1.pdf}
\hspace{0.5cm}
\includegraphics[height = 3cm, width = 4cm]{\pathPic/Subdivision/Tree2.pdf}
\hspace{0.5cm}
\includegraphics[height = 3cm, width = 4cm]{\pathPic/Subdivision/Cut2_3.pdf}
\caption{\label{figSmallTree}Subdivision of the triangle $\TRef$, some of its children and grand-children, with a decision function satisfying Assumptions \ref{assumBi}. The colored triangles satisfy $e_T(\chi_P) = 0$.}
\end{figure}

\begin{figure}
\centering
\includegraphics[height = 4cm, width = 4cm]{\pathPic/Subdivision/TreeTri.pdf}
\hspace{1cm}
\includegraphics[height = 4cm, width = 6cm]{\pathPic/Subdivision/TreeEq.pdf}
\caption{\label{figSmallTree2}Tree associated to the subdivision illustrated on Figure \ref{figSmallTree} (left), and equivalence classes of the elements of this tree for the relation of $D$-affine equivalence (right).}
\end{figure}

\proof
Figures \ref{figSmallTree} and \ref{figSmallTree2} reveal a surprising property of the master tree $\cPRef$. After a few steps, as illustrated on the right of Figure \ref{figSmallTree} we obtain two (white) triangles which are $D$-affine equivalent to the initial triangle $\TRef$, and three (colored) triangles on which the approximation error $e_T(\chi_P)$ is zero. It follows that, up to the relation of $D$-affine equivalence, the tree $\cPRef$ is \emph{self-similar} and is a repetition of the pattern presented on the right of Figure \ref{figSmallTree2}. 

We define an auxiliary tree $\cPRef'$ as follows. The nodes of $\cPRef'$ are the triangles $T_0\in \cPRef$ which are affine equivalent to $\TRef$ with respect to $D$. The children $T_1,T_2$ of a triangle $T_0$ in $\cPRef'$ are the grand-child and grand-grand-child of $T_0$ in $\cPRef$ which are affine equivalent to $\TRef$. Note that 
\be
\label{eqRatioArea}
|T_0| = 4 |T_1| = 8 |T_2|.
\ee
Let $\cT$ be a triangulation of $\TRef$ associated to a finite subtree $\cP$ of $\cPRef$. We denote by $\cP'$ the smallest subtree of $\cPRef'$ such that any leaf of $\cP'$ is contained in a leaf of $\cP$. %triangle in $\cP$ contains a triangle in $\cP'$. 
We denote by $\cT'$ the collection of leaves of $\cP'$. For instance, if $\cT$ is any of the three triangulations illustrated on Figure \ref{figSmallTree}, then $\cT'$ consists of the two white triangles in the right of Figure \ref{figSmallTree}. A triangle $T\in \cT$ contains a single triangle $T'\in \cT'$ if $e_T(\chi_P)\neq 0$, and none otherwise. Therefore 
\be
\label{eqCardTNeg}
\#(\cT')\leq \#(\cT).
\ee
Furthermore, since all the elements of $\cT'$ are $D$-affine equivalent to $\TRef$, we have 
\be
\label{eqErrorTNeg}
e_{\cT'}(\chi_P)^2 = \sum_{T\in \cT} e_T(\chi_P)^2 \geq \sum_{T\in \cT'} e_T(\chi_P)^2 = c_0 \sum_{T\in \cT'} |T|
\ee
where $c_0=e_{\TRef}(\chi_P)^2$. %, since all the elements of $\cT'$ are affine equivalent to $\TRef$ with respect to $D$.
For any triangle $T_0\in \cP'$, we denote by $\cE(T_0)$ the collection of the elements of $\cT'$ that it contains, 
$$
\cE(T_0) := \{T\in \cT' \sep T \subset T_0\},
$$
and we define %two numbers $a(T_0)$ and $n(T_0)$ as follows
$$
a(T_0) := \sum_{T\in \cE(T_0)} |T| \stext{ and } n(T_0) := \# (\cE(T_0)).
$$
We establish below that for any $T_0\in \cP'$, the following inequality holds
\be
\label{eqInducTree}
|T_0| \leq a(T_0) \, n(T_0)^\lambda.
\ee
Once this property is established, then choosing $T_0 = \TRef$ and combining this inequality %\iref{eqInducTree} 
with \iref{eqCardTNeg} and \iref{eqErrorTNeg} yields 
\begin{eqnarray*}
e_\cT(\chi_P)^2 &\geq&  c_0 \sum_{T\in \cT'} |T|\\
&=& c_0 \, a(\TRef)\\
&\geq & c_0 \, |\TRef| \, n(\TRef)^{-\lambda}\\
&=& c^2 \, \#(\cT')^{-\lambda}\\
&\geq & c^2 \, \#(\cT)^{-\lambda},
\end{eqnarray*}
where $c^2=c_0 \, |\TRef|$.
%$$
%e_{\cT}(\chi_P)^2 = c_0 \, a(\TRef) \geq c_0 \, |\TRef| \, n(\TRef)^{-\lambda}.
%$$
This establishes the announced result \iref{eqErrorChiNeg} and concludes the proof of this proposition.
In order to prove \iref{eqInducTree} we use an induction argument on the tree $\cP'$, and for that purpose we distinguish two cases.
\begin{enumerate}[i)]
\item If $T_0$ is a leaf of $\cP'$, then $T_0\in \cT'$ and therefore $a(T_0) = |T_0|$ and $n(T_0) =1$, hence \iref{eqInducTree} holds.
\item Otherwise $T_0$ has two children $T_1$ and $T_2$ in $\cP'$, and we may assume as an induction hypothesis that 
\be
\label{eqHR}
|T_1| \leq a(T_1) \, n(T_1)^\lambda \stext{ and } |T_2| \leq a(T_2) \, n(T_2)^\lambda.
\ee
Applying the holder inequality 
$$
u_1v_1+ u_2v_2 \leq (u_1^p+u_2^p)^{\frac 1 p} (v_1^q+ v_2^q)^{\frac 1 q}
$$ 
to the numbers 
$$
u_i = a(T_i)^{\frac 1 p}, \quad v_i = n(T_i)^{\frac 1 q}, \quad  p=1+\lambda, \quad q= \frac{1+\lambda}\lambda = \frac p \lambda,
$$
and elevating to the power $p$, we obtain 
\be
\label{eqHolderTree}
\left(\left(a(T_1) \, n(T_1)^{\lambda}\right)^{\frac 1 {p}} + \left(a(T_2) \, n(T_2)^{\lambda}\right)^{\frac 1 {p}} \right)^{p} \leq (a(T_1)+a(T_2)) \left(n(T_1)+ n(T_2)\right)^\lambda.
\ee
%$$
%\left(\left(a(T_1) \, n(T_1)^{\lambda}\right)^{\frac 1 {1+\lambda}} + \left(a(T_2) \, n(T_2)^{\lambda}\right)^{\frac 1 {1+\lambda}} \right)^{1+\lambda} \leq (a(T_1)+a(T_2)) \left(n(T_1)+ n(T_2)\right)^\lambda.
%$$ 
If follows that 
\begin{eqnarray*}
|T_0| &=& \left(\left(\frac {|T_1|} 4\right)^{\frac1{p}} +  \left(\frac {|T_2|} 8\right)^{\frac1{p}}\right)^p\\
&=& \left(|T_1|^{\frac 1 {p}}+ |T_2|^{\frac 1 {p}} \right)^{p}\\
&\leq & \left(\left(a(T_1) \, n(T_1)^{\lambda}\right)^{\frac 1 {p}} + \left(a(T_2) \, n(T_2)^{\lambda}\right)^{\frac 1 {p}} \right)^{p} \\
&\leq & (a(T_1)+a(T_2)) \left(n(T_1)+ n(T_2)\right)^\lambda.\\
&=& a(T_0) \, n(T_0)^\lambda,
\end{eqnarray*}
where we use successively \iref{defLambdaNeg}, \iref{eqRatioArea}, \iref{eqHR}, \iref{eqHolderTree} and the equalities $a(T_0) = a(T_1)+a(T_2)$ and $n(T_0)=n(T_1)+n(T_2)$. Again \iref{eqInducTree} holds, and by induction it holds for any element of $\cP'$.
\sq
\end{enumerate}


\begin{figure}
\centering
\includegraphics[height = 2.6cm, width = 3cm]{\pathPic/Subdivision/lemma2_1.pdf}
\hspace{1cm}
\includegraphics[height = 2.6cm, width = 3cm]{\pathPic/Subdivision/lemma2_2.pdf}
\caption{\label{figRefine2}Bisection of a triangle, some of its children, grand-children and grand-grand-children, with decision function satisfying Assumptions \ref{assumBi}}
\end{figure}

We now turn to the proof of the upper estimate \iref{eqUpperBi}, and for that purpose we begin with a geometrical lemma which uses the two assumptions \iref{assumBi} to analyse the first steps of the refinement procedure.

\begin{lemma}
\label{lemmaSmallRef2}
Let $T$ be a triangle such that $e_T(\chi_P)\neq 0$.
If the decision function satisfies \iref{assumBi}, then one of the following holds
\begin{enumerate}[i)]
\item A child $T'$ produced by the bisection of $T$ satisfies $e_{T'}(\chi_P) = 0$.
\item Applying iteratively the refinement procedure to $T$, some of its children, grand-children and grand-grand-children we obtain a triangulation $\cT$ of $T$ such that
\begin{itemize} 
\item $\#(\cT)\leq 5$, and $|T'| \geq \frac 1 {2^4} |T|$ for all $T'\in \cT$.
\item The approximation error $e_{T'}(\chi_P)$ is non-zero for at most two triangles $T'\in \cT$. Denoting these triangles by $T_1,T_2$, one of the following two possibilities holds %we have either %there exists $i\in \{0,1,2\}$ such that 
$$
|T| = 4 |T_1| = 8|T_2| \stext{ or } |T| = 2 |T_1| = 16|T_2|.
$$
\end{itemize}
\end{enumerate}
\end{lemma}

\proof
Rather than reading a long discussion, the author invites the reader to check that, if i) is impossible, then one of the two possibilities illustrated on Figure \ref{figRefine2} occurs and satisfies ii).
\sq

\begin{prop}
\label{propSpeedBi}
Let $\cT_{N_0}$ be an arbitrary triangulation in $\R^2$ and let $(\cT_N)_{N\geq N_0}$ be the sequence of triangulations generated by the greedy algorithm applied to the function $f=\chi_P$ and starting from the triangulation $\cT_0$. If the decision function satisfies Assumptions \ref{assumBi}, then 
$$
e_{\cT_N} (\chi_P) \leq C N^{-\lambda/2},
$$
where $\lambda/2 = 0.732\cdots$ is defined by \iref{defLambdaNeg}.
\end{prop}

\proof
A proof of this proposition can be obtained by a straightforward adaptation of Lemma \ref{lemmaTEpsMu} and Proposition \ref{propSpeedTri} in the next section. This adaptation is left as an exercise to the reader.
\sq
%\begin{remark}
%The proof of Proposition \iref{propNegResult} can be extended to decision functions $d_T(s,f)$ that do not satisfy the assumption a). The author suspects that assumption b) can also be removed, but does not know how to prove it.
%%The proof of the The previous theorem is based on the assumption that the decision function satisfies the a) and b). It is easy to prove that a) can be removed, but the author does not know if the result still holds if the assumption b) is removed.
%\end{remark}

\subsection{Six bisection choices}
\label{secTriSec}
The previous section contains a negative result, Proposition \ref{propNegResult}, showing that the greedy refinement procedure does not achieve desired the convergence speed \iref{eqEstimChi} when it is based on the three bisection choices $S_T^3$ and a decision function satisfying the natural assumptions \ref{assumBi}.
%e_{\cT_N}(\chi_P) \leq CN^{-1}.

In this section the segment along which a triangle $T$ is bisected is picked among the six possibilities in $S_T^6$, illustrated on Figure \ref{figTriSec}, instead of the three possibilities in $S_T^3$. If the decision function satisfies Assumptions \ref{assumTri}, then the desired convergence speed \iref{eqEstimChi} is achieved, see Proposition \ref{propSpeedTri}. This result can be seen as a first step towards the construction of a hierarchical and anisotropic refinement algorithm well adapted to the approximation of cartoon functions.

%A possible cure for this problem is to increase the number of bisection possibilities. Instead of $3$ cut choices, we attempted to allow six cut choices, as illustrated in the right of Figure \ref{figTriSec}. When these additional choices are allowed, and provided the decision function satisfies some assumptions, the previous negative result does not hold anymore.


The following assumptions on the decision function $d_T(s,f)$ are illustrated on Figure \ref{figDecision3}. Their purpose is to create, through the refinement process, a thin layer of triangles along the line $D$. Please note that  for any triangle $T$ any for any segment $s\in S_T^6$, the two children of $T$ have areas $\frac 1 3 |T|$ and $\frac 2 3 |T|$.
\begin{assumptions}
\label{assumTri}
Let $T$ be a triangle such that $e_T(\chi_P) \neq 0$. 
In the following we work under the assumption that 
segment $s\in S_T^6$ %(joining a vertex $v_1$ of $T$ to the barycenter midpoint of the opposite edge $e$) 
which minimizes the decision function $d_T(s,\chi_P)$ satisfies the following properties.
%
%We assume in the following that the decision function, which selects the bisection among the six possible choices, satisfies the two following properties.
\begin{enumerate}[a)]
\item If there is such a possibility in $S_T^6$, the bisection of $T$ along $s$ creates a child $T'$ such that $e_{T'}(\chi_P) = 0$ and $|T'| = \frac 2 3 |T|$.
\item If a) is impossible, then whenever there is such a possibility in $S_T^6$, the bisection of $T$ along $s$ creates a child $T'$ such that $e_{T'}(\chi_P) = 0$ and $|T'| = \frac 1 3 |T|$.
\item If a) and b) are impossible then the decision function selects a segment $s = [v_1,b] \in S_T^6$ joining a vertex $v_1$ of the triangle $T$ to the barycenter $b=\frac 1 3 v_2+ \frac 2 3 v_3$ of the other vertices. The choice of $s$ must be such that the line $D$ intersects the segment $[b,v_3]$.
\end{enumerate}
\end{assumptions}


\begin{figure}
\centering
\includegraphics[height = 2.6cm, width = 4.5cm]{\pathPic/Subdivision/Cut3_6.pdf}
\includegraphics[height = 2.6cm, width = 4.5cm]{\pathPic/Subdivision/Cut3_4.pdf}
\includegraphics[height = 2.6cm, width = 4.5cm]{\pathPic/Subdivision/Cut3_5.pdf}
\caption{\label{figDecision3} Illustrations of Assumptions \ref{assumTri}, a) left, b) center and c) right. The line $D$ (Thick), forbidden bisection choices (dashed), authorized bisection choices (full).}
\end{figure}

The next lemma uses these three assumptions to analyse the first steps of the refinement procedure on a triangle $T$.

\begin{lemma}
\label{lemmaSmallRef3}
Let $T$ be a triangle such that $e_T(\chi_P)\neq 0$.
%Let $T$ be a triangle such that $D\cap \mathring T\neq \emptyset$. 
If the decision function satisfies \iref{assumTri}, then one of the following holds
\begin{enumerate}[i)]
\item A child $T'$ produced by the bisection of $T$ satisfies $e_{T'}(\chi_P) = 0$.
\item Applying iteratively the refinement procedure to $T$, some of its children, grand-children and grand-grand-children we obtain a triangulation $\cT$ of $T$ such that
\begin{itemize} 
\item $\#(\cT)\leq 7$, and $|T'| \geq \frac 1 {3^4} |T|$ for all $T'\in \cT$.
\item The approximation error $e_{T'}(\chi_P)$ is non-zero for at most two triangles $T'\in \cT$. Denoting these by $T_1,T_2$, there exists $i\in \{0,1,2\}$ such that 
\be
\label{eqRatioTChild}
\frac {|T_1|} {|T|} \leq \frac 1 3 \times \left(\frac {3-i} 3\right)^2 \stext{ and } \frac {|T_2|}{|T|} \leq \frac 2 9 \times \left(\frac {i+1} 3\right)^2.
\ee
\end{itemize}
\end{enumerate}
\end{lemma}

\proof
Rather than reading a long discussion, the author invites the reader to check that, if i) is impossible, then one of the three possibilities illustrated on Figure \ref{figRefine3} occurs and satisfies ii).
\sq

Let $T_r$ be a triangle such that $e_{T_r}(\chi_P)\neq 0$. The decision function applied to $T_r$ and its descendants defines a master tree $\cP_r$ of triangles.
If $\cP$ is a finite subtree of $\cP_r$, (in other words $\cP$ contains $T_r$, and the nodes of $\cP$ have either two or no children), then the leaves of $\cP$ define a triangulation $\cT$ of $T_r$. The next lemma describes some of these triangulations.


\begin{lemma}
\label{lemmaTEpsMu}
For any $0<\ve\leq 1$, there exists a triangulation $\cT_\ve$ of $T_r$ associated to a finite subtree of $\cP_r$, which satisfies
$
\#(\cT_\ve) \leq C \ve^{-\mu}
$
and 
\be
\label{eqTAreaEps}
\max \{ |T| \sep T \in \cT_\ve \text{ and } e_T(\chi_P) \neq \emptyset \} \ \leq  \ve |T_0|
\ee
where $C=30$ and $\mu = 0.329\cdots$ is the solution of 
\be
\label{defMuTri}
\left(\frac 4 {27}\right)^\mu + \left(\frac 8 {81}\right)^\mu = 1.
\ee
As a result, the master tree $\cP_r$ contains at most $C\ve^{-\mu}$ triangles $T$ such that $e_T(\chi_P)^2 \geq \ve |T_r|$.
 % and $\lambda = ...$.
%As a result there exists at most $C\ve^{-1/3}$ triangles $T$ in the master tree $\cP_r$ of area $|T|\geq \ve |T_0|$ and such that $e_T(\chi_P)\neq 0$.
%
%Then for each integer $N\geq 1$ there exists a triangulation $\cT$ of $T$ produced by the refinement procedure such that 
%$
%\#(\cT) \leq N
%$
%and 
%$$
%\max \{ |T| \sep T\in \cT \text{ and } D \cap \mathring T \neq \emptyset \} \leq C N^{-\lambda}
%$$
%where $C=...$ and $\lambda = ...$.
\end{lemma}

\begin{figure}
\centering
\includegraphics[height = 3cm, width = 4cm]{\pathPic/Subdivision/Cut3_1.pdf}
\hspace{1cm}
\includegraphics[height = 3cm, width = 4cm]{\pathPic/Subdivision/Cut3_2.pdf}
\hspace{1cm}
\includegraphics[height = 3cm, width = 4cm]{\pathPic/Subdivision/Cut3_3.pdf}
\caption{\label{figRefine3}Bisection of a triangle, some of its children, grand-children and grand-grand-children, with a decision function satisfying Assumptions \ref{assumTri}.}
\end{figure}

\proof
We consider a second tree $\cP_r'$ of triangles, with root $T_r$. 
A triangle $T\in \cP_r'$ such that $e_T(\chi_P) = 0$ has no children. A triangle $T\in \cP_r'$ such that  $e_T(\chi_P)\neq 0$ has at most $7$ children, those described in Lemma \ref{lemmaSmallRef3}. Two cases are possible : 
\begin{enumerate}[i)]
\item The triangle $T$ has two children and one of them, denoted by $T'$, satisfies $e_{T'}(\chi_P)=0$. The child $T'$ of $T$ is therefore a leaf of the tree $\cP_r'$. 
\item The triangle $T$ has at most $7$ children, and at most two of them $T_1,T_2$ are not leaves of the tree $\cP_r'$.  Furthermore the areas of $T_1,T_2$ satisfy \iref{eqRatioTChild} for some $i\in \{0,1,2\}$. 
\end{enumerate}

We denote by $\cP'_\ve$ the subtree of $\cP'_r$ created as follows : we start from the root $T_r$, and we include the children of a triangle $T$ if and only if $e_T(\chi_P) \neq 0$ and $|T|>\ve|T_r|$.
We define $\cT_\ve$ as the collection of leaves of $\cP'_\ve$ and we remark that \iref{eqTAreaEps} is satisfied. 
Note that the parent $T\in \cP'_\ve$ of any triangle $T'\in \cP'_\ve$ satisfies $|T| \geq \ve |T_0|$. Lemma \ref{lemmaSmallRef3} therefore implies that 
\be
\label{eqAreaBelow}
|T'|\geq \frac  {\ve |T_r|}  {3^4} \stext{ for any } T'\in \cP'_\ve.
\ee
We associate to each triangle $T_0\in \cP'_\ve$ the number 
$$
n(T_0) := \# \{T\in \cT_\ve \sep T\subset T_0\},
$$
and we intend to show that for any triangle $T_0$ in the tree $\cP'_\ve$ one has
%For each triangle $T_0\in \cP_\ve$, let us show that 
\be
\label{eqRecTree3}
n(T_0) +5 \leq C \left(\frac {|T_0|}{\ve |T_r|}\right)^\mu
\ee
Once this point is established, choosing $T_0 =T_r$ concludes the proof of the first part of this proposition.
For that purpose, we proceed by induction on the tree $\cP'_\ve$. We first remark that 
for any leaf $T_0$ of $\cP'_\ve$ is follows from \iref{eqAreaBelow} that 
%we obtain using \i
%If $T_0$ is a leaf of $\cP_\ve$, then %by definition of the tree $\cP'_\ve$ 
%the parent $T$ of $T_0$ has an area $|T|\geq \ve |T_r|$. It follows from Lemma \iref{lemmaSmallRef3} that $|T_0| \geq \frac {|T|} {3^4}$ and therefore 
$$
C \left(\frac {|T_0|}{\ve |T_r|}\right)^\mu \geq C \left(\frac 1 {3^4}\right)^\mu \geq 6 = n(T_0)+5.
$$

If $T_0$ is not a leaf of $\cP'_\ve$, then %$|T_0| \geq \ve |T_r|$. Furthermore 
we may assume as an induction hypothesis that \iref{eqRecTree3} holds for all the children of $T_0$. We now distinguish between the two types of nodes i) and ii) of the tree $\cP'_\ve$, and we obtain the following.
\begin{enumerate}[{Type} i)]
\item The triangle $T_0$ has two children, $T_1$, $T_2$, where $T_2$ is a leaf of the tree $\cP'_\ve$. Since $T_0$ is not a leaf of $\cP'_\ve$, it satisfies $|T_0|\geq \ve |T_r|$. Furthermore $|T_1| \leq \frac 2 3 |T_0|$, 
hence  
\begin{eqnarray*}
C \left(\frac {|T_0|}{\ve |T|}\right)^\mu &=& C \left(\frac 2 3 \times \frac { |T_0|}{\ve |T_r|}\right)^\mu + \left(1-\left(\frac 2 3\right)^\mu\right) \left( \frac { |T_0|}{\ve |T_r|}\right)^\mu\\ 
&\geq & C  \left( \frac {|T_1|}{\ve |T_r|}\right)^\mu + C \left(1-\left(\frac 2 3\right)^\mu\right)\\
&\geq & n(T_1)+5 +1 \\
&=& n(T_0)+5.
%C \left(\left(\frac 3 2\right)^{\lambda}-1) \left(\frac |T_1|\right)
\end{eqnarray*}
Therefore $T_0$ satisfies \iref{eqRecTree3}.
\item
The triangle $T_0$ has at most seven children, and at most two of them, denoted by $T_1$, $T_2$, are not leaves. Hence $n(T_0) \leq n(T_1)+n(T_2)+5$. 
Using the estimate \iref{eqRatioTChild} on the areas of $T_1$ and $T_2$, and the definition \iref{defMuTri} of $\mu$, we obtain
$$
\left(\frac{|T_1|}{|T_0|}\right)^\mu+ \left(\frac{|T_2|}{|T_0|}\right)^\mu \leq 1.
$$
Therefore 
\begin{eqnarray*}
C  \left(\frac {|T_0|}{\ve |T_r|}\right)^\mu &\geq & C  \left(\frac {|T_1|}{\ve |T_r|}\right)^\mu + C  \left(\frac {|T_2|}{\ve |T|}\right)^{\lambda}  \\
&\geq & n(T_1)+5+ n(T_2)+5\\
%& \geq & n(T_1)+ n(T_2)+5\\
& \geq & n(T_0)+5,
\end{eqnarray*}
which concludes the proof of \iref{eqRecTree3}. 
\end{enumerate}
We now turn to the second part of the proposition, and for that purpose we denote by $\cP_\ve$ the subtree of $\cP_r$ associated to the triangulation $\cT_\ve$. Note that this tree is distinct from the subtree $\cP'_\ve$ of $\cP_r'$. In particular $\cP_\ve$ is a binary tree while $\cP'_\ve$ is not (the tree $\cP'_\ve$ can be obtained by grouping some of the elements of $\cP_\ve$ in a single node with some of their descendants).

Since $\cP_\ve$ is a binary tree, the cardinality of the set $\cP_\ve\sm \cT_\ve$ of its inner nodes has a simple expression
$$
\#(\cP_\ve \sm \cT_\ve) = \#(\cT_\ve)-1.
$$
Furthermore, any triangle $T \in \cP_r$ which does not belong to $\cP_\ve\sm \cT_\ve$ is an element of $\cT_\ve$ or one of its descendants, hence $T$ satisfies $e_T(\chi_P) = 0$ or $e_T(\chi_P)^2\leq |T|< \ve |T_r|$.
%Furthermore let $T \in \cP_r$ be a triangle which is not an inner node of $\cP_\ve$. Then either $T\in \cT_\ve$, in which case $e_T (\chi_P)^2 \leq |T| \leq \ve |T_0|$, or $\mathring T \cap D = \emptyset$, in which case $e_T(\chi_P) = 0$.
Therefore
$$
\#(\{T \in \cP_r \sep e_T(\chi_P)^2 \geq \ve |T_r|\}) \leq \#(\cP_\ve\sm \cT_\ve) = \#(\cT_\ve)-1\leq C \ve^{-\mu},
$$
which concludes the proof.
\sq

\begin{prop}
\label{propSpeedTri}
Let $\cT_{N_0}$ be an arbitrary triangulation in $\R^2$ and let $(\cT_N)_{N\geq N_0}$ be the sequence of triangulations generated by the greedy algorithm applied to the function $f=\chi_P$ and starting from the triangulation $\cT_0$. If the decision function satisfies the assumptions \ref{assumTri}, then 
\be
\label{eqErrorNu}
e_{\cT_N} (\chi_P) \leq C N^{-\nu},
\ee
where $\nu = \frac 1 {2 \mu} -\frac 1 2= 1.0188\cdots$. 
\end{prop}

\proof
Let $T_0$ be a triangle, let $f\in L^2(T)$ and let $T_1$, $T_2$ be the children produced by some bisection of $T$. Then
% it follows from 
\begin{eqnarray*}
e_{T_1}(f)^2+e_{T_2}(f)^2 &=& \inf_{\pi_1, \pi_2\in \sP_1} \|f-\pi_1\|_{L^2(T_1)}^2+\|f-\pi_2\|_{L^2(T_2)}^2\\
&\leq & \inf_{\pi\in \sP_1} \|f-\pi\|_{L^2(T_1)}^2+\|f-\pi\|_{L^2(T_2)}^2\\
& = & e_{T_0}(f).
\end{eqnarray*}
Hence 
$$
\max\{e_{T_1}(f),e_{T_2}(f)\} \leq e_{T_0}(f).
$$
The decision function applied to the triangles in $\cT_0$ and their descendants defines a collection $\cP_0$ of $N_0$ master trees. It follows from the previous inequality that the approximation error $e_T(\chi_P)$ is larger on a triangle $T$ than on any of its descendants.

At each step $N \geq N_0$, the greedy algorithm selects for bisection a triangle in $T_N \in \cT_N$ which maximizes the approximation error $e_T(\chi_P)$ among all $T \in \cT_N$.
As a result we have for %, the sequence $(T_N)_{N \geq N_0}$ of triangles selected for bisection by the greedy algorithm satisfies for 
any $N\geq N_0$,
$$
e_{T_{N_0}}(\chi_P) \geq e_{T_{N_0+1}}(\chi_P) \geq \cdots \geq e_{\cT_N}(\chi_P) \geq \max \left\{e_T(\chi_P) \sep T \in \cP_0 \sm \{T_0, \cdots, T_N\}\right\}.
$$
We thus have for any $N\geq 0$, since $\#(\cT_N)=N$,
\be
\label{eqErrorGreedyDec}
e_{\cT_N}(\chi_P)^2 = \sum_{T\in \cT_N} e_T(\chi_P)^2 \leq N \ e_{T_N} (\chi_P)^2.
\ee
According to Lemma \ref{lemmaTEpsMu}, for any $0<\ve \leq 1$ the collection $\cP_0$ of $N_0$ trees contains at most $C_0 \ve^{-\mu}$ triangles $T$ such that $e_T(\chi_P)^2 \geq \ve$, where $C_0$ is independent of $\ve$. Choosing $\ve = C_0^{\frac 1 \mu} N^{-\frac 1 \mu}$ we obtain  
$$
e_{T_N}(\chi_P)^2 \leq C_0^{\frac 1 \mu} N^{-\frac 1 \mu}.
$$
Combining this with \iref{eqErrorGreedyDec} yields \iref{eqErrorNu} which concludes the proof.
\sq

\begin{remark}
\label{remarkExcessiveSpeed}
The convergence speed obtained in Proposition \ref{propSpeedTri} actually exceeds the desired error estimate \iref{eqEstimChi}. This point is due to the fact that  $f=\chi_P$ is a particularly simple cartoon function.
For a function cartoon $f$ which is discontinuous along curved edges, instead of a straight line, or which is not piecewise affine, the convergence speed \iref{eqEstimChi} is optimal.
\end{remark}

\subsection{Partitions of a domain into convex polygons} %Replacing triangles with convex polygons} %Partitions into A modification of the refinement procedure}
\label{secConvexCut}

We suggest in this section another modification of the refinement procedure, in an attempt to improve the result of Proposition \ref{propSpeedTri}. This proposition in indeed not completely satisfactory, in particular because of the following three reasons.
%which is motivated by the following three 
%The result previous proposition is not completely satisfactory however, for three main reasons.
\begin{itemize}
\item The decision function $d_T(s,f)$ needs to satisfy Assumptions \ref{assumTri}. Unfortunately numerical results  suggest that the natural decision function \iref{eqDecisionL2Bi} does not satisfy these assumptions, and the author has not found a decision function with a simple expression which satisfies these assumptions.
%cannot think of a simple  
%The assumption
%The choice of the decision function is essential, and the author cannot find a decision function that is both appropriate for edge regions and for smooth regions.
% it might be and we have no idea of a simple such function. %decision the decision functions encountered earlier may not
\item The number of segments $s\in S_T^6$ along which a triangle $T$ may be bisected has increased from $3$ to $6$. 
From the point of view of data compression, the hierarchical bisection tree is therefore more expensive to encode. From the theoretical point of view, the algorithm could be regarded as less elegant. 
\item Since the cartoon function $f=\chi_P$ is particularly simple, see Remark \ref{remarkExcessiveSpeed}, a convergence speed faster that \iref{eqErrorNu} could be expected. For example an exponential convergence speed $e_{\cT_N}(\chi_P)\leq C e^{-\beta N}$ where $\beta>0$.
%The exponent $\alpha$ is only slightly greater than $2$, while one could expect an exponential rate of approximation $|\{f\neq f_N\}| \leq C e^{-\beta N}$.
\end{itemize}

The modification of the algorithm described below solves these three points, at the following cost. The modified greedy algorithm does not produce triangulations any more, but partitions into convex polygons of the domain $\Omega$ on which the function $f$ to be approximated is defined. %of definition of the function $f$ to be approximated.

We denote by $\cC$ the collection of bounded closed and convex sets of nonempty interior included in $\R^2$. We denote by the capital letter $T$ the elements of $\cC$, whether they are triangles or not, and by $\cT$ any partition of a domain $\Omega$ into elements of $\cC$. 
The definitions \iref{defErrTL2} and \iref{defErrCTL2} of the approximation errors $e_T(f)$ and $e_\cT(f)$ are unchanged.
%If $\cT$ is a partition of a polygonal domain $\Omega$ into elements of of $\cC$, then 
%
%
%Despite this difference, we use the letter $T$ for bounded closed and convex, and $\cT$ for partitions of a domain $\Omega$ into bounded convex polygons. The definitions \iref{defErrorTL2} and \iref{defErrorCTL2} of the approximation errors are unchanged.
%
%%In order to emphasize this difference, we use the notation $C$ instead of $T$ for convex polygons, and $\cC$ instead of $\cT$ for partitions into convex polygons.
%%The $L^2$ approximation error $e_C(f)$ of a function $f$ on a convex polygon $C$ is defined 
%%
%%by generic convex polygon by $C$, and a partition of a polygonal domain 
%%For any convex polygon $C$, and any $f\in L^2(C)$, we define $e_C(f)$ as in 

%Let $C\subset \R^2$ be a bounded closed and convex set, and let $a,b,c\in \partial C$. 

Let $T\in \cC$ be a bounded closed and convex set, and let $a,b,c\in \partial T$ be three distinct points on the boundary of $T$.
If none of the segments $[a,b]$, $[b,c]$ or $[c,a]$ is included in $\partial T$, then the complementary in $T$ of the triangle of vertices $a,b,c$ has three connected components.
We denote by $T_a$ the adherence of the connected component which does not contain $a$, and  %, in such way that $[b,c] \subset \partial T_a$. 
we define $T_b$ and $T_c$ likewise, see Figure \ref{figCvxCut}. 
The bisection of $T$ along the segment $[b,c]$, $[c,a]$ or $[a,b]$ produces a pair of children $\{T_a, \overline {T\sm T_a}\}$,  $\{T_b, \overline {T\sm T_b}\}$ or $\{T_c, \overline {T\sm T_c}\}$ which also belong to $\cC$. 
%produced by the bisection of $T$ along the segment $[b,c]$, $[c,a]$ or $[a,b]$ all belong to $ \cC$.
%(strictly speaking, $C_a$ depends on the three points $a,b,c$). 
We define 
$$
\tau(T \sep a,b,c) := \min \{|T_a|, |T_b|, |T_c|\}
$$
and we set the convention $\tau(T \sep a,b,c) = 0$ for any $a,b,c\in \partial C$ such that the complementary in $T$ of the triangle of vertices $a,b,c$ has only two connected components. We also define
\be
\label{defTauT}
\tau(T) := \sup_{a,b,c\in \partial T} \tau(T \sep a,b,c).
\ee
%where the supremum is taken among all $a,b,c\in \partial T$, with the conventio

\begin{figure}
\centering
\includegraphics[width = 4cm, height=4cm]{\pathPic/Subdivision/Cvx1Names.pdf}
\hspace{1cm}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Subdivision/Cvx2.pdf}
\hspace{1cm}
\includegraphics[width = 4cm, height=4cm]{\pathPic/Subdivision/Cvx3.pdf}
\caption{\label{figCvxCut} Bisection of a convex $T\in \cC$ along the set of segments $S_T^{3*}$ determined by three points $a,b,c\in \partial T$ which maximize \iref{defTauT}.}
\end{figure}

\begin{prop}
\label{propConvex}
The supremum \iref{defTauT} is attained and for any $a,b,c$ satisfying $\tau(T\sep a,b,c) = \tau(T)$, and we have $|T_a| = |T_b| = |T_c| = \tau(T)$.
Furthermore there exists $\delta>0$ such that for any $T \in \cC$, one has 
\be
\label{eqDeltaTC}
\delta |T| \leq \tau(T). %\leq \frac 1 4 |T|. (* useless and hard to prove...*)
\ee
\end{prop}

\proof
For any fixed $T\in \cC$, the boundary $\partial T$ is compact and the map
$$
(a,b,c)\in (\partial T)^3 \mapsto \tau(T\sep a,b,c)
$$
is continuous. Hence the maximum \iref{defTauT} is attained. Furthermore let $a,b,c \in \partial T$ and let us assume that $|T_a| > |T_b|$, then moving the point $c\in \partial T$ in the direction of $T_a$ continuously decreases $|T_a|$ and increases $|T_b|$. As a result, if the triplet $(a,b,c)\in (\partial T)^3$ maximizes \iref{defTauT}, then one must have $|T_a| = |T_b|=|T_c|$.

For any $T\in \cC$, we denote by $b(T)\in \R^2$ the barycenter of $T$ and by $m(T)\in S_2^+$ the matrix of the second order moments of $T$. They are defined by  
$$
b(T) := \frac 1 {|T|} \int_T z \, dz \stext{ and } m(T) := \int_T (z-b(T)) (z-b(T))^\trans dz. %\frac 1 {|T|} 
$$
If $\Phi(z) = z_0 + \phi(z)$ is an affine change of coordinates on $\R^2$, where $z_0\in \R^2$ and $\phi\in \GL_2$, then 
\be
\label{eqChgMoments}
b(\Phi(T)) = z_0+b(T) \stext{ and } m(\Phi(T)) = |\det\phi| \ \phi \, m(T) \, \phi^\trans.
\ee
Note also that 
\be
\label{eqChgTau}
\frac{\tau(T)}{|T|} = \frac{\tau(\Phi(T))} {|\Phi(T)|}.
\ee
We denote by $\cC_0\subset \cC$ the collection of centered and normalized convex sets
%A classical argument shows that the set $\cC_0$ of centered and norm
%Let $\cC_0$ be the collection 
$$
\cC_0 := \{T\in \cC \sep b(T)=0 \text{ and } m(T) = \Id\}.
$$
It follows from \iref{eqChgMoments} that for each $T\in \cC$ there exists an affine change of coordinates $\Phi$ such that $\Phi(T)\in \cC_0$. 
A classical argument %[Minkowski??] 
shows that $\cC_0$ is a compact set with respect to the Hausdorff distance.
Furthermore, the map 
$$
T \mapsto \frac{\tau(T)}{|T|}
$$
is continuous on the set $\cC$ with respect to the Hausdorff distance, hence it is bounded below by a positive constant $\delta>0$ on the compact set $\cC_0$. Recalling \iref{eqChgTau}, we obtain \iref{eqDeltaTC} and we conclude the proof of this proposition.
\sq

We denote by $S_T^{3*}$ the collection $S_T^{3*} = \{[a,b],[b,c],[c,a]\}$ of segments joining the three points $a,b,c\in (\partial T)^3$ which maximize \iref{defTauT}. Some convex polygons and the associated optimal triplets $(a,b,c)\in (\partial T)^3$ are illustrated on Figure \ref{figCvxCut}. If there are several triplets $(a,b,c)$ realizing this maximum, for instance if $T$ is a disc or a regular polygon, then we consider the minimal triplet with respect to the lexicographic order on $(\R^2)^3$.

From an algorithmic point of view, for any convex polygon $T\in \cC$ the points $(a,b,c)$ which maximize \iref{defTauT} can be found by solving a finite number of third degree equations (one for each triplet of distinct faces of $T$). 

\begin{assumptions}
\label{assumConv}
Let $T\in \cC$ be such that $e_T(\chi_P)\neq 0$. 
In the following we work under the assumption that the segment $s\in S_T^{3*}$ which minimizes the decision function $d_T(s,\chi_P)$ satisfies the following property. %We assume in the following that the decision function $d_T(s,\chi_P)$ satisfies the foll
\begin{enumerate}[a)]
\item The bisection of $T$ along $s$ creates a child $T'$ such that $e_{T'}(\chi_P) = 0$. (This is always possible).
\end{enumerate}
\end{assumptions}

\begin{figure}	
	\centering
		\includegraphics[width = 4cm, height=4cm]{\pathPic/Subdivision/Numerical/CutsLineHoriz.pdf}
		\hspace{1cm}
		\includegraphics[width = 4cm, height=4cm]{\pathPic/Subdivision/Numerical/CutsLine8Horiz.pdf}
		\caption{\label{figExpApprox}
		Left : A convex set (red, dashed), the segments $S_T^{3*}$ (blue, dotted), the line $D$ (black, thick).
		Right : After $8$ steps of the greedy algorithm, with a decision function satisfying Assumptions \ref{assumConv}.}
\end{figure}

The following corollary shows that, under the previous assumption on the decision function, the refinement procedure based on these bisection choices creates an exponentially thin layer around the discontinuity of the function $f=\chi_P$, as illustrated on Figure \ref{figExpApprox}.

\begin{corollary}
\label{corolExpApprox}
Let $\Omega\subset \R^2$ be a convex polygon, and let $(\cT_N)_{N\geq 1}$ be the sequence of partitions of $\Omega$ into convex polygons generated by the greedy algorithm applied to the function $f=\chi_P$ and starting from $\cT_1 = \{\Omega\}$. If the decision function satisfies \iref{assumConv} then
$$
e_{\cT_N}(\chi_P)^2\leq |\Omega| \, (1-\delta)^{N-1},
$$ 
where $\delta$ is the positive constant from Proposition \ref{propConvex}.
\end{corollary}

\proof
It follows from the assumptions \ref{assumConv} that for all $N \geq 1$ at most a single element $T\in \cT_N$ satisfies $e_T(\chi_P)\neq 0$. We denote this element by $T_N$, and we remark that $T_{N+1}$ is a child of $T_N$.
It follows from Proposition \iref{propConvex} that  $|T_{N+1}|\leq (1-\delta) |T_N|$, for any $N \geq 1$, hence 
$$
e_{\cT_N}(\chi_P)^2 = e_{T_N} (\chi_P)^2 \leq |T_N| \leq  |\Omega| \, (1-\delta)^{N-1},
$$
which concludes the proof. See Figure \ref{figExpApprox} for an illustration.
\sq



\noindent
The bisection of $T\in \cC$ along a segment $s\in S_T^{3*}$ creates two children $T_s^1$ and $T_s^2$. In terms of the notations previously used in this section, the bisection along $s=[b,c]\in S_T^{3*}$ creates the two children $T_s^1 = T_a$ and $T_s^2 = \overline{T\sm T_a}$. %using the previous notations
From this point, we assume that the decision function $d_T(s,f)$ is defined by %We consider the decision function $d_T(s,f)$ defined by 
\be
\label{decisionConv}
d_T(s,f) := \min\left\{\frac {e_{T_s^1}(f)}{|T_s^1|^{\frac 3 2}}, \ \frac {e_{T_s^2}(f)}{|T_s^2|^{\frac 3 2}}\right\}.
\ee
If the approximation error of $f$ on $T_s^1$ or $T_s^2$ is zero, then $d_T(s,f)=0$. Therefore this decision function satisfies Assumptions \ref{assumConv}, and leads to an exponentially fast convergence if $f=\chi_P$ according to Corollary \ref{corolExpApprox}.

Let us consider a quadratic function $f(z) =\frac 1 2 z^\trans Q z$, where $Q$ is a $2\times 2$ symmetric matrix, to be approximated on a domain $\Omega$. As seen in the previous chapters, the elements of a partition $\cT$ of $\Omega$ should adopt, for an efficient approximation of $f$, an aspect ratio dictated by the hessian matrix $d^2 f=Q$ of $f$ (at least in an average sense).
The numerical experiments presented in Figure \ref{figCvxQuad} suggest that the greedy algorithm, based on the bisection choices $S_T^{3*}$ and the decision function \iref{decisionConv}, generates such partitions. Unfortunately, the author could not prove this property.

\begin{figure}
	\centering
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Numerical/CvxNum50_100.pdf}
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Numerical/CvxNum200_100.pdf}
		\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/Numerical/CvxNum30_1.pdf}
		\caption{\label{figCvxQuad} Triangulations produced by the greedy algorithm applied to the function $f(x,y)=x^2+100 y^2$ with the decision function \iref{decisionConv} and 50 (i) and 200 (ii) elements. Likewise for the function $f(x,y) = x^2+y^2$ and 30 elements (iii).}
\end{figure}

Eventually, numerical experiments were also led for characteristic function $f=\chi_D$ of the unit disc $D = \{(x,y)\in \R^2 \sep x^2+y^2\leq 1\}$. They seem to indicate that the partitions $(\cT_N)_{N \geq 1}$ of the triangle of vertices $(0,0), (2,0),(0,2)$ generated by the greedy algorithm do satisfy the desired error estimate
$$
e_{\cT_N}(\chi_D) \leq CN^{-1},
$$
see Figure \ref{figHorizonQuad}. However, again, the author could not establish this property.

For better numerical precision, the numerical experiments illustrated in Figures \ref{figExpApprox}, \ref{figCvxQuad} and \ref{figHorizonQuad} were conducted without discretizing function $f$ of interest %the quadratic function or the characteristic function of interest, 
but using its explicit form in order to have an exact expression of the $L^2$ approximation error.

\begin{figure}
	\centering
		\includegraphics[width=4.5cm,height=4.5cm]{\pathPic/Subdivision/Numerical/Horizon200.pdf} 
		\includegraphics[width=4.5cm,height=4.5cm]{\pathPic/Subdivision/Numerical/Horizon200Detail.pdf}
		\includegraphics[width=4.5cm,height=4cm]{\pathPic/Subdivision/Numerical/GraphCvxHoriz.pdf} 		\caption{\label{figHorizonQuad}
		Triangulation produced by the greedy algorithm applied to the function $f=\chi_D$, with the decision function \iref{decisionConv} and $200$ elements (i). Detail (ii). Decay of the error $e_{\cT_N}(\chi_D)$, in logarithmic scale, for $1\leq N\leq 40000$.}
\end{figure}


\section{A robust greedy algorithm, based on rectangles} %Optimal convergence}
\label{secGreedyRect}

%(*define $L^\infty$ approx errors*)

%Given an polygonal domain $\Omega$, and a function $f$ on $\Omega$, the refinement procedures presented previously in this part of the thesis produce partitions $\cT_N$ of $\Omega$ into triangles, or convex polygons in (??), which are adapted to the approximation of $f$ with piecewise linear elements.
%The cells, triangles or convex polygons, used in these partitions may have arbitrary sizes, aspect ratios and orientation.
%
%Unfortunately, the theoretical results presented in the previous subsections on these algorithm suffer from the two following issues.
%\begin{enumerate}
%\item
%%Unfortunately, the theoretical results presented in the previous subsections only apply to a restricted set of functions. 
%\emph{They only apply to restricted sets of functions.\\}
%The function $f$ to be approximated needs indeed to be $C^2$ and stricly convex in Theorems [??] and [??], quadratic (of arbitrary signature) in Theorems \ref{thOptiL2LInf} and \ref{thOptiL2LInfNeg}, or the characteristic function $f=\chi_P$ of a half plane in Propositions \ref{propSpeedBi}, \ref{propSpeedTri} and Corollary \ref{corolExpApprox}.
%
%\item
%\emph{The asymptotical behavior only of the approximation error is controlled. } %, as the number of elements tends to infinity.\\}
%%\emph{Theorems (??) and (??) are based on a saturation hypothesis. \\}
%For instance Theorems (??) and (??), which apply to $C^2$ and strictly convex functions, are based on a saturation hypothesis, namely the the key results Propositions (??) and (??), which state that the sizes of all triangles tend to zero.
%Once the triangles are sufficiently small, a perturbation analysis shows that they adopt the optimal aspect ratio, using the fact that the function to be approximated, which is $C^2$, is locally close to a quadratic function.\\
%In other words let  $(\cT_N)_{N\geq N_0}$ be the sequence of triangulations generated by the greedy algorithm. The asymptotic behavior of the approximation error $e_{\cT_N}(f)_p$ as $N \to \infty$ is optimal according to Theorems (??) and (??), but little is known on the first values of $e_{\cT_N}(f)_p$. How does it compare to a basic uniform refinement ?
%\end{enumerate}

%We study in this section another variation of the greedy algorithm, based  which has the advantage of being particularly robust, as shown in Theorem \ref{thRect}. Indeed : 

We study in this section another variation of the greedy algorithm which is simpler than the previous ones but also more ``robust''.
Indeed, it produces partitions $(\cT_N)_{N \geq 1}$ of the unit square $\Omega = [0,1]^2$ into rectangles aligned with the horizontal or vertical axes, instead of triangulations built of triangles of arbitrary direction. Furthermore, on each element of the partition, the target function $f$ is approximated by constants instead of affine functions, and the approximation error is measured in $L^\infty$ norm instead of $L^p$ norm where $p$ is an arbitrary exponent.

These important simplifications allow us to establish a particularly general result, Theorem \ref{thRect}. This Theorem contains an  error estimate \iref{eqAsymptRect} which applies to any function $f\in C^1(\Omega)$ and is asymptotically optimal as the cardinality $\#(\cT_N) = N$ tends to $\infty$. Furthermore this theorem also contains a second error estimate \iref{eqRobustRect} which gives some valuable (yet non optimal) information for any value of $N\geq 1$. 
%This second  feature is not present in our previous results Theorems \ref{optitheo} and \ref{optitheoLInf} .

In order to state our main result, we introduce some notation.
A rectangle $T\subset \R^2$ is a set of the form
$$
T = I \times J 
$$
where $I$ and $J$ are compact intervals of $\R$. %We denote by $|I|$ and $|J|$ the 
For any rectangle $T$ and any $f$ in $C^0(T)$, we denote by $e_T(f)$ the difference between the supremum an the infimum of $f$ on $T$.
$$
e_T(f) := \sup_T f - \inf_T f.
$$
Note that $e_T(f)$ is also the double of the error of best approximation of $f$ on $T$ in the $L^\infty$ norm,
$$
e_T(f) = 2\inf_{c\in \R} \|f-c\|_{L^\infty(T)} .
$$
If a function $f\in C^1(T)$ attains its maximum on the rectangle $T$ at the point $z_M = (x_M,y_M)$, and its minimum at the point $z_m =(x_m,y_m)$ then observe that 
\begin{eqnarray*}
f(z_M) - f(z_m) &\leq& \left|\int_{x_m}^{x_M}  \partial_x f(x,y_m) dx\right| + \left|\int_{y_m}^{y_M}  \partial_y f(x_M,y) dy \right| \\
&\leq& |x_M-x_m| \|\partial_x f\|_{L^\infty(T)} + |y_M-y_m| \|\partial_y f\|_{L^\infty(T)}. 
\end{eqnarray*}
Therefore if $T = I \times J$, we obtain %where $I$ and $J$ are compact intervals of $\R$, then observe that 
\be
\label{eqErrorBoundAff}
e_T(f) \leq |I| \|\partial_x f\|_{L^\infty(T)} + |J| \|\partial_y f\|_{L^\infty(T)}.
\ee
For any partition $\cT$ of a rectangle $T$ into smaller rectangles, and for any $f\in C^0(T)$, we denote by $e_\cT(f)$ maximum of $e_T(f)$ among all $T \in \cT$. 
$$
e_\cT(f) := \max_{T\in \cT} e_T(f) 
$$
We clearly also have 
$$
e_\cT(f) = 2\min_{g\in V_\cT} \|f-g\|_{L^\infty(T)},
$$
 %the double of the error of best approximation of $f$ on $T$ by functions which are piecewise constant on the partition $\cT$.
where $V_\cT$ is the collection of functions on $T$ which are constant on the interior of each $T\in \cT$.

\begin{remark}
Please note that the definition of $e_T(f)$ in this section differs a lot from the definition of $e_T(f)$ in the previous section. Indeed, $e_T(f)$ stands here for the double of the best approximation of $f$ in $L^\infty(T)$ norm by a constant $c\in \R$, whereas $e_T(f)$ stands in the previous section for the  best approximation of $f$ in $L^2(T)$ norm by an affine function $\pi \in \P_1$.
\end{remark}

\begin{figure}
\centerline{
\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/CMrectsplit.pdf}
\hspace{1cm}
\includegraphics[width=4cm,height=4cm]{\pathPic/Subdivision/CMtrisplit6.pdf}
}
\caption{Anisotropic partitions obtained by rectangle split (left)
and triangle bisection (right)}
\label{CManisopart}
\end{figure}

For any rectangle $T$ we denote by $(T_d,T_u)$ the down and up rectangles
which are obtained by a horizontal split of $T$ through its barycenter
and by $(T_l,T_r)$ the left and right rectangles
which are obtained by a vertical split of $T$ through its barycenter.
For any function $f\in C^0(T)$, we define 
$$
e_{T,h}(f) := \max\{e_{T_d}(f), e_{T_u}(f)\} \stext{ and } e_{T,v}(f) := \max\{e_{T_l}(f), e_{T_r}(f)\}
$$

The greedy algorithm studied in this section takes as input a function $f\in C^0(\Omega)$, where $\Omega = [0,1]^2$ is the unit square, and a parameter $\rho\in [0,1]$. 
Given a partition $\cT$ of $\Omega$ into rectangles aligned with the coordinate axes, the greedy algorithm produces in one step a refinement $\cT'$ of $\cT$, satisfying $\#(\cT') = \#(\cT)+1$, proceeding as follows.
%It produces a sequence $(\cT_N)_{N\geq 1}$ of hierarchical partitions of $\Omega$ into dyadic rectangles, proceeding as follows.
\begin{enumerate}
\item Select a rectangle $T\in \cT$ which maximizes $e_T(f)$.
\item (Greedy split) If 
\be
\label{eqCompTChild}
\min\{e_{T,h}(f), e_{T,v}(f)\}\leq \rho \,e_T(f),
\ee
then bisect the rectangle $T$ horizontally if $e_{T,h}(f)\leq e_{T,v}(f)$ and vertically otherwise, thus producing two children $T_1,T_2$ of $T$. Define 
$$
\cT' := \cT-\{T\}+ \{T_1,T_2\}.
$$
\item (Security split) If 
\be
\label{eqCompTChild2}
\min\{e_{T,h}(f), e_{T,v}(f)\} > \rho \,e_T(f),
\ee
then bisect the rectangle $T$ horizontally if $|I|\geq |J|$ and vertically otherwise where $I,J$ are the two compact intervals such that $T = I\times J$. This bisection produces two children $T_1,T_2$ of $T$ and we define 
$$
\cT' := \cT-\{T\}+ \{T_1,T_2\}.
$$
\end{enumerate}

Starting from the partition $\cT_1 = \{\Omega\}$ of the square $\Omega = [0,1]^2$, the greedy algorithm produces step after step a sequence $(\cT_N)_{N\geq 1}$ of partitions of $\Omega$ into dyadic rectangles, satisfying $\#(\cT_N) = N$.
The parameter $\rho\in [0,1]$ is chosen by the user. It should not be chosen too
small in order to avoid that all splits are of safety type which would then
lead to isotropic partitions. 
The choice $\rho=1$ is not indicated either. Indeed let $f(x,y) := \sin(4 \pi x)$, then for any rectangle $T$ of the form $T = [0,1] \times J$, where $J$ is a compact interval, one has 
$$
e_T(f) = e_{T,h}(f) = e_{T,v}(f) = 2.
$$
If a rectangle $T= [0,1] \times J$ is selected for bisection and if $\rho=1$, then $T$ is bisected horizontally and we are facing a similar situation for its children $T_u$ and $T_d$.
As a result, the greedy algorithm produces a sequence $(\cT_N)_{N\geq 1}$ of partitions of $\Omega$ consisting of rectangles of the form $[0,1]\times J$ where $J$ are dyadic intervals. This shows that the approximations produced by the algorithm fail to converge towards $f$, and the global error remains $e_{\cT_N}(f) = 1$ for all $N \geq 1$.
On the contrary, it is established in \cite{CMi2} that for any choice of $\rho\in [0,1[$ and any $f\in C^0(\Omega)$, the partitions $(\cT_N)_{N\geq 1}$ produced by the greedy algorithm satisfy $e_{\cT_N}(f) \to 0$ as $N \to \infty$.

We now prove that
using the specific value $\rho=\frac 1 {\sqrt 2}$
the modified greedy refinement algorithm has optimal convergence properties
similar to Theorem \ref{thUpper} %\iref{CMlimsupsigmaNanisorect}
in the case where we measure the error in the $L^\infty$ norm.
Similar results can be obtained when the error is measured in $L^p$ with $p<\infty$,
at the price of more technicalities.

\begin{theorem}
\label{thRect}
There exists a constant $C>0$ such that for any $f\in C^1(\Omega)$, the partition
$\cT_N$ produced by the modified greedy refinement algorithm with parameter $\rho=\frac 1 {\sqrt 2}$
satisfy the asymptotic convergence estimate
\be
\label{eqAsymptRect}
\limsup_{N\to +\infty} \, N^{\frac 1 2} e_{\cT_N}(f) \leq C \left\|\sqrt{|\partial_x f\ \partial_y f|}\right\|_{L^2}
\ee
Furthermore for all $N \geq 1$ one has 
\be
\label{eqRobustRect}
e_{\cT_N}(f)\leq C \|\nabla f\|_{L^\infty(\Omega)}N^{-\frac 1 2}.
\ee
\end{theorem}

The asymptotical error estimate \iref{eqAsymptRect} is the best than one should hope to obtain. %optimal up to a multiplicative constant. 
Indeed it follows from Theorem \ref{thLower} that there exists a constant $c>0$ independent of $f$ and such that 
\be
\label{eqLowerRect}
\liminf_{N\to +\infty} \, N^{\frac 1 2} e_{\cT'_N}(f) \geq c \left\|\sqrt{|\partial_x f\ \partial_y f|}\right\|_{L^2},
\ee
for any admissible sequence $(\cT'_N)_{N\geq N_0}$ of partitions of $\Omega$ into rectangles. (Admissibility is a minor technical condition, see Definition \ref{defAdmiRect}) %, provided it satisfies the technical condition of admissibility (??).

\begin{remark}
\label{remRobustRect}
Theorem \ref{thRect} traduces the particularly ``robust'' behavior of the variation of the greedy algorithm studied in this section. Let us emphasize two important differences between this result and the previous ones presented  in this part of the thesis.

Firstly Theorem \ref{thRect} applies to any function $f\in C^1(\Omega)$. In contrast our previous results on greedy algorithms require more than a simple regularity assumption from the function $f$ which is approximated. 
For instance Theorems \ref{optitheo} and \ref{optitheoLInf} only apply to strictly convex (and $C^2$) functions.
Theorems \ref{thOptiL2LInf} and \ref{thOptiL2LInfNeg} apply to quadratic functions, and Propositions \ref{propSpeedBi}, \ref{propSpeedTri} and Corollary \ref{corolExpApprox} apply to the characteristic function $f=\chi_P$ of a half plane.

Secondly Theorem \ref{thRect} guarantees an upper bound on $e_{\cT_N}(f)$ for any value of $N$.
This theorem contains indeed two inequalities \iref{eqAsymptRect} and \iref{eqRobustRect} which address different regimes of the parameter $N$. 
For ``small'' values of $N$, the error bound \iref{eqRobustRect} is the same as the error bound associated to a 
uniform refinement of the square $\Omega$. It is a valuable yet non optimal information.
For asymptotically large values of $N$ the error bound \iref{eqAsymptRect} is obtained using a saturation analysis which involves in particular in \iref{eqUnifCont} the modulus of continuity of $\nabla f$. Our previous results Theorems \ref{optitheo} and \ref{optitheoLInf} only contain this type of estimate. 

In contrast Theorems (??) and (??) previously presented in this part of the thesis only contain an asymptotical estimate on the approximation error, and little is known on the approximation error $e_{\cT_N}(f)$ before this asymptotical regime.


%The function $f$ to be approximated needs indeed to be $C^2$ and stricly convex in Theorems [??] and [??], quadratic (of arbitrary signature) in Theorems \ref{thOptiL2LInf} and \ref{thOptiL2LInfNeg}, or the characteristic function $f=\chi_P$ of a half plane in Propositions \ref{propSpeedBi}, \ref{propSpeedTri} and Corollary \ref{corolExpApprox}.


\begin{enumerate}
\item
\emph{Theorem \ref{thRect} applied to any function $f\in C^1$.\\}
In contrast our previous results on greedy algorithms apply to functions satisfying an assumption which is generally not a regularity assumption. 
The function $f$ to be approximated needs indeed to be $C^2$ and stricly convex in Theorems [??] and [??], quadratic (of arbitrary signature) in Theorems \ref{thOptiL2LInf} and \ref{thOptiL2LInfNeg}, or the characteristic function $f=\chi_P$ of a half plane in Propositions \ref{propSpeedBi}, \ref{propSpeedTri} and Corollary \ref{corolExpApprox}.

\item
\emph{Theorem \ref{thRect} guarantees an upper bound on $e_{\cT_N}(f)$ for any value of $N$.} %that this algorithm outperforms The asymptotical behavior only of the approximation error is controlled. } %, as the number of elements tends to infinity.\\}
%\emph{Theorems (??) and (??) are based on a saturation hypothesis. \\}

This theorem contains indeed two inequalities \iref{eqAsymptRect} and \iref{eqRobustRect} which address different regimes of the parameter $N$. 
For ``small'' values of $N$, the error bound \iref{eqRobustRect} is the same as the error bound associated to a 
%non-adaptive 
uniform refinement of the square $\Omega$.

%produced guarantees that the approximation error $e_{\cT_N}(f)$ is not worse than the approximation error produced by the standard uniform refinement procedure.

For asymptotically large values of $N$ the error bound \iref{eqAsymptRect} is the best possible error bound according to \iref{eqLowerRect}. It is obtained using a saturation analysis which involves in particular in \iref{eqUnifCont} the modulus of continuity of $\nabla f$. 

In contrast Theorems (??) and (??) previously presented in this part of the thesis only contain an asymptotical estimate on the approximation error, and little is known on the approximation error $e_{\cT_N}(f)$ before this asymptotical regime.
%. It does not seem possible to 

%It is not possible to know in advance 
%Indeed, equation \iref{eqRectRobust} guarantees that for small 

%In contrast Theorems (??) and (??) are based on a saturation result, namely Propositions (??) and (??), which state that the sizes of all triangles tend to zero.
%Once the triangles are sufficiently small, a perturbation analysis shows that they adopt the optimal aspect ratio, using the fact that the function to be approximated, which is $C^2$, is locally close to a quadratic function. However little is known on the approximation error $e_{\cT_N}(f)$ before this asymptotical regime.

%In other words let  $(\cT_N)_{N\geq N_0}$ be the sequence of triangulations generated by the greedy algorithm. The asymptotic behavior of the approximation error $e_{\cT_N}(f)_p$ as $N \to \infty$ is optimal according to Theorems (??) and (??), but little is known on the first values of $e_{\cT_N}(f)_p$. How does it compare to a basic uniform refinement ?
\end{enumerate}
\end{remark}

\noindent
Here and after, we use the $\ell^\infty$ norm on $\RR^2$ for
measuring the gradient: for $z=(x,y)\in\Omega$
$$
|\nabla f(z)|:=\max \{|\partial_x f(z)|,|\partial_y f(z)|\},
$$
and
$$
\|\nabla f\|_{L^\infty(T)}:= \sup_{z\in T}|\nabla f(z)|=\max\{\|\partial_x f\|_{L^\infty(T)},\|\partial_y f\|_{L^\infty(T)}\}.
$$
We consider a fixed function $f\in C^1(\Omega)$ and we denote by $(\cT_N)_{N\geq 1}$ the sequence of partitions of  the square $\Omega = [0,1]^2$ into dyadic rectangles generated by the greedy algorithm. Furthermore we define for each n 
$$
\ve(N) := e_{\cT_N}(f)
$$
%We recall that the local $L^\infty$-error on $T$ is given by
%$$
%e_{T}(f)= \frac 1 2 \left(\max_{z\in T} f(z) - \min_{z\in T} f(z) \right).
%$$
%We also recall from the proof of Theorem \ref{CMtheogreedyconv} that
%$$
%\e(N):=\max_{T\in\cT_N} e_{T}(f) \to 0 \;\; {\rm as}\;\; N\to +\infty.
%$$
Finally we sometimes use the notation $x(z)$ and $y(z)$ to denote the coordinates 
of a point $z\in\RR^2$.
The proof of this Theorem \ref{thRect} requires a preliminary result.

\begin{lemma}
\label{CMlemmaRobust}
Let $T_0=I_0\times J_0 \in\cT_M$ be a dyadic rectangle obtained 
at some stage $M$ of the refinement algorithm, and let $T=I\times J\in \cT_N$
be a dyadic rectangle obtained at some later stage $N>M$ and such
that $T\subset T_0$. We then have 
\be
\label{eqLemmaRobust}
|I|\geq \min\left \{|I_0|, \frac {\ve(N)} {4\|\nabla f \|_{L^\infty(T_0)}} \right \} \stext{ and } 
|J|\geq \min\left \{|J_0|, \frac {\ve(N)} {4\|\nabla f \|_{L^\infty(T_0)}}\right \}.
\ee
\end{lemma}
\proof
Since the coordinates $x$ and $y$ play symmetrical roles, it suffices to prove the first inequality.
We reason by contradiction. If the inequality does not hold, there exists 
a rectangle $T'=I'\times J'$ in the chain that led from $T_0$ to $T_1$
which is such that
\be
\label{eqIRobust}
|I'| < \frac  {\ve(N)} {2\|\nabla f \|_{L^\infty(T_0)}},
\ee
and such that $T'$ is split vertically by the algorithm. If this was a safety split, 
we would have that $|J'|\leq |I'|$
and therefore 
$$
e_{T'}(f) \leq (|I'|+|J'|) \|\nabla f \|_{L^\infty(T)} \leq 2|I'|\|\nabla f \|_{L^\infty(T)} < \ve(N),
$$ 
which is a contradiction, since all ancestors of $T$ should satisfy $e_{T'}(f)\geq \ve(N)$. 
Hence this split was necessarily a greedy split.

Let $z_m:={\rm Argmin}_{z\in T'} f(z)$ and $z_M:={\rm Argmax}_{z\in T'} f(z)$, and let $T''$ be the child of $T'$ (after the vertical split) containing $z_M$. Then $T''$ also contains a point $z'_m$ such that $|x(z'_m) - x(z_m)|\leq |I'|/2$ and $y(z'_m) = y(z_m)$. It follows that
\begin{eqnarray*}
e_{T',v}(f) &\geq &e_{T''}(f) \\
& \geq& f(z_M) - f(z'_m)\\
 & \geq& f(z_M) - f(z_m)- \|\partial_x f\|_{L^\infty(T')} \frac {|I'|} 2\\
 & \geq & e_{T'}(f) - \frac 1 4 \ve(N)\\ 
&  \geq& \frac 3 4 e_{T'}(f) \\
& > & \rho e_{T'}(f).
\end{eqnarray*}
where we used \iref{eqIRobust} to obtain the fourth line.
The error was therefore insufficiently reduced which contradicts a greedy split.
\sq

\noindent
{\bf Proof of Inequality \iref{eqRobustRect}}
We first observe that for any $N \geq 1$,
$$
\ve(N) \leq \ve(1) = \sup_\Omega f - \inf_\Omega f \leq 2 \|\nabla f\|_{L^\infty(\Omega)}.
$$
Applying Lemma \ref{CMLemmaRobust} to the rectangle $\Omega = [0,1] \times [0,1]$ we obtain that for any rectangle $T = |I| \times |J| \in \cT_N$ one has 
$$
\min\{|I|, |J|\} \geq \frac {\ve(N)} {4 \|\nabla f \|_{L^\infty(\Omega)}}.
$$
Therefore 
$$
1= |\Omega| = \sum_{T = I \times J \in \cT_N} |I| \times |J| \geq N \left( \frac {\ve(N)} {4 \|\nabla f \|_{L^\infty(\Omega)}} \right)^2, %\min_{T \in \cT_N}  |T| \geq N \min_{T = I \times J \in \cT_N}
$$
hence 
\be
\label{eqEpsToZero}
N^{\frac 1 2 } \ve(N) \leq 4 \|\nabla f \|_{L^\infty(\Omega)},
\ee
which concludes the proof of \iref{eqRobustRect}. 
\sq\\

\noindent
{\bf Proof of Inequality \iref{eqAsymptRect}} %Theorem \ref{thRect}:}
We consider a small but fixed $\delta >0$, and we define $h(\delta)$ as the maximal $h>0$ such that
\be
\label{eqUnifCont}
\forall z,z'\in \Omega,\ |z-z'|\leq 2h(\delta) \Rightarrow |\nabla f(z)-\nabla f(z')|\leq  \delta.
\ee
For any rectangle $T=I\times J\subset \Omega$, we thus have 
\be
\label{CMeqhdelta}
\begin{array}{ccc}
e_{T}(f) &\geq& (\|\partial_x f\|_{L^\infty(T)}-\delta) \min\{h(\delta),|I|\}, \\
e_{T}(f) &\geq& (\|\partial_y f\|_{L^\infty(T)}-\delta) \min\{h(\delta),|J|\}.
\end{array}
\ee
Let $\delta>0$ and $M=M(f,\delta)$ be the smallest value of $N$ such that $\e(N)\leq 9\delta h(\delta)$.
For all $N\geq M$, and therefore $\e(N)\leq 9\delta h(\delta)$, we consider the 
partition $\cT_N$ which is a refinement of $\cT_{M}$. For any rectangle $T_0=I_0\times J_0 \in \cT_M$,
we denote by $\cT_N(T_0)$ the set of rectangles of $\cT_N$ that are contained $T_0$.
We thus have
$$
\cT_N:=\bigcup_{T_0\in\cT_M}\cT_N(T_0),
$$
and $\cT_N(T_0)$ is a partition of $T_0$. We shall next bound by below
the side length of $T=I\times J$ contained in $\cT_N(T_0)$,
distinguishing different cases depending on the behaviour of $f$ on $T_0$.
\nl
\nl
{\it Case 1.} If $T_0\in\cT_M$ is such that $\|\nabla f\|_{L^\infty(T_0)} \leq 10 \delta$,
then a direct application of Lemma \ref{CMlemmaRobust} shows that for all $T=I\times J\in \cT_N(T_0)$ we have 
\be
\label{CMeqFlat}
|I|\geq \min\left \{|I_0|, \frac {\ve(N)} {40\delta}\right \} \stext{ and } |J|\geq \min\left \{|J_0|, \frac {\ve(N)} {40\delta}\right \}
\ee
\nl
{\it Case 2.} If $T_0\in\cT_M$ is such that
$\|\partial_x f\|_{L^\infty(T_0)} \geq 10 \delta$ and $\|\partial_y f\|_{L^\infty(T_0)} \geq 10 \delta$,
we then claim that for all $T=I\times J\in \cT_N(T_0)$ we have
\be
\label{CMeqAffine}
|I| \geq \min\left\{|I_0|, \frac{\ve(N)} {20\|\partial_x f\|_{L^\infty(T_0)}}\right\} \stext{ and } 
|J| \geq \min\left\{|J_0|, \frac{\ve(N)} {20\|\partial_x f\|_{L^\infty(T_0)}}\right\},
\ee
and that furthermore 
\be
|T_0| \ \|\partial_x f\|_{L^\infty(T_0)} \|\partial_y f\|_{L^\infty(T_0)} \leq \left (\frac {10}9\right )^2 \int_{R^*} |\partial_x f\ \partial_y f| dx dy.
\label{CMintegralstatement}
\ee
This last statement easily follows by the following observation: 
recalling \iref{CMeqhdelta} we obtain
$$
9\delta h(\delta)\geq e_{T_0}(f) \geq (\|\partial_y f\|_{L^\infty}(T_0)-\delta)\min\{h(\delta),|J_0|\}
\geq 9\delta\min\{h(\delta),|J_0|\},
$$
therefore $|J_0| \leq h(\delta)$. Similarly $|I_0|\leq h(\delta)$and 
%combining 
%\iref{CMeqhdelta} with the fact that $\|\partial_x f\|_{L^\infty(T_0)} \geq 10 \delta$ and $\|\partial_y f\|_{L^\infty(T_0)} \geq 10 \delta$
%and that 
%$$
%e_{T}(f)\leq \e(N) \leq 9\delta h(\delta),
%$$ 
%we obtain that $|I|\leq h(\delta)$ and $|J|\leq h(\delta)$. 
therefore  for all $z\in T_0$
$$
|\partial_x f(z)|\geq \|\partial_x f\|_{L^\infty(T_0)} - \delta \geq \frac 9 {10}\|\partial_x f\|_{L^\infty(T_0)},
$$
and 
$$
|\partial_y f(z)|\geq \|\partial_y f\|_{L^\infty(T_0)} - \delta \geq \frac 9 {10}\|\partial_y f\|_{L^\infty(T_0)},
$$
Integrating over $T_0$ yields \iref{CMintegralstatement}.
Furthermore we the previous equations show that $\partial_x f$ and $\partial_y f$ have a constant sign on $T_0$. Let us assume that both are positive, then for any rectangle $T = [a,b] \times [c,d]\subset T_0$ we obtain 
\begin{eqnarray*}
e_T(f) & = & \sup_T f-\inf_T f \\
& \geq & f(b,d) - f(a,c)\\
& \geq & \int_a^b \partial_x f(x,c) dx+ \int_c^d \partial_y f (b,y) dy\\
& \geq & \frac 9 {10} \left((b-a) \|\partial_x f\|_{L^\infty(T_0)} + (d-c) \|\partial_y f\|_{L^\infty(T_0)}\right)
\end{eqnarray*}
A similar reasoning can be applied if $\partial_x f$ or $\partial_y f$ is negative is negative on $T_0$. Recalling \iref{eqErrorBoundAff} we therefore obtain for any $T \subset T_0$
%Moreover for any rectangle $T\subset T_0$, we have
\be
\label{CMestimAffine}
\frac 9 {10} \leq \frac {e_{T}(f) }{\|\partial_x f\|_{L^\infty(T_0)}|I|+\|\partial_y f\|_{L^\infty(T_0)} |J|}\leq 1.
\ee
Clearly the two inequalities in \iref{CMeqAffine} are symmetrical, and it suffices to prove the first one. 
Similar to the proof of Lemma \ref{CMlemmaRobust}, we 
reason by contradiction, assuming that a rectangle $T'=I'\times J'$ with $|I'| \|\partial_x f\|_{L^\infty(T_0)}< \frac{\ve(N)}{10}$ 
was split vertically by the algorithm in the chain leading from $T_0$ to $T$. 
A simple computation using inequality \iref{CMestimAffine} shows that 
$$
\frac{e_{T',h}(f) }{e_{T'}(f)}\leq 
\frac{e_{T',h}(f)}{e_{T',v}(f)} \leq \frac 5 9 \times \frac{1+2\sigma}{1+\sigma/2}  \stext{ with } \sigma := \frac{\|\partial_x f\|_{L^\infty(T_0)} |I'|}{\|\partial_y f\|_{L^\infty(T_0)} |J'|}.
$$
In particular if $\sigma<0.2$ the we obtain that 
$$
e_{T',h}(f) \leq \rho e_{T'} (f) \stext{ and } e_{T',h}(f) \leq e_{T',v} (f),
$$
hence the algorithm performs a horizontal greedy split on $T'$, which contradicts our assumption.
Therefore $\sigma\geq 0.2$, but this also leads to a contradiction since
$$
\ve(N) \leq  e_{T'}(f) \leq \|\partial_x f\|_{L^\infty(T_0)} |I'|+ \|\partial_y f\|_{L^\infty(T_0)} |J'| 
\leq (1+\sigma^{-1}) \frac {\e(N)} {10} < \ve(N)
$$
\nl
\nl
{\it Case 3.} If $T_0\in\cT_M$ is such that $\|\partial_x f\|_{L^\infty(T_0)} \leq 10 \delta$ and $\|\partial_y f\|_{L^\infty(T_0)} 
\geq 10 \delta$, we then claim that for all $T=I\times J\in \cT_N(T_0)$ we have
\be
\label{CMeq1d}
|I| \geq \min\left \{|I_0|, \frac{\ve(N)} {C\delta}\right \} \text{ and } |J| \geq \min\left \{|J_0|, \frac {\ve(N)} {4 \|\nabla f\|_{L^\infty}}\right \}, \text{ with } C=200,
\ee
with symmetrical result if $T_0$ is such that $\|\partial_x f\|_{L^\infty(T_0)} \geq 10 \delta$ and $\|\partial_y f\|_{L^\infty(T_0)} 
\leq 10 \delta$. The second part of \iref{CMeq1d} is a direct consequence of Lemma
\ref{CMlemmaRobust}, hence we focus on the first part.
Applyting the second inequality of \iref{CMeqhdelta} to $T=T_0$, we obtain
$$
9\delta h(\delta)\geq e_{T_0}(f) \geq (\|\partial_y f\|_{L^\infty}(T_0)-\delta)\min\{h(\delta),|J_0|\}
\geq 9\delta\min\{h(\delta),|J_0|\},
$$
from which we infer that $|J_0| \leq h(\delta)$. If $z_1,z_2\in T_0$ and $x(z_1) = x(z_2)$ we therefore have 
$|\partial_y f(z_1)| \geq |\partial_y f(z_2)|-\delta$. It follows that for any rectangle $T=I \times J\subset T_0$ we have
\be
\label{CMerror1D}
(\|\partial_y f\|_{L^\infty(T)}-\delta) |J| \leq e_{T}(f) \leq \|\partial_y f\|_{L^\infty(T)} |J|+ 10\delta |I|.
\ee
We then again reason by contradiction, assuming that a rectangle $T'=I'\times J'$ with 
\be
\label{eqLengthR}
|I'| \leq \frac{2\ve(N)}{C\delta}
\ee
was split vertically by the algorithm in the chain leading from $T_0$ to $T$. 
If $\|\partial_y f\|_{L^\infty(T')} \leq 10\delta $, then $\|\nabla f\|_{L^\infty(T')}\leq 10\delta$ and 
Lemma \ref{CMlemmaRobust} shows that $T'$ should not have been split vertically, which is a contradiction.
Otherwise $\|\partial_y f\|_{L^\infty(T')} -\delta \geq \frac 9{10} \|\partial_y f\|_{L^\infty(T')}$, and we obtain using \iref{CMerror1D} and \iref{eqLengthR} that 
$$
\frac 9 {10} \|\partial_y f\|_{L^\infty(T')} |J'|\leq e_{T'}(f) \leq \|\partial_y f\|_{L^\infty(T')} |J'|+ 10 \delta \, \frac{2\ve(N)}{C\delta}.
$$
Recalling that $e_{T'}(f) \geq \ve(N)$ we obtain
\be
\label{CMestimDy}
\left(1-\frac{20} C\right)e_{T'}(f) \leq \|\partial_y f\|_{L^\infty(T')} |J'|\leq \frac {10} 9 e_{T'}(f).
\ee
We now consider the children $T'_v$ and $T'_h$ of $T'$
of maximal error after a horizontal and vertical split
respectively, and we inject \iref{CMestimDy} in \iref{CMerror1D}. 
It follows that
\begin{eqnarray*}
e_{T',h}(f) &=&e_{T'_h}(f)\\
&  \leq  &\|\partial_y f\|_{L^\infty(T')} \frac{|J'|} 2+ 10\delta |I'| \\
&  \leq &\frac 5 9 e_{T'}(f)+ \frac{20\ve(N)}C \\
& \leq  &\left(\frac 5 9+\frac{20} C\right)  e_{T'}(f)= \frac{59}{90} e_{T'}(f),
\end{eqnarray*}
and
\begin{eqnarray*}
e_{T',v}(f) & =&e_{T'_h}(f)\\
 &\geq &(\|\partial_y f\|_{L^\infty(T')}-\delta) |J| \\
&  \geq &\frac 9 {10} \|\partial_y f\|_{L^\infty(T')} |J'|  \\
& \geq &\frac 9 {10} \left(1-\frac{20} C\right) e_{T'}(f)= \frac {81}{100}e_{T'}(f).
\end{eqnarray*}
Therefore $e_{T',v}(f) > e_{T',h}(f)$
which is a contradiction, since our decision rule would then select a horizontal split.\\

We now recall that $\ve(N)\to 0$ as $N \to \infty$, see \iref{eqEpsToZero}, and we choose $N$ large enough so that 
the minimum in \iref{CMeqFlat}, \iref{CMeqAffine} and \iref{CMeq1d} is
are always equal to the second term. % (recall that we already established \iref{eqRobustRect} which shows that $\ve(N)\to 0$ as $N \to \infty$). 
For all  $T\in \cT_N(T_0)$, we respectively find that 
$$
\frac{\ve(N)^2} {|T|}\leq  C
\left\{\begin{array}{ccl}
\delta^2 & \text{ if } & \|\nabla f\|_{L^\infty(T_0)}\leq 10\delta\\
\frac 1 {|T_0|} \int_{T_0} |\partial_x f\ \partial_y f| & \text{ if } &   \|\partial_x f\|_{L^\infty(T_0)} \geq 10 \delta \text{ and } \|\partial_y f\|_{L^\infty(T_0)} \geq 10 \delta\\
 \delta \|\nabla f\|_{L^\infty} & \text{ if } & \|\partial_x f\|_{L^\infty(T_0)} \leq 10 \delta \text{ and } \|\partial_y f\|_{L^\infty(T_0)} \geq 10 \delta \text{ (or reversed).}
\end{array}\right.
$$
with $C= \max\{40^2,\ 20^2 (10/9)^2,\ 800\}=1600$. For $z\in \Omega$, we set
$\psi_N(z) := \frac 1 {|T|}$ where $T\in \cT_N$ is such $z\in T$, and we obtain
$$
N=\#(\cT_N)  = \int_{\Omega} \psi_N(z) dz \leq C\ve(N)^{-2} \left(  \int_{\Omega} |\partial_x f\ \partial_y f| dx dy+ \delta \|\nabla f\|_{L^\infty}+\delta^2\right).
$$
Therefore 
$$
\limsup_{N \to \infty} N^{\frac 1 2} \ve(N) \leq 40 \left(\int_{\Omega} |\partial_x f\ \partial_y f| dx dy+ \delta \|\nabla f\|_{L^\infty}+\delta^2\right)
$$
Taking the limit as $\delta \to 0$, we obtain the announced result
$$
\limsup_{N\to \infty} \, N^{\frac 1 2} \ve(N)\leq 40\left \| \sqrt {|\partial_x f\partial_y f|}\right \|_{L^2},
$$
which concludes the proof. \hfill $\Box$

\begin{remark} 
The proof of the Theorem can be adapted 
to any choice of parameter $\rho\in ]\frac 1 2,1[$.
\end{remark}

